A Subpolynomial Approximation Algorithm for Graph Crossing Number in Low-Degree Graphs

We consider the classical Minimum Crossing Number problem: given an $n$-vertex graph $G$, compute a drawing of $G$ in the plane, while minimizing the number of crossings between the images of its edges. This is a fundamental and extensively studied problem, whose approximability status is widely open. In all currently known approximation algorithms, the approximation factor depends polynomially on $\Delta$ -- the maximum vertex degree in $G$. The best current approximation algorithm achieves an $O(n^{1/2-\varepsilon}\cdot \text{poly}(\Delta\cdot\log n))$-approximation, for a small fixed constant $\epsilon$, while the best negative result is APX-hardness, leaving a large gap in our understanding of this basic problem. In this paper we design a randomized $O\left(2^{O((\log n)^{7/8}\log\log n)}\cdot\text{poly}(\Delta)\right )$-approximation algorithm for Minimum Crossing Number. This is the first approximation algorithm for the problem that achieves a subpolynomial in $n$ approximation factor (albeit only in graphs whose maximum vertex degree is subpolynomial in $n$). In order to achieve this approximation factor, we design a new algorithm for a closely related problem called Crossing Number with Rotation System, in which, for every vertex $v\in V(G)$, the circular ordering, in which the images of the edges incident to $v$ must enter the image of $v$ in the drawing is fixed as part of the input. Combining this result with the recent reduction of [Chuzhoy, Mahabadi, Tan '20] immediately yields the improved approximation algorithm for Minimum Crossing Number. We introduce several new technical tools, that we hope will be helpful in obtaining better algorithms for the problem in the future.

==> 2nd_disengagement.tex <==


\subsubsection{The Second-Level Disengagement}


\begin{figure}[t]
\centering
	\subfigure[Clusters $Y_{(a,a')}$ and its child-cluster $Y_{(b,b')}$ (clusters $C_a$ and $C_{a'+1}$ do not belong to $Y_{(a,a')}$).]{\scalebox{0.15}{\includegraphics{figs/instance_for_level_2_1.jpg}}\label{fig: path_cluster_H}
	}
	%\hspace{4pt}
	\subfigure[The layout of graph $G_{Y_{(a,a')}}$.]{\scalebox{0.15}{\includegraphics{figs/instance_for_level_2_2.jpg}}\label{fig: path_cluster_G}}
	\caption{An illustration of an instance $G_{Y_{(a,a')}}$ after the first-level disengagement.}%\label{fig: path_cluster}
\end{figure}





\subsubsection*{Step 1. Constructing Inner and Outer Paths}












\subsubsection*{Step 2. Constructing Sub-Instances}













\newpage


==> Appx-proofs-high-level-sec_bkup1014.tex <==

\section{Proofs Omitted from \Cref{sec: high level}}
\subsection{Proof of \Cref{claim: bound by level}}
\label{Appx: inductive bound proof}
The proof is by induction on $h(I)$. The base case is when $h(I)=0$, so $v(I)$ is a leaf vertex of $T^*$, and hence of $T$. Denote $I=(G,\Sigma)$.
%First we show that, if $I=(G,\Sigma)$ is a leaf subinstance of $I^*$, then the algorithm computes a solution to instance $I$ of cost at most $\mu^{2c'}\cdot \optcrors(I)$. 
If $\optcrors(I)=0$, then the algorithm returns a solution of cost $0$. Otherwise, $\optcrors(I)\geq 1$, and, if $|E(G)|\leq \mu^{c'}$, then the algorithm returns  the trivial solution, of cost at most $|E(G)|^2\leq |E(G)|\cdot \mu^{c'}\leq |E(G)|\cdot \mu^{\tilde c}$, assuming that $\tilde c\geq c'$. Lastly, if $\optcrors(I)>|E(G)|^2/\mu^{c'}$, then, since the trivial solution $\phi'$ is considered by the algorithm, it returns a solution of cost at most $|E(G)|^2\leq \optcrors(I)\cdot \mu^{c'}$.



% In this case, either $\optcrors(I)=0$, and our algorithm returns a solution to $I$ of cost $0$; or $|E(G)|\leq \mu^{c'}$, and the algorithm returns the trivial solution, of cost at most $|E(G)|^2\leq |E(G)|\cdot \mu^{c'}\leq |E(G)|\cdot \mu^{\tilde c}$, assuming that $\tilde c\geq c'$.

We assume that the claim holds for all vertices $v(I)$ of $T^*$ with $h(I)<q$, for some $q\geq 0$, and consider any vertex $v(I)$ of the tree $T^*$ such that $h(I)=q$. Let $v(I_1),\ldots,v(I_k)$ be the child vertices of $v(I)$ in the tree $T^*$. Denote $I=(G,\Sigma)$ and $|E(G)|=m$. Additionally, for all $1\leq r\leq k$, denote $I_r=(G_r,\Sigma_r)$ and $m_r=|E(G_r)|$.
 
Since $I$ is not a leaf instance of $T$, $|E(G)|\geq \mu^{c'}$ must hold. 
Since we have assumed that $\event$ does not happen, from \Cref{thm: main}, either $\optcrors(I)> |E(G)|^2/\mu^{c'}$, or $\sum_{r=1}^k\optcrors(I_r)\leq \optcrors(I)\cdot 2^{c_g(\log m)^{3/4}\log\log m} +m\cdot\mu^{c_g}$, and the algorithm $\algcombine$, when given as input a solution $\phi(I')$ to each instance $I'\in \iset^i_j$, returns a solution $\phi$ to instance $I$ with $\cro(\phi)\le c_g\cdot (\sum_{I'\in \iset_j}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{c_g}$. Notice that, in the former case, the algorithm is guaranteed to return a solution to $I$ whose cost is at most $|E(G)|^2\leq \optcrors(I)\cdot \mu^{c'}$, since the trivial solution $\phi'$ is considered as one of the possible solutions. From now on we focus on latter case. For all $1\leq r\leq k$, let $\phi_r$ be the solution to instance $I_r$ that the algorithm computes recursively. From the induction hypothesis, for all $1\leq r\leq k$:
%
\[\cro(\phi_r)\leq  2^{\tilde c\cdot h(I_r)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I_r)+(\log m^*)^{4c_g h(I_r)}\mu^{2c'\cdot \tilde c}\cdot m_r.\]
%
Notice that, for all $1\leq r\leq k$, $h(I_r)\leq q-1$. Moreover, from  \Cref{thm: main}, $\sum_{r=1}^km_r\leq m\cdot(\log m)^{c_g}\leq m\cdot(\log m^*)^{c_g}$. Lastly, as noted already, for some constant $\tilde c'$,  $\sum_{r=1}^k\optcrors(I_r)\leq \optcrors(I)\cdot 2^{\tilde c'(\log m)^{3/4}\log\log m} +m\cdot\mu^{c_g}$ must hold. 
We assume that $\tilde c$ is a large enough constant, so that $\tilde c\geq 2\tilde c'$. 
Altogether, we get that:
%
\[
\begin{split}
\sum_{r=1}^k\cro(\phi_r)&\leq 2^{\tilde c\cdot (q-1)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \sum_{r=1}^k\optcrors(I_r)+(\log m^*)^{4c_g (q-1)}\mu^{2c'\cdot \tilde c}\cdot \sum_{r=1}^km_r
\\
&\leq 2^{\tilde c\cdot (q-1)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \left ( \optcrors(I)\cdot 2^{\tilde c'(\log m)^{3/4}\log\log m} +m\cdot\mu^{c_g}\right )\\
&\hspace{6cm}+(\log m^*)^{4c_g (q-1)}\mu^{2c'\cdot \tilde c}\cdot m\cdot(\log m^*)^{c_g}\\
&\leq 2^{\tilde c\cdot (q-0.5)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+ (\log m^*)^{4c_gq-3c_g}\mu^{2c'\cdot \tilde c}\cdot m\\
&\hspace{6cm}+2^{\tilde c\cdot (q-1)\cdot (\log m^*)^{3/4}\log\log m^*} \cdot\mu^{c_g}\cdot m.
\end{split}\]
%
Since $q\leq \dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$  from \Cref{obs: few recursive levels},
the last term is bounded by:
%
\[ 2^{\tilde c\cdot (\log m^*)^{7/8}/c^*} \cdot\mu^{c_g}\cdot m  \leq \mu^{2c'\tilde c}\]
(since $\mu =2^{c^*(\log m^*)^{7/8}\log\log m^*}$). Therefore, we get that:
%
\[\sum_{r=1}^k\cro(\phi_r)\leq  2^{\tilde c\cdot (q-0.5)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+ (\log m^*)^{4c_gq-2c_g}\mu^{2c'\cdot \tilde c}\cdot m. \]
%

The solution that our algorithm returns for instance $I$ is obtained by applying Algorithm \algcombine from \Cref{thm: main} to solutions $\phi_1,\ldots,\phi_k$ to instances $I_1,\ldots,I_r$. Since event $\event$ does not happen, the cost of the resulting solution is bounded by:
%
\[
\begin{split}
&c_g\cdot\bigg(\sum_{r=1}^k\cro(\phi_r)\bigg) +(\optcrors(I)+m)\cdot\mu^{c_g}\\
&\hspace{1cm}\leq c_g\cdot 2^{\tilde c\cdot (q-0.5)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+\mu^{c_g}\cdot \optcrors(I)\\
&\hspace{3cm}+ c_g\cdot(\log m^*)^{4c_gq-2c_g}\mu^{2c'\cdot \tilde c}\cdot m+\mu^{c_g}\cdot m\\
&\hspace{1cm}\leq 2^{\tilde c\cdot q\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+(\log m^*)^{4c_gq}\mu^{2c'\cdot \tilde c}\cdot m,
\end{split}
\]
%
as required.
%\end{proof}

==> REF.tex <==
@string{STOC = "Proceedings of the Symposium on Theory of Computing"}

@string{FOCS = "Proceedings of the Symposium on Foundations of Computer Science"}

@string{SODA = "Proceedings of the ACM-SIAM Symposium on Discrete Algorithms"}

@string(SOCG="Proceedings of the ACM Symposium on Computational Geometry")

@string{PODS = "Proceedings of the ACM Symposium on Principles of Database Systems"}

@string{SIGMOD = "Proceedings of the ACM SIGMOD International Conference on Management of Data (SIGMOD)"}

@string{VLDB = "Proceedings of the International Conference on Very Large Databases (VLDB)"}

@article{mehlhorn1996embedding,
	title={On the embedding phase of the Hopcroft and Tarjan planarity testing algorithm},
	author={Mehlhorn, Kurt and Mutzel, Petra},
	journal={Algorithmica},
	volume={16},
	number={2},
	pages={233--242},
	year={1996},
	publisher={Springer}
}

@inproceedings{ambuhl2007inapproximability,
	title={Inapproximability results for sparsest cut, optimal linear arrangement, and precedence constrained scheduling},
	author={Ambuhl, Christoph and Mastrolilli, Monaldo and Svensson, Ola},
	booktitle={48th Annual IEEE Symposium on Foundations of Computer Science (FOCS'07)},
	pages={329--337},
	year={2007},
	organization={IEEE}
}

@article{robertson1994quickly,
	title={Quickly excluding a planar graph},
	author={Robertson, Neil and Seymour, Paul and Thomas, Robin},
	journal={Journal of Combinatorial Theory, Series B},
	volume={62},
	number={2},
	pages={323--348},
	year={1994},
	publisher={Elsevier}
}

@article{cabello2013hardness,
  title={Hardness of approximation for crossing number},
  author={Cabello, Sergio},
  journal={Discrete \& Computational Geometry},
  volume={49},
  number={2},
  pages={348--358},
  year={2013},
  publisher={Springer}
}

@inproceedings{fulek2011adjacent,
  title={Adjacent crossings do matter},
  author={Fulek, Radoslav and Pelsmajer, Michael J and Schaefer, Marcus and {\v{S}}tefankovi{\v{c}}, Daniel},
  booktitle={International Symposium on Graph Drawing},
  pages={343--354},
  year={2011},
  organization={Springer}
}

@article{szekely2004successful,
  title={A successful concept for measuring non-planarity of graphs: the crossing number},
  author={Sz{\'e}kely, L{\'a}szl{\'o} A},
  journal={Discrete Mathematics},
  volume={276},
  number={1-3},
  pages={331--352},
  year={2004},
  publisher={Elsevier}
}

@inproceedings{pelsmajer2005odd,
  title={Odd crossing number is not crossing number},
  author={Pelsmajer, Michael J and Schaefer, Marcus and {\v{S}}tefankovi{\v{c}}, Daniel},
  booktitle={International Symposium on Graph Drawing},
  pages={386--396},
  year={2005},
  organization={Springer}
}

@article{pach2000crossing,
  title={Which crossing number is it anyway?},
  author={Pach, J{\'a}nos and T{\'o}th, G{\'e}za},
  journal={Journal of Combinatorial Theory, Series B},
  volume={80},
  number={2},
  pages={225--246},
  year={2000},
  publisher={Elsevier}
}

@article{schaefer2012graph,
  title={The graph crossing number and its variants: A survey},
  author={Schaefer, Marcus},
  journal={The electronic journal of combinatorics},
  pages={DS21--Sep},
  year={2012}
}

@article{robertson1986graph,
  title={Graph minors. V. Excluding a planar graph},
  author={Robertson, Neil and Seymour, Paul D},
  journal={Journal of Combinatorial Theory, Series B},
  volume={41},
  number={1},
  pages={92--114},
  year={1986},
  publisher={Academic Press}
}

@inproceedings{chuzhoy2019towards,
  title={Towards tight (er) bounds for the excluded grid theorem},
  author={Chuzhoy, Julia and Tan, Zihan},
  booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={1445--1464},
  year={2019},
  organization={SIAM}
}


@article{confluent,
	title={(Almost) tight bounds and existence theorems for single-commodity confluent flows},
	author={Chen, Jiangzhuo and Kleinberg, Robert D and Lov{\'a}sz, L{\'a}szl{\'o} and Rajaraman, Rajmohan and Sundaram, Ravi and Vetta, Adrian},
	journal={Journal of the ACM (JACM)},
	volume={54},
	number={4},
	pages={16--es},
	year={2007},
	publisher={ACM New York, NY, USA}
}

@article{chuzhoy2016improved,
  title={Improved bounds for the excluded grid theorem},
  author={Chuzhoy, Julia},
  journal={arXiv preprint arXiv:1602.02629},
  year={2016}
}

@inproceedings{chuzhoy2012polylogarithmic,
  title={A polylogarithmic approximation algorithm for edge-disjoint paths with congestion 2},
  author={Chuzhoy, Julia and Li, Shi},
  booktitle={2012 IEEE 53rd Annual Symposium on Foundations of Computer Science},
  pages={233--242},
  year={2012},
  organization={IEEE}
}

@inproceedings{andrews2010approximation,
  title={Approximation algorithms for the edge-disjoint paths problem via Raecke decompositions},
  author={Andrews, Matthew},
  booktitle={2010 IEEE 51st Annual Symposium on Foundations of Computer Science},
  pages={277--286},
  year={2010},
  organization={IEEE}
}

@article{pach1996applications,
  title={Applications of the crossing number},
  author={Pach, J{\'a}nos and Shahrokhi, Farhad and Szegedy, Mario},
  journal={Algorithmica},
  volume={16},
  number={1},
  pages={111--117},
  year={1996},
  publisher={Springer}
}

@article{khandekar2009graph,
  title={Graph partitioning using single commodity flows},
  author={Khandekar, Rohit and Rao, Satish and Vazirani, Umesh},
  journal={Journal of the ACM (JACM)},
  volume={56},
  number={4},
  pages={1--15},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@incollection{whitney1992congruent,
  title={Congruent graphs and the connectivity of graphs},
  author={Whitney, Hassler},
  booktitle={Hassler Whitney Collected Papers},
  pages={61--79},
  year={1992},
  publisher={Springer}
}

@article{lipton1979separator,
  title={A separator theorem for planar graphs},
  author={Lipton, Richard J and Tarjan, Robert Endre},
  journal={SIAM Journal on Applied Mathematics},
  volume={36},
  number={2},
  pages={177--189},
  year={1979},
  publisher={SIAM}
}

@article{diks1993edge,
  title={Edge separators of planar and outerplanar graphs with applications},
  author={Diks, Krzysztof and Djidjev, Hristo N and Sykora, Ondrej and Vrto, Imrich},
  journal={Journal of Algorithms},
  volume={14},
  number={2},
  pages={258--279},
  year={1993},
  publisher={Elsevier}
}

@incollection{pelsmajer2009odd,
  title={Odd crossing number and crossing number are not the same},
  author={Pelsmajer, Michael J and Schaefer, Marcus and {\v{S}}tefankovic, Daniel},
  booktitle={Twentieth Anniversary Volume:},
  pages={1--13},
  year={2009},
  publisher={Springer}
}

@article{gomory1961multi,
  title={Multi-terminal network flows},
  author={Gomory, Ralph E and Hu, Tien Chung},
  journal={Journal of the Society for Industrial and Applied Mathematics},
  volume={9},
  number={4},
  pages={551--570},
  year={1961},
  publisher={SIAM}
}

@incollection{whitney1992congruent,
  title={Congruent graphs and the connectivity of graphs},
  author={Whitney, Hassler},
  booktitle={Hassler Whitney Collected Papers},
  pages={61--79},
  year={1992},
  publisher={Springer}
}

@article{hopcroft1974efficient,
  title={Efficient planarity testing},
  author={Hopcroft, John and Tarjan, Robert},
  journal={Journal of the ACM (JACM)},
  volume={21},
  number={4},
  pages={549--568},
  year={1974},
  publisher={ACM New York, NY, USA}
}

@inproceedings{chekuri2004edge,
  title={Edge-disjoint paths in planar graphs},
  author={Chekuri, Chandra and Khanna, Sanjeev and Shepherd, F Bruce},
  booktitle={45th Annual IEEE Symposium on Foundations of Computer Science},
  pages={71--80},
  year={2004},
  organization={IEEE}
}

@inproceedings{chuzhoy2012routing,
  title={Routing in undirected graphs with constant congestion},
  author={Chuzhoy, Julia},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
  pages={855--874},
  year={2012}
}

@inproceedings{chuzhoy2012vertex,
  title={On vertex sparsifiers with Steiner nodes},
  author={Chuzhoy, Julia},
  booktitle={Proceedings of the forty-fourth annual ACM symposium on Theory of computing},
  pages={673--688},
  year={2012}
}

@inproceedings{chuzhoy2020towards,
  title={Towards Better Approximation of Graph Crossing Number},
  author={Chuzhoy, Julia and Mahabadi, Sepideh and Tan, Zihan},
  year={To appear at FOCS'20},
}


@article{chekuri2016polynomial,
  title={Polynomial bounds for the grid-minor theorem},
  author={Chekuri, Chandra and Chuzhoy, Julia},
  journal={Journal of the ACM (JACM)},
  volume={63},
  number={5},
  pages={1--65},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@article{ajtai82,
  author = {M.~Ajtai and V.~Chv\'{a}tal and M.~Newborn and E.~Szemer\'{e}di},
  title = {Crossing-free subgraphs},
  journal = {Theory and Practice of Combinatorics},
  year = {1982},
  pages = {9-12}
}

@inproceedings{Ambuhl07,
  author = {C.~Ambuhl and M.~Mastrolilli and O.~Svensson},
  title = {Inapproximability Results for Sparsest Cut, Optimal Linear Arrangement, and Precedence Constrained Scheduling},
  booktitle = {Proceedings of the 48th Annual IEEE Symposium on Foundations of Computer Science},
  year = {2007},
  pages = {329--337}
}

@article{ARV,
  author    = {Sanjeev Arora and
               Satish Rao and
               Umesh V. Vazirani},
  title     = {Expander flows, geometric embeddings and graph partitioning},
  journal   = {J. ACM},
  volume    = {56},
  number    = {2},
  year      = {2009},
  ee        = {http://doi.acm.org/10.1145/1502793.1502794},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{bannister2014crossing,
  title={Crossing minimization for 1-page and 2-page drawings of graphs with bounded treewidth},
  author={Bannister, Michael J and Eppstein, David},
  booktitle={International Symposium on Graph Drawing},
  pages={210--221},
  year={2014},
  organization={Springer}
}


@article{bhatt1984framework,
  title={A framework for solving VLSI graph layout problems},
  author={Bhatt, Sandeep N and Leighton, Frank Thomson},
  journal={Journal of Computer and System Sciences},
  volume={28},
  number={2},
  pages={300--343},
  year={1984},
  publisher={Elsevier}
}


@inproceedings{chekuri2004edge,
  title={Edge-disjoint paths in planar graphs},
  author={Chekuri, Chandra and Khanna, Sanjeev and Shepherd, F Bruce},
  booktitle={45th Annual IEEE Symposium on Foundations of Computer Science},
  pages={71--80},
  year={2004},
  organization={IEEE}
}

@inproceedings{chekuri2005multicommodity,
  title={Multicommodity flow, well-linked terminals, and routing problems},
  author={Chekuri, Chandra and Khanna, Sanjeev and Shepherd, F Bruce},
  booktitle={Proceedings of the thirty-seventh annual ACM symposium on Theory of computing},
  pages={183--192},
  year={2005},
  organization={ACM}
}

@inproceedings{chekuri2013approximation,
  title={Approximation algorithms for Euler genus and related problems},
  author={Chekuri, Chandra and Sidiropoulos, Anastasios},
  booktitle={2013 IEEE 54th Annual Symposium on Foundations of Computer Science},
  pages={167--176},
  year={2013},
  organization={IEEE}
}


@Misc{Tasos-comm,
	author       = {Anastasios Sidiropoulos},
	howpublished = {{Personal communication}},
	year         = {2010},
}

@article{chen2007almost,
  title={(Almost) tight bounds and existence theorems for single-commodity confluent flows},
  author={Chen, Jiangzhuo and Kleinberg, Robert D and Lov{\'a}sz, L{\'a}szl{\'o} and Rajaraman, Rajmohan and Sundaram, Ravi and Vetta, Adrian},
  journal={Journal of the ACM (JACM)},
  volume={54},
  number={4},
  pages={16},
  year={2007},
  publisher={ACM}
}


@inproceedings{chimani2011tighter,
  title={A tighter insertion-based approximation of the crossing number},
  author={Chimani, Markus and Hlin{\v{e}}n{\`y}, Petr},
  booktitle={International Colloquium on Automata, Languages, and Programming},
  pages={122--134},
  year={2011},
  organization={Springer}
}

@incollection{crossing-survey,
	author    = {Christoph Buchheim and
	Markus Chimani and
	Carsten Gutwenger and
	Michael J{\"{u}}nger and
	Petra Mutzel},
	title     = {Crossings and Planarization},
	booktitle = {Handbook on Graph Drawing and Visualization},
	pages     = {43--85},
	year      = {2013},
	timestamp = {Wed, 12 Jul 2017 09:11:51 +0200},
	biburl    = {https://dblp.org/rec/bib/reference/crc/BuchheimCGJM13},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{chuzhoy2011algorithm,
  title={An algorithm for the graph crossing number problem},
  author={Chuzhoy, Julia},
  booktitle={Proceedings of the forty-third annual ACM symposium on Theory of computing},
  pages={303--312},
  year={2011},
  organization={ACM}
}

@inproceedings{chuzhoy-lowerbound,
  title={},
  author={Chuzhoy, Julia and Madan, Vivek and Mahabadi, Sepideh},
  booktitle={Private Communication},
  year={2016},
}

@inproceedings{chuzhoy2016improved,
  title={Improved approximation for node-disjoint paths in planar graphs},
  author={Chuzhoy, Julia and Kim, David HK and Li, Shi},
  booktitle={Proceedings of the forty-eighth annual ACM symposium on Theory of Computing},
  pages={556--569},
  year={2016},
  organization={ACM}
}

@inproceedings{chuzhoy2011graph,
  title={On graph crossing number and edge planarization},
  author={Chuzhoy, Julia and Makarychev, Yury and Sidiropoulos, Anastasios},
  booktitle={Proceedings of the twenty-second annual ACM-SIAM symposium on Discrete algorithms},
  pages={1050--1069},
  year={2011},
  organization={SIAM}
}

@article{didimo2019survey,
  title={A survey on graph drawing beyond planarity},
  author={Didimo, Walter and Liotta, Giuseppe and Montecchiani, Fabrizio},
  journal={ACM Computing Surveys (CSUR)},
  volume={52},
  number={1},
  pages={1--37},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@article{even2002improved,
  title={Improved approximations of crossings in graph drawings and VLSI layout areas},
  author={Even, Guy and Guha, Sudipto and Schieber, Baruch},
  journal={SIAM Journal on Computing},
  volume={32},
  number={1},
  pages={231--252},
  year={2002},
  publisher={SIAM}
}

@article{crossing_np_complete,
  author = {M.~R.~Garey and D.~S.~Johnson},
  title = {Crossing number is {NP}-complete},
  journal = {SIAM J.~Algebraic Discrete Methods},
  volume = {4},
  number = {3},
  year = {1983},
  pages = {312-316}
}

@article{Grohe04,
 author = {M.~Grohe},
 title = {Computing crossing numbers in quadratic time},
 journal = {J.~Comput.~Syst.~Sci.},
 volume = {68},
 number = {2},
 year = {2004},
 pages = {285--302},
}

@article{Hlineny06a,
  author    = {P.~Hlinen{\'y}},
  title     = {Crossing number is hard for cubic graphs},
  journal   = {J. Comb. Theory, Ser. B},
  volume    = {96},
  number    = {4},
  year      = {2006},
  pages     = {455--471}
}

@inproceedings{hlinveny2006crossing,
  title={On the crossing number of almost planar graphs},
  author={Hlin{\v{e}}n{\`y}, Petr and Salazar, Gelasio},
  booktitle={International Symposium on Graph Drawing},
  pages={162--173},
  year={2006},
  organization={Springer}
}

@article{hlinveny2015crossing,
  title={Crossing number is hard for kernelization},
  author={Hlin{\v{e}}n{\`y}, Petr and Der{\v{n}}{\'a}r, Marek},
  journal={arXiv preprint arXiv:1512.02379},
  year={2015}
}


@inproceedings{KawarabayashiR07,
  author    = {K.~Kawarabayashi and
               B.~A.~Reed},
  title     = {Computing crossing number in linear time},
  booktitle = {STOC},
  year      = {2007},
  pages     = {382--390}
}


@inproceedings{KawarabayashiSidi17,
	author    = {Ken{-}ichi Kawarabayashi and
	Anastasios Sidiropoulos},
	title     = {Polylogarithmic Approximation for Minimum Planarization (Almost)},
	booktitle = {58th {IEEE} Annual Symposium on Foundations of Computer Science, {FOCS}
	2017, Berkeley, CA, USA, October 15-17, 2017},
	pages     = {779--788},
	year      = {2017},
	url       = {https://doi.org/10.1109/FOCS.2017.77},
	doi       = {10.1109/FOCS.2017.77},
	timestamp = {Tue, 04 Dec 2018 10:17:29 +0100},
	biburl    = {https://dblp.org/rec/bib/conf/focs/KawarabayashiS17},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{kawarabayashi2019polylogarithmic,
  title={Polylogarithmic approximation for Euler genus on bounded degree graphs},
  author={Kawarabayashi, Ken-ichi and Sidiropoulos, Anastasios},
  booktitle={Proceedings of the 51st Annual ACM SIGACT Symposium on Theory of Computing},
  pages={164--175},
  year={2019},
  organization={ACM}
}

@book{matousek_book,
  author = {J.~Matou\v{s}ek},
  title = {Lectures on discrete geometry},
  publisher = {Springer-Verlag},
  year = {2002}
}

@article{leighton1999multicommodity,
  title={Multicommodity max-flow min-cut theorems and their use in designing approximation algorithms},
  author={Leighton, Tom and Rao, Satish},
  journal={Journal of the ACM (JACM)},
  volume={46},
  number={6},
  pages={787--832},
  year={1999},
  publisher={ACM}
}

@book{leighton_book,
  author = {F.~T.~Leighton},
  title = {Complexity issues in {VLSI}: optimal layouts for the shuffle-exchange graph and other networks},
  year = {1983},
  publisher = {MIT Press}
}


@article{planar-separator,
author = {Richard J. Lipton and Robert Endre Tarjan},
title = {A Separator Theorem for Planar Graphs},
publisher = {SIAM},
year = {1979},
journal = {SIAM Journal on Applied Mathematics},
volume = {36},
number = {2},
pages = {177-189},
url = {http://link.aip.org/link/?SMM/36/177/1},
doi = {10.1137/0136016}
}

@article{pach_survey,
  author = {J.~Pach and G.~T\'{o}th},
  title = {Thirteen problems on crossing numbers},
  journal = {Geombinatorics},
  volume = {9},
  number = {4},
  pages = {194-207},
  year = {2000}
}

@inproceedings{pelsmajer2007crossing,
  title={Crossing numbers and parameterized complexity},
  author={Pelsmajer, Michael J and Schaefer, Marcus and {\v{S}}tefankovi{\v{c}}, Daniel},
  booktitle={International Symposium on Graph Drawing},
  pages={31--36},
  year={2007},
  organization={Springer}
}


@inproceedings{racke2002minimizing,
  title={Minimizing congestion in general networks},
  author={Racke, Harald},
  booktitle={The 43rd Annual IEEE Symposium on Foundations of Computer Science, 2002. Proceedings.},
  pages={43--52},
  year={2002},
  organization={IEEE}
}

@incollection{richter_survey,
  author =	 "R.~B.~Richter and G.~Salazar",
  title =	 "Crossing numbers",
  booktitle =	 "Topics in Topological Graph Theory",
  editor =	 "L.~W.~Beineke and R.~J.~Wilson",
  publisher =	 "Cambridge University Press",
  year =	 2009,
  chapter =	 "7",
  pages =	 "133--150"
}


@inproceedings{shahrokhi1994book,
  title={Book embeddings and crossing numbers},
  author={Shahrokhi, Farhad and S{\`y}kora, Ondrej and Sz{\'e}kely, L{\'a}szl{\'o} A and Vrt'o, Imrich},
  booktitle={International Workshop on Graph-Theoretic Concepts in Computer Science},
  pages={256--268},
  year={1994},
  organization={Springer}
}

@article{turan_first,
  author = {P.~Tur\'{a}n},
  title = {A note of welcome},
  journal = {J.~Graph Theory},
  volume = {1},
  year = {1977},
  pages = {1-5}
}

@misc{vrto_biblio,
  author = {Imrich Vrto},
  title = {Crossing numbers of graphs: A bibliography},
  howpublished = {\url{http://www.ifi.savba.sk/~imrich}}
}

@incollection{whitney1992congruent,
  title={Congruent graphs and the connectivity of graphs},
  author={Whitney, Hassler},
  booktitle={Hassler Whitney Collected Papers},
  pages={61--79},
  year={1992},
  publisher={Springer}
}


@article{robertson1986graph,
  title={Graph minors. VI. Disjoint paths across a disc},
  author={Robertson, Neil and Seymour, Paul D},
  journal={Journal of Combinatorial Theory, Series B},
  volume={41},
  number={1},
  pages={115--138},
  year={1986},
  publisher={Elsevier}
}

@article{pelsmajer2011crossing,
  title={Crossing numbers of graphs with rotation systems},
  author={Pelsmajer, Michael J and Schaefer, Marcus and {\v{S}}tefankovi{\v{c}}, Daniel},
  journal={Algorithmica},
  volume={60},
  number={3},
  pages={679--702},
  year={2011},
  publisher={Springer}
}

==> WL-flower_decomp.tex <==
\subsubsection*{Step 1: Separating high-degree vertices}
\label{sec:size_reduction}

In the first step, we recursively decompose $G'$ into a set $\cset_1$ of clusters, such that each cluster contains at most one high-degree vertex, as follows.
Throughout, we maintain a set $\hat\cset$ of clusters of $G$. Initially, $\hat\cset=\set{G}$.
While there exists some cluster $C\in \hat\cset$ that contains at least two high-degree vertices, algorithm continues to be executed as follows.
We pick arbitrarily a cluster $C\in \hat\cset$ with at least two high-degree vertices. Let $u,u'$ be two high-degree vertices of $C$. We compute a $u$-$u'$ min-cut of $C$, and let $C_u, C_{u'}$ be the two clusters obtained from $C$ by deleting the edges in the min-cut. We then replace the cluster $C$ in $\hat\cset$ with clusters $C_u, C_{u'}$ and continue to the next iteration. This completes the description of the first step. Let $\cset_1$ be the set of clusters that we obtain ta the end of the first step. Clearly, each cluster of $\cset_1$ contains at most one high-degree vertex.

We now show that $|\inE(\cset_1)|=O(m/\mu^2)$. Since a high-degree vertex has degree at least $m/\mu^8$, initially $G$ contains at most $\mu^8$ high-degree vertices. Therefore, in the first step we performed at most $\mu^8$ min-cut computations. On the other hand, since $G$ is not $\mu$-interesting, all min-cuts that we computed in the first step has size at most $m/\mu^{12}$. It follows that $|E(\cset_1)|\le O(\mu^8)\cdot O(m/\mu^{12})=O(m/\mu^4)$.


\subsubsection*{Step 2: Trimming clusters with a high-degree vertex} 

In this step, we further process the clusters of $\cset_1$ that contains a high-degree vertex one-by-one, as follows.
Let $C$ be a cluster in $\cset_1$ that contains a unique high-degree vertex $u$.
We compute a min-cut $(A,B)$ of $\tilde C$ separating $u$ from all vertices of $\Gamma(C)$ (recall that $\Gamma(C)$ the set of endpoints of edges in $\delta(C)$ that do not lie in $C$), with $u\in A$. Let $C'$ be the subgraph of $C$ induced by vertices of $A$.
Therefore, $|E(C',C\setminus C')|\le |\delta(C)|$.
We decompose the cluster $C$ into $C'$ and $C\setminus C'$.
Note that $C'$ is connected and still contains a unique high-degree vertex $u$, and there is a set of edge-disjoint paths in $C'$ connecting $\delta(C')$ to $u$.
Also note that and the subgraph $C\setminus C'$ does not contain any high-degree vertex, and it may not be connected. 
We replace the cluster $C$ in $\hat\cset$ by cluster $C'$ and connected components of $C\setminus C'$.  
%We then mark the connected components of $C''$ inactive. If $|E(C')|>m/\mu^2$, then we mark $C'$ active; otherwise we mark it inactive. This completes the description of an iteration.

We further process the cluster $C'$ as follows.
Let $d=m/\mu^{10}$.
Denote $\delta(u)=\set{e_1,\ldots,e_{\deg(u)}}$, where the edges are indexed according to the ordering $\oset_u$ in $\Sigma$.
Denote $r=\lceil\frac{\deg(u)}{d}\rceil$.
For each $1\le i\le r-1$, let $E_i=\set{e_{(i-1)d+1},\ldots,e_{id}}$, and let $E_{r}=\set{e_{(r-1)d+1},\ldots,e_{\deg(u)}}$.
Clearly, sets $E_1,E_2,\ldots,E_r$ are consecutive subsets of edges in $\delta(u)$, each containing at most $d$ edges. 
Let the cluster $\tilde C'$ be obtained from $C'$ by replacing the vertex $u$ with $r$ distinct new vertices $u_1,\ldots,u_r$, such that for each $1\le i\le r$, the edges of $E_i$ are incident to $u_i$. 
Denote $U=\set{u_1,\ldots,u_r}$. 
For each $1\le i\le r$, we compute a min-cut $(A_i,B_i)$ of $\tilde C'$, that separates $u_i$ from all vertices in $U\setminus \set{u_i}$, with $u_i\in A_i$. 
From Lemma~\ref{lem:min-cut_structure}, the sets $\set{A_i}_{1\le i\le r}$ are mutually disjoint.
We denote by $X_i$ the subgraph of $C'$ induced by vertices of $A_i$, so the clusters $X_1,\ldots,X_r$ are mutually vertex-disjoint. Note that, since $G$ is not $\mu$-interesting, for each $1\le i\le r$, $|E(X_i,C'\setminus X_i)|\le m/\mu^{12}$, so $\sum_{1\le i\le r} |E(X_i,C'\setminus X_i)|\le O(\deg(u)/d)\cdot O(m/\mu^{12})\le O(\deg(u)/\mu^2)$.
%We call $X_i$ a \emph{sub-cluster} of $C$. 
%and we denote $\xset=\set{X_1,\ldots,X_r}$.
For each $1\le i\le r$, we denote $\tilde E_i=\delta(X_i)$. 
%See Figure~\ref{fig:flower_edge} for an illustration.
We use the following observation.

\begin{observation}
\label{obs: pedal-well-linked}
For each $1\le i\le r$, there is a set $\qset_i$ of paths in $X_i$ connecting edges of $\tilde  E_i$ to $u_i$, such that $\cong_{X_i}(\qset_i)\le O(1)$.
\end{observation} 
\begin{proof}
The set $\tilde E_i$ can be partitioned into two subsets: set $\tilde E'_i$ of edges connecting a vertex of $X_i$ to some vertex of $\tilde C\setminus X_i$, and set $\tilde E''_i$ of edges connecting a vertex of $X_i$ to some vertex of $G\setminus C'$. 
%Note that $\tilde E''_i\subseteq\delta(C')$.

We first show that there is a set $\qset'_i$ of edge-disjoint paths in $X_i$ connecting edges of $\tilde E'_i$ to $u_i$.
Assume not, then there exists a cut $(A'_i, B'_i)$ in $X_i$ separating all vertices of $\Gamma(X_i)$ from $u_i$, such that $|E(A'_i,B'_i)|\le |\Gamma(X_i)|$. Clearly, the cut $(A'_i,V(\tilde C')\setminus A'_i)$ also separates $u_i$ from all vertices in $U\setminus\set{u_i}$, causing a contradiction to the minimality of the cut $(A_i,B_i)$.

We then show that there is a set $\qset''_i$ of paths in $X_i$ connecting edges of $\tilde E'_i$ to $u_i$, such that $\cong_{X_i}(\qset'')\le 2$.
Note that $\tilde E''_i\subseteq\delta(C')$, and recall that there is a set $\pset$ of edge-disjoint paths connecting $\delta(C')$ to $u$. 
Let $\pset_i\subseteq \pset$ be the subset of paths connecting edges of $\tilde E''_i$ to $u$. Consider a path $P_e\in \pset_i$ that connects the edge $e\in \tilde E''_i$ to $u$. Either it lies entirely in cluster $X_i$, or it starts at $e$, goes over some edges of $X_i$, and leaves cluster $X_i$ via some edge $e'\in \tilde E'_i$.
In the latter case, let $P'_e$ be path obtained by concatenating (i) the maximal beginning subpath of $P$ (the subpath containing $e$) that lies in $X_i$; and (ii) the path of $\qset'_i$ that connects the edge $e'$ to $u$ minus the edge $e'$. Clearly, $P'_e$ connects edge $e$ to $u$ and lies entirely in $X_i$. We let the set $\qset''_i$ contains (i) all paths of $\pset_i$ that lies entirely in $X_i$; and (ii) for each path $P_e\in \pset_i$ that connects the edge $e$ to $u$, the path $P'_e$. It remains to show that $\cong_{X_i}(\qset'')\le 2$.
Since the paths in $\pset_i$ are edge-disjoint, each path in $\pset_i$ contains a distinct edge of $\tilde E'_i$, if any.
Therefore, for each edge $e\in X_i$, $\cong_{\qset''_i}(e)\le \cong_{\pset_i}(e)+\cong_{\qset'_i}(e)\le 2$.

Observation~\ref{obs: pedal-well-linked} now follows by letting $\qset_i=\qset'_i\cup \qset''_i$. 
\end{proof}


\begin{figure}[h]
	\includegraphics[scale=0.3]{figs/flower_edge.jpg}
	\caption{An illustration of the edge sets in a flower cluster.\label{fig:flower_edge}}
\end{figure} 


Let $C''$ be the cluster obtained by first taking the union of clusters $X_1,\ldots,X_r$, and then unifying the vertices $v_1,\ldots,v_r$ back to the original vertex $v$. 
Put in other words, $C''$ is the subgraph of $C'$ induced by vertices of $\bigcup_{1\le i\le r}V(X_i)$. 
See Figure~\ref{fig:flower_edge} for an illustration. 
From Observation~\ref{obs: pedal-well-linked} and the definitions of good cluster and flower cluster: if $E(C'')|>m/\mu^2$, $C''$ is a flower cluster; otherwise, it is a good cluster.
We decompose the cluster $C'$ into $C''$ and $C'\setminus C''$ by deleting from $C'$ the edges of $E(C'',C'\setminus C'')$.
Note that and the subgraph $C'\setminus C''$ does not contain any high-degree vertex, and it may not be connected. We replace the cluster $C'$ in $\hat\cset$ by cluster $C''$ and connected components of $C'\setminus C''$.

Let $\cset_2$ be the set of clusters that we obtain after processing every cluster of $\cset_1$ that contains a high-degree node in this way. We now show that $|\inE(\cset_2)|=O(m/\mu)$.
Let $C$ be any cluster in $\cset_1$ that contains a high-degree vertex. Recall that $C$ is first decomposed into $C'$ and $C\setminus C'$, and then $C'$ is further decomposed into $C''$ and $C'\setminus C''$. Therefore, from the above discussion, the number of edges between sub-clusters of $C$ in $\cset_2$ is $|E(C',C\setminus C')|+|E(C'',C'\setminus C'')|\le |\delta(C)|+O(\deg(u)/\mu)$. Summing over all clusters $C\in \cset_1$ that contains a high-degree vertex, we get that $|\inE(\cset_2)|\le O(|\inE(\cset_1)|)+O(|E(C)|/\mu^2)\le O(m/\mu^2)$.


\subsubsection*{Step 3: Size reduction via balanced cuts}

The set $\cset_2$ of clusters we obtain after the second step can be further decomposed into three subsets: set $\cset^f_2$ of flower clusters, set $\cset^g_2$ of good clusters, and the set $\cset'_2$ that contains all other clusters. Note that no clusters in $\cset'_2$ contain high-degree vertices. In this step, we will further decompose clusters of $\cset'_2$ into good clusters.

We first iteratively decompose clusters of $\cset'_2$ that contains more than $m/\mu^2$ edges into smaller clusters, as follows.
Throughout, we maintain a set $\hat\cset$ of clusters of $G$. Initially, $\hat\cset=\cset'_2$. The algorithm in this step proceeds in iterations and continues to be executed as long as $\hat\cset$ contains a cluster with more than $m/\mu^2$ edges.
In each iteration, we pick arbitrarily a cluster $C$ in $\hat \cset$ with $|E(C)|\ge m/\mu^2$. We apply the algorithm in Theorem~\ref{thm:most_balanced_sparsest-cut} to $C$ and obtain a cut $(A,B)$ of $C$, and check the size of $|E(A,B)|$. If $|E(A,B)|\ge m\cdot \log n/\mu^4$, then we report $\optcrors(G',\Sigma')\ge |E(G')|^2/\mu^{10}$ and the algorithm is aborted. If $|E(A,B)|\le O(m\cdot \log n/\mu^4)$, then replace the cluster $C$ with the subgraphs of $C$ induced by $A$ and $B$, respectively.
This completes the description of the algorithm in this step.

We first show that, whenever we claim that $\optcrors(G',\Sigma')\ge |E(G')|^2/\mu^{10}$, the claim is correct.
\begin{observation}
\label{obs: abort_correctly}
Let $(A,B)$ be the cut of $C$ that we obtained in some iteration of the algorithm. If $|E(A,B)|\ge m\cdot \log n/\mu^4$, then $\optcrors(G',\Sigma')\ge |E(G')|^2/\mu^{10}$.
\end{observation}
\begin{proof}
Assume the contrast that $\optcrors(G',\Sigma')\le |E(G')|^2/\mu^{10}$. Note that, if we denote by $\Sigma_C$ the rotation system on $C$ induced by $\Sigma'$, then $\optcro(C)\le \optcrors(C,\Sigma_C)\le \optcrors(G',\Sigma')$. Recall that $C$ has no high-degree vertices, so $\Delta(C)\le m/\mu^8$.
Therefore, from Lemma~\ref{lem:min_bal_cut}, the size of the minimum balanced cut in $C$ is at most  $O\big(\sqrt{\optcro(C)+|E(C)|\cdot\Delta(C)}\big)\le O\big( \sqrt{m^2/\mu^{10}+m\cdot(m/\mu^8)}\big)\leq  O(m/\mu^{4})$. Then from Theorem~\ref{thm:most_balanced_sparsest-cut}, the size of the cut $(A,B)$ is at most $O(\sqrt{\log n}\cdot m/\mu^{4})<m\cdot \log n/\mu^4$, a contradiction.
\end{proof}

Let $\cset'_3$ be the set of clusters that we obtain from decomposing the clusters of $\cset'_2$ in this step. Denote $\cset_3=\cset^f_2 \cup\cset^g_2 \cup \cset'_3$. 
We now show that, if the algorithm is not aborted, then $|\inE(\cset_3)|=O(m\log n/\mu^2)$.
Note that $\inE(\cset_3)\setminus \inE(\cset_2)=\inE(\cset'_3)\setminus \inE(\cset'_2)$, namely the new edges in $\inE(\cset_3)$ come from decomposing the clusters in $\inE(\cset'_2)$. From the algorithm in this step, each resulting cluster in  $\inE(\cset_3)$ has size at least $\Omega(m/\mu^2)$. Therefore, the number of balanced-cut computations that we have performed in this step is at most $\mu^2$. From Observation~\ref{obs: abort_correctly}, if the algorithm is not aborted, then each cut that we computed has size at most $m\cdot \log n/\mu^4$. Therefore, the total number of inter-cluster edges that we have created in this step is $O(m\cdot \log n/\mu^4)\cdot O(\mu^2)=O(m\cdot \log n/\mu^2)$. As a result, $|\inE(\cset_3)|\le |\inE(\cset_2)|+O(m\cdot \log n/\mu^2)=O(m\cdot \log n/\mu^2)$.



\subsubsection*{Step 4: Well-linked decomposition}

Recall that after the third step, we obtain a set $\cset_3$ of clusters with $|\inE(\cset_3)|\le O(m\cdot \log n/\mu^2)$, that can be further decomposed into
$\cset_3=\cset^f_2 \cup\cset^g_2 \cup \cset'_3$, where the set $\cset^f_2$ contains flower clusters, the set $\cset^g_2$ contains good clusters, and the set $\cset'_3$ contains clusters with at most $m/\mu^2$ edges and no high-degree vertices.

In this step, we further decompose clusters in $\cset'_3$ to get good clusters. Specifically, for each cluster $C$ of $\cset'_3$, we apply the algorithm of Theorem~\ref{thm:well_linked_decomposition} to it, and obtain a set $\set{C_1,\ldots,C_k}$ of clusters. We then replace the cluster $C$ in $\cset'_3$ with clusters $C_1,\ldots,C_k$. This completes the description of this step.

Let $\cset^g_4$ be the set of clusters that we obtain from decomposing the clusters of $\cset'_2$ in this step. From Theorem~\ref{thm:well_linked_decomposition}, every cluster of $\cset^g_4$ is $\alpha$-boundary-well-linked. Since every cluster of $\cset^g_4$ contains at most $m/\mu^2$ edges, by definition, every cluster of $\cset^g_4$ is a good cluster. Therefore, if we denote by $\cset^*$ the set of clusters that we obtain after the four steps, then each cluster of $\cset^*$ is either a good cluster or a flower cluster.

It remains to show that $|\inE(\cset^*)|\le O(m/\mu)$. Note that $\inE(\cset^*)\setminus \inE(\cset_3)=\inE(\cset^g_4)\setminus \inE(\cset'_3)$.
From Theorem~\ref{thm:well_linked_decomposition}, $|\inE(\cset^g_4)\setminus \inE(\cset'_3)|\le O(|\inE(\cset_3)|)\le O(m\cdot \log n/\mu^2)$. Therefore, $|\inE(\cset^*)|\le O(|\inE(\cset_3)|)\le O(m\cdot \log n/\mu^2)$.

This completes the proof of Lemma~\ref{lem:main_decomposition}.














%\subsubsection{Technical Lemmas}

\iffalse
\begin{theorem}[Theorem 3 of \cite{chuzhoy2012vertex}]
	There is an efficient algorithm, that given any graph $G=(V,E)$ and any cluster $S\subseteq V$ of vertices with $|\delta(S)|=z$, computes a set $\rset$ of clusters of $S$, such that, 
	\begin{itemize}
		\item the vertex sets $\set{V(R)}_{R\in \rset}$ partitions $V(S)$;
		\item for each cluster $R\subseteq\rset$, $|\delta(R)|\le |\delta(S)|$;
		\item for each cluster $R\subseteq\rset$, $R$ is $\Omega(\log^{-3/2}z)$-boundary-well-linked;
		\item $\sum_{R\in \rset}|\delta(R)|\le 1.2|\delta(S)|$.
	\end{itemize}


	
\begin{lemma}
	\label{lem:min-cut_structure}
	Let $G$ be any graph, and let $x,y,s,t$ be vertices of $G$. Let $(X,Y)$ be the minimum $x$-$y$ cut, and let $(S,T)$ be the minimum $s$-$t$ cut. Then one of the following must hold:
	\begin{itemize}
		\item $S\subseteq X, Y\subseteq T$; or 
		\item $X\subseteq S,T\subseteq Y$; or
		\item $T\subseteq X, Y\subseteq S$; or
		\item $X\subseteq T, S\subseteq Y$.
	\end{itemize}
	In other words, the two cuts are laminar, and one side of the first cut must be contained in one side of the second cut and vice versa.
\end{lemma}
	\fi



==> apd_local_non_int.tex <==
\section{Proof of Lemma~\ref{lem:local_non_int}}
\label{apd:locally_non_interfering}

 In this section we provide the proof of Lemma~\ref{lem:local_non_int}. 
 
 We view the paths in $\tilde\pset$ as originating from $v$ and ending at $v'$.
 First, we perform the standard re-routing to the paths of $\tilde\pset$ and obtain another set $\tilde\pset'$ of paths, such that $E(\tilde\pset')\subseteq E(\tilde\pset)$, and the graph consisting of directed paths in $\tilde\pset'$ is a DAG.
 This defines a topological order on vertices of $G$.
 We will sequentially perform, for each vertex $u\in V(G)\setminus\set{v,v'}$  according to this topological order, a \emph{route-swap} operation to all the paths that contains $u$, that is defined as follows. 
 
 Consider the graph $G[\tilde\pset',u]$ and think of the edges in $G[\tilde\pset',u]$ as directed edges, so each edge is an \emph{in-edge} if it is directed towards $u$, and is an \emph{out-edge} otherwise. We first recompute a matching between the in-edges and the out-edges, such that the paths formed by the new pairs of edges are locally non-interfering at $u$. Let $(e_{in}, e_{out})$ be a pair in the matching, where $e_{in}$ originally belongs to the path $P$ of $\tilde{\pset'}$ and $e_{out}$ originally belongs to the path $P$ of $\tilde{\pset'}$. We define a new path from this pair $(e_{in}, e_{out})$ as the concatenation of the subpath of $P$ between $v$ and $u$, and the subpath of $P'$ between $u$ and $v'$. We replace the paths in $\tilde\pset'$ that contains $u$ with all the new paths that we defined according the the matching. This completes the description of a route-swap operation.
 See Figure~\ref{fig:route_swap} for an illustration.
 \begin{figure}[h]
 	\label{fig:route_swap}
 	\centering
 	\subfigure[Before: the paths are not locally non-interfering at $u$.]
 	{\scalebox{0.33}{\includegraphics{figs/route_swap_1}}}
 	\hspace{0cm}
 	\subfigure[After: the paths are locally non-interfering at $u$.]
 	{\scalebox{0.33}{\includegraphics{figs/route_swap_2}}}
 	\caption{An illustration of a route-swap operation.} 
 \end{figure}
 It is not hard to see that, after the route-swap operation at $u$, the paths in $\tilde\pset'$ are locally non-interfering at $u$. Therefore, if we denote by $\pset$ the resulting set of paths that we obtain, then the paths in $\pset$ are locally non-interfering at all vertices of $V(G)\setminus\set{v,v'}$. This completes the proof of Lemma~\ref{lem:local_non_int}.


==> apd_many_paths-backup.tex <==
\section{Proofs Omitted from \Cref{sec: many paths}}
\label{Proofs Omitted from many paths}




\subsection{Proof of \Cref{obs: combine solutions for split}}
\label{subsec: combine solutions for split}

We denote $I_F=(G_F,\Sigma_F)$,  $I_{F_1}=(G_{F_1},\Sigma_{F_1}), I_{F_2}=(G_{F_2},\Sigma_{F_2})$. We also denote the skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$, the augmneting structure $\aset=(\Pi_F=\set{P_1,P_2},\set{b_u}_{u\in V(K\cup P_1\cup P_2)}, \psi')$, and $K'=K\cup P_1\cup P_2$.

We construct the solution $\phi$ to instance $I_F$ gradually. We start by letting
$\phi$ be the drawing $\psi'$ of graph $K'$, and then gradually modify it.

Consider the clean solution $\phi_1$ to the $F_1$-instance $I_{F_1}$. From the definition of augmentation, there must be a single connected component $C\in \cset(F_1)$, with $P_1\cup P_2\subseteq C$. We let $\sigma$ be a closed curve that follows the boundary of $C$ just inside the face $F_1$, and we let $D$ be the disc whose boundary is $\sigma$, and whose interior contains the images of all vertices of $G_{F_1}$. We can define a similar disc $D'$ in the current drawing $\phi$ of $K'$. We then move the contents of the disc $D$ in drawing $\phi_1$ to disc $D'$ in drawing $\phi$, so that the boundaries of both discs coinside. In this way, we ``plant'' the drawing $\phi_1$ of $G_{F_1}$ inside face $F_1$ in $\phi$ (we need to extend the images of the edges incident to the vertices of $C$ so that they terminate at their endpoints in $C$, similarly to their drawing in $\phi_1$). We use a similar procedure to ``plant'' the drawing $\phi_2$  of $G_{F_2}$ inside face $F_2$ of $\phi$. 

So far we have constructed a drawing $\phi$ of graph $G_F\setminus E^{\del}$, in which  all vertices and edges are drawn in face $F$, the rotation system induced by $\Sigma_F$ is respected, and the number of crossings is $\cro(\phi_1)+\cro(\phi_2)$. In order to complete the drawing $\phi$ of graph $G_F$, it remains to ``insert'' the images of the edges of $E^{\del}$ into this drawing. 
We do so using the following lemma from \cite{chuzhoy2020towards}.

\begin{lemma}[Lemma 9.2 of \cite{chuzhoy2020towards}]
	There is an efficient algorithm, that, given an instance $(H,\Sigma)$ of the \CNwRS problem, a subset $E'\subseteq E(H)$ of edges of $H$, and a drawing $\phi$ of graph $H\setminus E'$ that respects $\Sigma$, compute a drawing $\phi'$ of $H$ that respects $\Sigma$, such that $\cro(\phi')\le \cro(\phi)+|E'|\cdot |E(H)|$.
\end{lemma}

There is one subtlety in using the above lemma directly in order to insert the edges of $E^{\del}$ into the drawing $\phi$: we need to ensure that the drawing remains clean, so the images of the newly inserted edges may not cross the images of the edges of $\partial(F)$. This is easy to achieve, for example, by making a large number copies of every edge in $\partial(F)$, so that the copy of each such edge $e$ that is furthest from the boundary of $F$ will not be crossed by any newly inserted edges (as otherwise we would create a crossing with every copy of $e$, resulting in too many crossings). Another equivalent approach is to first contract every connected component of $\partial(F)$ into a supernode, insert the edges of $E^{\del}$ into the resulting drawing of the contracted instance, and then un-contract the supernodes. In either case, we obtain a clean drawing $\phi$ of instance $I_F$, in which the number of crossings is bounded by $\cro(\phi_1)+\cro(\phi_2)+|E^{\del}|\cdot |E(G_F)|$.
%--------------------------
%--------------------------
%--------------------------
%--------------------------
%--------------------------
\subsection{Proof of \Cref{claim: find potential augmentors}}
\label{subsec: proof of finding potential augmentors}

Consider the contracted instance $\hat I_F=(\hat G_F,\hat \Sigma_F)$. Since this instance is wide,  there is a vertex $v\in V(\hat G_F)$, a partition $(E_1,E_2)$ of the edges of $\delta_{\hat G_F}(v)$, such that the edges of $E_1$ appear consequently in the rotation $\oset_v\in \hat \Sigma_F$, and so do the edges of $E_2$. Additionally, there is a collection $\pset$  of at least $\floor{m/\mu^{\interestconst}}$ simple edge-disjoint cycles in $\hat G_F$, such that every cycle $P\in \pset$ contains one edge of $E_1$ and one edge of $E_2$.

Note that we can compute the vertex $v$, the partition $(E_1,E_2)$ of the edges of $\delta_{\hat G_F}(v)$, and the set $\pset$ of cycles with the above properties efficiently. We partition the cycles of $\pset$ into three subsets: set $\pset^0$ contains all cycles $P\in \pset$, such that no vertex of $O$ is a supernode. Set $\pset^1$ contains all cycles $P\in\pset$, such that exactly one vertex of $P$ is a supernode. Set $\pset^2$ contains all remaining cycles. Clearly, at least one of the three cycle sets $\pset^1,\pset^2,\pset^3$ must contain at least $\frac{|E(G_F)|}{6\mu^{\thec}}$, cycles. We now consider three cases, depending on which of the three sets contains this many cycles.

\paragraph{Case 1: $|\pset^0|\geq \frac{|E(G_F)|}{6\mu^{\thec}}$.}
In this case, every path in $\pset^0$ is also a path in graph $G_F$, and path set $\pset^0$ is a type-1 potential $F$-augmenting set for $\kset$. We return path set $\pset^0$.



\paragraph{Case 2: $|\pset^1|\geq \frac{|E(G_F)|}{6\mu^{\thec}}$.}

Assume first that vertex $v$ is a supernode, that is, for some connected component $C\in \cset(F)$, $v=v_C$. Note that $\delta_{\hat G_F}(C)\subseteq  E^F(C)$. Recall that the ordering $\oset_{v_C}\in \hat\Sigma_F$ of the edges of $\delta_{\hat G_F}(C)$ is induced by the ordering $\oset^F(C)$ of the edges in $E^F(C)$. Therefore, there is a partition $(E_1',E_2')$ of the edges of $E^F(C)$ with $E_1\subseteq E_1'$, $E_2\subseteq E_2'$, such that the edges of $E_1'$ appear consecutively in the ordering $\oset^F(C)$. We fix any such partition $(E_1',E_2')$. Every cycle in $\pset^1$ then naturally defines a path in graph $G_F$, that has an edge of $E_1'$ as its first edge, and an edge of $E_2'$ as its last edge. Since no other supernodes may lie on the paths of $\pset^1$, we obtain a valid type-2 potential $F$-augmenting set of cardinality at least 
$\frac{|E(G_F)|}{6\mu^{\thec}}$.

Assume now that $v$ is not a supernode. 
For every connected component $C\in \cset(F)$, let $\pset^1(C)\subseteq \pset^1$ be the subset of cycles containing the supernode $v_C$. 
Since $|\cset(F)|=r$, there is some component $C\in \cset(F)$ with $|\pset^1(C)|\geq \frac{|E(G_F)|}{6r\mu^{\thec}}$. We fix this connected component $C$, and we denote $\qset=\pset^1(C)$. 

Note that every cycle $Q\in \qset$ can be thought of as a concatenation of two edge-disjoint paths, both of which connect $v_C$ to $v$. We denote by $Q_1$ the path containing an edge of $E_1$, and by $Q_2$ the path containing an edge of $E_2$. We then denote $\qset_1=\set{Q_1\mid Q\in \qset}$ and $\qset_2=\set{Q_2\mid Q\in \qset}$. Let $E'_1$ denote the set of all edges of $\hat G_F$ that are incident to vertex $v_C$, and lie on the paths of $\qset_1$. We define edge set $E'_2$ for the paths of $\qset_2$ similarly. Note that the edges of $E'_1\cup E'_2$ in graph $\hat G_F$ correspond to a subset of edges of $E^F(C)$ in graph $G_F$. We say that a partition $(E_1'',E_2'')$ of the edges of $E^F(C)$ is a \emph{good partition} iff the following hold:

\begin{itemize}
	\item the edges of $E_1''$ appear consecutively in the ordering $\oset^F(C)$;
	
	\item $|E_1''\cap E_1'|\geq |E_1'|/2$; and
	
	\item $|E_2''\cap E_2'|\geq 3|E_2'|/4$.
\end{itemize}

Note that we can efficiently compute a good partition of the edges in $E^F(C)$ if such a partition exists, and we can also efficiently determine whether a good partition of the edges in $E^F(C)$ exists. 
Assume first that a good partition of the edges in $E^F(C)$ exists, and let  $(E_1'',E_2'')$ be a good partition that we have computed. Let $\qset^*\subseteq \qset$ be the set of all cycles $Q\in \qset$, such that path $Q_1$ contains an edge of $E_1''$, and path $Q_2$ contains an edge of $E_2''$. From the definition of a good partition, it is easy to verify that $|\qset^*|\geq |\qset|/4\geq \frac{|E(G_F)|}{24r\mu^{\thec}}$ must hold. We then return path set $\qset^*$, which must be  a valid type-2 potential $F$-augmenting set. If we establish that no good partition of the edges in $E^F(C)$ exists, then we report that in every solution $\phi$ to instance $I_F$ with $\cro(\phi)\leq \frac{|E(G_F)|^2}{2^{20}\cdot \mu^{2\thec}\cdot r^2}$, either some pair of edges in $\partial(F)$ cross, or the number of crossings in which edges of $\partial(F)$ participate is at least $\frac{|E(G_F)|}{64\cdot \mu^{\thec}\cdot r}$. We now prove that in this case, this indeed must indeed be true.

\begin{observation}\label{obs: no augmenting set}
	If no good partition of the edges in $E^F(C)$ exists, then in every solution $\phi$ to instance $I_F$ in every solution $\phi$ to instance $I_F$ with $\cro(\phi)\leq \frac{|E(G_F)|^2}{2^{20}\cdot \mu^{2\thec}\cdot r^2}$, either some pair of edges in $\partial(F)$ cross, or the number of crossings in which edges of $\partial(F)$ participate is at least $\frac{|E(G_F)|}{64\cdot \mu^{\thec}\cdot r}$.
\end{observation}

\begin{proof}
	Denote $|\qset|=k$, and denote the edges of $E_1$ by $e_1,\ldots,e_k$, and the edges of $E_2$ by $e_{k+1,\ldots,e_{2k}}$, so that the edges $e_1,\ldots,e_{2k}$ appear in the rotation $\oset_v\in \hat \Sigma_F$ in the order of their indices (recall that the edges in $E_1$ must appear consecutively in $\oset_v$). 
	
	Assume for contradiction that there exists a drawing $\phi$ of $I_F$ with $\cro(\phi)\leq \frac{|E(G_F)|^2}{2^{20}\cdot \mu^{2\thec}\cdot r^2}$, such that no pair of edges of $\partial(F)$ cross, and the edges of $\partial(F)$ participate in fewer than $\frac{|E(G_F)|}{64r\mu^{\thec}}$  crossings. 
	
	We say that a path $Q_1\in \qset_1$ is \emph{good} iff the edges of $Q_1$ participate in fewer than $k/32$ crossings in $\phi$. Let $\qset'_1\subseteq \qset_1$ be the set containing all good paths. Observe that, $|\qset'_1|\geq 7k/8$ must hold. Indeed, otherwise, since the paths in $\qset_1$ are edge-disjoint we get that:
	
	
	\[\cro(\phi')\geq |\qset_1\setminus\qset'_1|\cdot \frac k {32}\geq \frac{k}{8}\cdot \frac{k}{256}>\frac{|E(G_F)|^2}{2^{20}\cdot \mu^{2\thec}\cdot r^2},  \]
	
	since $k\geq \frac{|E(G_F)|}{6r\mu^{\thec}}$.
	We conclude that $|\qset'_1|\geq 7k/8$. Let $\qset''_1\subseteq \qset'_1$ be the set of all good paths $Q_1\in \qset'_1$, such that no crossing $(e,e')_p$ in $\phi$ exists with $e\in E(Q_1)$ and $e'\in E(K)$. Since we have assumed that the edges of $\partial(F)$ participate in at most $\frac{|E(G_F)|}{64r\mu^{\thec}}$ crossings in $\phi$, $|\qset''_1|\geq 3k/4$.
	
	Let $1\leq i\leq k$ be the smallest index such that the path $Q_1\in \qset''_1$ contains the edge $e_i\in E_1$, and let $1\leq j\leq k$ be the largest index such that the path $Q_1'\in \qset''_1$ contains the edge $e_j\in E_1$. 
	Since $|\qset''_1|\geq 3k/4$, $j-i\geq 3k/4-1$ must hold.
	Since paths $Q_1,Q_1'$ are good, there are at most $k/16$ paths $Q_1''\in \qset''_1$, such that there is a crossing in $\phi$ between an edge of $E(Q_1'')$ and an edge of $E(Q_1)\cup E(Q_1')$. Let $\tilde \qset_1\subseteq \qset_1''\setminus\set{Q_1,Q_1'}$ be the set of all paths $Q_1''$, such that there is no crossing in $\phi$  between an edge of $E(Q_1'')$ and an edge of $E(Q_1)\cup E(Q_1')$. From the above discussion, $|\tilde \qset_1|\geq k/2$.
	
	Let $\tilde \qset_2\subseteq \qset_2$ be the set of all paths $Q_2\in \qset_2$, such that  there is no crossing in $\phi$  between an edge of $E(Q_2)$ and an edge of $E(Q_1)\cup E(Q_1')\cup E(C)$. Using the same reasoning as above, $|\tilde \qset_2|\geq |\qset_2|-k/16-\frac{|E(G_F)|}{64r\mu^{\thec}}\geq  3k/4$.
	
	Let $\psi$ be a drawing that is obtained from $\phi$ by deleting the images of all vertices and edges from it, except for the vertices and edges of $Q_1\cup Q_1'\cup C$. 
	Since we have assumed that the edges of $\partial(F)$ cannot cross each other in $\phi$, and since the edges of $Q_1\cup Q_1'$ may not cross the edges of $C$, the only possible crossings in $\psi$ are between edges of $E(Q_1)\cup E(Q_1')$.
	Note that vertex $v$ lies on the boundary of exactly two faces of  drawing $\psi$, that we denote by $F_1$ and $F_2$, respectively. For every edge $e_{\ell}\in E_1$ with $i<\ell<j$, the segment of $\phi(e)$ that is contained in the tiny $v$-disc $D_{\phi}(v)$ must then lie in $F_1$, and for every edge $e\in E_2$, the segment of $\phi(e)$ that is contained in the tiny $v$-disc $D_{\phi}(v)$ must then lie in $F_2$ (up to switching the names of the two faces). \mynote{would be good to add a figure here.}
	Therefore, for every path $\tilde Q_1\in \tilde \qset_1$, the image of the first edge of $\tilde Q_1$ in $\phi$ must intersect $F_1$, and for every path $\tilde Q_2\in \tilde \qset_2$, the image of the first edge of $\tilde Q_2$ in $\phi$ must intersect $F_2$. Since the edges that belong to the paths in $\tilde \qset_1\cup \tilde \qset_2$ may not cross edges of $E(Q_1)\cup E(Q'_1)\cup E(C)$ in drawing $\phi$, we get that, for every path $\tilde Q_1\in \tilde \qset_1$, the image of $\tilde Q_1$ in $\phi$ must be contained in $F_1$, and for every path $\tilde Q_2\in \tilde \qset_2$, the image of $\tilde Q_2$ in $\phi$ must be contained in $F_2$.
	Let $\tilde E_1$ be the set of all edges of $E^F(C)$ that lie on the paths in $\tilde \qset_1$, and let $\tilde E_2$ be defined similarly for $\tilde \qset_2$. Since the drawing of $C$ induced by $\phi$ is planar, there must be a partition $(E_1'',E_2'')$ of the edges of $E^F(C)$, such that the edges of $E''_1$ appear consecutively in the ordering $\oset^F(C)$; $\tilde E_1\subseteq E''_1$, and $\tilde E_2\subseteq E_2''$. Since $|E''_1|\geq |\tilde E_1|\geq k/2$, while $|E''_2|\geq |\tilde E_2|\geq 3k/4$, we get that $(E_1'',E_2'')$ is a good partition of $E^F(C)$.
\end{proof}

\paragraph{Case 3: $|\pset^2|\geq \frac{|E(G_F)|}{6\mu^{\thec}}$.}

Consider some cycle $P\in \pset^2$, and recall that at least two vertices of $P$ are supernodes. We can then mark all supernode vertices on cycle $P$, and use them to partition $P$ into a collection $\rset(P)$ of  edge-disjoint paths, such that, for every path $R\in \rset(P)$, the endpoints of $R$ are two distinct supernodes, and none of the inner vertices of $R$ is a supernode. Note that $|\rset(P)|\geq 2$ must hold. Let $\rset=\bigcup_{P\in \pset^2}\rset(P)$, so $|\rset|\geq 2|\pset_2|$. Then there must be two distinct connected component $C,C'\in \cset(F)$, and a subset $\rset(C)\subseteq \rset$ of at least $\frac{|\rset|}{r^2|}\geq \frac{|E(G_F)|}{6r^2\cdot \mu^{\thec}}$ paths, such that every path $R\in \rset(C)$ originates at vertex $v_C$, terminates at vertex $v_{C'}$, and contains no supernodes as inner vertices. Since the paths in $\rset(C)$ do not contain supernodes as inner vertices, they naturally define a collection $\rset'$ of edge-disjoint paths in graph $G_F$, where every path $R\in \rset'$ connects a vertex of $C$ to a vertex of $C'$ and does not contain vertices of $\partial(F)$ as inner vertices. Therefore, $\rset'$ is a type-3 potential $F$-augmenting path set, whose cardinality is at least $\frac{|E(G_F)|}{6r^2\cdot \mu^{\thec}}$, as required. 



==> apd_prelim-backup.tex <==
\section{Proofs Omitted from Section~\ref{sec:long prelim}}
\label{sec: apd_prelim}





%\section{Proofs Omitted from \Cref{sec:long prelim}}

\subsection{Proof of \Cref{lem: find reordering}}
\label{subsec: compute reordering}

Suppose we are given a graph $G$, and, for every vertex $v\in V(G)$, an oriented circular ordering $(\oset_v,b_v)$ of edges in $\delta_G(v)$. 
We say that a drawing $\phi$ of $G$ \emph{respects the oriented orderings of the vertices of $G$} iff for every vertex $v\in V(G)$, the oriented circular order in which the images of the edges of $\delta_G(v)$ enter $v$ is $(\oset_v,b_v)$. 
We use the following theorem from~\cite{pelsmajer2011crossing}.
\begin{theorem}[Corollary 5.6 of~\cite{pelsmajer2011crossing}]
	\label{thm: compute_reordering_curves}
	There is an efficient algorithm, that, given a two-vertex loopless multigraph $G$ (so $V(G)=\set{v,v'}$ and $E(G)$ only contains parallel edges connecting $v$ to $v'$), and, for each vertex $v\in V(G)$, an oriented ordering  $(\oset_v,b_v)$ of its incident edges, computes a drawing $\phi$ of $G$ that respects the given oriented orderings, such that $\cro(\phi)$ is at most twice the minimum number of crossings of any drawing of $G$ that respects the oriented orderings.
\end{theorem}

The proof of Lemma~\ref{lem: find reordering} easily follows \Cref{thm: compute_reordering_curves}. Recall that we are given a pair $(\oset,b)$, $(\oset',b')$ of oriented orderings of a collection $U$ of elements. We construct a two-vertex loopless graph $G$ with oriented ordering on its vertices, as follows. Denote $U=\set{u_1,\ldots,u_r}$.
The vertex set of $G$ is $\set{v,v'}$. The edge set of $G$ consists of $r$ parallel edges connecting $v$ to $v'$, that we denote by $e_{u_1}, e_{u_2},\ldots e_{u_r}$, respectively. 
The oriented ordering $(\oset,b)$ of the elements of $U$ naturally defines an oriented ordering $(\hat \oset,b)$ of the edges of $G$, and similarly, the oriented ordering $(\oset,b')$ of the elements of $U$ defiens an oriented ordering $(\hat \oset,b')$ of the edges of $G$. 
We define the oriented orderings for the vertices of $G$ as follows: $(\oset_v,b_v)=(\hat \oset,b)$ and $(\oset_{v'},b_{v'})=(\hat \oset',- b')$. 


Consider any drawing $\phi$ of $G$ on the sphere that respects the oriented orderings for $v,v'$ defined above. Let $D'=D_{\phi}(v')$ be a tiny $v'$-disc. For all $1\leq i\leq r$, we denote the unique point on the image of edge $e_{u_i}$ that lies on the boundary of $D'$ by by $p'_i$. 
Similarly, we let $\hat D=D_{\phi}(v)$ be a tiny $v$-disc, and, for  all $1\leq i\leq r$, we denote the unique point on the image of edge $e_{u_i}$ that lies on the boundary of $\hat D$ by $p_i$. Let $D$ be the disc whose boundary is the same as the boundary of $\hat D$, but whose interior is disjoint from that of $\hat D$. Then $D'\subseteq D$, and the boundaries of the two discs are disjoint. Furthermore, points $p_1,\ldots,p_r$ appear on the boundary of $D$ according to the oriented ordering $(\oset,b)$, and points $p'_1,\ldots,p'_r$ appear on the boundary of $D'$ according to the oriented ordering $(\oset',b')$.
For all $1\leq i\leq r$, let $\gamma_i$ be the segment of the image of the edge $e_{u_i}$ between points $p_i$ and $p'_i$. Then $\set{\gamma_i\mid 1\leq i\leq r}$ is a set of reordering curves for the orderings $(\oset,b)$ and $(\oset',b')$, and moreover, the cost of this curve set is exactly the number of crossings in $\phi$. 


Using a similar reasoning, any set $\Gamma$ of reordering curves for the orderings $(\oset,b)$ and $(\oset',b')$ can be converted into a drawing of graph $G$ that respects the oriented orderings at vertices $v$ and $v'$, in which the number of crossings is exactly the cost of $\Gamma$. Therefore, there is a drawing of $G$ that respects the oriented orderings at $v$ and $v'$, whose number of crossings is bounded by $\dist((\oset,b),(\oset',b'))$.  We Apply the algorithm from Theorem~\ref{thm: compute_reordering_curves} to graph $G$, and then compute a set of reordering curves from the resulting drawing of $G$ as described above. From the above discussion, the cost of the resulting set of curves is at most $2\cdot \dist((\oset,b),(\oset',b'))$.


%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------



\subsection{Proof of \Cref{lem: ordering modification}}

\label{apd: Proof of find reordering}

The proof easily follows from \Cref{lem: find reordering}.
We denote $\delta_G(v)=\set{e_1,\ldots,e_r}$, and, for all $1\leq i\leq r$, we let $p_i$ be the unique point of $\phi(e_i)$ lying on the boundary of the disc $D$. Let $\sigma_i$ be the segment of $\phi(e_i)$ that is disjoint from the interior of the disc $D$. In other words, if $e_i=(v,u_i)$, then $\sigma_i$ is a curve connecting $\phi(u_i)$ to $p_i$. 
Note that the points $p_1,\ldots,p_r$ appear on the boundary of $D$ according to the circular ordering $\oset'_v$ of their corresponding edges.
We assume w.l.o.g. that the orientation of the ordering is $b_v'=-1$.

Let $D'$ be another disc, that is contained in $D$, with $\phi(v)$ lying in the interior of $D'$, such that the boundaries of $D$ and $D'$ are disjoint. 
We place points $p_1',\ldots,p'_r$ on the boundary of the disc $D'$, so that all resulting points are distinct, and they appear on the boundary of $D'$ in the order $\oset_v$ of their corresponding edges, using a positive orientation of the ordering. For all $1\leq i\leq r$, we can compute a simple curve $\gamma_i$, connecting $\phi(v)$ to $p'_i$, such that $\gamma_i$ is contained in $D'$ and only intersects the boundary of $D'$ at its endpoint $p'_i$. We also ensure that all resulting curves $\gamma_1,\ldots,\gamma_r$ are mutually internally disjoint. Using the algorithm from \Cref{lem: find reordering}, we compute a collection $\Gamma=\set{\gamma_1',\ldots,\gamma'_r}$ of {reordering curves}, where for $1\leq i\leq r$, curve $\gamma'_i$ connects $p_i$ to $p'_i$, is contained in $D$, and is disjoint from the interior of $D'$. Note that the total number of crossings between the curves in $\Gamma$ is at most $2\dist{((\oset_v,1),(\oset'_v,-1))}$. For all $1\leq i\leq r$, we define a new image of the edge $e_i$ to be the concatenation of the curves $\sigma_i,\gamma'_i$, and $\gamma_i$. The images of all remaining edges and vertices of $G$ remain unchanged. Denote the resulting drawing of the graph $G$ by $\phi'$. It is immediate to verify that the edges of $\delta_G(v)$ enter the image of $v$ in the order $\oset_v$ in $\phi'$, and that the drawings of $\phi$ and $\phi'$ are identical except for the segments of the images of the edges in $\delta_G(v)$ that lie inside the disc $D$. It is also immediate to verify that $\cro(\phi')\leq \cro(\phi)+
2\dist{((\oset_v,1),(\oset'_v,-1))}$.

We  repeat the same algorithm again, only this time the points $p_1',\ldots,p'_r$  are placed on the boundary of disc $D'$ in the order $\oset_v$ of their corresponding edges, using a negative orientation of the ordering. The remainder of the algorithm remains unchanged, and produces a drawing $\phi''$ of $G$. As before, the edges of $\delta_G(v)$ enter the image of $v$ in the order $\oset_v$ in $\phi''$, and that the drawings of $\phi$ and $\phi''$ are identical except for the segments of the images of the edges in $\delta_G(v)$ that lie inside the disc $D$. Moreover, $\cro(\phi'')\leq \cro(\phi)+
2\dist{((\oset_v,-1),(\oset'_v,-1))}$. Let $\phi^*$ be the drawing with smaller number of crossings, among $\phi'$ and $\phi''$. Our algorithm returns the drawing $\phi^*$ as its final outcome. From the above discussion, $\cro(\phi^*)\leq \cro(\phi)+
2\dist{(\oset_v,\oset'_v)}$.




%----------------------------
%old stuff until %-------------
%----------------------------
\iffalse
Assume without loss of generality that the curves of $\Gamma$ enter $z$ in the oriented ordering $(\oset,0)$. We first apply the algorithm from \Cref{lem: find reordering} to compute (i) a $2$-approximation $a_0$ of $\dist((\oset,0),(\oset',0))$, and (ii) a $2$-approximation $a_1$ of $\dist((\oset,0),(\oset',1))$.
Assume without loss of generality that $a_0\le a_1$, so $a_0\le 2\cdot \dist(\oset,\oset')$.

For each $u\in U$, we denote by $p_u$ the intersection between the curve $\gamma_u$ and the boundary of $D$.
We erase the segments of curves of $\Gamma$ inside the disc $D$. We then place another disc $D'$ around $z$ inside the disc $D$, and let $\set{p'_u}_{u\in U}$ be a set of points appearing on the boundary of disc $D'$ in the order $(\oset',0)$. We use \Cref{lem: find reordering} to compute a set $\tilde\Gamma=\set{\tilde\gamma_u\mid u\in U}$ of reordering curves, where for each $u\in U$, the curve $\tilde\gamma_u$ connects $p_u$ to $p'_u$.
We then define, for each $u\in U$, the curve $\gamma'_u$ as the union of (i) the subcurve of $\gamma_u$ outside the disc $D$ (connecting its endpoint outside $D$ to $p_u$); (ii) the curve $\tilde\gamma_u$ (connecting $p_u$ to $p'_u$); and (iii) the straight line-segment connecting $p'_u$ to $z$. It is clear that (i) the curves $\set{\gamma'_u\mid u\in U}$ enter $z$ in the order $(\oset',0)$; (ii) for each $u\in U$, the curve $\gamma_u$ differs from the curve $\gamma'_u$ only within some tiny disc $D$ that contains $z$; and (iii) the number of crossings between curves of $\Gamma'$ within disc $D$ is at most $2\cdot \dist(\oset,\oset')$.
\fi





\iffalse{some other proof}
\begin{proof}
	This is a sketch, needs to be formalized. Let's look at the optimal set $\Gamma^*$ of reordering curves, and let $\gamma'_i$ be the curve participating in fewest crossings. Let's say this number of crossings is $N$. Then the cost of $\Gamma$ is at least $Nr/2$. The main claim is that there exists a collection $\Gamma'$ of reordering curves, of cost at most $2\cost(\Gamma^*)$, in which $\gamma_i$ does not participate in crossings. Assume first that the claim is correct. Finding such a drawing is straightforward. We rotate the discs so that $p'_i,p_i$ appear aligned, and connect them with a straight line, that becomes the drawing of $\Gamma_i$. Cutting $D\setminus D'$ along this line, we obtain a rectangle, whose vertical sides are the cut line, top horizontal line is boundary of $D$, and bottom horizontal line is boundary of $D'$. In this rectangle we just connect $p_j,p_j'$ with a straight line, adjusting the drawings as needed so no three curves meet at the same point. It is easy to see that resulting curves $\gamma_j,\gamma_k$ will only cross if the left-to-right ordering of $p_j,p_k$ is opposite from that of $p'_j,p'_k$. In any drawing where no curve crosses $\gamma_i$ any such pair of curves will cross as well. So we obtain a drawing of cost at most $\cost(\Gamma')\leq 2\cost(\Gamma^*)$.
	
	Next, we show that there exists a collection $\Gamma'$ of curves of cost at most $2\cost(\Gamma^*)$ in which no curve crosses $\gamma_i$. In fact we compute $\Gamma'$ exactly as shown above. We just need to argue that the cost of this set of curves is at most $\Gamma^*$. In order to do so, we partition $\Gamma^*\setminus\set{\gamma_i}$ into two subsets: set $\Gamma_1$ containing all curves that don't cross $\gamma_i$, and set $\Gamma_2$ containing remaining curves. Consider now any pair $\gamma_j,\gamma_k$ of curves in $\Gamma'$, and assume that they cross (the drawing that we compute ensures that every pair of curves crosses at most once). in the new drawing. As observed above, this can only happen if the left-to-right ordering of $p_j,p_k$ on the top edge of the rectangle is opposite from that of $p'_j,p'_k$ on the bottom edge.
	
	We now consider three cases. First, if the original curves routing elements $u_i,u_j$ lied in $\Gamma_1$, then the two corresponding curves had to cross in $\Gamma^*$ as well. Second, if the two original curves lied in $\Gamma_2$, then, as we will show later, they also had to cross before. So the case that remains is when one of the curves is in $\Gamma_1$ and another is in $\Gamma_2$. But because $|\Gamma_2|\leq N$, we will have at most $Nr$ such new crossings. Because $\cost(\Gamma^*)\geq Nr/2$, we get that $\cost(\Gamma')\leq \cost(\Gamma^*)+Nr\leq 5\cost(\Gamma')$. It now remains to prove the following claim.
	
	\begin{claim}
		Consider two elements $u_j,u_k$, such that the left-to-right ordering of $p_j,p_k$ on the top edge of the rectangle is opposite from the left-to-right ordering of $p'_j,p'_k$ on the bottom edge. Let $\gamma'_j,\gamma'_k$ be the two curves of $\Gamma^*$ corresponding to these elements, and assume that $\gamma'_i,\gamma'_k\in \Gamma_2$ (so both curves cross $\gamma_i$). Then $\gamma'_j,\gamma'_k$ must cross. 
	\end{claim}
	
	\begin{proof}
		Assume that $p_j$ appears to the left of $p_k$ on the top edge of the rectangle.
		Consider the annulus $A=D\setminus D'$, and the drawings of $\gamma_i,\gamma'_j$ in it. We can assume that the two curves cross at most once. Consider a face $F$ of the resulting drawing whose boundary contains $p_k$. The three boundary edges of this face are: the segment of the top boundary of the rectangle from $p_j$ to $p_i$; segment of $\gamma'_i$ from $p_i$ to its meeting point $q$ with $\gamma'_j$; and segment of $\gamma'_j$ from $p_j$ to $q$. In particular, $p'_k$ does not lie on the boundary of $F$.
		Assume for contradiction that $\gamma'_j,\gamma'_k$ do not cross. Then curve $\gamma'_k$ has to cross the boundary of $F$, which can only done by crossing the segment $\sigma$ of the boundary that lies on $\gamma'_i$. Denote this crossing point by $q'$. This is the only crossing between $\gamma'_k$ and $\gamma'_i$. If we denote by $F'$ the unique face that shares the boundary segment $\sigma$ with $F$, then that face does not contain $p'_k$ on its boundary (a figure is needed). Therefore, to reach $p'_k$, curve $\gamma'_k$ either needs to cross $\gamma'_j$, or to cross $\gamma'_i$ once again.
	\end{proof}
\end{proof}
\fi


\iffalse
\mynote{previous proof, should keep only one}


We now prove \Cref{lem: ordering modification} using \Cref{lem: find reordering}.
Assume without loss of generality that the curves of $\Gamma$ enter $z$ in the oriented ordering $(\oset,0)$. We first apply the algorithm from \Cref{lem: find reordering} to compute (i) a $2$-approximation $a_0$ of $\dist((\oset,0),(\oset',0))$, and (ii) a $2$-approximation $a_1$ of $\dist((\oset,0),(\oset',1))$.
Assume without loss of generality that $a_0\le a_1$, so $a_0\le 2\cdot \dist(\oset,\oset')$.

For each $u\in U$, we denote by $p_u$ the intersection between the curve $\gamma_u$ and the boundary of $D$.
We erase the segments of curves of $\Gamma$ inside the disc $D$. We then place another disc $D'$ around $z$ inside the disc $D$, and let $\set{p'_u}_{u\in U}$ be a set of points appearing on the boundary of disc $D'$ in the order $(\oset',0)$. We use \Cref{lem: find reordering} to compute a set $\tilde\Gamma=\set{\tilde\gamma_u\mid u\in U}$ of reordering curves, where for each $u\in U$, the curve $\tilde\gamma_u$ connects $p_u$ to $p'_u$.
We then define, for each $u\in U$, the curve $\gamma'_u$ as the union of (i) the subcurve of $\gamma_u$ outside the disc $D$ (connecting its endpoint outside $D$ to $p_u$); (ii) the curve $\tilde\gamma_u$ (connecting $p_u$ to $p'_u$); and (iii) the straight line-segment connecting $p'_u$ to $z$. It is clear that (i) the curves $\set{\gamma'_u\mid u\in U}$ enter $z$ in the order $(\oset',0)$; (ii) for each $u\in U$, the curve $\gamma_u$ differs from the curve $\gamma'_u$ only within some tiny disc $D$ that contains $z$; and (iii) the number of crossings between curves of $\Gamma'$ within disc $D$ is at most $2\cdot \dist(\oset,\oset')$.
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------
%----------------------------
%----------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm: type-1 uncrossing}}
\label{apd: type-1 uncrossing}

%\mynote{please replace intersections between curves with crossings. subcurve should be subcurve. Note that the proof needs to assume that each curve is simple. This needs to be fixed. A single disc should be denoted by $D$, $\dset$ is for a set of discs.}

Let $Z$ be the set of crossings points between the curves of $\Gamma$. For each such crossing point $z\in Z$, we consider a tiny disc $D_z$, that contains the point $z$ in its interior. We select the discs $D_z$ to ensure that all such discs are disjoint, and, moreover, if $z$ is a crossing point between curves $\gamma_1,\gamma_2$, then for every curve $\gamma\in \Gamma\setminus\set{\gamma_1,\gamma_2}$, $\gamma\cap D_z=\emptyset$, while for every curve $\gamma\in \set{\gamma_1\cup \gamma_2}$,  $\gamma\cap D_z$ is a simple open curve whose endpoints lie on the boundary of $D_z$.

We start with $\Gamma_1'=\Gamma_1$, and then iteratively modify the curves in $\Gamma_1'$, as long as there is a pair of distinct curves $\gamma_1,\gamma_2\in \Gamma$ that cross more than once. 
Each iteration is executed as follows. Let $\gamma_1,\gamma_2\in \Gamma_1'$ be a pair of curves that cross more than once, and let  $z,z'$ be two crossing points between $\gamma_1,\gamma_2$, that appear consecutively on $\gamma_1$. In other words, no other point that appears between $z$ and $z'$ on $\gamma_1$ may belong to $\gamma_2$.
We denote by $s_1,t_1$ the endpoints of $\gamma_1$, such that $z$ appears closer to $s_1$ than $z'$ on $\gamma_1$.
Similarly, we denote by $s_2,t_2$ the endpoints of  $\gamma_2$, such that $z$ appears closer to $s_2$ than $z'$ on $\gamma_2$.
%\mynote{this should be rephrased, the sentence is not clear}.We define the endpoints $s_{b}, t_{b}$ similarly \mynote{better to spell this out, that $s_b$ is closer to $z$; similarly may mean the opposite}.
We denote by $x_1,x_2$ the two points of $\gamma_1$ that lie on the boundary of disc $D_z$, and denote by $x_3,x_4$ the two points of $\gamma_1$ lying on the boundary of disc $D_{z'}$,
such that the points $x_1,z,x_2,x_3,z',x_4$ appear on $\gamma_1$ in this order.
We define points $y_1,y_2,y_3,y_4$ on $\gamma_2$ similarly (see \Cref{fig:non_crossing_representation1}).

\begin{figure}[h]
	\centering
	\subfigure[Before: Curve $\gamma_1$ is shown in blue and curve $\gamma_2$ is shown in red. The disc on the left is $D_z$, and the disc on the right is $D_{z'}$.]{\scalebox{0.45}{\includegraphics{figs/type_1_uncross_proof_1.jpg}} \label{fig:non_crossing_representation1}
	}
	\hspace{0cm}
	\subfigure[After: Curve $\gamma'_1$ is shown in blue and curve $\gamma'_2$ is shown in red.]{
		\scalebox{0.45}{\includegraphics{figs/type_1_uncross_proof_2.jpg}}\label{fig:non_crossing_representation2}}
	\caption{An illustration of an iteration of type-1 uncrossing.}\label{fig: type_1_uncross_proof}
\end{figure}

In order to execute the iteration, we slightly modify the curves $\gamma_1, \gamma_2$, by ``swapping'' their segments between points $x_2,x_3$ and $y_2,y_3$, respectively, and slightly ``nudging'' them inside the discs $D_z,D_{z'}$, as show in \Cref{fig: type_1_uncross_proof}. We now describe the construction of the new curves $\gamma_1',\gamma_2'$ more formally.
Note that the points $x_1,x_2,y_1,y_2$ appear on the boundary of $D_z$ clockwise in either the order  $(x_1,y_1,x_2,y_2)$ or the order $(x_1,y_2,x_2,y_1)$.
%\mynote{is this correct? I think there should be at least 2 possible orders (one order if you allow any orientation, but you seem to select a fixed orientation)} 
Therefore, we can find two disjoint simple curves $\eta_1$ and $\eta_2$ that are contained in disc $D_z$, with $\eta_1$ connecting $x_1$ to $y_2$, and $\eta_2$ connecting $y_1$ to $x_2$.
Similarly, we compute two disjoint simple curves curves $\eta'_1,\eta'_2$, that are contained in disc $D_{z'}$, with $\eta_1'$ connecting $y_3$ to $x_4$, and $\eta_2'$ connecting $x_3$ to $y_4$ (see \Cref{fig:non_crossing_representation2}). 

We let $\gamma_1'$ be a curve, that is constructed by concatenating the following five curves: (1) the segment of $\gamma_1$ from $s_1$ to $x_1$; (2) curve $\eta_1$; (3) the segment of $\gamma_2$ from $y_2$ to $y_3$; (4) curve $\eta'_1$; and (5) the segment of $\gamma_1$ from $x_4$ to $t_1$.  Similarly, let $\gamma_2'$ be a  curve, that is constructed by concatenating the following five curves: (1) the segment of $\gamma_2$ from $s_2$ to $y_1$; (2) curve $\eta_2$; (3) the segment of $\gamma_1$ from $x_2$ to $x_3$; (4) curve $\eta'_2$; and (5) the segment of $\gamma_2$ from $y_4$ to $t_2$. We then remove any self loops from the two curves, to obtain the final curves $\gamma'_1,\gamma_2'$, that replace the curves $\gamma_1,\gamma_2$ in $\Gamma_1'$. Note that $\gamma'_1$ has the same endpoints as $\gamma_1$, and the same is true for $\gamma'_2$ and $\gamma_2$. It is also easy to verify that, at the end of the iteration, the number of crossings between the curves of $\Gamma_1'\cup \Gamma_2$ strictly decreases, and the number of crossings between the curves of $\Gamma_1'$ and the curves of $\Gamma_2$, that we denoted by $\chi(\Gamma_1',\Gamma_2)$, does not grow. Moreover, for every curve $\gamma\in \Gamma_2$, the number of crossings of $\gamma$ with the curves in $\Gamma_1'$ may not grow either. Once the algorithm terminates, we obtain the desired set $\Gamma_1'$ of curves, in which every pair of distinct curves crosses at most once. From the above discussion, it is immediate to verify that the curves in $\Gamma_1$ have all required properties. Since the curves in $\Gamma$ are in general position, the number of iterations is bounded by the number of crossing points between the curves.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of \Cref{claim: curves in a disc}}
\label{apd: Proof of curves in a disc}

We start by constructing a collection $\Gamma'=\set{\gamma'_i\mid 1\leq i\leq k}$ of curves that are in general position, such that for all $1\leq i\leq k$, curve $\gamma'_i$ has $s_i$ and $t_i$ as its endpoints, and is contained in disc $D$. In order to construct the set $\Gamma'$ of curves, we let $p$ be any point in the interior of the disc $D$, and $r>0$ be some value, such that a circle of radius $r$ that is centered at point $p$ is contained in the disc $D$. For all $1\leq i\leq k$, let $\ell_i$ be a straight line, connecting point $s_i$ to $p$, and $\ell'_i$ a straight line, connecting point $t_i$ to $p$. We can assume that both lines are contained in the disc $D$, by stretching the disc as needed. For all $1\leq i\leq k$, we choose a radius $0<r_i<r$, so that $0<r_1<\cdots<r_k<r$ holds. For an index $1\leq i\leq k$, we let $C_i$ be the boundary of a circle of radius $r_i$ that is centered at point $p$, and we let $q_i,q'_i$ be the points on lines $\ell_i$ and $\ell'_i$, respectively, that lie on $C_i$. We let curve $\gamma'_i$ be a concatenation of three curves: the segment of $\ell_i$ from $s_i$ to $q_i$; a segment of $C_i$ between $q_i$ and $q'_i$; and the segment of $\ell'_i$ from $q'_i$ to $t_i$. Consider the resulting set 
 $\Gamma'=\set{\gamma'_i\mid 1\leq i\leq k}$ of curves. Clearly, for all $1\leq i\leq k$, curve $\gamma'_i$ has $s_i$ and $t_i$ as its endpoints, and is contained in disc $D$. 
 It is also easy to verify that curves of $\Gamma'$ are in general position. 
 
Next, we use the algorithm from \Cref{thm: type-1 uncrossing} to perform a type-1 uncrossing of the curves in $\Gamma'$. Specifically, we set $\Gamma_1=\Gamma'$ and $\Gamma_2=\emptyset$. We denote by $\Gamma=\Gamma_1'=\set{\gamma_i\mid 1\leq i\leq k}$ the set of curves that the algorithm outputs. Recall that, for all $1\leq i\leq k$, curve $\gamma_i$ has $s_i$ and $t_i$ as its endpoints; the curves in $\Gamma$ are in general position; and every pair of curves in $\Gamma$ cross at most once. From the description of the type-1 uncrossing operation it is easy to verify that all curves in $\Gamma$ are contained in the disc $D$.  

Consider now two pairs $(s_i,t_i),(s_j,t_j)$ of points, with $i\neq j$. Note that curve $\gamma_i$ partitions the disc $D$ into two regions, that we denote by $F$ and $F'$. If the two pairs $(s_i,t_i),(s_j,t_j)$ cross, then $s_j,t_j$ may not lie on the boundary of the same region, and so curve $\gamma_j$ must cross curve $\gamma_i$ exactly once. If the two pairs do not cross, then $s_j,t_j$ either both lie on the boundary of $F$, or they both lie on the boundary of $F'$. It is then impossible that curves $\gamma_i,\gamma_j$ cross exactly once, and, since every pair of curves crosses at most once, they cannot cross.
 
\iffalse 
 
We first set, for each $1\le i\le k$, a curve $\gamma'_i$ to be the straight line segment connecting $s_i$ to $t_i$. It is easy to see that every pair of curves in $\Gamma'=\set{\gamma'_i\mid 1\le i\le k}$ cross at most once, and a pair $\gamma'_i,\gamma'_j$ of curves cross iff the two pairs $(s_i,t_i), (s_j,t_j)$ of points cross.
If the curves of $\Gamma'$ are in general position (namely no point belongs to at least three curves of $\Gamma'$), then we set, for each $1\le i \le k$, $\gamma_i=\gamma'_i$, and return the collection $\Gamma=\set{\gamma_i\mid 1\le i\le k}$ of curves. It is easy to verify that $\Gamma$ satisfies the required property.
If the curves $\Gamma'$ are not in general position, then we let, for each $1\le i\le k$, a curve $\gamma_i$ be obtained by slightly perturbing the curve $\gamma'_i$. See \Cref{fig: perturb} for an illustration. We then return the collection $\Gamma=\set{\gamma_i\mid 1\le i\le k}$ of curves. It is easy to verify that $\Gamma$ satisfies the required property.

\begin{figure}[h]
	\centering
	\subfigure[Before: Curves $\gamma'_1,\gamma'_2,\gamma'_3$ contain the same point.]{\scalebox{1.1}{\includegraphics[scale=0.4]{figs/perturb_before.jpg}}}
	\hspace{0.7cm}
	\subfigure[After: Curves $\gamma_1,\gamma_2,\gamma_3$ are in general position.]{\scalebox{1.1}{\includegraphics[scale=0.4]{figs/perturb_after.jpg}}}
	\caption{An illustration of slight perturbation of curves in the proof of \Cref{claim: curves in a disc}.\label{fig: perturb}}
\end{figure}
\fi







%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of Theorem~\ref{thm: new type 2 uncrossing}}
\label{apd: new type 2 uncrossing}

We start with an initial set $\Gamma'=\set{\gamma'(Q)\mid Q\in \qset}$ of curves, where, for each path $Q\in \qset$, $\gamma'(Q)$ is the image of the path $Q$ in $\phi$. In other words, $\gamma'(Q)$ is a concatenation of the images of the edges of $Q$ in $\phi$. Note however that the resulting set $\Gamma'$ of curves is not in general position. This is since a vertex $v\in V(G)$ may serve as an inner vertex on more than two paths of $\qset$, and in such a case its image $\phi(v)$ serves as an inner point on more than two curves in $\Gamma'$.
Let $V'\subseteq V(G)$ be the set of all vertices $v\in V(G)$, such that more than two paths in $\qset$ contain $v$.

In our first step, we transform the set $\Gamma'$ of curves so that the resulting curves are in general position, while ensuring that the endpoints of each curve $\gamma'(Q)$ remain unchanged, and each such curve $\gamma'(Q)$ remains aligned with the graph $\bigcup_{Q'\in \qset}Q'$. We do so by performing \emph{nudging operation} around every vertex $v\in V_1$, as follows.

Consider any vertex $v\in V_1$, and let $\qset^v\subseteq \qset$ be the set of all paths containing vertex $v$. Note that $v$ must be an inner vertex on each such path. For convenience, we denote $\qset^v=\set{Q_1,\ldots,Q_z}$. Consider the tiny $v$-disc $D=D_{\phi}(v)$. For all $1\leq i\leq z$, denote by $a_i$ and $b_i$ the two points on curve $\gamma(Q_i)$ that lie on the boundary of disc $D$. Use the algorithm from \Cref{claim: curves in a disc} to compute a collection $\set{\sigma_1,\ldots,\sigma_z}$ of curves, such that, for all $1\leq i\leq z$, curve $\sigma_i$ connects $a_i$ to $b_i$, and the interior of the curve is contained in the interior of $D$. Recall that every pair of resulting curves crosses at most once, and every point in the interior of $D$ may be contained in at most two curves.
For all $1\leq i\leq z$, we modify the curve $\gamma(Q_i)$, by replacing the segment of the curve that is contained in disc $D$ with $\sigma_i$.
Once every vertex $v\in V_1$ is processed, we obtain a collection $\Gamma''=\set{\gamma''(Q)\mid Q\in \qset}$ of curves, where for all $Q\in \qset$, curve $\gamma''(Q)$ connects $\phi(s(Q))$ to $\phi(t(Q))$. Moreover, it is easy to verify that each resulting curve $\gamma''(Q)\in \Gamma''$ is aligned with the graph $\bigcup_{Q'\in \qset}Q'$, and that the curves in $\Gamma''$ are in general position.
 
o
First, for each path $Q\in \qset$, we define curve $\gamma'(Q)$ to be the concatenation of all curves representing images of edges in $E(Q)$ in $\phi$. Clearly, the curve $\gamma'(Q)$ connects $\phi(s_Q)$ to $\phi(t_Q)$. We designate $\phi(s_Q)$ as its first endpoint $s(\gamma'(Q))$ and $\phi(t_Q)$ as its last endpoint $t(\gamma'(Q))$.
We then denote $\Gamma'=\set{\gamma'(Q)}$.


In the second step, we iteratively modify the curves in $\Gamma'$ as follows.
Throughout, we maintain (i) a set $\hat{\Gamma}$ of curves, that is initialized to be $\Gamma'$; and (ii) a set $Z$ of points that lie in at least two curves of $\hat\Gamma$ and is an inner point of at least one of these two curves.
The algorithm continues to be executed as long as set $Z$ is not empty.
We now describe an iteration.
We first arbitrarily pick a point $z$ from $Z$. Clearly, $z$ is either a crossing between two edges of $E(\qset)$ in $\phi$, or is the image of some vertex of $V(\qset)$ in $\phi$. 
Let $D_z$ be a tiny disc around the point $z$.
Let $\gamma_{1},\ldots,\gamma_{k}$ be the curves in $\hat \Gamma$ that contains $z$.
For each $1\le i\le k$, if $z$ is an inner point of $\gamma_{i}$, then recall that $s(\gamma_i)$ the first endpoint of $\gamma_i$ and $t(\gamma_i)$ is the last endpoint of $\gamma_i$, and we denote by $s'_i, t'_i$ the intersections between curve $\gamma_i$ and the boundary $D_z$, so the points $s(\gamma_i),s'_i,z,t'_i,t(\gamma_i)$ appear on the directed curve $\gamma_i$ in this order.
If $z$ is the first endpoint of $\gamma_i$, then we denote $s'_i=z$ and denote by $t'_i$ the intersection between $\gamma_i$ and the boundary of $D_z$, so the points $s'_i,z,t'_i,t(\gamma_i)$ appear on the directed curve $\gamma_i$ in this order.
If $z$ is the last endpoint of $\gamma_i$, then we denote $t'_i=z$ and denote by $s'_i$ the intersection between $\gamma_i$ and the boundary of $D_z$, so the points $s(\gamma_i),s'_i,z,t'_i$ appear on the directed curve $\gamma_i$ in this order.

\begin{figure}[h]
	\centering
	\subfigure[Before: Curves $\gamma_1,\gamma_2,\gamma_3,\gamma_4,\gamma_5$ are shown in red, yellow, pink, black and green respectively.]{\scalebox{0.33}{\includegraphics[scale=0.4]{figs/type_2_uncross_proof_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.1cm}
	\subfigure[Curves of $\set{\eta^i_z\mid 1\le i\le k}$ connecting points of $S'$ to points of $T'$ are shown in dash blue lines.]{
		\scalebox{0.33}{\includegraphics[scale=0.4]{figs/type_2_uncross_proof_2.jpg}}}
	\hspace{0.1cm}
	\subfigure[After: New curves $\hat\gamma_1,\hat\gamma_2,\hat\gamma_3,\hat\gamma_4,\hat\gamma_5$ are shown in red, yellow, pink, black and green respectively.]{
		\scalebox{0.33}{\includegraphics[scale=0.4]{figs/type_2_uncross_proof_3.jpg}}}
	\caption{An illustration of an iteration of the iterative algorithm for modifying the curves in $\hat \Gamma$.}\label{fig: type_2_uncross_proof}
\end{figure}

We define the multisets $S'=\set{s'_i\mid 1\le i\le k}$ and $T'=\set{t'_i\mid 1\le i\le k}$. 
We now modify the curves $\gamma_1,\ldots,\gamma_k$ as follows. 
We move the point $z$ (along with all points $s'_i=z$ and $t'_j=z$) to the boundary of $D_z$. Now all points of $S'\cup T'$ lie on the boundary of $D_z$.
We then construct a set of curves within $D_{z}$ in rounds as follows. In each round, pick a pair $s_i,t_j$ of vertices, where $s_i\in S'$ and $t_j\in T'$, that appears consecutively on the boundary of $D_z$. Clearly such a pair of vertices exist. We then draw a curve connecting $s_i$ to $t_j$ without crossing all curves that are constructed before, and then delete $s_i,t_j$ from sets $S',T'$, respectively. It is easy to verify that, at the end of this process, we will obtain a set $\set{\eta^{i}_z\mid 1\le i\le k}$ of curves, such that
\begin{itemize}
	\item for each $1\le i\le k$, the curve $\eta_z^i$ connects $s'_i$ to a distinct point $t'_{x_i}$ of $T'$; 
	\item for each $1\le i\le k$, the curve $\eta_z^i$  lies entirely in the disc $D_z$; and 
	\item the curves in $\set{\eta^{i}_z\mid 1\le i\le k}$ are mutually disjoint, except that they may share $z$ as an endpoint.
\end{itemize}

See Figure~\ref{fig: type_2_uncross_proof} for an illustration.
For each $1\le i\le k$, we denote by $\gamma^s_i$ the subcurve of $\gamma_i$ between $s_i$ and $s'_i$, and by $\gamma^t_i$ the subcurve of $\gamma_i$ between $t'_i$ and $t_i$. 
We now move the point $z$ (along with all points $s'_i=z$ and $t'_j=z$) to back to its original position. 
We then define, for each $1\le i\le k$, a new curve $\hat \gamma_i$ to be the sequential concatenation of curves $\gamma^s_i, \eta^i_z, \gamma^t_{x_i}$. 
See Figure~\ref{fig: type_2_uncross_proof} for an illustration.
We then replace the curves $\gamma_1,\ldots,\gamma_k$ in $\hat\Gamma$ with the new curves $\hat\gamma_1,\ldots,\hat\gamma_k$. This completes the description of an iteration.
%We remark that it is possible that some curve $\gamma_i$ has $z$ as its first endpoint or its last endpoint, and in this case the curve modification can be implemented in a similar way, which we omit here.

Let $\Gamma''$ be the set of curves that we obtain at the end of the algorithm.

It is easy to verify that, in the iteration described above, for each $1\le i\le k$, the first endpoint of the new curve $\hat\gamma_i$ is identical to that of the original curve $\gamma_i$, and similarly the multiset of the last endpoints of new curves $\hat\gamma_1,\ldots,\hat\gamma_k$ is identical to that of the original curves $\gamma_1,\ldots,\gamma_k$.
%Therefore, the multisets $S(\Gamma'')=S(\Gamma')$ and $T(\Gamma'')=T(\Gamma')$. 
It is also easy to verify that the point $z$ is no longer contains in any of the new curves $\hat\gamma_1,\ldots,\hat\gamma_k$ as an inner vertex (and so it does not belong to set $Z$ anymore), while other points in $Z$ remains in $Z$, and there are no new points added to $Z$.
So in each iteration, one point is removed from set $Z$, and therefore the algorithm of processing $\Gamma'$ will terminate in $O(\chi(\Gamma'))$ rounds.
Moreover, from the terminating criterion of the algorithm, the curves in the resulting set $\Gamma''$ no longer cross with each other. 

In the last step, we remove self-crossings of all curves of $\Gamma''$. Let $\Gamma$ be the set of curves we obtain. 
We designate the curve in $\Gamma$ with first endpoint $\phi(s(Q))$ as $\gamma(Q)$. We now show that the set $\Gamma$ of curves satisfy all properties required in \Cref{thm: new type 2 uncrossing}.
From the above discussion, it is clear that the second, the fourth and the fifth properties are satisfied. We now show that the curves in $\Gamma$ are aligned with graph $\bigcup_{Q'\in \qset}Q'$. 
Clearly, in each iteration of the above curve modification process, we re-draw the curve only within a tiny disc around a crossing of two edges or around the image of a vertex of $V(\qset)$, and then (possibly) change the course of curves.
In the self-loop removing step, it is clear that the self-crossing has to be the crossing of two edges in $E(\qset)$.
Therefore, those re-drawn segments and the self-crossing points can be viewed as segments $\sigma_1,\ldots,\sigma_{r}$ of the curves, and since we start from the curves in $\Gamma'$ which only contain images of edges of $E(Q)$, the other segments $\sigma'_1,\ldots,\sigma'_{r-1}$ are all contiguous segments of non-zero length of the image of some edge in $\phi$. 
We last show that the third property is satisfied. In fact, if $u^*$ is the common first endpoint of all curves in $\Gamma'$, then point $u^*$ never belongs to set $Z$ and is therefore not processed. This implies that the first segments of all curves of $\Gamma'$ has not been changed, and therefore, for each path $Q\in \qset$, curve $\gamma(Q)$ contains the segment of the image of $e_1(Q)$ that lies in the disc $D_{\phi}(u^*)$.
This completes the proof of \Cref{thm: new type 2 uncrossing}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of \Cref{cor: new type 2 uncrossing}}
\label{apd: cor new type 2 uncrossing}


For each edge $e\in E(\qset)$, we denote by $\phi(e)$ the curve that represents the image of $e$ in $\phi$, and then we create a set $\Pi_e$ of $\cong_{G}(\qset,e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi$, that lies in an arbitrarily thin strip around $\phi(e)$.
We next assign, for each edge $e\in E(\qset)$ and for each path in $\qset$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
Therefore, each curve in $\bigcup_{e\in E(\qset)}\Pi_e$ is assigned to exactly one path of $\qset$,
and each path $Q\in\qset$ is assigned with, for each edge $e\in E(Q)$, a curve in $\Pi_e$. Let $\gamma'(Q)$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\qset)}\Pi_e$ that are assigned to path $Q$, so $\gamma'(Q)$ connects the the image $\phi(s_Q)$ of the first endpoint $s_Q$ of $Q$ to the image $\phi(t_Q)$ of the last endpoint $t_Q$ of $Q$ in $\phi$.

We then perform the iterative curve-modification algorithm presented in \Cref{apd: new type 2 uncrossing} to set $\Gamma'=\set{\gamma'(Q)}$ of curves and obtain a set $\Gamma''$ of curves. We then remove self-crossings in the same way as \Cref{apd: new type 2 uncrossing}. Let $\Gamma$ be the set of curves we obtain. 
We designate the curve in $\Gamma$ with first endpoint $\phi(s(Q))$ as $\gamma(Q)$. We now show that the set $\Gamma$ of curves satisfy all properties required in \Cref{cor: new type 2 uncrossing}.
From the analysis in \Cref{apd: new type 2 uncrossing}, it is clear that the first, the second, and the third properties are satisfied. We now show that the fourth property is also satisfied.
Note that, although the curves in $\Gamma$ are not rigorously graph-aligned curves, they can be partitioned into consecutive segments $(\sigma_1,\sigma_1',\sigma_2,\sigma_2',\ldots,\sigma'_{r-1},\sigma_r)$, such that each $\sigma'_1$, although not necessarily a contiguous segment of the image of some edge of $E(\qset)$ in $\qset$, but it lies entirely within an arbitrarily thin strip of a contiguous segment of the image of some edge of $E(\qset)$ in $\qset$. Moreover, for each edge $e'\in E(G\setminus C)$, the number of segments of curves in $\Gamma$ that lie entirely within the thin strip of $\phi(e)$ is bounded by $\cong_G(\qset,e')$.
From the fact that the curves in $\Gamma$ do not cross each other, for every edge $e\in E(C)$, the number of crossings between the image of edge $e$ in $\phi$ and the curves in $\Gamma$ is bounded by the sum of, over all edges $e'\in E(G\setminus C)$, the number of crossings between $e$ and $e'$ in $\phi$, times $\cong_G(\qset, e)$, which is in turn bounded by $\chi_{\phi}(e, G\setminus C)\cdot \cong_G(\qset)$.
This completes the proof of \Cref{cor: new type 2 uncrossing}.





\subsection{Proof of \Cref{obs: splicing}}
\label{apd: Proof of splicing}

We first show that $S(\pset')=S(\pset)$ and $T(\pset')=T(\pset)$.
We denote by $s$ and $t$ the first and the last endpoints of $P$, respectively, and by $s'$ and $t'$ the first and the last endpoints of $P'$, respectively.
From the construction, the first endpoint of $\tilde P$ is $s$ and the last endpoint of $\tilde P$ is $t'$; and the first endpoint of $\tilde P'$ is $s'$ and the last endpoint of $\tilde P'$ is $t$.
Since the first endpoints and the last endpoints of other paths are not changed, $S(\pset')=S(\pset)$ and $T(\pset')=T(\pset)$.

Assume that both $\tilde P,\tilde P'$ are simple paths. We will show that $|\Pi^T(\pset')|<|\Pi^T(\pset)|$.
Specifically, we will construct a mapping $f$ that maps each triple in $\Pi^T(\pset')$ to a triple in $\Pi^T(\pset)$, such that $f$ is injective but not surjective.
%


Note that $\pset'\setminus\set{\tilde P, \tilde P'}=\pset\setminus\set{P,  P'}$. We denote $\hat \pset=\pset\setminus\set{P,  P'}$.
Since the set $\Pi^T(\pset)$ contains the triple $(P,P',v)$, $v$ must be an inner vertex of both $P$ and $P'$.
Since we have assumed that paths $\tilde P, \tilde P'$ are simple paths, $v$ is the only vertex shared by paths $\tilde P$ and $\tilde P'$, and $v$ is the only vertex shared by paths $P$ and $P'$. From the construction, the intersection of paths $\tilde P,\tilde P'$ at $v$ is non-transversal with respect to $\Sigma$. 
Therefore, each triple in $\Pi^T(\pset')$ is of one of the following types:
\begin{itemize}
	\item $(Q,Q',v')$ where $Q,Q'\in \hat\pset$;
	\item $(Q,\tilde P ,v')$ or $(Q,\tilde P' ,v')$ where $Q\in \hat\pset$ and $v'\ne v$;
	\item $(Q,\tilde P ,v)$ or $(Q,\tilde P' ,v)$ where $Q\in \hat\pset$.
\end{itemize}



First, it is easy to see that, for every triple $(Q,Q',v')\in \Pi^T(\pset')$ such that $Q,Q'\in \pset'\setminus\set{\tilde P, \tilde P'}$, the triple $(Q,Q',v')$ also belongs to the set $\Pi^T(\pset)$.
We then map such a triple to itself.

Second, consider a triple $(Q,\tilde P,v')$ in $\Pi^T(\pset')$ such that $Q\in \hat \pset$ and $v'\ne v$. If vertex $v'$ belongs to the subpath of $\tilde P$ from $s$ to $v$, then it is easy to verify that the triple $(Q,P,v')$ belongs to $\Pi^T(\pset)$, and we map the triple $(Q,\tilde P,v')$ to the triple $(Q,P,v')$.
If $v'$ belongs to the subpath of $P$ from $v$ to $t'$, then it is easy to verify that the triple $(Q,P',v')$ belongs to $\Pi^T(\pset)$, and we map the triple $(Q,\tilde P,v')$ to the triple $(Q,P',v')$.
Similarly, for each triple $(Q,\tilde P',v')\in\Pi^T(\pset')$, either the triple $(Q,P,v')$ or the triple $(Q,P',v')$ belongs to $\Pi^T(\pset)$, and we map the triple $(Q,\tilde P',v')$ to either $(Q,P,v')$ or $(Q,P',v')$ accordingly.


Last, we consider the triples in $\Pi^T(\pset')$ of the third type.
We denote by $e_a,e_b$ the edges of $P$ incident to $v$, where $e_a$ precedes $e_b$ in $P$ (recall that $v$ is an inner vertex of $P$). We define edges $e'_a,e'_b$ similarly for path $P'$. 
Assume that $\delta(v)=\set{e_a,e^1_1,\ldots,e^1_{r_1},e_b,e^2_1,\ldots,e^2_{r_2},e_a',e^3_1,\ldots,e^1_{r_3},e_b',e^4_1,\ldots,e^1_{r_4}}$, where edges are indexed according to the ordering $\oset_v\in \Sigma$.
We denote $E_1=\set{e^1_1,\ldots,e^1_{r_1}}$, $E_2=\set{e^2_1,\ldots,e^2_{r_2}}$,
$E_3=\set{e^3_1,\ldots,e^3_{r_3}}$ and
$E_4=\set{e^4_1,\ldots,e^4_{r_4}}$.
See \Cref{fig: splicing_1} for an illustration.
%
Consider now a path $Q\in \hat \pset$, and we denote by $e^Q_a,e^Q_b$ the paths of $Q$ incident to $v$, where $e^Q_a$ precedes $e^Q_b$ in $Q$.
We distinguish between the following cases.

\textbf{Case 1. $(Q,P,v), (Q,P',v)\in \Pi^T(\pset)$.} In this case, if set $\Pi^T(\pset')$ contains the triple $(Q,\tilde P, v)$, then we map it to the triple $(Q,P,v)$, and if set $\Pi^T(\pset')$ contains the triple $(Q,\tilde P', v)$, then we map it to the triple $(Q,P',v)$.

\textbf{Case 2. $(Q,P,v), (Q,P',v)\notin \Pi^T(\pset)$.} In this case, it is easy to verify that both edges $e'_a,e'_b$ belong to the same set of $E_1,E_2,E_3,E_4$. Therefore, the intersection between $Q$ and $\tilde P$ at $v$ is non-transversal, namely the set $\Pi^T(\pset')$ does not contain the triple $(Q,\tilde P,v)$. Similarly, the set $\Pi^T(\pset')$ does not contain the triple $(Q,\tilde P' ,v)$, either.

\textbf{Case 3. $(Q,P,v)\in \Pi^T(\pset), (Q,P',v)\notin \Pi^T(\pset)$.} In this case, it is easy to verify that either $e^Q_a\in E_1$ and $e^Q_b\in E_4$ (or symmetrically $e^Q_a\in E_4$ and $e^Q_b\in E_1$), or $e^Q_a\in E_2$ and $e^Q_b\in E_3$ (or symmetrically $e^Q_a\in E_3$ and $e^Q_b\in E_2$). In the former case (see \Cref{fig: splicing_2}), the intersection between paths $Q$ and $\tilde P$ at $v$ is transversal, while the intersection between paths $Q$ and $\tilde P'$ at $v$ is non-transversal. In other words, the set $\Pi^T(\pset')$ contains the triple $(Q,\tilde P,v)$ but not the triple $(Q,\tilde P' ,v)$. We then map $(Q,\tilde P,v)$ to the triple $(Q,P,v)$.
In the latter case (see \Cref{fig: splicing_3}), the intersection between paths $Q$ and $\tilde P'$ at $v$ is transversal, while the intersection between paths $Q$ and $\tilde P$ at $v$ is non-transversal. In other words, the set $\Pi^T(\pset')$ contains the triple $(Q,\tilde P',v)$ but not the triple $(Q,\tilde P ,v)$. We then map triple $(Q,\tilde P',v)$ to the triple $(Q,P,v)$.

\begin{figure}[h]
	\centering
	\subfigure[A schematic view of edges $e_a$, $e_b$, $e'_a$, $e'_b$ and edge sets $\set{E_i}_{1\le i\le 4}$.]{\scalebox{0.9}{\includegraphics[scale=0.4]{figs/splicing_1.jpg}}\label{fig: splicing_1}
	}
	\hspace{0.3cm}
	\subfigure[An illustration of the former case in Case 3.]{\scalebox{0.9}{\includegraphics[scale=0.4]{figs/splicing_2.jpg}}\label{fig: splicing_2}}
	\hspace{0.3cm}
	\subfigure[An illustration of the latter case in Case 3.]{
		\scalebox{0.9}{\includegraphics[scale=0.4]{figs/splicing_3.jpg}}\label{fig: splicing_3}}
	\caption{An illustration of edges and edge sets in the proof of \Cref{obs: splicing}.}
\end{figure}

It is easy to verify that the mapping we construct is injecture. We now show that it is surjective. In fact, since the intersection between paths $P,P'$ at $v$ is transversal, the set $\Pi^T(\pset)$ contains the triple $(P,P',v)$. However, it is easy to verify that no triple in  $\Pi^T(\pset')$ is mapped to the triple $(P,P',v)$. Therefore, the mapping we construct is surjective. This completes the proof of \Cref{obs: splicing}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of Lemma~\ref{lem: non_interfering_paths}}
\label{apd: Proof of non_interfering_paths}

We note that the proof of a similar version of Lemma~\ref{lem: non_interfering_paths} was included in the proof of Lemma 9.5 in \cite{chuzhoy2020towards}.
For completeness, we provide its proof here.

We first pre-process the set $\rset$ of paths by removing self-loops of all paths of $\rset$.
Let $\rset^*$ be the set of paths we get.
The algorithm is iterative. Throughout, we maintain a set $\hat \rset$ of paths in $G$, that is initialized to be $\rset^*$. The algorithm proceeds in iterations and continues to be executed as long as the set $\Pi^T(\hat\rset)$ for the current path set $\hat\rset$ is non-empty.
We now describe an iteration of the algorithm.
Let $(P,P',v)$ be any triple in $\Pi^T(\hat\rset)$. We perform the path splicing to paths $P,P'$ at vertex $v$. Let $\tilde P,\tilde P'$ be the paths we get.
We let path $\hat P$ be obtained from $\tilde P$ by removing self-loops of $\tilde P$, and we define path $\hat P'$ similarly. So $\hat P,\hat P'$ are simple paths. We then replace the paths $P,P'$ in $\hat\rset$ by paths $\hat P,\hat P'$ and continue to the next iteration. This completes the description of the algorithm.
Let $\rset'$ be the set of paths we obtain at the end of the algorithm.

We first show that the algorithm indeed terminates after $|V(G)|\cdot |E(G)|\cdot |\rset|^3$ rounds. We let $x(\hat \rset)=|\Pi^T(\hat\rset)|$ and $y(\hat\rset)=\sum_{e\in E(G)}\cong_{G}(\hat \rset, e)$. Clearly, over the course of the algorithm, $x(\hat \rset)\le |V(G)|\cdot |\rset|^2$, since all paths in $\hat \rset$ are simple and every pair of simple paths in $G$ share at most $|V(G)|$ vertices, and $y(\hat \rset)\le |E(G)|\cdot |\rset|$, since $|\hat\rset|=|\rset|$ always holds and every edge appears in at most $|\rset|$ paths in $\hat \rset$. Note that, from \Cref{lem: non_interfering_paths}, in one iteration of the algorithm, either the value of $y(\hat\rset)$ decreases by at least $1$ (if the pair $\tilde P,\tilde P'$ of paths we obtained in the splicing step are not both simple and we need to remove self-loops of at least one of them afterwards); or the value of $y(\hat\rset)$ stays the same and the value of $x(\hat\rset)$ decreases by at least $1$ (if the pair $\tilde P,\tilde P'$ of paths we obtained in the splicing step are both simple and the size of $|\Pi^T(\hat{\rset})|$ decreases by at least $1$). Also note that the algorithm will terminate whenever $x(\hat\rset)=0$. Altogether, we get that the algorithm must terminate after at most $|V(G)|\cdot |E(G)|\cdot |\rset|^3$ rounds.

We now show that the set $\rset'$ satisfies the desired properties in \Cref{lem: non_interfering_paths}. First, note we have pre-processed the set $\rset$ of paths into the set $\rset^*$ of simple paths, and from the description of the algorithm, at any time, the set $\hat \rset$ will only contain simple paths. We then conclude that the resulting set $\rset'$ only contains simple paths as well.
Second, note that the pre-processing step of removing self-loops does not change the first or the last endpoint of any path in $\rset$, so $S(\rset^*)=S(\rset)$ and $T(\rset^*)=T(\rset)$. Additionally, from \Cref{obs: splicing}, the path-splicing step does not change the set of first endpoints or the set of first endpoints, so $S(\rset')=S(\rset^*)$ and $T(\rset')=T(\rset^*)$. Altogether, we get that $S(\rset')=S(\rset)$ and $T(\rset')=T(\rset)$. Third, since the algorithm does not terminate as long as the set $\hat{\rset}$ of paths is not non-transversal with respect to $\Sigma$, the resulting path set $\rset'$ is non-transversal with respect to $\Sigma$.
Fourth, it is easy to observe that, in either a self-loop-removing step or a path-splicing step, we do not increase the congestion on any edge. Therefore, for the resulting path set $\rset'$, it must hold that, for each edge $e\in E(G)$, $\cong_G(\rset',e)\le \cong_G(\rset,e)$.











\iffalse{for edge-disjoint path}

%We view the given set $\rset$ of paths as originating from $v$ and terminating at $v'$. 
Let $H=\bigcup_{P\in \rset}P$ be the subgraph of $\hat G$ consisting of paths of $\rset$.
Our first step is to compute a set $\hat\rset$ of $|\hat \rset|=|\rset|$ edge-disjoint paths connecting $v$ to $v'$, using standard max-flow algorithms.
We view the paths in $\hat\rset$ as being directed from $v$ to $v'$. Let $\hat H$ be the directed graph obtained by taking the union of the directed paths in $\hat\rset$, so $\hat H$ is a subgraph of $H$. From the max-flow algorithm, we can further assume there is an ordering $\Omega$ of its vertices, such that, for every pair $x,y$ of vertices in $\hat H$, if there is a path of $\hat \rset$ in which $x$ appears before $y$, then $x$ also appears before $y$ in the ordering $\Omega$. 
For each vertex $u\in V(\hat H)$, we denote by $\delta^+(u)$ the set of edges leaving $u$ in $\hat H$, and by $\delta^-(u)$ the set of edges entering $u$ in $\hat H$. Clearly, if $u\ne v,v'$, then $|\delta^+(u)|=|\delta^-(u)|$.
We use the following simple observation.

\begin{observation}
	\label{obs:rerouting_matching}
	We can efficiently compute, for each vertex $u\in V(\hat H)\setminus \set{v,v'}$, a perfect matching $M(u)\subseteq \delta^-(u)\times \delta^+(u)$ between the edges of $\delta^-(u)$ and the edges of $\delta^+(u)$, such that, for each pair of matched pairs $(e^-_1,e^+_1)$ and $(e^-_2,e^+_2)$ in $M(u)$, the intersection of the path that consists of the edges $e^-_1,e^+_1$ and the path that consists of edges $e^-_2,e^+_2$ at vertex $u$ is non-transversal with respect to $\hat\Sigma$.
\end{observation}
\begin{proof}
	We start with $M(u)=\emptyset$ and perform $|\delta^-(u)|$ iterations. In each iteration, we select a pair $e^-\in \delta^-(u), e^+\in \delta^+(u)$ of edges that appear consecutively in the rotation $\oset_v$ of $\tilde\Sigma$. We add $(e^-,e^+)$ to $M(u)$, delete them from $\delta^-(u)$ and $\delta^+(u)$ respectively, and then continue to the next iteration. It is immediate to verify that the resulting matching $M(u)$ satisfies the desired properties.
\end{proof}

We now gradually modify the set $\hat\rset$ of paths in order to obtain a set $\rset'$ of edge-disjoint paths connecting $v$ to $v'$, that is non-transversal with respect to $\hat \Sigma$.
We process all vertices of $V(\hat H)\setminus \set{v,v'}$ one-by-one, according to the ordering $\Omega$. We now describe an iteration in which a vertex $u$ is processed. Let $\hat \rset_u\subseteq \hat \rset$ be the set of paths containing $u$. For each path $P\in \hat \rset_u$, we delete the unique edge of $\delta^+(u)$ that lies on this path, thereby decomposing $P$ into two-subpaths: path $P^-$ connecting $v$ to $u$; and path $P^+$ connecting some vertex $u'$ that is the endpoint of an edge of $\delta^+(u)$ to $v'$. Define $\hat \rset^-_u=\set{P^-\mid P\in \hat \rset_u}$ and 
$\hat \rset^+_u=\set{P^+\mid P\in \hat \rset_u}$.
We will glue these paths together using the edges in $\delta^+(u)$ and the matching $M(u)$ produced in Observation \ref{obs:rerouting_matching}. Specifically, we construct a new set $\rset'$ of paths that contains, for each path $P\in \hat \rset$, a new path $P'$, as follows. Consider a path $P\in \hat \rset$. If $P\notin \hat \rset_u$, then we let $P'=P$. Otherwise, consider the unique path $P^-\in \hat \rset^-_u$ that is a subpath of $P$, and let $e^-_P$ be the last edge on this path. Let $e^+$ be the edge in $\delta^+(u)$ that is matched with $e^-_P$ in $M(u)$, and let $\hat P^+$ be the unique path in $\hat \rset^+_u$ that contains $e^+$.
We then define the new path $P'$ to be the concatenation of the path $P^-$, the edge $e^+$, and the path $\hat P^+$. This finishes the description of an iteration.
%Let $\rset'$ be the final set of path that we obtain from the above process. 
It is easy to verify that $|\rset'|=|\hat \rset|=|\rset|$, $E(\rset')\subseteq E(\hat\rset)\subseteq E(\rset)$, and the set $\rset'$ of paths is locally non-interfering with respect to $\hat\Sigma$.

\fi

\iffalse
%% For general paths
Our first step is to compute another one-to-one routing $\hat\rset$ of vertice of $S$ to vertices of $T$, via $|\hat \rset|=|\rset|$ simple paths, such that for every $e\in E( G)$, $\cong_{ G}(\hat\rset,e)\le \cong_{ G}(\rset,e)$, using standard max-flow algorithms.
%Let $H=\bigcup_{P\in \rset}P$ be the subgraph of $G$ consisting of paths of $\rset$.
We first construct a graph $H$ as follows.
We start from the graph $\bigcup_{P\in \rset}P$.
%, where we view the paths in $\rset$ as being directed from its endpoint in $S$ to its endpoint in $T$. 
%Let $\hat H$ be the directed graph obtained by taking the union of the directed paths in $\rset$, so $\hat H$ is a subgraph of $H$.
%We further modify the graph $\hat H$ as follows. 
We then replace each edge $e$ of $E(\rset)$ with $\cong_{G}(\rset,e)$ copies of it, and let each path of $\rset$ that contains $e$ takes a distinct copy. 
Finally, we add two new vertices $s,t$, and then add, for each vertex $v\in S$, an edge $(s,v)$; and for each vertex $v'\in S$, an edge $(v',t)$.
This finishes the definition of $H$.
Now paths of $\rset$ are edge-disjoint paths in $H$.
For each vertex $v\in V(H)\setminus \set{s,t}$, we define its rotation $\oset'_v$ as follows. We start with its oritinal rotation $\oset_v\in \Sigma$, and then replace, for each edge $e$, the edge $e$ in the ordering $\oset_v$ by its $\cong_{G}(\rset,e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, and the ordering among the copies is arbitrary.
Now we compute the a set $\hat \rset$ of $|\hat \rset|=|\rset|$ edge-disjoint paths connecting $s$ to $t$ in $H$. It is easy to see that such a set of path exists.
We view these paths as directed from $s$ to $t$.
From the max-flow algorithm, we can further assume there is an ordering $\Omega$ of its vertices, such that, for every pair $x,y$ of vertices in $H$, if there is a path of $\hat\rset$ in which $x$ appears before $y$, then $x$ also appears before $y$ in the ordering $\Omega$. 
For each vertex $u\in V(H)$, we denote by $\delta^+(u)$ the set of edges leaving $u$ in $H$, and by $\delta^-(u)$ the set of edges entering $u$ in $H$. Clearly, if $u\ne s,t$, then $|\delta^+(u)|=|\delta^-(u)|$.

We now gradually modify the set $\hat\rset$ of paths in order to obtain a set $\hat\rset'$ of edge-disjoint paths in $H$ connecting $s$ to $t$, that is non-transversal with respect to the new orderings in $\set{\oset'_v\mid v\in V(H)\setminus\set{s,t}}$.
We process all vertices of $V(H)\setminus \set{s,t}$ one-by-one, according to the ordering $\Omega$. We now describe an iteration in which a vertex $u$ is processed. Let $\hat \rset_u\subseteq \hat \rset$ be the set of paths containing $u$. For each path $P\in \hat \rset_u$, we delete the unique edge of $\delta^+(u)$ that lies on this path, thereby decomposing $P$ into two-subpaths: path $P^-$ connecting $s$ to $u$; and path $P^+$ connecting some vertex $u'$ that is the endpoint of an edge of $\delta^+(u)$ to $t$. Define $\hat \rset^-_u=\set{P^-\mid P\in \hat \rset_u}$ and 
$\hat \rset^+_u=\set{P^+\mid P\in \hat \rset_u}$.
We will glue these paths together using the edges in $\delta^+(u)$ and the matching $M(u)$ produced in \Cref{obs:rerouting_matching_cong}. Specifically, we construct a new set $\hat\rset'$ of paths that contains, for each path $P\in \hat \rset$, a new path $P'$, as follows. Consider a path $P\in \hat \rset$. If $P\notin \hat \rset_u$, then we let $P'=P$. Otherwise, consider the unique path $P^-\in \hat \rset^-_u$ that is a subpath of $P$, and let $e^-_P$ be the last edge on this path. Let $e^+$ be the edge in $\delta^+(u)$ that is matched with $e^-_P$ in $M(u)$, and let $\hat P^+$ be the unique path in $\hat \rset^+_u$ that contains $e^+$.
We then define the new path $P'$ to be the concatenation of the path $P^-$, the edge $e^+$, and the path $\hat P^+$. This finishes the description of an iteration.
%Let $\rset'$ be the final set of path that we obtain from the above process. 
It is easy to verify that $|\hat\rset'|=|\hat \rset|=|\rset|$, $E_{H}(\hat \rset')\subseteq E_{H}(\hat\rset)$, and the set $\hat\rset'$ of paths is non-transversal with respect to the orderings in $\set{\oset'_v\mid v\in V(H)\setminus\set{s,t}}$.
Finally, we let the set $\rset'$ contains, for each path $P'\in \hat\rset'$, the original path of $P'\setminus\set{s,t}$ in $H$ (namely, if $P'\setminus\set{s,t}$ contains a copy of $e$, then its original path contains the edge $e$). 
It is easy to verify that $|\rset'|=|\rset|$, for each $e\in  G$, $\cong_{G}(\rset',e)\le \cong_{G}(\rset,e)$, and the set $\rset'$ of paths is non-transversal with respect to $\Sigma$.

\fi







%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\subsection{Proof of \Cref{obs:rerouting_matching_cong}}
\label{apd: Proof of rerouting_matching_cong}


Denote $E=\delta_G(v)$. We first define a multiset $E'$ and an ordering $\oset'$ on $E'$ as follows. Set $E'$ contains, for each edge $e\in E$, $(n^-_e+n^+_e)$ copies of $e$, in which $n^-_e$ copies are labelled $-$, and other $n^+_e$ copies are labelled $+$. The ordering $\oset'$ on $E'$ is obtained from the ordering $\oset_v$ on $E$ by replacing, for each $e\in E'$, the edge $e$ in the ordering $\oset_v$ with its $(n^-_e+n^+_e)$ copies in $E'$, that appear consecutively at the location of $e$ in $\oset_v$, and the ordering among these copies is arbitrary.
Since $\sum_{e\in E}n^-_e=\sum_{e\in E}n^+_e$, the number of edges in $E'$ that are labelled $-$ is the same as the number of edges in $E'$ that are labelled $+$.
We now iteratively construct a set $M'$ of ordered pairs as follows.
We start with $M'=\emptyset$ and perform iterations.
In each iteration, we find a pair of edges in $E'$ that appears consecutively in $\oset'$, such that one of them (denoted by $e'_1$) is labelled $-$ and the other (denoted by $e'_2$) is labelled $+$. It is clear that such a pair always exists. Note that it is possible that $e'_1$ and $e'_2$ are distinct copies of the same edge of $E$.
We then add the ordered pair $(e'_1,e'_2)$ to $M'$, and delete $e'_1,e'_2$ from $E'$ and $\oset'$.
It is clear that after this iteration, the number of remaining edges in $E'$ (and in $\oset'$) that are labelled $-$ is still the same as the number of remaining edges in $E'$ (and in $\oset'$) that are labelled $+$. Therefore, at the end of the process, $E'$ and $\oset'$ become empty and $M'$ contains $\sum_{e\in E}n^+_e$ ordered pairs of edges in $E'$. Moreover, for each pair of ordered pairs in $M'$, the intersection between the paths consisting of corresponding pairs of edges is non-transversal with respect to $\oset'$. 
We then let set $M$ contains, for each pair $(e'_1,e'_2)\in M$, a pair $(e_1,e_2)$, where $e_1$ is the original edge of $e'_1$ in $E$ and $e_2$ is the original edge of $e'_2$ in $E$. It is clear that for each pair of ordered pairs in $M$, the intersection between the paths consisting of corresponding pairs of edges is non-transversal with respect to $\oset'$. 



\fi


















%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\subsection{Proof of \Cref{lem: non transversal cost of cycles bounded by cr}}
\label{apd: Proof of non transversal cost of cycles bounded by cr}

 
Consider a pair $R,R'$ of edge-disjoint cycles with $R\in \rset$ and $R'\in \rset'$. We denote by $\gamma$ the closed curve obtained by taking the union of the images of all edges of $R$ in $\phi$, and we define the closed curve $\gamma'$ similarly. Since $R$ and $R'$ are edge-disjoint, and since $\phi$ is a feasible solution to instance $I=(G,\Sigma)$, curves $\gamma$ and $\gamma'$ are in general position. Let $X(\gamma,\gamma')$ be the set of crossings between curves $\gamma,\gamma'$ that are not vertex-images in $\phi$, so $|X(\gamma,\gamma')|=\chi(\gamma,\gamma')$. We will show that, if the intersection between $R$ and $R'$ are transversal at exactly one of their shared vertices, then $X(\gamma,\gamma')\ne \emptyset$.


Assume for contradiction that $X(\gamma,\gamma')=\emptyset$. Let $v_1,\ldots,v_k$ be the shared vertices between $R$ and $R'$, and let $x_1,\ldots,x_k$ be the images of $v_1,\ldots,v_k$ in $\phi'$, respectively. Assume without loss of generality that vertices $v_1,\ldots,v_k$ appear sequentially on cycle $R$, and the intersection between $R$ and $R'$ is transversal at $v_1$. 
We give a direction for the closed curve $\gamma$ as follows: $x_1\to x_2\to\ldots\to x_k\to x_1$.
Clearly, the curve $\gamma$ partitions the sphere into internally-disjoint discs, and since $R$ is a simple cycle, vertex $x_1$ lies on the boundary of exactly two of these discs, that we denote by $D_{+}$ and $D_{-}$.
%Let $D$ be the disc such that (i) the boundary of $D$ is the union of disjoint segments of $\gamma$; (ii) the point $x_1$ belongs to the boundary of $D$; and (iii) the interior of $D$ that contains a point to the right of $x_1$ (when travelling along the curve $\gamma$ in the direction defined above) does not contain any point of $\gamma$. Clearly, such a disc exists and is unique.
Since cycles $R,R'$ are disjoint and the intersection of them is transversal at $v_1$, if we denote by $\gamma'_+$ the tiny segment of curve $\gamma'$ that has $x_1$ as an endpoint and goes a little in one direction of $\gamma'$, and denote by $\gamma'_-$ the tiny segment of curve $\gamma'$ that has $x_1$ as an endpoint and goes a little in the other direction of $\gamma'$, then one of segments $\gamma'_+, \gamma'_+$ belong to $D_{+}$ and the other belongs to $D_{-}$. Therefore, since $\gamma'$ is a closed curve, $\gamma'$ has to intersect the boundary of disc $D_{+}$ at some other point $x'$. However, since $R$ and $R'$ are edge-disjoint and the intersections of $R$ and $R'$ are non-transversal at $v_2,\ldots,v_k$, $x$ cannot be any of $\set{x_2,\ldots,x_k}$. Therefore, $x'$ has to be some non-vertex-image crossings between $\gamma$ and $\gamma'$.

We now complete the proof of \Cref{lem: non transversal cost of cycles bounded by cr}. 
For every cycle $R\in \rset$, we denote by $\gamma_R$ the closed curve obtained by taking the union of the images of all edges of $R$ in $\phi$, and for each cycle $R\in \rset'$, we define the closed curve $\gamma_R'$ similarly.
Then it is easy to verify that every crossing $(e,e')$ in drawing $\phi$ belongs to at most $\bigg(\cong_G(\rset,e)\cdot \cong_G(\rset',e')+\cong_G(\rset,e')\cdot \cong_G(\rset',e)\bigg)$ sets among all sets of $\set{X(\gamma_R,\gamma_{R'})\mid R\in \rset, R'\in \rset'}$.
Since for every pair $R, R'$ of edge-disjoint cycles with $R\in \rset, R'\in \rset'$, the intersection of $R$ and $R'$ is transversal at at most one of their common vertices, we get that
\[
\begin{split}
\ntcost(\rset,\rset';\Sigma)\le & \sum_{R\in \rset, R'\in \rset'} |X(\gamma_{R}, \gamma_{R'})|\\
\le & \sum_{e,e'\in E(G)}\chi_{\phi}(e,e')\cdot \bigg(\cong_G(\rset,e)\cdot \cong_G(\rset',e')+\cong_G(\rset,e')\cdot \cong_G(\rset',e)\bigg).
\end{split}
\]













%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of \Cref{thm: new nudging}}
\label{apd: Proof of curve_manipulation}

We first prove the following lemma.

%\mynote{can we say that $\gamma'$ also has endpoints $s_{\gamma},t_{\gamma}$? can we say after the lemma that if the curves in $\Gamma$ intersect at $p$ in a non-transversal manner then the resulting cuves are disjoint?}
\begin{lemma}[Nudging]
	\label{obs: curve_manipulation}
	There exists an efficient algorithm, that, given a point $p$ in the plane, a disc $D$ containing $p$, and a set $\Gamma$ of curves, such that every curve $\gamma$ of $\Gamma$ contains the point $p$ and intersects the boundary of $D$ at two distinct points $s_{\gamma},t_{\gamma}$, and $p$ is the only point in $D$ that belongs to at least two curves of $\Gamma$, computes, for each curve $\gamma\in \Gamma$, a curve $\gamma'$, such that
	\begin{itemize}
		\item for each curve $\gamma\in \Gamma$, the curve $\gamma'$ does not contain $p$, and is identical to the curve $\gamma$ outside the disc $D$;
		%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
		\item the segments of curves of $\set{\gamma'\mid \gamma\in \Gamma}$ inside disc $D$ are in general position; 
		\item for each pair $\gamma_1,\gamma_2$ of curves in $\Gamma$, the new curves $\gamma_1,\gamma_2$ cross inside $D$ iff the order in which the points $s_{\gamma_1},t_{\gamma_1},s_{\gamma_2},t_{\gamma_2}$ appear on the boundary of $D$ is either $(s_{\gamma_1},s_{\gamma_2},t_{\gamma_1},t_{\gamma_2})$ or $(s_{\gamma_1},t_{\gamma_2},t_{\gamma_1},s_{\gamma_2})$.
		%the number of crossings between curves of $\set{\gamma'\mid \gamma\in \Gamma}$ inside  $D$ is at most  the number of pairs $\gamma_1,\gamma_2$ in $\Gamma$, such that the order in which the points $s_{\gamma_1},t_{\gamma_1},s_{\gamma_2},t_{\gamma_2}$ appear on the boundary of $D$ is either $(s_{\gamma_1},s_{\gamma_2},t_{\gamma_1},t_{\gamma_2})$ or $(s_{\gamma_1},t_{\gamma_2},t_{\gamma_1},s_{\gamma_2})$.
		%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
	\end{itemize}
\end{lemma}

\begin{proof}
	%Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
	%For each curve $\gamma\in \Gamma$, we denote by $s_{\gamma}$ and $t_{\gamma}$ the intersections between $\gamma$ and the boundary of $D$.
	We first compute, for each $\gamma\in \Gamma$, a curve $\tilde\gamma$ inside disc $D$ connecting $s_{\gamma}$ to $t_{\gamma}$, such that (i) the curves in $\set{\tilde\gamma\mid \gamma\in \Gamma}$ are in general position; and (ii) for each pair $\gamma_1,\gamma_2$ of curves in $\Gamma$, the curves $\tilde\gamma_1$ and $\tilde\gamma_2$ intersects iff the order in which the points $s_{\gamma_1},t_{\gamma_1},s_{\gamma_2},t_{\gamma_2}$ appear on the boundary of $D$ is either $(s_{\gamma_1},s_{\gamma_2},t_{\gamma_1},t_{\gamma_2})$ or $(s_{\gamma_1},t_{\gamma_2},t_{\gamma_1},s_{\gamma_2})$.
	It is clear that this can be achieved by first setting, for each curve $\gamma$, the curve $\tilde \gamma$ to be the line segment connecting $s_{\gamma}$ to $t_{\gamma}$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\tilde \gamma\mid \gamma\in \Gamma}$.
	We now define, for each $\gamma\in \Gamma$, the curve $\tilde\gamma$ to be the union of the part of $\gamma$ outside $D$ and the curve $\tilde\gamma$.
	See Figure~\ref{fig: curve_con} for an illustration.
	Clearly, all conditions of \Cref{obs: curve_manipulation} are satisfied.
\end{proof}

\begin{figure}[h]
	\centering
	\subfigure[Before: Curves of $\Gamma$ are shown in distinct colors. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
	\hspace{1pt}
	\subfigure[After: Curves of $\set{\tilde\gamma\mid \gamma\in \Gamma}$ are shown in dash lines.]{
		\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
	\caption{An illustration of the proof of \Cref{obs: curve_manipulation}.}\label{fig: curve_con}
\end{figure}

We now use \Cref{obs: curve_manipulation} to prove \Cref{thm: new nudging}.

Denote $G'=G\setminus C$ and denote $\hat \qset=\qset\cup \qset'$.
For each $e\in E(G')$, we let set $\Pi_{e}$ contain $\cong_{G'}(\hat \qset,e)$ curves connecting the endpoints of $e$ that are internally disjoint and lying inside an arbitrarily thin strip around the curve $\phi(e)$. We then assign, for each path $Q\in \hat \qset$ and each edge $e\in E(Q)$, a distinct curve of $\Pi_{e}$ to $Q$, so each curve in $\bigcup_{e\in E(G')}\Pi_{e}$ is assigned to exactly one path of $Q$. 
For each $e\in \delta_G(C)$, let $\zeta_Q$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(G')}\Pi_{e}$ that are assigned to $Q$, so $\zeta_Q$ connects $\phi(s_Q)$ to $\phi(t^*)$.
We denote $Z=\set{\zeta_Q\mid Q\in \hat \qset}$.
In fact, when we assign curves of $\bigcup_{e\in \delta_{G'}(t^*)}\Pi_{e}$ to path of $\hat\qset$, we additionally ensure that the order in which the curves of $\set{\zeta_Q\mid Q\in \hat \qset}$ enter $\phi(t^*)$ is identical to $\oset^{\guided}(\hat\qset,\oset_{t^*})$, the ordering guided by the set $\hat\qset$ of paths and the ordering $\oset_{t^*}$. Note that this can be easily achieved according the the definition of $\oset^{\guided}(\hat\qset,\oset_{t^*})$. 
%The next step of constructing the drawing $\hat{\phi}$ is dependent on whether or not $C$ is a light cluster.


We then modify the curves of $Z$ as follows.
For each vertex $v\in V(G')$, we denote by $x_v$ the point that represents the image of $v$ in $\phi$, and we let $X$ contain all points of $\set{x_v\mid v\in V(G')}$ that are crossings between curves in $Z$, so $x_{t^*}\notin X$. 
We then iteratively process all points of $X$ as follows.
Consider a point $x_v$ of $X$ and let $D_{\phi}(v)$ be a tiny $v$-disc. 
Let $Z(v)$ be the subset of all curves in $Z$ that contains $x_v$.
Let $Z'(v)$ be the set of curves we obtain by applying the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $Z(v)$ within disc $D_{\phi}(v)$. We then replace curves of $Z(v)$ in $Z$ by curves of $Z'(v)$, and continue to the next iteration. Let $\Gamma'$ be the set of curves that we obtain after processing all points of $X$ in this way.
Note that the curves of $\Gamma'$ might be non-simple,  and a pair of curves in $\Gamma'$ may cross more than once. We then remove self-loops from all curves of $\Gamma'$, and perform type-1 uncrossing (the algorithm from \Cref{thm: type-1 uncrossing}) to curves of $\Gamma'$, and finally denote by $\Gamma=\set{\gamma(Q)\mid Q\in \hat\qset}$ the set of curves we obtained. This finishes the construction of the set $\Gamma$ of curves.

From \Cref{obs: curve_manipulation} and the construction of $\Gamma$, it is easy to verify that the first and the second properties are satisfied.
We now show that $\Gamma$ satisfies the fourth property.
Since our operations at vertex-images only modify the image of curves within tiny discs around inner-vertex-images but does not change the course of any curves, and since type-1 uncrossing does not change the last segment of curves in $\Gamma'$ (and therefore does not change the ordering in which curves of $\Gamma'$ enter $\phi(t^*)$), the curves of $\Gamma$ enter $\phi(t^*)$ in the order $\oset^{\guided}(\hat\qset,\oset_{t^*})$.
We next show that $\Gamma$ satisfies the fifth property.
Note that the curves of $\Gamma$ all lie within thin strips of the image of edges of $E(\hat\qset)$ in $\phi$, and for each edge $e'\in E(G')$, the number of segments in $\Gamma$ that lie entirely within the thin strip of $\phi(e')$ is bounded by $\cong_{G'}(\hat\qset,e')$. Therefore, the number of crossings between the image of any edge $e\in E(C)$ and the curves of $\Gamma$ is bounded by the sum, over all edges $e'\in E(G')$, the number of crossings between $e$ and $e'$ in $\phi$, times $\cong_G(\hat\qset, e')$, which is in turn bounded by $\chi_{\phi}(e, G\setminus C)\cdot \cong_G(\hat\qset)$.

It remains to show that $\Gamma$ satisfies the third property, and this is the only place where we treat path sets $\qset$ and $\qset'$ differently. First, since we performed type-1 uncrossing to the set $\Gamma'$ of curves in the last step, the number of crossings between curves of $\Gamma(\qset')=\set{\gamma(Q)\mid Q\in \qset'}$ is at most $|\qset'|^2$.
%
Second, we bound the number of crossings between curves of $\Gamma(\qset)=\set{\gamma(Q)\mid Q\in \qset}$, as follows.
On the one hand, it is easy to verify that, if we denote $Z(\qset)=\set{\zeta_Q\mid Q\in \qset}$, then the number of non-vertex-image crossings between curves of $Z(\qset))$ is at most $\chi^2_{\phi}(\qset)$.
Note that
\[
\begin{split}
\chi^2_{\phi}(\qset)
\le & \sum_{e,e'\in E(G)}\chi_{\phi}(e,e')\cdot \cong_G(\qset,e)\cdot \cong_G(\qset,e')\\
\le & \sum_{e,e'\in E(G)}\chi_{\phi}(e,e')\cdot \frac{(\cong_G(\qset,e))^2+ (\cong_G(\qset,e'))^2}{2}\\
\le & \sum_{e\in E(G)}\chi_{\phi}(e)\cdot(\cong_G(\qset,e))^2.
\end{split}
\]
On the other hand, in the step where we repeatedly apply the algorithm from \Cref{obs: curve_manipulation} to the set $Z$ of curves, it is not hard to verify that, if a crossing between two curves $\gamma(Q)$ and $\gamma(Q')$ (where $Q,Q'\in \qset$) is introduced in this step, then either they share an edge, or their intersection is transversal at a common inner vertex. The number of pairs of paths in $\qset$ that share an edge is bounded by $\sum_{e\in E(G)}(\cong_G(\qset,e))^2$. The number of pairs of paths in $\qset$ whose intersection is transversal at some of their common inner vertex is bounded by $\ntcost(\qset;\Sigma)$.
Third, using similar arguments, we can show that the number of crossings between a curve of $\Gamma(\qset)$ and a curve of $\Gamma(\qset')$ is at most $$\ntcost(\qset,\qset';\Sigma)+\sum_{e\in E(G)} \cong_G(\qset,e)\cdot\cong_G(\qset',e)+
\sum_{e,e'\in E(G)}
\chi_{\phi}(e,e')\cdot \cong_G(\qset,e)\cdot\cong_G(\qset',e').$$
Altogether, they imply that $\Gamma$ satisfies the third property.
%
This completes the proof of \Cref{thm: new nudging}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of \Cref{lem: curves from non-transversal paths}}
\label{apd: Proof of curves from non-transversal paths}

We construct a feasible solution $\phi'$ of $(G',\Sigma')$ as follows.
Recall that we are given a solution $\phi$ of instance $(G,\Sigma)$. We start with drawing $\phi(G\setminus E(\pset))$, the drawing of subgraph $G\setminus E(\pset)$ induced by $\phi$. It remains to add the images of $\set{e_P\mid P\in \pset}$ to $\phi(G\setminus E(\pset))$, which we do as follows.

For each path $P\in \pset$, we denote $\gamma_P=\phi(P)$ the image of $P$ in $\phi$, so $\gamma_P$ is a curve (possibly non-simple) connecting $\phi(s)$ to $\phi(t)$.
Denote $\Gamma=\set{\gamma_P\mid P\in \pset}$. 
We iteratively modify the curves in $\Gamma$, by processing all vertices of $V(\pset)$ one-by-one as follows.
Consider a vertex $v\in V(P)$. Denote $\Gamma_v=\set{\gamma_P\mid v\in V(P)}$. We apply \Cref{obs: curve_manipulation} to curves in $\Gamma_v$ within an arbitrarily small disc $D_v$ around $\phi(v)$, and get a new set $\Gamma'_v=\set{\gamma'_P\mid \gamma_P\in \Gamma_v}$ of curves. We then replace the curves of $\Gamma_v$ in $\Gamma$ with curves of $\Gamma_v$. This completes the iteration of processing vertex $v$. 
Note that, since the paths of $\pset$ are edge-disjoint and non-transversal with respect to $\Sigma$, the curves of $\Gamma_v$ do not cross in $D_v$.
Let $\Gamma^*=\set{\gamma_P\mid P\in \pset}$ be the set of curves we get after processing all vertices of $V(P)$ in this way.

Note that curves of $\Gamma^*$ may be non-simple. We then delete self-loops of for each curve of $\Gamma^*$. We then add curves of $\Gamma^*$ to the drawing $\phi(G\setminus E(\pset))$, where for each $P\in \pset$, the curve $\gamma^*_{P}$ is designated as the image of $e_P$.
Let $\phi'$ be the resulting drawing. It is easy to verify that the $\phi'$ is a feasible solution of the instance $(G',E')$.
Since we have not created additional crossings in the process of obtaining the curves of $\Gamma^*$, any crossing in $\phi'$ is also a crossing in $\phi$. We then conclude that $\cro(\phi')\le \cro(\phi)$.
\fi








%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of \Cref{claim: remove congestion}}
\label{apd: Proof of remove congestion}

Denote $k=|\pset|$.
We define an $s$-$t$ flow network $H$, as follows. We start with the graph $G$, and set the capacity of every edge in $G$ to be $1$. Add a source vertex $s$, and a destination vertex $t$, and, for every vertex $v\in V(G)$, add an edge $(s,v)$ of capacity $n_S(v)$, and an edge $(t,v)$ of capacity $n_T(v)$ to $H$. Notice that the set $\pset$ of paths naturally defines a valid $s$-$t$ flow of value $k/\rho$ in this network, where we send $1/\rho$ flow units on each path in $\pset$. From the integrality of flow, since all edge capacities in $H$ are integral, there is an integral $s$-$t$ flow in $H$, of value at least $k/\rho$. This integral flow immediately defines the desired collection $\pset'$ of edge-disjoint paths in graph $G$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\iffalse
\subsection{Proof of \Cref{lem: opt of contracted instance}}
\label{apd: Proof of opt of contracted instance}

\znote{To Complete.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi






%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse{previous type-2 unucrossing}



\subsection{Proof of Theorem~\ref{thm: type-2 uncrossing}}
\label{apd: type-2 uncrossing}

%\mynote{again, you assume simple curves?}

We use similar arguments as in the proof of Theorem~\ref{thm: type-1 uncrossing}.

Let $Z$ be the set of points that lie on at least two curves of $\Gamma$. For each point $z\in Z$, let $D_z$ be an arbitrarily small disc around point $z$, such that, if $z$ lies on curves $\gamma_{1},\ldots,\gamma_{k}$, then
\begin{itemize}
	\item the disc $D_z$ is disjoint from all curves of $\Gamma\setminus\set{\gamma_{1},\ldots,\gamma_{k}}$;
	\item for each $1\le i\le k$, the intersection between disc $D_z$ and curve $\gamma_i$ is a simple subcurve of $\gamma_i$; and
	\item for each $1\le i\le k$, the curve $\gamma_i$ intersects the boundary of $D_z$ at two distinct points.
\end{itemize}
Moreover, all discs in $\set{D_z}_{z\in Z}$ are mutually disjoint.

We now process the sets $\Gamma_1,\ldots,\Gamma_r$ of curves one-by-one. 
We will describe the algorithm for processing the set $\Gamma_1$, and the algorithms for processing sets $\Gamma_2,\ldots,\Gamma_r$ are the same.
The algorithm for processing the set $\Gamma_1$ is iterative.
Throughout, we maintain (i) a set $\hat{\Gamma}_1$ of curves, that is initialized to be $\Gamma_1$; and (ii) a set $\hat Z$ of points that lie in at least two curves of $\hat\Gamma_1\cup (\Gamma\setminus \Gamma_1)$, that is initialized to be $Z$.
The algorithm continues to be executed as long as there is still a point that lies on at least two curves of $\hat \Gamma_1$ and is an inner point of each of these curves.
We now describe an iteration.
We first arbitrarily pick such a point $z$, and let $\gamma_{1},\ldots,\gamma_{k}$ be the curves that contains $z$.
For each $1\le i\le k$, we denote by $s_i$ the first endpoint of $\gamma_i$ and by $t_i$ the last endpoint of $\gamma_i$, and denote by $s'_i, t'_i$ the intersections between curve $\gamma_i$ and the boundary of disc $D_z$, such that the points $s_i,s'_i,z,t'_i,t_i$ appear on the directed curve $\gamma_i$ in this order.


\begin{figure}[h]
	\centering
	\subfigure[Before: Curves $\gamma_1,\gamma_2,\gamma_3,\gamma_4,\gamma_5$ are shown in red, yellow, pink, black and green respectively. The points of $S'\cup T'$  appear on the boundary of disc $D_z$.]{\scalebox{0.33}{\includegraphics[scale=1.0]{figs/type_2_uncross_proof_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.1cm}
	\subfigure[The set $\set{\eta^i_z\mid 1\le i\le k}$ of curves connecting distinct vertices of $S'$ to distinct vertices of $T'$ are shown in dash purple lines.]{
		\scalebox{0.33}{\includegraphics[scale=1.0]{figs/type_2_uncross_proof_2.jpg}}}
	\hspace{0.1cm}
	\subfigure[After: New curves $\hat\gamma_1,\hat\gamma_2,\hat\gamma_3,\hat\gamma_4,\hat\gamma_5$ are shown in red, yellow, pink, black and green respectively. Point $z$ no longer lies in any of these curves.]{
		\scalebox{0.33}{\includegraphics[scale=1.0]{figs/type_2_uncross_proof_3.jpg}}}
	\caption{An illustration of an iteration in type-1 uncrossing.}\label{fig: type_2_uncross_proof}
\end{figure}

We now modify the curves $\gamma_1,\ldots,\gamma_k$ as follows. Denote $S'=\set{s'_i\mid 1\le i\le k}$ and $T'=\set{t'_i\mid 1\le i\le k}$. We first use the algorithm in~\Cref{obs:rerouting_matching_cong} to compute a set $\set{\eta^{i}_z\mid 1\le i\le k}$ of curves, such that
\begin{itemize}
	\item for each $1\le i\le k$, the curve $\eta_z^i$ connects $s'_i$ to a distinct point $t'_{x_i}$ of $T'$; 
	\item for each $1\le i\le k$, the curve $\eta_z^i$  lies entirely in the disc $D_z$; and 
	\item the curves in $\set{\eta^{i}_z\mid 1\le i\le k}$ are mutually disjoint.
\end{itemize}
Note that the algorithm in~\Cref{obs:rerouting_matching_cong} only gives us a matching between points in $S'$ and points $T'$, but it can be easily tranformed into a set of curves satisfying the above properties.
See Figure~\ref{fig: type_2_uncross_proof} for an illustration.
For each $1\le i\le k$, we denote by $\gamma^s_i$ the subcurve of $\gamma_i$ between $s_i$ and $s'_i$, and by $\gamma^t_i$ the subcurve of $\gamma_i$ between $t'_i$ and $t_i$. 
We then define, for each $1\le i\le k$, a new curve $\hat \gamma_i$ to be the sequential concatenation of curves $\gamma^s_i, \eta^i_z, \gamma^t_{x_i}$. 
See Figure~\ref{fig: type_2_uncross_proof} for an illustration.
We then replace the curves $\gamma_1,\ldots,\gamma_k$ in $\hat\Gamma_1$ with the new curves $\hat\gamma_1,\ldots,\hat\gamma_k$. This completes the description of an iteration.
Let $\Gamma'_1$ be the set of curves that we obtain at the end of the algorithm, and let $Z'$ be set of points that lie on at least two curves of $\Gamma'_1\cup (\Gamma\setminus \Gamma_1)$.

It is easy to verify that, in the iteration described above, the multiset of the first endpoints of new curves $\hat\gamma_1,\ldots,\hat\gamma_k$ is identical to that of the original curves $\gamma_1,\ldots,\gamma_k$ and similarly the multiset of the last endpoints of new curves $\hat\gamma_1,\ldots,\hat\gamma_k$ is identical to that of the original curves $\gamma_1,\ldots,\gamma_k$.
Therefore, $S(\Gamma'_1)=S(\Gamma_1)$ and $T(\Gamma'_1)=T(\Gamma_1)$. 
It is also easy to verify that the point $z$ no longer lies in any of the new curves $\hat\gamma_1,\ldots,\hat\gamma_k$, while other points in $\hat Z$ remains in $\hat Z$, and there are no new points added to $\hat Z$.
So in each iteration, one point is removed from $\hat Z$, and therefore the algorithm of processing $\Gamma_1$ will terminate in $O(\chi(\Gamma_1))$ rounds.
Moreover, from the terminating criterion of the algorithm, the curves in the resulting set $\Gamma_1'$ no longer cross with each other. 

For each $1\le i\le r$, let $\Gamma'_i$ be the set of curves that we obtain from processing the set $\Gamma_i$ of curves using the same algorithm.
We now show that the sets $\Gamma_1,\ldots,\Gamma_r$ satisfy the conditions in \Cref{thm: type-2 uncrossing}.
%, for each $1\le i\le r$, and let $\Gamma'=\bigcup_{1\le i\le r}\Gamma_i$.
First, from the above discussion, for each $1\le i\le r$, $S(\Gamma'_i)=S(\Gamma_i)$ and $T(\Gamma'_i)=T(\Gamma_i)$.
Second, if we denote by $Z'$ the set of points that lie in at least two curves of $\Gamma'=\Gamma_0\cup(\bigcup_{1\le i\le r}\Gamma'_i)$, then clearly $Z'\subseteq Z$, and for each $1\le i\le r$, $Z'$ does not contain a point lying in at least two curves of $\Gamma'_i$.
It follows that for each $1\le i\le r$, curves in $\Gamma_i$ do not cross each other; for every curve $\gamma\in \Gamma_0$, $\chi(\gamma,\Gamma'\setminus \Gamma_0)\le \chi(\gamma,\Gamma\setminus \Gamma_0)$; and 
$\chi(\Gamma')\le \chi(\Gamma)$.
Last, it is easy to verify from the algorithm that, 
if a point is an endpoint of a curve in $\Gamma'$, then it may not be an inner point of any other curve in $\Gamma'$.
Moreover, if a point of $Z$ lie in more than 2 curves in $\Gamma'$, then it has to be an endpoint of every curve that contains it. 
Therefore, curves in $\Gamma'$ are in general position.
This completes the proof of \Cref{thm: type-2 uncrossing}.

{previous type-2 uncrossing}
\fi







%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of Corollary~\ref{cor: approx_balanced_cut}}

\label{apd: Proof of approx_balanced_cut}

%\mynote{please get rid of $\Gamma$}
Denote $G=(V,E)$.
Let $H$ be the graph obtained from $G$ by subdividing each edge $e$ of $G$ with a new vertex $x_e$. 
Note that, even if $G$ is a multigraph, $H$ is a simple graph.
%Namely, every edge $e=(u,u')$ of $G$ is replaced by a path $(u,u_1,\ldots,u_{\ell-1},u')$. 
%For each edge $e$ of $G$, we denote by $\Gamma_e$ the set of vertices in $H$ that are used to subdivide the edge $e$ in $G$.
We denote $\Upsilon=\set{x_e\mid e\in E}$, so $V(H)=V\cup \Upsilon$.
Let $(S,T)$ be a cut in $G$. We say that a cut $(S',T')$ in $H$ \emph{extends $(S,T)$}, iff $S\subseteq S'$, $T\subseteq T'$, $x_e\in S'$ for all edges $e\in E_G(S)$, and $x_e\in T'$ for all edges $e\in E_G(T)$.
We use the following observation.
\begin{observation}
\label{obs: balanced_vertex_edge_cut}
Let $(S,T)$ be a cut in $G$ and $(S',T')$ a cut in $H$ that extends $(S,T)$, then
\begin{itemize}
\item $|E_G(S,T)|=|E_H(S',T')|$;
\item if $(S,T)$ is a $\theta$-edge-balanced cut in $G$ for some real number $0<\theta<1/2$, then the cut $(S',T')$ is a $(\theta/3)$-vertex-balanced cut in $H$; and
\item if $(S',T')$ is a $\theta$-vertex-balanced cut in $H$ for some real number $0<\theta<1/2$, then the cut $(S,T)$ is a $(\theta/2)$-edge-balanced cut in $G$.
\end{itemize}
\end{observation}
\begin{proof}
From the construction of $H$, since the cut $(S',T')$ extends $(S,T)$, if an edge $e'$ belong to $E_H(S',T')$, then  one endpoint of $e'$ has to be $x_e$ for some $e\in E_G(S,T)$, and the other endpoint is an endpoint of $e$ in either $S$ or $T$, depending on whether the vertex $x_e$ belongs to $S'$ or $T'$.
On the other hand, for each edge $e\in E_G(S,T)$ with $e=(u,u')$ and $u\in S, u'\in T$, consider the edges $(u,x_e)$ and $(u',x_e)$ of $H$. It is easy to see that, if the cut $(S',T')$ extends $(S,T)$, then exactly one of edges $(u,x_e), (u',x_e)$ belongs to $E_H(S',T')$. Altogether, $|E_G(S,T)|=|E_H(S',T')|$.

If $(S,T)$ is a $\theta$-edge-balanced cut in $G$, namely $|E_G(S)|,|E_G(T)|\ge \theta\cdot|E|$, note that $|V(S')|\ge |E_G(S)|+|S|$, and $|V(H)|=|E|+|V|$. 
Since $G$ is connected, $|E|\ge |V|-1\ge |V|/2$, so $|E|\ge (|E|+|V|)/3$. 
Therefore, 
$$|V(S')|\ge |E_G(S)|\ge \theta\cdot |E|\ge \theta\cdot (|E|+|V|)/3\ge 
(\theta/3)\cdot|V(H)|.$$ 
Similarly, $|V(T')|\ge(\theta/3)\cdot|V(H)|$, and therefore $(S',T')$ is a $(\theta/3)$-vertex-balanced cut in $H$.

If $(S',T')$ is a $\theta$-vertex-balanced cut in $G$, 
namely $|S'|,|T'|\ge \theta\cdot |V(H)|$,
then 
\[
|E_G(S)|\ge |S'|/2 \ge (\theta/2)\cdot|V(H)| \ge (\theta/2)\cdot|E|.
\] Similarly, $|E_G(T)|\ge (\theta/2)\cdot|E|$, and therefore $(S,T)$ is a $(\theta/2)$-edge-balanced cut in $G$.
\end{proof}

We now use Lemma~\ref{obs: balanced_vertex_edge_cut} to prove Corollary~\ref{cor: approx_balanced_cut}. Recall that we are given a constant $\hat c$ with $0<\hat c< 1/2$. 
We first apply Theorem~\ref{thm: ARV} with parameter $c=\hat c/3$ and obtain a constant $c'$ with $0<c'<c$, and an algorithm $\aset^{c,c'}_{\text{vertex}}$ that, given any connected simple graph $\tilde G$, computes a $c'$-vertex-balanced cut of $\tilde G$, whose size is at most $\alphasc(n)$ times the size of a minimum $c$-vertex-balanced cut of $\tilde G$.

We set the constant $\hat c'=c'/4$, and construct an algorithm $\aset^{\hat c,\hat c'}_{\text{edge}}$ that, given any connected multigraph $G$, computes a $\hat c'$-edge-balanced cut of $G$, whose size is at most $O(\alphasc(n))$ times the size of a minimum $\hat c$-edge-balanced cut of $G$, as follows.
Let $G$ be the input connected multigraph. We first construct the graph $H$ by subdividing each edge of $G$ as described above. Note that $H$ is a simple graph. We then apply the algorithm $\aset^{c,c'}_{\text{vertex}}$ to graph $H$ and obtain a $c'$-vertex-balanced cut $(A,B)$ of $H$, such that $|E_H(A,B)|$ is at most $O(\alphasc(n)\cdot X)$, where $X$ is the size of a minimum $c$-vertex-balanced cut in $H$. 
We will process the cut $(A,B)$ of $H$ to obtain a cut $(A^*,B^*)$ of $G$, in several steps. 


\paragraph{Step 1.}
We start with some definitions.
Given a cut $(\hat A,\hat B)$ of $H$, we say that a vertex $x_e\in \Upsilon$ is \emph{$\hat A$-isolated} iff $x_e\in \hat A$, and if we denote by $u,v$ the endpoints of $e$ as an edge in $E$, then $u,v$ belong to $\hat B$ as vertices of $V(H)$.
Similarly, we say that a vertex $x_e\in \Upsilon$ is \emph{$\hat B$-isolated} iff $x_e\in \hat B$, and if $e=(u,v)$, then $u,v\in \hat A$.
In the first step, we will process the cut $(A,B)$ given by the algorithm $\aset^{c,c'}_{\text{vertex}}$ and obtain another cut $(A_1,B_1)$ of $H$, such that there are either only $A_1$-isolated vertices or only $B_1$-isolated vertices, but not both. Specifically, we start with the cut $(A,B)$, and while there is a $A$-isolated vertex $u$ and a $B$-isolated vertex $u'$, we move $u$ from $A$ to $B$ and move $u'$ from $B$ to $A$. 
It is clear that, after such a round of ``exchanging isolated vertices'', the number of $A$-isolated vertices and the number of $B$-isolated vertices are both decreased by $1$, the sizes of $A$ and $B$ do not change, and the number of edges in the cut $(A,B)$ is decreased by $4$. Therefore, this step will terminate after $O(n^2)$ rounds.
Let $(A_1, B_1)$ be the cut obtained at the end of this step, then it is clear that there are either only $A_1$-isolated vertices or only $B_1$-isolated vertices.
It is also clear that $|E(A_1,B_1)|\le |E(A,B)|$, and $|A_1|=|A|$ and $|B_1|=|B|$. Therefore, $|A_1|,|B_1|\ge c'\cdot|V(H)|$.
We assume without loss of generality that there are only $B_1$-isolated vertices. 


\paragraph{Step 2.}
%If the number of $B_1$-isolated vertices is at most $|B_1|/2$, then in this step we simply move all $B_1$-isolated vertices from $B_1$ to $A_1$. We assume from now on that the number of $B_1$-isolated vertices is at least $|B_1|/2$.
We start with some definitions. Given a cut $(\hat A,\hat B)$ of $H$ such that there is no $\hat A$-isolated vertices, we say that a vertex $u\in V$ is $\hat A$-dominated, iff $u\in \hat A$, and among the edges $e_1,\ldots,e_d$ of $\delta_G(u)$ (where $d=\deg_G(u)$), at least $(c'/2)$-fraction of the corresponding vertices $x_{e_1},\ldots,x_{e_d}$ are $\hat B$-isolated. We use the following claim.
\begin{claim}
\label{clm: dominated_vertex}
If the number of $B_1$-isolated vertices is at least $(c'/2)\cdot |E|$, then there is at least one $A_1$-dominated vertex.
\end{claim}
\begin{proof}
Assume the constrast that the number of $B_1$-isolated vertices is less than $(c'/2)\cdot V(H)$, while there is no $A_1$-dominated vertex. Then we have
\[
\begin{split}
\big|\set{e\mid x_e \text{ is $B_1$-dominated}}\big|
& =  \frac{1}{2}\cdot \sum_{v\in V}\big|\set{e\in \delta_G(v)\mid x_e \text{ is $B_1$-dominated}}\big|\\
& <  \frac{1}{2}\cdot \sum_{v\in V}\frac{c'}{2}\cdot |\delta_G(v)| =\frac{c'}{4}\cdot 2\cdot|E|=\frac{c'}{2}\cdot |E|,
\end{split}
\]
a contradiction to the fact that number of $B_1$-isolated vertices is at least $(c'/2)\cdot |E|$.
\end{proof}

We now describe the algorithm in this step. We start with the cut $(A_1,B_1)$. Recall that we have assumed that there are only $B_1$-isolated vertices. 
We proceed in iterations, and terminate as long as the number of $B_1$-isolated vertices is at most $|B_1|/2$.
While the number of $B_1$-isolated vertices is at least $|B_1|/2$, since $|B_1|\ge c'\cdot |V(H)|\ge c'\cdot |E|$, the number of $B_1$-isolated vertices is at least $(c'/2)\cdot |E|$. From Claim~\ref{clm: dominated_vertex}, there is at least one $A_1$-dominated vertex. We then find an $A_1$-dominated vertex $u$ (by examining each vertex of $V$), so $u\in A_1$. Denote $d=\deg_G(u)$ and $\delta_G(u)=\set{e_1,\ldots,e_d}$, and assume that the vertex $x_{e_1}$ is a $B_1$-isolated vertex. 
We then move $u$ from $A_1$ to $B_1$ and move $x_{e_1}$ from $B_1$ to $A_1$. This completes the description of an iteration. Note that, after each iteration of processing the $A_1$-dominated vertex $u$, the size of $A_1$ and $B_1$ remain the same, the number of $B_1$-isolated vertices is decreased by at least $(c'/2)\cdot d$, and the size of $|E(A_1,B_1)|$ is increased by at most $(1-c'/2)\cdot d$.
Therefore, the algorithm in this step will terminate in $O(n^2)$ rounds.
Let $(A_2,B_2)$ be the cut obtained at the end of this step. It is easy to see that $|A|=|A_1|=|A_2|$, $|B|=|B_1|=|B_2|$, the number of $B_2$-isolated vertices is at least $|B_2|/2$, and
$|E(A_2,B_2)|\le \frac{1-c'/2}{c'/2}\cdot |E(A_1,B_1)|$.

We define the cut $(A_3,B_3)$ from the cut $(A_2,B_2)$ by moving all $B_2$-isolated vertices from $B_2$ to $A_2$. Then $|A_3|\ge |A_2|$, $|B_3|\ge |B_2|/2$ and $|E(A_3,B_3)|\le |E(A_2,B_2)|$. Lastly we define $A^*=A_3\cap V$ and $B^*=B_3\cap V$, so $(A^*, B^*)$ is a cut of $G$ with no $A^*$-isolated vertices or $B^*$-isolated vertices, and therefore the cut $(A_3,B_3)$ in $H$ extends $(A^*,B^*)$.
We then let the cut $(A^*,B^*)$ be the output of our algorithm $\aset_{\text{edge}}^{\hat c,\hat c'}$. This completes the description of the algorithm.

It remains to prove the correctness of the algorithm. On one hand, since $(A,B)$ is a $c'$-vertex balanced cut of $H$, $|A_3|\ge |A_2|=|A|\ge c'\cdot |V(H)|$ and $|B_3|\ge |B_2|/2=|B|/2\ge (c'/2)\cdot |V(H)|$. Therefore $(A_3,B_3)$ is a $(c'/2)$-vertex balanced cut of $H$. From 
Observation~\ref{obs: balanced_vertex_edge_cut}, $(A^*, B^*)$ is a $(c'/4)$-edge-balanced cut in $G$. On the other hand, let $(\tilde A,\tilde B)$ be a minimum $\hat c$-edge-balanced cut in $G$, and denote its size by $Y$. Then from Observation~\ref{obs: balanced_vertex_edge_cut}, any cut in $H$ that extends $(\tilde A,\tilde B)$ is a $(\hat c/3)$-vertex-balanced cut in $H$, so $Y\ge X$ (recall that $\hat c/3=c$). Since $c'$ is a constant,
\[
|E(A^*,B^*)|=|E(A_3,B_3)|\le |E(A_2,B_2)|\le  \frac{1-c'/2}{c'/2}\cdot |E(A,B)|= O(\alphasc(n) \cdot X)\le  O(\alphasc(n) \cdot Y),
\]
and it follows that our cut $(A^*,B^*)$ has size at most $O(\alphasc(n))$ times the size of a minimum $\hat c$-edge-balanced cut of $G$.
This completes the proof of Corollary~\ref{cor: approx_balanced_cut}.













\iffalse
\begin{observation}
For any constant $c$, there is a minimum $c$-vertex-balanced cut that is a regular cut.
\end{observation}
\begin{proof}
Let $(A,B)$ be a minimum $c$-vertex-balanced cut. We construct another cut $(\hat A, \hat B)$ as follows. Let $V_A=A\cap V, V_B=A\cap V$.
We first add vertices of $V_A$ to $\hat A$ and add vertices of $V_B$ to $\hat B$. 
For each edge $e\in E_G(V_A)$, we add all vertices of $\Gamma_e$ to $\hat A$. Similarly, for each edge $e\in E_G(V_B)$, we add all vertices of $\Gamma_e$ to $\hat B$. Next, for each edge $e=(u,u')$ with $u\in A$ and $u'\in B$, denote $\gamma_e=\set{u_1,\ldots,u_{\ell-1}}$, and we add vertices $u_1,\ldots,u_{|\Gamma_e\cap A|}$ to $\hat A$, and the rest of $\Gamma_e$ to $\hat B$.
\end{proof}

We now set $\hat c=$ and $\hat c'=$, and use the algorithm in Theorem~\ref{thm: ARV} to compute a $\hat c$-vertex balanced cut of $H$, that we denote by $(A,B)$. From Theorem~\ref{thm: ARV}, the value of $|E(A,B)|$ is at most $O(\alphasc)$ times the size of a minimum $\hat c'$-vertex-balanced of $G$.
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of Theorem~\ref{lem:min_bal_cut}}

\label{apd: Proof of min_bal_cut}

We use the following theorem from~\cite{lipton1979separator}.

\begin{theorem}[Theorem 4 from~\cite{lipton1979separator}]
\label{thm: weighted_planar_separator}
Let $G$ be any $n$-vertex \textbf{simple} planar graph having nonnegative vertex costs summing to no more than one. Then the vertices of $G$ can be partitioned into three sets $A,B,C$, such that no edge joins a vertex in $A$ with a vertex in $B$, neither $A$ nor $B$ has total cost exceeding $2/3$, and $C$ contains no more than $\sqrt{8n}$ vertices.
\end{theorem}

Let $G=(V,E)$ be the input multigraph and let $\phi$ be an optimal drawing of $G$ in the plane.
We define a graph $G'$ in three steps as follows.
We start with graph $G$. 
In the first step, we subdivide each edge $e$ of $G$ with a new vertex $y_e$. Namely, every edge $e=(u,u')$ of $G$ is replaced by a path $(u,y_e,u')$ of length $2$, and we denote $\Upsilon=\set{y_e\mid e\in E}$.
Let $\hat G_1$ be the resulting graph after this step, so $\hat G_1$ is a simple graph and $V(\hat G_1)=V\cup \Upsilon$ and $|V(\hat G_1)|=n+|E|$. Moreover, the drawing $\phi$ of $G$ naturally induces a drawing $\hat \phi_1$ of $\hat G_1$ with $\cro(\phi)=\cro(\hat{\phi}_1)$.
We say that the edge $e=(u,u')$ in $E$ \emph{gives birth to} the edges $(u,y_e)$ and $(u',y_e)$ of $\hat G_1$.
In the second step, for every crossing in $\hat\phi_1$ caused by a pair $e,e'$ of edges of $\hat G_1$, where $e=(u,v)$ and $e'=(u',v')$, we add a new node $x_{e,e'}$ to $\hat G_1$, and replace the edges $e,e'$ with four new edges, connecting $x_{e,e'}$ to $u,u',v,v'$, respectively. 
Let $\hat G_2$ be the resulting graph after this step.
Denote $X=\set{x_{e,e'}\mid \text{there is a crossing in $\hat\phi_1$ caused by }e,e'}$, so $V(\hat G_2)=V\cup\Upsilon\cup X$ and $|V(\hat G_2)|=\optcro(G)+n+|E|$.
Clearly, $\hat G_2$ is a simple planar graph, and the drawing $\hat\phi_1$ of $\hat G_1$ naturally induces a planar drawing $\hat\phi_2$ of $\hat G_2$.
In the third step, we iteratively process every vertex $v$ of $\hat G_2$ with $\deg_{\hat G_2}(v)>4$.
Note that any vertex $v$ with $\deg_{\hat G_2}(v)>4$ has to be some vertex $v\in V$ with $\deg_G(v)=\deg_{\hat G_2}(v)>4$. 
We now describe an iteration of processing such a vertex $v$.
Denote $d=\deg_{\hat G_2}(v)$ and denote $\delta_{\hat G_2}(v)=\set{e_1,\ldots,e_d}$.
We replace the vertex $v$ with a $\deg_{\hat G_2}(v)\times \deg_{\hat G_2}(v)$-grid, that we denote by $H_v$, where the vertex appearing at the intersection of the $i$-th row and the $j$-th column is denoted by $v_{i,j}$, for each $1\le i,j\le d$. We then let, for each $1\le t\le d$, the edge $e_t$ be incident to the vertex $v_{1,t}$.
This completes the description of an iteration, and also completes the description of this step. 
Let $G'=(V',E')$ be the resulting graph after this step. 
Clearly, $G'$ is a simple planar graph, since we can obtain a planar drawing of $G'$ from the planar drawing $\hat \phi_2$ of $\hat G_2$ by replacing the image of each vertex $v$ with $\deg_{\hat G_2}(v)>4$ by the image of the grid $H_v$. 
We denote $V_{\le 4}=\set{v\in V\mid \deg_G(v)\le 4}$ and $V_{>4}=\set{v\in V\mid \deg_G(v)> 4}$, then $V'=V_{\le 4}\cup \Upsilon\cup X\cup (\bigcup_{v\in V_{>4}}V(H_v))$.
Therefore, $|V'|\le \optcro(G)+|E|+\sum_{v\in V(G)}(\deg_{G}(v))^2\le \optcro(G)+2\Delta|E|$, where $\Delta$ is the maximum vertex degree of $G$.
%Note that the vertices of $\Upsilon$ have degree $2$ in $\hat G_1$, have degree $2$ in $\hat G_2$, and therefore also belongs to $V'$.
Note that the maximum vertex degree of $G'$ is $4$, since every vertex of $\hat G_2$ with degree greater than $4$ is replaced with a grid, whose maximum vertex degree is $4$. 

 
We now assign weight $1/|\Upsilon|$ to all vertices of $\Upsilon$ in $G'$, and weight $0$ to all other vertices of $G'$. Then we apply Theorem~\ref{thm: weighted_planar_separator} to $G'$ with the above vertex weights. Let $(A,B,C)$ be the partition of $V'$ that we obtain, so $|\Upsilon\cap A|\le (2/3)\cdot |\Upsilon|$, $|\Upsilon\cap B|\le (2/3)\cdot |\Upsilon|$, and $|C|\le \sqrt{8|V'|}=\sqrt{8\cdot\optcro(G)+16\Delta\cdot |E|}$.
We now construct a cut of the original graph $G$ based on the partition $(A,B,C)$ of $V'$, as follows.

We construct a set $\tilde E$ of edges of $G$ as follows. Initially we set $\tilde E=\emptyset$. We first add, for each vertex $v\in C\cap V_{\le 4}$, all edges of $\delta_G(v)$ to $\tilde E$. Note that there are at most $4\cdot|C\cap V_{\le 4}|$ such edges.
We then add, for each vertex $y_e\in C\cap \Upsilon$ (where $e$ represents an edge of $E$), the edge $e$ to $\tilde E$. Note that there are at most $|C\cap\Upsilon|$ such edges.
Next, for each vertex $x_{e,e'}\in C\cap X$ where $e,e'$ are edges of $\hat G_1$, let $\hat e$ and $\hat e'$ be the edges of $E$ that give birth to edges $e$ and $e'$ respectively, and we add edges $\hat e,\hat e'$ to $\tilde E$. Note that there are at most $2\cdot|C\cap X|$ such edges.
Lastly, we process the vertices of $V_{> 4}$ one-by-one to complete the construction of $\tilde E$, as follows.

Consider a vertex $v\in V_{>4}$ and the $(d\times d)$-grid $H_v$, where $d=\deg_G(v)$ and we denote $\delta_G(v)=\set{e_1,\ldots,e_d}$. Recall that for each $1\le t\le d$, the edge $e_t$ is incident to the vertex $v_{1,t}$.
Denote by $V_1$ the set of vertices on the first row of $H_v$, namely $V_1=\set{v_{1,1},\ldots,v_{1,d}}$. Denote $A_1=A\cap V_1$, $B_1=B\cap V_1$, and $C_1=C\cap V_1$. If $|A_1|\le |B_1|$, then we add the edges of $\set{e_t\mid v_{1,t}\in A_1\cup C_1}$ to $\tilde E$, otherwise we add the edges of $\set{e_t\mid v_{1,t}\in B_1\cup C_1}$ to $\tilde E$. This completes the description of processing a vertex $v\in V_{>4}$, and also completes the construction of $\tilde E$. We use the following claim.
\begin{claim}
\label{clm: grid well-linked}
If $|A_1|\le |B_1|$, then $\big|\set{e_t\mid v_{1,t}\in A_1\cup C_1}\big|=|A_1|+|C_1|\le |C\cap V(H_v)|$. 
\end{claim}
\begin{proof}
Define the graph $H'_v$ to be the graph obtained from $H_v$ by deleting all vertices of $C_1$ and their incident edges.
Clearly, $|C\cap V(H_v)|=|C_1|+|C\cap V(H'_v)|$, and therefore it suffices to show that $|C\cap V(H'_v)|\ge |A_1|$.
From Theorem~\ref{thm: weighted_planar_separator}, no edge of $G'$ joins a vertex in $A$ with a vertex in $B$. Therefore, the vertices of $C\cap V(H'_v)$ forms a vertex cut in $H'_{v}$ separating vertices of $A_1$ from vertices of $B_1$. We now show that there is a set of $|A_1|$ node-disjoint paths in $H'_v$, each connecting a distinct vertex of $A_1$ to a vertex of $B_1$. Note that, from the max-flow mincut-theorem, this implies that $|C_1|\ge |A_1|$, and the claim follows.

To construct a set $\pset$ of $|A_1|$ node-disjoint paths connecting vertices of $A_1$ to vertices of $B_1$, we consider the index set $I=\set{i\mid v_{1,i}\in A_1\cup B_1}$. While there is a pair $i,i'$ of indices of $I$, such that $i<i'$, $v_{i},v_{i'}$ belongs to different sets of $A_1,B_1$, and there is no other $j\in I$ with $i<j<i'$, we define the path $P_{i,i'}$ to be the sequential concatenation of the path $(v_{1,i},v_{2,i},\ldots,v_{i',i})$, the path $(v_{i',i},v_{i',i+1},\ldots,v_{i',i'})$, and the path $(v_{i',i'},v_{i'-1,i'},\ldots,v_{1,i'})$. We then add the path $P_{i,i'}$ to $\pset$, delete $i,i'$ from $I$ and continue to the next iteration.
It is clear that, at the end of the process, $I$ does not contain any index $i$ with $v_{1,i}\in A_1$, and for each $v_{1,j}\in A_1$, there is a path $P_{j,j'}$ connecting $v_{1,j}$ to some vertex $v_{1,j'}$ of $B_1$, so $|\pset|=|A_1|$. It is also easy to verify that the paths of $\pset$ are node-disjoint. 
\end{proof}

Similarly, we can show that if $|A_1|> |B_1|$, then $\big|\set{e_t\mid v_{1,t}\in B_1\cup C_1}\big|=|B_1|+|C_1|\le |C\cap V(H_v)|$. Therefore, the number of edges that we added to $\tilde E$ when processing a vertex $v\in V_{>4}$ is at most $|C\cap V(H_v)|$.
Altogether, 
\[
|\tilde E|\le 
4\cdot|C\cap V_{\le 4}|+|C\cap\Upsilon|+2\cdot|C\cap X|+\sum_{v\in V_{>4}}|C\cap V(H_v)|\le 4\cdot |C|=\sqrt{2^{7}\cdot\optcro(G)+2^8\Delta\cdot |E|}.
\]

%Recall that $|\Upsilon\cap A|\le (2/3)\cdot|\Upsilon|$ and $|\Upsilon\cap B|\le (2/3)\cdot|\Upsilon|$.
Let $(\tilde{A},\tilde{B})$ be the cut obtained by removing the edges of $\tilde E$ from $G$, such that the corresponding vertex $y_e\in \Upsilon$ for any edge $e\in E_G(\tilde A)$ lies in $A$, and the corresponding vertex $y_e\in \Upsilon$ for any edge $e\in E_G(\tilde B)$ lies in $B$.
It is easy to see that there is no edge in $G\setminus \tilde E$ connecting a vertex of $\tilde A$ with a vertex of $\tilde B$.
It suffices to show that $|E_G(\tilde A)|\ge |E|/4$ and $|E_G(\tilde B)|\ge |E|/4$. 
We now show that $|E_G(\tilde A)|\ge |E|/4$, and the proof for $|E_G(\tilde B)|\ge |E|/4$ is symmetric.
Denote $E^A=\set{e \in E\mid y_e\in (\Upsilon\cap A)}$. It is easy to see that $(E^A\setminus \tilde E)\subseteq E_G(\tilde A)$. 
Recall that $|\Upsilon\cap B|\le (2/3)\cdot|\Upsilon|$, so $|\Upsilon\cap C|+|\Upsilon\cap A|\ge |\Upsilon|/3=|E|/3$.
Therefore, 
$$|E_G(\tilde A)|\ge |E^A\setminus \tilde E|\ge |E^A|-|\tilde E|\ge (|E|/3-|\Upsilon\cap C|)-|\tilde E|\ge |E|/3-2\sqrt{2^{7}\cdot\optcro(G)+2^8\Delta|E|}
\ge |E|/4,
$$
where the last inequality follows from $\Delta\le |E|^2/2^{100}$ and $\optcro(G)\le |E|/2^{100}$. This completes the proof of
Theorem~\ref{lem:min_bal_cut}.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\subsection{Proof of Theorem~\ref{thm: bandwidth_means_boundary_well_linked}}
\label{apd: Proof of bandwidth_means_boundary_well_linked}

We define an instance of the max-flow problem as follows.
We contract all vertices of $T_1$ into a single vertex $u_1$, and contract all vertices of $T_2$ into a single vertex $u_2$. 
Let $H$ be the resulting graph.
%The capacities on all edges of $\delta_{H'}(u_1)$ and all edges of $\delta_{H'}(u_2)$ are defined to be $1$.
The capacities on all edges of $E(H)$ are defined to be $\ceil{1/\alpha}$.
Since the capacity for each edge is integral, to complete the proof of Theorem~\ref{thm: bandwidth_means_boundary_well_linked}, it suffices to show that the maximum $u_1$-$u_2$ flow in $H$ has value $|T_1|$. 
From the max-flow min-cut theorem, it suffices to show that the minimum $u_1$-$u_2$ cut in $H$ has value at least $|T_1|$. 
Let $(A,B)$ be any in $H$ with $u_1\in A$ and $u_2\in B$. It is clear that $((A\setminus\set{u_1})\cup T_1, (B\setminus\set{u_2})\cup T_2)$ is a cut in $G$ separating vertices of $T_1$ from vertices of $T_2$, and all edges in $E((A\setminus\set{u_1})\cup T_1, (B\setminus\set{u_2})\cup T_2)$ also belong to $E_H(A,B)$ as an edge in $H$.
%Assume that $a$ edges of $\delta(u_1)$ and $b$ edges of $\delta(u_2)$ belong to the cut $E(A,B)$. Since vertices of $T$ are $\alpha$-well-linked in $G$, $|E(A,B)|\ge a+b+\alpha\cdot \ceil{1/\alpha}\cdot\min\set{|T_1|-a,|T_2|-b}\ge |T_1|$ (recall that $|T_1|=|T_2|$). 
Since vertices of $T$ are $\alpha$-well-linked in $G$, 
$|E((A\setminus\set{u_1})\cup T_1, (B\setminus\set{u_2})\cup T_2)|\ge\alpha\cdot|T_1|$, and therefore the capacity of the cut $(A,B)$ in $H$ has capacity at least $\alpha\cdot|T_1|\cdot \ceil{1/\alpha} \ge |T_1|$ (recall that $|T_1|=|T_2|$).
This completes the proof of Theorem~\ref{thm: bandwidth_means_boundary_well_linked}.

\iffalse
We subdivide every edge $e\in \delta(S)$ by a vertex $x_e$, and we denote $\Upsilon=\set{x_e\mid e\in \delta(S)}$. 
We then let $H$ be the subgraph of the resulting graph induced by vertices of $V(S)\cup \Upsilon$. Since $S$ has the $\alpha$-bandwidth property, vertices of $\Upsilon$ are $\alpha$-well-linked in $H$.

%We define an instance of the max-flow problem as follows. 
We contract all vertices of $\set{x_e\mid e\in E_1}$ into a single vertex $u_1$, and contract all vertices of $\set{x_e\mid e\in E_2}$ into a single vertex $u_2$. 
Let $H'$ be the resulting graph.
The capacities on all edges of $\delta_{H'}(u_1)$ and all edges of $\delta_{H'}(u_2)$ are defined to be $1$.
The capacities on all edges of $E(S)$ are defined to be $\ceil{1/\alpha}$.
Since the capacity for each edge is integral, to complete the proof of Theorem~\ref{thm: bandwidth_means_boundary_well_linked}, it suffices to show that the maximum $u_1$-$u_2$ flow in $H'$ has value $|E_1|$. 
From the max-flow min-cut theorem, it suffices to show that the minimum $u_1$-$u_2$ cut in $H'$ has value at least $|E_1|$. 
Consider any cut $(A,B)$ in $H'$, with $u_1\in A$ and $u_2\in B$. Assume that $a$ edges of $\delta(u_1)$ and $b$ edges of $\delta(u_2)$ belong to the cut $E(A,B)$. Since vertices of $\Upsilon$ are $\alpha$-well-linked in $H$, $|E(A,B)|\ge a+b+\alpha\cdot \ceil{1/\alpha}\cdot\min\set{|E_1|-a,|E_2|-b}\ge |E_1|$ (recall that $|E_1|=|E_2|$). This completes the proof of Theorem~\ref{thm: bandwidth_means_boundary_well_linked}.
\fi











%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of Theorem~\ref{thm:well_linked_decomposition}}
\label{apd: Proof of well_linked_decomposition}

We use the following lemma.

\begin{lemma}
\label{lem: decrease in total budget}
For any integers $a,b,c>0$ such that $c=O\big(\frac{\min\set{a,b}}{\log^{1.5}n}\big)$,
$$(a+b)\cdot\log_{3/2} (2(a+b))> (a+c)\cdot\log_{3/2} (2(a+c))+(b+c)\cdot\log_{3/2} (2(b+c)).$$
\end{lemma}
\begin{proof} Assume without loss of generality that $a\ge b$, we have
%\begin{equation}
\[\begin{split}
& \text{ }(a+b)\cdot\log_{3/2} (2(a+b))- (a+c)\cdot\log_{3/2} (2(a+c))-(b+c)\cdot\log_{3/2} (2(b+c))\\
\ge & \text{ } (a+b)\cdot\log_{3/2} (2(a+b))- (a+c)\cdot\log_{3/2} (2(a+b))-(b+c)\cdot\log_{3/2} (2(b+c))\\
= & \text{ } (b-c)\cdot\log_{3/2} (2(a+b))-(b+c)\cdot\log_{3/2} (2(b+c))\\
= & \text{ } (b-c)\cdot\bigg(\log_{3/2} (2(a+b))-(1+\frac{2c}{b-c})\cdot\log_{3/2} (2(b+c))\bigg)\\
= & \text{ } (b-c)\cdot\bigg(\log_{3/2} (2(b+c))+1-(1+\frac{2c}{b-c})\cdot\log_{3/2} (2(b+c))\bigg)\\
= & \text{ } (b-c)\cdot\bigg(\log_{3/2} (2(b+c))+1-(1+\frac{2}{\log^{1.5} n})\cdot\log_{3/2} (2(b+c))\bigg)\\
= & \text{ } (b-c)\cdot\bigg(1-\frac{\log_{3/2} (2(b+c))}{\log^{1.5} n}\bigg)> 0
\end{split}\]
%\end{equation}
\end{proof}

We decompose the cluster $S$ into small clusters and compute routing paths from the boundary edges of these small clusters to the boundary of $S$ as follows. Throughout, we maintain (i) a set $\hat\rset$ of sub-clusters of $S$, that is initialized to be $\hat\rset=\set{S}$; and (ii) for each edge $e\in E(S)\cup \delta_G(S)$, a real number $b(e)$ called the \emph{budget} of edge $e$, that is defined as follows. If $e$ is incident to a vertex $v\in V(S)$ such that $|\delta(v)\cap \delta(S)|\ge 0.9\cdot|\delta(S)|$, then the budget of $e$ is defined to be $1$ and will stay unchanged throughout the algorithm. If $e$ is not incident to such a vertex, then
\begin{itemize}
\item if $e\in \Eout(\hat{\rset})$, then $b(e)=\alpha\cdot\bigg(\log_{3/2}(2|\delta_G(R)|)+\log_{3/2}(2|\delta_G(R')|)\bigg)$, where $R,R'$ are the two clusters of $\hat \rset$ that contain an endpoint of $e$; 
\item if $e\in \delta_G(S)$, then $b(e)=\alpha\cdot\log_{3/2}(2|\delta_G(R)|)$, where $R$ is the unique cluster of $\hat \rset$ that contains an endpoint of $e$; and
\item if $e\notin (\Eout(\hat{\rset})\cup \delta_G(S))$, then $b(e)=0$.
\end{itemize}
Denote $z=|\delta_G(S)|$, so if there is no vertex $v\in V(S)$ such that $|\delta(v)\cap \delta(S)|\ge 0.9\cdot|\delta(S)|$, then initially the total budget on all edges is $\alpha\cdot z\cdot\log_{3/2}(2z)$, otherwise the total initial budget is $|\delta(v)|+ \alpha(|\delta(S)|-|\delta(v)|)\cdot \log_{3/2}(2(|\delta(S)|-|\delta(v)|))$.
The algorithm proceeds in iterations, and will be terminated if the following two conditions are satisfied: (i) all clusters of $\hat\rset$ have the $\alpha$-bandwidth property; and (ii) for each cluster $R\in \hat \rset$, we have computed a set $\pset(R)$ of paths routing edges of $\delta_G(R)$ to edges of $\delta_G(S)$ as required in \Cref{thm:well_linked_decomposition}.

We now describe the execution of an iteration. Assume first that $\hat \rset$ contains a cluster that does not have the $\alpha$-bandwidth property. Let $R$ be such a cluster.
Consider the graph $R^+$ (see \Cref{def: Graph C^+}). We apply the algorithm  \algsc to graph $R^+$ and terminal set $T(R)$, to obtain an $\alphasc(m)$-approximate sparsest cut $(X,Y)$ in graph $R^+$ with respect to the set $T(R)$ of terminals.
Since $R$ does not have the $\alpha$-bandwidth property, $|E(X,Y)|\le \alpha\cdot \alphasc(m)\cdot \min\set{|X\cap T(R)|,|Y\cap T(R)}$.
Denote $X'=X\setminus T(R)$ and $Y'=Y\setminus T(R)$, so $(X',Y')$ is a partition of $R$. We then replace the cluster $R$ in $\hat \rset$ with clusters $X',Y'$ and continue to the next iteration.
We now show that in this case, the total budget of all edges decrease after this iteration. Denote $z_{X'}=|\delta_G(X')|$, $z_{Y'}=|\delta_G(Y')|$ and $z'=|E(X,Y)|$. Assume first that no vertex $v$ of $R$ satisfies that $|\delta(v)\cap \delta(S)|\ge 0.9\cdot|\delta(S)|$.
In this case, the decrease in budget of all edges of $\delta_G(R)\cap \delta_G(X')$ is $\alpha z_{X'}\cdot(\log_{3/2}(2(z_{X'}+z_{Y'}))-\log_{3/2}(2(z_{X'}+z')))$.
Similarly, the decrease in budget of all edges of $\delta_G(R)\cap \delta_G(Y')$ is $\alpha z_{Y'}\cdot(\log_{3/2}(2(z_{X'}+z_{Y'}))-\log_{3/2}(2(z_{Y'}+z')))$.
On the other hand, the increase in budget of all edges of $E(X,Y)$ is $\alpha\cdot z'\cdot (\log_{3/2}(2(z_{X'}+z'))+\log_{3/2}(2(z_{Y'}+z')))$.
Therefore, the decrease in budget of all edges is
\[
\alpha\cdot\bigg((z_{X'}+z_{Y'})\cdot\log_{3/2}(2(z_{X'}+z_{Y'}))-(z_{X'}+z')\log_{3/2}(2(z_{X'}+z'))-(z_{Y'}+z')\log_{3/2}(2(z_{Y'}+z'))\bigg).
\]
Since $\alpha=O(\frac{1}{\log^2 m})$, $\alpha\cdot \alphasc=O(\frac{1}{\log^{1.5} m})$ and so $z'=O(\frac{\min\set{z_{X'},z_{Y'}}}{\log^{1.5} m})$.
From \Cref{lem: decrease in total budget}, the above value is positive, so the total budget decrease after this iteration.
Assume now that there exists a vertex $v\in V(R)$ satisfies that $|\delta(v)\cap \delta(S)|\ge 0.9\cdot|\delta(S)|$. Clearly, there can be at most one such vertex. Assume without loss of generality that $v\in X'$, then since $z'=O(\frac{\min\set{z_{X'},z_{Y'}}}{\log^{1.5} m})$, the total budget of all new edges of $E(X,Y)$ is at most $2z'\cdot \log (2m)$, which is smaller than the decrease of total budget of all edges in $\delta_G(Y')$. Altogether, total budget decreases after this iteration.


Assume now that $\hat \rset$ contains a cluster $R$ that does not yet have the set $\pset(R)$ of paths routing edges of $\delta_G(R)$ to edges of $\delta_G(S)$ as required in \Cref{thm:well_linked_decomposition}.
Let graph $G'$ be obtained from $G$ by first contracting all vertices of $R$ into a single vertex $v_R$ and then contracting vertices of $V\setminus S$ into a single vertex $v^*$. Observe that $\delta_{G'}(v_R)=\delta_G(R)$ and $\delta_{G'}(v^*)=\delta_G(S)$. 
We now compute the min-cut in $G'$ separating $v_R$ from $v^*$. If the min-cut has capacity at least $|\delta_{G'}(v_R)|/100$, then from the max-flow min-cut theorem, we can efficiently find a set of $|\delta_{G'}(v_R)|$ paths connecting $v_R$ to $v^*$ in $G'$, causing congestion at most $100$ in $G'$, and this set of paths can be immediately converted to a set $\pset(R)$ of paths routing edges of $\delta_G(R)$ to edges of $\delta_G(S)$ as required in \Cref{thm:well_linked_decomposition}, causing congestion at most $100$.
Assume now that min-cut has capacity less than $|\delta_{G'}(v_R)|/100$. Let $(X,Y)$ be the min-cut where $v_R\in X$. Let $X'$ be the cluster obtained from $X$ by uncontracting the vertex $v_R$ back to the cluster $R$. We replace the cluster $R$ in $\hat{\rset}$ by cluster $X'$, and the for every other cluster $R'\in \hat \rset$ such that $R'\cap X'\ne \emptyset$ but $R'\not\subseteq X'$, we replace $R'$ by cluster $R'\setminus X'$. This completes the description of this iteration.
We now show that in this case, the total budget of all edges decrease after this iteration.

Consider the set $\hat \rset$ of clusters before this iteration. Let $\hat\rset_1\subseteq \hat \rset$ be the set of clusters $R'$ such that $R'\subseteq X'$.
Let $\hat\rset_2\subseteq \hat \rset$ be the set of clusters $R'$ such that $R'\cap X'\ne \emptyset$ but $R'\not\subseteq X'$.
First consider the cluster $R$. Denote $z_R=|\delta_G(R)|$, then at least $0.99z_R$ edges of $\delta_G(R)$ loses their budget, so the budget decrease on these edges is at least $\alpha\cdot 0.99z_R\log_{3/2}(2z_R)$.
Second consider the cluster $X'$. Since $|\delta_G(X')|\le |\delta_G(R)|/100$, so the budget increase on edges of $\delta_G(X')$ is at most $\alpha\cdot0.01z_R\log_{3/2}(0.02z_R)$.
Third, it is easy to verify that the budget increase of a cluster $R'\in \hat\rset_1$ is already counted in the budget increase on edges of $\delta_G(X')$.
Last, consider a cluster $R'\in \hat\rset_2$. We denote $R'_X=R'\cap X'$ and $R'_Y=R'\setminus R'_X$.
We denote $Z'_1=|E(R'_X,X'\setminus R'_X)|$, $Z'_2=|E(R'_Y,X'\setminus R'_X)|$, 
$Z'_3=|E(R'_Y,S\setminus (X'\cup R'_X))|$,
$Z'_4=|E(R'_X,S\setminus (X'\cup R'_X))|$,
and $Z^*=|E(R'_X,R'_Y)|$.
We denote by $z'_1,z'_2,z'_3,z'_4,z^*$ the cardinalities of these sets, and denote $z'=z'_1+z'_2+z'_3+z'_4$.
From the minimality of the cut $(X,Y)$, we get that $z'_1\ge z^*+z_4$ and $z'_3\ge z^*+z_2$. Observe that the budget of edges in $Z'_2\cup Z'_4$ are already counted in the budget increase on edges of $\delta_G(X')$. Also observe that the total budget of edges in $Z'_3$ decreases (since $z'_3+z'_2+z^*\le z'$). Moreover, the increase in budget of edges in $Z^*$ that are not counted in the budget increase on edges of $\delta_G(X')$ is $\alpha\cdot z^*\log (2(z'_3+z'_2+z^*))$, while the the decrease in budget of edges in $Z'_1$ that are not counted in the budget decrease on edges of $\delta_G(R)$ is $\alpha\cdot z'_1\log (2z')$, so the total budget change of all edges incident to $R'$ is negative. Altogether, the total budget decreases.

Therefore, we can now conclude that, when the algorithm terminates, the number of edges connecting different clusters of $\hat{\rset}$ is at most $\alpha \cdot z\cdot\log_{3/2}(2z)$, and therefore $\sum_{R\in \rset}|\delta(R)|\le |\delta(S)|\cdot\left(1+O(\alpha\cdot \log m)\right)$.
%, and moreover, if initially there is a vertex $v\in V(S)$ such that $|\delta(v)\cap \delta(S)|\geq 0.9|\delta(S)|$, then $\sum_{R\in \rset}|\delta(R)|\le|\delta(v)|+ \left(|\delta(S)|-|\delta(v)|\right )\cdot\left(1+O(\alpha\cdot \log m)\right)$. 
It is easy to verify that all other properties of \Cref{thm:well_linked_decomposition} are also satisfied.



\iffalse{the proof below does not find the routing paths}
Consider the following algorithm of decomposing the cluster $S$ with the parameter $\alpha$. Throughout, we maintain a set $\hat\rset$ of sub-clusters of $S$, that is initialized to be $\hat\rset=\set{S}$. The algorithm proceeds in iterations, and is terminated whenever all clusters of $\hat\rset$ have the $\hat\alpha$-bandwidth property. In each iteration, we find a cluster $R\in \hat\rset$ that does not have the $\alpha$-bandwidth property, compute a cut $(A,B)$ of $R$ with $|E(A,B)|\le \alpha\cdot \min\set{|\delta(A)\cap\delta(R)|,|\delta(B)\cap\delta(R)|}$, replace the cluster $R$ in $\hat\rset$ with the subgraph of $R$ induced by $A$ and the subgraph of $R$ induced by $B$, and then proceed to the next iteration.
We use the following theorem, which is a corollary of Theorem 2.8 in~\cite{chuzhoy2012routing}.

\begin{theorem}[Corollary of Theorem 2.8 in \cite{chuzhoy2012routing}]
	Assume $\alpha<1/(48\log n)$ and let $\hat\rset$ be the partition of $S$ produced by the above algorithm, then $\sum_{R\in \rset}|\delta(R)|\le |\delta(S)|\cdot(1+32\alpha\log n)$.
\end{theorem}

However, the above algorithm is not efficient, since it is NP-hard to determine if a cluster $R$ has the $\alpha$-bandwidth property.
We modify the above algorithm as follows. When checking if a cluster $R$ has the $\alpha$-bandwidth property, we set up an instance of the sparsest cut problem on a graph $H_R$, that is obtained as follows. We subdivide each edge $e\in \delta(R)$ by a vertex $x_e$, and let $H$ be the subgraph of the resulting graph induced by $V(R)\cup \set{x_e\mid e\in \delta(R)}$. We then compute the sparsest cut in $H_R$, with the set $\set{x_e\mid e\in \delta(R)}$ of terminals, using the algorithm \algsc.
If the sparsity of the cut that we obtain is greater than $\alphasc(n)\cdot\alpha$, then from the algorithm \algsc, the cluster $R$ has the bandwidth property. Otherwise, we proceed as if we obtain an $\alpha$-sparse cut. Namely, if $(A,B)$ is the sparsest cut we get from \algsc, then we replace the cluster $R$ in $\hat\rset$ with the subgraph of $R$ induced by $A$ and the subgraph of $R$ induced by $B$, and then proceed to the next iteration.

Since the algorithm \algsc is efficient, our modified algorithm is efficient. 
Let $\rset$ be the resulting set of clusters of $S$.
We now show that the set $\rset$ satisfies the properties of Theorem~\ref{thm:well_linked_decomposition}.
It is immediate from the algorithm that the vertex sets $\set{V(R)}_{R\in \rset}$ partitions $V(S)$, and each cluster $R\in \rset$ has the $\alpha$-bandwidth property. Since $\alpha<1/(48\log^2n)$, $\alphasc(n)\cdot\alpha<1$, so every time in the algorithm when a cluster $R$ is decomposed into two smaller clusters $R'$ and $R''$, $|\delta(R)|>|\delta(R')|$ and $|\delta(R)|>|\delta(R'')|$. Therefore, for each $R\in \rset$, $|\delta(R)|\le |\delta(S)|$. The last property follows from the proof of Theorem 2.8 in \cite{chuzhoy2012routing}, and the fact that we only decompose a cluster $R\in \hat \rset$ when the sparsity of the cut that we obtained is below $\alpha\cdot\alphasc(n)$.
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of \Cref{lem: routing path extension}}
\label{apd: Proof of routing path extension}

Denote $z=\ceil{\frac{|T|}{|T'|}}$. We arbitrarily partition the vertices of $T\setminus T'$ into $(z-1)$ subsets $T_1,\ldots,T_{z-1}$ of cardinality at most $|T'|$ each.  
%For convenience, rename $T'$ by $T_0$.
Consider some index $1\leq i\leq z-1$. Since vertices of $T$ are $\alpha$-well-linked in $G$, using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\jset'_i$ of paths in graph $G$, routing vertices of $T_i$ to vertices of $T'$, such that $\cong_G(\jset'_i)\le \ceil{1/\alpha}$, and each vertex of $T'\cup T_i$ is the endpoint of at most one path in $\jset'_i$. 
By concatenating the paths in $\jset'_i$ with paths in $\pset'$, we obtain a collection $\jset_i$ of paths in graph $G$ routing vertices of $T_i$ to $x$, that cause edge-congestion $\ceil{1/\alpha}$. 
Define $\pset=\pset'\cup(\bigcup_{i=1}^{z-1}\jset_i)$.
It is clear that the paths in $\pset$ route the vertices of $T$ to $x$.
Moreover, for every edge $e\in E(G)$,
\[
\begin{split}
\cong_G(\pset,e) & \le
\cong_G(\pset',e)+\sum_{1\le i\le z-1}\cong_G(\jset_i,e)\\
& = z\cdot \cong_G(\pset',e)+\sum_{1\le i\le z-1}\cong_G(\jset'_i,e)\\
& \le \ceil{\frac{|T|}{|T'|}}\bigg(\cong_G(\pset',e)+\ceil{1/\alpha}\bigg).
\end{split}
\]











\input{appx-layered-wld.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of Claim~\ref{claim: embed expander}}

\label{apd: Proof of embed expander}


We use the cut-matching game of Khandekar, Rao and Vazirani~\cite{khandekar2009graph}, defined as follows. The game is played between two players, called the cut player and the matching player. The input to the game is an even integer $N$.  
The game is played in iterations. We start with a graph $W$ with vertex set $V$ of cardinality $N$ and an empty edge set. In every iteration, some edges are added to $W$. The game ends when $W$ becomes a $\half$-expander. 
The goal of the cut player is to construct a $\half$-expander in as few iterations as
possible, whereas the goal of the matching player is to prevent the construction of the expander for as long as possible. The iterations proceed as follows.  In every iteration $j$, the cut player chooses a partition $(Z_j, Z'_j)$ of $V$ with $|Z_j| = |Z'_j|$, and the
matching player chooses a perfect matching $M_j$ that matches the nodes of $Z_j$ to the nodes of $Z'_j$.  The edges of $M_j$ are then
added to $W$.  Khandekar, Rao, and Vazirani~\cite{khandekar2009graph} showed that there is a randomized efficient algorithm for the cut player (that is, an algorithm that, in every iteration $j$, given the current graph $W$, computes a partition $(Z_j,Z'_j)$ of $V$ with $|Z_j| = |Z'_j|$), that guarantees that after
$O(\log^2{N})$ iterations, with high probability, the graph $W$ is a $(1/2)$-expander, regardless of the specific matchings chosen by the matching player. 

We use the above cut-matching game in order to compute an expander $W$  with vertex set $T$, and to embed it into $G$, using standard techniques.
If $|T|$ is an even integer, then we start with the graph $W$ containing the vertices of $T$; otherwise, we let $t\in T$ be an arbitrary vertex, and we start with $V(W)=T\setminus\set{t}$. Initially, $E(W)=\emptyset$. We then perform iterations. In the $i$th iteration, we apply the algorithm of the cut player to the current graph $W$, and obtain a partition  $(Z_i,Z'_i)$ of its vertices with $|Z_j| = |Z'_j|$. Using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked},  we compute a collection $\pset_i$ of paths in graph $G$, routing vertices of $Z_i$ to vertices of $Z'_i$, so that every vertex of $Z_i\cup Z'_i$ is an endpoint of exactly one path in $\pset_i$, and the paths in $\pset_i$ cause congestion at most $\ceil{1/\alpha}\leq 2/\alpha$ in $G$. Let $M_i$ be a perfect matching between vertices of $Z_i$ and vertices of $Z'_i$ defined by the set $\pset_i$ of paths: that is, we add to $M_i$ a pair $(t,t')$ of vertices iff some path in $\pset_i$ has endpoints $t$ and $t'$. We then treat $M_i$ as the response of the matching player, and add the edges of $M_i$ to $W$, completing the current iteration of the game.

Let $W$ be the graph obtained after $i^*=O(\log^2k)$ iterations, that is guaranteed to be a $1/2$-expander with high probability. We then set $\pset=\bigcup_{i=1}^{i^*}\pset_i$. It is immediate to verify that $\pset$ is an embedding of $W$ into $G$. Since each path set $\pset_i$ causes congestion $O(1/\alpha)$, and $i^*\leq O(\log^2k)$, the paths in $\pset$ cause congestion $O((\log^2 k)/\alpha)$. If $|T|$ is even, then we have constructed the desired expander and its embedding into $G$ as required. If $|T|$ is odd, then we add the terminal $t$ to the graph $W$. Let $P$ be any path in graph $G$, connecting $t$ to any terminal $t'\in T\setminus\set{t}$; such a path must exist since the set of terminals is $\alpha$-well-linked in $G$. We then add edge $(t,t')$ to graph $W$, and we let its embedding be $P(e)=P$; we add path $P$ to $\pset$. It is easy to verify that this final graph $W$ is $1/4$ expander, provided that the original graph $W$ obtained at the end of the cut-matching game was a $1/2$-expander. We have also obtained an embedding of $W$ into $G$ with congestion $O((\log^2k)/\alpha)$.














%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of Observation~\ref{obs: cr of exp}}

\label{apd: Proof of cr of exp}


%	Recall that $W$ is a graph with $k$ vertices, that is a $1/4$-expander, and its maximum vertex degree is $O(\log^2k)$. 
Let $W'$ be the graph obtained from $W$ by discarding parallel edges. It is immediate to verify that graph $W'$ is a $\phi$-expander, for $\phi=\Omega(1/\log^2 k)$. 
From \Cref{lem:min_bal_cut}, the minimum $1/4$-edge-balanced cut in graph $W'$ has size at most:


\[O\left(\sqrt{\optcro(W')+|E(W')|\cdot \log^2k} \right)\leq O\left(\sqrt{\optcro(W)+k\cdot \log^4k} \right).\] 


On the other hand, since $W'$ is a $\phi$-expander, and its vertices have degrees $O(\log^2k)$, the size of the minimum $1/4$-edge-balanced cut is $\Omega(k/\log^4k)$. We conclude that $\optcro(W)\geq \Omega(k^2/\log^8k)$.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\subsection{Proof of Corollary~\ref{cor: routing well linked vertex set}}

\label{apd: Proof of routing well linked vertex set}


The proof relies on known results for routing on expanders, that are summarized in the next claim, that is well-known, and follows  immediately from the results of \cite{leighton1999multicommodity}. A proof can be found, e.g. in \cite{chuzhoy2012routing}.

\begin{claim}[Corollary C.2 in \cite{chuzhoy2012routing}]\label{claim: routing on expander}
	There is an efficient randomized algorithm that, given as input an $n$-vertex $\phi$-expander $H$, and any partial matching $M$ over the vertices of $H$, computes, for every pair $(u,v)\in M$, a path $P(u,v)$ connecting $u$ to $v$ in $H$, such that with high probability, the set $\set{P(u,v)\mid (u,v)\in M}$ of paths causes congestion $O(\log^2 n/\phi)$ in $H$. %The algorithm succeeds with high probability.
\end{claim}


We start by computing a graph $W$ with $V(W)=T$, and its embedding $\pset=\set{P(e)\mid e\in E(W)}$ into $G$ with congestion $O((\log^2k)/\alpha)$ using the algorithm from \Cref{claim: embed expander} (recall that, with high probability, $W$ is an $(1/4)$-expander). Next,
we use the algorithm from \Cref{claim: routing on expander} to compute a collection $\rset'=\set{P(u,v)\mid (u,v)\in M}$ of paths in graph $W$, where for all $(u,v)\in M$, a path $P(u,v)$ connects $u$ to $v$ in $W$, such that the congestion of the set $\rset'$ of paths in $W$ is $O(\log^2k)$ with high probability. 

Lastly, we consider the paths $P(u,v)\in \rset'$ one-by-one. We transform each such path $P(u,v)$ into a path $R(u,v)$ connecting $u$ to $v$ in graph $G$ by replacing, for every edge $e\in P(u,v)$, the edge $e$ with the path $P(e)\in \pset$ embedding the edge $e$ into $G$. Once every edge of $P(u,v)$ is processed, let $R(u,v)$ denote the final path. Since the paths in $\rset'$ cause congestion at most $O(\log^2k)$ in $W$ (with high probability), while the paths in $\pset$ cause congestion $O(\log^2k/\alpha)$ in $G$, we get that with high probability, the paths in the resulting set $\rset=\set{R(u,v)\mid (u,v)\in M}$ cause congestion $O(\log^4k/\alpha)$ in $G$.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of Corollary~\ref{cor: embed complete graph}}

\label{apd: Proof of embed complete graph}




We partition the set $E(K)$ of edges into $3z$ matchings $M_1,\ldots,M_{3z}$, and then use \Cref{cor: routing well linked vertex set} to compute, for each $1\leq i\leq 3z$, a set $\tilde \rset_i=\set{\tilde P(e)\mid e\in M_i}$ of paths in graph $G$, where for all $e=(t,t')\in M_i$, path $\tilde P(e)$ connects $t$ to $t'$, and with high probability, the paths in $\tilde \pset_i$ cause edge-congestion $O(\log^4z/\alpha)$ in graph $G$. Let $\tilde \pset=\bigcup_{i=1}^{3z}\tilde \pset_i$. Then $\tilde \pset$ is an embedding of $K_z$ into $G$, and with high probability, the congestion of this embedding is $O(z\log^4z)/\alpha$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%









\subsection{Proof of Claim~\ref{clm: contracted_graph_well_linkedness}}

\label{apd: Proof of contracted_graph_well_linkedness}

Let $(A,B)$ be an arbitrary cut in $G$, and we denote $T_A=T\cap A$ and $T_B=T\cap B$. Assume without loss of generality that $|T_A|\le |T_B|$. It suffices to show that $|E_G(A,B)|\ge (\alpha_1\alpha_2)\cdot |T_A|$.

Denote $H=G_{|\cset}$.  From the definition of $H$, its vertices can be partitioned into two sets: set $V'$ contains all vertices that does not belong to any cluster of $\cset$, and set $V''$ that contains all super-nodes that correspond to clusters in $\cset$. So $V'=V(G)\setminus (\bigcup_{C\in \cset}V(C))$ and $V''=\set{v_C\mid C\in \cset}$.
Moreover, since no vertices of $T$ lies in any cluster of $\cset$, $T\subseteq V'$.

We construct a cut $(A',B')$ in $H$ based on the cut $(A,B)$ in $G$ as follows.
For each vertex $v\in V'$, we add $v$ to $A'$ iff $v$ belongs to $A$ as a vertex in $G$, and we add $v$ to $B'$ iff $v$ belongs to $B$ as a vertex in $G$.
It remains to specify whether the super-node $v_C$ belongs to $A'$ or $B'$ for each cluster $C\in \cset$.
Consider a cluster $C\in \cset$, the set $\delta_G(C)$ of edges can be partitioned into four subsets: $\hat E_A, \hat E_B, \hat E_{AB}, \hat E_{BA}$ as follows. Let $e=(u,u')$ be an edge of $\delta_G(C)$, where $u\in C$ and $u'\notin C$. 
If $u,u'\in A$, then $e\in \hat E_A$. 
If $u,u'\in B$, then $e\in \hat E_B$. 
If $u\in A,u'\in B$, then $e\in \hat E_{AB}$.
If $u\in B,u'\in A$, then $e\in \hat E_{BA}$.
If $|\hat E_A|+|\hat E_{AB}|\le |\hat E_B|+|\hat E_{BA}|$, then the supernode $v_C$ is added to $B'$; otherwise the supernode $v_C$ is added to $A'$. This completes the definition of the cut $(A',B')$. Clearly, $T\cap A'=T_A$ and $T\cap B'=T_B$. Since $T$ is $\alpha_2$-well-linked in $H$, $|E_{H}(A',B')|\ge \alpha_2 \cdot|T_A|$.

We claim that $|E_G(A,B)|\ge \alpha_1\cdot |E_{H}(A',B')|$. Note that, if this is true, then it follows that $|E_G(A,B)|\ge (\alpha_1\alpha_2)\cdot |T_A|$ and the proof of Claim~\ref{clm: contracted_graph_well_linkedness} is completed.

It remains to show that $|E_G(A,B)|\ge \alpha_1\cdot |E_{H}(A',B')|$. On one hand, from the definition of $H$, $V'\cap A=V'\cap A'$ and $V'\cap B=V'\cap B'$, so an edge in $E_{H}(V'\cap A', V'\cap B')$ is also an edge in $E_{G}(A, B)$. On the other hand, let $C$ be any cluster of $\cset$. Assume first that $v_C\in B'$, then $|\hat E_A|+|\hat E_{AB}|\le |\hat E_B|+|\hat E_{BA}|$. Since cluster $C$ has $\alpha_1$-bandwidth property, $|E_G(A\cap C,B\cap C)|\ge \alpha_1\cdot (|\hat E_A|+|\hat E_{AB}|)=\alpha_1\cdot |\delta_{H}(v_C)\cap E_H(A',B')|$. Similarly, if $v_C\in A'$, then 
$|E_G(A\cap C,B\cap C)|\ge \alpha_1\cdot |\delta_{H}(v_C)\cap E_H(A',B')|$.
Altogether,
\[
\begin{split}
|E_{G}(A,B)| &\ge |E_{G}(A\cap V',B\cap V')|+\sum_{C\in \cset}|E_{G}(A\cap C,B\cap C)|\\
&\ge |E_{H}(A'\cap V',B'\cap V')|+\sum_{C\in \cset}\alpha_1\cdot |\delta_{H}(v_C)\cap E_H(A',B')|\\
&\ge \alpha_1\cdot|E_{H}(A',B')|.
\end{split}
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of \Cref{cor: contracted_graph_well_linkedness}}

\label{apd: Proof of cor contracted_graph_well_linkedness}



Let $G^+$ be the graph obtained from $G$ by subividing each edge $e\in \delta_G(R)$ with a new vertex $t_e$. 
Denote $T=\set{t_e\mid e\in \delta_G(R)}$.
Recall that the augmentation $R^+$ of cluster $R$ in $G$ is defined to be the subgraph of $G^+$ induced by all vertices of $V(R)\cup T$.
Denote $\hat G^+ = G^+_{\mid \cset}$ and $\hat R^+ = R^+_{\mid \cset}$. Recall that $\hat R=R_{\mid \cset}$. It is easy to verify that $\delta_{\hat G}(\hat R)=T$, and $\hat R^+$ is the augmentation of cluster $\hat R$ in graph $\hat G$. Therefore, since $\hat R$ has the $\alpha_2$-bandwidth property in $\hat G$, $T$ is  $\alpha_2$-well-linked in $\hat G^+$.

Note that $\cset$ is a collection of disjoint clusters of $G$, and $T\cap (\bigcup_{C\in \cset}V(C))=\emptyset$. 
Moreover, note that each cluster $C\in \cset$ has the $\alpha_1$-bandwidth property, and the set $T$ of vertices is $\alpha_2$-well-linked in $\hat G^+$.
From \Cref{clm: contracted_graph_well_linkedness}, we get that $T$ is $(\alpha_1\alpha_2)$-well-linked in graph $G^+$. Equivalently, the cluster $R$ has $(\alpha_1\alpha_2)$-bandwidth property in $G$.



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Proof of \Cref{claim: routing in contracted graph}}
\label{apx: contracted graph routing}

For convenience, we denote $G_{|\cset}$ by $\hat G$, and we denote $|T|=k$.
We assume w.l.o.g. that the paths in $\pset$ are simple, and we direct each such path towards $x$. We then graduately modify the paths in $\pset$, by processing the clusters of $\cset$ one-by-one. 

Consider now any such cluster $C\in \cset$, and let $\pset(C)\subseteq \pset$ be the subset of paths that contain the vertex $v(C)$. For each such path $P\in \pset(C)$, let $e_P(C)$ and $e_P'(C)$ denote the edges appearing immediately before and immediately after $v(C)$ on $P$. We then denote $E_1(C)=\set{e_P(C)\mid P\in \pset(C)}$ and $E_2(C)=\set{e'_P(C)\mid P\in \pset(C)}$. Since cluster $C$ has the $\alpha$-bandwidth property, from \Cref{cor: bandwidth_means_boundary_well_linked}, there is a collection $\rset(C)$ of paths in graph $C\cup\delta(C)$ of cardinality $|\pset(C)|$, where each path connects a distinct edge of $E_1(C)$ to a distinct edge of $E_2(C)$, and every edge in $C$ participates in at most $\ceil{1/\alpha}$ such paths. We modify the paths in set $\pset(C)$ as follows. First, for each path $P\in \pset(C)$, we delete the vertex $v(C)$ from $P$, together with its two incident edges. Let $P_1,P_2$ be the two resulting sub-paths of $P$. Next, we let $\pset_1(C)=\set{P_1\mid P\in \pset(C)}$, and $\pset_2(C)=\set{P_2\mid P\in \pset(C)}$. Lastly, let $\pset'(C)$ be the set of paths obtained by concatenating the paths in $\pset_1(C),\rset(C)$ and $\pset_2(C)$. We then delete from $\pset$ the paths that belong to $\pset(C)$, and add the paths of $\pset'(C)$ instead. It is easy to verify that the resulting set $\pset$ of paths still routes the vertices of $T$ to $x$.

Once we complete processing every cluster $C\in \cset$, we obtain a collection $\pset'$ of $k$ paths, routing the vertices of $T$ to the vertex $x$. Since the paths of $\pset$ at the beginning of the algorithms are edge-disjoint paths in $G_{|\cset}$, it is easy to see that, for each edge $e\in \bigcup_{C\in \cset}E(C)$, $\cong_G(\pset',e)\le 1$, and for each edge $e\notin \bigcup_{C\in \cset}E(C)$, $\cong_{G}(\pset',e)\leq \ceil{1/\alpha}\leq 2/\alpha$. From \Cref{claim: remove congestion}, we conclude that there is a collection $\pset''$ of at least $\alpha k/2$ edge-disjoint paths in graph $G$, where each path in $\pset''$ connects a distinct vertex of $T$ to $x$. We can compute such a collection $\pset''$ of paths via standard maximum $s$-$t$ flow computation.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of \Cref{lem: crossings in contr graph}}
\label{apd: Proof of crossings in contr graph}

Let $\phi^*$ be an optimal solution to instance $I$. Let $G'$ be the graph that is obtained from $G$ by subdividing every edge $e\in \bigcup_{C\in \cset}\delta_G(C)$ with a vertex $t_e$, and let $T=\set{t_e\mid e\in \bigcup_{C\in \cset}\delta_G(C)}$ be the resulting set of new vertices. For every cluster $C\in \cset$, we denote by $T_C=\set{t_e\mid e\in\delta_G(C)}$, and we let $C'$ be the sub-graph of $G'$ induced by $C\cup T_C$. Clearly, the set $T_C$ of vertices is $\alpha$-well-linked in $C'$. Observe that drawing $\phi^*$ of $G$ naturally defines a drawing $\phi'$ of graph $G'$, with $\cro(\phi^*)=\cro(\phi')$.


Consider now some cluster $C\in \cset$. %For every edge $e\in E(C')$, we let $\cro(e)$ be the number of crossings in the drawing $\phi'$ in which edge $e$ participates, and we denote by $\cro(C')=\sum_{e\in E(C')}\cro(e)$. 
Recall that \Cref{lem: simple guiding paths} provides a randomized algorithm that computes a distribution $\dset$ over the set of all internal $C$-routers. We then let $\qset=\set{Q(e)\mid e\in \delta_G(C)}$ be a (random) set of paths sampled from distribution $\dset$. From \Cref{lem: simple guiding paths}, for each edge $e\in E(C)$, $\expect{\cong(\qset,e)}\leq  O(\log^4m/\alpha)$.
Let $u$ be the common endpoints of paths in $\qset$.
%computes a vertex $u\in V(C')$, and a collection $\qset=\set{Q_t\mid t\in T_C}$ of paths, where path $Q_t$ connects $t$ to $u$, such that, for every edge $e\in E(C')$, $\expect{\cong(\qset,e)}\leq  O(\log^4n/\alpha)$.
%Therefore, there exists a vertex $u\in V(C')$, and a collection $\qset=\set{Q_t\mid t\in T_C}$ of paths, where path $Q_t$ connects $t$ to $u$, such that $\sum_{e\in E(C')}\cong(\qset,e)\cdot \cro(e)\leq  O(\log^4n\cro(C')/\alpha)$. 
We slightly modify $u$ and $\qset$, as follows: if $u\not\in T_C$, then we set $u_C=u$ and $\qset(C)=\qset$. Assume now that $u\in T_C$. Recall that, from the definition of graph $C'$, every vertex in $T_C$ has degree exactly $1$ in $C'$. We then let $u_C$ be the unique neighbor of $u$ in $C'$.  We modify each path $Q_t\in \qset$ as follows: if $t\neq u$, then we truncate the path at vertex $u_C$, so it connects $t$ to $u_C$; otherwise, we let $Q_t$ be the path consisting of a single edge $(u,u_C)$. We denote the final set of paths by $\qset(C)$; each path in $\qset(C)$ connects a distinct vertex of $T_C$ to $u_C$, and it is easy to verify that 
for every  edge $e\in E(C')$, $\expect{\cong(\qset(C),e)}\leq  O(\log^4m/\alpha)$.
%$\sum_{e\in E(C')}\cong(\qset(C),e)\cdot \cro(e)\leq  O(\log^4n\cro(C')/\alpha)$ continues to hold. Since every vertex $t\in T_C$ has degree $1$ in $C'$, exactly one path in $\qset(C)$ contains the unique edge incident to $t$ in $C'$ -- the path $Q_t$.
%Lastly, we modify the paths in $\qset(C)$ using \Cref{lem: non_interfering_paths}, so that the paths in $\qset(C)$ are locally non-interfering with respect to $\Sigma$.
We denote $\qset=\bigcup_{C\in \cset}\qset(C)$, so for every edge $e\in E(G')$, $\expect{\cong(\qset(C),e)}\leq  O(\log^4m/\alpha)$.

For each $C\in \cset$, we then apply the algorithm from \Cref{cor: new type 2 uncrossing} to graph $G'$, drawing $\phi'$, cluster $C'$ and the set $\qset(C)$ of paths, where $u_C$ is viewed as the last endpoint of every path in $\qset(C)$. Let $\Gamma_C=\set{\gamma_C(e)\mid e\in \delta_{G'}(C)}$ be the set of curves we get, where the curve $\gamma_C(e)$ corresponds to the path in $\qset(C)$ that has $t_e$ as its first endpoint. We now view, for each cluster $C\in\cset$ and each edge $e\in \delta_{G'}(C)$, the curve $\gamma_C(e)$ as the image of $e$. Then we obtain a drawing $\phi''$ of $G'$, and moreover, from 
\Cref{cor: new type 2 uncrossing},
\[
\begin{split}
\expect[]{\cro(\phi'')}\le
&\text{ }\cro(\phi')+\sum_{e,e' \text{ from different clusters of }\cset}\chi_{\phi'}(e,e')\cdot\expect[]{\cong(\qset,e)}\cdot\expect[]{\cong(\qset,e')}\\
\le &\text{ } O\left( \optcrors(I)\cdot \frac{\log^8 n}{\alpha^2}\right).
\end{split}
\]
Clearly, drawing $\phi''$ naturally defines a drawing $\phi'''$ of $G$, with $\cro(\phi''')=\cro(\phi'')$, such that
for every verteex $x\in V(G_{\mid \cset}\cap V(G))$, the ordering of the edges of $\delta_G(x)$ as they enter $x$ in $\phi'''$ is consistent with the the ordering of the edges of $\delta_G(x)$ as they enter $x$ in $\phi^*$, which is $\oset_x\in \Sigma$. This completes the proof of \Cref{lem: crossings in contr graph}.






\iffalse
Let $\cset=\set{C_1,\ldots,C_r}$.
We partition the set $E(G')$ of edges into subsets $E_0,E_1,\ldots,E_r$ as follows: for all $1\leq i\leq r$, $E_i=E(C'_i)$, and $E_0$ contains all edges that do not lie in any cluster $C'_1,\ldots,C'_r$. We let $\chi_1$ be the set of all crossings $(e,e')$ in $\phi'$, with $e,e'$ lying in the same set $E_i$, for $0\leq i\leq r$, and we let $\chi_2$ be the set of all crossings $(e,e')$ in $\phi'$ where $e\in E_i$, $e'\in E_j$, and $i\neq j$.


Consider now some index $1\leq i\leq r$, and some edge $e\in E(C'_i)$. If $e$ does not participate in any path in $\qset(C_i)$, then we set $n_e=1$; otherwise, we let $n_e=\cong(\qset(C_i),e)$ be the number of paths in $\qset(C_i)$, in which the edge $e$ participates. For each edge $e\in E_0$, we set $n_e=1$.

Let $G''$ be the graph obtained from $G'$, where we replace every edge $e\in E(G')$ with $n_e$ parallel copies. For all $0\leq i\leq r$, we denote by $E'_i$ the set of edges of $G''$ corresponding to the edges of $E_i$. Drawing $\phi'$ of $G'$ naturally defines a drawing $\phi''$ of $G''$: for every edge $e\in E(G')$, we draw the $n_e$ parellel copies of the edge $e$ next to each other, in parallel to the original drawing of the edge $e$ and very close to it.

We denote by $\chi_1'$ the set of all crossings $(e,e')$ in the resulting drawing $\phi''$, where both $e$ and $e'$ lie in the same set $E'_i$ of edges, for any $0\leq i\leq r$, and we let $\chi_2'$ be the set of all crossings $(e,e')$ in $\phi''$, where $e\in E_i'$, $e'\in E_j'$, and $0\leq i<j\leq r$. We use the following simple observation to bound the number of crossigns in $\chi_2'$.

\begin{observation}\label{obs: number of type 2 crossings}
	\[\expect{|\chi_2'|}\leq |\chi_2|\cdot O(\log^8n/\alpha^2).\]
\end{observation}

\begin{proof}
	Consider some crossing $(e_1,e_2)\in \chi_2'$. Then there must be a crossing $(e_1',e_2')\in \chi_2$, where $e_1$ is a copy of $e_1'$ and $e_2$ is a copy of $e_2'$. We say that crossing $(e_1',e_2')$ is responsible for the crossing $(e_1,e_2)$. We have now assigned, to each crossing in $\chi_2'$, a crossing in $\chi_2$ that is responsible for it.
	
	Consider now some crossing $(e,e')\in \chi_2$. The number of crossings in $\chi_2'$ that it is responsible for is precisely $n_e\cdot n_{e'}$. Assume that $e\in E_i,e'\in E_j$, for some $0\leq i,j\leq r$, with $i\neq j$. Since $i\neq j$, $n_e$ and $n_{e'}$ are independent random variables. Therefore, $\expect{n_e\cdot n_{e'}}=\expect{n_e}\cdot \expect{n_{e'}}\leq O(\log^8n/\alpha^2)$.
	
	Altogether, we get that:
	
	\[\expect{|\chi_2'|}\leq \expect{\sum_{(e,e')\in \chi_2}n_e\cdot n_{e'}}\leq \sum_{(e,e')\in \chi_2}\expect{n_e\cdot n_{e'}}\leq |\chi_2|\cdot O(\log^8n/\alpha^2).\]
\end{proof}

Let $\chi_0$ be the set of all crossings $(e,e')$ in the drawing $\phi'$ in which $e,e'\in E_0$.

For all $1\leq i\leq r$, let $C''_i$ be the subgraph of $G''$ induced by the vertices of $C'_i$. We can now define a set $\qset'(C_i)$ of paths in graph $C''_i$, routing the vertices of $T_{C_i}$ to $u_C$, such that the paths in $\qset'(C_i)$ are edge-disjoint. In order to do so, we simply assign, for each edge $e\in E_i$, a distinct copy of $e$ to every path $Q_t\in \qset(C_i)$ that contains $e$.

Next, we define a collection $\Gamma_0,\Gamma_1,\ldots,\Gamma_r$ of curves, as follows. For each edge $e\in E_0$, we add a curve $\gamma(e)$ to $\Gamma_0$, where $\gamma(e)$ is the image of the edge $e$ in the drawing $\phi''$.

Consider now some index $1\leq i\leq r$. We start by letting $\Gamma_i$ contain the set of images of all paths in $\qset'(C_i)$ in the drwaing $\phi'$; in other words, we can denote $\Gamma_i=\set{\gamma_i(t)\mid t\in T_C}$, where $\gamma_i(t)$ is the image of the unique path $Q'_t\in \qset'(C_i)$, connecting $t$ to $u(C_i)$. We direct all curves in $\Gamma_i$ towards the image of $u(C_i)$, and we delete loops from each resulting curve, so that all curves in set $\Gamma_i$ become simple.

Consider the resulting collection $\Gamma=\Gamma_0\cup\Gamma_1\cup\cdots \Gamma_r$ of curves. Let $p$ be any point that lies on more than two such curves. 
Assume first that $p$ is an image of some vertex $v\in V(G'')$. If there is some index $1\leq i\leq r$, such that $v\in V(C_i)$, then every curve $\gamma\in \Gamma$ that contains $v$ must belong to $\Gamma_i$. Otherwise, for every curve $\gamma\in \Gamma$ with $p\in \gamma$, point $p$ is an endpoint of $\gamma$. 
Assume now that $p$ is not an image of a vertex in $V(G'')$, so it is an inner point on the image of some edge of $G''$. I this case, from the definition of a graph drawing, $p$ may lie on images of at most two edges of $G''$, and so it may not belong to more than three curves of $\Gamma$.

To conclude, if a point $p$ lies on more than $2$ curves of $\Gamma$, then either it is an endpoint of every curve $\gamma$ containing $p$, or there is some index $1\leq i\leq r$, such that every curve $\gamma$ containing $p$ belongs to $\Gamma_i$.

Therefore, 
we then use the algorithm from \Cref{thm: type-2 uncrossing} in order to uncross each set $\Gamma_i$ of curves, for $1\leq i\leq r$. Recall that we obtain new sets $\Gamma'_1,\ldots,\Gamma'_r$ of curves. For each $1\leq i\leq r$ and $t\in T_C$, we denote by $\gamma'_i(t)$ the unique curve in $\Gamma'_i$ that originates at the image of $t$ and terminates at the image of $u(C_i)$.


\mynote{from here on needs to be fixed once the statement of  \Cref{thm: type-2 uncrossing} is fixed}
Recall that \Cref{thm: type-2 uncrossing}, we are guaranteed that, if $p$ is a point lying on more than two curves in $\Gamma_0\cup \Gamma'_1\cup\cdots\cup\Gamma'_r$, then $p$ is an endpoint of all these curves, and that the total number of crossings between all curves in $\Gamma_0\cup \Gamma'_1\cup\cdots\cup\Gamma'_r$ is bounded by $|\chi_2'|+|\chi_0|$.


We are now ready to define the drawing $\phi$ of graph $G_{|\cset}$. We start from the drawing $\phi'$ of $G'$. 
For every cluster $C_i\in \cset$, we delete the images of all vertices of $C$, except for $u_C$, and of all edges of $E(C')$. The image of $u_C$ becomes the image of the vertex $v(C)$ representing the cluster $C$ in the contracted graph. We then add the curves in $\Gamma'_i$ to this drawing; recall that each such curve connects $u(C)$ to a distinct vertex $t\in T_C$. Once all clusters $C_i\in \cset$ are processed, we obtain  a drawing of a graph $\hat G$, that is obtained from $G_{|\cset}$ by subdividing every edge $e\in \bigcup_{C\in \cset}\delta(v(C))$ with a vertex $t_e$. The set of images of the edges of $\hat G$ in this drawing is precisely $\Gamma_0\cup \Gamma'_1\cup\cdots\cup\Gamma'_r$, and so the number of crossings in this drawing is bounded by $|\chi_2'|+|\chi_0|$. This drawing of $\hat G$ immediately defines a drawing of $G_{|\cset}$, by surpressing the images of all vertices $\set{t_e\mid e\in \bigcup_{C\in \cset}\delta(v(C))}$. The number of crossings in this final drawing is bounded by $|\chi_2'|+|\chi_0|$. Clearly, $|\chi_0|\leq \optcrors(I)$, since we did not modify the drawings of the edges in $E_0$, and each edge $e\in E_0$ has $n_e=1$. 
From 
\Cref{obs: number of type 2 crossings},
$\expect{|\chi_2'|}\leq |\chi_2|\cdot O(\log^8n/\alpha^2)$. Moreover, since we did not modify the drawings of the edges in $E_0$, it is easy to verify that for every vertex $x\in V(G_{|\cset})\cap V(G)$, the ordering of the edges of $\delta_G(x)$ as they enter $x$ in the final drawing $\phi$ is consistent with the ordering $\oset_x\in \Sigma$.

\znote{to modify using new type-2 uncrossing}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
\subsection{Proof of \Cref{lem: convert path}}
\label{apd: Proof of convert path}


\znote{To add}.




\fi






%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of \Cref{lem: GH tree path vs contraction}}
\label{apd: Proof of GH tree path vs contraction}

For each $1\le i\le n-1$, we denote $S_{i}=\set{v_1,\ldots,v_i}$ and  $\notS_{i}=\set{v_{i+1},\ldots,v_n}$.

Let $v_C,v_{C'}$ be two vertices that appear consecutively on the contracted path $\tau_{\cset}$, where $v_C$ corresponds to cluster $C$ and $v_{C'}$ corresponds to cluster $C'$ ($C,C'\in \cset$). We denote $C=\set{v_p,\ldots,v_r}$ and $C'=\set{v_{r+1},\ldots,v_q}$.
Since path $\tau$ is a Gomory-Hu tree of $G$, then the cut $(S_r,\notS_r)$ is a min-cut in $G$ separating $v_r$ from $v_{r+1}$. 
On the other hand, note that any cut separating $v_C$ from $v_{C'}$ in the contracted graph $G_{\cset}$ corresponds to a cut in the original graph $G$ separating $v_r$ from $v_{r+1}$, with the same set of edges. Moreover, if we denote by $S,\notS$ the components of $\tau$ obtained by removing the edge $(v_C,v_{C'})$ from $\tau$, then the cut $(S,\notS)$ in $G_{\cset}$ corresponds to the cut $S_r,\notS_r$ in $G$. Therefore, the cut $(S,\notS)$ is a min-cut in $G_{\cset}$ separating $v_C$ from $v_{C'}$. It follows that $\tau_{|\cset}$ is a Gomory-Hu tree of the contracted graph $G_{|\cset}$.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of Lemma~\ref{lem: multiway cut with paths sets}}

\label{apd: Proof of multiway cut with paths sets}

We use the following lemma.
\begin{lemma}
\label{lem: cut_uncrossing}
Let $S=\set{s_1,\ldots,s_k}$ be a set of vertices of $G$. For any pair $1\le i,j\le k$, if $(U_i,\overline{U_i})$ is a minimum cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$ with $s_i\in U_i$, and $(U_j,\overline{U_j})$ is a minimum cut in $G$ separating $\set{s_j}$ from $S\setminus \set{s_j}$ with $s_j\in U_j$, then $(U_i\setminus U_j, \overline{U_i\setminus U_j})$ is a minimum cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$, and $(U_j\setminus U_i, \overline{U_j\setminus U_i})$ is a minimum cut in $G$ separating $\set{s_j}$ from $S\setminus \set{s_j}$.
\end{lemma}
\begin{proof}
If $U_i\cap U_j=\emptyset$ then there is nothing to prove. We now assume that $U_i\cap U_j\ne\emptyset$.
We denote $A=U_i\setminus U_j$, $B=U_j\setminus U_i$, $C=U_i\cap U_j$, and $D=\overline{U_i\cup U_j}$.
Note that $s_i\in U_i$ and $s_i\notin U_j$, so $A\ne \emptyset$, and similarly $B\ne \emptyset$.
Note that the cut $(A,B\cup C\cup D)$ is also a cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$.
Since $(U_i,\overline{U_i})$ is a minimum cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$,
\[
|E(A,B)|+|E(A,D)|+|E(C,B)|+|E(C,D)|\le |E(A,B)|+|E(A,C)|+|E(A,D)|.
\]
We get that $|E(C,B)|+|E(C,D)|\le |E(A,C)|$.
Similarly, note that the cut $(B,A\cup C\cup D)$ is also a cut in $G$ separating $\set{s_j}$ from $S\setminus \set{s_j}$, while $(U_j,\overline{U_j})$ is a minimum cut in $G$ separating $\set{s_j}$ from $S\setminus \set{s_j}$. Therefore,
\[
|E(A,B)|+|E(D,B)|+|E(A,C)|+|E(D,C)|\le |E(B,A)|+|E(B,C)|+|E(B,D)|.
\]
We get that $|E(A,C)|+|E(C,D)|\le |E(B,C)|$.
Altogether, $|E(C,D)|=0$ and $|E(A,C)|=|E(B,C)|$. Therefore,
$|E(A,B\cup C\cup D)|=|E(U_i,\overline{U_i})|$ and  
$|E(B,A\cup C\cup D)|=|E(U_j,\overline{U_j})|$, which means that 
$(U_i\setminus U_j, \overline{U_i\setminus U_j})$ is a minimum cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$, and $(U_j\setminus U_i, \overline{U_j\setminus U_i})$ is a minimum cut in $G$ separating $\set{s_j}$ from $S\setminus \set{s_j}$.
\end{proof}

We now complete the proof of Lemma~\ref{lem: multiway cut with paths sets} using Lemma~\ref{lem: cut_uncrossing}.
Recall that we are given a set $S=\set{s_1,\ldots,s_k}$ of vertices of $G$. We first compute, for each $1\le i\le k$, a minimum cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$, that we denote by $(U_i,\overline{U_i})$, with $s_i\in U_i$. We then let $A_i=U_i\setminus (\bigcup_{1\le j\le k, j\ne i}U_j)$, for each $1\le i\le k$. 
It is clear that, for all $1\le i\le k$, $S\cap A_i=\set{s_i}$, and for all $1\le i<j\le k$, $A_i\cap A_j=\emptyset$.
We claim that the cut $(A_i,\overline{A_i})$ is a min-cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$.
To see that, we start with $A^*_i=U_i$, and then sequentially for $j=1,\ldots, i-1,i+1,\ldots,k$, we delete from $A^*_i$ the elements that belong to $U_j$. From Lemma~\ref{lem: cut_uncrossing}, after each round, the cut $(A^*_i,\overline{A^*_i})$ remains a min-cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$, and at the end, $A^*_i=U_i\setminus (\bigcup_{1\le j\le k, j\ne i}U_j)$.

It remains to compute, for each $1\le i\le k$, a set $\qset_i$ of paths connecting edges of $\delta(A_i)$ to $s_i$. We set up an instancee of max-flow problem as follows.
We define the graph $H_i$ to be the graph obtained from $G[A_i]\cup \delta_G(A_i)$, (where $G[A_i]$ is the subgraph of $G$ induced by vertices of $A_i$) by contracting all vertices that do not belong to $A_i$ but are connected by an edge to some vertex of $A_i$ into a single vertex, that we denote by $t_i$. We then compute in graph $H_i$ the max-flow from $s_i$ to $t_i$, with each edge of $H_i$ assigned with unit capacity. It is easy to see that we can obtain a set of $|\delta_G(A_i)|$ paths in $H_i$ connecting edges of $\delta_G(A_i)$ to $u$, and we denote this set by $\qset_i$. Since otherwise, from the max-flow min-cut theorem, we will obtain a cut (other than the cut $(A_i,\set{t_i})$) in $H_i$ separating $s_i$ from $t_i$ that contains strictly less edges than $(A_i,\set{t_i})$, causing a contradiction to the fact that the cut $(A_i,\overline{A_i})$ is a min-cut in $G$ separating $\set{s_i}$ from $S\setminus \set{s_i}$.




\subsection{Proof of \Cref{obs: grid 1st row well-linked}}
\label{apd: Proof grid 1st row well-linked}


We denote by $T$ the first row of the $(r\times r)$-grid.
Consider any partition $(A,B)$ of the vertex set of the $(r\times r)$-grid. 
Denote $A_1=T\cap A$ and $B_1=T\cap B$, and assume without loss of generality that $|A_1|\le |B_1|$.
We will show that there exists a set of $|A_1|$ node-disjoint paths connecting vertices of $A_1$ to vertices of $B_1$, which implies that $|E(A,B)|\ge \min\set{|A\cap T|,|B\cap T|}$.

The node-disjoint paths are constructed similarly as in
the proof of \Cref{clm: grid well-linked}.
We maintain an index set $I$, initializing $I=\set{1,\ldots,r}$.
While there is a pair $i,i'$ of indices of $I$, such that $i<i'$, $v_{i},v_{i'}$ belongs to different sets of $A_1,B_1$, and there is no other $j\in I$ with $i<j<i'$, we define the path $P_{i,i'}$ to be the sequential concatenation of the path $(v_{1,i},v_{2,i},\ldots,v_{i',i})$, the path $(v_{i',i},v_{i',i+1},\ldots,v_{i',i'})$, and the path $(v_{i',i'},v_{i'-1,i'},\ldots,v_{1,i'})$. We then add the path $P_{i,i'}$ to $\pset$, delete $i,i'$ from $I$ and continue to the next iteration.
It is clear that, at the end of the process, $I$ does not contain any index $i$ with $v_{1,i}\in A_1$, and for each $v_{1,j}\in A_1$, there is a path $P_{j,j'}$ connecting $v_{1,j}$ to some vertex $v_{1,j'}$ of $B_1$, so $|\pset|=|A_1|$. It is also easy to verify that the paths of $\pset$ are node-disjoint. 


































%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> appx-procsplit2-backup.tex <==
\subsection{Proof of \Cref{lem: alg procsplit'}}
\label{subsec: proof of procsplit'} 


In order to simplify the notation, we denote instance $I_F=(G_F,\Sigma_F)$ by $I=(G,\Sigma)$, and we denote $|E(G)|$ by $m$. Since instance $I$ is not acceptable, face $F$ may not be a forbidden face of $\tilde \fset(W)$. Recall that we have computed a set $\sset(F)\subseteq\cset(W)$ of connected components, and, for each such component $C\in \sset(F)$, a subgraph $J_{C,F}$ that is a core. Intuitively, vertices and edges of  $J_{C,F}$ must serve as the boundary of face $F$ in any $\wset$-compatible drawing of $W$, and in particular their images lie on the boundary of the region $F$ in the drawing $\phi$ of graph $\cG'$, given by Property \ref{prop: drawing} of valid input. We have also defined, for each component $C\in \sset(F)$, a core structure $\jset_{C,F}$, whose corresponding core is $J_{C,F}$, and we have defined a collection  $\kset_{ F}=\set{\jset_{C, F}\mid C\in \sset( F)}$ of core structures associated with $F$. From the definition of a $\wset$-decomposition, for all $C\in \sset(F)$, $\jset_{C,F}$ is a valid core structure for $I$, and so $\kset_F$ is a valid skeleton structure for instance $I$. In order to simplify the notation, we denote $\kset_F=\set{\jset_{C,F}\mid C\in \sset(F)}$ by $\kset=\set{\jset_1,\ldots,\jset_z}$, and for all $1\leq i\leq z$, we denote the core associated with the cores structure $\jset_i$ by $J_i$. Since, from \Cref{lem: compute phase 2 decomposition}, $|\ckset|\leq \mu^{100}$, from the definition of a skeleton augmentation, $|\cset(W)|\leq \mu^{100}$, and so $z\leq \mu^{100}$ holds. We also denote by $K=\bigcup_{i=1}^zJ_i$ the skeleton associated with the skeleton structure $\kset$.

As before, we denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G=\cG'\setminus E^{\del}$, and let $\tilde \Sigma$ be the rotation system for graph $\tilde G$ induced by $\cSigma'$. Let $\tilde I=(\tilde G,\tilde \Sigma)$ be the resulting instance of \cnwrs. Recall that Property \ref{prop: drawing} of valid input to Procedure $\procsplit'$ ensures that there is a solution $\phi$ to instance $\tilde I$, that is $\wset$-compatible. Additionally,  $\cro(\phi)\leq (\cm')^2/\mu^{60b}$, $|\chi^{\dirty}(\phi)|\leq \cm'/\mu^{60b}$, the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\cro(\phi)\mu^{26b}/\cm'$.


As in the original procedure \procsplit, the algorithm consists of two steps. In the first step, we compute a promising path set and an enhancement of the skeleton $\kset$. In the second step we complete the construction of the new skeleton augmenting structure $\wset'$ and the new $\wset'$-decompositon $\gset'$ of graph $\cG'$.

\subsubsection{Step 1: Computing Skeleton Enhancement}

As before, we start by computing a promising path set, that will then be used in order to compute an enhancement of skeleton $\kset$. In the algorithm for $\procsplit$, the construction of the promising path set exploited the fact that the input instance $I$ was wide. Here, instead, we exploit the fact that instaince $I$ is not acceptable. The resulting promising path set will be somewhat smaller, and it will only be of type 2 or type 3.

From the definition of aceptable subinstances, there must be an index $1\leq i^*\leq z$, and a partition $(E_1,E_2)$ of the edges of $\delta_G(J_{i^*})$, such that the edges of $E_1$ appear consecutively in the ordering $\oset(J_{i^*})$, and the following holds. Let $(\tilde E',\tilde E'')$ be the partitition of the edges in set $\tilde E=\bigcup_{i=1}^z\delta_G(J_i)$, where $\tilde E'=E_1$, and $\tilde E''=\tilde E\setminus \tilde E'$. As before, let 
$\tilde H$ be the graph that is obtained from graph $G$ by, first subdividing every edge $e\in \tilde E$ with a vertex $t_e$, and then deleting all vertices and edges of $K$ from it. Then the minimum cut in graph $\tilde H$ separating the vertices of $\set{t_e\mid e\in \tilde E'}$ from the vertices of  $\set{t_e\mid e\in \tilde E''}$ must contain at least $\cm'/\mu^{2b}$ edges. Equivalently, there is a set $\pset$ of $\ceil{\cm'/\mu^{2b}}$ edge-disjoint paths in graph $\tilde H$, connecting vertices of 
$\set{t_e\mid e\in \tilde E'}$ to vertices of  $\set{t_e\mid e\in \tilde E''}$. We can assume w.l.o.g. that the paths of $\pset$ do not contain the vertices of $\set{t_e\mid e\in \tilde E}$ as inner vertices.

Set $\pset$ of paths in graph $\tilde H$ naturally defines a collection of at least $\ceil{\cm'/\mu^{2b}}$ edge-disjoint paths in graph $G$, where every path has an edge of $\tilde E'=E_1$ as its first edge, and an edge of $\tilde E''$ as its last edge, and it does not contain any vertices of $K$ as inner vertices. Abusing the notation, we denote this path set by $\pset$ as well. We partition path set $\pset$ into two $z$ subsets $\pset^1,\ldots,\pset^z$, as follows: consider any path $P\in \pset$. Recall that the last edge of $P$ lies in $\tilde E=\bigcup_{i=1}^z\delta_G(J_i)$. We add path $P$ to set $\pset^i$ if the last edge of $P$ lies in $\delta_G(Z_i)$. Clearly, there must be an index $1\leq i\leq z$, such that $|\pset^i|\geq \frac{|\pset|}z \geq \frac{\cm'}{\mu^{2b}\cdot z}\geq \frac{\cm'}{\mu^{2b+100}}\geq \frac{m}{\mu^{2b+100}}$. We then let $\pset'$ be that path set $\pset_i$. Observe that, if $i=i^*$, then $\pset'$ is a promising path set of type $2$, and every path in $\pset'$ has an edge of $E_1$ as its first edge, and an edge of $E_2$ as its last edge. Otherwise, $\pset'$ is a promising path set of type $3$. We let $i^{**}$ be the index for which the last edge of every path in $\pset'$ lies in $\delta_G(J_{i^{**}})$ (so it is possible that $i^{**}=i^*$).

Note that the existence of the path set $\pset'$ implies that $m\geq \cm'/\mu^{2b}$ holds. Let $\pset''\subseteq \pset'$ be an arbitrary subset of $\ceil{\frac{4m}{\mu^{3b}}}$ paths. We construct an enhancement $\Pi=(P_1,P_2)$ from the path set $\pset''$ exactly like in the algorithm for \procsplit. Recall that the algorithm first constructs a collection $\pset^*$ of edge-disjoint non-transversal paths using the paths in $\pset''$, and then selects one or two such paths into the enhancement. The only difference is that the parameter $k'=|\pset^*|$ is now somewhat smaller, $k'=\ceil{\frac{4m}{\mu^{3b}}}$, and so the probability that a path $P\in \pset^*$ is selected into the enhancement is now bounded by $2\mu^{3b}/m\leq 2\mu^{5b}/\cm'$ (since, as observed above, $m\geq \cm'/\mu^{2b}$). Another difference is that, since the promising path set $\pset''$ may only be of type 2 or 3, the resulting enhancement is also guaranteed to be of type 2 or 3. We denote by $P^*_1$ and $P^*_2$ the paths of $\pset^*$ that were chosen into the enhancement (where it is possible that $P^*_2=P^*_1$), and we denote the enhancement itself by $\Pi=\set{P_1,P_2}$.


Next, we define the bad events and bound their probabilities. This part is almost identical to that in Procedure \procsplit. The main differences are that (i) the parameter $k'$ is now smaller by factor $\mu^{\Theta(1)}$, so various parameters need to be scaled by this factor; (ii) the required failure probability is smaller than that from Procedure \procsplit by factor $\mu^{\Theta(1)}$; and (iii) the drawing  of $I$ induced by the drawing $\phi$ of $\tilde I$ is no longer guaranteed to be semi-clean with respect to $K$ (instead we will exploit the fact that the edges of $W$ participate in relatively few crossings in $\phi$).

\paragraph{Good Paths and Bad Event $\event_1'$.}

We use the following modified definition of good paths.

\begin{definition}[Good path]
	We say that a path $P\in \pset^*$ is \emph{good} if the following happen:
	
	\begin{itemize}
		\item the number of crossings in which the edges of $P$ participate in $\phi$ is at most $\frac{\cro(\phi)\mu^{15b}}{4m}$; and
		
		\item there is no crossing in $\phi$ between an edge of $P$ and an edge of $W$.
	\end{itemize} A path that is not good is called a \emph{bad path}.
\end{definition}


We now bound the number of bad paths in $\pset^*$.

\begin{observation}\label{obs: number of bad paths2}
	The number of bad paths in $\pset^*$ is at most $\frac{10m}{\mu^{15b}}$.
\end{observation}

\begin{proof}
Since the paths in $\pset^*$ are edge-disjoint, and every crossing involves two edges, the number of paths $P\in \pset^*$ such that there are more than $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ in which the edges of $P$ participate, is at most $\frac{8m}{\mu^{15b}}$. Additionally, we are guaranteed that $|\chi^{\dirty}(\phi)|\le \frac{\cm'}{\mu^{60b}}\leq \frac m{\mu^{58b}}$ (since $m\geq \frac{\cm'}{\mu^{2b}}$). Therefore, the number of paths $P\in \pset^*$, for which there is a crossing between an edge of $P$ and an edge of $\cK$ is bounded by  $\frac m {\mu^{58b}}$.

Lastly, we are guaranteed that the total number of crossings in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\frac{\cro(\phi)\mu^{26b}}{\cm'}\leq \frac{\cm'}{\mu^{17b}}\leq \frac{m}{\mu^{15b}}$, since $\cro(\phi)\leq \frac{(\cm')^2}{\mu^{60b}}$.
Overall, the number of bad paths in $\pset^*$ is bounded by $\frac{10m}{\mu^{15b}}$.
\end{proof}


We say that bad event $\event_1$ happens if at least one of the paths $P_1^*,P_2^*$ that was chosen from $\pset^*$ in order to construct the enhancement is bad. Since the number of bad paths is bounded by $\frac{4m}{\mu^{15b}}$, and a path of $\pset^*$ is chosen to the enhancement with probability at most $\frac{2\mu^{3b}}{m}$, we immediately get the following observation.

\begin{claim}\label{claim: event 1 prob2}
	$\prob{\event_1'}\leq 8/\mu^{12b}$.
\end{claim}

\paragraph{Heavy and Light Vertices, and Bad Event $\event_2'$.}

We use a parameter $h=\frac{\cro(\phi)\mu^{31b}}{m}$. We say that a vertex $x\in V(G)$ is \emph{heavy} if at least $h$ paths of $\pset^*$ contain $x$; otherwise, we say that $x$ is \emph{light}.
As before, we denote by $E'$ the set of all edges $e\in E(G)$, such that $e$ is incident to some light vertex $x$ that lies in $V(P^*_1)\cup V(P^*_2)$, and $e\not\in E(\firstpath)\cup E(\secondpath)$. We say that bad event $\event_2'$ happens if $|E'|>\frac{\cro(\phi)\mu^{48b}}{m}$.
We now bound the probability of bad event $\event_2'$.

\begin{claim}\label{claim: second bad event bound2}
	$\prob{\event_2'}\leq 1/\mu^{12}$.
\end{claim}
\begin{proof}
	Consider some light vertex $x\in V(G)$. Since $x$ lies on fewer than $h$ paths of $\pset^*$, and each such path is chosen to the enhancement with probability at most $2\mu^{3b}/m$, the probability that $x$ lies in $V(P_1^*)\cup V(P^*_2)$ is bounded by $\frac{2h\mu^{3b}}{m}$.
	
	Consider now some edge $e=(x,y)\in E(G)$. Edge $e$ may lie in $E'$ only if $x$ is a light vertex lying in $V(P_1^*)\cup V(P^*_2)$, or the same is true for $y$. Therefore, the probability that $e\in E'$ is at most $ \frac{4h\mu^{3b}}{m} $, and $\expect{|E'|}\leq 4h\mu^{3b}\leq \frac{4\cro(\phi)\mu^{35b}}{m}$, since $h=\frac{\cro(\phi)\mu^{31b}}{m}$. From Markov's inequality, $\prob{|E'|>\frac{\cro(\phi)\mu^{48b}}{m}}\leq \frac{1}{\mu^{12b}}$.
\end{proof}









\paragraph{Unlucky Paths and Bad Event $\event_3'$.}
The definition of unlucky paths is identical to that in the proof of \Cref{thm: procsplit}, except that we use a slightly different parameter. 

\begin{definition}[Unlucky Paths]
	Let $x\in V(G)\setminus V(K)$ be a vertex, and let $P\in \pset^*$ be a good path that contains $x$. Let $e,e'$ be the two edges of $P$ that are incident to $x$. Let  $\hat E_1(x)\subseteq \delta_G(x)$ be the set of edges $\hat e\in \delta_G(x)$, such that $\hat e$ lies between $e$ and $e'$ in the rotation $\oset_x\in \Sigma$ (in clock-wise orientation), and $\hat e$ lies on some good path of $\pset^*$. Let $\hat E_2(x)\subseteq \delta_G(x)$ be the set of edges $\hat e\in \delta_G(x)$, such that $\hat e$ lies between $e'$ and $e$ in the rotation $\oset_x\in \Sigma$ (in clock-wise orientation), and $\hat e$ lies on some good path of $\pset^*$.
	We say that path $P$ is \emph{unlucky with respect to vertex $x$} if either  $|\hat E_1(x)|<\frac{\cro(\phi)\mu^{15b}}{m}$ or $|\hat E_2(x)|< \frac{\cro(\phi)\mu^{15b}}{m}$ holds.
	We say that a path $P\in \pset^*$ is an \emph{unlucky path} if there is at least one heavy vertex $x\in V(G)\setminus V(K)$, such that $P$ is unlucky with respect to $x$.
\end{definition}

We use the following claim in order to bound the number of unlucky paths. The claim 
is an analogue of \Cref{claim: bound unlucky paths}, and its proof is almost identical, with minor changes due to difference in parameters. For completeness, we include a proof in Section \ref{sec: bound unlucky paths2} of Appendix.

\begin{claim}\label{claim: bound unlucky paths2}
	Assume that Event $\event_1'$ did not happen. Then for every vertex $x\in V(G)\setminus V(K)$, the total number of good paths in $\pset^*$ that are unlucky with respect to $x$ is at most $\frac{2^{14}\cro(\phi)\mu^{15b}}{m}$.
\end{claim}



We say that bad event $\event'_3$ happens if at least one of $P_1^*$, $P_2^*$ is an unlucky path. 

\begin{claim}\label{claim: third event bound2}
	$\prob{\event'_3}\leq 9/\mu^{12b}$.
\end{claim}

\begin{proof}
	Clearly, $\prob{\event'_3}\leq \prob{\event'_1}+\prob{\event'_3\mid \neg\event'_1}$. From \Cref{claim: event 1 prob2},
	$\prob{\event'_1}\leq 8/\mu^{12b}$. We now bound $\prob{\event_3'\mid \neg\event_1'}$.
	
	
	Recall that a heavy vertex must have degree at least $h=\frac{\cro(\phi)\mu^{31b}}{m}$ in $G$. Therefore, the total number of heavy vertices in $G$ is at most $\frac{2m}{h}\leq \frac{2m^2}{ \cro(\phi)\mu^{31b}}$. From \Cref{claim: bound unlucky paths2}, if Event $\event'_1$ did not happen, then for every heavy vertex $x\in V(G)\setminus V(K)$, there are at most $\frac{2^{14}\mu^{15b}\cro(\phi)}{m}$ paths in $\pset^*$ that are good and unlucky for $x$. Therefore, the total number of good paths in $\pset^*$ that are unlucky with respect to some heavy vertex is at most:
	%
	\[\frac{2m^2}{ \cro(\phi)\mu^{31b}}\cdot \frac{2^{14}\mu^{15b}\cro(\phi)}{m} 
	\leq \frac{2^{15}\cdot m}{\mu^{16b}}.
	\]
	%
	Since $|\pset^*|\geq  \frac{4m}{\mu^{3b}}$, from	\Cref{obs: number of bad paths2}, at least $ \frac{2m}{\mu^{3b}}$ paths in $\pset^*$ are good.
	
	We select two paths into the enhancement $\Pi$, and, if Event $\event_1'$ did not happen, every good path is equally likely to be selected. Therefore, the probability that a good path that is unlucky is selected into the enhancement, conditioned on the event $\event_1$ not happening is bounded by:
	%
	\[\frac{2^{15}\cdot m}{\mu^{16b}}\cdot  \frac{\mu^{3b}}{m}\leq \frac{2^{15}}{\mu^{13b}}\leq \frac{1}{\mu^{12b}}, \]
	%
	since $\mu$ is large enough. We conclude that $\prob{\event'_3\mid \neg\event'_1}\leq 1/\mu^{12b}$, and 	$\prob{\event'_3}\leq 9/\mu^{12b}$.	
\end{proof}





Recall that we have denoted by $E'$ the set of all edges that are incident to the light vertices of $\firstpath\cup \secondpath$, excluding the edges of $E(\firstpath)\cup E(\secondpath)$. 


Denote $\tilde G'=\tilde G\setminus E'$, and let $\tilde \Sigma'$ be the rotation system for graph $G'$ induced by $\tilde \Sigma$. For convenience, we also denote $G'=G\setminus E'$ and we let $\Sigma'$ be the rotation system for graph $G'$ induced by $\tilde \Sigma$. Denote $\tilde I'=(\tilde G',\tilde \Sigma')$, and $I'-(G',\Sigma')$. Let $\Pi=\set{P_1,P_2}$ be the enhancement of skeleton $K$ that we have constructed. We denote $K'=K\cup P_1\cup P_2$, and we let $W'=W\cup P_1\cup P_2$ be the new augmentation of the original skeleton $\cK$ for graph $\cG'$.  Drawing $\phi$ of graph $\tilde G=\cG'\setminus E^{\del}$ naturally defines a drawing of graph $\tilde G'$. Moreover, if Event $\event'_1$ did not happen, then there are no crossings in this drawing between the edges of $E(P_1)\cup E(P_2)$ and the edges of $E(W)$. However, it is possible that this drawing contains crossings between pairs of edges in $E(P_1)\cup E(P_2)$. In the next claim we show that, if events $\event'_1$ and $\event'_3$ did not happen, then drawing $\phi$ can be modified to obtain a drawing $\phi'$ of $\tilde G'$, in which the edges of $W'$ do not cross each other, and the induced drawing of $W$ remains identical to that induced by $\phi$. 
We do so in the following claim, that is an analogue of \Cref{claim: new drawing}.
%The proof of the following claim is deferred to Section \ref{sec:getting new drawing} of Appendix.

\begin{claim}\label{claim: new drawing2}
	Assume that neither of the events $\event'_1$ and $\event'_3$ happened. Then there is a  solution $\phi'$ to instance $\tilde I'=(\tilde G',\tilde \Sigma')$, in which there are no crossings between pairs of edges in $E(W')$. Moreover, the drawing of $W$ induced by $\phi'$ is identical to the drawing of $W$ induced by $\phi$, drawing $\phi'$ is $\wset$-compatible, and, for every edge $e\in E(\tilde G')$, the number of crossings in which $e$ participates in $\phi'$ is bounded by the number of crossings in which $e$ participates in $\phi$. In particular,
	$\cro(\phi')\leq \cro(\phi)$ and $\chi^{\dirty}(\phi')\subseteq \chi^{\dirty}(\phi)$ hold.
\end{claim}

The proof of \Cref{claim: new drawing2} is essentially identical to the proof of \Cref{claim: new drawing}. Recall that the main idea in the proof is to remove, one by one, the loops in the images of the paths $P_1,P_2$ in the drawing $\phi$. The reason these loops can be removed without increasing the number of crossings is that every vertex whose image lies on such a loop must be a light vertex (see, e.g., \Cref{obs: no heavy vertices on loops}). This, in turn, relies on the fact that the parameter used in the definition of unlucky paths is greater than the parameter used in the definition of bad paths. While both parameters are now scaled by factor $\mu^{\Theta(b)}$, this relationship between them continues to hold, and so the analogue of  \Cref{obs: no heavy vertices on loops} continues to hold as well. We also need to show that the analogue of \Cref{obs: case 3 not crossing} continues to hold, that is, there are no crossings $(e,e')_p$ in $\phi$ where $e\in E(P_1)$ and $e'\in E(P_2)$. The proof of the observation relies on the fact that that the parameter bounding the number of crossings in which the edges of a good path may participate (denoted by $N$), is less than $k'/100$, and that the number of bad paths in $\pset^*$ is bounded by $k'/16$. While both parameters $N$ and $k'$ are now different, namely $N=\frac{\cro(\phi)\mu^{15b}}{4m}$ and $k'=4m/\mu^{3b}$, it is still the case that $N<k'/100$ (since, from Condition \ref{prop: drawing}, $\cro(\phi)\leq (\cm')^2/\mu^{60b}$, and $m\geq \cm'/\mu^{2b}$). The number of bad paths is bounded by  $\frac{10m}{\mu^{15b}}<k'/16$ from \Cref{obs: number of bad paths2}. The remainder of the proof of  \Cref{claim: new drawing2} is identical to the proof of \Cref{claim: new drawing} and is omitted here.

As before, drawing $\phi'$ of $\tilde G'$ is derived from drawing $\phi$ of $\tilde G$, and neither are known to our algorithm. Note that, since $\jset_{i^*}$ is a valid core structure for instance $I$, the image of the paths $P_1,P_2$ of the enhancement in $\phi'$ must intersect the region $F$. If Event $\event_1'$ does not happen, then the images of paths $P_1,P_2$ do not cross the images of the edges of $W$ in $\phi$, and so the images of both paths are contained in region $F$. This remains true for drawing $\phi'$ of graph $\tilde G'$. Therefore, in the drawing of the new augmented skeleton $W'$ induced by $\phi'$, the images of the edges of $W'$ do not cross each other, and the images of paths $P_1,P_2$ are contained in region $F$. It is easy to verify that the images of the two paths partition face $F$ into two new regions, that we denote by $F_1$ and $F_2$.






\paragraph{Terrible Vertices and Bad Event $\event'_4$.}

As before, for a vertex $x\in V(G)$, we denote by $N(x)$ the number of paths in $\pset^*$ containing $x$, by $N^{\bad}(x)$ the number of bad paths in $\pset^*$ containing $x$, and  by $N^{\good}(x)$ the number of good paths in $\pset^*$ containing $x$. The definition of the notion of a terrible vertex remains the same as before:

\begin{definition}[Terrible Vertex]
	A vertex $x\in V(G)$ is \emph{terrible} if it is a heavy vertex, and $N^{\bad}(x)\geq N^{\good}(x)/64$.
\end{definition}


As before, we say that a bad event $\event'_4$ happens if any vertex of $\firstpath\cup \secondpath$ is a terrible vertex. We bound the probability of Event $\event'_4$ in the following claim, whose proof is essentially identical to the proof of \Cref{claim: no terrible vertices}. Since we use slightly different parameters, we provide the proof here for completeness.

\begin{claim}\label{claim: no terrible vertices2}
	$\prob{\event_4'}\leq \frac{2^{14}\log m}{\mu^{12b}}$.
\end{claim}

\begin{proof}
	Let $U$ be the set of all heavy vertices of $G$. We group the vertices $x\in U$ geometrically into classes, using the parameter $N(x)$. Recall that $h=\frac{\cro(\phi)\mu^{31b}}{m}$, and, for every heavy vertex $x\in U$, $N(x)\geq h$. Let $q=2\ceil{\log m}$. For $1\leq i\leq q$, we let the class $S_i$ contain all vertices $x\in U$ with $2^{i-1}\cdot h\leq N(x)<2^i\cdot h$. 
	Let $S'_i\subseteq S_i$ be the set containing all terrible vertices of $S_i$. For every vertex $x\in S'_i$, $N^{\bad}(x)\geq N^{\good}(x)/64$. Since $N(x)=N^{\bad}(x)+N^{\good}(x)$, we get that $N^{\bad}(x)\geq N(x)/65\geq 2^{i-1}\cdot h/65$. From \Cref{obs: number of bad paths2}, the total number of bad paths is at most $\frac{10m}{\mu^{15b}}$, so
	%
	\[|S'_i|\leq  \frac{10m/\mu^{15b}}{2^{i-1}\cdot h/65}\leq \frac{650m}{ 2^{i-1}\cdot h\cdot \mu^{15b}}.\] %  =\frac{9m^2}{ 2^{i-1}\cdot \cro(\phi)\mu^{2150}}, \]
	%since $h=\cro(\phi)\mu^{1450}/m$.
	Recall that the probability that a path $P\in \pset^*$ is selected into the enhancement is at most $\frac{2\mu^{3b}}{m}$. A vertex $x\in S'_i$ may lie in $V(\firstpath)\cup V(\secondpath)$ only if at least one of the $N(x)$ paths of $\pset^*$ containing $x$ is selected into the enhancement. Therefore, $\prob{x\in (V(\firstpath)\cup V(\secondpath))}\leq \frac{2\mu^{3b}\cdot N(x)}{m}\leq \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}$.
	
	
	Overall, the probability that some vertex of $S'_i$ belongs to $V(\firstpath)\cup V(\secondpath)$ is at most 
	$$|S'_i|\cdot \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}\leq \frac{650m}{ 2^{i-1}\cdot h\cdot \mu^{15b}}\cdot \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}\leq \frac{2^{12}}{\mu^{12b}}.$$ 
	
	Using the union bound over all $q=2\ceil{\log m}$ classes, we get that the probability of Event $\event'_4$ is bounded by $\frac{2^{14}\log m}{\mu^{12b}}$.
\end{proof}


\paragraph{Bad Event $\event'$.}
Let $\event'$ be the bad event that at least one of the events $\event'_1,\event'_2,\event'_3,\event'_4$ happen. From the Union Bound and Claims \ref{claim: event 1 prob2}, \ref{claim: second bad event bound2}, \ref{claim: third event bound2} and \ref{claim: no terrible vertices2}, $\prob{\event'}\leq O\left( \frac{\log m}{\mu^{12b}}\right ) \leq \frac{1}{\mu^{11b}}$, by definition of $\mu$.


\subsubsection{Step 2: Completing the Construction of $\wset'$ and $\gset'$}


In this step we complete the construction of the skeleton augmenting structure $\wset'$ and of the $\wset'$-decomposition of $\cG'$ $\gset'$. This step is very similar to the second step of Procedure \procsplit, with several key differences. The first difference is that we no longer need to take care of the case where $\Pi$ is a type-1 enhancement. The second difference is that the parameters are now somewhat different. The third difference, which is more major than the first two, is that we will not be able to guarantee that the final drawing of the graph $\tilde G\setminus E^{\del}(F)$ that we obtain, induces drawings of graphs $G_{F_1},G_{F_2}$ that are semi-clean with respect to their skeletons. We will still, however, need to ensure that the drawing is $\wset'$-compatible, so every core of $\set{J_1,\ldots,J_z}$ is drawn in the ``correct'' face (for example, if $J_i\subseteq G_{F_1}$, then core $J_i$ should be drawn inside). This will require an additional step, in which we disconnect some of the cores from the corresponding graph $G_1$ or $G_2$.

We consider the instance $I'=(G',\Sigma')$, where $G'=\tilde G\setminus E'$, and $\Sigma'$ is the rotation system for $G'$ induced by $\cSigma'$. We will also consider the solution $\phi'$ to instance $I'$ given by  \Cref{claim: new drawing} (assuming that bad event $\event'$ did not happen).

We start by computing an orientation $b'_u$ for every vertex $u\in V(W')$, and a drawing $\rho_{C'}$ of every connected component $C'\in \cset(W')$. We then split graph $G$ into two subgraphs $G_1$ and $G_2$, and complete the construction of the skeleton augmenting structure. Lastly, we will remove some additional edges from the resulting graph, to ensure that there is a good drawing of that graph that is $\wset'$-compatible.
We consider two cases, depending on whether the original promising path $\pset$ was of type $2$ or $3$.



\subsubsection*{Case 1: $\pset$ was a type-2 promising  path set}

The first case happens when the promising path set $\pset$ was of type-2. Recall that the endpoints of all paths in $\pset$ are contained in $V(\thecore)$, and we have computed a partition $(E_1,E_2)$ of the edges of $\delta_G(\thecore)$, so the edges of $E_1$ are consecutive in the ordering $\oset(\thecore)$. Recall that, in this case, $\Pi=\set{P_1,P_2}$, where $P_1$ is either a path or a cycle that contains an edge of $E_1$ as its first edge, and an edge of $E_2$ as its second edge, and $P_2=\emptyset$. For convenience of notation, we denote $P_1$ by $P$.

Recall that, from \Cref{claim: new drawing2}, if Event $\event'$ does not happen, then  drawing $\phi'$ of $G'$ contains no crossings between the edges of $E(W')$. 
Throughout, we denote by $\gamma$ the image of the path $P$ in $\phi'$. 

In order to construct the skeleton augmenting structure $\wset'$, we first let $W'=W\cup P$ be the skeleton augmentation associated with $\wset'$. Next, we define a drawing $\rho_C$ for every component $C\in \cset(W)$.

Let $C^*\in \cset(W)$ be the connected component with $\thecore\subseteq C^*$, and denote by $\tilde C=C^*\cup P$. Since path $P$ must be internally disjoint from all vertices of $W$, it is immediate to verify that $\cset(W')=(\cset(W)\setminus C^*)\cup \tilde C)$. For every component $C\in \cset(W')\setminus \set{\tilde C}$, its drawing $\rho_C$ in $\wset'$ remains the same as in $\wset$. Consider now the component $\tilde C$. Recall that we are given, as part of skeleton augmenting structure $\wset$ a drawing $\rho_{C^*}$ of graph $C^*$ and an orientation $b'_u$ of every vertex $u\in V(C^*)$. We are also given a face $F'\in \fset(\rho_{C^*})$, such that the face $F$ in drawing $\phi$ is contained in the region $F'$. Since drawing $\phi'$ is $\wset$-compatible, and it does not contain any crossings between the edges of $W'$, we are guaranteed that path $P$ is drawn inside the region $F'$ of $\phi'$, in a natural way. Since the orientations of all vertices of $C^*$ in $\phi'$ are consistent with those given by $\wset$, and since the drawing of $C^*$ induced by $\phi'$ is $\rho_{C^*}$, we can efficiently compute a drawing $\rho_{\tilde C}$ of graph $\tilde C$, that is identical to the drawing of $\tilde C$ induced by $\phi'$. This drawing of $\tilde C$ is a unique planar drawing of the graph that has the following properties:

\begin{itemize}
	\item the drawing of $C^*$ induced by $\rho_{\tilde C}$ is $\rho_{C^*}$;
	\item the image of path $P$ is contained in region $F'$; 
	\item the drawing is consistent with the rotation system $\cSigma'$; and
	\item  the orientation of every vertex $u\in V(C^*)$ in the drawing is the orientation $b'_u$ given by $\wset'$.
\end{itemize}

If $F=F^*(\rho_{C^*})$, then we will designate one of the face $F_1$ or $F_2$ as the outer face of the drawing $\rho_{\tilde C}$ later.


So far we have defined the new skeleton augmentation $W'$ and a drawing $\rho_C$ of every connected component $C\in \cset(W)$. Next, we define the orientation $b'_u$ of every vertex $u\in V(W')$. For vertices $u\in V(W')\cap V(W)$, the orientation $b'_u$ in $\wset'$ remains the same as the orientation $b'_u$ in $\wset$. It now remains to define the orientation $b'_u$ of vertices $u\in V(P)\setminus V(C^*)$. The procedure for computing these orienttions is very similar to the one from Procedure $\procsplit$.


We first recall the definition of the circular ordering $\oset(\thecore)$ of the edges of $\delta_G(\thecore)$.  In order to define the ordering, we considered the disc $D(\thecore)$ in the drawing $\rho_{\thecore}$ of $\thecore$ defined by the core structure $\jset_{i^*}$. Recall that the drawing $\rho_{\thecore}$ is the drawing of $\thecore$ induced by the drawing $\rho_{C^*}$ of $C^*$. In this drawing, the orientation of every vertex $u\in V(\thecore)$ is $b'_u$. We have defined, for every edge $e\in \delta_G(\thecore)$, a point $p(e)$ on the boundary of the disc $D(\thecore)$, and we let $\oset(\thecore)$ be the circular ordering of the edges of $\delta_G(\thecore)$, in which the  points $p(e)$ corresponding to these edges  appear on the boundary of the disc $D(\thecore)$, as we traverse it in counter-clock-wise direction. If the drawing of $\thecore$ in $\phi'$ is identical to $\rho_{\thecore}$ (including the orientation), then we say that the orientation of the ordering $\oset(\thecore)$ in $\phi'$ is $1$. In this case, we are guaranteed that for every vertex $u\in V(\thecore)$, its orientation in $\phi'$ is $b'_u$. Otherwise, the drawing of $\thecore$ in $\phi'$ is the mirror image of $\rho_{\thecore}$. We then say that the orientation of the ordering $\oset(\thecore)$ in $\phi'$ is $-1$. In this case, we are guaranteed that for every vertex $u\in V(\thecore)$, its orientation in $\phi'$ is $-b'_u$.


For every vertex $u\in V(P)\cup V(\thecore)$, we consider the tiny $u$-disc $D_{\phi'}(u)$ in the drawing $\phi'$.  For every edge $e\in \delta_{G}(u)\setminus E'$, we denote by $\sigma(e)$ the segment of $\phi'(e)$ that is drawn inside the disc $D_{\phi'}(u)$. Since edge $e$ belongs to graph $G$, $\sigma(e)$ must be contained in the region $F\in \fset(W)$ of the drawing $\phi'$.  Let $\tilde E=\left (\bigcup_{u\in V(P)\cup V(\thecore)}\delta_{G'}(u)\right )\setminus (E(P)\cup E(\thecore))$. 
The image of path $P$ in $\phi'$ splits region $F$ into two regions, that we denote by $F_1$ and $F_2$. We let $e_1\in E_1$ be any edge that does not lie on path $P$, and we assume without loss of generality that $\sigma(e_1)\subseteq F_1$.

We partition edge set $\tilde E$ into a set $\tilde E^{\inn}$ of \emph{inner edges} and the set $\tilde E^{\out}$ of outer edges, as before: Edge set $\tilde E^{\inn}$ contains all edges $e\in \tilde E$ with $\sigma(e)$ contained in the face $F_1$ of $\tilde \rho$, and $\tilde E^{\out}$ contains all remaining edges (so for every edge $e\in \tilde E^{\out}$, $\sigma(e)$ is contained in $F_2$). As before, we show an algorithm that correctly computes the orientation of every vertex $u\in V(P)$ in the drawing $\phi'$, and the partition $(\tilde E^{\inn},\tilde E^{\out})$ of the edges of $\tilde E$.


\paragraph{Computing Vertex Orientations on Path $P$ and the Partition $(\tilde E^{\inn},\tilde E^{\out})$.}

The algorithm for computing vertex orientations for vertices of $P$, and the partition $(\tilde E^{\inn},\tilde E^{\out})$ of the edges of $\tilde E$ is identical to that from Procedure \procsplit. The main difference is the change in the parameters. We provide the algorithm and its analysis for completeness.

Consider any vertex $u\in V(P)$. Let $\hat e(u)$, $\hat e'(u)$ be the two edges of $P$ that are incident to $u$, where we assume that $\hat e(u)$ appears earlier on $P$ (we assume that $P$ is directed from an edge of $E_1$ to an edge of $E_2$). Edges $\hat e(u),\hat e'(u)$ partition the edge set $\delta_{G'}(u)\setminus\set{\hat e(u),\hat e'(u)}$ into two subsets, that we denote by $\hat E_1(u)$ and $\hat E_2(u)$, each of which appears consecutively in the rotation $\oset_u\in \Sigma'$.
Note that either (i) $\hat E_1(u)\subseteq \tilde E^{\inn}$ and $\hat E_2(u)\subseteq \tilde E^{\out}$ holds, or (ii) $\hat E_2(u)\subseteq \tilde E^{\inn}$ and $\hat E_1(u)\subseteq \tilde E^{\out}$ holds.


We now construct edge sets $\tilde E_1',\tilde E_2'$, and fix an orientation $b'_u$ for every vertex $u\in V(P)\setminus V(\thecore)$. We then show that $\tilde E_1'=\tilde E^{\inn}$, $\tilde E_2=\tilde E^{\out}$, and that the orientations of all vertices of $P$ that we compute are consistent with the drawing $\phi'$.

Recall that we have computed a drawing $\rho_{\tilde C}$ of $\tilde C=C^*\cup P$, that is identical to the drawing of $\tilde C$ induced by $\phi'$. We let $\tilde \rho$ be the drawing of $\thecore\cup P$ that is induced by $\rho_{\tilde C}$.
Since we have assumed that $\sigma(e_1)$ is contained in the face $F_1$, for every edge $e\in \delta_G(\thecore)$, we can correctly determine whether $e\in \tilde E^{\inn}$ or $e\in \tilde E^{\out}$. In the former case, we add $e$ to $\tilde E_1'$, and in the latter case we add $e$ to $\tilde E_2'$. 
Therefore, for every path $P'\in \pset^*$, the first and the last edges of $P$ are already added to either $\tilde E_1'$ or $\tilde E_2'$.

Next, we process every inner vertex $u$ on path $P$.
Consider any such vertex $u$. As before, if $u$ is a light vertex, then its orientation $b'_u$ can be chosen arbitrarily, as $\deg_{\tilde G'}(u)=2$. 

Assume now that $u$ is a heavy vertex. 
In order to decide on the orientation of $u$, we let $\pset(u)$ contain all paths $P'\in \pset^*\setminus\set{P}$ with $u\in P'$.  We partition the set $\pset(u)$  of paths into four subsets: set $\pset_1(u)$ contains all paths $P'$ whose first edge lies in $\tilde  E_1'$, and the first edge that is incident to $u$ lies in $\hat E_1(u)$. Set $\pset_2(u)$  contains all paths $P'$ whose first edge lies in $\tilde  E_2'$, and the first edge that is incident to $u$ lies in $\hat E_2(u)$. Similarly, set $\pset'_1(u)$ contains   all paths $P'\in \pset(u)$ whose first edge lies in $\tilde  E_1'$ and the first edge that is incident to $u$ lies in $\hat E_2(u)$, while set $\pset'_2(u)$ contains  all paths $P'\in \pset'(u)$, whose first edge lies in $\tilde  E_2'$ and the first edge that is incident to $u$ lies in $\hat E_1(u)$. We let $w(u)=|\pset_1|+|\pset_2|$, and $w'(u)=|\pset'_1|+|\pset'_2|$.
If $w(u)\leq  w'(u)$, then we set $b'_u=-1$, add the edges of $\hat E_1(u)$ to $\tilde E'_1$, and add the edges of $\hat E_2(u)$ to $\tilde E'_2$.  Otherwise we set $b'_u=1$,  add the edges of $\hat E_1(u)$ to $\tilde E'_2$, and add the edges of $\hat E_2(u)$ to $\tilde E'_1$.

This completes the algorithm for computing the orientations of the inner vertices of $P$, and of the partition $(\tilde E_1',\tilde E_2')$ of the edge set $\tilde E$.
We use the following claim to show that both are computed correctly. %The claim is an analogue of \Cref{claim: orientations and edge split is computed correctly} for Case 1. Its proof is similar, but contains some subtleties, since the images of some paths in $\pset^*$ may now cross the images of the edges of $\thecore$.

\begin{claim}\label{claim: orientations and edge split is computed correctly Case2.2}
	Assume that Event $\event'$ did not happen. If the orientation of the ordering $\oset(\thecore)$  in $\phi'$ is $1$, then for every vertex $u\in V(P)\cup V(C^*)$, the orientation of $u$ in $\phi'$ is $b'_u$.
	Otherwise, for every vertex $u\in  V(P)\cup V(C^*)$, the orientation of $u$ in $\phi'$ is $-b_u$. In either case,
	$\tilde E_1'=\tilde E^{\inn}$ and $\tilde E_2'=\tilde E^{\out}$. 
\end{claim}

\begin{proof}
	We assume without loss of generality that the orientation of the ordering $\oset(\thecore)$  in $\phi'$ is $1$. The argument for the other case is symmetric. From the above discussion, for every vertex $u\in V(\thecore)$, the orientation of $u$ in $\phi'$ is $b'_u$. It is now enough to show that, if $u\in P$ is a heavy vertex, then the orientation of $u$ in $\phi'$ is $b_u$.
	
	Recall that we denoted $N(u)=|\pset(u)|$, and we have denoted by $N^{\bad}(u)$ and $N^{\good}(u)$ the total number of bad and good paths in $\pset(u)$, respectively. Since we have assumed that bad event $\event_4'$ did not happen, vertex $u$ is not a terrible vertex, that is, $N^{\bad}(u)\leq N^{\good}(u)/64$. Since $N(u)=N^{\bad}(u)+N^{\good}(u)$, we get that $N^{\bad}(u)<N(u)/65$. 
	
	
	Assume first that the orientation of vertex $u$ in $\phi'$ is $-1$. In this case, for every edge $e\in \hat E_1(u)\cup \tilde E_1'$, the segment $\sigma(e)$ lies in face $F_1$ of $\tilde \rho$, while for every edge $e'\in \hat E_2(u)\cup \tilde  E_2'$, the segment $\sigma(e')$ lies in face $F_2$. 
	We claim that in this case $w'(u)>w(u)$ must hold, and so our algorithm sets $b_u=-1$ correctly. Indeed, assume otherwise. 
	Then $w'(u)\geq N(u)/2$. Let $\qset$ denote the set of all good paths in $\pset'_1(u)\cup \pset'_2(u)$. Then $|\qset|\geq w'(u)-N^{\bad}(u)\geq N(u)/2-N(u)/65\geq N(u)/4\geq h/4$, since $u$ is a heavy vertex. 
	We now show that, for every path $Q\in \qset$, there must be a crossing between an edge of $Q$ and an edge of $P$ in $\phi'$.
	
	Indeed, consider any path $Q\in \qset$. Since $Q\in \pset'_1(u)\cup \pset'_2(u)$, the image of the path $Q$ must cross the boundary of the face $F_1$ in $\rho$. Since path $Q$ is a good path, and it does not contain vertices of $\thecore$ as inner vertices, no inner point of the image of $Q$ in $\phi'$ may belong to the image of $\thecore$ in $\phi'$. Since the paths in $\pset$ are transversal, it then follows that there must be a crossing between an edge of $Q$ and an edge of $P$ in $\phi'$. But then the edges of $P$ participate in at least $\frac h 2\geq \frac{\cro(\phi)\mu^{31b}}{2m}$ crossings in $\phi'$, and hence in $\phi$.
	
	 However, since we have assumed that bad event $\event_1$ did not happen, $P$ is a good path, and so its edges may participate in at most 	$\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$, a contradiction. Therefore, when the orientation of $u$ in $\phi'$ is $-1$, our algorithm correctly sets $b_u=-1$. 
	In the case where the orientation of $u$ in $\phi'$ is $1$, the analysis is symmetric.
\end{proof}


In order to complete the construction of the skeleton augmenting structure $\wset'$, it remains to define, for every pair $C,C'\in \cset(W')$ of distinct connected components, a face $R_C(C')$ of $\fset(\rho_C)$. Additionally, if face $F$ is the outer face in the drawing $\rho_{C^*}$ of component $C^*$, then we need to designate one of the faces $F_1,F_2$ as the outer face of the drawing $\rho_{\tilde C}$ of component $\tilde C$. We do so in the next step, once we split the graph $G'$ into two subgraphs, $G_1$ and $G_2$.


\paragraph{Computing the Split.}

We construct a flow network $\tilde H'$ as follows. We start with $\tilde H'=G'$, and then, for all $1\leq i\leq z$ with $i\neq i^*$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$ with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $P\cup \thecore$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $\tilde H'$, and we denote by $E''=E_H(A,B)$.  The following claim, that is an analogue of \Cref{claim: cut set small case2},  bounds the cardinality of $E''$. 

\begin{claim}\label{claim: cut set small case2.2}
	If bad event $\event'$ did not happen, then $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
\end{claim}


The proof of the claim is essentially identical to the proof of \Cref{claim: cut set small case2.2}. We assume for contradiction that Event $\event'$ did not  happen, but $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
We can then use Max Flow -- Min Cut theorem to construct a collection  $\qset$ of edge-disjoint paths in graph $G'$, such that, for every path $Q\in \qset$, drawing $\phi'$ must contain at least one crossing between an edge of $Q$ and an edge of $W\cup P$. Since Event $\event'$ did not happen, path $P$ is good, so its edges participate in at most $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ and hence in $\phi'$. Additionally, edges of $\cK$ participate in at most $|\chi^{\dirty}(\phi)|$ crossings in $\phi$ (and hence in $\phi'$), and edges of $W\setminus K$ participate in at most $\frac{\cro(\phi)\cdot \mu^{26b}}{\cm'}\leq \frac{\cro(\phi)\cdot \mu^{26b}} m$ crossings from Property \ref{prop: drawing}. Overall, there are fewer than $\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ crossings in $\phi'$ in which edges of $P\cup W$ participate, a contradiction.






We now construct the initial graphs $G_1,G_2$ associated with the faces $F_1$ and $F_2$, respectively; the final graphs $G_1',G_2'$ will be obtained by deleting some edges from $G_1$ and $G_2$.
In order to do so, we define two vertex sets $A',B'$ in graph $G'$, as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every index $1\leq i\leq r$ with $i\neq i^*$, if $v_{J_i}\in A$, then we replace $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 


Additionally, we let $J\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F$. Similarly, we let $J'\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F_2$. 

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J)$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma'$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. 
We need the following observation that, intuitively, shows that graphs $G_1$ and $G_2$ are significantly smaller than the original graph $G$.

\begin{observation}\label{obs: few edges in split graphs case2.2}
	If Event $\event$ did not happen, then $|E(G_1)\setminus E(W')|,|E(G_2)\setminus E(W')|\leq |E(G)\setminus E(W)|-\frac{\cm'}{\mu^{5b}}$.
\end{observation}

The proof of the observation is identical to the proof of \Cref{obs: few edges in split graphs case2}, and follows from the fact that, from the definition of the process for computing an enhancement, at least $k'/4$ edges of $E_1$ must lie in $\tilde E_1'$, and at least $k'/4$ edges of $E_1'$ must lie in $\tilde E_2$.  Since $k'=\ceil{\frac{4m}{\mu^{3b}}}$ and $m\geq \cm'/\mu^{2b}$, the claim follows. 


Let $\tilde G''=\tilde G'\setminus E''=\tilde G\setminus (E'\cup E'')$, and let $\tilde \Sigma''$ be the rotation system for graph $\tilde G''$ induced by $\tilde \Sigma$. We denote $\tilde I''=(\tilde G'',\tilde \Sigma'')$ the resulting instance of \cnwrs.
Let $\phi''$ be the drawing of $\tilde G''$ that is induced by the drawing $\phi'$ of $\tilde G'$. We also denote $G''=G'\setminus E''=G\setminus (E'\cup E'')$. Notice that $E(G_1)\cup E(G_2)=E(G'')$.

We now complete the construction of the skeleton augmenting structure $\wset'$. For all $1\leq i\leq z$, let $C_i\in \cset(W)$ be the connected component that contains the core $J_i$, and let $F^i\in \fset(\rho_{C_i})$ be the face that corresponds to face $F$ of $\tilde \fset(\wset)$ (in other words, face $F$ in the drawing of $W$ induced by $\phi$ is contained in region $F^i$). From the construction of the set $\tilde \fset(\wset)$ of faces, in the decomposition forest $H(\wset)$, either  vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees in the forest; or one of these vertices is the parent-vertex of the remaining vertices. We assume w.l.o.g. that in the latter case, vertex $x_{C_1}$ is the parent of vertices $x_{C_2},\ldots,x_{C_z}$ in the forest $H(\wset)$.


Consider any pair $C,C'\in \cset(W')$ of distinct connected components. Assume first that $C,C'\neq \tilde C$. In this case, face $R_{C}(C')$ remains the same in $\wset'$ in the augmenting structure $\wset$. Since drawing $\phi$ if $\tilde G$ was $\wset$-compatible, and drawing $\phi''$ is obtained from $\phi$ by deleting some edges that do not belong to $W'$, and possibly making some additional local changes within the region $F$, the image of component $C'$ in $\phi''$ remains contained in face $R_C(C')$.


Assume now that $C'=\tilde C$. In this case, we let the face $R_{C'}(\tilde C)$ in $\wset'$ be the face $R_{C'}(C_{i^*})$ of $\wset$. It is easy to verify that the drawing of component $\tilde C$ in $\phi''$ remains in the region $R_{C'}(C_{i^*})$.

Next, we assume that $C=\tilde C$. Recall that component $C_{i^*}$ of $W$ is replaced by component $\tilde C=C_{i^*}\cup P$ in $W'$. Assume first that $C'\not\in\set{C_1,\ldots,C_z}$. Then face $R=R_{C_{i^*}}(C)$ in $\wset$ is differen from the face $F^{i^*}\in \fset(\rho_{C_{i^*}})$ (which in turn corresponds to face $F$). Then $R$ remains a face of $\fset(\rho_{\tilde C})$, and we set $R_{\tilde C}(C)=R$. Using the same reasoning as above, the image of component $C'$ in $\phi''$ is indeed contained in region $R$.

Lastly, assume that $C=\tilde C$ and $C'=C_i$ for some $1\leq i\leq z$ with $i\neq i'$. Assume first that $i^*=1$, and vertex $x_{C_1}$ is the parent vertex of vertices $x_{C_2},\ldots,x_{C_z}$. In this case, face $F^1\in \fset(\rho_{C_1})$ is not the infinite face $F^*(\rho_{C_1})$, and $R_{C_i}(C_1)=F^*(\rho_{C_i})$ in $\wset$. Face $F^1$ of $\rho_{C_1}$ is partitioned into two faces in $\rho_{\tilde C}$, that we denote by $F^1_1$ and $F^1_2$, respectively. If $J_i\subseteq G_1$, then we set $R_{C_1}(C_i)=F^1_1$, and otherwise we set $R_{C_1}(C_i)=F^1_2$. (We note that in this case we are not guaranteed that the image of component $C_i$ in $\phi''$ is contained in the ``correct'' region; we fix this later).

If vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees of $H(\wset)$, then we define the regions $R_{\tilde C}(C_i)$ for $i\neq i^*$ similarly. In this case, face $F^{i^*}$ is the infinite face of drawing $\rho_{C_{i^*}}$, and we designate one of the two new faces $F^{i^*}_1,F^{i^*}_2$ of drawing $\rho_{\tilde C}$ (that are both contained in $F^{i^*}$) as the infinite face arbitrarily.

Lastly, we assume that $i^*\neq 1$, and vertex $x_{C_1}$ is the parent vertex of vertices $x_{C_2},\ldots,x_{C_z}$. In this case, face $F^{i^*}$ is the infinite face of drawing $\rho_{C_{i^*}}$. As before, face $F^{i^*}$ of $\rho_{C_{i^*}}$ is partitioned into two new faces, $F^{i^*}_1$ and $F^{i^*}_2$ in drawing $\rho_{\tilde C}$. If $J_1\subseteq G_1$, then we let $F^{i^*}_1$ be the infinite face of the drawing $\rho_{\tilde C}$, and otherwise we let $F^{i^*}_2$ be the infinite face of  $\rho_{\tilde C}$. For all $1\leq i\leq z$ with $i\neq i^*$, if $J_i\subseteq G_1$ then we let $R_{\tilde C}(C_i)=F^{i^*}_1$, and otherwise we let $R_{\tilde C}(C_i)=F^{i^*}_2$. 

This completes the definition of the new skeleton augmneting structure $\wset'$.
At this point, we could set $E^{\del}=E'\cup E''$, and define $\gset'=(\gset\setminus G)\cup (G'_1\cup G'_2)$, letting $G'_1$ be associated with face $F_1\in \tilde \fset(\wset')$, $G'_2$ with face $F_2$, and each remaining graph of $\gset'$ with the same face as before. The resulting collection $\gset'$ of graphs would indeed be a valid $\wset'$-decomposition of graph $\tilde G''$. But unfortunately the drawing $\phi''$ of $\tilde G''$ is not necessarily $\wset'$-compatible. This is because it is possible that some connected component $C_i$, whose corresponding core $J_i$ is contained in graph $G_1'$ is not drawn in face $F_1$, and similarly, for some connected component $C_{i'}$ with $J_{i'}\subseteq G_2'$, it is possible that $C_{i'}$ is not drawin in $F_2$. In the next step, we ``fix'' this issue, by possibly removing some additional edges from graph $\tilde G'$. We start with the following observation.


\begin{observation}\label{obs: disconnect cores} Assume that Event $\event'$ did not happen.
	Consider any index $1\leq i\leq z$ with $i\neq i^*$, such that $J_i\subseteq G_1$ but the image of $C_i$ in $\phi''$ is not contained in $F_1$. Then there is a collection $\hat E_i\subseteq E(G_1)\setminus E(W')$ of at most 
	$\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ edges, such that in graph $G_1\setminus \hat E_i$ there is no path connecting a vertex of $J_i$ to a vertex of $J$. Similarly, if $J_i\subseteq G_2$ but the image of $C_i$ in $\phi''$ is not contained in $F_2$, then there is a collection $\hat E_i\subseteq E(G_2)\setminus E(W')$ of at most 
	$\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ edges, such that in graph $G_2\setminus \hat E_i$ there is no path connecting a vertex of $J_i$ to a vertex of $J'$.
\end{observation}
\begin{proof}
	Consider any index $1\leq i\leq z$ with $i\neq i^*$, such that $J_i\subseteq G_1$ but the image of $C_i$ in $\phi''$ is not contained in $F_1$. Assume for contradiction that a minimum-cardinality set $\hat E_i\subseteq E(G_1)\setminus E(W')$ of edges for which graph $G_1\setminus \hat E_i$ has no path connecting a vertex of $J_i$ to a vertex of $J$ has cardinality greater than
	$\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
	
	
	Let $\tilde H$ be the graph that is obtained from $G_1$ by contracting every core $J_{\ell}\subseteq G_1$ with $\ell\not\in\set{i,i^*}$ into a vertex $v_{\ell}$. From the maximum flow / minimum cut theorem, there is a collection $\qset'$ of of at least $\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ edge-disjoint paths in graph $\tilde H$, each of which connects a vertex of $J_i$ to a vertex of $J\cup P$. Consider any such path $Q'\in \qset'$. Note that every edge of $Q'$ also belongs to graph $G_1$. We claim that there must be a crossing in $\phi''$ between an edge of $Q'$ and an edge of $J\cup P$.
	
	Indeed, path $Q'$ naturally defines a path $Q$ in graph $G_1$, connecting a vertex of $J_i$ to a vertex of $J\cup P$. Consider the last edge $e$ on path $Q$. Then  $e\in \tilde E'_1$ must hold, and so the image of $e$ in $\phi''$ must intersect the face $F_1$. Therefore, if we denote by $\gamma$ the image of $J\cup P$ in $\phi''$, then there is some edge $e'\in E(Q)$, whose image in $\phi''$ crosses $\gamma$. Edge $e'$ may not belong to any core $J_{\ell}$ or to path $P$, since the edges of $W\cup P$ do not cross each other in $\phi''$. Therefore, $e'\in E(Q')$ must hold.
	
	We conclude that there are at least $|\qset'|\geq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ crossings in $\phi''$ in which edges of $E(P)\cup E(J)$ participate. Since we have assumed that event $\event'$ did not happen, path $P$ is good, and so its edges participate in at most 
	$\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ and hence in $\phi''$. Additionally, edges of $\cK$ participate in at most $|\chi^{\dirty}(\phi)|$ crossings in $\phi$ (and hence in $\phi''$), and edges of $W\setminus K$ participate in at most $\frac{\cro(\phi)\cdot \mu^{26b}}{\cm'}\leq \frac{\cro(\phi)\cdot \mu^{26b}} m$ crossings from Property \ref{prop: drawing}. Since $J\subseteq W$, there fewer than $\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ crossings in $\phi''$ in which edges of $E(J)\cup E(P)$ participate, a contradiction.
	
	The proof for cores $J_i\subseteq G_2$ with the image of $C_i$ in $\phi''$ drawn outside of $F_2$ is symmetric.
\end{proof}
	
	
We now define another collection $E'''\subseteq E(G'')\setminus E(W')$ of edges to be deleted from graph $\tilde G''$, and we define a new graph $\tilde G'''=\tilde G''\setminus E'''$. Initially, we set $\tilde G'''=\tilde G''$ and $E'''=\emptyset$. We then process every core $J_i$, for $1\leq i\leq z$ and $i\neq i^*$ one by one. Consider an interation when a core $J_i$ is processed. Assume w.l.o.g. that $J_i\subseteq G_1$; the case where $J_i\subseteq G_2$ is symmetric. Let $E^i\subseteq E(G_1)\setminus (E'''\cup E(W'))$ be a minimum-cardinality subset of edges whoe removal in $G_1$ disconnects vertices of $J_i$ from vertices of $J\cup P$. such an edge set can be found efficiently by computing a minimum $s$-$t$ cut in a graph obtained from $G_1\setminus E'''$ by  contracting each connected component of $W'\cap G_1$ into a supernode, and 
letting $s$ and $t$ be the supernodes representing $J_i$ and $J\cup P$ respectively. We now consider two cases. If $|E^i|>\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$, then, from \Cref{obs: disconnect cores}, the image of $J_i$ in $\phi''$ must appear inside the region $F_1$. Since the drawing of $W'$ induced by $\phi''$ is planar, the image of the connected component $C_i$ of $\cset(W')$ that contains $J_i$ also appears inside the region $F_1$ in $\phi''$. The second case happens if $|E^i|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$. In this case, we add the edges of $E^i$ to set $E'''$, and we delete them from graph $\tilde G''$, and from the drawing $\phi''$ of $\tilde G''$. @@@@
	
	




@@@



\subsubsection*{Case 2: $\pset$ was a type-3 promising  path set}

%\newcommand{\othercore}{J_{i^{**}}}
In the second case, $\pset$ was a type-3 promising  path set. We let $1\leq i^*<i^{**}\leq r$ be the indices for which all paths in $\pset$ originate at vertices of $\thecore$ and terminate at vertices of $\othercore$. We denote $E_1=\delta_G(\thecore)$ and $E_2=\delta_G(\thecore)$. 
If the two paths chosen from $\pset^*$ share at least one vertex of $V(G)\setminus V(K)$, then we have constructed a type-2 enhancement whose both endpoints lie in $\thecore$. In this case, the algorithm and its analysis are practically identical to those from Case 2 and are omitted here. We now assume that the two chosen paths are disjoint from each other. For convenience of notation, we denote $P=\firstpath$ and $P'=\secondpath$. Throughout, we denote by $\tilde J$ the graph obtained from the union of $\thecore,\othercore,P$ and $P'$.
Recall that, from \Cref{claim: new drawing}, if neither of the events $\event_1,\event_3$ happened, drawing $\phi'$ contains no crossings between the edges of $E(K')$. 
Throughout, we denote by $\gamma$ the image of path $P$ and by $\gamma'$ the image of path $P'$ in $\phi'$. 

Consider now a drawing $\tilde \rho$ of graph $\tilde J$ induced by $\phi'$. This drawing has no crossings, and it has two faces, that we denote by $F_1$ and $F_2$, respectively, whose boundaries contain both curves $\gamma$ and $\gamma'$. Since the drawing of $\thecore$ induced by $\tilde \rho$ is $\rho_{\thecore}$ and the same is true for $\othercore$, and since the orientations of all vertices in $V(\thecore)$ are fixed with respect to each other, the orientations of all vertices in $V(\othercore)$ are fixed with respect to each other, and the paths $P$ and $P'$ do not share inner vertices, we can compute the drawing $\tilde \rho$ efficiently, though we do not know its orientation in $\phi'$.

As in previous two cases, for every vertex $u\in V(\tilde J)$, we consider the tiny $u$-disc $D_{\phi'}(u)$.  For every edge $e\in \delta_{G'}(u)$, we denote by $\sigma(e)$ the segment of $\phi'(e)$ that is drawn inside the disc $D_{\phi'}(u)$. Let $\tilde E=\left (\bigcup_{u\in V(\tilde J)}\delta_{G'}(u)\right )\setminus E(\tilde J)$. We partition edge set $\tilde E$ into a set $\tilde E^{\inn}$ of \emph{inner edges} and the set $\tilde E^{\out}$ of outer edges exactly as before: Edge set $\tilde E^{\inn}$ contains all edges $e\in \tilde E$ with $\sigma(e)\subseteq F_1$, and $\tilde E^{\out}$ contains all remaining edges. Let $e_1$ be an arbitrary fixed edge of $E_1$ that does not lie on $P$ or $P'$. As before, we assume without loss of generality that $e_1\in \tilde E^{\inn}$. 

The algorithm for computing the orientation of the inner vertices of $P$ and $P'$ is practically identical to the one used in Case 2, with a minor difference in the analysis that we highlight below. 

We define an orientation of the ordering $\oset(\thecore)$ in $\phi'$ exactly as in Case 2. As in Case 1, we can now efficiently determine, for every edge $e\in E_1\cup E_2$, whether it belongs to $E^{\inn}$ or $E^{\out}$. In the former case, we add the edge to set $\tilde E_1'$, and in the latter case, we add it to $\tilde E_2'$. 
The algorithm for computing the orientation of every inner vertex $u$ of $P$ and $P'$  is identical to that used in Case 2. 
The proof that the orientations of the vertices are computed correctly with respect to $\phi'$  provided that Event $\event$ does not happen (that is, an analogue of \Cref{claim: orientations and edge split is computed correctly Case2}) is also almost identical. The only difference is that now the images of the paths in sets $\pset_1(u),\pset_2(u),\pset'_1(u),\pset'_2(u)$ may cross the images of the edges of $\othercore$. However, the total number of such paths, whose images cross the edges of $E(\thecore)\cup E(\othercore)$, remains bounded by $N^{\bad}(u)$, so the same calculations work in Case 3 as well.


\paragraph{Computing the Split.}

The algorithm for computing the drawing $\tilde \rho$ of the graph $K'=K\cup P$ and of the split $(I_1,I_2)$ of the instance $I$ is almost identical to that in Cases 1 and 2. We provide a sketch below, highlighting the differences. 


We construct a flow network $H$ as follows. We start with $H=G'$, and then, for all $1\leq i\leq r$ with $i\not\in\set{i^*,i^{**}}$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$  with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $\tilde J$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $H$, and we denote by $E''=E_H(A,B)$.  The following claim, that is an analogue of \Cref{claim: cut set small case2} for Case 2. The proof is virtually identical and is omitted here.

\begin{claim}\label{claim: cut set small case3}
	If Events $\event$ did not happen, then $|E''|\leq \frac{64\mu^{700}\cro(\phi)}{m}+|\chi^{\dirty}(\phi)|$.
\end{claim}


The drawing $\rho'$ of the graph $K'$ is constructed exactly as before: we start with the drawing $\tilde \rho$ of $\tilde J$, and then plant the discs $D_i$ corresponding to the cores $J_i\in \kset\setminus\set{\thecore,\othercore}$ inside face $F$ or inside face $F'$, depending on whether the corresponding supernode $v_{J_i}$ lies in $A$ or $B$. 

Consider now the split  $(\kset_1,\kset_2)$ of $\kset$ along the resulting enhancement structure $\aset$.
Then $\kset_1$ contains all core structures $\jset_i$ with $v_{J_i}\in A$, while $\kset_2$ contains all core structures $\jset_i$ with $v_{J_i}\in B$. Additionally, $\kset_1$ contains a core structure $\jset$, whose corresponding core $J$ contains all vertices and edges of $\tilde J$ that lie on the boundary of face $F$ in drawing $\tilde \rho$. The drawing $\rho_J$ associated with $J$ is its induced drawing in $\tilde \rho$, with face $F$ serving as the infinite face. Similarly, $\kset_2$ contains a core structure $\jset'$, whose corresponding core $J'$ contains all vertices and edges of $\tilde J$ that lie on the boundary of face $F'$ in drawing $\tilde \rho$. The drawing $\rho_{J'}$ associated with $J'$ is its induced drawing in $\tilde \rho$, with face $F'$ serving as the infinite face. Notice that $V(J)\cup V(J')=V(\tilde J)$, and $E(J)\cup E(J')=E(\tilde J)$.

The split $(I_1=(G_1,\Sigma_1),I_2=(G_2,\Sigma_2))$ of instance $I$ along the enhacement structure $\aset$ is defined exactly as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every core structure $\jset_i\in\kset\setminus\set{\thecore,\othercore}$, if $v_{J_i}\in A$, then we replace $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 
%Additionally, we let $J\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F$, and we let $\rho_J$ denote the drawing of $J$ induced by $\tilde \rho$, where we view $F$ as the infinite face of the drawing. Similarly, we let $J'\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F'$, and we let $\rho_{J'}$ denote the drawing of $J'$ induced by $\tilde \rho$, where we view $F'$ as the infinite face of the drawing. Note that $V(J')\cup V(J'')=V(J)$, and edge sets $E(J'),E(J'')$ define a partition of $E(J)$.

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J))$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. The proof that $(I_1,I_2)$ is a split of $I$ along $\aset$ is the same as in Case 2, and is omitted here. 
We denote $E^{\del}=E(G)\setminus (E(G_1)\cup E(G_2))$. As before, $E^{\del}=E'\cup E''$, and, if Event $\event$ did not happen, then $|E^{\del}|\leq \frac{2\cro(\phi)\cdot \mu^{2150}}m +|\chi^{\dirty}(\phi)| < \frac{\cro(\phi)\cdot \mu^{2200}}{m}+|\chi^{\dirty}(\phi)|$.
As in Case 2, it is easy to verify that $|\kset_1|,|\kset_2|\leq r$ must hold.



The following observation is an analogue of \Cref{obs: few edges in split graphs case2} for Case 3. The proof is virtually identical (with a very slight change in parameters) and is omitted here.

\begin{observation}\label{obs: few edges in split graphs case3}
	If Event $\event$ did not happen, then $|E(G_1)|,|E(G_2)|\leq m-\frac{m}{32\mu^{300}}$.
\end{observation}


The next observation is an analogue of \Cref{obs: semi-clean case 2} for Case 3. Its proof is almost identical to that of \Cref{obs: semi-clean case 2}. We provide a proof sketch in Section \ref{subsec: getting semi-clean solution for case 3} of Appendix.


\begin{observation}\label{obs: semi-clean case 3}
	If bad event $\event$ does not happen, then 	
	there is a semi-clean solution $\phi_1$ for instance $I_1$ with respect to $\kset_1$, and a semi-clean solution $\phi_2$ for instance $I_2$ with respect to $\kset_2$, such that $|\chi^*(\phi_1)|+|\chi^*(\phi_2)|\leq |\chi^*(\phi)|$, and $|\chi^{\dirty}(\phi_1)|+ |\chi^{\dirty}(\phi_2)|\leq |\chi^{\dirty}(\phi)|+\frac{64\mu^{700}\cro(\phi)}{m}$.
\end{observation}

Altogether, if Event $\event$ did not happen, then the algorithm produces a valid output for \procsplit. Since the probability of Event $\event$ is at most $1/\mu^{399}$, this completes the proof of \Cref{thm: procsplit}.

@@@================


\paragraph{The Math}

\begin{itemize}
	\item $\cm'/\mu^{2b}\leq m\leq \cm'$.
	\item Goal fail probability for each bad event is $1/\mu^{12b}$
	\item A path is selected into enhancement with probability  $\frac{2\mu^{3b}}{m}$
	\item A bad path participates in $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings, at most $\frac{10m}{\mu^{15b}}$ bad paths.
	\item number of edges we can delete: at most $ \frac{\cro(\phi)\cdot \mu^{120b}}{m}$, increase in $N(\phi)$ at most $\cro(\phi)\mu^{17b}/\cm'$
	
	\item unlucky path: at most $\frac{\cro(\phi)\mu^{15b}}{m}$ paths on each side.
	
	
	\item $h=\frac{\cro(\phi)\mu^{31b}}{m}$, bad event $\event_2'$ happens if $|E'|>\frac{\cro(\phi)\mu^{48b}}{m}$.
	
	\item selecting unlucky paths: there are at most $\frac{2^{14}\cro(\phi)\mu^{15b}}{m}$ unucky paths for each heavy vertex. Number of heavy vertices: $m/h$. So total number of unlucky paths: $\frac{2^{14}\cro(\phi)\mu^{15b}}{h}$. A path is selected with probability $\frac{2\mu^{3b}}{m}$. So probability that any unlucky path is selected: $\frac{2^{15}\cro(\phi)\mu^{18b}}{hm}$. This must be at most $1/\mu^{12b}$. So $h=\frac{2^{15}\cro(\phi)\mu^{30b}}{m}$. Let's make it $h=\frac{\cro(\phi)\mu^{31b}}{m}$
\end{itemize}


\paragraph{Valid Input for $\procsplit'$.}
A valid input to Procedure $\procsplit'$ consists of a skeleton augmenting structure $\wset$ for $\ckset$ (whose corresponding skeleton augmentation we denote by $W$), parameters $g_1,g_2$, a $\wset$-decomposition $\gset$ of $\cG'$, and a face $F\in \tilde \fset(\wset)$, for which the following hold. Denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G=\cG'\setminus E^{\del}$, and let $\tilde \Sigma$ be the rotation system for graph $\tilde G$ induced by $\cSigma'$. Let $\tilde I=(\tilde G,\tilde \Sigma)$ be the resulting instance of \cnwrs. Then:


\mynote{note that I replaced $30$ with $60$ in property C2 twice. This needs to be propagated in this section, and probably also back. I also added $g_1,g_2$ and the conditions on them}
\begin{properties}{C}
	\item Instance  $I_F=(G_F,\Sigma_F)$ associated with the graph $G_F\in \gset$ is not acceptable; and \label{prop: instance unacceptable}
	
	\item there exists a solution $\phi$ to instance $\tilde I$, that is semi-clean with respect to $\ckset$, and has the following additional properties: \label{prop: drawing}
	\begin{itemize}
		\item drawing $\phi$ is $\wset$-compatible;
		\item $\cro(\phi)\leq \min\set{g_1,(\cm')^2/\mu^{60b}}$;
		\item $|\chi^{\dirty}(\phi)|\leq \set{g_2,\cm'/\mu^{60b}}$ (as before, a crossing of $\phi$ is dirty if it envolves an edge of the skeleton $\cK$); and
		\item the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\cro(\phi)\mu^{26b}/\cm'$.
	\end{itemize}
\end{properties} 

As before, the semi-clean solution $\phi$ is not known to the algorithm.






\mynote{this was updated to a new bound on $E^{\del}(F)$. The remainder of this section needs to be  updated to reflect all this.}

\paragraph{Valid Output for $\procsplit'$.}
A valid output for Procedure $\procsplit'$ consists of 
a skeleton augmenting structure $\wset'$ for $\ckset$ (whose corresponding skeleton augmentation we denote by $W'$), an edge set $E^{\del}(F)\subseteq E(G_F)\setminus E(W')$ of cardinality at most $\left(\frac{g_1}{|E(G_F)|}+g_2\right )\cdot \mu^{120b}$, and a $\wset'$-decomposition $\gset'$ of grpah $\cG'$, for which the following hold. 
Denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G'=\cG'\setminus (E^{\del}\cup E^{\del}(F))$, and let $\tilde \Sigma'$ be the rotation system for graph $\tilde G'$ induced by $\cSigma'$. Let $\tilde I'=(\tilde G',\tilde \Sigma')$ be the resulting instance of \cnwrs. Then:



\begin{properties}{P}
	\item $W\subseteq W'$, and $\tilde \fset(\wset')=\left(\tilde\fset(\wset)\setminus\set{F}\right)\bigcup\set{F_1,F_2}$;\label{prop: same faces}
	
	\item for every face $F'\in \tilde \fset(\wset)\setminus\set{F}$, the graph $G_{F'}$ associated with face $F'$ in the decomposition $\gset$ is identical to the graph $G'_{F'}$ associated with face $F'$ in the decomposition $\gset'$; \label{prop: same graphs}
	
	\item if $G_F$ is the graph associated with face $F$ in $\gset$, and $G_{F_1},G_{F_2}$ are the graphs associated with faces $F_1$ and $F_2$, respectively, in $\gset'$, then $E(G_F)\setminus (E(G_{F_1})\cup E(G_{F_2}))= E^{\del}(F)$. Moreover, $|E(G_{F_1})\setminus E(W')|, |E(G_{F_2})\setminus E(W')|\leq |E(G_{F})\setminus E(W)|-\cm'/\mu^{5b}$; \label{prop: small instances} and
	
	
	\item  there exists a solution $\phi'$ to instance $\tilde I'$, that is semi-clean with respect to $\ckset$, and has the following additional properties: \label{prop: drawing after}
	\begin{itemize}
		\item drawing $\phi'$ is $\wset'$-compatible;
		\item $\cro(\phi')\leq \cro(\phi)$;
		\item $|\chi^{\dirty}(\phi)|\leq |\chi^{\dirty}(\phi')|$; and
		\item if we denote by $N(\phi)$ the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate, and define $N(\phi')$ similarly for $\phi'$, then $N(\phi')\leq N(\phi)+\cro(\phi)\mu^{17b}/\cm'$
	\end{itemize}
\end{properties}  


We summarize our algorithm for Procedure $\procsplit'$ in the following lemma.

\begin{lemma}\label{lem: alg procsplit'}
	There is an efficient randomized algorithm, that, given a valid input to Procedure $\procsplit'$, with probability at least $1-1/\mu^{10b}$ produces a valid output for Procedure $\procsplit'$.
\end{lemma}

============

\subsection*{The Math}
\begin{itemize}
	\item Acceptable instance definition will give a path set containing $\cm'/\mu^{2b}$ paths. In particular, $m\geq \cm'/\mu^{2b}$ and $m\leq \cm'$. So number of paths is at least $m/\mu^{2b}$. This will give promising set containing at least $m/\mu^{2b+100}$ paths. Let's take a subset of $4m/\mu^{3b}$ such paths. So $k'=4m/\mu^{3b}$.
	
%	\item Number of edges in each instance goes down by at least $m/\mu^{3b}\geq \cm'/\mu^{5b}$. So total number of phases is $\mu^{5b}$, in every phase we split at most $\mu^{2b}$ instances. Number of iterations: $\mu^{7b}$. We need success probability $1-1/\mu^{2b}$ overall. So in each iteration let's aim for failure probability $1/\mu^{9b}$. (but define events to get $1/\mu^{12b}$ because they will add up).
	
	\item A path is chosen into enhancement with probability at most $2\mu^{3b}/m\leq 2\mu^{5b}/\cm'$. Expected number of crossings involving it is $\cro(\psi)\mu^{3b}/m$. So to get failure probability $1/\mu^{12b}$, we'll say that the path is bad if it participates in more than $\cro(\psi)\mu^{15b}/m$ crossings.  This is at most $\cro(\psi)\mu^{17b}/\cm'$. This will be times 2 for the 2 paths. 
	
	\item So: total number of crossings in $\psi$ involving edges of the skeleton will be bounded by $\cro(\psi)\mu^{21b}/\cm'$. We should make it $\cro(\psi)\mu^{25b}/\cm'$ in step claim statement.
	
	\item what is the probability that a chosen path crosses some edge of the skeleton? At most $\frac{\cro(\psi)\mu^{22b}}{\cm'}\cdot\frac{\mu^{5b}}{\cm'}\leq  \frac{\cro(\psi)\mu^{27b}}{(\cm')^2}$. This needs to be less than $1/\mu^{12b}$. OK if $\cro(\psi)\leq (\cm')^2\cdot \mu^{60b}$.
	
	
	\item in acceptable instance, the cut size is at most $\cm'/\mu^{2b}$. Number of crossings with edges of $W$ is $\cro(\psi)\mu^{25b}/\cm'$. We need $\cro(\psi)\mu^{25b}/\cm'\ll \cm'/\mu^{2b}$, which is OK because $\cro(\psi)\ll (\cm')^2/\mu^{60}$.
\end{itemize}



\subsection*{The definitions (copied from before)}

\paragraph{Skeleton Augmentation.}

Consider the instance $\cI'=(\cG',\cSigma')$ and the corresponding skeleton structure $\check \kset=(\jset_1,\ldots,\jset_r)$ that serve as input to \Cref{thm: phase 2}, and the skeleton $\cK$ corresponding to skeleton structure $\ckset$. 
An augmentation of the skeleton $\cK$ is a subgraph $W\subseteq \cG'$ that has the following properties.

\begin{itemize}
	\item $\cK\subseteq W$, and every connected component $C$ of $W$ contains at least one core $J_i$, whose corresponding core structure $\jset_i$ lies in $\ckset$ (we note that $C$ may contain more than one such core); and
	\item for every connected component $C$ of $W$, for every edge $e\in E(C)$, graph $C\setminus\set{e}$ is connected.
\end{itemize}


\paragraph{Skeleton Augmenting Structure}

\begin{enumerate}
\item The first ingredient is an augmentation $W$ of the skeleton $\cK$.

\item The second ingredient is an orientaton $b'_u\in \set{-1,1}$ for every vertex $u\in V(W)$, such that the following holds. For all $1\leq i\leq r$, either (i) for every vertex $u\in V(J_i)$, the orientation $b'_u$ is identical to the orientation $b_u$ that is given as part of the core structure $\jset_i$; or (ii) for every vertex $u\in V(J_i)$, $b'_u=b_u$ holds.

\item The third ingredient is a drawing $\rho_C$ of each connected component $C\in \cset(W)$ in the plane, that contains no crossings, and is consistent with the rotation system $\Sigma$ and the orientations $\set{b'_u}_{u\in V(C)}$. We additionally require that, for all $1\leq i\leq r$ with $J_i\subseteq C$, there is a disc $D_i$ containing the images of all vertices and edges of $J_i$. The drawing of $J_i$ inside $D_i$ must be identical to the drawing $\rho_{J_i}$ that is given as part of the core structure $\jset_i$ (up to orientation that may be arbitrary), with disc $D_i$ in $\rho_C$ coinciding with disc $D(J_i)$ in $\rho_{J_i}$. The only vertices of $C$ whose image in $\rho_C$ appears in disc $D_i$ are the vertices of $J_i$. The only edges of $C$ whose image in $\rho_C$ is contained in $D_i$ are the edges of $J_i$. The only edges whose image in $\rho_C$ intersects $D_i$ are edges of $\delta_C(J_i)$, and, for each such edge $e$, the intesection of the image of $e$ with disc $D_i$ is a contiguous curve that may not intersect the interior of any forbidden face $F\in \fset(\rho_{J_i})$.

As before, we denote by $\fset(\rho_C)$ the collection of all faces of $\rho_C$, and by  $F^*(\rho_C)$ the infinite face of the drawing. Notice that, for all $1\leq i\leq r$ with $J_i\subseteq C$, every forbidden face $F\in \fset^{\forbidden}(\rho_{J_i})$ is also a face of $\fset(\rho_C)$. We view $F$ also as a forbidden face of the drawing $\rho_C$, and we denote by $\fset^{\forbidden}(\rho_C)\subseteq \fset(\rho_C)$ the set of all forbidden faces for $\rho_C$. In other words, $\fset^{\forbidden}(\rho_C)$ is the union, over all indices $1\leq i\leq r$ with $J_i\subseteq C$, of $\fset^{\forbidden}(\rho_{J_i})$.

\item The fourth and the last ingredient in a skeleton augmenting structure is, for every unordered pair $C,C'\in \cset(W)$ of distinct connected components of $W$, a face $R_C(C')\in \fset(\rho_C)\setminus\fset^{\forbidden}(\rho_C)$, and a face $R_{C'}(C)\in \fset(\rho_{C'})\setminus \fset^{\forbidden}(\rho_{C'})$, so that either $R_C(C')=F^*(\rho_C)$, or $R_{C'}(C)=F^*(\rho_{C'})$ holds. 
We additionally require that, for every triple $C,C',C''\in \cset(W)$ of distinct components, if $R_C(C')=F^*(\rho_{C})$ and $R_{C'}(C'')=F^*(\rho_{C'})$, then $R_C(C'')=F^*(\rho_{C})$ holds.
\end{enumerate}



\begin{definition}[$\wset$-compatible drawings]
	Consider a skeleton augmenting structure \newline 
	$\wset=(W,\set{b'_u}_{u\in V(W)},\set{\rho_C}_{C\in \cset(W)}, \set{R_C(C')}_{C,C'\in \cset(W)})$, and let $\phi$ be a drawing of the augmented skeleton $W$ in the plane. We say that $\phi$ is a $\wset$-compatible drawing of $W$, if the following hold:
	
	\begin{itemize}
		\item drawing $\phi$ contains no crossings;
		\item for every connected component $C\in \cset(W)$, the drawing of $C$ induced by $\phi$ is identical to the drawing $\rho_C$ (but the orientation may be arbitrary); and
		\item for every pair $C,C'\in \cset(W)$ of distinct connected components, the image of $C'$ is contained in the region $R_{C}(C')\in \fset(\rho_C)$ of the drawing $\phi$, and  the image of $C$ is contained in the region $R_{C'}(C)\in \fset(\rho_{C'})$ of the drawing $\phi$.
	\end{itemize}
	
	As before, we denote by $\fset(\phi)$ the set of all faces of the drawing $\phi$, and by $F^*(\phi)$ the infinite face of the drawing. Note that for every component $C\in \cset(W)$, for every forbidden face $F\in \fset^X(\rho_C)$, $F\in \fset(\phi)$ must hold. Moreover, if $J=\partial_{\rho_C}(F)$, then $J=\partial_{\phi}(F)$. We denote by $\fset^X(\phi)=\bigcup_{C\in \cset(W)}\fset^X(\rho_C)$. 
	
	Given any subgraph $G'$ of $\cG'$ and a drawing $\phi'$ of $G'$, we say that $\phi$ is $\wset$-compatible if the drawing $\phi$ of $W$ induced by $\phi'$ is $\wset$-compatible, and, moreover, for every forbidden face $F\in \fset^{\forbidden}(\phi)$, no vertex of $G'$ has its image in the interior of $F$.
\end{definition}



\paragraph{$\wset$-Decomposition of $\cG'$ and Face-Based Instances}

Given a skeleton augmeting structure $\wset$, a $\wset$-decomposition of the input graph $\cG'$ is a collection $\gset=\set{G_{\tilde F}\mid \tilde F\in \tilde \fset(\wset)}$ of subgraphs of $\cG'$, for which the following hold. For every face $\tilde F\in \tilde \fset(\wset)$, let $\Sigma_{\tF}$ be the rotation system for the graph $G_{\tF}\in \gset$ induced by $\cSigma'$, and let $I_{\tF}=(G_{\tF},\Sigma_{\tF})$ be the resulting instance of \cnwrs. Then:

\begin{itemize}
	\item for every face $\tilde F\in \tilde \fset(\wset)$, for every component $C\in \sset(\tilde F)$, $J_{C,\tF}\subseteq G_{\tilde F(\wset)}$, and $\jset_{C,\tF}$ is a valid core structure for $I_{\tF}$ (see Definitions \ref{def: valid core 1} and \ref{def: valid core 2}). Moreover, if $\tilde F\in \tilde \fset^{\forbidden}(\wset)$, and $C$ is the unique component of $\sset(\tilde F)$, then $G_{\tilde F}=J_{C,\tilde F}$;
	
	
	
	\item for every face $\tilde F\in \tilde \fset(\wset)$, for every vertex $u\in V(G_F)\cap W$, there must be a component $C\in \sset(\tilde F)$ with $u\in V(J_{C,\tilde F})$; and
	
	\item for every pair $\tilde F,\tilde F'\in \tilde\fset(\wset)$ of distinct faces, $V(G_{\tilde F}\cap V(G_{\tilde F'}\subseteq  V(W)$, and $E(G_{\tilde F}\cap E(G_{\tilde F'}\subseteq  E()W)$.
\end{itemize} 



\paragraph{Acceptable Subinstances.}
Consider a skeleton augmentating structure $\wset$, a $\wset$-decomposition $\gset$ of graph $\cG'$, and a face $\tilde F\in \tilde \fset(\wset)\setminus \tilde \fset^{\forbidden}(\wset)$. Recall that we have defined a collection $\kset_{\tilde F}$ of core structures associated with face $\tilde F$, that we now denote, for convenience, by  $\kset_{\tilde F}=\set{\jset_1^{\tF},\ldots,\jset^{\tF}_z}$. For all $1\leq i\leq z$, let $J^{\tF}_i$ be the core associated with the core structure $\jset_{\tF}$. 
%As before, we let $\Sigma_{\tF}$ be the rotation system for the graph $G_{\tF}\in \gset$ induced by $\cSigma'$, and we let $I_{\tF}=(G_{\tF},\Sigma_{\tF})$ be the resulting instance of \cnwrs.
Recall that $\kset_{\tF}$ is a valid skeleton structure for instance $I_{\tF}=(G_{\tF},\Sigma_{\tF})$ of \cnwrs. We denote by $K_{\tF}=\bigcup_{i=1}^zJ_i^{\tF}$ the skeleton graph associated with $\kset_{\tF}$.

For all $1\leq i\leq z$,
we denote by $\tilde E_i=\delta_{G_{\tF}}(J^{\tF}_i)$ the set of all edges of $G_{\tF}$ that are incident to the vertices of the core $J_i^{\tF}$. Since $\jset^{\tF}_i$ is a valid core structure for instance $I_{\tF}$, we can define an ordering $\oset(J^{\tF}_i)$ of the edges of $\tilde E_i$ exactly as before. We then define $\tilde E^{\tF}=\bigcup_{i=1}^z\tilde E_i$. 
Next, we define interesting partitions of the edges of $\tilde E^{\tF}$.



\begin{definition}[Interesting Partitions of Edges.]
	Consider  some partition $(\tilde E',\tilde E'')$ of the edges of $\tilde E^{\tF}$. We say that this partition is \emph{interesting} if there is some index $1\leq i\leq z$, and a partition $(A,A')$ of the edges of $\tilde E_i$ into two subsets, where the edges of $A$ appear consecutively in the ordering $\oset(J_i^{\tF})$ and so do the edges of $A'$, such that   $\tilde E'=A$, and $\tilde E''=\tilde E\setminus \tilde E'$ hold.
\end{definition}

We are now ready to define acceptable instances.

\begin{definition}[Acceptable Instance]
	Let  $\wset$ be a skeleton augmentating structure, let $\gset$ be a $\wset$-decomposition graph $\cG'$, and let $\tilde F\in \tilde \fset(\wset)\setminus \tilde \fset^{\forbidden}(\wset)$ be a face. Consider a graph $H_{\tF}$ that is obtained from graph $G_{\tF}$ by first subdividing every edge $e\in \tilde E^{\tF}$ with a vertex $t_e$, and then deleting all vertices and edges of $K_{\tF}$ from it. We say that instance $G_{\tF}$ is \emph{acceptable} iff for every interesting partition $(\tilde E',\tilde E'')$ of the edges of $\tilde E^{\tF}$, there is a cut $(X,Y)$ in graph $H_{\tF}$ with vertex set $\set{t_e\mid e\in \tilde E'}$ contained in $X$, vertex set $\set{t_e\mid e\in \tilde E'}$ contained in $Y$, and $|E_{H_{\tF}}(X,Y)|\leq \cm'/\mu^{2b}$.
\end{definition}

==> appx-procsplit2.tex <==
\subsection{Proof of \Cref{lem: alg procsplit'}}
\label{subsec: proof of procsplit'} 


In order to simplify the notation, we denote instance $I_F=(G_F,\Sigma_F)$ by $I=(G,\Sigma)$, and we denote $|E(G)|$ by $m$. Since instance $I$ is not acceptable, face $F$ may not be a forbidden face of $\tilde \fset(W)$. Recall that we have computed a set $\sset(F)\subseteq\cset(W)$ of connected components, and, for each such component $C\in \sset(F)$, a subgraph $J_{C,F}$ that is a core. Intuitively, vertices and edges of  $J_{C,F}$ must serve as the boundary of face $F$ in any $\wset$-compatible drawing of $W$, and in particular their images lie on the boundary of the region $F$ in the drawing $\phi$ of graph $\cG'$, given by Property \ref{prop: drawing} of valid input. We have also defined, for each component $C\in \sset(F)$, a core structure $\jset_{C,F}$, whose corresponding core is $J_{C,F}$, and we have defined a collection  $\kset_{ F}=\set{\jset_{C, F}\mid C\in \sset( F)}$ of core structures associated with $F$. From the definition of a $\wset$-decomposition, for all $C\in \sset(F)$, $\jset_{C,F}$ is a valid core structure for $I$, and so $\kset_F$ is a valid skeleton structure for instance $I$. In order to simplify the notation, we denote $\kset_F=\set{\jset_{C,F}\mid C\in \sset(F)}$ by $\kset=\set{\jset_1,\ldots,\jset_z}$, and for all $1\leq i\leq z$, we denote the core associated with the cores structure $\jset_i$ by $J_i$. Since, from \Cref{lem: compute phase 2 decomposition}, $|\ckset|\leq \mu^{100}$, from the definition of a skeleton augmentation, $|\cset(W)|\leq \mu^{100}$, and so $z\leq \mu^{100}$ holds. We also denote by $K=\bigcup_{i=1}^zJ_i$ the skeleton associated with the skeleton structure $\kset$.

As before, we denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G=\cG'\setminus E^{\del}$, and let $\tilde \Sigma$ be the rotation system for graph $\tilde G$ induced by $\cSigma'$. Let $\tilde I=(\tilde G,\tilde \Sigma)$ be the resulting instance of \cnwrs. Recall that Property \ref{prop: drawing} of valid input to Procedure $\procsplit'$ ensures that there is a solution $\phi$ to instance $\tilde I$, that is $\wset$-compatible. Additionally,  $\cro(\phi)\leq (\cm')^2/\mu^{60b}$, $|\chi^{\dirty}(\phi)|\leq \cm'/\mu^{60b}$, the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\cro(\phi)\mu^{26b}/\cm'$.


As in the original procedure \procsplit, the algorithm consists of two steps. In the first step, we compute a promising path set and an enhancement of the skeleton $\kset$. In the second step we complete the construction of the new skeleton augmenting structure $\wset'$ and the new $\wset'$-decompositon $\gset'$ of graph $\cG'$.

\subsubsection{Step 1: Computing Skeleton Enhancement}

As before, we start by computing a promising path set, that will then be used in order to compute an enhancement of skeleton $\kset$. In the algorithm for $\procsplit$, the construction of the promising path set exploited the fact that the input instance $I$ was wide. Here, instead, we exploit the fact that instaince $I$ is not acceptable. The resulting promising path set will be somewhat smaller, and it will only be of type 2 or type 3.

From the definition of aceptable subinstances, there must be an index $1\leq i^*\leq z$, and a partition $(E_1,E_2)$ of the edges of $\delta_G(J_{i^*})$, such that the edges of $E_1$ appear consecutively in the ordering $\oset(J_{i^*})$, and the following holds. Let $(\tilde E',\tilde E'')$ be the partitition of the edges in set $\tilde E=\bigcup_{i=1}^z\delta_G(J_i)$, where $\tilde E'=E_1$, and $\tilde E''=\tilde E\setminus \tilde E'$. As before, let 
$\tilde H$ be the graph that is obtained from graph $G$ by, first subdividing every edge $e\in \tilde E$ with a vertex $t_e$, and then deleting all vertices and edges of $K$ from it. Then the minimum cut in graph $\tilde H$ separating the vertices of $\set{t_e\mid e\in \tilde E'}$ from the vertices of  $\set{t_e\mid e\in \tilde E''}$ must contain at least $\cm'/\mu^{2b}$ edges. Equivalently, there is a set $\pset$ of $\ceil{\cm'/\mu^{2b}}$ edge-disjoint paths in graph $\tilde H$, connecting vertices of 
$\set{t_e\mid e\in \tilde E'}$ to vertices of  $\set{t_e\mid e\in \tilde E''}$. We can assume w.l.o.g. that the paths of $\pset$ do not contain the vertices of $\set{t_e\mid e\in \tilde E}$ as inner vertices.

Set $\pset$ of paths in graph $\tilde H$ naturally defines a collection of at least $\ceil{\cm'/\mu^{2b}}$ edge-disjoint paths in graph $G$, where every path has an edge of $\tilde E'=E_1$ as its first edge, and an edge of $\tilde E''$ as its last edge, and it does not contain any vertices of $K$ as inner vertices. Abusing the notation, we denote this path set by $\pset$ as well. We partition path set $\pset$ into two $z$ subsets $\pset^1,\ldots,\pset^z$, as follows: consider any path $P\in \pset$. Recall that the last edge of $P$ lies in $\tilde E=\bigcup_{i=1}^z\delta_G(J_i)$. We add path $P$ to set $\pset^i$ if the last edge of $P$ lies in $\delta_G(Z_i)$. Clearly, there must be an index $1\leq i\leq z$, such that $|\pset^i|\geq \frac{|\pset|}z \geq \frac{\cm'}{\mu^{2b}\cdot z}\geq \frac{\cm'}{\mu^{2b+100}}\geq \frac{m}{\mu^{2b+100}}$. We then let $\pset'$ be that path set $\pset_i$. Observe that, if $i=i^*$, then $\pset'$ is a promising path set of type $2$, and every path in $\pset'$ has an edge of $E_1$ as its first edge, and an edge of $E_2$ as its last edge. Otherwise, $\pset'$ is a promising path set of type $3$. We let $i^{**}$ be the index for which the last edge of every path in $\pset'$ lies in $\delta_G(J_{i^{**}})$ (so it is possible that $i^{**}=i^*$).

Note that the existence of the path set $\pset'$ implies that $m\geq \cm'/\mu^{2b}$ holds. Let $\pset''\subseteq \pset'$ be an arbitrary subset of $\ceil{\frac{4m}{\mu^{3b}}}$ paths. We construct an enhancement $\Pi=(P_1,P_2)$ from the path set $\pset''$ exactly like in the algorithm for \procsplit. Recall that the algorithm first constructs a collection $\pset^*$ of edge-disjoint non-transversal paths using the paths in $\pset''$, and then selects one or two such paths into the enhancement. The only difference is that the parameter $k'=|\pset^*|$ is now somewhat smaller, $k'=\ceil{\frac{4m}{\mu^{3b}}}$, and so the probability that a path $P\in \pset^*$ is selected into the enhancement is now bounded by $2\mu^{3b}/m\leq 2\mu^{5b}/\cm'$ (since, as observed above, $m\geq \cm'/\mu^{2b}$). Another difference is that, since the promising path set $\pset''$ may only be of type 2 or 3, the resulting enhancement is also guaranteed to be of type 2 or 3. We denote by $P^*_1$ and $P^*_2$ the paths of $\pset^*$ that were chosen into the enhancement (where it is possible that $P^*_2=P^*_1$), and we denote the enhancement itself by $\Pi=\set{P_1,P_2}$.


Next, we define the bad events and bound their probabilities. This part is almost identical to that in Procedure \procsplit. The main differences are that (i) the parameter $k'$ is now smaller by factor $\mu^{\Theta(1)}$, so various parameters need to be scaled by this factor; (ii) the required failure probability is smaller than that from Procedure \procsplit by factor $\mu^{\Theta(1)}$; and (iii) the drawing  of $I$ induced by the drawing $\phi$ of $\tilde I$ is no longer guaranteed to be semi-clean with respect to $K$ (instead we will exploit the fact that the edges of $W$ participate in relatively few crossings in $\phi$).

\paragraph{Good Paths and Bad Event $\event_1'$.}

We use the following modified definition of good paths.

\begin{definition}[Good path]
	We say that a path $P\in \pset^*$ is \emph{good} if the following happen:
	
	\begin{itemize}
		\item the number of crossings in which the edges of $P$ participate in $\phi$ is at most $\frac{\cro(\phi)\mu^{15b}}{4m}$; and
		
		\item there is no crossing in $\phi$ between an edge of $P$ and an edge of $W$.
	\end{itemize} A path that is not good is called a \emph{bad path}.
\end{definition}


We now bound the number of bad paths in $\pset^*$.

\begin{observation}\label{obs: number of bad paths2}
	The number of bad paths in $\pset^*$ is at most $\frac{10m}{\mu^{15b}}$.
\end{observation}

\begin{proof}
Since the paths in $\pset^*$ are edge-disjoint, and every crossing involves two edges, the number of paths $P\in \pset^*$ such that there are more than $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ in which the edges of $P$ participate, is at most $\frac{8m}{\mu^{15b}}$. Additionally, we are guaranteed that $|\chi^{\dirty}(\phi)|\le \frac{\cm'}{\mu^{60b}}\leq \frac m{\mu^{58b}}$ (since $m\geq \frac{\cm'}{\mu^{2b}}$). Therefore, the number of paths $P\in \pset^*$, for which there is a crossing between an edge of $P$ and an edge of $\cK$ is bounded by  $\frac m {\mu^{58b}}$.

Lastly, we are guaranteed that the total number of crossings in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\frac{\cro(\phi)\mu^{26b}}{\cm'}\leq \frac{\cm'}{\mu^{17b}}\leq \frac{m}{\mu^{15b}}$, since $\cro(\phi)\leq \frac{(\cm')^2}{\mu^{60b}}$.
Overall, the number of bad paths in $\pset^*$ is bounded by $\frac{10m}{\mu^{15b}}$.
\end{proof}


We say that bad event $\event_1$ happens if at least one of the paths $P_1^*,P_2^*$ that was chosen from $\pset^*$ in order to construct the enhancement is bad. Since the number of bad paths is bounded by $\frac{4m}{\mu^{15b}}$, and a path of $\pset^*$ is chosen to the enhancement with probability at most $\frac{2\mu^{3b}}{m}$, we immediately get the following observation.

\begin{claim}\label{claim: event 1 prob2}
	$\prob{\event_1'}\leq 8/\mu^{12b}$.
\end{claim}

\paragraph{Heavy and Light Vertices, and Bad Event $\event_2'$.}

We use a parameter $h=\frac{\cro(\phi)\mu^{31b}}{m}$. We say that a vertex $x\in V(G)$ is \emph{heavy} if at least $h$ paths of $\pset^*$ contain $x$; otherwise, we say that $x$ is \emph{light}.
As before, we denote by $E'$ the set of all edges $e\in E(G)$, such that $e$ is incident to some light vertex $x$ that lies in $V(P^*_1)\cup V(P^*_2)$, and $e\not\in E(\firstpath)\cup E(\secondpath)$. We say that bad event $\event_2'$ happens if $|E'|>\frac{\cro(\phi)\mu^{48b}}{m}$.
We now bound the probability of bad event $\event_2'$.

\begin{claim}\label{claim: second bad event bound2}
	$\prob{\event_2'}\leq 1/\mu^{12}$.
\end{claim}
\begin{proof}
	Consider some light vertex $x\in V(G)$. Since $x$ lies on fewer than $h$ paths of $\pset^*$, and each such path is chosen to the enhancement with probability at most $2\mu^{3b}/m$, the probability that $x$ lies in $V(P_1^*)\cup V(P^*_2)$ is bounded by $\frac{2h\mu^{3b}}{m}$.
	
	Consider now some edge $e=(x,y)\in E(G)$. Edge $e$ may lie in $E'$ only if $x$ is a light vertex lying in $V(P_1^*)\cup V(P^*_2)$, or the same is true for $y$. Therefore, the probability that $e\in E'$ is at most $ \frac{4h\mu^{3b}}{m} $, and $\expect{|E'|}\leq 4h\mu^{3b}\leq \frac{4\cro(\phi)\mu^{35b}}{m}$, since $h=\frac{\cro(\phi)\mu^{31b}}{m}$. From Markov's inequality, $\prob{|E'|>\frac{\cro(\phi)\mu^{48b}}{m}}\leq \frac{1}{\mu^{12b}}$.
\end{proof}









\paragraph{Unlucky Paths and Bad Event $\event_3'$.}
The definition of unlucky paths is identical to that in the proof of \Cref{thm: procsplit}, except that we use a slightly different parameter. 

\begin{definition}[Unlucky Paths]
	Let $x\in V(G)\setminus V(K)$ be a vertex, and let $P\in \pset^*$ be a good path that contains $x$. Let $e,e'$ be the two edges of $P$ that are incident to $x$. Let  $\hat E_1(x)\subseteq \delta_G(x)$ be the set of edges $\hat e\in \delta_G(x)$, such that $\hat e$ lies between $e$ and $e'$ in the rotation $\oset_x\in \Sigma$ (in clock-wise orientation), and $\hat e$ lies on some good path of $\pset^*$. Let $\hat E_2(x)\subseteq \delta_G(x)$ be the set of edges $\hat e\in \delta_G(x)$, such that $\hat e$ lies between $e'$ and $e$ in the rotation $\oset_x\in \Sigma$ (in clock-wise orientation), and $\hat e$ lies on some good path of $\pset^*$.
	We say that path $P$ is \emph{unlucky with respect to vertex $x$} if either  $|\hat E_1(x)|<\frac{\cro(\phi)\mu^{15b}}{m}$ or $|\hat E_2(x)|< \frac{\cro(\phi)\mu^{15b}}{m}$ holds.
	We say that a path $P\in \pset^*$ is an \emph{unlucky path} if there is at least one heavy vertex $x\in V(G)\setminus V(K)$, such that $P$ is unlucky with respect to $x$.
\end{definition}

We use the following claim in order to bound the number of unlucky paths. The claim 
is an analogue of \Cref{claim: bound unlucky paths}, and its proof is almost identical, with minor changes due to difference in parameters. For completeness, we include a proof in Section \ref{sec: bound unlucky paths2} of Appendix.

\begin{claim}\label{claim: bound unlucky paths2}
	Assume that Event $\event_1'$ did not happen. Then for every vertex $x\in V(G)\setminus V(K)$, the total number of good paths in $\pset^*$ that are unlucky with respect to $x$ is at most $\frac{2^{14}\cro(\phi)\mu^{15b}}{m}$.
\end{claim}



We say that bad event $\event'_3$ happens if at least one of $P_1^*$, $P_2^*$ is an unlucky path. 

\begin{claim}\label{claim: third event bound2}
	$\prob{\event'_3}\leq 9/\mu^{12b}$.
\end{claim}

\begin{proof}
	Clearly, $\prob{\event'_3}\leq \prob{\event'_1}+\prob{\event'_3\mid \neg\event'_1}$. From \Cref{claim: event 1 prob2},
	$\prob{\event'_1}\leq 8/\mu^{12b}$. We now bound $\prob{\event_3'\mid \neg\event_1'}$.
	
	
	Recall that a heavy vertex must have degree at least $h=\frac{\cro(\phi)\mu^{31b}}{m}$ in $G$. Therefore, the total number of heavy vertices in $G$ is at most $\frac{2m}{h}\leq \frac{2m^2}{ \cro(\phi)\mu^{31b}}$. From \Cref{claim: bound unlucky paths2}, if Event $\event'_1$ did not happen, then for every heavy vertex $x\in V(G)\setminus V(K)$, there are at most $\frac{2^{14}\mu^{15b}\cro(\phi)}{m}$ paths in $\pset^*$ that are good and unlucky for $x$. Therefore, the total number of good paths in $\pset^*$ that are unlucky with respect to some heavy vertex is at most:
	%
	\[\frac{2m^2}{ \cro(\phi)\mu^{31b}}\cdot \frac{2^{14}\mu^{15b}\cro(\phi)}{m} 
	\leq \frac{2^{15}\cdot m}{\mu^{16b}}.
	\]
	%
	Since $|\pset^*|\geq  \frac{4m}{\mu^{3b}}$, from	\Cref{obs: number of bad paths2}, at least $ \frac{2m}{\mu^{3b}}$ paths in $\pset^*$ are good.
	
	We select two paths into the enhancement $\Pi$, and, if Event $\event_1'$ did not happen, every good path is equally likely to be selected. Therefore, the probability that a good path that is unlucky is selected into the enhancement, conditioned on the event $\event_1$ not happening is bounded by:
	%
	\[\frac{2^{15}\cdot m}{\mu^{16b}}\cdot  \frac{\mu^{3b}}{m}\leq \frac{2^{15}}{\mu^{13b}}\leq \frac{1}{\mu^{12b}}, \]
	%
	since $\mu$ is large enough. We conclude that $\prob{\event'_3\mid \neg\event'_1}\leq 1/\mu^{12b}$, and 	$\prob{\event'_3}\leq 9/\mu^{12b}$.	
\end{proof}





Recall that we have denoted by $E'$ the set of all edges that are incident to the light vertices of $\firstpath\cup \secondpath$, excluding the edges of $E(\firstpath)\cup E(\secondpath)$. 


Denote $\tilde G'=\tilde G\setminus E'$, and let $\tilde \Sigma'$ be the rotation system for graph $G'$ induced by $\tilde \Sigma$. For convenience, we also denote $G'=G\setminus E'$ and we let $\Sigma'$ be the rotation system for graph $G'$ induced by $\tilde \Sigma$. Denote $\tilde I'=(\tilde G',\tilde \Sigma')$, and $I'-(G',\Sigma')$. Let $\Pi=\set{P_1,P_2}$ be the enhancement of skeleton $K$ that we have constructed. We denote $K'=K\cup P_1\cup P_2$, and we let $W'=W\cup P_1\cup P_2$ be the new augmentation of the original skeleton $\cK$ for graph $\cG'$.  Drawing $\phi$ of graph $\tilde G=\cG'\setminus E^{\del}$ naturally defines a drawing of graph $\tilde G'$. Moreover, if Event $\event'_1$ did not happen, then there are no crossings in this drawing between the edges of $E(P_1)\cup E(P_2)$ and the edges of $E(W)$. However, it is possible that this drawing contains crossings between pairs of edges in $E(P_1)\cup E(P_2)$. In the next claim we show that, if events $\event'_1$ and $\event'_3$ did not happen, then drawing $\phi$ can be modified to obtain a drawing $\phi'$ of $\tilde G'$, in which the edges of $W'$ do not cross each other, and the induced drawing of $W$ remains identical to that induced by $\phi$. 
We do so in the following claim, that is an analogue of \Cref{claim: new drawing}.
%The proof of the following claim is deferred to Section \ref{sec:getting new drawing} of Appendix.

\begin{claim}\label{claim: new drawing2}
	Assume that neither of the events $\event'_1$ and $\event'_3$ happened. Then there is a  solution $\phi'$ to instance $\tilde I'=(\tilde G',\tilde \Sigma')$, in which there are no crossings between pairs of edges in $E(W')$. Moreover, the drawing of $W$ induced by $\phi'$ is identical to the drawing of $W$ induced by $\phi$, drawing $\phi'$ is $\wset$-compatible, and, for every edge $e\in E(\tilde G')$, the number of crossings in which $e$ participates in $\phi'$ is bounded by the number of crossings in which $e$ participates in $\phi$. In particular,
	$\cro(\phi')\leq \cro(\phi)$ and $\chi^{\dirty}(\phi')\subseteq \chi^{\dirty}(\phi)$ hold.
\end{claim}

The proof of \Cref{claim: new drawing2} is essentially identical to the proof of \Cref{claim: new drawing}. Recall that the main idea in the proof is to remove, one by one, the loops in the images of the paths $P_1,P_2$ in the drawing $\phi$. The reason these loops can be removed without increasing the number of crossings is that every vertex whose image lies on such a loop must be a light vertex (see, e.g., \Cref{obs: no heavy vertices on loops}). This, in turn, relies on the fact that the parameter used in the definition of unlucky paths is greater than the parameter used in the definition of bad paths. While both parameters are now scaled by factor $\mu^{\Theta(b)}$, this relationship between them continues to hold, and so the analogue of  \Cref{obs: no heavy vertices on loops} continues to hold as well. We also need to show that the analogue of \Cref{obs: case 3 not crossing} continues to hold, that is, there are no crossings $(e,e')_p$ in $\phi$ where $e\in E(P_1)$ and $e'\in E(P_2)$. The proof of the observation relies on the fact that that the parameter bounding the number of crossings in which the edges of a good path may participate (denoted by $N$), is less than $k'/100$, and that the number of bad paths in $\pset^*$ is bounded by $k'/16$. While both parameters $N$ and $k'$ are now different, namely $N=\frac{\cro(\phi)\mu^{15b}}{4m}$ and $k'=4m/\mu^{3b}$, it is still the case that $N<k'/100$ (since, from Condition \ref{prop: drawing}, $\cro(\phi)\leq (\cm')^2/\mu^{60b}$, and $m\geq \cm'/\mu^{2b}$). The number of bad paths is bounded by  $\frac{10m}{\mu^{15b}}<k'/16$ from \Cref{obs: number of bad paths2}. The remainder of the proof of  \Cref{claim: new drawing2} is identical to the proof of \Cref{claim: new drawing} and is omitted here.

As before, drawing $\phi'$ of $\tilde G'$ is derived from drawing $\phi$ of $\tilde G$, and neither are known to our algorithm. Note that, since $\jset_{i^*}$ is a valid core structure for instance $I$, the image of the paths $P_1,P_2$ of the enhancement in $\phi'$ must intersect the region $F$. If Event $\event_1'$ does not happen, then the images of paths $P_1,P_2$ do not cross the images of the edges of $W$ in $\phi$, and so the images of both paths are contained in region $F$. This remains true for drawing $\phi'$ of graph $\tilde G'$. Therefore, in the drawing of the new augmented skeleton $W'$ induced by $\phi'$, the images of the edges of $W'$ do not cross each other, and the images of paths $P_1,P_2$ are contained in region $F$. It is easy to verify that the images of the two paths partition face $F$ into two new regions, that we denote by $F_1$ and $F_2$.






\paragraph{Terrible Vertices and Bad Event $\event'_4$.}

As before, for a vertex $x\in V(G)$, we denote by $N(x)$ the number of paths in $\pset^*$ containing $x$, by $N^{\bad}(x)$ the number of bad paths in $\pset^*$ containing $x$, and  by $N^{\good}(x)$ the number of good paths in $\pset^*$ containing $x$. The definition of the notion of a terrible vertex remains the same as before:

\begin{definition}[Terrible Vertex]
	A vertex $x\in V(G)$ is \emph{terrible} if it is a heavy vertex, and $N^{\bad}(x)\geq N^{\good}(x)/64$.
\end{definition}


As before, we say that a bad event $\event'_4$ happens if any vertex of $\firstpath\cup \secondpath$ is a terrible vertex. We bound the probability of Event $\event'_4$ in the following claim, whose proof is essentially identical to the proof of \Cref{claim: no terrible vertices}. Since we use slightly different parameters, we provide the proof here for completeness.

\begin{claim}\label{claim: no terrible vertices2}
	$\prob{\event_4'}\leq \frac{2^{14}\log m}{\mu^{12b}}$.
\end{claim}

\begin{proof}
	Let $U$ be the set of all heavy vertices of $G$. We group the vertices $x\in U$ geometrically into classes, using the parameter $N(x)$. Recall that $h=\frac{\cro(\phi)\mu^{31b}}{m}$, and, for every heavy vertex $x\in U$, $N(x)\geq h$. Let $q=2\ceil{\log m}$. For $1\leq i\leq q$, we let the class $S_i$ contain all vertices $x\in U$ with $2^{i-1}\cdot h\leq N(x)<2^i\cdot h$. 
	Let $S'_i\subseteq S_i$ be the set containing all terrible vertices of $S_i$. For every vertex $x\in S'_i$, $N^{\bad}(x)\geq N^{\good}(x)/64$. Since $N(x)=N^{\bad}(x)+N^{\good}(x)$, we get that $N^{\bad}(x)\geq N(x)/65\geq 2^{i-1}\cdot h/65$. From \Cref{obs: number of bad paths2}, the total number of bad paths is at most $\frac{10m}{\mu^{15b}}$, so
	%
	\[|S'_i|\leq  \frac{10m/\mu^{15b}}{2^{i-1}\cdot h/65}\leq \frac{650m}{ 2^{i-1}\cdot h\cdot \mu^{15b}}.\] %  =\frac{9m^2}{ 2^{i-1}\cdot \cro(\phi)\mu^{2150}}, \]
	%since $h=\cro(\phi)\mu^{1450}/m$.
	Recall that the probability that a path $P\in \pset^*$ is selected into the enhancement is at most $\frac{2\mu^{3b}}{m}$. A vertex $x\in S'_i$ may lie in $V(\firstpath)\cup V(\secondpath)$ only if at least one of the $N(x)$ paths of $\pset^*$ containing $x$ is selected into the enhancement. Therefore, $\prob{x\in (V(\firstpath)\cup V(\secondpath))}\leq \frac{2\mu^{3b}\cdot N(x)}{m}\leq \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}$.
	
	
	Overall, the probability that some vertex of $S'_i$ belongs to $V(\firstpath)\cup V(\secondpath)$ is at most 
	$$|S'_i|\cdot \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}\leq \frac{650m}{ 2^{i-1}\cdot h\cdot \mu^{15b}}\cdot \frac{2^{i+1}\cdot h\cdot \mu^{3b}}{m}\leq \frac{2^{12}}{\mu^{12b}}.$$ 
	
	Using the union bound over all $q=2\ceil{\log m}$ classes, we get that the probability of Event $\event'_4$ is bounded by $\frac{2^{14}\log m}{\mu^{12b}}$.
\end{proof}


\paragraph{Bad Event $\event'$.}
Let $\event'$ be the bad event that at least one of the events $\event'_1,\event'_2,\event'_3,\event'_4$ happen. From the Union Bound and Claims \ref{claim: event 1 prob2}, \ref{claim: second bad event bound2}, \ref{claim: third event bound2} and \ref{claim: no terrible vertices2}, $\prob{\event'}\leq O\left( \frac{\log m}{\mu^{12b}}\right ) \leq \frac{1}{\mu^{11b}}$, by definition of $\mu$.


\subsubsection{Step 2: Completing the Construction of $\wset'$ and $\gset'$}


In this step we complete the construction of the skeleton augmenting structure $\wset'$ and of the $\wset'$-decomposition of $\cG'$ $\gset'$. This step is very similar to the second step of Procedure \procsplit, with several key differences. The first difference is that we no longer need to take care of the case where $\Pi$ is a type-1 enhancement. The second difference is that the parameters are now somewhat different. The third difference, which is more major than the first two, is that we will not be able to guarantee that the final drawing of the graph $\tilde G\setminus E^{\del}(F)$ that we obtain, induces drawings of graphs $G_{F_1},G_{F_2}$ that are semi-clean with respect to their skeletons. We will still, however, need to ensure that the drawing is $\wset'$-compatible, so every core of $\set{J_1,\ldots,J_z}$ is drawn in the ``correct'' face (for example, if $J_i\subseteq G_{F_1}$, then core $J_i$ should be drawn inside). This will require an additional step, in which we disconnect some of the cores from the corresponding graph $G_1$ or $G_2$.

We consider the instance $I'=(G',\Sigma')$, where $G'=\tilde G\setminus E'$, and $\Sigma'$ is the rotation system for $G'$ induced by $\cSigma'$. We will also consider the solution $\phi'$ to instance $I'$ given by  \Cref{claim: new drawing} (assuming that bad event $\event'$ did not happen).

We start by computing an orientation $b'_u$ for every vertex $u\in V(W')$, and a drawing $\rho_{C'}$ of every connected component $C'\in \cset(W')$. We then split graph $G$ into two subgraphs $G_1$ and $G_2$, and complete the construction of the skeleton augmenting structure. Lastly, we will remove some additional edges from the resulting graph, to ensure that there is a good drawing of that graph that is $\wset'$-compatible.
We consider two cases, depending on whether the original promising path $\pset$ was of type $2$ or $3$.



\subsubsection*{Case 1: $\pset$ was a Type-2 Promising  Path Set}

The first case happens when the promising path set $\pset$ is of type 2. Recall that the endpoints of all paths in $\pset$ are contained in $V(\thecore)$, and that we have computed a partition $(E_1,E_2)$ of the edges of $\delta_G(\thecore)$, so the edges of $E_1$ are consecutive in the ordering $\oset(\thecore)$, and every path  of $\pset^*$ has an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge. Recall that, in this case, $\Pi=\set{P_1,P_2}$, where $P_1\in \pset^*$ is either a path or a cycle, and $P_2=\emptyset$. For convenience of notation, we denote $P_1$ by $P$.

Recall that, from \Cref{claim: new drawing2}, if Event $\event'$ does not happen, then  drawing $\phi'$ of $G'=G\setminus E'$ contains no crossings between the edges of $E(W')$. 
Throughout, we denote by $\gamma$ the image of the path $P$ in $\phi'$. 



In order to construct the skeleton augmenting structure $\wset'$, we first let $W'=W\cup P$ be the skeleton augmentation associated with $\wset'$. Next, we define a drawing $\rho_C$ for every component $C\in \cset(W)$.

Let $C_{i^*}\in \cset(W)$ be the connected component with $\thecore\subseteq C_{i^*}$, and denote by $\tilde C=C_{i^*}\cup P$. Since path $P$ is internally disjoint from all vertices of $W$, it is immediate to verify that $\cset(W')=(\cset(W)\setminus C_{i^*})\cup \tilde C)$. For every component $C\in \cset(W')\setminus \set{\tilde C}$, its drawing $\rho_C$ in $\wset'$ remains the same as in $\wset$. 

Consider now the component $\tilde C$. Recall that we are given, as part of skeleton augmenting structure $\wset$ a drawing $\rho_{C_{i^*}}$ of graph $C_{i^*}$ and an orientation $b'_u$ of every vertex $u\in V(C_{i^*})$. We are also given a face $F^{i^*}\in \fset(\rho_{C_{i^*}})$, such that the face $F$ in drawing $\phi$ is contained in the region $F^{i^*}$. Since drawing $\phi$ is $\wset$-compatible, and it does not contain any crossings between the edges of $W'$, we are guaranteed that path $P$ is drawn inside the region $F^{i^*}$ of $\phi'$, in a natural way. Since the orientations of all vertices of $C_{i^*}$ in $\phi'$ are consistent with those given by $\wset$, and since the drawing of $C_{i^*}$ induced by $\phi'$ is $\rho_{C_{i^*}}$, we can efficiently compute a drawing $\rho_{\tilde C}$ of graph $\tilde C$, that is identical to the drawing of $\tilde C$ induced by $\phi'$. This drawing  is the unique planar drawing of of $\tilde C$ that has the following properties:

\begin{itemize}
	\item the drawing of $C_{i^*}$ induced by $\rho_{\tilde C}$ is $\rho_{C_{i^*}}$;
	\item the image of path $P$ is contained in region $F^{i^*}$; 
	\item the drawing is consistent with the rotation system $\cSigma'$; and
	\item  the orientation of every vertex $u\in V(C_{i^*})$ in the drawing is the orientation $b'_u$ given by $\wset$.
\end{itemize}


Notice that the set $\fset(\rho_{\tilde C})$ of faces of this new drawing of graph $\tilde C$ is precisely $(\fset(\rho_{C_{i^*}})\setminus F^{i^*})\cup (F^{i^*}_1,F^{i^*}_2)$, where $F^{i^*}_1$ and $F^{i^*}_2$ are the two new faces that are obtained by partitioning the face $F^{i^*}$ with the image of path $P$. We assume w.l.o.g. that region $F^{i^*}_1$ in the drawing of $W'$ induced by $\phi'$ contains the face $F_1$ of this drawing, and region $F^{i^*}_2$ contains the face $F_2$.
If $F^{i^*}=F^*(\rho_{C_{i^*}})$ is the infinite face of the drawing $\rho_{C_{i^*}}$, then we will designate one of the faces $F^{i^*}_1$ or $F^{i^*}_2$ as the infinite face of the drawing $\rho_{\tilde C}$ later.


So far we have defined the new skeleton augmentation $W'$ and a drawing $\rho_C$ of every connected component $C\in \cset(W)$. Next, we define the orientation $b'_u$ of every vertex $u\in V(W')$. For vertices $u\in V(W')\cap V(W)$, the orientation $b'_u$ in $\wset'$ remains the same as the orientation $b'_u$ in $\wset$. It now remains to define the orientation $b'_u$ of vertices $u\in V(P)\setminus V(C_{i^*})$. The procedure for computing these orienttions is very similar to the one from Procedure $\procsplit$.


We first recall the definition of the circular ordering $\oset(\thecore)$ of the edges of $\delta_G(\thecore)$.  In order to define the ordering, we considered the disc $D(\thecore)$ in the drawing $\rho_{\thecore}$ of $\thecore$ defined by the core structure $\jset_{i^*}$. Recall that the drawing $\rho_{\thecore}$ is the drawing of $\thecore$ induced by the drawing $\rho_{C_{i^*}}$ of $C_{i^*}$. In this drawing, the orientation of every vertex $u\in V(\thecore)$ is $b'_u$. We have defined, for every edge $e\in \delta_G(\thecore)$, a point $p(e)$ on the boundary of the disc $D(\thecore)$, and we let $\oset(\thecore)$ be the circular ordering of the edges of $\delta_G(\thecore)$, in which the  points $p(e)$ corresponding to these edges  appear on the boundary of the disc $D(\thecore)$, as we traverse it in counter-clock-wise direction. If the drawing of $\thecore$ in $\phi'$ is identical to $\rho_{\thecore}$ (including the orientation), then we say that the orientation of the ordering $\oset(\thecore)$ in $\phi'$ is $1$. In this case, we are guaranteed that for every vertex $u\in V(\thecore)$, its orientation in $\phi'$ is $b'_u$. Otherwise, the drawing of $\thecore$ in $\phi'$ is the mirror image of $\rho_{\thecore}$. We then say that the orientation of the ordering $\oset(\thecore)$ in $\phi'$ is $-1$. In this case, we are guaranteed that for every vertex $u\in V(\thecore)$, its orientation in $\phi'$ is $-b'_u$.


For every vertex $u\in V(P)\cup V(\thecore)$, we consider the tiny $u$-disc $D_{\phi'}(u)$ in the drawing $\phi'$.  For every edge $e\in \delta_{G}(u)\setminus E'$, we denote by $\sigma(e)$ the segment of $\phi'(e)$ that is drawn inside the disc $D_{\phi'}(u)$. Since edge $e$ belongs to graph $G$, $\sigma(e)$ must be contained in the region $F\in \fset(W)$ of the drawing $\phi'$.  Let $\tilde E=\left (\bigcup_{u\in V(P)\cup V(\thecore)}\delta_{G'}(u)\right )\setminus (E(P)\cup E(\thecore))$. 
The image of path $P$ in $\phi'$ splits region $F$ into two regions, that we denote by $F_1$ and $F_2$. We let $e_1\in E_1$ be any edge that does not lie on path $P$, and we assume without loss of generality that $\sigma(e_1)\subseteq F_1$.

We partition edge set $\tilde E$ into a set $\tilde E^{\inn}$ of \emph{inner edges} and the set $\tilde E^{\out}$ of outer edges, as before: Edge set $\tilde E^{\inn}$ contains all edges $e\in \tilde E$ with $\sigma(e)$ contained in the region $F_1$ of $\phi'$, and $\tilde E^{\out}$ contains all remaining edges (so for every edge $e\in \tilde E^{\out}$, $\sigma(e)$ is contained in $F_2$). As before, we show an algorithm that correctly computes the orientation of every vertex $u\in V(P)$ in the drawing $\phi'$, and the partition $(\tilde E^{\inn},\tilde E^{\out})$ of the edges of $\tilde E$.


\paragraph{Computing Vertex Orientations on Path $P$ and the Partition $(\tilde E^{\inn},\tilde E^{\out})$.}

The algorithm for computing vertex orientations for vertices of $P$, and the partition $(\tilde E^{\inn},\tilde E^{\out})$ of the edges of $\tilde E$ is identical to that from Procedure \procsplit. The main difference is the change in the parameters. We provide the algorithm and its analysis for completeness.

Consider any vertex $u\in V(P)$. Let $\hat e(u)$, $\hat e'(u)$ be the two edges of $P$ that are incident to $u$, where we assume that $\hat e(u)$ appears earlier on $P$ (we assume that $P$ is directed from an edge of $E_1$ to an edge of $E_2$). Edges $\hat e(u),\hat e'(u)$ partition the edge set $\delta_{G'}(u)\setminus\set{\hat e(u),\hat e'(u)}$ into two subsets, that we denote by $\hat E_1(u)$ and $\hat E_2(u)$, each of which appears consecutively in the rotation $\oset_u\in \Sigma'$.
Note that either (i) $\hat E_1(u)\subseteq \tilde E^{\inn}$ and $\hat E_2(u)\subseteq \tilde E^{\out}$ holds, or (ii) $\hat E_2(u)\subseteq \tilde E^{\inn}$ and $\hat E_1(u)\subseteq \tilde E^{\out}$ holds.


We now construct edge sets $\tilde E_1',\tilde E_2'$, and fix an orientation $b'_u$ for every vertex $u\in V(P)\setminus V(\thecore)$. We then show that $\tilde E_1'=\tilde E^{\inn}$, $\tilde E_2=\tilde E^{\out}$, and that the orientations of all vertices of $P$ that we compute are consistent with the drawing $\phi'$.

Recall that we have computed a drawing $\rho_{\tilde C}$ of $\tilde C=C_{i^*}\cup P$, that is identical to the drawing of $\tilde C$ induced by $\phi'$. We let $\tilde \rho$ be the drawing of $\thecore\cup P$ that is induced by $\rho_{\tilde C}$.
Since we have assumed that $\sigma(e_1)$ is contained in the face $F_1$, for every edge $e\in \delta_G(\thecore)$, we can correctly determine whether $e\in \tilde E^{\inn}$ or $e\in \tilde E^{\out}$. In the former case, we add $e$ to $\tilde E_1'$, and in the latter case we add $e$ to $\tilde E_2'$. 
Therefore, for every path $P'\in \pset^*$, the first and the last edges of $P$ are already added to either $\tilde E_1'$ or $\tilde E_2'$.

Next, we process every inner vertex $u$ on path $P$.
Consider any such vertex $u$. As before, if $u$ is a light vertex, then its orientation $b'_u$ can be chosen arbitrarily, as $\deg_{\tilde G'}(u)=2$. 

Assume now that $u$ is a heavy vertex. 
In order to decide on the orientation of $u$, we let $\pset(u)$ contain all paths $P'\in \pset^*\setminus\set{P}$ with $u\in P'$.  We partition the set $\pset(u)$  of paths into four subsets: set $\pset_1(u)$ contains all paths $P'$ whose first edge lies in $\tilde  E_1'$, and the first edge that is incident to $u$ lies in $\hat E_1(u)$. Set $\pset_2(u)$  contains all paths $P'$ whose first edge lies in $\tilde  E_2'$, and the first edge that is incident to $u$ lies in $\hat E_2(u)$. Similarly, set $\pset'_1(u)$ contains   all paths $P'\in \pset(u)$ whose first edge lies in $\tilde  E_1'$ and the first edge that is incident to $u$ lies in $\hat E_2(u)$, while set $\pset'_2(u)$ contains  all paths $P'\in \pset'(u)$, whose first edge lies in $\tilde  E_2'$ and the first edge that is incident to $u$ lies in $\hat E_1(u)$. We let $w(u)=|\pset_1|+|\pset_2|$, and $w'(u)=|\pset'_1|+|\pset'_2|$.
If $w(u)\leq  w'(u)$, then we set $b'_u=-1$, add the edges of $\hat E_1(u)$ to $\tilde E'_1$, and add the edges of $\hat E_2(u)$ to $\tilde E'_2$.  Otherwise we set $b'_u=1$,  add the edges of $\hat E_1(u)$ to $\tilde E'_2$, and add the edges of $\hat E_2(u)$ to $\tilde E'_1$.

This completes the algorithm for computing the orientations of the inner vertices of $P$, and of the partition $(\tilde E_1',\tilde E_2')$ of the edge set $\tilde E$.
We use the following claim to show that both are computed correctly. %The claim is an analogue of \Cref{claim: orientations and edge split is computed correctly} for Case 1. Its proof is similar, but contains some subtleties, since the images of some paths in $\pset^*$ may now cross the images of the edges of $\thecore$.

\begin{claim}\label{claim: orientations and edge split is computed correctly Case2.2}
	Assume that Event $\event'$ did not happen. If the orientation of the ordering $\oset(\thecore)$  in $\phi'$ is $1$, then for every vertex $u\in V(P)\cup V(C_{i^*})$, the orientation of $u$ in $\phi'$ is $b'_u$.
	Otherwise, for every vertex $u\in  V(P)\cup V(C_{i^*})$, the orientation of $u$ in $\phi'$ is $-b_u$. In either case,
	$\tilde E_1'=\tilde E^{\inn}$ and $\tilde E_2'=\tilde E^{\out}$. 
\end{claim}

\begin{proof}
	We assume without loss of generality that the orientation of the ordering $\oset(\thecore)$  in $\phi'$ is $1$. The argument for the other case is symmetric. From the above discussion, for every vertex $u\in V(\thecore)$, the orientation of $u$ in $\phi'$ is $b'_u$. It is now enough to show that, if $u\in P$ is a heavy vertex, then the orientation of $u$ in $\phi'$ is $b_u$.
	
	Recall that we denoted $N(u)=|\pset(u)|$, and we have denoted by $N^{\bad}(u)$ and $N^{\good}(u)$ the total number of bad and good paths in $\pset(u)$, respectively. Since we have assumed that bad event $\event_4'$ did not happen, vertex $u$ is not a terrible vertex, that is, $N^{\bad}(u)\leq N^{\good}(u)/64$. Since $N(u)=N^{\bad}(u)+N^{\good}(u)$, we get that $N^{\bad}(u)<N(u)/65$. 
	
	
	Assume first that the orientation of vertex $u$ in $\phi'$ is $-1$. In this case, for every edge $e\in \hat E_1(u)\cup \tilde E_1'$, the segment $\sigma(e)$ lies in face $F_1$ of $\tilde \rho$, while for every edge $e'\in \hat E_2(u)\cup \tilde  E_2'$, the segment $\sigma(e')$ lies in face $F_2$. 
	We claim that in this case $w'(u)>w(u)$ must hold, and so our algorithm sets $b_u=-1$ correctly. Indeed, assume otherwise. 
	Then $w'(u)\geq N(u)/2$. Let $\qset$ denote the set of all good paths in $\pset'_1(u)\cup \pset'_2(u)$. Then $|\qset|\geq w'(u)-N^{\bad}(u)\geq N(u)/2-N(u)/65\geq N(u)/4\geq h/4$, since $u$ is a heavy vertex. 
	We now show that, for every path $Q\in \qset$, there must be a crossing between an edge of $Q$ and an edge of $P$ in $\phi'$.
	
	Indeed, consider any path $Q\in \qset$. Since $Q\in \pset'_1(u)\cup \pset'_2(u)$, the image of the path $Q$ must cross the boundary of the face $F_1$ in $\rho$. Since path $Q$ is a good path, and it does not contain vertices of $\thecore$ as inner vertices, no inner point of the image of $Q$ in $\phi'$ may belong to the image of $\thecore$ in $\phi'$. Since the paths in $\pset$ are transversal, it then follows that there must be a crossing between an edge of $Q$ and an edge of $P$ in $\phi'$. But then the edges of $P$ participate in at least $\frac h 2\geq \frac{\cro(\phi)\mu^{31b}}{2m}$ crossings in $\phi'$, and hence in $\phi$.
	
	 However, since we have assumed that bad event $\event_1$ did not happen, $P$ is a good path, and so its edges may participate in at most 	$\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$, a contradiction. Therefore, when the orientation of $u$ in $\phi'$ is $-1$, our algorithm correctly sets $b_u=-1$. 
	In the case where the orientation of $u$ in $\phi'$ is $1$, the analysis is symmetric.
\end{proof}


In order to complete the construction of the skeleton augmenting structure $\wset'$, it remains to define, for every pair $C,C'\in \cset(W')$ of distinct connected components, a face $R_C(C')$ of $\fset(\rho_C)$. Additionally, if face $F^{i^*}\in \fset(\rho_{C_{i^*}})$ is the outer face of the drawing $\rho_{C_{i^*}}$ of component $C_{i^*}$, then we need to designate one of the faces $F^{i^*}_1$ or $F^{i^*}_2$ as the outer face of the drawing $\rho_{\tilde C}$ of component $\tilde C$. We do so in the next step, once we split the graph $G'$ into two subgraphs, $G_1$ and $G_2$.


\paragraph{Computing the Split.}

We construct a flow network $\tilde H'$ as follows. We start with $\tilde H'=G'$, and then, for all $1\leq i\leq z$ with $i\neq i^*$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$ with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $P\cup \thecore$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $\tilde H'$, and we denote by $E''=E_{\tilde H'}(A,B)$.  The following claim, that is an analogue of \Cref{claim: cut set small case2},  bounds the cardinality of $E''$. 

\begin{claim}\label{claim: cut set small case2.2}
	If bad event $\event'$ did not happen, then $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
\end{claim}


The proof of the claim is essentially identical to the proof of \Cref{claim: cut set small case2.2}. We assume for contradiction that Event $\event'$ did not  happen, but $|E''|> \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
We can then use Max Flow -- Min Cut theorem to construct a collection  $\qset$ of edge-disjoint paths in graph $G'$, such that, for every path $Q\in \qset$, drawing $\phi'$ must contain at least one crossing between an edge of $Q$ and an edge of $W\cup P$. Since Event $\event'$ did not happen, path $P$ is good, so its edges participate in at most $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ and hence in $\phi'$. Additionally, edges of $\cK$ participate in at most $|\chi^{\dirty}(\phi)|$ crossings in $\phi$ (and hence in $\phi'$), and edges of $W\setminus K$ participate in at most $\frac{\cro(\phi)\cdot \mu^{26b}}{\cm'}\leq \frac{\cro(\phi)\cdot \mu^{26b}} m$ crossings from Property \ref{prop: drawing2}. Overall, there are fewer than $\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ crossings in $\phi'$ in which edges of $P\cup W$ participate, a contradiction.






We now construct the  graphs $G_1,G_2$ associated with the faces $F_1$ and $F_2$, respectively.
In order to do so, we define two vertex sets $A',B'$ of graph $G'$, as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every index $1\leq i\leq r$ with $i\neq i^*$, if $v_{J_i}\in A$, then we replace vertex $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 


Additionally, we let $J\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\rho_{\tilde C}$ lie on the boundary of face $F^{i^*}_1$. Similarly, we let $J'\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images  in $\rho_{\tilde C}$ lie on the boundary of face $F^{i^*}_2$. 

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J))$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma'$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. 
We need the following observation that, intuitively, shows that graphs $G_1$ and $G_2$ are significantly smaller than the original graph $G$.

\begin{observation}\label{obs: few edges in split graphs case2.2}
	If Event $\event'$ did not happen, then $|E(G_1)\setminus E(W')|,|E(G_2)\setminus E(W')|\leq |E(G)\setminus E(W)|-\frac{\cm'}{\mu^{5b}}$.
\end{observation}

The proof of the observation is identical to the proof of \Cref{obs: few edges in split graphs case2}, and follows from the fact that, from the definition of the process for computing an enhancement, at least $k'/4$ edges of $E_1$ must lie in $\tilde E_1'$, and at least $k'/4$ edges of $E_1'$ must lie in $\tilde E_2$.  Since $k'=\ceil{\frac{4m}{\mu^{3b}}}$ and $m\geq \cm'/\mu^{2b}$, the claim follows. 



Let $E^{\del}(F)=E'\cup E''$. If bad event $\event'$ did not happen, then, from the definition of bad event $\event_2'$, $|E'|\leq  \frac{\cro(\phi)\mu^{48b}}{m}$ and, from \Cref{claim: cut set small case2.2}, $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
Since $\cro(\phi)\leq g_1$ and $|\chi^{\dirty}(\phi)|\leq g_2$, we get that, if bad event $\event'$ did not happen, then $|E^{\del}(F)|\leq \frac{g_1\cdot \mu^{48}}{m}+g_2$, as required.


Let $\tilde G''=\tilde G'\setminus E''=\tilde G\setminus E^{\del}$, and let $\tilde \Sigma''$ be the rotation system for graph $\tilde G''$ induced by $\tilde \Sigma$. We denote $\tilde I''=(\tilde G'',\tilde \Sigma'')$ the resulting instance of \cnwrs.
Let $\phi''$ be the drawing of $\tilde G''$ that is induced by the drawing $\phi'$ of $\tilde G'$. We also denote $G''=G'\setminus E''=G\setminus E^{\del}$. Notice that $E(G_1)\cup E(G_2)=E(G'')$.



We now complete the construction of the skeleton augmenting structure $\wset'$. For all $1\leq i\leq z$, let $C_i\in \cset(W)$ be the connected component that contains the core $J_i$, and let $F^i\in \fset(\rho_{C_i})$ be the face that corresponds to face $F$ of $\tilde \fset(\wset)$ (in other words, face $F$ in the drawing of $W$ induced by $\phi$ is contained in region $F^i$). From the construction of the set $\tilde \fset(\wset)$ of faces, in the decomposition forest $H(\wset)$, either  vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees in the forest; or one of these vertices is the parent-vertex of the remaining vertices. We assume w.l.o.g. that in the latter case, vertex $x_{C_1}$ is the parent of vertices $x_{C_2},\ldots,x_{C_z}$ in the forest $H(\wset)$.


Consider any pair $C,C'\in \cset(W')$ of distinct connected components. Assume first that $C,C'\neq \tilde C$. In this case, face $R_{C}(C')$ remains the same in $\wset'$ in the augmenting structure $\wset$. Since drawing $\phi$ of $\tilde G$ was $\wset$-compatible, and drawing $\phi''$ is obtained from $\phi$ by deleting some edges that do not belong to $W'$, and possibly making some additional local changes within the region $F$, the image of component $C'$ in $\phi''$ remains contained in region $R_C(C')$.


Assume now that $C'=\tilde C$. In this case, we let the face $R_{C'}(\tilde C)$ in $\wset'$ be the face $R_{C'}(C_{i^*})$ of $\wset$. It is easy to verify that the drawing of component $\tilde C$ in $\phi''$ remains in the region $R_{C'}(C_{i^*})$.

Next, we assume that $C=\tilde C$. Recall that component $C_{i^*}$ of $W$ is replaced by component $\tilde C=C_{i^*}\cup P$ in $W'$.
Assume first that in $\wset$, $R_{C_{i^*}}(C')\neq F^{i^*}$. In this case, face $R_{C_{i^*}}(C')$ remains a face of $\rho_{\tilde C}$, and the image of component $C'$ appears in region $R_{C_{i^*}}(C')$ in $\phi'$. We then set $R_{\tilde C}(C')=R_{C_{i^*}}(C')$ in $\wset'$.

It now remains to consider pairs $C,C'$ of components of $W'$ with $C=\tilde C$, such that $R_{C_{i^*}}(C')=F^{i^*}$ in $\wset$. We start with the following observation.



\begin{observation}\label{obs: cores drawn correctly} Assume that Event $\event'$ did not happen.
	Consider any index $1\leq i\leq z$ with $i\neq i^*$. If $J_i\subseteq G_1$, then the image of $C_i$ appears in region  $F_1^{i^*}$ in $\phi''$, and if $J_i\subseteq G_2$, then the image of $C_i$ appears in region $F_2^{i^*}$ in $\phi''$.
\end{observation}
\begin{proof}
	Assume for contradiction that Event $\event'$ did not happen, and there is an index $1\leq i\leq z$ with $J_i\subseteq G_1$, such that the image of $C_i$ is not contained in region $F_1^{i^*}$ of $\phi''$.
	
	Let $E^*$ be the set of edges $e\in E(\tilde G'')$, such that the image of $e$ in $\phi''$ crosses the image of some edge of $W'$. Recall that $|\chi^{\dirty}(\phi)|\leq g_2$ and the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\frac{\cro(\phi)\cdot \mu^{26b}}{\cm'}$, from Property \ref{prop: drawing}. If Event $\event'$ did not happen, then the number of crossings in which the edges of $P$ participate is at most $\frac{\cro(\phi)\mu^{15b}}{4m}\leq \frac{\cro(\phi)\mu^{17b}}{\cm}$. Therefore, overall, $|E^*|\leq g_2+\frac{2\cro(\phi)\cdot \mu^{26b}}{\cm'}\leq \left (\frac{g_1}{\cm'}+g_2\right )\cdot \mu^{100b}$.
From Property \ref{prop: new}, there must be a path $P'$ in graph $\tilde G'\setminus E^*$ connecting a vertex of $C_i$ to a vertex of $C_{i^*}\cup P$. We assume w.l.o.g. that $P'$ does not contain any vertex of $V(C_i)\cup V(C_{i^*})\cup V(P)$ as an inner vertex. We will reach a contradiction by showing that there is some edge $e\in E(P')$, whose image crosses the image of an edge of $J_{i^*}\cup P$ in $\phi''$. This is impossible because then $e$ should have been added to $E^*$.
	
Let $\psi$ be a drawing obtained from drawing $\phi''$ by deleting the images of all edges of $E^*$ from the drawing. We view $\psi$ as a drawing on the sphere, and we define, for all $1\leq \ell\leq z$, a disc $D(J_{\ell})$, whose boundary follows the image of the core $J_{\ell}$ inside the face $F$, as before. Note that the image of the connected component $C_{\ell}$ of $W$ must be contained in the disc $D(J_{\ell})$.

Since path $P'$ originates at a vertex of $C_i$ and terminates at a vertex of $C_{i^*}\cup P$, its image must intersect region $F$. We denote by $Q_1,Q_2,\ldots,Q_h$ maximal subpaths of the path $P'$, such that for all $1\leq h'\leq h$, the image of the path $Q_{h'}$ in $\psi$ is contained in the interior of region $F$, except for its endpoints that lie on the boundary of $F$. We assume that paths $Q_1,\ldots,Q_h$ appear on path $P'$ in this order. For all $1\leq h'\leq h$, we denote by $1\leq a_{h'}\leq z$ the index for which the first vertex of $Q_{h'}$ belongs to core $J_{a_{h'}}$, so $a_1=i$. From the definition of the paths $Q_1,\ldots,Q_h$, for all $1\leq h'\leq h$, the last vertex of $Q_{h'-1}$ must also belong to core $J_{a_{h'}}$, and the last vertex of $Q_h$ must belong to and the last vertex of $Q_h$ must belong to $J_{i^*}\cup J_{i^{**}}\cup  P\cup P'$.  

Consider now some index $1\leq h'\leq h$. Let $e_{h'}$ be the first edge on path $Q_{h'}$, and let $e'_{h'}$ be the last edge on path $Q_{h'}$. Since the images of the edges of path $P'$  in $\psi$ may not cross the images of any edges of $W$, and the image of $P'$ intersects the interior of $F$, we get that $\psi(e_{h'})\subseteq F$. Moreover, since an endpoint of $e_{h'}$ belongs to $J_{a_{h'}}$, from the definition of valid core structure (see \Cref{def: valid core 2}), $e_{h'}\in E(G)$ must hold. Using a similar reasoning, $e'_{h'}\in E(G)$. Since no inner vertex of $Q_{h'}$ belongs to $J_{i^*}\cup P$, and since $V(G_1)\cap V(G_2)\subseteq V(J_{i^*})\cup V(P)$, it must be the case that either $Q_{h'}\subseteq G_1$, or $Q_{h'}\subseteq G_2$. Since $J_i=J_{a_1}\subseteq G_1$, and since, for all $1\leq h'< h$ the last vertex of $Q_{h'}$ and the first vertex of $Q_{h'+1}$ belong to the same core $J_{a_{h'}}$, it must be the case that for all $1\leq h'\leq h$, $Q_{h'}\subseteq G_1$. 

 Recall that the image $\rho_{\tilde C}$ of graph $\tilde C=C_{i^*}\cup P$ has two faces, that we denoted by $ F^{i^*}_1$ and $ F^{i^*}_2$, that correspond to regions $F_1$ and $F_2$ of the drawing of $W'$ induced by $\phi'$, respectively. Clearly, for all $1\leq h'\leq h$, the image of $J_{h'}$ is either contained in $F^{i^*}_1$, or it is contained in $ F^{i^*}_2$. The image of $J_{i}$ is contained by $ F^{i^*}_2$ from our assumption that it is not contained in $F^{i^*}_1$. However, if we denote by $e^*$ the last edge on path $Q_h$, then the image of $e^*$ must be contained in $ F^{i^*}_1$, since $e^*\in E(G_1)$, and so $e^*\in \tilde E_1$ must hold. 
We conclude that the image of some path $Q_{h'}$ must intersect both regions $F^{i^*}_1$ and $F^{i^*}_2$, which may only happen if the image of some edge $e\in E(P')$ crosses the image of some edge $e\in E(P\cup C^*)$ in $\psi$, which is  impossible.
	
	The proof for the case where $J_i\subseteq G_2$ is symmetric.
\end{proof}

We now consider pairs $C,C'$ of connected components of $W'$, where $C=\tilde C$, and $R_{C_{i^*}}(C')=F^{i^*}$.

We consider three cases. The first case is when vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees of the forest $H(\wset)$. In this case, there must be an index $1\leq i\leq z$ with $i\neq i^*$, such that  vertex $x_{C'}$ is a descendant of vertex $x_{C_i}$, or $x_{C'}=x_{C_i}$. If $J_i\subseteq G_1$, then we set $R_{\tilde C}(C')=F^{i^*}_1$, and otherwise, we set $R_{\tilde C}(C')=F^{i^*}_2$. From \Cref{obs: cores drawn correctly}, it is easy to verify that the image of component $C'$ in the drawing $\phi''$ is indeed contained in region $R_{\tilde C}(C')$.

The second case is when vertex $x_{C_1}$ is a parent-vertex of vertices $x_{C_2},\ldots,x_{C_z}$ in forest $H(\wset)$, and $i^*=1$. In this case, there must be an index $2\leq i\leq z$, such that vertex $x_{C'}$ is a descendant of vertex $x_{C_i}$, or $x_{C'}=x_{C_i}$. We set $R_{\tilde C}(C')$ exactly as in Case 1.

The third and the last case is when vertex $x_{C_1}$ is a parent-vertex of vertices $x_{C_2},\ldots,x_{C_z}$ in forest $H(\wset)$, and $i^*=1$.
If there is an index  $1\leq i\leq z$ with $i\neq i^*$, such that  vertex $x_{C'}$ is a descendant of vertex $x_{C_i}$, or $x_{C'}=x_{C_i}$, then we set the region $R_{\tilde C}(C')$ exactly like in Cases 1 and 2. Otherwise, either $C'=C_1$, or vertex $x_{C'}$ is an ancestor of vertex $x_{C_1}$. In this case, if $C_1\subseteq G_1$, then we set $R_{\tilde C}(C')=F^{i^*}_1$, and otherwise we set $R_{\tilde C}(C')=F^{i^*}_2$. As before, from  \Cref{obs: cores drawn correctly}, it is easy to verify that the image of component $C'$ in the drawing $\phi''$ is indeed contained in region $R_{\tilde C}(C')$.


This completes the definition of the regions $R_{C}(C')$ of pairs $C,C'\in \cset(W')$ of distinct connected components. From the above discussion, for each such pair $C,C'$ of regions, the image of component $C'$ in $\phi''$ is contained in region $R_{C}(C')$.

Finally, we need to consider the case where face $F^{i^*}$ is the infinite face of the drawing $\rho_{C_{i^*}}$. In this case, we need to designate one of the two new faces $F^{i^*}_1$ or $F^{i^*}_2$ as the infinite face of the new drawing $\rho_{\tilde C}$ of graph $\tilde C$, in a way that is consistent with the drawing $\phi''$. If vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees of the forest $H(\wset)$, then we designate one of the two faces  $F^{i^*}_1$, $F^{i^*}_2$ as the infinite face of $\rho_{\tilde C}$ arbitrarily. Otherwise, vertex  $x_{C_1}$ is a parent-vertex of vertices $x_{C_2},\ldots,x_{C_z}$ in forest $H(\wset)$, and, since $F^{i^*}=F^*(\rho_{C_{i^*}})$, $i^*\neq 1$ must hold. If $C_1\subseteq G_1$, then we let $F^{i^*}_1$ be the infinite face of $\rho_{\tilde C}$, and otherwise we let $F^{i^*}_2$ be the infinite face of $\rho_{\tilde C}$. It is easy to verify that this choice is consistent with the drawing $\phi''$. 

To summarize, we have constructed a skeleton augmenting structure $\wset'$, whose corresponding skeleton augmentation is denoted by $W'$, and a set $E^{\del}(F)\subseteq E(G)\setminus E(W')$ of edges. If bad event $\event'$ did not happen, then, as we have shown already, $|E^{\del}(F)|\leq \frac{g_1\cdot \mu^{48}}{m}+g_2$ holds. 
Our construction guarantees that $W\subseteq W'$ and $\tilde \fset(\wset')=\left(\tilde\fset(\wset)\setminus\set{F}\right)\bigcup\set{F_1,F_2}$.



Let $\gset'$ be a collection of graphs constructed as follows. For every face $F'\in \tilde \fset(\wset)\setminus\set{F}$, we add the graph $G_{F'}\in \gset$ to $\gset'$. Additionally, we add graph $G_{F_1}=G_1$ that is associated with the new face $F_1\in \tilde \fset(\wset')$, and graph $G_{F_2}=G_2$, that is associated with face $F_2\in \tilde \fset(\wset')$.

From our construction, $E(G_F)\setminus (E(G_{F_1})\cup E(G_{F_2}))= E^{\del}(F)$. Moreover, from \Cref{obs: few edges in split graphs case2.2}
	If Event $\event'$ did not happen, then $|E(G_{F_1})\setminus E(W')|,|E(G_{F_2})\setminus E(W')|\leq |E(G_F)\setminus E(W)|-\frac{\cm'}{\mu^{5b}}$.
	
Recall that we denoted $\tilde G''=\tilde G\setminus E^{\del}(F)=\cG'\setminus(E^{\del}\cup E^{\del}(F))$, and we let $\tilde \Sigma''$ be the rotation system for graph $\tilde G''$ induced by $\cSigma'$. We have shown that, if bad event $\event'$ does not happen, then there is a solution $\phi''$	to the resulitng instance $\tilde I''=(\tilde G'',\tilde \Sigma'')$ that is $\wset'$-compatible. Since drawing $\phi$ ws semi-clean with respect to $\ckset$, it is easy to verify that drawing $\phi''$ has this property as well. Additionally, from our construction, $\cro(\phi'')\leq \cro(\phi)$ and  $|\chi^{\dirty}(\phi)|\leq |\chi^{\dirty}(\phi')|$. Lastly, let  $N(\phi)$ be the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate, and define $N(\phi'')$ similarly for $\phi''$, then $N(\phi'')-N(\phi)$ is bounded by the number of crossings in $\phi$, in which the edges of the path $P$ participate. If bad event $\event'$ does not happen, then $N(\phi'')-N(\phi)\leq \frac{\cro(\phi)\cdot \mu^{15b}}{4m}\leq \frac{\cro(\phi)\cdot \mu^{17b}}{\cm'}$, since $m\geq \cm'/\mu^{2b}$ must hold. We conclude that, if bad event $\event'$ does not happen, and path set $\pset$ was a promising path set of type $2$, then we obtain a valid output for Procedure $\procsplit'$. Since $\prob{\event'}\leq \frac{1}{\mu^{11b}}$, this concludes the analysis of the algorithm for Case 1.






\subsubsection*{Case 2: $\pset$ was a type-3 promising  path set}

In the second case, the promising set $\pset$ of paths was of type 3. We let $1\leq i^{**}\leq z$ be the index for which all paths in $\pset$ terminate at vertices of $\othercore$. 
 
If the two paths chosen from $\pset^*$ share at least one vertex of $V(G)\setminus V(K)$, then we have constructed a type-2 enhancement whose both endpoints lie in $\thecore$. In this case, the algorithm and its analysis are practically identical to those from Case 1 and are omitted here. We now assume that the two chosen paths are disjoint from each other. For convenience of notation, we denote $P=\firstpath$ and $P'=\secondpath$. Throughout, we denote by $\tilde J$ the graph obtained from the union of $\thecore,\othercore,P$ and $P'$. We also let $\tilde C=C_{i^*}\cup C_{i^{**}}\cup P\cup P'$.
Recall that we set $W'=W\cup P\cup P'$.
Recall also that, from \Cref{claim: new drawing2}, if Event $\event'$ does not happen, then  drawing $\phi'$ of $G'=G\setminus E'$ contains no crossings between the edges of $E(W')$. 
Throughout, we denote by $\gamma$ the image of path $P$ and by $\gamma'$ the image of path $P'$ in $\phi'$. 



In order to construct the skeleton augmenting structure $\wset'$, we first let $W'=W\cup P\cup P'$ be the skeleton augmentation associated with $\wset'$. Next, we define a drawing $\rho_C$ for every component $C\in \cset(W)$.

For every component $C\in \cset(W')\setminus \set{\tilde C}$, its drawing $\rho_C$ in $\wset'$ remains the same as in $\wset$. 
Consider now the component $\tilde C$. We would like to ensure that the drawing $\rho_{\tilde C}$ of $\tilde C$ that we define is identical to the drawing of $\tilde C$ induced by $\phi'$. Recall that we are given, as part of skeleton augmenting structure $\wset$, a drawing $\rho_{C_{i^*}}$ of graph $C_{i^*}$, a drawing $\rho_{C_{i^{**}}}$ of graph $C_{i^{**}}$, and an orientation $b'_u$ of every vertex $u\in V(C_{i^*})\cup  V(C_{i^*})$. We are also given a face $F^{i^*}\in \fset(\rho_{C_{i^*}})$, such that the face $F$ in drawing $\phi$ is contained in the region $F^{i^*}$, and a face $F^{i^{**}}\in \fset(\rho_{C_{i^{**}}})$, such that the face $F$ in drawing $\phi$ is contained in the region $F^{i^{**}}$. Since drawing $\phi$ is $\wset$-compatible, and it does not contain any crossings between the edges of $W'$, we are guaranteed that paths  $P$ and $P'$ are drawn inside the region $F^{i^*}\cap F^{i^{**}} $ of $\phi'$, in a natural way.
However, we do not know the orientations of the drawings $\rho_{C_{i^*}}$ of $C_{i^*}$ and $\rho_{C_{i^{**}}}$ of $C_{i^{**}}$ with respect to each other in $\phi'$. We overcome this difficulty in the same way as in Procedure \procsplit.

We recall how the paths $P$ and $P'$ were constructed. 
We started with a set $\pset^*$ of $k'=\ceil{\frac{4m}{\mu^{3b}}}$ simple edge-disjoint paths in graph $G$, with every path originating at a vertex of $J_{i^*}$ and terminating at a vertex of $J_{i^{**}}$. Additionally, the paths in $\pset^*$ are internally disjoint from the skeleton $K$, and they are non-transversal with respect to $\Sigma$. We denoted by $E^*_1\subseteq \delta(J_{i^{*}})$ the subset of edges that belong to the paths of $\pset^*$, letting $E^*_1=\set{e_1,\ldots,e_{k'}}$, where the edges are indexed in the order of their appearence in the ordering $\oset(J_{i^{*}})$. For all $1\leq j\leq k'$, we denoted by $P_j\in \pset^*$ the unique path originating at the edge $e_j\in E^*_1$. We then selected an index $\floor{k'/8}<j^*<\ceil{k'/4}$ uniformly at random, that determined the chosen paths $P_{j^*}$ and $P_{j^*+\floor{k'/2}}$. Since we assumed that the chosen paths do not share any vertices of $V(G)\setminus V(K)$, we eventually set $P=P_{j^*}$ and $P'=P_{j^*+\floor{k'/2}}$.

We choose another index $j^*< j^{**}<j^*+\floor{k'/2}$ uniformly at random, and we let $P''=P_{j^{**}}$. We say that a bad event $\event'_5$ happens if  $P''$ is a bad path, or some edge $e\in E(P'')$ crosses the image of an edge of $P\cup P'$ in the drawing $\phi$. From \Cref{obs: number of bad paths2}, the number of bad paths in $\pset^*$ is at most $\frac{10m}{\mu^{15b}}$. Moreover, if bad event $\event'$ did not happen, then both paths $P$ and $P'$ are good, and so the number of crossings in which the edges of $E(P)\cup E(P')$ participate in $\phi$  is  at most $\frac{\cro(\phi)\mu^{15b}}{4m}\leq \frac{m}{4\mu^{15b}}$  (from Property \ref{prop valid input drawing2} of valid input to Procedure \procsplit, and since $m\leq \cm'$). Therefore, if Event $\event'$ did not happen, there are at most $\frac{12m}{\mu^{15b}}$ indices $1\leq i\leq k$, such that path $P_i$ is bad, or some edge of $P_i$ crosses an edge of $E(P)\cup E(P')$ in $\phi$.
Since $k'=\ceil{\frac{4m}{\mu^{3b}}}$, $\prob{\event_5'\mid \neg\event'}\leq \frac{3}{\mu^{12b}}$.



Consider the graph $\tilde C'=C_{i^*}\cup C_{i^{**}}\cup P\cup P'\cup P''$. If bad events $\event',\event_5$ did not happen, then there is a unique planar drawing $\tilde \rho'$ of graph $\tilde C'$ that has the following properties:

\begin{itemize}
	\item the drawing of $C_{i^*}$ induced by $\tilde \rho'$ is $\rho_{C_{i^*}}$;
	\item the drawing of $C_{i^{**}}$ induced by $\tilde \rho'$ is $\rho_{C_{i^{**}}}$;
	\item the images of path $P$, $P'$ and $P''$ are contained in region $F^{i^*}\cap F^{i^{**}}$; 
	\item the drawing is consistent with the rotation system $\cSigma'$; 
	\item  the orientation of every vertex $u\in V(C_{i^*})$ in the drawing is the orientation $b'_u$ given by $\wset$; and
	\item either the orientation of every vertex $u\in V(C_{i^{**}})$ in the drawing is the orientation $b'_u$ given by $\wset$ (in which case we say that the orientations of $C_{i^*}$ and $C_{i^{**}}$ agree), or  the orientation of every vertex $u\in V(C_{i^{**}})$ in the drawing is $-b'_u$ (in which case we say that the orientations of $C_{i^*}$ and $C_{i^{**}}$ disagree).
\end{itemize}

Drawing $\tilde \rho'$ with all above properties can be computed efficiently. We then let $\rho_{\tilde C}$ be the drawing of $\tilde C$ induced by $\tilde \rho'$. From the above discussion, if neither of the events $\event',\event'_5$ happened, then $\rho_{\tilde C}$ is identical to the drawing of $\tilde C$ induced by $\phi'$.


Notice that the set $\fset(\rho_{\tilde C})$ of faces of this new drawing of graph $\tilde C$ is precisely $\left (\fset(\rho_{C_{i^*}})\cup \fset(\rho_{C_{i^{**}}}\right )\setminus \set{F^{i^*},F^{i^{**}}})\cup (F^{i^*}_1,F^{i^*}_2)$, where $F^{i^*}_1$ and $F^{i^*}_2$ are the two new faces that are obtained by partitioning the region $F^{i^*}\cap F^{i^{**}}$ with the images of paths $P$ and $P'$. We assume w.l.o.g. that region $F^{i^*}_1$ in the drawing of $W'$ induced by $\phi'$ contains the face $F_1$ of this drawing, and region $F^{i^*}_2$ contains the face $F_2$.

Notice that, in the skeleton structure $\wset$,  $R_{C_{i^*}}(C_{i^{**}})=F^{i^*}$ and $R_{C_{i^{**}}}(C_{i^{*}})=F^{i^{**}}$ must hold. Moreover, from the definition of skeleton augmenting structure, either $F^{i^*}=F^*(\rho_{C_{i^*}})$, or  $F^{i^{**}}=F^*(\rho_{C_{i^{**}}})$ must hold. 
If $F^{i^*}=F^*(\rho_{C_{i^*}})$ but $F^{i^{**}}\neq F^*(\rho_{C_{i^{**}}})$, then face $F^*(\rho_{C_{i^{**}}})$ is also a face of $\rho_{\tilde C}$, and we set this face to be the infinite face $F^*(\rho_{\tilde C})$. Similarly, if  $F^{i^{**}}= F^*(\rho_{C_{i^{**}}})$ but $F^{i^*}\neq F^*(\rho_{C_{i^*}})$, then face $F^*(\rho_{C_{i^{*}}})$ is also a face of $\rho_{\tilde C}$, and we set this face to be the infinite face $F^*(\rho_{\tilde C})$. If  $F^{i^*}=F^*(\rho_{C_{i^*}})$ and $F^{i^{**}}\neq F^*(\rho_{C_{i^{**}}})$, then  we will designate one of the faces $F^{i^*}_1$ or $F^{i^*}_2$ as the infinite face of the drawing $\rho_{\tilde C}$ later.


So far we have defined the new skeleton augmentation $W'$ and a drawing $\rho_C$ of every connected component $C\in \cset(W)$. Next, we define the orientation $b'_u$ of every vertex $u\in V(W')$. For vertices $u\in (V(W')\cap V(W))\setminus V(C_{i^{**}})$, the orientation $b'_u$ in $\wset'$ remains the same as the orientation $b'_u$ in $\wset$. 
If the orientations of $C_{i^*}$ and $C_{i^{**}}$ agree in drawing $\tilde \rho'$, then for every vertex $u\in V(C_{i^{**}})$, the  orientation $b'_u$ in $\wset'$ remains the same as the orientation $b'_u$ in $\wset$; otherwise, for every vertex $u\in V(C_{i^{**}})$, the  orientation $b'_u$ is reversed in $\wset'$.
It now remains to define the orientation $b'_u$ of vertices $u\in (V(P)\cup V(P'))\setminus (V(C_{i^*})\cup V(C_{i^{**}})$. The procedure for computing these orientations is very similar to the one from Procedure $\procsplit$.


As in Case 1, for every vertex $u\in V(\tilde C)$, we consider the tiny $u$-disc $D_{\phi'}(u)$.  For every edge $e\in \delta_{G}(u)\setminus E'$, we denote by $\sigma(e)$ the segment of $\phi'(e)$ that is drawn inside the disc $D_{\phi'}(u)$. Since edge $e$ belongs to graph $G$, $\sigma(e)$ must be contained in the region $F\in \fset(W)$ of the drawing $\phi'$.  Let $\tilde E=\left (\bigcup_{u\in V(P)\cup V(P')\cup V(\thecore)\cup V(\othercore)}\delta_{G'}(u)\right )\setminus (E(P)\cup E(P')\cup E(\thecore)\cup E(\othercore))$. 
The images of paths $P$ and $P'$ in $\phi'$ split region $F$ into two regions, that we denote by $F_1$ and $F_2$. We let $e_1\in E_1$ be any edge that does not lie in $E(P)\cup E(P')$, and we assume without loss of generality that $\sigma(e_1)\subseteq F_1$.


We partition edge set $\tilde E$ into a set $\tilde E^{\inn}$ of \emph{inner edges} and the set $\tilde E^{\out}$ of outer edges, as before: Edge set $\tilde E^{\inn}$ contains all edges $e\in \tilde E$ with $\sigma(e)$ contained in the face $F_1$ of $\rho_{\tilde C}$, and $\tilde E^{\out}$ contains all remaining edges (so for every edge $e\in \tilde E^{\out}$, $\sigma(e)$ is contained in $F_2$). As before, we show an algorithm that correctly computes the orientation of every vertex $u\in (V(P)\cup V(P'))\setminus (V(\thecore)\cup V(\othercore))$ in the drawing $\phi'$, and the partition $(\tilde E^{\inn},\tilde E^{\out})$ of the edges of $\tilde E$.

The algorithm for computing the orientation of the inner vertices of $P$ and $P'$ is practically identical to the one used in Case 1, and modifies it in the same way as the algorithm for Case 3 in \procsplit modified the algorithm for Case 2. We omit it here. 
In order to complete the construction of the skeleton augmenting structure $\wset'$, it remains to define, for every pair $C,C'\in \cset(W')$ of distinct connected components, a face $R_C(C')$ of $\fset(\rho_C)$. Additionally, if  $F^{i^*}=F^*(\rho_{C_{i^*}})$ and $F^{i^{**}}\neq F^*(\rho_{C_{i^{**}}})$, then  we  need to designate one of the faces $F^{i^*}_1$ or $F^{i^*}_2$ as the outer face of the drawing $\rho_{\tilde C}$ of component $\tilde C$. We do so in the next step, once we split the graph $G'$ into two subgraphs, $G_1$ and $G_2$.


\paragraph{Computing the Split.}
The construction of the flow network $\tilde H'$ an $s$-$t$-cut $(A,B)$ in $\tilde H'$, and edge set $E''=E_{\tilde H'}(A,B)$ are identical to those in Case 3 of Step 2 of Procedure \procsplit. Using the same arguments as in the proof of \Cref{claim: cut set small case2.2}, if neither of the bad events $\event',\event'_5$ happened, then $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.



%The proof of the claim is essentially identical to the proof of \Cref{claim: cut set small case2.2}. We assume for contradiction that Event $\event'$ did not  happen, but $|E''|\leq \frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$.
%We can then use Max Flow -- Min Cut theorem to construct a collection  $\qset$ of edge-disjoint paths in graph $G'$, such that, for every path $Q\in \qset$, drawing $\phi'$ must contain at least one crossing between an edge of $Q$ and an edge of $W\cup P$. Since Event $\event'$ did not happen, path $P$ is good, so its edges participate in at most $\frac{\cro(\phi)\mu^{15b}}{4m}$ crossings in $\phi$ and hence in $\phi'$. Additionally, edges of $\cK$ participate in at most $|\chi^{\dirty}(\phi)|$ crossings in $\phi$ (and hence in $\phi'$), and edges of $W\setminus K$ participate in at most $\frac{\cro(\phi)\cdot \mu^{26b}}{\cm'}\leq \frac{\cro(\phi)\cdot \mu^{26b}} m$ crossings from Property \ref{prop: drawing}. Overall, there are fewer than $\frac{\cro(\phi)\mu^{30b}}{m}+|\chi^{\dirty}(\phi)|$ crossings in $\phi'$ in which edges of $P\cup W$ participate, a contradiction.






We now construct the  graphs $G_1,G_2$ associated with the faces $F_1$ and $F_2$, respectively.
In order to do so, we define two vertex sets $A',B'$ of graph $G'$, as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every index $1\leq i\leq r$ with $i\not\in\set{ i^*,i^{**}}$, if $v_{J_i}\in A$, then we replace vertex $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 


Additionally, we let $J\subseteq \thecore\cup\othercore\cup P\cup P'$ be the graph containing all vertices and edges of $\thecore\cup\othercore\cup P\cup P'$, whose images in $\rho_{\tilde C}$ lie on the boundary of face $F^{i^*}_1$. Similarly, we let $J'\subseteq \thecore\cup \othercore\cup P\cup P'$ be the graph containing all vertices and edges of $\thecore\cup\othercore\cup P\cup P'$, whose images  in $\rho_{\tilde C}$ lie on the boundary of face $F^{i^*}_2$. 

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J))$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma'$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. 
The following observation is an analogue of \Cref{obs: few edges in split graphs case2.2} and its proof follows from the same arguments. 



\begin{observation}\label{obs: few edges in split graphs case2.3}
	If Event $\event'$ did not happen, then $|E(G_1)\setminus E(W')|,|E(G_2)\setminus E(W')|\leq |E(G)\setminus E(W)|-\frac{\cm'}{\mu^{5b}}$.
\end{observation}




Let $E^{\del}(F)=E'\cup E''$. As in Case 1, if bad event $\event'$ did not happen, then $|E^{\del}(F)|\leq \frac{g_1\cdot \mu^{48}}{m}+g_2$, as required.
As in Case 1, we let $\tilde G''=\tilde G'\setminus E''=\tilde G\setminus E^{\del}$, and let $\tilde \Sigma''$ be the rotation system for graph $\tilde G''$ induced by $\tilde \Sigma$. We denote $\tilde I''=(\tilde G'',\tilde \Sigma'')$ the resulting instance of \cnwrs.
Let $\phi''$ be the drawing of $\tilde G''$ that is induced by the drawing $\phi'$ of $\tilde G'$. We also denote $G''=G'\setminus E''=G\setminus E^{\del}$. As before, $E(G_1)\cup E(G_2)=E(G'')$.



We now complete the construction of the skeleton augmenting structure $\wset'$. For all $1\leq i\leq z$, let $C_i\in \cset(W)$ be the connected component that contains the core $J_i$, and let $F^i\in \fset(\rho_{C_i})$ be the face that corresponds to face $F$ of $\tilde \fset(\wset)$ (in other words, face $F$ in the drawing of $W$ induced by $\phi$ is contained in region $F^i$). From the construction of the set $\tilde \fset(\wset)$ of faces, in the decomposition forest $H(\wset)$, either  vertices $x_{C_1},\ldots,x_{C_z}$ are the roots of the trees in the forest; or one of these vertices is the parent-vertex of the remaining vertices. We assume w.l.o.g. that in the latter case, vertex $x_{C_1}$ is the parent of vertices $x_{C_2},\ldots,x_{C_z}$ in the forest $H(\wset)$.



Consider any pair $C,C'\in \cset(W')$ of distinct connected components. Assume first that $C,C'\neq \tilde C$. In this case, face $R_{C}(C')$ remains the same in $\wset'$ in the augmenting structure $\wset$. Since drawing $\phi$ of $\tilde G$ was $\wset$-compatible, and drawing $\phi''$ is obtained from $\phi$ by deleting some edges that do not belong to $W'$, and possibly making some additional local changes within the region $F$, the image of component $C'$ in $\phi''$ remains contained in region $R_C(C')$ in $\phi''$.


Assume now that $C'=\tilde C$. It is easy to verify that, in this case,  in $\wset$, $R_{C'}(C_{i^*})=R_{C'}(C_{i^{**}})$ must hold.
Indeed, if $R_{C'}(C_{i^*})\neq F^*(\rho_{C'})$, then vertex $x_{C'}$ must be an ancestor of vertex $x_{C_{i^*}}$ in forest $H(\wset)$. Similarly, if $R_{C'}(C_{i^{**}})\neq F^*(\rho_{C'})$, then vertex $x_{C'}$ must be an ancestor of vertex $x_{C_{i^{**}}}$ in forest $H(\wset)$. Since vertices $x_{C_{i^*}}$ and  $x_{C_{i^{**}}}$ are either sibling vertices in $H(\wset)$, or one of them is a parent vertex of another, if vertex $x_{C'}$ is an ancestor of one of these two vertices, then it must be an ancestor of another. Moreover, since both components $C_{i^*},C_{i^{**}}$ belong to the set $\sset(F)$ of components corresponding to region $F$, $R_{C'}(C_{i^*})=R_{C'}(C_{i^{**}})$ must hold. We then set face $R_{C'}(\tilde C)$ in $\wset'$ to be the face $R_{C'}(C_{i^{*}})$ in $\wset$.
 It is easy to verify that the drawing of component $\tilde C$ in $\phi''$ remains in the region $R_{C'}(C_{i^*})$.



Next, we assume that $C=\tilde C$. Recall that components $C_{i^*}, C_{i^{**}}$ of $W$ are replaced by component $\tilde C=C_{i^*}\cup C_{i^{**}}\cup  P\cup P'$ in $W'$. We use the following observation, that is an analogue of  \Cref{obs: cores drawn correctly} for Case 1. The proof is almost identical and is provided here for completeness.


\begin{observation}\label{obs: cores drawn correctly2} Assume that neither of the Events $\event',\event'_5$ happenned.
	Consider any index $1\leq i\leq z$ with $i\not\in\set{ i^*,i^{**}}$. If $J_i\subseteq G_1$, then the image of $C_i$ appears in region  $F_1^{i^*}$ in $\phi''$, and if $J_i\subseteq G_2$, then the image of $C_i$ appears in region $F_2^{i^*}$ in $\phi''$.
\end{observation}
\begin{proof}
	Assume for contradiction that neither of the Events $\event',\event'_5$ happenned, and there is an index $1\leq i\leq z$ with $J_i\subseteq G_1$, such that the image of $C_i$ is not contained in region $F_1^{i^*}$ of $\phi''$.
	
	Let $E^*$ be the set of edges $e\in E(\tilde G'')$, such that the image of $e$ in $\phi''$ crosses the image of some edge of $W'$. Using the same accounting as in the proof of \Cref{obs: cores drawn correctly}, 
	 $|E^*|\leq \left (\frac{g_1}{\cm'}+g_2\right )\cdot \mu^{100b}$ must hold.
	From Property \ref{prop: new}, there must be a path $\tilde P$ in graph $\tilde G'\setminus E^*$, connecting a vertex of $C_i$ to a vertex of $C_{i^*}\cup C_{i^{**}}\cup P\cup P'$. We assume w.l.o.g. that $\tilde P$ does not contain any vertex of $V(C_i)\cup V(C_{i^*})\cup  V(C_{i^{**}}) V(P)\cup V(P')$ as an inner vertex. We will reach a contradiction by showing that there is some edge $e\in E(\tilde P)$, whose image crosses the image of an edge of $J_{i^*}\cup J_{i^{**}}\cup P \cup P'$ in $\phi''$. This is impossible because then $e$ should have been added to $E^*$.
	
	Let $\psi$ be a drawing obtained from drawing $\phi''$ by deleting the images of all edges of $E^*$ from the drawing. We view $\psi$ as a drawing on the sphere, and we define, for all $1\leq \ell\leq z$, a disc $D(J_{\ell})$, whose boundary follows the image of the core $J_{\ell}$ inside the face $F$, as before. As before, the image of the connected component $C_{\ell}$ of $W$ must be contained in the disc $D(J_{\ell})$.
	
	Since path $\tilde P$ originates at a vertex of $C_i$ and terminates at a vertex of $C_{i^*}\cup C_{i^{**}}\cup P\cup P'$, its image must intersect the interior of region $F$. We denote by $Q_1,Q_2,\ldots,Q_h$ maximal subpaths of the path $\tilde P$, such that for all $1\leq h'\leq h$, the image of the path $Q_{h'}$ in $\psi$ is contained in the interior of region $F$, except for its endpoints, that lie on the boundary of $F$. We assume that paths $Q_1,\ldots,Q_h$ appear on path $\tilde P$ in this order. For all $1\leq h'\leq h$, we denote by $1\leq a_{h'}\leq z$ the index for which the first vertex of $Q_{h'}$ belongs to core $J_{a_{h'}}$, so $a_1=i$. From the definition of the paths $Q_1,\ldots,Q_h$, for all $1\leq h'\leq h$, the last vertex of $Q_{h'-1}$ must also belong to core $J_{a_{h'}}$, and the last vertex of $Q_h$ must belong to $J_{i^*}\cup J_{i^{**}}\cup  P\cup P'$. 
	
	
	
	Consider now some index $1\leq h'\leq h$. Let $e_{h'}$ be the first edge on path $Q_{h'}$, and let $e'_{h'}$ be the last edge on path $Q_{h'}$. Since the images of the edges of path $\tilde P$  in $\psi$ may not cross the images of any edges of $W$, and the image of $\tilde P$ intersects the interior of $F$, we get that $\psi(e_{h'})\subseteq F$. Moreover, since an endpoint of $e_{h'}$ belongs to $J_{a_{h'}}$, from the definition of valid core structure (see \Cref{def: valid core 2}), $e_{h'}\in E(G)$ must hold. Using a similar reasoning, $e'_{h'}\in E(G)$. Since no inner vertex of $Q_{h'}$ belongs to $J_{i^*}\cup J_{i^{**}}\cup P\cup P'$, and since $V(G_1)\cap V(G_2)\subseteq V(J_{i^*})\cup V(J_{i^{**}})\cup V(J_{i^*})\cup V(P)\cup V(P')$, it must be the case that either $Q_{h'}\subseteq G_1$, or $Q_{h'}\subseteq G_2$. Since $J_i=J_{a_1}\subseteq G_1$, and since, for all $1\leq h'< h$ the last vertex of $Q_{h'}$ and the first vertex of $Q_{h'+1}$ belong to the same core $J_{a_{h'}}$, it must be the case that for all $1\leq h'\leq h$, $Q_{h'}\subseteq G_1$. 
	
	Recall that the image $\rho_{\tilde C}$ of graph $\tilde C=C_{i^*}\cup C_{i^{**}}\cup P\cup P'$ has two special faces, that we denoted by $ F^{i^*}_1$ and $ F^{i^*}_2$, which correspond to regions $F_1$ and $F_2$ of the drawing of $W'$ induced by $\phi'$, respectively. Clearly, for all $1\leq h'\leq h$, the image of $J_{h'}$ is either contained in $F^{i^*}_1$, or it is contained in $ F^{i^*}_2$. The image of $J_{i}$ is contained by $ F^{i^*}_2$ from our assumption that it is not contained in $F^{i^*}_1$. However, if we denote by $e^*$ the last edge on path $Q_h$, then the image of $e^*$ must be contained in $ F^{i^*}_1$, since $e^*\in E(G_1)$, and so $e^*\in \tilde E_1$ must hold. 
	We conclude that the image of some path $Q_{h'}$ must intersect both regions $F^{i^*}_1$ and $F^{i^*}_2$, which may only happen if the image of some edge $e\in E(\tilde P)$ crosses the image of some edge $e\in E(P\cup P'\cup C_{i^*}\cup C_{i^{**}})$ in $\psi$, which is  impossible.
	
	The proof for the case where $J_i\subseteq G_2$ is symmetric.
\end{proof}



We now consider some component $C'\in \cset(W')\setminus \set{\tilde C}$ and compute the region $R=R_{\tilde C}(C')$, such that the image of $C'$ in $\phi''$ is contained in $R$.

We need to consider several cases. Assume first that vertices $x_{C_{i^*}}$ and $x_{C_{i^{**}}}$ are siblings in the forest $H(\wset)$. 
If vertex $x_{C'}$ is a descenadnt of some vertex $x_{C_i}$, where $1\leq i\leq z$, $i\not\in \set{i^*,i^{**}}$, and $x_i$ is not a parent-vertex of $x_{C_{i^*}}$, then region $R=R_{\tilde C}(C')$ is determined as follows. If $J_i\subseteq G_1$, then we set $R_{\tilde C}(C')=F^{i^*}_1$, and otherwise we set $R_{\tilde C}(C')=F^{i^*}_2$. If $C'=C_i$ for some index $1\leq i\leq z$ with $i\not\in \set{i^*,i^{**}}$, such that and $x_i$ is not a parent-vertex of $x_{C_{i^*}}$, then we let $R_{\tilde C}(C')=F^{i^*}_1$ if $J_i\subseteq G_1$, and we let $R_{\tilde C}(C')=F^{i^*}_2$ otherwise. If vertex $x_{C'}$ is a descendant of $C_{i^*}$, then face $R_{C_{i^*}}(C')$ of $\fset(\rho_{C_{i^*}})$ is also a face of $\fset(\rho_{\tilde C})$, and we set $R_{\tilde C}(C')=R_{C_{i^*}}(C')$. If $x_{C'}$ is a descendant of $x_{C_{i^{**}}}$, then we set $R_{\tilde C}(C')$ similarly. 
If vertices $x_{C_{i^*}}, x_{C_{i^{**}}}$ are both roots of trees in the forest $H(\wset)$, then we designate face $F^{i^*}_1$ of $\fset(\rho_{\tilde C})$ as the infinite face of the drawing. In this case, for every component $C'\in  \cset(W')\setminus \set{\tilde C}$, vertex $x_{C'}$ is either a descendant of a vertex $x_{C_i}$ for $1\leq i\leq z$, or $x_{C'}\not\in \set{x_{C_1},\ldots,x_{C_z}}$, so region $R_{\tilde C}(C')$ is defined already. Otherwise, vertex $x_{C_1}$ is the parent-vertex of both $x_{C_{i^*}}$ and  $ x_{C_{i^{**}}}$. If $J_1\subseteq G_1$, then we designate face $F^{i^*}_1$ of $\fset(\rho_{\tilde C})$ as the infinite face of the drawing, and, for every component $C'\in \cset(W')$ such that $x_{C'}$ is not a descendant of $x_{C_1}$, we set $R_{\tilde C}(C')=F^{i^*}_1$. Otherwise, we designate face $F^{i^*}_2$ of $\fset(\rho_{\tilde C})$ as the infinite face of the drawing, and, for every component $C'\in \cset(W')$ such that $x_{C'}$ is not a descendant of $x_{C_1}$, we set $R_{\tilde C}(C')=F^{i^*}_2$.

It remains to consider the case where one of the vertices $x_{C_{i^*}}$, $x_{C_{i^{**}}}$ is the parent-vertex of the other in forest $H(\wset)$. We assume w.l.o.g. that $x_{C_{i^*}}$ is the parent of $x_{C_{i^{**}}}$. In this case, the infinite face $F^*(\rho_{C_{i^*}})$ is also a face of drawing $\rho_{\tilde C}$ of $\tilde C$, and it is designated as the infinite face of  $\rho_{\tilde C}$ of drawing  Consider now some component $C'\in \cset(W')\setminus \tilde{C}$. If vertex $x_{C'}$ is a descendant of any vertex of $\set{x_{C_i}\mid 1\leq i\leq z; i\neq i^*}$, or $x_{C'}\in \set{x_{C_i}\mid 1\leq i\leq z; i\not\in \set{i^*,i^{**}}}$,  then we set $R_{\tilde C}(C')$ exactly as before. Otherwise, we set $R_{\tilde C}(C')=F^*(\rho_{\tilde C})=F^*(\rho_{C_{i^*}})$.


This completes the definition of the regions $R_{C}(C')$ of pairs $C,C'\in \cset(W')$ of distinct connected components. It is easy to verify that, for each such pair $C,C'$ of regions, the image of component $C'$ in $\phi''$ is contained in region $R_{C}(C')$.
We have also defined the infinite face of the drawing $\rho_{\tilde C}$.

To summarize, we have constructed a skeleton augmenting structure $\wset'$, whose corresponding skeleton augmentation is denoted by $W'$, and a set $E^{\del}(F)\subseteq E(G)\setminus E(W')$ of edges. If neither of the bad events $\event',\event'_5$ happenned, then, as we have shown already, $|E^{\del}(F)|\leq \frac{g_1\cdot \mu^{48}}{m}+g_2$ holds. 
Our construction guarantees that $W\subseteq W'$ and $\tilde \fset(\wset')=\left(\tilde\fset(\wset)\setminus\set{F}\right)\bigcup\set{F_1,F_2}$.
The construction of the $\wset'$-decomposition $\gset'$ remains the same as in Case 1, and the remainder of the analysis remains the same as before.  We conclude that, if neither of the bad events $\event'$, $\event'_5$ happenned, and path set $\pset$ was a promising path set of type $3$, then we obtain a valid output for Procedure $\procsplit'$. Since 
$\prob{\event'}\leq \frac{1}{\mu^{11b}}$ and $\prob{\event_5'\mid \neg\event'}\leq \frac{3}{\mu^{12b}}$, the probability that at least one of these two events happens is at most $\frac{1}{\mu^{11b}}+\frac{3}{\mu^{12b}}\leq \frac{1}{\mu^{10b}}$. This concludes the analysis of the algorithm for Case 2.




==> appx-wld-basic.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Proof of Theorem~\ref{thm:well_linked_decomposition}}
\label{apd: Proof of well_linked_decomposition}


\mynote{I am rewriting this proof right now. Please don't change this file.}
 
Our algorithm maintains a collection $\rset$ of clusters of $S$, that is initialized to $\rset=\set{S}$. Throughout the algorithm, we ensure that the clusters in $\rset$ are disjoint, and that $\bigcup_{R\in \rset}V(R)=V(S)$. For a given collection $\rset$ of clusters with the above properties, we define a \emph{budget} $b(e)$ for every edge $e\in E(G)$, as follows. If $e\in \delta_G(S)$, and its endpoint $v$ that lies in $S$ belongs to a cluster $R\in\rset$, then we set the budget $b(e)=1+8\alpha \cdot \cdot \alphasc(m)\cdot \log_{3/2}(|\delta_G(R)|)$. If edge $e$ has its endpoints in two distinct clusters $R,R'\in \rset$, then we set $b(e)=2+8\alpha\cdot \alphasc(m)\cdot \log_{3/2}(|\delta_G(R)|)+8\alpha \cdot \alphasc(m)\cdot \log_{3/2}(|\delta_G(R')|)$. Otherwise, we set $b(e)=0$.
Notice that, for every edge $e\in E(G)$, $b(e)\leq 3$ always holds. Additionally, for every edge $e\in \bigcup_{R\in \rset}\delta_G(R)$, $b(e)\geq 2$ if the endpoints of $e$ lie in two different clusters of $\rset$, and $b(e)\geq 1$ if $e\in \delta_G(S)$. Therefore, if we denote by $B=\sum_{e\in E(G)}b(e)$ the total budget in the system, then, throughout the algorithm, $B\geq \sum_{R\in \rset}|\delta_G(R)|$ holds. Lastly, observe that, at the beginning of the algorithm, $B\leq |\delta_G(S)|\cdot (1+O(\alpha\cdot \alphasc(m)\cdot \log m))$. Throughout the algorithm, we will modify the clusters in set $\rset$, which will lead to changes in budgets of the edges of $G$. We will ensure however that the total budget $B$ never increases, and so, if $\rset$ is the final set of clusters that we obtain, then $\sum_{R\in \rset}|\delta_G(R)|\leq B\leq (1+O(\alpha\cdot \alphasc(m)\cdot \log m))=(1+O(\alpha\cdot \log^{1.5} m))$ holds.


Throughout the algorithm, we maintain a partition of the set $\rset$ of clusters into two subsets: set $\rset^A$ of \emph{active} clusters, and set $\rset^I$ of \emph{inactive} clusters. We will ensure that every cluster $R\in \rset^I$ has the $\alpha$-bandwidth property. Additionally, we will store, with every inactive cluster $R\in \rset^I$, a set $\pset(R)=\set{P(e)\mid e\in \delta_G(R)}$ of paths in graph $G$, (that we refer to as \emph{witness path set for $R$}), that causes edge-congestion at most $100$, and, for every edge $e\in \delta_G(R)$, path $P(e)$ has $e$ as its first edge and some edge of $\delta_G(S)$ as its last edge, and all inner vertices of $P(e)$ lie in $V(S)\setminus V(R)$. At the beginning of the algorithm, we set $\rset^A=\rset=\set{S}$ and $\rset^I=\emptyset$. The algorithm proceeds in iterations, as long as $\rset^A\neq \emptyset$.

We now describe a single iteration. The iteration selects an arbitrary cluster $R\in \rset^A$ to process. It then either establishes that $R$ has the $\alpha$-bandwidth property in graph $G$, and computes a witness path set for $R$ (in which case $R$ is moved from $\rset^A$ to $\rset^I$); or it modifies the set $\rset$ of clusters in a way that ensures that the total budget of all edges decreases by at least $1/m$. An iteration that processes a cluster $R\in \rset^A$ consists of two steps. The purpose of the first step is to either establish the $\alpha$-bandwidth property of cluster $R$, or to replace it with a collection of smaller clusters in $\rset$. The purpose of the second step is to either compute the witness set $\pset(R)$ of paths for cluster $R$, or to modify the set $\rset$ of clusters in a way that decreases the total budget of all edges. We now describe each of the two steps in turn.




\paragraph{Step 1: Bandwidth Property.}

Let $R^+$ be the augmentation of the cluster $R$ in graph $G$. Recall that $R^+$ is a graph that is obtained from $G$ through the following process. First, we subdivide every edge $e\in \delta_G(R)$ with a vertex $t_e$, and we let $T=\set{t_e\mid e\in \delta_G(R)}$ be the resulting set of vertices. We then let $R^+$ be the subgraph of the resulting graph induced by vertex set $V(R)\cup T$. We apply the algorithm  \algsc  for computing approximate sparsest cut to graph $R^+$, with the set $T$ of vertices, to obtain a $\alphasc(m)$-approximate sparsest cut $(X,Y)$ in graph $R^+$ with respect to vertex set $T$. 
We now consider two cases. The first case happens if $|E(X,Y)|> \alpha\cdot \alphasc(m)\cdot \min\set{|X\cap T|,|Y\cap T}$. In this case, we are guaranteed that the smallest sparsity of any $T$-cut in graph $R^+$ is at least $\alpha$, or equivalently, set $T$ of vertices is $\alpha$-well-linked in $R^+$. From \Cref{obs: wl-bw}, cluster $R$ has the $\alpha$-bandwidth property in graph $G$. In this case, we proceed to the second step of the algorithm.

Assume now that $|E(X,Y)|\leq \alpha\cdot \alphasc(m)\cdot \min\set{|X\cap T|,|Y\cap T}$. 
Since $\alpha< \min\set{1/\alphasc(m),1/(48\log^2 m)}$, we get that the sparsity of the cut $(X,Y)$ is less than $1$.  Consider now any vertex $t\in T$, and let $v$ be the unique neighbor  of $t$ in $R^+$. We can assume w.l.o.g. that either $t,v$ both lie in $X$, or they both lie in $Y$. Indeed, if $t\in X$ and $v\in Y$, then moving vertex $t$ from $X$ to $Y$ does not increase the sparsity of the cut $(X,Y)$. This is because, for any two reals $1\leq a<b$, $\frac{a-1}{b-1}\leq \frac a b$. Similarly, if $t\in Y$ and $v\in X$, then moving $t$ from $Y$ to $X$ does not increase the sparsity of the cut $(X,Y)$. Therefore, we assume from now on, that for every vertex $t\in T$, if $v$ is the unique neighbor of $t$ in $R^+$, then either $v,t\in X$, or $v,t\in Y$ holds.

Consider now the partition $(X',Y')$ of $V(R)$, where $X'=X\setminus T$ and $Y'=Y\setminus T$. It is easy to verify that $|\delta_G(R)\cap \delta_G(X')|=|X\cap T|$, and $|\delta_G(R)\cap \delta_G(Y')|=|Y\cap T|$. Let $E'=E_G(X',Y')$, and assume w.l.o.g. that $|\delta_G(R)\cap \delta_G(X')|\leq |\delta_G(R)\cap \delta_G(Y')|$. Then $|E'|\leq \alpha\cdot \alphasc(m)\cdot |\delta_G(R)\cap \delta_G(X')|$ must hold. We remove cluster $R$ from sets $\rset$ and $\rset^A$, and we add instead every connected component of graphs $G[X']$ and $G[Y']$ to both sets. It is immediate to verify that $\rset$ remains a collection of disjoint clusters of $G$, and that $\bigcup_{R'\in \rset}V(R')=V(G)$. We now show that the total budget $B$ decreases by at least $1/m$ as the result of this operation.

Note that the only edges whose budgets may change as the result of this operation are edges of $\delta_G(R)\cup E'$. Observe that, for each edge $e\in \delta_G(R)\cap \delta_G(Y')$, its budget $b(e)$ may not increase. Since we have assumed that $|\delta_G(R)\cap \delta_G(X')|\leq |\delta_G(R)\cap \delta_G(Y')|$, and since $|E'|<|\delta_G(R)|/8$, we get that $|\delta_G(X')|\leq 2|\delta_G(R)|/3$. Therefore, for every edge $e\in \delta_G(X')\cap \delta_G(R)$, its budget $b(e)$ decreases by at least $8\alpha \cdot \alphasc(m)\cdot\log_{3/2}(|\delta_G(R)|)-8\alpha \cdot \alphasc(m)\cdot\log_{3/2}(|\delta_G(X')|)$. Since $|\delta_G(X')|\leq 2|\delta_G(R)|/3$, we get that $ \log_{3/2}(|\delta_G(R)|)\leq \log_{3/2}(3|\delta_G(X')|/2)\leq 1+\log_{3/2}(|\delta_G(X')|$. We conclude that the budget $b(e)$ of each edge $e\in \delta_G(X')\cap \delta_G(R)$ decreases by at least $8\alpha\cdot \alphasc(m)$.
On the other hand, the budget of every edge $e\in E'$ increases by at most $3$. Since $|E'|\leq \alpha\cdot \alphasc(m)\cdot |\delta_G(R)\cap \delta_G(X')|$, we get that the decrease in the budget $B$ is at least:

\[
\begin{split}
8\alpha\cdot |\delta_G(X')\cap \delta_G(R)|-3|E'|&\geq 8\alpha\cdot \alphasc(m)\cdot |\delta_G(X')\cap \delta_G(R)|- \alpha\cdot \alphasc(m)\cdot |\delta_G(R)\cap \delta_G(X')| 
\\&\geq 7 \alpha\cdot \alphasc(m)\cdot |\delta_G(R)\cap \delta_G(X')|\\&>1/m,\end{split}\]


since $\alpha\geq 1/m$.
To conclude, if $|E(X,Y)|\leq \alpha\cdot \alphasc(m)\cdot \min\set{|X\cap T|,|Y\cap T}$, then we have modified the set $\rset$ of clusters, so that the total budget $B$ decreases by at least $1/m$, and all invatiants hold. In this case, we terminate the current iteration.

From now on we assume that $|E(X,Y)|> \alpha\cdot \alphasc(m)\cdot \min\set{|X\cap T|,|Y\cap T}$, which, as observed already, implies that cluster $R$ has the $\alpha$-bandwidth property. We now proceed to describe the second step of the algorithm.


\paragraph{Step 2: Witness Path Set.}
In the second step, we attempt to compute a witness path set $\pset(R)$ for cluster $R$. If we succeed in doing so, we will move cluster $R$ from $\rset^A$ to $\rset^I$. Otherwise, we will further modify cluster set $\rset$ so that all invariants will continue to hold and the total budget will decrease by at least $1/m$.

We construct the following flow network. Starting from graph $G$, we contract all vertices of $R$ into a source vertex $s$, and we contract all vertices of $V(G)\setminus V(S)$ into a destination vertex $t$. Denote the resulting graph by $H$, and observe that $\delta_H(s)=\delta_G(R)$, and $\delta_H(t)=\delta_G(S)$. We set the capacity $c(e)$ of every edge incident to $s$ to $1$, and the capacity of every other edge in graph $H$ to $100$. We then compute the maximum $s$-$t$ flow $f$ in the resulting flow network.

We consider two cases. The first case is when the value of the flow $f$ is $|\delta_H(s)|$. Since all edge capacities are inegral, we can assume that flow $f$ is integral as well. Note that in this case, for every path $P$ connecting $s$ to $t$, either $f(P)=0$ or $f(P)=1$ must hold, as the capacities of all edges incident to $s$ are $1$. Therefore, flow $f$ naturally defines a collection $\pset'(R)$ of $s$-$t$ paths, that cause congestion at most $100$ in $H$, and each edge $e\in \delta_G(s)$ serves as the first edge of exactly one such path. Path set $\pset'(R)$ then naturally defines a witness path set $\pset(R)=\set{P(e)\mid e\in \delta_G(R)}$ for cluster $R$ in graph $G$, that cause edge-congestion at most $100$, and, for every edge $e\in \delta_G(R)$, path $P(e)$ has $e$ as its first edge and some edge of $\delta_G(S)$ as its last edge, with all inner vertices of $P(e)$ lying in $V(S)\setminus V(R)$. We then move cluster $R$ from $\rset^A$ to $\rset^I$ and terminate the current iteration. It is easy to verify that all invariants continue to hold, and the total budget $B$ does not change.

It remains to consider the second case, where the value of the flow $f$ is less than $|\delta_H(s)|$. We compute a minimum $s$-$t$ cut $(A',B')$ in graph $H$, whose value is less than $|\delta_H(s)|$. We partition the edge set $E(A',B')$ into two subsets: set $E'=E(A',B')\cap \delta_H(s)$, and set $E''=E(A',B')\setminus E'$. Recall that the capacity of every edge in $E'$ is $1$, while the capacity of every edge in $E''$ is $100$. Therefore, $|E'|+100|E''|<|\delta_G(R)|$.

Observe that cut $(A',B')$ in $H$ naturally defines cut $(A,B)$ of graph $S$: we let $A=(A'\setminus \set{s})\cup V(R)$, and $B=V(S)\setminus A)$. Notice that $E_G(A,B)\subseteq E_H(A',B')$ (as some edges in $\delta_G(S)$ may have contributed to cut $(A',B')$ but no longer contribute to cut $(A,B)$. We perform the following modifications to cluster sets $\rset,\rset^I$, and $\rset^A$. First, we remove cluster $R$ from $\rset$ and from $\rset^A$, and we add every connected component of $S[A]$ to both sets instead. Next, we consider every cluster $R'\in \rset$ with $R'\cap A\neq \emptyset$. We remove cluster $R'$ from $\rset$, and we add instead every connected component of $S[V(R')\setminus A]$. We also remove cluster $R'$ from the cluster set in $\set{\rset^I,\rset^A}$ to which it belongs, and we add every connected component of  $S[V(R')\setminus A]$ to set $\rset^I$. This completes the description of the modification of cluster sets $\rset,\rset^I,\rset^A$. Note that all clusters in $\rset$ remain disjoint, and $\bigcup_{R''\in \rset'}V(R'')=V(S)$ continues to hold. It remains to show that the total budget $B$ decreases by at least $1/m$. 

Observe first that every edge in $\delta_G(A)$ belongs to the edge set $E_{H}(A',B')$. Since $|E_{H}(A',B')|<|\delta_H(s)|=|\delta_G(R)|$, we get that $|\delta_G(A)|<|\delta_G(R)|$. Therefore, the budgets of the edges in $\delta_G(A)\cap \delta_G(R)$ did not increase. All remaining edges of $\delta_G(A)$ lie in edge set $E''$. Therefore,
the only edges whose budget may have increased are the edges of $E_G(A,B)\cap E''$.

For each edge $e\in E_{G}(A,B)\cap E''$, its budget may have grown from $0$ to at most $3$, while the number of all such edges is $|E''|<(|\delta_G(R)|-|E'|)/100$. Therefore, the total increase in the budget $B$ due to the edges of  $E_{G}(A,B)\cap E''$ is at most $(|\delta_G(R)|-|E'|)/30$. We show that this increase is compensated by the decrease in the budgets of the edges of $\delta_G(R)\setminus E'$. Consider any edge $e\in \delta_G(R)\setminus E'$. Edge $e$ had budget at least $1$ originally, but after the current iteration, since the endpoints of $e$ both lie in $A$, its budget becomes $0$. Therefore, the decease in the budget $B$ due to the edges of $\delta_G(R)\setminus E'$ is at least $|\delta_G(R)\setminus E'|$. Overall, we get that the decrease in the budget $B$ is at least:

\[ |\delta_G(R)\setminus E'|- (|\delta_G(R)|-|E'|)/100\geq 1/m.\] 



This concludes the description of the iteration. The algorithm terminates when $|\rset^I|=\emptyset$ holds, at which point from the invariants we obtain the final cluster set $\rset$, together with witness path sets $\set{\pset(R)}_{R\in \rset}$ with all required properties. 
In particular, as observed above, since the budget of every edge in $\bigcup_{R\in \rset}\delta_G(R)$ is at least $1$, and the total budget $B$ never increases, $\sum_{R\in \rset}|\delta_G(R)|\leq B\leq (1+O(\alpha\cdot \alphasc(m)\cdot \log m))=(1+O(\alpha\cdot \log^{1.5} m))$ holds.
It remains to prove that the algorithm is efficient. Clearly, the algorithm for executing each iteration is efficient. We now show that the number of iterations is bounded by $O(m^2)$. Consider any iteration $i$ of the algorithm. Recall that, as the result of iteration $i$, either the budget $B$ decreased by at least $1/m$ (in which case we say that $i$ is a type-$1$ iteration); or budget $B$ did not change, but the number of clusters in set $\rset^I$ decreased by $1$ (in which case we say that $i$ is a type-$2$ iteration). It is then immediate to see that the number of type-$1$ iterations, over the course of the algorithm, is bounded by $O(m)$. Since every cluster of $\rset$ must contain at least one vertex, and $|V(S)|\leq m$ (because $S$ is a connected graph), the number of type-$2$ iterations between every consecutive pair of type-$1$ iterations is bounded by $O(m)$. Therefore, the total number of iterations of the algorithm is $O(m^2)$, and so the algorithm is efficient.


==> bad_and_problematic_index.tex <==

\subsubsection{Bad Indices and their Properties}

We denote the clusters in $\cset$ by $C_1,C_2,\ldots,C_r$. For convenience, for each $1\leq i\leq r$, we denote the vertex $v(C_i)$ of the graph $H=G_{|\cset}$ by $x_i$. Recall that we have assumed that the Gomory-Hu tree $\tau$ of $H$ is a path. We assume without loss of generality that the clusters are indexed according to their appearance on the path $\tau$. For $1\leq i\leq r$, we let $S_i=\set{x_1,\ldots,x_i}$ and let $\notS_i=\set{x_{i+1},\ldots,x_r}$. Recall that, by the definition of the Gomory-Hu tree, $(S_i, \notS_i)$ is a minimum cut in graph $H$ separating vertex $x_i$ from vertex $x_{i+1}$. From the properties of minimum cut, there is a set of paths in graph $H$, routing the edges of $\delta_H(S_i)$ to vertex $x_{i}$ inside $S_i$, and there is a set of paths in graph $H$, routing the edges of $\delta_H(\notS_i)$ to vertex $x_{i+1}$ inside $\notS_i$.
%\znote{notations $\rset$ and $\rset'$ are not used?}

%For all $1\leq i<j\leq r$, we denote by $E_{i,j}$ the set of paths in graph $G$ connecting vertices of $C_i$ to vertices of $C_j$.
Recall that every edge in graph $H$ corresponds to some edge in $\inE(\cset)$, and we do not distinguish between these edges. In particular, for all $1\le i,j\le r$, we will also view edges of $E(C_i,C_j)$ as parallel edges connecting vertex $x_i$ to vertex $x_j$ in graph $H$.
For each $1\le i\le k$, we denote
$\hat E_i=E(C_i,C_{i+1})$,
$E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, and 
$E_i^{\through}=\bigcup_{i'<i,j'>i+1}E(C_{i'},C_{j'})$.
%Consider now the cut $(S_i,\notS_i)$, for some $1\leq i<r$. We partition the set $\delta_H(S_i)$ of edges into four subsets. We denote by $\hat E_i$ the set of all parallel edges connecting $x_i$ to $x_{i+1}$. We denote by $E_i^{\rig}$ the set of all edges $(x_i,x_j)$, where $j>i+1$. We denote by $E_i^{\lef}$ the set of all edges $(x_j,x_{i+1})$ where $j<i$, and we denote by $E_i^{\through}$ the set of all remaining edges of $\delta_H(S_i)$; note that, if $e=(x_j,x_{j'})\in E_i^{\through}$, with $j<j'$, then $j<i$ and $j'>i+1$ must hold. 
We need the following  observation.

\begin{observation}\label{obs: bad inded structure}
For all $1\leq i<r$, the following hold:
\begin{itemize}
\item $|\hat E_i|\geq |E_i^{\through}|$;
\item $|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$; and
\item $|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{itemize}
\end{observation}
\begin{proof}
Consider the cut $(\set{x_{i}},V(H)\setminus \set{x_i})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$. Note that this cut separates $x_i$ from $x_{i-1}$. Since the minimum cut separating $x_i$ from $x_{i-1}$ in $H$ is $(S_{i-1},\notS_{i-1})$, and $|E(S_{i-1},\notS_{i-1})|=|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|$, we get that $|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$,
and so  
\begin{equation}
\label{eqn1}
|E_{i+1}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+ |E_i^{\rig}|.
\end{equation}
Consider the cut $(\set{x_{i+1}},V(H)\setminus \set{x_{i+1}})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$. Note that this cut separates $x_{i+1}$ from $x_{i+2}$. Since the minimum cut separating $x_{i+1}$ from $x_{i+2}$ in $H$ is $(S_{i+1},\notS_{i+1})$, and $|E(S_{i+1},\notS_{i+1})|=|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|$, we get that $|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$, 	
and so 
\begin{equation}
\label{eqn2}
|E_i^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|E_{i+1}^{\lef}|.
\end{equation}
Combining \Cref{eqn1,eqn2}, we get that $|\hat E_i|\geq |E_i^{\through}|$. By rearranging the sides of the two inequalities, we get that 	
$|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$, and
$|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{proof}

\begin{definition}
We say that index $i$ is \emph{bad} iff $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|>10000|\hat E_i|$.
\end{definition} 

We prove the following observation.
\begin{observation}\label{obs: bad instance}
If index $i$ is bad, then $|E_{i+1}^{\lef}|-|\hat E_i| \leq |E_i^{\rig}|\leq |E_{i+1}^{\lef}|+|\hat E_i|$, and moreover $4998|E_{i+1}^{\lef}|/4999 \leq |E_i^{\rig}|\leq 4999|E_{i+1}^{\lef}|/4998$.
If index $i$ is not bad, then $|\hat E_i|\ge |E_{i+1}^{\lef}|/5001$ and $|\hat E_i|\ge |E_{i}^{\rig}|/5001$.
\end{observation}
\begin{proof}
Assume first that $i$ is bad. Since $|E_i^{\through}|\leq |\hat E_i|$, we get that either $|E_i^{\rig}|\geq 4999|\hat E_i|$, or $|E_{i+1}^{\lef}|\geq 4999|\hat E_i|$. Assume without loss of generality that  $|E_i^{\rig}|\geq |E_{i+1}^{\lef}|$, so $|E_i^{\rig}|\geq 4999 |\hat E_i|$. Since, from \Cref{obs: bad inded structure}, 
$|\hat E_i| \geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$, we get that $|E_{i+1}^{\lef}|\geq |E_i^{\rig}|-|\hat E_i|\geq 4998|E_i^{\rig}|/4999$.

Assume now that $i$ is not bad. By definition, $10000|\hat E_i|\ge |E^\rig_i|+|E^\lef_{i+1}|+|E^{\through}_i|$. Combined with \Cref{obs: bad inded structure}, we get that $|\hat E_i|\ge |E^\lef_{i+1}|/5001$ and $|\hat E_i|\ge |E^\rig_{i}|/5001$.
\end{proof}



Let $1\le i\le r$ be some index.
We define indices $\LMP(i)$ and $\RMP(i)$ as follows.
Recall that $E^{\rig}_{i}$ is the set of all edges $(x_{i},x_z)$ with $z>i+1$. We let $\RMP(i)$ be the smallest integer $z>i+1$, such that at least half the edges in $E^{\rig}_{i}$ have their endpoints in $\set{x_{i+2},\ldots,x_z}$. It is easy to see that at least half the edges in $E^{\rig}_{i}$ must have their endpoints in $\set{x_{z},\ldots,x_r}$. Similarly, we let $\LMP(i)$ be the largest integer $z<i$, such that at least half the edges in $E^{\lef}_{i+1}$ have their endpoints in $\set{x_{z},\ldots,x_{i-1}}$. It is easy to see that at least half the edges in $E^{\lef}_{i+1}$ must have their endpoints in $\set{x_{1},\ldots,x_z}$. We need the following crucial observation and claim.

\begin{observation}\label{obs: large capacity up to midpoint}
	Let $1\leq i\leq r$ be an index. Then for every index $i<z<\RMP(i)-1$, $|\hat E_z|\geq |E^{\rig}_{i}|/2$; similarly, for every index $\LMP(i)<z'< i$, $|\hat E_{z'}|\geq |E^{\lef}_{i+1}|/2$.
\end{observation}
\begin{proof}
	Fix an index $1\leq i\leq r$ and another index $i<z<\RMP(i)-1$. Recall that there is a subset $E'\subseteq E^{\rig}_{i}$ of at least $|E^{\rig}_{i}|/2$ edges that have an endpoint in $\set{x_{\RMP(i)},\ldots,x_r}$. It is easy to verify that $E'\subseteq E_{z}^{\through}$. From \Cref{obs: bad inded structure}, $|\hat E_z|\geq |E_{z}^{\through}|\geq |E^{\rig}_{i}|/2$. The proof for index $\LMP(i)<z'< i$ is symmetric.
\end{proof}


\begin{claim}\label{claim: inner and outer paths}
	Let $a$ be some bad index and let $z\in \set{1,\ldots,r}$ be another index such that $a<z<\RMP(a)$.
	If we denote by $X$ the cluster of $H$ induced by vertices $x_{a+1},\ldots,x_z$, then (i) there is a set $\hat\qset(X)$ of paths routing the edges of $\delta_H(X)$ to vertex $x_z$ in $X$ with congestion $O(1)$; and (ii) there is a set $\hat\pset(X)$ of paths routing the edges of $\delta_H(X)$ to vertex $x_{z+1}$ outside $X$ with congestion $O(1)$.
	
	Similarly, 
	let $a'$ be some bad index and let $z'\in \set{1,\ldots,r}$ be another index such that $\LMP(a')<z'<a$.
	If we denote by $X'$ the cluster of $H$ induced by vertices $x_{z'},\ldots,x_{a'-1}$, then (i) there is a set $\hat\qset(X')$ of paths routing the edges of $\delta_H(X')$ to vertex $x_{z'}$ in $X'$ with congestion $O(1)$; and (ii) there is a set $\hat\pset(X')$ of paths routing the edges of $\delta_H(X')$ to vertex $x_{z'-1}$ outside $X$ with congestion $O(1)$.
\end{claim}

\begin{proof}
	We only prove the claim for cluster $X$, and the proof for cluster $X'$ is symmetric.
	
	We first prove (i). We partition the set $\delta_H(X)$ into two subsets: set $E_1$ contains all edges of $\delta_H(X)$ with an endpoint in $S_a$ (recall that $S_a=\set{x_1,\ldots,x_a}$); and set $E_2$ contains all edges of $\delta_H(X)$ with an endpoint in $\notS_z$ (recall that $\notS_z=\set{x_{z+1},\ldots,x_q}$). 
	Recall that, from the properties of minimum cut, there is a set $\rset$ of edge-disjoint paths routing the edges of $E_2$ to vertex $x_z$ inside $S_z$. 
	Let $\rset^{in}\subseteq \rset$ be the subset of all paths of $\rset$ that are entirely contained in $X$, and we denote $\rset^{out}=\rset\setminus \rset^{in}$.
	For each path $R\in \rset^{out}$, we view $x_z$ as its last vertex and the edge of $E_2$ as its first edge, and we denote by $e_R$ the first edge of $E_1$ that appears on $R$. It is clear that edges in $\set{e_{R}\mid R\in \rset^{out}}$ are mutually distinct.
	On the other hand, since $E_1\subseteq \hat E_a\cup E_{a+1}^{\lef}\cup E_a^{\through}$ and $a$ is a bad index, combined with \Cref{obs: bad inded structure}, we get that $|E_1|\leq |\hat E_a|+| E_{a+1}^{\lef}|+|E_a^{\through}|\leq 2|E_a^{\rig}|$. Moreover, from \Cref{obs: large capacity up to midpoint}, for all $a<z'\leq z$, $|\hat E_{z'}|\geq |E_a^{\rig}|/2\ge |E_1|/4$. 
	Therefore, 
	there is a set $\hat\qset_1=\set{\hat Q_e\mid e\in E_1}$ of paths, routing edges of $E_1$ to $x_z$ in $X$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{X}(\hat\qset_1)\le 4$; and similarly,
	there is a set $\hat{\rset}^{out}=\set{\hat R\mid R\in \rset^{out}}$ of paths, routing edges of $\set{e_R\mid R\in \rset^{out}}$ to $x_z$ in $X$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{X}(\hat{\rset}^{out})\le 4$.
	We now define $\hat\qset^{out}$ to be the set that contains, for each path $R\in \rset^{out}$, the concatenation of (i) the subpath of $R$ between its first edge (in $E_2$) and edge $e_R$ (not included); and (ii) the path $\hat R\setminus \set{e_R}$.
	We now let $\hat\qset_2=\rset^{in}\cup\hat\qset^{out}$ and $\hat\qset(X)=\hat\qset_1\cup \hat\qset_2$.
	It is clear that the set $\hat\qset(X)$ contains, for each edge of $\delta_H(X)$, a path routing the edge to $x_z$ in $X$, and
	$$\cong_{X}(\hat\qset(X))\le \cong_{X}(\hat\qset_1)+\cong_{X}(\hat\qset_2)\le 4+\cong_{X}(\rset^{in})+\cong_{X}(\hat\qset^{out})=4+1+(1+4)=10.$$
	%It is now easy to see that there is a set $\qset'(R')$ of paths in $R'$, routing the edges of $\delta(R')$ to vertex $x_z$, with congestion at most $4$.
	%A similar reasoning shows that there is a set $\qset'(R'')$ of paths in $R''$, routing the edges of $\delta(R')$ to vertex $x_{z+1}$, with congestion at most $4$.
	
	\begin{figure}[h]
		\centering
		\subfigure[Cluster $X$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_1.jpg}}\label{fig: path_cluster_H}
		}
		\hspace{4pt}
		\subfigure[Cluster $X'$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_2.jpg}}\label{fig: path_cluster_G}}
		\caption{An illustration of clusters $X,X'$ in $H$.}%\label{fig: path_cluster}
	\end{figure}
	
	We now prove (ii).
	From the properties of minimum cuts, there is a set $\rset_1$ of edge-disjoint paths routing edges of $E_1$ to $x_{a}$ in $S_{a}$ (and therefore outside $X$).
	Similarly, there is a set $\rset_2$ of edge-disjoint paths routing the edges of $E_2$ to $x_{z+1}$ inside $\notS_{z}$ (and therefore outside $X$). As observed before, $|E_1|\leq 2|E_a^{\rig}|$. Moreover, there is a set $E'\subseteq E_a^{\rig}$ of at least $|E_a^{\rig}|/2$ edges, each of which connects $x_a$ to a vertex in $\set{x_{z+1},\ldots,x_r}$. 
	For each edge $e\in E_1$, we assign to it an edge $e'$ of $E'$, such that each edge of $E'$ is assigned to at most $4$ edges of $E'_1$. 
	Observe that $E'\subseteq \delta_H(\notS_{z})$, so there is a set $\rset_3$ of $|E'|\geq |E_a^{\rig}|/2$ edge-disjoint paths routing the edges of $E'$ to $x_{z+1}$, that are disjoint from $X$. 
	We now define $\hat{\pset}_1$ to be the set that contains, for each edge $e\in E_1$, the union of (i) the path in $\rset_1$ routing $e$ to $x_a$ in $S_a$; and (ii) the path in $\rset_3$ that routing $e'$ to $x_{z+1}$ in $\notS_z$.
	We let $\hat{\pset}(X)=\rset_2\cup \hat{\pset}_1$.
	It is clear that the set $\hat\pset(X)$ contains, for each edge of $\delta_H(X)$, a path routing the edge to vertex $x_{z+1}$ outside $X$, and
	$$\cong_{H}(\hat\qset(X))\le
	\cong_{H}(\rset_2)+\cong_{H}(\hat\pset_1)\le 1+\cong_{H}(\rset_1)+4\cdot\cong_{H}(\rset_3)=1+(1+4)=6.$$
\end{proof}












\subsubsection{Problematic Indices and Inner Paths}


\iffalse
We say that an index $1\le i\le r$ is \emph{left-problematic}, iff $i$ is bad and
%there exists another index $1\le i'\le i-1$, such that
$|E(x_{\LMP(i)},x_{i+1})|\ge 0.99\cdot|E^{\lef}_{i+1}|$;
and similarly, we say that $i$ is \emph{right-problematic}, iff $i$ is bad and
%there exists another index $i+1< i'\le n$, such that
$|E(x_{i},x_{\RMP(i)})|\ge 0.99\cdot|E^{\rig}_{i}|$.
\fi

\iffalse
\begin{definition}
	We say that an index $i$ is \emph{left-problematic} iff (i) index $i$ is bad; (ii) index $\LMP(i)$ is bad; and (iii) $|E(x_{i},x_{\LMP(i)})|\ge 0.99\cdot|E^{\lef}_{i+1}|$.
	Similarly, we say that an index $i$ is \emph{right-problematic} iff (i) index $i$ is bad; (ii) index $\RMP(i)$ is bad; and (iii) $|E(x_{i},x_{\LMP(i)})|\ge 0.99\cdot|E^{\rig}_{i}|$.
\end{definition}
\fi


\begin{definition}
	We say that an ordered pair $(i,i')$ (with $i<i'$) of indices is \emph{problematic}, iff 
	\begin{itemize}
		\item both indices $i,i'$ are bad;
		\item $i=\LMP(i')$ and $i'+1=\RMP(i)$; and
		\item $|E(x_{i},x_{i'+1})|\ge 0.99\cdot\max\set{|E^{\lef}_{i'+1}|,|E^{\rig}_{i}|}$.
	\end{itemize} 
\end{definition}
We say that an index $i$ is \emph{left-problematic}, iff there exists an index $i'<i$, such that the pair $(i',i)$ is problematic. Similarly, we say that an index $i$ is \emph{right-problematic}, iff there exists an index $i'>i$, such that the pair $(i,i')$ is problematic.


Define $E'=E(H)\setminus (\bigcup_{1\le i\le r-1}\hat E_i)$.
In other words, $E'$ is the subset of edges in $E^{\out}(\cset)$ connecting a pair $C_i,C_j$ of clusters of $\cset$, with $j\ge i+2$, and if we view $E'$ as a set of edges in $H$, then $E'$ contains all edges connecting a pair $x_i,x_j$ of vertices in $H$ with $j\ge i+2$.
For an edge $e\in E'$ connecting $x_i$ to $x_j$, we say that a path $P$ in $H$ is a \emph{left inner path} of $e$, iff the endpoints of $P$ are $x_i$ and $x_{i+1}$, and $P$ only contains vertices of $S_{i+1}$; we say that a path $P$ in $H$ is a \emph{right inner path} of $e$, iff the endpoints of $P$ are $x_{j-1}$ and $x_{j}$, and $P$ only contains vertices of $\notS_{j-2}$; and we say that a path $P$ in $H$ is a \emph{middle inner path} of $e$, iff path $P$ sequentially visits vertices $x_{i+1}, x_{i+2},\dots,x_{j-1}$.
See \Cref{fig: LMR_inner} for an illustration.
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.20]{figs/LMR_inner.jpg}
	\caption{An illustration of left inner path (orange), middle inner path (purple) and right inner path (green) of edge $(x_i,x_j)\in E'$.}\label{fig: LMR_inner}
\end{figure}
%
We use the following observations and claims.
\begin{observation}
\label{obs: middle_inner_paths}
We can efficiently construct, for each edge $e\in E'$, a middle inner path $P^{\textsf{Mid}}_e$ of $e$, such that the paths in
$\pset^{\textsf{Mid}}=\set{P^{\textsf{Mid}}_e\mid e\in E'}$ are edge-disjoint.
\end{observation}
\begin{proof}
From the definition of middle inner paths, for each index $1\le i\le r$, the only edges in $E'$ whose middle inner paths contain an edge of $\hat E_i$ are edges of $E^{\through}_i$. From \Cref{obs: bad inded structure}, $|E^{\through}_i|\le \hat E_i$. Therefore, we can assign a distinct edge of $\hat E_i$ to each edge of $E^{\through}_i$. It is clear that, for each edge $e\in E'$, the union of all edges that are assigned to it forms a middle inner path of $e$. \Cref{obs: middle_inner_paths} then follows.
\end{proof}

\begin{claim}
If index $i$ is not left-problematic, then we can efficiently construct a set $\pset^{\lef}_i$ that contains, for each edge $e\in E^{\rig}_i$, a left inner path $P^{\lef}_e$ of $e$, such that $\cong_H(\pset^{\lef}_i)\le O(1)$. Similarly, if index $i$ is not right-problematic, then we can efficiently construct a set $\pset^{\rig}_i$ that contains, for each edge $e\in E^{\lef}_{i+1}$, a right inner path $P^{\rig}_e$ of $e$, such that $\cong_H(\pset^{\rig}_i)=O(1)$.
\end{claim}
\begin{proof}
We only consider the case where index $i$ is not left-problematic. The proof of the case where index $i$ is not right-problematic is symmetric. From the definition of a left-problematic index, either index $i$ is not bad, or $|E(x_{i+1},x_{\LMP(i)})|\le  0.99\cdot |E^{\lef}_{i+1}|$, or $|E(x_{i+1},x_{\LMP(i)})|\le  0.99\cdot |E^{\rig}_{\LMP(i)}|$, or index $i$ is bad, $|E(x_{i+1},x_{\LMP(i)})|> 0.99\cdot |E^{\lef}_{i+1}|$, but index $\LMP(i)$ is not bad. We consider each of these cases in turn.

\paragraph{Case 1. Index $i$ is not bad.}
From \Cref{obs: problematic instance}, $|\hat E_i|\ge |E^\rig_{i}|/5001$. Therefore, we simply let set $\pset^{\lef}_i$ contain, for each edge $e\in \hat E_{i}$, at most $5001$ paths that contain the single edge $e$, such that $|\pset^{\lef}_i|=|E^\rig_i|$. It is clear that these paths have endpoints $x_i$ and $x_{i+1}$, and $\cong_H(\pset^{\lef}_i)\le O(1)$.

\paragraph{Case 2. $|E(x_{i+1},x_{\LMP(i)})|\le  0.99\cdot |E^{\lef}_{i+1}|$.}
Since set $E^{\lef}_{i+1}$ is the union of sets $E(x_{i+1},\set{x_{\LMP(i)+1},\ldots,x_{i-1}})$, $E(x_{i+1},x_{\LMP(i)})$ and $E(x_{i+1},S_{\LMP(i)-1})$, either $|E(x_{i+1},\set{x_{\LMP(i)+1},\ldots,x_{i-1}})|\ge 0.005 |E^{\lef}_{i+1}|$ holds, or $|E(x_i,S_{\LMP(i)-1})|\ge 0.005 |E^{\lef}_{i+1}|$ holds. We consider these cases in turn.

\paragraph{Case 2.1. $|E(x_{i+1},\set{x_{\LMP(i)+1},\ldots,x_{i-1}})|\ge 0.005 \cdot|E^{\lef}_{i+1}|$.}
Denote $\tilde E_i=E(x_{i+1},\set{x_{\LMP(i)+1},\ldots,x_{i-1}})$.
Recal that from \Cref{obs: large capacity up to midpoint}, for each $\LMP(i)< z < i$, $|\hat E_{z}|\ge |E^{\lef}_{i+1}|/2$.
We first process all edges of $\tilde E_i$ iteratively as follows. Throughout, for each edge $\hat e\in \bigcup_{\LMP(i)+1\le t\le i-1}\hat E_t$, we maintain an integer $z_{\hat e}$ indicating how many times the edge $\hat e$ has been used, that is initialized to be $0$. 
Consider an iteration of processing an edge $e\in \tilde E_i$. Assume $e$ connects $x_{i+1}$ to $x_j$, for some $\LMP(i)\le t\le i-1$, we then pick, for each $j\le t\le i-1$, an edge $\hat e$ of $\hat E_t$ with minimum $z_{\hat e}$ over all edges of $\hat E_t$, and let $P^{\lef}_e$ be the path obtained by taking the union of $e$ and all picked edges.
It is easy to see that the path $P^{\lef}_e$ sequentially visits nodes $x_{i+1}, x_j, x_{j+1},\ldots,x_i$ (and so have endpoints $x_{i+1},x_i$). 
We then increase the value of $z_{\hat e}$ by $1$ for all picked edges $\hat e$, and proceed to the next iteration. Let $\tilde\pset^{\lef}_i$ be the set of left inner paths after we processed all edges of $E'$ in this way, so $|\tilde\pset^{\lef}_i|=|\tilde E_i|\ge 0.005|E^{\lef}_i|$,
and it is clear that $\cong_H(\tilde\pset^{\lef}_i)\le 2$.
We then let set $\pset^{\lef}_i$ contain, at most $200$ copies of each path in $\tilde\pset^{\lef}_i$, so left-inner paths in set $\pset^{\lef}_i$ connect $x_{i+1}$ to $x_i$, and $\cong_H(\pset^{\lef}_i)=O(1)$.


\paragraph{Case 2.2. $|E(x_{i+1},S_{\LMP(i)-1})|\ge 0.005 |E^{\lef}_{i+1}|$.} 
Note that $E(x_{i+1},S_{\LMP(i)-1})\subseteq E^{\through}_{\LMP(i)}$, so $|\hat E_{\LMP(i)}|\ge |E(x_{i+1},S_{\LMP(i)-1})|\ge 0.005 |E^{\lef}_{i+1}|$, and we can construct the set $\pset^{\lef}_i$ of left-inner paths in the same way as Case 2.1, by processing edges of $\tilde E_i\cup E(x_{i+1},x_{\LMP(i)})$, with $\cong_H(\pset^{\lef}_i)=O(1)$.


\paragraph{Case 3. $|E(x_{i+1},x_{\LMP(i)})|\le  0.99\cdot |E^{\rig}_{\LMP(i)}|$.}
Since set $E^{\rig}_{\LMP(i)}$ is the union of three disjoint edge sets $E(x_{\LMP(i)},\set{x_{\LMP(i)+2},\ldots,x_{i}})$, $E(x_{i+1},x_{\LMP(i)})$ and $E(x_{\LMP(i)},\notS_{i+1})$, either $|E(x_{\LMP(i)},\set{x_{\LMP(i)+2},\ldots,x_{i}})|\ge 0.005 |E^{\lef}_{i+1}|$ holds, or $|E(x_{\LMP(i)},\notS_{i+1})|\ge 0.005 |E^{\lef}_{i+1}|$ holds. 
It is easy to see that, in the former case, we can construct the set $\pset^{\lef}_i$ of left-inner paths in the same way as Case 2.1, with $\cong_H(\pset^{\lef}_i)=O(1)$. 
Assume now that the latter case happens
Note that $E(x_{\LMP(i)},\notS_{i+1})\subseteq E^{\through}_i$, so $|\hat E_i|\ge |E^{\through}_i|\ge |E(x_{\LMP(i)},\notS_{i+1})|\ge 0.005 |E^{\lef}_{i+1}|$, and therefore index $i$ is not bad. Therefore we can can construct the set $\pset^{\lef}_i$ of left-inner paths in the same way as Case 1.




\paragraph{Case 4. Index $i$ is bad, $|E(x_{i},x_{\LMP(i)})| >  0.99\cdot |E^{\lef}_{i+1}|$, but index $\LMP(i)$ is not bad.}
%\paragraph{Case 3. Both indices $i$, $\LMP(i)$ are bad but $|E(x_{i},x_{\LMP(i)})|\le  0.99\cdot |E^{\lef}_{i+1}|$.}
We first show that, for each index $\LMP(i)\le  z < i$, $|\hat E_{z}|\ge |E^{\lef}_{i+1}|/6000$.
First, from \Cref{obs: large capacity up to midpoint}, for each $\LMP(i)< z < i$, $|\hat E_{z}|\ge |E^{\lef}_{i+1}|/2$.
%It remains to show that $|\hat E_{\LMP(i)}|\ge |E^{\lef}_{i+1}|/5001$.
%Since $i$ is bad, from \Cref{obs: problematic instance}, $0.999|E_{i+1}^{\lef}| \leq |E_i^{\rig}|\leq 1.001|E_{i+1}^{\lef}|$.
Since $\LMP(i)$ is not bad, from \Cref{obs: problematic instance}, $|\hat E_{\LMP(i)}|\ge |E^\rig_{\LMP(i)}|/5001$.
Note that $E(x_{i},x_{\LMP(i)})\subseteq E^{\rig}_{\LMP(i)}$,
$|\hat E_{\LMP(i)}|\ge |E(x_{i},x_{\LMP(i)})|/5001\ge |E^{\lef}_{i+1}|/6000$.
Altogether, we get that for each $\LMP(i)\le  z < i$, $|\hat E_{z}|\ge |E^{\lef}_{i+1}|/6000$.
It is easy to see that we can construct the set $\pset^{\lef}_i$ of left-inner paths in the same way as in Case 2.1, with $\cong_H(\pset^{\lef}_i)=O(1)$.
\end{proof}



\begin{observation}
\label{obs: problematic pair non-crossing}
Problematic pairs do not interleave. 
In other words, if $(i_1,i'_1)$, $(i_2,i'_2)$ are problematic pairs, with $i_1<i_2$, then either $i_1<i_2<i'_2<i'_1$, or $i_1<i'_1<i_2<i'_2$.
\end{observation}
\begin{proof}
Assume for the sake of contradiction that $i_1<i_2<i'_1<i'_2$.
Note that $E(x_{i_1},x_{i'_1+1})\subseteq E^{\through}_{i_2}$ and $E(x_{i_2},x_{i'_2+1})\subseteq E^{\through}_{i'_1}$.
Therefore,
\[|E(x_{i_1},x_{i'_1+1})| \le |E^{\through}_{i_2}| \le |\hat E_{i_2}|
\le \frac{|E(x_{i_2},x_{i'_2+1})|}{0.99\times 4998}
\le \frac{|E^{\through}_{i'_1}|}{0.99\times 4998}
\le \frac{|\hat E_{i'_1}|}{0.99\times 4998}
\le \frac{|E(x_{i_1},x_{i'_1+1})|}{(0.99\times 4998)^2},\]
a contradiction.
\end{proof}



\begin{observation}
\label{obs: nested problematic pair}
If index pairs $(i_1,i'_1), (i_2,i'_2)$ are problematic and satisfy that $i_1<i_2<i'_2<i'_1$, then $|E(x_{i_1},x_{i'_1+1})|\le |E(x_{i_2},x_{i'_2+1})|/4000$.
\end{observation}
\begin{proof}
Note that $E(x_{i_1},x_{i'_1+1})\subseteq E^{\through}_{i_2}$, so
$|E(x_{i_1},x_{i'_1+1})| \le |E^{\through}_{i_2}| \le |\hat E_{i_2}|
	\le |E(x_{i_2},x_{i'_2+1})|/(0.99\cdot 4998)
	\le |E(x_{i_2},x_{i'_2+1})|/4000$.
\end{proof}







%We use the following claim. 
%Let $G$ be a graph and let $P$ be a path with $V(P)=V(G)$. Denote $P=(v_1,\ldots,v_n)$, where vertices appear on $P$ in this order. For each $1\le i\le n-1$, we denote $S_i=\set{v_1,\ldots,v_i}$ and $\notS_i=\set{v_{i+1},\ldots,v_n}$.
%Note that edges of $P$ may or may not belong to graph $G$. We say that graph $G$ has the \emph{$\alpha$-cut property with respect to $P$}, iff for each $1\le i\le n-1$, we have $|E_G(v_i,v_{i+1})|\ge \alpha\cdot |E_G(S_i,\notS_i)|$.
\begin{claim}
	\label{claim: alpha cut property}
	Let $(a,z)$ be some problematic pair of indices.
	%Let $X$ be the subgraph of $G$ induced by clusters $C_{a+1},\ldots,C_z$, and define 
	%Let $G'$ be the graph obtained from $G$ by contracting all clusters $C_1,\ldots,C_{a},C_{z+1},\ldots,C_r$ into a single vertex $v^*$. 
	%Define $\cset'=\set{C_{a+1},\ldots,C_z,v^*}$ as a set of clusters in $G'$ and 
	Define $H'$ to be the graph obtained from $H$ by contracting vertices $x_1,\ldots,x_{a},x_{z+1},\ldots,x_r$ into a single vertex $v^*$.
	%, so $V(H')=\set{x_{a+1},\ldots,x_z,v^*}$.
	%Define path $\tau'=(x_{a+1},\ldots,x_z,v^*)$. Then the graph $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for some $\alpha=O(1)$.
	Then for each $a< z'< z$,  
	$$|E_{H'}(x_{z'},x_{z'+1})|\ge \frac{|E_{H'}(\set{x_{a+1},\ldots,x_{z'}},\set{v^*})|}{6}.$$
\end{claim}
%
%
\begin{figure}[h]
	\centering
	\subfigure[Edge sets $E'_1,E'_2$ in graph $H$.]{\scalebox{0.12}{\includegraphics{figs/cut_property_1.jpg}}}
	\hspace{4pt}
	\subfigure[Edge sets $E'_1,E'_2$ in graph $H'$.]{\scalebox{0.12}{\includegraphics{figs/cut_property_2.jpg}}}
	\caption{An illustration of edge sets in $H$ and $H'$.}\label{fig: cut_property}
\end{figure}
%
%
\begin{proof}
	Fix some $z'$ with $a<z'< z$. We denote $S'_{z'}=\set{x_{a+1},\ldots,x_{z'}}$ and $\notS_{z'}'=\set{x_{z'+1},\ldots,x_z}$.
	%, and denote by $E'$ the set of edges in the cut $(S'_{z'},\notS_{z'}'\cup\set{v^*})$ of $H$.
	Note that vertices of $S'_{z'},\notS'_{z'}$ are also vertices of $V(H)$.
	We denote $E'_1=E_H(S'_{z'},\notS_z)$ and $E'_2=E_H(S'_{z'},S_a)$. Note that edges of $E'_1,E'_2$ are also edges of $H'$, and $E_{H'}(\set{x_{a+1},\ldots,x_{z'}},\set{v^*})=E'_1\cup E'_2$. 
	See \Cref{fig: cut_property} for an illustration.
	
	On the one hand, $E'_1\subseteq E^{\lef}_{z+1}\cup E^{\through}_z$.
	Since $(a,z)$ is a problematic pair, $|E(x_a,x_{z+1})|\ge 0.99\cdot |E^{\lef}_{z+1}|$. 
	Therefore,
	 $$|E'_1|\le |E^{\lef}_{z+1}|+|E^{\through}_z|\le 1.01\cdot|E^{\lef}_{z+1}|\le  1.03\cdot|E(x_a,x_{z+1})|\le 1.03\cdot|\hat E_{z'}|= 1.03\cdot|E_{H'}(x_{z'},x_{z'+1})|.$$
	On the other hand, from \Cref{obs: bad inded structure}, $|E'_2|\le |E^{\rig}_{a}|+|E^{\lef}_{a+1}|+|E^{\through}_{a}|\le 2\cdot|E^{\rig}_{a}|$, and from \Cref{obs: large capacity up to midpoint}, $|E_{H'}(x_{z'},x_{z'+1})|=|\hat E_{z'}|\ge |E^{\rig}_{a}|/2$.
	Therefore, $|E'_2|\le 4\cdot |E_{H'}(x_{z'},x_{z'+1})|$. Altogether, 
	$|E_1'|+|E_2'|\le 6\cdot |E_{H'}(x_{z'},x_{z'+1})|$.
	\iffalse
	Consider now the cut $(S_z,\set{v^*})$ in $H$. 
	We define sets $E',E'_1,E'_2,E'_3$ similarly. Clearly, $E'_1=\emptyset$. Observe that $E_H(x_z,x_{z+1})\subseteq E(S_z,\set{v^*})$, so it suffices to show that $|E'_2|+|E'_3|\le O(|E(x_z,x_{z+1})|)$.
	Since $z$ is not a bad index, $|E^{\rig}_{z}|+|E^{\lef}_{z+1}|+|E^{\through}_{z}|\le 100\cdot|E(x_{z},x_{z+1})|$.
	Note that 
	$$|E'_2|\le 2\cdot|E^{\rig}_{a}|\le 2(|E(x_a,x_{z+1})|+|E^{\through}_{z}|)\le 2(|E^{\lef}_{z+1}|+|E^{\through}_{z}|),$$ 
	and
	$$|E'_3|\le |E(S'_z,x_{z+1})|+|E^{\through}_{z}|\le |E^{\lef}_{z+1}|+|E^{\through}_{z}|.$$
	So in this case $|E'|\le 300\cdot |E(x_{z'},x_{z'+1})|\le 300\cdot|E(S_z,\set{v^*})|$.
	This completes the proof that $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for $\alpha=300$.
	\fi
\end{proof}




==> bad_index.tex <==

\subsubsection{Bad Indices and their Basic Properties}

In this subsection we define bad indices and analyze its properties.

For each $1\leq i\leq r$, we define $S_i=\set{x_1,\ldots,x_i}$ and $\notS_i=\set{x_{i+1},\ldots,x_r}$. Recall that, by the definition of the Gomory-Hu tree, $(S_i, \notS_i)$ is a minimum cut in graph $H$ separating vertex $x_i$ from vertex $x_{i+1}$. From the properties of minimum cut, there is a set of edge-disjoint paths in graph $H$, routing the edges of $\delta_H(S_i)$ to vertex $x_{i}$ inside $S_i$, and there is a set of edge-disjoint paths in graph $H$, routing the edges of $\delta_H(\notS_i)$ to vertex $x_{i+1}$ inside $\notS_i$.
%\znote{notations $\rset$ and $\rset'$ are not used?}

\begin{definition}
	We say that index $i$ is \emph{bad} iff $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|>10000|\hat E_i|$.
\end{definition}

\begin{observation}\label{obs: bad inded structure}
For all $1\leq i<r$, the following hold:
\begin{itemize}
\item $|\hat E_i|\geq |E_i^{\through}|$;
\item $|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$; and
\item $|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{itemize}
\end{observation}
\begin{proof}
Consider the cut $(\set{x_{i}},V(H)\setminus \set{x_i})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$. Note that this cut separates $x_i$ from $x_{i-1}$. Since the minimum cut separating $x_i$ from $x_{i-1}$ in $H$ is $(S_{i-1},\notS_{i-1})$, and $|E(S_{i-1},\notS_{i-1})|=|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|$, we get that $|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$,
and so  
\begin{equation}
\label{eqn1}
|E_{i+1}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+ |E_i^{\rig}|.
\end{equation}
Consider the cut $(\set{x_{i+1}},V(H)\setminus \set{x_{i+1}})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$. Note that this cut separates $x_{i+1}$ from $x_{i+2}$. Since the minimum cut separating $x_{i+1}$ from $x_{i+2}$ in $H$ is $(S_{i+1},\notS_{i+1})$, and $|E(S_{i+1},\notS_{i+1})|=|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|$, we get that $|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$, 	
and so 
\begin{equation}
\label{eqn2}
|E_i^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|E_{i+1}^{\lef}|.
\end{equation}
Combining \Cref{eqn1,eqn2}, we get that $|\hat E_i|\geq |E_i^{\through}|$. By rearranging the sides of the two inequalities, we get that 	
$|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$, and
$|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{proof}
 

We prove the following observation.
\begin{observation}\label{obs: bad instance}
If $i$ is a bad index, then $|E_{i+1}^{\lef}|-|\hat E_i| \leq |E_i^{\rig}|\leq |E_{i+1}^{\lef}|+|\hat E_i|$, and moreover $4998|E_{i+1}^{\lef}|/4999 \leq |E_i^{\rig}|\leq 4999|E_{i+1}^{\lef}|/4998$.
If index $i$ is not bad, then $|\hat E_i|\ge |E_{i+1}^{\lef}|/5001$ and $|\hat E_i|\ge |E_{i}^{\rig}|/5001$.
\end{observation}
\begin{proof}
Assume first that index $i$ is bad. Since $|E_i^{\through}|\leq |\hat E_i|$, we get that either $|E_i^{\rig}|\geq 4999|\hat E_i|$, or $|E_{i+1}^{\lef}|\geq 4999|\hat E_i|$. Assume without loss of generality that  $|E_i^{\rig}|\geq |E_{i+1}^{\lef}|$, so $|E_i^{\rig}|\geq 4999 |\hat E_i|$. Since, from \Cref{obs: bad inded structure}, 
$|\hat E_i| \geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$, we get that $|E_{i+1}^{\lef}|\geq |E_i^{\rig}|-|\hat E_i|\geq 4998|E_i^{\rig}|/4999$.

Assume now that $i$ is not bad. By definition, $10000|\hat E_i|\ge |E^\rig_i|+|E^\lef_{i+1}|+|E^{\through}_i|$. Combined with \Cref{obs: bad inded structure}, we get that $|\hat E_i|\ge |E^\lef_{i+1}|/5001$ and $|\hat E_i|\ge |E^\rig_{i}|/5001$.
\end{proof}

\paragraph{Nice pair of clusters.} Let $a<b<c$ be indices. We say that the pair $C_{(a,b]}, C_{(b,c]}$ of clusters are \emph{nice}, iff $|E(C_{(a,b]},C_{(b,c]})|\ge |E(C_{(a,b]},C_{(c,r]})|/1000$
and $|E(C_{(a,b]},C_{(b,c]})|\ge |E(C_{(b,c]},C_{(0,a]})|/10000$.
In other words, if we let $\cset'$ be the set of clusters obtained from $\cset$ by replacing clusters $C_{a+1},\ldots,C_c$ with clusters $C_{(a,b]}, C_{(b,c]}$ then the Gomory-Hu tree $\tau'$ of the contracted subugraph $G_{\mid \cset'}$ is a path where the index corresponding to cluster $C_{(a,b]}$ is not a bad index.
We use the following claim and its immediate corollary.

\begin{claim}
\label{clm: contraction does not create new bad indices}
Let $a<b<c$ be indices where $b$ is not bad. Then the pair $C_{(a,b]}, C_{(b,c]}$ of clusters is nice.
\end{claim}
\begin{proof}
Note that $E(C_{(a,b]},C_{(c,r]})\subseteq \big(E(C_{(a,b-1]},C_{(c,r]})\cup E(C_{b},C_{(c,r]})\big)\subseteq \big(E^{\through}_b\cup E^{\rig}_b\big)$, and note that $\hat E_b\subseteq E(C_{(a,b]},C_{(b,c]})$. Since index $b$ is not bad, from \Cref{obs: bad instance} and \Cref{obs: bad inded structure}, we get that $|\hat E_b|\ge |E^{\through}_b|$ and $|\hat E_b|\ge |E^{\rig}_b|/5001$, and therefore $|\hat E_b|\ge |E^{\through}_b\cup E^{\rig}_b|/10000$. It follows that $|E(C_{(a,b]},C_{(b,c]})|\ge |E(C_{(a,b]},C_{(c,r]})|/1000$. Similarly, we can show that $|E(C_{(a,b]},C_{(b,c]})|\ge |E(C_{(b,c]},C_{(0,a]})|/10000$.
\end{proof}

\begin{corollary}
\label{cor: nice pairs imply no bad index}
Let $\yset$ be a $\cset$-respecting partition of $G$ into a sequence $\yset=\set{Y_1,\ldots,Y_k}$ of clusters, such that every pair $Y_s,Y_{s+1}$ of clusters is nice. Then Gomory-Hu tree of the contracted graph $H'=G_{\mid \yset}$ is the path $(y_1,\ldots,y_k)$ (where $y_s$ is the vertex of $H'$ that corresponds to $Y_s$), and it has no bad indices.
\end{corollary}


\paragraph{Left and right midpoints.}
Let $1\le i\le r$ be some index.
We define indices $\LMP(i)$ and $\RMP(i)$ as follows.
Recall that $E^{\rig}_{i}$ is the set of all edges $(x_{i},x_z)$ with $z>i+1$. We let $\RMP(i)$ be the smallest integer $z>i+1$, such that at least half the edges in $E^{\rig}_{i}$ have their endpoints in $\set{x_{i+2},\ldots,x_z}$. It is easy to see that at least half the edges in $E^{\rig}_{i}$ must have their endpoints in $\set{x_{z},\ldots,x_r}$. Similarly, we let $\LMP(i)$ be the largest integer $z<i$, such that at least half the edges in $E^{\lef}_{i+1}$ have their endpoints in $\set{x_{z},\ldots,x_{i-1}}$. It is easy to see that at least half the edges in $E^{\lef}_{i+1}$ must have their endpoints in $\set{x_{1},\ldots,x_z}$. We need the following crucial observation and claim.

\begin{observation}\label{obs: large capacity up to midpoint}
	Let $1\leq i\leq r$ be an index. Then for every index $i<z<\RMP(i)-1$, $|\hat E_z|\geq |E^{\rig}_{i}|/2$; similarly, for every index $\LMP(i)<z'< i$, $|\hat E_{z'}|\geq |E^{\lef}_{i+1}|/2$.
\end{observation}
\begin{proof}
	Fix an index $1\leq i\leq r$ and another index $i<z<\RMP(i)-1$. Recall that there is a subset $E'\subseteq E^{\rig}_{i}$ of at least $|E^{\rig}_{i}|/2$ edges that have an endpoint in $\set{x_{\RMP(i)},\ldots,x_r}$. It is easy to verify that $E'\subseteq E_{z}^{\through}$. From \Cref{obs: bad inded structure}, $|\hat E_z|\geq |E_{z}^{\through}|\geq |E^{\rig}_{i}|/2$. The proof for index $\LMP(i)<z'< i$ is symmetric.
\end{proof}



For each pair $1\le j< j'\le r$, we define $X_{[j,j']}$ as the subgraph of $H$ induced by all vertices $x_t$ with index $t$ belonging to the interval $[j,j']$. We define clusters
$X_{(j,j']}$,
$X_{[j,j')}$, and
$X_{(j,j')}$ similarly. We use the following claim.

\begin{claim}\label{claim: inner and outer paths}
Let $a,z$ be indices such that $a$ is bad and $a<z<\RMP(a)$.
Then (i) there is a set $\hat\qset(X_{(a,z]})$ of paths routing the edges of $\delta_H(X_{(a,z]})$ to vertex $x_z$ in $X_{(a,z]}$ with congestion $O(1)$; and (ii) there is a set $\hat\pset(X)$ of paths routing the edges of $\delta_H(X_{(a,z]})$ to vertex $x_{z+1}$ outside $X_{(a,z]}$ with congestion $O(1)$.
	
Similarly, let $a',z'$ be indices such that $a'$ is bad and $\LMP(a')<z'<a'$.
Then there exists (i) a set $\hat\qset(X_{[z',a')})$ of paths routing edges of $\delta_H(X_{[z',a')})$ to $x_{z'}$ in $X_{[z',a')}$ with congestion $O(1)$; and (ii) a set $\hat\pset(X_{[z',a')})$ of paths routing edges of $\delta_H(X_{[z',a')})$ to $x_{z'-1}$ outside $X_{[z',a')}$ with congestion $O(1)$.
\end{claim}

\begin{proof}
	We only prove the claim for cluster $X_{(a,z]}$, and the proof for cluster $X_{[z',a')}$ is symmetric.
	
	Denote $X=X_{(a,z]}$. We first prove (i). We partition the set $\delta_H(X)$ into two subsets: set $E_1$ contains all edges of $\delta_H(X)$ with an endpoint in $S_a$ (recall that $S_a=\set{x_1,\ldots,x_a}$); and set $E_2$ contains all edges of $\delta_H(X)$ with an endpoint in $\notS_z$ (recall that $\notS_z=\set{x_{z+1},\ldots,x_q}$). 
	Recall that, from the properties of minimum cut, there is a set $\rset$ of edge-disjoint paths routing the edges of $E_2$ to vertex $x_z$ inside $S_z$. 
	Let $\rset^{in}\subseteq \rset$ be the subset of all paths of $\rset$ that are entirely contained in $X$, and we denote $\rset^{out}=\rset\setminus \rset^{in}$.
	For each path $R\in \rset^{out}$, we view $x_z$ as its last vertex and the edge of $E_2$ as its first edge, and we denote by $e_R$ the first edge of $E_1$ that appears on $R$. It is clear that edges in $\set{e_{R}\mid R\in \rset^{out}}$ are mutually distinct.
	On the other hand, since $E_1\subseteq \hat E_a\cup E_{a+1}^{\lef}\cup E_a^{\through}$ and $a$ is a bad index, combined with \Cref{obs: bad inded structure}, we get that $|E_1|\leq |\hat E_a|+| E_{a+1}^{\lef}|+|E_a^{\through}|\leq 2|E_a^{\rig}|$. Moreover, from \Cref{obs: large capacity up to midpoint}, for all $a<z'\leq z$, $|\hat E_{z'}|\geq |E_a^{\rig}|/2\ge |E_1|/4$. 
	Therefore, 
	there is a set $\hat\qset_1=\set{\hat Q_e\mid e\in E_1}$ of paths, routing edges of $E_1$ to $x_z$ in $X$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{X}(\hat\qset_1)\le 4$; and similarly,
	there is a set $\hat{\rset}^{out}=\set{\hat R\mid R\in \rset^{out}}$ of paths, routing edges of $\set{e_R\mid R\in \rset^{out}}$ to $x_z$ in $X$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{X}(\hat{\rset}^{out})\le 4$.
	We now define $\hat\qset^{out}$ to be the set that contains, for each path $R\in \rset^{out}$, the concatenation of (i) the subpath of $R$ between its first edge (in $E_2$) and edge $e_R$ (not included); and (ii) the path $\hat R\setminus \set{e_R}$.
	We now let $\hat\qset_2=\rset^{in}\cup\hat\qset^{out}$ and $\hat\qset(X)=\hat\qset_1\cup \hat\qset_2$.
	It is clear that the set $\hat\qset(X)$ contains, for each edge of $\delta_H(X)$, a path routing the edge to $x_z$ in $X$, and
	$$\cong_{X}(\hat\qset(X))\le \cong_{X}(\hat\qset_1)+\cong_{X}(\hat\qset_2)\le 4+\cong_{X}(\rset^{in})+\cong_{X}(\hat\qset^{out})=4+1+(1+4)=10.$$
	%It is now easy to see that there is a set $\qset'(R')$ of paths in $R'$, routing the edges of $\delta(R')$ to vertex $x_z$, with congestion at most $4$.
	%A similar reasoning shows that there is a set $\qset'(R'')$ of paths in $R''$, routing the edges of $\delta(R')$ to vertex $x_{z+1}$, with congestion at most $4$.
	
	\begin{figure}[h]
		\centering
		\subfigure[Cluster $X$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_1.jpg}}\label{fig: path_cluster_H}
		}
		\hspace{4pt}
		\subfigure[Cluster $X'$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_2.jpg}}\label{fig: path_cluster_G}}
		\caption{An illustration of clusters $X,X'$ in $H$.}%\label{fig: path_cluster}
	\end{figure}
	
	We now prove (ii).
	From the properties of minimum cuts, there is a set $\rset_1$ of edge-disjoint paths routing edges of $E_1$ to $x_{a}$ in $S_{a}$ (and therefore outside $X$).
	Similarly, there is a set $\rset_2$ of edge-disjoint paths routing the edges of $E_2$ to $x_{z+1}$ inside $\notS_{z}$ (and therefore outside $X$). As observed before, $|E_1|\leq 2|E_a^{\rig}|$. Moreover, there is a set $E'\subseteq E_a^{\rig}$ of at least $|E_a^{\rig}|/2$ edges, each of which connects $x_a$ to a vertex in $\set{x_{z+1},\ldots,x_r}$. 
	For each edge $e\in E_1$, we assign to it an edge $e'$ of $E'$, such that each edge of $E'$ is assigned to at most $4$ edges of $E'_1$. 
	Observe that $E'\subseteq \delta_H(\notS_{z})$, so there is a set $\rset_3$ of $|E'|\geq |E_a^{\rig}|/2$ edge-disjoint paths routing the edges of $E'$ to $x_{z+1}$, that are disjoint from $X$. 
	We now define $\hat{\pset}_1$ to be the set that contains, for each edge $e\in E_1$, the union of (i) the path in $\rset_1$ routing $e$ to $x_a$ in $S_a$; and (ii) the path in $\rset_3$ that routing $e'$ to $x_{z+1}$ in $\notS_z$.
	We let $\hat{\pset}(X)=\rset_2\cup \hat{\pset}_1$.
	It is clear that the set $\hat\pset(X)$ contains, for each edge of $\delta_H(X)$, a path routing the edge to vertex $x_{z+1}$ outside $X$, and
	$$\cong_{H}(\hat\qset(X))\le
	\cong_{H}(\rset_2)+\cong_{H}(\hat\pset_1)\le 1+\cong_{H}(\rset_1)+4\cdot\cong_{H}(\rset_3)=1+(1+4)=6.$$
\end{proof}

\iffalse
\begin{claim}
	\label{claim: alpha cut property}
	Let $a$ be a bad index and let $z$ be an index such that $a<z<\RMP(a)$.
	%Let $X$ be the subgraph of $G$ induced by clusters $C_{a+1},\ldots,C_z$, and define 
	%Let $G'$ be the graph obtained from $G$ by contracting all clusters $C_1,\ldots,C_{a},C_{z+1},\ldots,C_r$ into a single vertex $v^*$. 
	%Define $\cset'=\set{C_{a+1},\ldots,C_z,v^*}$ as a set of clusters in $G'$ and 
	Define $H'$ to be the graph obtained from $H$ by contracting vertices $x_1,\ldots,x_{a},x_{z+1},\ldots,x_r$ into a single vertex $v^*$.
	%, so $V(H')=\set{x_{a+1},\ldots,x_z,v^*}$.
	%Define path $\tau'=(x_{a+1},\ldots,x_z,v^*)$. Then the graph $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for some $\alpha=O(1)$.
	Then for each $a< z'< z$,  
	$$|E_{H'}(x_{z'},x_{z'+1})|\ge \frac{|E_{H'}(\set{x_{a+1},\ldots,x_{z'}},\set{v^*})|}{6}.$$
\end{claim}
%
%
\begin{figure}[h]
	\centering
	\subfigure[Edge sets $E'_1,E'_2$ in graph $H$.]{\scalebox{0.12}{\includegraphics{figs/cut_property_1.jpg}}}
	\hspace{4pt}
	\subfigure[Edge sets $E'_1,E'_2$ in graph $H'$.]{\scalebox{0.12}{\includegraphics{figs/cut_property_2.jpg}}}
	\caption{An illustration of edge sets in $H$ and $H'$.}\label{fig: cut_property}
\end{figure}
%
%
\begin{proof}
	Fix some $z'$ with $a<z'< z$. We denote $S'_{z'}=\set{x_{a+1},\ldots,x_{z'}}$ and $\notS_{z'}'=\set{x_{z'+1},\ldots,x_z}$.
	%, and denote by $E'$ the set of edges in the cut $(S'_{z'},\notS_{z'}'\cup\set{v^*})$ of $H$.
	Note that vertices of $S'_{z'},\notS'_{z'}$ are also vertices of $V(H)$.
	We denote $E'_1=E_H(S'_{z'},\notS_z)$ and $E'_2=E_H(S'_{z'},S_a)$. Note that edges of $E'_1,E'_2$ are also edges of $H'$, and $E_{H'}(\set{x_{a+1},\ldots,x_{z'}},\set{v^*})=E'_1\cup E'_2$. 
	See \Cref{fig: cut_property} for an illustration.
	
	On the one hand, $E'_1\subseteq E^{\lef}_{z+1}\cup E^{\through}_z$.
	Since $(a,z)$ is a problematic pair, $|E(x_a,x_{z+1})|\ge 0.99\cdot |E^{\lef}_{z+1}|$. 
	Therefore,
	 $$|E'_1|\le |E^{\lef}_{z+1}|+|E^{\through}_z|\le 1.01\cdot|E^{\lef}_{z+1}|\le  1.03\cdot|E(x_a,x_{z+1})|\le 1.03\cdot|\hat E_{z'}|= 1.03\cdot|E_{H'}(x_{z'},x_{z'+1})|.$$
	On the other hand, from \Cref{obs: bad inded structure}, $|E'_2|\le |E^{\rig}_{a}|+|E^{\lef}_{a+1}|+|E^{\through}_{a}|\le 2\cdot|E^{\rig}_{a}|$, and from \Cref{obs: large capacity up to midpoint}, $|E_{H'}(x_{z'},x_{z'+1})|=|\hat E_{z'}|\ge |E^{\rig}_{a}|/2$.
	Therefore, $|E'_2|\le 4\cdot |E_{H'}(x_{z'},x_{z'+1})|$. Altogether, 
	$|E_1'|+|E_2'|\le 6\cdot |E_{H'}(x_{z'},x_{z'+1})|$.
	\iffalse
	Consider now the cut $(S_z,\set{v^*})$ in $H$. 
	We define sets $E',E'_1,E'_2,E'_3$ similarly. Clearly, $E'_1=\emptyset$. Observe that $E_H(x_z,x_{z+1})\subseteq E(S_z,\set{v^*})$, so it suffices to show that $|E'_2|+|E'_3|\le O(|E(x_z,x_{z+1})|)$.
	Since $z$ is not a bad index, $|E^{\rig}_{z}|+|E^{\lef}_{z+1}|+|E^{\through}_{z}|\le 100\cdot|E(x_{z},x_{z+1})|$.
	Note that 
	$$|E'_2|\le 2\cdot|E^{\rig}_{a}|\le 2(|E(x_a,x_{z+1})|+|E^{\through}_{z}|)\le 2(|E^{\lef}_{z+1}|+|E^{\through}_{z}|),$$ 
	and
	$$|E'_3|\le |E(S'_z,x_{z+1})|+|E^{\through}_{z}|\le |E^{\lef}_{z+1}|+|E^{\through}_{z}|.$$
	So in this case $|E'|\le 300\cdot |E(x_{z'},x_{z'+1})|\le 300\cdot|E(S_z,\set{v^*})|$.
	This completes the proof that $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for $\alpha=300$.
	\fi
\end{proof}
\fi

\begin{observation}
\label{obs: bad index non-interleaving}
Let $i < i'$ be two bad indices, then either $\RMP(i)\le i'+1$, or $\LMP(i')\ge i$.
\end{observation}
\begin{proof}
Assume for contradiction that $\LMP(i')<i<i'<\RMP(i)-1$.
Note that $E(x_{i},\bar S_{\RMP(i)-1})\subseteq E^{\through}_{i'}$ and $E(x_{i'},S_{\LMP(i')})\subseteq E^{\through}_{i}$.
Therefore,
\[|E(x_{i},\bar S_{\RMP(i)-1})| \le |E^{\through}_{i'}| \le |\hat E_{i'}|
	\le \frac{|E(x_{i'},S_{\LMP(i')})|}{0.5\times 4998}
	\le \frac{|E^{\through}_{i}|}{0.5\times 4998}
	\le \frac{|\hat E_{i}|}{0.5\times 4998}
	\le \frac{|E(x_{i_1},\bar S_{\RMP(i)-1})|}{(0.5\times 4998)^2},\]
a contradiction.
\end{proof}




















==> basic_disengagement.tex <==


\subsection{First Key Tool: Basic Disengagement of Clusters}
\label{subsec: basic disengagement}


%\mynote{A useful thing to keep in mind: the set $\qset(C)$ of paths that I construct for each cluster $C$ has the following property, that seems to be useful. Each path $Q\in \qset(C)$ can be partitioned into two subpaths: $Q_1,Q_2$, where $Q_1$ has an edge of $\delta_G(C)$ as its endpoint, and $Q_2$ has $u(C)$ as its last endoint. We ensure that the set $\qset_1(C)\set{Q_1\mid Q\in \qset(C)}$ cause low congestion (e.g. $\poly\log n$, though in fact it will be a bit higher) on every edge. Path set $\qset_2(C)=\set{Q_2\mid Q\in \qset(C)}$ is confluent (so whenever two paths meet they continue together). Paths in $\qset_2(C)$ may cause high congestion, but expected congestion squared of every edge is low. Paths in $\qset_1(C)$ and paths in $\qset_1(C)$ may share vertices and edges. However, I can ensure that about $1/4$ of the paths in $\qset_1(C)$ are disjoint from all paths in $\qset_2(C)$. With some work I can increase this fraction of paths. If this is critical I could try to get paths in $\qset_1(C)$ and $\qset_2(C)$ completely disjoint but I don't know if this is doable. }


Throughout this subsection, we assume that we are given an instance $(G,\Sigma)$ of the \CNwRS problem, and we fix its optimal solution $\phi^*$. 
For brevity of notations, we will omit subscript $\phi^*$ when we use the notations $\chi_{\phi^*}(\cdot),\chi^1_{\phi^*}(\cdot),\chi^2_{\phi^*}(\cdot),\chi_{\phi^*}(\cdot,\cdot)$.
%We assume that no pair of edges cross more than once in $\phi^*$. For a subgraph $C$ of $G$, we denote by $\cro(C)$ the total number of crossings in the drawing $\phi^*$ in which the edges of $C$ participate.
%We need the following definition of a cost of path sets that we will use throughout the paper.\paragraph{Costs of Paths Sets.}

Let $C$ be a cluster of $G$, and let $\qset$ be a set of paths in $C$. 
Recall that for a pair $Q,Q'\in \qset$ of paths, we have denoted by $\chi(Q,Q')$ be the total number of crossings $(e,e')_p$ in the drawing $\phi^*$, where $(e,e')$ is an ordered pair of edges, with $e\in E(Q)$ and $e'\in E(Q')$. 
Note that the paths $Q,Q'$ are allowed to share edges, so a crossing $(e,e')_p$ with $e,e'\in E(Q)\cap E(Q')$ is counted twice in $\chi(Q,Q')$.
For a subgraph $H$ of $G$ that is not necessarily disjoint with $C$, we denote $\chi(\qset,H)=\sum_{Q\in \qset}\chi(Q,H)$.
\iffalse
\mynote{last sentence is not ideal. It sounds like you need to define this notion for *every* subgraph $H$, when in fact what you are saying is "for a subgraph $H$ of $G$, and a set $\qset$ of paths...."}
%Similarly, we denote $\chi^1(\qset)=\sum_{q\in \qset}\chi^1(Q)$. 
Define $C^+=C\cup\delta(C)$. \mynote{this is not consistent with how we define $C^+$ in other places (subdivide edges in $\delta_G(C)$ by terminals, let $C^+$ be the subgraph induced by $V(C)$ plus terminals. Better to use the same definition or name it something else.}
%For a path $Q\in \qset$, we denote by $\chi'_C(Q)$ the total number of crossings $(e,e')$ in the drawing $\phi^*$, where $e\in E(Q)$, and $e'\not\in E(C)\cup \delta(C)$. 

The cost of the set $\qset$ of paths with respect to cluster $C$ %is partitioned into two parts: $\cost^1_C(\qset)=\sum_{Q\in \qset}\chi(Q,G\!\setminus\! C^+)$, and $\cost^2_C(\qset)=\min\set{|\qset|^2,\sum_{\stackrel{Q,Q'\in \qset:}{Q\neq Q'}}\chi(Q,Q')}$. Lastly, we set $\cost_C(\qset)=\cost_C^1(\qset)+\cost_C^2(\qset)$.
is defined as: $\cost_C(\qset)=\chi(\qset,G\!\setminus\! C^+)+\min\set{|\qset|^2,\sum_{\stackrel{Q,Q'\in \qset:}{Q\neq Q'}}\chi(Q,Q')}$.
\fi

\iffalse{backup definitions}
\paragraph{Routing Paths and Orderings.}
Given a cluster $C$ of $G$, let $u(C)$ be an arbitrary vertex of $C$. We say that a path set $\qset(C)$ is a \emph{set of paths routing the edges of $\delta_G(C)$ to $u(C)$ inside $C$} iff $\qset(C)=\set{Q_C(e)\mid e\in \delta_G(C)}$, and for all $e\in \delta(C)$, path $Q_C(e)$ has $e$ as its first edge and $u(C)$ as its last vertex, and moreover $Q(e)\setminus\set{e}$ is contained in $C$.  Similarly, given a vertex $u'(C)\not\in C$, we say that path set $\pset(C)$ is a \emph{set of paths routing the edges of $\delta(C)$ to $u'(C)$ outside of $C$} iff $\pset(C)=\set{P_C(e)\mid e\in \delta_G(C)}$, and for all $e\in \delta(C)$, path $P_C(e)$ has $e$ as its first edge, $u'(C)$ as its last vertex, and, except for its first vertex, is completely disjoint from $C$.

Assume now that we are given a cluster $C\subseteq G$, a vertex $u(C)\in V(C)$, and a set $\qset(C)$ of paths routing the edges of $\delta_G(C)$ to $u(C)$ inside $C$,  such that the paths in $\qset(C)$ are non-transversal with respect to $\Sigma$.
%\znote{it seems that here we are not guaranteed that paths in $\qset(C)$ are edge-disjoint, but the notion of non-transversal-ness is only defined for a set of edge-disjoint paths.}
Recall that we are given an ordering $\oset_{u(C)}\in \Sigma$ of the edges in $\delta_G(u(C))$. We use this ordering and the set $\qset(C)$ of paths in order to define a circular ordering of the edges of $\delta_G(C)$, that we denote by $\hat \oset(C,\qset)$. Intuitively, this is the ordering in which the paths in $\qset(C)$ enter $u(C)$.
Formally, for every path $Q\in \qset(C)$, let $e^*(Q)$ be the last edge lying on path $Q$, that must belong to $\delta_G(C)$. We first define a circular ordering of the paths in $\qset(C)$, as follows: the paths are ordered according to the circular ordering of their last edges $e^*(Q)$ in $\oset_{u(C)}\in \Sigma$, breaking ties arbitrarily. Since every path $Q\in \qset(C)$ is associated with a unique edge in $\delta_G(C)$, that serves as the first edge on path $Q$, this ordering of the paths in $\qset(C)$ immediately defines a circular ordering $\hat \oset(C,\qset(C))$ of the edges of $\delta_G(C)$.
\fi


\paragraph{Basic Disengagement.}
Assume now that we are given a collection $\cset$ of disjoint sub-graphs of $G$ that we call \emph{clusters}, and that, for each such cluster $C\in \cset$, we are given (i) a vertex $u(C)\in V(C)$, and a set $\qset(C)=\set{Q_C(e)\mid e\in \delta_G(C)}$ of paths that are non-transversal with respect to $\Sigma$, routing the edges of $\delta_G(C)$ to $u(C)$ inside $C$; and
(ii) a vertex $u'(C)\notin V(C)$, and a set $\qset'(C)=\set{Q'_C(e)\mid e\in \delta_G(C)}$ of paths that are non-transversal with respect to $\Sigma$, routing the edges of $\delta_G(C)$ to $u'(C)$ outside of $C$.
%that we call \emph{guiding paths}, where for each edge $e\in \delta_G(C)$, path $Q(e)$ has $e$ as its first edge, and $u(C)$ as its last vertex.
%We say that the paths in $\qset(C)$ \emph{route the edges of $\delta_G(C)$ to $u(C)$ inside $C$}. Assume further that the paths in $\qset(C)$ are non-transversal. 
%\znote{same here?}
Denote $\qset=\bigcup_{C\in \cset}\qset(C)$, and $\qset'=\bigcup_{C\in \cset}\qset'(C)$.

We construct a collection $\iset(\cset,\qset,\qset')$ of sub-instances of instance $I$, that we refer to as the \emph{decomposition of instance $I$ via $(\cset,\qset,\qset')$}.

First, for every cluster $C\in \cset$, we construct an instance $I_C=(G_C,\Sigma_C)$. Graph $G_C$ is obtained from graph $C^+$ by unifying all endpoints of edges in $\delta_G(C)$ that do not lie in $C$ into a single vertex $v^*_C$. Note that for every vertex $x\in V(C)\setminus \set{v^*(C)}$, $\delta_{G_C}(x)=\delta_G(x)$. The ordering of the edges in $\delta_{G_C}(x)$ in $\Sigma_C$ remains the same as in $\Sigma$. For vertex $v^*(C)$, the set of its incident edges in $G_C$ is precisely $\delta_G(C)$. We define the ordering $\oset_{v^*(C)}$ of these edges in $\Sigma_C$ to be $\hat\oset(C,\qset(C))$.
%-- intuitively, this is the order in which the corresponding paths in $\qset(C)$ enter $u(C)$.

In addition to the instances $\set{I_C}_{C\in \cset}$, we define one more instance $\hat I(\cset,\qset)=(\hat G,\hat \Sigma)$. We define the graph $\hat G=G_{|\cset}$, and we denote the vertex in $\hat G$ representing the cluster $C$ by $u^*_C$. %\mynote{this would be good to connect to the definition of contracted graphs. Also, we sometimes call $u(C)$ the supernode corresponding to $C$, and sometimes it is the center vertex of $C$. Need to stick to one notation.} 
Note that for every vertex $x\in V(\hat G)\setminus \set{u^*_C}_{C\in \cset}$, $\delta_{\hat G}(x)=\delta_G(x)$, and the ordering $\oset_x$ of the edges incident to $x$ remains the same as in $\Sigma$. For a vertex $u^*_C$, where $C\in \cset$, the set of its incident edges is $\delta_G(C)$. We define the ordering $\oset_{u^*_C}$ in $\hat \Sigma$ to be the canonical ordering $\hat\oset(C,\qset(C),\Sigma)$ (see definition in \Cref{sec: canonical ordering}).
% -- the order in which the paths of $\qset(C)$ enter $u(C)$.

We let $\iset(\cset,\qset,\qset')=\set{\hat I(\cset,\qset)}\cup \set{I_C}_{C\in \cset}$ be the resulting collection of instances. 
We start by proving the following lemma.
%showing that all these instances have solutions whose total cost can be bounded in terms of $\cro(\phi^*)$, the costs of the path sets $\set{\qset(C)}_{C\in \cset}$ and the number of crossings between paths in $\qset'(C)$ and $C$ in $\phi^*$, for all clusters $C\in \cset$.


%\mynote{Please replace $\temp$ in this lemma with the right expression, that depends on parameters of the lemma.}
%\znote{done, and the proof is also adjusted.}
%Assume that for each cluster $C\in \cset$ and for each edge $e'\in E(C)$, $\mathbb{E}[\cong(\qset(C),e')]\le M_1$.

\begin{lemma}\label{lem: low solution costs}
$\sum_{I'\in \iset(\cset,\qset,\qset')}\optcrors(I')\leq \optcrors(I)+2\cdot\chi^2(\qset)+2\cdot\sum_{e'\in E(G)}(\cong(\qset,e'))^2+\\
\chi(\qset,G\setminus \bigcup_{C\in \cset}C)+\sum_{C\in \cset}\bigg(\chi(\qset'(C),C)+\chi(\qset'(C),\qset(C))\bigg)$.
\end{lemma}

%\znote{to be specific, if we denote $E'=E(G)\setminus \bigcup_{C\in \cset}E(C)$, then RHS should be }
%\znote{expand}
\begin{proof}
Recall that $\phi^*$ is an optimal solution of instance $I$. 
We show that we can construct 
\begin{itemize}
\item for each cluster $C\in \cset$, a solution $\phi_{C}$ of instance $I_C$ from $\phi^*$, such that \\
$\cro(\phi_C)\le \chi^2(C)+ \chi(\qset'(C),C)+\chi(\qset'(C),\qset(C))+\sum_{e'\in E(C)}\bigg(\cong(\qset(C),e')\bigg)^2+\chi^2(\qset(C))$;
%$\cro(\phi_{C})\le \chi(\qset'(C),C)+O(\chi^2(C)\cdot\temp)$
\item a solution $\hat \phi$ of instance $\hat I(\cset,\qset)$ from $\phi^*$, such that\\
$\cro(\hat \phi)\le \chi^2(G\setminus \bigcup_{C\in\cset}C)+\chi^2(\qset)+\chi(\qset,G\setminus \bigcup_{C\in \cset}C)+\sum_{e'\in E(G)}\bigg(\cong(\qset,e')\bigg)^2$.
%$\cro(\hat \phi)\le O(\cro(\phi^*)\cdot\temp)$.
\end{itemize}
Since $\chi^2(G\setminus \bigcup_{C\in\cset}C)+\sum_{C\in \cset}\chi^2(C)\le \cro(\phi^*)=\optcrors(I)$, it is not hard to see that the above bounds implies \Cref{lem: low solution costs}.
\iffalse{with temp}
Note that this implies \Cref{lem: low solution costs}, since
\[
\begin{split}
\sum_{I'\in \iset(\cset,\qset,\qset')}\optcrors(I') = & \text{ }
\optcrors(\hat I(\cset,\qset))+\sum_{C\in \cset}\optcrors(I_C)\\
\leq & \text{ } \cro(\hat \phi)+\sum_{C\in \cset}\cro(\phi_C)\\
\leq & \text{ }O(\cro(\phi^*)\cdot\temp)+\sum_{C\in \cset}\bigg(\chi(\qset'(C),C)+O(\chi^2(C)\cdot\temp)\bigg)\\
\leq & \text{ } O\bigg(\optcrors(I)\cdot\temp+\sum_{C\in \cset}\chi(\qset'(C),C)\bigg),
\end{split}
\]
where the last inequality is due to $\sum_{C\in \cset}\chi^2(C)\le \cro(\phi^*)=\optcrors(I)$.
\fi

We first construct the solution $\hat \phi$ for the instance $\hat I(\cset,\qset)$, as follows.
We start with drawing $\phi^*$, and process the clusters of $\cset$ one-by-one.
We now describe the iteration of processing a cluster $C$.
Recall that we are given, for each cluster $C\in\cset$, a vertex $u(C)\in V(C)$ and a set $\qset(C)$ of paths routing the edges of $\delta_G(C)$ inside $C$ that are  non-transversal with respect to $\Sigma$.
For each $e'\in E(C)$, we denote by $\pi_{e'}$ the curve that represents the image of $e'$ in $\phi^*$, and we let set $\Pi_{e'}$ contain $\cong_C(\qset(C),e')$ curves connecting the endpoints of $e'$ that are internally mutually non-crossing and lying inside an arbitrarily thin strip around $\pi_{e'}$. We then assign, for each edge $e\in \delta_G(C)$ and each edge $e'\in E(Q_C(e))$, a distinct curve of $\Pi_{e'}$ to $e$. So each curve in $\bigcup_{e'\in E(C)}\Pi_{e'}$ is assigned to exactly one edge of $\delta_G(C)$. 
For each $e\in \delta_G(C)$, let $\gamma_e$ be the curve obtained by concatenating all curves in $\bigcup_{e'\in E(C)}\Pi_{e'}$ that are assigned to $e$, so $\gamma_e$ connects the endpoint of $e$ outside $C$ to $z_C$, where $z_C$ is the image of $u(C)$ in $\phi^*$.
We denote $\Gamma_C=\set{\gamma_e\mid e\in \delta_G(C)}$.
In fact, when we assign curves of $\bigcup_{e'\in \delta_{G_C}(u(C))}\Pi_{e'}$ to edges of $\delta_G(C)$, we additionally ensure that, if we view $\gamma_e$ as the image of $e$ for each $e\in \delta_G(C)$, then the order in which the curves of $\set{\gamma_e\mid e\in \delta_G(C)}$ enter $z_C$ is identical to $\hat \oset(C,\qset(C))$. Note that this can be easily achieved according the the definition of $\hat \oset(C,\qset(C))$. 

%\mynote{I don't see how this is true. If a subset of paths of $\qset(C)$ share the last edge, then their ordering in $\oset(C,\qset(C))$ is arbitrary, by definition. I am assuming that you are assigning parallel edges to each path in $\qset(C)$ so that the resulting paths in the multigraph with parallel edges are non-transversal. It's not clear that you can do both at the same time. A possible solution (that doesn't work, just noting it here) is to define the ordering $\oset(C,\qset)$ by first replacing every edge with parallel edges, then assigning the parallel edges to every path in $\qset(C)$ so that they meet at vertices non-transverally, and then define the ordering $\oset(C,\qset(C)$ based on the order in which the resulting paths enter $u(C)$. The reason this does not work is that we don't know the flip of a vertex. So if there are $y$ parallel edges $(a,b)$, but we don't know the flip of $a$ and $b$ with respect to each other, we don't know how to order the paths as they move from $a$ to $b$.  }
%\znote{I am not assigning parallel edges to each path in $\qset(C)$ so that the resulting paths in the multigraph with parallel edges are non-transversal. In fact I allow the curves to be crossing each other (at image of vertices) in a non-transversal way here. Just need to make sure that they enter the image of $u(C)$ in the order $\hat\oset(\qset(C))$ that we have defined. Eventually after nudging (\Cref{obs: curve_manipulation}) we will pay $\sum_{e'\in E(C)}\cong(\qset(C),e)^2$ for these non-transversal crossings.}

%\znote{modify the language here after putting Obs 5.19 to an individual subsection.}
For each vertex $v\in V(C)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*$ (namely $x_v=\phi^*(v)$), and we let $X$ contains all points of $\set{x_v\mid v\in V(C)}$ that are crossings between curves in $\Gamma_C$. 
We then process all points of $X$ as follows.
Consider a point $x_v$ of $X$ and let $D_v$ be an arbitrarily small disc around $x_v$. 
Let $\Gamma_C(v)$ be the subset of all curves in $\Gamma_C$ that contains $x_v$.
Let $\tilde\Gamma_C(v)$ be the set of curves we obtain by applying the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\Gamma_C(v)$ within an arbitrarily small disc around $x_v$. We then replace curves of $\Gamma_C(v)$ in $\Gamma_C$ by curves of $\tilde\Gamma_C(v)$, and continue to the next iteration. Let $\tilde\Gamma_C=\set{\tilde\gamma_e\mid e\in \delta_G(C)}$ be the set of curves that we obtain after processing all points in $X$ in this way.
Note that the curves of $\tilde\Gamma_C$ might be non-simple. Let $\tilde\Gamma'_C=\set{\tilde\gamma'_e\mid e\in \delta_G(C)}$ be the set of curves that we obtain after removing self-loops from all curves of $\tilde\Gamma_C$.
From \Cref{obs: curve_manipulation}, curves of $\tilde\Gamma'_C$ are in general position. We now view $z_C$ as the image of $u^*_C$, and for each edge $e\in \delta_{G}(C)$, the curve $\tilde\gamma'_e$ as the image of $e$. 
This completes the iteration of processing cluster $C$.
Define $G'=G\setminus \bigcup_{C\in \cset}C$.
It is easy to see that
%\znote{the bound on number of crossings needs to be modified.}
\iffalse{analysis with temp}
\[
\begin{split}
\chi(\tilde\Gamma'_C)
= & \sum_{(e,e'):\text{ } e,e'\text{ cross in }\phi^*}\cong_{G}(\qset(C),e)\cdot \cong_{G}(\qset(C),e')\\
\le & 
\sum_{(e,e'): \text{ } e,e'\text{ cross in }\phi^*}\frac{(\cong_{G}(\qset(C),e))^2+(\cong_{G}(\qset(C),e'))^2}{2}\\
= & \text{ } \frac{1}{2}\cdot \sum_{e\in E(\qset(C))}\chi(e,C)\cdot(\cong_{G}(\qset(C),e))^2
\le O(\chi^2(C)\cdot\temp).
\end{split}
\]
and
\[
\begin{split}
\chi(\tilde\Gamma'_C,\phi^*(G\setminus \bigcup_{C\in \cset}C))
= & \sum_{e\in E(C^+)}\sum_{e'\in E(G\setminus C^+)}
\mathbf{1}[e,e'\text{ cross in }\phi^*]\cdot \cong_{G}(\qset(C),e)\\
= & \sum_{e\in E(C^+)}\chi(e,G\setminus \bigcup_{C\in \cset}C)\cdot \cong_{G}(\qset(C),e).
\end{split}
\]
\fi

\[
\chi(\tilde\Gamma'_C)
\le  \sum_{e'\in E(C)}\bigg(\cong(\qset(C),e')\bigg)^2+\sum_{Q,Q'\in \qset(C)}\chi(Q,Q').
\]
and
\iffalse{analysis with temp}
\[
\begin{split}
\chi(\tilde\Gamma'_C,\phi^*(G\setminus \bigcup_{C\in \cset}C))
= & \sum_{e\in E(C)}\sum_{e'\in E(G\setminus C)}
\mathbf{1}[e,e'\text{ cross in }\phi^*]\cdot \cong_{G}(\qset(C),e)\\
= & \sum_{e\in E(C)}\chi(e,G\setminus \bigcup_{C\in \cset}C)\cdot \cong_{G}(\qset(C),e)\\
= & \text{ }\chi^1(C)\cdot M_1.
\end{split}
\]
\fi
\[
\chi(\tilde\Gamma'_C,\phi^*(G'))\le \sum_{Q\in \qset(C)}\chi(Q, G').
\]

Let $\set{\tilde\Gamma'_C\mid C\in \cset}$ be the sets of curves that we obtain after processing all clusters of $\cset$ in the same way. It is clear that, if we view (i) for each $C\in \cset$, the point $\phi^*(u(C))$ as the image of $u^*_C$; and (ii) for each $C\in \cset$ and for each $e\in \delta_G(C)$, the curve $\tilde\gamma'_e\in \tilde\Gamma'_C$ as the image of $e$, then we obtain a drawing of $\hat G$ that respects the rotation system $\Sigma$, that we denote by $\hat\phi$. Moreover, 
\iffalse{analysis with temp}
\[
\begin{split}
\cro(\hat \phi)
= & \text{ }\chi^2(G\setminus \bigcup_{C\in \cset}C)+\sum_{C\in \cset}(\chi(\tilde\Gamma'_C)+\chi(\tilde\Gamma'_C, \phi^*(G\setminus \bigcup_{C\in \cset}C))) +  \sum_{C,C'\in \cset, C\ne C'}\chi(\tilde\Gamma'_C, \tilde\Gamma'_{C'})\\
\le &\text{ }\sum_{(e,e'): \text{ } e,e'\text{ cross in }\phi^*}\max\set{\frac{\cong_{G}(\qset,e)^2}{2},1}+\max\set{\frac{\cong_{G}(\qset,e')^2}{2},1}\\
= & \text{ } \sum_{e\in E(G)}\chi(e)\cdot\max\set{\frac{\cong_{G}(\qset,e)^2}{2},1}\\
\le & \sum_{e\in E(G)}\chi(e)\cdot O(\temp)= O(\cro(\phi^*)\cdot\temp).
\end{split}
\]
\fi
\[
\begin{split}
\cro(\hat \phi)
= & \text{ }\chi^2(G')+\sum_{C\in \cset}(\chi(\tilde\Gamma'_C)+\chi(\tilde\Gamma'_C, \phi^*(G'))) +  \sum_{C,C'\in \cset, C\ne C'}\chi(\tilde\Gamma'_C, \tilde\Gamma'_{C'})\\
\le &\text{ }\chi^2(G')+\sum_{C\in \cset}\bigg(\chi^2(\qset(C))+\chi(\qset(C),G')+\sum_{e'\in E(C)}\cong(\qset(C),e')^2\bigg) +\sum_{C,C'\in \cset, C\ne C'}\chi(\qset(C), \qset(C'))\\
= & \text{ }\chi^2(G')+\chi^2(\qset)+\chi(\qset,G')+\sum_{e'\in E(G)}\cong(\qset,e')^2.
\end{split}
\]


We now fix a cluster $C\in \cset$ and construct the solution $\phi_C$ as follows.
Recall that $V(G_C)=V(C)\cup\set{v^*_C}$ and $E(G_C)=E_G(C)\cup \delta_{G_C}(v^*_C)$.
%\znote{need a vertex $u'_C\notin C$ and a set $\pset_C$ of paths routing edges of $\delta(C)$ to $u'_C$ outside $C$.}
Also recall that we are given a vertex $u'(C)\notin C$ and a set $\qset'(C)$ of paths routing edges of $\delta_G(C)$ to $u'(C)$ outside of $C$. We start with the drawing of $C\cup E(\qset'(C))$ induced by $\phi^*$. We do not modify the drawing of $C$, and we construct the drawings of edges of $\delta_{G_C}(v^*_C)$ as follows.
For each $e'\in E(\qset'(C))$, we denote by $\pi_{e'}$ the curve that represents the image of $e'$ in $\phi^*$, and we let set $\Pi_{e'}$ contain $\cong_G(\qset'(C),e')$ curves connecting the endpoints of $e'$ lying inside an arbitrarily thin strip around $\pi_{e'}$. We then assign, for each edge $e\in \delta_G(C)$ and for each edge $e'\in E(Q'_C(e))$, a distinct curve in $\Pi_{e'}$ to $e$. So each curve in $\bigcup_{e'\in E(\qset'(C))}\Pi_{e'}$ is assigned to exactly one edge of $\delta_G(C)$. For each edge $e\in \delta_G(C)$, let $\gamma_e$ be the curve obtained by concatenating all curves in $\bigcup_{e'\in E(\qset'(C))}\Pi_{e'}$ that are assigned to $e$, so $\gamma_e$ connects the endpoint of $e$ in $C$ to $z'_C$, where $z'_C$ is the image of $u'(C)$ in $\phi^*$. We denote $\Gamma'_C=\set{\gamma'_e\mid e\in \delta_G(C)}$, and we view $z'_C$ as the last endpoint of curves in $\Gamma'_C$. We let $\Gamma_0$ contains all curves representing the image of some edge in $E(C)$, and then apply \Cref{thm: type-2 uncrossing} to sets $\Gamma_0,\Gamma'_C$ of curves. Let $\Gamma''_C=\set{\gamma''_e\mid e\in \delta_G(C)}$ be the set of curves that we obtain. Now if we view the curve $\gamma''_e$ as the image of $e$ for each edge $e\in \delta_G(C)$, then combined with the drawing of $C$ induced by the drawing $\phi^*$, we obtain a drawing of $G_C$, that we denote by $\phi'_C$. Clearly, the drawing $\phi'_C$ respects the rotation defined in $\Sigma_C$ at all vertices of $C$. However, it may not respect the rotation $\oset_{v^*_C}$, namely the image of edges of $\delta_{G_C}(v^*_C)$ may not enter $z'_C$ in the order $\oset_{v^*_C}$. To obtain a feasible solution to the instance $I_C$, we further modify the drawing $\phi'_C$ as follows.

Let $D_{z'_C}$ be an arbitrarily small disc around point $z'_C$. For each $e\in \delta_{G_C}(v^*_C)$, we denote by $p_e$ the intersection between the curve $\gamma''_e$ and the boundary of $D_{z'_C}$.
We erase the drawing of $\phi'_C$ inside the disc $D_{z'_C}$. We then place another disc $D'_{z'_C}$ inside the disc $D_{z'_C}$, and let $\set{p'_e}_{e\in \delta_{G_C}(v^*_C)}$ be a set of points appearing on the boundary of disc $D'_{z'_C}$ in the order $\oset_{v^*_C}$. We use \Cref{lem: find reordering} to compute a set $\set{\zeta_e}_{e\in \delta_{G_C}(v^*_C)}$ of reordering curves, where for each $e\in \delta_{G_C}(v^*_C)$, the curve $\zeta_e$ connects $p_e$ to $p'_e$.
We then define, for each $e\in \delta_{G_C}(v^*_C)$, the curve $\eta_e$ as the union of (i) the subcurve of $\gamma''_e$ outside the disc $D_{z'_C}$ (connecting its endpoint in $C$ to $p_e$); (ii) the curve $\zeta_e$ (connecting $p_e$ to $p'_e$); and (iii) the straight line-segment connecting $p'_e$ to $z'_C$. We now view the curve $\eta_e$ as the image of $e$ for all edges $e\in \delta_{G_C}(v^*_C)$. We denote by $\phi_C$ the drawing obtained by the union of all curves in $\set{\eta_e}_{e\in \delta_{G_C}(v^*_C)}$ and the image of $C$ in $\phi'_C$. Clearly, the drawing $\phi_C$ is a feasible solution to the instance $I_C$. 

It remains to show that 
$$\cro(\phi_C)\le \chi^2(C)+ \chi(\qset'(C),C)+\chi(\qset'(C),\qset(C))+\sum_{e'\in E(C)}\bigg(\cong(\qset(C),e')\bigg)^2+\chi^2(\qset(C)).$$
First, since we have not modified the drawing of $C$, the number of crossings between edges of $E_G(C)$ are bounded by $\chi^2(C)$. 
Second, from the definition of curves of $\Gamma'_C$, the number of crossings between image of $C$ and the curves of $\Gamma'_C$ is at most $\chi(\qset'(C),C)$. From~\Cref{thm: type-2 uncrossing} and the construction of curves in $\set{\eta_e}_{e\in \delta_G(C)}$, the number of crossings between image of $C$ and the curves of $\set{\eta_e}_{e\in \delta_G(C)}$ is also at most $\chi(\qset'(C),C)$.
Third, from~\Cref{thm: type-2 uncrossing},$\chi(\Gamma''_C)=0$. Therefore, all the crossings between curves of $\set{\eta_e}_{e\in \delta_G(C)}$ lie inside the disc $D_{z'}$.
We denote by $(\oset,b'_C)$ the oriented ordering in which the curves of $\Gamma''_C$ enter $z'$. From \Cref{lem: find reordering}, the number of crossings inside $D_{z'}$ is at most $2\cdot\dist((\oset,b'_C),(\oset_{v^*_C},b_C))$, where $b_C$ is the orientation for the unoriented circular ordering at vertex $u(C)$. 
Recall that $\oset_{v^*_C}=\hat\oset(\qset(C),C)$.
%Therefore, it suffices to show that $\dist((\oset,b'_C),(\hat\oset(C,\qset(C)),b_C))=O(\chi(\qset(C))\cdot\temp+\chi(\qset'(C),C))$.
We now show that $\dist((\oset,b'_C),(\hat\oset(C,\qset(C)),b_C))=O(\chi(\qset(C))\cdot\temp+\chi(\qset'(C),C))$.
In fact, we will construct a set of reordering curves for $(\oset,b'_C)$ and $(\oset_{v^*_C},b_C)$.
Recall that we have constructed, for each $e\in \delta_G(C)$, a curve $\tilde\gamma'_e$ connecting $e$ to $z$. We define, for each $e\in \delta_G(C)$, the curve $\xi_e$ to be the union of $\eta_e$ and $\tilde \gamma'_e$, so all curves of $\set{\xi_e}_{e\in \delta_G(C)}$ connects $z$ to $z'$. Note that the curves of $\Xi_C=\set{\xi_e}_{e\in \delta_G(C)}$ enter $z$ in the order $(\hat\oset(C,\qset(C)),b_C)$ and enter $z'$ in the order $(\oset,b'_C)$, so $\dist((\oset,b'_C),(\hat\oset(C,\qset(C)),b_C))\le \chi(\Xi_C)$.
%\znote{the bound on number of crossings needs to be modified.}
Note that
$$\chi(\Xi_C)
\le \chi(\qset'(C),\qset(C))+ \chi(\tilde\Gamma'_C)
\le \chi(\qset'(C),\qset(C))+ \sum_{e'\in E(C)}\bigg(\cong(\qset(C),e')\bigg)^2+\sum_{Q,Q'\in \qset(C)}\chi(Q,Q'),$$
so $\cro(\phi_C)\le \chi^2(C)+ \chi(\qset'(C),C)+\chi(\qset'(C),\qset(C))+\sum_{e'\in E(C)}\bigg(\cong(\qset(C),e')\bigg)^2+\chi^2(\qset(C))$.
\end{proof}


$\ $

Lastly, we show that we can combine solutions to instances in $\iset(\cset,\qset,\qset')$, to obtain a solution to instance $I$ without increasing the total number of crossings.

\begin{lemma}\label{lem: combine solutions}
There is an efficient algorithm, that, given, for each instance $I'\in \iset(\cset,\qset,\qset')$, a solution $\phi(I')$, computes a solution for instance $I$ of value at most $\sum_{I'\in \iset(\cset,\qset,\qset')}\cro(\phi(I'))$.
\end{lemma}

\begin{proof}
For each $C\in \cset$, we rename the solution $\phi(I_C)$ to the instance $I_C$ by $\phi_C$, and we rename the solution  $\phi(\hat I(\cset,\qset))$ to the instance $\hat I(\cset,\qset)$ by $\hat \phi$. We will construct a solution $\phi$ for instance $I$, from the solutions $\hat{\phi}$ and $\set{\phi_C}_{C\in \cset}$, as follows.

We start with the drawing $\hat \phi$, and process clusters of $\cset$ one-by-one. Recall that the instance $I(\cset,\qset)=(\hat G,\hat \Sigma)$, where graph $\hat G$ contains a vertex $u^*_C$ for every cluster $C\in \cset$. Moreover, the incident edges of $u^*_C$ in $G$ is $\delta_G(C)$, and $\oset_{u^*_C}=\hat \oset(\qset(C),C)$.
Also recall that, for each cluster $C\in \cset$, the graph $G_C$ contains a vertex $v^*_C$ with $\delta_{G_C}(v^*_C)=\delta_G(C)$, and $\oset_{v^*_C}=\hat \oset(\qset(C),C)$.
We now describe an iteration of processing cluster $C$. 
Let $D_C$ be an arbitrarily small disc around the image of $u^*_C$ in $\hat\phi$. For each edge $e\in \delta_G(C)$, we denote by $p_e$ the intersection of the image of $e$ in $\hat \phi$ with the boundary of $D_C$, so the points $\set{p_e}_{e\in \delta_G(C)}$ appear on the boundary of $D_C$ in the order $\hat\oset(C,\qset(C))$.
Similarly, let $D'_C$ be an arbitrarily small disc around the image of $v^*_C$ in $\phi_C$, and we define points $\set{p'_e}_{e\in \delta_G(C)}$ similarly, so they appear on the boundary of $D'_C$ in the order $\hat\oset(C,\qset(C))$.
We now erase the part of the drawing $\hat\phi$ inside the disc $D_C$, and place the drawing of $\phi_C$ outside the disc $D'_C$ inside $D_C$, such that the boundary of $D_C$ coincides with the boundary of $D'_C$, while the interior of $D_C$ coincides with the exterior of $D'_C$, and for each edge $e\in \delta_G(C)$, the points $p_e$ and $p'_e$ coincide (note that this can be achieved since points in $\set{p_e}_{e\in \delta_G(C)}$ appear on the boundary of $D_C$ in the same order as points in $\set{p_e}_{e\in \delta_G(C)}$ appear on the boundary of $D_C$). This completes the iteration of processing $C$. 
For each $e\in \delta_G(C)$, we view the union of (i) the subcurve of the image of $e$ in $\hat \phi$ between the image of its non-$u^*_C$ endpoint and the point $p_e$; and (ii) the subcurve of the image of $e$ in $\phi_C$ between the image of its non-$v^*_C$ endpoint and the point $p'_e$, as the image of $e$.
Clearly, after the iteration of processing $C$, we have not created any additional crossings.

Let $\phi$ be the drawing that we obtain after processing all clusters of $\cset$ in this way. It is easy to verify that $\phi$ is a feasible solution to the instance $I$. Since we have not created additional crossings in each iteration, $\cro(\phi)\le \cro(\hat \phi)+\sum_{C\in \cset}\cro(\phi_C)$.
This completes the proof of \Cref{lem: combine solutions}.
\end{proof}

%\mynote{above two lemmas still need proofs. Note the new definition of costs of paths. This is needed to make the cluster decomposition go through.}

%path $P$ in $G$, its cost $\cost(P)$ is the total number of crossings in $\phi^*$ in which the edges of $P$ participate. Given a set $\qset$ of paths, its cost is: $\cost(\qset)=\sum_{P\in \qset}\cost(P)$. Given a sub-graph $C\subseteq G$, we denote by $\cro(C)$ the total number of crossings in $\phi^*$ in which the edges of $C$ participate. 
%Given a pair $P,Q$ of paths in $G$, we also denote by $\cro(P,Q)$ the total number of crossings $(e,e')$ in $\phi^*$ such that either (i) $e\in E(P)$ and $e'\in E(Q)$ holds, or (ii) $e\in E(Q)$ and $E'\in E(P)$ holds (notice that, for a pair $e,e'\in E(Q)\cap E(P)$ of edges, if crossing $(e,e')$ exists, then is only counted once in $\cro(P,Q)$; if $P=Q$, then $\cro(P,P)$ is the number of crossings in $\phi^*$ between pairs of edges $(e,e')$ where both $e,e'\in E(P)$.). Given two sets $\pset,\qset$ of paths, we denote by $\cost(\pset,\qset)=\sum_{P\in \pset,Q\in \qset}\cro(P,Q)$.


\iffalse
Recall that given an instance $(G,\Sigma)$ of the \CNwRS problem, we say that another instance $(G',\Sigma')$ is its \emph{sub-instance} iff graph $G'$ is obtained from a sub-graph of $G$ by contracting some of its vertex sets into super-nodes. The ordering $\oset(u)$ for the edges incident to super-nodes may be arbitrary, but the ordering of edges incident to other vertices is determined by the ordering in $\Sigma$.

Suppose we are given any collection $\cset$ of disjoint sub-graphs of $G$, such that $\bigcup_{C\in \cset}V(C)=V(G)$. We denote by $\inE_{\cset}$ the set of all edges of $G$ whose endpoints lie in different clusters, and by $\innerE_{\cset}$ the set of all edges of $G$ whose endpoints lie in the same cluster, so $\inE_{\cset}\cup \innerE_{\cset}=E(G)$.



The main theorem of this subsection is the following.
\mynote{maybe define the sub-instances before the theorem statement to make it more concrete?}
\znote{Yes. I am about to suggest this as well.}

\begin{theorem}[Basic Disengagement of Clusters]\label{thm: disengagement}
There is an efficient algorithm, that, given an instance $(G,\Sigma)$ of the \CNwRS problem, and a collection $\cset$ of disjoint sub-graphs of $G$, such that $\bigcup_{C\in \cset}V(C)=V(G)$, and, for every cluster $C\in \cset$, a vertex $u(C)\in C$, and a vertex $u'(C)\not \in C$, together with a  collection $\qset(C)$ of paths routing the edges of $\delta(C)$ to $u(C)$ inside $C$ with congestion $\eta$, and a collection $\pset(C)$ of edge-disjoint paths routing the edges of $\delta(C)$ to $u'(C)$ outside of $C$ with congestion $\eta$, computes a collection $\iset$ of sub-instances of $(G,\Sigma)$, with the following properties:

\begin{itemize}
	\item For every cluster $C\in \cset$, there is a unique instance $(H_C,\Sigma_C)$, with $C\subseteq H_C$. Moreover, $|E(H_C)|\leq |E(C)|+|\inE_{\cset}|$;
	
	
	\item $\sum_{(H,\Sigma')\in \iset}|E(H)|\leq \sum_{C\in \cset}|E(C)|+2|\inE_{\cset}|$; and
	
	\item $\sum_{(H,\Sigma')\in \iset}\optcrors(H,\Sigma')\leq \eta^2\optcrors(G,\Sigma)\poly\log n$.
\end{itemize}

 Moreover, there is an efficient algorithm, that, given, for each instance $I'\in \iset$, a feasible solution $\phi_I$, computes a feasible solution  $\phi$ to instance $I$ with $\cro(\phi)\leq O\left (\sum_{I\in \iset}\cro(\phi_I)\right ) \cdot \poly\log n$.

\end{theorem}

The proof of the theorem is somewhat involved and technical, and is deferred to Section \ref{sec:disengagement}.
 \mynote{this theorem stands on its own and the proof can be done without taking care of the path case. We use it later.}

\fi




==> cut_property.tex <==
\subsection{The Cut Property}

We first introduce a useful definition that will be repeatedly used in this section.

Let $G$ be a graph and let $P$ be a path with $V(P)=V(G)$. Denote $P=(v_1,\ldots,v_n)$, where vertices appear on $P$ in this order. For each $1\le i\le n-1$, we denote $S_i=\set{v_1,\ldots,v_i}$ and $\notS_i=\set{v_{i+1},\ldots,v_n}$.
%Note that edges of $P$ may or may not belong to graph $G$.
We say that graph $G$ has the \emph{$\alpha$-cut property with respect to $P$}, iff for each $1\le i\le n-1$, we have $|E_G(v_i,v_{i+1})|\ge \alpha\cdot |E_G(S_i,\notS_i)|$.
We use the following simple observations.



%\mynote{There are several issues with this observation. First, there is a confusion between $\alpha$ and $\beta$. Second, if $\rset^{\lef}$ is a path set tied to index $i$, then you should call it $\rset_i^{\lef}$. It's not clear to me if you are trying to bound the congestion of each $\rset_i^{\lef}$ separately, or of $\bigcup_i\rset_i^{\lef}$ together (I guess you eventually use both bounds)}
\begin{observation}
If graph $G$ has the $\alpha$-cut property with respect to $P$, then there exist, for each $1\le i\le n-1$, a set $\rset_i^{\lef}$ of paths routing edges of $E_G(S_i,\notS_i)$ to $v_i$ using only edges of $\bigcup_{1\le t\le i-1}E(v_t,v_{t+1})$, and a set $\rset_i^{\rig}$ of paths routing edges of $E_G(S_i,\notS_i)$ to $v_{i+1}$ using only edges of $\bigcup_{i\le t\le n-1}E(v_t,v_{t+1})$, such that the congestion caused by paths in $\bigcup_i(\rset_i^{\lef}\cup \rset_i^{\rig})$ is at most $\ceil{1/\alpha}$.
\end{observation}

%As a comparison, if $G$ has a Gomory-Hu tree $\tau$ that is a path, and if we denote $\tau=(v_1,\ldots,v_n)$, then from the properties of minimum cuts, for each $1\le i\le n-1$, there is a set $\hat\rset^{\lef}_i$ of edge-disjoint paths routing edges of $E(S_i,\notS_i)$ to $v_i$ within $S_i$. Here by saying that $G$ has the $\alpha$-cut property with respect to $P$, we require that such a set of routing paths use only edges of $\bigcup_{1\le t\le i-1}E_G(v_t,v_{t+1})$, but we allow them to have $\ceil{1/\alpha}$ congestion.

==> decomposition-phase1-backup.tex <==
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
\subsection{Phase 1: Flower Clusters, Small Clusters, and Initial Disengagement}
\label{subsec: phase 2 flower vs small cluster partition}
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------


The first phase consists of three steps. In the first step, we carve flower clusters out of the graph $G$. In the second step, we decompose the remainder of the graph $G$ into small clusters. Lastly, we perform a disengagement step for all resulting clusters in the third step.

\subsubsection{Step 1: Carving out Flower Clusters}

Let $S=\set{s_1,\ldots,s_k}$ be the set of all vertices of $G$ that have degree at least $m/\mu^4$. Notice that, since we have assumed that no edge connects a pair of high-degree vertices, and $|E(G)|\leq 3m$, $k\leq 3\mu^4$ must hold. 
In this step, we use with the following lemma, in order to carve flower clusters out of graph $G$.


\begin{lemma}\label{lemma: carve out flower clusters}
	There is an efficient algorithm that computes a collection $\cset^f=\set{C^f_1,\ldots,C^f_k}$ of disjoint clusters of $G$, such that for all $1\leq i\leq k$, $C^f_i$ is a flower cluster with center $s_i$. The algorithm also computes, for each resulting flower cluster $C^f_i$, the corresponding set $\xset(C^f_i)$ of petals.
\end{lemma}
\begin{proof}	
We start with the following simple claim that allows us to compute an initial collection $\set{C_1,\ldots,C_k}$ of clusters with some useful properties. Eventually, for all $1\leq i\leq k$, we will define a flower cluster $C_i^f\subseteq C_i$.

\begin{claim}\label{claim: flowers initial}
	There is an efficient algorithm to compute $k$ disjoint vertex-induced subgraphs $C_1,\ldots, C_k$, such that for all $1\leq i\leq k$, $s_i\in V(C_i)$, $\delta_G(s_i)\subseteq E(C_i)$, and $|\delta_G(C_i)|\leq 3m/\mu^{46}$. Additionally, the algorithm computes, for all $1\leq i\leq k$, a set $\qset_i$ of edge-disjoint paths routing the edges of $\delta_G(C_i)$ to $s_i$ inside $C_i$.
\end{claim}

\begin{proof}
We use \Cref{lem: multiway cut with paths sets} to compute, for all $1\leq i\leq k$, a set $A_i$ of vertices of $G$, such that $S\cap A_i=\set{s_i}$, and $(A_i,V(G)\setminus A_i)$ is a minimum cut separating $s_i$ from the vertices of $S\setminus\set{s_i}$ in $G$, and the vertex sets $A_1,\ldots,A_k$ are all mutually disjoint from each other. Recall that the algorithm also computes,
for all $1\leq i\leq k$, a set $\qset_i$ of edge-disjoint paths, routing the edges of $\delta_G(A_i)$ to vertex $s_i$ inside $G[A_i]$.

Recall that we have assumed that, for all $1\leq i\leq r$, for every edge $e=(s_i,v_e)\in \delta_G(s_i)$, the degree of vertex $v_e$ in $G$ is at most $2$, and $v_e$ is the neighbor of at most one vertex in $S$ -- vertex $s_i$. If such a vertex $v_e$ does not lie in $A_i$, then we move it to $A_i$ (if $v_e$ lies in some other vertex set $A_{i'}$, we remove it from that vertex set). Since the degree of $v_e$ in $G$ is $2$, this does not increase the cardinalities of edge sets $\delta_G(A_{i'})$ for any $1\leq i'\leq k$. Moreover, we can adjust the sets of paths $\set{\qset_i}_{i=1}^k$, such that, for all $1\leq i\leq k$, set $\qset_i$ remains a set of edge-disjoint paths routing the edges of $\delta_G(A_i)$ to $s_i$ inside $G[A_i]$.

For all $1\leq i\leq k$, we denote $C_i=G[A_i]$. Note that, from the maximum flow / minimum cut theorem, for each $i$, there is a collection $\pset_i$ of at least $|\delta_G(C_i)|$ edge-disjoint paths connecting $s_i$ to vertices of $S\setminus \set{s_i}$. Since $|S|=k\leq 3\mu^4$, there is some vertex $s_j\in S\setminus\set{s_i}$, such that at least $|\delta_G(C_i)|/k\geq |\delta_G(C_i)|/(3\mu^4)$ of the paths in $\pset_i$ connect $s_i$ to $s_j$. Since instance $I$ is non-interesting, the number of such paths must be bounded by $m/\mu^{50}$, and so for all $1\leq i\leq k$, $|\delta_G(C_i)|\leq 3m/\mu^{46}$.
\end{proof}

Next, for all $1\leq i\leq k$, we will compute a flower cluster $C^f_i\subseteq C_i$, with center $s_i$, together with a set $\xset_i$ of its petals, such that $|\delta_G(C_i^f)|\leq  32m/\mu^{42}$. The following claim will complete the proof of \Cref{lemma: carve out flower clusters}.



\begin{claim}\label{claim: compute flowers}
	There is an efficient algorithm, that, for all $1\leq i\leq k$, computes a flower cluster $C^f_i\subseteq C_i$ with center $s_i$, together with a set $\xset_i$ of petals.
\end{claim}
\begin{proof}
	Fix an index $1\leq i\leq k$. For simplicity of notation, in the remainder of the proof, we denote $C_i$ by $C$, $s_i$ by $s$, and the set $\qset_i$ of paths by $\qset$. Recall that $|\delta_G(C)|\leq 3m/\mu^{46}$.
	
	
	%\mynote{did we define degrees in prelims? can we use $\deg$ for degree throughout?}
	Since $\deg_G(s)\geq m/\mu^4$, and $\delta_G(s)=\delta_C(s)$, we get that $\deg_C(s)\geq m/\mu^4$. Let $r=\floor{d_C(s)\cdot \frac{8\mu^4}{m}}$. Since $m/\mu^4 \leq \deg_C(s)\leq m$, we get that $8\leq r\leq 8\mu^4$. We compute a partition $E_1,\ldots,E_r$ of the edges of $\delta_C(s)$ into disjoint subsets, each of which contains at most $\floor{m/(2\mu^4)}$ edges that appear in the ordering $\oset_{s}\in \Sigma$ consecutively. From our choice of $r$, we get that $r\cdot\floor{m/(2\mu^4)}\geq d_G(s)$, so such a partition must exist.
	
	Consider now a graph $H$ that is defined as follows. We start with the graph $C\cup \delta_G(C)$. Let $R$ be the set of all endpoints of the edges of $\delta_G(C)$ that do not lie in $C$. We unify all such vertices into a vertex $a_0$. Next, we subdivide every edge $e\in \delta_C(s)$ with a new vertex $v_e$, and delete vertex $s$ from the resulting graph. Finally, for all $1\leq j\leq r$, we unify the vertices in set $V_j=\set{v_e\mid e\in E_j}$ into a single vertex $a_j$, obtaining the graph $H$. 
	Denote $Z=\set{a_0,a_1,\ldots,a_r}$. Note that $d_H(a_0)=|\delta_G(C)|\leq 3m/\mu^{46}$, so for all $1\leq j\leq r$, there are at most $3m/\mu^{46}$ edge-disjoint paths connecting $a_0$ to $a_j$.
	From the definition of interesting instances, for all $1\leq j<j'\leq r$, the maximum number of edge-disjoint paths connecting $a_j$ to $a_{j'}$ is at most $m/\mu^{50}$. Therefore, for all $1\leq j\leq r$, there is a cut separating $a_{j}$ from all vertices of $Z\setminus a_j$, containing at most $3m/\mu^{46}+rm/\mu^{50}\leq 12m/\mu^{46}$ edges.
	
	We apply the algorithm from  \Cref{lem: multiway cut with paths sets} to graph $H$ and vertex set $Z$. For all $1\leq j\leq r$, we denote by $A'_j$ the set of vertices that the algorithm returns for vertex $a_j$. Recall that, if $e=(s,v)$ is an edge of $E_j$, then vertex $v$ must have degree at most $2$ in graph $G$. We can then assume without loss of generality that $v$ lies in $A_j'$; if it lies in another set $A_{j'}'$, or it does not lie in any such set, we can simply move it to $A_j'$; this will not increase the values of the cuts $|E(A'_{j'},V(C)\setminus A'_{j'})|$ for any $j'$. We can also adjust the sets of paths $\qset'_j$ that the algorithm from \Cref{lem: multiway cut with paths sets} returns for each $1\leq j\leq r$, so that paths in $\qset'_j$ are edge-disjoint and route edges of $\delta_H(A'_j)$ to vertex $a_j$ inside the cluster $H[A'_j]$.
	
	For all $1\leq j\leq k$, let $X_j$ be the subgraph of $C$ induced by the vertex set $(A'_j\setminus\set{a_j})\cup \set{s}]$. We then let $C^f$ be the subgraph of $G$ induced by vertex set $\bigcup_{j=1}^kV(X_j)$. We claim that $C^f$ is a flower cluster with center $s$ and the set  $\xset=\set{X_1,\ldots,X_r}$ of petals.
	We now verify that $C^f$ and $\xset$ have all required properties. 
	
	First, it is immediate to verify that $C^f$ is a vertex-induced subgraph of $G$, for all $1\leq j\leq r$, $X_j$ is a vertex-induced subgraph of $C^f$, $\bigcup_{j=1}^rV(X_j)=V(C^f)$, and for all $1\leq j<j'\leq r$, $X_j\cap X_{j'}=\set{u}$. This establishes Properties \ref{prop: flower cluster vertex induced petals too} and \ref{prop: flower cluster petal intersection}. 
	
	Consider now some index $1\leq j\leq r$. Since we have assumed that, for every edge $e=(u,v)\in E_j$, $v\in A_j'$ holds, we get that $E_j\subseteq X_j$. Since $\delta_G(s)\subseteq \delta_C(s)$, and edge sets $E_1,\ldots,E_r$ partition $\delta_C(s)$, this establishes Property \ref{prop: flower cluster edges near center partition}. $\delta_G(s)\subseteq C^f$. %In particular, $d_{C^f}(s)\geq m/\mu^4$.
	
	
	Recall that for all $1\leq j\leq r$, $|\delta_C(X_j)\setminus \delta_C(s)|\le 12m/\mu^{46}$ (since $(A'_j,V(H)\setminus A'_j)$ is a minimum cut in $H$ separating $a_{j}$ from all vertices of $Z\setminus a_j$, whose value we have bounded above.) Therefore, $|\delta_G(C^f)|\leq r\cdot 12m/\mu^{46}\leq (8\mu^4)\cdot (12m/\mu^{46})\leq 96m/\mu^{42}$, and moreover the total number of edges $e=(u,v)$ with $u,v$ lying in different sets $X_1,\ldots,X_r$ is also bounded by  $96m/\mu^{42}$. This  establishes Property \ref{prop: flower cluster small boundary}.  Since no vertex of $S$ may lie in $C^f$ (as $C^f\subseteq C$), all vertices of $V(C)\setminus \set{s}$ have degrees at most $m/\mu^4$ in $G$. This establishes Property \ref{prop: flower center has large degree, everyone else no}.
	 
	 
	 Lastly, we need to establish Property \ref{prop: flower cluster routing}. Consider any petal $X_j\in \xset$. %We partition the edges of $\delta_G(X_j)\setminus\delta_G(s)$ into two susbsets: set $E'_j$ connects vertices of $X_j$ to vertices of $\bigcup_{j'\neq j}X_{j'}$, and set $E''_j$ contains all remaining edges, that must lie in $\delta_G(C)$.
	 From the definition of graph $H$, and since vertex $a_0$ may not belong to  set $A'_j$, we get that $\delta_H(A'_j)=\delta_G(X_j)\setminus \delta_G(s)$. Recall that  the algorithm from  \Cref{lem: multiway cut with paths sets} provided a set $\qset'_j$ of edge-disjoint paths that route the edges of $\delta_H(A'_j)$ to vertex $a_j$ inside the cluster $H[A'_j]$. By replacing vertex $a_j$ with vertex $s$ on each such path,  we obtain a collection $\qset''_j$ of edge-disjoint paths in graph $C^f$, that route the edges of $\delta_G(X_j)$ to $s$ inside $X_j$. 
	 We conclude that $C^f$ is a valid flower cluster with center $s$ and set $\xset$ of petals.
%	Recall that, since for all $1\leq j\leq r$, $(A^i_j,V(C_i)\setminus A^i_j)$ is a minimum cut separating $a_{j}$ from all vertices of $Z\setminus a_j$, $|E(A^i_j,V(C_i)\setminus A^i_j)|\leq 4m/\mu^{12}$. Since $\delta_G(C_i)\leq m/\mu^{12}$, and $\delta_G(X_j)\subseteq \delta_G(C_i)\cup E(A^i_j,V(C_i)\setminus A^i_j)$, we get that $|\delta_G(X_j)|\leq 5m/\mu^{12}$, and moreover $\delta_G(C')\leq 5mr/\mu^{12}+m/\mu^{12}$. Since $r\leq 4\mu^4$, we get that $\delta_G(C')\leq 5m/\mu^8$. Notice however that $|E(C'_i)|\geq d_{C_i}(s_i)$, while $r\leq d_{C_i}(s_i)\cdot 4\mu^4/m$. Therefore, we conclude that $|\delta_G(C'_i)|\leq 4|E(C_i')|/\mu^8+m/\mu^{12}\leq 8|E(C_i')|/\mu^8$, as $|E(C_i')|\geq \delta_{C_i}(s_i)\geq m/\mu^4$.
%	
%	We show that cluster $C'_i$ has all required properties. Consider some index $1\leq j\leq r$. From the definition of vertex set $A^i_j$, if we denote by $E'_j$ the edges that are incident to $s_i$ and lie in $X_j$, then $E'_j\subseteq E_j$ musthold, so $|E'_j|\leq m/(2\mu^4)$. Note that, if edge $e=(s_i,v)\in E_j$ does not lie in graph $X_j$, then $v\not\in A^i_j$.
\end{proof}
\end{proof}


%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
%--------------------------------
\subsubsection{Step 2: Small Clusters}
Let $C_0$ be the cluster that is obtained from graph $G$ after we delete all vertices lying in $\bigcup_{C\in \cset^f}V(C)$ from it, that is, $C_0=G\setminus(\bigcup_{C\in \cset^f}V(C))$.
Note that, since $|\cset^f|\leq 3\mu^4$, and, for all $C\in \cset^f$, $|\delta_G(C)|\leq 96m/\mu^{42}$, we get that $|\bigcup_{C\in \cset^f}|\delta_G(C)|\leq  (3\mu^4)\cdot (96m/\mu^{42})\leq 288m/\mu^{38}$, and so  $|\delta_G(C_0)|\leq 288m/\mu^{38}$.
 In this step, our goal is to further decompose cluster $C_0$ into a collection $\cset^s$ of clusters, that we refer to as \emph{small clusters}. We will require that each cluster $C\in \cset^s$ has the $\alpha_0$-bandwidth property, for an appropriately chosen parameter $\alpha_0$, and that $|E(C)|\leq |E(G)|/\mu^2$. Moreover, we will require that the total number of edges whose endpoints lie in different clusters of $\cset^f\cup \cset^s$ is relatively small. We show an algorithm that either computes such a decomposition of $C_0$, or establishes that $\optcrors(G,\Sigma)$ is sufficiently large, by utilizing the following lemma; the lemma will also be used later in this section in a slightly different setting, so it is stated for a more general setting than what is needed here.

\begin{lemma}\label{lem: decomposition into small clusters}
	There is an efficient algorithm, whose input consists of a graph $H$, a set  $T\subseteq V(H)$ of $k$ vertices called terminals (where possibly $T=\emptyset$), and parameters  $m,\tau\geq 0$, such that  $ |E(H)|\leq m$, $k\leq m/(32\tau\log m)$; every vertex in $T$ has degree $1$ in $H$; and maximum vertex degree in $H$ is at most $\frac{m}{c^*\tau^3 \log^5 m}$, for a large enough constant $c^*$.
	The algorithm
	either correctly certifies that $\optcro(H)\geq  \Omega \left( \frac{m^2}{ \tau^4\log^5 m} \right )$, or computes a collection $\cset$ of disjoint vertex-induced subgraphs of $H\setminus T$ called clusters, with the following properties:
	
	\begin{itemize}
		\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property, where $\alpha'=\frac{1}{16\alphasc(m)\cdot \log m}=\Omega\left(\frac{1}{\log^{1.5}m}\right )$;
		
		\item $\bigcup_{C\in \cset}V(C)=V(H)\setminus T$; 
		
		\item for every cluster $C\in \cset$, $|E(C)|\leq m/\tau$; and
		
		\item $|\bigcup_{C\in \cset}\delta_H(C)|\leq m/\tau$. 
		
	\end{itemize}
\end{lemma}

The proof of the lemma is very similar to the proof of \Cref{thm: basic decomposition of a graph} and is delayed to Section \ref{sec: appx-decomposition-small-clusters} of Appendix.



We consider the graph $C_0^+$, that is an augmentation of cluster $C_0$. Recall that $C_0^+$ is obtained from graph $G$, by first subdividing every edge $e\in \delta_G(C_0)$ with a vertex $t_e$, setting $T=\set{t_e\mid e\in \delta_G(C_0)}$, and letting $C_0^+$ be the subgraph of the resulting graph induced by $T\cup V(C_0)$. 
We apply the algorithm from \Cref{lem: decomposition into small clusters} to graph $H=C_0^+$, the set $T$ of terminals, and parameter $\tau=160\mu$.
Recall that, since $C_0$ contains no high-degree vertices, maximum vertex degree in $C_0$ is bounded by $\frac{m}{\mu^4}\leq \frac{m}{c^*\tau^3 \log^5 m}$. Recall also that $|T|=|\delta_G(C_0)|\leq 288m/\mu^{38}\leq m/(32\tau\log m)$.
If the algorithm from \Cref{lem: decomposition into small clusters} certifies that $\optcro(C_0^+)\geq  \Omega \left( \frac{m^2}{ \tau^4\log^5 m} \right )$, then we terminate the algorithm and  return FAIL. Notice that we are guaranteed that $\optcrors(I)\geq  \Omega \left( \frac{m^2}{ \mu^5} \right )$.

Therefore, we assume from now on that the algorithm from \Cref{lem: decomposition into small clusters} computed a collection $\cset^s$ of disjoint clusters, such that $\bigcup_{C\in \cset}V(C)=V(C_0)$, every cluster $C\in \cset$ has the $\alpha'$-bandwidth property in $G$, where $\alpha'=\frac{1}{16\alphasc(m)\cdot \log m}=\Omega\left(\frac{1}{\log^{1.5}m}\right )$, for every cluster $C\in \cset^s$, $|E(C)|\leq m/(160\mu)$; and
 $|\bigcup_{C\in \cset^s}\delta_G(C)|\leq m/(160\mu)$.
We refer to clusters in set $\cset^s$ as \emph{small clusters}.
Let $\cset=\cset^s\cup \cset^f$. Recall that $\Eout(\cset)$ is the set of all edges whose endpoints lie in different clusters of $\cset$. 
Since $|\bigcup_{C\in \cset^s}\delta_G(C)|\leq m/(160\mu)$,
$|\cset^f|\leq 3\mu^4$, and, for all $C\in \cset^f$, $|\delta_G(C)|\leq 96m/\mu^{42}$, we get that:

\begin{equation}\label{eq: num of edges between clusters}
\Eout(\cset)|\leq \frac m {160\mu}+(3\mu^4)\cdot \frac{96m}{\mu^{42}}\leq \frac m{80\mu}.
\end{equation}




\subsubsection{Step 3: Initial Disengagement}

In this step, we consider the set $\cset=\cset^s\cup \cset^f$ of clusters. Recall that all clusters in $\cset$ are disjoint and $\bigcup_{C\in \cset}V(C)=V(G)$. Moreover, every cluster in $\cset^s$ has the $\alpha'$-bandwidth property, for $\alpha'=\frac{1}{16\alphasc(m)\cdot \log m}$, while every cluster in $\cset^f$ has $1$-bandwidth property. Since $m\geq \mu^4$, we then get that every cluster in $\cset$ has the $\alpha_0=1/\log^3m$-bandwidth property.






\mynote{needs fixing -- need to restate in terms of $\nu$-decomposition}
 We apply the algorithm from \Cref{thm: disengagement - main} to instance $I=(G,\Sigma)$ of \CNwRS, and the set $\cset$ of clusters. Let $\iset_1$ be the resulting collection of subinstances of $I$ that the algorithm computes. Recall that we are guaranteed that, for each subinstance $I'=(G',\Sigma')\in \iset_1$, there is at most one cluster $C\in \cset$ with $E(C)\subseteq E(G')$, and all other edges of $G'$ lie in set $\Eout(\cset)$. We are also guaranteed that $\sum_{I'=(G',\Sigma')\in \iset_1}|E(G')|\leq O(|E(G)|)$, and  $\expect{\sum_{I'\in \iset_1}\optcrors(I')}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$.
Let $\aset_1$ denote the efficient algorithm, that, given a solution $\phi(I')$ to each instance $I'\in \iset_1$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq O\left (\sum_{I'\in \iset_1}\cro(\phi(I'))\right )$.
We have therefore shown an efficient randomized algorithm that computes a $\nu_0$-decomposition $\iset_1$ of instance $I$, for $\nu_0= 2^{O((\log m)^{3/4}\log\log m)}$.

We partition instances in $\iset_1$ into two subsets, set $\iset'_1$ containing all instances $I'=(G',\Sigma')$ with $|E(G')|\leq m/\mu$, and set $\iset''_1$ containing all remaining instances. We refer to instances in $\iset''_1$ as \emph{problematic instances}. Consider now any problematic instance $I'=(G',\Sigma')\in \iset''_1$. 
Recall that, from the guarantees of \Cref{thm: disengagement - main}, there is at most one cluster $C\in \cset$ with $C\subseteq G'$, and all edges of $G'$ lie in $E(C')\cup \Eout(\cset)$.
Since we are guaranteed that $|\bigcup_{C\in \cset}\delta(C)|\leq |\bigcup_{C\in \cset^s}\delta(C)|+|\bigcup_{C\in \cset^f}\delta(C)|\leq m/(160\mu)+288m/\mu^{38}\leq m/(80\mu)$, we get that $|E(G')\setminus E(C')|\leq m/(80\mu)$, and $|E(C')|\geq m/\mu-m/(80\mu)$. In particular, cluster $C'$ may not be a small cluster, so it must be a flower cluster. We say that $C'$ is a flower cluster associated with the problematic instance $I'\in \iset''_1$. In the remaining phases, we will further decompose each problematic instance into subinstances, proving the following theorem.



\newpage
\begin{theorem}\label{thm: decomposing problematic instances}
	There is an efficient randomized algorithm, that, given a problematic instance $I'=(G',\Sigma')\in \iset''_1$, either returns FAIL, or computes a $\nu_1$-decomposition $\tilde \iset(I')$ of $I'$, where $\nu_1=2^{O((\log m)^{3/4}\log\log m)}$, such that,  for each instance $\tilde I=(\tilde G,\tilde \Sigma)\in \tilde \iset(I')$, $|E(\tilde G)|\leq m/\mu$. Moreover, if $\optcrors(I')< m^2/\left (\mu^{13}\cdot 2^{c'(\log m)^{3/4}\log\log m}\right )$ for some large enough constant $c'$, then the probability that the algorithm returns FAIL is at most $1/\mu^3$.
\end{theorem}


Before providing the proof of \Cref{thm: decomposing problematic instances}, we show that the proof of  \Cref{lem: not many paths} follows from it.
We apply the algorithm from  \Cref{thm: decomposing problematic instances}  to every problematic instance $I'\in \iset''_1$. Assume first that, for each such instance $I'$, the algortihm returns a $\nu_1$-decomposition $\tilde \iset(I')$ of $I'$, such that,  for each instance $\tilde I=(\tilde G,\tilde \Sigma)\in \tilde \iset(I')$, $|E(\tilde G)|\leq m/\mu$. In this case, we return the collection 
$\iset=\iset'_1\cup \left(\bigcup_{I'\in \iset''_1}\tilde \iset(I')\right )$ of instances. From 
 from \Cref{claim: compose algs}, since $\nu_1\cdot\nu_2= 2^{O((\log m)^{3/4}\log\log m)}$, $\iset$ is indeed a $\nu$-decomposition of $I$, and, from the above discussion, we are guaranteed that, for every instance $\tilde I=(\tilde G,\tilde \Sigma)\in \iset$, $|E(\tilde G)|\leq m/\mu$.
 
 If, for any problematic instance $I'\in \iset''_1$, the algorithm from  \Cref{thm: decomposing problematic instances} returned FAIL, then our algorithm returns FAIL as well.
 
 Assume now that $\optcrors(I)<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$ for some large enough constant $c^*$. We will show that in this case, the probability that our algorithm returns FAIL is at most $1/\mu$. Since we have assumed that $m>\mu^{30}$ (from the statement of \Cref{lem: not many paths}), and $m^*$ is large enough, we can assume that $\sqrt{m}>2^{c^*(\log m)^{3/4}\log\log m}$, and so $|E(G)|<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$. 
 
 Recall that $\iset_1$ is a $2^{O((\log m)^{3/4}\log\log m)}$-decomposition of instance $I$, and so:
 
  $$\expect{\sum_{I'\in \iset_1}\optcrors(I')}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right ).$$
  
  In particular, there is some constant $c$, such that  $\expect{\sum_{I'\in \iset_1''}\optcrors(I')}\leq 2^{c(\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$. Let $\event$ be the bad event that $\sum_{I'\in \iset_1''}\optcrors(I')> 8\mu\cdot 2^{c(\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$. From Markov's inequality, the probability that $\event$ happens is at most $1/(8\mu)$. 
  
  Assume now that $\optcrors(I)<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$, and that the bad event $\event$ does not happen. Then for every problematic instance $I'\in \iset''_1$:
 
 
 \[  
 \begin{split}
 \optcrors(I')&\leq 8\mu\cdot  2^{c(\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )\\
 &\leq 8\mu\cdot 2^{c(\log m)^{3/4}\log\log m)}\cdot \frac{2m^2}{\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}}\\
 &\leq  \frac{m^2}{\mu^{13}\cdot 2^{c'(\log m)^{3/4}\log\log m}},
 \end{split}
\]

where $c'$ is the constant from \Cref{thm: decomposing problematic instances}, assuming that $c^*$ is a large enough constant. Therefore, if  $\optcrors(I)<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$ and Event $\event$ does not happen, then, for every problematic instance $I'\in \iset''_1$, the probability that the algorithm from 
 \Cref{thm: decomposing problematic instances} returns FAIL is at most $1/(\mu^3)$. Since $\sum_{I'=(G',\Sigma')\in \iset_1}|E(G')|\leq O(|E(G)|)$, and, for every problematic instance $I''=(G',\Sigma')\in \iset''_1$, $|E(G')|\geq m/\mu$, we get that $|\iset''_1|\leq O(\mu)$. Therefore, if $\optcrors(I)<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$ and $\event$ does not happen, then the probability that the algorithm from 
 \Cref{thm: decomposing problematic instances} returns FAIL for any problematic instance $I'\in \iset''_2$ is at most $1/(2\mu)$. Since the probability that event $\event$ happens is at most $1/(8\mu)$, we get that, if $\optcrors(I)<m^2/\left (\mu^{14}\cdot 2^{c^*(\log m)^{3/4}\log\log m}\right )$, then  the probability that our algorithm returns FAIL is at most $1/\mu$.



\iffalse
\mynote{ please restate the thm in terms of computing a $\nu'$-decomposition}
\begin{theorem}\label{thm: decomposing problematic instances}
	There is an efficient randomized algorithm, that, given a problematic instance $I'=(G',\Sigma')\in \iset''_1$, computes a collection $\tilde \iset(I')$ of subinstances of $I'$, with the following properties:
	
	\begin{itemize}
		\item $\sum_{\tilde I=(\tilde G,\tilde \Sigma)\in \tilde \iset(I')}|E(\tilde G)|\leq O(|E(G')|)$;
		
		
		\item for each subinstance $\tilde I=(\tilde G,\tilde \Sigma)\in \tilde \iset$, $|E(\tilde G)|\leq m/\mu$;
		 and
		
		\item $\expect{\sum_{\tilde I\in \tilde \iset}\optcrors(\tilde I)}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I')+|E(G')|\right )$.
	\end{itemize}
	Additionally, there is an efficient algorithm $\aset(I')$, that, given a solution $\phi(\tilde I)$ to each instance $\tilde I\in \tilde \iset$, computes a solution $\phi$ to instance $I'$, with $\cro(\phi)\leq O\left (\sum_{\tilde I\in \tilde \iset(I')}\cro(\phi(\tilde I))\right )$.
\end{theorem}
\fi



\iffalse
Indeed, we let $\iset=\iset'_1\cup \left (\bigcup_{I'\in \iset''_1}\tilde \iset(I')\right )$. It is immediate to verify that for every instance $I'=(G',\Sigma')\in \iset$, $|E(G')|\leq m/\mu$. Additionally: 

\[\begin{split}
\sum_{I'=(G',\Sigma')\in \iset}|E(G')|&=\sum_{I'=(G',\Sigma')\in \iset'_1}|E(G')|+\sum_{I'\in \iset''_1}\sum_{\tilde I=(\tilde G,\tilde \Sigma)\in \tilde \iset(I')}|E(\tilde G)|\\
&\leq \sum_{I'=(G',\Sigma')\in \iset'_1}|E(G')|+\sum_{I'=(G',\Sigma')\in \iset''_1}O(|E(G')|)\\
&\leq O(|E(G)|).
\end{split}\]


Similarly:


\[\begin{split}
\expect{\sum_{I'\in \iset}\optcrors(I')}&=\sum_{I'\in \iset'_1}\expect{\optcrors(I')}+\sum_{I'\in \iset''_1}\sum_{\tilde I\in \tilde \iset(I')}\expect{\optcrors(\tilde I)}\\
&\leq \sum_{I'\in \iset'_1}\expect{\optcrors(I')}  +\sum_{I'=(G',\Sigma')\in \iset''_1}\left (\expect{\optcrors(I')}+|E(G')|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}\\
&\leq \left (\optcrors(I)+|E(G)|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}.
\end{split}\]



Lastly, assume that we are  given, for each instance $I'\in \iset_1$, a feasible solution $\phi(I')$ to $I'$. For every instance $I''\in \iset''_1$, we use Algorithm $\aset(I'')$, that computes a solution $\phi(I'')$ to instance $I''$ of cost at most  $O\left (\sum_{\tilde I\in \tilde \iset(I'')}\cro(\phi(\tilde I))\right )$. We then apply algorithm $\aset_1$ to the resulting solutions to all instances in $\iset_1$, to obtain a solution to instance $I$ of cost at most $O\left (\sum_{ I'\in \iset_1}\cro(\phi(I))\right )$.

\fi

In order to complete the proof of  \Cref{lem: not many paths}, it is now enough to prove  \Cref{thm: decomposing problematic instances}. From now on, we fix a single a problematic instance $I'=(G',\Sigma')\in \iset''_1$, and its corresponding flower cluster $C'\in\cset^f$, and provide an algorithm to compute a decomposition of $I'$ into subclusters with required properties.



==> decomposition-step-backup.tex <==
\subsection{Splitting an $F$-Subinstance}
\label{subsec: decomposition step}


In this subsection we describe our main subroutine, called \procsplit. The goal of the subroutine is to split a given $F$-instance into two. In order to simplify the statement of the main result of this subsection, we start by defining a valid input and a valid output of the subroutine. Recall that $\cI=(\cG,\cSigma)$ is the input instance of $\cnwrs$ for \Cref{lem: many paths}, and $|E(\cG)|=\cm$.


\paragraph{Valid Input for \procsplit.}
A valid input for \procsplit consists of an instance  $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, and face $F\in \fset(\kset)$, such that $I=(G,\Sigma)$ is a valid $F$-subinstance of $I$. In other words, every vertex of $\kset$ must lie in $\partial(F)$.  Additionally, we require that:

\begin{itemize}
	\item Graph $G$ is a subgraph of $\cG$, with $|E(G)|>\cm/\mu$, and $\Sigma$ is the rotation system for $G$ induced by $\cSigma$; and
	\item The contracted instance $\hat I$ corresponding to instance $I$ is narrow.
\end{itemize} 

We denote $r=|\cset(F)|$.

\paragraph{Valid Output for \procsplit.}
A valid output for \procsplit consists of an  $F$-augmenting structure $\aset=(\Pi_F=\set{P_1,P_2},\set{b_u}_{u\in V(K\cup P_1\cup P_2)}, \psi')$ and a split $(I_{F_1}=(G_{F_1},\Sigma_{F_1}), I_{F_2}=(G_{F_2},\Sigma_{F_2}))$ of instance $I$ along $\aset$.


The main theorem of this subsection summarizes the properties of Procedure \procsplit.

\begin{theorem}\label{thm: procsplit}
	There is an efficient randomized algorithm, that, given a valid input $I,\kset,F$ to procedure \procsplit, either returns FAIL, or produces a valid output $\aset, I_{F_1}=G_{F_1},\Sigma_{F_1}), I_{F_2}=(G_{F_2},\Sigma_{F_2})$ to the procedure, such that the following hold. If there is a semi-clean solution $\phi$ to the $F$-instance $I$ with $\cro(\phi)\leq \frac{|E(G)|^2}{r^2\cdot \mu^{c''}}$ and $|\chi^{\dirty}(\phi)|\leq \frac{|E(G)|}{ \mu^{c''}\cdot r}$, where $c''$ is a large enough constant, then:
	
	\begin{itemize}
		\item $|E(G)\setminus (E(G_1)\cup E(G_2))|\leq \frac{\cro(\phi)\cdot \mu^{O(1)}}{|E(G)|}$; and
		\item there are semi-clean solutions $\phi_1$ and $\phi_2$ to instances $I_{F_1}$ and $I_{F_2}$ respectively, with $|\chi^{\dirty}(\phi_1)|\leq X$, $|\chi^{\dirty}(\phi_2)|\leq x$, and $\expect{\cro^*(\phi_1)+\cro^*(\phi_2)}\leq \cro^*(\phi)$. 
	\end{itemize}
Lastly, if there is  a semi-clean solution $\phi$ to the $F$-instance $I$ with $\cro(\phi)\leq \frac{|E(G)|^2}{r^2\cdot \mu^{c''}}$ and $|\chi^{\dirty}(\phi)|\leq \frac{|E(G)|}{ \mu^{c''}\cdot r}$, then the probability that the algorithm returns FAIL is at most $1/\mu^{32}$.
\end{theorem}

We will refer to the algorithm from \Cref{thm: procsplit} as \procsplit. The remainder of this subsection is dedicated to proving \Cref{thm: procsplit}. The algorithm consists of three steps. In the first step, we compute an augmentation $\Pi_F=\set{P_1,P_2}$, and analyze its properties. In the second step, we fix the orientations $b_u$ for vertices $u\in (V(P_1)\cup V(P_2))\setminus V(K)$. We will also show that the semi-clean solution $\phi$ to instance $I$ can be modified to obey these orientations. Then in the third step we compute both the split $(I_{F_1},I_{F_2})$, and the drawing $\psi'$ of $K\cup P_1\cup P_2$. We now describe each of the steps in turn.


\subsubsection{Step 1: Computing an $F$-Augmentation}
In order to compute an $F$-augmentation, we will first compute a large \emph{potential $F$-augmenting set}. Intuitively, a potential $F$-augmenting set is a large collection of edge-disjoint cycles or paths, each of which is a valid $F$-augmentation. As before, we partition the potential $F$-augmenting sets into three types, that will give rise to the three different types of $F$-augmnetations. The reason we do it here is that different types of $F$-augmentations will be used in Phase 1 and Phase 2 of the algorithm, and we would like our partitioning subroutine to be general enough so it can be used for both.


\begin{definition}[Potential $F$-Augmenting Path Set]
	Given an  instance $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in \fset(\kset)$, a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$,
	and a set $\pset$ of simple edge-disjoint paths in graph $G_F$, that are internally disjoint from $\partial(F)$, we say that $\pset$ is
	a \emph{potential $F$-augmenting set} for the skeleton structure $\kset$, if one of the following holds:
	
	\begin{itemize}
		\item (type-1 potential $F$-augmenting set): there is a vertex $v\in V(G_F)$ and a partition $(E_1,E_2)$ of the edges of $\delta_{G_F}(v)$ into two subsets, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma_F$, and every path in $\pset$ is a cycle that contains exactly one edge of $E_1$ and one edge of $E_2$ (we will view vertex $v$ as the endpoint of the cycle); or
		
		%		\item (type-2 potential $F$-augmenting set): 
		%		a vertex $v\in V(G_F)$, a partition $(E_1,E_2)$ of the edges of $\delta_{G_F}(v)$ and a cycle set $\wset$ as in type-1, except that now $v\in \partial(F)$ holds; all other vertices of the cycles in $\wset$ are disjoint from $\partial(F)$ as before; or
		
		\item (type-2 potential $F$-augmenting set): there is a connected component $C\in \partial(F)$ and a partition $(E_1,E_2)$ of the edges of $E^F(C)$, such that the edges of $E_1$ appear consecutively in the ordering $\oset^F(C)$, and every path in $\pset$ has an edge of $E_1$ as its first edge, and an edge of $E_2$ as its last edge; or
		
		\item (type-3  potential $F$-augmenting path set): there are two distinct connected components $C,C'\in \cset(F)$, such that each path in $\pset$ originates at a vertex of $C$ and terminates at a vertex of $C'$. %Moreover, if we denote by $E_1=\set{e_1,\ldots,e_{|\pset|}}\subseteq E^F(C)$ the set of edges containing the first edge on each path in $\pset$,  indexed according to their ordering in $\oset^F(C)$, and, for all $1\leq i\leq |\pset|$, by $e'_i$ the last edge on the unique path $P\in \pset$ that contains edge $e_i$, then edges $e'_1,\ldots,e'_{|\pset|}$ appear in the ordering $\oset^F(C')$ in the order of their indices.
	\end{itemize}
\end{definition}

We note that, as with type-2 $F$-augmentations, some paths in type-2 potential $F$-augmenting set may be cycles.

In our partitioning procedure, we will start with a given potential $F$-augmenting set $\pset$, and we will construct an $F$-augmentation of $\kset$ by simply selecting a path of $\pset$ uniformly at random. 
The following observation is immediate from the above definitions.


\begin{observation}\label{obs: potential to actual augmentors}
	For all $1\leq i\leq 3$, if $\pset$ is a type-$i$ potential $F$-augmenting set, then every path $P\in \pset$ is a type-$i$ $F$-augmentation of $\kset$.
\end{observation}


Next, we show that if a contracted instance associated with a valid $F$-subinstance $I_F$ is wide, then we can efficiently compute a wide enough potential $F$-augmenting path set. The proof is deferred to Section \ref{subsec: proof of finding potential augmentors} of Appendix.

\begin{claim}\label{claim: find potential augmentors}
	There is an efficient algorithm, whose input is
	an  instance $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in \fset(\kset)$ with $|\cset(F)|=r$, and a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$, such that the corresponding contracted instance $\hat I_F=(\hat G_F,\hat \Sigma_F)$ is wide. The algorithm   either computes a potential $F$-augmenting path set $\pset$ of cardinality $\ceil{\frac{|E(G_F)|}{24\mu^{\thec}\cdot r^2}}$, or
	correctly establishes that
	in every solution $\phi$ to instance $I_F$ with $\cro(\phi)\leq \frac{|E(G_F)|^2}{2^{20}\cdot \mu^{2\thec}\cdot r^2}$, either some pair of edges in $\partial(F)$ cross, or the number of crossings in which edges of $\partial(F)$ participate is at least $\frac{|E(G_F)|}{64\cdot \mu^{\thec}\cdot r}$.
\end{claim}

==========================================


\begin{theorem}\label{lem: many paths}
	There is an efficient randomized algorithm, that, given an interesting subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$, computes a non-empty collection $\iset$ of subinstances of $I$, such that:
	
	\begin{itemize}
		\item for each instance $I'=(G',\Sigma')\in \iset$, if $I'$ is an interesting instance, then $|E(G')|\le m/\mu$; 
		\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$; and
		\item
		there is an efficient algorithm, that, given a solution $\phi(I')$ to every instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq  \sum_{I'\in \iset}\cro(\phi(I')) + (m+\optcrors(I))\cdot\mu^{O(1)}$. \znote{constants subject to change}
	\end{itemize}
	
	Additionally, if $\optcrors(I)\leq m^2/\mu^{c'}$, then with probability at least $31/32$:
	$$\sum_{I'\in \iset}\optcrors(I')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}.$$
\end{theorem}

==> decomposition-step.tex <==
\subsection{Splitting a Subinstance: Procedure \procsplit}
\label{subsec: decomposition step}

In this subsection we provide our main procedure, called $\procsplit$, whose goal is to split a given subinstance of the input instance $\cI=(\cG,\cSigma)$ into two via a core enhancement structure. 

\paragraph{Valid Input for \procsplit.}
A valid input to Procedure \procsplit consists of an instance  $I=(G,\Sigma)$  of $\cnwrs$, a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ for $I$, and a promising set $\pset$ of paths for $I$ and $\jset$ of cardinality $\floor{\frac{|E(G)|}{\mu^b}}$ for some constant $b$, for which the following hold:

\begin{properties}{C}
	\item graph $G$ is a subgraph of $\cG$, and $\Sigma$ is the rotation system for $G$ induced by $\cSigma$; and  \label{prop valid input size}
	%	\item $|E(G)|\geq \cm/\mu$; \label{prop many edges}
	\item there exists a solution $\phi$ to instance $I$ that is $\jset$-valid, such that $\cro(\phi)\leq \frac{|E(G)|^2}{\mu^{60b}}$ and $|\chi^{\dirty}(\phi)|\leq \frac{|E(G)|}{ \mu^{60b}}$. \label{prop valid input drawing}
\end{properties} 

We emphasize that the solution $\phi$ is not given as part of input and it is not known to the algorithm.


\paragraph{Valid Output for \procsplit.}
A valid output for \procsplit consists of a
$\jset$-enhancement structure $\aset$, and
a split $(I_1=(G_1,\Sigma_1),I_2=(G_2,\Sigma_2))$ of $I$ along $\aset$. Let $P^*$ be the enhancement path of $\aset$, and let $(\jset_1,\jset_2)$ be the split of the core structure $\jset$ along $\aset$.
Denote $E^{\del}(I)=E(G)\setminus (E(G_1)\cup E(G_2))$. Let $G'=G\setminus E^{\del}(I)$, let $\Sigma'$ be the rotation system for $G'$ induced by $\Sigma$, and let $I'=(G',\Sigma')$ be the resulting instance of \cnwrs. We require that the following properties hold:


\begin{properties}{P}
	\item $|E^{\del}(I)|\leq \frac{\cro(\phi)\cdot \mu^{2200}}{|E(G)|}+|\chi^{\dirty}(\phi)|$ \mynote{??};\label{prop output deleted edges}
	\item  $|E(G_1)|,|E(G_2)|\leq |E(G)|-\frac{|E(G)|}{32\mu^{b}}$; and \label{prop: smaller graphs}
	\item there is a $\jset$-valid solution $\phi'$ for instance $I'$ that is compatible with $\phi$, in which the images of the edges of $E(J)\cup E(P^*)$ do not cross each other, $\cro(\phi')\leq \cro(\phi)$, and the number of crosings in which the edges of $P^*$ participate is at most \mynote{?? $\cro(\phi)\mu^{26b}/\cm'$}.\label{prop output drawing}
\end{properties}  


The main theorem of this subsection summarizes the properties of Procedure \procsplit.

\begin{theorem}\label{thm: procsplit}
	There is an efficient randomized algorithm, that, given a valid input  $I=(G,\Sigma)$, $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$, $\pset$ to procedure \procsplit, with probability at least $1-1/\mu^{10b}$ computes a valid output for the procedure.
\end{theorem}
We will refer to the algorithm from \Cref{thm: procsplit} as \procsplit. The remainder of this subsection is dedicated to the proof of \Cref{thm: procsplit}. Throughout the proof, we denote $m=|E(G)|$. The algorithm consists of two steps. In the first step, we compute an enhancement $P$ of the core structure $\jset$ and analyze its properties. In the second step, we comlete the construction of the enhancement structure $\aset$ and of the split $(I_1,I_2)$ of instance $I$ along $\aset$. We now describe each of the steps in turn. In order to simplify the exposition, throughout this subsection, we use ``enhancement'' and ``enhancement structure'' when we refer to an enhancement of $\jset$ and enhancement structure for $\jset$. For simplicity of notation, we also denote the drawing $\rho_J$ of the core $J$ by $\rho$, and the face $F^*_{\rho_J}$ of this drawing by $F^*$.


\input{interesting-phase1-step1}
\input{interesting-phase1-step2}














































==> decomposition_1.tex <==

\section{Proof of Lemma \ref{lem: not many paths} -- Computing the Decomposition}

\input{decomposition-new}


%\subsection{Phase 1: Initial Decomposition}

\iffalse

Assume we are given a valid sub-instance $(G',\Sigma')$, where $G'$ is not $\mu$-interesting. We denote $m=|E(G')|$.
We say that a vertex $v$ is a \emph{high-degree vertex}, if its degree is at least $m/\mu^8$.


We say that a cluster $C$ of $G$ is a \emph{good cluster}, if $|E(C)|\le m/\mu^2$, and $C$ is $\alpha$-boundary-well-linked.

We say that a cluster $C$ of $G$ is a \emph{flower cluster}, iff $|E(C)|> m/\mu^2$, $C$ contains a unique high-degree vertex $u$, and there is a set $\set{C_1,\ldots,C_k}$ of clusters of $C$, such that
\begin{itemize}
\item for each $1\le i\le k$, $u\in V(C_i)$;
\item the vertex sets $\set{V(C_i)\setminus \set{u}}_{1\le i\le k}$ forms a partition of $V(C)\setminus \set{u}$;
\item for each $1\le i\le k$, there is a set $\qset_i$ of paths in $C_i$ connecting edges of $\delta(C_i)$ to $u$, such that the paths of $\qset_i$ cause congestion $O(1)$.
\end{itemize}

\fi


\newpage

The main result of this section is the following lemma.

\begin{lemma}
\label{lem:main_decomposition}
There is an efficient algorithm, that, given any sub-instance $(G',\Sigma')$ (with $|E(G')|=m$),
either correctly claims that $\optcrors(G',\Sigma')\ge |E(G')|^2/\mu^{10}$,
or computes a set $\cset$ of vertex-disjoint clusters of $G'$, such that each cluster of $\cset$ is either a good cluster or a flower cluster, the vertex sets $\set{V(C)}_{C\in \cset}$ partitions $V(G')$, and $|\inE(\cset)|= O(m/\mu)$.
\end{lemma}

In the remainder of this section we provide the proof of Lemma~\ref{lem:main_decomposition}.




==> disengage_path-backup.tex <==
\subsection{Special Case: No Problematic Indices}
\label{subsec: no prob edges}



\mynote{A quick note that may be useful later. Suppose we have clusters $C_1,\ldots,C_r$ organized on a path, and there is no bad index. Suppose now we apply *basic disengagement* procedure (exactly as described in Sec 6.2) iteratively, first disengaging $C_1$, and getting graph $G_1$, where $C_1$ becomes a single vertex, then disengaging $C_2$ from $G_1$, and so on. As the result, instances that we obtain are *exactly* the instances created in this section, including the specific rotation around the two contracted vertices. This means that we don't need to worry about combining the solutions of the resulting instances together - the algorithm for basic disengagement does it (applying Lemma 6.3 as is). But the algorithm for basic disengagement won't give us the bound that we need on the total solution costs of the new instances (if we use Lemma 6.2 as is, the cost may be too high, because we'll be charging to same crossings again and again). This bound has to rely on the fact that we can route every edge connecting two non-consecutive clusters via a central path.
	One question that I'm wondering about is whether it is critical that, for an edge $e$ connecting $C_i$ to $C_j$, is routing path $P(e)$ has to go through the central path. I believe that there must be a portion of $P(e)$ between $C_i$ and $C_j$ that goes between the two clusters on a central path. But if before that it jumps to some clusters that lie before $C_i$ or after $C_j$ I think it does not matter to us. This may be good to understand because this may allow us to weaken the condition of "no bad index". If we decide to extend this algorithm to the case of a path-of-stars, this understanding may be helpful.}

In this subsection we show the proof of Lemma~\ref{lem: path case}, with the additional assumption that no index $i$ is problematic. That is, for each $1\le i\le k-1$, $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|\le 100|\hat E_i|$.
Recall that we are given, for each $1\le i\le k$, a vertex $u_i$ of $C_i$, and a set $\qset_i$ of paths in $C_i$ connecting the edges of $\delta(C_i)$ to $u_i$, such that for every edge $e\in E(C_i)$, $\mathbb{E}[\cong_{C_i}(\qset_i,e)^2]\le \temp$.
%\znote{assuming that $u_i$ and $\qset_i$ can be found in the decomposition step.}
%\znote{To set}

Recall that $\inE(\cset)$ is the set of edges connecting distinct clusters of $\cset$. 
We denote by $E'$ the subset of edges in $\inE(\cset)$ connecting a pair $C_i,C_j$ of clusters of $\cset$, with $j\ge i+2$.
%For each $1\le i\le k$, we denote $E_i=E(C_i,C_{i+1})$.
Therefore, $E(G)=E'\cup\left(\bigcup_{1\le i\le k-1}\hat E_i\right)\cup \left(\bigcup_{1\le i\le k}E(C_i)\right)$.
Recall that $H=G_{|\cset}$, and the node in $H$ that represents the cluster $C_i$ in $G$ is denoted by $x_i$.
Therefore, each edge in $E'\cup \left(\bigcup_{1\le i\le k-1}\hat E_i\right)$ corresponds to an edge in $H$, and we do not distinguish between them. 


We now start to describe the algorithm that construct the sub-instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$.
The algorithm proceeds in two stages. In the first stage, we compute, for each edge of $E'$, two auxiliary paths in $G$, that we call its \emph{inner path} and \emph{outer path} respectively. In the second stage, we use these auxiliary paths to define the sub-instances and show that they satisfy the properties of \Cref{lem: path case}.
In the remainder of this section, we describe the first stage in \Cref{sec: inner and outer paths} and the second stage in \Cref{sec: disengaged instances}, and then complete the proof of \Cref{lem: path case} in \Cref{sec: path case with no problematic index}.




\subsubsection{Compute Inner and Outer Paths}
\label{sec: inner and outer paths}


In the first stage, we will compute, for each pair $i,j$ of indices (with $i\le j-2$) and for each edge $e\in E'$ that connects a vertex of $C_i$ to a vertex of $C_j$, a path $P_e$ connecting $u_i$ to $u_j$ that only uses edges of $\bigcup_{i\le t\le j-1}\hat E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$, and a path $P^{\out}_e$ connecting $u_i$ to $u_j$ that only uses edge $e$ and edges of $E(C_i)\cup E(C_j)$. We call path $P_e$ the \emph{inner path} of $e$ and path $P^{\out}_e$ the \emph{outer path} of $e$.

We first compute the outer paths. Let $e$ be an edge of $E'$ connecting a vertex of $C_i$ to a vertex of $C_j$, so $e\in \delta(C_i)$ and $e\in \delta(C_j)$. Recall that the set $\qset_i$ contains a path $Q_i(e)$, connecting $e$ to $u_i$, and the set $\qset_j$ contains a path $Q_j(e)$, connecting $e$ to $u_j$.
We simply define its outer path $P^{\out}_e$ to be the union of path $Q_i(e)$ and path $Q_j(e)$.
It is clear that path $P^{\out}_e$ connects $u_i$ to $u_j$, and only uses edge $e$ and edges of $E(C_i)\cup E(C_j)$.
Throughout the section, we view $u_j$ as the first endpoint of $P^{\out}_e$ and $u_i$ as its last endpoint. We denote $\pset^{\out}=\set{P_e^{\out}\mid e\in E'}$, and for each $1\le i\le k$, we denote $\pset^{\out}_{*,i}=\set{P^{\out}_e \mid e\in E^{\lef}_{i}}$ and $\pset^{\out}_{i,*}=\set{P^{\out}_e \mid e\in E^{\rig}_{i}}$.
%\znote{notation to be coordinated}

We now compute the set $\pset=\set{P_e}_{e\in E'}$ of inner paths in three steps. In the first step, we compute a set $\tilde \pset$ of paths in $H$. In the second step, we transform the set $\tilde \pset$ of paths in $H$ into a set $\pset^*$ of paths in $G$.
In the third step, we further process paths in $\pset^*$ to obtain the set $\pset$ of inner paths for edges of $E'$.
We now describe each step in more details.

\paragraph{Step 1.}
In this step we process edges in $E'$ one-by-one. Throughout, for each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, we maintain an integer $z_{\hat e}$ indicating how many times the edge $\hat e$ has been used, that is initialized to be $0$. 
%Throughout, all edges of $\in \bigcup_{1\le i\le k-1}\hat E_i$ are either marked \emph{used} or \emph{not used}. Initially, all edges are not used.
Consider an iteration of processing an edge $e\in E'$. Assume $e$ connects $C_i$ to $C_j$ in $G$, we then pick, for each $i\le t\le j-1$, an edge $\hat e$ of $\hat E_t$ with minimum $z_{\hat e}$ over all edges of $\hat E_t$, and let $\tilde P_e$ be the path obtained by taking the union of all picked edges.
Note that, in $H$, each edge of $\hat E_t$ connects $x_t$ to $x_{t+1}$, so the path $\tilde P_e$ sequentially visits nodes $x_i, x_{i+1},\dots,x_j$. 
We then increase the value of $z_{\hat e}$ by $1$ for all picked edges $\hat e$, and proceed to the next iteration. After processing all edges of $E'$, we obtain a set $\tilde\pset=\set{\tilde P_e}_{e\in E'}$ of paths in $H$.
%{\color{red} We further assume that, for each $1\le i\le k$, $|E(S_i,\overline{S_i})|\le \beta\cdot |E_i|$, where we can think of $\beta=\poly\log n$.}
We use the following observation.

\begin{observation}
\label{obs:central_congestion}
For each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, $\cong_{H}(\tilde\pset,\hat e)\le 100$.
%The paths in $\tilde\pset$ are edge-disjoint.
\end{observation}
\begin{proof}
	%For each $1\le i\le k-1$, we denote by $E^*_i$ as the set of edges in $E'$ that connects a vertex of $\set{v_1,\ldots,v_{i-1}}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$, we denote by $E^{\lef}_i$ as the set of edges in $E'$ that connects $v_{i+1}$ to a vertex of $\set{v_1,\ldots,v_{i-1}}$, and we denote $E^{\rig}_i$ as the set of edges in $E'$ that connects $v_{i}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$.
	From the algorithm, for each $1\le i\le k-1$, the paths of $\tilde\pset$ that contains an edge of $\hat E_i$ are $\set{\tilde P_e\mid e\in \big(E_i^{\rig} \cup E_{i+1}^{\lef} \cup E_i^{\through}\big)}$.
	Since $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|\le 100|\hat E_i|$, each edge of $\hat E_i$ is used is used at most $100$ times. Observation~\ref{obs:central_congestion} then follows.
\end{proof}

\iffalse
We now further process the set $\tilde\pset$ of paths to obtain another set $\tilde\pset'$ of paths with some additional properties, as follows.

\paragraph{Step 2.1.} Let $\tilde G'$ be the graph obtained from $\tilde G$ by replacing each edge $e$ with $\beta$ parallel copies $e_1,\ldots,e_\beta$ connecting its endpoints. Now for each path $\tilde P\in \tilde{\pset}$, we define a path $\tilde P^*$ as the union of, for each edge $e\in \tilde P$, a copy $e_t$ of $e$, such that, for all paths of $\tilde\pset$ that contains the edge $e$, their corresponding paths in $\set{\tilde P^*\mid e\in \tilde P}$ contain distinct copies of $e$. We denote $\tilde\pset^*=\set{\tilde P^*\mid \tilde P\in \tilde \pset}$. From the above discussion, the paths of $\tilde\pset^*$ are edge-disjoint.
\fi

\paragraph{Step 2.}
In this step we compute a set $\pset^*$ of paths in $G$, using the paths in $\tilde\pset$ and path sets $\set{\qset_i}_{1\le i\le k}$, as follows.
Recall that the set $\qset_i$ contains, for each edge $e\in\delta(C_i)$, a path $Q_i(e)$ connecting $e$ to $u_i$.
Also recall that, in graph $G$, an edge $\hat e\in \hat E_i$ belongs to both $\delta(C_i)$ and $\delta(C_{i+1})$.
Therefore, for an edge $\hat e\in \hat E_i$, the union of path $Q_i(\hat e)$ and path $Q_{i-1}(\hat e)$ is a path connecting $u_i$ to $u_{i+1}$.
Now consider an edge $e\in E'$ connecting a vertex of $C_i$ to a vertex of $C_{j}$ (with $i\le j-2$), and the corresponding path $\tilde P_e=(\hat e_i,\hat e_{i+1},\ldots,\hat e_{j-1})$ in $\tilde\pset$, where $\hat e_t\in \hat E_t$ for each $i\le t\le j-1$. We define the path $P^*_e$ as the sequential concatenation of paths $Q_{i}(\hat e_i)\cup Q_{i+1}(\hat e_i), Q_{i+1}(\hat e_{i+1})\cup Q_{i+2}(\hat e_{i+1}),\ldots,Q_{j-1}(\hat e_{j-1})\cup Q_{j}(\hat e_{j-1})$.
It is clear that path $P^*_e$ only contains edges of $\bigcup_{i\le t\le j-1}\hat E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$, and sequentially visits vertices $u_i,u_{i+1},\ldots,u_{j}$.
Denote $\pset^*=\set{P^*_e\mid e\in E'}$.
From Observation~\ref{obs:central_congestion}, it is easy to see that for each edge $e\in \bigcup_{1\le i\le k}E(C_i)$, $\cong_{G}(\pset^*,e)\le 100\cdot\cong_{G}(\qset_i,e)$.


%Recall that, for each $1\le i\le k$, the set $\qset_i$ of paths connects edges of $\delta(C_i)$ to $u_i$. Note that $\hat E_i\in \delta(C_i)$ and $\hat E_i\in \delta(C_{i+1})$. For each edge $e\in \hat E_i$, let $\hat Q_e$ be the path obtained by taking the union of the path in $\qset_i$ connecting $e$ to $u_i$, the edge $e$, and the path in $\qset_{i+1}$ connecting $e$ to $u_{i+1}$, so path $\hat Q_e$ connects $u_i$ to $u_{i+1}$. Denote $\hat\qset_i=\set{\hat Q_e\mid e\in \hat E_i}$, and denote $\hat\qset=\bigcup_{1\le i\le k-1}\hat\qset_i$.
\iffalse

It would be convenient to state our algorithm if the core paths of $\pset$ are edge-disjoint. 
For which, we construct another instance $(G',\Sigma')$ of \CNwRS, as follows. 
Denote $\qset=\bigcup_{1\le i\le k}\qset_i$.
We start with the instance $(G,\Sigma)$.
For each edge $e\in E(\qset)$, we replace $e$ with $2\cdot\cong_{\qset}(e)$ parallel copies.
For each edge $e\in E(\pset)\setminus E(\qset)$, we replace $e$ with $2$ parallel copies.
For each vertex $v$ such that $\delta(v)\cap E(\pset\cup\qset)= \emptyset$, we define its rotation $\oset'_v$ to be identical to the its rotation $\oset_v$ in $\Sigma$. 
For each vertex $v$ such that $\delta(v)\cap E(\pset\cup\qset)\ne \emptyset$, we define its rotation $\oset'_v$ as follows. We start with the rotation $\oset_v$, and then (i) replace, for each edge $e\in \delta(v)\cap E(\qset)$, the edge $e$ in the ordering $\oset_v$ by its $2\cdot\cong_{\qset}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, 
and the ordering among the copies is arbitrary; and
(ii) replace, for each edge $e\in \delta(v)\cap E(\pset)$, the edge $e$ in the ordering $\oset_v$ by its $2$ copies that appears consecutively at the location of $e$ in $\oset_v$, 
and the ordering among the copies is arbitrary. 


We use the following observation.
\begin{observation}
$\optcrors(G,\Sigma)\le \optcrors(G',\Sigma')\le O(\optcrors(G,\Sigma)\cdot\poly\log n)$. 
Moreover, given a drawing $\phi\in \Phi(G,\Sigma)$, we can efficiently compute a drawing $\phi'\in \Phi(G',\Sigma')$, with $\cro(\phi')\le O(\cro(\phi)\cdot\poly\log n)$. 
%given a drawing $\phi'\in \Phi(G',\Sigma')$, we can efficiently compute a drawing $\phi\in \Phi(G,\Sigma)$, with $\cro(\phi)\le\cro(\phi')$.
\end{observation}
\begin{proof}
\end{proof}

Now for each path $P\in \pset$, we define a path $P'$ in $G'$ as the union of, for each edge $e\in P$, a copy $e_t$ of $e$, such that for all paths of $\pset$ that contains the edge $e$, their corresponding paths in $\set{P'\mid P\in \pset, e\in P}$ contain distinct copies of $e$. We denote $\pset'=\set{P'\mid  P\in \pset}$. 
%We define the set $\qset'$ from $\hat\qset$ similarly. 
From the above discussion, the paths of $\pset'$ are edge-disjoint.
Moreover, note that $V(G)=V(G')$, and if a path $P\in \pset$ connects $u_i$ to $u_j$ in $G$, then the corresponding path $P'$ connects $u_i$ to $u_j$ in $G'$.
\fi


\paragraph{Step 3.}
In this step we further process paths in $\pset^*=\set{P^*_e\mid e\in E'}$ to obtain the set $\pset=\set{P_e\mid e\in E'}$ of inner paths for edges of $E'$.
\iffalse
\begin{itemize}
	\item $|\pset|=|\tilde\pset'|$;
	\item for each pair $1\le i,j\le k$, the number of paths in $\pset'$ connecting $u_i$ to $u_j$ is the same as that of $\pset^*$; and 
	\item the paths in $\pset^*$ are non-transversal with respect to $\Sigma'$.
\end{itemize}
\fi
For each path $P^*\in \pset^*$ connecting $u_i$ to $u_{j}$ (recall that such a path visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially), we define, for each $i\le t\le j-1$, the path $P^*_{(i)}$ to be the subpath of $P^*$ between $u_{i}$ and $u_{i+1}$. For each $1\le i\le k-1$, we denote $\pset^*_{(i)}=\set{P^*_{(i)}\text{ } \bigg|\text{ } u_i,u_{i+1}\in V(P^*),P^*\in \pset^*}$, so all paths in $\pset^*_{(i)}$ connects $u_i$ to $u_{i+1}$.
We then apply the algorithm in Lemma~\ref{lem: non_interfering_paths} to the set $\pset^*_{(i)}$ of paths, and obtain a set $\rset^*_{(i)}$ of $|\rset^*_{(i)}|=|\pset^*_{(i)}|$ paths connecting $u_i$ to $u_{i+1}$, such that for every $e\in E(G)$, $\cong_{G}(\rset^*_{(i)},e)\le \cong_{G}(\pset^*_{(i)},e)$, and the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.

%We use the following observation, whose proof appears in Appendix~\ref{apd: Proof of rerouting_matching_cong}.

%\znote{Need to rethink which definition to include for ``non-transversal".}



%We now construct the inner paths $\pset=\set{P_e\mid e\in E'}$ as follows.
We now re-organize the paths in sets $\rset^*_{(1)},\ldots, \rset^*_{(k-1)}$ to obtain the set $\pset$ of inner paths.
%We now construct the set $\pset^*$ of paths.
Note that, if we select, for each $i\le t\le j-1$, a path of $\rset^*_{(i)}$, then, by taking the union of them, we can obtain a path $\hat P$ connecting $u_i$ to $u_j$. 
We call the selected path of $\rset^*_{(t)}$ the \emph{$t$-th segment} of $\hat P$. Therefore, a path connecting $u_i$ to $u_j$ obtained in this way is the union of its $i$-th segment, its $(i+1)$-th segment, $\ldots$ , and its $(j-1)$-th segment.
We now incrementally construct the set $\pset$ of paths.
Intuitively, we will silmutaneously construct all paths of $\pset$ in $k-1$ iterations, where in the $i$-th iteration, we will determine the $i$-th segment of all paths in $\pset$.

%For each $1\le i<j\le k$, we denote by $p_{i,j}$ the number of paths in $\pset^*$ connecting $u_i$ to $u_j$. 
Throughout, we will maintain a set $\hat{\pset}=\set{\hat P_e\mid e\in E'}$ of paths, where each path $\hat P_e$ is indexed by an edge $e$ of $E'$. 
Assume that the edge $e$ connects a vertex of $C_i$ to a vertex of $C_j$ (with $j\ge i+2$), then the path $\hat P_e$ is supposed to originate at $u_i$ and terminate at $u_j$.
We call $u_i$ the \emph{destined origin} of $\hat P_e$ and call $u_i$ the \emph{destined terminal} of $\hat P_e$.
Initially, $\hat{\pset}$ contains $|E'|$ paths, and all paths in $\hat{\pset}$ contain no edge. 
%and for each $1\le i<j\le k$, there are $p_{i,j}$ paths of $\hat{\pset}$ whose destined origin is $u_i$ and destined terminal is $u_j$.
We will sequentially process vertices $u_1,\ldots,u_{k-1}$, and, for each $1\le i\le k-1$, upon processing vertex $u_i$, determine which path of $\rset^*_{(i)}$ serves as the $i$-th segment of which path of $\hat\pset$.

We now fix an index $1\le i\le k-1$ and describe the iteration of processing vertex $u_i$. The current set $\hat\pset$ of paths can be partitioned into four sets: set $\hat\pset^{o}_i$ contains all paths of $\hat\pset$ whose destined origin is $u_i$; set $\hat\pset^{t}_i$ contains all paths of $\hat\pset$ whose destined terminal is $u_i$; set $\hat\pset^{\thr}_i$ contains all paths whose destined origin is $u_{i'}$ for some index $i'<i$ and whose destined terminal is $u_{j'}$ for some index $j'>i$; and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ contains all other paths. 
Note that the paths in set $\hat\pset^{t}_i$ and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ do not contain an $i$-th segment, so in this iteration we will determine the $i$-th segment of paths in the sets $\hat\pset^{o}_i$ and $\hat\pset^{\thr}_i$.
%On one hand, notice that all paths in $\hat\pset^{t}_i$ already connects its destined origin to $u_i$, and we will not modify them anymore, since these paths are already completed.

Note that the paths in $\hat\pset^{o}_i$ currently contain no edge, %and we arbitrarily designate, for each path in $\hat\pset^{o}_i$, a distinct path of $\pset^*_{(i)}$ as its $i$-th segment.
and the paths in $\hat\pset^{\thr}_i$ currently contain up to its $(i-1)$-th segment. 
%and in this iteration we will designate paths of $\pset^*_{(i)}$ as their $i$-th segments, as follows. 
We then denote
\begin{itemize}
\item by $L^-_i$ the multi-set of the current last edges of paths in $\hat\pset^{\thr}_i$;
\item by $L^+_i$ the multi-set of the first edges of paths in $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of any path in $\hat{\pset}$); and
\item by $L^{\out}_i$ the multi-set of last edges of paths in  $\pset^{\out}_{i,*}=\set{P^{\out}_e \mid e\in E^{\rig}_i}$.
\end{itemize} 
%$L^-_i$ the multi-set of edges of $\delta(u_i)$ that currently serves as the last edge of paths in $\hat\pset^{\thr}_i$, denote by $L^+_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of to any path in $\hat{\pset}$), and denote by $L^{\out}_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\set{P^{\out}_e \mid e\in E(C_i,C_j)\text{ for some }j>i+1}$.
%It is clear that $R^-_i, R^+_i$ are two disjoint subsets of $\delta(u_i)$ with $|R^-_i|=|R^+_i|$. 
Clearly, elements in sets $L^-_i, L^+_i,L^{\out}_i$ are edges of $\delta(u_i)$. 
We then define, for each $e\in \delta(u_i)$, $n^-_e=n_{L^-_i}(e)+n_{L^{\out}_i}(e)$ and
$n^+_e=n_{L^+_i}(e)$.
%\znote{see new notations in prelim (second paragraph in \Cref{sec:prelim})}
We use the following simple observation.
\begin{observation}
For each edge $e\in \delta(u_i)$, $\sum_{e\in \delta(u_i)}n^-_e=\sum_{e\in \delta(u_i)}n^+_e$.
\end{observation}
\begin{proof}
On one hand, $\sum_{e\in \delta(u_i)}n_{L^{\out}_i}(e)=|\bigcup_{j>i+1}E(C_i,C_j)|=|\hat\pset^{o}_i|$, and $\sum_{e\in \delta(u_i)}n_{L^{-}_i}(e)=|L^-_i|=|\hat\pset^{\thr}_i|$. 
On the other hand, recall that $|\rset^*_{(i)}|=|\pset^*_{(i)}|$, $\pset^*_{(i)}=\set{P^*_{(i)}\text{ } \bigg|\text{ } u_i,u_{i+1}\in V(P^*),P^*\in \pset^*}$ and the only edges in $E'$ such that path $P^*_e$ contains vertices $u_i,u_{i+1}$ are edges of $E^{\thr}_i\cup E^{\rig}_i$. Therefore,
$\sum_{e\in \delta(u_i)}n_{L^{+}_i}(e)=|L^+_i|=|\rset^*_{(i)}|=|\pset^*_{(i)}|=|E^{\thr}_i|+|E^{\rig}_i|=|\hat\pset^{\thr}_i|+|\hat\pset^{o}_i|$.
\end{proof}

We apply the algorithm in \Cref{obs:rerouting_matching_cong} to graph $G$, vertex $u_i$, rotation $\oset_{u_i}$ and integers $\set{n^-_e,n^+_{e}}_{e\in \delta(u_i)}$.
Let $M$ be the multi-set of ordered pairs of the edges of $\delta(u_i)$ that we obtain. 
%we can efficiently computes a perfect matching $M\subseteq E^-\times E^+$ between the edges of $E^-$ and the edges of $E^+$, such that, for each pair of matched pairs $(e^-_1,e^+_1)$ and $(e^-_2,e^+_2)$ in $M$, the intersection of the path that consists of the edges $e^-_1,e^+_1$ and the path that consists of edges $e^-_2,e^+_2$ at vertex $u$ is non-transversal with respect to $\oset_v$.
We then designate: 
\begin{itemize}
\item for each path $\hat P_e\in \hat\pset^{\thr}_i$ with $e^-$ as its current last edge, a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$; and
\item for each path $P^{\out}_e\in\pset^{\out}_{i,*}$ with $e^-$ as its last edge (recall that we view $u_i$ as the last endpoint of such a path), a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$;
\end{itemize}
such that each path of $\rset^*_{(i)}$ is assigned to exactly one path of $\hat \pset^{\thr}_i\cup \pset^{\out}_{i,*}$.
This completes the description of the $i$-th iteration.
See Figure~\ref{fig: inner_path} for an illustration.





\begin{figure}[h]
	\centering
	\subfigure[Layout of edges in $\delta(u_i)$: only the last/first edges of paths are shown. Here $\pset^{\out}_{*,i}=\set{P^{\out}_e \mid e\in E^{\lef}_{i}}$.]{\scalebox{0.32}{\includegraphics{figs/inner_path_1.jpg}}}
	\hspace{1pt}
	\subfigure[Sets $L^-_i, L^+_i,L^{\out}_i$ and the pairing (shown in dash pink lines) given by the algorithm in \Cref{obs:rerouting_matching_cong}.]{
		\scalebox{0.32}{\includegraphics{figs/inner_path_2.jpg}}}
	\caption{An illustration of an iteration in Step 3 of computing inner paths.}\label{fig: inner_path}
\end{figure}







Let $\pset$ be the set of paths that we obtain after $k-1$ iterations of processings vertices $u_1,\ldots,u_{k-1}$, and we rename the path $\hat P_e$ at the end of the algorithm by $P_e$, and say that $P_e$ is the inner path of $e$, for every edge $e\in E'$.
It is clear that $|\pset|=|E'|$. It is also easy to see from the algorithm that, for each edge $e\in E'$ connecting $C_i$ to $C_j$ (with $j\ge i+2$), the inner path $P_e$ starts at $u_i$ and ends at $u_j$ (as it is supposed to), and it contains, for each $i\le t\le j-1$, a path of $\rset^*_{(i)}$ as its $t$-th segment.
Therefore, path $P_e$ visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially.
%and for each pair $1\le i,j\le k$ with $j>i+1$, $\pset$ contains $p_{i,j}$ paths originating $u_i$ and terminating at $u_j$. 

The following observations are immediate from our algorithm of constructing the inner paths.
\begin{observation}
\label{obs: non_transversal_1}
For each $1\le i\le k-1$, if we denote, for each $e\in E_i^{\rig}$, by $R_e$ the path consisting of the last edge of path $P^{\out}_e$ and the first edge of path $P_e$, then the paths in $\set{P_e\mid e\in \bigcup_{ i'<i<j'}E(C_{i'},C_{j'})}$ and $\set{R_e\mid e\in E_i^{\rig}}$ are non-transversal at $u_i$.
\end{observation}

%It is also easy to see that the paths in $\pset$ are non-transversal with respect to $\Sigma$, which we show in the following observation.
\begin{observation}
\label{obs: non_transversal_2}
The inner paths in $\pset$ are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
On one hand, note that for each $1\le i\le k-1$, the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.
Since the $i$-th segments of paths in $\pset$ are paths in $\rset^*_{(i)}$, it follows that the paths of $\pset$ are non-transversal at all vertices of $V(G)\setminus\set{u_1,\ldots,u_k}$.
On the other hand, from the algorithm and \Cref{obs:rerouting_matching_cong}, it is easy to verify that the paths of $\pset$ are also non-transversal at $u_1,\ldots,u_k$.
\end{proof}

\begin{observation}
\label{obs: edge_occupation in outer and inner paths}
Each edge $e\in E'$ belongs to exactly one outer path and no inner paths, each edge of $\bigcup_{1\le i\le k-1}\hat E_i$ belongs to no outer paths and $O(1)$ inner paths; and each edge of $\bigcup_{1\le i\le k}E(C_i)$ belongs to no outer paths and $O(\cong_G(\qset_i,e))$ inner paths.
\end{observation}

%Finally we designate, for each edge $e\in \inE(\cset)$, a distinct path of $\pset^*$ that connects $u_i$ to $u_j$, that we denote by $P^*_e$, as its \emph{representative} path. 


%Note that we will not compute a drawing of $G'$, we only use the non-transversal paths and their relative ordering in $G'$ to help define disengaged instance of $G$.



%Denote by $\oset^*_{i}$ the ordering of paths in $\pset^*$ that contains $u_i$, defined by the rotation $\oset'_{v_i}\in \Sigma'$ at $v$.\znote{To elaborate.}Note that $\oset^*_{i}$ is also an ordering on the edges of $\bigcup_{j_1\le i\le j_2}E'_{j_1,j_2}$.



\subsubsection{Construct Sub-Instances}
\label{sec: disengaged instances}


%\znote{$E_i^{\rig}$, $E_i^{\lef}$ and  $E^{\thr}_i$ are distinct from previous sections. to be coordinated later}

%We are now ready to construct the disengaged instances.
Recall that $\cset=\set{C_1,\ldots,C_k}$.
In this subsection we will construct, for each cluster $C_i\in \cset$, an sub-instance $I_i=(G_i,\Sigma_i)$ of $(G,\Sigma)$, such that the instances $\iset=\set{I_1,\ldots,I_k}$ satisfy the properties in \Cref{lem: path case}.
%We start with some definitions. 
For each $1\le i\le k$, recall that $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$. We denote $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$.

%We will use the instance $(G',\Sigma')$.For each $1\le i\le k$, the rotation $\oset'_{u_i}\in \Sigma'$ at vertex $u_i$ is an cyclic ordering on edges of $\delta_{G'}(u_i)$. Denote by $F^{\lef}_{i}$ the set of edges in $\delta_{G'}(u_i)$ that serves as the last edge of a path of $\pset^*_{(i-1)}$, and denote by $F^{\rig}_{i}$ the set of edges in $\delta_{G'}(u_i)$ that serves as the first edge of a path of $\pset^*_{(i)}$. We denote by $\oset^{\lef}_i$ the ordering on $F^{\lef}_{i}$ induced by $\oset'_{u_i}$, and we denote by $\oset^{\rig}_i$ the ordering on $F^{\rig}_{i}$ induced by $\oset'_{u_i}$. As there is an one-to-one correspondence between edges in $F^{\lef}_{i}$ and paths in $\pset^*_{(i-1)}$, we also say that $\oset^{\lef}_i$ is an ordering on the set $\pset^*_{(i-1)}$ of paths. We prove the following claim.
\iffalse
\begin{claim}
\label{clm: rotation_distance}
There exist integers $b_1,\ldots,b_k\in \set{0,1}$, such that $\sum_{1\le i\le k-1}\dist((\oset^{\rig}_i,b_i), (\oset^{\lef}_{i+1},b_{i+1}))\le O(\optcrors(G',\Sigma')\cdot\poly\log n)$.
\end{claim}
\begin{proof}
\end{proof}
\fi

\iffalse
We first construct instance $(G_k,\Sigma_k)$ as follows.
The graph $G_k$ is obtained from $G$ by contracting all vertices in $G\setminus C_k$ into a single vertex, that we denote by $v^{\lef}_k$. 
Notice that the edges incident to $v^{\lef}_k$ correspond to the edges of $\delta(C_k)$.
The ordering of a vertex of $v\ne v^{\lef}_k$ in $\Sigma_k$ is identical to the ordering $\oset_v$ of $v$ in the given rotation system $\Sigma$.
Note that $\delta_{G_k}(v^{\lef}_k)=\delta_G(C_k)=\delta_H(u_k)$, 
and there is an one-to-one correspondence between edges in $\delta_H(u_k)$ and paths in $\pset^*_{(i-1)}$.
The ordering of the vertex $v^{\lef}_k$ in $\Sigma_k$ is then defined to be $\oset^{\rig}_{k-1}$ (which is an ordering on the set $\pset^*_{(i-1)}$, and is therefore also an ordering on $\delta_{G_k}(v^{\lef}_k)$).

The instance $(G_1,\Sigma_1)$ is defined similarly. 
The graph $G_1$ is obtained from $G$ by contracting all vertices in $G\setminus C_1$ into a single vertex, that we denote by $v^{\rig}_1$. 
We will not distinguish between edges incident to $v^{\lef}_1$ and edges of $\delta(C_k)$. 
The ordering of a vertex $v\ne v^{\rig}_1$ in $\Sigma_1$ is identical to the ordering $\oset_v$ in $\Sigma$.
Note that $\delta_{G_1}(v^{\rig}_1)=\delta_G(C_1)=\delta_H(u_1)$, 
and there is an one-to-one correspondence between edges in $\delta_H(u_1)$ and paths in $\pset^*_{(1)}$.
The ordering of the vertex $v^{\rig}_1$ in $\Sigma_1$ is then defined to be $\oset^{\lef}_2$ (which is an ordering on the set $\pset^*_{(1)}$, and is therefore also an ordering on $\delta_{G_1}(v^{\rig}_1)$).
\fi

\paragraph{Instances $(G_2,\Sigma_2),\ldots,(G_{k-1},\Sigma_{k-1})$.}
We first fix some index $2\le i\le k-1$ and define the instance $(G_i,\Sigma_i)$ as follows.
The graph $G_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_i$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_i$, and finally deleting self-loops on super-nodes $v^{\lef}_i$ and $v^{\rig}_i$. So $V(G_i)=V(C_i)\cup \set{ v^{\lef}_i,v^{\rig}_i}$. See \Cref{fig: disengaged instance} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}$ and $E^{\rig}_{i}$ are shown in green. Edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.32}{\includegraphics{figs/disengaged_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{1pt}
	\subfigure[Graph $G_i$. The edges incident to $v_i^{\rig}$ are $\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$,  and the edges incident to $v_i^{\lef}$ are $\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.32}{\includegraphics{figs/disengaged_instance_2.jpg}}}
	\caption{An illustration of the disengaged instance.}\label{fig: disengaged instance}
\end{figure}

The ordering on the incident edges of a vertex $v\in V(C_i)$ in $\Sigma_i$ is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the orderings on the incident edges of super-nodes $v^{\lef}_i,v^{\rig}_i$. 
We first consider the super-node $v^{\lef}_i$.
Note that $\delta_{G_i}(v^{\lef}_i)=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e\in \hat E_{i-1}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ connecting $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\thr}_i\cup E^{\lef}_i$ that connects a vertex of $C_{i'}$ to a vertex of $C_{j'}$ with $i'<i<j'$, we denote by $W_e$ the path obtained by concatenating
(i) the subpath of $P^{\out}_e$ between (including) edge $e$ and its last endpoint $u_{i'}$; and
(ii) the subpath of $P_e$ between its first endpoint $u_{i'}$ and the vertex $u_{i-1}$.
Clearly, the path $W_e$ defined above connects $e$ to $u_{i-1}$.
We denote $\wset^{\lef}_i=\set{W_e\mid e\in E^{\thr}_i\cup E^{\lef}_i}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E_{i-1}}$, and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.
Intuitively, the rotation $\oset^{\lef}_i$ is the ordering in which the paths in $\wset^{\lef}_i$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_i$, let $e^*_W$ be the last edge lying on path $W$, that must belong to $\delta_{G}(u_{i-1})$. We first define a circular ordering of the paths in $\wset^{\lef}_i$, as follows: the paths are ordered according to the circular ordering of their last edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_i$ is associated with a unique edge in $\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$, that serves as the first edge on path $W$, this ordering of the paths in $\wset^{\lef}_i$ immediately defines a circular ordering of the edges of $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$, that we denote by $\oset^{\lef}_i$. See Figure~\ref{fig: v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i-1}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\lef}_{i}=\set{e^g_1,e^g_2}$ and $E^{\thr}_{i}=\set{e^r_1,e^r_2}$.
	Paths of $\wset^{\lef}_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.36}{\includegraphics{figs/rotation_left_1.jpg}}}
	\hspace{1pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\lef}_i)$ and the rotation $\oset^{\lef}_i$. $\delta_{G_i}(v^{\lef}_i)=\set{\hat e_1,\hat e_2,\hat e_3,\hat e_4,e^g_1,e^g_2, e^r_1,e^r_2}$, and the rotation $\oset^{\lef}_i$ on them around $v^{\lef}_i$ is shown above.]{
		\scalebox{0.28}{\includegraphics{figs/rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{i}$ on vertex $v^{\rig}_i$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e'\in \hat E_{i}$, recall that $Q_{i}(\hat e')$ is the path in $C_{i}$ connecting $\hat e'$ to $u_{i}$.
For each edge $e\in E^{\thr}_i\cup E^{\rig}_i$ that connects a vertex of $C_{i'}$ to a vertex of $C_{j'}$ with $i'\le i<j'$, we denote by $W_e$ the path obtained by concatenating
(i) the subpath of $P^{\out}_e$ between (including) edge $e$ and its last endpoint $u_{i'}$; and
(ii) the subpath of $P_e$ between its first endpoint $u_{i'}$ and vertex $u_{i}$ (note that for an edge $e\in E^{\rig}_{i}$, such a subpath only contains a single node $u_i$).
Clearly, the path $W_e$ defined above connects $e$ to $u_{i}$.
We denote $\wset^{\rig}_i=\set{W_e\text{ }\big|\text{ } e\in E^{\thr}_i\cup E^{\rig}_i}\cup \set{Q_{i}(\hat e')\text{ }\big|\text{ }  \hat e'\in \hat E_{i}}$.
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}$.
See Figure~\ref{fig: v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i}=\set{\hat e_1',\ldots,\hat e_4'}$, $E^{\lef}_{i}=\set{\tilde e^g_1,\tilde e^g_2}$ and $E^{\thr}_{i}=\set{e^r_1,e^r_2}$.
	Paths of $\wset^{\rig}_i$ excluding their first edges are shown in dash lines. ]{\scalebox{0.36}{\includegraphics{figs/rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{1pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\rig}_i)$ and the rotation $\oset^{\lef}_i$. $\delta_{G_i}(v^{\rig}_i)=\set{\hat e_1',\hat e_2',\hat e_3',\hat e_4',\tilde e^g_1,\tilde e^g_2, e^r_1,e^r_2}$, and the rotation $\oset^{\rig}_i$ on them around $v^{\rig}_i$ is shown above.]{
		\scalebox{0.28}{\includegraphics{figs/rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_right rotation}
\end{figure}

\paragraph{Instances $(G_1,\Sigma_1)$ and $(G_k,\Sigma_k)$.}
The instances $(G_1,\Sigma_1)$ and $(G_k,\Sigma_k)$ are defined similarly, but instead of two super-nodes, the graphs $G_1$ and $G_k$ contain one super-node each.
In particular, graph $G_1$ is obtained from $G$ by contracting clusters $C_2,\ldots, C_k$ into a super-node, that we denote by $v^{\rig}_1$, and then deleting self-loops on it.
So $V(G_1)=V(C_1)\cup \set{v^{\rig}_{1}}$ and $\delta_{G_1}(v^{\rig}_{1})=\hat E_1\cup E^{\rig}_1$.
The rotation of a vertex $v\in V(C_1)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\rig}_1$ is defined in a similar way as $\oset^{\rig}_i$ for any index $2\le i\le k-1$.
 Graph $G_k$ is obtained from $G$ by contracting clusters $C_1,\ldots, C_{k-1}$ into a super-node, that we denote by $v^{\lef}_k$, and then deleting self-loops on it.
So $V(G_k)=V(C_k)\cup \set{v^{\lef}_{k}}$ and $\delta_{G_k}(v^{\lef}_{k})=\hat E_{k-1}\cup E^{\lef}_k$.
The rotation of a vertex $v\in V(C_k)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\lef}_k$ is defined in a similar way as $\oset^{\lef}_i$ for any index $2\le i\le k-1$.







We will use the following claims later for completing the proof of \Cref{lem: path case} in the special case where there is no problematic index $i$.

\begin{observation}
\label{obs: disengaged instance size}
$\sum_{1\le i\le k}|E(G_i)|= 2m$, and for each $1\le i\le k$, $|E(G_i)|\le m/\mu$.
\end{observation}
\begin{proof}
Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le k}$, each graph of $\set{G_i}_{1\le i\le k}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node. Therefore, each edge of $G_i$ corresponds to an edge in $E(G)$ (and we do not distinguish between them).
So we can write $E(G_i)=E_G(C_i)\cup E_G(C_i,\overline{C_i})$. 
Therefore, for each $1\le i\le k$, $|E(G_i)|=|E_G(C_i)|+|E_G(C_i,\overline{C_i})|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu$.
On the other hand, since clusters $C_1,\ldots,C_k$ are vertex-disjoint, every edge of $E(G)$ appears twice in the graphs $\set{G_i}_{1\le i\le k}$. It follows that $\sum_{1\le i\le k}|E(G_i)|= 2m$.
\end{proof}


\begin{observation}
\label{obs: rotation for stitching}
For each $1\le i\le k-1$, if we view edge sets $\delta_{G_i}(v^{\rig}_i),\delta_{G_{i+1}}(v^{\lef}_{i+1})$ as subsets of $E(G)$, then $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$, and
$\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{observation}
\begin{proof}
Recall that for each $1\le i\le k-1$, 
$\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})=\hat E_{i}\cup E^{\thr}_{i+1}\cup E^{\lef}_{i+1}$. From the definition of sets $E_i^{\thr},E_{i+1}^{\thr}, E^{\rig}_i, E^{\lef}_{i+1}$,
\[
\begin{split}
E_i^{\thr}\cup E^{\rig}_i
 = & \set{e\in E(C_{i'},C_{j'})\mid i'<i<j'\text{ or }i'=i<j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'\le i<j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'< i+1\le j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'<i+1<j'\text{ or }i'<i+1=j'}=E^{\thr}_{i+1}\cup E^{\lef}_{i+1}.
\end{split}
\]
Therefore, $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$.
Moreover, from the definition of path sets $\wset^{\rig}_i$ and $\wset^{\lef}_{i+1}$, it is not hard to verify that, for every edge $e\in \delta_{G_i}(v^{\rig}_i)$, the path in $\wset^{\rig}_i$ that contains $e$ as its first edge is identical to the path in $\wset^{\lef}_{i+1}$ that contains $e$ as its first edge. According to the way that rotations $\oset^{\rig}_i,\oset^{\lef}_{i+1}$ are defined, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{proof}




\subsubsection{Completing the Proof of \Cref{lem: path case} in the Special Case}
\label{sec: path case with no problematic index}

In this section we complete the proof of \Cref{lem: path case} in the special case where there is no problematic index. Specifically, we use the following two claims, whose proofs will be provided later.

\begin{claim}
	\label{claim: existence of good solutions special}
	$\sum_{1\le i\le k}\optcrors(G_i,\Sigma_i)\le O((\optcrors(G,\Sigma)+|E(G)|)\cdot \temp)$.
\end{claim}

\begin{claim}
\label{claim: stitching the drawings together}
There is an efficient algorithm, that given, for each $1\le i\le k$, a feasible solution $\phi_i$ to the instance $(G_i,\Sigma_i)$, computes a solution to the instance $(G,\Sigma)$, such that $\cro(\phi)\le \sum_{1\le i\le k}\cro(\phi_i)$.
\end{claim}

We use the algorithm described in~\Cref{sec: disengaged instances} and~\Cref{sec: inner and outer paths}, and return the disengaged instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$ as the collection of sub-instances of $(G,\Sigma)$. 
From the previous subsections, the algorithm for producing the sub-instances is efficient.
On the other hand, it follows immediately from \Cref{obs: disengaged instance size}, \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together} that the sub-instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$ satisfy the properties in \Cref{lem: path case}.
This completes the proof of \Cref{lem: path case}.

We now provide the proofs of \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together}.

$\ $

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
We will construct, for each $1\le i\le k$, a drawing $\phi_i$ of $G_i$ that respects the rotation system $\Sigma_i$, based on the optimal drawing $\phi^*$ of the instance $(G,\Sigma)$, such that $\sum_{1\le i\le k}\cro(\phi_i)\le O((\cro(\phi^*)+|E(G)|)\cdot \temp)$. The \Cref{claim: existence of good solutions special} then follows.

\paragraph{Drawings $\phi_2,\ldots,\phi_{k-1}$.}
First we fix some index $2\le i\le k-1$, and describe the construction of the drawing $\phi_i$. We start with some definitions.
Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
We define the auxiliary path set $\wset_i=\wset^{\lef}_i\cup \wset^{\rig}_i$, so 
$$\wset_i=\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}\cup \set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}},$$
where for each $e\in E^{\lef}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$; for each $e\in E^{\rig}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between $u_{i+1}$ and its last endpoint; and for each $e\in E^{\thr}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$, the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$, and the subpath of $P_e$ between $u_{i+1}$ and its last endpoint.
We use the following observation.
\begin{observation}
	\label{obs: wset_i_non_interfering}
	The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
\end{proof}


For uniformity of notations, for each edge $\hat e\in \hat E_i$, we rename the path $Q_{i+1}(\hat e)$ by $W_{\hat e}$, and similarly for each edge $\hat e\in \hat E_{i-1}$, we rename the path $Q_{i-1}(\hat e)$ by $W_{\hat e}$. Therefore, $\wset_i=\set{W_e\mid e\in E(G_i)\setminus E(C_i)}$.
Put in other words, the set $\wset_i$ contains, for each edge $e$ in $G_i$ that is incident to $v^{\lef}_i$ or $v^{\rig}_i$, a path named $W_e$.
It is easy to see that all paths in $\wset_i$ are internally disjoint from $C_i$.
We further partition the set $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_e\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.

We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
Specifically, we proceed in the following four steps.



\paragraph{Step 1.}
For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
We denote by $\Pi_e$ the set of these curves.
We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.

%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
Therefore, $\hat{\chi}_i(P)$ is well-defined.
For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.

\iffalse
We use the following observation.
\znote{maybe remove this observation?}

%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.

\begin{observation}
\label{obs: curves_crossings}
The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
\end{observation}
\begin{proof}
We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.

We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
\end{proof}
\fi

\paragraph{Step 2.}
For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
\iffalse{just for backup}
\begin{proof}
	Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
	For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
	We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
	It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
	We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
	See Figure~\ref{fig: curve_con} for an illustration.
	Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
	It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
	Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
	Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
	Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
\end{proof}
\begin{figure}[h]
	\centering
	\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
	\hspace{1pt}
	\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
		\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
	\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
\end{figure}
\fi

%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
We use the following observation.
\begin{observation}
\label{obs: general_position}
Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
\end{observation}
\begin{proof}
From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
\end{proof}




%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.


\paragraph{Step 3.} 
So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.


Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.





\paragraph{Step 4.}
Let $\dset$ be an arbitrarily small disc around $z_{\rig}$ in the drawing $\phi'_i$, and let $\dset'$ be another small disc around $z_{\rig}$ that is strictly contained in $\dset$.
We first erase the drawing of $\phi'_i$ inside the disc $\dset$, and for each edge $e\in \delta(v^{\rig}_i)$, we denote by $p_{e}$ the intersection between the curve representing the image of $e$ in $\phi'_i$ and the boundary of $\dset$.
We then place, for each edge $e\in \delta(v^{\rig}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{\rig}_{i}$. 
We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{\rig}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$.
Finally, for each edge $e\in \delta(v^{\rig}_i)$, let $\gamma_e$ be the concatenation of (i) the image of $e$ in $\phi'_i$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z_{\rig}$ in $\dset'$.
We view $\gamma_e$ as the image of edge $e$, for each $e\in \delta(v^{\rig}_i)$. 
We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$, and therefore it respects the rotation system $\Sigma_i$.

We use the following claim.
\begin{claim}
\label{clm: rerouting_crossings}
The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
\end{claim}
\begin{proof}
Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	
%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.

We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
\begin{figure}[h]
\centering
\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
\end{figure}
\end{proof}

From the above discussion and Claim~\ref{clm: rerouting_crossings}, for each $2\le i\le k-1$, 
\[
\cro(\phi_i)=\chi^2(C_i)+O\left(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right).
\]



\iffalse
We now estimate the number of crossings in $\phi_i$ in the next claim.
\begin{claim}
\label{clm: number of crossings in good solutions}
$\cro(\phi_i)=\chi^2(C_i)+O\left(\sum_{W\in \tilde\wset_i}\cro(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)$.
\end{claim}
\begin{proof}
$2\cdot \sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2=\sum_{v\in V(G)}\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2.$
\znote{need to redefine the orderings $\oset^{\lef}_i$ and $\oset^{\rig}_i$ to get rid of $\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2$ here, which we may not be able to afford.}
\end{proof}
\fi


\paragraph{Drawings $\phi_1$ and $\phi_{k}$.}
The drawings $\phi_1$ and $\phi_{k}$ are constructed similarly. We describe the construction of $\phi_1$, and the construction of $\phi_1$ is symmetric.
Recall that the graph $G_1$ contains only one super-node $v_1^{\rig}$, and $\delta_{G_1}(v_1^{\rig})=\hat E_1\cup E^{\rig}_1$. We define $\wset_1=\set{W_e\mid e\in E^{\rig}_1}\cup \set{Q_2(\hat e)\mid \hat e\in \hat E_1}$. For each $\hat e\in \hat E_1$, we rename the path $Q_2(\hat e)$ by $W_e$, so $\wset_1$ contains, for each edge $e\in \delta_{G_1}(v^1_{\rig})$, a path named $W_e$ connecting its endpoints to $u_2$. Via similar analysis in \Cref{obs: wset_i_non_interfering}, it is easy to show that the paths in $\wset_1$ are non-transversal with respect to $\Sigma$.

We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{k-1}$. 
We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{k-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]




We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le k}\cro(\phi_i)$.
Recall that, for each $1\le i\le k$, $\tilde \wset_i=\set{W_e\mid e\in \hat E_{i-1}\cup \hat E_{i-1}\cup E^{\lef}_{i}\cup E^{\rig}_{i}}$, where $E^{\lef}_{i}=E(C_i,\bigcup_{1\le j\le i-2}C_j)$, and 
$E^{\rig}_{i}=E(C_i,\bigcup_{i+2\le j\le k}C_j)$. Therefore, for each edge $e\in E'\cup (\bigcup_{1\le i\le k-1}\hat E_i)$, the path $W_e$ belongs to exactly $2$ sets of $\set{\tilde\wset_i}_{1\le i\le k}$.
Recall that the path $W_e$ only uses edges of the inner path $P_e$ and the outer path $P^{\out}_e$.
Let $\tilde\wset=\bigcup_{1\le i\le k}\tilde\wset_i$, from \Cref{obs: edge_occupation in outer and inner paths}, 
for each edge $e\in E'\cup (\bigcup_{1\le i\le k-1}\hat E_i)$, $\cong_G(\tilde\wset,e)=O(1)$, and
for $1\le i\le k$ and for each edge $e\in E(C_i)$, $\cong_G(\tilde\wset,e)=O(\cong_G(\qset_i,e))$.

Therefore, on one hand,
\[
\begin{split}
\sum_{1\le i\le k}\sum_{W\in \tilde\wset_i}\hat\chi_i(W)
& \le 
\sum_{(e,e'): e,e'\text{ cross in }\phi^*} 2\cdot \cong_G(\tilde \wset,e)\cdot\cong_G(\tilde \wset,e')\\
& \le 
\sum_{(e,e'): e,e'\text{ cross in }\phi^*} \left(\cong_G(\tilde \wset,e)^2+\cong_G(\tilde \wset,e')^2\right)\\
& \le 
\sum_{e\in E(G)} \chi(e)\cdot \cong_G(\tilde \wset,e)^2
= O(\cro(\phi^*)\cdot\temp),
\end{split}
\]
and on the other hand,
\[
\begin{split}
\sum_{1\le i\le k}\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2
%= \sum_{e\in E(G)} \sum_{1\le i\le k} \cong_G(\tilde \wset_i,e)^2 
& \le  \sum_{e\in E(G)} \left(\sum_{1\le i\le k} \cong_G(\tilde \wset_i,e)\right)^2\\
& \le O\left(\sum_{e\in E(G)} \cong_G(\tilde \wset,e)^2 \right)\\
& \le O\left(|E(G)|+\sum_{1\le i\le k}\sum_{e\in E(C_i)} \cong_G(\qset_i,e)^2\right)=O(|E(G)|\cdot\temp).
\end{split}
\]
Moreover, $\sum_{1\le i\le k}\chi^2(C_i)\le O(\cro(\phi^*))$, and $\sum_{1\le i\le k}\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})\le O(\cro(\phi^*)\cdot\temp)$.

Altogether,
\[
\begin{split}
\sum_{1\le i\le k}\cro(\phi_i)
& \le 
O\left(\sum_{1\le i\le k} 
\left(
\chi^2(C_i)+ \hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)
\right)\\
& \le O(\cro(\phi^*))+O(\cro(\phi^*)\cdot\temp)+O(\cro(\phi^*)\cdot\temp)+O(|E(G)|\cdot\temp)\\
& \le O((\cro(\phi^*)+|E(G)|)\cdot\temp).
\end{split}
\]

This completes the proof of \Cref{claim: existence of good solutions special}.
\end{proofof}






$\ $



\iffalse
We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

We first define an instance $(\hat G_i,\hat\Sigma_i)$ as follows. We start with the subgraph of $G$ induced by all edges of $E_G(C_i)$ and $E(\wset_i)$, and then create, for each edge $e$ in the subgraph, $\cong_{\wset_i}(e)$ parallel copies of it. This finishes the description of graph $\hat G_i$.
For each vertex $v$ in $\hat G_i$, we define its rotation $\hat\oset_v$ as follows. We start with the rotation $\oset_v\in \Sigma$, and then replace, for each edge $e\in E(\wset_i)$, the edge $e$ in the ordering $\oset_v$ by its $\cong_{\wset_i}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, where the ordering among the copies is arbitrary. 
On the one hand, in graph $\hat G_i$, we can make paths of $\wset_i$ edge-disjoint by letting, for each edge $e\in E(\wset_i)$, each path of $\wset_i$ that contains $e$ now take a distinct copy of $e$ in $\hat G_i$.
On the other hand, a drawing $\hat \phi_i$ of the instance $(\hat G_i,\hat\Sigma_i)$ can be easily computed from $\phi^*$, as follows.
We start with $\hat\phi'_i$, the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$. Then for each edge of $\wset_i$, let $\gamma_e$ be the curve that represents the image of $e$, and we create $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting endpoints of $e$, that lies in an arbitrarily thin strip around $\gamma_e$. We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

For each edge $e\in E_G(C_i)$, we denote by $\gamma_e$ the curve in $\hat \phi_i$ that represents the image of $e$; and for each path $W\in \wset_i$, we denote by $\gamma_W$ the curve in $\hat \phi_i$ that represents the image of $W$.
We define $\Gamma_0=\set{\gamma_e\mid e\in E_G(C_i)}$ and $\Gamma_1=\set{\gamma_W\mid W\in \wset_i}$. It is immediate to verify that the sets $\Gamma_0,\Gamma_1$ of curves satisfy the condition of \Cref{thm: type-2 uncrossing}. We then apply the algorithm in \Cref{thm: type-2 uncrossing} to $\Gamma_0,\Gamma_1$, and let $\Gamma_1'$ be the set of curves that we obtain.
From \Cref{thm: type-2 uncrossing}, the curves in $\Gamma_1'$ do not intersect internally between each other, and have the same sets of first endpoints and last endpoints.
We now show that we can obtain a drawing $\phi_i$ of the instance $(G_i,\Sigma_i)$ using the curves $\Gamma_0,\Gamma_1'$.
For each edge $e\in E_G(C_i)$, we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
For each edge path $W\in \wset$, from \Cref{thm: type-2 uncrossing}, there is a curve $\gamma'\in \Gamma_1'$ connecting the endpoint of $W$ to we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
\znote{maybe we need another type of uncrossing here.}
\fi



\begin{proofof}{Claim~\ref{claim: stitching the drawings together}}
We first define a set $\set{(U_i,\Sigma'_i)\mid 1\le i\le k}$ of instances of \CNwRS as follows.
We define $U_1=G$, and for each $2\le i\le k$, we define $U_i$ to be the graph obtained from $G$ by contracting the clusters $C_1,\ldots, C_{i-1}$ into a vertex $v^{\lef}_i$.
Note that each edge in $U_i$ is also an edge in $G$, and we do not distinguish between them.
Note that $U_1=G$, we define the rotation system $\Sigma'_1$ on $U_1$ to be $\Sigma$.
For each $2\le i\le k$, we define the rotation system $\Sigma'_i$ on $U_i$ as follows.
For each vertex $v\in \bigcup_{i\le t\le k}V(C_t)$, note that its incident edges in $U_i$ are the edges of $\delta_G(v)$, and its rotation in $\Sigma'_i$ is defined to be $\oset_v$, the rotation on $v$ in the input rotation system $\Sigma$.
For vertex $v^{\lef}_i$, note that its incident edges are the edges of $\delta_{G_i}(v^{\lef}_i)$, and its rotation in $\Sigma'_i$ is defined to be $\oset^{\lef}_i$, the rotation on $v^{\lef}_i$ of instance $(G_i,\Sigma_i)$.


Note that $U_k=G_k$ and $\Sigma'_k=\Sigma_k$, so the drawing $\phi_k$ of the instance $(G_k,\Sigma_k)$ is also a drawing of the instance $(U_k,\Sigma'_k)$. For clarity, when we view this drawing as a solution to the instance $(U_k,\Sigma'_k)$, we rename it by $\psi_k$.
We will sequentially, for $i=k-1,\ldots,1$, compute a drawing of the instance $(U_i,\Sigma'_i)$ using the drawing $\psi_{i+1}$ of $(U_{i+1},\Sigma'_{i+1})$ and the drawing $\phi_i$ of $(G_{i},\Sigma_{i})$, and eventually, we return the drawing $\psi_1$ of $(U_{1},\Sigma'_{1})$ as the solution to the instance $(G,\Sigma)$.

We now fix an index $1\le  i< k-1$ and construct the drawing $\psi_i$ to the instance $(U_{i},\Sigma'_{i})$, assuming that we have computed a drawing $\psi_{i+1}$ to the instance $(U_{i+1},\Sigma'_{i+1})$, as follows.
Recall that $V(G_i)=V(C_i)\cup\set{v^{\lef}_i,v^{\rig}_i}$ if $i\ge 2$ and $V(G_i)=V(C_i)\cup\set{v^{\rig}_i}$ if $i=1$, and $\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.  Moreover, from \Cref{obs: rotation for stitching} and the definition of instance $(U_{i+1},\Sigma'_{i+1})$, the rotation on $v^{\rig}_i$ in $\Sigma_{i}$ is identical to the rotation on $v^{\lef}_{i+1}$ in $\Sigma'_{i+1}$.
Denote $F=\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.
Let $\dset$ be an arbitrarily small disc around the image of $v_{i+1}^{\lef}$ in $\psi_{i+1}$. For each edge $e\in F$, we denote by $p_e$ the intersection between the image of $e$ with the boundary of $\dset$. 
Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset$ is $\oset^{\lef}_{i+1}$.
We erase the drawing of $\psi_{i+1}$ inside the disc $\dset$, and view the area inside the disc $\dset$ as the outer face of the drawing.
Similarly, let $\dset'$ be an arbitrarily small disc around the image of $v_{i}^{\rig}$ in $\phi_{i}$. For each edge $e\in F$, we denote by $p'_e$ the intersection between the image of $e$ with the boundary of $\dset'$. 
Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is $\oset^{\rig}_{i}$.
We erase the drawing of $\phi_{i}$ inside the disc $\dset'$, and let $\dset''$ be another disc that is strictly contained in $\dset'$. We now place the drawing of $\psi_{i+1}$ inside $\dset'$ (after we erase part of it inside $\dset$), so that the boundary of $\dset$ in $\psi_{i+1}$ coincide with the boundary of $\dset''$ in $\phi_{i}$, while the interior of $\dset$ coincides with the exterior of $\dset''$. We then compute a set $\set{\zeta_e\mid e\in F}$ of curves lying in $\dset'\setminus \dset''$, where for each $e\in F$, the curve $\zeta_e$ connects $p'_e$ to $p_e$, such that all curves of $\set{\zeta_e\mid e\in F}$ are mutually disjoint. Note that this can be done since the order in which $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is identical to $\set{p'_e}_{e\in F}$ appear on the boundary of $\dset$.
We denote by $\psi_i$ the resulting drawing we obtained.
See Figure~\ref{fig: stitching} for an illustration.
Clearly, $\psi_i$ is a drawing of $U_i$ that respects $\Sigma'_i$ if we view, for each edge $e\in F$, the union of (i) the image of $e$ in $\phi_i$ outside the disc $\dset'$; (ii) the curve $\zeta_e$; and (iii) the image of $e$ in $\psi_{i+1}$ inside the disc $\dset''$, as the image of $e$.
\begin{figure}[h]
	\centering
	\subfigure[The drawing $\psi_{i+1}$, where the boundary of $\dset$ is shown in dash black.]{\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.45cm}
	\subfigure[The drawing $\psi_{i+1}$ after we erase its part inside $\dset$ and view the interior of $\dset$ as the outer face.]{
		\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_2.jpg}}}
	\hspace{0.45cm}
	\subfigure[The drawing $\psi_i$, where the curves of $\set{\zeta_e\mid e\in F}$ are shown in dash line segments.]{
		\scalebox{0.36}{\includegraphics[scale=1.0]{figs/stitching_3.jpg}}}
	\caption{An illustration of an iteration in type-1 uncrossing.}\label{fig: stitching}
\end{figure}
Clearly, any crossing in the drawing $\psi_i$ is either a crossing of $\phi_i$ or a crossing of $\psi_{i+1}$, so $\cro(\psi_i)\le \cro(\psi_{i+1})+\cro(\phi_{i})$.
Therefore, if we rename the drawing $\psi_1$ of the instance $(U_1,\Sigma'_1)$ by $\phi$, then $\phi$ is a drawing of $G$ that respects $\Sigma$, and $\cro(\phi)\le \sum_{1\le i\le k}\cro(\phi_i)$.
\end{proofof}














==> disengage_path.tex <==
\subsection{Special Case: No Problematic Indices}
\label{subsec: no prob edges}



\mynote{A quick note that may be useful later. Suppose we have clusters $C_1,\ldots,C_r$ organized on a path, and there is no bad index. Suppose now we apply *basic disengagement* procedure (exactly as described in Sec 6.2) iteratively, first disengaging $C_1$, and getting graph $G_1$, where $C_1$ becomes a single vertex, then disengaging $C_2$ from $G_1$, and so on. As the result, instances that we obtain are *exactly* the instances created in this section, including the specific rotation around the two contracted vertices. This means that we don't need to worry about combining the solutions of the resulting instances together - the algorithm for basic disengagement does it (applying Lemma 6.3 as is). But the algorithm for basic disengagement won't give us the bound that we need on the total solution costs of the new instances (if we use Lemma 6.2 as is, the cost may be too high, because we'll be charging to same crossings again and again). This bound has to rely on the fact that we can route every edge connecting two non-consecutive clusters via a central path.
	One question that I'm wondering about is whether it is critical that, for an edge $e$ connecting $C_i$ to $C_j$, is routing path $P(e)$ has to go through the central path. I believe that there must be a portion of $P(e)$ between $C_i$ and $C_j$ that goes between the two clusters on a central path. But if before that it jumps to some clusters that lie before $C_i$ or after $C_j$ I think it does not matter to us. This may be good to understand because this may allow us to weaken the condition of "no bad index". If we decide to extend this algorithm to the case of a path-of-stars, this understanding may be helpful.}

In this subsection we show the proof of Lemma~\ref{lem: path case}, with the additional assumption that no index $i$ is problematic. That is, for each $1\le i\le k-1$, $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|\le 100|\hat E_i|$.
Recall that we are given, for each $1\le i\le k$, a vertex $u_i$ of $C_i$, and a set $\qset_i$ of paths in $C_i$ connecting the edges of $\delta(C_i)$ to $u_i$, such that for every edge $e\in E(C_i)$, $\mathbb{E}[\cong_{C_i}(\qset_i,e)^2]\le \temp$.
%\znote{assuming that $u_i$ and $\qset_i$ can be found in the decomposition step.}
%\znote{To set}

Recall that $\inE(\cset)$ is the set of edges connecting distinct clusters of $\cset$. 
We denote by $E'$ the subset of edges in $\inE(\cset)$ connecting a pair $C_i,C_j$ of clusters of $\cset$, with $j\ge i+2$.
%For each $1\le i\le k$, we denote $E_i=E(C_i,C_{i+1})$.
Therefore, $E(G)=E'\cup\left(\bigcup_{1\le i\le k-1}\hat E_i\right)\cup \left(\bigcup_{1\le i\le k}E(C_i)\right)$.
Recall that $H=G_{|\cset}$, and the node in $H$ that represents the cluster $C_i$ in $G$ is denoted by $x_i$.
Therefore, each edge in $E'\cup \left(\bigcup_{1\le i\le k-1}\hat E_i\right)$ corresponds to an edge in $H$, and we do not distinguish between them. 


We now start to describe the algorithm that construct the sub-instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$.
The algorithm proceeds in two stages. In the first stage, we compute, for each edge of $E'$, two auxiliary paths in $G$, that we call its \emph{inner path} and \emph{outer path} respectively. In the second stage, we use these auxiliary paths to define the sub-instances and show that they satisfy the properties of \Cref{lem: path case}.
In the remainder of this section, we describe the first stage in \Cref{sec: inner and outer paths} and the second stage in \Cref{sec: disengaged instances}, and then complete the proof of \Cref{lem: path case} in \Cref{sec: path case with no problematic index}.




\subsubsection{Compute Inner and Outer Paths}
\label{sec: inner and outer paths}


In the first stage, we will compute, for each pair $i,j$ of indices (with $i\le j-2$) and for each edge $e\in E'$ that connects a vertex of $C_i$ to a vertex of $C_j$, a path $P_e$ connecting $u_i$ to $u_j$ that only uses edges of $\bigcup_{i\le t\le j-1}\hat E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$, and a path $P^{\out}_e$ connecting $u_i$ to $u_j$ that only uses edge $e$ and edges of $E(C_i)\cup E(C_j)$. We call path $P_e$ the \emph{inner path} of $e$ and path $P^{\out}_e$ the \emph{outer path} of $e$.

We first compute the outer paths. Let $e$ be an edge of $E'$ connecting a vertex of $C_i$ to a vertex of $C_j$, so $e\in \delta(C_i)$ and $e\in \delta(C_j)$. Recall that the set $\qset_i$ contains a path $Q_i(e)$, connecting $e$ to $u_i$, and the set $\qset_j$ contains a path $Q_j(e)$, connecting $e$ to $u_j$.
We simply define its outer path $P^{\out}_e$ to be the union of path $Q_i(e)$ and path $Q_j(e)$.
It is clear that path $P^{\out}_e$ connects $u_i$ to $u_j$, and only uses edge $e$ and edges of $E(C_i)\cup E(C_j)$.
Throughout the section, we view $u_j$ as the first endpoint of $P^{\out}_e$ and $u_i$ as its last endpoint. We denote $\pset^{\out}=\set{P_e^{\out}\mid e\in E'}$, and for each $1\le i\le k$, we denote $\pset^{\out}_{*,i}=\set{P^{\out}_e \mid e\in E^{\lef}_{i}}$ and $\pset^{\out}_{i,*}=\set{P^{\out}_e \mid e\in E^{\rig}_{i}}$.
%\znote{notation to be coordinated}

We now compute the set $\pset=\set{P_e}_{e\in E'}$ of inner paths in three steps. In the first step, we compute a set $\tilde \pset$ of paths in $H$. In the second step, we transform the set $\tilde \pset$ of paths in $H$ into a set $\pset^*$ of paths in $G$.
In the third step, we further process paths in $\pset^*$ to obtain the set $\pset$ of inner paths for edges of $E'$.
We now describe each step in more details.

\paragraph{Step 1.}
In this step we process edges in $E'$ one-by-one. Throughout, for each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, we maintain an integer $z_{\hat e}$ indicating how many times the edge $\hat e$ has been used, that is initialized to be $0$. 
%Throughout, all edges of $\in \bigcup_{1\le i\le k-1}\hat E_i$ are either marked \emph{used} or \emph{not used}. Initially, all edges are not used.
Consider an iteration of processing an edge $e\in E'$. Assume $e$ connects $C_i$ to $C_j$ in $G$, we then pick, for each $i\le t\le j-1$, an edge $\hat e$ of $\hat E_t$ with minimum $z_{\hat e}$ over all edges of $\hat E_t$, and let $\tilde P_e$ be the path obtained by taking the union of all picked edges.
Note that, in $H$, each edge of $\hat E_t$ connects $x_t$ to $x_{t+1}$, so the path $\tilde P_e$ sequentially visits nodes $x_i, x_{i+1},\dots,x_j$. 
We then increase the value of $z_{\hat e}$ by $1$ for all picked edges $\hat e$, and proceed to the next iteration. After processing all edges of $E'$, we obtain a set $\tilde\pset=\set{\tilde P_e}_{e\in E'}$ of paths in $H$.
%{\color{red} We further assume that, for each $1\le i\le k$, $|E(S_i,\overline{S_i})|\le \beta\cdot |E_i|$, where we can think of $\beta=\poly\log n$.}
We use the following observation.

\begin{observation}
\label{obs:central_congestion}
For each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, $\cong_{H}(\tilde\pset,\hat e)\le 100$.
%The paths in $\tilde\pset$ are edge-disjoint.
\end{observation}
\begin{proof}
	%For each $1\le i\le k-1$, we denote by $E^*_i$ as the set of edges in $E'$ that connects a vertex of $\set{v_1,\ldots,v_{i-1}}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$, we denote by $E^{\lef}_i$ as the set of edges in $E'$ that connects $v_{i+1}$ to a vertex of $\set{v_1,\ldots,v_{i-1}}$, and we denote $E^{\rig}_i$ as the set of edges in $E'$ that connects $v_{i}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$.
	From the algorithm, for each $1\le i\le k-1$, the paths of $\tilde\pset$ that contains an edge of $\hat E_i$ are $\set{\tilde P_e\mid e\in \big(E_i^{\rig} \cup E_{i+1}^{\lef} \cup E_i^{\through}\big)}$.
	Since $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|\le 100|\hat E_i|$, each edge of $\hat E_i$ is used is used at most $100$ times. Observation~\ref{obs:central_congestion} then follows.
\end{proof}

\iffalse
We now further process the set $\tilde\pset$ of paths to obtain another set $\tilde\pset'$ of paths with some additional properties, as follows.

\paragraph{Step 2.1.} Let $\tilde G'$ be the graph obtained from $\tilde G$ by replacing each edge $e$ with $\beta$ parallel copies $e_1,\ldots,e_\beta$ connecting its endpoints. Now for each path $\tilde P\in \tilde{\pset}$, we define a path $\tilde P^*$ as the union of, for each edge $e\in \tilde P$, a copy $e_t$ of $e$, such that, for all paths of $\tilde\pset$ that contains the edge $e$, their corresponding paths in $\set{\tilde P^*\mid e\in \tilde P}$ contain distinct copies of $e$. We denote $\tilde\pset^*=\set{\tilde P^*\mid \tilde P\in \tilde \pset}$. From the above discussion, the paths of $\tilde\pset^*$ are edge-disjoint.
\fi

\paragraph{Step 2.}
In this step we compute a set $\pset^*$ of paths in $G$, using the paths in $\tilde\pset$ and path sets $\set{\qset_i}_{1\le i\le k}$, as follows.
Recall that the set $\qset_i$ contains, for each edge $e\in\delta(C_i)$, a path $Q_i(e)$ connecting $e$ to $u_i$.
Also recall that, in graph $G$, an edge $\hat e\in \hat E_i$ belongs to both $\delta(C_i)$ and $\delta(C_{i+1})$.
Therefore, for an edge $\hat e\in \hat E_i$, the union of path $Q_i(\hat e)$ and path $Q_{i-1}(\hat e)$ is a path connecting $u_i$ to $u_{i+1}$.
Now consider an edge $e\in E'$ connecting a vertex of $C_i$ to a vertex of $C_{j}$ (with $i\le j-2$), and the corresponding path $\tilde P_e=(\hat e_i,\hat e_{i+1},\ldots,\hat e_{j-1})$ in $\tilde\pset$, where $\hat e_t\in \hat E_t$ for each $i\le t\le j-1$. We define the path $P^*_e$ as the sequential concatenation of paths $Q_{i}(\hat e_i)\cup Q_{i+1}(\hat e_i), Q_{i+1}(\hat e_{i+1})\cup Q_{i+2}(\hat e_{i+1}),\ldots,Q_{j-1}(\hat e_{j-1})\cup Q_{j}(\hat e_{j-1})$.
It is clear that path $P^*_e$ only contains edges of $\bigcup_{i\le t\le j-1}\hat E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$, and sequentially visits vertices $u_i,u_{i+1},\ldots,u_{j}$.
Denote $\pset^*=\set{P^*_e\mid e\in E'}$.
From Observation~\ref{obs:central_congestion}, it is easy to see that for each edge $e\in \bigcup_{1\le i\le k}E(C_i)$, $\cong_{G}(\pset^*,e)\le 100\cdot\cong_{G}(\qset_i,e)$.


%Recall that, for each $1\le i\le k$, the set $\qset_i$ of paths connects edges of $\delta(C_i)$ to $u_i$. Note that $\hat E_i\in \delta(C_i)$ and $\hat E_i\in \delta(C_{i+1})$. For each edge $e\in \hat E_i$, let $\hat Q_e$ be the path obtained by taking the union of the path in $\qset_i$ connecting $e$ to $u_i$, the edge $e$, and the path in $\qset_{i+1}$ connecting $e$ to $u_{i+1}$, so path $\hat Q_e$ connects $u_i$ to $u_{i+1}$. Denote $\hat\qset_i=\set{\hat Q_e\mid e\in \hat E_i}$, and denote $\hat\qset=\bigcup_{1\le i\le k-1}\hat\qset_i$.
\iffalse

It would be convenient to state our algorithm if the core paths of $\pset$ are edge-disjoint. 
For which, we construct another instance $(G',\Sigma')$ of \CNwRS, as follows. 
Denote $\qset=\bigcup_{1\le i\le k}\qset_i$.
We start with the instance $(G,\Sigma)$.
For each edge $e\in E(\qset)$, we replace $e$ with $2\cdot\cong_{\qset}(e)$ parallel copies.
For each edge $e\in E(\pset)\setminus E(\qset)$, we replace $e$ with $2$ parallel copies.
For each vertex $v$ such that $\delta(v)\cap E(\pset\cup\qset)= \emptyset$, we define its rotation $\oset'_v$ to be identical to the its rotation $\oset_v$ in $\Sigma$. 
For each vertex $v$ such that $\delta(v)\cap E(\pset\cup\qset)\ne \emptyset$, we define its rotation $\oset'_v$ as follows. We start with the rotation $\oset_v$, and then (i) replace, for each edge $e\in \delta(v)\cap E(\qset)$, the edge $e$ in the ordering $\oset_v$ by its $2\cdot\cong_{\qset}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, 
and the ordering among the copies is arbitrary; and
(ii) replace, for each edge $e\in \delta(v)\cap E(\pset)$, the edge $e$ in the ordering $\oset_v$ by its $2$ copies that appears consecutively at the location of $e$ in $\oset_v$, 
and the ordering among the copies is arbitrary. 


We use the following observation.
\begin{observation}
$\optcrors(G,\Sigma)\le \optcrors(G',\Sigma')\le O(\optcrors(G,\Sigma)\cdot\poly\log n)$. 
Moreover, given a drawing $\phi\in \Phi(G,\Sigma)$, we can efficiently compute a drawing $\phi'\in \Phi(G',\Sigma')$, with $\cro(\phi')\le O(\cro(\phi)\cdot\poly\log n)$. 
%given a drawing $\phi'\in \Phi(G',\Sigma')$, we can efficiently compute a drawing $\phi\in \Phi(G,\Sigma)$, with $\cro(\phi)\le\cro(\phi')$.
\end{observation}
\begin{proof}
\end{proof}

Now for each path $P\in \pset$, we define a path $P'$ in $G'$ as the union of, for each edge $e\in P$, a copy $e_t$ of $e$, such that for all paths of $\pset$ that contains the edge $e$, their corresponding paths in $\set{P'\mid P\in \pset, e\in P}$ contain distinct copies of $e$. We denote $\pset'=\set{P'\mid  P\in \pset}$. 
%We define the set $\qset'$ from $\hat\qset$ similarly. 
From the above discussion, the paths of $\pset'$ are edge-disjoint.
Moreover, note that $V(G)=V(G')$, and if a path $P\in \pset$ connects $u_i$ to $u_j$ in $G$, then the corresponding path $P'$ connects $u_i$ to $u_j$ in $G'$.
\fi


\paragraph{Step 3.}
In this step we further process paths in $\pset^*=\set{P^*_e\mid e\in E'}$ to obtain the set $\pset=\set{P_e\mid e\in E'}$ of inner paths for edges of $E'$.
\iffalse
\begin{itemize}
	\item $|\pset|=|\tilde\pset'|$;
	\item for each pair $1\le i,j\le k$, the number of paths in $\pset'$ connecting $u_i$ to $u_j$ is the same as that of $\pset^*$; and 
	\item the paths in $\pset^*$ are non-transversal with respect to $\Sigma'$.
\end{itemize}
\fi
For each path $P^*\in \pset^*$ connecting $u_i$ to $u_{j}$ (recall that such a path visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially), we define, for each $i\le t\le j-1$, the path $P^*_{(i)}$ to be the subpath of $P^*$ between $u_{i}$ and $u_{i+1}$. For each $1\le i\le k-1$, we denote $\pset^*_{(i)}=\set{P^*_{(i)}\text{ } \bigg|\text{ } u_i,u_{i+1}\in V(P^*),P^*\in \pset^*}$, so all paths in $\pset^*_{(i)}$ connects $u_i$ to $u_{i+1}$.
We then apply the algorithm in Lemma~\ref{lem: non_interfering_paths} to the set $\pset^*_{(i)}$ of paths, and obtain a set $\rset^*_{(i)}$ of $|\rset^*_{(i)}|=|\pset^*_{(i)}|$ paths connecting $u_i$ to $u_{i+1}$, such that for every $e\in E(G)$, $\cong_{G}(\rset^*_{(i)},e)\le \cong_{G}(\pset^*_{(i)},e)$, and the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.

%We use the following observation, whose proof appears in Appendix~\ref{apd: Proof of rerouting_matching_cong}.

%\znote{Need to rethink which definition to include for ``non-transversal".}



%We now construct the inner paths $\pset=\set{P_e\mid e\in E'}$ as follows.
We now re-organize the paths in sets $\rset^*_{(1)},\ldots, \rset^*_{(k-1)}$ to obtain the set $\pset$ of inner paths.
%We now construct the set $\pset^*$ of paths.
Note that, if we select, for each $i\le t\le j-1$, a path of $\rset^*_{(i)}$, then, by taking the union of them, we can obtain a path $\hat P$ connecting $u_i$ to $u_j$. 
We call the selected path of $\rset^*_{(t)}$ the \emph{$t$-th segment} of $\hat P$. Therefore, a path connecting $u_i$ to $u_j$ obtained in this way is the union of its $i$-th segment, its $(i+1)$-th segment, $\ldots$ , and its $(j-1)$-th segment.
We now incrementally construct the set $\pset$ of paths.
Intuitively, we will silmutaneously construct all paths of $\pset$ in $k-1$ iterations, where in the $i$-th iteration, we will determine the $i$-th segment of all paths in $\pset$.

%For each $1\le i<j\le k$, we denote by $p_{i,j}$ the number of paths in $\pset^*$ connecting $u_i$ to $u_j$. 
Throughout, we will maintain a set $\hat{\pset}=\set{\hat P_e\mid e\in E'}$ of paths, where each path $\hat P_e$ is indexed by an edge $e$ of $E'$. 
Assume that the edge $e$ connects a vertex of $C_i$ to a vertex of $C_j$ (with $j\ge i+2$), then the path $\hat P_e$ is supposed to originate at $u_i$ and terminate at $u_j$.
We call $u_i$ the \emph{destined origin} of $\hat P_e$ and call $u_i$ the \emph{destined terminal} of $\hat P_e$.
Initially, $\hat{\pset}$ contains $|E'|$ paths, and all paths in $\hat{\pset}$ contain no edge. 
%and for each $1\le i<j\le k$, there are $p_{i,j}$ paths of $\hat{\pset}$ whose destined origin is $u_i$ and destined terminal is $u_j$.
We will sequentially process vertices $u_1,\ldots,u_{k-1}$, and, for each $1\le i\le k-1$, upon processing vertex $u_i$, determine which path of $\rset^*_{(i)}$ serves as the $i$-th segment of which path of $\hat\pset$.

We now fix an index $1\le i\le k-1$ and describe the iteration of processing vertex $u_i$. The current set $\hat\pset$ of paths can be partitioned into four sets: set $\hat\pset^{o}_i$ contains all paths of $\hat\pset$ whose destined origin is $u_i$; set $\hat\pset^{t}_i$ contains all paths of $\hat\pset$ whose destined terminal is $u_i$; set $\hat\pset^{\thr}_i$ contains all paths whose destined origin is $u_{i'}$ for some index $i'<i$ and whose destined terminal is $u_{j'}$ for some index $j'>i$; and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ contains all other paths. 
Note that the paths in set $\hat\pset^{t}_i$ and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ do not contain an $i$-th segment, so in this iteration we will determine the $i$-th segment of paths in the sets $\hat\pset^{o}_i$ and $\hat\pset^{\thr}_i$.
%On one hand, notice that all paths in $\hat\pset^{t}_i$ already connects its destined origin to $u_i$, and we will not modify them anymore, since these paths are already completed.

Note that the paths in $\hat\pset^{o}_i$ currently contain no edge, %and we arbitrarily designate, for each path in $\hat\pset^{o}_i$, a distinct path of $\pset^*_{(i)}$ as its $i$-th segment.
and the paths in $\hat\pset^{\thr}_i$ currently contain up to its $(i-1)$-th segment. 
%and in this iteration we will designate paths of $\pset^*_{(i)}$ as their $i$-th segments, as follows. 
We then denote
\begin{itemize}
\item by $L^-_i$ the multi-set of the current last edges of paths in $\hat\pset^{\thr}_i$;
\item by $L^+_i$ the multi-set of the first edges of paths in $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of any path in $\hat{\pset}$); and
\item by $L^{\out}_i$ the multi-set of last edges of paths in  $\pset^{\out}_{i,*}=\set{P^{\out}_e \mid e\in E^{\rig}_i}$.
\end{itemize} 
%$L^-_i$ the multi-set of edges of $\delta(u_i)$ that currently serves as the last edge of paths in $\hat\pset^{\thr}_i$, denote by $L^+_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of to any path in $\hat{\pset}$), and denote by $L^{\out}_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\set{P^{\out}_e \mid e\in E(C_i,C_j)\text{ for some }j>i+1}$.
%It is clear that $R^-_i, R^+_i$ are two disjoint subsets of $\delta(u_i)$ with $|R^-_i|=|R^+_i|$. 
Clearly, elements in sets $L^-_i, L^+_i,L^{\out}_i$ are edges of $\delta(u_i)$. 
We then define, for each $e\in \delta(u_i)$, $n^-_e=n_{L^-_i}(e)+n_{L^{\out}_i}(e)$ and
$n^+_e=n_{L^+_i}(e)$.
%\znote{see new notations in prelim (second paragraph in \Cref{sec:prelim})}
We use the following simple observation.
\begin{observation}
For each edge $e\in \delta(u_i)$, $\sum_{e\in \delta(u_i)}n^-_e=\sum_{e\in \delta(u_i)}n^+_e$.
\end{observation}
\begin{proof}
On one hand, $\sum_{e\in \delta(u_i)}n_{L^{\out}_i}(e)=|\bigcup_{j>i+1}E(C_i,C_j)|=|\hat\pset^{o}_i|$, and $\sum_{e\in \delta(u_i)}n_{L^{-}_i}(e)=|L^-_i|=|\hat\pset^{\thr}_i|$. 
On the other hand, recall that $|\rset^*_{(i)}|=|\pset^*_{(i)}|$, $\pset^*_{(i)}=\set{P^*_{(i)}\text{ } \bigg|\text{ } u_i,u_{i+1}\in V(P^*),P^*\in \pset^*}$ and the only edges in $E'$ such that path $P^*_e$ contains vertices $u_i,u_{i+1}$ are edges of $E^{\thr}_i\cup E^{\rig}_i$. Therefore,
$\sum_{e\in \delta(u_i)}n_{L^{+}_i}(e)=|L^+_i|=|\rset^*_{(i)}|=|\pset^*_{(i)}|=|E^{\thr}_i|+|E^{\rig}_i|=|\hat\pset^{\thr}_i|+|\hat\pset^{o}_i|$.
\end{proof}

We apply the algorithm in \Cref{obs:rerouting_matching_cong} to graph $G$, vertex $u_i$, rotation $\oset_{u_i}$ and integers $\set{n^-_e,n^+_{e}}_{e\in \delta(u_i)}$.
Let $M$ be the multi-set of ordered pairs of the edges of $\delta(u_i)$ that we obtain. 
%we can efficiently computes a perfect matching $M\subseteq E^-\times E^+$ between the edges of $E^-$ and the edges of $E^+$, such that, for each pair of matched pairs $(e^-_1,e^+_1)$ and $(e^-_2,e^+_2)$ in $M$, the intersection of the path that consists of the edges $e^-_1,e^+_1$ and the path that consists of edges $e^-_2,e^+_2$ at vertex $u$ is non-transversal with respect to $\oset_v$.
We then designate: 
\begin{itemize}
\item for each path $\hat P_e\in \hat\pset^{\thr}_i$ with $e^-$ as its current last edge, a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$; and
\item for each path $P^{\out}_e\in\pset^{\out}_{i,*}$ with $e^-$ as its last edge (recall that we view $u_i$ as the last endpoint of such a path), a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$;
\end{itemize}
such that each path of $\rset^*_{(i)}$ is assigned to exactly one path of $\hat \pset^{\thr}_i\cup \pset^{\out}_{i,*}$.
This completes the description of the $i$-th iteration.
See Figure~\ref{fig: inner_path} for an illustration.





\begin{figure}[h]
	\centering
	\subfigure[Layout of edges in $\delta(u_i)$: only the last/first edges of paths are shown. Here $\pset^{\out}_{*,i}=\set{P^{\out}_e \mid e\in E^{\lef}_{i}}$.]{\scalebox{0.32}{\includegraphics{figs/inner_path_1.jpg}}}
	\hspace{1pt}
	\subfigure[Sets $L^-_i, L^+_i,L^{\out}_i$ and the pairing (shown in dash pink lines) given by the algorithm in \Cref{obs:rerouting_matching_cong}.]{
		\scalebox{0.32}{\includegraphics{figs/inner_path_2.jpg}}}
	\caption{An illustration of an iteration in Step 3 of computing inner paths.}\label{fig: inner_path}
\end{figure}







Let $\pset$ be the set of paths that we obtain after $k-1$ iterations of processings vertices $u_1,\ldots,u_{k-1}$, and we rename the path $\hat P_e$ at the end of the algorithm by $P_e$, and say that $P_e$ is the inner path of $e$, for every edge $e\in E'$.
It is clear that $|\pset|=|E'|$. It is also easy to see from the algorithm that, for each edge $e\in E'$ connecting $C_i$ to $C_j$ (with $j\ge i+2$), the inner path $P_e$ starts at $u_i$ and ends at $u_j$ (as it is supposed to), and it contains, for each $i\le t\le j-1$, a path of $\rset^*_{(i)}$ as its $t$-th segment.
Therefore, path $P_e$ visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially.
%and for each pair $1\le i,j\le k$ with $j>i+1$, $\pset$ contains $p_{i,j}$ paths originating $u_i$ and terminating at $u_j$. 

The following observations are immediate from our algorithm of constructing the inner paths.
\begin{observation}
\label{obs: non_transversal_1}
For each $1\le i\le k-1$, if we denote, for each $e\in E_i^{\rig}$, by $R_e$ the path consisting of the last edge of path $P^{\out}_e$ and the first edge of path $P_e$, then the paths in $\set{P_e\mid e\in \bigcup_{ i'<i<j'}E(C_{i'},C_{j'})}$ and $\set{R_e\mid e\in E_i^{\rig}}$ are non-transversal at $u_i$.
\end{observation}

%It is also easy to see that the paths in $\pset$ are non-transversal with respect to $\Sigma$, which we show in the following observation.
\begin{observation}
\label{obs: non_transversal_2}
The inner paths in $\pset$ are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
On one hand, note that for each $1\le i\le k-1$, the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.
Since the $i$-th segments of paths in $\pset$ are paths in $\rset^*_{(i)}$, it follows that the paths of $\pset$ are non-transversal at all vertices of $V(G)\setminus\set{u_1,\ldots,u_k}$.
On the other hand, from the algorithm and \Cref{obs:rerouting_matching_cong}, it is easy to verify that the paths of $\pset$ are also non-transversal at $u_1,\ldots,u_k$.
\end{proof}

\begin{observation}
\label{obs: edge_occupation in outer and inner paths}
Each edge $e\in E'$ belongs to exactly one outer path and no inner paths, each edge of $\bigcup_{1\le i\le k-1}\hat E_i$ belongs to no outer paths and $O(1)$ inner paths; and each edge of $\bigcup_{1\le i\le k}E(C_i)$ belongs to no outer paths and $O(\cong_G(\qset_i,e))$ inner paths.
\end{observation}

%Finally we designate, for each edge $e\in \inE(\cset)$, a distinct path of $\pset^*$ that connects $u_i$ to $u_j$, that we denote by $P^*_e$, as its \emph{representative} path. 


%Note that we will not compute a drawing of $G'$, we only use the non-transversal paths and their relative ordering in $G'$ to help define disengaged instance of $G$.



%Denote by $\oset^*_{i}$ the ordering of paths in $\pset^*$ that contains $u_i$, defined by the rotation $\oset'_{v_i}\in \Sigma'$ at $v$.\znote{To elaborate.}Note that $\oset^*_{i}$ is also an ordering on the edges of $\bigcup_{j_1\le i\le j_2}E'_{j_1,j_2}$.



\subsubsection{Construct Sub-Instances}
\label{sec: disengaged instances}


%\znote{$E_i^{\rig}$, $E_i^{\lef}$ and  $E^{\thr}_i$ are distinct from previous sections. to be coordinated later}

%We are now ready to construct the disengaged instances.
Recall that $\cset=\set{C_1,\ldots,C_k}$.
In this subsection we will construct, for each cluster $C_i\in \cset$, an sub-instance $I_i=(G_i,\Sigma_i)$ of $(G,\Sigma)$, such that the instances $\iset=\set{I_1,\ldots,I_k}$ satisfy the properties in \Cref{lem: path case}.
%We start with some definitions. 
For each $1\le i\le k$, recall that $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$. We denote $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$.

%We will use the instance $(G',\Sigma')$.For each $1\le i\le k$, the rotation $\oset'_{u_i}\in \Sigma'$ at vertex $u_i$ is an cyclic ordering on edges of $\delta_{G'}(u_i)$. Denote by $F^{\lef}_{i}$ the set of edges in $\delta_{G'}(u_i)$ that serves as the last edge of a path of $\pset^*_{(i-1)}$, and denote by $F^{\rig}_{i}$ the set of edges in $\delta_{G'}(u_i)$ that serves as the first edge of a path of $\pset^*_{(i)}$. We denote by $\oset^{\lef}_i$ the ordering on $F^{\lef}_{i}$ induced by $\oset'_{u_i}$, and we denote by $\oset^{\rig}_i$ the ordering on $F^{\rig}_{i}$ induced by $\oset'_{u_i}$. As there is an one-to-one correspondence between edges in $F^{\lef}_{i}$ and paths in $\pset^*_{(i-1)}$, we also say that $\oset^{\lef}_i$ is an ordering on the set $\pset^*_{(i-1)}$ of paths. We prove the following claim.
\iffalse
\begin{claim}
\label{clm: rotation_distance}
There exist integers $b_1,\ldots,b_k\in \set{0,1}$, such that $\sum_{1\le i\le k-1}\dist((\oset^{\rig}_i,b_i), (\oset^{\lef}_{i+1},b_{i+1}))\le O(\optcrors(G',\Sigma')\cdot\poly\log n)$.
\end{claim}
\begin{proof}
\end{proof}
\fi

\iffalse
We first construct instance $(G_k,\Sigma_k)$ as follows.
The graph $G_k$ is obtained from $G$ by contracting all vertices in $G\setminus C_k$ into a single vertex, that we denote by $v^{\lef}_k$. 
Notice that the edges incident to $v^{\lef}_k$ correspond to the edges of $\delta(C_k)$.
The ordering of a vertex of $v\ne v^{\lef}_k$ in $\Sigma_k$ is identical to the ordering $\oset_v$ of $v$ in the given rotation system $\Sigma$.
Note that $\delta_{G_k}(v^{\lef}_k)=\delta_G(C_k)=\delta_H(u_k)$, 
and there is an one-to-one correspondence between edges in $\delta_H(u_k)$ and paths in $\pset^*_{(i-1)}$.
The ordering of the vertex $v^{\lef}_k$ in $\Sigma_k$ is then defined to be $\oset^{\rig}_{k-1}$ (which is an ordering on the set $\pset^*_{(i-1)}$, and is therefore also an ordering on $\delta_{G_k}(v^{\lef}_k)$).

The instance $(G_1,\Sigma_1)$ is defined similarly. 
The graph $G_1$ is obtained from $G$ by contracting all vertices in $G\setminus C_1$ into a single vertex, that we denote by $v^{\rig}_1$. 
We will not distinguish between edges incident to $v^{\lef}_1$ and edges of $\delta(C_k)$. 
The ordering of a vertex $v\ne v^{\rig}_1$ in $\Sigma_1$ is identical to the ordering $\oset_v$ in $\Sigma$.
Note that $\delta_{G_1}(v^{\rig}_1)=\delta_G(C_1)=\delta_H(u_1)$, 
and there is an one-to-one correspondence between edges in $\delta_H(u_1)$ and paths in $\pset^*_{(1)}$.
The ordering of the vertex $v^{\rig}_1$ in $\Sigma_1$ is then defined to be $\oset^{\lef}_2$ (which is an ordering on the set $\pset^*_{(1)}$, and is therefore also an ordering on $\delta_{G_1}(v^{\rig}_1)$).
\fi

\paragraph{Instances $(G_2,\Sigma_2),\ldots,(G_{k-1},\Sigma_{k-1})$.}
We first fix some index $2\le i\le k-1$ and define the instance $(G_i,\Sigma_i)$ as follows.
The graph $G_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_i$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_i$, and finally deleting self-loops on super-nodes $v^{\lef}_i$ and $v^{\rig}_i$. So $V(G_i)=V(C_i)\cup \set{ v^{\lef}_i,v^{\rig}_i}$. See \Cref{fig: disengaged instance} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}$ and $E^{\rig}_{i}$ are shown in green. Edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.32}{\includegraphics{figs/disengaged_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{1pt}
	\subfigure[Graph $G_i$. The edges incident to $v_i^{\rig}$ are $\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$,  and the edges incident to $v_i^{\lef}$ are $\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.32}{\includegraphics{figs/disengaged_instance_2.jpg}}}
	\caption{An illustration of the disengaged instance.}\label{fig: disengaged instance}
\end{figure}

The ordering on the incident edges of a vertex $v\in V(C_i)$ in $\Sigma_i$ is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the orderings on the incident edges of super-nodes $v^{\lef}_i,v^{\rig}_i$. 
We first consider the super-node $v^{\lef}_i$.
Note that $\delta_{G_i}(v^{\lef}_i)=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e\in \hat E_{i-1}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ connecting $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\thr}_i\cup E^{\lef}_i$ that connects a vertex of $C_{i'}$ to a vertex of $C_{j'}$ with $i'<i<j'$, we denote by $W_e$ the path obtained by concatenating
(i) the subpath of $P^{\out}_e$ between (including) edge $e$ and its last endpoint $u_{i'}$; and
(ii) the subpath of $P_e$ between its first endpoint $u_{i'}$ and the vertex $u_{i-1}$.
Clearly, the path $W_e$ defined above connects $e$ to $u_{i-1}$.
We denote $\wset^{\lef}_i=\set{W_e\mid e\in E^{\thr}_i\cup E^{\lef}_i}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E_{i-1}}$, and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.
Intuitively, the rotation $\oset^{\lef}_i$ is the ordering in which the paths in $\wset^{\lef}_i$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_i$, let $e^*_W$ be the last edge lying on path $W$, that must belong to $\delta_{G}(u_{i-1})$. We first define a circular ordering of the paths in $\wset^{\lef}_i$, as follows: the paths are ordered according to the circular ordering of their last edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_i$ is associated with a unique edge in $\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$, that serves as the first edge on path $W$, this ordering of the paths in $\wset^{\lef}_i$ immediately defines a circular ordering of the edges of $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\rig}_i$, that we denote by $\oset^{\lef}_i$. See Figure~\ref{fig: v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i-1}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\lef}_{i}=\set{e^g_1,e^g_2}$ and $E^{\thr}_{i}=\set{e^r_1,e^r_2}$.
	Paths of $\wset^{\lef}_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.36}{\includegraphics{figs/rotation_left_1.jpg}}}
	\hspace{1pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\lef}_i)$ and the rotation $\oset^{\lef}_i$. $\delta_{G_i}(v^{\lef}_i)=\set{\hat e_1,\hat e_2,\hat e_3,\hat e_4,e^g_1,e^g_2, e^r_1,e^r_2}$, and the rotation $\oset^{\lef}_i$ on them around $v^{\lef}_i$ is shown above.]{
		\scalebox{0.28}{\includegraphics{figs/rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{i}$ on vertex $v^{\rig}_i$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e'\in \hat E_{i}$, recall that $Q_{i}(\hat e')$ is the path in $C_{i}$ connecting $\hat e'$ to $u_{i}$.
For each edge $e\in E^{\thr}_i\cup E^{\rig}_i$ that connects a vertex of $C_{i'}$ to a vertex of $C_{j'}$ with $i'\le i<j'$, we denote by $W_e$ the path obtained by concatenating
(i) the subpath of $P^{\out}_e$ between (including) edge $e$ and its last endpoint $u_{i'}$; and
(ii) the subpath of $P_e$ between its first endpoint $u_{i'}$ and vertex $u_{i}$ (note that for an edge $e\in E^{\rig}_{i}$, such a subpath only contains a single node $u_i$).
Clearly, the path $W_e$ defined above connects $e$ to $u_{i}$.
We denote $\wset^{\rig}_i=\set{W_e\text{ }\big|\text{ } e\in E^{\thr}_i\cup E^{\rig}_i}\cup \set{Q_{i}(\hat e')\text{ }\big|\text{ }  \hat e'\in \hat E_{i}}$.
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}$.
See Figure~\ref{fig: v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i}=\set{\hat e_1',\ldots,\hat e_4'}$, $E^{\lef}_{i}=\set{\tilde e^g_1,\tilde e^g_2}$ and $E^{\thr}_{i}=\set{e^r_1,e^r_2}$.
	Paths of $\wset^{\rig}_i$ excluding their first edges are shown in dash lines. ]{\scalebox{0.36}{\includegraphics{figs/rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{1pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\rig}_i)$ and the rotation $\oset^{\lef}_i$. $\delta_{G_i}(v^{\rig}_i)=\set{\hat e_1',\hat e_2',\hat e_3',\hat e_4',\tilde e^g_1,\tilde e^g_2, e^r_1,e^r_2}$, and the rotation $\oset^{\rig}_i$ on them around $v^{\rig}_i$ is shown above.]{
		\scalebox{0.28}{\includegraphics{figs/rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_right rotation}
\end{figure}

\paragraph{Instances $(G_1,\Sigma_1)$ and $(G_k,\Sigma_k)$.}
The instances $(G_1,\Sigma_1)$ and $(G_k,\Sigma_k)$ are defined similarly, but instead of two super-nodes, the graphs $G_1$ and $G_k$ contain one super-node each.
In particular, graph $G_1$ is obtained from $G$ by contracting clusters $C_2,\ldots, C_k$ into a super-node, that we denote by $v^{\rig}_1$, and then deleting self-loops on it.
So $V(G_1)=V(C_1)\cup \set{v^{\rig}_{1}}$ and $\delta_{G_1}(v^{\rig}_{1})=\hat E_1\cup E^{\rig}_1$.
The rotation of a vertex $v\in V(C_1)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\rig}_1$ is defined in a similar way as $\oset^{\rig}_i$ for any index $2\le i\le k-1$.
 Graph $G_k$ is obtained from $G$ by contracting clusters $C_1,\ldots, C_{k-1}$ into a super-node, that we denote by $v^{\lef}_k$, and then deleting self-loops on it.
So $V(G_k)=V(C_k)\cup \set{v^{\lef}_{k}}$ and $\delta_{G_k}(v^{\lef}_{k})=\hat E_{k-1}\cup E^{\lef}_k$.
The rotation of a vertex $v\in V(C_k)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\lef}_k$ is defined in a similar way as $\oset^{\lef}_i$ for any index $2\le i\le k-1$.







We will use the following claims later for completing the proof of \Cref{lem: path case} in the special case where there is no problematic index $i$.

\begin{observation}
\label{obs: disengaged instance size}
$\sum_{1\le i\le k}|E(G_i)|= 2m$, and for each $1\le i\le k$, $|E(G_i)|\le m/\mu$.
\end{observation}
\begin{proof}
Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le k}$, each graph of $\set{G_i}_{1\le i\le k}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node. Therefore, each edge of $G_i$ corresponds to an edge in $E(G)$ (and we do not distinguish between them).
So we can write $E(G_i)=E_G(C_i)\cup E_G(C_i,\overline{C_i})$. 
Therefore, for each $1\le i\le k$, $|E(G_i)|=|E_G(C_i)|+|E_G(C_i,\overline{C_i})|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu$.
On the other hand, since clusters $C_1,\ldots,C_k$ are vertex-disjoint, every edge of $E(G)$ appears twice in the graphs $\set{G_i}_{1\le i\le k}$. It follows that $\sum_{1\le i\le k}|E(G_i)|= 2m$.
\end{proof}


\begin{observation}
\label{obs: rotation for stitching}
For each $1\le i\le k-1$, if we view edge sets $\delta_{G_i}(v^{\rig}_i),\delta_{G_{i+1}}(v^{\lef}_{i+1})$ as subsets of $E(G)$, then $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$, and
$\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{observation}
\begin{proof}
Recall that for each $1\le i\le k-1$, 
$\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})=\hat E_{i}\cup E^{\thr}_{i+1}\cup E^{\lef}_{i+1}$. From the definition of sets $E_i^{\thr},E_{i+1}^{\thr}, E^{\rig}_i, E^{\lef}_{i+1}$,
\[
\begin{split}
E_i^{\thr}\cup E^{\rig}_i
 = & \set{e\in E(C_{i'},C_{j'})\mid i'<i<j'\text{ or }i'=i<j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'\le i<j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'< i+1\le j'}\\
 = & \set{e\in E(C_{i'},C_{j'})\mid i'<i+1<j'\text{ or }i'<i+1=j'}=E^{\thr}_{i+1}\cup E^{\lef}_{i+1}.
\end{split}
\]
Therefore, $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$.
Moreover, from the definition of path sets $\wset^{\rig}_i$ and $\wset^{\lef}_{i+1}$, it is not hard to verify that, for every edge $e\in \delta_{G_i}(v^{\rig}_i)$, the path in $\wset^{\rig}_i$ that contains $e$ as its first edge is identical to the path in $\wset^{\lef}_{i+1}$ that contains $e$ as its first edge. According to the way that rotations $\oset^{\rig}_i,\oset^{\lef}_{i+1}$ are defined, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{proof}




\subsubsection{Completing the Proof of \Cref{lem: path case} in the Special Case}
\label{sec: path case with no problematic index}

In this section we complete the proof of \Cref{lem: path case} in the special case where there is no problematic index. Specifically, we use the following two claims, whose proofs will be provided later.

\begin{claim}
	\label{claim: existence of good solutions special}
	$\sum_{1\le i\le k}\optcrors(G_i,\Sigma_i)\le O((\optcrors(G,\Sigma)+|E(G)|)\cdot \temp)$.
\end{claim}

\begin{claim}
\label{claim: stitching the drawings together}
There is an efficient algorithm, that given, for each $1\le i\le k$, a feasible solution $\phi_i$ to the instance $(G_i,\Sigma_i)$, computes a solution to the instance $(G,\Sigma)$, such that $\cro(\phi)\le \sum_{1\le i\le k}\cro(\phi_i)$.
\end{claim}

We use the algorithm described in~\Cref{sec: disengaged instances} and~\Cref{sec: inner and outer paths}, and return the disengaged instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$ as the collection of sub-instances of $(G,\Sigma)$. 
From the previous subsections, the algorithm for producing the sub-instances is efficient.
On the other hand, it follows immediately from \Cref{obs: disengaged instance size}, \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together} that the sub-instances $(G_1,\Sigma_1),\ldots,(G_k,\Sigma_k)$ satisfy the properties in \Cref{lem: path case}.
This completes the proof of \Cref{lem: path case}.

We now provide the proofs of \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together}.

$\ $

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
We will construct, for each $1\le i\le k$, a drawing $\phi_i$ of $G_i$ that respects the rotation system $\Sigma_i$, based on the optimal drawing $\phi^*$ of the instance $(G,\Sigma)$, such that $\sum_{1\le i\le k}\cro(\phi_i)\le O((\cro(\phi^*)+|E(G)|)\cdot \temp)$. The \Cref{claim: existence of good solutions special} then follows.

\paragraph{Drawings $\phi_2,\ldots,\phi_{k-1}$.}
First we fix some index $2\le i\le k-1$, and describe the construction of the drawing $\phi_i$. We start with some definitions.
Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
We define the auxiliary path set $\wset_i=\wset^{\lef}_i\cup \wset^{\rig}_i$, so 
$$\wset_i=\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}\cup \set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}},$$
where for each $e\in E^{\lef}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$; for each $e\in E^{\rig}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between $u_{i+1}$ and its last endpoint; and for each $e\in E^{\thr}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$, the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$, and the subpath of $P_e$ between $u_{i+1}$ and its last endpoint.
We use the following observation.
\begin{observation}
	\label{obs: wset_i_non_interfering}
	The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
\end{proof}


For uniformity of notations, for each edge $\hat e\in \hat E_i$, we rename the path $Q_{i+1}(\hat e)$ by $W_{\hat e}$, and similarly for each edge $\hat e\in \hat E_{i-1}$, we rename the path $Q_{i-1}(\hat e)$ by $W_{\hat e}$. Therefore, $\wset_i=\set{W_e\mid e\in E(G_i)\setminus E(C_i)}$.
Put in other words, the set $\wset_i$ contains, for each edge $e$ in $G_i$ that is incident to $v^{\lef}_i$ or $v^{\rig}_i$, a path named $W_e$.
It is easy to see that all paths in $\wset_i$ are internally disjoint from $C_i$.
We further partition the set $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_e\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.

We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
Specifically, we proceed in the following four steps.



\paragraph{Step 1.}
For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
We denote by $\Pi_e$ the set of these curves.
We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.

%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
Therefore, $\hat{\chi}_i(P)$ is well-defined.
For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.

\iffalse
We use the following observation.
\znote{maybe remove this observation?}

%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.

\begin{observation}
\label{obs: curves_crossings}
The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
\end{observation}
\begin{proof}
We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.

We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
\end{proof}
\fi

\paragraph{Step 2.}
For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
\iffalse{just for backup}
\begin{proof}
	Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
	For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
	We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
	It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
	We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
	See Figure~\ref{fig: curve_con} for an illustration.
	Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
	It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
	Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
	Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
	Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
\end{proof}
\begin{figure}[h]
	\centering
	\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
	\hspace{1pt}
	\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
		\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
	\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
\end{figure}
\fi

%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
We use the following observation.
\begin{observation}
\label{obs: general_position}
Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
\end{observation}
\begin{proof}
From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
\end{proof}




%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.


\paragraph{Step 3.} 
So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.


Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.





\paragraph{Step 4.}
Let $\dset$ be an arbitrarily small disc around $z_{\rig}$ in the drawing $\phi'_i$, and let $\dset'$ be another small disc around $z_{\rig}$ that is strictly contained in $\dset$.
We first erase the drawing of $\phi'_i$ inside the disc $\dset$, and for each edge $e\in \delta(v^{\rig}_i)$, we denote by $p_{e}$ the intersection between the curve representing the image of $e$ in $\phi'_i$ and the boundary of $\dset$.
We then place, for each edge $e\in \delta(v^{\rig}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{\rig}_{i}$. 
We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{\rig}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$.
Finally, for each edge $e\in \delta(v^{\rig}_i)$, let $\gamma_e$ be the concatenation of (i) the image of $e$ in $\phi'_i$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z_{\rig}$ in $\dset'$.
We view $\gamma_e$ as the image of edge $e$, for each $e\in \delta(v^{\rig}_i)$. 
We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$, and therefore it respects the rotation system $\Sigma_i$.

We use the following claim.
\begin{claim}
\label{clm: rerouting_crossings}
The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
\end{claim}
\begin{proof}
Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	
%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.

We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
\begin{figure}[h]
\centering
\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
\end{figure}
\end{proof}

From the above discussion and Claim~\ref{clm: rerouting_crossings}, for each $2\le i\le k-1$, 
\[
\cro(\phi_i)=\chi^2(C_i)+O\left(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right).
\]



\iffalse
We now estimate the number of crossings in $\phi_i$ in the next claim.
\begin{claim}
\label{clm: number of crossings in good solutions}
$\cro(\phi_i)=\chi^2(C_i)+O\left(\sum_{W\in \tilde\wset_i}\cro(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)$.
\end{claim}
\begin{proof}
$2\cdot \sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2=\sum_{v\in V(G)}\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2.$
\znote{need to redefine the orderings $\oset^{\lef}_i$ and $\oset^{\rig}_i$ to get rid of $\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2$ here, which we may not be able to afford.}
\end{proof}
\fi


\paragraph{Drawings $\phi_1$ and $\phi_{k}$.}
The drawings $\phi_1$ and $\phi_{k}$ are constructed similarly. We describe the construction of $\phi_1$, and the construction of $\phi_1$ is symmetric.
Recall that the graph $G_1$ contains only one super-node $v_1^{\rig}$, and $\delta_{G_1}(v_1^{\rig})=\hat E_1\cup E^{\rig}_1$. We define $\wset_1=\set{W_e\mid e\in E^{\rig}_1}\cup \set{Q_2(\hat e)\mid \hat e\in \hat E_1}$. For each $\hat e\in \hat E_1$, we rename the path $Q_2(\hat e)$ by $W_e$, so $\wset_1$ contains, for each edge $e\in \delta_{G_1}(v^1_{\rig})$, a path named $W_e$ connecting its endpoints to $u_2$. Via similar analysis in \Cref{obs: wset_i_non_interfering}, it is easy to show that the paths in $\wset_1$ are non-transversal with respect to $\Sigma$.

We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{k-1}$. 
We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{k-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]




We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le k}\cro(\phi_i)$.
Recall that, for each $1\le i\le k$, $\tilde \wset_i=\set{W_e\mid e\in \hat E_{i-1}\cup \hat E_{i-1}\cup E^{\lef}_{i}\cup E^{\rig}_{i}}$, where $E^{\lef}_{i}=E(C_i,\bigcup_{1\le j\le i-2}C_j)$, and 
$E^{\rig}_{i}=E(C_i,\bigcup_{i+2\le j\le k}C_j)$. Therefore, for each edge $e\in E'\cup (\bigcup_{1\le i\le k-1}\hat E_i)$, the path $W_e$ belongs to exactly $2$ sets of $\set{\tilde\wset_i}_{1\le i\le k}$.
Recall that the path $W_e$ only uses edges of the inner path $P_e$ and the outer path $P^{\out}_e$.
Let $\tilde\wset=\bigcup_{1\le i\le k}\tilde\wset_i$, from \Cref{obs: edge_occupation in outer and inner paths}, 
for each edge $e\in E'\cup (\bigcup_{1\le i\le k-1}\hat E_i)$, $\cong_G(\tilde\wset,e)=O(1)$, and
for $1\le i\le k$ and for each edge $e\in E(C_i)$, $\cong_G(\tilde\wset,e)=O(\cong_G(\qset_i,e))$.

Therefore, on one hand,
\[
\begin{split}
\sum_{1\le i\le k}\sum_{W\in \tilde\wset_i}\hat\chi_i(W)
& \le 
\sum_{(e,e'): e,e'\text{ cross in }\phi^*} 2\cdot \cong_G(\tilde \wset,e)\cdot\cong_G(\tilde \wset,e')\\
& \le 
\sum_{(e,e'): e,e'\text{ cross in }\phi^*} \left(\cong_G(\tilde \wset,e)^2+\cong_G(\tilde \wset,e')^2\right)\\
& \le 
\sum_{e\in E(G)} \chi(e)\cdot \cong_G(\tilde \wset,e)^2
= O(\cro(\phi^*)\cdot\temp),
\end{split}
\]
and on the other hand,
\[
\begin{split}
\sum_{1\le i\le k}\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2
%= \sum_{e\in E(G)} \sum_{1\le i\le k} \cong_G(\tilde \wset_i,e)^2 
& \le  \sum_{e\in E(G)} \left(\sum_{1\le i\le k} \cong_G(\tilde \wset_i,e)\right)^2\\
& \le O\left(\sum_{e\in E(G)} \cong_G(\tilde \wset,e)^2 \right)\\
& \le O\left(|E(G)|+\sum_{1\le i\le k}\sum_{e\in E(C_i)} \cong_G(\qset_i,e)^2\right)=O(|E(G)|\cdot\temp).
\end{split}
\]
Moreover, $\sum_{1\le i\le k}\chi^2(C_i)\le O(\cro(\phi^*))$, and $\sum_{1\le i\le k}\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})\le O(\cro(\phi^*)\cdot\temp)$.

Altogether,
\[
\begin{split}
\sum_{1\le i\le k}\cro(\phi_i)
& \le 
O\left(\sum_{1\le i\le k} 
\left(
\chi^2(C_i)+ \hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)
\right)\\
& \le O(\cro(\phi^*))+O(\cro(\phi^*)\cdot\temp)+O(\cro(\phi^*)\cdot\temp)+O(|E(G)|\cdot\temp)\\
& \le O((\cro(\phi^*)+|E(G)|)\cdot\temp).
\end{split}
\]

This completes the proof of \Cref{claim: existence of good solutions special}.
\end{proofof}






$\ $



\iffalse
We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

We first define an instance $(\hat G_i,\hat\Sigma_i)$ as follows. We start with the subgraph of $G$ induced by all edges of $E_G(C_i)$ and $E(\wset_i)$, and then create, for each edge $e$ in the subgraph, $\cong_{\wset_i}(e)$ parallel copies of it. This finishes the description of graph $\hat G_i$.
For each vertex $v$ in $\hat G_i$, we define its rotation $\hat\oset_v$ as follows. We start with the rotation $\oset_v\in \Sigma$, and then replace, for each edge $e\in E(\wset_i)$, the edge $e$ in the ordering $\oset_v$ by its $\cong_{\wset_i}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, where the ordering among the copies is arbitrary. 
On the one hand, in graph $\hat G_i$, we can make paths of $\wset_i$ edge-disjoint by letting, for each edge $e\in E(\wset_i)$, each path of $\wset_i$ that contains $e$ now take a distinct copy of $e$ in $\hat G_i$.
On the other hand, a drawing $\hat \phi_i$ of the instance $(\hat G_i,\hat\Sigma_i)$ can be easily computed from $\phi^*$, as follows.
We start with $\hat\phi'_i$, the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$. Then for each edge of $\wset_i$, let $\gamma_e$ be the curve that represents the image of $e$, and we create $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting endpoints of $e$, that lies in an arbitrarily thin strip around $\gamma_e$. We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

For each edge $e\in E_G(C_i)$, we denote by $\gamma_e$ the curve in $\hat \phi_i$ that represents the image of $e$; and for each path $W\in \wset_i$, we denote by $\gamma_W$ the curve in $\hat \phi_i$ that represents the image of $W$.
We define $\Gamma_0=\set{\gamma_e\mid e\in E_G(C_i)}$ and $\Gamma_1=\set{\gamma_W\mid W\in \wset_i}$. It is immediate to verify that the sets $\Gamma_0,\Gamma_1$ of curves satisfy the condition of \Cref{thm: type-2 uncrossing}. We then apply the algorithm in \Cref{thm: type-2 uncrossing} to $\Gamma_0,\Gamma_1$, and let $\Gamma_1'$ be the set of curves that we obtain.
From \Cref{thm: type-2 uncrossing}, the curves in $\Gamma_1'$ do not intersect internally between each other, and have the same sets of first endpoints and last endpoints.
We now show that we can obtain a drawing $\phi_i$ of the instance $(G_i,\Sigma_i)$ using the curves $\Gamma_0,\Gamma_1'$.
For each edge $e\in E_G(C_i)$, we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
For each edge path $W\in \wset$, from \Cref{thm: type-2 uncrossing}, there is a curve $\gamma'\in \Gamma_1'$ connecting the endpoint of $W$ to we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
\znote{maybe we need another type of uncrossing here.}
\fi



\begin{proofof}{Claim~\ref{claim: stitching the drawings together}}
We first define a set $\set{(U_i,\Sigma'_i)\mid 1\le i\le k}$ of instances of \CNwRS as follows.
We define $U_1=G$, and for each $2\le i\le k$, we define $U_i$ to be the graph obtained from $G$ by contracting the clusters $C_1,\ldots, C_{i-1}$ into a vertex $v^{\lef}_i$.
Note that each edge in $U_i$ is also an edge in $G$, and we do not distinguish between them.
Note that $U_1=G$, we define the rotation system $\Sigma'_1$ on $U_1$ to be $\Sigma$.
For each $2\le i\le k$, we define the rotation system $\Sigma'_i$ on $U_i$ as follows.
For each vertex $v\in \bigcup_{i\le t\le k}V(C_t)$, note that its incident edges in $U_i$ are the edges of $\delta_G(v)$, and its rotation in $\Sigma'_i$ is defined to be $\oset_v$, the rotation on $v$ in the input rotation system $\Sigma$.
For vertex $v^{\lef}_i$, note that its incident edges are the edges of $\delta_{G_i}(v^{\lef}_i)$, and its rotation in $\Sigma'_i$ is defined to be $\oset^{\lef}_i$, the rotation on $v^{\lef}_i$ of instance $(G_i,\Sigma_i)$.


Note that $U_k=G_k$ and $\Sigma'_k=\Sigma_k$, so the drawing $\phi_k$ of the instance $(G_k,\Sigma_k)$ is also a drawing of the instance $(U_k,\Sigma'_k)$. For clarity, when we view this drawing as a solution to the instance $(U_k,\Sigma'_k)$, we rename it by $\psi_k$.
We will sequentially, for $i=k-1,\ldots,1$, compute a drawing of the instance $(U_i,\Sigma'_i)$ using the drawing $\psi_{i+1}$ of $(U_{i+1},\Sigma'_{i+1})$ and the drawing $\phi_i$ of $(G_{i},\Sigma_{i})$, and eventually, we return the drawing $\psi_1$ of $(U_{1},\Sigma'_{1})$ as the solution to the instance $(G,\Sigma)$.

We now fix an index $1\le  i< k-1$ and construct the drawing $\psi_i$ to the instance $(U_{i},\Sigma'_{i})$, assuming that we have computed a drawing $\psi_{i+1}$ to the instance $(U_{i+1},\Sigma'_{i+1})$, as follows.
Recall that $V(G_i)=V(C_i)\cup\set{v^{\lef}_i,v^{\rig}_i}$ if $i\ge 2$ and $V(G_i)=V(C_i)\cup\set{v^{\rig}_i}$ if $i=1$, and $\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.  Moreover, from \Cref{obs: rotation for stitching} and the definition of instance $(U_{i+1},\Sigma'_{i+1})$, the rotation on $v^{\rig}_i$ in $\Sigma_{i}$ is identical to the rotation on $v^{\lef}_{i+1}$ in $\Sigma'_{i+1}$.
Denote $F=\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.
Let $\dset$ be an arbitrarily small disc around the image of $v_{i+1}^{\lef}$ in $\psi_{i+1}$. For each edge $e\in F$, we denote by $p_e$ the intersection between the image of $e$ with the boundary of $\dset$. 
Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset$ is $\oset^{\lef}_{i+1}$.
We erase the drawing of $\psi_{i+1}$ inside the disc $\dset$, and view the area inside the disc $\dset$ as the outer face of the drawing.
Similarly, let $\dset'$ be an arbitrarily small disc around the image of $v_{i}^{\rig}$ in $\phi_{i}$. For each edge $e\in F$, we denote by $p'_e$ the intersection between the image of $e$ with the boundary of $\dset'$. 
Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is $\oset^{\rig}_{i}$.
We erase the drawing of $\phi_{i}$ inside the disc $\dset'$, and let $\dset''$ be another disc that is strictly contained in $\dset'$. We now place the drawing of $\psi_{i+1}$ inside $\dset'$ (after we erase part of it inside $\dset$), so that the boundary of $\dset$ in $\psi_{i+1}$ coincide with the boundary of $\dset''$ in $\phi_{i}$, while the interior of $\dset$ coincides with the exterior of $\dset''$. We then compute a set $\set{\zeta_e\mid e\in F}$ of curves lying in $\dset'\setminus \dset''$, where for each $e\in F$, the curve $\zeta_e$ connects $p'_e$ to $p_e$, such that all curves of $\set{\zeta_e\mid e\in F}$ are mutually disjoint. Note that this can be done since the order in which $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is identical to $\set{p'_e}_{e\in F}$ appear on the boundary of $\dset$.
We denote by $\psi_i$ the resulting drawing we obtained.
See Figure~\ref{fig: stitching} for an illustration.
Clearly, $\psi_i$ is a drawing of $U_i$ that respects $\Sigma'_i$ if we view, for each edge $e\in F$, the union of (i) the image of $e$ in $\phi_i$ outside the disc $\dset'$; (ii) the curve $\zeta_e$; and (iii) the image of $e$ in $\psi_{i+1}$ inside the disc $\dset''$, as the image of $e$.
\begin{figure}[h]
	\centering
	\subfigure[The drawing $\psi_{i+1}$, where the boundary of $\dset$ is shown in dash black.]{\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.45cm}
	\subfigure[The drawing $\psi_{i+1}$ after we erase its part inside $\dset$ and view the interior of $\dset$ as the outer face.]{
		\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_2.jpg}}}
	\hspace{0.45cm}
	\subfigure[The drawing $\psi_i$, where the curves of $\set{\zeta_e\mid e\in F}$ are shown in dash line segments.]{
		\scalebox{0.36}{\includegraphics[scale=1.0]{figs/stitching_3.jpg}}}
	\caption{An illustration of an iteration in type-1 uncrossing.}\label{fig: stitching}
\end{figure}
Clearly, any crossing in the drawing $\psi_i$ is either a crossing of $\phi_i$ or a crossing of $\psi_{i+1}$, so $\cro(\psi_i)\le \cro(\psi_{i+1})+\cro(\phi_{i})$.
Therefore, if we rename the drawing $\psi_1$ of the instance $(U_1,\Sigma'_1)$ by $\phi$, then $\phi$ is a drawing of $G$ that respects $\Sigma$, and $\cro(\phi)\le \sum_{1\le i\le k}\cro(\phi_i)$.
\end{proofof}














==> disengage_with_routing.tex <==
\subsection{A Special Case}


In this section we provide the proof of  \Cref{thm: disengagement - main} in a special case. Specifically, we will assume that the Gomory-Hu tree of the contracted graph $G_{\mid\cset}$ is a path, and we are additionally given a set of paths called the \emph{inner paths} that will be defined later.

Let $H=G_{\mid\cset}$ be the contracted graph. 
We denote the clusters in $\cset$ by $C_1,C_2,\ldots,C_r$. For convenience, for each $1\leq i\leq r$, we denote by $x_i$ the vertex of graph $H$ that represents the cluster $C_i$. Throughout this subsection, we assume that the Gomory-Hu tree $\tau$ of graph $H$ is a path, and we assume without loss of generality that the clusters are indexed according to their appearance on the path $\tau$. Note that each edge in $\Eout(\cset)$ corresponds to an edge in $H$, and we do not distinguish between them.
%For all $1\le i,j\le r$, we will also view edges of $E(C_i,C_j)$ as parallel edges connecting vertex $x_i$ to vertex $x_j$ in graph $H$.
For each $1\le i\le r$, we define edge sets
$\hat E_i=E(C_i,C_{i+1})$,
$E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, $E_i^{\thr}=\bigcup_{i'<i<j'}E(C_{i'},C_{j'})$, $E_i^{\through}=\bigcup_{i'<i,j'>i+1}E(C_{i'},C_{j'})$ and we define vertex sets  $S_i=\set{x_1,\ldots,x_i}$ and $\notS_i=\set{x_{i+1},\ldots,x_r}$.
We need the following  observation.

\begin{observation}\label{obs: bad inded structure}
	For all $1\leq i<r$, the following hold:
	\begin{itemize}
		\item $|\hat E_i|\geq |E_i^{\through}|$;
		\item $|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$; and
		\item $|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
	\end{itemize}
\end{observation}
\begin{proof}
	Consider the cut $(\set{x_{i}},V(H)\setminus \set{x_i})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$. Note that this cut separates $x_i$ from $x_{i-1}$. Since the minimum cut separating $x_i$ from $x_{i-1}$ in $H$ is $(S_{i-1},\notS_{i-1})$, and $|E(S_{i-1},\notS_{i-1})|=|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|$, we get that $|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$,
	and so  
	\begin{equation}
	\label{eqn1}
	|E_{i+1}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+ |E_i^{\rig}|.
	\end{equation}
	Consider the cut $(\set{x_{i+1}},V(H)\setminus \set{x_{i+1}})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$. Note that this cut separates $x_{i+1}$ from $x_{i+2}$. Since the minimum cut separating $x_{i+1}$ from $x_{i+2}$ in $H$ is $(S_{i+1},\notS_{i+1})$, and $|E(S_{i+1},\notS_{i+1})|=|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|$, we get that $|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$, 	
	and so 
	\begin{equation}
	\label{eqn2}
	|E_i^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|E_{i+1}^{\lef}|.
	\end{equation}
	Combining \Cref{eqn1,eqn2}, we get that $|\hat E_i|\geq |E_i^{\through}|$. By rearranging the sides of the two inequalities, we get that 	
	$|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$, and
	$|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{proof}


Define $E'=E(H)\setminus (\bigcup_{1\le i\le r-1}\hat E_i)$.
Equivalently, $E'$ is the subset of $E^{\out}(\cset)$ that contains all edges connecting a pair $C_i,C_j$ of clusters in $\cset$, with $j\ge i+2$, and when $E'$ is viewed as a set of edges in $H$, then $E'$ contains all edges connecting a pair $x_i,x_j$ of vertices in $H$ with $j\ge i+2$.

\paragraph{Inner Paths.} For an edge $e\in E'$ connecting $x_i$ to $x_j$ in $H$, we say that a path $P$ in $H$ is a \emph{left inner path} of $e$, iff the endpoints of $P$ are $x_i$ and $x_{i+1}$, and $P$ only contains vertices of $S_{i+1}$; we say that a path $P$ in $H$ is a \emph{right inner path} of $e$, iff the endpoints of $P$ are $x_{j-1}$ and $x_{j}$, and $P$ only contains vertices of $\notS_{j-2}$; and we say that a path $P$ in $H$ is a \emph{middle inner path} of $e$, iff path $P$ sequentially visits vertices $x_{i+1}, x_{i+2},\dots,x_{j-1}$.
We say that a path $P$ is an \emph{inner path} of $e$, iff $P$ is the union of (i) a left inner path of $e$; (ii) a middle inner path of $e$; and (iii) a right inner path of $e$.
See \Cref{fig: LMR_inner} for an illustration.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.20]{figs/LMR_inner.jpg}
	\caption{An illustration of left inner path (orange), middle inner path (purple) and right inner path (green) of edge $(x_i,x_j)\in E'$.}\label{fig: LMR_inner}
\end{figure}

In the remainder of this subsection, we will additionally assume that we are given, for each edge $e\in E'$, an inner path $P_e$ of $e$ in graph $H$, such that the set $\set{P_e}_{e\in E'}$ of paths causes congestion at most $\eta$, for some $\eta=2^{O((\log m)^{3/4}\log\log m)}$.

We now provide the proof of \Cref{thm: disengagement - main} with these additional assumptions. We will use the parameters $\eta=2^{O((\log m)^{3/4}\log\log m)}$, $\beta^*=2^{O(\sqrt{\log m}\cdot \log\log m)}$, and $\eta^*=2^{O((\log m)^{3/4}\log\log m)}$.

\subsubsection{Computing Guiding Paths and Auxiliary Cycles}
\label{sec: guiding and auxiliary paths}

We first apply the algorithm from \Cref{thm:algclassifycluster} to each cluster of $\cset$.
In particular, for each $1\le i\le r$, we apply the \algclassifycluster to the instance $(G,\Sigma)$ and the cluster $C_i$ (recall that cluster $C_i$ has the $\alpha_0$-bandwidth property, where $\alpha_0=1/\log^3m$) for $100\log n$ times. If any application of \algclassifycluster returns a distribution $\dset(C_i)$ over sets of guiding paths in $\Lambda(C_i)$, such that $C_i$ is $\beta^*$-light with respect to $\dset(C_i)$, then we continue to sample a set of guiding paths from $\dset(C_i)$. Let $\qset_i$ be the set we obtain, and let $u_i$ be the vertex of $C_i$ that serves as the common endpoint of all paths in $\qset_i$. If all applications of \algclassifycluster return FAIL, then consider the graph $C_i^+$ (see \Cref{def: Graph C^+}). We apply the algorithm from \Cref{lem: simple guiding paths} to cluster $C^+_i$ and and set $T(C_i)$, and let $u_i$ be the vertex and $\qset_i$ be the set of paths that we obtain. Clearly, $\qset_i$ can be also viewed as a set of paths routing edges of $\delta_G(C_i)$ to $u_i$. From \Cref{lem: simple guiding paths}, for each edge $e\in E(C_i)$, $\expect{\cong(\qset_i,e)}\leq  O(\log^4m/\alpha_0)$. Finally, for each $1\le i\le r$ and for each $e\in \delta(C_i)$, we denote by $Q_i(e)$ the path of $\qset_i$ that routes $e$ to $u_i$.

We then apply the algorithm from \Cref{lem: non_interfering_paths} to each set $\qset_i$ of paths and the rotation system $\Sigma$, and rename the sets of paths we obtain as $\qset_1,\ldots,\qset_r$. Now we are guaranteed that, for each $1\le i\le r$, the set $\qset_i$ of paths is non-transversal with respect to $\Sigma$.


\paragraph{Bad Event $\xi_i$.} For each index $1\le i\le r$, we say that the event $\xi_i$ happens, iff $C_i$ is not an $\eta^*$-bad cluster, but all the $100\log n$ applications of \algclassifycluster return FAIL.
From \Cref{thm:algclassifycluster}, $\Pr[\xi_i]\le (1/2)^{100\log n}=O(n^{-50})$. Then from the union bound over all $1\le i\le r$, $\Pr[\bigcup_{1\le i\le r}\xi_i]\le O(n^{-49})$.



We then compute a set $\rset^*$ of cycles in $G$, using the set $\set{P_e}_{e\in E'}$ of inner paths and the path sets $\set{\qset_i}_{1\le i\le r}$, as follows.
Consider an edge $e\in E'$ and its inner path $P_e$ in $H$.
We denote $P_e=(e_1,\ldots,e_k)$, and for each $1\le j\le k$, we denote $e_j=(x_{t_{j-1}}, x_{t_{j}})$ (and so $e=(x_{t_0},x_{t_k})$ as an edge in $H$).
Recall that the set $\qset_i$ contains, for each edge $e\in\delta(C_i)$, a path $Q_i(e)$ routing edge $e$ to $u_i$.
We then define path $P^*_e$ as the sequential concatenation of paths $Q_{t_{0}}(e_1),Q_{t_{1}}(e_1), Q_{t_{1}}(e_2),Q_{t_{2}}(e_2),\ldots, Q_{t_{r-1}}(e_k),Q_{t_{r}}(e_k)$.
It is clear that path $P^*_e$ sequentially visits the vertices $u_{t_0},u_{t_1},\ldots,u_{t_k}$ in $G$.
%We call $P^*_e$ the \emph{auxiliary} path of $e$.
Since edge $e$, as an edge of $G$, connects a vertex of $C_{t_0}$ to a vertex of $C_{t_k}$. We then define path $P^{**}_e$ to be the union of paths $Q_{t_{k}}(e)$ and $Q_{t_{0}}(e)$, so path $P^{**}_e$ connects $u_{t_k}$ to $u_{t_0}$.
Finally, we define cycle $R^*_e$ to be the union of paths $P^*_e$ and paths $P^{**}_e$, and we denote $\rset^*=\set{R^*_e\mid e\in E'}$.
See \Cref{fig: LMR_auxi} for an illustration.
%We call $R^*_e$ the \emph{auxiliary cycle} of edge $e$.
%We define an orientation on cycle $R^*_e$ as follows. We start from vertex $u_{t_0}$, follow the path $P^*_e$ to sequentially visit vertices $u_{t_1},\ldots, u_{t_k}$, and finally follow the path $P^{**}_e$ to come back to vertex $u_{t_0}$.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.24]{figs/auxiliary_path.jpg}
	\caption{An illustration of the auxiliary cycle $R^*_e$ of an edge $e$ (solid red): left auxiliary path shown in orange, middle auxiliary path  shown in purple and right auxiliary path  shown in green.}\label{fig: LMR_auxi}
\end{figure}

Recall that the set $\set{P_e}_{e\in E'}$ of inner paths is guaranteed to cause congestion at most $\beta$ in graph $H$, then from the construction of cycles in $\rset^*$, it is easy to see that, for each edge $e\in E'$, $\cong_{G}(\rset^*,e)\le O(\beta)$, and
for each edge $e\in \bigcup_{1\le i\le r}E(C_i)$, $\expect[]{\cong_{G}(\rset^*,e)^2}\le O(\beta^2\cdot\beta^*)$.

%\subsubsection*{Step 3. De-Interfering Auxiliary Cycles}

\znote{to modify from here, define left/mid/right auxiliary path}

We further modify the cycles in $\rset^*$ to obtain a new set $\rset$ of cycles, such that the intersection of every pair of cycles in $\rset$ is non-transversal with respect to $\Sigma$ at at most one of their shared vertices.

Let $R,R'$ be a pair of cycles in $\rset^*$ and let $v$ be a shared vertex of $R$ and $R'$. We say that the tuple $(R,R',v)$ is \emph{bad}, iff the intersection of cycles $R,R'$ at $v$ is transversal with respect to $\Sigma$. We iteratively process the set $\rset^*$ of cycles as follows. While there exist a pair $R,R'$ of cycles in $\rset^*$ and two vertices $v_1,v_2\in V(R)\cap V(R')$, such that the tuples $(R,R',v)$ and $(R,R',v)$ are bad, we process cycles $R,R'$ as follows. 

Eventually, for each $e\in E'$, we obtain a cycle $R_e$ in $G$ that is called the \emph{auxiliary cycle} of edge $e$.


\subsubsection{Constructing Sub-Instances}
\label{sec: compute advanced disengagement}

In this step we will construct, for each cluster $C_i\in \cset$, an sub-instance $I_i=(G_i,\Sigma_i)$ of $(G,\Sigma)$, such that the instances $\iset=\set{I_1,\ldots,I_r}$ satisfy the properties in \Cref{thm: disengagement - main}.
Recall that, for each $1\le i\le r$, $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, and $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$.

\paragraph{Instances $(G_2,\Sigma_2),\ldots,(G_{r-1},\Sigma_{r-1})$.}
We first fix some index $2\le i\le r-1$ and define the instance $(G_i,\Sigma_i)$ as follows.
The graph $G_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_i$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_i$, and finally deleting self-loops on the super-nodes $v^{\lef}_i$ and $v^{\rig}_i$. So $V(G_i)=V(C_i)\cup \set{ v^{\lef}_i,v^{\rig}_i}$. See \Cref{fig: disengaged instance} for an illustration. 

\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}\cup E^{\rig}_{i}$ are shown in green, and edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.32}{\includegraphics{figs/disengaged_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{5pt}
	\subfigure[Graph $G_i$. Note that $\delta_{G_i}(v_i^{\rig})=\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$, and $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.32}{\includegraphics{figs/disengaged_instance_2.jpg}}}
	\caption{An illustration of the construction of sub-instance $(G_i,\Sigma_i)$.}\label{fig: disengaged instance}
\end{figure}

We now define the orderings in $\Sigma_i$. First, for each vertex $v\in V(C_i)$, the ordering on its incident edges is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the rotations of super-nodes $v^{\lef}_i,v^{\rig}_i$. 
We first consider $v^{\lef}_i$.
Note that $\delta_{G_i}(v^{\lef}_i)=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$.
For each edge $\hat e\in \hat E_{i-1}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ routing edge $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\lef}_i\cup E^{\thr}_i$, we denote by $W^{\lef}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i-1}$ and contains its entire left auxiliary path.
We then denote 
$$\wset^{\lef}_i=\set{W^{\lef}_i(e)\mid e\in E^{\thr}_i\cup E^{\lef}_i}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E_{i-1}}.$$
%and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.
\znote{need to treat the red edges that enter $C_{i-1}$ specially}

Intuitively, the rotation on vertex $v^{\lef}_i$ is defined to be the ordering in which the paths in $\wset^{\lef}_i$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_i$, let $e^*_W$ be the unique edge of path $W$ that is incident to $u_{i-1}$. We first define a circular ordering of the paths in $\wset^{\lef}_i$, as follows: the paths are ordered according to the circular ordering of their corresponding edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_i$ is associated with a unique edge in $\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, this ordering of the paths in $\wset^{\lef}_i$ immediately defines a circular ordering of the edges of $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, that we denote by $\oset^{\lef}_i$. See Figure~\ref{fig: v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i-1}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\lef}_{i}=\set{e^g_1}$ and $E^{\thr}_{i}=\set{e^r_1}$.
	Paths of $\wset^{\lef}_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.13}{\includegraphics{figs/rotation_left_1.jpg}}}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\lef}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\lef}_i)=\set{\hat e_1,\hat e_2,\hat e_3,\hat e_4,e^g_1, e^r_1}$. The rotation $\oset^{\lef}_i$ on them around $v^{\lef}_i$ is shown above.]{
		\scalebox{0.16}{\includegraphics{figs/rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{i}$ on vertex $v^{\rig}_i$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e'\in \hat E_{i}\cup E_i^{\rig}$, recall that $Q_{i}(\hat e')$ is the path in $C_{i}$ routing edge $\hat e'$ to vertex $u_{i}$.
For each edge $e\in E^{\thr}_i$, we denote by $W^{\rig}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i}$ and contains its entire left auxiliary path.
We then denote 
$$\wset^{\rig}_i=\set{W^{\rig}_i(e)\text{ }\big|\text{ } e\in E^{\thr}_i}\cup \set{Q_{i}(\hat e')\text{ }\big|\text{ }  \hat e'\in \hat E_{i}\cup E^{\rig}_i}.$$
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is then defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}\in \Sigma$.
See Figure~\ref{fig: v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i}=\set{\hat e_1',\ldots,\hat e_4'}$, $E^{\rig}_{i}=\set{\tilde e^g_1}$ and $E^{\thr}_{i}=\set{\tilde e^r_1}$.
	Paths of $\wset^{\rig}_i$ excluding their first edges are shown in dash lines. ]{\scalebox{0.13}{\includegraphics{figs/rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\rig}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\rig}_i)=\set{\hat e_1',\hat e_2',\hat e_3',\hat e_4',\tilde e^g_1,\tilde e^r_1}$. The rotation $\oset^{\rig}_i$ on them around $v^{\rig}_i$ is shown above.]{
		\scalebox{0.16}{\includegraphics{figs/rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_right rotation}
\end{figure}

\paragraph{Instances $(G_1,\Sigma_1)$ and $(G_r,\Sigma_r)$.}
The instances $(G_1,\Sigma_1)$ and $(G_r,\Sigma_r)$ are defined similarly, but instead of two super-nodes, the graphs $G_1$ and $G_r$ contain one super-node each.
In particular, graph $G_1$ is obtained from $G$ by contracting clusters $C_2,\ldots, C_r$ into a super-node, that we denote by $v^{\rig}_1$, and then deleting self-loops on it.
So $V(G_1)=V(C_1)\cup \set{v^{\rig}_{1}}$ and $\delta_{G_1}(v^{\rig}_{1})=\hat E_1\cup E^{\rig}_1$.
The rotation of a vertex $v\in V(C_1)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\rig}_1$ is defined in a similar way as $\oset^{\rig}_i$ for any index $2\le i\le r-1$.
Graph $G_r$ is obtained from $G$ by contracting clusters $C_1,\ldots, C_{r-1}$ into a super-node, that we denote by $v^{\lef}_r$, and then deleting self-loops on it.
So $V(G_r)=V(C_r)\cup \set{v^{\lef}_{r}}$ and $\delta_{G_r}(v^{\lef}_{r})=\hat E_{r-1}\cup E^{\lef}_r$.
The rotation of a vertex $v\in V(C_r)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\lef}_r$ is defined in a similar way as $\oset^{\lef}_i$ for any index $2\le i\le r-1$.


We will use the following claims later for completing the proof of \Cref{thm: disengagement - main} in the special case.

\begin{observation}
\label{obs: disengaged instance size}
$\sum_{1\le i\le r}|E(G_i)|\le O(|E(G)|)$, and for each $1\le i\le r$, $|E(G_i)|\le m/\mu$. \znote{parameter?}
\end{observation}
\begin{proof}
Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le r}$, each graph of $\set{G_i}_{1\le i\le r}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node, so each edge of $G_i$ corresponds to an edge in $E(G)$.
Therefore, for each $1\le i\le r$, 
$$|E(G_i)|=|E_G(C_i)|+|\delta_G(C_i)|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu.$$

Note that $E(G_i)=E(C_i)\cup \hat E_i\cup \hat E_{i-1}\cup E_i^{\lef} \cup E_i^{\rig}\cup E_i^{\thr}$.
First, each edge of $\bigcup_{1\le i\le r}E(C_i)$ appears in exactly one graphs of $\set{G_i}_{1\le i\le r}$. 
Second, each edge of $\bigcup_{1\le i\le r}\hat E_i$ appears in exactly two graphs of $\set{G_i}_{1\le i\le r}$.
Consider now an edge $e\in E'$. If $e$ connects a vertex of $C_i$ to a vertex of $C_j$ for some $j\ge i+2$, then $e$ will appear as an edge in $E_i^{\rig}\subseteq E(G_i)$ and an edge in $E_j^{\lef}\subseteq E(G_j)$, and it will appear as an edge in $E_k^{\thr}\subseteq E(G_k)$ for all $i<k<j$.
On one hand, we have $\sum_{1\le i\le r}|E_i^{\lef} \cup E_i^{\rig}|\le 2|E(G)|$. 
On the other hand, note that $E_k^{\thr}=E(C_{k-1},C_{k+1})\cup E^{\through}_{k-1}\cup E^{\through}_{k}$, and each edge of $e$ appears in at most two graphs of $\set{G_i}_{1\le i\le r}$ as an edge of $E(C_{k-1},C_{k+1})$.
Moreover, from \Cref{obs: bad inded structure}, $|E^{\through}_{k-1}|\le |\hat E_{k-1}|$ and $|E^{\through}_{k}|\le |\hat E_{k}|$.
Altogether, we have
\begin{equation}
\begin{split}
\sum_{1\le i\le r}|E(G_i)| & =
\sum_{1\le i\le r}\left(
|E(C_i)|+ |\hat E_i|+ |\hat E_{i-1}|+ |E_i^{\lef}| + |E_i^{\rig}|+|E_i^{\thr}|
\right)\\
& = \sum_{1\le i\le r}
|E(C_i)|+ \sum_{1\le i\le r} \left(|E_i^{\lef}| + |E_i^{\rig}|\right)+ \sum_{1\le i\le r}\left(|E_i^{\thr}|+ |\hat E_i|+ |\hat E_{i-1}|\right)\\
& \le |E(G)|+ 2\cdot |E(G)| + \sum_{1\le i\le r}\left(|E(C_{i-1},C_{i+1})|+ 2|\hat E_i|+ 2|\hat E_{i-1}|\right)\\
& \le 8\cdot |E(G)|.
\end{split}
\end{equation}
This completes the proof of \Cref{obs: disengaged instance size}.
\end{proof}


\begin{observation}
\label{obs: rotation for stitching}
For each $1\le i\le r-1$, if we view the edge in $\delta_{G_i}(v^{\rig}_i)$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})$ as edges of $E(G)$, then $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$, and moreover, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{observation}
\begin{proof}
	Recall that for each $1\le i\le r-1$, 
	$\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})=\hat E_{i}\cup E^{\thr}_{i+1}\cup E^{\lef}_{i+1}$. From the definition of sets $E_i^{\thr},E_{i+1}^{\thr}, E^{\rig}_i, E^{\lef}_{i+1}$,
	\[
	\begin{split}
	E_i^{\thr}\cup E^{\rig}_i
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i<j'\text{ or }i'=i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'\le i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'< i+1\le j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i+1<j'\text{ or }i'<i+1=j'}=E^{\thr}_{i+1}\cup E^{\lef}_{i+1}.
	\end{split}
	\]
	Therefore, $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$.
	Moreover, from the definition of path sets $\wset^{\rig}_i$ and $\wset^{\lef}_{i+1}$, it is not hard to verify that, for every edge $e\in \delta_{G_i}(v^{\rig}_i)$, the path in $\wset^{\rig}_i$ that contains $e$ as its first edge is identical to the path in $\wset^{\lef}_{i+1}$ that contains $e$ as its first edge. According to the way that rotations $\oset^{\rig}_i,\oset^{\lef}_{i+1}$ are defined, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{proof}





\subsubsection{Completing the Proof of \Cref{thm: disengagement - main} in the Special Case}
\label{sec: path case with no problematic index}

In this section we complete the proof of \Cref{thm: disengagement - main} in the special case where the Gomory-Hu tree of $H=G_{\mid \cset}$ is a path and we are additionally given, for each edge $e\in E'$, an inner path $P_e$ in graph $H$, such that set $\set{P_e}_{e\in E'}$ of paths causes congestion at most $\eta$ in $H$, for some $\eta=2^{O((\log m)^{3/4}\log\log m)}$.
Specifically, we use the following two claims, whose proofs will be provided later.

\begin{claim}
\label{claim: existence of good solutions special}
$\expect{\sum_{1\le i\le r}\optcrors(G_i,\Sigma_i)}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$.
\end{claim}

\begin{claim}
	\label{claim: stitching the drawings together}
	There is an efficient algorithm, that given, for each $1\le i\le r$, a feasible solution $\phi_i$ to the instance $(G_i,\Sigma_i)$, computes a solution to the instance $(G,\Sigma)$, such that $\cro(\phi)\le \sum_{1\le i\le r}\cro(\phi_i)$.
\end{claim}

We use the algorithm described in~\Cref{sec: guiding and auxiliary paths} and~\Cref{sec: compute advanced disengagement}, and return the disengaged instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ as the collection of sub-instances of $(G,\Sigma)$. 
From the previous subsections, the algorithm for producing the sub-instances is efficient.
On the other hand, it follows immediately from \Cref{obs: disengaged instance size}, \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together} that the sub-instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ satisfy the properties in \Cref{thm: disengagement - main}.
This completes the proof of \Cref{thm: disengagement - main}.

We now provide the proofs of \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together}.

$\ $

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
Let $\phi^*$ be an optimal drawing of the instance $(G,\Sigma)$.
We will construct, for each $1\le i\le r$, a drawing $\phi_i$ of $G_i$ that respects the rotation system $\Sigma_i$, based on the drawing $\phi^*$, such that $\sum_{1\le i\le r}\cro(\phi_i)\le O((\cro(\phi^*)+|E(G)|)\cdot 2^{O((\log m)^{3/4}\log\log m)})$, and \Cref{claim: existence of good solutions special} then follows.
	
	\paragraph{Drawings $\phi_2,\ldots,\phi_{r-1}$.}
	First we fix some index $2\le i\le r-1$, and describe the construction of the drawing $\phi_i$. We start with some definitions.
	Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
	We define the auxiliary path set $\wset_i=\wset^{\lef}_i\cup \wset^{\rig}_i$, so 
	$$\wset_i=\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}\cup \set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}},$$
	where for each $e\in E^{\lef}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$; for each $e\in E^{\rig}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between $u_{i+1}$ and its last endpoint; and for each $e\in E^{\thr}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$, the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$, and the subpath of $P_e$ between $u_{i+1}$ and its last endpoint.
	
\iffalse
	We use the following observation.
	\begin{observation}
		\label{obs: wset_i_non_interfering}
		The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
	\end{observation}
	\begin{proof}
		Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
		And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
		Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
		From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
	\end{proof}
\fi
	
	
	For uniformity of notations, for each edge $\hat e\in \hat E_i$, we rename the path $Q_{i+1}(\hat e)$ by $W_{\hat e}$, and similarly for each edge $\hat e\in \hat E_{i-1}$, we rename the path $Q_{i-1}(\hat e)$ by $W_{\hat e}$. Therefore, $\wset_i=\set{W_e\mid e\in E(G_i)\setminus E(C_i)}$.
	Put in other words, the set $\wset_i$ contains, for each edge $e$ in $G_i$ that is incident to $v^{\lef}_i$ or $v^{\rig}_i$, a path named $W_e$.
	It is easy to see that all paths in $\wset_i$ are internally disjoint from $C_i$.
	We further partition the set $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_e\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.
	
	We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
	Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
	We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
	Specifically, we proceed in the following four steps.
	
	
	
	\paragraph{Step 1.}
	For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
	We denote by $\Pi_e$ the set of these curves.
	We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
	Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
	and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
	In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
	And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
	Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
	We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.
	
	%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
	We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
	%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
	For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
	Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
	Therefore, $\hat{\chi}_i(P)$ is well-defined.
	For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.
	
	\iffalse
	We use the following observation.
	\znote{maybe remove this observation?}
	
	%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.
	
	\begin{observation}
		\label{obs: curves_crossings}
		The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
		%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
		and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
	\end{observation}
	\begin{proof}
		We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
		Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
		Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
		It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		
		We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
		Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
		It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	\end{proof}
	\fi
	
	\paragraph{Step 2.}
	For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
	We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
	Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
	We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
	(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
	%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
	(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
	(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
	\iffalse{just for backup}
	\begin{proof}
		Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
		For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
		We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
		It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
		We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
		See Figure~\ref{fig: curve_con} for an illustration.
		Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
		It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
		Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
		Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
		Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	\end{proof}
	\begin{figure}[h]
		\centering
		\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
		\hspace{1pt}
		\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
			\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
		\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
	\end{figure}
	\fi
	
	%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
	We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
	This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
	We use the following observation.
	\begin{observation}
		\label{obs: general_position}
		Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
	\end{observation}
	\begin{proof}
		From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
	\end{proof}
	
	
	
	
	%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.
	
	
	\paragraph{Step 3.} 
	So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
	where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
	and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
	Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
	Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
	Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
	We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
	We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.
	
	
	Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
	Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
	It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
	However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.
	
	
	
	
	
	\paragraph{Step 4.}
	Let $\dset$ be an arbitrarily small disc around $z_{\rig}$ in the drawing $\phi'_i$, and let $\dset'$ be another small disc around $z_{\rig}$ that is strictly contained in $\dset$.
	We first erase the drawing of $\phi'_i$ inside the disc $\dset$, and for each edge $e\in \delta(v^{\rig}_i)$, we denote by $p_{e}$ the intersection between the curve representing the image of $e$ in $\phi'_i$ and the boundary of $\dset$.
	We then place, for each edge $e\in \delta(v^{\rig}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{\rig}_{i}$. 
	We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{\rig}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$.
	Finally, for each edge $e\in \delta(v^{\rig}_i)$, let $\gamma_e$ be the concatenation of (i) the image of $e$ in $\phi'_i$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z_{\rig}$ in $\dset'$.
	We view $\gamma_e$ as the image of edge $e$, for each $e\in \delta(v^{\rig}_i)$. 
	We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$, and therefore it respects the rotation system $\Sigma_i$.
	
	We use the following claim.
	\begin{claim}
		\label{clm: rerouting_crossings}
		The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	\end{claim}
	\begin{proof}
		Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
		From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		
		%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
		For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
		Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
		We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.
		
		We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
		From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
		Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
		%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
		\begin{figure}[h]
			\centering
			\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
			\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
		\end{figure}
	\end{proof}
	
	From the above discussion and Claim~\ref{clm: rerouting_crossings}, for each $2\le i\le r-1$, 
	\[
	\cro(\phi_i)=\chi^2(C_i)+O\left(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right).
	\]
	
	
	
	\iffalse
	We now estimate the number of crossings in $\phi_i$ in the next claim.
	\begin{claim}
		\label{clm: number of crossings in good solutions}
		$\cro(\phi_i)=\chi^2(C_i)+O\left(\sum_{W\in \tilde\wset_i}\cro(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)$.
	\end{claim}
	\begin{proof}
		$2\cdot \sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2=\sum_{v\in V(G)}\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2.$
		\znote{need to redefine the orderings $\oset^{\lef}_i$ and $\oset^{\rig}_i$ to get rid of $\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2$ here, which we may not be able to afford.}
	\end{proof}
	\fi
	
	
	\paragraph{Drawings $\phi_1$ and $\phi_{r}$.}
	The drawings $\phi_1$ and $\phi_{r}$ are constructed similarly. We describe the construction of $\phi_1$, and the construction of $\phi_1$ is symmetric.
	Recall that the graph $G_1$ contains only one super-node $v_1^{\rig}$, and $\delta_{G_1}(v_1^{\rig})=\hat E_1\cup E^{\rig}_1$. We define $\wset_1=\set{W_e\mid e\in E^{\rig}_1}\cup \set{Q_2(\hat e)\mid \hat e\in \hat E_1}$. For each $\hat e\in \hat E_1$, we rename the path $Q_2(\hat e)$ by $W_e$, so $\wset_1$ contains, for each edge $e\in \delta_{G_1}(v^1_{\rig})$, a path named $W_e$ connecting its endpoints to $u_2$. Via similar analysis in \Cref{obs: wset_i_non_interfering}, it is easy to show that the paths in $\wset_1$ are non-transversal with respect to $\Sigma$.
	
	We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
	We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{r-1}$. 
	We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
	Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
	%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
	We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
	Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
	\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
	Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
	\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{r-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]
	
	
	
	
	We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le r}\cro(\phi_i)$.
	Recall that, for each $1\le i\le r$, $\tilde \wset_i=\set{W_e\mid e\in \hat E_{i-1}\cup \hat E_{i-1}\cup E^{\lef}_{i}\cup E^{\rig}_{i}}$, where $E^{\lef}_{i}=E(C_i,\bigcup_{1\le j\le i-2}C_j)$, and 
	$E^{\rig}_{i}=E(C_i,\bigcup_{i+2\le j\le r}C_j)$. Therefore, for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, the path $W_e$ belongs to exactly $2$ sets of $\set{\tilde\wset_i}_{1\le i\le r}$.
	Recall that the path $W_e$ only uses edges of the inner path $P_e$ and the outer path $P^{\out}_e$.
	Let $\tilde\wset=\bigcup_{1\le i\le r}\tilde\wset_i$, from \Cref{obs: edge_occupation in outer and inner paths}, 
	for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, $\cong_G(\tilde\wset,e)=O(1)$, and
	for $1\le i\le r$ and for each edge $e\in E(C_i)$, $\cong_G(\tilde\wset,e)=O(\cong_G(\qset_i,e))$.
	
	Therefore, on one hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{W\in \tilde\wset_i}\hat\chi_i(W)
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} 2\cdot \cong_G(\tilde \wset,e)\cdot\cong_G(\tilde \wset,e')\\
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} \left(\cong_G(\tilde \wset,e)^2+\cong_G(\tilde \wset,e')^2\right)\\
	& \le 
	\sum_{e\in E(G)} \chi(e)\cdot \cong_G(\tilde \wset,e)^2
	= O(\cro(\phi^*)\cdot\temp),
	\end{split}
	\]
	and on the other hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2
	%= \sum_{e\in E(G)} \sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)^2 
	& \le  \sum_{e\in E(G)} \left(\sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)\right)^2\\
	& \le O\left(\sum_{e\in E(G)} \cong_G(\tilde \wset,e)^2 \right)\\
	& \le O\left(|E(G)|+\sum_{1\le i\le r}\sum_{e\in E(C_i)} \cong_G(\qset_i,e)^2\right)=O(|E(G)|\cdot\temp).
	\end{split}
	\]
	Moreover, $\sum_{1\le i\le r}\chi^2(C_i)\le O(\cro(\phi^*))$, and $\sum_{1\le i\le r}\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})\le O(\cro(\phi^*)\cdot\temp)$.
	
	Altogether,
	\[
	\begin{split}
	\sum_{1\le i\le r}\cro(\phi_i)
	& \le 
	O\left(\sum_{1\le i\le r} 
	\left(
	\chi^2(C_i)+ \hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)
	\right)\\
	& \le O(\cro(\phi^*))+O(\cro(\phi^*)\cdot\temp)+O(\cro(\phi^*)\cdot\temp)+O(|E(G)|\cdot\temp)\\
	& \le O((\cro(\phi^*)+|E(G)|)\cdot\temp).
	\end{split}
	\]
	
	This completes the proof of \Cref{claim: existence of good solutions special}.
\end{proofof}






$\ $



\iffalse
We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

We first define an instance $(\hat G_i,\hat\Sigma_i)$ as follows. We start with the subgraph of $G$ induced by all edges of $E_G(C_i)$ and $E(\wset_i)$, and then create, for each edge $e$ in the subgraph, $\cong_{\wset_i}(e)$ parallel copies of it. This finishes the description of graph $\hat G_i$.
For each vertex $v$ in $\hat G_i$, we define its rotation $\hat\oset_v$ as follows. We start with the rotation $\oset_v\in \Sigma$, and then replace, for each edge $e\in E(\wset_i)$, the edge $e$ in the ordering $\oset_v$ by its $\cong_{\wset_i}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, where the ordering among the copies is arbitrary. 
On the one hand, in graph $\hat G_i$, we can make paths of $\wset_i$ edge-disjoint by letting, for each edge $e\in E(\wset_i)$, each path of $\wset_i$ that contains $e$ now take a distinct copy of $e$ in $\hat G_i$.
On the other hand, a drawing $\hat \phi_i$ of the instance $(\hat G_i,\hat\Sigma_i)$ can be easily computed from $\phi^*$, as follows.
We start with $\hat\phi'_i$, the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$. Then for each edge of $\wset_i$, let $\gamma_e$ be the curve that represents the image of $e$, and we create $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting endpoints of $e$, that lies in an arbitrarily thin strip around $\gamma_e$. We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

For each edge $e\in E_G(C_i)$, we denote by $\gamma_e$ the curve in $\hat \phi_i$ that represents the image of $e$; and for each path $W\in \wset_i$, we denote by $\gamma_W$ the curve in $\hat \phi_i$ that represents the image of $W$.
We define $\Gamma_0=\set{\gamma_e\mid e\in E_G(C_i)}$ and $\Gamma_1=\set{\gamma_W\mid W\in \wset_i}$. It is immediate to verify that the sets $\Gamma_0,\Gamma_1$ of curves satisfy the condition of \Cref{thm: type-2 uncrossing}. We then apply the algorithm in \Cref{thm: type-2 uncrossing} to $\Gamma_0,\Gamma_1$, and let $\Gamma_1'$ be the set of curves that we obtain.
From \Cref{thm: type-2 uncrossing}, the curves in $\Gamma_1'$ do not intersect internally between each other, and have the same sets of first endpoints and last endpoints.
We now show that we can obtain a drawing $\phi_i$ of the instance $(G_i,\Sigma_i)$ using the curves $\Gamma_0,\Gamma_1'$.
For each edge $e\in E_G(C_i)$, we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
For each edge path $W\in \wset$, from \Cref{thm: type-2 uncrossing}, there is a curve $\gamma'\in \Gamma_1'$ connecting the endpoint of $W$ to we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
\znote{maybe we need another type of uncrossing here.}
\fi



\begin{proofof}{Claim~\ref{claim: stitching the drawings together}}
	We first define a set $\set{(U_i,\Sigma'_i)\mid 1\le i\le r}$ of instances of \CNwRS as follows.
	We define $U_1=G$, and for each $2\le i\le r$, we define $U_i$ to be the graph obtained from $G$ by contracting the clusters $C_1,\ldots, C_{i-1}$ into a vertex $v^{\lef}_i$.
	Note that each edge in $U_i$ is also an edge in $G$, and we do not distinguish between them.
	Note that $U_1=G$, we define the rotation system $\Sigma'_1$ on $U_1$ to be $\Sigma$.
	For each $2\le i\le r$, we define the rotation system $\Sigma'_i$ on $U_i$ as follows.
	For each vertex $v\in \bigcup_{i\le t\le r}V(C_t)$, note that its incident edges in $U_i$ are the edges of $\delta_G(v)$, and its rotation in $\Sigma'_i$ is defined to be $\oset_v$, the rotation on $v$ in the input rotation system $\Sigma$.
	For vertex $v^{\lef}_i$, note that its incident edges are the edges of $\delta_{G_i}(v^{\lef}_i)$, and its rotation in $\Sigma'_i$ is defined to be $\oset^{\lef}_i$, the rotation on $v^{\lef}_i$ of instance $(G_i,\Sigma_i)$.
	
	
	Note that $U_k=G_k$ and $\Sigma'_k=\Sigma_k$, so the drawing $\phi_k$ of the instance $(G_k,\Sigma_k)$ is also a drawing of the instance $(U_k,\Sigma'_k)$. For clarity, when we view this drawing as a solution to the instance $(U_k,\Sigma'_k)$, we rename it by $\psi_k$.
	We will sequentially, for $i=r-1,\ldots,1$, compute a drawing of the instance $(U_i,\Sigma'_i)$ using the drawing $\psi_{i+1}$ of $(U_{i+1},\Sigma'_{i+1})$ and the drawing $\phi_i$ of $(G_{i},\Sigma_{i})$, and eventually, we return the drawing $\psi_1$ of $(U_{1},\Sigma'_{1})$ as the solution to the instance $(G,\Sigma)$.
	
	We now fix an index $1\le  i< r-1$ and construct the drawing $\psi_i$ to the instance $(U_{i},\Sigma'_{i})$, assuming that we have computed a drawing $\psi_{i+1}$ to the instance $(U_{i+1},\Sigma'_{i+1})$, as follows.
	Recall that $V(G_i)=V(C_i)\cup\set{v^{\lef}_i,v^{\rig}_i}$ if $i\ge 2$ and $V(G_i)=V(C_i)\cup\set{v^{\rig}_i}$ if $i=1$, and $\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.  Moreover, from \Cref{obs: rotation for stitching} and the definition of instance $(U_{i+1},\Sigma'_{i+1})$, the rotation on $v^{\rig}_i$ in $\Sigma_{i}$ is identical to the rotation on $v^{\lef}_{i+1}$ in $\Sigma'_{i+1}$.
	Denote $F=\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.
	Let $\dset$ be an arbitrarily small disc around the image of $v_{i+1}^{\lef}$ in $\psi_{i+1}$. For each edge $e\in F$, we denote by $p_e$ the intersection between the image of $e$ with the boundary of $\dset$. 
	Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset$ is $\oset^{\lef}_{i+1}$.
	We erase the drawing of $\psi_{i+1}$ inside the disc $\dset$, and view the area inside the disc $\dset$ as the outer face of the drawing.
	Similarly, let $\dset'$ be an arbitrarily small disc around the image of $v_{i}^{\rig}$ in $\phi_{i}$. For each edge $e\in F$, we denote by $p'_e$ the intersection between the image of $e$ with the boundary of $\dset'$. 
	Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is $\oset^{\rig}_{i}$.
	We erase the drawing of $\phi_{i}$ inside the disc $\dset'$, and let $\dset''$ be another disc that is strictly contained in $\dset'$. We now place the drawing of $\psi_{i+1}$ inside $\dset'$ (after we erase part of it inside $\dset$), so that the boundary of $\dset$ in $\psi_{i+1}$ coincide with the boundary of $\dset''$ in $\phi_{i}$, while the interior of $\dset$ coincides with the exterior of $\dset''$. We then compute a set $\set{\zeta_e\mid e\in F}$ of curves lying in $\dset'\setminus \dset''$, where for each $e\in F$, the curve $\zeta_e$ connects $p'_e$ to $p_e$, such that all curves of $\set{\zeta_e\mid e\in F}$ are mutually disjoint. Note that this can be done since the order in which $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is identical to $\set{p'_e}_{e\in F}$ appear on the boundary of $\dset$.
	We denote by $\psi_i$ the resulting drawing we obtained.
	See Figure~\ref{fig: stitching} for an illustration.
	Clearly, $\psi_i$ is a drawing of $U_i$ that respects $\Sigma'_i$ if we view, for each edge $e\in F$, the union of (i) the image of $e$ in $\phi_i$ outside the disc $\dset'$; (ii) the curve $\zeta_e$; and (iii) the image of $e$ in $\psi_{i+1}$ inside the disc $\dset''$, as the image of $e$.
	\begin{figure}[h]
		\centering
		\subfigure[The drawing $\psi_{i+1}$, where the boundary of $\dset$ is shown in dash black.]{\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_1.jpg}}%\label{fig:non_crossing_representation}
		}
		\hspace{0.45cm}
		\subfigure[The drawing $\psi_{i+1}$ after we erase its part inside $\dset$ and view the interior of $\dset$ as the outer face.]{
			\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_2.jpg}}}
		\hspace{0.45cm}
		\subfigure[The drawing $\psi_i$, where the curves of $\set{\zeta_e\mid e\in F}$ are shown in dash line segments.]{
			\scalebox{0.36}{\includegraphics[scale=1.0]{figs/stitching_3.jpg}}}
		\caption{An illustration of constructing the drawing $\psi_i$ from $\psi_{i+1}$.}\label{fig: stitching}
	\end{figure}
	Clearly, any crossing in the drawing $\psi_i$ is either a crossing of $\phi_i$ or a crossing of $\psi_{i+1}$, so $\cro(\psi_i)\le \cro(\psi_{i+1})+\cro(\phi_{i})$.
	Therefore, if we rename the drawing $\psi_1$ of the instance $(U_1,\Sigma'_1)$ by $\phi$, then $\phi$ is a drawing of $G$ that respects $\Sigma$, and $\cro(\phi)\le \sum_{1\le i\le r}\cro(\phi_i)$.
\end{proofof}























==> disengagement.tex <==

\section{Disengagement of Clusters -- Proof of  Theorem \ref{thm: disengagement}}
\label{sec:disengagement}

This section is dedicated to the proof of Theorem \ref{thm: disengagement}. We start by defining a laminar family of cuts, and stating two main theorem for disengaging clusters in such a family.


\subsection{Laminar Family of Cuts}

\mynote{A useful trick: For each cluster $C\in \cset$, make $n_e$ extra copies of each edge $e$, where $n_e$ is the number of times $e$ participates in paths in $\qset(C)$. Because the cost of $\qset(C)$ is small, the number of new crossings introduced will be small. This is done before the disengagement. But from now on we can assume that all paths sets $\qset(C)$ (and also $\pset(C)$ because of how they are constructed) are edge-disjoint. So we don't need to deal with $\cost(\pset,\qset)$ which is tricky to figure out, and instead can just do $\cro(\pset,\qset)$ which is easier.  In the following subsections we are still using costs and we are not assuming that paths sets $\pset(S),\qset(S)$ are edge-disjoint, but it will be better to switch to this to make things cleaner and simpler.}





Suppose we are given a cluster $S$, a vertex $u\in S$, and a set $\qset$ of paths connecting $\delta(S)$ to $u$ inside $S$, such that the paths in $\qset$ are locally non-interfering. We define a circular ordering $\oset_{\qset}(\delta(S))$ of the edges in $\delta(S)$, as follows. Recall that $\qset=\set{Q(e)\mid e\in \delta(S)}$, and path $Q(e)$ connects the endpoint of edge $e$ lying in $S$ to the vertex $u$. Denote by $\hat e$ the last edge on path $Q(e)$. Consider the multi-set $\hat E=\set{\hat e\mid e\in \delta(S)}$ of edges (this set is a multi-set, since it is possible that, for a pair $e,e'\in \delta(S)$ of edges, $e\neq e'$ but $\hat e=\hat e'$). We define a circular ordering $\hat \oset$ of the edges of $\hat E$ as follows: the ordering is consistent with the ordering $\oset_u\in \Sigma$ of the edges of $\delta(u)$, where ties (between copies of the same edge) are broken arbitrarily \znote{maybe not arbitrarily? if $e\ne e'$ and $\hat e=\hat e'$, then probably we need to go to the other endpoint of $\hat e=\hat e'$ (let's call it $u'$) and look at what edges of $\delta(u')$ the paths $Q(e)$ and $Q(e')$ uses and then determine how to break this tie according to the ordering $\oset_{u'}$} \mynote{It is OK to make the ordering arbitrary because the costs of paths in $\qset$ will be low, so reordering paths terminating at the same edge is fine. In the laminar family = path case we won't have a single $u'$ vertex so we may be forced to use this sort of ordering. Also it's not immediately clear that we can order according to $u'$ because the orientations are not fixed. HOwever: if we do the fix with introducing many copies of each edge, making the paths in $\qset$ edge-disjoint and fixing some ordering of resulting edges around each vertex, this issue won't arise}. The ordering $\hat \oset$ of the edges in $\hat E$ immediately defines the circular ordering $\oset_{\qset}(\delta(S))$ of the edges in $\delta(S)$: if circular ordering of the edges in $\hat E$ is $\hat e_1,\hat e_2,\ldots,\hat e_r$, then the corresponding ordering of the edges in $\delta(S)$ is $e_1,e_2,\ldots,e_r$. We say that $\oset_{\qset}(\delta(S))$ is the \emph{ordering of the edges of $\delta(S)$ determined by $\qset$}. Intuitively, the ordering $\oset_{\qset}(\delta(S))$ is determined by the order in which the images of the paths in $\qset$ enter the vertex $u$ in any feasible solution to instance $(G,\Sigma)$ of the problem.


\subsection{Disengagement Algorithm}
Suppose we are given an instance $(G,\Sigma)$ of \CNwRS, and a laminar family $\lset$ of sub-graphs of $G$, with $G\in \lset$. Assume further that for every cluster $S\in \lset$, graph $S\setminus \bigcup_{S'\in \wset}S'$ is non-empty, and that we are given a vertex $u(S)\in S\setminus\bigcup_{S'\in \wset}S'$, together with a set $\qset(S)$ of paths, routing the edges of $\delta(S)$ to $u(S)$ inside $S$, so that the paths in $\qset(S)$ are locally non-interfering. Assume further that for every cluster $S\in \lset\setminus\set{G}$, we are given a set $\pset(S)$ of paths, routing the edges of $\delta(S)$ to $u'(S)$ outside $S$, where $S'$ is the parent-cluster of $S$, so that the paths in $\pset(S)$ are locally non-interfering.

We construct a new family $\fset=\set{(G_S,\Sigma_S)\mid S\in \lset}$ of instances of \CNwRS, that are sub-instances of $(G,\Sigma)$, as follows.

Consider the cluster $S\in \lset$. 
In order to construct the instance $(G_S,\Sigma_S)$, we start with the graph $S'$, where $S'$ is the parent-cluster of $S$, if $S\neq G$, and $S'=G$ otherwise. If $S\neq G$, then we create a super-node $v^*$, by contracting all vertices in $S'\setminus S$ into a single vertex. Notice that the edges incident to $v^*$ correspond to the edges of $\delta(S)$ (for simplicity, we will not distinguish between them). The circular ordering of the edges incident to $v^*$ is $\oset_{\qset(S)}(\delta(S))$ (the order in which the corresponding paths in $\qset(S)$ enter $u(S)$).
Next, we denote $\wset(S)=\set{S_1,\ldots,S_q}$. For all $1\leq i\leq q$, we contract all vertices of $S_i$ into a super-node $v_i$. Notice that the edges incident to $v_i$ correspond to the edges of $\delta(S_i)$; we do not distinguish between them. The ordering of the edges incident to $v_i$ in the new instance is determined by $\oset_{\qset(S_i)}(\delta(S_i))$ -- the order in which the corresponding paths in $\qset(S_i)$ enter $u(S_i)$.

This completes the definition of the family $\fset$ of instances. We need the following observation.

\begin{observation}\label{obs: new graph}
	For all $S\in \lset$, graph $G_S$ contains all edges of $S\setminus\bigcup_{i=1}^qS_i$, and the total number of all additional edges in $G_S$ is bounded by $|\delta(S')|+\sum_{i=1}^q|\delta(S_i)|$. 
Moreover, $\sum_{S\in \lset}|E(S)|\leq |E(G)|+\sum_{S\in \lset}|\delta(S)|$.
\end{observation}


Next, we show that the sum of optimal solution costs of the resulting instances is bounded.


\begin{lemma}\label{lem: disengagement - type 1}
$\sum_{S\in \lset}\optcrors(G_S,\Sigma_S)\leq O(\optcrors(G,\Sigma))+O\left (\sum_{S\in \lset}\cost(\qset(S))+\cost(\qset(S),\pset(S))\right )$.
\end{lemma}
The proof of the lemma is somewhat technical and deferred to Section \ref{subsec: type 1 disengagement}.
Lastly, we show that the solutions to instances in $\fset$ can be combined together to obtain a solution to instance $(G,\Sigma)$.

\begin{lemma}\label{lem: disengagement putting together}
	There is an efficient algorithm, that, given, for every instance $(G_S,\Sigma_S)\in \fset$, a solution $\phi_S$ of cost $\chi_S$, constructs a solution to instance $(G,\Sigma)$ of cost at most $\sum_{(S,\Sigma)\in \fset}\chi_S$.
\end{lemma}

The proof of the lemma appears in Section \ref{sec: disengagement putting together}.







\subsection{Cost of Disengagement: Proof of Lemma \ref{lem: disengagement - type 1}}
\label{subsec: type 1 disengagement}


\mynote{this is copied from the log}
We start with the graph $G$, and we consider the child clusters of $G$ one-by-one. Starting with the optimal drawing of $G$, we then ``pull'' the drawing of each child $S$ of $G$ out of $G$ (just like we did with the clusters in $\cset$). Then we repeat the procedure with each child cluster of $G$, pulling out the grandchildren.

In order to analyze this, we need to look closer at the procedure of pulling the drawing of a single cluster. So let's consider the child cluster $S$ of $G$. We assume that we are given some current drawing $\phi$ of $G$ (where possibly we have already pulled the drawings of some clusters out). We call this procedure the \emph{disengagement of $S$ from $G$}.

Let us look at this disengagement procedure closer, and let us analyze the increase in the number of crossings due to it. The procedure consists of these steps. For brevity, we denote the edge set $\delta(S)$ by $E'$, its endpoints lying in $S$ by $X$, and its endpoints lying in $G\setminus S$ by $Y$.

%(for simplicity, in the calculation below I'll treat the paths sets $\pset=\pset_S$ and $\qset=\qset_S$ as being edge-disjoint each; will need to revisit the calculations later but I think it's safe to do this).
\begin{itemize}
	\item Take the current drawing $\phi$ of $G$. Make a disc $D$ around $u_S$. Delete from $\phi$ the drawing of $S$ and the drawing of $E'$. Make a small disc $D'$ containing $D$. 
	
	\item Add back the paths in $\qset\cup E'$, so that they terminate at the boundary of $D'$. For every edge $e\in E'$, let $\gamma(e)$ be the drawing of the path in $\qset$ that used to terminate at an endpoint of $e$ that lies in $X$. We \emph{uncross} the curves $\gamma(e)$ so they don't cross each other. Therefore, the number of crossings that curves in $\Gamma=\set{\gamma(e)\mid e\in E'}$  cause can be bounded by the following:
	
	\begin{itemize}
		\item $\cro(\qset,G\setminus (S\cup E'\cup \pset)$;
		\item $\cro(\qset,\pset)$;
		\item $\cro(E',G\setminus (S\cup E'\cup \pset))$;
		\item $\cro(E',\pset)$.
	\end{itemize}
	This is because we do not allow the drawings of the curves in $\Gamma$ to cross themselves.
	
	\item Consider the original optimal drawing $\phi^*$ of $G$. Delete from this drawing everything, except for $S,E',\pset$. For every edge $e\in E'$, the curve obtained by concatenating the drawing of the edge $e$ of $E'$ incident to $x$, and the corresponding path of $\pset$ is denote by $\gamma'(e)$. Let $\Gamma'=\set{\gamma'(e)\mid e\in E'}$. We uncross the curves $\Gamma'$ as before. Then we place the resulting drawing in disc $D$, so that the curves of $\Gamma'$ terminate on its boundary. The total number of crossings caused by the curves in $\Gamma'$ is bounded by the following;
	
	
	\begin{itemize}
		\item $\cro(\pset, S\setminus \qset)$;
		\item $\cro(\pset,\qset)$;
		\item $\cro(E',S\setminus \qset)$;
		\item $\cro(E',\qset)$.
	\end{itemize}
	
	So far increase in the total number of crossings that we have obtained 
	can be bounded by $\cro(\pset,\qset)$. Now it remains to reorder the curves in $\Gamma$ and in $\Gamma'$ so the order in which they hit the boundary of $D$ or $D'$ is the same as the order of the paths in $\qset$ around $u_S$.
	
	\item First reordering: Consider the part of the drawing inside the disc $D$. By concatenating the paths in $\qset$ with the curves in $\Gamma'$, we get a collection $\Gamma_1$ of curves connecting $u$ to the boundary of $D$. The order in which these paths leave $u$ and the order in which they arrive at the boundary of $D$ may be different, because these curves may cross. The number of such crossings though is at most: $\cro(\qset,\qset)+\cro(\qset,E')+\cro(\qset,\pset)$, because the curves in $\Gamma'$ are not allowed to cross each other. By doing the same crossings in the opposite order, we can ensure that the ordering of the curves in $\Gamma_1$ as they hit the boundary of $D$ is the same as their ordering in which they leave $u$. This increases the number of crossings by an additional $\cro(\qset,\qset)+\cro(\qset,E')+\cro(\qset,\pset)$.
	
	\item Second reordering: now we consider the part of the drawing outside the disc $D$. By concatenating the images of the paths in $\pset$ and the curves in $\Gamma$, we obtain the set $\Gamma_2$ of curves. Recall that we have uncrossed the curves in $\Gamma$. If we did not uncross them, then the order in which the curves in $\Gamma_2$ hit the boundary of $D'$ would be exactly the right order -- the order in which the paths in $\qset$ hit $u$. So we could redo all these crossings to achieve the right order. The total number of such crossings is bounded by $\cro(\qset,E')+\cro(\qset,\qset)+\cro(E',E')$. (note that the term $\cro(E',E')$ is not an actual increase in the number of crossings, because these crossings are present in the drawing of $G$ and we haven't used them yet).
\end{itemize}

Summing everything up, the total increase in the number of crossings due to the disengagement of $S$ is bounded by:

\[ 2\cro(\pset,\qset)+2\cro(\qset,\qset)+\cro(\qset,E') \]

This is bounded by a constant times the number of crossings in which the edges of $\qset$ participate. So if every edge of $G$ participates in at most $\poly\log n$ sets $\qset_S$, the total increase due to disengagement of all clusters is at most $\cro\poly\log n$.




%\subsection{Combining Disengaged Solutions: Proof of Lemma \ref{lem: disengagement putting together}}\label{sec: disengagement putting together}












\iffalse
\subsection{Step 1: Computing a Laminar Family of Clusters}

%Throughout, for any two subgraphs $X,Y$ of $G$, we denote by $\cro(X,Y)$ the total number of crossings in the optimal drawing between edges of $X$ and edges of $Y$. Similarly, for two sets $\pset,\qset$ of paths, we denote by $\cro(\pset,\qset)$ the total number of crossings in the optimal drawing between edges of paths in $\pset$ and edges of paths in $\qset$. The cost of the set $\pset$ of paths is the total number of crossings in which the edges of $\pset$ participate in the optimal drawing of $G$. 


Let $\lset$ be a laminar family of clusters of $G$, with $G\in \lset$. We say that $\lset$ is a \emph{nice} family, iff

\mynote{I think the right thing to do it is not to make any requirements from $\qset_S$ and $\pset_S$, just say that we assume that we are given two such sets of paths. Then say what is the increase in the cost of disengagement as a function of the costs of these sets. By the way, the definition of $\cro(\pset,\qset)$ ignores the fact that the paths in $\qset$ may not be edge-disjoint. It should be defined differently (every crossing between the edge of $\qset$ and the edge of $\pset$ must contribute the product of its congestion in $\pset$ and in $\qset$.)}

\begin{itemize}
\item for every cluster $S\in \lset$, we are given a vertex $u_S\in S$, and a set $\qset_S$ of paths connecting the edges of $\delta(S)$ to $u_S$, such that the cost of the paths in $\qset_S$ is at most $\cro(S,S) \poly\log n$. Important: the paths in $\qset_S$ do not contain the edges of $\delta(S)$.
\item for every cluster $S\in \lset$, we are given a vertex $u'_S\not\in S$, and a set $\pset_S$ of paths connecting the edges of $\delta(S)$ to $u'_S$, such that the total number of crossings between the paths in $\pset_S$ and the edges of $S$ is at most $\cro(S,G)\poly\log n$. Again, the paths in $\pset_S$ do not contain the edges of $\delta(S)$.
\item the total cost of all edges in $\bigcup_S\qset_S$ %\znote{$\bigcup_S(\pset_S\cup \qset_S)$?} 
is bounded by $\cro\poly\log n$.
\end{itemize} 

For every cluster $S\in \lset$, we define a \CNwRS instance $(G_S,\Sigma_S)$, as follows. We start with $S$, and, if $S\neq G$, we add another vertex $v^*$ that represents the parent cluster $S^*$ of $S$. We add an edge $(v^*,u)$ for every edge $(v,u)\in E(G)$ with $v\in S^*$, $u\in S$. Then, for every child cluster $S_i$ of $S$, we contract $S_i$ into a single vertex $v_i$. The ordering of edges around $v^*$ is defined according to the ordering in which the paths in $\qset_S$ hit $u_S$. For each $i$, the ordering of edges around $v_i$ is defined according to the ordering in which the paths in $\qset_{S_i}$ hit $u_{S_i}$.


The main result of this section is the following lemma.

\begin{lemma}
\label{lem:laminar}
Let $\lset$ be a laminar family of clusters of $G$, then
\begin{enumerate}
\item $\sum_{S\in \lset}\optcrors(G_S,\Sigma_S)\le (\log n)^{O(1)}\cdot \optcrors(G,\Sigma)$;
\item if we are given, for each $1\le i\le k$, a drawing $\phi_i\in \Phi(G_i,\Sigma_i)$, then we can efficiently compute a drawing $\phi\in \Phi(G,\Sigma)$, such that $\cro(\phi)\le\sum_{1\le i\le k}\cro(\phi_i)$.
\end{enumerate}
\end{lemma}

Note that, if we can further guarantee that $|E(G_S)|\le |E(G)|/\mu$ for each $S\in \lset$, we will be done. 

The remainder of this section is devoted to prove Lemma~\ref{lem:laminar}.
\fi


==> finish-proof-interesting-backup2.tex <==
\subsubsection{Completing the Proof of \Cref{lem: many paths}}
\label{subsubsec: finish the proof}
Given an input instance $\cI=(\cG,\cSigma)$, we first apply the algorithm from \Cref{thm: phase 1} to this input. If the algorithm fails, then we terminate the algorithm and return FAIL as well. Recall that, from \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/\mu^3$. Assume now that the algorithm from \Cref{thm: phase 1} did not fail. In this case, if  $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then with probability at least $(1-1/\mu^3)$, the algorithm is successful. We denote by $\tilde \event_1'$ the bad event that the application of this algorithm is unsuccessful, so $\prob{\tilde \event_1'}\leq 1/\mu^3$. Let $\iset$ be the collection of subinstances of $\cI$ computed by the algorithm from \Cref{thm: phase 1}. 

Throughout this subsection, we use the universal constant $b^*=2400$.
Recall that, if Event $\tilde \event'_1$ did not happen, then for every instance $I\in \iset$, there is a solution $\psi(I)$ to $I$, that is semi-clean with respect to $\kset(I)$, such that 
$\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$, and $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. We set the parameter $b$ to be a large enough constant, so that $b\geq 4b^*$ holds.
%
Recall that, for every instance $I=(G,\Sigma)\in \iset$, we have denoted by $\hat I=(\hat G,\hat \Sigma)$ the corresponding $\kset(I)$-contracted instance, and by $\hat m(I)=|E(\hat G)|$. We say that instance $I$ is \emph{small} if $\hat m(I)\leq \frac{\cm}{\mu^{b^*}}$, and otherwise it is \emph{large}. 
%We partition the set $\iset$ of instances into three subsets: set $\iset_1$ containing all small instances; and set $\iset_2$ containing all remaining instances.
%set $\iset_2$ containing all large instances $I=(G,\Sigma)\in \iset$ for which either $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{60b}$ holds, and set $\iset_3$ containing all remaining instances.
%Since the algorithm from \Cref{thm: phase 1} guarantees that $\sum_{I\in \iset}\hat m(I)\le \cm$, we get that $|\iset_2|\leq \mu^{b^*}$. We let $\hat \iset_1=\set{\hat I\mid I\in \iset_1}$ contain the set of all contracted instances corresponding to the instances of $\iset_1$, and we define set $\hat \iset_2$ of instances corresponding to the instances of $\iset_2$ similarly.
%\znote{We do not know $\cro(\psi(I))$ and $\chi^{\dirty}(\psi(I))$ so we cannot distinguish $\iset_2$ from $\iset_3$?}

We now proceed in $z= 2\log m$ phases, where in the $j$th phase, we compute the $j$th collection $\iset^{(j)}$ of subinstances of $I$, such that the properties required in \Cref{lem: many paths} are satisfied.

Consider now an index $1\le j\le 2\log m$ and we describe the $j$th phase. Throughout the phase, we use the parameters $g^j_1=2^j$ and $g^j_2=g^j_1\cdot \mu^{b^*}/\cm$.
We intend to apply the algorithm from \Cref{thm: phase 2} to large instances in $\iset$ with parameters $g^j_1,g^j_2$. But note that the algorithm requires that the input instance $I=(G,\Sigma)$ has a skeleton $K(I)$ that is $g_3(I)$-connected in the input graph $G$ (where $g_3(I)=\big(\frac{g_1^j}{|E(G)|}+g_2^j\big)\cdot\mu^{300b}$), which is not necessarily true for the large instances in $\iset$. Therefore, we first pre-process instances in $\iset$, such that the resulting instances are either small or satisfying this connectedness property, as follows.

\newcommand{\tempiset}{\iset_{\sf temp}}
\newcommand{\hattempiset}{\hat{\iset}_{\sf temp}}

\subsubsection*{Pre-processing instances in $\iset$}

The pre-processing procedure is iterative. Throughout, we use a parameter $\tilde g=\big(\frac{g^j_1\mu^{b^*}}{\cm}+g^j_2\big)\cdot\mu^{300b}$.
The procedure maintains a collection $\tempiset$ of subinstances of $I$, that is initialized to be $\tempiset=\iset$. We denote $\hattempiset=\set{\hat I\mid I\in \tempiset}$.
Each instance in $\tempiset$ is either marked \emph{active} or \emph{inactive}. Initially, all large instances are marked active and all small instances are marked inactive.
We will maintain the following invariant throughout the algorithm.
%
\begin{properties}{IP}
\item for each inactive instance $I=(G,\Sigma)\in \tempiset$, either $I$ is small, or $I$ satisfies that, if we denote by $K(I)$ the skeleton of $I$, then $K(I)$ is $\tilde g$-connected in $G$;
\label{prop: inactive}
\item for each instance $\hat I=(\hat G,\hat \Sigma)\in \hattempiset$, either $|E(\hat G)|\le \cm/\mu$, or $\hat I$ is not wide;
\label{prop: wide or not}
\item $\sum_{I\in \tempiset}\hat m(I)\le \cm$; and
\label{prop: number of edges}
\item there exists, for every instance $I\in \tempiset$, a solution $\psi(I)$ to $I$ that is semi-clean with respect to $\kset(I)$, such that
$\sum_{I\in \tempiset}\cro(\psi(I))\le 2\cdot \optcrors(\cI)$, and $\sum_{I\in \tempiset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$.
\label{prop: good drawings}
\end{properties}
%
From \Cref{thm: phase 1} and our initial setting, these invariant holds at the beginning of the pre-processing procedure.

The procedure continues to be executed as long as the collection $\tempiset$ contains an active instance. 
%$\hat m(I)>\cm/\mu^{b^*}$ (that is, instance $I$ is large), and, if we denote by $K(I)$ the skeleton of $I$ that corresponds to its skeleton structure $\kset(I)$, then $K(I)$ is not $\tilde g$-connected in $G$.
We now describe an iteration of the procedure.
Let $I=(G,\Sigma)$ be an active instance in $\tempiset$. If instance $I$ is small, then we mark it inactive and terminate the iteration. Clearly all invariants continue to hold after this iteration in this case.
Assume now that instance $I$ is large. 
Let $\kset(I)=\set{\jset_1,\ldots,\jset_{r}}$ be the skeleton structure for $I$, and for each $1\le i\le r$, let $J_i$ be the core associated with $\jset_i$. 
Consider its $\kset(I)$-contracted instance $\hat I=(\hat G, \hat \Sigma)$. Recall that graph $\hat G$ is obtained from graph $G$ by contracting, for each $1\le i\le r$, all vertices of the core $J_i$ into a supernode $v_{J_i}$. We now compute, for every pair $1\le i<i'\le r$, a minimum $v_{J_i}$-$v_{J_{i'}}$ cut in $\hat G$.
If for all pairs $1\le i<i'\le r$, the $v_{J_i}$-$v_{J_{i'}}$ minimum-cut in $\hat G$ has value at least $\tilde g$, then we simply mark the instance $I$ in $\iset$ inactive, and terminate this iteration.
Clearly all invariants continue to hold after this iteration in this case.
Assume now that there exists a pair $1\le i<i'\le r$, such that the $v_{J_i}$-$v_{J_{i'}}$ minimum-cut in $\hat G$ has value less than $\tilde g$. 
%Let $(A,B)$ be the $v_{J_i}$-$v_{J_{i'}}$ cut that we computed.
Let $\hat G_1,\ldots,\hat G_s$ be the graphs obtained from $\hat G$ by deleting the edge of the minimum-cut. Consider now an $1\le i\le s$. Assume that supernodes corresponding to cores $J_{p_1},\ldots, J_{p_t}$ belong to graph $\hat G_i$. 
We define instance $I_i=(G_i,\Sigma_i)$ as follows. Graph $G_i$ is the graph obtained from $\hat G_i$ by un-contracting every supernode $v_{J_{p_q}}$ back to its corresponding core $J_{p_q}$, so $G_i$ is a subgraph of $G$, and $\Sigma_i$ is the rotation system on $G_i$ that is induced by $\Sigma$. We then define its core structure to be $\kset(I_i)=\set{\jset_{p_1},\ldots,\jset_{p_q}}$.
We then replace the instance $I$ in $\tempiset$ with new instances $I_1,\ldots,I_s$, all marked active, and terminate this iteration.

We now verify that all invariants continue to hold after this iteration in this case.
First, since we marked all new instance that are added to collection $\tempiset$ active, Invariant \ref{prop: inactive} holds.
Second, since for every new instance $I_i=(G_1,\Sigma_i)$, graph $G_i$ is a subgraph of $G$, and $\hat G_i$ is a subgraph of $\hat G$. If $|E(\hat G)|\le \cm/\mu$, then $|E(\hat G_i)|\le \cm/\mu$; if $\hat I$ is node wide, then $\hat I_i$ is also not wide. Therefore,
\ref{prop: wide or not} holds.
Third, since $\hat G_1\cup\ldots\cup\hat G_s\subseteq \hat G$, $\sum_{1\le i\le s}\hat m(I_i)\le \hat m(I)$ and so
\ref{prop: number of edges} holds.
Last, note that the Invariant \ref{prop: good drawings} holds before this iteration. Let $\psi(I)$ be the semi-clean solution associated with instance $I$. We simply define, for each $1\le i\le s$,  $\psi(I_i)$ to be the drawing of $G_i$ induced by drawing $\psi(I)$. It is easy to verify that $\psi(I_i)$ is a semi-clean solution to $I_i$ with respect to its skeleton structure. Moreover, since $G_1,\ldots,G_s$ are disjoint subgraphs of $G$,  
$\sum_{1\le i\le s}\cro(\psi(I_i))\le \cro(\psi(I))$, and $\sum_{1\le i\le s}|\chi^{\dirty}(\psi(I_i))|\leq  |\chi^{\dirty}(\psi(I))|$.
Therefore, \ref{prop: good drawings} also holds.

Note that the collection of all cores in all skeleton structures is never changed, and initially, the number of cores in all active instances in $\iset$ is at most $\mu^{b^*}\cdot \mu^{100}$ (since the number of active instances is at most $\mu^{b^*}$ and each such instances has at most $\mu^{100}$ cores). When the pre-processing process terminates, every resulting instance contains at least one core.
Therefore, the number of iterations is at most $\mu^{b^*}\cdot \mu^{100}$. Note that in each iteration we have deleted at most $\tilde g$ edges. Therefore, if we denote by $\hat E_{\sf temp}$ the set of all deleted edges throughout this procedure, then
$|\hat E_{\sf temp}|\le \mu^{b^*}\cdot \mu^{100}\cdot \tilde g$.

Let $\iset^*$ be the resulting collection we obtained at the end of the pre-processing procedure. Since all instances in $\iset^*$ are inactive, from Invariant \ref{prop: inactive}, for each instance $I=(G,\Sigma)\in \iset^*$, either $I$ is small, or its skeleton $K(I)$ is $\tilde g$-connected in $G$.
Moreover, it is easy to verify that, for each instance $I\in \iset^*$, its skeleton structure has size at most $\mu^{100}$.

Denote $\hat \iset^*=\set{\hat I\mid I\in \iset^*}$. We prove the following observation.

\begin{observation}
\label{obs: algo combine drawings}
There is an efficient algorithm, that, given a solution $\phi(\hat I)$ to each instance $\hat I\in \hat \iset^*$, computes a solution $\check \phi$ to instance $\cI$, with $\cro(\check \phi)\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+g_1^j\cdot\mu^{3b^*+300b}$.
\end{observation}
\begin{proof}
It would be convenient for us to associate a (rooted) partitioning tree $\tau$ for the pre-processing procedure, whose node correspond to all instance that every appeared in the collection $\tempiset$, as follows.
Initially, $\tau$ contains a root denoted by $v^*$, and, for each instance $I\in \iset$, a node $v(I)$ representing instance $I$.
Consider now an iteration that some instance $I$ is processed and eventually replaced by new instances $I_1,\ldots,I_s$. We add to $\tau$ nodes $v(I_1),\ldots,v(I_s)$ to them, that become the child nodes of $v(I)$ in $\tau$. We continue until the end of the algorithm. This completes the construction of tree $\tau$. It is easy to see that the instances in the resulting collection $\iset^*$ correspond to leaf nodes in $\tau$.

We now describe the algorithm for computing a solution $\check \phi$ to instance $\cI$. Assume now we are given, for each instance $I\in \iset^*$ that correspond to some leaf node in $\tau$, a solution $\phi(\hat I)$ to instance $\hat I$.
We iteratively process non-root nodes of $\tau$ in a bottom-up fashion, as follows. 
In each iteration, we take a node $v(I)$ corresponding to instance $I$, such that all its child nodes $v(I_1),\ldots,v(I_s)$ are either leaf nodes or have been processed.
Consider the iteration of the pre-processing procedure in which some instance $I$ is processed and eventually replaced by new instances $I_1,\ldots,I_s$. We denote by $\hat I=(\hat G,\hat \Sigma), \hat I_1=(\hat G_1,\hat \Sigma_1),\ldots,\hat I_s=(\hat G_s,\hat \Sigma_s)$ their contracted instances, respectively.
From the algorithm, graph $\hat G_1\cup \ldots\cup \hat G_s$ are the connected components obtained from $\hat G$ by deleting a set $\hat E$ of edges. We first obtain a drawing of $\hat G\setminus \hat E$ by placing drawings $\phi(\hat I_1),\ldots,\phi(\hat I_s)$ in mutually disjoint discs in the plane.
We then use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $\hat E$ into the drawing of $\hat G\setminus \hat E$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$, such that $\cro(\phi(\hat I))\le \sum_{1\le i\le s}\cro(\phi(\hat I_s))+|E(\hat G)|\cdot |\hat E|$.
In this way we process all non-root nodes, such that at the end, we obtained, for each instance $I\in \iset$, a solution $\phi(\hat I)$ to its contracted instance $\hat I$, with $\sum_{I\in \iset}\cro(\phi(\hat I))\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\cm \cdot \hat E_{\sf temp}$. 
Finally, we apply the algorithm from \Cref{thm: phase 1} to the solutions $\phi(\hat I)$ for instances $I\in\iset$ and obtain a solution $\check\phi$ for $\cI$ with $\cro(\check \phi)\le \sum_{\hat I\in \hat \iset}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}$.
Since $|\hat E_{\sf temp}|\le \mu^{b^*}\cdot \mu^{100}\cdot \tilde g$, altogether we get that
$$\cro(\check \phi)
\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+\cm\cdot\mu^{b^*}\cdot \mu^{100}\cdot \tilde g
\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+g_1^j\cdot\mu^{3b^*+300b},$$
as $b^*>100$.
\end{proof}

\subsubsection*{The algorithm for comuting the collection $\iset^{(j)}$}
We now partition the resulting collection $\iset^*$ into two subsets: set $\iset^*_1$ contains all small instances in $\iset^*$; and set $\iset^*_2$ contains all remaining instances. 
We denote $\hat \iset_1=\set{\hat I\mid I\in 
\iset^*_1}$.
Since every instance in $\iset^*_2$ is large (that is, $\hat m(I)\ge \cm/\mu^{b^*}$), from Invariant \ref{prop: number of edges}, we get that $|\iset^*_2|\le \mu^{b^*}$.
From the pre-processing step, for each instance $I=(G,\Sigma)\in \iset^*_2$, its skeleton $K(I)$ is $\tilde g$-connected in $G$. Since $|E(G)|\ge \cm/\mu^{b^*}$, $\tilde g\ge \left(
\frac{g_1^j}{|E(G)|}+g_2^j \right)$, so its skeleton $K(I)$ is $g_3(I)$-connected in $G$, for $g_3(I)=\left(
\frac{g_1^j}{|E(G)|}+g_2^j \right)$.

For each instance $I\in \iset^*$, we denote by $\psi(I)$ the solution to $I$ guaranteed by Invariant \ref{prop: good drawings}.
We use the following observation.
\begin{observation}
\label{obs: not too large}
	If $\optcrors(\cI)\le \cm^2/\mu^{61b-2b^*}$, then for each instance $I=(G,\Sigma)\in \iset^*_2$, the drawing $\psi(I)$ satisfies that $\cro(\psi(I))\le |E(G)|^2/\mu^{60b}$ and $|\chi^{\dirty}(\psi(I))|\le  |E(G)|/\mu^{60b}$.
\end{observation}
\begin{proof}
	Let $I=(G,\Sigma)$ be an instance in $\iset^*_2$, so $|E(G)|\ge \cm/\mu^{b^*}$.
	Recall that, from \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\le 2\cdot\optcrors(\cI)$, so $\cro(\psi(I))\le 2\cdot\optcrors(\cI)$. Therefore, if $\optcrors(\cI)\le \cm^2/\mu^{61b-2b^*}$, then
	\[
	\cro(\psi(I))\le 2\cdot\optcrors(\cI) \le \frac{2\cdot \cm^2}{\mu^{61b-2b^*}}\le 
	\frac{ \cm^2}{\mu^{60b-2b^*}} 
	= \frac{ (\cm/\mu^{b^*})^2}{\mu^{60b}} 
	\le \frac{|E(G)|^2}{\mu^{60b}}.
	\]
	Also recall that, from \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\le \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so $|\chi^{\dirty}(\psi(I))| < \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. Therefore,
	\[
	|\chi^{\dirty}(\psi(I))|\le \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm} 
	\le \frac{\cm\cdot \mu^{b^*}}{\mu^{61b-2b^*}}
	\le \frac{\cm}{\mu^{60b+b^*}}
	= \frac{(\cm/\mu^{b^*})}{\mu^{60b}}
	\le \frac{|E(G)|}{\mu^{60b}},
	\]
	since $b\ge 4b^*$. 
\end{proof}

Finally, we consider every instance $I\in \iset^*_2$ one by one. 
For each such instance $I$, we apply the algorithm from \Cref{thm: phase 2} to instance $I$, skeleton structure $\kset(I)$, the parameters $b,g^j_1,g^j_2$ defined above.  
We denote by $I'=(G',\Sigma')$ the resulting instance of \cnwrs, and by $\hat I'$ the $\kset(I)$-contraction of this instance. We then denote $\hat \iset'_2=\set{\hat I'\mid I\in \iset^*_2}$. The final output of our algorithm is the collection $\iset^{(j)}=\hat\iset_1\cup\hat \iset'_2$ of subinstances of $\cI$. 




\subsubsection*{The analysis of the algorithm}

We now verify that the output collections $\iset^{(1)},\ldots,\iset^{(z)}$ of subinstances of $\cI$ have all required properties. 
Consider an index $1\le j\le z$ and consider the algorithm for constructing collection $\iset^{(j)}$.
%First, the algorithm from \Cref{thm: phase 1} ensures that, for every instance $I\in \iset$, if the corresponding contracted instance $\hat I=(\hat G,\hat \Sigma)$  is a wide instance, then $|E(\hat G)|\le \cm/\mu$. 

First, from Invariant \ref{prop: wide or not}, for every instance $I\in \iset^*$, if the corresponding contracted instance $\hat I=(\hat G,\hat \Sigma)$  is a wide instance, then $|E(\hat G)|\le \cm/\mu$.
If instance $I$ lies in $\iset^*_2$, and $\hat I'=(\hat G',\hat\Sigma')$ is the $\kset(I)$-contraction of instance $I'$, then $|E(\hat G')|\leq |E(\hat G)|$, and, if $\hat I$ is not a wide instance, then neither is $\hat I'$. This is since graph $\hat G'$ can be obtained from graph $\hat G$ by deleting the edges of $E^{\del}(I)$ from it. Therefore, we are guaranteed that, for every instance $I'=(G',\Sigma')\in \iset^{(j)}$, if $I'$ is a wide instance, then $|E(G')|\le \cm/\mu$.

Second, from Invariant \ref{prop: number of edges},
%The algorithm from \Cref{thm: phase 1} also guarantees that $\sum_{I\in  \iset}\hm(I)\le \cm$.
$\sum_{I\in  \iset^*}\hm(I)\le \cm$.
Since, for every instance $I\in \iset^*_2$, the corresponding resulting instance $\hat I'=(\hat G',\Sigma')\in \hat \iset_2'$ has $|E(\hat G')|\leq \hat m(I)$, we get that $\sum_{I'=(G',\Sigma')\in \iset^{(j)}}|E(G')|\le \cm$.

Third, we construct an algorithm that, given a solution to each instance in $\iset^{(j)}$, computes a solution $\phi$ to instance $\cI$.
For each instance $I\in \iset^*_2$,  we let $\hat I=(\hat G,\hat \Sigma)$ be the corresponding  $\kset(I)$-contracted instance, and let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance corresponding to the instance $I'$. Note that $V(\hat G)=V(\hat G')$ and $E(\hat G')=E(\hat G)\setminus E^{\del}(I)$. We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\del}(I)$ into the solution $\phi(\hat I')$ to instance $\hat I'$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$.
Then we use the algorithm from \Cref{obs: algo combine drawings} to compute a drawing of $\cI$. It is clear that the algorithm is efficient.


%\znote{the algorithm for computing the drawing}

From now on, we let $j^*$ be the unique integer that $2^{j^*-1}< 2\cdot \optcrors(\cI)\le 2^{j^*}$. Since $\optcrors(\cI)\le \cm^2$, $j^*\le 2\log m$, so $1\le j^*\le z$. We will show that the collection $\iset^{(j^*)}$ satisfies the property required in the last bullet of \Cref{lem: many paths}. Consider now the algorithm for constructing the collection $\iset^{(j^*)}$.

Recall that we have set $g_1^{j^*}=2^{j^*}$ and $g_2^{j^*}=g_1^{j^*}\cdot \mu^{b^*}/\cm$. 
%
Therefore, from Invariant \ref{prop: good drawings}, the semi-clean solutions $\psi(I)$ to $I$ for instances $I\in \iset^*$ satisfy that
$\sum_{I\in \tempiset}\cro(\psi(I))\le g_1^{j^*}$ and $\sum_{I\in \tempiset}|\chi^{\dirty}(\psi(I))|\leq  g_2^{j^*}$.
So for each instance $I\in \iset^*$, $\cro(\psi(I))\le g_1^{j^*}$ and $|\chi^{\dirty}(\psi(I))| \leq  g_2^{j^*}$.
%From \Cref{thm: phase 1}, if $\optcrors(\cI)\le \cm^2/\mu^{c'}$, and the bad event $\tilde \event'_1$ does not happen, then for each instance $I\in \iset$ there exists a semi-clean solution $\psi(I)$ to
Combined with \Cref{obs: not too large}, we get that, for each instance $I=(G,\Sigma)\in \iset^*_2$, both $\cro(\psi(I))\le \min\set{g_1^*,|E(G)|^2/\mu^{60b}}$ and $|\chi^{\dirty}(\psi(I))|\le \min\set{g_2^*, |E(G)|/\mu^{60b}}$ hold.
(We have used the fact that \fbox{$c'>61b-2b^*$}.)

For each instance $I\in \iset^*_2$, we denote by $\tilde \event_2(I)$ the bad event that the application of the algorithm from \Cref{thm: phase 2} was unsuccessful, so $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$.
%
Let $\tilde \event_2'$ be the bad event that any of the events in $\set{\tilde \event_2(I)\mid I\in \iset^*_2}$ happened. Since, from the above discussion, $|\iset^*_2| \leq \mu^{b^*}$, and, for every instance $I\in \iset^*_2$, $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$, while $b>2b^*$, from the Union Bound, we get that $\prob{\tilde \event_2'}<1/\mu^4$. Lastly, we let $\tilde \event'$ be the bad event that either $\tilde \event_1'$ or $\tilde \event_2'$ happened. Clearly, $\prob{\tilde \event'}\leq \prob{\tilde \event_1'}+\prob{\tilde \event_2'}\leq 1/\mu^2$.
We use the following two observations in order to complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: composing contracted solutions}
Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then there is an efficient algorithm, that, given a solution $\phi(I')$ for every instance $I'\in \iset^{(j^*)}$, computes a solution $\check \phi$ to instance $\cI$, with $\cro(\check\phi)\leq  \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I')) + \optcrors(\check I)\cdot\mu^{O(1)}$.
\end{observation}
\begin{proof}
We assume that $\optcrors(I)\leq m^2/\mu^{c'}$, Event $\tilde \event'$ did not happen, and that  we are given a solution $\phi(I')$ to every instance $I'\in \iset^{(j^*)}$. We now show an efficient algorithm to compute a solution $\check \phi$ to instance $\cI$. In order to do so, we first consider every instance $I\in \iset^*_2$ one by one, and compute a solution $\phi(\hat I)$ to instance $\hat I$, from the solution $\phi(\hat I')$ to instance $\hat I'$. 

Consider now some instance $I=(G,\Sigma)\in \iset^*_2$. Let $\hat I=(\hat G,\hat \Sigma)$ be the corresponding  $\kset(I)$-contracted instance, and let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance corresponding to the instance $I'$. Note that $V(\hat G)=V(\hat G')$ and $E(\hat G')=E(\hat G)\setminus E^{\del}(I)$. We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\del}(I)$ into the solution $\phi(\hat I')$ to instance $\hat I'$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$, whose cost is at most $\cro(\phi(\hat I'))+|E^{\del}(I)|\cdot |E(G)|$. If Event $\tilde \event'$ does not happen, then $|E^{\del}(I)|\leq \big(\frac{g_1^{j^*}}{|E(G)|}+g_2^{j^*}\big)\cdot\mu^{O(1)}=\frac{\optcrors(\cI)\cdot\mu^{O(1)}}{|E(G)|}$, and so $\cro(\phi(\hat I))\leq \cro(\phi(\hat I'))+\optcrors(\cI)\cdot \mu^{O(1)}$.
Now using the algorithm from \Cref{obs: algo combine drawings},
%
%We have now obtained, for every instance $I\in \iset$, a solution $\phi(\hat I)$ to the corresponding contracted instance $\hat I$. This solution immediately defines a solution $\phi(I)$ to instance $I$ that is clean with respect to $\kset(I)$, with $\cro(\phi(I))\leq \cro(\phi(\hat I))$. 
%Lastly, using the algorithm from \Cref{thm: phase 1}, 
we obtain a solution 
$\check\phi$ to instance $\cI$, whose cost is bounded by:
%
\[
\begin{split}
\cro(\check \phi)&\leq  \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I)) + \optcrors(\cI)\cdot\mu^{O(1)}\\
&\leq \sum_{I\in \iset^*_1}\cro(\phi(\hat I))+\sum_{I\in \iset^*_2}\left (\cro(\phi(\hat I'))+\optcrors(\cI)\cdot \mu^{O(1)}\right )+\optcrors(\cI)\cdot\mu^{O(1)}\\
&\le \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I'))+|\iset^*_2|\cdot\optcrors(\cI)\cdot\mu^{O(1)}+\optcrors(\cI)\cdot\mu^{O(1)}\\
&\le \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)},
\end{split}
\]
%
as $|\iset^*_2|=\mu^{O(1)}$.
%From \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and Event $\tilde \event'$ did not happen, then $\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$. Therefore, we get that $\cro(\check \phi)\leq \sum_{I'\in \hat \iset'}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)}$.
\end{proof}


%Lastly, the following observation will complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: cheap solutions to final instances}
	Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then $\sum_{I'\in \iset^{(j^*)}}\optcrors(I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}$.
\end{observation}
\begin{proof}
	We bound $\sum_{I\in \iset^*_1}\optcrors(\hat I)$ and $\sum_{I\in \iset^*_2}\optcrors(\hat I')$ separately.
	
	From \Cref{thm: phase 2}, if Event $\tilde \event'$ did not happen, then, for every instance $I=(G,\Sigma)\in \iset^*_2$, 
	there is a solution $\psi(I')$ to the corresponding instance $I'$, that is clean with respect to $\kset(I)$, with $\cro(\psi(I'))\leq \cro(\psi(I))\cdot (\log \cm)^{O(1)}+|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}$. 
	From \Cref{obs: clean solution to contracted}, there is a solution to the corresponding contracted instance $\hat I'$, of cost at most $\cro(\psi(I'))$. Altogether, we get that:
	%
	\[\begin{split}
	\sum_{I\in \iset^*_2}\optcrors(\hat I')&\leq \sum_{I\in \iset^*_2}\left(\cro(\psi(I))+\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}\right )\cdot (\log \cm)^{O(1)}.\\
	&\leq \sum_{I\in \iset^*_2}\cro(\psi(I))\cdot (\log \cm)^{O(1)}+\left (\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right )^2\cdot (\log \cm)^{O(1)}\\
	&\hspace{4cm}+ \frac{\cm\cdot (\log \cm)^{O(1)}}{\mu^b}\cdot\left(\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right ).
	\end{split}
	\]
	%
	From Invariant \ref{prop: good drawings}, $\sum_{I\in \iset^*}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$ and $\sum_{I\in \iset^*}|\chi^{\dirty}(\psi(I))|\leq \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. Additionally, since we have assumed that $\optcrors(I)\leq m^2/\mu^{c'}$ for a large enough constant $c'>2b^*$, 
	$$\left (\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right )^2\leq \frac{(\optcrors(\cI))^2 \mu^{2b^*}}{\cm^2}\leq \optcrors(\cI).$$ Altogether, we get that:
	%
	\[
	\begin{split}
	 \sum_{I\in \iset^*_2}\optcrors(\hat I')&\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}+\frac{\optcrors(\cI)\cdot \mu^{b^*}\cdot  (\log \cm)^{O(1)}}{\mu^b}\\
	 &\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}, \end{split}\]
	since $b>4b^*$.
%	
%	Lastly, since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}\hat m(I)\le \cm$, and since $b>b^*$, $\sum_{I\in \iset_3}\optcrors(\hat I')\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}$.  

Next, we bound $\sum_{I\in \iset^*_1}\optcrors(\hat I)$. Consider some instance $I=(G,\Sigma)\in \iset^*_1$ and the solution $\psi(I)$ that is semi-clean with respect to $\kset(I)$. Let $K(I)$ be the skeleton associated with the skeleton structure $\kset(I)$. Let $E^{\dirty}(I)\subseteq E(G)\setminus E(K(I))$ be the set of all edges $e$, such that the image of $e$ in $\psi(I)$ crosses the image of some edge of $K(I)$.  Let $\hat I=(\hat G,\hat \Sigma)$ be the $\kset(I)$-contracted instance corresponding to instance $I$.


Denote $G'=G\setminus E^{\dirty}(I)$, and let $\Sigma'$ be the rotation system for graph $G'$ that is induced by $\Sigma$. Observe that $\kset(I)$ is a valid skeleton structure for the resulting instance $I'=(G',\Sigma')$. Let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance associated with $I'$. Observe that the drawing $\psi(I)$ of instance $I$ induces a drawing $\psi(I')$ of instance $I'$ that is clean with respect to $\kset(I)$. From \Cref{obs: clean solution to contracted}, there is a solution $\psi(\hat I')$ to the contracted instance $\hat I'$ with $\cro(\psi(\hat I'))\leq \cro(\psi(I'))\leq \cro(\psi(I))$. 
We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\dirty}(I)$ into the drawing $\psi(\hat I')$ to obtain a drawing $\psi(\hat I)$ of instance $\hat I$, with the number of crossings bounded by $\cro(\psi(\hat I'))+|E^{\dirty}(I)|\cdot |E(\hat G)|\leq \cro(\psi(I))+|E^{\dirty}(I)|\cdot |E(\hat G)|$.

Recall that $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$ (since instance $I$ is small), so $\cro(\psi(\hat I))
\leq \cro(\psi(I))+|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}$. %(since $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$). 
We then get that:
%
\[\sum_{I\in \iset^*_1} \optcrors(\hat I)\leq 
\sum_{I\in \iset^*_1}\cro(\psi(I))+\sum_{I\in \iset^*_1}|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}.
\]
%
From Invariant \ref{prop: good drawings}, $\sum_{I\in \iset^*}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$ and $\sum_{I\in \iset^*}|\chi^{\dirty}(\psi(I))|\leq \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$.
Therefore, 
$$\sum_{I\in \iset^*_1} \optcrors(\hat I)\leq  2\cdot\optcrors(\cI)+\frac{\cm}{\mu^{b^*}} \cdot  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\leq O(\optcrors(\cI)).$$


\iffalse{analysis for previous iset_2, which should be an empty set}
Assume now that $I\in \iset_2$. We partition the set $\iset_2$ of instances into two subsets: set $\iset_2'$ containing all instances $I=(G,\Sigma)$ with $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, and set $\iset_2''$ containing all remaining instances.
As before, for every instance $I=(G,\Sigma)\in \iset_2$, we denote by $\hat m(I)$ the number of edges in the contracted graph $\hat I$. 


Next, we bound $\sum_{I\in \iset_2'}\cro(\psi(\hat I'))$. Recall that for every instace $I=(G,\Sigma)\in \iset_2'$:
%
\[\cro(\psi(I))> \frac{|E(G)|^2}{\mu^{60b}}\geq \frac{(\hat m(I))^2}{\mu^{60b}}\geq \frac{\hat m(I)\cdot \cm}{\mu^{60b+b^*}},\]
%
since instance $I$ must be large. Since,  
from \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)\leq 2\cm^2/\mu^{c'}$, we get that $\sum_{I\in \iset_2'}\hat m(I)\leq \frac{2\cm}{\mu^{c'-60b-b^*}}$. Lastly, since, from  \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that:
%
\[\begin{split}
\sum_{I\in \iset_2'} \optcrors(\hat I)&\leq 
\sum_{I\in \iset_2'}\cro(\psi(I))+\sum_{I\in \iset_2'}|\chi^{\dirty}(I)|\cdot \hm(I)\\
&\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2'}\hat m(I) \right )\\
&\leq 2\cdot\optcrors(\cI)+\frac{2\cm}{\mu^{c'-60b-b^*}}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
&\leq O(\optcrors(\cI)).\end{split}
\]
%
It now remains to consider instances $I\in \iset_2''$. Recall that, for each such instance $I=(G,\Sigma)$,  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{60b}$. 
 Since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that $\sum_{I\in \iset_2''}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}$. 
 Therefore:
%
 \[\begin{split}
 \sum_{I\in \iset_2''} \optcrors(\hat I)&\leq 
 \sum_{I\in \iset_2''}\cro(\psi(I))+\sum_{I\in \iset_2''}|\chi^{\dirty}(I)|\cdot \hm(I)\\
 &\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2''}\hat m(I) \right )\\
 &\leq 2\cdot\optcrors(\cI) + \frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
 &\leq O(\optcrors(\cI))
 ,\end{split}
 \]
 %
 since $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and $c'$ is a large enough constant.
 \fi
 
 

Altogether, we get that 
$$\sum_{I'\in \iset^{(j^*)}}\optcrors(I')=\sum_{I\in \iset^*_1}\optcrors(\hat I)+\sum_{I\in \iset^*_2}\optcrors(\hat I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}.$$
\end{proof}



\iffalse

The calculations

---------------------------------------------------



\begin{itemize}
	\item $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)$
	
	\item $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$
	
	\item in $\iset_2$: either $\cro(\psi(I))> |E(G)|/\mu^{2b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$.
	
	\item when pulling edges back, we will pay $\sum_{I\in \iset_2}\hm(I)\cdot |\chi^{\dirty}(\psi(I))|$.
	
	\item let's say that $\iset_2'$ contains all instances with $\cro(\psi(I))> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{2b}$. But $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)<\cm/\mu^{c'}$. So $\sum_{I\in \iset_2'}\hat m(I)\leq \mu^{2b}\cdot \cm/\mu^{c'}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so total increase in number of crossings is less than $\optcrors(\cI)$.
	
	\item Now $\iset_2''$ contains all instances with $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$. But $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. So $\sum_{I\in \iset_2}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+b}}{\cm}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so the total increase in number of crossings is at most $\frac{(\optcrors(\cI))^2\cdot \mu^{2b^*+b}}{(\cm)^2}$. Assuming that $\optcrors(\cI)<\cm^2/\mu^{c'}$ it's at most $\optcrors(\cI)$.
\end{itemize}





----------------------------------------------
\fi

$\ $

In the remainder of this section we focus on the proof of \Cref{thm: phase 2}. Throughout the proof, we denote the instance $I=(G,\Sigma)$ that serves as the input to the algorithm by $\cI'=(\cG',\cSigma')$, with $|E(\cG')|$ denoted by $\cm'$. We denote the skeleton structure $\kset(I)$ by $\check \kset=(\jset_1,\ldots,\jset_r)$, where $r\leq \mu^{100}$. For all $1\leq i\leq r$, we denote $\jset_i=(J_i,\set{b_u}_{u\in V(J_i)},\rho_{J_i})$. 
We start with the intuition for the proof. We denote by $\check K=\bigcup_{i=1}^rJ_i$ the skeleton of $\cG'$ associated with the skeleton structure $\check \kset$. We can assume that there exists a solution $\check \psi$ to instance $\cI$ that is semi-clean with respect to $\check\kset$. 
%(as otherwise we can let $E^{\del}(\cI')=E(\cG)\setminus E(\check K)$ \znote{what does this mean?} ). 

==> finish-proof-interesting-backup3.tex <==
\subsubsection{Completing the Proof of \Cref{lem: many paths}}
\label{subsubsec: finish the proof}
Given an input instance $\cI=(\cG,\cSigma)$, we first apply the algorithm from \Cref{thm: phase 1} to this input. If the algorithm fails, then we terminate the algorithm and return FAIL as well. Recall that, from \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/\mu^3$. Assume now that the algorithm from \Cref{thm: phase 1} did not fail. In this case, if  $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then with probability at least $(1-1/\mu^3)$, the algorithm is successful. We denote by $\tilde \event_1'$ the bad event that the application of this algorithm is unsuccessful, so $\prob{\tilde \event_1'}\leq 1/\mu^3$. Let $\iset$ be the collection of subinstances of $\cI$ computed by the algorithm from \Cref{thm: phase 1}. 

Throughout this subsection, we use the universal constant $b^*=2400$.
Recall that, if Event $\tilde \event'_1$ did not happen, then for every instance $I\in \iset$, there is a solution $\psi(I)$ to $I$, that is semi-clean with respect to $\kset(I)$, such that 
$\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$, and $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. We set the parameter $b$ to be a large enough constant, so that $b\geq 4b^*$ holds.
%
Recall that, for every instance $I=(G,\Sigma)\in \iset$, we have denoted by $\hat I=(\hat G,\hat \Sigma)$ the corresponding $\kset(I)$-contracted instance, and by $\hat m(I)=|E(\hat G)|$. We say that instance $I$ is \emph{small} if $\hat m(I)\leq \frac{\cm}{\mu^{b^*}}$, and otherwise it is \emph{large}. 
%We partition the set $\iset$ of instances into three subsets: set $\iset_1$ containing all small instances; and set $\iset_2$ containing all remaining instances.
%set $\iset_2$ containing all large instances $I=(G,\Sigma)\in \iset$ for which either $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{60b}$ holds, and set $\iset_3$ containing all remaining instances.
%Since the algorithm from \Cref{thm: phase 1} guarantees that $\sum_{I\in \iset}\hat m(I)\le \cm$, we get that $|\iset_2|\leq \mu^{b^*}$. We let $\hat \iset_1=\set{\hat I\mid I\in \iset_1}$ contain the set of all contracted instances corresponding to the instances of $\iset_1$, and we define set $\hat \iset_2$ of instances corresponding to the instances of $\iset_2$ similarly.
%\znote{We do not know $\cro(\psi(I))$ and $\chi^{\dirty}(\psi(I))$ so we cannot distinguish $\iset_2$ from $\iset_3$?}

We now proceed in $z= 2\log m$ phases, where in the $j$th phase, we compute the $j$th collection $\iset^{(j)}$ of subinstances of $I$, such that the properties required in \Cref{lem: many paths} are satisfied.

Consider now an index $1\le j\le 2\log m$ and we describe the $j$th phase. Throughout the phase, we use the parameters $g^j_1=2^j$ and $g^j_2=g^j_1\cdot \mu^{b^*}/\cm$.
We intend to apply the algorithm from \Cref{thm: phase 2} to large instances in $\iset$ with parameters $g^j_1,g^j_2$. But note that the algorithm requires that the input instance $I=(G,\Sigma)$ has a skeleton $K(I)$ that is $g_3(I)$-connected in the input graph $G$ (where $g_3(I)=\big(\frac{g_1^j}{|E(G)|}+g_2^j\big)\cdot\mu^{300b}$), which is not necessarily true for the large instances in $\iset$. Therefore, we first pre-process instances in $\iset$, such that the resulting instances are either small or satisfying this connectedness property, as follows.

\newcommand{\tempiset}{\iset_{\sf temp}}
\newcommand{\hattempiset}{\hat{\iset}_{\sf temp}}

\subsubsection*{Pre-processing instances in $\iset$}

The pre-processing procedure is iterative. Throughout, we use a parameter $\tilde g=\big(\frac{g^j_1\mu^{b^*}}{\cm}+g^j_2\big)\cdot\mu^{300b}$.
The procedure maintains a collection $\tempiset$ of subinstances of $I$, that is initialized to be $\tempiset=\iset$. We denote $\hattempiset=\set{\hat I\mid I\in \tempiset}$.
Each instance in $\tempiset$ is either marked \emph{active} or \emph{inactive}. Initially, all large instances are marked active and all small instances are marked inactive.
We will maintain the following invariant throughout the algorithm.
%
\begin{properties}{IP}
\item for each inactive instance $I=(G,\Sigma)\in \tempiset$, either $I$ is small, or $I$ satisfies that, if we denote by $K(I)$ the skeleton of $I$, then $K(I)$ is $\tilde g$-connected in $G$;
\label{prop: inactive}
\item for each instance $\hat I=(\hat G,\hat \Sigma)\in \hattempiset$, either $|E(\hat G)|\le \cm/\mu$, or $\hat I$ is not wide;
\label{prop: wide or not}
\item $\sum_{I\in \tempiset}\hat m(I)\le \cm$; and
\label{prop: number of edges}
\item there exists, for every instance $I\in \tempiset$, a solution $\psi(I)$ to $I$ that is semi-clean with respect to $\kset(I)$, such that
$\sum_{I\in \tempiset}\cro(\psi(I))\le 2\cdot \optcrors(\cI)$, and $\sum_{I\in \tempiset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$.
\label{prop: good drawings}
\end{properties}
%
From \Cref{thm: phase 1} and our initial setting, these invariant holds at the beginning of the pre-processing procedure.

The procedure continues to be executed as long as the collection $\tempiset$ contains an active instance. 
%$\hat m(I)>\cm/\mu^{b^*}$ (that is, instance $I$ is large), and, if we denote by $K(I)$ the skeleton of $I$ that corresponds to its skeleton structure $\kset(I)$, then $K(I)$ is not $\tilde g$-connected in $G$.
We now describe an iteration of the procedure.
Let $I=(G,\Sigma)$ be an active instance in $\tempiset$. If instance $I$ is small, then we mark it inactive and terminate the iteration. Clearly all invariants continue to hold after this iteration in this case.
Assume now that instance $I$ is large. 
Let $\kset(I)=\set{\jset_1,\ldots,\jset_{r}}$ be the skeleton structure for $I$, and for each $1\le i\le r$, let $J_i$ be the core associated with $\jset_i$. 
Consider its $\kset(I)$-contracted instance $\hat I=(\hat G, \hat \Sigma)$. Recall that graph $\hat G$ is obtained from graph $G$ by contracting, for each $1\le i\le r$, all vertices of the core $J_i$ into a supernode $v_{J_i}$. We now compute, for every pair $1\le i<i'\le r$, a minimum $v_{J_i}$-$v_{J_{i'}}$ cut in $\hat G$.
If for all pairs $1\le i<i'\le r$, the $v_{J_i}$-$v_{J_{i'}}$ minimum-cut in $\hat G$ has value at least $\tilde g$, then we simply mark the instance $I$ in $\iset$ inactive, and terminate this iteration.
Clearly all invariants continue to hold after this iteration in this case.
Assume now that there exists a pair $1\le i<i'\le r$, such that the $v_{J_i}$-$v_{J_{i'}}$ minimum-cut in $\hat G$ has value less than $\tilde g$. 
%Let $(A,B)$ be the $v_{J_i}$-$v_{J_{i'}}$ cut that we computed.
Let $\hat G_1,\ldots,\hat G_s$ be the graphs obtained from $\hat G$ by deleting the edge of the minimum-cut. Consider now an $1\le i\le s$. Assume that supernodes corresponding to cores $J_{p_1},\ldots, J_{p_t}$ belong to graph $\hat G_i$. 
We define instance $I_i=(G_i,\Sigma_i)$ as follows. Graph $G_i$ is the graph obtained from $\hat G_i$ by un-contracting every supernode $v_{J_{p_q}}$ back to its corresponding core $J_{p_q}$, so $G_i$ is a subgraph of $G$, and $\Sigma_i$ is the rotation system on $G_i$ that is induced by $\Sigma$. We then define its core structure to be $\kset(I_i)=\set{\jset_{p_1},\ldots,\jset_{p_q}}$.
We then replace the instance $I$ in $\tempiset$ with new instances $I_1,\ldots,I_s$, all marked active, and terminate this iteration.

We now verify that all invariants continue to hold after this iteration in this case.
First, since we marked all new instance that are added to collection $\tempiset$ active, Invariant \ref{prop: inactive} holds.
Second, since for every new instance $I_i=(G_1,\Sigma_i)$, graph $G_i$ is a subgraph of $G$, and $\hat G_i$ is a subgraph of $\hat G$. If $|E(\hat G)|\le \cm/\mu$, then $|E(\hat G_i)|\le \cm/\mu$; if $\hat I$ is node wide, then $\hat I_i$ is also not wide. Therefore,
\ref{prop: wide or not} holds.
Third, since $\hat G_1\cup\ldots\cup\hat G_s\subseteq \hat G$, $\sum_{1\le i\le s}\hat m(I_i)\le \hat m(I)$ and so
\ref{prop: number of edges} holds.
Last, note that the Invariant \ref{prop: good drawings} holds before this iteration. Let $\psi(I)$ be the semi-clean solution associated with instance $I$. We simply define, for each $1\le i\le s$,  $\psi(I_i)$ to be the drawing of $G_i$ induced by drawing $\psi(I)$. It is easy to verify that $\psi(I_i)$ is a semi-clean solution to $I_i$ with respect to its skeleton structure. Moreover, since $G_1,\ldots,G_s$ are disjoint subgraphs of $G$,  
$\sum_{1\le i\le s}\cro(\psi(I_i))\le \cro(\psi(I))$, and $\sum_{1\le i\le s}|\chi^{\dirty}(\psi(I_i))|\leq  |\chi^{\dirty}(\psi(I))|$.
Therefore, \ref{prop: good drawings} also holds.

Note that the collection of all cores in all skeleton structures is never changed, and initially, the number of cores in all active instances in $\iset$ is at most $\mu^{b^*}\cdot \mu^{100}$ (since the number of active instances is at most $\mu^{b^*}$ and each such instances has at most $\mu^{100}$ cores). When the pre-processing process terminates, every resulting instance contains at least one core.
Therefore, the number of iterations is at most $\mu^{b^*}\cdot \mu^{100}$. Note that in each iteration we have deleted at most $\tilde g$ edges. Therefore, if we denote by $\hat E_{\sf temp}$ the set of all deleted edges throughout this procedure, then
$|\hat E_{\sf temp}|\le \mu^{b^*}\cdot \mu^{100}\cdot \tilde g$.

Let $\iset^*$ be the resulting collection we obtained at the end of the pre-processing procedure. Since all instances in $\iset^*$ are inactive, from Invariant \ref{prop: inactive}, for each instance $I=(G,\Sigma)\in \iset^*$, either $I$ is small, or its skeleton $K(I)$ is $\tilde g$-connected in $G$.
Moreover, it is easy to verify that, for each instance $I\in \iset^*$, its skeleton structure has size at most $\mu^{100}$.

Denote $\hat \iset^*=\set{\hat I\mid I\in \iset^*}$. We prove the following observation.

\begin{observation}
\label{obs: algo combine drawings}
There is an efficient algorithm, that, given a solution $\phi(\hat I)$ to each instance $\hat I\in \hat \iset^*$, computes a solution $\check \phi$ to instance $\cI$, with $\cro(\check \phi)\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+g_1^j\cdot\mu^{3b^*+300b}$.
\end{observation}
\begin{proof}
It would be convenient for us to associate a (rooted) partitioning tree $\tau$ for the pre-processing procedure, whose node correspond to all instance that every appeared in the collection $\tempiset$, as follows.
Initially, $\tau$ contains a root denoted by $v^*$, and, for each instance $I\in \iset$, a node $v(I)$ representing instance $I$.
Consider now an iteration that some instance $I$ is processed and eventually replaced by new instances $I_1,\ldots,I_s$. We add to $\tau$ nodes $v(I_1),\ldots,v(I_s)$ to them, that become the child nodes of $v(I)$ in $\tau$. We continue until the end of the algorithm. This completes the construction of tree $\tau$. It is easy to see that the instances in the resulting collection $\iset^*$ correspond to leaf nodes in $\tau$.

We now describe the algorithm for computing a solution $\check \phi$ to instance $\cI$. Assume now we are given, for each instance $I\in \iset^*$ that correspond to some leaf node in $\tau$, a solution $\phi(\hat I)$ to instance $\hat I$.
We iteratively process non-root nodes of $\tau$ in a bottom-up fashion, as follows. 
In each iteration, we take a node $v(I)$ corresponding to instance $I$, such that all its child nodes $v(I_1),\ldots,v(I_s)$ are either leaf nodes or have been processed.
Consider the iteration of the pre-processing procedure in which some instance $I$ is processed and eventually replaced by new instances $I_1,\ldots,I_s$. We denote by $\hat I=(\hat G,\hat \Sigma), \hat I_1=(\hat G_1,\hat \Sigma_1),\ldots,\hat I_s=(\hat G_s,\hat \Sigma_s)$ their contracted instances, respectively.
From the algorithm, graph $\hat G_1\cup \ldots\cup \hat G_s$ are the connected components obtained from $\hat G$ by deleting a set $\hat E$ of edges. We first obtain a drawing of $\hat G\setminus \hat E$ by placing drawings $\phi(\hat I_1),\ldots,\phi(\hat I_s)$ in mutually disjoint discs in the plane.
We then use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $\hat E$ into the drawing of $\hat G\setminus \hat E$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$, such that $\cro(\phi(\hat I))\le \sum_{1\le i\le s}\cro(\phi(\hat I_s))+|E(\hat G)|\cdot |\hat E|$.
In this way we process all non-root nodes, such that at the end, we obtained, for each instance $I\in \iset$, a solution $\phi(\hat I)$ to its contracted instance $\hat I$, with $\sum_{I\in \iset}\cro(\phi(\hat I))\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\cm \cdot \hat E_{\sf temp}$. 
Finally, we apply the algorithm from \Cref{thm: phase 1} to the solutions $\phi(\hat I)$ for instances $I\in\iset$ and obtain a solution $\check\phi$ for $\cI$ with $\cro(\check \phi)\le \sum_{\hat I\in \hat \iset}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}$.
Since $|\hat E_{\sf temp}|\le \mu^{b^*}\cdot \mu^{100}\cdot \tilde g$, altogether we get that
$$\cro(\check \phi)
\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+\cm\cdot\mu^{b^*}\cdot \mu^{100}\cdot \tilde g
\le \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I))+\optcrors(\cI)\cdot\mu^{5000}+g_1^j\cdot\mu^{3b^*+300b},$$
as $b^*>100$.
\end{proof}

\subsubsection*{The algorithm for comuting the collection $\iset^{(j)}$}
We now partition the resulting collection $\iset^*$ into two subsets: set $\iset^*_1$ contains all small instances in $\iset^*$; and set $\iset^*_2$ contains all remaining instances. 
We denote $\hat \iset_1=\set{\hat I\mid I\in 
\iset^*_1}$.
Since every instance in $\iset^*_2$ is large (that is, $\hat m(I)\ge \cm/\mu^{b^*}$), from Invariant \ref{prop: number of edges}, we get that $|\iset^*_2|\le \mu^{b^*}$.
From the pre-processing step, for each instance $I=(G,\Sigma)\in \iset^*_2$, its skeleton $K(I)$ is $\tilde g$-connected in $G$. Since $|E(G)|\ge \cm/\mu^{b^*}$, $\tilde g\ge \left(
\frac{g_1^j}{|E(G)|}+g_2^j \right)$, so its skeleton $K(I)$ is $g_3(I)$-connected in $G$, for $g_3(I)=\left(
\frac{g_1^j}{|E(G)|}+g_2^j \right)$.

For each instance $I\in \iset^*$, we denote by $\psi(I)$ the solution to $I$ guaranteed by Invariant \ref{prop: good drawings}.
We use the following observation.
\begin{observation}
\label{obs: not too large}
	If $\optcrors(\cI)\le \cm^2/\mu^{61b-2b^*}$, then for each instance $I=(G,\Sigma)\in \iset^*_2$, the drawing $\psi(I)$ satisfies that $\cro(\psi(I))\le |E(G)|^2/\mu^{60b}$ and $|\chi^{\dirty}(\psi(I))|\le  |E(G)|/\mu^{60b}$.
\end{observation}
\begin{proof}
	Let $I=(G,\Sigma)$ be an instance in $\iset^*_2$, so $|E(G)|\ge \cm/\mu^{b^*}$.
	Recall that, from \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\le 2\cdot\optcrors(\cI)$, so $\cro(\psi(I))\le 2\cdot\optcrors(\cI)$. Therefore, if $\optcrors(\cI)\le \cm^2/\mu^{61b-2b^*}$, then
	\[
	\cro(\psi(I))\le 2\cdot\optcrors(\cI) \le \frac{2\cdot \cm^2}{\mu^{61b-2b^*}}\le 
	\frac{ \cm^2}{\mu^{60b-2b^*}} 
	= \frac{ (\cm/\mu^{b^*})^2}{\mu^{60b}} 
	\le \frac{|E(G)|^2}{\mu^{60b}}.
	\]
	Also recall that, from \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\le \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so $|\chi^{\dirty}(\psi(I))| < \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. Therefore,
	\[
	|\chi^{\dirty}(\psi(I))|\le \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm} 
	\le \frac{\cm\cdot \mu^{b^*}}{\mu^{61b-2b^*}}
	\le \frac{\cm}{\mu^{60b+b^*}}
	= \frac{(\cm/\mu^{b^*})}{\mu^{60b}}
	\le \frac{|E(G)|}{\mu^{60b}},
	\]
	since $b\ge 4b^*$. 
\end{proof}

Finally, we consider every instance $I\in \iset^*_2$ one by one. 
For each such instance $I$, we apply the algorithm from \Cref{thm: phase 2} to instance $I$, skeleton structure $\kset(I)$, the parameters $b,g^j_1,g^j_2$ defined above.  
We denote by $I'=(G',\Sigma')$ the resulting instance of \cnwrs, and by $\hat I'$ the $\kset(I)$-contraction of this instance. We then denote $\hat \iset'_2=\set{\hat I'\mid I\in \iset^*_2}$. The final output of our algorithm is the collection $\iset^{(j)}=\hat\iset_1\cup\hat \iset'_2$ of subinstances of $\cI$. 




\subsubsection*{The analysis of the algorithm}

We now verify that the output collections $\iset^{(1)},\ldots,\iset^{(z)}$ of subinstances of $\cI$ have all required properties. 
Consider an index $1\le j\le z$ and consider the algorithm for constructing collection $\iset^{(j)}$.
%First, the algorithm from \Cref{thm: phase 1} ensures that, for every instance $I\in \iset$, if the corresponding contracted instance $\hat I=(\hat G,\hat \Sigma)$  is a wide instance, then $|E(\hat G)|\le \cm/\mu$. 

First, from Invariant \ref{prop: wide or not}, for every instance $I\in \iset^*$, if the corresponding contracted instance $\hat I=(\hat G,\hat \Sigma)$  is a wide instance, then $|E(\hat G)|\le \cm/\mu$.
If instance $I$ lies in $\iset^*_2$, and $\hat I'=(\hat G',\hat\Sigma')$ is the $\kset(I)$-contraction of instance $I'$, then $|E(\hat G')|\leq |E(\hat G)|$, and, if $\hat I$ is not a wide instance, then neither is $\hat I'$. This is since graph $\hat G'$ can be obtained from graph $\hat G$ by deleting the edges of $E^{\del}(I)$ from it. Therefore, we are guaranteed that, for every instance $I'=(G',\Sigma')\in \iset^{(j)}$, if $I'$ is a wide instance, then $|E(G')|\le \cm/\mu$.

Second, from Invariant \ref{prop: number of edges},
%The algorithm from \Cref{thm: phase 1} also guarantees that $\sum_{I\in  \iset}\hm(I)\le \cm$.
$\sum_{I\in  \iset^*}\hm(I)\le \cm$.
Since, for every instance $I\in \iset^*_2$, the corresponding resulting instance $\hat I'=(\hat G',\Sigma')\in \hat \iset_2'$ has $|E(\hat G')|\leq \hat m(I)$, we get that $\sum_{I'=(G',\Sigma')\in \iset^{(j)}}|E(G')|\le \cm$.

Third, we construct an algorithm that, given a solution to each instance in $\iset^{(j)}$, computes a solution $\phi$ to instance $\cI$.
For each instance $I\in \iset^*_2$,  we let $\hat I=(\hat G,\hat \Sigma)$ be the corresponding  $\kset(I)$-contracted instance, and let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance corresponding to the instance $I'$. Note that $V(\hat G)=V(\hat G')$ and $E(\hat G')=E(\hat G)\setminus E^{\del}(I)$. We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\del}(I)$ into the solution $\phi(\hat I')$ to instance $\hat I'$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$.
Then we use the algorithm from \Cref{obs: algo combine drawings} to compute a drawing of $\cI$. It is clear that the algorithm is efficient.


%\znote{the algorithm for computing the drawing}

From now on, we let $j^*$ be the unique integer that $2^{j^*-1}< 2\cdot \optcrors(\cI)\le 2^{j^*}$. Since $\optcrors(\cI)\le \cm^2$, $j^*\le 2\log m$, so $1\le j^*\le z$. We will show that the collection $\iset^{(j^*)}$ satisfies the property required in the last bullet of \Cref{lem: many paths}. Consider now the algorithm for constructing the collection $\iset^{(j^*)}$.

Recall that we have set $g_1^{j^*}=2^{j^*}$ and $g_2^{j^*}=g_1^{j^*}\cdot \mu^{b^*}/\cm$. 
%
Therefore, from Invariant \ref{prop: good drawings}, the semi-clean solutions $\psi(I)$ to $I$ for instances $I\in \iset^*$ satisfy that
$\sum_{I\in \tempiset}\cro(\psi(I))\le g_1^{j^*}$ and $\sum_{I\in \tempiset}|\chi^{\dirty}(\psi(I))|\leq  g_2^{j^*}$.
So for each instance $I\in \iset^*$, $\cro(\psi(I))\le g_1^{j^*}$ and $|\chi^{\dirty}(\psi(I))| \leq  g_2^{j^*}$.
%From \Cref{thm: phase 1}, if $\optcrors(\cI)\le \cm^2/\mu^{c'}$, and the bad event $\tilde \event'_1$ does not happen, then for each instance $I\in \iset$ there exists a semi-clean solution $\psi(I)$ to
Combined with \Cref{obs: not too large}, we get that, for each instance $I=(G,\Sigma)\in \iset^*_2$, both $\cro(\psi(I))\le \min\set{g_1^*,|E(G)|^2/\mu^{60b}}$ and $|\chi^{\dirty}(\psi(I))|\le \min\set{g_2^*, |E(G)|/\mu^{60b}}$ hold.
(We have used the fact that \fbox{$c'>61b-2b^*$}.)

For each instance $I\in \iset^*_2$, we denote by $\tilde \event_2(I)$ the bad event that the application of the algorithm from \Cref{thm: phase 2} was unsuccessful, so $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$.
%
Let $\tilde \event_2'$ be the bad event that any of the events in $\set{\tilde \event_2(I)\mid I\in \iset^*_2}$ happened. Since, from the above discussion, $|\iset^*_2| \leq \mu^{b^*}$, and, for every instance $I\in \iset^*_2$, $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$, while $b>2b^*$, from the Union Bound, we get that $\prob{\tilde \event_2'}<1/\mu^4$. Lastly, we let $\tilde \event'$ be the bad event that either $\tilde \event_1'$ or $\tilde \event_2'$ happened. Clearly, $\prob{\tilde \event'}\leq \prob{\tilde \event_1'}+\prob{\tilde \event_2'}\leq 1/\mu^2$.
We use the following two observations in order to complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: composing contracted solutions}
Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then there is an efficient algorithm, that, given a solution $\phi(I')$ for every instance $I'\in \iset^{(j^*)}$, computes a solution $\check \phi$ to instance $\cI$, with $\cro(\check\phi)\leq  \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I')) + \optcrors(\check I)\cdot\mu^{O(1)}$.
\end{observation}
\begin{proof}
We assume that $\optcrors(I)\leq m^2/\mu^{c'}$, Event $\tilde \event'$ did not happen, and that  we are given a solution $\phi(I')$ to every instance $I'\in \iset^{(j^*)}$. We now show an efficient algorithm to compute a solution $\check \phi$ to instance $\cI$. In order to do so, we first consider every instance $I\in \iset^*_2$ one by one, and compute a solution $\phi(\hat I)$ to instance $\hat I$, from the solution $\phi(\hat I')$ to instance $\hat I'$. 

Consider now some instance $I=(G,\Sigma)\in \iset^*_2$. Let $\hat I=(\hat G,\hat \Sigma)$ be the corresponding  $\kset(I)$-contracted instance, and let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance corresponding to the instance $I'$. Note that $V(\hat G)=V(\hat G')$ and $E(\hat G')=E(\hat G)\setminus E^{\del}(I)$. We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\del}(I)$ into the solution $\phi(\hat I')$ to instance $\hat I'$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$, whose cost is at most $\cro(\phi(\hat I'))+|E^{\del}(I)|\cdot |E(G)|$. If Event $\tilde \event'$ does not happen, then $|E^{\del}(I)|\leq \big(\frac{g_1^{j^*}}{|E(G)|}+g_2^{j^*}\big)\cdot\mu^{O(1)}=\frac{\optcrors(\cI)\cdot\mu^{O(1)}}{|E(G)|}$, and so $\cro(\phi(\hat I))\leq \cro(\phi(\hat I'))+\optcrors(\cI)\cdot \mu^{O(1)}$.
Now using the algorithm from \Cref{obs: algo combine drawings},
%
%We have now obtained, for every instance $I\in \iset$, a solution $\phi(\hat I)$ to the corresponding contracted instance $\hat I$. This solution immediately defines a solution $\phi(I)$ to instance $I$ that is clean with respect to $\kset(I)$, with $\cro(\phi(I))\leq \cro(\phi(\hat I))$. 
%Lastly, using the algorithm from \Cref{thm: phase 1}, 
we obtain a solution 
$\check\phi$ to instance $\cI$, whose cost is bounded by:
%
\[
\begin{split}
\cro(\check \phi)&\leq  \sum_{\hat I\in \hat \iset^*}\cro(\phi(\hat I)) + \optcrors(\cI)\cdot\mu^{O(1)}\\
&\leq \sum_{I\in \iset^*_1}\cro(\phi(\hat I))+\sum_{I\in \iset^*_2}\left (\cro(\phi(\hat I'))+\optcrors(\cI)\cdot \mu^{O(1)}\right )+\optcrors(\cI)\cdot\mu^{O(1)}\\
&\le \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I'))+|\iset^*_2|\cdot\optcrors(\cI)\cdot\mu^{O(1)}+\optcrors(\cI)\cdot\mu^{O(1)}\\
&\le \sum_{I'\in \iset^{(j^*)}}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)},
\end{split}
\]
%
as $|\iset^*_2|=\mu^{O(1)}$.
%From \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and Event $\tilde \event'$ did not happen, then $\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$. Therefore, we get that $\cro(\check \phi)\leq \sum_{I'\in \hat \iset'}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)}$.
\end{proof}


%Lastly, the following observation will complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: cheap solutions to final instances}
	Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then $\sum_{I'\in \iset^{(j^*)}}\optcrors(I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}$.
\end{observation}
\begin{proof}
	We bound $\sum_{I\in \iset^*_1}\optcrors(\hat I)$ and $\sum_{I\in \iset^*_2}\optcrors(\hat I')$ separately.
	
	From \Cref{thm: phase 2}, if Event $\tilde \event'$ did not happen, then, for every instance $I=(G,\Sigma)\in \iset^*_2$, 
	there is a solution $\psi(I')$ to the corresponding instance $I'$, that is clean with respect to $\kset(I)$, with $\cro(\psi(I'))\leq \cro(\psi(I))\cdot (\log \cm)^{O(1)}+|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}$. 
	From \Cref{obs: clean solution to contracted}, there is a solution to the corresponding contracted instance $\hat I'$, of cost at most $\cro(\psi(I'))$. Altogether, we get that:
	%
	\[\begin{split}
	\sum_{I\in \iset^*_2}\optcrors(\hat I')&\leq \sum_{I\in \iset^*_2}\left(\cro(\psi(I))+\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}\right )\cdot (\log \cm)^{O(1)}.\\
	&\leq \sum_{I\in \iset^*_2}\cro(\psi(I))\cdot (\log \cm)^{O(1)}+\left (\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right )^2\cdot (\log \cm)^{O(1)}\\
	&\hspace{4cm}+ \frac{\cm\cdot (\log \cm)^{O(1)}}{\mu^b}\cdot\left(\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right ).
	\end{split}
	\]
	%
	From Invariant \ref{prop: good drawings}, $\sum_{I\in \iset^*}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$ and $\sum_{I\in \iset^*}|\chi^{\dirty}(\psi(I))|\leq \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. Additionally, since we have assumed that $\optcrors(I)\leq m^2/\mu^{c'}$ for a large enough constant $c'>2b^*$, 
	$$\left (\sum_{I\in \iset^*_2}|\chi^{\dirty}(\psi(I))|\right )^2\leq \frac{(\optcrors(\cI))^2 \mu^{2b^*}}{\cm^2}\leq \optcrors(\cI).$$ Altogether, we get that:
	%
	\[
	\begin{split}
	 \sum_{I\in \iset^*_2}\optcrors(\hat I')&\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}+\frac{\optcrors(\cI)\cdot \mu^{b^*}\cdot  (\log \cm)^{O(1)}}{\mu^b}\\
	 &\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}, \end{split}\]
	since $b>4b^*$.
%	
%	Lastly, since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}\hat m(I)\le \cm$, and since $b>b^*$, $\sum_{I\in \iset_3}\optcrors(\hat I')\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}$.  

Next, we bound $\sum_{I\in \iset^*_1}\optcrors(\hat I)$. Consider some instance $I=(G,\Sigma)\in \iset^*_1$ and the solution $\psi(I)$ that is semi-clean with respect to $\kset(I)$. Let $K(I)$ be the skeleton associated with the skeleton structure $\kset(I)$. Let $E^{\dirty}(I)\subseteq E(G)\setminus E(K(I))$ be the set of all edges $e$, such that the image of $e$ in $\psi(I)$ crosses the image of some edge of $K(I)$.  Let $\hat I=(\hat G,\hat \Sigma)$ be the $\kset(I)$-contracted instance corresponding to instance $I$.


Denote $G'=G\setminus E^{\dirty}(I)$, and let $\Sigma'$ be the rotation system for graph $G'$ that is induced by $\Sigma$. Observe that $\kset(I)$ is a valid skeleton structure for the resulting instance $I'=(G',\Sigma')$. Let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance associated with $I'$. Observe that the drawing $\psi(I)$ of instance $I$ induces a drawing $\psi(I')$ of instance $I'$ that is clean with respect to $\kset(I)$. From \Cref{obs: clean solution to contracted}, there is a solution $\psi(\hat I')$ to the contracted instance $\hat I'$ with $\cro(\psi(\hat I'))\leq \cro(\psi(I'))\leq \cro(\psi(I))$. 
We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\dirty}(I)$ into the drawing $\psi(\hat I')$ to obtain a drawing $\psi(\hat I)$ of instance $\hat I$, with the number of crossings bounded by $\cro(\psi(\hat I'))+|E^{\dirty}(I)|\cdot |E(\hat G)|\leq \cro(\psi(I))+|E^{\dirty}(I)|\cdot |E(\hat G)|$.

Recall that $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$ (since instance $I$ is small), so $\cro(\psi(\hat I))
\leq \cro(\psi(I))+|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}$. %(since $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$). 
We then get that:
%
\[\sum_{I\in \iset^*_1} \optcrors(\hat I)\leq 
\sum_{I\in \iset^*_1}\cro(\psi(I))+\sum_{I\in \iset^*_1}|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}.
\]
%
From Invariant \ref{prop: good drawings}, $\sum_{I\in \iset^*}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$ and $\sum_{I\in \iset^*}|\chi^{\dirty}(\psi(I))|\leq \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$.
Therefore, 
$$\sum_{I\in \iset^*_1} \optcrors(\hat I)\leq  2\cdot\optcrors(\cI)+\frac{\cm}{\mu^{b^*}} \cdot  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\leq O(\optcrors(\cI)).$$


\iffalse{analysis for previous iset_2, which should be an empty set}
Assume now that $I\in \iset_2$. We partition the set $\iset_2$ of instances into two subsets: set $\iset_2'$ containing all instances $I=(G,\Sigma)$ with $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, and set $\iset_2''$ containing all remaining instances.
As before, for every instance $I=(G,\Sigma)\in \iset_2$, we denote by $\hat m(I)$ the number of edges in the contracted graph $\hat I$. 


Next, we bound $\sum_{I\in \iset_2'}\cro(\psi(\hat I'))$. Recall that for every instace $I=(G,\Sigma)\in \iset_2'$:
%
\[\cro(\psi(I))> \frac{|E(G)|^2}{\mu^{60b}}\geq \frac{(\hat m(I))^2}{\mu^{60b}}\geq \frac{\hat m(I)\cdot \cm}{\mu^{60b+b^*}},\]
%
since instance $I$ must be large. Since,  
from \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)\leq 2\cm^2/\mu^{c'}$, we get that $\sum_{I\in \iset_2'}\hat m(I)\leq \frac{2\cm}{\mu^{c'-60b-b^*}}$. Lastly, since, from  \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that:
%
\[\begin{split}
\sum_{I\in \iset_2'} \optcrors(\hat I)&\leq 
\sum_{I\in \iset_2'}\cro(\psi(I))+\sum_{I\in \iset_2'}|\chi^{\dirty}(I)|\cdot \hm(I)\\
&\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2'}\hat m(I) \right )\\
&\leq 2\cdot\optcrors(\cI)+\frac{2\cm}{\mu^{c'-60b-b^*}}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
&\leq O(\optcrors(\cI)).\end{split}
\]
%
It now remains to consider instances $I\in \iset_2''$. Recall that, for each such instance $I=(G,\Sigma)$,  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{60b}$. 
 Since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that $\sum_{I\in \iset_2''}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}$. 
 Therefore:
%
 \[\begin{split}
 \sum_{I\in \iset_2''} \optcrors(\hat I)&\leq 
 \sum_{I\in \iset_2''}\cro(\psi(I))+\sum_{I\in \iset_2''}|\chi^{\dirty}(I)|\cdot \hm(I)\\
 &\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2''}\hat m(I) \right )\\
 &\leq 2\cdot\optcrors(\cI) + \frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
 &\leq O(\optcrors(\cI))
 ,\end{split}
 \]
 %
 since $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and $c'$ is a large enough constant.
 \fi
 
 

Altogether, we get that 
$$\sum_{I'\in \iset^{(j^*)}}\optcrors(I')=\sum_{I\in \iset^*_1}\optcrors(\hat I)+\sum_{I\in \iset^*_2}\optcrors(\hat I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}.$$
\end{proof}



\iffalse

The calculations

---------------------------------------------------



\begin{itemize}
	\item $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)$
	
	\item $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$
	
	\item in $\iset_2$: either $\cro(\psi(I))> |E(G)|/\mu^{2b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$.
	
	\item when pulling edges back, we will pay $\sum_{I\in \iset_2}\hm(I)\cdot |\chi^{\dirty}(\psi(I))|$.
	
	\item let's say that $\iset_2'$ contains all instances with $\cro(\psi(I))> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{2b}$. But $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)<\cm/\mu^{c'}$. So $\sum_{I\in \iset_2'}\hat m(I)\leq \mu^{2b}\cdot \cm/\mu^{c'}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so total increase in number of crossings is less than $\optcrors(\cI)$.
	
	\item Now $\iset_2''$ contains all instances with $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$. But $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. So $\sum_{I\in \iset_2}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+b}}{\cm}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so the total increase in number of crossings is at most $\frac{(\optcrors(\cI))^2\cdot \mu^{2b^*+b}}{(\cm)^2}$. Assuming that $\optcrors(\cI)<\cm^2/\mu^{c'}$ it's at most $\optcrors(\cI)$.
\end{itemize}





----------------------------------------------
\fi

$\ $

In the remainder of this section we focus on the proof of \Cref{thm: phase 2}. Throughout the proof, we denote the instance $I=(G,\Sigma)$ that serves as the input to the algorithm by $\cI'=(\cG',\cSigma')$, with $|E(\cG')|$ denoted by $\cm'$. We denote the skeleton structure $\kset(I)$ by $\check \kset=(\jset_1,\ldots,\jset_r)$, where $r\leq \mu^{100}$. For all $1\leq i\leq r$, we denote $\jset_i=(J_i,\set{b_u}_{u\in V(J_i)},\rho_{J_i})$. 
We start with the intuition for the proof. We denote by $\check K=\bigcup_{i=1}^rJ_i$ the skeleton of $\cG'$ associated with the skeleton structure $\check \kset$. We can assume that there exists a solution $\check \psi$ to instance $\cI$ that is semi-clean with respect to $\check\kset$. 
%(as otherwise we can let $E^{\del}(\cI')=E(\cG)\setminus E(\check K)$ \znote{what does this mean?} ). 

==> finish-proof-interesting_bkup0925.tex <==
\subsubsection{Completing the Proof of \Cref{lem: many paths}}
\label{subsubsec: finish the proof}
Given an input instance $\cI=(\cG,\cSigma)$, we first apply the algorithm from \Cref{thm: phase 1} to this input. If the algorithm fails, then we terminate the algorithm and return FAIL as well. Recall that, from \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/\mu^3$. Assume now that the algorithm from \Cref{thm: phase 1} did not fail. In this case, if  $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, then with probability at least $(1-1/\mu^3)$, the algorithm is successful. We denote by $\tilde \event_1'$ the bad event that the application of this algorithm is unsuccessful, so $\prob{\tilde \event_1'}\leq 1/\mu^3$. Let $\iset$ be the collection of subinstances of $\cI$ computed by the algorithm from \Cref{thm: phase 1}. Recall that, if Event $\tilde \event'_1$ did not happen, then there is some constant $b^*$, and, for every instance $I\in \iset$, there is a solution $\psi(I)$ to $I$, that is semi-clean with respect to $\kset(I)$, such that 
$\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$, and $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. We set the parameter $b$ to be a large enough constant, so that $b\geq 2b^*$ holds.



Recall that, for every instance $I=(G,\Sigma)\in \iset$, we have denoted by $\hat I=(\hat G,\hat \Sigma)$ the corresponding $\kset(I)$-contracted instance, and by $\hat m(I)=E(\hat G)$. We say that instance $I$ is \emph{small} if $\hat m(I)\leq \frac{\cm}{\mu^{b^*}}$, and otherwise it is \emph{large}. We partition the set $\iset$ of instances into three subsets: set $\iset_1$ containing all small instances; set $\iset_2$ containing all large instances $I=(G,\Sigma)\in \iset$ for which either $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{60b}$ holds, and set $\iset_3$ containing all remaining instances. Since the algorithm from \ref{thm: phase 1} guarantees that $\sum_{I\in \iset}\hat m(I)\le \cm$, we get that $|\iset_2\cup \iset_3|\leq \mu^{b^*}$. We let $\hat \iset_1=\set{\hat I\mid I\in \iset_1}$ contain the set of all contracted instances corresponding to the instances of $\iset_1$, and we define set $\hat \iset_2$ of instances corresponding to the instances of $\iset_2$ similarly.
\znote{We do not know $\cro(\psi(I))$ and $\chi^{\dirty}(\psi(I))$ so we cannot distinguish $\iset_2$ from $\iset_3$?}


Next, we consider every instance $I\in \iset_3$ one by one. For each such instance $I$, we apply the algorithm from \Cref{thm: phase 2} to instance $I$, skeleton structure $\kset(I)$, and the parameter $b$ defined above. Let $\tilde \event_2(I)$ be the bad event that this application of the algorithm was unsuccessful, so $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$. We denote by $I'=(G',\Sigma')$ the resulting instance of \cnwrs,  and by $\hat I'$ the $\kset(I)$-contraction of this instance. We then denote $\hat \iset_3'=\set{\hat I'\mid I\in \iset_3}$. The final output of our algorithm is the collection $\iset'=\hat\iset_1\cup\hat \iset_2\cup \hat \iset_3'$ of subinstances of $\cI$. 






We now verify that $\iset'$ has all required properties. First, the algorithm from \Cref{thm: phase 1} ensures that, for every instance $I\in \iset$, if the corresponding contracted instance $\hat I=(\hat G,\hat \Sigma)$  is a wide instance, then $|E(\hat G)|\le \cm/\mu$. If instance $I$ lies in $\iset_3$, and $\hat I'=(\hat G',\hat\Sigma')$ is the $\kset(I)$-contraction of instance $I'$, then $|E(\hat G')|\leq |E(\hat G)|$, and, if $\hat I$ is not a wide instance, then neither is $\hat I'$. This is since graph $\hat G'$ can be obtained from graph $\hat G$ by deleting the edges of $E^{\del}(I)$ from it. Therefore, we are guaranteed that, for every instance $I'=(G',\Sigma')\in \iset'$, if $I'$ is a wide instance, then $|E(G')|\le \cm/\mu$.

The algorithm from \Cref{thm: phase 1} also guarantees that  $\sum_{I\in  \iset}\hm(I)\le \cm$. Since, for every instance $I\in \iset_3$, the corresponding instance $\hat I'=(\hat G',\Sigma')\in \hat \iset_3'$ has $|E(\hat G')|\leq \hat m(I)$, we get that $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le \cm$.

Let $\tilde \event_2'$ be the bad event that any of the events in $\set{\tilde \event_2(I)\mid I\in \iset_3}$ happened. Since, from the above discussion, $|\iset_3| \leq \mu^{b^*}$, and, for every instance $I\in \iset_3$, $\prob{\tilde \event_2(I)}\leq 1/\mu^{2b}$, while $b>2b^*$, from the Union Bound, we get that $\prob{\tilde \event_2'}<1/\mu^4$. Lastly, we let $\tilde \event'$ be the bad event that either $\tilde \event_1'$ or $\tilde \event_2'$ happened. Clearly, $\prob{\tilde \event'}\leq \prob{\tilde \event_1'}+\prob{\tilde \event_2'}\leq 1/\mu^2$.
We use the following two observations in order to complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: composing contracted solutions}
	Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then there is an efficient algorithm, that, given a solution $\phi(I')$ for every instance $I'\in \iset'$, computes a solution $\check \phi$ to instance $\cI$, with $\cro(\check\phi)\leq  \sum_{I'\in \iset'}\cro(\phi(I')) + \optcrors(\check I)\cdot\mu^{O(1)}$.
	\end{observation}
\begin{proof}
We assume that $\optcrors(I)\leq m^2/\mu^{c'}$, Event $\tilde \event'$ did not happen, and that  we are given a solution $\phi(I')$ to every instance $I'\in \iset'$. We now show an efficient algorithm to compute a solution $\check \phi$ to instance $\cI$. In order to do so, we consider every instance $I\in \iset_3$ one by one, and compute a solution $\phi(\hat I)$ to instance $\hat I$, from the solution $\phi(\hat I')$ to instance $\hat I'$. 

Consider now some instance $I=(G,\Sigma)\in \iset_3$. Let $\hat I=(\hat G,\hat \Sigma)$ be the corresponding  $\kset(I)$-contracted instance, and let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance corresponding to the instance $I'$. Note that $V(\hat G)=V(\hat G')$ and $E(\hat G')=E(\hat G)\setminus E^{\del}(I)$. We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\del}(I)$ into the solution $\phi(\hat I')$ to instance $\hat I'$, obtaining a solution $\phi(\hat I)$ to instance $\hat I$, whose cost is at most $\cro(\phi(\hat I'))+|E^{\del}(I)|\cdot |E(G)|$. If Event $\tilde \event'$ does not happen, then $|E^{\del}(I)|\leq \frac{\cro(\psi(I))\cdot \mu^{O(1)}}{|E(G)|}$, and so $\cro(\phi(\hat I))\leq \cro(\phi(\hat I'))+\cro(\psi(I))\cdot \mu^{O(1)}$.
%
%We have now obtained, for every instance $I\in \iset$, a solution $\phi(\hat I)$ to the corresponding contracted instance $\hat I$. This solution immediately defines a solution $\phi(I)$ to instance $I$ that is clean with respect to $\kset(I)$, with $\cro(\phi(I))\leq \cro(\phi(\hat I))$. 
Lastly, using the algorithm from \Cref{thm: phase 1}, we obtain a solution 
$\check\phi$ to instance $\cI$, whose cost is bounded by:
%
\[
\begin{split}
\cro(\check \phi)&\leq  \sum_{\hat I\in \hat \iset}\cro(\phi(\hat I)) + \optcrors(\cI)\cdot\mu^{O(1)}\\
&\leq \sum_{I\in \iset_1\cup \iset_2}\cro(\phi(\hat I))+\sum_{I\in \iset_3}\left (\cro(\phi(\hat I'))+\cro(\psi(I))\cdot \mu^{O(1)}\right )+\optcrors(\cI)\cdot\mu^{O(1)}\\
&=\sum_{I'\in \hat \iset'}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)}+\sum_{I\in \iset_3}\cro(\psi(I))\cdot \mu^{O(1)}.
\end{split}
\]
%
From \Cref{thm: phase 1}, if $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and Event $\tilde \event'$ did not happen, then 
$\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$.
Therefore, we get that $\cro(\check \phi)\leq \sum_{I'\in \hat \iset'}\cro(\phi(I'))+\optcrors(\cI)\cdot\mu^{O(1)}$.
\end{proof}


Lastly, the following observation will complete the proof of \Cref{lem: many paths}.

\begin{observation}\label{obs: cheap solutions to final instances}
	Assume that $\optcrors(I)\leq m^2/\mu^{c'}$, and that event $\tilde \event'$ did not happen. Then $\sum_{I'\in \iset'}\optcrors(I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}$.
\end{observation}
\begin{proof}
	We bound $\sum_{I\in \iset_1\cup \iset_2}\optcrors(\hat I)$ and $\sum_{I\in \iset_3}\optcrors(\hat I')$ separately.
	
	From \Cref{thm: phase 2}, if Event $\tilde \event'$ did not happen, then, for every instance $I=(G,\Sigma)\in \iset_3$, 
	there is a solution $\psi(I')$ to the corresponding instance $I'$, that is clean with respect to $\kset(I)$, with $\cro(\psi(I'))\leq \cro(\psi(I))\cdot (\log \cm)^{O(1)}+|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}$. 
	From \Cref{obs: clean solution to contracted}, there is a solution to the corresponding contracted instance $\hat I'$, of cost at most $\cro(\psi(I'))$. Altogether, we get that:
	%
	\[\begin{split}
	\sum_{I\in \iset_3}\optcrors(\hat I')&\leq \sum_{I\in \iset_3}\left(\cro(\psi(I))+\sum_{I\in \iset_3}|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}\right )\cdot (\log \cm)^{O(1)}.\\
	&\leq \sum_{I\in \iset_3}\cro(\psi(I))\cdot (\log \cm)^{O(1)}+\left (\sum_{I\in \iset_3}|\chi^{\dirty}(\psi(I))|\right )^2\cdot (\log \cm)^{O(1)}\\
	&\hspace{4cm}+ \frac{\cm\cdot (\log \cm)^{O(1)}}{\mu^b}\cdot\left(\sum_{I\in \iset_3}|\chi^{\dirty}(\psi(I))|\right ).
	\end{split}
	\]
	%
	From \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)$ and $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq O\left(\frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\right )$. Additionally, since we have assumed that $\optcrors(I)\leq m^2/\mu^{c'}$ for a large enough constant $c'$, $\left (\sum_{I\in \iset_3}|\chi^{\dirty}(\psi(I))|\right )^2\leq \frac{(\optcrors(\cI))^\cdot \mu^{2b^*}}{\cm^2}\leq \optcrors(\cI)$. Altogether, we get that:
	%
	\[
	\begin{split}
	 \sum_{I\in \iset_3}\optcrors(\hat I')&\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}+\frac{\optcrors(\cI)\cdot \mu^{b^*}\cdot  (\log \cm)^{O(1)}}{\mu^b}\\
	 &\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}, \end{split}\]
	since $b>b^*$.
%	
%	Lastly, since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}\hat m(I)\le \cm$, and since $b>b^*$, $\sum_{I\in \iset_3}\optcrors(\hat I')\leq \optcrors(\cI)\cdot  (\log \cm)^{O(1)}$.  

Next, we bound $\sum_{I\in \iset_1\cup \iset_2}\optcrors(\hat I)$. Consider some instance $I=(G,\Sigma)\in \iset_1$ and the solution $\psi(I)$ that is semi-clean with respect to $\kset(I)$. Let $K(I)$ be the skeleton associated with the skeleton structure $\kset(I)$. Let $E^{\dirty}(I)\subseteq E(G)\setminus E(K(I))$ be the set of all edges $e$, such that the image of $e$ in $\psi(I)$ crosses the image of some edge of $K(I)$.  Let $\hat I=(\hat G,\hat \Sigma)$ be the $\kset(I)$-contracted instance corresponding to instance $I$.


Denote $G'=G\setminus E^{\dirty}(I)$, and let $\Sigma'$ be the rotation system for graph $G'$ that is induced by $\Sigma$. Observe that $\kset(I)$ is a valid skeleton structure for the resulting instance $I'=(G',\Sigma')$. Let $\hat I'=(\hat G',\hat \Sigma')$ be the $\kset(I)$-contracted instance associated with $I'$. Observe that the drawing $\psi(I)$ of instance $I$ induces a drawing $\psi(I')$ of instance $I'$ that is clean with respect to $\kset$. From \Cref{obs: clean solution to contracted}, there is a solution $\psi(\hat I')$ to the contracted instance $\hat I'$ with $\cro(\psi(\hat I'))\leq \cro(\psi(I'))\leq \cro(\psi(I))$. 
We use the algorithm from \Cref{lem: edge insertion} in order to insert the edges of $E^{\dirty}(I)$ into the drawing $\psi(\hat I')$ to obtain a drawing $\psi(\hat I)$ of instance $\hat I$, with the number of crossings bounded by $\cro(\psi(\hat I'))+|E^{\dirty}(I)|\cdot |E(\hat G)|\leq \cro(\psi(I))+|E^{\dirty}(I)|\cdot |E(\hat G)|$.

We now consider three cases. First, if $I\in \iset_1$, then $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$, so $\cro(\psi(\hat I))
\leq \cro(\psi(I))+|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}$ (since $|E(\hat G)|\leq \frac{\cm}{\mu^{b^*}}$). We then get that:
%
\[\sum_{I\in \iset_1} \optcrors(\hat I)\leq 
\sum_{I\in \iset_1}\cro(\psi(I))+\sum_{I\in \iset_1}|\chi^{\dirty}(I)|\cdot  \frac{\cm}{\mu^{b^*}}.
\]
%
From \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\leq 2\cdot\optcrors(\cI)$ and $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq O\left(\frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\right )$.
Therefore, $\sum_{I\in \iset_1} \optcrors(\hat I)\leq  2\optcrors(\cI)+\frac{\cm}{\mu^{b^*}} \cdot  O\left(\frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\right )\leq O(\optcrors(\cI))$.

Assume now that $I\in \iset_2$. We partition the set $\iset_2$ of instances into two subsets: set $\iset_2'$ containing all instances $I=(G,\Sigma)$ with $\cro(\psi(I))> |E(G)|^2/\mu^{60b}$, and set $\iset_2''$ containing all remaining instances.
As before, for every instance $I=(G,\Sigma)\in \iset_2$, we denote by $\hat m(I)$ the number of edges in the contracted graph $\hat I$. 


Next, we bound $\sum_{I\in \iset_2'}\cro(\psi(\hat I'))$. Recall that for every instace $I=(G,\Sigma)\in \iset_2'$:
%
\[\cro(\psi(I))> \frac{|E(G)|^2}{\mu^{60b}}\geq \frac{(\hat m(I))^2}{\mu^{60b}}\geq \frac{\hat m(I)\cdot \cm}{\mu^{60b+b^*}},\]
%
since instance $I$ must be large. Since,  
from \Cref{thm: phase 1}, $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)\leq 2\cm^2/\mu^{c'}$, we get that $\sum_{I\in \iset_2'}\hat m(I)\leq \frac{2\cm}{\mu^{c'-60b-b^*}}$. Lastly, since, from  \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that:
%
\[\begin{split}
\sum_{I\in \iset_2'} \optcrors(\hat I)&\leq 
\sum_{I\in \iset_2'}\cro(\psi(I))+\sum_{I\in \iset_2'}|\chi^{\dirty}(I)|\cdot \hm(I)\\
&\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2'}\hat m(I) \right )\\
&\leq 2\cdot\optcrors(\cI)+\frac{2\cm}{\mu^{c'-60b-b^*}}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
&\leq O(\optcrors(\cI)).\end{split}
\]
%
It now remains to consider instances $I\in \iset_2''$. Recall that, for each such instance $I=(G,\Sigma)$,  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{60b}$. 
 Since, from \Cref{thm: phase 1}, $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, we get that $\sum_{I\in \iset_2''}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}$. 
 Therefore:
%
 \[\begin{split}
 \sum_{I\in \iset_2''} \optcrors(\hat I)&\leq 
 \sum_{I\in \iset_2''}\cro(\psi(I))+\sum_{I\in \iset_2''}|\chi^{\dirty}(I)|\cdot \hm(I)\\
 &\leq 2\cdot\optcrors(\cI)+\left ( \sum_{I\in \iset}|\chi^{\dirty}(\psi(I))| \right )\cdot \left ( \sum_{I\in \iset_2''}\hat m(I) \right )\\
 &\leq 2\cdot\optcrors(\cI) + \frac{\optcrors(\cI)\cdot \mu^{b^*+60b}}{\cm}\cdot \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}\\
 &\leq O(\optcrors(\cI))
 ,\end{split}
 \]
 %
 since $\optcrors(\cI)\leq \cm^2/\mu^{c'}$, and $c'$ is a large enough constant.

Overall, we get that $\sum_{I'\in \iset'}\optcrors(I')=\sum_{I\in \iset_1}\optcrors(\hat I)+\sum_{I\in \iset_2'}\optcrors(\hat I)+\sum_{I\in \iset_2''}\optcrors(\hat I)+\sum_{I\in \iset_3}\optcrors(\hat I')\leq  \optcrors(I)\cdot (\log \cm)^{O(1)}$.
\end{proof}



\iffalse

The calculations

---------------------------------------------------



\begin{itemize}
	\item $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)$
	
	\item $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$
	
	\item in $\iset_2$: either $\cro(\psi(I))> |E(G)|/\mu^{2b}$, or  $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$.
	
	\item when pulling edges back, we will pay $\sum_{I\in \iset_2}\hm(I)\cdot |\chi^{\dirty}(\psi(I))|$.
	
	\item let's say that $\iset_2'$ contains all instances with $\cro(\psi(I))> |E(G)|/\mu^{2b}>\hat m(I)/\mu^{2b}$. But $\sum_{I\in \iset}\cro(\psi(I))\leq 2\optcrors(\cI)<\cm/\mu^{c'}$. So $\sum_{I\in \iset_2'}\hat m(I)\leq \mu^{2b}\cdot \cm/\mu^{c'}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so total increase in number of crossings is less than $\optcrors(\cI)$.
	
	\item Now $\iset_2''$ contains all instances with $|\chi^{\dirty}(\psi(I))|> |E(G)|/\mu^{2b}$. But $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$. So $\sum_{I\in \iset_2}\hat m(I)<\frac{\optcrors(\cI)\cdot \mu^{b^*+b}}{\cm}$. The increase is this multiplied by $\sum_{I\in \iset}|\chi^{\dirty}(\psi(I))|\leq  \frac{\optcrors(\cI)\cdot \mu^{b^*}}{\cm}$, so the total increase in number of crossings is at most $\frac{(\optcrors(\cI))^2\cdot \mu^{2b^*+b}}{(\cm)^2}$. Assuming that $\optcrors(\cI)<\cm^2/\mu^{c'}$ it's at most $\optcrors(\cI)$.
\end{itemize}





----------------------------------------------
\fi



In the remainder of this section we focus on the proof of \Cref{thm: phase 2}. Throughout the proof, we denote the instance $I=(G,\Sigma)$ that serves as the input to the algorithm by $\cI'=(\cG',\cSigma')$, with $|E(\cG')|$ denoted by $\cm'$. We denote the skeleton structure $\kset(I)$ by $\check \kset=(\jset_1,\ldots,\jset_r)$, where $r\leq \mu^{100}$. For all $1\leq i\leq r$, we denote $\jset_i=(J_i,\set{b_u}_{u\in V(J_i)},\rho_{J_i})$. 
We start with the intuition for the proof. We denote by $\check K=\bigcup_{i=1}^rJ_i$ the skeleton of $\cG'$ associated with the skeleton structure $\check \kset$. We can assume that there exists a solution $\check \psi$ to instance $\cI$ that is semi-clean with respect to $\check\kset$ (as otherwise we can let $E^{\del}(\cI')=E(\cG)\setminus E(\check K)$ \znote{what does this mean?} ). 

==> flower_disengagement.tex <==
\subsection{Phase 3: Handling Augmented Flower Clusters}

==> guiding-paths-backup.tex <==
\newpage
\section{Third Key Tool: Computing Guiding Paths}
\label{subsec: guiding paths}

We start with intuition. Consider an instance $I=(G,\Sigma)$ of the \cnwrs problem, and let $C\subseteq G$ be a subgraph of $G$ that we refer to as a cluster. Fix an optimal solution $\phi^*$ to instance $I$; we define $\cro(C)$ as usual with respect to $\phi^*$ -- the number of crossings in $\phi^*$ in which the edges of $C$ participate. For a set $\qset$ of paths in $G$, the cost $\cost(\qset)$ is also defined as before, with respect to $\phi^*$. 

Assume that the boundary of $C$ is $\alpha$-well-linked in $C$, and denote $|E(C)|/|\delta(C)|=\eta$. We show below a randomized algorithm that either computes a vertex $u\in V(C)$ and a set $\qset$ of paths routing $\delta(C)$ to $u$, whose expected cost is comparable to $\cro(C)$; or with high probability correctly establishes that $\cro(C)>|\delta(C)|^2/\poly(\eta)$.
We say that cluster $C$ is \emph{good} if the former outcome happens, and we say that it is \emph{bad} otherwise.

Intuitively, given our input instance $I=(G,\Sigma)$, we can compute a decomposition $\cset$ of $G$ into clusters, such that for each cluster $C\in \cset$, the boundary of $C$ is $1/\poly\log m$-well-linked in $C$, and moreover $|\delta(C)|\geq |E(C)|/\poly(\mu)$. In order to compute the decomposition, we start with $\cset$ containing a single cluster $G$, and the interate. In every iteration, we select a cluster $C\in \cset$, and then either compute a sparse balanced cut $(A,B)$ in $C$, or compute a cut $(A,B)$ that is sparse with respect to the edges of $\delta(C)$ (that is, $|E(A,B)|<\min\set{|\delta(C)\cap \delta(A)|,|\delta(C)\cap \delta(B)|}/\poly\log n$; or return FAIL. In the former two cases, we replace $C$ with $C[A]$ and $C[B]$ in $\cset$, while in the latter case we declare the cluster $C$ \emph{settled}; we will show that in this case the boundary of $C$ is $1/\poly\log n$-well-linked in $C$ and $|\delta(C)|\geq |E(C)|/\poly(\mu)$. The algorithm terminates once every cluster in $\cset$ is settled. We show that each of the resulting clusters $C\in \cset$ is sufficiently small (that is, $|E(C)|\leq m/\mu$), and the total number of edges connecting different clusters is also sufficiently small (at most $m/\mu$). If each resulting cluster is a good cluster, then we obtain the desired decomposition $\cset$, together with the desired collections $\set{\qset(C)}_{C\in \cset}$ of paths. Unfortunately, some of the clusters $C\in \cset$ may be bad. For each such cluster we are guaranteed with high probability that $\cro(C)>|\delta(C)|^2/\poly(\mu)$, but unfortunately the sum of values of $|\delta(C)|^2$ over all bad clusters $C$ may be quite small, significantly smaller than say $|E(G)|^2$, so we cannot conclude that $\opt(I)\geq |E(G)|^2/\poly(\mu)$. 

In order to overcome this difficulty, we partition the set $\cset$ of clusters into a set $\cset'$ of good clustes, and a set $\cset''$ of bad clusters. Let $G'=G\setminus (\bigcup_{C\in \cset'}C)$, and let $G''=G'_{|\cset''}$ be obtained from $G'$ by  contracting each bad cluster into a super-node. We then apply the same decomposition algorithm to graph $G''$. We continue this process until no bad clusters remain, so we have obtained a decomposition of $G$ into a collection of good clusters, or we compute a bad cluster $C$ with $|\delta(C)|\geq |E(G)|/\poly(\mu)$, so we can conclude that $\opt(I)\geq|E(G)|^2/\poly(\mu)$.

In order to be able to carry out this process, we need an algorithm that, given a cluster $C$, either computes the desired set $\qset$ of paths routing the edges of $\delta(C)$ to some vertex $u$ of $C$, such that the cost of $\qset$ is low; or establishes that $\cro(C)>|\delta(C)|^2/\poly(\mu)$. But because we will need to apply this algorithm to graphs obtained from sub-graphs of $G$ by contracting some bad clusters, we need a more general algorithm, that is summarized in the following theorem.



%We now describe a basic tool that will be used in the remainder of the decomposition. Suppose we are given a graph $H$, and a set $T$ of its vertices called terminals, where every terminal has degree $1$ in $H$. Let $\cset$ be a collection of disjoint subgraphs of $H$ called clusters, such that no terminal lies in a cluster of $\cset$. Assume further that for every cluster $C\in \cset$, the boundary of $C$.

%In this subsection, as before, we assume that we are given an instance $I=(G,\Sigma)$ of the \cnwrs problem. As before, we fix an optimal solution $\phi^*$ for this problem. The goal of this section is to prove the following theorem.



Suppose we are given a graph $H$ and a set $T$ of its vertices called terminals. Let $\Lambda(H,T)$ denote the set of all pairs $(\qset,x)$, where $x$ is a vertex of $H$, and $\qset$ is a collection of paths routing the vertices of $T$ to $x$ in $\qset$. A \emph{distribution} $\dset$ over pairs in $\Lambda(H,T)$ is an assignment, to every pair $(\qset,x)\in \Lambda(H,T)$, of a probability value $p(\qset,x)\geq 0$, such that $\sum_{(\qset,x)\in \Lambda(H,T)}p(\qset,x)=1$. The distribution $\dset$ is specified by listing all pairs $(\qset,x)\in \Lambda(H,T)$ of pairs with $p(\qset,x)>0$, together with the corresponding probability value $p(\qset,x)$.
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------

\begin{theorem}\label{thm: find guiding paths}
	There is a large enough constant $c_0$, and an efficient randomized algrorithm, that receives as input an instance $I=(H,\Sigma)$ of \cnwrs, where $|V(H)|=n$, a set $T\subseteq V(H)$ of $k$ vertices of $H$ called terminals, and a collection $\cset$ of disjoint subgraphs of $H$, such that for some parameters $\eta,\eta'\geq 1$ and $0\leq \alpha,\alpha'\leq 1$, the following conditions hold:
	
	\begin{itemize}
		\item $|T|\geq |E(H_{|\cset})|/\eta$; 
		\item every terminal $t\in T$ has degree $1$ in $H$;
		\item for all $C\in \cset$, $V(C)\cap T=\emptyset$;
		\item set $T$ of terminals is $\alpha$-well-linked in the contracted graph $H_{|\cset}$; 
		
		\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property; and
		\item for every cluster $C\in \cset$, if $\Sigma_C$ is the rotation system for $C$ that is consistent with $\Sigma$, then $\optcro(C,\Sigma_C)\geq \frac{|\delta(C)|^2}{\eta'}$.
	\end{itemize}
	
	The algorithm either returns FAIL, or computes a distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$, such that for all $e\in E(C)$, $\expect{(\cong(\qset,e))^2}\leq O(\log^8k/(\alpha\alpha')^2)$ \mynote{OK to make smaller}. Moreover, if $\optcrors(I)\geq 
	\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{28}k}$, then the probability that the algorithm returns FAIL is at most $1/2$. 
	\mynote{need to be careful with this. OK to put $\eta'+\poly\eta$ on the bottom, not OK to put $\eta'\eta$. This is because instance size in the recursion will decrease by factor $\eta$ only.}
\end{theorem}

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------



The remainder of this section is dedicated to the proof of \Cref{thm: find guiding paths}. 
%For convenience, we define a new instance $I'=(H,\Sigma')$ of the \cnwrs problem, as follows. We start from graph $G$, and subdivide every edge $e\in \delta_G(C)$ with a vertex $t(e)$. Denote the resulting graph by $G'$, and let $T=\set{t(e)\mid e\in \delta_G(C)}$. Note that the solution $\phi^*$ to instance $I$ naturally defines a solution  $\phi'$ to the instance defined by graph $G'$ and rotation system $\Sigma$ (the newly added vertices $t$ each have degree $2$ so the ordering $\oset_t$ of their incident edges can be defined arbitrarily.) For subgraphs $X\subseteq G'$, we define $\cro(X)$ with respect to this drawing $\phi'$.

%We then let $H$ be the sub-graph of the resulting graph induced by $C\cup T$, and we let $\Sigma'$ be the corresponding rotation system that is consistent with the original rotation system $\Sigma$ for $G$. Note that, if $u$ is any vertex of $V(H)\setminus T$, and $\qset=\set{Q(t)\mid t\in T}$ is a collection of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, then set $\qset$ naturally defines a set $\qset'$ of paths in graph $G'$, routing the edges of $\delta_{G'}(H)$ to $u$ inside $H$, and so we can define $\cost_H(\qset')$ as usual, with respect to the drawing $\phi'$ of $G'$. Set $\qset$ of paths also naturally defines a set $\qset''$ of paths in graph $G$, routing the edges of $\delta_G(C)$ to $u$ inside $C$, and moreover $\cost_C(\qset)$ in graph $G$ is bounded by $\cost_H(\qset')$ in graph $G'$.

%Therefore, from now on our goal is to compute a vertex $u\in V(H)\setminus T$, and a collection $\qset=\set{Q(t)\mid t\in T}$ of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, so that the cost $\expect{\cost_{H}(\qset)}\leq O(\optcrors(I')\cdot 2^{O((\log^{1/4} m))})$.

For conveninence, we denote the contracted graph $H_{|\cset}$ by $\hH$,  and we denote $|E(\hH)|=\hm$. From the statement of \Cref{thm: find guiding paths}, $k\geq \hm/\eta$. Observe that, from \Cref{clm: contracted_graph_well_linkedness}, the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$.


We start with some intuition. Assume first that graph $H$ contains a grid (or a grid minor) of size $(\Omega(k\alpha\alpha'/\poly\log n)\times (k\alpha \alpha'/\poly\log n))$, and a collection $\pset$ of paths connecting every terminal to a distinct vertex on the first row of the grid, such that the paths in $\pset$ cause a low edge-congestion. For this special case, the algorithm of \cite{Tasos-comm}  (see also Lemma D.10 in the full version of \cite{chuzhoy2011algorithm}) provides the distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$ with the required properties. Moreover, if $H$ is  a bounded-degree planar graph, with a set $T$ of terminals that is $(\alpha\alpha')$-well-linked, 
then there is an efficient algorithm to compute such a grid minor, together with the required collection $\pset$ of paths. If $H$ is planar but no longer bounded-degree, we can still compute a grid-like structure in it, and apply the same arguments as in \cite{Tasos-comm} in order to compute the desired distribution $\dset$. The difficulty in our case is that the graph $H$ may be far from being planar, and, even though, from the Excluded Grid theorem of Robertson and Seymour \mynote{add references to the original thm proof and our new proofs}, it must contain a large grid-like structure, without having a drawing of $H$ in the plane with a small number of crossing, we do not know how to compute such a structure.

The proof of the theorem consists of five steps. In the first step, we will  either establish that $\optcrors(I)$ is sufficiently large (so the algorithm can return FAIL), or compute a subgraph $\hH'\subseteq \hH$, and a partition $(X,Y)$ of $V(\hH')$, such that each of the clusters $\hH'[X],\hH'[Y]$ has the $\hat \alpha$-bandwidth property, for $\hat \alpha=\Omega(\alpha/\log^4n)$, together with a large collection of edge-disjoint paths routing the terminals to the edges of $E_{\hH'}(X,Y)$ in graph $\hH'$. Intuitively, we will view from this point onward the edges of $E_{\hH'}(X,Y)$ as a new set of terminals, that we denote by $\tilde T$ (more precisely, we subdivide each edge of $E_{\hH'}(X,Y)$ with a new vertex that becomes a new terminal). We show that it is sufficient to prove an analogue of \Cref{thm: find guiding paths} for this new set $\tT$ of terminals. The clusters $\hH'[X],\hH'[Y]$ of graph $\hH'$ naturally define a partition $(H_1,H_2)$ of the graph $H$ into two disjoint clusters. In the second step, we either establish that $\optcrors(I)$ is suffciently large 
(so the algorithm can return FAIL), or
compute some vertex $x$ of $H_1$, and a collection $\pset$ of paths in graph $H_1$, routing the terminals of $\tilde T$ to $x$, such that the paths in $\pset$ cause a relatively low edge-congestion.
We exploit this set $\pset$ of paths in order to define an ordering of the termianls in $\tilde T$, which is in turn exploited in the third step in order to compute a ``skeleton'' for the grid-like structure. We compute the grid-like structure itself in the fourth step. In the fifth and the final step, we generalize the arguments from \cite{Tasos-comm}  and  \cite{chuzhoy2011algorithm} in order to obtain the desired distribution $\dset$.


Before we proceed, we need to consider two simple special cases. In the first case,  $\sum_{C\in \cset}|\delta(C)|^2$ is large. In the second case, we can route a large subset of the terminals to a single vertex of $V(\hat H)\cap V(H)$ in the graph $\hat H$ via edge-disjont paths.

\paragraph{Special  Case 1: $\sum_{C\in \cset}|\delta(C)|^2$ is large.}
We consider the special case where $\sum_{C\in \cset}|\delta(C)|^2\geq \frac{(k\alpha^4\alpha')^2}{c_0\log^{50}n}$, where $c_0$ is the constant from the statement of \Cref{thm: find guiding paths}.
In this case, since we are guaranteed that, for every cluster $C\in \cset$, $\optcrors(C,\Sigma_C)\geq |\delta(C)|^2/\eta'$, we get that:


\[\optcrors(I)\geq \sum_{C\in \cset}\optcrors(C,\Sigma_C)\geq \sum_{C\in \cset}\frac{|\delta(C)|^2}{\eta'}\geq \frac{(k\alpha^4\alpha')^2}{c_0\eta'\log^{50}n}.\]

Therefore, if $\sum_{C\in \cset}|\delta(C)|^2\geq (k\alpha^4\alpha')^2/(c_0\log^{50}n)$, the algorithm returns FAIL and terminates. We assume from now on that:

\begin{equation}\label{eq: boundaries squared sum bound}
\sum_{C\in \cset}|\delta(C)|^2< \frac{(k\alpha^4\alpha')^2}{c_0\log^{50}n}
\end{equation}



\paragraph{Special Case 2: Routing of terminals to a single vertex.}
The second special case happens if there exists a collection $\pset_0$ of at least $\frac{k\alpha\alpha'}{1024\cCMG^2\log^4k}$ edge-disjoint paths in graph $H$ routing some subset $T_0\subseteq T$ of terminals to some vertex $x$ (here, $\cCMG$ is the constant from \Cref{claim: embed expander}).
 
Note that, if Special Case 1 did not happen, then $x$ may not be a supernode. Indeed, assume that $x=v_C$ for some cluster $C\in \cset$. Then:


\[(\delta_H(C))^2\geq \Omega\left(\frac{(k\alpha \alpha')^2}{\log^8k}\right )\geq \frac{(k\alpha^4\alpha')^2}{c_0\log^{28}n},\] 

assuming that $c_0$ is a large enough constant, a contradiction. Therefore, we can assume that $x$ is not a supernode.
Denote $z=|\pset_0|\geq \frac{k\alpha\alpha'}{1024\cCMG^2\log^4k}$.
We compute a single set $\qset$ of paths routing the set $T$ of terminals to $x$, with congestion $O(\log^4k/(\alpha \alpha')^2)$, as follows. We partition the set $T\setminus T_0$ of terminals into $q=\ceil{k/z}\leq O(\log^4k/(\alpha\alpha'))$ subsets, each of which contains at most $z$ vertices. 
Consider now some index $1\leq i\leq q$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\pset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\pset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\pset_i'$. By concatenating the paths in $\pset_i'$ with paths in $\pset_0$, we obtain a collection $\pset_i$ of paths in graph $H$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\alpha\alpha'))$. Let $\qset=\bigcup_{i=0}^q\pset_i$ be the resulting set of paths. Observe that set $\qset$ contains $k$ paths, routing the terminals in $T$ to the vertex $x$ in graph $H$, with $\cong_H(\qset)\leq O(q/(\alpha\alpha'))\leq O(\log^4k/(\alpha\alpha')^2)$. We return a distribution $\dset$ consisting of a single pair $(\qset,u)$, and terminate the algorithm. 

In the remainder of the algorithm, we assume that neither of the two special cases happened. We now describe each step of the algorithm in turn.




%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 1: Splitting the Contracted Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


In this step, we split the contracted graph $\hH$, using the algorithm  summarized in the following theorem.

\begin{theorem}\label{thm: splitting}
	There is an efficient randomized algorithm that with probability at most $1/\poly(n)$ returns FAIL, and, if it does not return FAIL, then it  computes a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that:
	
	\begin{itemize}
		\item each of the clusters $\hH'[X]$ and $\hH'[Y]$ has the $\halpha'$-bandwidth property, for $\halpha'=\Omega(\alpha/\log^4n)$; and
		
		\item there is a set $\rset$ of at least $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
	\end{itemize}

\end{theorem}


\begin{proof}
We start by applying the algorithm from \Cref{claim: embed expander} to graph $\hH$ and the set $T$ of terminals, to obtain a graph $W$ with $V(W)=T$ and maximum vertex degree $O(\log^2k)$, and an embedding $\hpset$ of $W$ into $\hH$ with congestion $O((\log^2k)/\alpha)$. Let $\hat\event$ be the bad event that $W$ is not a $1/4$-expander. Then $\prob{\hat \event}\leq 1/\poly(k)$.

Let $\hH'$ be the graph that is obtained from $\hH$ by deleting from it all edges and vertices except those that participate in the paths in $\hpset$. Equivalently, graph $\hH'$ is obtained from the union of all paths in $\hpset$. We need the following observation.

\begin{observation}\label{obs: expansion and degree}
	If event $\hat \event$ did not happen, then the set $T$ of vertices is $\halpha$-well-linked in $\hH'$, for $\halpha=\frac{\alpha}{4\cCMG\log^2k}$, and the maximum vertex degree in $\hH'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}$.
\end{observation}

\begin{proof}
	Assume that Event $\hat \event$ did not happen. We first prove that the set $T$ of terminals is $\halpha$-well-linked in $\hH$. Consider any paritition $(A,B)$ of vertices of $\hH'$, and denote $T_A=T\cap A$, $T_B=T\cap B$. Assume w.l.o.g. that $|T_A|\leq |T_B|$. Then it is sufficient to show that $|E_{\hH'}(A,B)|\geq \halpha\cdot |T_A|$.
	
	Consider the partition $(T_A,T_B)$ of the vertices of $W$, and denote $E'=E_{W}(T_A,T_B)$. Since $W$ is a $1/4$-expander, $|E'|\geq |T_A|/4$ must hold. Consider now the set $\hat \rset\subseteq \hpset$ of paths containing the embeddings $P(e)$ of every edge $e\in E'$. Each path $R\in \hat \rset$ connects a vertex of $T_A$ to a vertex of $T_B$, so it must contain an edge of $|E_{\hH}(A,B)|$. Since $|\hat\rset|\geq |T_A|/4$, and the paths in $\hpset$ cause edge-congestion at most $(\cCMG\log^2k)/\alpha$, we get that $|E_{\hH}(A,B)|\geq \alpha\cdot |T_A|/(4\cCMG\log^2k)\geq \halpha |T_A|$.
	
	Assume now that maximum vertex degree in $\hH'$ is greater than $d$, and let $x$ be a vertex whose degree is at least $d$. Let $\hat\qset\subseteq \tpset$ be the set of all paths containing the vertex $x$.
Consider any such path $Q\in \hat\qset$. The endpoints of this path are two distinct terminals $t,t'\in T$. We let $Q'\subseteq Q$ be the sub-path of $Q$ between the terminal $t$ and the vertex $x$, and we let $\qset'=\set{Q'\mid Q\in \hat\qset}$.

Recall that every vertex in $W$ has degree at most $\cCMG\log^2k$, and so a terminal in $T$ may be an endpoint of at most $\cCMG\log^2k$ paths in $\hpset$. Therefore, there is a subset $\qset''\subseteq \qset'$ of at least $d/(\cCMG\log^2k)$ paths, each of which originates at a distinct terminal.
But then, from \Cref{claim: routing in contracted graph}, there is a collection $\qset'''$ of edge-disjoint paths in graph $H$, routing a subset of terminals to $x$ of cardinality at least:

\[\frac{\alpha'|\qset''|} 2\geq \frac{\alpha' d}{2\cCMG\log^2k}\geq  \frac{\alpha \alpha' k}{1024\cCMG\log^4k},\]

 contradicting the fact that Special Case 2 did not happen.
\end{proof}



Next, we use the following lemma that allows us to compute the required sets $X$, $Y$ of vertices. The proof follows immediately from techniques that were introduced in \cite{chuzhoy2012routing} and then refined in \cite{chuzhoy2012polylogarithmic,chekuri2016polynomial,chuzhoy2016improved}. Unfortunately, all these proofs assumed that the input graph has a bounded vertex degree, and additionally the proofs are somewhat more involved than the proof that we need here (this is because these proofs could only afford a $\poly\log k$ loss in the cardinality of the path set $\rset$ relatively to $|T|$, while we can afford a $\poly\log n$ loss). Therefore, we provide a complete proof of the lemma in Section \ref{sec: splitting} of the Appendix for completeness.


\begin{lemma}\label{lem: splitting}
	There is an efficient algorithm that, given as input an $n$-vertex graph $G$, and a subset $T$ of $k$ vertices of $G$ called terminals, together with a parameter $0<\talpha<1$, such that the maximum vertex degree in $G$ is at most $\talpha k/64$, and every vertex of $T$ has degree $1$ in $G$, either returns FAIL, or computes a partition $(X,Y)$ of $V(G)$, such that:
	
	\begin{itemize}
		\item each of the clusters $G[X]$, $G[Y]$ has the $\talpha'$-bandwidth property, for $\talpha'=\Omega(\talpha/\log^2n)$; and
		\item there is a set $\rset$ of at least $\Omega(\talpha^3k/\log^2n)$ edge-disjoint paths in graph $G$, routing a subset of terminals to edges of $E_G(X,Y)$.
	\end{itemize}

Moreover, if the vertex set $T$ is $\talpha$-well-linked in $G$, then the algorithm never returns FAIL.
\end{lemma}

We apply the algorithm from \Cref{lem: splitting} to graph $\hH'$, the set $T$ of terminals, and parameter $\talpha=\halpha=\frac{\alpha}{4\cCMG\log^2k}$. Recall that we are guaranteed that maximum vertex degree in $\hat H'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}\leq \frac{\talpha k}{64}$.
Note that the algorithm from  \Cref{lem: splitting} may only return FAIL if the set $T$ of terminals is not $\halpha$-well-linked in $\hH'$, which, from \Cref{obs: expansion and degree}, may only happen if Event $\hat \event$ happened, which in turn may only happen with probability $1/\poly(k)$. If the algorithm from \Cref{lem: splitting} returned FAIL, then we restart the algorithm that we have described so far from scratch. We do so at most $1/\poly\log n$ times, and if, in every iteration, the algorithm from \Cref{lem: splitting} returns FAIL, then we return FAIL as the outcome of the algorithm for \Cref{thm: splitting}. Clearly, this may only happen with probability at most $1/\poly(n)$. Therefore, we assume that in one of the iterations, the algorithm from \Cref{lem: splitting} did not return FAIL. From now on we consider the outcome of that iteration.

 Let $(X,Y)$ be the partition of $V(\hH')$ that the algorithm returns. We are then guaranteed that each of the clusters $\hH'[X],\hH'[Y]$ has the $\talpha'$-bandwidth property, where $\talpha'=\Omega(\halpha/\log^2n)=\Omega(\alpha/\log^4n)$. The algorithm also ensures that there is a collection $\rset$ of edge-disjoint paths in $\hH'$, routing a subset of the terminals to edges of $E_{\hH'}(X,Y)$, with:

\[ |\rset|\geq \Omega(\talpha^3k/\log^2n)=\Omega(\alpha^3k/\log^8n). \]


This completes the proof of \Cref{thm: splitting}.
\end{proof}


If the algorithm from \Cref{thm: splitting} returned FAIL (which may only happen with probability at most $1/\poly(n)$), then we terminate the algorithm and return FAIL as well. Therefore, we assume from now on that the algorithm from \Cref{thm: splitting} returned a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that each of the clusters $\hH'[X]$ and $\hH'[Y]$ has the $\halpha'$-bandwidth property, for $\halpha'=\Omega(\alpha/\log^4n)$, and
 there is a set $\rset$ of at least $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
Notice that we can compute the path set $\rset$ with the above properties efficiently, using standard Maximum $s$-$t$ flow.
Let $E'\subseteq E_{\hH'}(X,Y)$ be the subset of edges containing the last edge on every path in $\rset$, so, by reversing the direction of the paths in $\rset$, we can view the set $\rset$ of paths as routing the edges of $E'$ to the terminals.
In the remainder of this step, we will slightly modify the graphs $H$ and $\hat H$, and we will continue working with the modified graphs in the following steps.

Let $\hH''\subseteq\hH'$ be the graph obtained from $\hH'$ by first deleting all edges of $E_{\hH'}(X,Y)\setminus E'$ from it, and then subdividing every edge $e\in E'$ with a vertex $t_e$. We denote $\tilde T=\set{t_e\mid e\in E'}$, and we refer to vertices of $\tilde T$ as \emph{pseudo-terminals}. Recall that $|\tilde T|=|\rset|=\Omega(\alpha^3k/\log^8n)$, and there is a set $\rset'$ of edge-disjoint paths in the resulting graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$.
We let $\hH_1$ be the subgraph of $\hH''$, that is induced by the set $X\cup \tilde T$ of vertices, and we similarly define $\hH_2=\hH''[Y\cup \tilde T]$. From the $\halpha'$-bandwidth property of the clusters $\hH'[X]$ and $\hH'[Y]$, we are guaranteed that the vertices of $\tilde T$ are $ \halpha'$-well-linked in both $\hH_1$ and in $\hH_2$, where $\halpha'= \Omega(\alpha/\log^4n)$. Let $\cset'\subseteq \cset$ be the subset of all clusters $C$ whose corresponding supernode $v_C$ lies in grpah $\hH''$.

For convenience, we also subdivide, in graph $H$, every edge $e\in E'$, with the vertex $t_e$, so graph $\hH''$ can be now viewed as a subgraph of the contracted graph $H_{|\cset}$.

Next, we let $H'\subseteq H$ be the subgraph of $H$ that corresponds to the graph $\hH''$: namely, graph $H'$ is obtained from $\hH''$ by replacing every supernode $v_C$ with the corresponding cluster $C\in \cset'$. Equivalently, we can obtain graph $H'$ from $H$, by deleting every edge of $E(\hH)\setminus E(\hH'')$ and every regular (non-supernode) vertex of $V(\hH)\setminus V(\hH'')$. Additionally, for every cluster $C\in \cset\setminus \cset'$, we delete all edges and vertices of $C$ from $H'$. We also define a rotation system $\Sigma'$ for graph $H'$, which is identical to $\Sigma$ (vertices $t_e\in \tilde T$ all have degree $2$, so their corresponding ordering $\oset_{t_e}$ of incident edges can be set arbitrarily). 


We partition the set $\cset'$ of clusters into two subsets: set $\cset_X$ contains all clusters $C\in \cset'$ with $v_C\in X$, and set $\cset_Y$ contains all clusters $C\in \cset'$ with $v_C\in Y$. We can similarly define the graphs $H_1,H_2\subseteq H'$, that correspond to the contracted graphs $\hat H_1$ and $\hat H_2$, respectively: let $X'$ contain all vertices $x\in V(H')$, such that either $x\in C$ for some cluster $C\in \cset_X$, or $x$ is a regular vertex of $\hat H''$ lying in $X$. Similarly, we let $Y'$ contain all vertices $y\in V(H)$, such that either $y\in C$ for some cluster $C\in \cset_Y$, or $y$ is a regular vertex of $\hat H''$ lying in $Y$. We then let $H_1=H'[X\cup \tilde T]$, and $H_2=H'[Y\cup \tilde T]$.

The following observation, summarizing some properties of graph $H'$, is immediate:

\begin{observation}\label{obs: properties of new graph}
	\ 
	
	\begin{itemize}
		\item $\optcrors(H',\Sigma')\leq \optcrors (H,\Sigma)$;
		\item $\hat H''=H'_{|\cset'}$; 
		\item $|E(\hat H'')|\leq 2|E(\hat H)|\leq 2\eta k\leq O(|\tilde T|\eta \log^8k/\alpha^3)$; and
		\item graph $\hat H_1$ is a contracted graph of $H_1$ with respect to  $\cset_X$, and graph $H_2$ is a contracted graph of $H_2$ with respect to $\cset_Y$. In other words, $\hat H_1=(H_1)_{|\cset_X}$, and $\hat H_2=(H_2)_{|\cset_Y}$.
	\end{itemize}
\end{observation}

(for third assertion we have used the fact that $k\geq |E(\hat H)|/\eta$ from the statement of \Cref{thm: find guiding paths}, and $|\tilde T|\geq \Omega(\alpha^3k/\log^8n)$.)


Recall that $\Lambda(H',\tilde T)$ denotes the set of all pairs $(\qset,x)$, where $x$ is a vertex of $H'$, and $\qset$ is a collection of paths in graph $H'$, routing the vertices of $\tilde T$ to $x$. In the following observation, we show that it is now enough to compute a distribution $\dset'$ over pairs $(\qset,x)\in \Lambda(H',\tilde T)$, such that for every edge $e\in E(H')$, $\expect{\cong_{H'}(\qset,e)}$ is low, in order to obtain the desired distribution $\dset$ over pairs in $\Lambda(H,T)$.


\begin{observation}\label{obs: convert distributions}
	There is an efficient algorithm, that, given a distribution $\dset'$ over pairs  $(\qset',x')\in \Lambda(H',\tilde T)$,
	such that for every edge $e'\in E(H')$, $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e'))^2}\leq \beta$ holds,
	 computes a distribution $\dset$ over pairs  $(\qset,x)\in \Lambda(H,T)$, such that for every edge $e\in E(H)$, $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\beta \log^{16}n}{\alpha^8(\alpha')^4}\right )$.
\end{observation}
\begin{proof}
	Recall that there is a set $\rset'$ of edge-disjoint paths in graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$, and moreover, such a path set can be found efficiently via a standard maximum $s$-$t$ flow computation.
	Since $\hat H''=H'_{|\cset'}$, from \Cref{claim: routing in contracted graph}, we can efficiently compute a set $\rset_0$ of edge-disjoint paths in graph $H''$, routing a subset $T_0\subseteq T$ of terminals to $\tT$, with $|\rset_0|\geq \alpha'\cdot |\rset'|=\alpha'\cdot |\tilde T|=\Omega(\alpha'\alpha^3k/\log^8n)$. 
	%Let 
	%$T_0\subseteq T$ the set of terminals that serve as endpoints of paths in $\pset_0$. 
	
	Let $z=\ceil{k/|T_0|}=O(\log^{8}n/(\alpha^3\alpha')$. Next, we partition the terminals of $T\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $|T_0|$ each. Consider now some index $1\leq i\leq z$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in graph $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\rset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\rset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\rset'_i$. By concatenating the paths in $\rset'_i$ with paths in $\rset_0$, we obtain a collection $\rset_i$ of paths in graph $H$, routing the terminals in $T_i$ to vertices of $\tilde T$, such that every vertex of $\tilde T\cup \rset_0$ is an endpoint of at most one path in $\rset_i$. Let $\rset^*=\bigcup_{i=0}^z\rset_i$ be the resulting set of paths. Observe that set $\rset^*$ contains $k$ paths, each of which connects a distinct terminal of $T$ to a vertex of $\tilde T$, and every vertex of $\tilde T$ serves as an endpoint of at most $z=O(\log^{8}n/(\alpha^3\alpha')$ such paths. The paths of $\rset^*$ cause congestion at most $O(z/\alpha\alpha')\leq O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$.
	
	
	Recall that $H'\subseteq H$. Consider some pair $(\qset',x')\in \Lambda(H',\tilde T)$ with probability $p(\qset',x')>0$ in the distribution $\dset'$. We compute another path set $\qset$ in graph $H$, routing all terminals in $T$ to $x'$, and we will assign to the pair $(\qset,x')\in \Lambda(H,T)$ the same probability value $p(\qset',x')$. For ever pseudoterminal $\tilde t\in \tilde T$, let $Q'_{\tilde t}\in \qset'$ be the unique path originating at $\tilde t$. For every terminal $t\in T$, let $R'_t\in \rset^*$ be the unique path originating at terminal $t$, and let $\tilde t\in \tilde T$ be the other endpoint of path $R'_t$. We let $Q_t$ be the path obtained by concatenating the paths $R'_t$ and $Q'_{\tilde t}$, so path $Q_t$ connects $t$ to vertex $x'$. We then let $\qset=\set{Q_t\mid t\in T}$. Note that $\qset$ is a set of paths in graph $H$ routing the set $T$ of terminals to vertex $x'$, so $(\qset,x')\in \Lambda(H,T)$. We assign to the pair $(\qset,x')$ probability $p(\qset',x')$. Note that, since every pseudoterminal $\tilde t\in \tilde T$ may seve as an endpoint of at most $O(\log^{8}n/(\alpha^3\alpha')$ paths in $\rset^*$, and since the paths in $\rset^*$ cause edge-congestion at most $O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$, for every edge $e\in E(H)$, we get that:
	
	\[\cong_H(\qset,e)\leq O\left(\frac{\cong_{H'}(\qset',e) \cdot \log^8k}{\alpha^3 \alpha'}+\frac{\log^8k}{\alpha^4(\alpha')^2}\right ).  \]

Therefore, altogether, for every edge $e\in E(H)$:

\[\expect[(\qset,x')\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\log^{16}k}{\alpha^8(\alpha')^4}\right )\cdot \left (\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}+1\right ).  \]	
\end{proof}

From the above discussion, in order to complete the proof of \Cref{thm: find guiding paths}, it is now enough to design a randomized algorithm, that either computes a distribution $\dset'$ over pairs in $\Lambda(H',\tilde T)$ with $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}\leq xxx$, or returns FAIL. It is enough to ensure that,   if $\optcrors(H',\Sigma')\geq 
\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{28}k}$, then the probability that the algorithm returns FAIL is at most $1/2$.

In the remainder of the proof we focus on the above goal. It would be convenient for us to simplify the notation, by denoting $H'$ by $H$, $\hat H''$ by $\hat H$, $\tilde T$ by $T$, and $\halpha'$ by $\tilde \alpha$. We also denote $\cset'$ by $\cset$. We now summarize all properties of the new graphs $H,\hat H$ that we have established so far, and in the remainder of the proof of \Cref{thm: find guiding paths} we will only work with these new graphs. 



\paragraph{Summary of the outcome of Step 1.}
We can assume from now on that we are given a graph $H$, a rotation system $\Sigma$ for $H$, a set $\tilde T$ of terminals in graph $H$, and a collection $\cset$ of disjoint subgraphs (clusters) of $H\setminus \tT$. We denote $|\tT|=\tk$. The corresponding contracted graph is denoted by $\hat H=H_{|\cset}$. 
We are also given a partition $(X,Y)$ of $V(H)\setminus \tilde T$ (note that for convenience of notation, $X$ and $Y$ are now subsets of vertices of $H$, and not of $\hat H$), and a parition $\cset_X,\cset_Y$ of $\cset$, such that each cluster $C\in \cset_X$ has $V(C)\subseteq X$, and each cluster $C\in \cset_Y$ has $V(C)\subseteq Y$. We denote $H_1=H[X\cup \tilde T]$ and $H_2=H[Y\cup \tilde T]$. We also denote by $\hat H_1=(H_1)_{|\cset_X}$ the contracted graph of $H_1$ with respect to $\cset_X$, and similarly by $\hat H_2=(H_2)_{|\cset_Y}$ the contracted graph of $H_2$ with respect to $\cset_Y$. We have the following additional properties:

\begin{properties}{P}
	\item $\tk\geq \Omega(\alpha^3k/\log^8n)$;
	\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property;
	\item $|E(\hat H)|\leq O(\tk\cdot \eta \log^8k/\alpha^3)$; \label{prop after step 1: few edges}
	\item every vertex of $\tilde T$ has degree $1$ in $H_1$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_1$, for $\talpha=\Omega(\alpha/\log^4n)$;
	\item similarly, every vertex of $\tilde T$ has degree $1$ in $H_2$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_2$; and
\item	$\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(k\alpha^4\alpha')^2}{c_0\log^{50}n}\leq   \frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}$, where $c_1$ is some large enough constant, whose value we can set later. \label{prop after step 1: small squares of boundaries}
\end{properties}

Our goal is
to design an efficient randomized algorithm, that either computes a distribution $\dset$ over pairs in $\Lambda(H,\tilde T)$ with $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq xxx$ for every edge $e\in E(H)$, or returns FAIL.


Assume that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}$ for some large enough constant $c_1$. Then, since we can set $c_0$ to be a sufficiently large constant compared to $c_1$, $\optcrors(H,\Sigma)>\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$ must hold. 
%Note that, if we let $c_1$ be a large enough constant compared to $c_0$, then $\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}>
%\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$.
Therefore, it is enough to ensure that, if  
%$\optcrors(H,\Sigma)< \frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$, 
$\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}$ for some large enough constant $c_1$,
then the probability that the algorithm returns FAIL is at most $1/2$.

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\iffalse
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: a Modified Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $\hH$, that we denote by $H^+$. In order to define the graph $\hH^+$, we start by defining a rotation system $\hat \Sigma $ for graph $\hH$, as follows. Let $x\in V(\hH)$ be a vertex. If $x$ is a supernode, that is, $x=v(C)$ for some cluster $C\in \cset$, then we define the circular ordering $\hat\oset_x\in \hat \Sigma$ of the edges of $\delta_{\hat H}(x)$ to be arbitrary.
Otherwise, $x$ is a regular vertex, and it is a vertex of the original graph $H$. We then let $\hat \oset_x\in \hat \Sigma$ be identical to the ordering $\oset_x\in \Sigma$, where $\Sigma$ is the original rotation system for graph $H$.

We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(\hat H)$ one-by-one. We denote by $d(u)$ the degree of the vertex $u$ in graph $\hat H$. We now describe an iteration when a vertex $u\in V(\hat H)$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that incident to $u$ in $\hH$, indexed according to their ordering in $\hat \oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(\hat H)$ is processed, we add a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(x,y)\in E(H)$. Assume that $e$ is the $i$th edge of $x$ and the $j$th edge of $y$, that is, $e=e_i(x)=e_j(y)$. Then we add an edge $e'=(s_i(x),s_j(y))$ to graph $H^+$, and we view this edge as the copy of the edge $e\in E(\hat H)$. We will not distinguish between the edge $e$ of $\hat H$ (and the corresponding edge of $H$), and the edge $e'$ of $H^+$.

We note that every terminal $t\in T$ has degree $1$ in $\hat H$, so its corresponding grid $\Pi(t)$ consists of a single vertex, that we also denote by $t$. Therefore, set $T$ of terminals in $H$ naturally corresponds to a set of $k$ terminals in $H^+$, that we denote by $T$ as before.

This completes the definition of the graph $H^+$. Note that the maximum vertex degree in $H^+$ is $4$. We also define a rotation system $\Sigma^+$ for the graph $H^+$ in a natural way: for every vertex $u\in V(H)$, 
consider the standard drawing of the grid $\Pi(u)$, to which we add the drawings of the edges that are incident to vertices $s_1(u),\ldots,s_{d(u)}(u)$, so that the edges are drawn on the grid's exterior in a natural way (\mynote{add figure}). This layout defines an ordering $\oset^+(v)$ of the edges incident to every vertex $v\in \Gamma(u)$.

We start with the following simple claim.

\begin{claim}\label{claim: cheap solution to modified instance} There is a solution to the \CNwRS problem instance $(H^+,\Sigma^+)$ of cost at most ..., such that no inner edge of $H^+$ participates in any crossings in the solution.
\end{claim}

\begin{proof}
	We start by showing that $\optcrors(\hH,\hat \Sigma)\leq ...$. Recall that, from \Cref{lem: crossings in contr graph}, there is a drawing $\hat \phi$ of graph $\hH$ with at most $O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2$ crossings, such that for every vertex $x\in V(\hH)\cap V(H)$, the ordering of the edges of $\delta_{\hH}(x)$ as they enter $x$ in $\hat \phi$ is consistent with the ordering $\oset_x\in \Sigma$, and hence with the ordering $\hat \oset_x\in \hat \Sigma$. Drawing $\hat \phi$ of $\hat H$ may not be a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS since for some supernodes $v(C)$, the ordering of the edges that are incident to $v(C)$ in $\hat H$ as they enter the image of $v(C)$ in $\hat \phi$ may be different from $\hat \oset_{v(C)}$. For each such vertex $v(C)$, we may need to \emph{reorder} the images of the edges of $\delta_{\hH}(v(C))=\delta_H(C)$ near the image of $v(C)$, so that they enter the image of $v(C)$ in the correct order. This can be done by introducing at most $|\delta_H(C)|^2$ crossings for each such supernode $v(C)$. The resulting drawing $\hat \phi'$ of $\hat \phi$ is a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS, whose cost is bounded by:
	
	
	\[O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+\sum_{C\in \cset}|\delta_H(C)|^2\leq O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+  \]
	
	
\end{proof}
\fi
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: Routing the Terminals to a Single Vertex, and an Expanded Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

In this step we start by considering the graph $H_1$ and the set $\tT$ of terminals in it. Our goal is to compute a collection $\jset$ of paths in graph $H_1$, routing all terminals of $\tT$ to a single vertex, such that the paths in $\jset$ cause a relatively low congestion in graph $H_1$. We show that, if such a collection of paths does not exist, then $\optcrors(H,\Sigma)$ is high. Intuitively, we will use the set $\jset$ of paths in order to define an ordering of the terminals in $\tT$, which will in turn be used in order to compute a grid-like structure in graph $H_2$. Once we compute the desired set $\jset$ of paths, we will replace the graph $H$ with its low-degree analogue $H^+$, that we refer to as the \emph{expanded graph}. The remaining steps in the proof of \Cref{thm: find guiding paths} will use this expanded graph only.


% Recall that the terminals of $\tT$ are $\talpha$-well-linked in $\hat H_1$, and the degree of each terminal in $\hat H_1$ is $1$. 
 
We now proceed to describe the algorithm for Step 2. We consider every vertex $x\in V(H_1)$ one-by-one. For each such vertex $x$, we compute a set $\jset(x)$ of paths in graph $H_1$, with the following properties:

\begin{itemize}
	\item every path in $\jset(x)$ originates at a distinct vertex of $\tT$ and terminates at $x$;
	\item the paths in $\jset(x)$ are edge-disjoint; and
	\item $\jset(x)$ is a maximum-cardinality set of paths in $H_1$ with the above two properties.
\end{itemize}

Note that such a set $\jset(x)$ of paths can be computed via a standard maximum $s$-$t$ flow computation.
Throughout, we use a parameter $\tk'=\tk\alpha'\alpha^5/(c_2\eta\log^{36}n)$, where $c_2$ is a large enough constant whose value we set later. 

If, for every vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then we reurn FAIL and terminate the algorithm.  In the following lemma, whose proof is deferred to Section \ref{sec: few paths high opt} of Appendix we show that, in this case, $\optcrors(H,\Sigma)\geq 
 \Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$ must hold.
Note that, since we can set $c_1$ to be a large enough constant, we can ensure that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}$ holds in this case.

\begin{lemma}\label{lem: high opt or lots of paths}
If,  for every vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then $\optcrors(H,\Sigma)\geq 
\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$.
\end{lemma}


From now on we assume that there is some vertex $x\in V(H_1)$, for which $|\jset(x)|\geq \tk'$. We denote $\jset_0=\jset(x)$, and we let $T_0\subseteq \tT$ be the set of terminals that serve as endpoints of paths in $\jset_0$, so $|T_0|=|\jset_0|=\tk'$.



Let $z=\ceil{\tk/\tk'}=O\left(\frac{\eta\log^{36}n}{\alpha^5\alpha'}\right )$. Next, we arbitrarily partition the terminals of $\tT\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $\tk'$ each. Consider now some index $1\leq i\leq z$. Since the set $\tT$ of terminals is $(\talpha\alpha')$-well-linked in $H_1$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\jset_i'$ of paths in graph $H_1$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $T_i$ cause edge-congestion $O(1/(\talpha\alpha'))$, and each vertex of $T_i$ is the endpoint of at most one path in $\jset_i'$. By concatenating the paths in $\jset_i'$ with paths in $\jset_0$, we obtain a collection $\jset_i$ of paths in graph $H_1$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\talpha\alpha'))$. Let $\jset=\bigcup_{i=0}^z\jset_i$ be the resulting set of paths. Observe that set $\jset$ contains $\tk$ paths, routing the terminals in $\tT$ to the vertex $x$ in graph $H_1$, with $\cong_H(\jset)\leq O\left(\frac z{\talpha\alpha'}\right )\leq O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$. We denote by $\rho=O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$ this bound on $\cong_{H_1}(\pset')$. We assume w.l.o.g. that the paths in $\jset$ are simple. Since every terminal in $\tT$ has degree $1$ in $H_1$, no path in $\jset$ may contain a terminal in $\tT$ as its inner vertex.



In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $H$, that we call \emph{expanded graph}, and denote by $H^+$. 

For every edge $e\in E(H)$, let $N_e=\cong_H(\jset,e)$. Recall that for every edge $e\in E(H_1\setminus\tT)$, $N_e\leq \rho$, and for every other edge $e$ of $H$, $N_e\leq 1$.

Let $H'$ be obtained from graph $H$ by adding, for every edge $e\in E(H)$ with $N_e>1$, $N_e$ parallel copies of the edge $e$. We extend the rotation system $\Sigma$ for graph $H$ to a rotation system $\Sigma'$ for the resulting graph $H'$ in a natural way: consider any vertex $v\in V(H)$, and let $\delta_H(v)=\set{e_1,\ldots,e_r}$, where the edges are indexed in the order consistent with the ordering $\oset_v\in \Sigma$. For all $1\leq i\leq r$, let $E_i\subseteq E(H')$ be the set of parallel edges corresponding to edge $e_i$. We define an ordering $\oset'_v$ of edges in $\delta_{H'}(v)$, where for all $1\leq i\leq r$, the edges of $E_i$ appear consecutively in an arbitrary order, and the edges belonging to different sets are ordered according to the natural ordering $E_1,E_2,\ldots,E_r$ of their correspondng subsets. Consider now the resulting instance $(H',\Sigma')$ of \CNwRS. We obtain the following immediate observation:

\begin{observation}\label{obs: crossing number of modified graph}
$\optcrors(H',\Sigma')\leq O(\rho^2)\cdot\left(\optcrors(H,\Sigma)+|E(H)|\right )$.
\end{observation}
\begin{proof}
	Let $\phi$ be the optimal solution to instance $(H,\Sigma)$ of \CNwRS. We modify $\phi$ to obtain a feasible solution to instance $(H',\Sigma')$, as follows. First, for every edge $e\in E(H)$ with $N_e>1$, we create $N_e$ additional parallel copies of the edge $e$, that are drawn next to the image of edge $e$, in parallel to it. Notice that, if edges $e$ and $e'$ cross in drawing $\phi$, then each such crossing may give rise to at most $\rho^2$ crossings in this new drawing, as $N_e,N_{e'}\leq \rho^2$. The resulting drawing is not necessarily a feasible solution to instance $(H',\Sigma')$, since it may not respect the rotation system $\Sigma'$. But it is easy to transform it into a feasible solution to instance $(H',\Sigma')$ by introducing at most $\sum_{e\in E(H)}2|N_e|^2$ new crossings (this is since for every vertex $v\in V(H)$, if $\delta_H(v)=\set{e_1,\ldots,e_r}$, we may need to reorder the edges in each of the corresponding sets $E_1,\ldots,E_r$ as they enter $e$; this can be done by introducing at most $\sum_{i=1}^r|E_i|^2=\sum_{i=1}^rN_{e_i}^2$ new crossings).
	Altogether, we obtain a feasible solution to instance $(H',\Sigma')$ of \CNwRS with at most $O(\rho^2)\cdot\left(\optcrors(H,\Sigma)+|E(H)|\right )$ crossings.
\end{proof}

In order to define the graph $H^+$, we start by defining a rotation system $\hat \Sigma $ for graph $\hH$, as follows. Let $x\in V(\hH)$ be a vertex. If $x$ is a supernode, that is, $x=v(C)$ for some cluster $C\in \cset$, then we define the circular ordering $\hat\oset_x\in \hat \Sigma$ of the edges of $\delta_{\hat H}(x)$ to be arbitrary.
Otherwise, $x$ is a regular vertex, and it is a vertex of the original graph $H$. We then let $\hat \oset_x\in \hat \Sigma$ be identical to the ordering $\oset_x\in \Sigma$, where $\Sigma$ is the original rotation system for graph $H$.

Note that, if if   
$\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}$, then:

\[\begin{split}
\optcrors(H',\Sigma')&<\rho^2\left(\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}+|E(H)|\right )\\
&\leq 
\end{split}
\]

since
$\rho=O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$, and 
$|E(\hat H)|\leq O(\tk\cdot \eta \log^8k/\alpha^3)$ (from Property \ref{prop after step 1: few edges}).




We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(\hat H)$ one-by-one. We denote by $d(u)$ the degree of the vertex $u$ in graph $\hat H$. We now describe an iteration when a vertex $u\in V(\hat H)$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that incident to $u$ in $\hH$, indexed according to their ordering in $\hat \oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(\hat H)$ is processed, we add a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(x,y)\in E(H)$. Assume that $e$ is the $i$th edge of $x$ and the $j$th edge of $y$, that is, $e=e_i(x)=e_j(y)$. Then we add an edge $e'=(s_i(x),s_j(y))$ to graph $H^+$, and we view this edge as the copy of the edge $e\in E(\hat H)$. We will not distinguish between the edge $e$ of $\hat H$ (and the corresponding edge of $H$), and the edge $e'$ of $H^+$.

We note that every terminal $t\in T$ has degree $1$ in $\hat H$, so its corresponding grid $\Pi(t)$ consists of a single vertex, that we also denote by $t$. Therefore, set $T$ of terminals in $H$ naturally corresponds to a set of $k$ terminals in $H^+$, that we denote by $T$ as before.

This completes the definition of the graph $H^+$. Note that the maximum vertex degree in $H^+$ is $4$. We also define a rotation system $\Sigma^+$ for the graph $H^+$ in a natural way: for every vertex $u\in V(H)$, 
consider the standard drawing of the grid $\Pi(u)$, to which we add the drawings of the edges that are incident to vertices $s_1(u),\ldots,s_{d(u)}(u)$, so that the edges are drawn on the grid's exterior in a natural way (\mynote{add figure}). This layout defines an ordering $\oset^+(v)$ of the edges incident to every vertex $v\in \Gamma(u)$.

We start with the following simple claim.

\begin{claim}\label{claim: cheap solution to modified instance} There is a solution to the \CNwRS problem instance $(H^+,\Sigma^+)$ of cost at most ..., such that no inner edge of $H^+$ participates in any crossings in the solution.
\end{claim}

\begin{proof}
	We start by showing that $\optcrors(\hH,\hat \Sigma)\leq ...$. Recall that, from \Cref{lem: crossings in contr graph}, there is a drawing $\hat \phi$ of graph $\hH$ with at most $O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2$ crossings, such that for every vertex $x\in V(\hH)\cap V(H)$, the ordering of the edges of $\delta_{\hH}(x)$ as they enter $x$ in $\hat \phi$ is consistent with the ordering $\oset_x\in \Sigma$, and hence with the ordering $\hat \oset_x\in \hat \Sigma$. Drawing $\hat \phi$ of $\hat H$ may not be a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS since for some supernodes $v(C)$, the ordering of the edges that are incident to $v(C)$ in $\hat H$ as they enter the image of $v(C)$ in $\hat \phi$ may be different from $\hat \oset_{v(C)}$. For each such vertex $v(C)$, we may need to \emph{reorder} the images of the edges of $\delta_{\hH}(v(C))=\delta_H(C)$ near the image of $v(C)$, so that they enter the image of $v(C)$ in the correct order. This can be done by introducing at most $|\delta_H(C)|^2$ crossings for each such supernode $v(C)$. The resulting drawing $\hat \phi'$ of $\hat \phi$ is a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS, whose cost is bounded by:
	
	
	\[O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+\sum_{C\in \cset}|\delta_H(C)|^2\leq O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+  \]
	
	
\end{proof}





\paragraph{Summary of Step 2.}

If Step 2 did not return FAIL, then it has computed a set $\pset=\set{P_t\mid t\in \tT}$ of simple paths in graph $H_1$, routing the vertices of $\tT$ to some vertex $x$, with congestion at most $\rho=O\left(\frac{\eta\log^{30}n}{\alpha^6(\alpha')^2}\right )$, so that the paths in $\pset$ are locally non-interfering with respect to the rotation system $\Sigma$ for graph $H$.
We used this set $\pset$ of paths in a natural way in order to define a circular ordering $\oset^*$ of the terminals in $\tT$. The ordering is consistent with the order $\oset_x\in \Sigma$ of the edges incident to $x$, which can be viewed as defining an ordering of the paths in $\pset$, as the last edge on each such path is incident to $x$.





\subsection{Step 3: Constructing a Grid Skeleton}






\mynote{do this for $H$, not $\hH$, but for clusters, external edges are those entering cluster, the rest is internal.}
In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $\hH$, that we denote by $H^+$. In order to define the graph $\hH^+$, we start by defining a rotation system $\hat \Sigma $ for graph $\hH$, as follows. Let $x\in V(\hH)$ be a vertex. If $x$ is a supernode, that is, $x=v(C)$ for some cluster $C\in \cset$, then we define the circular ordering $\hat\oset_x\in \hat \Sigma$ of the edges of $\delta_{\hat H}(x)$ to be arbitrary.
Otherwise, $x$ is a regular vertex, and it is a vertex of the original graph $H$. We then let $\hat \oset_x\in \hat \Sigma$ be identical to the ordering $\oset_x\in \Sigma$, where $\Sigma$ is the original rotation system for graph $H$.

We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(\hat H)$ one-by-one. We denote by $d(u)$ the degree of the vertex $u$ in graph $\hat H$. We now describe an iteration when a vertex $u\in V(\hat H)$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that incident to $u$ in $\hH$, indexed according to their ordering in $\hat \oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(\hat H)$ is processed, we add a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(x,y)\in E(H)$. Assume that $e$ is the $i$th edge of $x$ and the $j$th edge of $y$, that is, $e=e_i(x)=e_j(y)$. Then we add an edge $e'=(s_i(x),s_j(y))$ to graph $H^+$, and we view this edge as the copy of the edge $e\in E(\hat H)$. We will not distinguish between the edge $e$ of $\hat H$ (and the corresponding edge of $H$), and the edge $e'$ of $H^+$.

We note that every terminal $t\in T$ has degree $1$ in $\hat H$, so its corresponding grid $\Pi(t)$ consists of a single vertex, that we also denote by $t$. Therefore, set $T$ of terminals in $H$ naturally corresponds to a set of $k$ terminals in $H^+$, that we denote by $T$ as before.

This completes the definition of the graph $H^+$. Note that the maximum vertex degree in $H^+$ is $4$. We also define a rotation system $\Sigma^+$ for the graph $H^+$ in a natural way: for every vertex $u\in V(H)$, 
consider the standard drawing of the grid $\Pi(u)$, to which we add the drawings of the edges that are incident to vertices $s_1(u),\ldots,s_{d(u)}(u)$, so that the edges are drawn on the grid's exterior in a natural way (\mynote{add figure}). This layout defines an ordering $\oset^+(v)$ of the edges incident to every vertex $v\in \Gamma(u)$.



We can uset the $\pset$ of paths in graph $H$ in order to define a set $\pset'$ of paths in graph $H^+$, routing all terminals to vertices of $\Pi(x)$, with edge-congestion $\rho$, such that the paths in $\pset'$ are locally non-interfering.
\mynote{explain?}




We now consider two cases. The first case happens, if there is some vertex $x\in V(H)$, with $|\rset(x)|\geq \tk'$, then we fix this vertex $x$, denote $\pset_0=\rset(x)$, and we denote by $T_0\subseteq \tT$ the set of terminals that serve as endpoints of paths in $\pset_0$. 

We assume w.l.o.g. that the paths in $\pset'$ are simple. Note that, since every terminal in $\tT$ has degree $1$ in $H_1$, a vertex of $\tT\cup \set{x}$ cannot serve as an inner vertex on any path in $\pset'$. We then use the algorithm from \Cref{lem: non_interfering_paths} in order to obtain another set $\pset$ of simple paths routing the vertices of $\tT$ to $x$ in graph $H_1$ with congestion at most $\rho$, so that the paths in $\pset$ are locally non-interfering with respect to the input rotation system $\Sigma$.

We exploit the paths in $\pset$ in order to define a circular ordering $\oset^*$ of the terminals in $\tT$, as follows. 
Recall that we are given, as part of the definition of the instance $I=(H,\Sigma)$ of the \cnwrs problem, a circular ordering $\oset_x$ of the edges of $\delta_H(x)$. We use this ordering $\oset_x$, in order to define an ordering $\oset^*$ of the terminals in $\tT$, in a natural way. Let $\delta_{H_1}(x)=\set{e_1,\ldots,e_{\lambda}}$, where the edges are indexed according to the ordering $\oset_x$. For all $1\leq j\leq \lambda$, let $\hat T_j\subseteq \tT$ be the set of all terminals $t$, such that the last edge on path $P_t\in \pset$ is $e_j$, where $P_t$ is the unique path in $\pset$ that originates from $t$. We order the terminals in $\tT$ so that terminals belonging to different subsets $\hat T_j$ appear in the natural order $\hat T_1,\hat T_2,\ldots,\hat T_{\lambda}$ of these subsets, while the ordering between the terminals lying in the same set $\hat T_j$ is chosen arbitrarily.

Intuitively, if $\optcrors(I)$ is significantly smaller than $(\tk/\rho)^2$, then there are not that many crossings between images of different paths in $\pset$. We will exploit this fact in order to construct a grid-like structure in the graph $H_2$, by exploiting the ordering $\oset^*$ of the terminals that we have just defined in the following steps.

Let $\rset$ be any collection of paths in this new graph $H^+$. We say that $\rset$ is a \emph{legal routing} iff $|\rset|=k$, and there is some vertex $u\in V(H)$, such that the paths in $\rset$ route the set $T$ of terminals to vertices of $\Gamma(u)$. Note that a legal routing $\rset$ naturally defines a collection $\rset'$ of paths in graph $H$ routing the set $T$ of terminals to vertex $u$, such that for every edge $e\in E(H)$, $\cong_{H}(\rset,e)\leq \cong_{H^+}(\rset,e)$; the set $\rset'$ of paths is obtained from the paths in $\rset$ by contracting all outer edges.

Assume now that we compute a distribution $\dset'$ over legal routings $\rset$, such that, for every outer edge $e\in E(H^+)$, $\expect{\cong_{H^+}(\rset,e)}\leq x$. Then we immediately obtain a distribution $\dset$ over @@@



\subsection{Plan for the rest of the proof}
\begin{itemize}
	\item select 1 path in $z$, where for example $z=\eta$, though can also use $\eta^2$. Will get a grid skeleton of size $z\times z$. 
	
	\item before that, throw away all paths that have more than $\eta/\alpha$ outer edges on them. Most paths will stay.
	
	\item now if we look at a vertical path, it has few outer edges, so for most cells it goes through it does not use an outer edge. Which means that all horizontal paths going through that cell meet in a single vertex (or go through a single cluster). Call such a cell good.
	
	\item at least half the cells are good. In a type-1 good cell all horizontal paths go through a single regular vertex. In a type-2 good cell they all go through 1 cluster. The hope is that there are few type-2 good cells.
	
	\item why: we have about $z^2$ good cells. Inside all good cells there are about $k^2/z^2$ inner edges (can make a cell good if both all horizontal paths meet at some vertex, and all vertical paths meet at some vertex, and then it should be the same vertex). The hope is that the clusters can only contribute $\sum_C|\delta(C)|^2$ vertices to the grid. This is because, if we look at a cluster $C$, the total number of vertical/horizontal paths entering $C$ is at most $\delta(C)$. Even if all pairs have their intersections inside this cluster, it can't contribute more than $|\delta(C)|^2$ such intersecting pairs. 
\end{itemize}








\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Leftovers%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
contracted graph $\hat H=H_{|\cset}$. Let $U=\set{v(C)\mid C\in \cset}$ be the set of super-node vertices of $\hH$, and let $U'$ be the set of all remaining vertices. We define a rotation system $\hat \Sigma$ for graph $\hat H$  as follows: for a super-node $v(C)\in U$, we let $\oset_{v(C)}$ be an arbitrary ordering of the edges incident to $v(C)$, and for a regular vertex $u\in U'$, we let $\oset_u$ be identical to the ordering in the rotation system $\Sigma$ in instance $I$. Recall that, from \Cref{lem: crossings in contr graph},  there is a drawing $\phi$ of $\hH$,  containing at most $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)$ crossings, such that for every regular vertex $u\in U'$, the ordering of the edges of $\delta_{\hH}(u)$ as they enter $u$ in $\phi$ is consistent with $\oset_u\in \Sigma$. We can use this drawing in order to define a solution $\phi'$ to instance $\hat I=(\hH,\hat \Sigma)$ of the \cnwrs problem, by reordering the edges entering every super-node $v(C)$ as needed. This can be done so that $\cro(\phi')\leq \cro(\phi)+\sum_{C\in \cset'}|\delta_H(C)|^2\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$. Therefore, $\optcrors(\hat I)\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$.


We are now ready to define graph $\hH^+$. In order to do so, we start with graph $\hH$, and process every vertex $u\in V(\hH)\setminus T$ (that may be a regular vertex or a super-node one-by-one). Consider any such vertex $u$, and let $e_1,\ldots,e_{d(u)}$ be the edges incident to $u$ in $\hH$, indexed according to their ordering in $\oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ vrid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. We replace vertex $u$ with the grid $\Pi(u)$, and, for all $1\leq i\leq d(u)$, if $e_i=(u',u)$, then we replace $e_i$ with a new edge $e'_i=(u',s_i(u))$. Once every vertex of $V(\hH)\setminus T$ is processed, we obtain the final graph $\hH^+$. For every vertex $u$, we clall the edges of the grid $\Pi(u)$ \emph{inner edges}. We call all edges of $E(\hH^+)$ that are not inner edges \emph{outer edges}. Notice that there is a $1$-to-$1$ correspondence between the outer edges and the edges of graph $\hat H$. The following observation is immediate.

\begin{observation}\label{obs: expanded contracted graph}
	The set $T$ of terminals is $(\alpha\alpha')$-well-linked in $\hH^+$, and there is a drawing $\phi''$ of graph $\hH^+$ with at most  $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$ crossings, such that the inner edges do not participate in any crossings in $\phi''$.
\end{observation}
\fi
 








==> guiding-paths-backup2.tex <==
\newpage
\section{Third Key Tool: Computing Guiding Paths}
\label{subsec: guiding paths}

We start with intuition. Consider an instance $I=(G,\Sigma)$ of the \cnwrs problem, and let $C\subseteq G$ be a subgraph of $G$ that we refer to as a cluster. Fix an optimal solution $\phi^*$ to instance $I$; we define $\cro(C)$ as usual with respect to $\phi^*$ -- the number of crossings in $\phi^*$ in which the edges of $C$ participate. For a set $\qset$ of paths in $G$, the cost $\cost(\qset)$ is also defined as before, with respect to $\phi^*$. 

Assume that the boundary of $C$ is $\alpha$-well-linked in $C$, and denote $|E(C)|/|\delta(C)|=\eta$. We show below a randomized algorithm that either computes a vertex $u\in V(C)$ and a set $\qset$ of paths routing $\delta(C)$ to $u$, whose expected cost is comparable to $\cro(C)$; or with high probability correctly establishes that $\cro(C)>|\delta(C)|^2/\poly(\eta)$.
We say that cluster $C$ is \emph{good} if the former outcome happens, and we say that it is \emph{bad} otherwise.

Intuitively, given our input instance $I=(G,\Sigma)$, we can compute a decomposition $\cset$ of $G$ into clusters, such that for each cluster $C\in \cset$, the boundary of $C$ is $1/\poly\log m$-well-linked in $C$, and moreover $|\delta(C)|\geq |E(C)|/\poly(\mu)$. In order to compute the decomposition, we start with $\cset$ containing a single cluster $G$, and the interate. In every iteration, we select a cluster $C\in \cset$, and then either compute a sparse balanced cut $(A,B)$ in $C$, or compute a cut $(A,B)$ that is sparse with respect to the edges of $\delta(C)$ (that is, $|E(A,B)|<\min\set{|\delta(C)\cap \delta(A)|,|\delta(C)\cap \delta(B)|}/\poly\log n$; or return FAIL. In the former two cases, we replace $C$ with $C[A]$ and $C[B]$ in $\cset$, while in the latter case we declare the cluster $C$ \emph{settled}; we will show that in this case the boundary of $C$ is $1/\poly\log n$-well-linked in $C$ and $|\delta(C)|\geq |E(C)|/\poly(\mu)$. The algorithm terminates once every cluster in $\cset$ is settled. We show that each of the resulting clusters $C\in \cset$ is sufficiently small (that is, $|E(C)|\leq m/\mu$), and the total number of edges connecting different clusters is also sufficiently small (at most $m/\mu$). If each resulting cluster is a good cluster, then we obtain the desired decomposition $\cset$, together with the desired collections $\set{\qset(C)}_{C\in \cset}$ of paths. Unfortunately, some of the clusters $C\in \cset$ may be bad. For each such cluster we are guaranteed with high probability that $\cro(C)>|\delta(C)|^2/\poly(\mu)$, but unfortunately the sum of values of $|\delta(C)|^2$ over all bad clusters $C$ may be quite small, significantly smaller than say $|E(G)|^2$, so we cannot conclude that $\opt(I)\geq |E(G)|^2/\poly(\mu)$. 

In order to overcome this difficulty, we partition the set $\cset$ of clusters into a set $\cset'$ of good clustes, and a set $\cset''$ of bad clusters. Let $G'=G\setminus (\bigcup_{C\in \cset'}C)$, and let $G''=G'_{|\cset''}$ be obtained from $G'$ by  contracting each bad cluster into a super-node. We then apply the same decomposition algorithm to graph $G''$. We continue this process until no bad clusters remain, so we have obtained a decomposition of $G$ into a collection of good clusters, or we compute a bad cluster $C$ with $|\delta(C)|\geq |E(G)|/\poly(\mu)$, so we can conclude that $\opt(I)\geq|E(G)|^2/\poly(\mu)$.

In order to be able to carry out this process, we need an algorithm that, given a cluster $C$, either computes the desired set $\qset$ of paths routing the edges of $\delta(C)$ to some vertex $u$ of $C$, such that the cost of $\qset$ is low; or establishes that $\cro(C)>|\delta(C)|^2/\poly(\mu)$. But because we will need to apply this algorithm to graphs obtained from sub-graphs of $G$ by contracting some bad clusters, we need a more general algorithm, that is summarized in the following theorem.



%We now describe a basic tool that will be used in the remainder of the decomposition. Suppose we are given a graph $H$, and a set $T$ of its vertices called terminals, where every terminal has degree $1$ in $H$. Let $\cset$ be a collection of disjoint subgraphs of $H$ called clusters, such that no terminal lies in a cluster of $\cset$. Assume further that for every cluster $C\in \cset$, the boundary of $C$.

%In this subsection, as before, we assume that we are given an instance $I=(G,\Sigma)$ of the \cnwrs problem. As before, we fix an optimal solution $\phi^*$ for this problem. The goal of this section is to prove the following theorem.



Suppose we are given a graph $H$ and a set $T$ of its vertices called terminals. Let $\Lambda(H,T)$ denote the set of all pairs $(\qset,x)$, where $x$ is a vertex of $H$, and $\qset$ is a collection of paths routing the vertices of $T$ to $x$ in $\qset$. A \emph{distribution} $\dset$ over pairs in $\Lambda(H,T)$ is an assignment, to every pair $(\qset,x)\in \Lambda(H,T)$, of a probability value $p(\qset,x)\geq 0$, such that $\sum_{(\qset,x)\in \Lambda(H,T)}p(\qset,x)=1$. The distribution $\dset$ is specified by listing all pairs $(\qset,x)\in \Lambda(H,T)$ of pairs with $p(\qset,x)>0$, together with the corresponding probability value $p(\qset,x)$.
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------

\begin{theorem}\label{thm: find guiding paths}
	There is a large enough constant $c_0$, and an efficient randomized algrorithm, that receives as input an instance $I=(H,\Sigma)$ of \cnwrs, where $|V(H)|=n$, a set $T\subseteq V(H)$ of $k$ vertices of $H$ called terminals, and a collection $\cset$ of disjoint subgraphs of $H$, such that for some parameters $0\leq \alpha,\alpha'\leq 1$ and $\eta,\eta'\geq 1$ with $\eta'\geq \eta^8$, the following conditions hold:
	
	\begin{itemize}
		
		\item $k\geq |E(H_{|\cset})|/\eta$ and $k\geq \eta^6$; 
		\item $\eta\geq \frac{c^*\log^{46}n}{\alpha^{10}(\alpha')^2}$ for some large enough constant $c^*$;
		\item every terminal $t\in T$ has degree $1$ in $H$;
		\item for all $C\in \cset$, $V(C)\cap T=\emptyset$;
		\item set $T$ of terminals is $\alpha$-well-linked in the contracted graph $H_{|\cset}$; 
		
		\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property; and
		\item for every cluster $C\in \cset$, if $\Sigma_C$ is the rotation system for $C$ that is consistent with $\Sigma$, then $\optcro(C,\Sigma_C)\geq \frac{|\delta(C)|^2}{\eta'}$.
	\end{itemize}
	
	The algorithm either returns FAIL, or computes a distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$, such that for all $e\in E(C)$, $\expect{(\cong(\qset,e))^2}\leq O(\log^8k/(\alpha\alpha')^2)$ \mynote{OK to make smaller}. Moreover, if $\optcrors(I)\geq 
	\frac{(k\alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}$, then the probability that the algorithm returns FAIL is at most $1/\poly(n)$. 
	\mynote{need to be careful with this. OK to put $\eta'+\poly\eta$ on the bottom, not OK to put $\eta'\eta$. This is because instance size in the recursion will decrease by factor $\eta$ only.}
\end{theorem}

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------



The remainder of this section is dedicated to the proof of \Cref{thm: find guiding paths}. 
%For convenience, we define a new instance $I'=(H,\Sigma')$ of the \cnwrs problem, as follows. We start from graph $G$, and subdivide every edge $e\in \delta_G(C)$ with a vertex $t(e)$. Denote the resulting graph by $G'$, and let $T=\set{t(e)\mid e\in \delta_G(C)}$. Note that the solution $\phi^*$ to instance $I$ naturally defines a solution  $\phi'$ to the instance defined by graph $G'$ and rotation system $\Sigma$ (the newly added vertices $t$ each have degree $2$ so the ordering $\oset_t$ of their incident edges can be defined arbitrarily.) For subgraphs $X\subseteq G'$, we define $\cro(X)$ with respect to this drawing $\phi'$.

%We then let $H$ be the sub-graph of the resulting graph induced by $C\cup T$, and we let $\Sigma'$ be the corresponding rotation system that is consistent with the original rotation system $\Sigma$ for $G$. Note that, if $u$ is any vertex of $V(H)\setminus T$, and $\qset=\set{Q(t)\mid t\in T}$ is a collection of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, then set $\qset$ naturally defines a set $\qset'$ of paths in graph $G'$, routing the edges of $\delta_{G'}(H)$ to $u$ inside $H$, and so we can define $\cost_H(\qset')$ as usual, with respect to the drawing $\phi'$ of $G'$. Set $\qset$ of paths also naturally defines a set $\qset''$ of paths in graph $G$, routing the edges of $\delta_G(C)$ to $u$ inside $C$, and moreover $\cost_C(\qset)$ in graph $G$ is bounded by $\cost_H(\qset')$ in graph $G'$.

%Therefore, from now on our goal is to compute a vertex $u\in V(H)\setminus T$, and a collection $\qset=\set{Q(t)\mid t\in T}$ of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, so that the cost $\expect{\cost_{H}(\qset)}\leq O(\optcrors(I')\cdot 2^{O((\log^{1/4} m))})$.

For conveninence, we denote the contracted graph $H_{|\cset}$ by $\hH$,  and we denote $|E(\hH)|=\hm$. From the statement of \Cref{thm: find guiding paths}, $k\geq \hm/\eta$. Observe that, from \Cref{clm: contracted_graph_well_linkedness}, the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$.


We start with some intuition. Assume first that graph $H$ contains a grid (or a grid minor) of size $(\Omega(k\alpha\alpha'/\poly\log n)\times (k\alpha \alpha'/\poly\log n))$, and a collection $\pset$ of paths connecting every terminal to a distinct vertex on the first row of the grid, such that the paths in $\pset$ cause a low edge-congestion. For this special case, the algorithm of \cite{Tasos-comm}  (see also Lemma D.10 in the full version of \cite{chuzhoy2011algorithm}) provides the distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$ with the required properties. Moreover, if $H$ is  a bounded-degree planar graph, with a set $T$ of terminals that is $(\alpha\alpha')$-well-linked, 
then there is an efficient algorithm to compute such a grid minor, together with the required collection $\pset$ of paths. If $H$ is planar but no longer bounded-degree, we can still compute a grid-like structure in it, and apply the same arguments as in \cite{Tasos-comm} in order to compute the desired distribution $\dset$. The difficulty in our case is that the graph $H$ may be far from being planar, and, even though, from the Excluded Grid theorem of Robertson and Seymour \mynote{add references to the original thm proof and our new proofs}, it must contain a large grid-like structure, without having a drawing of $H$ in the plane with a small number of crossing, we do not know how to compute such a structure.

The proof of the theorem consists of five steps. In the first step, we will  either establish that $\optcrors(I)$ is sufficiently large (so the algorithm can return FAIL), or compute a subgraph $\hH'\subseteq \hH$, and a partition $(X,Y)$ of $V(\hH')$, such that each of the clusters $\hH'[X],\hH'[Y]$ has the $\hat \alpha$-bandwidth property, for $\hat \alpha=\Omega(\alpha/\log^4n)$, together with a large collection of edge-disjoint paths routing the terminals to the edges of $E_{\hH'}(X,Y)$ in graph $\hH'$. Intuitively, we will view from this point onward the edges of $E_{\hH'}(X,Y)$ as a new set of terminals, that we denote by $\tilde T$ (more precisely, we subdivide each edge of $E_{\hH'}(X,Y)$ with a new vertex that becomes a new terminal). We show that it is sufficient to prove an analogue of \Cref{thm: find guiding paths} for this new set $\tT$ of terminals. The clusters $\hH'[X],\hH'[Y]$ of graph $\hH'$ naturally define a partition $(H_1,H_2)$ of the graph $H$ into two disjoint clusters. In the second step, we either establish that $\optcrors(I)$ is suffciently large 
(so the algorithm can return FAIL), or
compute some vertex $x$ of $H_1$, and a collection $\pset$ of paths in graph $H_1$, routing the terminals of $\tilde T$ to $x$, such that the paths in $\pset$ cause a relatively low edge-congestion.
We exploit this set $\pset$ of paths in order to define an ordering of the termianls in $\tilde T$, which is in turn exploited in the third step in order to compute a ``skeleton'' for the grid-like structure. We compute the grid-like structure itself in the fourth step. In the fifth and the final step, we generalize the arguments from \cite{Tasos-comm}  and  \cite{chuzhoy2011algorithm} in order to obtain the desired distribution $\dset$.


Before we proceed, we need to consider two simple special cases. In the first case,  $\sum_{C\in \cset}|\delta(C)|^2$ is large. In the second case, we can route a large subset of the terminals to a single vertex of $V(\hat H)\cap V(H)$ in the graph $\hat H$ via edge-disjont paths.

\paragraph{Special  Case 1: $\sum_{C\in \cset}|\delta(C)|^2$ is large.}
We consider the special case where $\sum_{C\in \cset}|\delta(C)|^2\geq \frac{(k \alpha^4 \alpha')^2}{c_0\log^{50}n}$, where $c_0$ is the constant from the statement of \Cref{thm: find guiding paths}.
In this case, since we are guaranteed that, for every cluster $C\in \cset$, $\optcrors(C,\Sigma_C)\geq |\delta(C)|^2/\eta'$, we get that:


\[\optcrors(I)\geq \sum_{C\in \cset}\optcrors(C,\Sigma_C)\geq \sum_{C\in \cset}\frac{|\delta(C)|^2}{\eta'}\geq \frac{(k \alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}.\]

Therefore, if $\sum_{C\in \cset}|\delta(C)|^2\geq \frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}$, the algorithm returns FAIL and terminates. We assume from now on that:

\begin{equation}\label{eq: boundaries squared sum bound}
\sum_{C\in \cset}|\delta(C)|^2<\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}
\end{equation}



\paragraph{Special Case 2: Routing of terminals to a single vertex.}
The second special case happens if there exists a collection $\pset_0$ of at least $\frac{k\alpha\alpha'}{1024\cCMG^2\log^4k}$ edge-disjoint paths in graph $H$ routing some subset $T_0\subseteq T$ of terminals to some vertex $x$ (here, $\cCMG$ is the constant from \Cref{claim: embed expander}).
 
Note that, if Special Case 1 did not happen, then $x$ may not be a supernode. Indeed, assume that $x=v_C$ for some cluster $C\in \cset$. Then:


\[(\delta_H(C))^2\geq \Omega\left(\frac{(k\alpha \alpha')^2}{\log^8k}\right )\geq \frac{(k\eta' \alpha^4 \alpha')^2}{c_0\eta'\log^{50}n},\] 

assuming that $c_0$ is a large enough constant, a contradiction (we have used the fact that $\eta'\geq \eta^8$). Therefore, we can assume that $x$ is not a supernode.
Denote $z=|\pset_0|\geq \frac{k\alpha\alpha'}{1024\cCMG^2\log^4k}$.
We compute a single set $\qset$ of paths routing the set $T$ of terminals to $x$, with congestion $O(\log^4k/(\alpha \alpha')^2)$, as follows. We partition the set $T\setminus T_0$ of terminals into $q=\ceil{k/z}\leq O(\log^4k/(\alpha\alpha'))$ subsets, each of which contains at most $z$ vertices. 
Consider now some index $1\leq i\leq q$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\pset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\pset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\pset_i'$. By concatenating the paths in $\pset_i'$ with paths in $\pset_0$, we obtain a collection $\pset_i$ of paths in graph $H$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\alpha\alpha'))$. Let $\qset=\bigcup_{i=0}^q\pset_i$ be the resulting set of paths. Observe that set $\qset$ contains $k$ paths, routing the terminals in $T$ to the vertex $x$ in graph $H$, with $\cong_H(\qset)\leq O(q/(\alpha\alpha'))\leq O(\log^4k/(\alpha\alpha')^2)$. We return a distribution $\dset$ consisting of a single pair $(\qset,u)$, and terminate the algorithm. 

In the remainder of the algorithm, we assume that neither of the two special cases happened. We now describe each step of the algorithm in turn.




%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 1: Splitting the Contracted Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


In this step, we split the contracted graph $\hH$, using the algorithm  summarized in the following theorem.

\begin{theorem}\label{thm: splitting}
	There is an efficient randomized algorithm that with probability at most $1/\poly(n)$ returns FAIL, and, if it does not return FAIL, then it  computes a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that:
	
	\begin{itemize}
		\item each of the clusters $\hH'[X]$ and $\hH'[Y]$ has the $\halpha'$-bandwidth property, for $\halpha'=\Omega(\alpha/\log^4n)$; and
		
		\item there is a set $\rset$ of at least $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
	\end{itemize}

\end{theorem}


\begin{proof}
We start by applying the algorithm from \Cref{claim: embed expander} to graph $\hH$ and the set $T$ of terminals, to obtain a graph $W$ with $V(W)=T$ and maximum vertex degree $O(\log^2k)$, and an embedding $\hpset$ of $W$ into $\hH$ with congestion $O((\log^2k)/\alpha)$. Let $\hat\event$ be the bad event that $W$ is not a $1/4$-expander. Then $\prob{\hat \event}\leq 1/\poly(k)$.

Let $\hH'$ be the graph that is obtained from $\hH$ by deleting from it all edges and vertices except those that participate in the paths in $\hpset$. Equivalently, graph $\hH'$ is obtained from the union of all paths in $\hpset$. We need the following observation.

\begin{observation}\label{obs: expansion and degree}
	If event $\hat \event$ did not happen, then the set $T$ of vertices is $\halpha$-well-linked in $\hH'$, for $\halpha=\frac{\alpha}{4\cCMG\log^2k}$, and the maximum vertex degree in $\hH'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}$.
\end{observation}

\begin{proof}
	Assume that Event $\hat \event$ did not happen. We first prove that the set $T$ of terminals is $\halpha$-well-linked in $\hH$. Consider any paritition $(A,B)$ of vertices of $\hH'$, and denote $T_A=T\cap A$, $T_B=T\cap B$. Assume w.l.o.g. that $|T_A|\leq |T_B|$. Then it is sufficient to show that $|E_{\hH'}(A,B)|\geq \halpha\cdot |T_A|$.
	
	Consider the partition $(T_A,T_B)$ of the vertices of $W$, and denote $E'=E_{W}(T_A,T_B)$. Since $W$ is a $1/4$-expander, $|E'|\geq |T_A|/4$ must hold. Consider now the set $\hat \rset\subseteq \hpset$ of paths containing the embeddings $P(e)$ of every edge $e\in E'$. Each path $R\in \hat \rset$ connects a vertex of $T_A$ to a vertex of $T_B$, so it must contain an edge of $|E_{\hH}(A,B)|$. Since $|\hat\rset|\geq |T_A|/4$, and the paths in $\hpset$ cause edge-congestion at most $(\cCMG\log^2k)/\alpha$, we get that $|E_{\hH}(A,B)|\geq \alpha\cdot |T_A|/(4\cCMG\log^2k)\geq \halpha |T_A|$.
	
	Assume now that maximum vertex degree in $\hH'$ is greater than $d$, and let $x$ be a vertex whose degree is at least $d$. Let $\hat\qset\subseteq \tpset$ be the set of all paths containing the vertex $x$.
Consider any such path $Q\in \hat\qset$. The endpoints of this path are two distinct terminals $t,t'\in T$. We let $Q'\subseteq Q$ be the sub-path of $Q$ between the terminal $t$ and the vertex $x$, and we let $\qset'=\set{Q'\mid Q\in \hat\qset}$.

Recall that every vertex in $W$ has degree at most $\cCMG\log^2k$, and so a terminal in $T$ may be an endpoint of at most $\cCMG\log^2k$ paths in $\hpset$. Therefore, there is a subset $\qset''\subseteq \qset'$ of at least $d/(\cCMG\log^2k)$ paths, each of which originates at a distinct terminal.
But then, from \Cref{claim: routing in contracted graph}, there is a collection $\qset'''$ of edge-disjoint paths in graph $H$, routing a subset of terminals to $x$ of cardinality at least:

\[\frac{\alpha'|\qset''|} 2\geq \frac{\alpha' d}{2\cCMG\log^2k}\geq  \frac{\alpha \alpha' k}{1024\cCMG\log^4k},\]

 contradicting the fact that Special Case 2 did not happen.
\end{proof}



Next, we use the following lemma that allows us to compute the required sets $X$, $Y$ of vertices. The proof follows immediately from techniques that were introduced in \cite{chuzhoy2012routing} and then refined in \cite{chuzhoy2012polylogarithmic,chekuri2016polynomial,chuzhoy2016improved}. Unfortunately, all these proofs assumed that the input graph has a bounded vertex degree, and additionally the proofs are somewhat more involved than the proof that we need here (this is because these proofs could only afford a $\poly\log k$ loss in the cardinality of the path set $\rset$ relatively to $|T|$, while we can afford a $\poly\log n$ loss). Therefore, we provide a complete proof of the lemma in Section \ref{sec: splitting} of the Appendix for completeness.


\begin{lemma}\label{lem: splitting}
	There is an efficient algorithm that, given as input an $n$-vertex graph $G$, and a subset $T$ of $k$ vertices of $G$ called terminals, together with a parameter $0<\talpha<1$, such that the maximum vertex degree in $G$ is at most $\talpha k/64$, and every vertex of $T$ has degree $1$ in $G$, either returns FAIL, or computes a partition $(X,Y)$ of $V(G)$, such that:
	
	\begin{itemize}
		\item each of the clusters $G[X]$, $G[Y]$ has the $\talpha'$-bandwidth property, for $\talpha'=\Omega(\talpha/\log^2n)$; and
		\item there is a set $\rset$ of at least $\Omega(\talpha^3k/\log^2n)$ edge-disjoint paths in graph $G$, routing a subset of terminals to edges of $E_G(X,Y)$.
	\end{itemize}

Moreover, if the vertex set $T$ is $\talpha$-well-linked in $G$, then the algorithm never returns FAIL.
\end{lemma}

We apply the algorithm from \Cref{lem: splitting} to graph $\hH'$, the set $T$ of terminals, and parameter $\talpha=\halpha=\frac{\alpha}{4\cCMG\log^2k}$. Recall that we are guaranteed that maximum vertex degree in $\hat H'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}\leq \frac{\talpha k}{64}$.
Note that the algorithm from  \Cref{lem: splitting} may only return FAIL if the set $T$ of terminals is not $\halpha$-well-linked in $\hH'$, which, from \Cref{obs: expansion and degree}, may only happen if Event $\hat \event$ happened, which in turn may only happen with probability $1/\poly(k)$. If the algorithm from \Cref{lem: splitting} returned FAIL, then we restart the algorithm that we have described so far from scratch. We do so at most $1/\poly\log n$ times, and if, in every iteration, the algorithm from \Cref{lem: splitting} returns FAIL, then we return FAIL as the outcome of the algorithm for \Cref{thm: splitting}. Clearly, this may only happen with probability at most $1/\poly(n)$. Therefore, we assume that in one of the iterations, the algorithm from \Cref{lem: splitting} did not return FAIL. From now on we consider the outcome of that iteration.

 Let $(X,Y)$ be the partition of $V(\hH')$ that the algorithm returns. We are then guaranteed that each of the clusters $\hH'[X],\hH'[Y]$ has the $\talpha'$-bandwidth property, where $\talpha'=\Theta(\halpha/\log^2n)=\Theta(\alpha/\log^4n)$. The algorithm also ensures that there is a collection $\rset$ of edge-disjoint paths in $\hH'$, routing a subset of the terminals to edges of $E_{\hH'}(X,Y)$, with:

\[ |\rset|\geq \Omega(\talpha^3k/\log^2n)=\Omega(\alpha^3k/\log^8n). \]


This completes the proof of \Cref{thm: splitting}.
\end{proof}


If the algorithm from \Cref{thm: splitting} returned FAIL (which may only happen with probability at most $1/\poly(n)$), then we terminate the algorithm and return FAIL as well. Therefore, we assume from now on that the algorithm from \Cref{thm: splitting} returned a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that each of the clusters $\hH'[X]$ and $\hH'[Y]$ has the $\halpha'$-bandwidth property, for $\halpha'=\Omega(\alpha/\log^4n)$, and
 there is a set $\rset$ of at least $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
Notice that we can compute the path set $\rset$ with the above properties efficiently, using standard Maximum $s$-$t$ flow.
Let $E'\subseteq E_{\hH'}(X,Y)$ be the subset of edges containing the last edge on every path in $\rset$, so, by reversing the direction of the paths in $\rset$, we can view the set $\rset$ of paths as routing the edges of $E'$ to the terminals.
In the remainder of this step, we will slightly modify the graphs $H$ and $\hat H$, and we will continue working with the modified graphs in the following steps.

Let $\hH''\subseteq\hH'$ be the graph obtained from $\hH'$ by first deleting all edges of $E_{\hH'}(X,Y)\setminus E'$ from it, and then subdividing every edge $e\in E'$ with a vertex $t_e$. We denote $\tilde T=\set{t_e\mid e\in E'}$, and we refer to vertices of $\tilde T$ as \emph{pseudo-terminals}. Recall that $|\tilde T|=|\rset|=\Omega(\alpha^3k/\log^8n)$, and there is a set $\rset'$ of edge-disjoint paths in the resulting graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$.
We let $\hH_1$ be the subgraph of $\hH''$, that is induced by the set $X\cup \tilde T$ of vertices, and we similarly define $\hH_2=\hH''[Y\cup \tilde T]$. From the $\halpha'$-bandwidth property of the clusters $\hH'[X]$ and $\hH'[Y]$, we are guaranteed that the vertices of $\tilde T$ are $ \halpha'$-well-linked in both $\hH_1$ and in $\hH_2$, where $\halpha'= \Omega(\alpha/\log^4n)$. Let $\cset'\subseteq \cset$ be the subset of all clusters $C$ whose corresponding supernode $v_C$ lies in grpah $\hH''$.

For convenience, we also subdivide, in graph $H$, every edge $e\in E'$, with the vertex $t_e$, so graph $\hH''$ can be now viewed as a subgraph of the contracted graph $H_{|\cset}$.

Next, we let $H'\subseteq H$ be the subgraph of $H$ that corresponds to the graph $\hH''$: namely, graph $H'$ is obtained from $\hH''$ by replacing every supernode $v_C$ with the corresponding cluster $C\in \cset'$. Equivalently, we can obtain graph $H'$ from $H$, by deleting every edge of $E(\hH)\setminus E(\hH'')$ and every regular (non-supernode) vertex of $V(\hH)\setminus V(\hH'')$. Additionally, for every cluster $C\in \cset\setminus \cset'$, we delete all edges and vertices of $C$ from $H'$. We also define a rotation system $\Sigma'$ for graph $H'$, which is identical to $\Sigma$ (vertices $t_e\in \tilde T$ all have degree $2$, so their corresponding ordering $\oset_{t_e}$ of incident edges can be set arbitrarily). 


We partition the set $\cset'$ of clusters into two subsets: set $\cset_X$ contains all clusters $C\in \cset'$ with $v_C\in X$, and set $\cset_Y$ contains all clusters $C\in \cset'$ with $v_C\in Y$. We can similarly define the graphs $H_1,H_2\subseteq H'$, that correspond to the contracted graphs $\hat H_1$ and $\hat H_2$, respectively: let $X'$ contain all vertices $x\in V(H')$, such that either $x\in C$ for some cluster $C\in \cset_X$, or $x$ is a regular vertex of $\hat H''$ lying in $X$. Similarly, we let $Y'$ contain all vertices $y\in V(H)$, such that either $y\in C$ for some cluster $C\in \cset_Y$, or $y$ is a regular vertex of $\hat H''$ lying in $Y$. We then let $H_1=H'[X\cup \tilde T]$, and $H_2=H'[Y\cup \tilde T]$.

The following observation, summarizing some properties of graph $H'$, is immediate:

\begin{observation}\label{obs: properties of new graph}
	\ 
	
	\begin{itemize}
		\item $\optcrors(H',\Sigma')\leq \optcrors (H,\Sigma)$;
		\item $\hat H''=H'_{|\cset'}$; 
		\item $|E(\hat H'')|\leq 2|E(\hat H)|\leq 2\eta k\leq O(|\tilde T|\eta \log^8k/\alpha^3)$; and
		\item graph $\hat H_1$ is a contracted graph of $H_1$ with respect to  $\cset_X$, and graph $H_2$ is a contracted graph of $H_2$ with respect to $\cset_Y$. In other words, $\hat H_1=(H_1)_{|\cset_X}$, and $\hat H_2=(H_2)_{|\cset_Y}$.
	\end{itemize}
\end{observation}

(for third assertion we have used the fact that $k\geq |E(\hat H)|/\eta$ from the statement of \Cref{thm: find guiding paths}, and $|\tilde T|\geq \Omega(\alpha^3k/\log^8n)$.)


Recall that $\Lambda(H',\tilde T)$ denotes the set of all pairs $(\qset,x)$, where $x$ is a vertex of $H'$, and $\qset$ is a collection of paths in graph $H'$, routing the vertices of $\tilde T$ to $x$. In the following observation, we show that it is now enough to compute a distribution $\dset'$ over pairs $(\qset,x)\in \Lambda(H',\tilde T)$, such that for every edge $e\in E(H')$, $\expect{\cong_{H'}(\qset,e)}$ is low, in order to obtain the desired distribution $\dset$ over pairs in $\Lambda(H,T)$.


\begin{observation}\label{obs: convert distributions}
	There is an efficient algorithm, that, given a distribution $\dset'$ over pairs  $(\qset',x')\in \Lambda(H',\tilde T)$,
	such that for every edge $e'\in E(H')$, $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e'))^2}\leq \beta$ holds,
	 computes a distribution $\dset$ over pairs  $(\qset,x)\in \Lambda(H,T)$, such that for every edge $e\in E(H)$, $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\beta \log^{16}n}{\alpha^8(\alpha')^4}\right )$.
\end{observation}
\begin{proof}
	Recall that there is a set $\rset'$ of edge-disjoint paths in graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$, and moreover, such a path set can be found efficiently via a standard maximum $s$-$t$ flow computation.
	Since $\hat H''=H'_{|\cset'}$, from \Cref{claim: routing in contracted graph}, we can efficiently compute a set $\rset_0$ of edge-disjoint paths in graph $H''$, routing a subset $T_0\subseteq T$ of terminals to $\tT$, with $|\rset_0|\geq \alpha'\cdot |\rset'|=\alpha'\cdot |\tilde T|=\Omega(\alpha'\alpha^3k/\log^8n)$. 
	%Let 
	%$T_0\subseteq T$ the set of terminals that serve as endpoints of paths in $\pset_0$. 
	
	Let $z=\ceil{k/|T_0|}=O(\log^{8}n/(\alpha^3\alpha')$. Next, we partition the terminals of $T\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $|T_0|$ each. Consider now some index $1\leq i\leq z$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in graph $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\rset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\rset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\rset'_i$. By concatenating the paths in $\rset'_i$ with paths in $\rset_0$, we obtain a collection $\rset_i$ of paths in graph $H$, routing the terminals in $T_i$ to vertices of $\tilde T$, such that every vertex of $\tilde T\cup \rset_0$ is an endpoint of at most one path in $\rset_i$. Let $\rset^*=\bigcup_{i=0}^z\rset_i$ be the resulting set of paths. Observe that set $\rset^*$ contains $k$ paths, each of which connects a distinct terminal of $T$ to a vertex of $\tilde T$, and every vertex of $\tilde T$ serves as an endpoint of at most $z=O(\log^{8}n/(\alpha^3\alpha')$ such paths. The paths of $\rset^*$ cause congestion at most $O(z/\alpha\alpha')\leq O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$.
	
	
	Recall that $H'\subseteq H$. Consider some pair $(\qset',x')\in \Lambda(H',\tilde T)$ with probability $p(\qset',x')>0$ in the distribution $\dset'$. We compute another path set $\qset$ in graph $H$, routing all terminals in $T$ to $x'$, and we will assign to the pair $(\qset,x')\in \Lambda(H,T)$ the same probability value $p(\qset',x')$. For ever pseudoterminal $\tilde t\in \tilde T$, let $Q'_{\tilde t}\in \qset'$ be the unique path originating at $\tilde t$. For every terminal $t\in T$, let $R'_t\in \rset^*$ be the unique path originating at terminal $t$, and let $\tilde t\in \tilde T$ be the other endpoint of path $R'_t$. We let $Q_t$ be the path obtained by concatenating the paths $R'_t$ and $Q'_{\tilde t}$, so path $Q_t$ connects $t$ to vertex $x'$. We then let $\qset=\set{Q_t\mid t\in T}$. Note that $\qset$ is a set of paths in graph $H$ routing the set $T$ of terminals to vertex $x'$, so $(\qset,x')\in \Lambda(H,T)$. We assign to the pair $(\qset,x')$ probability $p(\qset',x')$. Note that, since every pseudoterminal $\tilde t\in \tilde T$ may seve as an endpoint of at most $O(\log^{8}n/(\alpha^3\alpha')$ paths in $\rset^*$, and since the paths in $\rset^*$ cause edge-congestion at most $O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$, for every edge $e\in E(H)$, we get that:
	
	\[\cong_H(\qset,e)\leq O\left(\frac{\cong_{H'}(\qset',e) \cdot \log^8k}{\alpha^3 \alpha'}+\frac{\log^8k}{\alpha^4(\alpha')^2}\right ).  \]

Therefore, altogether, for every edge $e\in E(H)$:

\[\expect[(\qset,x')\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\log^{16}k}{\alpha^8(\alpha')^4}\right )\cdot \left (\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}+1\right ).  \]	
\end{proof}

From the above discussion, in order to complete the proof of \Cref{thm: find guiding paths}, it is now enough to design a randomized algorithm, that either computes a distribution $\dset'$ over pairs in $\Lambda(H',\tilde T)$ with $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}\leq xxx$, or returns FAIL. It is enough to ensure that,   if $\optcrors(H',\Sigma')\geq 
\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{28}k}$, then the probability that the algorithm returns FAIL is at most $1/\poly(n)$.

In the remainder of the proof we focus on the above goal. It would be convenient for us to simplify the notation, by denoting $H'$ by $H$, $\hat H''$ by $\hat H$, $\tilde T$ by $T$, and $\halpha'$ by $\tilde \alpha$. We also denote $\cset'$ by $\cset$. We now summarize all properties of the new graphs $H,\hat H$ that we have established so far, and in the remainder of the proof of \Cref{thm: find guiding paths} we will only work with these new graphs. 



\paragraph{Summary of the outcome of Step 1.}
We can assume from now on that we are given a graph $H$, a rotation system $\Sigma$ for $H$, a set $\tilde T$ of terminals in graph $H$, and a collection $\cset$ of disjoint subgraphs (clusters) of $H\setminus \tT$. We denote $|\tT|=\tk$. The corresponding contracted graph is denoted by $\hat H=H_{|\cset}$. 
We are also given a partition $(X,Y)$ of $V(H)\setminus \tilde T$ (note that for convenience of notation, $X$ and $Y$ are now subsets of vertices of $H$, and not of $\hat H$), and a parition $\cset_X,\cset_Y$ of $\cset$, such that each cluster $C\in \cset_X$ has $V(C)\subseteq X$, and each cluster $C\in \cset_Y$ has $V(C)\subseteq Y$. We denote $H_1=H[X\cup \tilde T]$ and $H_2=H[Y\cup \tilde T]$. We also denote by $\hat H_1=(H_1)_{|\cset_X}$ the contracted graph of $H_1$ with respect to $\cset_X$, and similarly by $\hat H_2=(H_2)_{|\cset_Y}$ the contracted graph of $H_2$ with respect to $\cset_Y$. 


Note that $\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}\leq O\left( \frac{(\tk\talpha\alpha')^2}{c_0\log^{20}n}\right )$. We will use a constant $c_1$, that is a large enough constant, whose value will be set later, and we set $c_0=c_1^2$. We can then assume that $\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}\leq  \frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}$. In particular, from Equation \ref{eq: boundaries squared sum bound}, we get that $\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(k\alpha^4\alpha')^2}{c_0\log^{50}n}\leq   \frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}$. Additionally, if 
 $\optcrors(H,\Sigma)>\frac{(\tk\talpha\alpha')^2}{c_1\eta'\log^{20}n}$, then $\optcrors(H,\Sigma)>\frac{(k\alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}$. 

We now summarize the properties of the graphs that we have defined and the relationships between the main parameters.

\begin{properties}{P}
	\item $\tk\geq \Omega(\alpha^3k/\log^8n)$;\label{prop after step 1: number of pseudoterminals}
	\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property; \label{prop after step 1: bandwidth property}
	\item $|E(\hat H)|\leq O(\tk\cdot \eta \log^8k/\alpha^3)$; \label{prop after step 1: few edges}
	\item every vertex of $\tilde T$ has degree $1$ in $H_1$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_1$, for $\talpha=\Theta(\alpha/\log^4n)$; \label{prop after step 1: terminals in H1}
	\item similarly, every vertex of $\tilde T$ has degree $1$ in $H_2$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_2$; and \label{prop after step 1: terminals in H1}
\item	$\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}
$, where $c_1$ is some large enough constant, whose value we can set later. \label{prop after step 1: small squares of boundaries}
\end{properties}

Our goal is
to design an efficient randomized algorithm, that either computes a distribution $\dset$ over pairs in $\Lambda(H,\tilde T)$ with $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq xxx$ for every edge $e\in E(H)$, or returns FAIL.


%Note that, if we let $c_1$ be a large enough constant compared to $c_0$, then $\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}>
%\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$.
It is enough to ensure that, if  
%$\optcrors(H,\Sigma)< \frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$, 
$\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$,
then the probability that the algorithm returns FAIL is at most $1/\poly(n)$.

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\iffalse
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: a Modified Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $\hH$, that we denote by $H^+$. In order to define the graph $\hH^+$, we start by defining a rotation system $\hat \Sigma $ for graph $\hH$, as follows. Let $x\in V(\hH)$ be a vertex. If $x$ is a supernode, that is, $x=v(C)$ for some cluster $C\in \cset$, then we define the circular ordering $\hat\oset_x\in \hat \Sigma$ of the edges of $\delta_{\hat H}(x)$ to be arbitrary.
Otherwise, $x$ is a regular vertex, and it is a vertex of the original graph $H$. We then let $\hat \oset_x\in \hat \Sigma$ be identical to the ordering $\oset_x\in \Sigma$, where $\Sigma$ is the original rotation system for graph $H$.

We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(\hat H)$ one-by-one. We denote by $d(u)$ the degree of the vertex $u$ in graph $\hat H$. We now describe an iteration when a vertex $u\in V(\hat H)$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that incident to $u$ in $\hH$, indexed according to their ordering in $\hat \oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(\hat H)$ is processed, we add a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(x,y)\in E(H)$. Assume that $e$ is the $i$th edge of $x$ and the $j$th edge of $y$, that is, $e=e_i(x)=e_j(y)$. Then we add an edge $e'=(s_i(x),s_j(y))$ to graph $H^+$, and we view this edge as the copy of the edge $e\in E(\hat H)$. We will not distinguish between the edge $e$ of $\hat H$ (and the corresponding edge of $H$), and the edge $e'$ of $H^+$.

We note that every terminal $t\in T$ has degree $1$ in $\hat H$, so its corresponding grid $\Pi(t)$ consists of a single vertex, that we also denote by $t$. Therefore, set $T$ of terminals in $H$ naturally corresponds to a set of $k$ terminals in $H^+$, that we denote by $T$ as before.

This completes the definition of the graph $H^+$. Note that the maximum vertex degree in $H^+$ is $4$. We also define a rotation system $\Sigma^+$ for the graph $H^+$ in a natural way: for every vertex $u\in V(H)$, 
consider the standard drawing of the grid $\Pi(u)$, to which we add the drawings of the edges that are incident to vertices $s_1(u),\ldots,s_{d(u)}(u)$, so that the edges are drawn on the grid's exterior in a natural way (\mynote{add figure}). This layout defines an ordering $\oset^+(v)$ of the edges incident to every vertex $v\in \Pi(u)$.

We start with the following simple claim.

\begin{claim}\label{claim: cheap solution to modified instance} There is a solution to the \CNwRS problem instance $(H^+,\Sigma^+)$ of cost at most ..., such that no inner edge of $H^+$ participates in any crossings in the solution.
\end{claim}

\begin{proof}
	We start by showing that $\optcrors(\hH,\hat \Sigma)\leq ...$. Recall that, from \Cref{lem: crossings in contr graph}, there is a drawing $\hat \phi$ of graph $\hH$ with at most $O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2$ crossings, such that for every vertex $x\in V(\hH)\cap V(H)$, the ordering of the edges of $\delta_{\hH}(x)$ as they enter $x$ in $\hat \phi$ is consistent with the ordering $\oset_x\in \Sigma$, and hence with the ordering $\hat \oset_x\in \hat \Sigma$. Drawing $\hat \phi$ of $\hat H$ may not be a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS since for some supernodes $v(C)$, the ordering of the edges that are incident to $v(C)$ in $\hat H$ as they enter the image of $v(C)$ in $\hat \phi$ may be different from $\hat \oset_{v(C)}$. For each such vertex $v(C)$, we may need to \emph{reorder} the images of the edges of $\delta_{\hH}(v(C))=\delta_H(C)$ near the image of $v(C)$, so that they enter the image of $v(C)$ in the correct order. This can be done by introducing at most $|\delta_H(C)|^2$ crossings for each such supernode $v(C)$. The resulting drawing $\hat \phi'$ of $\hat \phi$ is a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS, whose cost is bounded by:
	
	
	\[O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+\sum_{C\in \cset}|\delta_H(C)|^2\leq O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+  \]
	
	
\end{proof}
\fi
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

\iffalse
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: Routing the Terminals to a Single Vertex, and the Epanded Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


\mynote{need to redo this: the paths set should be in the contracted graph $\hH_1$}

In this step we start by considering the graph $H_1$ and the set $\tT$ of terminals in it. Our goal is to compute a collection $\jset$ of paths in graph $H_1$, routing all terminals of $\tT$ to a single vertex, such that the paths in $\jset$ cause a relatively low congestion in graph $H_1$. We show that, if such a collection of paths does not exist, then $\optcrors(H,\Sigma)$ is high. Intuitively, we will use the set $\jset$ of paths in order to define an ordering of the terminals in $\tT$, which will in turn be used in order to compute a grid-like structure in graph $H_2$. Once we compute the desired set $\jset$ of paths, we will replace the graph $H$ with its low-degree analogue $H^+$, that we refer to as the \emph{expanded graph}. The remaining steps in the proof of \Cref{thm: find guiding paths} will use this expanded graph only.


% Recall that the terminals of $\tT$ are $\talpha$-well-linked in $\hat H_1$, and the degree of each terminal in $\hat H_1$ is $1$. 
 
We now proceed to describe the algorithm for Step 2. We consider every \emph{regular} vertex (that is, a vertex that is not a supernode) $x\in V(\hat H_1)$ one by one. For each such vertex $x$, we compute a set $\jset(x)$ of paths in graph $\hat H_1$, with the following properties:

\begin{itemize}
	\item every path in $\jset(x)$ originates at a distinct vertex of $\tT$ and terminates at $x$;
	\item the paths in $\jset(x)$ are edge-disjoint; and
	\item $\jset(x)$ is a maximum-cardinality set of paths in $H_1$ with the above two properties.
\end{itemize}

Note that such a set $\jset(x)$ of paths can be computed via a standard maximum $s$-$t$ flow computation.
Throughout, we use a parameter $\tk'=\ceil{\tk\alpha^5/(c_2\eta\log^{36}n)}$, where $c_2$ is a large enough constant whose value we set later. 

If, for every regular vertex $x\in V(\hH_1)$, $|\jset(x)|<\tk'$, then we reurn FAIL and terminate the algorithm.  In the following lemma, whose proof is deferred to Section \ref{sec: few paths high opt} of Appendix we show that, in this case, $\optcrors(H,\Sigma)\geq 
 \Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$ must hold.
Note that, since we can set $c_1$ to be a large enough constant, we can ensure that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$ holds in this case.

\begin{lemma}\label{lem: high opt or lots of paths}
If,  for every regular vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then $\optcrors(H,\Sigma)\geq 
\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$.
\end{lemma}

\mynote{need to redo from here}

From now on we assume that there is some vertex $x\in V(H_1)$, for which $|\jset(x)|\geq \tk'$. We denote $\jset_0=\jset(x)$, and we let $T_0\subseteq \tT$ be the set of terminals that serve as endpoints of paths in $\jset_0$, so $|T_0|=|\jset_0|=\tk'$.



Let $z=\ceil{\tk/\tk'}=O\left(\frac{\eta\log^{36}n}{\alpha^5\alpha'}\right )$. Next, we arbitrarily partition the terminals of $\tT\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $\tk'$ each. Consider now some index $1\leq i\leq z$. Since the set $\tT$ of terminals is $(\talpha\alpha')$-well-linked in $H_1$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\jset_i'$ of paths in graph $H_1$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $T_i$ cause edge-congestion $O(1/(\talpha\alpha'))$, and each vertex of $T_i$ is the endpoint of at most one path in $\jset_i'$. By concatenating the paths in $\jset_i'$ with paths in $\jset_0$, we obtain a collection $\jset_i$ of paths in graph $H_1$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\talpha\alpha'))$. Let $\jset=\bigcup_{i=0}^z\jset_i$ be the resulting set of paths. Observe that set $\jset$ contains $\tk$ paths, routing the terminals in $\tT$ to the vertex $x$ in graph $H_1$, with $\cong_H(\jset)\leq O\left(\frac z{\talpha\alpha'}\right )\leq O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$. We denote by $\rho=O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$ this bound on $\cong_{H_1}(\pset')$. We assume w.l.o.g. that the paths in $\jset$ are simple. Since every terminal in $\tT$ has degree $1$ in $H_1$, no path in $\jset$ may contain a terminal in $\tT$ as its inner vertex.



In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $H$, that we call \emph{expanded graph}, and denote by $H^+$. 

For every edge $e\in E(H)$, let $N_e=\cong_H(\jset,e)$. Recall that for every edge $e\in E(H_1\setminus\tT)$, $N_e\leq \rho$, and for every other edge $e$ of $H$, $N_e\leq 1$.

\fi







%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: Routing the Terminals to a Single Vertex, and an Expanded Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

In this step we start by considering the graph $H_1$ and the set $\tT$ of terminals in it. Our goal is to compute a collection $\jset$ of paths in graph $H_1$, routing all terminals of $\tT$ to a single vertex, such that the paths in $\jset$ cause a relatively low congestion in graph $H_1$. We show that, if such a collection of paths does not exist, then $\optcrors(H,\Sigma)$ is high. Intuitively, we will use the set $\jset$ of paths in order to define an ordering of the terminals in $\tT$, which will in turn be used in order to compute a grid-like structure in graph $H_2$. Once we compute the desired set $\jset$ of paths, we will replace the graph $H$ with its low-degree analogue $H^+$, that we refer to as the \emph{expanded graph}. The remaining steps in the proof of \Cref{thm: find guiding paths} will use this expanded graph only.


% Recall that the terminals of $\tT$ are $\talpha$-well-linked in $\hat H_1$, and the degree of each terminal in $\hat H_1$ is $1$. 



\subsubsection{Routing the Terminals to a Single Vertex}
We consider every vertex $x\in V(H_1)$ one-by-one. For each such vertex $x$, we compute a set $\jset(x)$ of paths in graph $H_1$, with the following properties:

\begin{itemize}
	\item every path in $\jset(x)$ originates at a distinct vertex of $\tT$ and terminates at $x$;
	\item the paths in $\jset(x)$ are edge-disjoint; and
	\item $\jset(x)$ is a maximum-cardinality set of paths in $H_1$ with the above two properties.
\end{itemize}

Note that such a set $\jset(x)$ of paths can be computed via a standard maximum $s$-$t$ flow computation.
Throughout, we use a parameter $\tk'=\ceil{\tk\alpha'\alpha^5/(c_2\eta\log^{36}n)}$, where $c_2$ is a large enough constant whose value we set later. 

If, for every vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then we reurn FAIL and terminate the algorithm.  In the following lemma, whose proof is deferred to Section \ref{sec: few paths high opt} of Appendix we show that, in this case, $\optcrors(H,\Sigma)\geq 
\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$ must hold.
Note that, since we can set $c_1$ to be a large enough constant, we can ensure that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}$ holds in this case.

\begin{lemma}\label{lem: high opt or lots of paths}
	If,  for every vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then $\optcrors(H,\Sigma)\geq 
	\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$.
\end{lemma}


From now on we assume that there is some vertex $x\in V(H_1)$, for which $|\jset(x)|\geq \tk'$. 



\subsubsection{The Expanded Graph}

From now on we fix the vertex $x\in V(H_1)$. Let $\jset=\jset(x)$ be a set of at least $\tk'$ paths in graph $H_1$, routing a subset $\tT_0\subseteq \tT$ of terminals to vertex $x$. %Assume for now that we are given some fixed ordering $\tilde \oset$ of the terminals in $\tT$, and denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$.


We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(H_1)\setminus \tilde T$ one by one. We denote by $d(u)$ the degree of the vertex $u$ in graph $H_1$. We now describe an iteration when a vertex $u\in V(H_1)\setminus \tilde T$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that are incident to $u$ in $H_1$, indexed according to their ordering in $ \oset_u\in  \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$ indexed in their natural left-to-right order. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the resulting grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(H_1)\setminus \tT$ is processed, we add 
the vertices of $\tT$ to the graph $H^+$. Recall that every terminal $t\in \tT$ has degree $1$ in $H_1$. We denote the unique edge $e_t$ incident to $t$ by $e_1(t)$, and we denote $s_1(t)=t$.

Next, we add 
a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(u,v)\in E(H_1)$. Assume that $e$ is the $i$th edge of $u$ and the $j$th edge of $v$, that is, $e=e_i(u)=e_j(v)$. Then we add an edge $e'=(s_i(u),s_j(v))$ to graph $H^+$, and we view this edge as the \emph{copy of the edge $e\in E(H_1)$}. We will not distinguish between the edge $e$ of $H_1$, and the edge $e'$ of $H^+$.


Our last step is to add vertex $x$ to graph $H^+$, that connects to every terminal $t\in \tT$ with an edge $(x,t)$, that is also viewed as an outer edge. The following lemma, whose proof is deferred to Section \ref{sec:ordering of terminals} of Appendix, allows us to compute an ordering $\tilde \oset$ of the terminals, such that the graph $H^+$ has a drawing $\phi$ with few crossings, in which the inner edges do not participate in any crossings, and the images of edges incident to $x$ enter $x$ in order consistent with $\tilde \oset$.


\iffalse
Our last step is to add a $(\tk\times\tk)$-grid $\Pi(x)$ to graph $H^+$ corresponding to the vertex $x$. As before, the edges of the grid are inner edges for graph $H^+$, and we denote the vertices on the first row of the grid by $s_1(x),\ldots,s_{\tk}(x)$, indexed in their natural left-to-right order. For all $1\leq i\leq \tk$, we add an outer edge $(t_i,s_i(x))$ to graph $H^+$. This completes the definition of the graph $H^+$, provided that we are given an ordering $\tilde \oset$ of the terminals. The following lemma, whose proof is deferred to Section \ref{sec:ordering of terminals} of the Appendix, allows us to compute an ordering $\tilde \oset$ of the terminals, such that the resulting graph $H^+$ has a drawing $\phi$ with few crossings, in which the inner edges do not participate in any crossings.
\fi


\begin{lemma}\label{lem: find ordering of terminals}
	There is an efficient algorithm to compute an ordering $\tilde \oset$ of the terminals in $\tT$, such that there is a drawing $\phi$ of graph $H^+$ with at most $O\left(\optcrors(H,\Sigma)\cdot\frac{\eta^2\log^{74}n}{\alpha^{12}(\alpha')^4}\right ) +O \left (
	\frac{\tk \eta\log^{37}n}{\alpha^6(\alpha')^2}\right )$ crossings, in which all crossings in $\phi$ are between pairs of outer edges. Moreover, if we denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$, and, for each $1\leq i\leq t_{\tk}$, denote by $e_i=(t_i,x)$ the edge of $H^+$ connecting $t_i$ to $x$, then the images of the edges $e_1,\ldots,e_{\tk}$ enter the image of $x$ in this circular order in the drawing $\phi$.
\end{lemma}

From now on we fix the ordering $\tilde \oset$ of the terminals in $\tilde T$, and the drawing $\phi$ of $H^+$ (which is not known to us).



It will be convenient for us to slightly modify the graph $H^+$ as follows. We denote 
the terminals by  $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the circular ordering $\tilde \oset$. Let $H'$ be a graph obtained from $H^+$, by first deleting the vertex $x$ from it, and then adding, for all $1\leq i<\tk$, an edge $e^*_i=(t_i,t_{i+1})$, and another edge $e^*_{\tk}=(t_{\tk},t_1)$. We denote this set of the newly added edges by $E^*$, and we view them as inner edges. Note that the edges of $E^*$ form a simple cycle, that we denote by $L^*$. We also denote $H''=H'\setminus E^*$.

We note that the drawing $\phi$ can be easily extended to obtain the drawing of $H'$ in the plane, so that the inner edges of $H'$ do not participate in any crossings, and the image of the cycle $L^*$ (which must be a simple closed curve) is the boundary of the outer face.

In order to do so, we start with the drawing $\phi$ of $H^+$ on the sphere, and then draw a small disc $D$ with $x$ lying in its interior, and denote by $\eta$ its boundary. 
For every terminal $t_i\in \tT$, we denote by $e_i$ the unique edge incident to $t_i$ in $H''$, and by $e'_i=(t_i,x)$. We also denote by $\gamma_i,\gamma'_i$ the images of the edges $e_i,e'_i$ in the current drawing. Let $p_i$ be the unique point on the intersection of $\gamma'_i$ and $\eta$. We move the image of terminal $t_i$ to point $p_i$. We then modify the image of the edge $e_i$, so that it becomes a concatenation of $\gamma_i$, and the portion of $\gamma'_i$ lying outside the interior of $D$. Lastly, we draw the edges of $E^*$ in a natural way, where edge $e^*_i$ is simply a segment of $\eta$ between the images of $t_i$ and $t_{i+1}$, so that all resulting segments are mutually internally disjoint. Once we delete the vertex $x$ from this drawing, no part of the resulting drawing is contaiend in the interior of the disc $D$, and the image of the cycle $L^*$ is precisely $\eta$, so we can view the resuting drawing as a drawing in the plane, with $D$ being the outer face. Note that this transformation does not increase the number of crossings.


Observe that, if
$\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$, then:

\begin{equation}\label{eq: bound on cr}
\begin{split}
\cro(\phi)\leq &O\left(\frac{(\tilde k\tilde \alpha\alpha')^2\eta^2\log^{54}n}{c_1\eta'\alpha^{12}(\alpha')^4}\right ) + O\left (
\frac{\tk \eta\log^{37}n}{\alpha^6(\alpha')^2}\right ) \\
&\leq O\left(\frac{\tilde k^2\log^{46}n}{c_1\eta^6\alpha^{10}(\alpha')^2}\right ) + O\left (
\frac{\tk \eta\log^{37}n}{\alpha^6(\alpha')^2}\right ),
\end{split}
\end{equation}
since $\talpha=\Theta(\alpha/\log^4n)$ and $\eta'\geq \eta^8$ (from the statement of \Cref{thm: find guiding paths}).



Recall that, from the statement of 
\Cref{thm: find guiding paths}, $k\geq \eta^6$, and from Property \ref{prop after step 1: number of pseudoterminals},
  $\tilde k \geq \Omega(\alpha^3k/\log^8n)$. Therefore, $\tk\geq \Omega(\eta^6\alpha^3/\log^8n)$, and $\eta\leq O\left (\frac{\tk\log^8n}{\eta^5\alpha^3}\right )$. We can now bound the second term in Equation \ref{eq: bound on cr} as follows:
  
  

  \[ O\left (
  \frac{\tk \eta\log^{37}n}{\alpha^6(\alpha')^2}\right )
\leq O\left (
\frac{\tk^2\log^{45}n}{\eta^5\alpha^9(\alpha')^2}\right )
\]

We can assume that $\log n>c_1$, since otherwise, $n$, and therefore $k$, is bounded by a constant $2^{c_1}$. We can then use an arbitrary spanning tree $\tau$ of the graph $H$, 
rooted at an arbitrary vertex $y$, in order to define a collection $\qset$ of paths routing all terminals of $\tT$ to $y$, where for each terminal $t\in \tT$, the corresponding path $Q_t\in \qset$ is the unique path connecting $t$ to $y$ in the tree $\tau$. Since $|\tT|$ is bounded by a constant, for every edge $e\in E(H)$, $\cong_H(\qset,e)\leq O(1)$. We then return a distribution $\dset$ consisting of a single pair $(y,\qset)$, that has probability value $1$. Therefore, we assume from now on that $\log n>c_1$. From the above discussion, we conclude that, if $\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$, then $\cro(\phi)\leq 
O\left(\frac{\tilde k^2\log^{46}n}{c_1\eta^6\alpha^{10}(\alpha')^2}\right )$.


\mynote{@@ will need to redo this part to get fewer crossings as needed}
Recall that, from the conditions of \Cref{thm: find guiding paths}, $\eta\geq c^*\log^{46}n/(\alpha^{10}(\alpha')^4)$. Therefore, we can assume that, for some large enough constant $c_2$, if $\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$, then $\cro(\phi)\leq \frac{\tilde k^2}{\eta^5}$.
It is therefore enough for us to ensure that, if $\cro(\phi)>
 \frac{\tilde k^2}{\eta^5}$, then the  probability that the algorithm returns FAIL is at most $1/\poly(n)$.







Let $\Lambda'$ denote all pairs $(\qset,y)$, where $y$ is a vertex in graph $H$, and $\qset$ is a set of paths in graph $H^+\setminus\set{x}$, routing the set $\tT$ of terminals to vertices of $\Pi(y)$. 
Assume now that we compute a distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every {\bf outer} edge $e\in E(H^+\setminus \set{x})$, $\expect[(\qset,y)\in_{\dset}\Lambda']{(\cong_{H^+\setminus\set{x}}(\qset,e))^2}\leq \beta$. We then immediately obtain a distribution $\dset'$ over pairs in $\Lambda(H,\tT)$, where for every edge $e\in E(H)$, $\expect[(\qset',y)\in_{\dset'} \Lambda(H,\tT)]{(\cong_{H}(\qset',e))^2}\leq \beta$.
In order to obtain the distribution $\dset'$, for every pair $(\qset,y)\in \Lambda(H^+\setminus\set{x},\tT)$, whose probability value in $\dset$ is $p(\qset,y)>0$, we construct a pair $(\qset',y)\in \Lambda(H,\tT)$, as follows. For every terminal $t\in \tT$, let $Q_t\in \qset$ be the unique path connecting $t$ to a vertex of  $\Pi(y)$. By suppressing all inner edges on path $Q_t$, we obtain a path $Q'_t$ in graph $H$, connecting $t$ to $y$. We then set $\qset'=\set{Q'_t\mid t\in \tT}$. It is easy to verify that paths in $\qset'$ route $\tT$ to $y$ in graph $H$, and for every edge $e\in E(H)$, $\cong_H(\qset',e)\leq \cong_{H^+}(\qset,e)$. We assign to the pair $(\qset',y)$ the same probability value $p(\qset,y)$. Let $\dset'$ be the resulting distribution over pairs in $\Lambda(H,\tT)$. It is immediate to verify that $\expect[(\qset',y)\in_{\dset'} \Lambda(H,\tT)]{(\cong_{H}(\qset',e))^2}\leq \beta$.

 






\subsubsection{Summary of Step 2}
\label{step 2 summary}

In the remainder of the proof of \Cref{thm: find guiding paths} we will work with graph $H'$ only. Recall that graph $H'$ contains a set $E^*=\set{e_1,\ldots,e_{\tk}}$ of edges (that are considered to be inner edges), where for all $1\leq i\leq \tk$, $e_i=(t_i,t_{i+1})$ (we will use indices modulo $\tk$). The set $E^*$ of edges defines a cycle $L^*=(t_1,\ldots,t_{\tk})$ in graph $H'$. We also denoted $H''=H'\setminus E^*$. Recall that graph $H''$ is obtained from a subgraph $H_2\subseteq H$, by replacing every vertex $v\in V(H_2)\setminus \tT$ with a grid $\Pi(v)$. All edges lying in the resulting rids $\Pi(v)$, and the edges of $E^*$ are inner edges, while all other edges of $H'$ are outer edge. Each outer edge of $H'$ corresponds to some edge of graph $H_2$, and we do not distinguish between these edges. Note that in graph $H'$, all vertices have degrees at most $4$. We will also use the clustering $\cset_Y$ of graph $H_2$, and the fact that, from Property \ref{prop after step 1: small squares of boundaries}: 

\begin{equation}\label{eq: sum of squares}
\sum_{C\in \cset_Y}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}. \end{equation}





We further partition the outer edges of graph $H''$ into two subsets: type-1 outer edges and type-2 outer edges. Consider any outer edge $e$ in graph $H''$, and let $e'=(u,v)$ be the corresponding edge in graph $H$. If $u$ and $v$ both lie in the same cluster $C\in \cset$, then we say that $e$ is a \emph{type-2} outer edge, and otherwise it is a type-1 outer edge. 
Intuitively, for each type-1 outer edge, there is a corresponding edge in the contracted graph $\hat H$. From Property \ref{prop after step 1: few edges}, we obtain the following observation.


\begin{observation}\label{obs: few outer edges}
	There is a constant $c$, such that the total number of type-1 outer edges in $H''$ is bounded by $\highlightf{c\tk\cdot \eta \log^8k/\alpha^3}$. 
\end{observation}

======================

\highlightf[purple]{Calculations:}

final number of paths: at least $\alpha^*\tk/256$. Supergrid dimensions: $\lambda\times \lambda$. Want: at most $\lambda^2/32$ cells have an outer edge on each path. Number of paths per cell: $\alpha^*\tk/(256\lambda)$. So we need that:

\[\frac{\alpha^*\tk}{256\lambda}\cdot \frac{\lambda^2}{32}>\frac{c\tk\cdot \eta \log^8k}{\alpha^3}.  \]

To ensure this, enough to set:

\[\lambda=\frac{2^{16}c\cdot \eta \log^8n}{\alpha^*\alpha^3}.  \]

(and this is tight to within constants).


Because $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$.

If we ensure that $\highlightf{\eta>\frac{c^* \log^{12}n}{\alpha^4\alpha'}}$, then $\lambda<\eta^2$ will hold.

Group size: start with: 

\[\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}=\floor{\frac{\alpha^3(\alpha^*)^2\tk}{2^{32}c\eta\log^8n}}.\]

This is $\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$. If $\highlightf{\eta>\frac{c^* \log^{8}n}{\alpha^5(\alpha')^2}}$, we get that $\psi>\frac{16\tk}{\eta^2}$.

Overall, for this part, we need $\highlightf{\eta>\frac{c^* \log^{12}n}{\alpha^5(\alpha')^2}}$, which so far is ensured.

======================


Recall that from Property \ref{prop after step 1: terminals in H1}, every vertex of $\tilde T$ has degree $1$ in $H_2$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_2$. Combining this with the $\alpha'$-bandwidth property of every cluster $C\in \cset_Y$ from Property \ref{prop after step 1: bandwidth property}, from \Cref{clm: contracted_graph_well_linkedness}, the set $\tT$ of terminals is $\talpha\cdot \alpha'$-well-linked in $H_2$. Lastly, using the fact that each graph in $\set{\Pi(v)\mid v\in V(H_2)}$ has the $1$-bandwidth property, from \Cref{clm: contracted_graph_well_linkedness}, we get the following observation.


\begin{observation}\label{obs: terminals well linked in H''}
	The set $\tT$ of terminals is $\alpha^*$-well-linked in $H''$, where $\highlightf{\alpha^*=\talpha\cdot\alpha'=\Theta(\alpha\alpha'/\log^4n)}$. Moreover, each terminal in $\tT$ has degree $1$ in $H''$ and degree $2$ in $H'$.
\end{observation}
(we have used the fact that  
$\talpha=\Theta(\alpha/\log^4n)$ (see Property \ref{prop after step 1: terminals in H1})).


%Recall that we are given a circular ordering $\tilde \oset$ of the terminals in $\tT$. This ordering naturally defines an ordering $\oset_x$ of edges incident to $x$ in $H'$: if $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$, and for all $1\leq i\leq \tk$, $e_i$ is the edge $(x,t_i)$, then $\oset_x=\set{e_1,\ldots,e_{\tk}}$.



\begin{definition}[Legal drawing of $H'$]
We say that a darwing of graph $H'$ in the plane is \emph{legal} iff it has the following properties:

\begin{itemize}
	

	\item no inner edge of $H'$ participates in any crossing of $\phi^*$, and in particular the image of the cycle $L^*$ is a simple closed curve, denoted by $\eta$; and
	\item $\eta$ is the boundary of the outer face in the drawing.
\end{itemize}
\end{definition}

We let $\phi^*$ be a legal drawing of $H'$ with smallest number of crossings, and we denote by $\cro^*$ the number of crossings in $\phi^*$.



Denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals arae indexed according their ordering in $\tilde \oset$. We partition the set $\tT$ of terminals into four subsets $T_1,\ldots,T_4$, where $T_1,T_2,T_3$ contain $\floor{\tk/4}$ consecutive terminals from $\tT$ each, and $T_4$ contains the remaining terminals, in a natural way using the ordering $\tilde \oset$, that is, $T_1=\set{t_1,\ldots,t_{\floor{\tk/4}}}$, $T_2=\set{t_{\floor{\tk/4}+1},\ldots,t_{2\floor{\tk/4}}}$, $T_3=\set{t_{2\floor{\tk/4}+1},\ldots,t_{3\floor{\tk/4}}}$, and $T_4=\set{t_{3\floor{\tk/4}+1},\ldots,t_{\tk}}$. Clearly, each of the four sets contains at least $\floor{\tk/4}$ terminals.


For all $1\leq i\leq 4$, we let $\tilde \oset_i$ be the ordering of the terminals in $T_i$ consistent with their ordering on the boundary of the rectangle (where each ordering $\oset_i$ is no longer circular), so that the terminals in sets $T_1$ and in $T_3$ are indexed in their bottom-to-top order, and the terminals in $T_2$ and $T_4$ are indexed in their left-to-right order (so $\tilde \oset$ is obtained by concatenationg $\oset_1,\oset_2$, the reversed ordering $\oset_3$, and the reversed ordering $\oset_4$).






Recall that $\Lambda'$ is the set of all pairs $(\qset,y)$, where $y\in V(H)$, and $\qset$ is a collection of paths in graph $H''$, routing the set $\tT$ of terminals to the vertices of $\Pi(y)$.
Our goal is to design a randomized algorithm, that either computes a distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every outer edge $e\in E(H')$, $\expect[(\qset,y)\in_{\dset} \Lambda']{(\cong_{H'}(\qset,e))^2}\leq xxx$, or returns FAIL.
It is enough to ensure that, if $\cro(\phi)>
\frac{\tilde k^2}{c_2\eta^5}$ for some large enough constant $c_2$, then the  probability that the algorithm returns FAIL is at most $1/\poly(n)$.






\subsection{Step 3: Constructing a Grid Skeleton}





In this and the following step we will construct a grid-like structure in graph $H''$. Recall that the set $\tT$ of terminals is $\alpha^*$-well-linked in grpah $H''$.  From \Cref{thm: bandwidth_means_boundary_well_linked} there is a set $\pset'$ of paths in $H''$, routing all terminals of $T_1$ to terminals of $T_3$, with edge-congestion at most $\ceil{1/\alpha^*}$, such that the routing is one-to-one. From \Cref{claim: remove congestion}, there is a collection $\pset''$ of at least $|T_1|/\ceil{1/\alpha^*}=\floor{\tk/4}/\ceil{1/\alpha^*}\geq \alpha^*\tk/8$ edge-disjoint paths in $H''$, routing some subset of terminals of $T_1$ to a subset of terminal of $T_3$, in graph $H''$. Moreover, since graph $H''$ has maximum vertex degree at most $3$, using arguments similar to those in the proof of \Cref{claim: remove congestion}, there is a collection $\pset$ of $\floor{\alpha^*\tk/32}$ {\bf node-disjoint} paths in graph $H''$, routing some subset $A\subseteq T_1$ of terminals, to some subset $A'\subseteq T_3$ of terminals. We can compute such a set $\pset$ of paths efficiently using standard maximum $s$-$t$ flow algorithms.

Using similar reasoning, we can compute a collection $\rset$ of $\floor{\alpha^*\tk/32}$ node-disjoint paths in graph $H''$, routing some subset $B\subseteq T_2$ of terminals, to some subset $B'\subseteq T_4$ of terminals.

Intuitively, after we discard a small subset of paths from each of the sets $\pset,\rset$, the remaining paths will be used in order to construct a grid-like structure, where paths in $\pset$ will serve as horizontal paths of the grid, and paths in $\rset$ will serve as vertical paths. If the paths in the resulting sets do not form a grid-like structure, then we will terminate the algorithm with a FAIL. We will prove that, if $\cro^*<...$, then we will construct the grid-like structure successfully with probability at least $1-1/\poly(n)$.

We denote $\pset_0=\pset$ and $\rset_0=\rset$. Recall that so far, $\highlightf{|\pset_0|,|\rset_0|\geq \floor{\alpha^*\tk/32}}$. 




Intuitively, if the dimensions of the grid-like structure that we construct are $(h\times h)$, then we need $h$ to be quite close to $\tk$, since this grid-like structure will be exploited in order to define the distribution $\dset$ over pairs in $\Lambda'$.
We will first construct a smaller grid-like structure, that we call a \emph{grid skeleton}. We then extend this grid skeleton to construct a large enough grid-like structure.


We will use two additional parameters. The first parameter is:

\[\lambda=\frac{2^{24}c\cdot \eta \log^8n}{\alpha^*\alpha^3},\] 

where $c$ is the constant from \Cref{obs: few outer edges}. Notice that, since $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$. Moreover, since $\eta>\frac{c^* \log^{12}n}{\alpha^4\alpha'}$ for a large enough constant $c^*$, $\lambda<\eta^2$. The supergrid that we construct will have dimensions $(\Theta(\lambda)\times \Theta(\lambda))$. The second parameter is:

\[\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}=\floor{\frac{\alpha^3(\alpha^*)^2\tk}{2^{30}c\eta\log^8n}}.\]

Clearly, $|\rset_0|,|\pset_0|\geq \lambda\psi$.
Note that, since $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, $\psi\geq \Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$. Since $\highlightf{\eta>\frac{c^* \log^{8}n}{\alpha^5(\alpha')^2}}$, we get that $\psi>\frac{16\tk}{\eta^2}$.  Every cell of the supergrid will be associated with a collection of $\Theta(\psi)$ horizontal paths and $\Theta(\psi)$ vertical paths, that will help us formt he grid-like structure.

We discard paths from $\pset_0$ and from $\rset_0$ arbitrarily, until $|\pset_0|=|\rset_0|=\lambda\phi$ holds.

We denote by $A_0\subseteq T_1,A'_0\subseteq T_3$ the endpoints of the paths in $\pset_0$, and we denote by $B_0\subseteq T_2$, $B'_0\subseteq T_4$ the endpoints of the paths in $\rset_0$.

 
 
\subsubsection*{Grid Skeleton Construction}
 

\iffalse 
 Let $c$ be a constant, such that the number of type-1 outer edges is at most $c\tk\cdot \eta \log^8k/\alpha^3$. 
 
 We say that a path $P\in \pset_0\cup \rset_0$ is \emph{long} if it contains at least $128c\eta\log^8k/(\alpha^*\alpha^3)$ type-1 outer edges, and otherwise we call it short.
Since the total number of type-1 outer edges is at most $c\tk\cdot \eta \log^8k/\alpha^3$, and the paths in  $\pset_0$ are edge-disjoint, at most $\alpha^*\tk/128$ paths in $\pset_0$ may be long. We let $\pset_1\subseteq \pset_0$ be the set of all short paths, so $|\pset_1|\geq \alpha^*\tk/128$. Similarly, we let $\rset_1\subseteq \rset_0$ be the set of all short paths, so $|\rset_1|\geq \alpha^*\tk/128$. We denote by $A_1\subseteq A$, $A_1'\subseteq A'$ the sets of endpoints of the paths in $\pset_1$, and we similarly denote by $B_1\subseteq B$, $B_1'\subseteq B'$ the sets of endpoints o fthe paths in $\rset_1$.
\fi


 
We view the paths in $\pset_0$ as directed from vertices of $A_0$ to vertices of $A'_0$. Recall that $A_0\subseteq T_1$, so the ordering $\oset_1$ of the terminals in $T_1$ defines an ordering $\oset_{A_0}=\set{a_1,\ldots,a_{\lambda\psi}}$ of the terminals in $A_0$. This ordering in turn defines an ordering $\oset_{\pset_0}$ of the paths in $\pset_0$, as follows: if, for all $1\leq i\leq \lambda\psi$, $P_i\in \pset_0$ is the path originating from $a_i$, then $\oset_{\pset_0}=\set{P_1,\ldots,P_{\lambda\psi}}$.

Similarly, we view the paths in $\rset_0$ as directed from vertices of $B_0$ to vertices of $B_0'$. Ordering $\oset_2$ of terminals in $T_2$ defines an ordering $\oset_{B_0}=\set{b_1,\ldots,b_{\lambda\psi}}$ of the vertices in $B_0$, which in turn defines an ordering $\oset_{\rset_0}=\set{R_1,\ldots,R_{\lambda\psi}}$ of paths in $\rset_0$, where for all $i$, path $R_i$ originates at vertex $b_i$.


We partition the set $\pset_0$ of paths into  groups $\uset_1,\ldots,\uset_{\lambda}$ of cardinality $\psi$ each, using the ordering $\oset_{\pset_0}$, so for $1\leq i<\lambda$, set $\uset_i$ is the $i$th set of $\psi$ consecutive paths of $\pset_0$. 
Let $\lambda'= \floor{(\lambda-1)/2}$. 
For all $1\leq i\leq \lambda'$, we let $ P^*_i$ be a path that is chosen uniformly at random from set $\uset_{2i}$. Let $\pset^*=\set{ P^*_1,\ldots, P^*_{\lambda'}}$ be the resulting set of chosen paths. Intuitively, the path in $\pset^*$ will serve as the horizontal paths in the grid skeleton that we construct.
We then let $\pset_1\subseteq \pset_0$ be the set containing all paths in sets $\set{\uset_{2i-1}}_{i=1}^{\lambda'}$. 

We perform similar computation on the set $\rset_0$ of paths. First, we partition $\rset_0$ into  groups $\uset'_1,\ldots,\uset'_{\lambda}$ of cardinality $\psi$ each, using the ordering $\oset_{\rset_0}$, so for $1\leq i<\lambda$, set $\uset'_i$ is the $i$th set of $\psi$ consecutive paths of $\rset_0$. 
For all $1\leq i\leq \lambda'$, we let $ R^*_i$ be a path that is chosen uniformly at random from set $\uset_{2i}$. Let $\rset^*=\set{ R^*_1,\ldots,\tilde R^*_{\lambda'}}$ be the resulting set of chosen paths. Intuitively, the path in $\rset^*$ will serve as the vertical paths in the grid skeleton that we construct.
We then let $\rset_1\subseteq \rset_0$ be the set containing all paths in sets $\set{\uset'_{2i+1}}_{i=1}^{\lambda'-1}$.


We let $\event_1$ be the bad event that there are two distinct paths $Q,Q'\in \rset^*\cup \pset^*$, and two distinct edges $e\in E(Q)$, $e'\in E(Q')$, such that the images of $e$ and $e'$ cross.

\begin{observation}\label{obs: first bad event}
	If $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_1}\leq 1/64$.
\end{observation}

\begin{proof}
Consider any crossing $(e,e')$ in the drawing $\phi^*$. We say that crossing $(e,e')$ is \emph{selected} iff there are two distinct paths $Q,Q'\in \rset^*\cup \pset^*$ with  $e\in E(Q)$, $e'\in E(Q')$. Notice that $e$ may belong to at most two paths in $\rset_0\cup \pset_0$ (one path in each set), and the same is true for $e'$. Each path of $\rset_0\cup\pset_0$ is chosen to $\rset^*\cup \pset^*$ with probability at most $1/\psi$. Therefore, the probability that a path containing $e$, and a path containing $e'$ are chosen to $\rset^*\cup \pset^*$ is at most $4/\psi^2$. Since $\event_1$ can only happen if at least one crossing is chosen, from the union bound, 
$\prob{\event_1}\leq 4\cro^*/\psi^2$. Since $\psi>\frac{16\tk}{\eta^2}$, if $\cro^*<
\frac{\tilde k^2}{c_2\eta^5}$, then:

\[\prob{\event_1}\leq \frac{4\cro^*}{\psi^2}\leq \frac{1}{64c_2\eta}\leq \frac{1}{64}.\]	
\end{proof}




We say that a path $Q\in \rset_0\cup \pset_0$ is \emph{heavy} iff there are at least $\frac{\psi}{64\lambda}$ crossings $(e,e')$ in $\phi^*$, such that at least one of the edges $e,e'$ lies on path $Q$. We say that a bad event $\event_2$ happens iff at least one path in $\rset^*\cup \pset^*$ is heavy.

\begin{observation}\label{obs: first bad event}
	If $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_2}\leq 1/64$.
\end{observation}
\begin{proof}
	Note that every edge of $H''$ may lie on at most two paths of $\rset_0\cup \pset_0$, and every crossing $(e,e')$ involves two edges. Therefore, the total number of heavy paths in $\rset_0\cup \pset_0$ is bounded by $\frac{4\cro^*}{\psi/(64\lambda)}=\frac{16\lambda\cro^*}{\psi}$. Assuming that $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, and using the fact that $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$ and $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$, we get that the total number of heavy paths in $\rset_0\cup \pset_0$ is bounded by:
	
	
	\[ \frac{16\lambda\cro^*}{\psi}\leq O\left( \frac{\tilde k^2}{c_2\eta^5}\cdot \frac{\eta \log^{12}n}{\alpha^4\alpha'}\cdot\frac{\eta}{\tk}\cdot \frac{\log^8n}{\alpha^5(\alpha')^2} \right ) 
\leq	 O\left( \frac{\tilde k\log^{20}n}{c_2\eta^3\alpha^9(\alpha')^3} \right ).
	\]
	
Note that each heavy path may be selected to $\rset^*\cup \pset^*$  with probability at most $1/\psi$. Therfore, using the union bound and the fact that $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$, we get that:

\[\prob{\event_2}\leq 
O\left( \frac{\tilde k\log^{20}n}{\psi\cdot c_2\eta^3\alpha^9(\alpha')^3}\right )\leq
O\left( \frac{\log^{20}n}{\cdot c_2\eta^2\alpha^{14}(\alpha')^5}\right ).\]
	
Recall that, from the conditions of \Cref{thm: find guiding paths}, $\eta\geq c^*\log^{46}n/(\alpha^{10}(\alpha')^4)$, where $c^*$ is a sufficiently large constant. Therefore, if 
$\cro^*<
\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_2}\leq 1/64$.
\end{proof}


Let $\rset'\subseteq \rset_1$, $\pset'\subseteq \pset_1$ be the sets containing all paths $Q$, such that, in drawing $\phi^*$, some edge of $Q$ crosses some edge lying on the paths of $\rset^*\cup \pset^*$. We will also use the following observation:

\begin{observation}\label{obs: few bad paths}
	If $\event_2$ did not happen, then $|\rset'|,|\pset'|\leq \psi/32$.
\end{observation}
\begin{proof}
	Recall that $|\rset^*|+|\pset^*|\leq \lambda$. If bad event $\event_2$ did not happen, then for each path $Q\in \rset^*\cup \pset^*$, there are at most $\frac{\psi}{64\lambda}$ crossings in $\phi^*$, in which edges of $Q$ participate. Therefore, if event $\event_2$ did not happen, there are in total at most $\psi/64$ crossings $(e,e')$ in the drawing $\phi^*$, where at least one of the edges $e,e'$ lies on a path of $\pset^*\cup \qset^*$. Let $E'\subseteq E(H'')$ be the set of all edges $e$, such that there is an edge $e'$ lying on some path of $\pset^*\cup \qset^*$, and crossing $(e,e')$ is present in $\phi^*$. Then $|E'|\leq \psi/32$. Each path in $\rset'\cup \pset'$ must contain an edge of $E'$. As the paths in each of the sets $\rset',\pset'$ are disjoint, $|\rset'|,|\pset'|\leq \psi/32$ must hold.
\end{proof}





\paragraph{Summary of Step 3.}
In this step we have constructed a grid skeleton, that consists of two sets of paths: $\pset^*=\set{ P^*_1,\ldots, P^*_{\lambda'}}$, and $\rset^*=\set{ R^*_1,\ldots,\tilde R^*_{\lambda'}}$, where $\lambda'= \floor{(\lambda-1)/2}$. Recall that $\pset^*\subseteq \pset_0$, and the paths in $\pset^*$ are indexed according to their order in $\oset_{\pset_0}$. Recall that we have also defined the set  $\pset_1\subseteq \pset_0$ of paths, containing all paths in sets $\set{\uset_{2i-1}}_{i=1}^{\lambda'+1}$. It would be convinient for us to re-index the groups $\uset_i$ as follows: for  $1\leq i\leq \lambda'$, set $\uset_i=\uset_{2i-1}$. In other words, the paths of $\uset_0$ lie before path $P^*_1$  in the ordering $\oset_{\pset_0}$, the paths of $\uset_{\lambda'+1}$ lie after $P^*_{\lambda'}$ in this ordering, and, for $1\leq i<\lambda'$, the  paths of $\uset_i$ lie between paths $P^*_i$ and $P^*{i+1}$.
Similarly, $\rset^*\subseteq \rset_0$, and the paths in $\rset^*$ are indexed according to their order in $\oset_{\rset_0}$. We have also defined the set  $\rset_1\subseteq \rset_0$ of paths, containing all paths in sets $\set{\uset'_{2i-1}}_{i=1}^{\lambda'+1}$. As before, we re-index them as follows: for $1\leq i\leq\lambda'$, we set $\uset'_i=\uset'_{2i-1}$. Therefore, the paths of $\uset'_0$ lie before path $R^*_1$  in the ordering $\oset_{\rset_0}$, the paths of $\uset'_{\lambda'+1}$ lie after $R^*_{\lambda'}$ in this ordering, and, for $1\leq i<\lambda'$, the  paths of $\uset'_i$ lie between paths $R^*_i$ and $R^*{i+1}$.



From our definition, if $\event_1$ did not happen, then for every pair $Q,Q'\in \pset^*\cup \qset^*$ of distinct paths, their images in $\phi^*$ do not cross (but note that the image of a single path may cross itself). 

We have also defined a set $\pset'\subseteq \pset_1$ and a set $\rset'\subseteq \rset_1$ of paths, containing all paths $Q$ whose image crosses the image of some path in $\rset^*\cup \pset^*$ in drawing $\phi^*$. From \Cref{obs: few bad paths}, if Event $\event_2$ does not happen, then $|\pset'|,|\rset'|\leq \psi/32$.


It will be convenient for us to consider the $((\lambda'+1)\times (\lambda'+1))$-grid $\Pi^*$. We view the columns of the grid as corresponding to the left boundary of the bounding box $B^*$, the paths in $\set{R^*_1,\ldots,R^*_{\lambda'}}$, and the right boundary of the bounding box $B^*$.
For convenience, we index the columns of the grid from $0$ to $\lambda+1$, so the left boundary of the bounding box corresponds to column $0$, and, for $1\leq i\leq \lambda_i$, path $P^*_i$ represents the $i$th column of the grid, with the right boundary of $B^*$ repersenting the last column. Similarly, we view the bottom boundary of $B^*$, the paths in  $\set{P^*_1,\ldots,P^*_{\lambda'}}$, and the top boundary of $B^*$ as representing the rows of the grid, in the bottom-to-top order. As before, we index the rows of the grid so that the botommost row has index $0$ and the topmost row has index $\lambda'+1$. Notice however that the union of the paths in $\pset^*\cup \rset^*$ does not necessarily form a proper grid graph, as it is possible that, for a pair $P\in \pset^*$, $R\in \rset^*$ of paths, $P\cap R$ is a collection of several disjoint paths.

We will now consider the drawing $\phi^*$ of $H''$, and we will use it to define vertical and horizontal strips corresponding to paths in $\pset^*$ and $\rset^*$, respectively. We will also associate, with each cell of the grid $\Pi^*$, some region of the plane. We assume in the following definitions that Event $\event_1$ did not happen.


Consider first the image $\gamma_i$ of some path $P^*_i\in \pset^*$ in the drawing $\phi^*$.  Note that $\gamma_i$ is not necessarily a simple curve.
 We define two simple curves, $\gamma^t_i$ and $\gamma^b_i$, where $\gamma^t_i$ follows the image of $\gamma_i$ from the top, and $\gamma^b_i$ follows it from the bottom. In other words, we let $\gamma^b_i$ be a simple curve, contained in $\gamma_i$, with the same endpoints as $\gamma_i$, such that the following holds: if $K^b_i$ is the area of the bounding box $B^*$ below $\gamma_i$, including $\gamma_i^t$, then $\gamma_i\subseteq K^b_i$. We define the other curve, $\gamma^b_i$ symmetrically, so curve $\gamma_i$ is contained in the disc whose boundary is $\gamma_i^t\cup \gamma_i^b$. For convenience, we let $\gamma_0^t$ be the bottom boundary of the bounding box $B^*$, and $\gamma_{\lambda'+1}^b$ be the top boundary of the bounding box $B^*$.
 We now define, for all $0\leq i\leq \lambda'$, a region of the plane that we call the $i$th horizontal strip, and denote by $\hstrip_i$. This strip is simply the closed region of the bounding box between the curves $\gamma_i^t$ and $\gamma_{i-1}^b$. 
 

For every vertical path $R^*_i\in \rset^*$, we also define two curves, $\gamma^{\ell}_i$ and $\gamma^r_i$, that follow the image $\gamma_i$ of $R^*_i$ in $\phi^*$ on its left and on its right, respectively. We denote by $\gamma_0^r$ the left boundary of the bounding box $B^*$, and by $\gamma_{\lambda'+1}^{\ell}$ its right boundary. For all $0\leq i\leq \lambda'$, we define a vertical strip $\vstrip_i$ to be the closed region of the bounding box $B^*$ betwen $\gamma_i^r$ and $\gamma_i^{\ell}$.

The following observation is immediate.

\begin{observation}\label{obs: must cross chosen paths}
	If $R\in \rset_1$ is a path whose image in $\phi^*$ intersects the interior of more than one vertical strip in $\set{\vstrip_0,\ldots,\vstrip_{\lambda'+1}}$, then $R\in \rset'$. Similarly, if $P\in \pset_1$ is a path whose image in $\phi^*$ intersects the interior of more than one horizontal strip in $\set{\hstrip_0,\ldots,\hstrip_{\lambda'+1}}$, then $P\in \pset'$. 
\end{observation}

Lastly, for all $0\leq i,j\leq \lambda'$, we let $\cellr_{i,j}=\hstrip_i\cap \vstrip_j$ be a closed region of the plane that we associate with cell $\cell_{i,j}$ of the grid $\Pi^*$.




====================================

\highlightf{Calculations: heavy paths}

Path is heavy if it participates in $x$ crossings. All paths of skeleton will give $\lambda x$ crossings. Using $\lambda<\eta^2$, this is less than $x\eta^2$ crossings. This should be less than $\psi/16$. Because $\psi>\frac{16\tk}{\eta^2}$, enough that $x\eta^2<\tk/\eta^2$, or that $x<\tk/\eta^4$.

If we fix $x=\tk/\eta^4$. Then number of bad paths is at most: 

\[\frac{4\cro^*}{x}< 	\frac{\tilde k^2}{c_2\eta^5}/\frac{\tk}{\eta^4}=\frac{\tk}{c_2\eta}.  \]

A heavy path is selected with probability $1/\psi$. Probability that any heavy path is selected (from union bound) is at most:

\[ \frac{\tk}{c_2\eta\psi}. \]

If we use $\psi>\frac{16\tk}{\eta^2}$, this is not good enough. 

===============================

More detained calculation: all paths of skeleton will give $\lambda x$ crossings, and we want it to be less than $\psi/16$. so $x=\frac{\psi}{16\lambda}$ is fine. Now number of bad paths is at most:

\[\frac{4\cro^*}{x}< \frac{64\cro^*\lambda}{\psi}.\]

A heavy path is selected with probability $1/\psi$. Probability that any heavy path is selected (from union bound) is at most:

\[\frac{64\cro^*\lambda}{\psi^2}\]

So for us it is enough that $\cro^*<\psi^2\cdot 2^{12}/\lambda$.

We have:$ \psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$, so $\frac{\psi}{\lambda}\geq \frac{\alpha^*\tk}{128}$. Using $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\frac{\psi}{\lambda}\geq \Omega(\frac{\alpha\alpha'\tk}{\log^4n})$.

So now $\psi^2/\lambda=\Omega (\frac{\psi\alpha\alpha'\tk}{\log^4n} )$.

Can use now $\psi>\frac{16\tk}{\eta^2}$, so the expression becomes:

\[\Omega (\frac{\tk^2\alpha\alpha'}{\eta^2\log^4n} )  \]

Lastly, because $\eta>\log^4n/(c^*\alpha\alpha')$, we get that $\cro^*<\tk^2/(c_2\eta^5)$ is good enough.

%Using $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$, this is:


%\[\Omega (\frac{\tk^2\alpha^6(\alpha')^3}{\eta\log^{12}n} )\] 

=====================================





\subsection{Step 4: Constructing a Grid-Like Structure}

In this step we furthere delete some paths from sets $\rset_1$ and $\pset_1$ to ensure that the resulting paths form a grid-like structure. This is done in three stages. In the first stage, we discard some paths to ensure that every remaining path in $\rset_1$ intersects the paths in $\pset^*$ ``in order'' (we formally define what it means later). In the second stage, we associate, with every cell of the grid $\Pi^*$ a collection of horizontal and a collection of vertical paths. In the third stage, we ensure that for every cell of the grid $\Pi^*$, there are many inersections between its corresponding horizontal and vertical paths.

Before we continue, we discard some paths of $\rset^*\cup \pset^*$ that must lie in $\rset'\cup \pset'$. Specifically, consider some path $P\in \pset^*$, and assume that it lies in group $\uset_i$, for $0\leq i\leq \lambda'+1$. Let $(a,a')$ be the endpoints of path $P$, with $a\in T_1$ and $a'\in T_3$. Notice that from the definition, if $i>0$, then $a$ must lie, in the ordering $\oset_1$ of the terminals of $T_1$, after the endpoint of the path $P^*_i$ that belongs to $T_1$. Similarly, if $i<\lambda'+1$, then $a$ must lie before the endpoin of the path $P^*_{i+1}$ that belongs to $T_1$ in the same ordering. In particular, we are guaranteed that in the drawing $\phi^*$, the image of $P$ must intersect the interior of the horizontal strip $\hstrip_i$. Consider now the endpoint $a'$ of $P$. If $i>0$, let $a'_i$ be the endpoint of path $P_i^*$ that lies in $T_3$, and if $i<\lambda'+1$, let $a'_{i+1}$ be the endpoint of path $P_{i'+1}$ that lies in $T_3$. Note that, if $a'$ lies before $a'_i$ in the ordering $\oset_3$ of $T_3$, or if $a'$ lies after $a'_{i+1}$ in the ordering $\oset_3$, then the image of $P$ has to intersect the interior of an additional horizontal strip, and, from \Cref{obs: must cross chosen paths}, path $P$ must lie in $\pset'$. We discard each such path from set $\pset_1$ (and from the corresponding set $U_i$). This ensures that, if $P\in U_i$, then its endpoint $a'$ must lie between $a'_i$ and $a'_{i+1}$ in $\oset_3$, if $1\leq i\leq \lambda'$; it must lie before $a'_{i+1}$ if $i=0$, and it must lie after $a'_i$ if $i=\lambda'+1$.
We process the paths in $\rset_1$ similarly, discarding paths as needed. Notice that so far all paths that we have discarded from $\pset_1\cup \rset_1$ lie in $\pset'\cup \rset'$.


\subsubsection{In-Order Intersection}

In this stage we discard some additional paths from $\pset_1\cup \rset_1$, to ensure that every remaining path in $\pset_1$ interesects the paths in $\rset^*$ in-order (notion that we define below); we do the same for paths in $\rset_1$. We will ensure that all paths discarded at this stage lie in $\pset'\cup \rset'$.

Since the definitions and the algorithms for the paths in $\pset_1$ and for the paths in $\rset_1$ are symmetric, we only show how to process the paths in $\pset_1$ here.

Let $P\in \pset_1$ be any path, that we view as directed from its endpoint that lies in $T_1$ to its endpoint lying in $T_3$. Let $X(P)=\set{x_1,\ldots,x_r}$ denote all vertices of $P$ lying on paths in $R^*$, that is, $X(P)=V(P)\cap \left(\bigcup_{i=1}^{\lambda'}V(R^*_i)\right )$. We assume that the vertices of $X(P)$ are indexed in the order of their appearance on $P$. For each such vertex $x_j$, let $i_j$ be the index of the path $R^*_{i_j}\in \rset^*$ containing $x_j$.

\begin{definition}[In-order intersection]
	We say that path $P$ intersects the paths of $\rset^*$ in-order, iff $r\geq \lambda'$, $i_1=1$, $i_r=\lambda'$, and, for $1\leq j<r$, $|i_j-i_{j+1}|\leq 1$.
\end{definition}

Notice that the definition requires that path $P$ intersects every path of $\rset^*$ at least once; the first path of $\rset^*$ that it intersects must be $R_1^*$, and the last path must be $R_{\lambda'}^*$, and for every consecutive pair $x_j,x_{j+1}$ of vertices in $X(P)$, either both vertices lie on the same path of $\rset^*$, or they lie on consecutive paths of $\rset^*$. Notice that path $P$ is still allowed to intersect a path of $\rset^*$ many times, and may go back and forth across all these paths several times.

\begin{observation}\label{obs: not in order intersection}
	Assume that Event $\event_1$ did not happen. Let $P\in \pset_1$ be a path that  intersect the paths of $\rset^*$ not in-order. Then $P\in \pset'$ must hold.
\end{observation}

\begin{proof}
	Assume first that $i_1\neq 1$, that is, vertex $x_1$ lies on some path $R^*_i$ with $i\neq 1$. Let $p$ be a point on the image of path $P$ in $\phi^*$ that is very close to its first endpoint, so $p$ lies in the interior of the horizontal strip $\hstrip_1$, and let $p'$ be the image of the point $x_1$. Clearly, $p'$ does not lie in the interior or on the boundary of $\hstrip_1$, so the image of path $P$ must cross the top boundayr of $\hstrip_1$, which means that the image of some edge $P$ and the image of some edge of $R_1^*$ cross.
	
	The cases where $i_{r}\neq \lambda'$, or there is an index $1\leq j<r$ with $i_j-i_{j+1}> 1$ are treated similarly, as is the case when $r<\lambda'$.
\end{proof}


We discard from $\pset_1$ all paths $P$ that intersect the paths of $\rset^*$ not in-order. We denote by $\pset_2\subseteq \pset_1$ the set of remaining paths. We also update the groups $\uset_0,\ldots,\uset_{\lambda'+1}$ accordingly. Observe that so far all paths that we have discarded lie in  $\pset'$. 
From \Cref{obs: few bad paths}, assuming that Events $\event_1$ and $\event_2$ did not happen, the number of paths that we have discarded so far from $\pset_1$ is at most $\psi/32$. In particular, for all $0\leq i\leq \lambda'+1$, $|\uset_i|\geq 31\psi/32$ still holds.

We perform the same transformation on set $\rset_1$ of paths, obtaining a new set $\rset_2$ of paths, each of which intersects the paths of $\pset^*$ in-order. We also update the groups $\uset'_1,\ldots,\uset'_{\lambda'+1}$. As before, for all $0\leq i\leq \lambda'+1$, $|\uset'_i|\geq 31\psi/32$ still holds.






\subsubsection{Definining Paths Associated with Grid Cells}

For every path $P\in \pset_2$, for all $1\leq i\leq \lambda'$, we denote by $v_i(P)$ the last vertex on path $P$ that lies on the vertical path $R^*_i$; note that, from the definition of in-order intersection, such a path must exist. For all $1\leq i< \lambda'$, we define the $i$th segment of $P$, $\sigma_i(P)$, to be the subpath of $P$ between $v_i(P)$ and $v_{i+1}(P)$. We also let $\sigma_0(P)$ be the subpath of $P$ from its first vertex (which must be a terminal of $T_1$) to $v_1(P)$, and by $\sigma_{\lambda'}(P)$ the subpath of $P$ from $v_{\lambda'}(P)$ to the last vertex of $P$ (which must be a terminal of $T_3)$. 

Siilarly, for every path $R\in \rset_2$, for all $1\leq i\leq \lambda'$, we denote by $v_i(R)$ the first vertex on path $R$ that lies on the horizontal path $P^*_i$. For all $1\leq i< \lambda'$, we define the $i$th segment of $P$, $\sigma_i(R)$, to be the subpath of $R$ between $v_i(R)$ and $v_{i+1}(R)$. We also let $\sigma_0(R)$ be the subpath of $R$ from its first vertex (which must be a terminal of $T_2$) to $v_1(R)$, and by $\sigma_{\lambda'}(R)$ the subpath of $R$ from $v_{\lambda'}(R)$ to the last vertex of $R$ (which must be a terminal of $T_3)$. 


Consider now some cell $\cell_{i,j}$ of the grid $\Pi^*$, for some $0\leq i,j\leq \lambda'+1$. We define the set $\pset^{i,j}$ of horizontal paths, and the set $\rset^{i,j}$ of vertical paths associated with cell $\cell_{i,j}$, as follows. In order to define the set $\pset^{i,j}$ of horizontal paths, we consider the group $U_i$, and, for every path $P\in U_i$, we include its $j$th segment $\sigma_j(P)$ in $\pset^{i,j}$, so that:

\[\pset^{i,j}=\set{\sigma_j(P)\mid P\in \uset_i}.\]
	
	Similarly, we define:
	
	\[\rset^{i,j}=\set{\sigma_i(R)\mid R\in \uset'_j}.\]
	
	Note that the definition of the sets $\pset^{i,j},\rset^{i,j}$ of paths depends on the definition of the direction of the paths in $\pset_2,\rset_2$. For example, recall that we think of the vertices of $T_1$ as lying on the left boundary of the bounding box $B^*$, and the vertices of $T_3$ as lying on its right boundary, with the paths in $\pset_2$ directed from left to right. If we were to flip the bounding box $B^*$, so that the vertices of $T_3$ appear on its left boundary and the vertices of $T_1$ on its right boundary, with the paths in $\pset$ directed from left to right, then the definition of the sets $\pset^{i,j}$ of paths may change (as a path in $\pset_2$ may intersect a path of $\rset^*$ numerous times). 
	However, if we flip the bounding box $B^*$, so that the vertices of $T_1$ appear on its bottom boundary, the vertices of $T_3$ on its top boundary, and the vertices of $T_2$ and $T_4$ on its left and right boundaries, respectively, directing the paths in $\pset$ from bottom to top, and the paths in $\rset$ from left to right, the definition of path sets $\set{\pset^{i,j},\rset^{i,j}}_{0\leq i,j\leq \lambda'+1}$ will now change (but now paths of $\pset$ become vertical and paths of $\rset$ become horizontal). This transformation corresponds to flipping the grid $\Pi^*$ along its diagonal (from bottom left to top right), and so the cells that lied in the top right quandrant of the grid remain in the top right quadrant. We may need to use this transformation later, but for now we stay with the original notation.
	
	We also need the following observation.
	
	\begin{observation}\label{obs: paths in cells don't cross}
		Let $P\in \uset_i,R\in \uset'_j$ be a pair of paths, for some $0\leq i,j\leq \lambda'+1$, and assume that their subpaths $\sigma_j(P)\subseteq P,\sigma_i(R)\subseteq R$ do not share any vertices. Then either $P\in \pset'$, or $R\in \rset'$, or the images of $\sigma_j(P)$ and $\sigma_i(R)$ cross in the drawing $\phi^*$.
	\end{observation}
\begin{proof}
	Assume that $P\not\in \pset'$ and $R\not\in \rset'$, that is, the images of the paths $P,R$ do not cross the images of the paths in $\pset^*\cup \rset^*$ in $\phi^*$. From the definition of set $\uset_i$, the image of $P$ intersects the interior of the horizontal strip $\hstrip_i$, and path $P$ does not share any vertices with the paths of $\rset^*$. Therefore, the image of $P$ must be contained in the strip $\hstrip_i$, and it is disjoint from its top and bottom boundaries $\gamma^b_i,\gamma^t_{i+1}$. Using similar reasoning, the image of $R$ is contained in the strip $\vstrip_j$, and it is disjoint from its left and right boundaries, $\gamma^{\ell}_j,\gamma^r_{j+1}$. Consider now the segment $\sigma_j(P)$ of $P$, whose endpoints lie on $R^*_j$ and $R^*_{j+1}$, respectively. Let $\sigma'_j(P)\subseteq \sigma_j(P)$ be the shortest subpath of $\sigma_j(P)$ whose first endpoint lies on $R^*_j$, and whose last endpoint lies on $R^*_{j+1}$; such a path must exist because we can let $\sigma'_j(P)=\sigma_j(P)$. From the definition of in-order intersection,  no inner vertex of $\sigma'_j$ may lie on any path of $\rset^*$. It is then easy to verify that the image of $\sigma'_j(P)$ in $\phi^*$ must be contained in $\cellr_{i,j}$, and must split this region into two subregions: one whose top boundary contains a segment of $\gamma^b_{j+1}$, and one whose bottom boundary contains a segment of $\gamma^t_j$. 
	
	Using the same reasoning as above, we can select a segment $\sigma'_i(R)$, whose first endpoint lies on $P^*_i$, last endpoint lies on $P^*_{i+1}$, and all inner vertices are disjoint from the vertices lying on the paths in $\pset^*$.
	As before, the image of $\sigma'(R)$ must be contained in $\cellr_{i,j}$, but it connects a point on its top boundary to a point on its bottom boundary. Therefore, the image of $\sigma'_i(R)$ must cross the image of $\sigma'_j(P)$.
\end{proof}


\subsubsection{Completing the Construction of the Grid-Like Structure}


In order to complete the construction of the grid-like structure, we need to ensure that for every pair $0\leq i,j\leq \lambda'+1$ of indices, there are many intersection between the sets $\pset^{i,j}$ and $\rset^{i,j}$ of paths. More specifically, we need to ensure that every path $\sigma\in \pset^{i,j}$ intersects many paths in $\rset^{i,j}$, and vice versay. This is done to ensure well-linkedness properties: namely, that the collection of vertices containing the fist and the last vertex on every path of $\pset^{i,j}$ is sufficiently well-linked in the graph obtained from the union of the paths in $\rset^{i,j}\cup \pset^{i,j}$. This property, in turn, will be exploit in order to construct the sets $\qset$ of paths routing the terminals to sets of vertices $V(\Pi(v)))$ over which the distribution $\dset$ will be defined. This motivates the following definition.

\begin{definition}
	For a pair $0\leq i,j\leq \lambda'+1$ of indices, we say that a path $P\in \uset_i$ is \emph{bad for cell $\cell_{i,j}$} iff there are at least $\psi/16$ paths in $\rset^{i,j}$ that are disjoint from $\sigma_j(P)$. Similarly, we say that a path $R\in \uset'_j$ is bad for cell $\cell_{i,j}$ iff there are at least $\psi/16$ paths in $\pset^{i,j}$ that are disjoint from $\sigma_i(R)$.
\end{definition}

Consider now some index $0\leq i\leq \lambda'+1$. We say that a path $P\in \uset_i$ is \emph{bad} iff it is bad for at least one cell in $\set{\cell_{i,j}\mid 0\leq j\leq \lambda'+1}$. Similarly, for an index  $0\leq j\leq \lambda'+1$, a path $P\in \uset'_j$ is bad iff it is bad for at least one cell in $\set{\cell_{i,j}\mid 0\leq i\leq \lambda'+1}$. The following observation bounds the number of bad paths in each group $\uset_i$ of horizontal paths, and in each group $\uset'_j$ of vertical paths.


\begin{observation}\label{obs: few bad paths in each group}
Assume that $\cro^*\leq \frac{\tilde k^2}{c_2\eta^5}$, and that events $\event_1,\event_2$ did not happen. Then for all $0\leq i\leq \lambda'+1$, at most $\psi/16$ paths in $\uset_i$ are bad. Similarly, for all  $0\leq j\leq \lambda'+1$, at most $\psi/16$ paths in $\uset'_j$ are bad.
\end{observation}

\begin{proof}
Fix an index $0\leq i\leq \lambda'+1$, and the corresponding set $\uset_i\subseteq \pset_2$. We partition the set of all bad paths in $\uset_i$ into two subsets: set $\bset_1$ contains all bad paths lying in $\pset'$, and set $\bset_2$ contains all remaining bad paths. From \Cref{obs: few bad paths}, $|\bset_1|\leq \psi/32$.

We further partition the set $\bset_2$ of bad paths into subsets $\set{\bset_2^j\mid 0\leq j\leq \lambda'}$, where a path $P$ lies in $\bset_2^j$ if it is bad for cell $\cell_{i,j}$ (if path $P$ is bad for several cells, we add it to any of the corresponding sets). Consider now some index $0\leq j\leq \lambda'$, and some path $P\in \bset_2^j$. From the definition, there is a set $\Sigma'\subseteq \rset^{i,j}$ of at least $\psi/16$ paths that do not share any vertices with $P$. From \Cref{obs: few bad paths}, at most $\psi/32$ of these paths may lie in $\rset'$. let $\Sigma''\subseteq \Sigma'$ be the collection of the remaining paths, whose cardinality is at least $\psi/32$. From \Cref{obs: paths in cells don't cross}, for every path $\sigma'\in \Sigma'$, the images of $\sigma_j(P)$, and of $\sigma'$ must cross. We let $\chi_j(P)$ denote the set of all crossings $(e,e')$, where $e\in \sigma_j(P)$, and $e'$ is an edge on a path in $\Sigma'$, so $|\chi_j(P)|\geq \psi/32$. We then let $\chi_{i,j}=\bigcup_{P\in \bset_2^j}\chi_j(P)$, so $|\chi_{j}|\geq |\bset_2^j|\cdot \psi/32$. Lastly, we let $\chi=\bigcup_{j=0}^{\lambda'+1}\chi_j$. Notice that set $\chi$ contains at least $|\bset_2|\cdot \psi/32$ distinct crossings in the drawing $\phi^*$. Assume for contradiction that $|\bset_2|>\psi/32$. Then:

\[\cro^*>\frac{\psi^2}{2^{10}}>\frac{\tk^2}{4\eta^4}>\frac{\tilde k^2}{c_2\eta^5},\]

since $\psi>\frac{16\tk}{\eta^2}$, a contradiction. 
Therefore, $|\bset_2|\leq \psi/32$, and overall there are at most $\psi/16$ bad paths in $\uset_i$.

The proof for path sets $\uset'_j\subseteq \rset_2$ is identical.
\end{proof}


For all $0\leq i\leq \lambda'+1$, we discard every bad path from $\uset_i$. If $|\uset_i| <\ceil{7\psi/8}$ for any $i$, then we terminate the algorithm and return FAIL. Notice that in this case, from \Cref{obs: few bad paths in each group}, if  $\cro^*\geq \frac{\tilde k^2}{c_2\eta^5}$, then at least one of the events $\event_1,\event_2$ must have happened, and the probability for this is at most $1/2$. Therefore, we assume that for all 
$0\leq i\leq \lambda'+1$, $|\uset_i|\geq \ceil{7\psi/8}$ holds. We discard additional arbitrary paths from $\uset_i$, until $|\uset_i|= \ceil{7\psi/8}$.
We then let $\pset_3=\bigcup_{i=0}^{\lambda'+1}\uset_i$ denote the resulting set of paths. 

Similarly, for all $0\leq j\leq \lambda'+1$, we discard every bad path from $\uset'_j$. If, as the result, $|\uset'_j|$ falls below  $\ceil{7\psi/8}$, we terminate the algorithm and return FAIL. Otherwise, we discard additional arbitrary paths as needed, so that $|\uset'_i|=\ceil{7\psi/8}$ holds. We also let $\rset_3=\bigcup_{j=0}^{\lambda'+1}\uset'_j$


For all $0\leq i,j\leq \lambda'$, we also update the path sets $\pset^{i,j}$ and $\rset^{i,j}$ accordingly, discarding the paths that are no longer subpaths of paths in $\pset_3\cup \rset_3$. Since we are still guaranteed that $|\pset^{i,j}|,|\rset^{i,j}|= \ceil{7\psi/8}$, and since every path that is bad for cell $\cell_{i,j}$ was discarded, we are guaranteed that every path in $\pset^{i,j}$ intersects at least $\frac{7\psi}{8}-\frac{\psi}{16}=\frac{13\psi}{16}$ paths of $\rset^{i,j}$ and vice versa.
Since we use this fact later, we summarize it in the following observation.

\begin{observation}\label{obs: paths for cells}
	For all $0\leq i,j\leq \lambda'$, $|\pset^{i,j}|,|\rset^{i,j}|= \ceil{7\psi/8}$. Every path in 
$\pset^{i,j}$ intersects at least $\frac{13\psi}{16}$ paths of $\rset^{i,j}$ and vice versa.
\end{observation}

 This concludes the construction of the grid-like structure.

 


\subsection{Step 5: the Routing}


Recall that we have denoted by $\Lambda'$ the set of all pairs $(\qset,y)$, where $y$ is a vertex in graph $H$, and $\qset$ is a set of paths in graph $H''$, routing the set $\tT$ of terminals to vertices of $\Pi(y)$. In this final step we show an efficient algorithm to compute distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every outer edge $e\in E(H'')$, $\expect[(\qset,y)\in_{\dset}\Lambda']{(\cong_{H''}(\qset,e))^2}\leq xxx$.


Our algorithm closely follows the arguments of 
\cite{Tasos-comm}  (see also Lemma D.10 in the full version of \cite{chuzhoy2011algorithm}), who showed a similar result for a grid graph. In order to provide intuition, we first present their algorithm. Assume that we are given a $(q\times q)$ grid graph $G$ for some integer $q$, and let $T$ be the set of vertices lying on the first row of the grid. For convenience, assume that $q$ is an integral power of $2$. Our goal is to compute a distribution $\dset'$ over pairs in $\Lambda(G,T)$. In other words, the distribution is over pairs $(\qset,v)$, where $v$ is a vertex of $G$, and $\qset$ is a set of paths routing the terminals to $v$. We need to ensure that for every edge $e\in E(G)$, the expectation $\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}\leq O(\log q)$.

For every vertex $v$ in the top right quadrant of the grid, we will define a set $\qset(v)$ of paths in $G$, routing the terminals in $T$ to $v$. Our distribution $\dset$ then assigns, to every pair $(\qset(v),v)$, where $v$ is a vertex of $G$ lying in the top right quadrant of the grid, the same probability value $4/q^2$.

We now fix a vertex $v$ in the top right quadrant of the grid, and define the set $\qset(v)$ of paths. Let $r=\log(q/4)$. For $1\leq i\leq r$, let $S_i$ be a square subgrid of $G$, of size $(2^i\times 2^i)$, whose upper right $v_i$ has the same column-index as vertex $v$, and the same row-index as the bottom left corner of $S_{i-1}$ (we think of $S_1$ as a $(1\times 1)$-grid consisting only of vertex $v$). 
We refer to the subgrids $S_i$ of $G$ as \emph{squares}, and specifically to square $S_i$ as \emph{level-$i$ square}.
For all $1\leq i\leq r$, we denote by $T_i$ the set of vertices lying on the bottom boundary of $S_i$. Using the well-linkedness of the grids, it is easy to show that for all $1\leq i\leq r$, there is a collection $\pset_i$  of paths in graph $S_i$, routing vertices of $T_i$ to verticse of $T_{i-1}$ with congestion at most $2$, such that every vertex  of $T_{i-1}$ serves as endpoint of at most two such paths. For $1\leq i\leq r$, let
Let $\pset'_i$ be a multipset obtained from set $\pset_i$ by creating $2^{r-i+1}$ copies of every path in $\pset_i$. 
Let $T_{r+1}\subseteq T$ be a set of $|T_r|$ vertices lying on the bottom boundary of the grid $G$, that contains, for every vertex $t\in T_r$, a vertex $t'$ on the bottom boundary of $G$ with the same column index as $t$. Let $P_t$ be the subpath of the corresponding column of $G$ connecting $t$ to $t'$, and denote $\pset'_{r+1}=\set{P_t\mid t\in T_r}$.

By concatenating the paths in $\pset_1',\ldots,\pset'_{r+1}$, we obtain a collection $\qset'(v)$ of paths in grid $G$, routing the terminals in $T_{r+1}$ to vertex $v$. 

Notice that for $1\leq i\leq r$, for every edge $e$ lying in $S_i$, the congestion on 
edge $e$ due to paths in $\qset(v)$ is at most $2^{r-i+2}$.

The key in analyzing the expectation $\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}$
is to notice that, for all $1\leq i\leq r$, square $S_i$ is a $(2^i\times 2^i)$-subgrid of $G$, whose upper left corner is chosen uniformly at random from a set of $q^2/4$ possible  points. The total number of subgrids of $G$ of size $(2^i\times 2^i)$ that contain $e$ is $2^{2i}$, so the probability that any of them is selected is bounded by $2^{2i+2}/q^2$. Therefore, for all $1\leq i\leq r$, with probability at most $2^{2i+2-2r}$, edge $e$ belongs to square $S_i$, and in this case, $\cong_G(\qset,e)\leq 2^{r-i+2}$. Therefore, we get that:

\[\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}
\leq \sum_{i=1}^{r+1}2^{2i+2-2r}\cdot 2^{2r-2i+4}\leq O(r)=O(\log q).
\]

Using the well-linkedness of the terminals in $T$, it is immediate to extend the set $\qset'(v)$ of paths to a set $\qset(v)$ routing all terminals in $T$ to $v$, while increasing the congestion on every edge of $G$ by at most an additive constant. This provides the final distribution $\dset$ over pairs $(\qset(v),v)\in \Lambda(G,T)$.



We will simulate a similar process on the grid $\Pi^*$, and its corresponding grid-like structure that we have constructed. Notice however that $\Pi^*$ is only a $(\lambda'\times\lambda')$-grid (where $\eta\leq \lambda'\leq \eta^2$), while the number of terminals that we need to route is much larger (comparable to $|\rset_3|$). Therefore, we will attempt to route all terminals to a single cell $\cell_{i,j}$ in the top right quadrant of the grid (in other words, we will route them to vertices lying on paths  in $\pset^{i,j}\cup \rset^{i,j}$). This in itself is not sufficient, since we need to route them to a set $V(\Pi(y))$ of vertices, corresponding to a single vertex of the original graph $y$. This means that we may need to perform some routing within the cell $\cell_{i,j}$, that is, within the graph obtained from the union of the paths in $\pset^{i,j}\cup \rset^{i,j}$. While generally such a routing may be difficult to compute, we will select a large collection of cells (called good cells) in the top right quadrawnt of the grid, in which such routing is easy to obtain. We will then define, for each good cell, the corresponding set of paths routing the terminals to vertices of $V(\Pi(y))$, for some $y\in V(H)$. We do so by simulating the process described above: we define square subgrids $\set{S_i}$ of the grid $\Pi^*$, and we associate these subgrids with sets of horizontal and vertical paths (subpaths of some paths in $\pset_3\cup \rset_3$), so that the desired well-linkedness properties of graphs corresponding to each subgrid $S_i$ are preserved. Eventually, the distribution $\dset$ chooses one of the good squares uniformly at random, and uses the associated pair $(\qset,y)\in \Lambda'$ in order to route the terminals to vertices of $\Pi(y)$. The analysis of expected congestion squared on every edge is very similar to the one outlined above.

We start by defining the notion of good cells of the grid $\Pi^*$, and showing that a large enough number of such cells exists in the upper right quadrant of $\Pi^*$. We will then define square subgrids of $\Pi^*$ and associate sets of paths with each such subgrid to ensure the required well-linkedness properties. Lastly, we show how to construct the desired routing $\qset$ for each good cell.


\subsubsection{Good Cells}


Fix a pair of indices $0\leq i,j\leq \lambda'$, and consider the cell $\cell_{i,j}$ of the grid $\Pi^*$, and the two corresponding sets $\pset^{i,j}$, $\rset^{i,j}$ of paths.


\begin{definition}[Good cells]
A path $\sigma\in \pset^{i,j}\cup \rset^{i,j}$ is \emph{good} for cell $\cell_{i,j}$ iff $\sigma$ contains no outer edges. 
We say that cell $\cell_{i,j}$ is \emph{horizontally good} iff some path $\sigma \in \pset^{i,j}$ is good for $\cell_{i,j}$, and we say that it is \emph{vertically good} iff some path $\sigma\in \rset^{i,j}$ is good for $\cell_{i,j}$. If cell $\cell_{i,j}$ is horizontally or vertically good, then we say that it is a good cell, and otherwise we say that it is a bad cell.
\end{definition}

Assume that cell $\cell_{i,j}$ is horizontally good, and let $\sigma\in \pset^{i,j}$ be any horizontal path that is good for this cell. Since $\sigma$ contains no outer edges, there must be a vertex $y\in V(H)$, such that $V(\sigma)\subseteq V(\Pi(y))$. Recall that $|\rset^{i,j}|=\ceil{7\psi/8}$, and that $\sigma$ intersects at least $13\psi/16$ paths of $\rset^{i,j}$. Let $\hat \rset^{i,j}\subseteq \rset^{i,j}$ be a set of $\ceil{13\psi/16}$ paths, each of which shares at least one vertex with $\sigma$. Note that each such path then must contain a vertex of $\Pi(y)$. We denot by $\portals_{i,j}$ a set of vertices that contains, for every path $\sigma'\in \hat\rset^{i,j}$, the first vertex of $\sigma'$ (by definition, each such vertex must lie on path $P^*_i$ if $i>0$, or belong to $T_2$ otherwise). For convenience, we denote vertex $y$ by $y_{i,j}$.

Similarly, if cell $\cell_{i,j}$ is vertically good (bot not horizontally good), let $\sigma'\in \rset^{i,j}$ be any vertical path that is good for this cell. As before, $\sigma'$ contains no outer edges, there must be a vertex $y_{i,j}\in V(H)$, such that $V(\sigma')\subseteq V(\Pi(y_{i,j}))$. Recall that $\sigma'$ intersects at least $13\psi/16$ paths of $\pset^{i,j}$. Let $\hat \pset^{i,j}\subseteq \pset^{i,j}$ be a set of $\ceil{13\psi/16}$ paths, each of which shares at least one vertex with $\sigma'$. As before, every path in $\hat \pset^{i,j}$ must contain a vertex of $\Pi(y_{i,j})$. We denot by $\portals_{i,j}$ a set of vertices that contains, for every path $\sigma\in \hat\pset^{i,j}$, the first vertex of $\sigma$.

Let $A$ be the set of all pairs of indices $\floor{\lambda'/2}\leq i,j\leq \lambda'+1$, such that $\cell_{i,j}$ is good. Next, we show that $|A|$ is sufficiently large. Our routing algorithm will then choose a pair $(i,j)$ of indices from $A$ uniformly at random, and then route the terminals to the vertices in set $\portals_{i,j}$, from where they will be routed to vertices of $\Pi(y_{i,j})$.


\begin{claim}\label{claim: many good cells}
	$|A|\geq (\lambda')^2/16$.
\end{claim}

\begin{proof}
	Let $\bset$ be a collection of all bad cells $\cell_{i,j}$ lying in the top right quadrant, that is, $\floor{\lambda'/2}\leq i,j\leq \lambda'+1$. It is enough to show that $|\bset|<(\lambda')^2/16$.
	
	Consider now some bad cell $\cell_{i,j}\in \bset$. Consider now any path $Q\in \rset^{i,j}\cup \pset^{i,j}$. Since cell $\cell_{i,j}$ is bad, $Q$ must contain at least one outer edge. We say that $Q$ is a \emph{type-1} bad path for cell $\cell_{i,j}$ if it contains at least one type-1 outer edge (recall that a type-1 outer edge $e$ corresponds to some edge in graph $H$ that is {\bf not} contained in any cluster in $\cset$). Otherwise, every outer edge on path $Q$ is a type-2 outer edge, and in this case we say that $Q$ is a type-2 bad cluster for $\cell_{i,j}$. We say that cell $\cell_{i,j}$ is \emph{type-1 bad} iff at least $\psi/32$ paths of $\pset^{i,j}\cup \rset^{i,j}$ are type-1 bad for this cell, and otherwise it is type-2 bad. We partition the set $\bset$ of bad cells into two subsets: set $\bset_1$ contains all type-1 bad cells, and set $\bset_2$ contains all type-2 bad cells. It is now enough to prove that $|\bset_1|,|\bset_2|<(\lambda')^2/32$, which we do in the following two observations.
	
	
	\begin{observation}\label{obs: few type-1 bad cells}
		$|\bset_1|< (\lambda')^2/32$.
	\end{observation}
\begin{proof}
	Consider a type-1 bad cell $\cell_{i,j}\in \bset_1$, and let $\qset^{i,j}\subseteq \pset^{i,j}\cup \rset^{i,j}$ be a set of $\ceil{\psi/32}$ paths that are type-1 bad paths for cell $\cell_{i,j}$. Each path in $\qset^{i,j}$ must contain at least one type-1 bad edge. Since the paths in $\qset^{i,j}$ cause edge-congestion at most $2$, there is a set $E^{i,j}$ of at least $\psi/64$ type-1 outer edges of $H''$, lying on paths of $\qset^{i,j}$. Since every edge of $H''$ may lie on at most two paths in $\pset\cup \rset$, the total number of outer edges in $H''$ must be at least: 
	
	\[\frac{|\bset_1|\cdot \psi}{64}\geq \frac{(\lambda')^2\cdot \psi}{2^{11}}\geq  \frac{\lambda^2\cdot \psi}{2^{15}} ,\] 
	
	
	
	as $\lambda'=\floor{(\lambda-1)/2}\geq \lambda/4$.
	
	Recall that $\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$ and $\lambda=\frac{2^{24}c\cdot \eta \log^8n}{\alpha^*\alpha^3}$,  where $c$ is the constant from \Cref{obs: few outer edges}. Therefore, we get that the total number of outer edges in $H''$ is at least $\frac{2c\tk \eta \log^8n}{\alpha^3}$, contradicting \Cref{obs: few outer edges}.
\end{proof}


\begin{observation}\label{obs: few type-1 bad cells}
	$|\bset_2|< (\lambda')^2/32$.
\end{observation}	
\begin{proof}
		For a cluster $C\in \cset$, let $X(C)=\bigcup_{y\in V(C)}V(\Pi(y))$. Note that all terminals of $H$ lie outside of the clusters in $\cset$, and so $X(C)\cap \tT=\emptyset$. If a path $Q\in \pset_3\cup \rset_3$ contains a vertex of $X(C)$, then it must contain at least one edge of $\delta_H(C)$. As the paths in $\pset\cup \rset$ cause edge-congestion at most $2$, the total number of paths $Q\in \pset\cup \rset$ with a non-empty intersection with $X(C)$ is at most $2\delta_H(C)$.
	
	
	Let $\intpairs\subseteq \pset_3\times\rset_3$ be the collection of all pairs of paths $P\in \pset_3$, $R\in \rset_3$, such that $P$ and $R$ share at least one vertex. 
	For a cluster $C\in \cset$, let $\intpairs'_C\subseteq \intpairs$ denote denote the collection of all pairs $(P,R)\in \intpairs$ of paths, such that some vertex $v\in X(C)$ lies on both $P$ and $R$. Clearly, if $(P,R)\in \intpairs_C'$, then each of the paths $P$, $R$ must contain at least one edge of $\delta_H(C)$. Therefore, from the above discussion, $|\intpairs'_C|\leq 4|\delta_H(C)|^2$. Let $\intpairs'=\bigcup_{C\in \cset}\intpairs'_C$. Then:
	
	\[ |\intpairs'|\leq \sum_{C\in \cset}|\intpairs'_C|\leq  4\sum_{C\in \cset}|\delta_H(C)|^2. \]
	
	From Equation \ref{eq: sum of squares} (see \Cref{step 2 summary}), $
	\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}$, so we get that:
	
	\begin{equation}\label{eq: bounding num of intersection pairs}
	|\intpairs'|<\frac{4(\tk\talpha\alpha')^2}{c_1\log^{20}n},
	\end{equation} 
	
	where $c_1$ is an arbitrary large enough constant.
	
	In the remainder of the proof, we assume for contradiction that $|\bset_2|\geq (\lambda')^2/32$, and we will show that $|\intpairs'|\geq \frac{4(\tk\talpha\alpha')^2}{c_1\log^{20}n}$ must hold, contradicting Equation \ref{eq: bounding num of intersection pairs}.
	

Consider a type-2 bad cell $\cell_{i,j}\in \bset_2$. Recall that every path in $\pset^{i,j}\cup \rset^{i,j}$ contains at least one outer edge, and at most $\psi/32$ such paths contain a type-1 bad edge. Since, from \Cref{obs: paths for cells}, $|\pset^{i,j}|= \ceil{7\psi/8}$, 
there is a collection $\Sigma\subseteq \pset^{i,j}$ of at least  $3\psi/4$ paths $P$, such that all edges on $P$ are either inner edges, or type-2 outer edges. Therefore, if $P\in \Sigma$ is any such path, then there is some cluster $C\in \cset$ with $V(P)\subseteq X(C)$. Recall that, from \Cref{obs: paths for cells}, each path $P\in \Sigma$ intersects at least $\frac{13\psi}{16}$ paths of $\rset^{i,j}$. Clearly, if a path $R\in \rset^{i,j}$ intersects a path $P\in \Sigma$, then $(P,R)\in \intpairs'$. Therefore, intersections between pairs of paths in $\pset^{i,j}\times \rset^{i,j}$ contribute at least $\frac{13\psi}{16}\cdot \frac{3\psi}{4}\geq \frac{\psi^2}{2}$ pairs to set $\intpairs'$.
Therfore, if we denote by $\intpairs'_{i,j}$ the collection of all pairs $(P,R)\in \intpairs'$, where a subpath $\sigma$ of $P$ lies in $\pset^{i,j}$,  and a subpath $\sigma'$ of $R$ lies in $\pset^{i,j}$, and $\sigma,\sigma'$ contain a vertex $v\in X(C)$, for some cluster $C\in \cset$, then, from the above discussion, $|\intpairs'_{i,j}|\geq \frac{\psi^2}{2}$. We claim that for every pair $(P,R)\in \intpairs'$ of paths, there is at most one pair of indices $0\leq i,j\leq \lambda'+1$, such that $(P,R)\in \intpairs_{i,j}'$. Indeed, assume that $P\in \uset_i$ and $R\in \uset'_j$. For a pair $0\leq i',j'\leq \lambda'+1$ of indices, $\pset^{i',j'}$ contains a subpath of $P$ iff $i'=i$, and $\rset^{i',j'}$ contains a subpath of $R$ iff $j'=j$. So the only pair $(i',j')$ of indices for which $(P,R) \in \intpairs'_{i',j'}$ may hold is $(i,j)$. Overall, we get that $|\intpairs'|\geq |\bset_2|\cdot \psi^2/2$. Assuming that $|\bset_2|\geq (\lambda')^2/32$, since $\lambda'=\floor{(\lambda-1)/2}\geq \lambda/4$, we get that $|\intpairs'|\geq \frac{\lambda^2\psi^2}{32}$. 



	Recall that $\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$, and $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$. 
	We conclude that:
	
	
	\[|\intpairs'|\geq \frac{(\alpha^*)^2\tk^2}{2^{17}}\geq \Omega\left( \frac{(\alpha\alpha'\tk)^2}{\log^8n} \right ).  \] 
	
	Since we can choose $c_1$ to be a sufficiently large constant, this contradicts Equation \ref{eq: bounding num of intersection pairs}.
\end{proof}	
\end{proof}



\mynote{looks like there is no need to rotate. can define type-1 bad cell w.r.t. horizontal paths only. Same for good/bad (horizontally good is good enough). Will need to update.}


\iffalse
Good cell part:

will only look at cells in top left quadrant. May need to swap horizontal and vertical. Not completely symmetric b/c of bottom-up / left-right direction of paths (the segment are defined w.r.t. this direction).

A horizontal path $P$ is good for cell $(i,j)$ iff its segment contains no outer edges, so it is contained in $\Pi(v)$ of some vertex $v$. A cell is good if it has at least one good path. This means that all vertical paths in the cell also visit $\Pi(v)$ in the cell. We want to prove that at least $0.8$-fraction of the cells are good.

In a bad cell, partition paths into two types: type-1 path for cell $(i,j)$ contains an outer edge that is not contained in any cluster (type-1 outer edge), otherwise type-2. A bad cell is type-1 if at least 0.1-frac of the horizontal paths are type-1 for the cell, and type-2 otherwise.

If we have many type-1 cells, then we have about $\psi\lambda^2=\alpha^*\tk\lambda$ type-1 outer edges, contradicting Obs. 6.9.

(need to do same analysis with horizontal paths, there is no choice).

So at the end we'll have a constant fraction of cells that are type-2 cells for both vertical and horizontal paths. In each such cell we'll have about $\psi^2$ pairs of paths meet at vertices that are inner to clusters. So overall, we have $(\lambda^2\psi^2)$ pairs of paths meeting at vertices that are inner to clusters. but for a cluster $C$, we have at most $|\delta(C)|$ paths entering it, so at most $|\delta(C)|^2$ pairs of paths can meet in inner vertices of $C$. So total number of such intersections is at most $\sum_{C\in \cset}|\delta(C)|^2$, which should hopefully be less than $(\lambda\psi)^2=(\alpha^*)^2\tk^2$. We currently only have $\sum_C|\delta(C)|^2<(\tk\talpha\alpha')^2/\log^{20}n$. $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, so looks OK.



\subsection{Plan for the rest of the proof}
\begin{itemize}
	\item select 1 path in $z$, where for example $z=\eta$, though can also use $\eta^2$. Will get a grid skeleton of size $z\times z$. 
	
	\item before that, throw away all paths that have more than $\eta/\alpha$ outer edges on them. Most paths will stay.
	
	\item now if we look at a vertical path, it has few outer edges, so for most cells it goes through it does not use an outer edge. Which means that all horizontal paths going through that cell meet in a single vertex (or go through a single cluster). Call such a cell good.
	
	\item at least half the cells are good. In a type-1 good cell all horizontal paths go through a single regular vertex. In a type-2 good cell they all go through 1 cluster. The hope is that there are few type-2 good cells.
	
	\item why: we have about $z^2$ good cells. Inside all good cells there are about $k^2/z^2$ inner edges (can make a cell good if both all horizontal paths meet at some vertex, and all vertical paths meet at some vertex, and then it should be the same vertex). The hope is that the clusters can only contribute $\sum_C|\delta(C)|^2$ vertices to the grid. This is because, if we look at a cluster $C$, the total number of vertical/horizontal paths entering $C$ is at most $\delta(C)$. Even if all pairs have their intersections inside this cluster, it can't contribute more than $|\delta(C)|^2$ such intersecting pairs. 
\end{itemize}
\fi









\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Leftovers%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
contracted graph $\hat H=H_{|\cset}$. Let $U=\set{v(C)\mid C\in \cset}$ be the set of super-node vertices of $\hH$, and let $U'$ be the set of all remaining vertices. We define a rotation system $\hat \Sigma$ for graph $\hat H$  as follows: for a super-node $v(C)\in U$, we let $\oset_{v(C)}$ be an arbitrary ordering of the edges incident to $v(C)$, and for a regular vertex $u\in U'$, we let $\oset_u$ be identical to the ordering in the rotation system $\Sigma$ in instance $I$. Recall that, from \Cref{lem: crossings in contr graph},  there is a drawing $\phi$ of $\hH$,  containing at most $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)$ crossings, such that for every regular vertex $u\in U'$, the ordering of the edges of $\delta_{\hH}(u)$ as they enter $u$ in $\phi$ is consistent with $\oset_u\in \Sigma$. We can use this drawing in order to define a solution $\phi'$ to instance $\hat I=(\hH,\hat \Sigma)$ of the \cnwrs problem, by reordering the edges entering every super-node $v(C)$ as needed. This can be done so that $\cro(\phi')\leq \cro(\phi)+\sum_{C\in \cset'}|\delta_H(C)|^2\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$. Therefore, $\optcrors(\hat I)\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$.


We are now ready to define graph $\hH^+$. In order to do so, we start with graph $\hH$, and process every vertex $u\in V(\hH)\setminus T$ (that may be a regular vertex or a super-node one-by-one). Consider any such vertex $u$, and let $e_1,\ldots,e_{d(u)}$ be the edges incident to $u$ in $\hH$, indexed according to their ordering in $\oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ vrid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. We replace vertex $u$ with the grid $\Pi(u)$, and, for all $1\leq i\leq d(u)$, if $e_i=(u',u)$, then we replace $e_i$ with a new edge $e'_i=(u',s_i(u))$. Once every vertex of $V(\hH)\setminus T$ is processed, we obtain the final graph $\hH^+$. For every vertex $u$, we clall the edges of the grid $\Pi(u)$ \emph{inner edges}. We call all edges of $E(\hH^+)$ that are not inner edges \emph{outer edges}. Notice that there is a $1$-to-$1$ correspondence between the outer edges and the edges of graph $\hat H$. The following observation is immediate.

\begin{observation}\label{obs: expanded contracted graph}
	The set $T$ of terminals is $(\alpha\alpha')$-well-linked in $\hH^+$, and there is a drawing $\phi''$ of graph $\hH^+$ with at most  $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$ crossings, such that the inner edges do not participate in any crossings in $\phi''$.
\end{observation}
\fi
 








==> guiding-paths-backup3.tex <==
\newpage
\section{Constructing Guiding Paths - Proof of \Cref{thm: find guiding paths}}
\label{sec: guiding paths}

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------



%The remainder of this section is dedicated to the proof of \Cref{thm: find guiding paths}. 
%For convenience, we define a new instance $I'=(H,\Sigma')$ of the \cnwrs problem, as follows. We start from graph $G$, and subdivide every edge $e\in \delta_G(C)$ with a vertex $t(e)$. Denote the resulting graph by $G'$, and let $T=\set{t(e)\mid e\in \delta_G(C)}$. Note that the solution $\phi^*$ to instance $I$ naturally defines a solution  $\phi'$ to the instance defined by graph $G'$ and rotation system $\Sigma$ (the newly added vertices $t$ each have degree $2$ so the ordering $\oset_t$ of their incident edges can be defined arbitrarily.) For subgraphs $X\subseteq G'$, we define $\cro(X)$ with respect to this drawing $\phi'$.

%We then let $H$ be the sub-graph of the resulting graph induced by $C\cup T$, and we let $\Sigma'$ be the corresponding rotation system that is consistent with the original rotation system $\Sigma$ for $G$. Note that, if $u$ is any vertex of $V(H)\setminus T$, and $\qset=\set{Q(t)\mid t\in T}$ is a collection of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, then set $\qset$ naturally defines a set $\qset'$ of paths in graph $G'$, routing the edges of $\delta_{G'}(H)$ to $u$ inside $H$, and so we can define $\cost_H(\qset')$ as usual, with respect to the drawing $\phi'$ of $G'$. Set $\qset$ of paths also naturally defines a set $\qset''$ of paths in graph $G$, routing the edges of $\delta_G(C)$ to $u$ inside $C$, and moreover $\cost_C(\qset)$ in graph $G$ is bounded by $\cost_H(\qset')$ in graph $G'$.

%Therefore, from now on our goal is to compute a vertex $u\in V(H)\setminus T$, and a collection $\qset=\set{Q(t)\mid t\in T}$ of paths in $H$, where each path $Q(t)$ connects $t$ to $u$, so that the cost $\expect{\cost_{H}(\qset)}\leq O(\optcrors(I')\cdot 2^{O((\log^{1/4} m))})$.

For conveninence, we denote the contracted graph $H_{|\cset}$ by $\hH$,  and we denote $|E(\hH)|=\hm$. From the statement of \Cref{thm: find guiding paths}, $k\geq \hm/\eta$. Observe that, from \Cref{clm: contracted_graph_well_linkedness}, the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$. We will assume in the remainder of the proof that $\log n$ is greater than some large enough constant $c'_0$ (whose value we can set later). If this is not the case, then, $n$, and therefore $k$, is bounded by a constant $2^{c_0'}$. We can then use an arbitrary spanning tree $\tau$ of the graph $H$, 
rooted at an arbitrary vertex $y$, in order to define a collection $\qset$ of paths routing all terminals of $T$ to $y$, where for each terminal $t\in T$, the corresponding path $Q_t\in \qset$ is the unique path connecting $t$ to $y$ in the tree $\tau$. Since $|T|$ is bounded by a constant, for every edge $e\in E(H)$, $\cong_H(\qset,e)\leq O(1)$. We then return a distribution $\dset$ consisting of a single pair $(y,\qset)$, that has probability value $1$. Therefore, we assume from now on that $\log n>c_0'$ for some large enough constant $c_0'$ whose value we set later.


We start with some intuition. Assume first that graph $H$ contains a grid (or a grid minor) of size $(\Omega(k\alpha\alpha'/\poly\log n)\times \Omega(k\alpha \alpha'/\poly\log n))$, and a collection $\pset$ of paths connecting every terminal to a distinct vertex on the first row of the grid, such that the paths in $\pset$ cause a low edge-congestion. For this special case, the algorithm of \cite{Tasos-comm}  (see also Lemma D.10 in the full version of \cite{chuzhoy2011algorithm}) provides the distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$ with the required properties. Moreover, if $H$ is  a bounded-degree planar graph, with a set $T$ of terminals that is $(\alpha\alpha')$-well-linked, 
then there is an efficient algorithm to compute such a grid minor, together with the required collection $\pset$ of paths. If $H$ is planar but no longer bounded-degree, we can still compute a grid-like structure in it, and apply the same arguments as in \cite{Tasos-comm} in order to compute the desired distribution $\dset$. The difficulty in our case is that the graph $H$ may be far from being planar, and, even though, from the Excluded Grid theorem of Robertson and Seymour \cite{robertson1986graph,chuzhoy2019towards}, %\mynote{please add references to the original thm proof and our new proofs}
it must contain a large grid-like structure, without having a drawing of $H$ in the plane with a small number of crossing, we do not know how to compute such a structure.

The proof of \Cref{thm: find guiding paths} consists of five steps. In the first step, we will  either establish that $\optcrors(I)$ is sufficiently large (so the algorithm can return FAIL), or compute a subgraph $\hH'\subseteq \hH$, and a partition $(X,Y)$ of $V(\hH')$, such that each of the clusters $\hH'[X],\hH'[Y]$ has the $\hat \alpha$-bandwidth property, for $\hat \alpha=\Omega(\alpha/\log^4n)$, together with a large collection of edge-disjoint paths routing the terminals to the edges of $E_{\hH'}(X,Y)$ in graph $\hH'$. Intuitively, we will view from this point onward the edges of $E_{\hH'}(X,Y)$ as a new set of terminals, that we denote by $\tilde T$ (more precisely, we subdivide each edge of $E_{\hH'}(X,Y)$ with a new vertex that becomes a new terminal). We show that it is sufficient to prove an analogue of \Cref{thm: find guiding paths} for this new set $\tT$ of terminals. The clusters $\hH'[X],\hH'[Y]$ of graph $\hH'$ naturally define a partition $(H_1,H_2)$ of the graph $H$ into two disjoint clusters. In the second step, we either establish that $\optcrors(I)$ is suffciently large 
(so the algorithm can return FAIL), or
compute some vertex $x$ of $H_1$, and a collection $\pset$ of paths in graph $H_1$, routing the terminals of $\tilde T$ to $x$, such that the paths in $\pset$ cause a relatively low edge-congestion.
We exploit this set $\pset$ of paths in order to define an ordering of the terminals in $\tilde T$, which is in turn exploited in the third step in order to compute a ``skeleton'' for the grid-like structure. We compute the grid-like structure itself in the fourth step. In the fifth and the final step, we generalize the arguments from \cite{Tasos-comm}  and  \cite{chuzhoy2011algorithm} in order to obtain the desired distribution $\dset$ over pairs $(\qset,x)\in \Lambda(H,T)$.


Before we proceed, we need to consider four simple special cases. In the first case,  $\sum_{C\in \cset}|\delta(C)|^2$ is large. In the second case, we can route a large subset of the terminals to a single vertex of $V(\hat H)\cap V(H)$ in the graph $\hat H$ via edge-disjont paths. The third case is when $\optcrors(H,\Sigma)=0$, and the fourth special case is when $k< \eta^6$.

\paragraph{Special  Case 1: $\sum_{C\in \cset}|\delta(C)|^2$ is large.}
We consider the case where $\sum_{C\in \cset}|\delta(C)|^2\geq \frac{(k \alpha^4 \alpha')^2}{c_0\log^{50}n}$, where $c_0$ is the constant from the statement of \Cref{thm: find guiding paths}.
In this case, since we are guaranteed that, for every cluster $C\in \cset$, $\optcrors(C,\Sigma_C)\geq |\delta(C)|^2/\eta'$, we get that:
\[\optcrors(I)\geq \sum_{C\in \cset}\optcrors(C,\Sigma_C)\geq \sum_{C\in \cset}\frac{|\delta(C)|^2}{\eta'}\geq \frac{(k \alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}.\]
Therefore, if $\sum_{C\in \cset}|\delta(C)|^2\geq \frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}$, the algorithm returns FAIL and terminates. We assume from now on that:
\begin{equation}\label{eq: boundaries squared sum bound}
\sum_{C\in \cset}|\delta(C)|^2<\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}.
\end{equation}



\paragraph{Special Case 2: Routing of terminals to a single vertex.}
The second special case happens if there exists a collection $\pset_0$ of at least $\frac{k\alpha\alpha'}{1024\cCMG^3\log^6k}$ edge-disjoint paths in graph $\hH$ routing some subset $T_0\subseteq T$ of terminals to some vertex $x$ (here $\cCMG$ is the constant from \Cref{claim: embed expander}).
 
Note that, if Special Case 1 did not happen, and $c_0$ is a large enough constant, then $x$ may not be a supernode. Indeed, assume that $x=v_C$ for some cluster $C\in \cset$. Then:
\[|\delta(C)|^2\geq \Omega\left(\frac{(k\alpha \alpha')^2}{\log^{12}k}\right )\geq \frac{(k \alpha^4 \alpha')^2}{c_0\log^{50}n},\] 
which is, assuming that $c_0$ is a large enough constant, a contradiction. Therefore, we can assume that $x$ is not a supernode.
From \Cref{claim: routing in contracted graph}, since the clusters in $\cset$ have the $\alpha'$-bandwidth property, there is a collection $\pset'_0$ of paths in graph $H$, routing the vertices of $T_0$ to $x$, with edge-congestion at most $\ceil{1/\alpha'}\leq 2/\alpha'$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in graph $H$, from \Cref{lem: routing path extension}, there is a set $\qset$ of paths in graph $H$, routing the vertices of $T$ to $x$ with congestion at most:
\[\ceil{\frac{|T|}{|T_0|}}\left(\frac 2{\alpha'}+\ceil{\frac 1{\alpha\alpha'}}\right )\leq O\left (  \frac{\log^6k}{(\alpha\alpha')^2} \right).\]



\iffalse
Denote $z=|\pset_0|\geq \frac{k\alpha\alpha'}{1024\cCMG^2\log^4k}$.
We compute a single set $\qset$ of paths routing the set $T$ of terminals to $x$, with congestion $O(\log^4k/(\alpha \alpha')^2)$, as follows. We partition the set $T\setminus T_0$ of terminals into $q=\ceil{k/z}\leq O(\log^4k/(\alpha\alpha'))$ subsets, each of which contains at most $z$ vertices. 
Consider now some index $1\leq i\leq q$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\pset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\pset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\pset_i'$. By concatenating the paths in $\pset_i'$ with paths in $\pset_0$, we obtain a collection $\pset_i$ of paths in graph $H$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\alpha\alpha'))$. 


Let $\qset=\bigcup_{i=0}^q\pset_i$ be the resulting set of paths. Observe that set $\qset$ contains $k$ paths, routing the terminals in $T$ to the vertex $x$ in graph $H$, with $\cong_H(\qset)\leq O(q/(\alpha\alpha'))\leq O(\log^4k/(\alpha\alpha')^2)$.
\fi
Note that a set $\qset$ of paths with the above properties can be computed efficiently via standard maximum flow algorithm.
We return a distribution $\dset$ consisting of a single pair $(\qset,x)$ with probability value $1$, and terminate the algorithm. 
 Clearly, for every edge $e\in E(H)$, $\expect{(\cong(\qset,e))^2}\leq  O\left (\frac{\log^{32}n}{\alpha^{12}(\alpha')^8}\right )$.
 


\paragraph{Special Case 3: $\optcrors(H,\Sigma)=0$.}
Recall that we can efficiently check whether $\optcrors(H,\Sigma)=0$, using the algorithm from \Cref{thm: crwrs_planar}. Assume now that $\optcrors(H,\Sigma)=0$. We construct a graph $\tilde H$ from $H$, as follows. 

We start with $\tilde H=\emptyset$, and then process every vertex $u\in V(H)\setminus T$ one by one. We now describe an iteration when a vertex $u\in V(H)\setminus T$ is processed. We denote by $d(u)$ the degree of the vertex $u$ in graph $H$.  Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that are incident to $u$ in $H$, indexed according to their ordering in $ \oset_u\in  \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$ indexed in their natural left-to-right order. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $\tilde H$.
Once every vertex $u\in V(H)\setminus T$ is processed, we add 
the vertices of $T$ to the graph $\tilde H$. Recall that every terminal $t\in T$ has degree $1$ in $H$. We denote the unique edge $e_t$ incident to $t$ by $e_1(t)$, and we denote $s_1(t)=t$.
Next, we add another collection of to graph $\tilde H$, as follows. Consider any edge $e=(u,v)\in E(H)$. Assume that $e$ is the $i$th edge of $u$ and the $j$th edge of $v$, that is, $e=e_i(u)=e_j(v)$. Then we add an edge $e'=(s_i(u),s_j(v))$ to graph $\tilde H$, and we view this edge as the \emph{copy of the edge $e\in E(H)$}. From \Cref{clm: contracted_graph_well_linkedness}, the set $T$ of terminals is $(\alpha\cdot \alpha')$-well-linked in $H$. Notice that we can view the graph $H$ as the contracted graph of $\tilde H$ with respect to the set of clusters $\set{\Pi(v)\mid v\in V(H)\setminus T}$. Since each cluster in the set has the $1$-bandwidth property, from \Cref{clm: contracted_graph_well_linkedness}, set $T$ of terminals is $(\alpha\alpha')$-well-linked in $\tilde H$. Consider now the optimal solution $\phi^*$ to instance $(H,\Sigma)$ of \CNwRS, so drawing $\phi^*$ contains no crossings. It is easy to extend this drawing to a planar drawing of graph $\tilde H$: for every vertex $u\in V(H)\setminus T$, we consider a small disc $\eta(u)$ in $\phi^*$ that contains $u$ in its interior. We then delete the image of $u$ and segments of images of its incident edges lying in $\eta(u)$, and instead place the image of the grid $\Pi(u)$, drawn using its natural layout, so that the images of the vertices $s_1(u),\ldots,s_{d(u)}(u)$ appear on the boundary of the disc. To summarize, graph $\tilde H$ that we have defined is planar, it has maximum vertex degree at most $4$, and the set $T$ of terminals is $(\alpha\alpha')$-well-linked in $\tilde H$. We will use the following theorem from \cite{chuzhoy2019towards}.

\mynote{insert lemma here, finish constructing the distribution}.

\paragraph{Special Case 4: $k< \eta^6$, but $\optcrors(H,\Sigma)>0$.}
Assume that $k<\eta^6$. Note that $\frac{(k\alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}\leq \frac{\eta^{12}}{\eta'}<1$ in this case (as, from the statemnt of \Cref{thm: find guiding paths}, $\eta'>\eta^{13}$.) 
Since we have assumed that $\optcrors(H,\Sigma)>0$, we get that $\optcrors(H,\Sigma)\geq 1>\frac{(k\alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}$. We then simply return FAIL and terminate the algorithm.

In the remainder of the algorithm, we assume that neither of the four special cases happened. We now describe each step of the algorithm in detail.




%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 1: Splitting the Contracted Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


In this step, we split the contracted graph $\hH$, using the algorithm  summarized in the following theorem.

\begin{theorem}\label{thm: splitting}
There is an efficient randomized algorithm that returns FAIL with probability at most $1/\poly(k)$, and, if it does not return FAIL, then it  computes a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that:
\begin{itemize}
\item clusters $\hH'[X]$ and $\hH'[Y]$ both have the $\halpha'$-bandwidth property in $\hH'$, for $\halpha'=\Omega(\alpha/\log^4n)$; and
\item there is a set $\rset$ of $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
\end{itemize}
\end{theorem}


\begin{proof}
We start by applying the algorithm from \Cref{claim: embed expander} to graph $\hH$ and the set $T$ of terminals, to obtain a graph $W$ with $V(W)=T$ and maximum vertex degree at most $\cCMG\log^2k$, and an embedding $\hpset$ of $W$ into $\hH$ with congestion at most $(\cCMG\log^2k)/\alpha$. Let $\hat\event$ be the bad event that $W$ is not a $1/4$-expander. Then $\prob{\hat \event}\leq 1/\poly(k)$.
%Let $\hH'$ be the graph that is obtained from $\hH$ by deleting all edges and vertices except those participating in the paths in $\hpset$. Equivalently, graph $\hH'$ is obtained from the union of all paths in $\hpset$. 
Define graph $\hH'$ as the union of all paths in $\hat{\pset}$.
We need the following observation.

\begin{observation}\label{obs: expansion and degree}
	If event $\hat \event$ did not happen, then the set $T$ of vertices is $\halpha$-well-linked in $\hH'$, for $\halpha=\frac{\alpha}{4\cCMG\log^2k}$, and the maximum vertex degree in $\hH'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}$.
\end{observation}
\begin{proof}
	Assume that Event $\hat \event$ did not happen. We first prove that the set $T$ of terminals is $\halpha$-well-linked in $\hH$. Consider any paritition $(A,B)$ of vertices of $\hH'$, and denote $T_A=T\cap A$, $T_B=T\cap B$. Assume w.l.o.g. that $|T_A|\leq |T_B|$. Then it is sufficient to show that $|E_{\hH'}(A,B)|\geq \halpha\cdot |T_A|$.
	
	Consider the partition $(T_A,T_B)$ of the vertices of $W$, and denote $E'=E_{W}(T_A,T_B)$. Since $W$ is a $1/4$-expander, $|E'|\geq |T_A|/4$ must hold. Consider now the set $\hat \rset\subseteq \hpset$ of paths containing the embeddings $P(e)$ of every edge $e\in E'$. Each path $R\in \hat \rset$ connects a vertex of $T_A$ to a vertex of $T_B$, so it must contain an edge of $|E_{\hH}(A,B)|$. Since $|\hat\rset|\geq |T_A|/4$, and the paths in $\hpset$ cause edge-congestion at most $(\cCMG\log^2k)/\alpha$, we get that $|E_{\hH}(A,B)|\geq \alpha\cdot |T_A|/(4\cCMG\log^2k)\geq \halpha |T_A|$.
	
	Assume now that maximum vertex degree in $\hH'$ is greater than $d$, and let $x$ be a vertex whose degree is at least $d$. Let $\hat\qset\subseteq \hat\pset$ be the set of all paths containing the vertex $x$.
Consider any such path $Q\in \hat\qset$. The endpoints of this path are two distinct terminals $t,t'\in T$. We let $Q'\subseteq Q$ be the sub-path of $Q$ between the terminal $t$ and the vertex $x$, and we let $\qset'=\set{Q'\mid Q\in \hat\qset}$.

Recall that every vertex in $W$ has degree at most $\cCMG\log^2k$, and so a terminal in $T$ may be an endpoint of at most $\cCMG\log^2k$ paths in $\hpset$. Therefore, there is a subset $\qset''\subseteq \qset'$ of at least $d/(\cCMG\log^2k)$ paths in $\hH'$, each of which originates at a distinct terminal.
Since paths in $\qset''$ cause congestion at most $(\cCMG\log^2k)/\alpha$, from \Cref{claim: remove congestion}, there is a collection $\qset'''$ of edge-disjoint paths in graph $\hH'$, routing a subset of terminals to $x$ with:
$$|\qset'''|\geq |\qset''|\cdot \frac{\alpha}{\cCMG\log^2k}\geq \frac{d\alpha}{\cCMG^2\log^4k}\geq\frac{\alpha^2k}{512\cCMG^3\log^6k},$$
\iffalse
But then, from \Cref{claim: routing in contracted graph}, there is a collection $\qset'''$ of edge-disjoint paths in graph $H$, routing a subset of terminals to $x$ of cardinality at least:

\[\frac{\alpha'|\qset''|} 2\geq \frac{\alpha' d}{2\cCMG\log^2k}\geq  \frac{\alpha \alpha' k}{1024\cCMG\log^4k},\]
\fi
contradicting the fact that Special Case 2 did not happen.
\end{proof}

Next, we use the following lemma to compute the required sets $X$, $Y$ of vertices. The proof follows immediately from techniques that were introduced in \cite{chuzhoy2012routing} and then refined in \cite{chuzhoy2012polylogarithmic,chekuri2016polynomial,chuzhoy2016improved}. Unfortunately, all these proofs assumed that the input graph has a bounded max vertex-degree, and additionally the proofs are somewhat more involved than the proof that we need here (this is because these proofs could only afford a $\poly\log k$ loss in the cardinality of the path set $\rset$ relatively to $|T|$, while we can afford a $\poly\log n$ loss). Therefore, we provide a complete proof of the lemma in Section \ref{sec: splitting} of the Appendix for completeness.


\begin{lemma}\label{lem: splitting}
	There is an efficient algorithm that, given as input an $n$-vertex graph $G$, and a subset $T$ of $k$ vertices of $G$ called terminals, together with a parameter $0<\talpha<1$, such that the maximum vertex degree in $G$ is at most $\talpha k/64$, and every vertex of $T$ has degree $1$ in $G$, either returns FAIL, or computes a partition $(X,Y)$ of $V(G)$, such that:
	\begin{itemize}
		\item each of the clusters $G[X]$, $G[Y]$ has the $\talpha'$-bandwidth property, for $\talpha'=\Omega(\talpha/\log^2n)$; and
		\item there is a set $\rset$ of at least $\Omega(\talpha^3k/\log^2n)$ edge-disjoint paths in graph $G$, routing a subset of terminals to edges of $E_G(X,Y)$.
	\end{itemize}
Moreover, if the vertex set $T$ is $\talpha$-well-linked in $G$, then the algorithm never returns FAIL.
\end{lemma}

We apply the algorithm from \Cref{lem: splitting} to graph $\hH'$, the set $T$ of terminals, and parameter $\talpha=\halpha=\frac{\alpha}{4\cCMG\log^2k}$. Recall that we are guaranteed that the maximum vertex-degree in graph $\hat H'$ is at most $d=\frac{\alpha k}{512\cCMG\log^2k}\leq \frac{\talpha k}{64}$.
Note that the algorithm from  \Cref{lem: splitting} may only return FAIL if the set $T$ of terminals is not $\talpha$-well-linked in $\hH'$, which, from \Cref{obs: expansion and degree}, may only happen if event $\hat \event$ happened, which in turn may only happen with probability $1/\poly(k)$. If the algorithm from \Cref{lem: splitting} returned FAIL, then we terminate the algorithm and return FAIL as well. Therefore, we assume from now on that the algorithm from  \Cref{lem: splitting} did not return FAIL.
%
%
\iffalse restart the algorithm that we have described so far from scratch. We do so at most $1/\poly\log n$ times, and if, in every iteration, the algorithm from \Cref{lem: splitting} returns FAIL, then we return FAIL as the outcome of the algorithm for \Cref{thm: splitting}. Clearly, this may only happen with probability at most $1/\poly(n)$. Therefore, we assume that in one of the iterations, the algorithm from \Cref{lem: splitting} did not return FAIL. From now on we consider the outcome of that iteration.\fi
%
 Let $(X,Y)$ be the partition of $V(\hH')$ that the algorithm returns. We are then guaranteed that each of the clusters $\hH'[X],\hH'[Y]$ has the $\talpha'$-bandwidth property, where $\talpha'=\Theta(\talpha/\log^2n)=\Theta(\alpha/\log^4n)$. The algorithm also ensures that there is a collection $\rset$ of edge-disjoint paths in $\hH'$, routing a subset of the terminals to edges of $E_{\hH'}(X,Y)$, with $|\rset|\geq \Omega(\talpha^3k/\log^2n)=\Omega(\alpha^3k/\log^8n)$.
This completes the proof of \Cref{thm: splitting}.
\end{proof}


If the algorithm from \Cref{thm: splitting} returned FAIL (which may only happen with probability at most $1/\poly(k)$), then we terminate the algorithm and return FAIL as well. Therefore, we assume from now on that the algorithm from \Cref{thm: splitting} returned a subgraph $\hH'\subseteq \hH$ and a partition $(X,Y)$ of $V(\hH')$ such that each of the clusters $\hH'[X]$ and $\hH'[Y]$ has the $\halpha'$-bandwidth property, for $\halpha'=\Theta(\alpha/\log^4n)$, and
 there is a set $\rset$ of $\Omega(\alpha^3k/\log^8n)$ edge-disjoint paths in graph $\hH'$, routing a subset of terminals to edges of $E_{\hH'}(X,Y)$.
Notice that we can compute the path set $\rset$ with the above properties efficiently, using standard maximum flow algorithms. We assume w.l.o.g. that edges of $E_{\hH}(X,Y)$ do not serve as inner edges on paths in $\rset$.
Let $E'\subseteq E_{\hH'}(X,Y)$ be the subset of edges containing the last edge on every path in $\rset$, so, by reversing the direction of the paths in $\rset$, we can view the set $\rset$ of paths as routing the edges of $E'$ to the terminals.
In the remainder of this step, we will slightly modify the graphs $H$ and $\hat H$, and we will continue working with the modified graphs only in the following steps.

Let $\hH''\subseteq\hH'$ be the graph obtained from $\hH'$ by first deleting all edges of $E_{\hH'}(X,Y)\setminus E'$ from it, and then subdividing every edge $e\in E'$ with a vertex $t_e$. We denote $\tilde T=\set{t_e\mid e\in E'}$, and we refer to vertices of $\tilde T$ as \emph{pseudo-terminals}. Recall that $|\tilde T|=|\rset|=\Omega(\alpha^3k/\log^8n)$, and there is a set $\rset'$ of edge-disjoint paths in the resulting graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$.
We define $\hH_1=\hH''[X\cup \tilde T]$, the subgraph of $\hH''$ induced by the set $X\cup \tilde T$ of vertices, and we define $\hH_2=\hH''[Y\cup \tilde T]$ similarly. From the $\halpha'$-bandwidth property of the clusters $\hH'[X]$ and $\hH'[Y]$, we are guaranteed that the vertices of $\tilde T$ are $ \halpha'$-well-linked in both $\hH_1$ and in $\hH_2$, where $\halpha'= \Theta(\alpha/\log^4n)$. Let $\cset'\subseteq \cset$ be the subset of all clusters $C$ whose corresponding supernode $v_C$ lies in graph $\hH''$.

For convenience, we also subdivide, in graph $H$, every edge $e\in E'$, with the vertex $t_e$, so graph $\hH''$ can be now viewed as a subgraph of the contracted graph $H_{|\cset}$.

Next, we let $H'\subseteq H$ be the subgraph of $H$ that corresponds to the graph $\hH''$. Put in other words, graph $H'$ is obtained from $\hH''$ by replacing every supernode $v_C$ with the corresponding cluster $C\in \cset'$. Equivalently, we can obtain graph $H'$ from $H$, by deleting every edge of $E(\hH)\setminus E(\hH'')$ and every regular (non-supernode) vertex of $V(\hH)\setminus V(\hH'')$. Additionally, for every cluster $C\in \cset\setminus \cset'$, we delete all edges and vertices of $C$ from $H'$. We also define a rotation system $\Sigma'$ for graph $H'$, which is identical to $\Sigma$ (vertices $t_e\in \tilde T$ all have degree $2$, so their corresponding ordering $\oset_{t_e}$ of incident edges can be set arbitrarily). 


We partition the set $\cset'$ of clusters into two subsets: set $\cset_X$ contains all clusters $C\in \cset'$ with $v_C\in X$, and set $\cset_Y$ contains all clusters $C\in \cset'$ with $v_C\in Y$. We can similarly define the graphs $H_1,H_2\subseteq H'$, that correspond to the contracted graphs $\hat H_1$ and $\hat H_2$, respectively: let $X'$ contain all vertices $x\in V(H')$, such that either $x\in C$ for some cluster $C\in \cset_X$, or $x$ is a regular vertex of $\hat H''$ lying in $X$. Similarly, we let $Y'$ contain all vertices $y\in V(H)$, such that either $y\in C$ for some cluster $C\in \cset_Y$, or $y$ is a regular vertex of $\hat H''$ lying in $Y$. We then let $H_1=H'[X\cup \tilde T]$, and $H_2=H'[Y\cup \tilde T]$.

The following observation, summarizing some properties of graph $H'$, is immediate.
\begin{observation}\label{obs: properties of new graph}
Graph $H'$ satisties the following properties:
	\begin{itemize}
		\item $\optcrors(H',\Sigma')\leq \optcrors (H,\Sigma)$;
		\item $\hat H''=H'_{|\cset'}$; 
		\item $|E(\hat H'')|\leq 2|E(\hat H)|\leq 2\eta k\leq O(|\tilde T|\eta \log^8n/\alpha^3)$; and
		\item graph $\hat H_1$ is a contracted graph of $H_1$ with respect to  $\cset_X$, and graph $H_2$ is a contracted graph of $H_2$ with respect to $\cset_Y$. In other words, $\hat H_1=(H_1)_{|\cset_X}$, and $\hat H_2=(H_2)_{|\cset_Y}$.
	\end{itemize}
\end{observation}
For the third assertion we have used the fact that $k\geq |E(\hat H)|/\eta$ from the statement of \Cref{thm: find guiding paths}, and $|\tilde T|\geq \Omega(\alpha^3k/\log^8n)$.


Recall that $\Lambda(H',\tilde T)$ denotes the set of all pairs $(\qset,x)$, where $x$ is a vertex of $H'$, and $\qset$ is a collection of paths in graph $H'$, routing the vertices of $\tilde T$ to $x$. In the following observation, we show that, to obtain the desired distribution $\dset$ over pairs in $\Lambda(H,T)$, it is now sufficient to compute a distribution $\dset'$ over pairs $(\qset,x)\in \Lambda(H',\tilde T)$, such that for every edge $e\in E(H')$, $\expect{(\cong_{H'}(\qset,e))^2}$ is low.
\begin{observation}\label{obs: convert distributions}
	There is an efficient algorithm, that, given a distribution $\dset'$ over pairs  $(\qset',x')\in \Lambda(H',\tilde T)$,
	such that for every edge $e'\in E(H')$, $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e'))^2}\leq \beta$ holds,
	 computes a distribution $\dset$ over pairs  $(\qset,x)\in \Lambda(H,T)$, such that for every edge $e\in E(H)$, $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\beta \log^{16}n}{\alpha^8(\alpha')^4}\right )$.
\end{observation}
\begin{proof}
	Recall that $H'\subseteq H$. Consider some pair $(\qset',x')\in \Lambda(H',\tilde T)$, whose probability value in distribution $\dset'$ is $p(\qset',x')>0$. We compute another path set $\qset$ in graph $H$, routing all terminals in $T$ to $x'$, and we will assign to the pair $(\qset,x')\in \Lambda(H,T)$ the same probability value $p(\qset',x')$.

	Recall that there is a set $\rset'$ of edge-disjoint paths in graph $\hH''$, routing the vertices of $\tilde T$ to the vertices of $T$, and moreover, such a path set can be found efficiently via a standard maximum $s$-$t$ flow computation.
	Since $\hat H''=H'_{|\cset'}$, from \Cref{claim: routing in contracted graph}, we can efficiently compute a set $\rset_0$ of edge-disjoint paths in graph $H'$, routing a subset $T_0\subseteq T$ of terminals to $\tT$, with $|\rset_0|\geq \alpha'\cdot |\rset'|/2=\alpha'\cdot |\tilde T|/2=\Omega(\alpha'\alpha^3k/\log^8n)$. By concatenating the paths in $\rset_0$ and the paths in $\qset'$, we obtain a collection $\rset_0'$ of paths in graph $H'$, routing the terminals of $T_0$ to vertex $x'$, such that for every edge $e\in E(H)$, $\cong_H(\rset_0',e)\leq \cong_{H'}(\qset',e)+1$.
Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in graph $H$ (from \Cref{clm: contracted_graph_well_linkedness}), from \Cref{lem: routing path extension}, there exists a collection $\qset$ of paths in graph $H$, routing the terminals in $T$ to vertex $x'$, such that for every edge $e\in E(H)$:
\iffalse
\[
\begin{split}
\cong_{H}(\qset,e)&\leq  \ceil{\frac{|T|}{|T_0|}}\left(\cong_{H}(\rset'_0,e)+\ceil{\frac{1}{\alpha\alpha'}}\right )\\ 
&\leq O\left (\frac{\log^8n}{\alpha'\alpha^3}\right )\cdot \left(\cong_{H'}(\qset',e)+\frac{2}{\alpha\alpha'}\right )
\end{split}
\]
\fi
\[
\cong_{H}(\qset,e)\leq  \ceil{\frac{|T|}{|T_0|}}\left(\cong_{H}(\rset'_0,e)+\ceil{\frac{1}{\alpha\alpha'}}\right )
\leq O\left (\frac{\log^8n}{\alpha'\alpha^3}\right )\cdot \left(\cong_{H'}(\qset',e)+\frac{2}{\alpha\alpha'}\right ).
\]
\iffalse
	
	Let $z=\ceil{k/|T_0|}=O(\log^{8}n/(\alpha^3\alpha')$. Next, we partition the terminals of $T\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $|T_0|$ each. Consider now some index $1\leq i\leq z$. Since the set $T$ of terminals is $(\alpha\alpha')$-well-linked in graph $H$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\rset_i'$ of paths in graph $H$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $\rset'_i$ cause edge-congestion $O(1/(\alpha\alpha'))$, and each vertex of $T_0\cup T_i$ is the endpoint of at most one path in $\rset'_i$. By concatenating the paths in $\rset'_i$ with paths in $\rset_0$, we obtain a collection $\rset_i$ of paths in graph $H$, routing the terminals in $T_i$ to vertices of $\tilde T$, such that every vertex of $\tilde T\cup \rset_0$ is an endpoint of at most one path in $\rset_i$. Let $\rset^*=\bigcup_{i=0}^z\rset_i$ be the resulting set of paths. Observe that set $\rset^*$ contains $k$ paths, each of which connects a distinct terminal of $T$ to a vertex of $\tilde T$, and every vertex of $\tilde T$ serves as an endpoint of at most $z=O(\log^{8}n/(\alpha^3\alpha')$ such paths. The paths of $\rset^*$ cause congestion at most $O(z/\alpha\alpha')\leq O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$.
	
	
 For ever pseudoterminal $\tilde t\in \tilde T$, let $Q'_{\tilde t}\in \qset'$ be the unique path originating at $\tilde t$. For every terminal $t\in T$, let $R'_t\in \rset^*$ be the unique path originating at terminal $t$, and let $\tilde t\in \tilde T$ be the other endpoint of path $R'_t$. We let $Q_t$ be the path obtained by concatenating the paths $R'_t$ and $Q'_{\tilde t}$, so path $Q_t$ connects $t$ to vertex $x'$. We then let $\qset=\set{Q_t\mid t\in T}$. Note that $\qset$ is a set of paths in graph $H$ routing the set $T$ of terminals to vertex $x'$, so $(\qset,x')\in \Lambda(H,T)$. We assign to the pair $(\qset,x')$ probability $p(\qset',x')$. Note that, since every pseudoterminal $\tilde t\in \tilde T$ may seve as an endpoint of at most $O(\log^{8}n/(\alpha^3\alpha')$ paths in $\rset^*$, and since the paths in $\rset^*$ cause edge-congestion at most $O(\log^8k/(\alpha^4(\alpha')^2))$ in graph $H$, for every edge $e\in E(H)$, we get that:
	
	\[\cong_H(\qset,e)\leq O\left(\frac{\cong_{H'}(\qset',e) \cdot \log^8k}{\alpha^3 \alpha'}+\frac{\log^8k}{\alpha^4(\alpha')^2}\right ).  \]
\fi
Therefore, for every pair $(\qset',x')\in \Lambda(H',\tT)$, whose probability value in distribution $\dset'$ is $p(\qset',x')>0$, we have defined a pair $(\qset,x')\in \Lambda(H,T)$, and we have assigned to it the same probability value $p(\qset,x')=p(\qset',x')$. This completes the definition of the distribution $\dset$ over pairs in $\Lambda(H,T)$. From the above discussion,  for every edge $e\in E(H)$,
\[\expect[(\qset,x')\in \dset]{(\cong_{H}(\qset,e))^2}\leq O\left(\frac{\log^{16}k}{\alpha^8(\alpha')^4}\right )\cdot \left (\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}+1\right) \leq O\left(\frac{\beta \log^{16}n}{\alpha^8(\alpha')^4}\right ). \]	
\end{proof}


The following immediate corollary is obtained by plugging in the bounds we need into \Cref{obs: convert distributions}.

\begin{corollary}\label{cor: convert distribution fixed values}
	There is an efficient algorithm, that, given a distribution $\dset'$ over pairs  $(\qset',x')\in \Lambda(H',\tilde T)$,
	such that for every edge $e'\in E(H')$, $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e'))^2}\leq  O\left (\frac{\log^{16}n}{(\alpha\alpha')^4}\right )$ holds, produces a distribution $\dset$ over pairs  $(\qset,x)\in \Lambda(H,T)$, such that for every edge $e\in E(H)$: $$\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq  O\left (\frac{\log^{32}n}{\alpha^{12}(\alpha')^8}\right ).$$
\end{corollary}





Recall that  $\tk\geq \Omega\left(\frac{\alpha^3k}{\log^8n}\right )$, so $\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}\leq O\left( \frac{(\tk\halpha'\alpha')^2}{c_0\log^{20}n}\right )$. We will use a constant $c_1$, that is a large enough constant, whose value will be set later, and we set $c_0=c_1^2$. We can then assume that $\frac{(k\alpha^4 \alpha')^2}{c_0\log^{50}n}\leq  \frac{(\tk\halpha'\alpha')^2}{c_1\log^{20}n}$. In particular, from Equation \ref{eq: boundaries squared sum bound}, we get that $\sum_{C\in \cset}|\delta_{H'}(C)|^2<\frac{(k\alpha^4\alpha')^2}{c_0\log^{50}n}\leq   \frac{(\tk\halpha'\alpha')^2}{c_1\log^{20}n}$. Additionally, if 
$\optcrors(H',\Sigma')>\frac{(\tk\halpha'\alpha')^2}{c_1\eta'\log^{20}n}$, then $\optcrors(H,\Sigma)>\frac{(k\alpha^4 \alpha')^2}{c_0\eta'\log^{50}n}$. 




In order to complete the proof of \Cref{thm: find guiding paths}, it is now enough to design a randomized algorithm, that either computes a distribution $\dset'$ over pairs in $\Lambda(H',\tilde T)$ with $\expect[(\qset',x')\in \dset']{(\cong_{H'}(\qset',e))^2}\leq  O\left (\frac{\log^8n}{(\alpha\alpha')^2}\right )$, or returns FAIL. It is enough to ensure that,   if $\optcrors(H',\Sigma')\leq \frac{(\tk\halpha'\alpha')^2}{c_1\eta'\log^{20}n}$, then the probability that the algorithm returns FAIL is at most $1/2$.

In the remainder of the proof we focus on the above goal. It would be convenient for us to simplify the notation, by denoting $H'$ by $H$, $\hat H''$ by $\hat H$, and $\halpha'$ by $\tilde \alpha$. We also denote $\cset'$ by $\cset$. We now summarize all properties of the new graphs $H,\hat H$ that we have established so far, and in the remainder of the proof of \Cref{thm: find guiding paths} we will only work with these new graphs. 



\paragraph{Summary of the outcome of Step 1.}
We can assume from now on that we are given a graph $H$, a rotation system $\Sigma$ for $H$, a set $\tilde T$ of terminals in graph $H$, and a collection $\cset$ of disjoint subgraphs (clusters) of $H\setminus \tT$. We denote $|\tT|=\tk$. The corresponding contracted graph is denoted by $\hat H=H_{|\cset}$. 
We are also given a partition $(X,Y)$ of $V(H)\setminus \tilde T$ (note that for convenience of notation, $X$ and $Y$ are now subsets of vertices of $H$, and not of $\hat H$), and a parition $\cset_X,\cset_Y$ of $\cset$, such that each cluster $C\in \cset_X$ has $V(C)\subseteq X$, and each cluster $C\in \cset_Y$ has $V(C)\subseteq Y$. We denote $H_1=H[X\cup \tilde T]$ and $H_2=H[Y\cup \tilde T]$. We also denote by $\hat H_1=(H_1)_{|\cset_X}$ the contracted graph of $H_1$ with respect to $\cset_X$, and similarly by $\hat H_2=(H_2)_{|\cset_Y}$ the contracted graph of $H_2$ with respect to $\cset_Y$. 

We now summarize the properties of the graphs that we have defined and the relationships between the main parameters.
\begin{properties}{P}
	\item $\tk\geq \Omega(\alpha^3k/\log^8n)$;\label{prop after step 1: number of pseudoterminals}
	\item every cluster $C\in \cset$ has the $\alpha'$-bandwidth property; \label{prop after step 1: bandwidth property}
	\item $|E(\hat H)|\leq O(\tk\cdot \eta \log^8n/\alpha^3)$ (from \Cref{obs: properties of new graph}); \label{prop after step 1: few edges}
	\item every vertex of $\tilde T$ has degree $1$ in $H_1$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_1$, for $\talpha=\Theta(\alpha/\log^4n)$;\label{prop after step 1: terminals in H1}
	\item similarly, every vertex of $\tilde T$ has degree $1$ in $H_2$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_2$; and \label{prop after step 1: terminals in H2}
\item $\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}
$, where $c_1$ is some large enough constant, whose value we can set later. \label{prop after step 1: small squares of boundaries}
\end{properties}

Our goal is
to design an efficient randomized algorithm, that either computes a distribution $\dset$ over pairs in $\Lambda(H,\tilde T)$ with $\expect[(\qset,x)\in \dset]{(\cong_{H}(\qset,e))^2}\leq  O\left (\frac{\log^{16}n}{(\alpha\alpha')^4}\right )$ for every edge $e\in E(H)$, or returns FAIL.
%Note that, if we let $c_1$ be a large enough constant compared to $c_0$, then $\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1(\eta^4+\eta')\log^{20}n}>
%\frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$.
It is enough to ensure that, if  
%$\optcrors(H,\Sigma)< \frac{(k\alpha^4 \alpha')^2}{c_0(\eta^4+\eta')\log^{50}n}$, 
$\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$,
then the probability that the algorithm returns FAIL is at most $1/2$.

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\iffalse
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: a Modified Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $\hH$, that we denote by $H^+$. In order to define the graph $\hH^+$, we start by defining a rotation system $\hat \Sigma $ for graph $\hH$, as follows. Let $x\in V(\hH)$ be a vertex. If $x$ is a supernode, that is, $x=v(C)$ for some cluster $C\in \cset$, then we define the circular ordering $\hat\oset_x\in \hat \Sigma$ of the edges of $\delta_{\hat H}(x)$ to be arbitrary.
Otherwise, $x$ is a regular vertex, and it is a vertex of the original graph $H$. We then let $\hat \oset_x\in \hat \Sigma$ be identical to the ordering $\oset_x\in \Sigma$, where $\Sigma$ is the original rotation system for graph $H$.

We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(\hat H)$ one-by-one. We denote by $d(u)$ the degree of the vertex $u$ in graph $\hat H$. We now describe an iteration when a vertex $u\in V(\hat H)$ is processed. Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that incident to $u$ in $\hH$, indexed according to their ordering in $\hat \oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(\hat H)$ is processed, we add a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(x,y)\in E(H)$. Assume that $e$ is the $i$th edge of $x$ and the $j$th edge of $y$, that is, $e=e_i(x)=e_j(y)$. Then we add an edge $e'=(s_i(x),s_j(y))$ to graph $H^+$, and we view this edge as the copy of the edge $e\in E(\hat H)$. We will not distinguish between the edge $e$ of $\hat H$ (and the corresponding edge of $H$), and the edge $e'$ of $H^+$.

We note that every terminal $t\in T$ has degree $1$ in $\hat H$, so its corresponding grid $\Pi(t)$ consists of a single vertex, that we also denote by $t$. Therefore, set $T$ of terminals in $H$ naturally corresponds to a set of $k$ terminals in $H^+$, that we denote by $T$ as before.

This completes the definition of the graph $H^+$. Note that the maximum vertex degree in $H^+$ is $4$. We also define a rotation system $\Sigma^+$ for the graph $H^+$ in a natural way: for every vertex $u\in V(H)$, 
consider the standard drawing of the grid $\Pi(u)$, to which we add the drawings of the edges that are incident to vertices $s_1(u),\ldots,s_{d(u)}(u)$, so that the edges are drawn on the grid's exterior in a natural way (\mynote{add figure}). This layout defines an ordering $\oset^+(v)$ of the edges incident to every vertex $v\in \Pi(u)$.

We start with the following simple claim.

\begin{claim}\label{claim: cheap solution to modified instance} There is a solution to the \CNwRS problem instance $(H^+,\Sigma^+)$ of cost at most ..., such that no inner edge of $H^+$ participates in any crossings in the solution.
\end{claim}

\begin{proof}
	We start by showing that $\optcrors(\hH,\hat \Sigma)\leq ...$. Recall that, from \Cref{lem: crossings in contr graph}, there is a drawing $\hat \phi$ of graph $\hH$ with at most $O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2$ crossings, such that for every vertex $x\in V(\hH)\cap V(H)$, the ordering of the edges of $\delta_{\hH}(x)$ as they enter $x$ in $\hat \phi$ is consistent with the ordering $\oset_x\in \Sigma$, and hence with the ordering $\hat \oset_x\in \hat \Sigma$. Drawing $\hat \phi$ of $\hat H$ may not be a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS since for some supernodes $v(C)$, the ordering of the edges that are incident to $v(C)$ in $\hat H$ as they enter the image of $v(C)$ in $\hat \phi$ may be different from $\hat \oset_{v(C)}$. For each such vertex $v(C)$, we may need to \emph{reorder} the images of the edges of $\delta_{\hH}(v(C))=\delta_H(C)$ near the image of $v(C)$, so that they enter the image of $v(C)$ in the correct order. This can be done by introducing at most $|\delta_H(C)|^2$ crossings for each such supernode $v(C)$. The resulting drawing $\hat \phi'$ of $\hat \phi$ is a feasible solution to instance $(\hH,\hat \Sigma)$ of \CNwRS, whose cost is bounded by:
	
	
	\[O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+\sum_{C\in \cset}|\delta_H(C)|^2\leq O(\optcrors(H,\Sigma)\cdot \log^8n/(\alpha')^2+  \]
	
	
\end{proof}
\fi
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

\iffalse
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: Routing the Terminals to a Single Vertex, and the Epanded Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------


\mynote{need to redo this: the paths set should be in the contracted graph $\hH_1$}

In this step we start by considering the graph $H_1$ and the set $\tT$ of terminals in it. Our goal is to compute a collection $\jset$ of paths in graph $H_1$, routing all terminals of $\tT$ to a single vertex, such that the paths in $\jset$ cause a relatively low congestion in graph $H_1$. We show that, if such a collection of paths does not exist, then $\optcrors(H,\Sigma)$ is high. Intuitively, we will use the set $\jset$ of paths in order to define an ordering of the terminals in $\tT$, which will in turn be used in order to compute a grid-like structure in graph $H_2$. Once we compute the desired set $\jset$ of paths, we will replace the graph $H$ with its low-degree analogue $H^+$, that we refer to as the \emph{expanded graph}. The remaining steps in the proof of \Cref{thm: find guiding paths} will use this expanded graph only.


% Recall that the terminals of $\tT$ are $\talpha$-well-linked in $\hat H_1$, and the degree of each terminal in $\hat H_1$ is $1$. 
 
We now proceed to describe the algorithm for Step 2. We consider every \emph{regular} vertex (that is, a vertex that is not a supernode) $x\in V(\hat H_1)$ one by one. For each such vertex $x$, we compute a set $\jset(x)$ of paths in graph $\hat H_1$, with the following properties:

\begin{itemize}
	\item every path in $\jset(x)$ originates at a distinct vertex of $\tT$ and terminates at $x$;
	\item the paths in $\jset(x)$ are edge-disjoint; and
	\item $\jset(x)$ is a maximum-cardinality set of paths in $H_1$ with the above two properties.
\end{itemize}

Note that such a set $\jset(x)$ of paths can be computed via a standard maximum $s$-$t$ flow computation.
Throughout, we use a parameter $\tk'=\ceil{\tk\alpha^5/(c'\eta\log^{36}n)}$, where $c'$ is a large enough constant whose value we set later. 

If, for every regular vertex $x\in V(\hH_1)$, $|\jset(x)|<\tk'$, then we reurn FAIL and terminate the algorithm.  In the following lemma, whose proof is deferred to Section \ref{sec: few paths high opt} of Appendix we show that, in this case, $\optcrors(H,\Sigma)\geq 
 \Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$ must hold.
Note that, since we can set $c_1$ to be a large enough constant, we can ensure that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$ holds in this case.
The value of the constant $c'$ that is used in the definition of the parameter $\tk'$ is set in the proof of the lemma.

\begin{lemma}\label{lem: high opt or lots of paths}
If,  for every regular vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then $\optcrors(H,\Sigma)\geq 
\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$.
\end{lemma}

\mynote{need to redo from here}

From now on we assume that there is some vertex $x\in V(H_1)$, for which $|\jset(x)|\geq \tk'$. We denote $\jset_0=\jset(x)$, and we let $T_0\subseteq \tT$ be the set of terminals that serve as endpoints of paths in $\jset_0$, so $|T_0|=|\jset_0|=\tk'$.



Let $z=\ceil{\tk/\tk'}=O\left(\frac{\eta\log^{36}n}{\alpha^5\alpha'}\right )$. Next, we arbitrarily partition the terminals of $\tT\setminus T_0$ into $z$ subsets $T_1,\ldots,T_z$, of cardinality at most $\tk'$ each. Consider now some index $1\leq i\leq z$. Since the set $\tT$ of terminals is $(\talpha\alpha')$-well-linked in $H_1$ (from \Cref{clm: contracted_graph_well_linkedness}), using the algorithm from \Cref{thm: bandwidth_means_boundary_well_linked}, we can compute a collection $\jset_i'$ of paths in graph $H_1$, routing vertices of $T_i$ to vertices $T_0$, such that the paths in $T_i$ cause edge-congestion $O(1/(\talpha\alpha'))$, and each vertex of $T_i$ is the endpoint of at most one path in $\jset_i'$. By concatenating the paths in $\jset_i'$ with paths in $\jset_0$, we obtain a collection $\jset_i$ of paths in graph $H_1$, connecting every terminal of $T_i$ to $x$, that cause edge-congestion $O(1/(\talpha\alpha'))$. Let $\jset=\bigcup_{i=0}^z\jset_i$ be the resulting set of paths. Observe that set $\jset$ contains $\tk$ paths, routing the terminals in $\tT$ to the vertex $x$ in graph $H_1$, with $\cong_H(\jset)\leq O\left(\frac z{\talpha\alpha'}\right )\leq O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$. We denote by $\rho=O\left(\frac{\eta\log^{40}n}{\alpha^6(\alpha')^2}\right )$ this bound on $\cong_{H_1}(\pset')$. We assume w.l.o.g. that the paths in $\jset$ are simple. Since every terminal in $\tT$ has degree $1$ in $H_1$, no path in $\jset$ may contain a terminal in $\tT$ as its inner vertex.



In the remainder of the proof, it would be convenient for us to work with a low-degree equivalent of the graph $H$, that we call \emph{expanded graph}, and denote by $H^+$. 

For every edge $e\in E(H)$, let $N_e=\cong_H(\jset,e)$. Recall that for every edge $e\in E(H_1\setminus\tT)$, $N_e\leq \rho$, and for every other edge $e$ of $H$, $N_e\leq 1$.

\fi







%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
\subsection{Step 2: Routing the Terminals to a Single Vertex, and an Expanded Graph}
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

In this step we start by considering the graph $\hat H_1$ and the set $\tT$ of terminals in it. Our goal is to compute a collection $\jset$ of paths in graph $\hat H_1$, routing all terminals of $\tT$ to a single regular  vertex, such that the paths in $\jset$ cause a relatively low congestion in graph $\hat H_1$. We show that, if such a collection of paths does not exist, then $\optcrors(H,\Sigma)$ is high. Intuitively, we will use the set $\jset$ of paths in order to define an ordering of the terminals in $\tT$, which will in turn be used in order to compute a grid-like structure in graph $H_2$. Once we compute the desired set $\jset$ of paths, we will replace the graph $H$ with its low-degree analogue $H^+$, that we refer to as the \emph{expanded graph}. The remaining steps in the proof of \Cref{thm: find guiding paths} will use this expanded graph only.


% Recall that the terminals of $\tT$ are $\talpha$-well-linked in $\hat H_1$, and the degree of each terminal in $\hat H_1$ is $1$. 



\subsubsection{Routing the Terminals to a Single Vertex}
We process {\bf regular} vertices of $V(\hat H_1)$ (that is, vertices of $V(\hat H_1)\cap V(H_1)$) one-by-one. For each such vertex $x$, we compute a set $\jset(x)$ of paths in graph $\hat H_1$, with the following properties:

\begin{itemize}
	\item every path in $\jset(x)$ originates at a distinct vertex of $\tT$ and terminates at $x$;
	\item the paths in $\jset(x)$ are edge-disjoint; and
	\item $\jset(x)$ is a maximum-cardinality set of paths in $\hat H_1$ with the above two properties.
\end{itemize}

Note that such a set $\jset(x)$ of paths can be computed via a standard maximum $s$-$t$ flow computation.
Throughout, we use a parameter $\tk'=\tk\alpha^5/(c'\eta\log^{36}n)$, where $c'$ is a large enough constant whose value we set later. 

If, for every vertex $x\in V(H_1)$, $|\jset(x)|<\tk'$, then we reurn FAIL and terminate the algorithm.  In the following lemma, whose proof is deferred to Section \ref{sec: few paths high opt} of Appendix we show that, in this case, $\optcrors(H,\Sigma)\geq 
\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$ must hold.
Note that, since we can set $c_1$ to be a large enough constant, we can ensure that $\optcrors(H,\Sigma)>\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$ holds in this case.
The value of the constant $c'$ that is used in the definition of the parameter $\tk'$ is set in the proof of the lemma.

\begin{lemma}\label{lem: high opt or lots of paths}
	If,  for every vertex $x\in V(\hat H_1)\cap V(H_1)$, $|\jset(x)|<\tk'$, then $\optcrors(H,\Sigma)\geq 
	\Omega\left(\frac{(\tk\talpha \alpha')^2}{\eta'\log^{20}n}\right )$.
\end{lemma}


From now on we assume that there is some vertex $x\in V(\hat H_1)\cap V(H_1)$, for which $|\jset(x)|\geq \tk'$. 



\subsubsection{The Expanded Graph}

From now on we fix the vertex $x\in V(\hat H_1)\cap V(H_1)$, and we let $\jset=\jset(x)$ be the set of at least $\tk'$ paths in graph $\hH_1$, routing a subset $\tT_0\subseteq \tT$ of terminals to vertex $x$. %Assume for now that we are given some fixed ordering $\tilde \oset$ of the terminals in $\tT$, and denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$.


We are now ready to define the modified graph $H^+$. We start with $H^+=\emptyset$, and then process every vertex $u\in V(H_2)\setminus \tilde T$ one by one. We now describe an iteration when a vertex $u\in V(H_2)\setminus \tilde T$ is processed. We denote by $d(u)$ the degree of the vertex $u$ in graph $H_2$.  Let $e_1(u),\ldots,e_{d(u)}(u)$ be the edges that are incident to $u$ in $H_2$, indexed according to their ordering in $ \oset_u\in  \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ grid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$ indexed in their natural left-to-right order. 
We add the vertices and the edges of the grid $\Pi(u)$ to graph $H^+$. We refer to the edges in the resulting grids $\Pi(u)$ as \emph{inner edges}.
Once every vertex $u\in V(H_2)\setminus \tT$ is processed, we add 
the vertices of $\tT$ to the graph $H^+$. Recall that every terminal $t\in \tT$ has degree $1$ in $H_2$. We denote the unique edge $e_t$ incident to $t$ by $e_1(t)$, and we denote $s_1(t)=t$.

Next, we add 
a collection of \emph{outer edges} to graph $H^+$, as follows. Consider any edge $e=(u,v)\in E(H_2)$. Assume that $e$ is the $i$th edge of $u$ and the $j$th edge of $v$, that is, $e=e_i(u)=e_j(v)$. Then we add an edge $e'=(s_i(u),s_j(v))$ to graph $H^+$, and we view this edge as the \emph{copy of the edge $e\in E(H_2)$}. We will not distinguish between the edge $e$ of $H_2$, and the edge $e'$ of $H^+$.


Our last step is to add vertex $x$ to graph $H^+$, that connects to every terminal $t\in \tT$ with an edge $(x,t)$, that is also viewed as an outer edge. The following lemma, whose proof is deferred to Section \ref{sec:ordering of terminals} of Appendix, allows us to compute an ordering $\tilde \oset$ of the terminals, such that the graph $H^+$ has a drawing $\phi$ with few crossings, in which the inner edges do not participate in any crossings, and the images of edges incident to $x$ enter $x$ in order consistent with $\tilde \oset$.


\iffalse
Our last step is to add a $(\tk\times\tk)$-grid $\Pi(x)$ to graph $H^+$ corresponding to the vertex $x$. As before, the edges of the grid are inner edges for graph $H^+$, and we denote the vertices on the first row of the grid by $s_1(x),\ldots,s_{\tk}(x)$, indexed in their natural left-to-right order. For all $1\leq i\leq \tk$, we add an outer edge $(t_i,s_i(x))$ to graph $H^+$. This completes the definition of the graph $H^+$, provided that we are given an ordering $\tilde \oset$ of the terminals. The following lemma, whose proof is deferred to Section \ref{sec:ordering of terminals} of the Appendix, allows us to compute an ordering $\tilde \oset$ of the terminals, such that the resulting graph $H^+$ has a drawing $\phi$ with few crossings, in which the inner edges do not participate in any crossings.
\fi


\begin{lemma}\label{lem: find ordering of terminals}
	There is an efficient algorithm to compute an ordering $\tilde \oset$ of the terminals in $\tT$, such that there is a drawing $\phi$ of graph $H^+$ with at most $O\left(\optcrors(H,\Sigma)\cdot\frac{\eta^2\log^{74}n}{\alpha^{12}(\alpha')^4}\right ) +O \left (
	\frac{\tk \eta\log^{37}n}{\alpha^6(\alpha')^2}\right )$ crossings, in which all crossings in $\phi$ are between pairs of outer edges. Moreover, if we denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$, and, for each $1\leq i\leq t_{\tk}$, denote by $e_i=(t_i,x)$ the edge of $H^+$ connecting $t_i$ to $x$, then the images of the edges $e_1,\ldots,e_{\tk}$ enter the image of $x$ in this circular order in the drawing $\phi$.
\end{lemma}

From now on we fix the ordering $\tilde \oset$ of the terminals in $\tilde T$ given by \Cref{lem: find ordering of terminals}, and the drawing $\phi$ of $H^+$ (which is not known to us).



It will be convenient for us to slightly modify the graph $H^+$ as follows. We denote 
the terminals by  $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the circular ordering $\tilde \oset$. Let $H'$ be a graph obtained from $H^+$, by first deleting the vertex $x$ from it, and then adding, for all $1\leq i<\tk$, an edge $e^*_i=(t_i,t_{i+1})$, and another edge $e^*_{\tk}=(t_{\tk},t_1)$. We denote this set of the newly added edges by $E^*$, and we view them as inner edges. Note that the edges of $E^*$ form a simple cycle, that we denote by $L^*$. We also denote $H''=H'\setminus E^*$.

We note that the drawing $\phi$ of $H^+$ can be easily extended to obtain the drawing of $H'$ in the plane, so that the inner edges of $H'$ do not participate in any crossings, and the image of the cycle $L^*$ (which must be a simple closed curve) is the boundary of the outer face.

In order to do so, we start with the drawing $\phi$ of $H^+$ on the sphere, and then draw a small disc $D$ with $x$ lying in its interior, and denote by $\eta$ its boundary. 
For every terminal $t_i\in \tT$, we denote by $e_i$ the unique edge incident to $t_i$ in $H''$, and by $e'_i=(t_i,x)$. We also denote by $\gamma_i,\gamma'_i$ the images of the edges $e_i,e'_i$ in the current drawing. Let $p_i$ be the unique point on the intersection of $\gamma'_i$ and $\eta$. We move the image of terminal $t_i$ to point $p_i$. We then modify the image of the edge $e_i$, so that it becomes a concatenation of $\gamma_i$, and the portion of $\gamma'_i$ lying outside the interior of $D$. Lastly, we draw the edges of $E^*$ in a natural way, where edge $e^*_i$ is simply a segment of $\eta$ between the images of $t_i$ and $t_{i+1}$, so that all resulting segments are mutually internally disjoint. Once we delete the vertex $x$ from this drawing, no part of the resulting drawing is contained in the interior of the disc $D$, and the image of the cycle $L^*$ is precisely $\eta$, so we can view the resuting drawing as a drawing in the plane, with $D$ being the outer face. Note that this transformation does not increase the number of crossings.



The following observation follows by substituting parameters and bounds that we have already established. The proof is included in Section \ref{subsec: proof of obs on bounds on opt} of Appendix.

\begin{observation}\label{obs: bounds on opt}
	If $\optcrors(H,\Sigma)<\frac{(\tilde k\tilde \alpha\alpha')^2}{c_1\eta'\log^{20}n}$, then  $\cro(\phi)\leq 
	\cro(\phi)\leq \frac{\tilde k^2}{c_2\eta^5}$, for a large enough constant $c_2$.
\end{observation}



It is therefore enough for us to ensure that, if $\cro(\phi)<
 \frac{\tilde k^2}{\eta^5}$, then the  probability that the algorithm returns FAIL is at most $1/2$.






Let $\Lambda'$ denote all pairs $(\qset,y)$, where $y$ is a vertex in graph $H_2$, and $\qset$ is a set of paths in graph $H''$, routing the set $\tT$ of terminals to vertices of $\Pi(y)$. 
We also need the following simple observation, whose proof is deferred to Section \ref{subsec: transform paths 2} of the Appendix.

\begin{observation}\label{obs: transform paths 2}
There is an efficient algorithm, that, given a distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every {\bf outer} edge $e\in E(H'')$, $\expect[(\qset,y)\in_{\dset}\Lambda']{(\cong_{H''}(\qset,e))^2}\leq \beta$, computes  a distribution $\dset'$ over pairs in $\Lambda(H,\tT)$, where for every edge $e\in E(H)$, $\expect[(\qset',y)\in_{\dset'} \Lambda(H,\tT)]{(\cong_{H}(\qset',e))^2}\leq \beta$.
\end{observation}



 






\subsubsection{Summary of Step 2}
\label{step 2 summary}

In the remainder of the proof of \Cref{thm: find guiding paths} we will work with graph $H'$ only. Recall that graph $H'$ contains a set $E^*=\set{e_1,\ldots,e_{\tk}}$ of edges (that are considered to be inner edges), where for all $1\leq i\leq \tk$, $e_i=(t_i,t_{i+1})$ (we use indexing modulo $\tk$). The set $E^*$ of edges defines a cycle $L^*=(t_1,\ldots,t_{\tk})$ in graph $H'$. We also denoted $H''=H'\setminus E^*$. Recall that graph $H''$ is obtained from a subgraph $H_2\subseteq H$, by replacing every vertex $v\in V(H_2)\setminus \tT$ with a grid $\Pi(v)$. All edges lying in the resulting rids $\Pi(v)$, and the edges of $E^*$ are inner edges, while all other edges of $H'$ are outer edges. Each outer edge of $H'$ corresponds to some edge of graph $H_2$, and we do not distinguish between these edges. Note that in graph $H'$, all vertices have degrees at most $4$. We will also use the clustering $\cset_Y$ of graph $H_2$, and the fact that, from Property \ref{prop after step 1: small squares of boundaries}: 
\begin{equation}\label{eq: sum of squares}
\sum_{C\in \cset_Y}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}. \end{equation}
We further partition the outer edges of graph $H''$ into two subsets: type-1 outer edges and type-2 outer edges. Consider any outer edge $e$ in graph $H''$, and let $e'=(u,v)$ be the corresponding edge in graph $H$. If $u$ and $v$ both lie in the same cluster $C\in \cset_Y$, then we say that $e$ is a \emph{type-2} outer edge, and otherwise it is a type-1 outer edge. 
Intuitively, for each type-1 outer edge, there is a corresponding edge in the contracted graph $\hat H$. From Property \ref{prop after step 1: few edges}, we obtain the following observation.


\begin{observation}\label{obs: few outer edges}
	There is a universal constant $c$ (independent of $c_1$ and $c_2$), such that the total number of type-1 outer edges in $H''$ is bounded by ${c\tk\cdot \eta \log^8n/\alpha^3}$. 
\end{observation}




\iffalse
======================

\highlightf[purple]{Calculations:}

final number of paths: at least $\alpha^*\tk/256$. Supergrid dimensions: $\lambda\times \lambda$. Want: at most $\lambda^2/32$ cells have an outer edge on each path. Number of paths per cell: $\alpha^*\tk/(256\lambda)$. So we need that:

\[\frac{\alpha^*\tk}{256\lambda}\cdot \frac{\lambda^2}{32}>\frac{c\tk\cdot \eta \log^8k}{\alpha^3}.  \]

To ensure this, enough to set:

\[\lambda=\frac{2^{16}c\cdot \eta \log^8n}{\alpha^*\alpha^3}.  \]

(and this is tight to within constants).


Because $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$.

If we ensure that $\highlightf{\eta>\frac{c^* \log^{12}n}{\alpha^4\alpha'}}$, then $\lambda<\eta^2$ will hold.

Group size: start with: 

\[\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}=\floor{\frac{\alpha^3(\alpha^*)^2\tk}{2^{32}c\eta\log^8n}}.\]

This is $\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$. If $\highlightf{\eta>\frac{c^* \log^{8}n}{\alpha^5(\alpha')^2}}$, we get that $\psi>\frac{16\tk}{\eta^2}$.

Overall, for this part, we need $\highlightf{\eta>\frac{c^* \log^{12}n}{\alpha^5(\alpha')^2}}$, which so far is ensured.

======================
\fi

Recall that from Property \ref{prop after step 1: terminals in H1}, every vertex of $\tilde T$ has  $1$ in $H_2$, and vertex set $\tilde T$ is $\talpha$-well-linked in $\hat H_2$. Combining this with the $\alpha'$-bandwidth property of every cluster $C\in \cset_Y$ from Property \ref{prop after step 1: bandwidth property}, from \Cref{clm: contracted_graph_well_linkedness}, the set $\tT$ of terminals is $\talpha\cdot \alpha'$-well-linked in $H_2$. Lastly, using the fact that each graph in $\set{\Pi(v)\mid v\in V(H_2)}$ has the $1$-bandwidth property, from \Cref{clm: contracted_graph_well_linkedness}, we get the following observation.


\begin{observation}\label{obs: terminals well linked in H''}
	The set $\tT$ of terminals is $\alpha^*$-well-linked in $H''$, where ${\alpha^*=\talpha\cdot\alpha'=\Theta(\alpha\alpha'/\log^4n)}$. Moreover, each terminal in $\tT$ has degree $1$ in $H''$ and degree $3$ in $H'$.
\end{observation}
(we have used the fact that  
$\talpha=\Theta(\alpha/\log^4n)$ (see Property \ref{prop after step 1: terminals in H1})).


%Recall that we are given a circular ordering $\tilde \oset$ of the terminals in $\tT$. This ordering naturally defines an ordering $\oset_x$ of edges incident to $x$ in $H'$: if $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according to the ordering $\tilde \oset$, and for all $1\leq i\leq \tk$, $e_i$ is the edge $(x,t_i)$, then $\oset_x=\set{e_1,\ldots,e_{\tk}}$.

We will restrict our attention to special types of drawings of graph $H'$, called \emph{legal drawings}, that we define next.

\begin{definition}[Legal drawing of $H'$]
We say that a drawing of graph $H'$ in the plane is \emph{legal} iff it has the following properties:

\begin{itemize}
	

	\item no inner edge of $H'$ participates in any crossing of $\phi^*$, and in particular the image of the cycle $L^*$ is a simple closed curve, denoted by $\eta$; and
	\item $\eta$ is the boundary of the outer face in the drawing.
\end{itemize}
\end{definition}

We let $\phi^*$ be a legal drawing of $H'$ with smallest number of crossings, and we denote by $\cro^*$ the number of crossings in $\phi^*$.



Denote $\tT=\set{t_1,\ldots,t_{\tk}}$, where the terminals are indexed according their ordering in $\tilde \oset$. We partition the set $\tT$ of terminals into four subsets $T_1,\ldots,T_4$, where $T_1,T_2,T_3$ contain $\floor{\tk/4}$ consecutive terminals from $\tT$ each, and $T_4$ contains the remaining terminals, in a natural way using the ordering $\tilde \oset$, that is, $T_1=\set{t_1,\ldots,t_{\floor{\tk/4}}}$, $T_2=\set{t_{\floor{\tk/4}+1},\ldots,t_{2\floor{\tk/4}}}$, $T_3=\set{t_{2\floor{\tk/4}+1},\ldots,t_{3\floor{\tk/4}}}$, and $T_4=\set{t_{3\floor{\tk/4}+1},\ldots,t_{\tk}}$. Clearly, each of the four sets contains at least $\floor{\tk/4}$ terminals.

Recall that in a legal drawing $\phi$ of $H'$, the image of the cycle $L^*$ is a simple closed curve, that we denoted by $\eta$. It will be convenient for us to view this curve $\eta$ as the boundary of a rectangular area in the plane, that encloses the legal drawing of $H'$. We sometimes refer to this rectangular area as the \emph{bounding box} of the drawing, and denote it by $B^*$. We will think of the terminals in $T_1$ and $T_3$ as appearing on the left and on the right boundaries of $B^*$, respectively, and of the terminals in $T_2$ and $T_4$ as appearing on the top and the bottom boundaries of $B^*$, respectively. 

For all $1\leq i\leq 4$, we let $\tilde \oset_i$ be the ordering of the terminals in $T_i$ consistent with their ordering on the boundary of $B^*$ (where each ordering $\tilde\oset_i$ is no longer circular), so that the terminals in sets $T_1$ and in $T_3$ are indexed in their bottom-to-top order, and the terminals in $T_2$ and $T_4$ are indexed in their left-to-right order (so $\tilde \oset$ is obtained by concatenationg $\tilde\oset_1,\tilde\oset_2$, the reversed ordering $\tilde\oset_3$, and the reversed ordering $\tilde\oset_4$).






Recall that $\Lambda'$ is the set of all pairs $(\qset,y)$, where $y\in V(H_2)$, and $\qset$ is a collection of paths in graph $H''$, routing the set $\tT$ of terminals to the vertices of $\Pi(y)$.
Our goal is to design a randomized algorithm, that either computes a distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every outer edge $e\in E(H')$, $\expect[(\qset,y)\in_{\dset} \Lambda']{(\cong_{H'}(\qset,e))^2}\leq  O\left (\frac{\log^{16}n}{(\alpha\alpha')^4}\right )$, or returns FAIL.
It is enough to ensure that, if $\cro^*\leq 
\frac{\tilde k^2}{c_2\eta^5}$ for some large enough constant $c_2$, then the  probability that the algorithm returns FAIL is at most $1/4$.






\subsection{Step 3: Constructing a Grid Skeleton}





In this and the following step we will construct a grid-like structure in graph $H''$. Recall that the set $\tT$ of terminals is $\alpha^*$-well-linked in grpah $H''$.  From \Cref{thm: bandwidth_means_boundary_well_linked} there is a set $\pset'$ of paths in $H''$, routing all terminals of $T_1$ to terminals of $T_3$, with edge-congestion at most $\ceil{1/\alpha^*}$, such that the routing is one-to-one. From \Cref{claim: remove congestion}, there is a collection $\pset''$ of at least $|T_1|/\ceil{1/\alpha^*}=\floor{\tk/4}/\ceil{1/\alpha^*}\geq \alpha^*\tk/8$ edge-disjoint paths in $H''$, routing some subset of terminals of $T_1$ to a subset of terminal of $T_3$, in graph $H''$. Moreover, since graph $H''$ has maximum vertex degree at most $4$, using arguments similar to those in the proof of \Cref{claim: remove congestion}, there is a collection $\pset$ of $\floor{\alpha^*\tk/32}$ {\bf node-disjoint} paths in graph $H''$, routing some subset $A\subseteq T_1$ of terminals, to some subset $A'\subseteq T_3$ of terminals. We can compute such a set $\pset$ of paths efficiently using standard maximum $s$-$t$ flow algorithms.

Using similar reasoning, we can compute a collection $\rset$ of $\floor{\alpha^*\tk/32}$ node-disjoint paths in graph $H''$, routing some subset $B\subseteq T_2$ of terminals, to some subset $B'\subseteq T_4$ of terminals.

Intuitively, after we discard a small subset of paths from each of the sets $\pset,\rset$, the remaining paths will be used in order to construct a grid-like structure, where paths in $\pset$ will serve as horizontal paths of the grid, and paths in $\rset$ will serve as vertical paths. If the paths in the resulting sets do not form a grid-like structure, then we will terminate the algorithm with a FAIL. We will prove that, if $\cro^*\leq 
\frac{\tilde k^2}{c_2\eta^5}$ for a large enough constant $c_2$, then we will construct the grid-like structure successfully with probability at least $3/4$.

We denote $\pset_0=\pset$ and $\rset_0=\rset$. Recall that so far, ${|\pset_0|,|\rset_0|\geq \floor{\alpha^*\tk/32}}$. 




Intuitively, if the dimensions of the grid-like structure that we construct are $(h\times h)$, then we need $h$ to be quite close to $\tk$, since this grid-like structure will be exploited in order to define the distribution $\dset$ over pairs in $\Lambda'$.
We will first construct a smaller grid-like structure, that we call a \emph{grid skeleton}. This grid skeleton will be associated with a grid $\Pi^*$ of smaller dimensions, that we sometimes call a \emph{supergrid}. We then extend this grid skeleton to construct a large enough grid-like structure.


We will use two additional parameters. The first parameter is:
\[\lambda=\frac{2^{24}c\cdot \eta \log^8n}{\alpha^*\alpha^3},\] 
where $c$ is the constant from \Cref{obs: few outer edges}. Notice that, since $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$. Moreover, since $\eta>\frac{c^* \log^{12}n}{\alpha^4\alpha'}$ for a large enough constant $c^*$ (from the statement of \Cref{thm: find guiding paths}), $\lambda<\eta^2$. The supergrid that we construct will have dimensions $(\Theta(\lambda)\times \Theta(\lambda))$. The second parameter is:
%%
\[\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}=\floor{\frac{\alpha^3(\alpha^*)^2\tk}{2^{30}c\eta\log^8n}}.\]
%%
Clearly, $|\rset_0|,|\pset_0|\geq \lambda\psi$.
Note that, since $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, $\psi\geq \Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^{16}n}  \right)$. Since ${\eta>\frac{c^* \log^{16}n}{\alpha^5(\alpha')^2}}$ from the statement of \Cref{thm: find guiding paths}, we get that $\psi>\frac{16\tk}{\eta^2}$.  Every cell of the supergrid will be associated with a collection of $\Theta(\psi)$ horizontal paths and $\Theta(\psi)$ vertical paths, that will help us form the grid-like structure.

We discard paths from $\pset_0$ and from $\rset_0$ arbitrarily, until $|\pset_0|=|\rset_0|=\lambda\psi$ holds.

We denote by $A_0\subseteq T_1,A'_0\subseteq T_3$ the endpoints of the paths in $\pset_0$, and we denote by $B_0\subseteq T_4$, $B'_0\subseteq T_2$ the endpoints of the paths in $\rset_0$.

 
 
\subsubsection*{Grid Skeleton Construction}
 

\iffalse 
 Let $c$ be a constant, such that the number of type-1 outer edges is at most $c\tk\cdot \eta \log^8k/\alpha^3$. 
 
 We say that a path $P\in \pset_0\cup \rset_0$ is \emph{long} if it contains at least $128c\eta\log^8k/(\alpha^*\alpha^3)$ type-1 outer edges, and otherwise we call it short.
Since the total number of type-1 outer edges is at most $c\tk\cdot \eta \log^8k/\alpha^3$, and the paths in  $\pset_0$ are edge-disjoint, at most $\alpha^*\tk/128$ paths in $\pset_0$ may be long. We let $\pset_1\subseteq \pset_0$ be the set of all short paths, so $|\pset_1|\geq \alpha^*\tk/128$. Similarly, we let $\rset_1\subseteq \rset_0$ be the set of all short paths, so $|\rset_1|\geq \alpha^*\tk/128$. We denote by $A_1\subseteq A$, $A_1'\subseteq A'$ the sets of endpoints of the paths in $\pset_1$, and we similarly denote by $B_1\subseteq B$, $B_1'\subseteq B'$ the sets of endpoints o fthe paths in $\rset_1$.
\fi


 
We view the paths in $\pset_0$ as directed from vertices of $A_0$ to vertices of $A'_0$. Recall that $A_0\subseteq T_1$, so the ordering $\tilde\oset_1$ of the terminals in $T_1$ defines an ordering $\oset_{A_0}=\set{a_1,\ldots,a_{\lambda\psi}}$ of the terminals in $A_0$. This ordering in turn defines an ordering $\oset_{\pset_0}$ of the paths in $\pset_0$, as follows: if, for all $1\leq i\leq \lambda\psi$, $P_i\in \pset_0$ is the path originating from $a_i$, then $\oset_{\pset_0}=\set{P_1,\ldots,P_{\lambda\psi}}$.

Similarly, we view the paths in $\rset_0$ as directed from vertices of $B_0$ to vertices of $B_0'$. Ordering $\tilde\oset_4$ of terminals in $T_4$ defines an ordering $\oset_{B_0}=\set{b_1,\ldots,b_{\lambda\psi}}$ of the vertices in $B_0$, which in turn defines an ordering $\oset_{\rset_0}=\set{R_1,\ldots,R_{\lambda\psi}}$ of paths in $\rset_0$, where for all $i$, path $R_i$ originates at vertex $b_i$.


We partition the set $\pset_0$ of paths into  groups $\uset_1,\ldots,\uset_{\lambda}$ of cardinality $\psi$ each, using the ordering $\oset_{\pset_0}$, so for $1\leq i<\lambda$, set $\uset_i$ is the $i$th set of $\psi$ consecutive paths of $\pset_0$. 
Let $\lambda'= \floor{(\lambda-1)/2}$. 
For all $1\leq i\leq \lambda'$, we let $ P^*_i$ be a path that is chosen uniformly at random from set $\uset_{2i}$. Let $\pset^*=\set{ P^*_1,\ldots, P^*_{\lambda'}}$ be the resulting set of chosen paths. Intuitively, the path in $\pset^*$ will serve as the horizontal paths in the grid skeleton that we construct.
We then let $\pset_1\subseteq \pset_0$ be the set containing all paths in sets $\set{\uset_{2i-1}}_{i=1}^{\lambda'+1}$. 

We perform similar computation on the set $\rset_0$ of paths. First, we partition $\rset_0$ into  groups $\uset'_1,\ldots,\uset'_{\lambda}$ of cardinality $\psi$ each, using the ordering $\oset_{\rset_0}$, so for $1\leq i<\lambda$, set $\uset'_i$ is the $i$th set of $\psi$ consecutive paths of $\rset_0$. 
For all $1\leq i\leq \lambda'$, we let $ R^*_i$ be a path that is chosen uniformly at random from set $\uset_{2i}$. Let $\rset^*=\set{ R^*_1,\ldots, R^*_{\lambda'}}$ be the resulting set of chosen paths. Intuitively, the path in $\rset^*$ will serve as the vertical paths in the grid skeleton that we construct.
We then let $\rset_1\subseteq \rset_0$ be the set containing all paths in sets $\set{\uset'_{2i-1}}_{i=1}^{\lambda'+1}$.


We let $\event_1$ be the bad event that there are two distinct paths $Q,Q'\in \rset^*\cup \pset^*$, and two distinct edges $e\in E(Q)$, $e'\in E(Q')$, such that the images of $e$ and $e'$ cross in the drawing $\phi^*$ of $H'$.

\begin{observation}\label{obs: first bad event}
	If $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_1}\leq 1/64$.
\end{observation}

\begin{proof}
Consider any crossing $(e,e')$ in the drawing $\phi^*$. We say that crossing $(e,e')$ is \emph{selected} iff there are two distinct paths $Q,Q'\in \rset^*\cup \pset^*$ with  $e\in E(Q)$, $e'\in E(Q')$. Notice that $e$ may belong to at most two paths in $\rset_0\cup \pset_0$ (one path in each set), and the same is true for $e'$. Each path of $\rset_0\cup\pset_0$ is chosen to $\rset^*\cup \pset^*$ with probability at most $1/\psi$. Therefore, the probability that a path containing $e$, and a path containing $e'$ are chosen to $\rset^*\cup \pset^*$ is at most $4/\psi^2$. Since $\event_1$ can only happen if at least one crossing is chosen, from the union bound, 
$\prob{\event_1}\leq 4\cro^*/\psi^2$. Since $\psi>\frac{16\tk}{\eta^2}$, if $\cro^*<
\frac{\tilde k^2}{c_2\eta^5}$, then:

\[\prob{\event_1}\leq \frac{4\cro^*}{\psi^2}\leq \frac{1}{64c_2\eta}\leq \frac{1}{64}.\]	
\end{proof}




We say that a path $Q\in \rset_0\cup \pset_0$ is \emph{heavy} iff there are at least $\frac{\psi}{64\lambda}$ crossings $(e,e')$ in $\phi^*$, such that at least one of the edges $e,e'$ lies on path $Q$. We say that a bad event $\event_2$ happens iff at least one path in $\rset^*\cup \pset^*$ is heavy.

\begin{observation}\label{obs: first bad event}
	If $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_2}\leq 1/64$.
\end{observation}
\begin{proof}
	Note that every edge of $H''$ may lie on at most two paths of $\rset_0\cup \pset_0$, and every crossing $(e,e')$ involves two edges. Therefore, the total number of heavy paths in $\rset_0\cup \pset_0$ is bounded by $\frac{4\cro^*}{\psi/(64\lambda)}=\frac{2^8\lambda\cdot\cro^*}{\psi}$. Assuming that $\cro^*<
	\frac{\tilde k^2}{c_2\eta^5}$, and using the fact that $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^{16}n}  \right)$ and $\lambda=O\left( \frac{\eta \log^{12}n}{\alpha^4\alpha'}  \right )$, we get that the total number of heavy paths in $\rset_0\cup \pset_0$ is bounded by:
	
	
	\[ \frac{2^8\lambda\cdot\cro^*}{\psi}\leq O\left( \frac{\tilde k^2}{c_2\eta^5}\cdot \frac{\eta \log^{12}n}{\alpha^4\alpha'}\cdot\frac{\eta}{\tk}\cdot \frac{\log^{16}n}{\alpha^5(\alpha')^2} \right ) 
\leq	 O\left( \frac{\tilde k\log^{28}n}{c_2\eta^3\alpha^9(\alpha')^3} \right ).
	\]
	
Note that each heavy path may be selected to $\rset^*\cup \pset^*$  with probability at most $1/\psi$. Therfore, using the union bound and the fact that $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^{16}n}  \right)$, we get that:

\[\prob{\event_2}\leq 
O\left( \frac{\tilde k\log^{20}n}{\psi\cdot c_2\eta^3\alpha^9(\alpha')^3}\right )\leq
O\left( \frac{\log^{44}n}{\cdot c_2\eta^2\alpha^{14}(\alpha')^5}\right ).\]
	
Recall that, from the conditions of \Cref{thm: find guiding paths}, $\eta\geq c^*\log^{46}n/(\alpha^{10}(\alpha')^4)$, where $c^*$ is a sufficiently large constant. Therefore, if 
$\cro^*<
\frac{\tilde k^2}{c_2\eta^5}$, then $\prob{\event_2}\leq 1/64$.
\end{proof}


Let $\rset'\subseteq \rset_1$, $\pset'\subseteq \pset_1$ be the sets containing all paths $Q$, such that, in drawing $\phi^*$, the image of some edge of $Q$ crosses the image of some edge lying on the paths of $\rset^*\cup \pset^*$. Note that the drawing $\phi^*$ is not known to us, and so neither are the path sets $\rset',\pset'$. We will also use the following observation:

\begin{observation}\label{obs: few bad paths}
	If $\event_2$ did not happen, then $|\rset'|,|\pset'|\leq \psi/32$.
\end{observation}
\begin{proof}
	Recall that $|\rset^*|+|\pset^*|\leq \lambda$. If bad event $\event_2$ did not happen, then for each path $Q\in \rset^*\cup \pset^*$, there are at most $\frac{\psi}{64\lambda}$ crossings in $\phi^*$, in which edges of $Q$ participate. Therefore, if event $\event_2$ did not happen, there are in total at most $\psi/64$ crossings $(e,e')$ in the drawing $\phi^*$, where at least one of the edges $e,e'$ lies on a path of $\pset^*\cup \qset^*$. Let $E'\subseteq E(H'')$ be the set of all edges $e$, such that there is an edge $e'$ lying on some path of $\pset^*\cup \qset^*$, and crossing $(e,e')$ is present in $\phi^*$. Then $|E'|\leq \psi/32$. Each path in $\rset'\cup \pset'$ must contain an edge of $E'$. As the paths in each of the sets $\rset',\pset'$ are disjoint, $|\rset'|,|\pset'|\leq \psi/32$ must hold.
\end{proof}





\paragraph{Summary of Step 3.}
In this step we have constructed a grid skeleton, that consists of two sets of paths: $\pset^*=\set{ P^*_1,\ldots, P^*_{\lambda'}}$, and $\rset^*=\set{ R^*_1,\ldots,\tilde R^*_{\lambda'}}$, where $\lambda'= \floor{(\lambda-1)/2}$. Recall that $\pset^*\subseteq \pset_0$, and the paths in $\pset^*$ are indexed according to their order in $\oset_{\pset_0}$. Recall that we have also defined the set  $\pset_1\subseteq \pset_0$ of paths, containing all paths in sets $\set{\uset_{2i-1}}_{i=1}^{\lambda'+1}$. It would be convinient for us to re-index the groups $\uset_i$ as follows: for  $1\leq i\leq \lambda'+1$, set $\uset_i=\uset_{2i-1}$. In other words, the paths of $\uset_0$ lie before path $P^*_1$  in the ordering $\oset_{\pset_0}$, the paths of $\uset_{\lambda'+1}$ lie after $P^*_{\lambda'}$ in this ordering, and, for $1\leq i<\lambda'$, the  paths of $\uset_i$ lie between paths $P^*_i$ and $P^*_{i+1}$.
Similarly, $\rset^*\subseteq \rset_0$, and the paths in $\rset^*$ are indexed according to their order in $\oset_{\rset_0}$. We have also defined the set  $\rset_1\subseteq \rset_0$ of paths, containing all paths in sets $\set{\uset'_{2i-1}}_{i=1}^{\lambda'+1}$. As before, we re-index them as follows: for $1\leq i\leq\lambda'$, we set $\uset'_i=\uset'_{2i-1}$. Therefore, the paths of $\uset'_0$ lie before path $R^*_1$  in the ordering $\oset_{\rset_0}$, the paths of $\uset'_{\lambda'+1}$ lie after $R^*_{\lambda'}$ in this ordering, and, for $1\leq i<\lambda'$, the  paths of $\uset'_i$ lie between paths $R^*_i$ and $R^*_{i+1}$.



From our definition, if $\event_1$ did not happen, then for every pair $Q,Q'\in \pset^*\cup \qset^*$ of distinct paths, their images in $\phi^*$ do not cross (but note that the image of a single path may cross itself). 

We have also defined a set $\pset'\subseteq \pset_1$ and a set $\rset'\subseteq \rset_1$ of paths, containing all paths $Q$ whose image crosses the image of some path in $\rset^*\cup \pset^*$ in drawing $\phi^*$. From \Cref{obs: few bad paths}, if Event $\event_2$ does not happen, then $|\pset'|,|\rset'|\leq \psi/32$.
Note that the sets $\pset',\rset'$ of paths are not known to the algorithm.

It will be convenient for us to consider the $((\lambda'+1)\times (\lambda'+1))$-grid $\Pi^*$. We view the columns of the grid as corresponding to the left boundary of the bounding box $B^*$, the paths in $\set{R^*_1,\ldots,R^*_{\lambda'}}$, and the right boundary of the bounding box $B^*$.
For convenience, we index the columns of the grid from $0$ to $\lambda'+1$, so the left boundary of the bounding box corresponds to column $0$, and, for $1\leq i\leq \lambda'$, path $P^*_i$ represents the $i$th column of the grid, with the right boundary of $B^*$ repersenting the last column. Similarly, we view the bottom boundary of $B^*$, the paths in  $\set{P^*_1,\ldots,P^*_{\lambda'}}$, and the top boundary of $B^*$ as representing the rows of the grid, in the bottom-to-top order. As before, we index the rows of the grid so that the botommost row has index $0$ and the topmost row has index $\lambda'+1$. Notice however that the union of the paths in $\pset^*\cup \rset^*$ does not necessarily form a proper grid graph, as it is possible that, for a pair $P\in \pset^*$, $R\in \rset^*$ of paths, $P\cap R$ is a collection of several disjoint paths.

We will now consider the drawing $\phi^*$ of $H''$, and we will use it to define vertical and horizontal strips corresponding to paths in $\pset^*$ and $\rset^*$, respectively. We will also associate, with each cell of the grid $\Pi^*$, some region of the plane. We assume in the following definitions that Event $\event_1$ did not happen.


Consider first the image $\gamma_i$ of some path $P^*_i\in \pset^*$ in the drawing $\phi^*$.  Note that $\gamma_i$ is not necessarily a simple curve.
 We define two simple curves, $\gamma^t_i$ and $\gamma^b_i$, where $\gamma^t_i$ follows the image of $\gamma_i$ from the top, and $\gamma^b_i$ follows it from the bottom. In other words, we let $\gamma^b_i$ be a simple curve, whose every point lies on $\gamma_i$, that has the same endpoints as $\gamma_i$, such that the following holds: if $K^b_i$ is the area of the bounding box $B^*$ below $\gamma_i$, including $\gamma_i^t$, then $\gamma_i\subseteq K^b_i$. We define the other curve, $\gamma^b_i$ symmetrically, so curve $\gamma_i$ is contained in the disc whose boundary is $\gamma_i^t\cup \gamma_i^b$ (see \Cref{fig: top_bottom_curves}). For convenience, we let $\gamma_0^t$ be the bottom boundary of the bounding box $B^*$, and $\gamma_{\lambda'+1}^b$ be the top boundary of the bounding box $B^*$.
 We now define, for all $0\leq i\leq \lambda'$, a region of the plane that we call the $i$th horizontal strip, and denote by $\hstrip_i$. This strip is simply the closed region of the bounding box between the curves $\gamma_i^t$ and $\gamma_{i-1}^b$. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.35]{figs/top_curve.jpg}
\caption{An illustration of curves $\gamma^t_i$ and $\gamma^b_i$. The curve $\gamma_i$ is shown in purple.}\label{fig: top_bottom_curves}
\end{figure} 

For every vertical path $R^*_i\in \rset^*$, we also define two curves, $\gamma^{\ell}_i$ and $\gamma^r_i$, that follow the image $\gamma_i$ of $R^*_i$ in $\phi^*$ on its left and on its right, respectively. We denote by $\gamma_0^r$ the left boundary of the bounding box $B^*$, and by $\gamma_{\lambda'+1}^{\ell}$ its right boundary. For all $0\leq i\leq \lambda'$, we define a vertical strip $\vstrip_i$ to be the closed region of the bounding box $B^*$ betwen $\gamma_i^r$ and $\gamma_i^{\ell}$.

The following observation is immediate from the fact that the paths in $\pset_0$ are node-disjoint, and so are the paths in $\rset_0$.

\begin{observation}\label{obs: must cross chosen paths}
	If $R\in \rset_1$ is a path whose image in $\phi^*$ intersects the interior of more than one vertical strip in $\set{\vstrip_0,\ldots,\vstrip_{\lambda'+1}}$, then $R\in \rset'$. Similarly, if $P\in \pset_1$ is a path whose image in $\phi^*$ intersects the interior of more than one horizontal strip in $\set{\hstrip_0,\ldots,\hstrip_{\lambda'+1}}$, then $P\in \pset'$. 
\end{observation}

Lastly, for all $0\leq i,j\leq \lambda'$, we let $\cellr_{i,j}=\hstrip_i\cap \vstrip_j$ be a closed region of the plane that we associate with cell $\cell_{i,j}$ of the grid $\Pi^*$.
%\mynote{please define grid cells in prelims where grids are defined}



\iffalse
====================================

\highlightf{Calculations: heavy paths}

Path is heavy if it participates in $x$ crossings. All paths of skeleton will give $\lambda x$ crossings. Using $\lambda<\eta^2$, this is less than $x\eta^2$ crossings. This should be less than $\psi/16$. Because $\psi>\frac{16\tk}{\eta^2}$, enough that $x\eta^2<\tk/\eta^2$, or that $x<\tk/\eta^4$.

If we fix $x=\tk/\eta^4$. Then number of bad paths is at most: 

\[\frac{4\cro^*}{x}< 	\frac{\tilde k^2}{c_2\eta^5}/\frac{\tk}{\eta^4}=\frac{\tk}{c_2\eta}.  \]

A heavy path is selected with probability $1/\psi$. Probability that any heavy path is selected (from union bound) is at most:

\[ \frac{\tk}{c_2\eta\psi}. \]

If we use $\psi>\frac{16\tk}{\eta^2}$, this is not good enough. 

===============================

More detained calculation: all paths of skeleton will give $\lambda x$ crossings, and we want it to be less than $\psi/16$. so $x=\frac{\psi}{16\lambda}$ is fine. Now number of bad paths is at most:

\[\frac{4\cro^*}{x}< \frac{64\cro^*\lambda}{\psi}.\]

A heavy path is selected with probability $1/\psi$. Probability that any heavy path is selected (from union bound) is at most:

\[\frac{64\cro^*\lambda}{\psi^2}\]

So for us it is enough that $\cro^*<\psi^2\cdot 2^{12}/\lambda$.

We have:$ \psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$, so $\frac{\psi}{\lambda}\geq \frac{\alpha^*\tk}{128}$. Using $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, we get that $\frac{\psi}{\lambda}\geq \Omega(\frac{\alpha\alpha'\tk}{\log^4n})$.

So now $\psi^2/\lambda=\Omega (\frac{\psi\alpha\alpha'\tk}{\log^4n} )$.

Can use now $\psi>\frac{16\tk}{\eta^2}$, so the expression becomes:

\[\Omega (\frac{\tk^2\alpha\alpha'}{\eta^2\log^4n} )  \]

Lastly, because $\eta>\log^4n/(c^*\alpha\alpha')$, we get that $\cro^*<\tk^2/(c_2\eta^5)$ is good enough.

%Using $\psi=\Omega\left(\frac{\tk}{\eta}\cdot \frac{\alpha^5(\alpha')^2}{\log^8n}  \right)$, this is:


%\[\Omega (\frac{\tk^2\alpha^6(\alpha')^3}{\eta\log^{12}n} )\] 

=====================================
\fi




\subsection{Step 4: Constructing a Grid-Like Structure}

In this step we further delete some paths from sets $\rset_1$ and $\pset_1$ to ensure that the resulting paths form a grid-like structure. This is done in three stages. In the first stage, we discard some paths to ensure that every remaining path in $\rset_1$ intersects the paths in $\pset^*$ ``in order'' (we formally define this notion later), and process the paths in $\pset_1$ similarly. In the second stage, we associate, with every cell of the grid $\Pi^*$ a collection of horizontal paths and a collection of vertical paths. In the third stage, we ensure that for every cell of the grid $\Pi^*$, there are many inersections between its corresponding horizontal and vertical paths.

Before we continue, we discard some paths of $\rset^*\cup \pset^*$ that must lie in $\rset'\cup \pset'$. Specifically, consider some path $P\in \pset^*$, and assume that it lies in group $\uset_i$, for some $0\leq i\leq \lambda'+1$. Let $(a,a')$ be the endpoints of path $P$, with $a\in T_1$ and $a'\in T_3$. Notice that from the definition, if $i>0$, then $a$ must lie, in the ordering $\tilde\oset_1$ of the terminals of $T_1$, after the endpoint of the path $P^*_i$ that belongs to $T_1$. Similarly, if $i<\lambda'+1$, then $a$ must lie before the endpoin of the path $P^*_{i+1}$ that belongs to $T_1$ in the same ordering. In particular, we are guaranteed that in the drawing $\phi^*$, the image of $P$ must intersect the interior of the horizontal strip $\hstrip_i$. Consider now the endpoint $a'$ of $P$. If $i>0$, let $a'_i$ be the endpoint of path $P_i^*$ that lies in $T_3$, and if $i<\lambda'+1$, let $a'_{i+1}$ be the endpoint of path $P_{i'+1}$ that lies in $T_3$. Note that, if $a'$ lies before $a'_i$ in the ordering $\tilde\oset_3$ of $T_3$, or if $a'$ lies after $a'_{i+1}$ in the ordering $\tilde\oset_3$, then the image of $P$ has to intersect the interior of an additional horizontal strip, and, from \Cref{obs: must cross chosen paths}, path $P$ must lie in $\pset'$. We discard each such path from set $\pset_1$ (and from the corresponding set $U_i$). This ensures that, if $P\in U_i$, then its endpoint $a'$ must lie between $a'_i$ and $a'_{i+1}$ in $\tilde\oset_3$, if $1\leq i\leq \lambda'$; it must lie before $a'_{i+1}$ if $i=0$, and it must lie after $a'_i$ if $i=\lambda'+1$.
We process the paths in $\rset_1$ similarly, discarding paths as needed. Notice that so far all paths that we have discarded from $\pset_1\cup \rset_1$ lie in $\pset'\cup \rset'$.


\subsubsection{In-Order Intersection}

In this stage we discard some additional paths from $\pset_1\cup \rset_1$, to ensure that every remaining path in $\pset_1$ interesects the paths in $\rset^*$ in-order (notion that we define below); we do the same for paths in $\rset_1$. We will ensure that all paths discarded at this stage lie in $\pset'\cup \rset'$.

Since the definitions and the algorithms for the paths in $\pset_1$ and for the paths in $\rset_1$ are symmetric, we only describe the algorithm to process the paths in $\pset_1$ here.

Let $P\in \pset_1$ be any path, that we view as directed from its endpoint that lies in $T_1$ to its endpoint lying in $T_3$. Let $X(P)=\set{x_1,\ldots,x_r}$ denote all vertices of $P$ lying on paths in $R^*$, that is, $X(P)=V(P)\cap \left(\bigcup_{i=1}^{\lambda'}V(R^*_i)\right )$. We assume that the vertices of $X(P)$ are indexed in the order of their appearance on $P$. For each such vertex $x_j$, let $i_j$ be the index of the path $R^*_{i_j}\in \rset^*$ containing $x_j$.

\begin{definition}[In-order intersection]
	We say that path $P$ intersects the paths of $\rset^*$ in-order, iff $r\geq \lambda'$, $i_1=1$, $i_r=\lambda'$, and, for $1\leq j<r$, $|i_j-i_{j+1}|\leq 1$.
\end{definition}

Notice that the definition requires that path $P$ intersects every path of $\rset^*$ at least once; the first path of $\rset^*$ that it intersects must be $R_1^*$, and the last path must be $R_{\lambda'}^*$, and for every consecutive pair $x_j,x_{j+1}$ of vertices in $X(P)$, either both vertices lie on the same path of $\rset^*$, or they lie on consecutive paths of $\rset^*$. Notice that path $P$ is still allowed to intersect a path of $\rset^*$ many times, and may go back and forth across all these paths several times.

\begin{observation}\label{obs: not in order intersection}
	Assume that Event $\event_1$ did not happen. Let $P\in \pset_1$ be a path that  intersect the paths of $\rset^*$ not in-order. Then $P\in \pset'$ must hold.
\end{observation}

\begin{proof}
	Assume first that $i_1\neq 1$, that is, vertex $x_1$ lies on some path $R^*_i$ with $i\neq 1$. Let $p$ be a point on the image of path $P$ in $\phi^*$ that is very close to its first endpoint, so $p$ lies in the interior of the vertical strip $\vstrip_1$, and let $p'$ be the image of the point $x_1$. Clearly, $p'$ does not lie in the interior or on the boundary of $\vstrip_1$, so the image of path $P$ must cross the right boundary of $\vstrip_1$, which means that the image of some edge of $P$ and the image of some edge of $R_1^*$ cross in $\phi^*$.
	
	The cases where $i_{r}\neq \lambda'$, or there is an index $1\leq j<r$ with $i_j-i_{j+1}> 1$ are treated similarly, as is the case when $r<\lambda'$.
\end{proof}


We discard from $\pset_1$ all paths $P$ that intersect the paths of $\rset^*$ not in-order. We denote by $\pset_2\subseteq \pset_1$ the set of remaining paths. We also update the groups $\uset_0,\ldots,\uset_{\lambda'+1}$ accordingly. Observe that so far all paths that we have discarded from $\pset_1$ lie in  $\pset'$. 
From \Cref{obs: few bad paths}, assuming that Events $\event_1$ and $\event_2$ did not happen, the number of paths that we have discarded so far from $\pset_1$ is at most $\psi/32$. In particular, for all $0\leq i\leq \lambda'+1$, $|\uset_i|\geq 31\psi/32$ still holds.

We perform the same transformation on set $\rset_1$ of paths, obtaining a new set $\rset_2$ of paths, each of which intersects the paths of $\pset^*$ in-order. We also update the groups $\uset'_0,\ldots,\uset'_{\lambda'+1}$. As before, for all $0\leq i\leq \lambda'+1$, $|\uset'_i|\geq 31\psi/32$ still holds.






\subsubsection{Definining Paths Associated with Grid Cells}

For every path $P\in \pset_2$, for all $1\leq i\leq \lambda'$, we denote by $v_i(P)$ the first vertex on path $P$ that belongs to the vertical path $R^*_i$; note that, from the definition of in-order intersection, such a path must exist. For all $1\leq i< \lambda'$, we define the $i$th segment of $P$, $\sigma_i(P)$, to be the subpath of $P$ between $v_i(P)$ and $v_{i+1}(P)$. We also let $\sigma_0(P)$ be the subpath of $P$ from its first vertex (which must be a terminal of $T_1$) to $v_1(P)$, and by $\sigma_{\lambda'}(P)$ the subpath of $P$ from $v_{\lambda'}(P)$ to the last vertex of $P$ (which must be a terminal of $T_3)$. Note that the edges on paths $\sigma_0(P),\ldots,\sigma_{\lambda'}(P)$ partition $E(P)$.

Siilarly, for every path $R\in \rset_2$, for all $1\leq i\leq \lambda'$, we denote by $v_i(R)$ the first vertex on path $R$ that lies on the horizontal path $P^*_i$. For all $1\leq i< \lambda'$, we define the $i$th segment of $P$, $\sigma_i(R)$, to be the subpath of $R$ between $v_i(R)$ and $v_{i+1}(R)$. We also let $\sigma_0(R)$ be the subpath of $R$ from its first vertex (which must be a terminal of $T_4$) to $v_1(R)$, and by $\sigma_{\lambda'}(R)$ the subpath of $R$ from $v_{\lambda'}(R)$ to the last vertex of $R$ (which must be a terminal of $T_2$). 


Consider now some cell $\cell_{i,j}$ of the grid $\Pi^*$, for some $0\leq i,j\leq \lambda'+1$. We define the set $\pset^{i,j}$ of horizontal paths, and the set $\rset^{i,j}$ of vertical paths associated with cell $\cell_{i,j}$, as follows. In order to define the set $\pset^{i,j}$ of horizontal paths, we consider the group $\uset_i$, and, for every path $P\in \uset_i$, we include its $j$th segment $\sigma_j(P)$ in $\pset^{i,j}$, so that:
%
\[\pset^{i,j}=\set{\sigma_j(P)\mid P\in \uset_i}.\]
%	
Similarly, we define:
%	
\[\rset^{i,j}=\set{\sigma_i(R)\mid R\in \uset'_j}.\]
%	
\iffalse	
	Note that the definition of the sets $\pset^{i,j},\rset^{i,j}$ of paths depends on the definition of the direction of the paths in $\pset_2,\rset_2$. For example, recall that we think of the vertices of $T_1$ as lying on the left boundary of the bounding box $B^*$, and the vertices of $T_3$ as lying on its right boundary, with the paths in $\pset_2$ directed from left to right. If we were to flip the bounding box $B^*$, so that the vertices of $T_3$ appear on its left boundary and the vertices of $T_1$ on its right boundary, with the paths in $\pset$ directed from left to right, then the definition of the sets $\pset^{i,j}$ of paths may change (as a path in $\pset_2$ may intersect a path of $\rset^*$ numerous times). 
	However, if we flip the bounding box $B^*$, so that the vertices of $T_1$ appear on its bottom boundary, the vertices of $T_3$ on its top boundary, and the vertices of $T_2$ and $T_4$ on its left and right boundaries, respectively, directing the paths in $\pset$ from bottom to top, and the paths in $\rset$ from left to right, the definition of path sets $\set{\pset^{i,j},\rset^{i,j}}_{0\leq i,j\leq \lambda'+1}$ will now change (but now paths of $\pset$ become vertical and paths of $\rset$ become horizontal). This transformation corresponds to flipping the grid $\Pi^*$ along its diagonal (from bottom left to top right), and so the cells that lied in the top right quandrant of the grid remain in the top right quadrant. We may need to use this transformation later, but for now we stay with the original notation.
\fi
%
We need the following observation.
	
	\begin{observation}\label{obs: paths in cells don't cross}
		Let $P\in \uset_i,R\in \uset'_j$ be a pair of paths, for some $0\leq i,j\leq \lambda'+1$, and assume that their subpaths $\sigma_j(P)\subseteq P,\sigma_i(R)\subseteq R$ do not share any vertices. Then either $P\in \pset'$, or $R\in \rset'$, or the images of $\sigma_j(P)$ and $\sigma_i(R)$ cross in the drawing $\phi^*$.
	\end{observation}
\begin{proof}
	Assume that $P\not\in \pset'$ and $R\not\in \rset'$, that is, the images of the paths $P,R$ do not cross the images of the paths in $\pset^*\cup \rset^*$ in $\phi^*$. From the definition of set $\uset_i$, the image of $P$ intersects the interior of the horizontal strip $\hstrip_i$, and path $P$ does not share any vertices with the paths of $\pset^*$. Therefore, the image of $P$ must be contained in the strip $\hstrip_i$, and it is disjoint from its top and bottom boundaries $\gamma^b_i,\gamma^t_{i+1}$. Using similar reasoning, the image of $R$ is contained in the strip $\vstrip_j$, and it is disjoint from its left and right boundaries, $\gamma^{\ell}_j,\gamma^r_{j+1}$. Consider now the segment $\sigma_j(P)$ of $P$, whose endpoints lie on $R^*_j$ and $R^*_{j+1}$, respectively. Let $\sigma'_j(P)\subseteq \sigma_j(P)$ be the shortest subpath of $\sigma_j(P)$ whose first endpoint lies on $R^*_j$, and whose last endpoint lies on $R^*_{j+1}$; such a path must exist because we can let $\sigma'_j(P)=\sigma_j(P)$. From the definition of in-order intersection,  no inner vertex of $\sigma'_j$ may lie on any path of $\rset^*$. It is then easy to verify that the image of $\sigma'_j(P)$ in $\phi^*$ must be contained in $\cellr_{i,j}$, and it must split this region into two subregions: one whose top boundary contains a segment of $\gamma^b_{i+1}$, and one whose bottom boundary contains a segment of $\gamma^t_i$. 
	
	Using the same reasoning, we can select a segment $\sigma'_i(R)$, whose first endpoint lies on $P^*_i$, last endpoint lies on $P^*_{i+1}$, and all inner vertices are disjoint from the vertices lying on the paths in $\pset^*$.
	As before, the image of $\sigma'(R)$ must be contained in $\cellr_{i,j}$, but it connects a point on its top boundary to a point on its bottom boundary. Therefore, the image of $\sigma'_i(R)$ must cross the image of $\sigma'_j(P)$.
\end{proof}


\subsubsection{Completing the Construction of the Grid-Like Structure}


In order to complete the construction of the grid-like structure, we need to ensure that, for every pair $0\leq i,j\leq \lambda'+1$ of indices, there are many intersection between the sets $\pset^{i,j}$ and $\rset^{i,j}$ of paths. More specifically, we need to ensure that every path $\sigma\in \pset^{i,j}$ intersects many paths in $\rset^{i,j}$, and vice versa. This is needed in order to ensure well-linkedness properties: namely, that the collection of vertices containing the fist and the last vertex on every path of $\pset^{i,j}$ is sufficiently well-linked in the graph obtained from the union of the paths in $\rset^{i,j}\cup \pset^{i,j}$. This property, in turn, will be exploited in order to construct the sets $\qset$ of paths routing the terminals to sets of vertices $V(\Pi(v)))$ over which the distribution $\dset$ will be defined. This motivates the following definition.

\begin{definition}
	For a pair $0\leq i,j\leq \lambda'+1$ of indices, we say that a path $P\in \uset_i$ is \emph{bad for cell $\cell_{i,j}$} iff there are at least $\psi/16$ paths in $\rset^{i,j}$ that are disjoint from $\sigma_j(P)$. Similarly, we say that a path $R\in \uset'_j$ is bad for cell $\cell_{i,j}$ iff there are at least $\psi/16$ paths in $\pset^{i,j}$ that are disjoint from $\sigma_i(R)$.
\end{definition}

Consider now some index $0\leq i\leq \lambda'+1$. We say that a path $P\in \uset_i$ is \emph{bad} iff it is bad for at least one cell in $\set{\cell_{i,j}\mid 0\leq j\leq \lambda'+1}$. Similarly, for an index  $0\leq j\leq \lambda'+1$, a path $R\in \uset'_j$ is bad iff it is bad for at least one cell in $\set{\cell_{i,j}\mid 0\leq i\leq \lambda'+1}$. The following observation bounds the number of bad paths in each group $\uset_i$ of horizontal paths, and in each group $\uset'_j$ of vertical paths.


\begin{observation}\label{obs: few bad paths in each group}
Assume that $\cro^*\leq \frac{\tilde k^2}{c_2\eta^5}$, and that events $\event_1,\event_2$ did not happen. Then for all $0\leq i\leq \lambda'+1$, at most $\psi/16$ paths in $\uset_i$ are bad. Similarly, for all  $0\leq j\leq \lambda'+1$, at most $\psi/16$ paths in $\uset'_j$ are bad.
\end{observation}

\begin{proof}
Fix an index $0\leq i\leq \lambda'+1$, and the corresponding set $\uset_i\subseteq \pset_2$. We partition the set of all bad paths in $\uset_i$ into two subsets: set $\bset_1$ contains all bad paths lying in $\pset'$, and set $\bset_2$ contains all remaining bad paths. From \Cref{obs: few bad paths}, $|\bset_1|\leq \psi/32$.

We further partition the set $\bset_2$ of bad paths into subsets $\set{\bset_2^j\mid 0\leq j\leq \lambda'}$, where a path $P$ lies in $\bset_2^j$ if it is bad for cell $\cell_{i,j}$ (if path $P$ is bad for several cells, we add it to any of the corresponding sets). Consider now some index $0\leq j\leq \lambda'$, and some path $P\in \bset_2^j$. From the definition, there is a set $\Sigma'\subseteq \rset^{i,j}$ of at least $\psi/16$ paths that do not share any vertices with $P$. From \Cref{obs: few bad paths}, at most $\psi/32$ of these paths may lie in $\rset'$. Let $\Sigma''\subseteq \Sigma'$ be the collection of the remaining paths, whose cardinality is at least $\psi/32$. From \Cref{obs: paths in cells don't cross}, for every path $\sigma'\in \Sigma'$, the images of $\sigma_j(P)$, and of $\sigma'$ must cross. We let $\chi_j(P)$ denote the set of all crossings $(e,e')$, where $e\in \sigma_j(P)$, and $e'$ is an edge on a path in $\Sigma'$, so $|\chi_j(P)|\geq \psi/32$. We then let $\chi_{j}=\bigcup_{P\in \bset_2^j}\chi_j(P)$, so $|\chi_{j}|\geq |\bset_2^j|\cdot \psi/32$. Lastly, we let $\chi=\bigcup_{j=0}^{\lambda'+1}\chi_j$. Notice that set $\chi$ contains at least $|\bset_2|\cdot \psi/32$ distinct crossings in the drawing $\phi^*$. Assume for contradiction that $|\bset_2|>\psi/32$. Then:
%
\[\cro^*>\frac{\psi^2}{2^{10}}>\frac{\tk^2}{4\eta^4}>\frac{\tilde k^2}{c_2\eta^5},\]
%
since $\psi>\frac{16\tk}{\eta^2}$, a contradiction. 
Therefore, $|\bset_2|\leq \psi/32$, and overall there are at most $\psi/16$ bad paths in $\uset_i$.
The proof for path sets $\uset'_j\subseteq \rset_2$ is identical.
\end{proof}


For all $0\leq i\leq \lambda'+1$, we discard every bad path from $\uset_i$. If $|\uset_i| <\ceil{7\psi/8}$ for any $i$, then we terminate the algorithm and return FAIL. Notice that in this case, from \Cref{obs: few bad paths in each group}, if  $\cro^*< \frac{\tilde k^2}{c_2\eta^5}$, then at least one of the events $\event_1,\event_2$ must have happened, and the probability for this is at most $1/8$. Therefore, we assume that for all 
$0\leq i\leq \lambda'+1$, $|\uset_i|\geq \ceil{7\psi/8}$ holds. We discard additional arbitrary paths from $\uset_i$, until $|\uset_i|= \ceil{7\psi/8}$.
We then let $\pset_3=\bigcup_{i=0}^{\lambda'+1}\uset_i$ denote the resulting set of paths. 

Similarly, for all $0\leq j\leq \lambda'+1$, we discard every bad path from $\uset'_j$. If, as the result, $|\uset'_j|$ falls below  $\ceil{7\psi/8}$, we terminate the algorithm and return FAIL. Otherwise, we discard additional arbitrary paths as needed, so that $|\uset'_j|=\ceil{7\psi/8}$ holds. We also let $\rset_3=\bigcup_{j=0}^{\lambda'+1}\uset'_j$.


For all $0\leq i,j\leq \lambda'$, we also update the path sets $\pset^{i,j}$ and $\rset^{i,j}$ accordingly, discarding the paths that are no longer subpaths of paths in $\pset_3\cup \rset_3$. Since we are still guaranteed that $|\pset^{i,j}|,|\rset^{i,j}|= \ceil{7\psi/8}$, and since every path that is bad for cell $\cell_{i,j}$ was discarded, we are guaranteed that every path in $\pset^{i,j}$ intersects at least $\frac{7\psi}{8}-\frac{\psi}{16}=\frac{13\psi}{16}$ paths of $\rset^{i,j}$ and vice versa.
Since we use this fact later, we summarize it in the following observation.

\begin{observation}\label{obs: paths for cells}
	For all $0\leq i,j\leq \lambda'$, $|\pset^{i,j}|,|\rset^{i,j}|= \ceil{7\psi/8}$. Every path in 
$\pset^{i,j}$ intersects at least $\frac{13\psi}{16}$ paths of $\rset^{i,j}$ and vice versa.
\end{observation}

 This concludes the construction of the grid-like structure.

 


\subsection{Step 5: the Routing}


Recall that we have denoted by $\Lambda'$ the set of all pairs $(\qset,y)$, where $y$ is a vertex in graph $H$, and $\qset$ is a set of paths in graph $H''$, routing the set $\tT$ of terminals to vertices of $\Pi(y)$. In this final step we design an efficient algorithm to compute distribution $\dset$ over pairs $(\qset,y)\in \Lambda'$, such that for every outer edge $e\in E(H'')$, $\expect[(\qset,y)\in_{\dset}\Lambda']{(\cong_{H''}(\qset,e))^2}\leq  O\left (\frac{\log^{16}n}{(\alpha\alpha')^4}\right )$.


Our algorithm closely follows the arguments of 
\cite{Tasos-comm}  (see also Lemma D.10 in the full version of \cite{chuzhoy2011algorithm}), who showed a similar result for a grid graph. In order to provide intuition, we first present their algorithm. Assume that we are given a $(q\times q)$ grid graph $G$ for some integer $q$, and let $T$ be the set of vertices lying on the first row of the grid, that we refer to as terminals. For convenience, assume that $q$ is an integral power of $2$. Our goal is to compute a distribution $\dset'$ over pairs in $\Lambda(G,T)$. In other words, the distribution is over pairs $(\qset,v)$, where $v$ is a vertex of $G$, and $\qset$ is a set of paths routing the terminals to $v$. We need to ensure that for every edge $e\in E(G)$, the expectation $\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}\leq O(\log q)$.

For every vertex $v$ in the top right quadrant of the grid, we will define a set $\qset(v)$ of paths in $G$, routing the terminals in $T$ to $v$. Our distribution $\dset$ then assigns, to every pair $(\qset(v),v)$, where $v$ is a vertex of $G$ lying in the top right quadrant of the grid, the same probability value $4/q^2$.

We now fix a vertex $v$ in the top right quadrant of the grid, and define the set $\qset(v)$ of paths. Let $r=\log(q/4)$. For $1\leq i\leq r$, let $S_i$ be a square subgrid of $G$, of size $(2^i\times 2^i)$, whose upper right corner has the same column-index as vertex $v$, and the same row-index as the bottom left corner of $S_{i-1}$ (we think of $S_1$ as a $(1\times 1)$-grid consisting only of vertex $v$). 
We refer to the subgrids $S_i$ of $G$ as \emph{squares}, and specifically to square $S_i$ as \emph{level-$i$ square}.
For all $1\leq i\leq r$, we denote by $T_i$ the set of vertices lying on the bottom boundary of square $S_i$. Using the well-linkedness of the grids, it is easy to show that for all $1\leq i\leq r$, there is a collection $\pset_i$  of paths in graph $S_i$, routing vertices of $T_i$ to verticse of $T_{i-1}$ with congestion at most $2$, such that every vertex  of $T_{i-1}$ serves as endpoint of at most two such paths. For $1\leq i\leq r$, let
Let $\pset'_i$ be a multipset obtained from set $\pset_i$ by creating $2^{r-i+1}$ copies of every path in $\pset_i$. 
Let $T_{r+1}\subseteq T$ be a set of $|T_r|$ vertices lying on the bottom boundary of the grid $G$, that contains, for every vertex $t\in T_r$, vertex $t'$ on the bottom boundary of $G$ with the same column index as $t$. Let $P_t$ be the subpath of the corresponding column of $G$ connecting $t$ to $t'$, and denote $\pset'_{r+1}=\set{P_t\mid t\in T_r}$.

By concatenating the paths in $\pset_1',\ldots,\pset'_{r+1}$, we obtain a collection $\qset'(v)$ of paths in grid $G$, routing the terminals in $T_{r+1}$ to vertex $v$. 
%
Notice that for $1\leq i\leq r$, for every edge $e$ lying in $S_i$, the congestion on 
edge $e$ due to paths in $\qset(v)$ is at most $2^{r-i+2}$.
%
The key in analyzing the expectation $\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}$
is to notice that, for all $1\leq i\leq r$, square $S_i$ is a $(2^i\times 2^i)$-subgrid of $G$, whose upper right corner is chosen uniformly at random from a set of $q^2/4$ possible  points. The total number of subgrids of $G$ of size $(2^i\times 2^i)$ that contain $e$ is $2^{2i}$, so the probability that any of them is selected is bounded by $2^{2i+2}/q^2$. Therefore, for all $1\leq i\leq r$, with probability at most $2^{2i+2-2r}$, edge $e$ belongs to square $S_i$, and in this case, $\cong_G(\qset,e)\leq 2^{r-i+2}$. Therefore, we get that:
%
\[\expect[(\qset,v)\in_{\dset'}\Lambda(G,T)]{(\cong_G(\qset,e))^2}
\leq \sum_{i=1}^{r}2^{2i+2-2r}\cdot 2^{2r-2i+4}\leq O(r)=O(\log q).
\]
%
Using the well-linkedness of the terminals in $T$, it is immediate to extend the set $\qset(v)$ of paths to a set $\qset'(v)$ routing all terminals in $T$ to $v$, while increasing the congestion on every edge of $G$ by at most an additive constant and a multiplicative constant factor. This provides the final distribution $\dset$ over pairs $(\qset(v),v)\in \Lambda(G,T)$.



We will simulate a similar process on the grid $\Pi^*$, and its corresponding grid-like structure that we have constructed. Notice however that $\Pi^*$ is only a $(\lambda'\times\lambda')$-grid (where $\eta\leq \lambda'\leq \eta^2$), while the number of terminals that we need to route is much larger (comparable to $|\rset_3|$). Therefore, we will attempt to route all terminals to a single cell $\cell_{i,j}$ in the top right quadrant of the grid (in other words, we will route them to vertices lying on paths  in $\pset^{i,j}\cup \rset^{i,j}$). This in itself is not sufficient, since we need to route them to a set $V(\Pi(y))$ of vertices, corresponding to a single vertex $y$ of the original graph $H$. This means that we may need to perform some routing within the cell $\cell_{i,j}$, that is, within the graph obtained from the union of the paths in $\pset^{i,j}\cup \rset^{i,j}$. While generally such a routing may be difficult to compute, we will select a large collection of cells (called good cells) in the top right quadrant of the grid $\Pi^*$, in which such a routing is easy to obtain. We will then define, for each good cell, the corresponding set of paths routing the terminals to vertices of $V(\Pi(y))$, for some vertex $y\in V(H)$. We do so by simulating the process described above: we define square subgrids $\set{S_i}$ of the grid $\Pi^*$, and we associate these subgrids with sets of horizontal and vertical paths (subpaths of some paths in $\pset_3\cup \rset_3$), so that the desired well-linkedness properties of graphs corresponding to each subgrid $S_i$ are achieved. Eventually, the distribution $\dset$ chooses one of the good squares uniformly at random, and uses the associated pair $(\qset,y)\in \Lambda'$ in order to route the terminals to vertices of $\Pi(y)$. The analysis of expected congestion squared on every edge of $H''$ is very similar to the one outlined above.

We start by defining the notion of good cells of the grid $\Pi^*$, and showing that a large enough number of such cells exist in the upper right quadrant of $\Pi^*$. We will then define square subgrids of $\Pi^*$ and associate sets of paths with each such subgrid to ensure the required well-linkedness properties. Lastly, we show how to construct the desired routing $\qset$ for each good cell.


\subsubsection{Good Cells}


Fix a pair of indices $0\leq i,j\leq \lambda'$, and consider the cell $\cell_{i,j}$ of the grid $\Pi^*$, and the two corresponding sets $\pset^{i,j}$, $\rset^{i,j}$ of paths.


\begin{definition}[Good cells]
A path $\sigma\in \pset^{i,j}$ is \emph{good} for cell $\cell_{i,j}$ iff $\sigma$ contains no outer edges. 
We say that cell $\cell_{i,j}$ is \emph{good} iff some path $\sigma \in \pset^{i,j}$ is good for $\cell_{i,j}$; otherwise we say it is \emph{bad}. 
%A cell that is not good is called bad.
\end{definition}

Assume that cell $\cell_{i,j}$ is good, and let $\sigma\in \pset^{i,j}$ be any horizontal path that is good for this cell. Since $\sigma$ contains no outer edges, there must be a vertex $y\in V(H)$, such that $V(\sigma)\subseteq V(\Pi(y))$. Recall that, from \Cref{obs: paths for cells}, $|\rset^{i,j}|=\ceil{7\psi/8}$, and that $\sigma$ intersects at least $13\psi/16$ paths of $\rset^{i,j}$. Let $\hat \rset^{i,j}\subseteq \rset^{i,j}$ be a set of $\ceil{13\psi/16}$ paths, each of which shares at least one vertex with $\sigma$. Note that each such path then must contain a vertex of $\Pi(y)$. We denote by $\portals^{i,j}$ the set of vertices that contains, for every path $\sigma'\in \hat\rset^{i,j}$, the first vertex of $\sigma'$ (by definition, each such vertex must lie on path $P^*_i$ if $i>0$, or belong to $T_4$ otherwise). For convenience, we denote vertex $y$ by $y_{i,j}$.


Let $Z$ be the set of all pairs of indices $\floor{\lambda'/2}\leq i,j\leq \lambda'+1$, such that $\cell_{i,j}$ is good. Next, we show that $|Z|$ is sufficiently large. Our routing algorithm will then choose a pair $(i,j)$ of indices from $Z$ uniformly at random, and route the terminals to the vertices in set $\portals^{i,j}$, from where they will be routed to vertices of $\Pi(y_{i,j})$.


\begin{claim}\label{claim: many good cells}
	$|Z|\geq (\lambda')^2/16$.
\end{claim}

\begin{proof}
	Let $\bset$ be a collection of all bad cells $\cell_{i,j}$ lying in the top right quadrant, that is, $\floor{\lambda'/2}\leq i,j\leq \lambda'+1$. It is enough to show that $|\bset|<(\lambda')^2/16$.
	
	Consider now some bad cell $\cell_{i,j}\in \bset$. Consider now any path $Q\in \pset^{i,j}$. Since cell $\cell_{i,j}$ is bad, $Q$ must contain at least one outer edge. We say that $Q$ is a \emph{type-1} bad path for cell $\cell_{i,j}$ if it contains at least one type-1 outer edge (recall that a type-1 outer edge $e$ corresponds to some edge in graph $H$ that is {\bf not} contained in any cluster in $\cset$). Otherwise, every outer edge on path $Q$ is a type-2 outer edge, and in this case we say that $Q$ is a type-2 bad cluster for $\cell_{i,j}$. We say that cell $\cell_{i,j}$ is \emph{type-1 bad} iff at least $\psi/32$ paths of $\pset^{i,j}$ are type-1 bad for this cell, and otherwise it is type-2 bad. We partition the set $\bset$ of bad cells into two subsets: set $\bset_1$ contains all type-1 bad cells, and set $\bset_2$ contains all type-2 bad cells. It is now enough to prove that $|\bset_1|,|\bset_2|<(\lambda')^2/32$, which we do in the following two observations.
	
	
	\begin{observation}\label{obs: few type-1 bad cells}
		$|\bset_1|< (\lambda')^2/32$.
	\end{observation}
\begin{proof}
	Assume for contradiction that $|\bset_1|\geq (\lambda')^2/32$.
	Consider a type-1 bad cell $\cell_{i,j}\in \bset_1$, and let $\qset^{i,j}\subseteq \pset^{i,j}$ be a set of $\ceil{\psi/32}$ paths that are type-1 bad paths for cell $\cell_{i,j}$. Each path in $\qset^{i,j}$ must contain at least one type-1 bad edge. Since the paths in $\qset^{i,j}$ are edge-disjoint, there is a set $E^{i,j}$ of at least $\psi/32$ type-1 outer edges of $H''$, lying on paths of $\qset^{i,j}$. Since every edge of $H''$ may lie on at most one path in $\pset$, the total number of outer edges in $H''$ must be at least: 
%
\[\frac{|\bset_1|\cdot \psi}{32}\geq \frac{(\lambda')^2\cdot \psi}{2^{10}}\geq  \frac{\lambda^2\cdot \psi}{2^{14}} ,\] 
%
as $\lambda'=\floor{(\lambda-1)/2}\geq \lambda/4$.
Recall that $\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$ and $\lambda=\frac{2^{24}c\cdot \eta \log^8n}{\alpha^*\alpha^3}$,  where $c$ is the constant from \Cref{obs: few outer edges}. Therefore, we get that the total number of outer edges in $H''$ is at least $\frac{2c\tk \eta \log^8n}{\alpha^3}$, contradicting \Cref{obs: few outer edges}.
\end{proof}


\begin{observation}\label{obs: few type-1 bad cells}
	$|\bset_2|< (\lambda')^2/32$.
\end{observation}	
\begin{proof}
		For a cluster $C\in \cset$, let $X(C)=\bigcup_{y\in V(C)}V(\Pi(y))$. Note that all terminals of $H$ lie outside of the clusters in $\cset$, and so $X(C)\cap \tT=\emptyset$. If a path $Q\in \pset_3\cup \rset_3$ contains a vertex of $X(C)$, then it must contain at least one edge of $\delta_H(C)$. As the paths in $\pset\cup \rset$ cause edge-congestion at most $2$, the total number of paths $Q\in \pset\cup \rset$ with a non-empty intersection with $X(C)$ is at most $2\delta_H(C)$.
	
	
	Let $\intpairs\subseteq \pset_3\times\rset_3$ be the collection of all pairs of paths $P\in \pset_3$, $R\in \rset_3$, such that $P$ and $R$ share at least one vertex. 
	For a cluster $C\in \cset$, let $\intpairs'_C\subseteq \intpairs$ denote denote the collection of all pairs $(P,R)\in \intpairs$ of paths, such that some vertex $v\in X(C)$ lies on both $P$ and $R$. Clearly, if $(P,R)\in \intpairs_C'$, then each of the paths $P$, $R$ must contain at least one edge of $\delta_H(C)$. Therefore, from the above discussion, $|\intpairs'_C|\leq 4|\delta_H(C)|^2$. Let $\intpairs'=\bigcup_{C\in \cset}\intpairs'_C$. Then:
	%
	\[ |\intpairs'|\leq \sum_{C\in \cset}|\intpairs'_C|\leq  4\sum_{C\in \cset}|\delta_H(C)|^2. \]
	%
	From Equation \ref{eq: sum of squares} (see \Cref{step 2 summary}), $
	\sum_{C\in \cset}|\delta_H(C)|^2<\frac{(\tk\talpha\alpha')^2}{c_1\log^{20}n}$, so we get that:
	%
	\begin{equation}\label{eq: bounding num of intersection pairs}
	|\intpairs'|<\frac{4(\tk\talpha\alpha')^2}{c_1\log^{20}n},
	\end{equation} 
	%
	where $c_1$ is an arbitrary large enough constant.
	
	In the remainder of the proof, we assume for contradiction that $|\bset_2|\geq (\lambda')^2/32$, and we will show that $|\intpairs'|\geq \frac{4(\tk\talpha\alpha')^2}{c_1\log^{20}n}$ must hold, contradicting Equation \ref{eq: bounding num of intersection pairs}.
	

Consider a type-2 bad cell $\cell_{i,j}\in \bset_2$. Recall that every path in $\pset^{i,j}$ contains at least one outer edge, and at most $\psi/32$ such paths contain a type-1 bad edge. Since, from \Cref{obs: paths for cells}, $|\pset^{i,j}|= \ceil{7\psi/8}$, 
there is a collection $\Sigma\subseteq \pset^{i,j}$ of at least  $3\psi/4$ paths $P$, such that all edges on $P$ are either inner edges, or type-2 outer edges. Therefore, if $P\in \Sigma$ is any such path, then there is some cluster $C\in \cset$ with $V(P)\subseteq X(C)$. Recall that, from \Cref{obs: paths for cells}, each path $P\in \Sigma$ intersects at least $\frac{13\psi}{16}$ paths of $\rset^{i,j}$. Clearly, if a path $R\in \rset^{i,j}$ intersects a path $P\in \Sigma$, then $(P,R)\in \intpairs'$. Therefore, intersections between pairs of paths in $\pset^{i,j}\times \rset^{i,j}$ contribute at least $\frac{13\psi}{16}\cdot \frac{3\psi}{4}\geq \frac{\psi^2}{2}$ pairs to set $\intpairs'$.
Therfore, if we denote by $\intpairs'_{i,j}$ the collection of all pairs $(P,R)\in \intpairs'$, where a subpath $\sigma$ of $P$ lies in $\pset^{i,j}$,  and a subpath $\sigma'$ of $R$ lies in $\pset^{i,j}$, and $\sigma,\sigma'$ contain a vertex $v\in X(C)$, for some cluster $C\in \cset$, then, from the above discussion, $|\intpairs'_{i,j}|\geq \frac{\psi^2}{2}$. We claim that for every pair $(P,R)\in \intpairs'$ of paths, there is at most one pair of indices $0\leq i,j\leq \lambda'+1$, such that $(P,R)\in \intpairs_{i,j}'$. Indeed, assume that $P\in \uset_i$ and $R\in \uset'_j$. For a pair $0\leq i',j'\leq \lambda'+1$ of indices, $\pset^{i',j'}$ contains a subpath of $P$ iff $i'=i$, and $\rset^{i',j'}$ contains a subpath of $R$ iff $j'=j$. So the only pair $(i',j')$ of indices for which $(P,R) \in \intpairs'_{i',j'}$ may hold is $(i,j)$. Overall, we get that $|\intpairs'|\geq |\bset_2|\cdot \psi^2/2$. Assuming that $|\bset_2|\geq (\lambda')^2/32$, since $\lambda'=\floor{(\lambda-1)/2}\geq \lambda/4$, we get that $|\intpairs'|\geq \frac{\lambda^2\psi^2}{1024}$. 


Recall that $\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$, and $\alpha^*=\Theta(\talpha\alpha'/\log^4n)$. 
We conclude that:
%	
\[|\intpairs'|\geq \frac{(\alpha^*)^2\tk^2}{2^{22}}\geq \Omega\left( \frac{(\talpha\alpha'\tk)^2}{\log^8n} \right ).  \] 
%
Since we can choose $c_1$ to be a sufficiently large constant, this contradicts Equation \ref{eq: bounding num of intersection pairs}.
\end{proof}	
\end{proof}



\subsubsection{Square Subgrids and Corresponding Path Sets}

For integers $1\leq i,j\leq \lambda+1$ and $\ell\leq \min\set{i,j}$, a \emph{square subgrid $S(i,j,\ell)$ of $\Pi^*$} (that we also refer to as a \emph{square}) is defined as the collection of cells $\cellset(S)=\set{\cell_{i',j'}\mid i-\ell+1\leq i'\leq i;\quad j-\ell+1\leq j'\leq j}$. Intuitively, $S(i,j,\ell)$ is a subgrid of $\Pi^*$ of size $(\ell\times \ell)$, whose top right corner is the cell $\cell_{i,j}$.

Given a square $S=S(i,j,\ell)$, we associate with it a collection $\pset(S)$ of horizontal paths, and $\rset(S)$ of vertical paths, as follows. Intuitively,
consider the graph  obtained by taking the union of all paths $\pset^{i',j'}$, where $\cell_{i',j'}\in \cellset(S)$.
This graph is a collection of disjoint paths, each of which is a subpath of a distinct path in $\bigcup_{i'=i-\ell+1}^i\uset_{i'}$; we let $\pset(S)$ be this set of paths.
Formally, for all $i-\ell+1\leq i'\leq i$, for every path $P\in \uset_{i'}$, we include in $\pset(S)$ the subpath of $P$ from the first vertex of $\sigma_{j-\ell+1}(P)$ to the last vertex of $\sigma_{j}(P)$.
%
Similarly, set $\rset(S)$ contains, for all $j-\ell+1\leq j'\leq j$, for every path $R\in \uset'_{j'}$, the subpath of $R$ from the first vertex of $\sigma'_{i-\ell+1}(R)$ to the last vertex of $\sigma_{i}(R)$.
%
Notice that, from \Cref{obs: paths for cells}, $|\pset(S)|=|\rset(S)|= \ceil{7\psi/8}\cdot \ell$.

We denote by $\entryportals(S)$ the set of all vertices that serve as the first endpoint of the paths in $\pset(S)$, and by $\exitportals(S)$ the set of all vertices that serve as the last endpoint of the paths in $\pset(S)$. We denote by $G(S)$ the graph obtained by the union of the paths in $\pset(S)\cup \rset(S)$.


The following claim will be crucial for our algorithm for computing the routing paths for each good cell.

\begin{claim}\label{claim: routing in square}
Let $S=S(i,j,\ell)$ be a square of $\Pi^*$,	for some $1\leq i,j\leq \lambda+1$ and $\ell\leq \min\set{i,j}$, and let $Y\subseteq \entryportals(S)$, $Y'\subseteq\exitportals(S)$ be two subsets of vertices of cardinality $z$ each, where $z\leq \psi \ell/2$. Then there is a collection $\qset$ of edge-disjoint paths in graph $G(S)$, which is a one-to-one routing from $Y$ to $Y'$.
\end{claim}
\begin{proof}
	Assume for contradiction that the claim is false. Then, from the maximum flow / minimum cut theorem, there is a collection $E'$ of at most $z-1$ edges in graph $G(S)$, such that $G(S)\setminus E'$ contains no path connecting a vertex of $Y$ to a vertex of $Y'$. Recall that each vertex of $Y$ is an endpoint of a distinct path in $\pset(S)$, and all paths in $\pset(S)$ are edge-disjoint. Since $|Y|=z$, while $|E'|\leq z-1$, there is some path $P\in \pset(S)$, whose endpoint $y$ belongs to $Y$, such that $P$ contains no edge of $E'$. Using the same arguments, there is some path $P'\in \pset(S)$, whose endpoint $y'$ belongs to $Y'$, that contains no edge of $E'$. Clearly, $P\neq P'$ must hold, as otherwise there is a path in $G(S)\setminus E'$ connecting $y$ to $y'$ -- the path $P$. It is now enough to show that there is some path $R\in \rset(S)$, that contains no edge of $E'$, but $R\cap P\neq \emptyset$ and $R\cap P'\neq\emptyset$ hold. Indeed, in this case, $P\cup R\cup P'\subseteq G(S)\setminus E'$, and so $y$ remains connected to $y'$ in $G(S)\setminus E'$.
	
	We now show that path $R$ with such properties must exist. Let $\tilde P\in \pset_0$ be the path with $P\subseteq \tilde P$, and assume that $\tilde P\in \uset_{i'}$ Similarly, let $\tilde P'\in \pset_0$ be the path with $P'\subseteq \tilde P'$, and assume that $\tilde P'\in \uset_{i''}$ (where possibly $i'=i''$). Consider some index $j-\ell'+1\leq j'\leq \ell$. Recall
	$|\uset'_{j'}|=\ceil{7\psi/8}$, and, for every path $R\in \uset'_{j'}$, segment $\sigma_{i'}(R)$, lies in $\rset^{i',j'}$, and segment $\sigma'_{i''}(R)$ lies in $\rset^{i'',j'}$. Moreover, from \Cref{obs: paths for cells}, path $\sigma_{j'}(\tilde P)$ must intersect at least $\frac{13\psi}{16}$ paths of $\set{\sigma_{i'}(R)\mid \uset'_{j'}}$, and 
	similarly path $\sigma_{j'}(\tilde P')$ must intersect at least $\frac{13\psi}{16}$ paths of $\set{\sigma_{i''}(R)\mid \uset'_{j'}}$.
	 Therefore, there is a subset $\uset''_{j'}\subseteq \uset'_{j'}$ of at least $\psi/2$ paths $R$, such that both $P$ and $P'$ intersect the subpath of $R$ that belongs to $\rset(S)$. Overall, there are at least $\ell \psi/2$ paths $R\in \rset(S)$ that intersect the subpaths of $P$ and of $P'$ that lie in $\pset(S)$. Since $z\leq \ell\psi/2$, at least one such path is disjoint from $E'$.
\end{proof}



\subsubsection{Routing the Terminals to Good Cells}



We fix some good cell $\cell_{i,j}$ in the top right quadrant of the grid, that is, $\lambda'/2\leq i,j\leq\lambda'-1$. Recall that we have defined  a vertex $y_{i,j}\in V(H)$, and a collection $\hat \rset^{i,j}\subseteq \rset^{i,j}$ of $\psi'=\ceil{13\psi/16}$ paths, each of which contains a vertex of $\Pi(y_{i,j})$. We have also defined a set $\portals^{i,j}$ of vertices that contains, for every path $\sigma'\in \hat \rset^{i,j}$, the first vertex on $\sigma'$.

We define a set $\qset_{i,j}$ of paths in $H''$, routing the terminals of $\tT$ to vertices of $\Pi(y_{i,j})$, so $(\qset_{i,j},y_{i,j})\in \Lambda'$. In order to do so, we first define a path set $\qset'_{i,j}$, routing a constant fraction of the terminals of $T_4$ to vertices of $\Pi(y_{i,j})$, and then extend this path set in order to obtain routing of all terminals to vertices of $\Pi(y_{i,j})$.


\paragraph{Routing to $\cell_{i,j}$.}
In order to define the routing, we let $z=\floor{\log(\lambda'/4)}$, and we define $z+1$ squares $S_0^{i,j},S_1^{i,j},\ldots,S_z^{i,j}$. In order to simplify the notation, we will omit the superscript $i,j$ for now.

Square $S_0$ is $S(i,j,1)$, so it consists of a single cell $\cell_{i,j}$. We denote by $\portals_0^{i,j}=\portals^{i,j}$ the set of $\psi'$ vertices that we have defined. We let $\qset_0$ be the set of $\psi'$ paths, containing, for every path $\sigma'\in \hat\rset^{i,j}$, a subpath of $\sigma'$ between a vertex of $\portals_0^{i,j}$ and a vertex of $\Pi(y_{i,j})$. Therefore, $\qset_0$ is a set of $\psi'$ edge-disjoint paths, routing vertices of $\portals_0^{i,j}$ to vertices of $\Pi(y_{i,j})$, and all paths of $\qset_0$ are contained in $\rset(S_0)$. We say that cell $\cell_{i,j}$ is the bottom right corner of square $S_0$.

Fix some index $1\leq r\leq z$, and 
assume that we have defined squares $S_0,\ldots,S_{r-1}$. We now   define square $S_r$. We let $S_r=(i_r,j,2^r)$, so the length of the side of the square is $2^r$, and the coordinates of the top right corner of $S_r$ are $(i_r,j)$; here, $j$ is the column index of the initial cell $\cell_{i,j}$, and $i_r$ is the cell immediately under the right bottom corner cell of $S_{r-1}$. In other words, if $S_{r-1}=(i_{r-1},j,2^{r-1})$, then $i_r=i_{r-1}+2^{r-1}$.
We assume that we have also defined a collection $\portals_{r-1}\subseteq \entryportals(S_{r-1})$, containing $2^{r-1}\cdot \psi'$ vertices. Note that the top boundary of square $S_r$ appears immediately under bottom boundary of square $S_{r-1}$, so $\entryportals(S_{r-1})\subseteq \exitportals(S_r)$, and in particular $\portals_{r-1}\subseteq \exitportals(S_r)$. We select an arbitrary subset $\portals_r\subseteq \entryportals(S_r)$ of $2^r\cdot \psi'$ vertices. By partitioning set $\portals_r$ into two equal-cardinality subsets $Y_1,Y_2$, and applying \Cref{claim: routing in square} to each of them separately, we obtain two collections $\qset_{r}^1,\qset_{r}^2$ of edge-disjoint paths in graph $G(S_r)$, routing vertex sets $Y_1$ and $Y_2$, respectively, to vertex set $\portals_{r-1}$, in a one-to-one routing. Therefore, there is a set $\qset_{r}$ of paths in  $G(S_r)$, routing vertex set $\portals_r$ to vertex set $\portals_{r-1}$ with edge-congestion at most $2$, such that every vertex in $\portals_{r-1}$ is an endpoint of at most two such paths. Moreover, we can compute such set $\qset_r$ of paths efficiently via standard maximum flow.

Lastly, consider the last square $S_z$. We define a subset $T^*\subseteq T_4$ of terminals, as follows. For every vertex $v\in \portals_z$, let $R_v\in \rset$ be the vertical path containing $v$, and let $t_v\in T_4$ be the terminal that serves as an endpoint of path $R_v$. We then let $T^*=\set{t_v\mid v\in \portals_z}$, and we let $\qset_{z+1}$ be a set of paths containing, for every vertex $v\in \portals_z$, the subpath of $R_v$ between $t_v$ and $v$. Therefore, set $\qset_{z+1}$ of paths routes terminals of $T^*$ to vertices of $\portals_z$, and the paths in $\qset_{z+1}$ are edge-disjoint. It is also easy to verify that the paths in $\qset_{z+1}$ do not contain any edges from graphs $G(S_0)\cup \cdots\cup G(S_z)$.
Note that, since $\psi=\floor{\frac{\alpha^*\tk}{64\lambda}}$ and  $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$,
%
\[|T^*|=2^z\cdot \psi'= 2^{\floor{\log(\lambda'/4)}}\cdot \ceil{13\psi/16}=\Omega(\lambda'\cdot \psi)=\Omega(\lambda\psi)=\Omega(\alpha^*\tk)=\Omega(\tk\alpha\alpha'/\log^4n).
\]
%


To summarize, we have defined a collection $\set{S_0,\ldots,S_z}$ of squares in the grid $\Pi^*$, where for all $0\leq r\leq z$, square $S_r$ has dimensions $(2^r\times 2^r)$. The squares are aligned on the right, and are stacked on top of each other, with square $S_0$ containing a single cell, $\cell_{i,j}$. This guarantees that all corresponding graphs $G(S_r)$ are mutually disjoint, except that, for all $0\leq r<z$, $V(S_r)\cap V(S_{r+1})=\entryportals(S_r)$. We have defined, for all $0\leq r\leq z$, a set $\portals_r\subseteq \entryportals(S_r)$ of $2^r\cdot \psi'$ vertices, and a set $\qset_r$ of paths contained in $G(S_r)$, routing vertices of $\portals_r$ to vertices of $\portals_{r-1}$ with edge-congestion at most $2$, so that every vertex of $\portals_{r-1}$ serves as an endpoint of at most two such paths. Additionally, in graph $G(S_0)$, we have defined a set $\qset_0$ of $\psi'$ paths routing vertices of $\portals_0$ to vertices of $\Pi(y_{i,j})$, and an additional set $\qset_{z+1}$ of edge-disjoint paths routing terminals in $T^*$ to vertices of $\portals_z$ in a one-to-one routing, so that paths in $\qset_{z+1}$ do not contain edges of $G(S_0)\cup\cdots\cup G(S_z)$.

We are now ready to define a set $\qset'_{i,j}$ of paths, routing terminals of $T^*$ to vertices of $\Pi(y_{i,j})$. In order to do so, for all $0\leq r\leq z$, we let $\qset'_r$ be a multi-set of paths, contianing, for every path $\sigma'\in \qset_r$, $2^{z-r}$ copies of the path $\sigma'$. Therefore, paths in $\qset'_r$ cause edge-congestion $2^{z-r+1}$ in $G(S_r)$. Set $\qset'_{i,j}$ of paths is obtained by concatenating paths in sets $\qset_{z+1},\qset'_z,\ldots,\qset'_0$. It is easy to verify that paths in $\qset'_{i,j}$ route all terminals in $T^*$ to vertices of $\Pi(y_{i,j})$. 



Recall that $|T^*|=\Omega(\tk\alpha\alpha'/\log^4n)$, and $|\tT|=\tk$. 
Moreover, from \Cref{obs: terminals well linked in H''},
	The set $\tT$ of terminals is $\alpha^*$-well-linked in $H''$, where $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$.
From \Cref{lem: routing path extension}, 
there is a set $\qset_{i,j}$ of paths in graph $H''$, routing all vertices of $\tT$ to vertices of $\Pi(y_{i,j})$, such that, for every edge $e\in E(H'')$:
%
\[\cong_{H''}(\qset_{i,j},e)\le 
\ceil{\frac{\tk}{|T^*|}}\left (\cong_{H''}(\qset'_{i,j},e)+\ceil{1/\alpha^*}\right )\leq 
O\left (\frac{\log^4n}{\alpha\alpha'}\right )\cdot \left(\cong_{H''}(\qset'_{i,j},e)+\frac{\log^4n}{\alpha\alpha'}\right ).\]



\paragraph{Distribution $\dset$ and Analysis.}

The final distribution $\dset$ over pairs in $\Lambda'$ is defined as follows. For every pair $(i,j)$ of indices in $Z$, pair $(\qset_{i,j},y_{i,j})$ is assigned the same distribution $1/|Z|$; recall that, from \Cref{claim: many good cells}, 
	$|Z|\geq (\lambda')^2/16$.
	

We now fix some vertex $e\in E(H'')$, and analyze the expectation $\expect[(\qset_{i,j},y_{i,j})\in_\dset \Lambda']{(\cong_{H''}(\qset_{i,j},e))^2}$.

Recall that there is at most one path $P\in \pset$ that contains $e$, and at most one path $R\in \rset$ containing $e$. Moreover, there is at most one pair $(i_1,j_1)$ of indices with $e\in \sigma_{i_1,j_1}(P)$, and at most one pair $(i_2,j_2)$ of indices with $e\in \sigma_{i_2,j_2}(R)$.

We first focus on pair $(i_1,j_1)$ of indices, and the corresponding cell $\cell_{i_1,j_1}$. Fix some pair $(i,j)\in Z$ of indices, and $0\leq r\leq z$. If $\cell_{i_1,j_1}\in S_r^{i,j}$, then segment $\sigma_{i_1,j_1}(P)$ of $P$ may lie on at most $2^{z-r+1}$ paths in $\qset'_{i,j}$. Notice that there are at most $2^{2r+2}$ square subgrids $S$ of $\Pi^*$ of dimension $(2^r\times 2^r)$, that contain the cell $\cell_{i_1,j_1}$. For each such square $S$, there is exactly one pair $(i(S),j(S))$ of indices, for which $S_r^{i(S),j(S)}=S$. Since $|Z|\geq  (\lambda')^2/16$, the probability that an index $(i,j)\in Z$ is chosen for which $\cell_{i_1,j_1}$ lies in the square $S_r^{i,j}$ is at most $O(2^{2r+2}/(\lambda')^2)$. Recall that, if $\cell_{i_1,j_1}\in S_r^{i,j}$, then $\cong_{H''}(\qset'_{i,j})\leq 2^{z-r+1}\leq O(\lambda'/2^r)$. Moreover, if $\cell_{i_1,j_1}$ does not lie in any of the squares $S_0^{i,j},\ldots,S_z^{i,j}$, then $\cong_{H''}(\qset'_{i,j})\leq 1$. The analysis for cell $\cell_{i_2,j_2}$ is symmetric. Therefore, altogether (now taking into account both the cells $\cell_{i_1,j_1}$ and $\cell_{i_2,j_2}$), we get that:
%
\[\expect[(i,j)\in Z]{(\cong_{H''}(\qset'_{i,j},e))^2}\leq O(1)+\sum_{r=0}^zO\left (\frac{2^{2r+2}}{(\lambda')^2}\cdot\frac{(\lambda')^2}{2^{2r}}\right )=O\left( 
\frac{2^z}{\lambda'}\right )=O(z)\leq O(\log n).
\] 
%
Lastly, since $\cong_{H''}(\qset_{i,j},e)\le 
O\left (\frac{\log^4n}{\alpha\alpha'}\right )\cdot \left(\cong_{H''}(\qset'_{i,j},e)+\frac{\log^4n}{\alpha\alpha'}\right )$, we get that:
%
\[\expect[(\qset_{i,j},y_{i,j})\in_\dset \Lambda']{(\cong_{H''}(\qset_{i,j},e))^2}\leq O\left (\frac{\log^{16}n}{(\alpha\alpha')^4}\right ).\]
%
\iffalse
Good cell part:

will only look at cells in top left quadrant. May need to swap horizontal and vertical. Not completely symmetric b/c of bottom-up / left-right direction of paths (the segment are defined w.r.t. this direction).

A horizontal path $P$ is good for cell $(i,j)$ iff its segment contains no outer edges, so it is contained in $\Pi(v)$ of some vertex $v$. A cell is good if it has at least one good path. This means that all vertical paths in the cell also visit $\Pi(v)$ in the cell. We want to prove that at least $0.8$-fraction of the cells are good.

In a bad cell, partition paths into two types: type-1 path for cell $(i,j)$ contains an outer edge that is not contained in any cluster (type-1 outer edge), otherwise type-2. A bad cell is type-1 if at least 0.1-frac of the horizontal paths are type-1 for the cell, and type-2 otherwise.

If we have many type-1 cells, then we have about $\psi\lambda^2=\alpha^*\tk\lambda$ type-1 outer edges, contradicting Obs. 6.9.

(need to do same analysis with horizontal paths, there is no choice).

So at the end we'll have a constant fraction of cells that are type-2 cells for both vertical and horizontal paths. In each such cell we'll have about $\psi^2$ pairs of paths meet at vertices that are inner to clusters. So overall, we have $(\lambda^2\psi^2)$ pairs of paths meeting at vertices that are inner to clusters. but for a cluster $C$, we have at most $|\delta(C)|$ paths entering it, so at most $|\delta(C)|^2$ pairs of paths can meet in inner vertices of $C$. So total number of such intersections is at most $\sum_{C\in \cset}|\delta(C)|^2$, which should hopefully be less than $(\lambda\psi)^2=(\alpha^*)^2\tk^2$. We currently only have $\sum_C|\delta(C)|^2<(\tk\talpha\alpha')^2/\log^{20}n$. $\alpha^*=\Theta(\alpha\alpha'/\log^4n)$, so looks OK.



\subsection{Plan for the rest of the proof}
\begin{itemize}
	\item select 1 path in $z$, where for example $z=\eta$, though can also use $\eta^2$. Will get a grid skeleton of size $z\times z$. 
	
	\item before that, throw away all paths that have more than $\eta/\alpha$ outer edges on them. Most paths will stay.
	
	\item now if we look at a vertical path, it has few outer edges, so for most cells it goes through it does not use an outer edge. Which means that all horizontal paths going through that cell meet in a single vertex (or go through a single cluster). Call such a cell good.
	
	\item at least half the cells are good. In a type-1 good cell all horizontal paths go through a single regular vertex. In a type-2 good cell they all go through 1 cluster. The hope is that there are few type-2 good cells.
	
	\item why: we have about $z^2$ good cells. Inside all good cells there are about $k^2/z^2$ inner edges (can make a cell good if both all horizontal paths meet at some vertex, and all vertical paths meet at some vertex, and then it should be the same vertex). The hope is that the clusters can only contribute $\sum_C|\delta(C)|^2$ vertices to the grid. This is because, if we look at a cluster $C$, the total number of vertical/horizontal paths entering $C$ is at most $\delta(C)$. Even if all pairs have their intersections inside this cluster, it can't contribute more than $|\delta(C)|^2$ such intersecting pairs. 
\end{itemize}
\fi









\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Leftovers%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
contracted graph $\hat H=H_{|\cset}$. Let $U=\set{v(C)\mid C\in \cset}$ be the set of super-node vertices of $\hH$, and let $U'$ be the set of all remaining vertices. We define a rotation system $\hat \Sigma$ for graph $\hat H$  as follows: for a super-node $v(C)\in U$, we let $\oset_{v(C)}$ be an arbitrary ordering of the edges incident to $v(C)$, and for a regular vertex $u\in U'$, we let $\oset_u$ be identical to the ordering in the rotation system $\Sigma$ in instance $I$. Recall that, from \Cref{lem: crossings in contr graph},  there is a drawing $\phi$ of $\hH$,  containing at most $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)$ crossings, such that for every regular vertex $u\in U'$, the ordering of the edges of $\delta_{\hH}(u)$ as they enter $u$ in $\phi$ is consistent with $\oset_u\in \Sigma$. We can use this drawing in order to define a solution $\phi'$ to instance $\hat I=(\hH,\hat \Sigma)$ of the \cnwrs problem, by reordering the edges entering every super-node $v(C)$ as needed. This can be done so that $\cro(\phi')\leq \cro(\phi)+\sum_{C\in \cset'}|\delta_H(C)|^2\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$. Therefore, $\optcrors(\hat I)\leq O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$.


We are now ready to define graph $\hH^+$. In order to do so, we start with graph $\hH$, and process every vertex $u\in V(\hH)\setminus T$ (that may be a regular vertex or a super-node one-by-one). Consider any such vertex $u$, and let $e_1,\ldots,e_{d(u)}$ be the edges incident to $u$ in $\hH$, indexed according to their ordering in $\oset_u\in \hat \Sigma$. We let $\Pi(u)$ be a $(d(u)\times d(u))$ vrid, and we denote the vertices on the first row of this grid by $s_1(u),\ldots,s_{d(u)}(u)$. We replace vertex $u$ with the grid $\Pi(u)$, and, for all $1\leq i\leq d(u)$, if $e_i=(u',u)$, then we replace $e_i$ with a new edge $e'_i=(u',s_i(u))$. Once every vertex of $V(\hH)\setminus T$ is processed, we obtain the final graph $\hH^+$. For every vertex $u$, we clall the edges of the grid $\Pi(u)$ \emph{inner edges}. We call all edges of $E(\hH^+)$ that are not inner edges \emph{outer edges}. Notice that there is a $1$-to-$1$ correspondence between the outer edges and the edges of graph $\hat H$. The following observation is immediate.

\begin{observation}\label{obs: expanded contracted graph}
	The set $T$ of terminals is $(\alpha\alpha')$-well-linked in $\hH^+$, and there is a drawing $\phi''$ of graph $\hH^+$ with at most  $O(\optcrors(I)\cdot \log^8n/(\alpha')^2)+k^2/x$ crossings, such that the inner edges do not participate in any crossings in $\phi''$.
\end{observation}
\fi
 








==> guiding-paths-prelims.tex <==
\subsection{Guiding Paths, Guided Orderings and Guided Rotation System}
\label{subsec: guiding paths and orderings}



\begin{definition}[Routing Paths inside and outside a Cluster]
	Let $G$ be a graph and let $C\subseteq G$ be a cluster of $G$. We say that a set $\qset(C)=\set{Q_e\mid e\in \delta_G(C)}$ of paths \emph{route the edges of $\delta_G(C)$ inside $C$ to a vertex $v\in V(C)$}, iff for all $e\in \delta_G(C)$, path $Q_e$ has $e$ as its first edge, $v$ as its last vertex, and $Q_e\setminus\set{e}$ is contained in $C$.
	We say that a set $\qset'(C)=\set{Q_e\mid e\in \delta_G(C)}$ of paths \emph{route the edges of $\delta_G(C)$ outside $C$ to a vertex $v'\in V(G)\setminus V(C)$}, iff for all $e\in \delta_G(C)$, path $Q_e$ has $e$ as its first edge, $v'$ as its last vertex, and $Q_e\setminus\set{e}$ is disjoint from $C$.
\end{definition}

\begin{definition}[Guiding Paths and Guiding Pairs]
	Let $(G,\Sigma)$ be an instance of \CNwRS, and let $C\subseteq G$ be a cluster of $G$. Let $v\in V(C)$ be any vertex of $C$, and let $\qset(C)$ be a set of paths that route the edges of $\delta_G(C)$ to $v$ inside $C$, such that the paths in $\qset(C)$ are  non-transversal with respect to $\Sigma$. We say that the set $\qset(C)$ is a \emph{set of guiding paths}, and $(v,\qset(C))$ is a \emph{guiding pair} for cluster $C$. We denote by $\Lambda(C)$ the set of all guiding pairs $(v,\qset(C))$.
\end{definition}




\paragraph{Guided Orderings.}
Let $(G,\Sigma)$ be an instance of \CNwRS, $C\subseteq G$ a cluster of $G$, and $(v,\qset)\in \Lambda(C)$ a guiding pair for cluster $C$. 
Recall that we are given an ordering $\oset_{v}\in \Sigma$ of the edges in $\delta_G(v)$. We use this ordering and the set $\qset$ of guiding paths in order to define a circular ordering of the edges of $\delta_G(C)$, as follows. 
Intuitively, this is the ordering in which the paths in $\qset$ enter $v$ under the ordering $\oset_v$.
Formally, for every path $Q\in \qset$, let $e^*(Q)$ be the last edge lying on path $Q$, which by definition belongs to $\delta_G(v)$. We first define a circular ordering of the paths in $\qset$, as follows: the paths are ordered according to the circular ordering of their last edges $e^*(Q)$ in $\oset_{v}\in \Sigma$, breaking ties arbitrarily. Since every path $Q\in \qset$ is associated with a unique edge in $\delta_G(C)$, that serves as the first edge on $Q$, this ordering of the paths in $\qset$ immediately defines a circular ordering of the edges of $\delta_G(C)$, that we refer to as the ordering guided by $\qset$ and $\Sigma$, and denote by $\oset^{\guided}(\qset,\Sigma)$.


\paragraph{Guided Rotation System in a Contracted Graph.}
Assume that we are given an instance $I=(G,\Sigma)$ be an instance of the \cnwrs problem, a collection $\cset$ of disjoint clusters of $G$, and, for every cluster $C\in \cset$, a vertex $u(C)\in V(C)$, together with a set $\qset(C)$ of paths that are non-transversal with respect to $\Sigma$, routing  the edges of $\delta_G(C)$ to $u(C)$ inside $C$. Let $G'=G_{|\cset}$ be the contracted graph of $G$ with respect to $G'$, and let $\Sigma'$ be a rotation system for $G'$ that is defined as follows: for 
every regular vertex $v\in V(G)\cap V(G')$, the ordering $\oset'_v\in \Sigma'$ of the edges of $\delta_{G'}(v)=\delta_G(v)$ is identical to the ordering $\oset_v\in \Sigma$; for every supernode $v_C$, where $C$ is a cluster in $\cset$, the ordering $\oset'_{v(C)}\in \Sigma'$ of the edges of $\delta_{G'}(v(C))$ is defined to be ordering guided by the set $\qset(C)$ of paths and the rotation system $\Sigma$.  We refer to $\Sigma'$ as the  \emph{rotation system guided by $(\cset,\set{\qset(C)}_{C\in \cset},\Sigma)$}.


We use the following lemma, whose proof appears in \Cref{apd: Proof of opt of contracted instance}.

\begin{lemma}
	\label{lem: opt of contracted instance}
	Let $I=(G,\Sigma)$ be an instance of the \cnwrs problem, let $\phi^*$ be an optimal solution for $I$, and let $\chi$ be the set of pairs $(e,e')$ of edges of $G$, whose images cross in $\phi^*$. Assume further that we are given a collection $\cset$ of disjoint clusters of $G$, and, for every cluster $C\in \cset$, a guiding pair $(u(C),\qset(C))\in \Lambda(C)$. Let $G'=G_{|\cset}$, and let $\Sigma'$ be the $(\cset,\set{\qset(C)}_{C\in \cset},\Sigma)$-guided rotation system for $G'$. 
	Denote $\qset=\bigcup_{C\in \cset}\qset(C)$.
	Then:
	\[\optcrors(G',\Sigma')\le \optcrors(G,\Sigma)+\sum_{C\in \cset}\sum_{e\in E(C)}(\cong_G(\qset,e))^2+\sum_{(e,e')\in \chi}\cong_G(\qset,e)\cdot \cong_G(\qset,e').\]
\end{lemma}



\mynote{please add proof}

\begin{corollary}\label{cor: bounding crossing number of contracted graph}
	Let $I=(G,\Sigma)$ be an instance of the \cnwrs problem, and let $\cset$ be a collection of disjoint clusters of $G$. Suppose we are given, for every cluster $C\in \cset$, a distribution $\dset(C)$ over guiding pairs $(u(C),\qset(C))\in \Lambda(C)$, such that for every edge $e\in E(C)$, $\expect[(u(C),\qset(C))\in_{\dset(C)} \Lambda(C)]{(\cong_G(\qset(C),e))^2}\leq \beta$, for some $\beta\geq 1$. Let $\Sigma'$ be the the $(\cset,\set{\qset(C)}_{C\in \cset},\Sigma)$-guided rotation system for $G'$, where for all $C\in \cset$, pair $(u(C),\qset(C))$ is drawn from the distribution $\dset(C)$ independently at random. Then:
	
	
	\[\expect{\optcrors(G',\Sigma')}\le 4\beta \left(\optcrors(G,\Sigma)+|E(G)|\right ).\]
\end{corollary}



\iffalse
\mynote{I need the following lemma (this was proved as part of Lemma 7.1, but I need this here as a separate lemma). We are given instance $I=(G,\Sigma)$, a collection $\cset$ of clusters, and for each cluster $C\in \cset$, a set $\qset(C)$ of paths routing $\delta(C)$ to vertex $u(C)$ inside $C$. We consider $G'=G_{|\cset}$ the contracted graph, for which we define rotation system $\Sigma'$ that is consistent with $\Sigma$, but for every supernode $v(C)$, we define the rotation to be the order in which the paths in $\qset(C)$ enter $u(C)$ (like we do in basic disengagement). The claim is that this instance has a solution whose value is the summation, over all crossings $(e,e')$ in the optimal solution of $\cong(e)\cdot \cong(e')$ plus $\sum_{C\in \cset}\sum_{e\in E(C)}(\cong(e))^2$, where all congestions are with respect to $\bigcup_{C\in \cset}\qset(C)$.}
\fi



==> helpful_and_unhelpful_backup.tex <==
\subsection{Disengagement of Nice Instances -- Proof of \Cref{thm: advanced disengagement - disengage nice instances}}
\label{subsec: disengagement with bad chain}


In this section we prove \Cref{thm: advanced disengagement - disengage nice instances}. 
\znote{later: change the random path sets to distribution}

Assume that we are given a graph $G$ and a set $\cset=\set{C_1,\ldots,C_r}$ of vertex-disjoint clusters in $G$, such that $\bigcup_{1\le i\le r}V(C_i)=V(G)$. 
For each $1\le i\le r$, we define $\hat E_i=E(C_i,C_{i+1})$,  $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$, and we denote by $E'$ the subset of $E(G)$ that contains all edges connecting a pair $C_i,C_j$ of distinct clusters with $j\ge i+2$.

For each $1\le i\le r$, we say that cluster $C_i\in \cset$ is \emph{\singlecore}, iff its has the $\alpha_0$-bandwidth property for $\alpha_0=1/\log ^3m$.
%
%\mynote{I think poor is not a good term. Not sure why you don't use helpful/unhelpful. Don't use "random paths" in the definition. Define sets $\Lambda'(C),\Lambda''$ of collections of routing paths like we did for regular routing paths, then define distributions over them, etc.}
%
For each $2\le i\le r-1$, we say that cluster $C_i$ is \emph{\dualcore}, iff there exist two vertices $u^{\lef}_i,u^{\rig}_i\in V(C_i)$, that we call the \emph{left center} and \emph{right center} of $C_i$, respectively, and three random sets $\qset^{\lef}_i,\qset^{\rig}_i,\qset^{\thr}_i$ of paths, such that
\begin{itemize}
\item the paths of $\qset^{\lef}_i$ route edges of $\hat E_{i-1}\cup E^{\lef}_{i}$ to vertex $u^{\lef}_i$ inside $C_{i}\cup C_{i+1}$, and for each edge $e\in E(C_{i}\cup C_{i+1})$, $\expect[]{(\cong_{G}(\qset_{i}^{\lef}, e))^2}\le \beta$;
\item the paths of $\qset^{\rig}_i$ route edges of $\hat E_{i}\cup E^{\rig}_{i}$ to vertex $u^{\rig}_i$ inside $C_{i}\cup C_{i-1}$; and for each edge $e\in E(C_{i}\cup C_{i-1})$, $\expect[]{(\cong_{G}(\qset_{i}^{\rig}, e))^2}\le \beta$; and
\item $|\qset^{\thr}_i|=|E^{\thr}_i|$, paths of $\qset^{\thr}_i$ connect vertex $u^{\lef}_i$ to vertex $u^{\rig}_i$ in $C_{i}$, and $\cong_{G}(\qset_{i}^{\thr}) \le O(1)$.
\end{itemize}

%\mynote{to make this lemma more readable, I would first define helpful clusters, as the ones that are well-linked. Then define set $\pset$ of paths and its properties, maybe give it a name? Then state the lemma. Definition "sequentially visits (and only visits)" is not good. You need to do it formally, e.g. partition the path into segments, etc.}

Consider now the graph $H=G_{\mid \cset}$, 
For each $1\leq i\leq r$, we denote by $x_i$ the vertex of graph $H$ that represents the cluster $C_i$. 
%We denote $S_i=\set{x_1,\ldots,x_i}$, and $\notS_i=\set{x_{i+1},\ldots,x_r}$.
Note that each edge in $\Eout(\cset)$ corresponds to an edge in $H$, and we do not distinguish between them.
%
We say that a path $P$ in $H$ is an \emph{auxiliary path} of an edge $e=(x_i,x_j)$ in $H$ (where $j\ge i+2$), iff $P=(e_i,\ldots,e_{j-1})$, where for each $i\le t\le j-1$, $e_t$ is an edge in $H$ connecting $x_t$ to $x_{t+1}$.
Since such an edge $e=(x_i,x_j)$ is also an edge of $G$, we also say that the path $P$ in $H$ is an auxiliary path for the edge $e$ in $G$.



In this section we prove the following lemma.

\begin{lemma}\label{lem: disengagement with routing}
There is an efficient randomized algorithm, that takes as input an instance $I=(G,\Sigma)$ of \CNwRS with $|E(G)|=m$, a sequence $\cset=\set{C_1,\ldots,C_r}$ of vertex-disjoint clusters of $G$ such that the vertex sets $\set{V(C)}_{C\in \cset}$ partition $V(G)$, and a set $\pset=\set{P_e\mid e\in E'}$ of paths in $H$, that contains, for each edge $e\in E'$, an auxiliary path $P_e$ of $e$, such that
\begin{itemize}
\item $\bigcup_{1\le i\le r}V(C_i)=V$;
\item clusters $C_1,C_r$ are \singlecore clusters; each of $C_2,\ldots, C_{r-1}$ is either a \singlecore cluster or an \dualcore cluster; and if $C_i$ is an \dualcore cluster, then both $C_{i-1},C_{i+1}$ are \singlecore clusters; and
%\item for each edge $e\in E'$ connecting a vertex of $C_i$ to a vertex of $C_j$ with $i<j$, the path $P_e$ sequentially visits (and only visits) clusters $C_i,C_{i+1},\ldots, C_j$; and moreover, for each \dualcore cluster $C_t$ (where $i<t<j$) that $P_e$ visits, the subpath of $P_e$ within $C_t$ contains special vertices $u^{\lef}_t$ and $u^{\rig}_t$; \mynote{I think these paths only exist for edges whose both endpoints don't lie in poor clusters?} and
\item $\cong_H(\pset)=O(1)$.
\end{itemize}
The algorithm computes an $O(\beta^2)$-decomposition $\iset$ of instance $I$ with respect to $\cset$.
Additionally, there is an efficient algorithm $\aset$, that, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$.
\end{lemma}

The algorithm consists of several steps, and will be described in the following subsections. 

\znote{to add a high level explanation here and in each subsection}


\subsubsection{Computing Guiding Paths}
\label{sec: guiding and auxiliary paths}

%\mynote{you need first to explain what you are trying to do here, before you explain how you are doing it. otherwise it's hard to read. I for one have no idea what you are doing here. Best to state a theorem that summarizes the result of this step.}

First, for each \singlecore cluster $C_i\in \cset$, we apply the algorithm \algclassifycluster from \Cref{thm:algclassifycluster} to the instance $(G,\Sigma)$ and cluster $C_i$, with parameter $p=1/n^{100}$.
If it returns a distribution $\dset(C_i)$ over sets of guiding paths in $\Lambda(C_i)$, such that $C_i$ is $\beta^*$-light with respect to $\dset(C_i)$ (recall that $\beta^*=2^{O(\sqrt{\log m}\log\log m)}$), then we continue to sample a set of guiding paths from $\dset(C_i)$. Let $\qset_i$ be the set we obtain, and let $u_i$ be the vertex of $C_i$ that serves as the common endpoint of all paths in $\qset_i$. If the algorithm \algclassifycluster returns FAIL, then consider the augmentation $C_i^+$ of cluster $C_i$ (see \Cref{def: Graph C^+}). We apply the algorithm from \Cref{lem: simple guiding paths} to graph $C^+_i$ and set $T(C_i)$ of its vertices, and let $u_i$ be the vertex and $\qset_i$ be the set of paths that we obtain. Clearly, $\qset_i$ can be also viewed as a set of paths routing edges of $\delta_G(C_i)$ to $u_i$. From \Cref{lem: simple guiding paths}, for each edge $e\in E(C_i)$, $\expect{\cong(\qset_i,e)}\leq  O(\log^4m/\alpha_0)$. Finally, for each \singlecore cluster $C_i$, and for each edge $e\in \delta(C_i)$, we denote by $Q_i(e)$ the path of $\qset_i$ that routes $e$ to $u_i$.

\textbf{Bad Event $\xi_i$.} For each $1\le i\le r$, we say that the event $\xi_i$ happens, iff $C_i$ is a \singlecore cluster and not an $\eta^*$-bad cluster, but the algorithm \algclassifycluster returns  FAIL on it.
From \Cref{thm:algclassifycluster}, $\Pr[\xi_i]\le 1/n^{100}$. Then from the union bound over all $1\le i\le r$, $\Pr[\bigcup_{1\le i\le r}\xi_i]\le O(n^{-99})$.


Then, for each \singlecore cluster $C_i$, we apply the algorithm from \Cref{lem: non_interfering_paths} to the set $\qset_i$ of paths and the rotation system $\Sigma$, and rename the resulting path set by $\qset_i$.
Similarly, for each \dualcore cluster $C_i$, we apply the algorithm from \Cref{lem: non_interfering_paths} to the sets $\qset_i^{\lef}, \qset_i^{\rig}, \qset_i^{\thr}$ of paths separately, and rename the resulting path sets by $\qset_i^{\lef}, \qset_i^{\rig}, \qset_i^{\thr}$, respectively.
Now we are guaranteed that, for each \singlecore cluster $C_i$, the set $\qset_i$ of paths is non-transversal with respect to $\Sigma$, and for each \dualcore cluster $C_i$, the sets $\qset_i^{\lef}, \qset_i^{\rig}, \qset_i^{\thr}$ of paths are non-transversal with respect to $\Sigma$.


\subsubsection{Computing Auxiliary Cycles}

\begin{claim}
\label{claim: compute routing cycles}
We can efficiently compute a set $\rset=\set{R_e\mid e\in E'}$ that contains, for each edge $e\in E'$, a path $R_e$ in $G$, such that 
\begin{itemize}
\item for each edge $e$ connects $C_i$ to $C_j$ with $j\ge i+2$, the path $R_e$ has endpoints $u'_i,u'_j$, where:
if $C_i$ is \singlecore, then $u'_i=u_i$, otherwise $u'_i=u^{\rig}_i$; and similarly if $C_i$ is \singlecore, then $u'_j=u_j$, otherwise $u'_j=u^{\lef}_j$;
\iffalse{clearer and longer explanation}
\begin{itemize}
\item if both $C_i, C_j$ are \singlecore clusters, then $R_e$ has endpoints $u_i,u_j$;
\item if both $C_i, C_j$ are \dualcore clusters, then $R_e$ has endpoints $u^{\rig}_i, u^{\lef}_j$;
\item if $C_i$ is \singlecore and $C_j$ is \dualcore, then $R_e$ has endpoints $u_i, u^{\lef}_j$;
\item if $C_i$ is \dualcore and $C_j$ is \singlecore, then $R_e$ has endpoints $u^{\rig}_i, u_j$;
\end{itemize}
\fi
\item for each edge $e$ connects $C_i$ to $C_j$ with $j\ge i+2$, the path $R_e$ can be partitioned into subpaths $R_e=(K_i,\hat e_i,K_{i+1},\hat e_{i+1},\ldots,\hat e_{j-1},K_j)$, where for each index $i\le t\le j$, $K_j$ is a subpath that lies entirely in $C_t$, and $\hat e_t$ is an edge of $\hat E_t$;
\item for each $e\in E(G)$, $\expect[]{(\cong_G(\rset,e))^2}\le \beta$.
\end{itemize}
\end{claim}


\begin{proof}
For convenience, for an edge $e\in E'$ connecting a vertex of $C_i$ to a vertex of $C_j$ with $j\ge i+2$, we say that $i$ is the \emph{left index} of $e$ (which we sometimes denote by $i_e$) and $j$ is the \emph{right index} of $e$ (which we sometimes denote by $j_e$). 

We will gradually construct all paths of $\set{R_e\mid e\in E'}$ simultaneously. We start by setting, for each $e\in E'$, the initial path $R_e$ to be an empty path, and then sequentially process clusters $C_1,\ldots, C_r$. Upon processing the cluster $C_t$, we will construct the subpath $K_t(e)$ and the edge $\hat e_{t+1}$ for every $e\in E'$.
%
We now describe the iteration of processing cluster $C_t$. 
Note that in this iteration, we only need to deal with edges of $E'$ with $i_e\le t\le j_e$.

Assume first that $C_t$ is a \singlecore cluster.
We denote by $E_t^*$ the set of edges in $E(\pset)$ that connects $x_t$ to $x_{t+1}$, namely $E^*_t=E(\pset)\cap E_H(x_t,x_{t+1})$. Note that $E^*_t$ is also a set of edges in $G$ connecting $C_t$ to $C_{t+1}$, so $E^*_t\subseteq \hat E_t$.
First, for each edge $e\in E'$ with right index $t$, all its subpaths $K_i(e),\hat e_i,\ldots,\hat e_{t-1}$ have already been constructed. We simply define $K_t(e)$ to be $Q_t(\hat e_{t-1})$, the path in $\qset_t$ routing edge $\hat e_{t-1}$ to $u_t$ in $C_t$.
Second, for each edge $e\in E'$ with left index $t$, we simply designate (arbitrarily) a distinct edge of $E^*_i$ as $\hat e_t$, and then define $K_t(e)$ to be $Q_t(\hat e_{t})$, the path in $\qset_t$ routing edge $\hat e_{t}$ to $u_t$ in $C_t$.
Finally, consider the set $\set{\hat e_{t-1}\mid i_e < t<j_e}$ and the set of edges in $E^*_t$ that are not yet designated as $\hat e_t$ for any edge of $E'$, that we denote by $E^{**}_t$. Clearly, these two sets are equal-cardinality subsets of $\delta_G(C_t)$.
Since cluster $C_i$ has the $\alpha_0$-bandwidth property, from \Cref{cor: bandwidth_means_boundary_well_linked}, we can efficiently compute an one-to-one routing $\kset_i$ of edges of $\set{\hat e_{t-1}\mid i_e < t<j_e}$ to edges of $E^{**}_i$, such that $\cong_G(\kset_i)=\ceil{1/\alpha_0}$. Now for each edge $e\in E'$ with $i_e < t<j_e$, we designate the path in $\kset_i$ that starts at its previously constructed segment $\hat e_{t-1}$ as $K_t(e)$, and designate the last edge of $K_t(e)$ in $E^{**}_i$ as $\hat e_t$.


 

Assume now that $C_t$ is an \dualcore cluster. 
First, for each edge $e\in E'$ with right index $t$, the edge $\hat e_{t-1}$ has been defined in previous iterations, and we simply define $K_t(e)$ to be $Q^{\lef}_t(\hat e_{t-1})$, the path in $\qset^{\lef}_t$ routing edge $\hat e_{t-1}$ to $u_t$ in $C_t$.
Second, for each edge $e\in E'$ with left index $t$, we simply designate (arbitrarily) a distinct edge of $E^*_t$ as $\hat e_t$, and then define $K_t(e)$ to be $Q_t(\hat e_{t})$, the path in $\qset_t$ routing edge $\hat e_{t}$ to $u_t$ in $C_t$.
Finally, consider the edges of $E^{\thr}_t$ (namely edges $e$ with $i_e < t<j_e$). We denote by $E^{**}_t$ the set of edges in $E^*_t$ that are not designated as $\hat e_t$ for any edge of $E'$. For each edge $e\in E^{\thr}_t$, we designate a distinct edge of $E^{**}_t$ as $\hat e_t$, such that every edge of $E^{**}_t$ is assigned to exactly one edge of $ E^{\thr}_t$. Recall that we are given three sets of paths $\qset^{\lef}_i,\qset^{\rig}_i,\qset^{\thr}_i$. 
For each edge $e\in E^{\thr}_t$, we define $K_t(e)$ as the concatenation of (i) $Q^{\lef}_t(\hat e_{t-1})$, the path in $\qset_{t}^{\lef}$ that routes $\hat e$ to $u_t^{\lef}$; 
(ii) a distinct path in $Q^{\thr}_t(\hat e)$ that routes $u_t^{\lef}$ to $u_t^{\rig}$; and (iii) $Q^{\rig}_t(\hat e_t)$, the path in $\qset_{t}^{\rig}$ that routes $\hat e_t$ to $u_t^{\rig}$.

This completes the description of an iteration, and therefore completes the description of the algorithm. Clearly, after processing all clusters $C_1,\ldots, C_r$, we obtain a set $\rset$ that contains, for each edge $e\in E'$, a path $R_e$. It is not hard to verify that all properties of \Cref{claim: compute routing cycles} are satisfied.
\end{proof}




\iffalse{construct routing path if given routing paths}
\paragraph{Step 1.}
In the first step we will construct a set $\set{R^*_e}_{e\in E'}$ of cycles, using the input auxiliary paths of $\pset$. Specifically, we will construct, for each edge $e\in E'$ two paths $P^*_e,P^{**}_e$ with the same endpoints, and the cycle $R^*_e$ is then defined to be the union of paths $P^*_e,P^{**}_e$.

Consider now an edge $e\in E'$ and its input auxiliary path $P_e$ in $H$, and assume that $e$ connects $C_i$ to $C_j$ with $j\ge i+2$. Recall that path $P_e$ sequentially visits vertices $x_i,x_{i+1},\ldots, x_j$ in $H$. For convenience, we denote $P=(e_i,e_{i+1},\ldots,e_{j-1})$.

For each \singlecore cluster $C_t$ with $i<t<j$, we define the path $L_e^t$ as the union of the path $Q_i(e_{t-1})$ in $\qset_i$ that routes $e_{t-1}$ to $u_i$, and the path $Q_i(e_{t})$ in $\qset_i$ that routes $e_{t-1}$ to $u_i$. So path $L_e^t$ has $e_{t-1}$ as its first edge and $e_{t}$ as its last edge.
%
For each $i<t<j$ such that $C_t$ is a \dualcore cluster, we define the path $L_e^t$ as follows. Let $P_e^t$ be the subpath of $P_e$ between vertices $z_t$ and $z'_t$. Recall that path $P^t_e$ contains the special vertices $u^{\lef}_t,u^{\rig}_t$. We define $L_e^t$ as the sequential concatenation of (i) the path in $\qset_i^{\lef}$ that connects $e_{t-1}$ to $u^{\lef}_i$; (ii) the subpath of $P_e^t$ that connects $u^{\lef}_t$ to $u^{\rig}_t$; and (iii) the path in $\qset_i^{\rig}$ that connects $e_{t}$ to $u^{\rig}_i$. So path $L_e^t$ has $e_{t-1}$ as its first edge and $e_{t}$ as its last edge, and visits $u^{\lef}_t$ before $u^{\rig}_t$.
%
Similarly, if $C_i$ is not a \dualcore cluster, then we define $L_e^i$ to be the path $Q_i(e_{i+1})$ that routes $e_{i+1}$ to $u_i$, and if $C_i$ is a \dualcore cluster, then we define $L_e^i$ to be the path in $\qset_i^{\rig}$ that routes $e_{i+1}$ to $u^{\rig}_i$. The path $L_e^j$ is defined similarly.
Finally, the path $P^*_e$ is defined as the sequential concatenation of paths $L_e^i, L_e^{i+1},\ldots, L_e^{j-1},L_e^j$.
\fi

\znote{unhelpful clusters left and right paths currently pass through incorrect clusters}

\znote{to modify until the end of subsection}

We now construct path $P^{**}_e$.
If $C_i$ is not a \dualcore cluster, then we define $L_e^i$ to be the path $Q_i(e)$ that routes $e$ to $u_i$, and if $C_i$ is not a \dualcore cluster, then we define $L_e^i$ to be the path in $\qset_i^{\rig}$ that routes $e$ to $u^{\rig}_i$. The path $L_e^j$ is defined similarly.
The path $P^{**}_e$ is defined as the sequential concatenation of paths $L_e^i, e ,L_e^j$.
See \Cref{fig: auxiliary cycle} for an illustration.

%Recall that the set $\set{P_e}_{e\in E'}$ of paths is guaranteed to cause congestion at most $\beta$ in graph $G$, then from the construction of cycles in $\rset^*=\set{R^*_e\mid e\in E'}$, 

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.2]{figs/auxiliary_cycle.jpg}
	\caption{An illustration of paths $P^*_e$ (shown in red) and $P^{**}_e$ (shown in green) for edge $e=(v,v')$.}\label{fig: auxiliary cycle}
\end{figure}

Note that the given $\pset$ of paths is random, the sets $\qset_i$ for clusters $C_i$ that has the $\alpha_0$-bandwidth property are random, and the sets $\qset^{\lef}_i,\qset^{\rig}_i$ for \dualcore clusters $C_i$ are also random, so the set $\rset^*$ of cycles we constructed is also a random set. We use the following simple observation.

\begin{observation}
For each edge $e\in E'$, $\cong_{G}(\rset^*,e)\le \cong_{G}(\pset,e)$, and
for each edge $e\in \bigcup_{1\le i\le r}E(C_i)$, $\expect[]{\cong_{G}(\rset^*,e)^2}\le O\left(\beta^2\cdot\expect[]{\cong_{G}(\pset,e)^2}\right)\le O(\beta^4)$.
\end{observation}
\begin{proof}
	\znote{To Complete}
\end{proof}


%See \Cref{fig: LMR_auxi} for an illustration.
%We call $R^*_e$ the \emph{auxiliary cycle} of edge $e$.
%We define an orientation on cycle $R^*_e$ as follows. We start from vertex $u_{t_0}$, follow the path $P^*_e$ to sequentially visit vertices $u_{t_1},\ldots, u_{t_k}$, and finally follow the path $P^{**}_e$ to come back to vertex $u_{t_0}$.

\paragraph{Step 2.} In this step, we further process the set $\set{R^*_e}_{e\in E'}$ of cycles constructed in the first step to obtain the desired set $\set{R_e}_{e\in E'}$ of auxiliary cycles.

\znote{To Complete: de-interfere}

\znote{Need some bound on $\ntcost(\rset,\Sigma)$ here or in prelim?x}




\subsubsection{Constructing the Decomposition into Subinstances}


We use the algorithm \algbasicdisengagement defined in \Cref{subsec: basic disengagement} to construct subinstances of the input instance $(G,\Sigma)$. However, instead of directly applying the analysis in \Cref{subsec: basic disengagement} to bound the total cost of all these subintances, we will use an alternative way of analyzing their total cost, which the required bounds in \Cref{lem: disengagement with routing}. 

For each $1\le i\le r$, we define cluster $U_i=\bigcup_{1\le t\le i}C_t$, and $\notU_i=\bigcup_{i+x1\le t\le r}C_t$, so $U_r=G$. We define $\lset=\set{U_1,\ldots,U_r}$, so $\lset$ is a laminar family. In order to construct the subinstances using the algorithm \algbasicdisengagement, we need to also specify a distribution on sets of guiding paths for each cluster of $U_1,\ldots,U_{r-1}$, or equivalently construct a random set of guiding paths for each of these clusters, which we do next.

Consider first the cluster $U_1=C_1$. Recall that in \Cref{sec: guiding and auxiliary paths} we have obtained a random set $\qset_1$ of guiding paths in $C_1$, that route all edges of $\delta(C_1)$ to a vertex $u_1$ in $C_1$. We simply let the random set $\qset_1$ be the random set of guiding paths for $U_1$, that we denote by $\wset_1$. Consider now an index $i>1$ and the cluster $U_i$. 
We construct the random set $\wset_i$ of guiding paths as follows. 
Assume first that $C_i$ is a \singlecore cluster. For each edge $e\in \hat E_i$, we define $W_i(e)=Q_i(e)$, the path in $\qset_i$ that routes $e$ to $u_i$ in $C_i$. For each edge $e\in E(U_i, \notU_i)\setminus \hat E_i$, note that $e\in E'$, and we define path $W_i(e)$ as the subpath of cycle $R_e$ between (including) the edge $e$ and vertex $u_i\in C_i$, that lies entirely in $U_i$. We then let $\wset_i=\set{W_i(e)\mid e\in E(U_i, \notU_i)}$.
%
%
%We then define the circular ordering $\oset'_i$ on the set $E(U_i, V\setminus U_i)$ of edges as $\oset^{\guided}(\wset_i,\Sigma)$, the ordering guided by $\wset_i$ and $\Sigma$ (see definition in \Cref{subsec: guiding paths rotations}). See \Cref{fig: in rotation good} for an illustration.
%
%
Assume now that $C_i$ is an \dualcore cluster. Similarly, for each edge $e\in \hat E_i$, we define $W_i(e)=Q^{\rig}_i(e)$, the path in $\qset_i^{\rig}$ that routes edge $e$ to $u_i^{\rig}$, and for each edge $e\in E(U_i, \notU_i)\setminus \hat E_i$, note that $e\in E'$, and we define path $W_i(e)$ as the subpath of cycle $R_e$ between (including) the edge $e$ and vertex $u^{\rig}_i\in C_i$ that lies entirely in cluster  $U_i$.
We then let $\wset_i=\set{W_i(e)\mid e\in E(U_i, \notU_i)}$.

%We then define the circular ordering $\tilde\oset_i$ on the set $E(U_i, V\setminus U_i)$ of edges as $\oset^{\guided}(\wset_i,\Sigma)$, the ordering guided by $\wset_i$ and $\Sigma$.

\begin{figure}[h]
	\centering
	\subfigure[Set $E(U_i,\notU_i)=\hat E_i\cup E^{\rig}_{i}\cup E^{\lef}_{i+1}\cup E^{\through}_{i}$ where $\hat E_{i}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\rig}_{i}=\set{e^b}$, $E^{\lef}_{i+1}=\set{e^g_1,e^g_2}$ and $E^{\through}_{i}=\set{e^r}$.
	Paths of $\wset_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.13}{\includegraphics{figs/in_rotation_1.jpg}}}
	\hspace{3pt}
	\subfigure[The circular ordering $\tilde\oset_{i}$ on the edges of $E(U_i,\notU_i)$.]{
		\scalebox{0.14}{\includegraphics{figs/in_rotation_2.jpg}}}
	\caption{An illustration of path set $\wset_i$ and the circular ordering $\tilde\oset_{i}$.}\label{fig: in rotation good}
\end{figure}


%\mynote{Given the laminar family and the sets of in-guiding and out-guiding paths, you plug in the basic disengagement algorithm and get the subinstances. You can remind the reader what they are, but you cannot define them here because you want to use the results of that section. By the way, it may be good to give that algorithm a name (the basic disengagement one) because we invoke it a lot.}
We now apply the algorithm \algbasicdisengagement to each cluster $U_i\in \lset$ and its associated set $\wset_i$ of guiding paths, and let $I_1,\ldots, I_r$ be the subinstances we obtain. We recall here how the instances are constructed in \algbasicdisengagement. 
For each $1\le i\le r$, we denote $\tilde \oset_i=\oset^{\guided}(\wset_i,\Sigma)$, the ordering guided by $\wset_i$ and $\Sigma$ (see definition in \Cref{subsec: guiding paths rotations}), so $\tilde \oset_i$ is an ordering on the set $E(U_i, \notU_i)$ of edges. See \Cref{fig: in rotation good} for an illustration.
First, the instance $I_1=(G_1,\Sigma_1)$ is the cluster-based instance associated with cluster $C_1$, namely $(G_1,\Sigma_1)=(G_{C_1},\tilde \Sigma_{C_1})$. Recall that $V(G_{C_1})=V(C_1)\cup \set{v^*_1}$, and the rotation on $v^*_1$, the vertex obtained by contracting $G\setminus C_1$, is $\tilde \oset_1$ defined above. 
Then for each index $2\le i\le r-1$, the instance $I_i=(G_i,\Sigma_i)$ is obtained from the cluster-based instance $(G_{U_i},\tilde \Sigma_{U_i})$, by taking its contracted instance with respect to cluster $U_{i-1}$. See \Cref{fig: subinstance} for an illustration. So $V(G_i)=V(C_i)\cup \set{v^*_i, v'_i}$, where vertex $v^*_i$ is obtained by contracting $G\setminus U_i$ and vertex $v'_i$ is obtained by contracting $U_{i-1}$. The rotation on vertex $v^*_i$ is $\tilde \oset_i$, and the rotation on vertex $v'_i$ is $\tilde \oset_{i-1}$.
Finally, the instance $I_r=(G_r,\Sigma_r)$ is the contracted instance of $(G,\Sigma)$ with respect to cluster $U_{r-1}$. Recall that $V(G_r)=V(C_r)\cup \set{v'_r}$, and the rotation on $v'_r$, the vertex obtained from contracting the cluster $U_{r-1}$, is $\tilde \oset_{r-1}$. 


\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}\cup E^{\rig}_{i}$ are shown in green, and edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.14}{\includegraphics{figs/subinstance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{5pt}
	\subfigure[Graph $G_i$, where $\delta_{G_i}(v_i^{*})=\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$, and $\delta_{G_i}(v_i')=\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.12}{\includegraphics{figs/subinstance_2.jpg}}}
	\caption{An illustration of the construction of subinstance $(G_i,\Sigma_i)$.}\label{fig: subinstance}
\end{figure}



\subsubsection{Completing the Proof of \Cref{lem: disengagement with routing}}
\label{subsec: proof of disengagement with routing}

In this section we complete the proof of \Cref{lem: disengagement with routing}.
Since the subinstances are constructed using the algorithm \algbasicdisengagement, \Cref{lem: basic disengagement combining solutions} holds. In particular, if we are given, for each $1\le i\le r$, a solution $\phi_i$ to subinstance $I_i$, then we can efficiently combine them together to obtain a solution $\phi$ for the input instance $I$ of cost at most $\sum_{1\le i\le r}\cro(\phi_i)$.
On the other hand, from the construction of the subinstances $I_1,\ldots,I_r$, it is clear that, for each $1\le i\le r$, $E(C_i)\subseteq E(G_i)$, and all other edges of $G_i$ lie in $\Eout(\cset)$.

We next show in the following observation that $\sum_{1\le i\le r}|E(G_i)|\le O(|E(G)|)$.

\begin{observation}
\label{obs: disengaged instance size}
$\sum_{1\le i\le r}|E(G_i)|\le O(|E(G)|)$.
\end{observation}
\begin{proof}
	\iffalse 
	Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le r}$, each graph of $\set{G_i}_{1\le i\le r}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node, so each edge of $G_i$ corresponds to an edge in $E(G)$.
	Therefore, for each $1\le i\le r$, 
	$$|E(G_i)|=|E_G(C_i)|+|\delta_G(C_i)|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu.$$
	\fi
	%
	Note that $E(G_i)=E(C_i)\cup \hat E_i\cup \hat E_{i-1}\cup E_i^{\lef} \cup E_i^{\rig}\cup E_i^{\thr}$.
	First, each edge of $\bigcup_{1\le i\le r}E(C_i)$ appears in exactly one graphs of $\set{G_i}_{1\le i\le r}$. 
	Second, each edge of $\bigcup_{1\le i\le r}\hat E_i$ appears in exactly two graphs of $\set{G_i}_{1\le i\le r}$.
	Consider now an edge $e\in E'$. If $e$ connects a vertex of $C_i$ to a vertex of $C_j$ for some $j\ge i+2$, then $e$ will appear as an edge in $E_i^{\rig}\subseteq E(G_i)$ and an edge in $E_j^{\lef}\subseteq E(G_j)$, and it will appear as an edge in $E_k^{\thr}\subseteq E(G_k)$ for all $i<k<j$.
	
	For each $1\le i\le r$, we denote $E^{\through}_{i}=E(U_{i-1},U_{i+1})$.
	On one hand, we have $\sum_{1\le i\le r}|E_i^{\lef} \cup E_i^{\rig}|\le 2|E(G)|$. 
	On the other hand, note that $E_k^{\thr}=E(C_{k-1},C_{k+1})\cup E^{\through}_{k-1}\cup E^{\through}_{k}$, and each edge of $e$ appears in at most two graphs of $\set{G_i}_{1\le i\le r}$ as an edge of $E(C_{k-1},C_{k+1})$.
	Moreover, from \Cref{obs: bad inded structure}, $|E^{\through}_{k-1}|\le |\hat E_{k-1}|$ and $|E^{\through}_{k}|\le |\hat E_{k}|$.
	Altogether, we have
	\begin{equation}
	\begin{split}
	\sum_{1\le i\le r}|E(G_i)| & =
	\sum_{1\le i\le r}\left(
	|E(C_i)|+ |\hat E_i|+ |\hat E_{i-1}|+ |E_i^{\lef}| + |E_i^{\rig}|+|E_i^{\thr}|
	\right)\\
	& = \sum_{1\le i\le r}
	|E(C_i)|+ \sum_{1\le i\le r} \left(|E_i^{\lef}| + |E_i^{\rig}|\right)+ \sum_{1\le i\le r}\left(|E_i^{\thr}|+ |\hat E_i|+ |\hat E_{i-1}|\right)\\
	& \le |E(G)|+ 2\cdot |E(G)| + \sum_{1\le i\le r}\left(|E(C_{i-1},C_{i+1})|+ 2|\hat E_i|+ 2|\hat E_{i-1}|\right)\\
	& \le 8\cdot |E(G)|.
	\end{split}
	\end{equation}
	This completes the proof of \Cref{obs: disengaged instance size}.
\end{proof}



Therefore, to complete the proof of \Cref{lem: disengagement with routing}, it suffices to prove the following claim.
\begin{claim}
\label{claim: existence of good solutions special}
$\expect{\sum_{1\le i\le r}\optcrors(G_i,\Sigma_i)}\leq O(\beta^2\cdot \left(\optcrors(I)+|E(G)|\right ))$.
\end{claim}

The remainder of this subsection is dedicated to the proof of Claim~\ref{claim: existence of good solutions special}.
Let $\phi^*$ be an optimal drawing of the instance $(G,\Sigma)$.
We will construct, for each $1\le i\le r$, a solution $\phi_i$ to the instance $(G_i,\Sigma_i)$ using $\phi^*$, such that $\sum_{1\le i\le r}\cro(\phi_i)\le O(\beta^2\cdot(\cro(\phi^*)+|E(G)|))$, and \Cref{claim: existence of good solutions special} then follows.

\paragraph{Constructing the sets of out-guiding paths.} Before constructing the drawings for subinstances $I_1,\ldots,I_r$, we first construct, for each $1\le i\le r-1$, a random set $\wset'_i$ of out-guiding paths for cluster $U_i$, as follows.
Consider first the cluster $U_{r-1}=G\setminus C_r$. Recall that in \Cref{sec: guiding and auxiliary paths} we have obtained a random set $\qset_r$ of guiding paths in $C_r$, that route all edges of $\delta(C_r)$ to a vertex $u_r$ in $C_r$. We simply let $\wset'_{r-1}=\qset_r$. Consider now an index $i<r-1$ and the cluster $U_i$. 
We construct the random set $\wset'_i$ of guiding paths as follows. 
Assume first that $C_{i+1}$ is a \singlecore cluster. For each edge $e\in \hat E_i$, we define $W'_i(e)=Q_{i+1}(e)$, the path in $\qset_{i+1}$ that routes $e$ to $u_{i+1}$ within $C_{i+1}$. For each edge $e\in E(U_i, \notU_i)\setminus \hat E_i$, note that $e\in E'$, and we define path $W'_i(e)$ as the subpath of cycle $R_e$ between (including) the edge $e$ and vertex $u_{i+1}\in C_{i+1}$, that lies entirely within $\notU_i$.
%Denote $\wset_i=\set{W_i(e)\mid e\in E(U_i, V\setminus U_i)}$.
Assume now that $C_{i+1}$ is an \dualcore cluster. Similarly, for each edge $e\in \hat E_i$, we define $W'_i(e)=Q^{\lef}_{i+1}(e)$, the path in $\qset_{i+1}^{\lef}$ that routes edge $e$ to $u_{i+1}^{\lef}$, and for each edge $e\in E(U_i, \notU_i)\setminus \hat E_i$, note that $e\in E'$, and we define path $W'_i(e)$ as the subpath of cycle $R_e$ between (including) the edge $e$ and vertex $u^{\lef}_{i+1}\in C_{i+1}$ that lies entirely within $\notU_i$.
In both cases, wenote $\wset'_i=\set{W'_i(e)\mid e\in E(U_i, \notU_i)}$.

	
\paragraph{Drawings $\phi_2,\ldots,\phi_{r-1}$.}
First we fix some index $2\le i\le r-1$, and describe the construction of the drawing $\phi_i$. 
Assume first that both $C_{i-1},C_{i+1}$ are \singlecore clusters.
The cases where $C_{i-1}$ or $C_{i+1}$ is \dualcore can be dealt with similarly.
Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
Also recall that we have defined a set $\wset_{i-1}$ of paths that contains, for each edge $e\in E(U_{i-1},\notU_{i-1})=\hat E_{i-1}\cup E_i^{\lef}\cup E_i^{\thr}$, a path $W_{i-1}(e)$ routing $e$ to $u_{i-1}$ in $U_{i-1}$, and a set $\wset'_i$ of paths that contains, for each edge $e\in E(U_i,\notU_i)=\hat E_{i}\cup E_i^{\rig}\cup E_i^{\thr}$, a path $W'_i(e)$ routing $e$ to $u_{i+1}$ in $\notU_i$.
Clearly, all paths in $\wset_{i-1}$ and  $\wset'_{i}$ are internally disjoint from $C_i$. We will view $u_{i-1}$ as the last endpoint of all paths in $\wset_{i-1}$ and view $u_{i+1}$ as the last endpoint of all paths in $\wset'_{i}$.

We start with the image of cluster $C_i$ in $\phi^*$. We then add to it the image of vertices $v'_i, v^*_i$ and edges of $(\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$ as follows.
First, we apply the algorithm from \Cref{cor: new type 2 uncrossing} to graph $G$, drawing $\phi^*$ and the set $\wset'_{i}$ of paths, and obtain a set $\Gamma'_i=\set{\gamma'_e\text{ }\big|\text{ } e\in \big(\hat E_{i}\cup E_i^{\rig}\cup E_i^{\thr}\big)}$ of curves. 
Since all paths of $\wset'_{i}$ share the last endpoint $u_{i+1}$, all curves in $\Gamma'_i$ also share the last endpoint, that we denote by $z^*_i$.
We denote by $\oset^*_i$ the ordering in which curves of $\Gamma'_i$ enter $z^*_i$.
Similarly, we apply the algorithm from \Cref{thm: new nudging} to graph $G$, drawing $\phi^*$ and the set $\wset_{i-1}$ of paths, and obtain a set $\Gamma_{i-1}=\set{\gamma_e\text{ }\big|\text{ } e\in \big(\hat E_{i-1}\cup E_i^{\lef}\cup E_i^{\thr}\big)}$ of curves. Since all paths of $\wset_{i-1}$ share the last endpoint $u_{i-1}$, all curves in $\Gamma_{i-1}$ also share the last endpoint, that we denote by $z'_i$.

Lastly, we apply the algorithm from \Cref{lem: ordering modification} to the set $\hat E_{i}\cup E_i^{\rig}\cup E_i^{\thr}$ of edges (as elements), set $\Gamma'_i=\set{\gamma'_e\mid e\in \big(\hat E_{i}\cup E_i^{\rig}\cup E_i^{\thr}\big)}$ of curves, and the ordering $\tilde \oset_{i}$. We rename the set of curves we obtain by $\Gamma'_i$.
We now view $z^*_i$ as the image of $v^*_i$, view $z'_i$ as the image of $v'_i$, and view (i) for each $e\in \hat E_{i}\cup E_i^{\rig}$, the curve $\gamma'_e$ as the image of $e$; (ii) for each $e\in \hat E_{i-1}\cup E_i^{\lef}$, the curve $\gamma_e$ as the image of $e$; and (iii) for each $e\in E_i^{\thr}$, the concatenation of curves $\gamma_e$ and $\gamma'_e$ as the image of $e$. In this way, we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is easy to verify that $\phi_i$ respects the rotation system $\Sigma_i$.



\iffalse{previous rotation modification}
Let $\dset$ be a tiny disc around $z^*_{i}$, and let $\dset'$ be another small disc around $z^*_{i}$ that is strictly contained in $\dset$.
We first erase the image of all edges of $\delta(v^*_i)$ inside the disc $\dset$, and for each edge $e\in \delta(v^{*}_i)$, we denote by $p_{e}$ the intersection between the curve representing the current image of $e$ and the boundary of $\dset$.
	We then place, for each edge $e\in \delta(v^{*}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{*}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{*}_{i}$. 
	We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{*}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{*}_i)}$.
	Finally, for each edge $e\in \delta(v^{*}_i)$, let $\zeta_e$ be the concatenation of (i) the current image of $e$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z^{*}_i$ in $\dset'$.
	We view $\zeta_e$ as the image of edge $e$, for each $e\in \delta(v^{*}_i)$.

%
%	
We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{*}_i$ at $v^{*}_i$, and therefore it respects the rotation system $\Sigma_i$.
\fi

We now upper bound the number of crossings in the drawing $\phi_i$ that we have constructed.

First, since we have not modified the drawing of $C_i$, the number of crossings between edges of $E_G(C_i)$ are bounded by $\chi^2(C_i)$. 
Second, from the definition of curves of $\Gamma'_i$, the number of crossings between image of $C_i$ and the curves of $\Gamma'_i$ is at most $\chi(\wset'_i,C_i)$, and similarly the number of crossings between image of $C_i$ and the curves of $\Gamma_{i-1}$ is at most $\chi(\wset_{i-1},C_i)$.
%
Third, from \Cref{thm: new nudging}, the number of crossings between curves of $\Gamma_{i-1}$ is bounded by $\chi^2(\wset_{i-1})+\sum_{e\in E(G)}(\cong_G(\wset_{i-1},e))^2+\ntcost(\wset_{i-1},\Sigma)$.
%
Fourth, the number of crossings between curves of $\Gamma_{i-1}$ and curves of $\Gamma'_{i}$ is at most $\chi(\wset'_i,\wset_{i-1})$.
%
Lastly, from \Cref{lem: ordering modification}, the number of crossings in drawing $\phi_i$ inside the tiny $z^*_i$-disc is $O(\dist(\oset^*_i,\tilde\oset_i))$. We now give an upper bound of $\dist(\oset^*_i,\tilde\oset_i)$ as follows.

Recall that for each $e\in \hat E_{i}\cup E_i^{\rig}\cup E_i^{\thr}$, $W_i(e)$ is the subpath of cycle $R_e$ between (including) the edge $e$ and vertex $u_i$, that lies entirely within $U_i$.
We apply the algorithm from \Cref{thm: new nudging} to graph $G$, drawing $\phi^*$, cluster $C_{i+1}$ and the set $\wset_i$ of paths. Let $\Xi=\set{\xi_e\mid e\in E(U_i,\notU_i)}$ be the set of curves we get.
From \Cref{thm: new nudging}, the curves of $\Xi$ enter $y_i=\phi^*(u_i)$ in the order $\tilde\oset_i$, and we have
$\chi(\Xi)\le \chi^2(\wset_i)+\sum_{e\in E(G)}(\cong_G(\wset_i,e))^2+\ntcost(\wset_i,\Sigma)$.
We define, for each edge $e\in E(U_i,\notU_i)$, the curve $\zeta_e$ to be the union of $\xi_e$ and $\gamma'_e$. It is easy to verify that $\set{\zeta_e\mid e\in E(U_i,\notU_i)}$ is a set of reordering curves for $\oset^*_i$ and $\tilde\oset_i$, and so 
\[
\dist(\oset^*_i,\tilde\oset_i)\le \chi\big(\set{\zeta_e\mid e\in E(U_i,\notU_i)}\big)\le \chi^2(\wset_i)+\sum_{e\in E(G)}(\cong_G(\wset_i,e))^2+\ntcost(\wset_i,\Sigma)+\chi(\wset_i,\wset'_i).
\]


\iffalse{previous analysis of crossings}
	\begin{claim}
		\label{clm: rerouting_crossings}
		The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	\end{claim}
	\begin{proof}
		Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
		From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		
		%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
		For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
		Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
		We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.
		
		We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
		From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
		Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
		%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
		\begin{figure}[h]
			\centering
			\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
			\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
		\end{figure}
	\end{proof}
\fi

From the above discussion, for each $2\le i\le r-1$, 
\begin{equation*}
\begin{split}
	\cro(\phi_i)= & \text{ }\chi^2(C_i)+\chi(\wset'_i\cup \wset_{i-1},C_i)+\chi^2(\wset_{i-1})+\sum_{e\in E(G)}(\cong_G(\wset_{i-1},e))^2+\ntcost(\wset_{i-1},\Sigma)\\
	& + O\bigg(\chi^2(\wset_{i})+\sum_{e\in E(G)}(\cong_G(\wset_{i},e))^2+\ntcost(\wset_{i},\Sigma)+\chi(\wset_i,\wset'_i)\bigg).
\end{split}
\end{equation*}

	
\paragraph{Drawings $\phi_1$ and $\phi_{r}$.}
The drawings $\phi_1$ and $\phi_{r}$ are constructed similarly. We only describe the construction of $\phi_1$, and the construction of $\phi_r$ is symmetric.
Recall that graph $G_1$ contains only one super-node $v_1^{*}$, that is obtained by contracting $\notU_1$, and $\delta_{G_1}(v_1^{*})=\hat E_1\cup E^{\rig}_1$. 
We construct the set $\wset'_1$ of out-guiding paths in the same way as sets $\wset'_2,\ldots,\wset'_{r-1}$. Then we construct the drawing $\phi_1$ using the algorithm from \Cref{thm: cost of single cluster}.
From \Cref{obs: new crossings},
$$\cro(\phi_1)\le \chi^2(C_1)+ \chi(\wset'_1,C_1)+\chi(\wset'_1,\qset_1)+\chi^2(\qset_1)+\sum_{e\in E(C)}\cong(\qset_1,e)^2.$$
Similarly, the drawing $\phi_r$ that we obtained in the same way satisfies that 
\[\cro(\phi_r)\le \chi^2(C_r)+ \chi(\wset_{r-1},C_r)+\chi(\wset_{r-1},\qset_r)+\chi^2(\qset_r)+\sum_{e\in E(C)}\cong(\qset_r,e)^2.\]


\iffalse{previous construction of phi_1}
	We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
	We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{r-1}$. 
	We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
	Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
	%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
	We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
	Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
	\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
	Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
	\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{r-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]
\fi	
	
	
	
We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le r}\cro(\phi_i)$.
First note that $\sum_{1\le i\le r}\chi^2(C_i)\le O(\cro(\phi^*))$.
We then define $\wset=\bigcup_{1\le i\le r}(\wset_i\cup\wset'_i)$. It is easy to verify that, for each edge $e\in E(G)$, $\expect[]{(\cong_G(\wset,e))^2}\le O(\beta)$. Therefore, on the one hand,
\[
\sum_{1\le i\le r}\sum_{e\in E(G)}\expect[]{\cong_G(\wset_i,e)^2+\cong_G(\wset'_i,e)^2}
%= \sum_{e\in E(G)} \sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)^2 
\le \sum_{e\in E(G)} \expect[]{\cong_G(\wset,e)^2}\le O\big(|E(G)|\cdot\temp\big),
\]
 and on the other hand,
\[
\begin{split}
\sum_{1\le i\le r}\expect{\chi^2(\wset_i)+\chi(\wset_i,\wset'_i)} & =  \text{ } \expect{\sum_{e,e'\in E(G)}\chi(e,e')\cdot\cong_{G}(\wset,e)\cdot\cong_{G}(\wset,e')}\\
& \text{ } \le \expect{\sum_{e,e'\in E(G)}\chi(e,e')\cdot\frac{\cong_{G}(\wset,e)^2+\cong_{G}(\wset,e')^2}{2}}\\
& \text{ } \le \expect{\sum_{e\in E(G)}\chi(e,G)\cdot\frac{\cong_{G}(\wset,e)^2}{2}}\le O(\beta\cdot \cro(\phi^*)).
\end{split}\]
Moreover, $\sum_{1\le i\le r}\expect{\chi(\wset'_i,C_i)+\chi(\wset_{i-1},C_i)} \le \sum_{1\le i\le r}\expect{\chi(\wset,C_i)} \le O(\beta\cdot\cro(\phi^*))$.

From similar arguments, we can show that
$\sum_{1\le i\le r}\sum_{e\in E(C_i)}\expect{\cong_G(\qset_i,e)^2} \le O(\beta\cdot |E(G)|)$ and
$\sum_{1\le i\le r}\expect{\chi^2(\qset_i)} \le O(\beta\cdot\cro(\phi^*))$.
%
Altogether, they imply that $\sum_{1\le i\le r}\cro(\phi_i) \le O((\cro(\phi^*)+|E(G)|)\cdot\temp)$.
This completes the proof of \Cref{claim: existence of good solutions special}.































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse{previous bad-chain centered setting assumptions}


\paragraph{Assumption 1: The Gomory-Hu tree $\tau$ of graph $H$ is a path.}
Let $H=G_{\mid\cset}$ be the contracted graph. 
We denote the clusters in $\cset$ by $C_1,C_2,\ldots,C_r$. For convenience, for each $1\leq i\leq r$, we denote by $x_i$ the vertex of graph $H$ that represents the cluster $C_i$. Throughout this subsection, we assume that the Gomory-Hu tree $\tau$ of graph $H$ is a path, and we assume without loss of generality that the clusters are indexed according to their appearance on the path $\tau$. Note that each edge in $\Eout(\cset)$ corresponds to an edge in $H$, and we do not distinguish between them.

\paragraph{Assumption 2: Bad Chains of Single-Vertex Clusters.}
We allow some clusters of $\cset\setminus\set{C_1,C_r}$ to contain only a single vertex. Let indices $1< i\le j< n$ be such that clusters $C_{i-1},C_{j+1}$ are not single-vertex clusters, while all clusters $C_{i},\ldots,C_{j}$ are single-vertex clusters. 
We call the union of clusters $C_{i},\ldots,C_{j}$ a \emph{bad chain}, and we denote $\bc[i,j]=\bigcup_{i\le t\le j}C_t$. We call index $i$ the \emph{left endpoint} and index $j$ the \emph{right endpoint} of the bad chain.

Consider the graph $H=G_{\mid\cset}$. Note that each bad chain $\bc[i,j]$ belongs to graph $H$. Consider a bad chain $\bc[i,j]$, we say that a path $P$ is contained in the bad chain, iff $V(P)\subseteq \bc[i,j]$.
Let $x_s, x_t$ be two vertices (with $s<t$) that do not belong to any bad chains, and let $\bc[i_1,j_1],\ldots,\bc[i_k,j_k]$ be all bad chains whose endpoints lie in $\set{s+1,\ldots,t-1}$. Assume without loss of generality that $i_1\le j_1< i_2\le j_2 <\ldots <i_k\le j_k$.
We say that a path connecting $x_{s}$ to $x_{t}$ is \emph{nice}, iff it is the sequential concatenation of: a path that sequentially visits vertices $x_s,x_{s+1}\ldots,x_{i_1}$, a path connecting $x_{i_1}$ to $x_{j_1}$ that is contained in the bad chain $\bc[i_1,j_1]$, a path that sequentially visits vertices  $x_{j_1},x_{j_1+1}\ldots,x_{i_2}$, a path connecting $x_{i_2}$ to $x_{j_2}$ that is contained in the bad chain $\bc[i_2,j_2]$, \ldots , and a path that sequentially visits vertices  $x_{j_k},x_{j_k+1}\ldots,x_{t}$.
See \Cref{fig: nice path} for an illustration.
If vertex $x_s$ belongs to some bad chain $\bc[i_0,j_0]$, then for an $x_s$-$x_t$ path to be nice, the path must start with a path connecting $x_s$ to $x_{j_0}$ that is contained in the bad chain $\bc[i_0,j_0]$.
Similarly, if vertex $x_t$ belongs to some bad chain $\bc[i_{k+1},j_{k+1}]$, then a nice $x_s$-$x_t$ path must end with a path connecting $x_{i_{k+1}}$ to $x_{t}$ that is contained in the bad chain $\bc[i_{k+1},j_{k+1}]$.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.23]{figs/innerpath.jpg}
	\caption{An illustration of a nice path connecting $x_s$ to $x_t$. Bad chains are shown in pink.}\label{fig: nice path}
\end{figure}

\paragraph{Assumption 3: Auxiliary Paths.}
Let $E'$ be the subset of edges in $E^{\out}(\cset)$ that contains all edges connecting a pair $C_i,C_j$ of clusters in $\cset$, with $j\ge i+2$, and when $E'$ is viewed as a set of edges in $H$, then $E'$ contains all edges connecting a pair $x_i,x_j$ of vertices in $H$ with $j\ge i+2$.
We additionally assume that, for each edge $e\in E'$ that, when viewed as an edge in $H$, connects $x_i$ to $x_j$, we are given a nice path $P_e$ in $H$ connecting $x_i$ to $x_j$, that we call the \emph{auxiliary path} of $e$.
Additionally, all paths in $\set{P_e}_{e\in E'}$ cause congestion $O(1)$ in graph $H$.


We now start to describe the algorithm in the following subsections.



\subsubsection{Computing Guiding Paths and Auxiliary Cycles}
\label{sec: guiding and auxiliary paths}

We first apply the algorithm from \Cref{thm:algclassifycluster} to each non-single-vertex cluster of $\cset$.
In particular, for each non-single-vertex cluster $C_i$, we apply the algorithm \algclassifycluster to the instance $(G,\Sigma)$ and the cluster $C_i$ (recall that cluster $C_i$ has the $\alpha_0$-bandwidth property, where $\alpha_0=1/\log^3m$) for $100\log n$ times. If any application of \algclassifycluster returns a distribution $\dset(C_i)$ over sets of guiding paths in $\Lambda(C_i)$, such that $C_i$ is $\beta^*$-light with respect to $\dset(C_i)$, then we continue to sample a set of guiding paths from $\dset(C_i)$. Let $\qset_i$ be the set we obtain, and let $u_i$ be the vertex of $C_i$ that serves as the common endpoint of all paths in $\qset_i$. If all applications of \algclassifycluster return FAIL, then consider the graph $C_i^+$ (see \Cref{def: Graph C^+}). We apply the algorithm from \Cref{lem: simple guiding paths} to cluster $C^+_i$ and and set $T(C_i)$, and let $u_i$ be the vertex and $\qset_i$ be the set of paths that we obtain. Clearly, $\qset_i$ can be also viewed as a set of paths routing edges of $\delta_G(C_i)$ to $u_i$. From \Cref{lem: simple guiding paths}, for each edge $e\in E(C_i)$, $\expect{\cong(\qset_i,e)}\leq  O(\log^4m/\alpha_0)$. Finally, for each $1\le i\le r$ and for each $e\in \delta(C_i)$, we denote by $Q_i(e)$ the path of $\qset_i$ that routes $e$ to $u_i$.

We then apply the algorithm from \Cref{lem: non_interfering_paths} to each set $\qset_i$ of paths and the rotation system $\Sigma$, and rename the sets of paths we obtain as $\qset_1,\ldots,\qset_r$. Now we are guaranteed that, for each $1\le i\le r$, the set $\qset_i$ of paths is non-transversal with respect to $\Sigma$.


\textbf{Bad Event $\xi_i$.} For each index $1\le i\le r$, we say that the event $\xi_i$ happens, iff $C_i$ is a non-single-vertex cluster, $C_i$ is not an $\eta^*$-bad cluster, and all the $100\log n$ applications of \algclassifycluster return FAIL.
From \Cref{thm:algclassifycluster}, $\Pr[\xi_i]\le (1/2)^{100\log n}=O(n^{-50})$. Then from the union bound over all $1\le i\le r$, $\Pr[\bigcup_{1\le i\le r}\xi_i]\le O(n^{-49})$.

We then compute a set $\rset^*$ of cycles in $G$, using the set $\set{P_e}_{e\in E'}$ of inner paths and the path sets $\set{\qset_i}_{1\le i\le r}$, as follows.
Consider an edge $e\in E'$ and its inner path $P_e$ in $H$.
We denote $P_e=(e_1,\ldots,e_k)$, and for each $1\le j\le k$, we denote $e_j=(x_{t_{j-1}}, x_{t_{j}})$ (and so $e=(x_{t_0},x_{t_k})$ as an edge in $H$).
Recall that the set $\qset_i$ contains, for each edge $e\in\delta(C_i)$, a path $Q_i(e)$ routing edge $e$ to $u_i$.
We then define path $P^*_e$ as the sequential concatenation of paths $Q_{t_{0}}(e_1),Q_{t_{1}}(e_1), Q_{t_{1}}(e_2),Q_{t_{2}}(e_2),\ldots, Q_{t_{r-1}}(e_k),Q_{t_{r}}(e_k)$.
It is clear that path $P^*_e$ sequentially visits the vertices $u_{t_0},u_{t_1},\ldots,u_{t_k}$ in $G$.
%We call $P^*_e$ the \emph{auxiliary} path of $e$.
Since edge $e$, as an edge of $G$, connects a vertex of $C_{t_0}$ to a vertex of $C_{t_k}$. We then define path $P^{**}_e$ to be the union of paths $Q_{t_{k}}(e)$ and $Q_{t_{0}}(e)$, so path $P^{**}_e$ connects $u_{t_k}$ to $u_{t_0}$.
Finally, we define cycle $R^*_e$ to be the union of paths $P^*_e$ and paths $P^{**}_e$, and we denote $\rset^*=\set{R^*_e\mid e\in E'}$.

%See \Cref{fig: LMR_auxi} for an illustration.
%We call $R^*_e$ the \emph{auxiliary cycle} of edge $e$.
%We define an orientation on cycle $R^*_e$ as follows. We start from vertex $u_{t_0}$, follow the path $P^*_e$ to sequentially visit vertices $u_{t_1},\ldots, u_{t_k}$, and finally follow the path $P^{**}_e$ to come back to vertex $u_{t_0}$.
\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.24]{figs/auxiliary_path.jpg}
	\caption{An illustration of the auxiliary cycle $R^*_e$ of an edge $e$ (solid red): left auxiliary path shown in orange, middle auxiliary path  shown in purple and right auxiliary path  shown in green.}\label{fig: LMR_auxi}
\end{figure}
\fi

Recall that the set $\set{P_e}_{e\in E'}$ of inner paths is guaranteed to cause congestion at most $O(1)$ in graph $H$, then from the construction of cycles in $\rset^*$, it is easy to see that, for each edge $e\in E'$, $\cong_{G}(\rset^*,e)\le O(1)$, and
for each edge $e\in \bigcup_{1\le i\le r}E(C_i)$, $\expect[]{\cong_{G}(\rset^*,e)^2}\le O(\beta^*)$.

%\subsubsection*{Step 3. De-Interfering Auxiliary Cycles}


\iffalse{should be moved to the next subsection}

We further modify the cycles in $\rset^*$ to obtain a new set $\rset$ of cycles, such that the intersection of every pair of cycles in $\rset$ is non-transversal with respect to $\Sigma$ at no more than one of their shared vertices.
We will use the following lemma.

\znote{To complete the following lemma}

\begin{lemma}[De-interfering]
	There is an efficient algorithm, that given a graph $G$, a rotation system $\Sigma$, and a set $\pset$ of paths that share an endpoint $u$, computes a set $\pset'=\set{P'\mid P\in \pset}$ of paths, such that
\end{lemma}
\begin{proof}
	Let $R,R'$ be a pair of cycles in $\rset^*$ and let $v$ be a shared vertex of $R$ and $R'$. We say that the tuple $(R,R',v)$ is \emph{bad}, iff the intersection of cycles $R,R'$ at $v$ is transversal with respect to $\Sigma$. We iteratively process the set $\rset^*$ of cycles as follows. While there exist a pair $R,R'$ of cycles in $\rset^*$ and two vertices $v_1,v_2\in V(R)\cap V(R')$, such that the tuples $(R,R',v)$ and $(R,R',v)$ are bad, we process cycles $R,R'$ as follows. 
	
	Eventually, for each $e\in E'$, we obtain a cycle $R_e$ in $G$ that is called the \emph{auxiliary cycle} of edge $e$.	
\end{proof}

\fi



\znote{Todo: de-interfere auxiliary cycles to get cycles $\set{R_e}_{e\in E'}$.}



\subsubsection{Constructing Sub-Instances}
\label{sec: compute advanced disengagement}

In this step we will construct, for each non-single vertex cluster $C_i\in \cset$, a sub-instance $I_i=(G_i,\Sigma_i)$ of $(G,\Sigma)$, and for each bad chain $\bc[i,j]$, a sub-instance $I_{\bc[i,j]}$ of $(G,\Sigma)$, such that the set of all created sub-instances satisfy the properties in \Cref{thm: disengagement - main}.
%such that the instances $\iset=\set{I_1,\ldots,I_r}$ satisfy the properties in \Cref{thm: disengagement - main}.

For each index $1\le i\le r$, we define edge sets
$\hat E_i=E(C_i,C_{i+1})$,  $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, and $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$.
Let $\bc[i,j]$ be a bad chain. Similarly we define edge sets
$E_{[i,j]}^{\rig}=\bigcup_{k>j+1}E(\bc[i,j],C_k)$,  $E_{[i,j]}^{\lef}=\bigcup_{k<i-1}E(\bc[i,j],C_k)$, 
$\hat E_{[i,j]}^{\rig}=E(\bc[i,j],C_{j+1})$,  $\hat E_{[i,j]}^{\lef}=E(\bc[i,j],C_{i-1})$, and $E^{\thr}_{[i,j]}=\bigcup_{i'\le i-1,j'\ge j+1}E(C_{i'},C_{j'})$.

\paragraph{Cluster-based Instance $I_i=(G_i,\Sigma_i)$ ($2\le i\le r$).}
Let $C_i$ be some non-single-vertex cluster with $2\le i\le r$.
We define the instance $I_i=(G_i,\Sigma_i)$ as follows.
The graph $G_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_i$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_i$, and finally deleting self-loops on the super-nodes $v^{\lef}_i$ and $v^{\rig}_i$. So $V(G_i)=V(C_i)\cup \set{ v^{\lef}_i,v^{\rig}_i}$. See \Cref{fig: disengaged instance} for an illustration. 

\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}\cup E^{\rig}_{i}$ are shown in green, and edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.35}{\includegraphics{figs/disengaged_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{5pt}
	\subfigure[Graph $G_i$. $\delta_{G_i}(v_i^{\rig})=\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$, and $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.28}{\includegraphics{figs/disengaged_instance_2.jpg}}}
	\caption{An illustration of the construction of sub-instance $(G_i,\Sigma_i)$.}\label{fig: disengaged instance}
\end{figure}

We now define the orderings in $\Sigma_i$. First, for each vertex $v\in V(C_i)$, the ordering on its incident edges is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the rotations of super-nodes $v^{\lef}_i,v^{\rig}_i$. 
We first consider $v^{\lef}_i$.
Note that $\delta_{G_i}(v^{\lef}_i)=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$.
For each edge $\hat e\in \hat E_{i-1}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ routing edge $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\lef}_i\cup E^{\thr}_i$, we denote by $W^{\lef}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i-1}$ and does not contain $u_i$.
We then denote 
$$\wset^{\lef}_i=\set{W^{\lef}_i(e)\mid e\in E^{\thr}_i\cup E^{\lef}_i}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E_{i-1}}.$$
%and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.

Intuitively, the rotation on vertex $v^{\lef}_i$ is defined to be the ordering in which the paths in $\wset^{\lef}_i$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_i$, let $e^*_W$ be the unique edge of path $W$ that is incident to $u_{i-1}$. We first define a circular ordering of the paths in $\wset^{\lef}_i$, as follows: the paths are ordered according to the circular ordering of their corresponding edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_i$ is associated with a unique edge in $\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, this ordering of the paths in $\wset^{\lef}_i$ immediately defines a circular ordering of the edges of $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, that we denote by $\oset^{\lef}_i$. See Figure~\ref{fig: v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i-1}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\lef}_{i}=\set{e^g_1,e^g_2}$ and $E^{\thr}_{i}=\set{e^r_1,e^r_2}$.
	Paths of $\wset^{\lef}_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.13}{\includegraphics{figs/rotation_left_1.jpg}}}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\lef}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\lef}_i)=\set{\hat e_1,\hat e_2,\hat e_3,\hat e_4,e^g_1, e^g_2, e^r_1,e^r_2}$. The rotation $\oset^{\lef}_i$ on them around $v^{\lef}_i$ is shown above.]{
		\scalebox{0.16}{\includegraphics{figs/rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{i}$ on vertex $v^{\rig}_i$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e'\in \hat E_{i}\cup E_i^{\rig}$, recall that $Q_{i}(\hat e')$ is the path in $C_{i}$ routing edge $\hat e'$ to vertex $u_{i}$.
For each edge $e\in E^{\thr}_i$, we denote by $W^{\rig}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i}$ and contains $u_{i-1}$.
We then denote 
$$\wset^{\rig}_i=\set{W^{\rig}_i(e)\text{ }\big|\text{ } e\in E^{\thr}_i}\cup \set{Q_{i}(\hat e')\text{ }\big|\text{ }  \hat e'\in \hat E_{i}\cup E^{\rig}_i}.$$
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is then defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}\in \Sigma$.
See Figure~\ref{fig: v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i}=\set{\hat e_1',\ldots,\hat e_4'}$, $E^{\rig}_{i}=\set{\tilde e^g_1,\tilde e^g_2}$ and $E^{\thr}_{i}=\set{\tilde e^r_1,\tilde e^r_2}$.
	Paths of $\wset^{\rig}_i$ excluding their first edges are shown in dash lines. ]{\scalebox{0.13}{\includegraphics{figs/rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\rig}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\rig}_i)=\set{\hat e_1',\hat e_2',\hat e_3',\hat e_4',\tilde e^g_1,\tilde e^g_2,\tilde e^r_1,\tilde e^r_2}$. The rotation $\oset^{\rig}_i$ on them around $v^{\rig}_i$ is shown above.]{
		\scalebox{0.17}{\includegraphics{figs/rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_right rotation}
\end{figure}

\paragraph{Instances $I_1=(G_1,\Sigma_1)$ and $I_r=(G_r,\Sigma_r)$.}
The instances $(G_1,\Sigma_1)$ and $(G_r,\Sigma_r)$ are defined similarly to a cluster-centered instance, but instead of two super-nodes, the graphs $G_1$ and $G_r$ contain one super-node each.
In particular, graph $G_1$ is obtained from $G$ by contracting clusters $C_2,\ldots, C_r$ into a super-node, that we denote by $v^{\rig}_1$, and then deleting self-loops on it.
So $V(G_1)=V(C_1)\cup \set{v^{\rig}_{1}}$ and $\delta_{G_1}(v^{\rig}_{1})=\hat E_1\cup E^{\rig}_1$.
The rotation of a vertex $v\in V(C_1)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\rig}_1$ is defined in a similar way as $\oset^{\rig}_i$ for any index $2\le i\le r-1$.
Graph $G_r$ is obtained from $G$ by contracting clusters $C_1,\ldots, C_{r-1}$ into a super-node, that we denote by $v^{\lef}_r$, and then deleting self-loops on it.
So $V(G_r)=V(C_r)\cup \set{v^{\lef}_{r}}$ and $\delta_{G_r}(v^{\lef}_{r})=\hat E_{r-1}\cup E^{\lef}_r$.
The rotation of a vertex $v\in V(C_r)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\lef}_r$ is defined in a similar way as $\oset^{\lef}_i$ for any index $2\le i\le r-1$.


\paragraph{Bad Chain-based Instance $I_{\bc[i,j]}$.} Let $\bc[i,j]$ be a bad chain. We define the instance $I_{\bc[i,j]}=(G_{[i,j]},\Sigma_{[i,j]})$ as follows.
The graph $G_{[i,j]}$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_{[i,j]}$, and then contracting clusters $C_{j+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_{[i,j]}$, and finally deleting self-loops on the super-nodes $v^{\lef}_{[i,j]}$ and $v^{\rig}_{[i,j]}$. So $V(G_i)=\bc[i,j]\cup \set{v^{\lef}_{[i,j]},v^{\rig}_{[i,j]}}$. See \Cref{fig: bad instance} for an illustration. 

\begin{figure}[h]
	\centering
	\subfigure[Edges of $\hat E^{\lef}_{[i,j]}\cup \hat E^{\rig}_{[i,j]}$ are in orange, edges of $E^{\lef}_{[i,j]}$ and $E^{\rig}_{[i,j]}$ are in green and blue respectively and edges of $E^{\thr}_{[i,j]}$ are in red. ]{\scalebox{0.12}{\includegraphics{figs/badchain_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0pt}
	\subfigure[Graph $G_{[i,j]}$. $\delta(v_{[i,j]}^{\rig})=\hat E_{[i,j]}^{\rig} \cup E_{[i,j]}^{\rig} \cup E^{\thr}_{[i,j]}$, and $\delta(v_{[i,j]}^{\lef})=\hat E_{[i,j]}^{\lef} \cup E_{[i,j]}^{\lef} \cup E^{\thr}_{[i,j]}$.]{
		\scalebox{0.14}{\includegraphics{figs/badchain_instance_2.jpg}}}
	\caption{An illustration of the construction of sub-instance $(G_{[i,j]},\Sigma_{[i,j]})$.}\label{fig: bad instance}
\end{figure}

We now define the orderings in $\Sigma_i$. First, for each vertex $v\in \bc[i,j]$, the ordering on its incident edges is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the rotations of super-nodes $v^{\lef}_{[i,j]},v^{\rig}_{[i,j]}$. 
We first consider $v^{\lef}_{[i,j]}$.
Note that $\delta_{G_i}(v^{\lef}_{[i,j]})=\hat E^{\lef}_{[i,j]}\cup E^{\lef}_{[i,j]}\cup E^{\thr}_{[i,j]}$.
For each edge $\hat e\in \hat E^{\lef}_{[i,j]}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ routing edge $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\lef}_{[i,j]}\cup E^{\thr}_{[i,j]}$, we denote by $W^{\lef}_{[i,j]}(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i-1}$ and does not contain $u_i$.
We then denote 
$$\wset^{\lef}_i=\set{W^{\lef}_i(e)\mid e\in E^{\lef}_{[i,j]}\cup E^{\thr}_{[i,j]}}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E^{\lef}_{[i,j]}}.$$
%and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.

Intuitively, the rotation on vertex $v^{\lef}_{[i,j]}$ is defined to be the ordering in which the paths in $\wset^{\lef}_{[i,j]}$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_{[i,j]}$, let $e^*_W$ be the unique edge of path $W$ that is incident to $u_{i-1}$. We first define a circular ordering of the paths in $\wset^{\lef}_{[i,j]}$, as follows: the paths are ordered according to the circular ordering of their corresponding edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_{[i,j]}$ is associated with a unique edge in $\hat E^{\lef}_{[i,j]}\cup E^{\lef}_{[i,j]}\cup E^{\thr}_{[i,j]}$, this ordering of the paths in $\wset^{\lef}_{[i,j]}$ immediately defines a circular ordering of the edges of $\delta_{G_{[i,j]}}(v_{[i,j]}^{\lef})=\hat E^{\lef}_{[i,j]}\cup E^{\lef}_{[i,j]}\cup E^{\thr}_{[i,j]}$, that we denote by $\oset^{\lef}_{[i,j]}$. See Figure~\ref{fig: bad_v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[$\hat E^{\lef}_{[i,j]}=\set{\hat e_1,\hat e_2}$, $E^{\lef}_{[i,j]}=\set{e^g_1}$ and $E^{\thr}_{[i,j]}=\set{e^r_1}$.
	Paths of $\wset^{\lef}_{[i,j]}$ excluding their first edges are shown in dash lines.]{\scalebox{0.14}{\includegraphics{figs/badinstance_rotation_left_1.jpg}}}
	\hspace{3pt}
	\subfigure[$\delta(v^{\lef}_{[i,j]})=\set{\hat e_1,\hat e_2,e^g_1,e^r_1}$. The rotation $\oset^{\lef}_{[i,j]}$ on them around $v^{\lef}_{[i,j]}$ is shown above.]{
		\scalebox{0.18}{\includegraphics{figs/badinstance_rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_{[i,j]}$ on vertex $v^{\lef}_{[i,j]}$ in the instance $(G_{[i,j]}, \Sigma_{[i,j]})$.}\label{fig: bad_v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{[i,j]}$ on vertex $v^{\rig}_{[i,j]}$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_{[i,j]})=\hat E^{\rig}_{[i,j]}\cup E^{\rig}_{[i,j]}\cup E^{\thr}_{[i,j]}$.
For each edge $\hat e'\in \delta_{G_i}(v^{\rig}_{[i,j]})$, we denote by $W^{\rig}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{j}$ and does not contains $u_{j+1}$.
We then denote 
$$\wset^{\rig}_i=\set{W^{\rig}_i(e)\text{ }\big|\text{ } e\in \hat E^{\rig}_{[i,j]}\cup E^{\rig}_{[i,j]}\cup E^{\thr}_{[i,j]}}.$$
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is then defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}\in \Sigma$.
See Figure~\ref{fig: bad v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[$\hat E^{\rig}_{[i,j]}=\set{\hat e'_1,\hat e'_2}$, $E^{\rig}_{[i,j]}=\set{e^b_1}$ and $E^{\thr}_{[i,j]}=\set{e^r_1}$.
	Paths of $\wset^{\rig}_{[i,j]}$ excluding their first edges are shown in dash lines. ]{\scalebox{0.14}{\includegraphics{figs/badinstance_rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{3pt}
	\subfigure[$\delta(v^{\rig}_i)=\set{\hat e'_1,\hat e'_2,e^b_1,e^r_1}$. The rotation $\oset^{\rig}_{[i,j]}$ on them around $v^{\rig}_{[i,j]}$ is shown above.]{
		\scalebox{0.18}{\includegraphics{figs/badinstance_rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_{[i,j]}$ on vertex $v^{\rig}_{[i,j]}$ in the instance $(G_{[i,j]}, \Sigma_{[i,j]})$.}\label{fig: bad v_right rotation}
\end{figure}


We will use the following claims later for completing the proof of \Cref{thm: disengagement - main} in the special case.


\znote{the following two observations to modify}
\begin{observation}
	\label{obs: disengaged instance size}
	The total number of edges in all sub-instances we have defined is $O(|E(G)|)$.
\end{observation}
\begin{proof}
	\iffalse 
	Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le r}$, each graph of $\set{G_i}_{1\le i\le r}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node, so each edge of $G_i$ corresponds to an edge in $E(G)$.
	Therefore, for each $1\le i\le r$, 
	$$|E(G_i)|=|E_G(C_i)|+|\delta_G(C_i)|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu.$$
	\fi
	%
	Note that $E(G_i)=E(C_i)\cup \hat E_i\cup \hat E_{i-1}\cup E_i^{\lef} \cup E_i^{\rig}\cup E_i^{\thr}$.
	First, each edge of $\bigcup_{1\le i\le r}E(C_i)$ appears in exactly one graphs of $\set{G_i}_{1\le i\le r}$. 
	Second, each edge of $\bigcup_{1\le i\le r}\hat E_i$ appears in exactly two graphs of $\set{G_i}_{1\le i\le r}$.
	Consider now an edge $e\in E'$. If $e$ connects a vertex of $C_i$ to a vertex of $C_j$ for some $j\ge i+2$, then $e$ will appear as an edge in $E_i^{\rig}\subseteq E(G_i)$ and an edge in $E_j^{\lef}\subseteq E(G_j)$, and it will appear as an edge in $E_k^{\thr}\subseteq E(G_k)$ for all $i<k<j$.
	On one hand, we have $\sum_{1\le i\le r}|E_i^{\lef} \cup E_i^{\rig}|\le 2|E(G)|$. 
	On the other hand, note that $E_k^{\thr}=E(C_{k-1},C_{k+1})\cup E^{\through}_{k-1}\cup E^{\through}_{k}$, and each edge of $e$ appears in at most two graphs of $\set{G_i}_{1\le i\le r}$ as an edge of $E(C_{k-1},C_{k+1})$.
	Moreover, from \Cref{obs: bad inded structure}, $|E^{\through}_{k-1}|\le |\hat E_{k-1}|$ and $|E^{\through}_{k}|\le |\hat E_{k}|$.
	Altogether, we have
	\begin{equation}
	\begin{split}
	\sum_{1\le i\le r}|E(G_i)| & =
	\sum_{1\le i\le r}\left(
	|E(C_i)|+ |\hat E_i|+ |\hat E_{i-1}|+ |E_i^{\lef}| + |E_i^{\rig}|+|E_i^{\thr}|
	\right)\\
	& = \sum_{1\le i\le r}
	|E(C_i)|+ \sum_{1\le i\le r} \left(|E_i^{\lef}| + |E_i^{\rig}|\right)+ \sum_{1\le i\le r}\left(|E_i^{\thr}|+ |\hat E_i|+ |\hat E_{i-1}|\right)\\
	& \le |E(G)|+ 2\cdot |E(G)| + \sum_{1\le i\le r}\left(|E(C_{i-1},C_{i+1})|+ 2|\hat E_i|+ 2|\hat E_{i-1}|\right)\\
	& \le 8\cdot |E(G)|.
	\end{split}
	\end{equation}
	This completes the proof of \Cref{obs: disengaged instance size}.
\end{proof}


\begin{observation}
	\label{obs: rotation for stitching}
	For each $1\le i\le r-1$, if we view the edge in $\delta_{G_i}(v^{\rig}_i)$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})$ as edges of $E(G)$, then $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$, and moreover, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{observation}
\begin{proof}
	Recall that for each $1\le i\le r-1$, 
	$\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})=\hat E_{i}\cup E^{\thr}_{i+1}\cup E^{\lef}_{i+1}$. From the definition of sets $E_i^{\thr},E_{i+1}^{\thr}, E^{\rig}_i, E^{\lef}_{i+1}$,
	\[
	\begin{split}
	E_i^{\thr}\cup E^{\rig}_i
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i<j'\text{ or }i'=i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'\le i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'< i+1\le j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i+1<j'\text{ or }i'<i+1=j'}=E^{\thr}_{i+1}\cup E^{\lef}_{i+1}.
	\end{split}
	\]
	Therefore, $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$.
	Moreover, from the definition of path sets $\wset^{\rig}_i$ and $\wset^{\lef}_{i+1}$, it is not hard to verify that, for every edge $e\in \delta_{G_i}(v^{\rig}_i)$, the path in $\wset^{\rig}_i$ that contains $e$ as its first edge is identical to the path in $\wset^{\lef}_{i+1}$ that contains $e$ as its first edge. According to the way that rotations $\oset^{\rig}_i,\oset^{\lef}_{i+1}$ are defined, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{proof}

\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\iffalse{backup: original analysis of total cost of subinstances}

Specifically, we use the following two claims, whose proofs will be provided later.

\begin{claim}
	\label{claim: existence of good solutions special}
	$\expect{\sum_{1\le i\le r}\optcrors(G_i,\Sigma_i)}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$.
\end{claim}

\begin{claim}
	\label{claim: stitching the drawings together}
	There is an efficient algorithm, that given, for each $1\le i\le r$, a feasible solution $\phi_i$ to the instance $(G_i,\Sigma_i)$, computes a solution to the instance $(G,\Sigma)$, such that $\cro(\phi)\le \sum_{1\le i\le r}\cro(\phi_i)$.
\end{claim}

We use the algorithm described in~\Cref{sec: guiding and auxiliary paths} and~\Cref{sec: compute advanced disengagement}, and return the disengaged instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ as the collection of sub-instances of $(G,\Sigma)$. 
From the previous subsections, the algorithm for producing the sub-instances is efficient.
On the other hand, it follows immediately from \Cref{obs: disengaged instance size}, \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together} that the sub-instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ satisfy the properties in \Cref{thm: disengagement - main}.
This completes the proof of \Cref{thm: disengagement - main}.

We now provide the proofs of \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together}.

$\ $

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
	Let $\phi^*$ be an optimal drawing of the instance $(G,\Sigma)$.
	We will construct, for each $1\le i\le r$, a drawing $\phi_i$ of $G_i$ that respects the rotation system $\Sigma_i$, based on the drawing $\phi^*$, such that $\sum_{1\le i\le r}\cro(\phi_i)\le O((\cro(\phi^*)+|E(G)|)\cdot 2^{O((\log m)^{3/4}\log\log m)})$, and \Cref{claim: existence of good solutions special} then follows.
	
	\paragraph{Drawings $\phi_2,\ldots,\phi_{r-1}$.}
	First we fix some index $2\le i\le r-1$, and describe the construction of the drawing $\phi_i$. We start with some definitions.
	Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
	We define the auxiliary path set $\wset_i=\wset^{\lef}_i\cup \wset^{\rig}_i$, so 
	$$\wset_i=\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}\cup \set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}},$$
	where for each $e\in E^{\lef}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$; for each $e\in E^{\rig}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between $u_{i+1}$ and its last endpoint; and for each $e\in E^{\thr}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$, the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$, and the subpath of $P_e$ between $u_{i+1}$ and its last endpoint.
	
	\iffalse
	We use the following observation.
	\begin{observation}
		\label{obs: wset_i_non_interfering}
		The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
	\end{observation}
	\begin{proof}
		Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
		And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
		Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
		From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
	\end{proof}
	\fi
	
	
	For uniformity of notations, for each edge $\hat e\in \hat E_i$, we rename the path $Q_{i+1}(\hat e)$ by $W_{\hat e}$, and similarly for each edge $\hat e\in \hat E_{i-1}$, we rename the path $Q_{i-1}(\hat e)$ by $W_{\hat e}$. Therefore, $\wset_i=\set{W_e\mid e\in E(G_i)\setminus E(C_i)}$.
	Put in other words, the set $\wset_i$ contains, for each edge $e$ in $G_i$ that is incident to $v^{\lef}_i$ or $v^{\rig}_i$, a path named $W_e$.
	It is easy to see that all paths in $\wset_i$ are internally disjoint from $C_i$.
	We further partition the set $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_e\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.
	
	We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
	Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
	We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
	Specifically, we proceed in the following four steps.
	
	
	
	\paragraph{Step 1.}
	For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
	We denote by $\Pi_e$ the set of these curves.
	We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
	Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
	and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
	In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
	And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
	Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
	We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.
	
	%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
	We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
	%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
	For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
	Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
	Therefore, $\hat{\chi}_i(P)$ is well-defined.
	For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.
	
	\iffalse
	We use the following observation.
	\znote{maybe remove this observation?}
	
	%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.
	
	\begin{observation}
		\label{obs: curves_crossings}
		The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
		%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
		and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
	\end{observation}
	\begin{proof}
		We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
		Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
		Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
		It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		
		We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
		Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
		It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	\end{proof}
	\fi
	
	\paragraph{Step 2.}
	For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
	We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
	Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
	We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
	(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
	%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
	(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
	(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
	\iffalse{just for backup}
	\begin{proof}
		Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
		For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
		We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
		It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
		We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
		See Figure~\ref{fig: curve_con} for an illustration.
		Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
		It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
		Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
		Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
		Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	\end{proof}
	\begin{figure}[h]
		\centering
		\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
		\hspace{1pt}
		\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
			\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
		\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
	\end{figure}
	\fi
	
	%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
	We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
	This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
	We use the following observation.
	\begin{observation}
		\label{obs: general_position}
		Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
	\end{observation}
	\begin{proof}
		From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
	\end{proof}
	
	
	
	
	%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.
	
	
	\paragraph{Step 3.} 
	So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
	where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
	and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
	Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
	Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
	Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
	We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
	We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.
	
	
	Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
	Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
	It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
	However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.
	
	
	
	
	
	\paragraph{Step 4.}
	Let $\dset$ be an arbitrarily small disc around $z_{\rig}$ in the drawing $\phi'_i$, and let $\dset'$ be another small disc around $z_{\rig}$ that is strictly contained in $\dset$.
	We first erase the drawing of $\phi'_i$ inside the disc $\dset$, and for each edge $e\in \delta(v^{\rig}_i)$, we denote by $p_{e}$ the intersection between the curve representing the image of $e$ in $\phi'_i$ and the boundary of $\dset$.
	We then place, for each edge $e\in \delta(v^{\rig}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{\rig}_{i}$. 
	We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{\rig}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$.
	Finally, for each edge $e\in \delta(v^{\rig}_i)$, let $\gamma_e$ be the concatenation of (i) the image of $e$ in $\phi'_i$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z_{\rig}$ in $\dset'$.
	We view $\gamma_e$ as the image of edge $e$, for each $e\in \delta(v^{\rig}_i)$. 
	We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$, and therefore it respects the rotation system $\Sigma_i$.
	
	We use the following claim.
	\begin{claim}
		\label{clm: rerouting_crossings}
		The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	\end{claim}
	\begin{proof}
		Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
		From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		
		%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
		For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
		Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
		We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.
		
		We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
		From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
		Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
		%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
		\begin{figure}[h]
			\centering
			\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
			\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
		\end{figure}
	\end{proof}
	
	From the above discussion and Claim~\ref{clm: rerouting_crossings}, for each $2\le i\le r-1$, 
	\[
	\cro(\phi_i)=\chi^2(C_i)+O\left(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right).
	\]
	
	
	
	\iffalse
	We now estimate the number of crossings in $\phi_i$ in the next claim.
	\begin{claim}
		\label{clm: number of crossings in good solutions}
		$\cro(\phi_i)=\chi^2(C_i)+O\left(\sum_{W\in \tilde\wset_i}\cro(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)$.
	\end{claim}
	\begin{proof}
		$2\cdot \sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2=\sum_{v\in V(G)}\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2.$
		\znote{need to redefine the orderings $\oset^{\lef}_i$ and $\oset^{\rig}_i$ to get rid of $\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2$ here, which we may not be able to afford.}
	\end{proof}
	\fi
	
	
	\paragraph{Drawings $\phi_1$ and $\phi_{r}$.}
	The drawings $\phi_1$ and $\phi_{r}$ are constructed similarly. We describe the construction of $\phi_1$, and the construction of $\phi_1$ is symmetric.
	Recall that the graph $G_1$ contains only one super-node $v_1^{\rig}$, and $\delta_{G_1}(v_1^{\rig})=\hat E_1\cup E^{\rig}_1$. We define $\wset_1=\set{W_e\mid e\in E^{\rig}_1}\cup \set{Q_2(\hat e)\mid \hat e\in \hat E_1}$. For each $\hat e\in \hat E_1$, we rename the path $Q_2(\hat e)$ by $W_e$, so $\wset_1$ contains, for each edge $e\in \delta_{G_1}(v^1_{\rig})$, a path named $W_e$ connecting its endpoints to $u_2$. Via similar analysis in \Cref{obs: wset_i_non_interfering}, it is easy to show that the paths in $\wset_1$ are non-transversal with respect to $\Sigma$.
	
	We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
	We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{r-1}$. 
	We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
	Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
	%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
	We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
	Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
	\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
	Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
	\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{r-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]
	
	
	
	
	We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le r}\cro(\phi_i)$.
	Recall that, for each $1\le i\le r$, $\tilde \wset_i=\set{W_e\mid e\in \hat E_{i-1}\cup \hat E_{i-1}\cup E^{\lef}_{i}\cup E^{\rig}_{i}}$, where $E^{\lef}_{i}=E(C_i,\bigcup_{1\le j\le i-2}C_j)$, and 
	$E^{\rig}_{i}=E(C_i,\bigcup_{i+2\le j\le r}C_j)$. Therefore, for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, the path $W_e$ belongs to exactly $2$ sets of $\set{\tilde\wset_i}_{1\le i\le r}$.
	Recall that the path $W_e$ only uses edges of the inner path $P_e$ and the outer path $P^{\out}_e$.
	Let $\tilde\wset=\bigcup_{1\le i\le r}\tilde\wset_i$, from \Cref{obs: edge_occupation in outer and inner paths}, 
	for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, $\cong_G(\tilde\wset,e)=O(1)$, and
	for $1\le i\le r$ and for each edge $e\in E(C_i)$, $\cong_G(\tilde\wset,e)=O(\cong_G(\qset_i,e))$.
	
	Therefore, on one hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{W\in \tilde\wset_i}\hat\chi_i(W)
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} 2\cdot \cong_G(\tilde \wset,e)\cdot\cong_G(\tilde \wset,e')\\
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} \left(\cong_G(\tilde \wset,e)^2+\cong_G(\tilde \wset,e')^2\right)\\
	& \le 
	\sum_{e\in E(G)} \chi(e)\cdot \cong_G(\tilde \wset,e)^2
	= O(\cro(\phi^*)\cdot\temp),
	\end{split}
	\]
	and on the other hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2
	%= \sum_{e\in E(G)} \sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)^2 
	& \le  \sum_{e\in E(G)} \left(\sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)\right)^2\\
	& \le O\left(\sum_{e\in E(G)} \cong_G(\tilde \wset,e)^2 \right)\\
	& \le O\left(|E(G)|+\sum_{1\le i\le r}\sum_{e\in E(C_i)} \cong_G(\qset_i,e)^2\right)=O(|E(G)|\cdot\temp).
	\end{split}
	\]
	Moreover, $\sum_{1\le i\le r}\chi^2(C_i)\le O(\cro(\phi^*))$, and $\sum_{1\le i\le r}\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})\le O(\cro(\phi^*)\cdot\temp)$.
	
	Altogether,
	\[
	\begin{split}
	\sum_{1\le i\le r}\cro(\phi_i)
	& \le 
	O\left(\sum_{1\le i\le r} 
	\left(
	\chi^2(C_i)+ \hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)
	\right)\\
	& \le O(\cro(\phi^*))+O(\cro(\phi^*)\cdot\temp)+O(\cro(\phi^*)\cdot\temp)+O(|E(G)|\cdot\temp)\\
	& \le O((\cro(\phi^*)+|E(G)|)\cdot\temp).
	\end{split}
	\]
	
	This completes the proof of \Cref{claim: existence of good solutions special}.
\end{proofof}

\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse{incorrect analysis of non-interfering}
We use the following observation.
\begin{observation}
	\label{obs: wset_i_non_interfering}
	The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
	Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
	And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
	Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
	From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
\end{proof}
\fi








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse {previous nudging and uncrossing steps}

We further partition $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_i(e)\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.

We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
Specifically, we proceed in the following four steps.



\paragraph{Step 1.}
For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
We denote by $\Pi_e$ the set of these curves.
We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.

%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
Therefore, $\hat{\chi}_i(P)$ is well-defined.
For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.

\iffalse
We use the following observation.
\znote{maybe remove this observation?}

%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.

\begin{observation}
	\label{obs: curves_crossings}
	The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
	%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
	and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
\end{observation}
\begin{proof}
	We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
	Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
	Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
	It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	
	We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
	Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
	It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
\end{proof}
\fi

\paragraph{Step 2.}
For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
\iffalse{just for backup}
\begin{proof}
	Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
	For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
	We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
	It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
	We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
	See Figure~\ref{fig: curve_con} for an illustration.
	Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
	It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
	Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
	Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
	Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
\end{proof}
\begin{figure}[h]
	\centering
	\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
	\hspace{1pt}
	\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
		\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
	\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
\end{figure}
\fi

%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
We use the following observation.
\begin{observation}
	\label{obs: general_position}
	Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
\end{observation}
\begin{proof}
	From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
\end{proof}




%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.


\paragraph{Step 3.} 
So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.


Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.

\fi




==> hierarch-clustering.tex <==
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
\section{Main Tool: Subinstances and Hierarchical Bad Clusterings}
\label{sec: hierarchnical clustering}
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------
%----------------------------------------------


Let $I^*=(G^*,\Sigma^*)$ be the input instance of the \CNwRS problem. Throughout this paper, we always denote by $m^*$ the number of edges in $G^*$, and we use a parameter $\mu=2^{(\log m^*)^{3/4}}$. 
Our algorithm for solving the \CNwRS problem is recursive, and, over the course of the recursion, we will consider some instances $(G,\Sigma)$, that we call \emph{subinstances} of $G^*$.



\subsection{Subinstances of the Input instance} 
\label{subsec: subinstances}

A subinstance $I=(G,\Sigma)$ of the input instance $I^*=(G^*,\Sigma^*)$ is determined by a sub-graph $G'\subseteq G^*$, and a collection $\set{S_1,\ldots,S_q}$ of disjoint subsets of vertices of $G'$. Graph $G$ is obtained from $G'$ by unifying, for all $1\leq i\leq q$, all vertices of $S_i$ into a vertex $u_i$. We keep parallel edges but remove self-loops. For every regular vertex $v\in V(G)$ that is also a vertex of $G^*$, its rotation system $\oset_v$ in $\Sigma$ remains the same as in $\Sigma^*$, while for every vertex $u_i$ corresponding to set $S_i$, we will define its rotation system $\oset_{u_i}$ explicitly. Notice that the subinstance relation is transitive: if $(G_1,\Sigma_1)$ is a subinstance of $(G_0,\Sigma_0)$, and $(G_2,\Sigma_2)$ is a subinstance of $(G_1,\Sigma_1)$, then $(G_2,\Sigma_2)$ is a subinstance of $(G_0,\Sigma_0)$.

Our algorithm proceeds by first decomposing the input instance $I^*$ of \CNwRS into a collection $\set{I_1,\ldots,I_r}$ of subinstances. Each such subinstance is then solved recursively, and can be in turn further decomposed into subinstances. 

We will ensure that the total number of recursive levels is bounded by $\ell= \frac{\log(m^*)}{\log \mu}\leq (\log m^*)^{1/4}$.
 Each level $i$ of the recursion is then associated with a collection $\jset_i$ of subinstances of the input instance $I^*$. 





\subsection{Main Parameters}

 Before we define the hierarchical bad clustering we need to introduce some parameters.

Recall that we have defined the parameter $\mu=2^{(\log m^*)^{3/4}}$, and that the number of the recursive levels is $\ell\leq \frac{\log m^*}{\log \mu}\leq (\log m^*)^{1/4}$.

We will use the following parameters for bandwidth property of clusters: $\alpha^*=1/(\log m^*)^3$, and for $1\leq i\leq \ell$, $\alpha_i=(\alpha^*)^i$. Note that $\alpha_{\ell}=(\alpha^*)^{\ell}\leq 1/(\log m^*)^{3(\log m^*)^{1/4}}\geq 1/ 2^{O((\log m^*)^{1/4}\log\log m^*)}$.

The second central parameter that we use is: 
%
\[\eta^*=\frac{(\log m^*)^{50}}{\alpha_{\ell}^3}\leq  2^{O((\log m^*)^{1/4}\log\log m^*)}.\]
%
We also define $\eta_1=(\eta^*)^9$, and, for $1\leq i<\ell$, we let $\eta_{i+1}=\frac{\eta_i(\log m^*)^{51}}{\alpha^8\cdot \alpha_{\ell}^2}$.


Note that:
\begin{equation}\label{eq: bound on etaell}
\eta_{\ell}\leq \frac{\eta_1\cdot(\log m^*)^{O(\ell)}}{\alpha_{\ell}^{3\ell}}\leq (\eta^*)^9\cdot 2^{O((\log m^*)^{1/2}\log\log m^*)}\leq 2^{O((\log m^*)^{1/2}\log\log m^*)}.
\end{equation}


\subsection{Hierarchical Bad Clustering}
One of the main tools that our algorithm uses is Hierarchical Bad Clustering. Throughout this subsection, we assume that we are given some subinstance $I=(G,\Sigma)$ of the input instance $I^*$ of \CNwRS problem. 

Given a connected subgraph $C\subseteq G$ (that we refer to as a \emph{cluster}), we let the $\Sigma_C$ be the rotation system for the cluster $C$ that ins induced by the rotation system $\Sigma$ for $G$. Therefore, we can associate, with a cluster $C\subseteq G$, an instance $(C,\Sigma_C)$ of the \cnwrs problem. We denote by $k(C)=|\delta_G(C)|$.

We start by defining a level-1 bad cluster.

\begin{definition}[Level-1 bad cluster]
	We say that a connected vertex-induced subgraph $C\subseteq G$ is a \emph{level-1 bad cluster} iff:
	
	\begin{itemize}
		\item cluster $C$ has the $\alpha_1$-bandwidth property in $G$; 
		\item $\optcrors(C,\Sigma_C)\geq \frac{(k(C))^2}{\eta_1}$; and
		\item $\optcrors(C,\Sigma_C)\geq \frac{(|E(C)|+k(C))^2}{\eta_{\ell}}$.
	\end{itemize}
\end{definition}



In order to define a level-$i$ bad cluster, suppose we are given some subgraph $C$ of $G$, and a collection $\bset$ of disjoint subgraphs of $C$, each of which is a bad cluster from levels $1,\ldots,i-1$. Recall that $C_{|\bset}$ is a contracted graph, that is obtained from $C$, by contracting every cluster $B\in \bset$ into a supernode. We denote: $\mout_{\bset}(C)=|E(C_{|\bset})|+k(C)$.
Note that $C_{|\bset}$ is a subgraph of the contracted graph $G_{|\bset}$.

\begin{definition}[Level-i bad cluster]
	Given a connected a connected vertex-induced subgraph $C\subseteq G$, and a collection $\bset$ of disjoint vertex-induced subgraphs of $C$, such that for all $B\in \bset$, $B$ is a level-$i'$ bad cluster, for $1\leq i'< i$, we say that $C$ is a \emph{level-i bad cluster} (with respect to $\bset$) iff:
	
	\begin{itemize}
		\item cluster $C_{|\bset}$ has the $\alpha^*$-bandwidth property in $G_{|\bset}$; 
		\item $\optcrors(C,\Sigma_C)\geq \frac{(k(C))^2}{\eta_i}$; and
		\item $\optcrors(C,\Sigma_C)\geq \frac{(\mout(C))^2}{\eta_{\ell}}$.
	\end{itemize}
\end{definition}

We will denote by $\bset(C)$ the set $\bset$ of clusters, such that $C$ is a level-$i$ bad cluster with respect to $\bset$.
Notice that, from the above definition, if cluster $C$ is a level-$i$ bad cluster with respect to cluster set $\bset(C)$, then it is also a level-$j$ bad cluster, for all $j>i$ (this is true since we allow $\bset(C')=\emptyset$, in which case $C'_{|\bset(C')}=C'$. Therefore, we can assume w.l.o.g. that, if $C$ is a level-$i$ bad cluster with respect to a collection $\bset(C)$ of its subgraphs, then every clusters in $\bset(C)$ is a level-$(i-1)$ cluster.

We also associate, with each bad cluster $C$, a hierarchical decomposition $\hset(C)$. If $C$ is a level-$1$ bad cluster, then  $\hset(C)$ contains a single cluster -- the cluster $C$.
If $C$ is a level-$i$ bad cluster with respect to cluster set $\bset(C)$, then we set $\hset(C)=\bigcup_{C'\in \bset(C)}\hset(C')$.
We say that every cluster in set $\bset(C)$ is a \emph{child-cluster} of $C$, and all clusters in $\hset(C)$ are \emph{descendant-clusters} of $C$.


Whenever we say that we are given a level-$i$ bad cluster $C$, we assume that we are given its corresponding hierachical decomposition $\hset(C)$; note that the corresponding set $\bset(C)$ of clusters is implicit from $\hset(C)$.

We will use the following simple observation regarding bad clusters.

\begin{observation}\label{obs: bandwidth property}
	Let $I=(G,\Sigma)$ be an instance of \CNwRS and let $C\subseteq G$ be a level-$i$ bad cluster in $G$, for some $1\leq i\leq \ell$, with respect to the hierarchical decomposition $\hset(C)$. Then cluster $C$ has the $(\alpha^*)^i$-bandwidth property in graph $G$.
\end{observation}

\begin{proof}
	The proof is by induction on $i$. For $i=1$, if $C$ is a level-$1$ bad cluster, then, from the definition, $C$ has the $\alpha_1$-bandwidth property in $G$, and $\alpha_1=\alpha^*$.
	
	Consider now some cluster $C$, that is a level-$i$ bad cluster with respect to cluster set $\bset=\bset(C)$. From the induction hypothesis, each cluster $C'\in \bset$ has the $(\alpha^*)^{i-1}$-bandwidth property in $G$, and from the definition of level-$i$ bad cluster, graph $C_{|\bset}$ has the $\alpha^*$-bandwidth property in $G_{\bset}$. 
	
	Let $G'$ be the graph obtained from $G$ as follows. First, we subdivide every edge $e\in \delta_G(C)$ with a vertex $t_e$, and set $T=\set{t_e\mid e\in \delta_G(C)}$. We then let $G'$ be the subgraph of the resulting graph induced by $V(C)\cup T$. Consider now the graph $G'_{|\bset}$.
	Alternatively, this graph can be obtained from $G_{|\bset}$ via a similar procedure: subdivide every edge $e\in \delta_G(C)$ with a vertex $t_e$, and let $G'_{|\bset}$ be a subgraph of the resulting graph induced by $V(C_{|\bset})\cup T$. Since cluster $C_{|\bset}$ has the $\alpha^*$-bandwidth property in $G_{\bset}$, vertex set $T$ is $\alpha^*$-well-linked in $G'_{\bset}$. From \Cref{clm: contracted_graph_well_linkedness}, vertex set $T$ is $(\alpha^*)^{i-1}\cdot \alpha^*=(\alpha^*)^{i}$-well-linked in $G'$. It is then easy to verify that cluster $C$ has the $(\alpha^*)^{i}$-bandwidth property in $G$.
\end{proof}




In our recursive algorithm for the \cnwrs problem, for every instance $I=(G,\Sigma)\in \jset_i$ at the $i$th recursive level, we will also compute a collection $\bset$ of bad level-$i$ clusters for $G$. 
We denote by $\mout_{\bset}(G)=|E(G_{|\bset})|$ the number of edges in the corresponding contracted graph. We will ensure that, for every instance $I=(G,\Sigma)\in \jset_i$, $\mout_{\bset}(G)\leq m^*/\mu^{i-1}$. In other words, at every level of the recursion, the number of edges in the contracted graphs that we obtain decreases by factor $\mu$. Since  $\mu=2^{(\log m^*)^{3/4}}$, this ensures that the number of the recursive levels is indeed bounded by $\ell=(\log m^*)^{1/4}$.

It will be convenient for us to consider special drawings of the instances $I$, that are \emph{canonical} with respect to their corresponding bad clusterings. In the following subsection we define such drawings and provide some results regarding their existance, and an algorithm for computing such a drawing.



\subsection{Canonical Drawing with Respect to Bad Clusters}

Suppose we are given some subinstance $I=(G,\Sigma)$ of the input instance $I^*$ of \cnwrs, and a collection $\bset$ of disjoint level-$i$ bad clusters for $I$. We will consider special types of solutions to instance $I$, that are \emph{canonical} with respect to the clusters in $\bset$. In this subsection we start by defining such canonical solutions. We then prove that there is an efficient algorithm to compute a canonical solution to instance $I$, whose cost is comparable to $\optcrors(I)+\mout_{\bset}(G)$. Lastly, we show that any solution to instance $I$ can be converted into a canonical solution, with only a slight increase in the solution cost.

We now define canonical drawings. 

\begin{definition}[Canonical Drawing with Respect to Level-1 Bad Cluster]
	Let $I=(G,\Sigma)$ be an instance of $\cnwrs$, let $\phi$ be any solution to this instance, and let $C$ be a level-$1$ bad cluster for $I$.
	We say that $\phi$ is a \emph{canonical solution with respect to $C$} iff there is a disc $D(C)$ containing the image of all vertices and edges of $C$, such that the images of all vertices and edges of $G\setminus C$ are disjoint from $D(C)$, and for every edge $e\in \delta_G(C)$, the intersection of the image of $e$ with the disc $D(C)$ is a simple curve, so in particular the intersection of the image of $e$ with the boundary of $D$ is a single point.
\end{definition}



\begin{definition}[Canonical Drawing with Respect to Level-i Bad Cluster]
	Let $I=(G,\Sigma)$ be an instance of $\cnwrs$, let $\phi$ be any solution to this instance, and let $C$ be a level-$i$ bad cluster with respect to a collection $\bset(C)$ of disjoint level-$(i-1)$ bad clusters that are subgraphs of $C$.
	We say that $\phi$ is a \emph{canonical solution with respect to $C$} iff:
	
	\begin{itemize}
		\item for every cluster $C'\in \bset(C)$, drawing $\phi$ is canonical with respect to $C'$; and
		\item there is a disc $D(C)$ containing the image of all vertices and edges of $C$, such that the images of all vertices and edges of $G\setminus C$ are disjoint from $C$, and for every edge $e\in \delta_G(C)$, the intersection of the image of $e$ with the disc $D(C)$ is a simple curve.
	\end{itemize}
\end{definition}


The following simple claim allows us to compute a canonical solution for an instance $(G,\Sigma)$ of the \cnwrs problem with a set $\bset_i$ of disjoint level-$i$ bad clusters.

\begin{claim}\label{claim: find trivial canonical solution}
There is an efficient algorithm, that, given an instance $I=(G,\Sigma)$ of the \cnwrs problem, together with a collection $\bset_i$ of disjoint level-$i$ bad clusters for $I$, computes a solution $\phi$ to instance $I$, with at most $(\mout_{\bset_i}(G))^2+O\left(\optcrors(G,\Sigma)\cdot \eta_{\ell}\cdot i\right )$ crossings.
\end{claim}

\begin{proof}
	For all $1\leq i'< i$, we define a collection $\bset_{i'}$ of level-$i'$ bad clusters, as follows. Note that set $\bset_i$ of level-$i$ bad clusters is given as part of the input to the algorithm. For $1\leq i'<i$, assume that set $\bset_{i'+1}$ of level-$(i'+1)$ bad clusters is given. We then set $\bset_{i'}=\bigcup_{C'\in \bset_{i'+1}}\bset(C')$.
	
	%Recall that for every cluster $C\in \bset_i$, we are given a collection $\bset_{i-1}(C)$ of level-$(i-1)$ bad clusters, such that $C$ is a bad level-$i$ cluster with respect to $\bset_{i-1}(C)$. Denote $\bset_{i-1}=\bigcup_{C\in \bset_i}\bset_{i-1}(C)$. Similarly, for every cluster $C'\in \bset_{i-1}$, we are given a collection $\bset_{i-2}(C')$ of  level-$(i-2)$ bad clusters, such that $C'$ is a bad level-$i-1$ cluster with respect to $\bset_{i-2}(C')$. We then set $\bset_{i-2}=\bigcup_{C'\in \bset_{i-1}}\bset_{i-2}(C')$. Continuing in this manner, we can define, for all $0\leq i'< i$, a collection $\bset_{i'}$ of disjoint level-$i'$ bad clusters, where $\bset_{i'}=\bigcup_{C''\in \bset_{i'+1}}\bset_{i'}(C'')$.
	
	For all $1\leq i'\leq i$, we let $G_{i'}=G_{|\bset_{i'}}$ be the contracted graph constructed with respect to the clusters in $\bset_{i'}$. We define a rotation system $\Sigma_{i'}$ for graph $G_{i'}$ as follows. For every vertex $v\in V(G_{i'})$ that is also a vertex of $G$, its rotation $\oset^{i'}_v$ in $\Sigma_{i'}$ remains the same as in $\Sigma$. For a vertex $v\in V(G_{i'})$ that corresponds to some cluster $C'\in \bset_{i'}$, we let the rotation $\oset_v^{i'}\in \Sigma^{i'}$ be an arbitrary ordering of its incident edges in $G_{i'}$.
		
	We perform $i+1$ iterations. For $1\leq i'\leq i$, in iteration $i'$, we construct a solution $\phi_{i'}$ to instance $(G_{i'},\oset_{i'})$ of \cnwrs.
	
	In the first iteration, we consider instance $(G_i,\Sigma_i)$; recall that $G_i=G_{|\bset_i}$, and $|E(G_i)|=\mout_{\bset_i}(G)$. We use the algorithm from \Cref{thm: crwrs_uncrossing} to construct a solution $\phi_i$ to instance $(G_i,\Sigma_i)$, such that the number of crossings in $\phi_i$ is bounded by $|E(G_i)|^2\leq (\mout_{\bset_i}(G))^2$.
	
	We now fix some index $1\leq i'<i$, and assume that we are given a solution $\phi_{i'+1}$ to instance $(G_{i'+1},\Sigma_{i'+1})$. We show an algorithm to construct a solution $\phi_{i'}$ to instance $(G_{i'},\Sigma_{i'})$. 
	
	Consider a cluster $C'\in \bset_{i'}$, and the corresponding set $\bset(C')$ of clusters, such that $C'$ is a level-$i'$ bad cluster with respect to $\bset(C')$. Consider the contracted graph $\tilde C'=C'_{|\bset(C')}$, and recall that $|E(\tilde C')|+k(C')=\mout_{\bset(C')}(C)$. Denote $\tilde \bset_{i'}=\set{\tilde C'\mid C'\in \bset_{i'}}$. Observe that graph $G_{i'+1}$ is precisely the contracted graph of $G_{i'}$ with respect to $\bset_{i'}$, that is, $G_{i'+1}=(G_{i'})_{|\bset_{i'}}$. Intuitively, in order to obtain a solution $\phi_{i'}$ to instance $(G_{i'},\Sigma_{i'})$ from solution $\phi_{i'+1}$ to instance $(G_{i'+1},\Sigma_{i'+1})$, we need to replace, for every cluster $C'\in \beta_{i'}$, the image of the vertex $v(C')$ in $\phi_{i'}$ with a drawing of $\tilde C'$.
	
	We process each cluster $C'\in \bset_{i'}$ one by one. Consider the interation when cluster $C'$ is processed. We inflate the image of the vertex $v(C')$ in the current drawing, so it becomes a disc, that we denote by $D(C')$. We denote by $\lambda(C')$ the boundary of this disc. We also let $D'(C')$ be a slightly smaller disc lying in the interior of $D(C')$, whose boundary is denoted by $\lambda'(C')$. Using the algorithm from 
	\Cref{thm: crwrs_uncrossing}, we construct a drawing $\psi(\tilde C')$ of graph $\tilde C'$, with at most $|E(\tilde C')|^2$ crossings. We place this drawing inside the disc $D(C')$. Next, we consider the edges of $\delta_{G_{i'}}(\tilde C')$. Let $e=(u,v)$ be any such edge, with $v\in V(C')$ and $u\not\in V(C')$. Our current drawing contains a curve $\gamma_e$ (the image of the edge $e$ in $\phi_{i'+1}$), connecting the image of $u$ (or a supernode corresponding to a cluster of $\bset_{i'}$ containing $u$) to some point $p$ on $\lambda$. 
	We construct a curve $\gamma'_e$ inside the disc $D(C')$, connecting the image of $v$ to point $p$. It is easy to verify that the curves in set $\set{\gamma'_e\mid e\in \delta_{G_{i'}}(\tilde C')}$ can be constructed so that each such curve crosses the image of every edge of $\tilde C'$ at most once, and each pair of such curves crosses at most once. This step then adds at most $|\delta_G(C')|^2+|\delta_G(C')|\cdot |E(\tilde C')|$ new crossings.
	
	\mynote{maybe this should be explained better. Endpoints of edge $e$ may sit deep inside the subclusters.}
	
	Overall, the number of crossings that were added while processing cluster $C'$ is bounded by:
	
	\[ |E(\tilde C')|^2+|\delta_G(C')|^2+|\delta_G(C')|\cdot |E(\tilde C')| \leq (\mout_{\bset(C')})^2+k(C')\cdot \mout_{\bset(C')}+(k(C'))^2\leq O(\optcrors(C',\Sigma_{C'})\cdot \eta_{\ell})  \]
	
	(we have used the definition of type-$i'$ bad clusters for the last inequality.)
	
	Once every cluster $C'\in \bset_{i'}$ is processed, we obtain a solution $\phi_{i'}$ to instance  $(G_{i'},\Sigma_{i'})$. Since $\optcrors(G,\Sigma)\geq \sum_{C'\in \bset_{i'}}\optcrors(C',\Sigma_{C'})$, we get that:
	
	\[\cro(\phi_{i'})\leq \cro(\phi_{i'+1})+O\left(\eta_{\ell}\cdot \sum_{C'\in \bset_{i'}}\optcrors(C',\Sigma_{C'})\right )\leq \cro(\phi_{i'+1})+O\left (\optcrors(G,\Sigma)\cdot \eta_{\ell}\right ). \]
	
	In the last iteration, where $i'=0$, for every cluster $C'\in \bset_1$, we view $\bset(C')=\emptyset$, and $\tilde C'=C'$. The remainder of the algorithm remains unchanged. At the end of this iteration, we then obtain  drawing $\phi_0$ of instance $(G,\Sigma)$. It is immediate to verify that this drawing is canonical with respect to clusters in $\bset_i$. The number of crossings in drawing $\phi_i$ is bounded by $(\mout_{\bset_i}(G))^2$, while in each subsequent iteration, the number of crossings grows by at $O\left (\optcrors(G,\Sigma)\cdot \eta_{\ell}\right )$. Therefore, the total number of crossings in the final drawing is bounded by $(\mout_{\bset_i}(G))^2+O\left(\optcrors(G,\Sigma)\cdot \eta_{\ell}\cdot i\right )$.
\end{proof}

We obtain the following immediate corollary, that follows from the definition of a level-$i$ bad cluster.
Given any cluster $C$ of a graph $G$, we define its corresponding graph $C^+$ as follows. First, we subdivide every edge $e\in \delta_G(C)$ with a vertex $t_e$, and let $T=\set{t_e\mid e\in \delta_G(C)}$ be the set of these new vertices. We then let $C^+$ be the subgraph of the resulting graph induced by $V(C)\cup T$. Rotation system $\Sigma$ for $G$ naturally defines a rotation system $\Sigma_{C^+}$ for $C^+$.

\begin{corollary}\label{claim: find good drawing of type-i cluster}
	There is an efficient algorithm, that, given an instance $I=(G,\Sigma)$ of the \cnwrs problem, and a level-$i$ bad cluster $C$ for $G$, computes a solution $\phi(C^+)$ to instance $(C^+,\Sigma_{C^+})$ of \cnwrs, and a disc $D(C)$ containing the drawing $\phi(C)$, such that the vertices of $T$ are drawn on the boundary of $D(C)$, and $\cro(\phi(C^+))\leq O\left(\optcrors(C,\Sigma_C)\cdot \eta_{\ell}\cdot i\right )$. Moreover, the drawing $\phi(C^+)$ is canonical with respect to the clusters in $\bset(C)$.
\end{corollary}

\begin{proof}
The proof easily follows by applying the algorithm from \Cref{claim: find trivial canonical solution} to graph $C^+$. 
Let $\phi$ be the resulting drawing of $C^+$, together with the disc $D(C)$ containing the drawing of $C$. For every vertex $t\in T$, let $e_t$ be the unique edge of $C^+$ incident to $t$, and let $p_t$ be the unique point on the intersection of the image of $e_t$ and the boundary of disc $D(C)$. We slighlty modify the drawing $\phi$, by placing the image of every vertex $t\in T$ at point $p_t$, and then erasing the portion of the image of $e_t$ that lies outside the disc $D(C)$. From \Cref{claim: find trivial canonical solution}, the number of crossings in drawing $\phi$ is bounded by:


\[(\mout_{\bset(C)}(C^+))^2+O\left(\optcrors(C^+,\Sigma_{C}^+)\cdot \eta_{\ell}\cdot i\right ).\]

Since the vertices of $T$ have degree $1$ in $C^+$, it is easy to verify that $\optcrors(C^+,\Sigma_{C}^+)\leq \optcrors(C,\Sigma_C)$. Moreover, $\mout_{\bset(C)}(C^+)=\mout_{\bset(C)}(C)$, and, from the definition of a level-$i$ bad cluster, $(\mout_{\bset(C)}(C))^2\leq \optcrors(C,\Sigma_C)\cdot \eta_{\ell}$. Therefore, altogether, 
the number of crossings in the resulting drawing is at most $O\left(\optcrors(C,\Sigma_{C})\cdot \eta_{\ell}\cdot i\right )$.
\end{proof}


Lastly, we will use the following corollary to transform an arbitrary drawing of a graph $G$ into a drawing that is canonical with respect to a set $\bset_i$ of level-$i$ bad clusters of $G$.

\begin{lemma}\label{lemma: transform any drawing into canonical}
	There is an efficient algorithm, that, given an instance $I=(G,\Sigma)$ of the \cnwrs problem with $|V(G)|=n$, together with a collection $\bset_i$ of disjoint level-$i$ bad clusters for $I$, and a solution $\phi$ to instance $I$, computes a solution $\phi'$ to instance $I$ that is canonical with respect to all clusters in $\bset_i$, such that: 
	\[\cro(\phi')\leq O\left (\frac{\cro(\phi)\cdot \log^8n}{(\alpha^*)^{2i}}\right )+O\left(\optcrors(G,\Sigma)\cdot \eta_{\ell}\cdot i\right ).\]
\end{lemma}

\begin{proof}
	For convenience, we denote by $\hat G=G_{|\bset_i}$ the contracted graph of $G$ with respect to cluster set $\bset_i$.
From \Cref{obs: bandwidth property}, every cluster in $\bset_i$ has the $(\alpha^*)^i$-bandwidth property. We can then use the algorithm from \Cref{lem: crossings in contr graph} in order to compute a drawing $\hat \phi$ of $\hat G$, such that, for every  vertex $x\in V(\hat G)\cap V(G)$, the ordering of the edges of $\delta_G(x)$ as they enter $x$ in $\hat \phi$ is consistent with the ordering $\oset_x\in \Sigma$. Moreover, $\cro(\hat \phi)\leq O\left (\frac{\cro(\phi)\cdot \log^8n}{(\alpha^*)^{2i}}\right )$. Next, we process each cluster $C\in \bset_i$ one by one. Consider any such cluster $C$, and the image $p_C$ of the vertex $v_C$ representing the cluster $C$ in the contracted graph $\hat G$, in the current drawing.
We inflate point $p_C$ until it becomes a disc, that we denote by $D'(C)$. We denote by $\lambda'(C)$ the boundary of this disc. We also place a smaller disc $D(C)$ in the interior of $D'(C)$, and denote its boundary by $\lambda(C)$. Using the algorithm from 
\Cref{claim: find good drawing of type-i cluster}, we compute a solution $\psi(C^+)$ to instance $(C^+,\Sigma_{C^+})$ of \cnwrs, which is placed inside the disc $D(C)$, such that the images of the vertices in set $\set{t_e\mid e\in \delta_G(C)}$ appear on the boundary of disc $D(C)$. Recall that the drawing $\psi(C^+)$ is canonical with respect to the clusters in $\bset(C)$, and contains at most $O\left(\optcrors(C,\Sigma_C)\cdot \eta_{\ell}\cdot i\right )$ crossings.

Consider now some edge $e\in \delta_G(C)$, and assume that $e=(u,v)$, where $u\in V(C)$ and $v\not\in V(C)$. Let $\gamma_1(e)$ be the original image of the edge $e$; observe that $\gamma_1(e)$ connects the image of the vertex $v$ to some point $p_e$ on the boundary of the disc $D'(C)$. Let $\gamma_2(e)$ be the image of the edge $(u,t_e)$ in drawing $\psi(C^+)$, and the image of $t_e$ lies on the boundary of the disc $D(C)$. We define another curve, $\gamma_3(e)$, connecting the image of $t_e$ to point $p_e$, such that the curve $\gamma_3(e)$ is contained in $D'(C)\setminus D(C)$, except for its one endpoint that lies on the boundary of $D(C)$. We can define the curves in $\set{\gamma_3(e)\mid e\in \delta_G(C)}$ such that every pair of such curves crosses at most once. This incurs at most $(k(C))^2\leq \eta_{\ell}\optcrors(C,\Sigma_C)$ additional crossings. Note that the current iteration contributed at most $O\left(\optcrors(C,\Sigma_C)\cdot \eta_{\ell}\cdot i\right )$ new crossings to the current drawing.

Once every cluster $C\in \bset_i$ is processed, we obtain the final drawing $\phi'$, which is a solution to instance $(G,\Sigma)$, that is canonical with respect to all clusters in $\bset_i$. Since $\optcrors(G,\Sigma)\geq \sum_{C\in \bset_i}\optcrors(C,\Sigma_C)$, we get that:
%
\[
\begin{split}
\cro(\phi')&\leq O\left (\frac{\cro(\phi)\cdot \log^8n}{(\alpha^*)^{2i}}\right )+O\left(\sum_{C\in \bset_i}\optcrors(C,\Sigma_C)\cdot \eta_{\ell}\cdot i\right )\\
&\leq O\left (\frac{\cro(\phi)\cdot \log^8n}{(\alpha^*)^{2i}}\right )+O\left(\optcrors(G,\Sigma)\cdot \eta_{\ell}\cdot i\right ).\end{split}\]
\end{proof}


==> laminar.tex <==
\newpage

\section{Second Main Tool - Disengagement of Clusters}
\label{sec: not many paths}

%Assume we are given an instance $(G,\Sigma)$ of \CNwRS. Given a set $\pset$ of paths in a graph $G$, for each edge $e\in E(G)$, the \emph{congestion} of the paths in $\pset$ on edge $e$, that is denoted by $\cong_{\pset}(e)$, is defined to be the number of paths in $\pset$ in which $e$ participates. We denote by $\cong_{G}(\pset)=\max_{e\in E(G)}\set{\cong_{\pset}(e)}$ the congestion caused by the set $\pset$ of paths in $G$. 

%\input{cut_property}

%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------

\iffalse
%---------------------------
%---------------------------
%---------------------------
\subsection{First Tool: Well-Linkedness to Routing}


\begin{theorem}\label{thm: wl to paths}
	There is a randomized algorithm, that, given a graph $G$ and a cluster $C\subseteq G$, such that the boundary of $C$ is $\alpha$-well-linked in $C$, computes a vertex $u(C)\in C$, and a collection $\qset$ of paths routing $\delta_G(C)$ to $u(C)$ inside $C$, and a tree $\tau$ in $C\cup \delta(C)$ with root $u(C)$, such that the set $\qset$ of paths is the collection of all leaf-to-root paths in $\tau$ . Moreover, for every edge $e\in E(C)$ and value $\eta$, the probability that $e$ lies on more than $\eta$ paths in $\qset$ is bounded by $O(\frac{\poly\log n}{\alpha \eta})$.
\end{theorem}

\mynote{I have a proof in mind but I'm not 100\% sure. Also need to subdivide the edges of $\delta(C)$ and the resulting vertices should be the leaves of the tree.}



Consider now an instance $I=(G,\Sigma)$ of \cnwrs, and let $\cset$ be a collection of disjoint sub-graphs of $G$ called clusters, such that $\bigcup_{C\in \cset}V(C)=V(G)$. Assume further that the boundary of each cluster $C\in \cset$ is $\alpha$-well-linked in $C$. For each cluster $C\in \cset$, let $u(C)$ be a vertex of $C$, and $\qset(C)$ a set of paths routing the edges of $\delta(C)$ to $u(C)$. For every edge $e\in E(C)$, let $\eta(e)$ be the total number of paths in $\qset(C)$ that contain $e$. If an edge $e$ does not lie in any cluster in $\cset$, then we set $\eta(e)=0$.  Consider now a graph $G'$ that is obtained from $G$ by replacing every edge $e$ with $\eta(e)$ parallel edges if $\eta(e)>0$; otherwise we keep the edge $e$ as is. We refer to the set of parallel edges replacing $e$ as a \emph{bundle} of $e$, and denote it by $\beta(e)$. 
If $\eta(e)=0$, then we let $\beta(e)=\set{e}$.

Consider now some vertex $v\in V(G)$, and the set $\set{e_1,\ldots,e_r}$ of its incident edges, indexed in the order consistent with the ordering $\oset_v\in \Sigma$. Let $\oset'_v$ be a circular ordering of the edges of $\delta_{G'}(v)$. We say that $\oset'_v$ is \emph{consistent} with $\oset(v)$ iff for all $1\leq i\leq r$, all edges of $\beta(e_i)$ appear consecutively in $\oset'_v$, and the edges belonging to different bundles appear in the ordering $\beta(e_1),\beta(e_2),\ldots,\beta(e_r)$; the ordering of edges within each bundle may be arbitrary. We say that a rotation system $\Sigma'$ for graph $G'$ is \emph{consistent} with rotation system $\Sigma$ for $G$ iff for every vertex $v\in V(G)$, the ordering $\oset'_v\in \Sigma'$ of the edges of $\delta_{G'}(v)$ is consistent with the ordering $\oset_v\in \Sigma$ of the edges of $\delta_G(v)$.

\begin{lemma}\label{lem: computing the ordering}
	There is an efficient algorithm, that, given an instance $I=(G,\Sigma)$ of \cnwrs, a collection $\cset$ of disjoint sub-graphs of $G$, and, for each cluster $C\in \cset$, a vertex $u(C)$ and a set $\qset(C)$ of paths routing the edges of $\delta_G(C)$ to $u(C)$, constructs a rotation system $\Sigma'$ for the graph $G'$ defined above with respect to $\bigcup_{C\in \cset}\qset(C)$, that is consistent with the rotation system $\Sigma$. Moreover, $\optcrors(G',\Sigma')\leq \optcrors(G,\Sigma)+\sum_{e\in E(G)}\eta(e)\cdot \cro(e)$
\end{lemma}

\mynote{the above lemma is problematic. will need to think about it some more. We are allowing $\cro(\qset,\qset)$ crossings. But that means we need to be able to deal with cognestion squared, which we currently can't do.}
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------

\fi
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------

%\subsection{A Useful Lemma}



%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------\\
%---------------------------
%---------------------------



%\input{basic_disengagement}




\subsection{Second Key Tool: Advanced Disengagement of Clusters}


\mynote{if possible, please remove $\temp$ from lemma statement and use instead number of crossings between different paths sets, or congestion squared}
\begin{theorem}\label{thm: advanced disengagement of clusters}
	There is an efficient algorithm, that, given as input an instance $(G,\Sigma)$ of the \CNwRS problem, a collection $\cset$ of disjoint sub-graphs of $G$, and, for every cluster $C\in \cset$, a vertex $u(C)$ and a set $\qset(C)$ of paths routing the edges of $\delta(C)$ to vertex $u(C)$ inside $C$, such that:
	\begin{itemize}
		\item  $\bigcup_{C\in \cset}V(C)=V(G)$;
		\item $|\inE(\cset)|\leq |E(G)|/(100\mu)$;
		\item for every cluster $C\in \cset$, $|E(C)|\leq |E(G)|/(100\mu)$; and
		\item for every cluster $C\in \cset$ and for each edge $e\in C$, $(\cong_C(\qset(C),e))^2\le \temp$,			
	\end{itemize}

	 computes a collection $\iset=\set{I_1,\ldots,I_k}$ of sub-instances of $(G,\Sigma)$, with the following properties:
	
	\begin{itemize}
		\item for all $1\leq i\leq k$, $|E(G_i)|\leq |E(G)|/\mu$;
		\item $\sum_{i=1}^k|E(G_i)|\leq O(|E(G)|)$; and
		\item $\sum_{1\le i\le k}\optcrors(G_i,\Sigma_i)\le O((\optcrors(G,\Sigma)+|E(G)|)\cdot \temp)$.
	\end{itemize}
 Moreover, there is an efficient algorithm, that, given, for each $1\le i\le k$, a feasible solution $\phi_i$ for instance $(G_i,\Sigma_i)$, computes a feasible solution $\phi$ for instance $(G,\Sigma)$ with $\cro(\phi)\leq O\left (\sum_{1\le i\le k}\cro(\phi_i)\right )$.
\end{theorem}



The remainder of this subsection is dedicated to the proof of \Cref{thm: advanced disengagement of clusters}. We assume that we are given an instance $I=(G,\Sigma)$ of the \CNwRS problem, and a collection $\cset$ of disjoint sub-graphs of $G$, like in the statement of the corollary. Let $\phi^*$ be an optimal solution to instance $I$ of \CNwRS. 
%For every subgraph $H\subseteq G$, we denote by $\cro(H)$ the number of crossings in $\phi^*$ in which the edges of $H$ participate. 






We associate with the graph $G$ and the collection $\cset$ of clusters a \emph{contracted graph} $H=G_{|\cset}$, that is defined as follows. Start with $H=G$, and then, for every cluster $C\in \cset$, contract $C$ into a super-node $u(C)$. We delete all self loops but keep parallel edges.

Next, we compute a Gomory-Hu tree $\tau$ for graph $H$, that we root at an arbitrary vertex. Recall that $V(\tau)=V(H)$, and, for every non-root vertex $v$ in the tree, if $v'$ is the parent of vertex $v$ in the tree, and $\tau_v$ is the sub-tree of $\tau$ rooted at $v$, then, denoting $S=V(\tau_v)$, from Corollary~\ref{cor: G-H tree_edge_cut}, the minimum cut in graph $H$ separating $v$ from $v'$ is precisely $(S,V(H)\setminus S)$. 
%\mynote{is that the correct definition of Gomory-Hu trees?}\znote{Not exactly, but this is a corollary of Gomory-Hu trees. Given a graph $G$, a Gomory-Hu tree for $G$ is a weighted tree $\tau$ that satisfies: (i) $V(\tau)=V(G)$; (ii) for each pair $u,u'$ of vertices of $G$, $\text{min-cut}_G(u,v)=\text{min-cut}_T(u,v)$.}

As it turns out, the most difficult case for the proof of \Cref{thm: advanced disengagement of clusters} is when the graph $\tau$ is a path. In the following subsection, we prove the following lemma for this special case.
The statement of the lemma is almost identical to the statement of \Cref{thm: advanced disengagement of clusters}, except that we now assume that the tree $\tau$ for the graph $H$ is a path.

\begin{lemma}\label{lem: path case}
	There is an efficient algorithm, that, given as input an instance $(G,\Sigma)$ of the \CNwRS problem, a collection $\cset$ of disjoint sub-graphs of $G$, and, for every cluster $C\in \cset$, a vertex $u(C)$ and a set $\qset(C)$ of paths routing the edges of $\delta(C)$ to vertex $u(C)$ inside $C$, such that:
		
		\begin{itemize}
		\item  $\bigcup_{C\in \cset}V(C)=V(G)$;
		\item $|\inE(\cset)|\leq |E(G)|/(100\mu)$;
		\item for every cluster $C\in \cset$, $|E(C)|\leq |E(G)|/(100\mu)$;
		\item for every cluster $C\in \cset$ and for each edge $e\in C$, $(\cong_C(\qset(C),e))^2\le \temp$; and
		\item the Gomory-Hu tree $\tau$ for the graph $H=G_{|\cset}$ is a path,
		\end{itemize}
		
		computes a collection $\iset=\set{I_1,\ldots,I_k}$ of sub-instances of $(G,\Sigma)$, with the following properties:
		
		\begin{itemize}
			\item for all $1\leq i\leq k$, $|E(G_i)|\leq |E(G)|/\mu$;
			\item $\sum_{i=1}^k|E(G_i)|\leq O(|E(G)|)$; and
			\item $\sum_{1\le i\le k}\optcrors(G_i,\Sigma_i)\le O((\optcrors(G,\Sigma)+|E(G)|)\cdot \temp)$. %\znote{slightly modified here}.
		\end{itemize}
Moreover, there is an efficient algorithm, that, given, for each $1\le i\le k$, a feasible solution $\phi_i$ for instance $(G_i,\Sigma_i)$, computes a feasible solution $\phi$ for instance $(G,\Sigma)$ with $\cro(\phi)\leq O\left (\sum_{1\le i\le k}\cro(\phi_i)\right )$.
	\end{lemma}
	
	
We defer the proof of \Cref{lem: path case} to the following subsections, and we complete the proof of \Cref{thm: advanced disengagement of clusters} using the lemma here.

\mynote{plan: compute the path decomposition into $\log n$ levels. Then do disengagemnets with the paths as clusters. }



\subsection{Disengagement on a Path -- Proof of \Cref{lem: path case}}
\label{subsec: disengagement on a path}

We denote the clusters in $\cset$ by $C_1,C_2,\ldots,C_r$. For convenience, for each $1\leq i\leq r$, we denote the vertex $v(C_i)$ of the graph $H=G_{|\cset}$ by $x_i$. Recall that we have assumed that the tree $\tau$ is a path. We assume without loss of generality that the clusters are indexed according to their appearance on the path $\tau$. For $1\leq i\leq r$, we let $S_i=\set{x_1,\ldots,x_i}$ and let $\notS_i=\set{x_{i+1},\ldots,x_r}$. Recall that, by the definition of the Gomory-Hu tree, $(S_i, \notS_i)$ is a minimum cut in graph $H$ separating vertex $x_i$ from vertex $x_{i+1}$. From the properties of minimum cut, there is a set of paths in graph $H$, routing the edges of $\delta_H(S_i)$ to vertex $x_{i}$ inside $S_i$, and there is a set of paths in graph $H$, routing the edges of $\delta_H(\notS_i)$ to vertex $x_{i+1}$ inside $\notS_i$.
%\znote{notations $\rset$ and $\rset'$ are not used?}

%For all $1\leq i<j\leq r$, we denote by $E_{i,j}$ the set of paths in graph $G$ connecting vertices of $C_i$ to vertices of $C_j$.
Recall that every edge in graph $H$ corresponds to some edge in $\inE(\cset)$, and we do not distinguish between these edges. In particular, for all $1\le i,j\le r$, we will also view edges of $E(C_i,C_j)$ as parallel edges connecting vertex $x_i$ to vertex $x_j$ in graph $H$.
For each $1\le i\le k$, we denote
$\hat E_i=E(C_i,C_{i+1})$,
$E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, and 
$E_i^{\through}=\bigcup_{i'<i,j'>i+1}E(C_{i'},C_{j'})$.
%Consider now the cut $(S_i,\notS_i)$, for some $1\leq i<r$. We partition the set $\delta_H(S_i)$ of edges into four subsets. We denote by $\hat E_i$ the set of all parallel edges connecting $x_i$ to $x_{i+1}$. We denote by $E_i^{\rig}$ the set of all edges $(x_i,x_j)$, where $j>i+1$. We denote by $E_i^{\lef}$ the set of all edges $(x_j,x_{i+1})$ where $j<i$, and we denote by $E_i^{\through}$ the set of all remaining edges of $\delta_H(S_i)$; note that, if $e=(x_j,x_{j'})\in E_i^{\through}$, with $j<j'$, then $j<i$ and $j'>i+1$ must hold. 
We need the following  observation.

\begin{observation}\label{obs: bad inded structure}
	For all $1\leq i<r$, the following hold:
	
	\begin{itemize}
		\item 	$|\hat E_i|\geq |E_i^{\through}|$;
		\item $|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$; and
		\item	$|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
	\end{itemize}
\end{observation}

\begin{proof}
Consider the cut $(\set{x_{i}},V(H)\setminus \set{x_i})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|$. Note that this cut separates $x_i$ from $x_{i-1}$. Since the minimum cut separating $x_i$ from $x_{i-1}$ in $H$ is $(S_{i-1},\notS_{i-1})$, and $|E(S_{i-1},\notS_{i-1})|=|\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|$, we get that:


\[ |\hat E_{i-1}|+ |E_{i+1}^{\lef}|+|E_{i}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+|\hat E_{i-1}|+ |E_i^{\rig}|+|E_{i}^{\lef}|, \]

and so  


\[  |E_{i+1}^{\lef}|+|E_i^{\through}|\leq  |\hat E_i|+ |E_i^{\rig}|. \]

Consider the cut $(\set{x_{i+1}},V(H)\setminus \set{x_{i+1}})$ in $H$. Its size is $|\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|$. Note that this cut separates $x_{i+1}$ from $x_{i+2}$. Since the minimum cut separating $x_{i+1}$ from $x_{i+2}$ in $H$ is $(S_{i+1},\notS_{i+1})$, and $|E(S_{i+1},\notS_{i+1})|=|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|$, we get that:

	
\[|\hat E_{i+1}|+ |E_i^{\rig}|+|E_{i+1}^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|\hat E_{i+1}|+ |E_{i+1}^{\lef}|+|E_{i+1}^{\rig}|,   \]	
	
	and so 
	
\[ |E_i^{\rig}|+|E_i^{\through}|\leq |\hat E_i|+|E_{i+1}^{\lef}|.   \]	

By adding the two inequalities and rearranging the sides, we get that $|\hat E_i|\geq |E_i^{\through}|$. By rearranging the sides of the two inequalities, we get that 	
$|\hat E_i|-|E_i^{\through}|\geq |E_{i+1}^{\lef}|-|E_i^{\rig}|$, and
	$|\hat E_i|-|E_i^{\through}|\geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$.
\end{proof}


\begin{definition}
We say that index $i$ is \emph{problematic} iff $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|>100|\hat E_i|$.
\end{definition}


\begin{observation}\label{obs: problematic instance}
	If index $i$ is problematic then $|E_{i+1}^{\lef}|-|\hat E_i| \leq |E_i^{\rig}|\leq |E_{i+1}^{\lef}|+|\hat E_i|$, and moreover $48|E_{i+1}^{\lef}|/49 \leq |E_i^{\rig}|\leq 49|E_{i+1}^{\lef}|/48$.
\end{observation}
\begin{proof}
	Assume that index $i$ is problematic. Since $|E_i^{\through}|\leq |\hat E_i|$, we get that either $|E_i^{\rig}|\geq 49|\hat E_i|$, or $|E_{i+1}^{\lef}|\geq 49|\hat E_i|$. Assume without loss of generality that  $|E_i^{\rig}|\geq |E_{i+1}^{\lef}|$, so $|E_i^{\rig}|\geq 49 |\hat E_i|$. Since, from \Cref{obs: bad inded structure}, 
	 $|\hat E_i| \geq |E_i^{\rig}|-|E_{i+1}^{\lef}|$, we get that $|E_{i+1}^{\lef}|\geq |E_i^{\rig}|-|\hat E_i|\geq 48|E_i^{\rig}|/49$.
\end{proof}


We start by considering the special case where no index $i$ is problematic, and prove \Cref{lem: path case} for it in the \Cref{subsec: no prob edges}. We then show a reduction from the general case to this special case in \Cref{subsec: path with problematic indices}.

\input{disengage_path.tex}


\subsection{Completing the Proof of \Cref{lem: path case}}
\label{subsec: path with problematic indices}

In this subsection we complete the proof of \Cref{lem: path case}. Recall that we are given a collection $\cset=\set{C_1,\ldots,C_r}$ of clusters with $\bigcup_{i=1}^rV(C_i)=V(G)$, such that the Gomory-Hu tree $\tau$ for the contracted graph $H=G_{|\cset}$ is a path, with vertices $x_1,\ldots,x_r$ appearing on the path in this order, where vertex $x_i$ represents cluster $C_i$. We have already show how to complete the proof of  \Cref{lem: path case} if no index $1\leq i\leq r$ is problematic, so we assume now that at least one such index is problematic.
%We call the path $\tau$ the \emph{main path}, denoted by $P^*$.

Let $i_1<i_2<\cdots<i_q$ be all problematic indices. Consider some problematic index $i_j$.
By definition, $|E_{i_j}^{\rig}|+|E_{i_j+1}^{\lef}|+|E_{i_j}^{\through}|>100|\hat E_{i_j}|$.
We define indices $\LMP(i_j)$ and $\RMP(i_j)$ as follows.
Recall that $E^{\rig}_{i_j}$ is the set of all edges $(x_{i_j},x_z)$ with $z>i_j+1$. We let $\RMP(i_j)$ be the smallest integer $z>i_j+1$, such that at least half the edges in $E^{\rig}_{i_j}$ have their endpoints in $\set{x_{i_j+2},\ldots,x_z}$. It is easy to see that at least half the edges in $E^{\rig}_{i_j}$ must have their endpoints in $\set{x_{z},\ldots,x_q}$. Similarly, we let $\LMP(i_j)$ be the largest integer $z<i_j$, such that at least half the edges in $E^{\lef}_{i_j+1}$ have their endpoints in $\set{x_{z},\ldots,x_{i_j-1}}$. It is easy to see that at least half the edges in $E^{\lef}_{i_j+1}$ must have their endpoints in $\set{x_{1},\ldots,x_z}$. We need the following crucial observation.
	
\begin{observation}\label{obs: large capacity up to midpoint}
For all $1\leq j\leq q$, for every index $i_j<z<\RMP(i_j)$, $|\hat E_z|\geq |E^{\rig}_{i_j}|/2$;  and similarly, for every index $\LMP(i_j)<z'\leq i_j$, $|\hat E_{z'}|\geq |E^{\lef}_{i_j+1}|/2$.
\end{observation}
\begin{proof}
Fix an index $1\leq j\leq q$, and another index index $i_j<z<\RMP(i_j)$. Recall that there is a subset $E'\subseteq E^{\rig}_{i_j}$ of at least $|E^{\rig}_{i_j}|/2$ edges that have an endpoint in $\set{x_{\RMP(i_j)},\ldots,x_r}$. It is easy to verify that $E'\subseteq E_{z}^{\through}$. From \Cref{obs: bad inded structure}, $|\hat E_z|\geq |E_{z}^{\through}|\geq |E^{\rig}_{i_j}|/2$. The proof for index $\LMP(i_j)<z'\leq i_j$ is symmetric.
\end{proof}

\begin{claim}\label{claim: inner and outer paths}
Let $a$ be some problematic index and let $z\in \set{1,\ldots,r}$ be another index such that $a<z<\RMP(a)$.
If we denote by $Y$ the cluster of $H$ induced by vertices $x_{a+1},\ldots,x_z$, then (i) there is a set $\hat\qset(Y)$ of paths routing the edges of $\delta_H(Y)$ to vertex $x_z$ in $Y$ with congestion $O(1)$; and (ii) there is a set $\hat\pset(Y)$ of paths routing the edges of $\delta_H(Y)$ to vertex $x_{z+1}$ outside $Y$ with congestion $O(1)$.

Similarly, 
let $a'$ be some problematic index and let $z'\in \set{1,\ldots,r}$ be another index such that $\LMP(a')<z'<a$.
If we denote by $Y'$ the cluster of $H$ induced by vertices $x_{z'},\ldots,x_{a'-1}$, then (i) there is a set $\hat\qset(Y')$ of paths routing the edges of $\delta_H(Y')$ to vertex $x_{z'}$ in $Y'$ with congestion $O(1)$; and (ii) there is a set $\hat\pset(Y')$ of paths routing the edges of $\delta_H(Y')$ to vertex $x_{z'-1}$ outside $Y$ with congestion $O(1)$.
\end{claim}

\begin{proof}
We only prove the claim for cluster $Y$, and the proof for cluster $Y'$ is symmetric.

We first prove (i). We partition the set $\delta_H(Y)$ into two subsets: set $E_1$ contains all edges of $\delta_H(Y)$ with an endpoint in $S_a$ (recall that $S_a=\set{x_1,\ldots,x_a}$); and set $E_2$ contains all edges of $\delta_H(Y)$ with an endpoint in $\notS_z$ (recall that $\notS_z=\set{x_{z+1},\ldots,x_q}$). 
	Recall that, from the properties of minimum cut, there is a set $\rset$ of edge-disjoint paths routing the edges of $E_2$ to vertex $x_z$ inside $S_z$. 
	Let $\rset^{in}\subseteq \rset$ be the subset of all paths of $\rset$ that are entirely contained in $Y$, and we denote $\rset^{out}=\rset\setminus \rset^{in}$.
	For each path $R\in \rset^{out}$, we view $x_z$ as its last vertex and the edge of $E_2$ as its first edge, and we denote by $e_R$ the first edge of $E_1$ that appears on $R$. It is clear that edges in $\set{e_{R}\mid R\in \rset^{out}}$ are mutually distinct.
	On the other hand, since $E_1\subseteq \hat E_a\cup E_{a+1}^{\lef}\cup E_a^{\through}$ and $a$ is a problematic index, combined with \Cref{obs: bad inded structure}, we get that $|E_1|\leq |\hat E_a|+| E_{a+1}^{\lef}|+|E_a^{\through}|\leq 2|E_a^{\rig}|$. Moreover, from \Cref{obs: large capacity up to midpoint}, for all $a<z'\leq z$, $|\hat E_{z'}|\geq |E_a^{\rig}|/2\ge |E_1|/4$. 
	Therefore, 
	there is a set $\hat\qset_1=\set{\hat Q_e\mid e\in E_1}$ of paths, routing edges of $E_1$ to $x_z$ in $Y$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{Y}(\hat\qset_1)\le 4$; and similarly,
	there is a set $\hat{\rset}^{out}=\set{\hat R\mid R\in \rset^{out}}$ of paths, routing edges of $\set{e_R\mid R\in \rset^{out}}$ to $x_z$ in $Y$, using only edges of $\bigcup_{a< z'< z}\hat E_{z'}$, such that $\cong_{Y}(\hat{\rset}^{out})\le 4$.
	We now define $\hat\qset^{out}$ to be the set that contains, for each path $R\in \rset^{out}$, the concatenation of (i) the subpath of $R$ between its first edge (in $E_2$) and edge $e_R$ (not included); and (ii) the path $\hat R\setminus \set{e_R}$.
	We now let $\hat\qset_2=\rset^{in}\cup\hat\qset^{out}$ and $\hat\qset(Y)=\hat\qset_1\cup \hat\qset_2$.
	It is clear that the set $\hat\qset(Y)$ contains, for each edge of $\delta_H(Y)$, a path routing the edge to $x_z$ in $Y$, and
	$$\cong_{Y}(\hat\qset(Y))\le \cong_{Y}(\hat\qset_1)+\cong_{Y}(\hat\qset_2)\le 4+\cong_{Y}(\rset^{in})+\cong_{Y}(\hat\qset^{out})=4+1+(1+4)=10.$$
	%It is now easy to see that there is a set $\qset'(R')$ of paths in $R'$, routing the edges of $\delta(R')$ to vertex $x_z$, with congestion at most $4$.
	%A similar reasoning shows that there is a set $\qset'(R'')$ of paths in $R''$, routing the edges of $\delta(R')$ to vertex $x_{z+1}$, with congestion at most $4$.

\begin{figure}[h]
	\centering
	\subfigure[Cluster $Y$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_1.jpg}}\label{fig: path_cluster_H}
	}
	\hspace{4pt}
	\subfigure[Cluster $Y'$ and its relevant vertices and edge sets.]{\scalebox{0.3}{\includegraphics{figs/prob_index_2.jpg}}\label{fig: path_cluster_G}}
	\caption{An illustration of clusters $Y,Y'$ in $H$.}%\label{fig: path_cluster}
\end{figure}

We now prove (ii).
	From the properties of minimum cuts, there is a set $\rset_1$ of edge-disjoint paths routing edges of $E_1$ to $x_{a}$ in $S_{a}$ (and therefore outside $Y$).
	Similarly, there is a set $\rset_2$ of edge-disjoint paths routing the edges of $E_2$ to $x_{z+1}$ inside $\notS_{z}$ (and therefore outside $Y$). As observed before, $|E_1|\leq 2|E_a^{\rig}|$. Moreover, there is a set $E'\subseteq E_a^{\rig}$ of at least $|E_a^{\rig}|/2$ edges, each of which connects $x_a$ to a vertex in $\set{x_{z+1},\ldots,x_r}$. 
	For each edge $e\in E_1$, we assign to it an edge $e'$ of $E'$, such that each edge of $E'$ is assigned to at most $4$ edges of $E'_1$. 
	Observe that $E'\subseteq \delta_H(\notS_{z})$, so there is a set $\rset_3$ of $|E'|\geq |E_a^{\rig}|/2$ edge-disjoint paths routing the edges of $E'$ to $x_{z+1}$, that are disjoint from $Y$. 
	We now define $\hat{\pset}_1$ to be the set that contains, for each edge $e\in E_1$, the union of (i) the path in $\rset_1$ routing $e$ to $x_a$ in $S_a$; and (ii) the path in $\rset_3$ that routing $e'$ to $x_{z+1}$ in $\notS_z$.
	We let $\hat{\pset}(Y)=\rset_2\cup \hat{\pset}_1$.
	It is clear that the set $\hat\pset(Y)$ contains, for each edge of $\delta_H(Y)$, a path routing the edge to vertex $x_{z+1}$ outside $Y$, and
	$$\cong_{H}(\hat\qset(Y))\le
	\cong_{H}(\rset_2)+\cong_{H}(\hat\pset_1)\le 1+\cong_{H}(\rset_1)+4\cdot\cong_{H}(\rset_3)=1+(1+4)=6.$$
\end{proof}

\znote{to modify}
The plan for the remainder of the proof is the following. First, we will define a family $\xset$ of clusters of $G$,
%, where each cluster $X\in \xset$ naturally corresponds to a sub-path of $\tau$.  
and for each cluster $X\in \xset$, we will define a vertex $u(X)\in X$, with a set $\qset(X)$ of paths routing the edges of $\delta_G(X)$ to $u(X)$ inside $X$, and another vertex $u'(X)\not \in X$, with another set $\pset(X)$ of paths routing the edges of $\delta_G(X)$ to $u'(X)$ outside $X$.  Then we will disengage the clusters in $\xset$ using the basic disengagement (described in \Cref{subsec: basic disengagement}) and obtain, for every cluster $X\in \xset$, a sub-instance $I_X=(G_X,\Sigma_X)$. We will then show that this sub-instance can be further reduced to an instance $(G'_X,\Sigma'_X)$, such that,
if we denote by $\cset_X\subseteq \cset$ the set of clusters in $\cset$ that are contained in graph $X$, and denote by $H_X=(G'_X)_{|\cset_X}$ the corresponding contracted graph, and denote by $\tau_X$ the Gomory-Hu tree of $H_X$, then $\tau_X$ is a subpath of $\tau$ that contains no bad indices. 

Therefore, we can solve each resulting sub-instance using the algorithm from \Cref{subsec: no prob edges}. This leaves us with one final instance, that is obtained from the graph $G$, by contracting every cluster of $\bigcup_{X\in \xset}\cset_X$ into a single vertex. In our last step, we will define the clusters in this final instance in such a way that the Gomory-Hu tree of the corresponding contracted graph is a path with no problematic indices, and we will again use the algorithm from \Cref{subsec: no prob edges} to solve it.
\znote{path, directly with ``problematic indices''?}


\subsubsection{First-Level Disengagement}
\label{subsec: 1st disengagement}
In this step we define a collection $\xset$ of clusters, and for every cluster  $X\in \xset$, a vertex $u(X)\in X$ with a set $\qset(X)$ of paths routing the edges of $\delta_G(X)$ to $u(X)$ inside $X$, and another vertex $u'(X)\not \in X$ with another set $\pset(X)$ of paths routing the edges of $\delta_G(X)$ to $u'(X)$ outside $X$. Then we perform basic disengagement from \Cref{subsec: basic disengagement} to $G$, using the set $\xset$ of clusters and their corresponding path sets.
%In order to do so, we will initially define a collection $\xset'$ of clusters in $H$, which will then naturally define a collection  $\xset$ of clusters in $G$.

\subsubsection*{Step 1: Defining the Clusters}

We construct the collection $\xset$ iteratively. We start with $\xset=\emptyset$, and then process every consecutive pair of problematic indices, as follows.
Consider the index pair $i_j,i_{j+1}$ for some $1\le j\le q-1$.
For brevity, we denote $i_j=a$ and $i_{j+1}=b$.
We now distinguish between the following two cases.

\paragraph{Case 1. $\LMP(b)<\RMP(a)$.} 
%Assume first that Case 1 happens. 
By definition, $a<b$, $a<\RMP(a)$, and $\LMP(b)<b$. 
Now since $\LMP(b)<\RMP(a)$, we get that $\max\set{a,\LMP(b)}<\min\set{b,\RMP(a)}$.
Let $z$ be any index such that $\max\set{a,\LMP(b)}\le z<\min\set{b,\RMP(a)}$.
Denote by $Y_j$ the subgraph of $H$ induced by vertices $x_{a+1},\ldots,x_z$, and denote by $Y'_j$ the subgraph of $H$ induced by vertices $x_{z+1},\dots, x_{b}$. See \Cref{fig: path_cluster_H} for an illustration. From \Cref{claim: inner and outer paths}, there is a set $\hat\qset(Y_j)$ of paths routing the edges of $\delta_H(Y_j)$ to vertex $x_z$ in $Y_j$ with congestion $O(1)$; and there is a set $\hat\pset(Y_j)$ of paths routing the edges of $\delta_H(Y_j)$ to vertex $x_{z+1}$ outside $Y_j$ with congestion at most $6$.
Similarly, there is a set $\hat\qset(Y'_j)$ of paths  routing the edges of $\delta_H(Y'_j)$ to vertex $x_{z+1}$ in $Y'_j$ with congestion $O(1)$; and there is a set $\hat\pset(Y'_j)$ of paths routing the edges of $\delta_H(Y'_j)$ to vertex $x_{z}$ outside $Y'_j$ with congestion $O(1)$.

\begin{figure}[h]
	\centering
	\subfigure[Subgraphs $Y_j,Y'_j$ in $H$.]{\scalebox{0.34}{\includegraphics{figs/path_cluster_1.jpg}}\label{fig: path_cluster_H}
	}
	\hspace{4pt}
	\subfigure[Subgraphs $X_j,X'_j$ in $G$.]{\scalebox{0.34}{\includegraphics{figs/path_cluster_2.jpg}}\label{fig: path_cluster_G}}
	\caption{An illustration of subgraphs $Y_j,Y'_j$ in $H$ and subgraphs $X_j,X'_j$ in $G$.}%\label{fig: path_cluster}
\end{figure}

%Observe that cluster $Y_j$ and cluster $Y'_j$ both correspond to subpaths of $\tau$. 
We let $X_j$ be the subgraph of $G$ induced by $\bigcup_{x_k\in Y_j}C_j$, and let $X_j'$ be the subgraph of $G$ induced by $\bigcup_{x_k\in Y'_j}C_k$. We add clusters  $X_j,X_j'$ to the set $\xset$ of subgraphs of $G$. See \Cref{fig: path_cluster_G} for an illustration.



We define vertices $u(X_j),u'(X_j)$ and path sets $\qset(X_j),\pset(X_j)$ as follows.
We set $u(X_j)=u(C_z)$. 
For each edge $e\in \delta_G(X_j)$, we define a path $Q_{X_j}(e)$ as follows.
Let $(e_0,x_{\ell_0},e_1,x_{\ell_2},\ldots,x_{\ell_{t-1}},e_t,x_t)$ be the path in $\hat\qset(Y_j)$ that routes $e$ to $x_z$, where $e_0=e$ and $x_t=x_z$.
Recall that $e_0,e_1,\ldots,e_t$ are also edges in $G$.
We define path $Q_{X_j}(e)$ to be the sequential concatenation of: the edge $e_0$ in $G$; the path in $\qset(C_{\ell_0})$ routing $e_0$ to $u(C_{\ell_0})$; the path in $\qset(C_{\ell_0})$ routing $e_1$ to $u(C_{\ell_0})$; the edge $e_1$ in $G$; the path in $\qset(C_{\ell_1})$ routing $e_1$ to $u(C_{\ell_1})$, \ldots, the edge $e_t$ in $G$. Clearly, path $Q_{X_j}(e)$ routes $e$ to $u(X_j)$.
We then let set $\qset(X_j)$ contains, for each edge $e\in  \delta_G(X_j)$, the path $Q_{X_j}(e)$.
We set $u'(X_j)=u(C_{z+1})$, and we define the set $\pset(X_j)$ of paths using the path set $\hat\pset(Y_1)$ and the path sets $\set{\qset(C_k)\mid k\le a\text{ or }k> z}$ similarly.
We then set $u(X'_j)=u(C_{z+1})$ and $u'(X'_j)=u(C_{z})$, and define path sets $\qset(X'_j), \pset(X'_j)$ similarly.


\iffalse
We set $u(X_j)=u(C_z)$. Using the path sets $\qset(C_k)$ for all vertices $x_k\in Y_j$, combined with the set $\hat\qset(Y_j)$ of paths that we have constructed, we obtain a set $\qset(X_j)$ of paths routing the edges of $\delta_H(X_j)$ to the vertex $u(C_z)$ inside $X_j$. Similarly, we set $u(X_j')=u(C_{z+1})$, and use the path sets $\qset(C_k)$ for all vertices $x_k\in Y'_j$, together with the path set $\hat\qset(Y_j')$ that we have constructed, to obtain a set $\qset(X'_j)$ of paths routing the edges of $\delta_H(X'_j)$ to $u(X'_j)$.
Similarly, we set $u'(X_j)=u(C_{z+1})$. Using the path sets $\qset(C_k)$ for all vertices $x_k\in Y_j$, combined with the set $\hat\qset(Y_j)$ of paths that we have constructed, we obtain a set $\qset(X_j)$ of paths routing the edges of $\delta_H(X_j)$ to the vertex $u(C_z)$ inside $X_j$. Similarly, we set $u(X_j')=u(C_{z+1})$, and use the path sets $\qset(C_k)$ for all vertices $x_k\in Y'_j$, together with the path set $\hat\qset(Y_j')$ that we have constructed, to obtain a set $\qset(X'_j)$ of paths routing the edges of $\delta_H(X'_j)$ to $u(X'_j)$.

We also set $u'(\hat R')=u(C_{z+1})$, and $u'(\hat R'')=u(C_z)$, and define the set $\pset(\hat R')$ of paths connecting the edges of $\delta_H(\hat R')$ to $u'(\hat R')$ outside $\hat R'$, and the set $\pset(\hat R'')$ of paths connecting the edges of $\delta_H(\hat R'')$ to $u'(\hat R'')$ outside $\hat R''$, using the paths sets $\pset'(R')$, $\pset'(R'')$, $\bigcup_{x_k\in R'}\qset(C_k)$ and $\bigcup_{x_k\in R''}\qset(C_k)$ similarly.
%Note that the paths in each of the sets $\pset(\hat R')$, $\pset(\hat R'')$, $\qset(\hat R')$ and $\qset(\hat R'')$ cause congestion $O(1)$.
\fi

\paragraph{Case 2. $\RMP(a)\leq \LMP(b)$.} 
Denote $z=\RMP(a)$ and $z'=\LMP(b)$. 
Note that indices $z,z'$ may not be problematic.
We let $Y_j$ be the subgraph of $H$ induced by vertices $x_{a+1},\ldots,x_z$, and we let $Y_j'$ be the subgraph of $H$ induced by vertices $x_{z'+1},\ldots,x_b$. From \Cref{claim: inner and outer paths}, we can find a set $\hat\qset(Y_j)$ of paths routing edges of $\delta_{H}(Y_j)$ to $x_z$ inside $Y_j$, and a set $\hat\pset(Y_j)$ of paths routing edges of $\delta_{H}(Y_j)$ to $x_{z+1}$ outside $Y_j$. Similarly, we can find a set $\hat\qset(Y_j')$ of paths routing edges of $\delta_{H}(Y_j')$ to $x_{z'+1}$ inside $Y_j'$, and a set $\hat\pset(Y_j')$ of paths routing edges of $\delta_{H'}(Y_j')$ to $x_{z'}$ outside $Y_j'$. We define clusters $X_j,X_j'$ exactly as before, and then add them to set $\xset$ of clusters. The path sets $\qset(X_j)$, $\pset(X_j)$, $\qset(X_j')$, $\pset(X_j')$ are defined similarly.

%\paragraph{The pairs $(i_1,i_2)$ and $(i_{q-1},i_q)$.}

Finally, we additionally process the first index and the last index as follows.
For the first index $i_1$, we let $z'=\LMP(i_1)$, and define the cluster $Y'_0$ as subgraph of $H$ induced by $x_{z'+1},\ldots,x_{i_1}$. We define the corresponding cluster $X'_0$, vertices $u(X'_0),u'(X'_0)$ and path sets $\qset(X'_0),\pset(X'_0)$ similarly, and add it to the set $\xset$. 
For the last index $i_q$, we let $z'=\RMP(i_q)$, and define the cluster $Y_q$ as subgraph of $H$ induced by $x_{i_q+1},\ldots,x_{z'}$. We define the corresponding $X_q$, vertices $u(X_q),u'(X_q)$ and path sets $\qset(X_q),\pset(X_q)$ similarly, and add it to the set $\xset$. 
This completes the construction of the set $\xset$ of clusters and their affiliated vertices and path sets.
Clearly, the clusters of $\xset$ are vertex-disjoint subgraphs of $G$. See \Cref{fig: xset_cluster} for an illustration.
\begin{figure}[h]
\centering
\includegraphics[scale=0.55]{figs/xset_clusters.jpg}
\caption{An illustration of all clusters of $\xset$: clusters $C_i$ with a problematic index $i$ are shown in brown, and clusters $C_i$ that is not contained in any cluster of $\xset$ are shown in blue. }\label{fig: xset_cluster}
\end{figure}

We use the following observation, which, from the construction of clusters in $\xset$ and the definition of  corresponding path sets, is an easy corollary of \Cref{claim: inner and outer paths}.

\begin{observation}
\label{obs: congestion of basic disengagement paths}
Let $X$ be a cluster of $\xset$, then for each edge $e$ that belongs to some cluster $C\in \cset$, $\cong_G(\qset(X),e)\le O(\cong_G(\qset(C),e))$; and for each edge $e$ that does not belongs to any cluster of $\cset$, $\cong_G(\qset(X),e)\le O(1)$.
\end{observation}

\subsubsection*{Step 2: Computing the Basic Disengagement}

Now for each cluster $X\in \xset$, we apply the algorithm from \Cref{lem: non_interfering_paths} to the set $\qset(X)$ of paths, and obtain a set $\tilde\qset(X)$ of paths routing edges of $\delta_G(X)$ to $u(X)$ inside $X$, that are non-transversal with respect to $\Sigma$, such that for each $e\in E(G)$, $\cong_G(\tilde\qset(X),e)\le \cong_G(\qset(X),e)$.
Similarly, let $\tilde{\pset}(X)$ be the set of paths that we obtained from applying the algorithm from \Cref{lem: non_interfering_paths} to the set $\pset(X)$ of paths.
Denote $\tilde{\qset}=\bigcup_{X\in \xset}\tilde\qset(X)$ and $\tilde{\pset}=\bigcup_{X\in \xset}\tilde\pset(X)$.
We compute the colletion $\iset(\xset,\tilde{\qset},\tilde{\pset})$ of sub-instances of instance $(G,\Sigma)$, using the basic disengagement in \Cref{subsec: basic disengagement}.
From \Cref{lem: low solution costs},
$$\sum_{I'\in \iset(\xset,\tilde\qset,\tilde\pset)}\optcrors(I')\leq O\bigg(\optcrors(G,\Sigma)\cdot\temp+\sum_{X\in \xset}\sum_{\tilde P\in \tilde\pset(X)}\chi(\tilde P,X)\bigg).$$

From the properties of path set $\tilde{\pset}$, $\sum_{X\in \xset}\chi(\tilde \pset,X)\le \sum_{X\in \xset}\chi(\pset,X)$.
Then from \Cref{obs: congestion of basic disengagement paths}, for each cluster $X\in \xset$, 
$\chi(\pset,X)\le O(\chi^1(X)\cdot\temp)$. Moreover, since the clusters in $\xset$ are mutually disjoint, $\sum_{X\in \xset}O(\chi^1(X)\cdot\temp)\le O(\optcrors(G,\Sigma)\cdot\temp)$. Altogether, we get that
$$\sum_{I'\in \iset(\xset,\tilde\qset,\tilde\pset)}\optcrors(I')\leq O\bigg(\optcrors(G,\Sigma)\cdot\temp\bigg).$$


\subsubsection*{Step 3: Proving that Instances of $\set{I_X}_{X\in \xset}$ are Suitable for the Algorithm in \Cref{subsec: no prob edges}}

Recall that $\iset(\xset,\tilde{\qset},\tilde{\pset})=\set{\hat I_{\xset,\tilde\qset}}\cup\set{I_X}_{X\in \xset}$, where for each cluster $X\in \xset$, instance $I_X=(G_X,\Sigma_X)$ and graph $G_X$ is obtained from $G$ by contracting $G\setminus X$ into a single vertex $v^*$.
We will now show that, for each $X\in \xset$, we can efficiently construct a set $\cset_X$ of clusters in $G_X$, such that the contracted graph $H_X=(G_X)_{|\cset_X}$ has the $\alpha$-cut property with respect to some path $\tau_X$ on vertices of $V(H_X)$.
On the other hand, the instance $\hat I_{\xset,\tilde\qset}$ does not necessarily satisfy the above property, so we will need to perform another level of disengagement to it in \Cref{subsec: 2nd disengagement}.

%Consider now a cluster $X\in \xset$ and the graph $G_X$.

\iffalse
\znote{start here}
First, we consider a cluster $X_j$ that are constructed when processing some consecutive pair $(i_j,i_{j+1})$ of problematic indices in Case 1 and consider the instance $I_X\in \iset(\xset,\tilde\qset,\tilde\pset)$. The arguments for the cluster $X_j$ is symmetric.
The instance $I_X$
We will construct new graphs $G_{R'}, G_{R''}$ corresponding to the clusters $\hat R',\hat R''$. We will show that after a slight modification, the Gomory-Hu tree of the former graph becomes $\tau_{R'}$, the subpath of $\tau$ consisting of vertices of $R'$, and the Gomory-Hu tree of the latter graph becomes becomes $\tau_{R''}$, the subpath of $\tau$ consisting of vertices of $R''$. As we will show later, paths $\tau_{R'}$ and $\tau_{R''}$ do not contain problematic indices. 
\znote{How exactly?}
\fi

\iffalse
We now fix some $1\le j\le q-1$ and consider the clusters $X_j,X'_j$.
Recall that $X_j, X'_j$ are constructed when processing the consecutive pair $(i_j,i_{j+1})$ of problematic indices, based on the clusters $Y_j,Y_j'$ in $H$. 
%We will compute a set $\cset_X$ of disjoint clusters, whose vertex sets partition $V(G_X)$
We assume  that clusters $X_j, X'_j$ are produced in Case 1 of Step 1. 
The arguments for the case where $X_j, X'_j$ are produced in Case 2 of Step 1, and the clusters $X'_0,X_q$ which are obtained by additionally handling the first and the last indices can be handled similarly, are the same.
\fi

We use the following claim.
\begin{claim}
\label{claim: alpha cut property}
Let $a$ be some problematic index and $z$ be another index such that $a<z<\RMP(a)$.
Let $X$ be the subgraph of $G$ induced by clusters $C_{a+1},\ldots,C_z$, and define $G'$ as the graph obtained from $G$ by contracting $G\setminus X$ into a single vertex $v^*$. 
Define $\cset_X=\set{C_{a+1},\ldots,C_z,v^*}$ and let $H'=G'_{|\cset_X}$ be the contracted graph, where $V(H')=\set{x_{a+1},\ldots,x_z,v^*}$.
Define path $\tau'=(x_{a+1},\ldots,x_z,v^*)$. Then the graph $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for some $\alpha=O(1)$.
\end{claim}





\iffalse
We consider the cluster $X_j$, and the arguments for cluster $X'_j$ is symmetric.
For convenience, we rename $X_j$ by $X$, and rename the corresponding cluster $Y_j$ in $H$ by $Y$. 
\iffalse
We will construct a new instance $I'_{X}$, such that
\begin{enumerate}
	\item\label{pro: opt bound} $\optcrors(I'_{X})\le \chi(\tilde\pset(X),X)+O(\chi^2(X)\cdot\temp)$; and
	\item\label{pro: drawing transfer} there is an algorithm, that given a solution $\hat\phi'_X$, efficiently computes a solution $\hat\phi_X$ for instance $I_{X_j}$, such that $\cro(\hat\phi_X)\le 9\cdot \cro(\hat\phi'_X)$.
\end{enumerate}
\fi 
Recall that $X=\bigcup_{i_j< i\le z}C_i$, where $z<\RMP(i_j)$, and $V(Y)=\set{x_i\mid i_j< i\le z}$.
Also recall that $I_X=(G_X,\Sigma_X)$, where graph $G_X$ is obtained from $G$ by contracting all vertices of $G\setminus X$ into a single vertex, that we denote by $v^*$.
\iffalse
For a vertex $v\in X$, the ordering on $v$ in $\Sigma_X$ is identical to the ordering $\oset_v\in \Sigma$, and the ordering on vertex $v^*$ is $\hat{\oset}(\tilde\pset)$, the ordering in which paths of $\tilde{\pset}$ enters vertex $u(C_{z+1})$.
The new instance $I'_X=(G'_X,\Sigma'_X)$ is defined as follows.
Graph $G'_X$ is obtained from graph $G$ by first contracting all vertices of $\bigcup_{1\le t\le i_j}C_t$ into a single vertex $v^*_{\lef}$, and then contracting all vertices of $\bigcup_{z<t\ge r}C_t$ into a single vertex $v^*_{\rig}$.
Note that, if we further contract vertices $v^*_{\lef}$ and $v^*_{\rig}$ into a single vertex, then we obtain the graph $G_X$. The rotation system $\Sigma'_X$ is defined similarly. 
For a vertex $v\in X$, the ordering on $v$ in $\Sigma'_X$ is identical to the ordering $\oset_v\in \Sigma$.
The ordering on vertex $v^*_{\lef}$ is $\hat{\oset}(\tilde\pset)$, the ordering in which paths of $\tilde{\pset}$ enters vertex $u(C_{a})$, and the ordering on vertex $v^*_{\rig}$ is $\hat{\oset}(\tilde\pset)$, the ordering in which paths of $\tilde{\pset}$ enters vertex $u(C_{z+1})$. \znote{not rigorous here, to modify the previous definition}

We first prove \ref{pro: opt bound}. Recall in the proof of \Cref{lem: low solution costs}, we obtained from the optimal solution $\phi^*$ of instance $(G,\Sigma)$, a drawing $\phi_X$ of the instance $(G_X,\Sigma_X)$, such that $\cro(\phi_X)\le \chi(\tilde\pset(X),X)+O(\chi^2(X)\cdot\temp)$.
We now show that this drawing can be easily converted into a feasible solution $\phi'_X$ for instance $I'_X$, with at most same number of crossings. And then Property \ref{pro: opt bound} follows.
Denote $E_{\lef}= E_G(X,\bigcup_{1\le t\le i_j}C_t)$ and
$E_{\rig}= E_G(X,\bigcup_{z+1\le t\le r}C_t)$. 
Recall that drawing $\phi_X$ is obtained from the image $\phi(X\cup E(\tilde \pset(X)))$, by making copies of the image $\phi(E(\tilde \pset(X))$ to be concatenated into image $\set{\gamma_P\mid P\in \tilde\pset(X)}$ of paths in $\tilde\pset(X)$, and then nudging (applying \Cref{obs: curve_manipulation}) them at all common vertices.
Note that, for each edge $e\in E_G(X,\bigcup_{1\le t\le i_j}C_t)$ the path $\tilde P_e\in \tilde{\pset}$ contains $u(C_a)$ as its inner vertex. 
If we simply ``un-nudge'' the images of paths in $\pset$ at vertex $u(C_a)$, and then (i) view the image of vertex $u(C_a)$ as the image of $v^*_{\lef}$; (ii) view the image of vertex $u(C_{z+1})$ as the image of $v^*_{\rig}$ (we denote this point by $z$); (iii) for each edge $e\in E_{\lef}$, view the subcurve of $\gamma_{\tilde P_e}$ between its endpoint in $X$ and $z$ as the image of $e$; (iv) for each edge $e\in E_{\rig}$, view the curve $\gamma_{\tilde P_e}$ as the image of $e$; and (v) for each edge $e\in E(v^*_{\lef},v^*_{\rig})$, view the curve $\gamma_{\tilde P_e}$ between $z$ and $u(C_{z+1})$ as the image of $e$.

We now prove \ref{pro: drawing transfer}. 
We convert a feasible solution $\hat\phi_{X'}$ of the instance $(G_X,\Sigma_X)$ into a solution $\hat\phi_{X}$ of $(G'_{X},\Sigma'_{X})$ as follows.
We copy the image of each edge of $E(v^*_{\lef},v^*_{\rig})$ at most $3$ times, concatenate them with the image of $E_{\lef}$, nudging them at $v^*_{\lef}$ (which creates no additional crossings) and then view the resulting curves as the image of edges of $\delta_{G_X}(v^*)$. It is clear that each crossing in $\hat\phi_{X'}$ gives birth to at most $3^2=9$ crossings in $\hat\phi_{X}$. And \ref{pro: drawing transfer} then follows.
\fi

Let $\cset_X=\set{C_i\mid i_j<i\le z}\cup \set{v^*}$ be a set of vertex-disjoint clusters of $G_X$ whose vertex sets partition $V(G_X)$.
Let $H_X=(G_X)_{|\cset_X}$ be the contracted graph, so $V(H_X)=V(Y)\cup \set{v^*}$.
In fact, we can view $H_X$ as obtained from $H$ by contracting $H\setminus Y$ into a single vertex $v^*$.
We define the path $\tau_X=(x_{i_j+1},\ldots,x_z,v^*)$, and prove the following claim.
\begin{claim}
	Graph $H_X$ satisfies the $10$-cut property with respect to path $\tau_X$.
\end{claim}
\fi

Recall that $\xset=\set{X'_0,X_q}\cup\set{X_j,X'_j\mid 1\le j\le q-1}$.
From the construction of clusters of $\xset$ in the first step,
It is clear that \Cref{claim: alpha cut property} implies that the corresponding instances $\set{I_X}_{X\in \xset}$ are suitable for the algorithm in \Cref{subsec: no prob edges}. Therefore, it suffices to prove \Cref{claim: alpha cut property}.

\begin{figure}[h]
	\centering
	\subfigure[Subgraphs $Y_j,Y'_j$ in $H$.]{\scalebox{0.11}{\includegraphics{figs/cut_property_1.jpg}}}
	\hspace{4pt}
	\subfigure[Subgraphs $X_j,X'_j$ in $G$.]{\scalebox{0.11}{\includegraphics{figs/cut_property_2.jpg}}}
	\caption{An illustration of subgraphs $Y_j,Y'_j$ in $H$ and subgraphs $X_j,X'_j$ in $G$. \znote{figure broken}}\label{fig: cut_property}
\end{figure}

\begin{proofof}{\Cref{claim: alpha cut property}}
%For convenience we deonte $a=i_j$.
First fix some $z'$ with $a<z'< z$, so $z'$ is not a problematic index. Denote $S'_{z'}=\set{x_{a+1},\ldots,x_{z'}}$ and $\notS_{z'}'=\set{x_{z'+1},\ldots,x_z}$, and denote by $E'$ the set of edges in the cut $(S'_{z'},\notS_{z'}'\cup\set{v^*})$ of $H$.
Note that graph $H'$ can be viewed as obtained from $H$ (recall that $H=G_{|\cset}$) by contracting vertices of $\set{x_t\mid 1\le t\le a\text{ or }z< t\le r}$ into a vertex $v^*$, so each edge of $E'$ is also an edge of $H$, and vertices of $S'_{z'},\notS'_{z'}$ are also vertices of $V(H)$.
Clearly, set $E'$, as a set of edges in $H$, can be further partitioned into subsets as follows:
set $E'_1=E_H(S'_{z'},\notS'_{z'})$; 
set $E'_2=E_H(S'_{z'},S_a)$; and
set $E'_3=E_H(S'_{z'},\notS_z)$.
See \Cref{fig: cut_property} for an illustration.

Note that $|E'_1|+|E'_3|\le |E^{\rig}_{z'}|+|E^{\lef}_{z'+1}|+|E^{\through}_{z'}|$. Since $z'$ is not a problematic index, $|E'_1|+|E'_3|\le 100\cdot |E(x_{z'},x_{z'+1})|$.
On the other hand, from \Cref{obs: bad inded structure}, $|E'_2|\le |E^{\rig}_{a}|+|E^{\lef}_{a+1}|+|E^{\through}_{a}|\le 2\cdot|E^{\rig}_{a}|$, and from \Cref{obs: large capacity up to midpoint}, $|E(x_{z'},x_{z'+1})|\ge |E^{\rig}_{a}|/2$.
Therefore, $|E'_2|\le 4\cdot |E(x_{z'},x_{z'+1})|$. Altogether, 
$|E'|=|E_1'|+|E_2'|+|E_3'|\le 104\cdot |E(x_{z'},x_{z'+1})|$.

Consider now the cut $(S_z,\set{v^*})$ in $H$. 
We define sets $E',E'_1,E'_2,E'_3$ similarly. Clearly, $E'_1=\emptyset$. Observe that $E_H(x_z,x_{z+1})\subseteq E(S_z,\set{v^*})$, so it suffices to show that $|E'_2|+|E'_3|\le O(|E(x_z,x_{z+1})|)$.
Since $z$ is not a problematic index, $|E^{\rig}_{z}|+|E^{\lef}_{z+1}|+|E^{\through}_{z}|\le 100\cdot|E(x_{z},x_{z+1})|$.
Note that 
$$|E'_2|\le 2\cdot|E^{\rig}_{a}|\le 2(|E(x_a,x_{z+1})|+|E^{\through}_{z}|)\le 2(|E^{\lef}_{z+1}|+|E^{\through}_{z}|),$$ 
and
$$|E'_3|\le |E(S'_z,x_{z+1})|+|E^{\through}_{z}|\le |E^{\lef}_{z+1}|+|E^{\through}_{z}|.$$
So in this case $|E'|\le 300\cdot |E(x_{z'},x_{z'+1})|\le 300\cdot|E(S_z,\set{v^*})|$.
This completes the proof that $H'$ has the $\alpha$-cut property with respect to path $\tau'$, for $\alpha=300$.
\iffalse
It suffices to show that (i) there is a set of paths routing $E'$ to $x_i$ in $S'_i$ with congestion $10$; and (ii) there is a set of paths routing $E'$ to $x_i$ in $\notS'_i\cup\set{v^*}$ with congestion $10$.
	
	%Consider another graph $G'_X$, that is obtained from $G$ by contracting clusters $C_1,\ldots,C_{a}$ into a vertex $v^{\lef}$ and contracting clusters $C_{z+1},\ldots,C_{r}$ into a vertex $v^{\rig}$. Let $H'_X$ be its corresponding contracted graph, where $V(H'_X)=V(Y)\cup \set{v^{\lef},v^{\rig}}$. Note that $G_X$ can be viewed as obtained from $G'_X$ by contracting $v^{\lef},v^{\rig}$ into a single vertex $v^*$, and similarly $H_X$ can be viewed as obtained from $H'_X$ by contracting $v^{\lef},v^{\rig}$ into $v^*$.
	
	We first show (i).
	Note that $E'=\delta_{H_X}(S'_i)$.
	Similar as the proof of \Cref{claim: inner paths}, from the fact that $a$ is a problematic index (and \Cref{obs: bad inded structure}) and \Cref{obs: large capacity up to midpoint}, we can show that there is a set of paths routing $E'$ to $x_i$ in $S'_i$, with congestion $10$. This is since the proof of \Cref{claim: inner paths} only uses the fact that $z<\RMP(a)$, and here we have $i\le z<\RMP(a)$.
	
	We now show (ii). 
	Consider another graph $G'_X$, that is obtained from graph $G$ by contracting clusters $C_1,\ldots,C_{a}$ into a vertex $v^{\lef}$ and contracting clusters $C_{z+1},\ldots,C_{r}$ into a vertex $v^{\rig}$. Let $H'_X$ be its corresponding contracted graph, so $V(H'_X)=V(Y)\cup \set{v^{\lef},v^{\rig}}$. Note that graph $G_X$ can be also viewed as obtained from $G'_X$ by contracting $v^{\lef},v^{\rig}$ into a single vertex $v^*$, and similarly $H_X$ can be viewed as obtained from $H'_X$ by contracting $v^{\lef},v^{\rig}$ into $v^*$.
	We denote $E'_1=E_{H'_X}(v^{\lef},S'_i)$ and $E'_2=E_{H'_X}(v^{\rig},\notS'_i)\cup E_{H'_X}(S'_i,\notS'_i)$. 
	From the properties of minimum-cut, there is a set of edge-disjoint paths routing $E'_2$ to $v_{i+1}$ in $\notS'_i\cup v^{\rig}$.
	%We now show that $|E'_1|\le 4|E'_2|$. 
	Similar as the proof of \Cref{claim: outer paths}, we can show that $|E'_1|\le 2|E(x_a,v^{\rig})|$.
	Moreover, since $E(x_a,v^{\rig})\subseteq \delta_{H'_X}(\notS'_i\cup v^{\rig})$, there is a set of edge-disjoint paths routing $E(x_a,v^{\rig})$ to $v_{i+1}$, using only edges of $\bigcup_{i<z'<z}\hat{E}_{z'}$. 
	Therefore, the edges of $E'_1$ can be routed to $v_{i+1}$ in $\notS'_i\cup \set{v^{\rig}}$ with congestion $4$.
	Altogether, edges of $E'_1\cup E'_2$ can be routed to $v_{i+1}$ in $\notS'_i\cup \set{v^{\rig}}$ with congestion $5$ in graph $H'_X$. Therefore, as edges of $H_X$, they can be routed to $v_{i+1}$ in $\notS'_i\cup \set{v^{*}}$ with congestion $5$.
	%We denote $E_1=\delta_{H'_X}(v^{\lef})$ and $E_2=\delta_{H'_X}(v^{\rig})$, so edges of $E_1,E_2$ are also edges in $H_X$.
	%We first show (i). Note that $E'=$ Recall that in the proof of \Cref{claim: inner paths}, we have computed a set $\hat\qset_1$ of paths routing $E_1$ to $x_z$ in $Y$, using only edges of $\bigcup_{a<z'<z}\hat E_{z'}$.
	%Similar as the proof of \Cref{claim: inner paths}, from the fact that $a$ is a problematic index (and \Cref{obs: bad inded structure}) and \Cref{obs: large capacity up to midpoint}, we can derive that there is a set $\set$
\fi
\end{proofof}




\iffalse
Second, we consider a pair $\hat R',\hat R''$ of clusters that are constructed by performing some consecutive pair $(i_j,i_{j+1})$ of problematic index in Case 2.
As before, we consider the graph $H'$ obtained from $H$ by contracting the vertices of $R'$ into a vertex $v$, and the vertices of $R''$ into a vertex $v'$. The difference this time is that we are guaranteed that at least  half the edges in the original set $E_a^{\rig}$ have an endpoint in $v$. This ensures that index $a$ stops being problematic. Same happens for index $b$. 

Third, we consider the cluster $\hat R''$ obtained from processing the first index $i_1$ and the cluster $\hat R'$ obtained from processing the last index $i_q$. 
Once that cluster is contracted, the index will stop being problematic. Last problematic index is treated similarly.
\znote{end here}
\fi















\subsubsection{Second-Level Disengagement}
\label{subsec: 2nd disengagement}

%We now consider the sub-instances in $\iset(\xset,\tilde\qset,\tilde\pset)$ one-by-one, and compute a disengagement on each of them, such that in each of the resulting sub-instances, the Gomory-Hu tree of the contracted graph (obtained by contracting each cluster $C_i$ of $\cset$ into a single vertex $x_i$) is a path without problematic indices.


%\paragraph{Handling Instance $\hat I(\xset,\tilde \qset)$.}
In this step we further process the instance $\hat I(\xset,\tilde \qset)$ of $\iset(\xset,\tilde\qset,\tilde\pset)$. 
Recall that $\hat I(\xset,\tilde \qset)=(\hat G,\hat \Sigma)$, where the graph $\hat G$ is obtained from $G$ by contracting every cluster in $\xset$ into a single vertex $u^*(X)$.
%It is easy to verify that the Gomory-Hu tree of $\hat G$, which we denote by $\hat{\tau}$, is the path obtained from $\tau$ by contracting corresponding clusters of $\tau$ into vertices. However, path $\hat{\tau}$ may still contain bad indices. Therefore, we cannot apply the result of \Cref{subsec: no prob edges} here but need to decompose the graph $\hat G$ differently.
Denote $J=\bigg[1,\LMP(i_1)\bigg]\cup \bigg(\RMP(i_q),r\bigg]\cup\text{ }\bigcup_{1\le j\le q-1}\bigg(\RMP(i_j), \LMP(i_{j+1})\bigg]$,
so %the vertex set of $\hat G$ is 
$V(\hat G)=\set{u^*(X)\mid X\in \xset}\cup (\bigcup_{i\in J}V(C_i)).$



\subsubsection*{Step 1: Defining the Clusters}

We first construct a set $\hat\cset$ of clusters of $\hat G$.
We start with $\hat\cset=\emptyset$, and then process every consecutive pair of problematic indices, as follows.
Consider the index pair $i_j,i_{j+1}$ for some $1\le j\le q-1$.
For brevity, we denote $i_j=a$ and $i_{j+1}=b$.
Recall that we have constructed clusters $X_j,X'_j$ in Step 1 of the first-level disengagement in \Cref{subsec: 1st disengagement}, and they correspond to vertices $u^*(X_j),u^*(X_j)$ in $\hat G$.
We now distinguish between the following cases:
\begin{enumerate}
\item \label{blt: cluster construction Case 1} if $\LMP(b)<\RMP(a)$, then we add the cluster that contain two vertices $u^*(X_j),u^*(X'_j)$ (and edges connecting them) into $\hat{\cset}$ (see \Cref{fig: new_clusters_1});
\item \label{blt: cluster construction Case 2} if $\LMP(b)=\RMP(a)=t$, then we add the subgraph of $\hat G$ induced by $C_t\cup \set{u^*(X_j),u^*(X'_j)}$ into $\hat{\cset}$ (see \Cref{fig: new_clusters_2});
\item \label{blt: cluster construction Case 3} if $\LMP(b)>\RMP(a)$, then we add (i) the subgraph of $\hat G$ induced by $C_{\RMP(a)}\cup \set{u^*(X_j)}$ into $\hat{\cset}$; (ii) the subgraph of $\hat G$ induced by $C_{\LMP(b)}\cup \set{u^*(X'_j)}$ into $\hat{\cset}$; and (iii) for each $\RMP(a)<t<\LMP(b)$ (if there is any), the cluster $C_t$ to $\hat{\cset}$ (see \Cref{fig: new_clusters_3}). 
\end{enumerate}
\begin{figure}[h]
\centering
	\subfigure[Clusters of $\hat\cset$ in Case \ref{blt: cluster construction Case 1}.]{\scalebox{0.29}{\includegraphics[scale=1.0]{figs/new_cluster_1.jpg}}\label{fig: new_clusters_1}}
	\hspace{0.2cm}
	\subfigure[Clusters of $\hat\cset$ in Case \ref{blt: cluster construction Case 2}.]{
		\scalebox{0.29}{\includegraphics[scale=1.0]{figs/new_cluster_2.jpg}}\label{fig: new_clusters_2}}
	\hspace{0.2cm}
	\subfigure[Clusters of $\hat\cset$ in Case \ref{blt: cluster construction Case 3}.]{
		\scalebox{0.29}{\includegraphics[scale=1.0]{figs/new_cluster_3.jpg}}\label{fig: new_clusters_3}}
	\caption{Illustration of constructing clusters in $\hat{\cset}$.}
\end{figure}


Finally, we additionally process the first index and the last index as follows. For the first index $i_1$, we add the the subgraph of $\hat G$ induced by $C_{\LMP(i_1)}\cup \set{u^*(X'_0)}$ into $\hat{\cset}$; and then for each $1\le t<\LMP(b)$ (if there is any), the cluster $C_t$ to $\hat{\cset}$. 
For the last index $i_q$, we add the the subgraph of $\hat G$ induced by $C_{\RMP(i_q)}\cup \set{u^*(X_q)}$ into $\hat{\cset}$; and then for each $\RMP(b)<t\le r$ (if there is any), the cluster $C_t$ to $\hat{\cset}$. 
This completes the construction of clusters in $\cset$.

Recall that $H=G_{|\cset}$, and the Gomory-Hu tree for $H$ is the path $\tau=(x_1,\ldots,x_r)$.
We define $\hat H$ to be the graph obtained from $H$ by contracting, for each cluster $X\in \xset$ that we have constructed in the first-level disengagement, the vertices in the corresponding cluster $Y$ in $H$ into a single vertex.
Similarly, we define $\hat\tau$ as the path obtained from $\tau$ by contracting, for each $X\in \xset$, the vertices in its corresponding cluster $Y$ in $H$ into a single vertex, so $V(\hat\tau)=V(\hat H)$.
Since the vertices in each such cluster $Y$ induce a subpath in $\tau$, from \Cref{lem: GH tree path vs contraction}, the path $\hat\tau$ is a Gomory-Hu tree of $\hat H$.

Note that $V(\hat H)=\set{u^*(X)\mid X\in \xset}\cup\set{x_t\mid t\in J}$.
Now we define $H'$ as the graph obtained from $\hat H$ by contracting, for each cluster of $\cset$ that contains a vertex $u^*(X)$ and a cluster $C_t$, the corresponding vertices $u^*(X)$ (or two vertices $u^*(X)$ and $u^*(X')$) and $x_t$ into a single vertex. Clearly, $H'=\hat G_{|\hat{\cset}}$.
Similarly, we define $\tau'$ as the path obtained from $\hat\tau$ by contracting the same sets of vertices into a single vertex as $H'$, so $V(\hat\tau)=V(\hat H)$. From \Cref{lem: GH tree path vs contraction}, the path $\tau'$ is a Gomory-Hu tree of $H'$. 


\iffalse
First, for each $i\in J$, we add cluster $C_i$ to $\hat{\cset}$.
Second, we add single-vertex clusters $u^*(X'_0), u^*(X_q)$ to $\hat{\cset}$, and for each $1\le j\le q-1$ such that $\RMP(i_j)\leq \LMP(i_{j+1})$, we add single-vertex clusters $u^*(X_j),u^*(X'_j)$ to $\hat\cset$. 
Finally, for each $1\le j\le q-1$, we add a cluster that contains only two vertices $u^*(X_j),u^*(X'_j)$ and the edges between them to $\hat\cset$.
Denote $\hat H=\hat G_{|\hat\cset}$, so
$V(\hat H)=\set{u^*(X)\mid X\in \xset}\cup \set{x_i\mid i\in J}$.
It is easy to verify that, the Gomory-Hu tree of the contracted graph $\hat H$, that we denote by $\hat{\tau}$, is a path\znote{add cor in prelim}, where the order in which the vertices appear on $\hat{\tau}$ is consistent with the path $\tau$. 

We now show that the path $\hat{\tau}$ does not contain a problematic index.
First, it is easy to verify that every index $i\in J$ is not a problematic index, from \znote{add cor in prelim} and the fact that $x_i$ is not a problematic index in $\tau$.
\fi


\subsubsection*{Step 2: Constructing Paths Sets for Clusters in $\hat{\cset}$}

In the second step, we compute, for each cluster $C\in \hat\cset$, a vertex $u(C)$ and a set $\qset(C)$ of paths routing edges of $\delta(C)$ to $u(C)$ inside $C$.
We will repeatedly use the following observation.
\begin{observation}
\label{obs: forever not problematic}
Let $a< z$ be indices in $\set{1,\ldots, r}$ such that $a$ is problematic, $z$ is not problematic index and $z<\RMP(a)$, then $|\delta_H(\set{x_t\mid a< t\le z})|\le 504 \cdot |E(x_z,x_{z+1})|$.
\end{observation}
\begin{proof}
Since $z$ is not a problematic index, $|E^{\lef}_{z+1}|+|E^{\rig}_{z}|+|E^{\thr}_{z}|\le 100\cdot |E(x_z,x_{z+1})|=100\cdot |\hat E_z|$.
Denote $U=\set{x_t\mid a< t\le z}$.
Note that $U\subseteq S_z$, so 
$$|E(U,\notS_z)|\le |E(S_z,\notS_z)|\le |E^{\lef}_{z+1}|+|E^{\rig}_{z}|+|E^{\thr}_{z}|
\le 100\cdot|\hat E_z|.$$
On the other hand, since $z<\RMP(a)$, at least half of edges in $E^{\rig}_a$ has an endpoint in $\notS_z$. Therefore, 
$$|E(U,S_a)|\le |E^{\lef}_{a+1}|+|E(x_{a},U)|+|E^{\thr}_{a}|\le 2|E^{\rig}_a|\le 4|E(x_a,\notS_z)|\le 4(|E^{\lef}_{z+1}|+|\hat E_z|)\le 404\cdot |\hat E_z|.$$
Altogether, $|\delta_H(U)|=|E(U,\notS_z)|+|E(U,S_a)|\le 504\cdot |E(x_z,x_{z+1})|$.
\end{proof}


We distinguish between the following cases.

Consider first a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 1}. From the construction, $C$ contains only two vertices $u^*(X_j),u^*(X'_j)$.
Recall that the corresponding clusters $Y_i,Y'_i$ are obtained by splitting at a non-problematic index $z$ in $H$ (see \Cref{fig: path_cluster_H}). 
%From \Cref{obs: forever not problematic}, $|E(u^*(X_j),u^*(X'_j))|=|E(Y_i,Y'_i)|\ge |E(Y_i,Y'_i)|\ge |E(Y_i,\notS_z)|/100$ and similarly $|E(u^*(X_j),u^*(X'_j))|\ge |E(Y'_i,S_z)|/100$. On the other hand, $|E(Y_j,S_{i_j})|\le |E^{\lef}_{i_j+1}|+|\hat E_{i_j}|\le 2|E^{\rig}_{i_j}|$, and from \Cref{obs: large capacity up to midpoint}, $|E(x_z,x_{z+1})|\ge |E^{\rig}_{i_j}|/2$. Therefore, $|E(x_z,x_{z+1})|\ge |E(Y_j,S_{i_j})|/4$. Altogether, $|\delta_H(Y_i)|\le 104\cdot |E(x_z,x_{z+1})|$.
From \Cref{obs: forever not problematic}, $|\delta_H(Y_j)|\le 504\cdot |E(x_z,x_{z+1})|$.
We set $u(C)=u^*(X'_j)$. Then clearly there is a set $\qset(C)$ of paths routing the edges of $\delta(C)$ to $u(C)$ inside $C$, with congestion at most $504$.

Consider now a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 2}.
From the construction, $C$ contains the cluster $C_t$ and two vertices $u^*(X_j),u^*(X'_j)$.
From \Cref{claim: inner and outer paths}, there is a set $\hat\qset(Y_j)$ of paths routing edges of $\delta_H(Y_j)$ to $x_{t-1}$ in $Y_j$, with congestion $O(1)$; and there is a set $\hat\qset(Y'_j)$ of paths routing edges of $\delta_H(Y'_j)$ to $x_{t+1}$ in $Y'_j$, with congestion $O(1)$.
Moreover, from \Cref{obs: forever not problematic}, $|\delta_H(Y_j)|\le 504\cdot |E(x_{t-1},x_{t})|$ and 
$|\delta_H(Y'_j)|\le 504\cdot |E(x_{t},x_{t+1})|$.
Therefore, if we denote $U=Y_j\cup \set{x_t}\cup Y'_{j}$, then there exists a set $\hat{\qset}(U)$ of edges routing edges of $\delta_H(U)$ to $x_t$, with congestion $O(1)$.
We set $u(C)=u(C_t)$, then we can easily construct a set $\qset(C)$ of paths routing edges of $\delta(C)$ to $u(C)$, using the paths of $\hat{\qset}(U)$ and the paths of $\qset(C_t)$ that we are given, such that for each edge $e\in C$, $(\cong_{C}(\qset(C),e))^2\le O(\temp)$.


Consider now a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 3}. If $C=C_t$ for some $\RMP(i_j)<t<\LMP(i_{j+1})$, then we set $u(C)=u(C_t)$ and the path $\qset(C_t)$ is the desired path set we want.
If $C$ contains cluster $C_{RM(i_j)}$ and vertex $u^*(X_j)$, then from \Cref{obs: forever not problematic}, $|\delta(u^*(X_j))|\le O(|E(u^*(X_j),C_{RM(i_j)})|)$. 
Therefore, if we set $u(C)=u(C_{RM(i_j)})$, then it is easy to construct the desired set $\qset(C)$ of paths using the edges of $E(u^*(X_j),C_{RM(i_j)})$ and the path set $\qset(C_{RM(i_j)})$.
The way for handling the cluster that contains cluster $C_{LM(i_{j+1})}$ and vertex $u^*(X'_j)$ is symmetric.

The way for handling clusters that are constructed in processing the first and the last indices are the same as that of the clusters constructed in Case \ref{blt: cluster construction Case 3}.


\subsubsection*{Step 3: Proving that graph $H'$ has the $\alpha$-Cut Property for $\alpha=O(1)$}

\iffalse
From the proof of \Cref{claim: outer paths}, for each $1\le j\le q-1$, $|E_H(Y_j,Y'_j)|\ge |\delta_H(Y_j)|/6$. Therefore, there is a set $\hat{\qset}_j$ of paths routing the edges of $\delta_{\hat G}(U_j)$ to $u^*(X'_j)$ in $U_j$, that causes congestion at most $6$.
Note that this also immediately implies that the vertices in $\hat{\tau}$ that correspond to clusters $U_1,\ldots,U_{q-1}$ are not problematic indices.
It is then easy to verify that $\hat{\tau}$ does not contain a problematic index. 
%Denote $\hat\qset=\bigcup_{1\le j\le q-1}\hat\qset_j$.
\fi




We distinguish between the following cases.

Consider first a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 1}, so $V(C)=\set{u^*(X_j),u^*(X_j)}$.
Denote $a=i_j$ and $b=i_{j+1}$.
Assume first that indices $\LMP(b),\RMP(a)$ are both greater than $a$ and less than $b+1$ (see \Cref{fig: midpoints inside}). Let $C'$ be the cluster on the right of $C$ in path $\tau'$.
Since $\LMP(b)\ge a+1$, at least half the edges of $E^{\lef}_{b+1}$ have an endpoint in the cluster $Y_j\cup Y'_j$. Therefore, $|E(Y_j\cup Y'_j,x_{b+1})|\ge |E^{\lef}_{b+1}|/2\ge (|E^{\lef}_{b+1}|+|E^{\rig}_{b}|+|\hat E_{b}|)/6$, and it follows that the vertex in $\tau'$ that corresponds to cluster $C$ is not a problematic index.
Assume now that $\LMP(b)<a$ (see \Cref{fig: midpoints outside}).
In this case, we first show that $\RMP(a)\le b+1$, since otherwise, 
$$|\hat E_a|\le \frac{|E(x_a,\notS_{\RMP(a)-1})|}{20}
\le \frac{|E^{\thr}_b|}{20}\le \frac{|\hat E_b|}{20}\le \frac{|E(x_{b+1},\notS_{\LMP(b)})|}{400}\le \frac{|E^{\thr}_a|}{400}\le \frac{|\hat E_a|}{400},$$ 
a contradiction.
Note that $E(x_{b+1},S_{\LMP(B)})\subseteq E^{\thr}_a$, so $|E^{\lef}_{b+1}|\le 2|\hat E_a|$.




\begin{figure}[h]
	\centering
	\subfigure[Subgraphs $Y_j,Y'_j$ in $H$.]{\scalebox{0.3}{\includegraphics{figs/cut_prop_1.jpg}}
	\label{fig: midpoints inside}}
	\hspace{4pt}
	\subfigure[Subgraphs $X_j,X'_j$ in $G$.]{\scalebox{0.3}{\includegraphics{figs/cut_prop_2.jpg}}
	\label{fig: midpoints outside}}
	\caption{An illustration of subgraphs $Y_j,Y'_j$ in $H$ and subgraphs $X_j,X'_j$ in $G$.}\label{fig: cut property case_1}
\end{figure}

Consider now a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 2}.

Consider now a cluster $C$ that is constructed in Case \ref{blt: cluster construction Case 3}. 

We can now apply the result of \Cref{subsec: no prob edges} and obtain a set $\iset_{\hat G}$ of sub-instances that satisfy the properties of \Cref{lem: path case}, and $\sum_{I'\in \iset_{\hat G}}\optcrors(I')\le O((\optcrors(\hat G,\hat\Sigma)+|E(\hat G)|)\cdot \temp)$.


%We define a collection $\cset'$ of clusters for graph $G'$, as follows. Note that every cluster $C\in \cset$ is either contained in one of the graphs $\hat R',\hat R''$, or is disjoint from both graphs. We start by adding to $\cset'$ all clusters $C\in \cset$ that are disjoint from both graphs $\hat R'$, $\hat R''$, and then we add two more clusters: $\set{v}$, and $\set{v'}$. Note that $\bigcup_{C\in \cset'}V(C)=V(G')$. It is not hard to see that the Gomory-Hu tree for the corresponding graph $H'=G_{|\cset'}$ is a path, that is obtained from the path $P^*$, by contracting the vertices of $\rset'$ into a vertex $v$, and the vertices of $\rset''$ into a vertex $v'$. We denote this path by $P'=(x_1,\ldots,x_a,v,v',x_b,\ldots,x_r)$. Consider now the corresponding graph $H'$. Consider first the set  $E_a^{\rig}$ of edges in the original graph $H$. Recall that there is a subset $E'\subseteq E_a^{\rig}$ containing at least half the edges of $E_a^{\rig}$, that have an endpoint in $\set{x_{a+2},\ldots,x_{z+1}}$. All these edges are incident to either $v$ or $v'$ in the new graph $H'$. If at least a $1/10$-fraction of these edges are incident to $v$, then index $a$ is no longer problematic. The claim is that, if we define a cluster $C=\set{v,v'}$, then we can route the boundary of $C$ to $v$. Once $C$ becomes a cluster, it will be contracted in graph $H'$, and indices $a$ and $b$ will stop being problematic.








==> laminar_and_disengage_general.tex <==

\newpage

\subsubsection*{The General Case.}

We start with some pre-processing steps.
We first apply Lemma~\ref{lem: path set inside a well-linked cluster} to all clusters of $\cset^*$, and find, for each $C\in \cset^*$, a vertex $u_C\in C$ and a set $\qset^{in}_C$ of paths in $C$, routing edges of $\delta(C)$ to $u_C$, such that $\cost(\qset_C)\le O(\cro(C)\cdot (\poly\log n/\alpha^2))$.
We then define a circular ordering $\oset_C$ on the set $\delta(C)$ of edges as the following \znote{?}.
Second, consider a pair $C,C'$ of clusters in $\cset^*$ such that $S_{C'}$ is the parent cluster of $S_{C}$ in the laminar family $\lset$.
From the construction of $\lset$, the cut $(S_C,\overline{S_C})$ is the min-cut in $G'$ separating $C$ from $C'$.
We then apply Lemma~\ref{lem: cut-edge-to-cluster-boundary} to the clusters $C,C'$ and the min-cut $(S_C,\overline{S_C})$ separating them, and obtain a set of edge-disjoint paths in $S_C$ connecting edges of $E(S_C,\overline{S_C})$ to edges of $\delta(C)$, that we denote by $\qset^{cut}_C$.





We are now ready to construct the disengaged instance $(H_C,\Sigma_C)$ for clusters in $\cset^*$.
Consider a cluster $C\in \cset^*$ and the corresponding cluster $S_C\in \lset$. The graph $H_C$ is defined as follows.
We start with the graph $G'$. We first contract all vertices in $G\setminus S_{C}$ into a single vertex, that we denote by $v^{out}_C$. Notice that the edges incident to $v^{out}_C$ correspond to the edges of $\delta(S_C)$ (for simplicity, we will not distinguish between them). The circular ordering of the edges incident to $v^{out}_C$ is defined to be $\oset_C$.
Next, let $S_{C_1},\ldots,S_{C_q}$ be child clusters of $S_C$. For all $1\leq i\leq q$, we contract all vertices of $S_i$ into a super-node $v^{in}_{C,C_i}$. Notice that the edges incident to $v^{in}_{C,C_i}$ correspond to the edges of $\delta(S_{C_i})$; we do not distinguish between them. 
This finishes the construction of the graph $H_C$. We now define the rotation system $\Sigma_C$ on it. 
From the above discussion, $V(H_C)=V(C)\cup\set{v^{out}_C}\cup\set{v^{in}_{C,C_i}}_{1\le i\le q}$.
The orderings at the vertices of $C$ are identical to their orderings in $\Sigma'$.
The ordering of the edges incident to $v^{out}_C$ is defined to be $\oset_C$.
The ordering of the edges incident to $v^{in}_{C,C_i}$ is defined to be \znote{?}.

This completes the description of the instance $(H_C,\Sigma_C)$. See Figure~\ref{fig: disengaged_instance} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of the graph $G$.]{\scalebox{0.3}{\includegraphics{figs/dis_instance_before}}\label{fig: graph G}}
	\hspace{1cm}
	\subfigure[The graph $H_C$.]{
		\scalebox{0.3}{\includegraphics{figs/dis_instance_after}}\label{fig: C and disc}}
	%\hspace{1cm}
	%\subfigure[caption subfigure 3]{\scalebox{0.2}{\includegraphics{file3.pdf}}\label{fig: label3}}
	\caption{An illustration of the disengagement instance.\label{fig: disengaged_instance}}
\end{figure}




We will now analyze $\sum_{C\in \cset^*}\optcrors(H_C,\Sigma_C)$.
Recall that $\tau$ is the structural tree of $\lset$.
The vertex set $V(\tau)$ can be decomposed into two subsets: set $V_0(\tau)$ contains all nodes with degree $2$ in $\tau$, and set $V_1(\tau)$ contains all other nodes in $\tau$.
We partition $\cset^*$ into two subsets similarly: set $\cset^*_0$ contains the clusters in $\cset^*$ that correspond to nodes in $V_0(\tau)$, and set $\cset^*_1$ contains the clusters in $\cset^*$ that correspond to nodes in $V_1(\tau)$.

\begin{claim}
	$\sum_{C\in \cset^*_0}\optcrors(H_C,\Sigma_C)\le O(\optcrors(G',\Sigma')\poly\log n)$.
\end{claim} 

\subsubsection{Technical Lemmas}


\begin{lemma}
\label{lem: cut-edge-to-cluster-boundary}
There is an efficient algorithm, that, given any pair $C_1,C_2$  vertex-disjoint clusters of $G$, and any min-cut $(A_1,A_2)$ in $G$ separating $C_1$ from $C_2$, with $V(C_1)\subseteq A_1$ and $V(C_2)\subseteq A_2$, computes, for each $i\in \set{1,2}$, there exists a set $\pset_i$ of edge-disjoint paths in $A_i$ routing the edges of $E(A_1,A_2)$ to edges of $\delta(C_i)$.
\end{lemma}

\begin{lemma}
\label{lem: path set inside a well-linked cluster}
There is an efficient algorithm, that, given any $\alpha$-boundary-linked cluster $C$, computes a vertex $u_C\in C$ and a set $\qset_C$ of paths, routing edges of $\delta(C)$ to $u_C$, such that $\cost(\qset_C)\le O(\cro(C)\cdot (\poly\log n/\alpha^2))$.
\end{lemma}







==> laminar_and_disengage_path.tex <==
\subsection{Phase 2: Laminar Family and Disengagement of Clusters}

In this section we assume that the given sub-instance $(G',\Sigma')$ (with $|E(G')|=m$) satisfies that $\optcrors(G',\Sigma')\ge |E(G')|^2/\mu^{10}$, and in the first phase, we have computed a set $\cset^*$ of clusters, such that
such that each cluster of $\cset^*$ is either a good cluster or a flower cluster, the vertex sets $\set{V(C)}_{C\in \cset^*}$ partitions $V(G')$, and $|\inE(\cset^*)|= O(m/\mu)$.

\subsubsection*{Step 1: Compute a laminar family of clusters}

Let $\tilde G$ be the graph obtained from $G'$ by contracting each cluster of $\cset^*$ into a single vertex, while keeping parallel edges and deleting self-loops. For each cluster $C\in \cset^*$, let $v_C$ be the node in $\tilde G$ obtained from contracting the cluster $C$.

We compute the Gomory-Hu tree of $\tilde G$, and let $\tilde \tau$ be the tree that we obtain. We root $\tilde \tau$ at an arbitrary node. We now define, based on the structure of the rooted tree $\tilde \tau$, a laminar family $\tilde \lset$ of clusters in $\tilde G$, as follows.
For each node $v_C$, we define the cluster $\tilde S_C$ to be the subgraph of $\tilde G$ induced by all nodes in the subtree of $\tilde \tau$ rooted at the node $v_C$. 
We then let $\tilde \lset=\set{\tilde S_C\mid C\in \cset^*}$.
It is easy to verify that the $\tilde \lset$ is a laminar family of clusters of $\tilde G$.
We define a corresponding laminar family $\lset$ of clusters in $G$ as follows. For each cluster $\tilde S_C\in \tilde \lset$, we define the cluster $S_C$ as the subgraph of $\tilde G$ induced by vertices of $\bigcup_{v_{C'}\in \tilde S_C}V(C')$. 
It is easy to verify that the $\lset$ is a laminar family of clusters of $G$.

We denote by $\tau$ the structure tree of $\lset$. 
It is easy to verify that, if we identify the node of $\tau$ that represents the cluster $S_C$ with the node of $\tilde \tau$ that represents the cluster $\tilde S_C$, then $\tau=\tilde \tau$.

\iffalse
We use the following claim.
\begin{claim}
Each cluster $S_C\in \lset$ is $\alpha$-boundary-well-linked.
\end{claim}
\begin{proof}
Let $S_{C'}$ be the parent cluster of $S_C$.
$(S_C,\overline{S_C})$ is the min-cut in $G'$ separating $C$ from $C'$. Recall that $C$ is $\alpha$-boundary-well-linked. Combined with Lemma~\ref{lem: cut-edge-to-cluster-boundary}, we can derive that $S_C$ is also $\alpha$-boundary-well-linked.
\end{proof}
\fi


\subsubsection*{Step 2: Disengaging the clusters}

In this step we construct, for each cluster $C\in \cset^*$, an instance $(H_C,\Sigma_C)$  of \CNwRS, that we call the \emph{disengaged instance} for cluster $C$.
We first consider the special case where the structure tree $\tau$ of the laminar family $\lset$ is a path. The algorithm of constructing the disengaged instances in this special case will serve as a building block for the algorithm in the general case.


\subsubsection*{Special Case: $\tau$ is a path.}
\znote{Not ready yet. Please do not read.}

Denote $\cset^*=\set{C_1,\ldots,C_k}$. Let $S_{C_1},\ldots,S_{C_k}$ be the clusters in $\lset$, with $S_{C_k}\subseteq S_{C_{k-1}}\subseteq \ldots \subseteq S_{C_1}=G$.
From the construction of $\lset$, for each $1\le i\le k$, $S_{C_i}=\bigcup_{i\le j\le k}C_j$.
Recall that, for each $1\le i\le k$, the cluster $C_i$ is $\alpha$-boundary-well-linked. We apply Lemma~\ref{lem: path set inside a well-linked cluster} to each cluster $C_i$, and obtain a vertex of $C_i$, which we denote by $u_i$, and a set of paths in $C_i$ connecting the edges of $\delta(C_i)$ to $u_i$, which we denote by $\qset_i$.
From Lemma~\ref{lem: path set inside a well-linked cluster}, $\cost(\qset_i)\le O(\cro(C)\cdot (\poly\log n/\alpha^2))$.


\paragraph{Step 2.1. Compute Central Paths.}
Recall that $\inE(\cset^*)$ is the set of edges connecting distinct clusters of $\cset^*$. 
We define $E'$ to be the subset of edges in $\inE(\cset^*)$ connecting a pair $C_i,C_j$ of distinct clusters of $\cset^*$, with $j\ge i+2$.
For each $1\le i\le k$, we denote $E_i=E(C_i,C_{i+1})$.
Therefore, $E(G)=E'\cup\left(\bigcup_{1\le i\le k-1}E_i\right)\cup \left(\bigcup_{1\le i\le k}E(C_i)\right)$.
We will first compute, for each edge $e\in E'$ that connects a vertex of $C_i$ to a vertex of $C_j$, a path $P_e$ connecting $u_i$ to $u_j$, that only uses edges of $\bigcup_{i\le t\le j-1}E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$. We call the path $P_e$ the \emph{central path} of $e$.

The central paths $\set{P_e}_{e\in E'}$ are computed as follows. Recall that $\tilde G$ is the graph obtained from $G$ by contracting each cluster of $\set{C_1,\ldots,C_k}$ into a single vertex, while keeping parallel edges and deleting self-loops. Denote by $v_i$ the node in $\tilde G$ that represents the cluster $C_i$ in $G$.
Note that each edge in $E'\cup \left(\bigcup_{1\le i\le k-1}E_i\right)$ corresponds to an edge in $\tilde G$, and we do not distinguish between them. 
We now process the edges in $E'$ one-by-one. Throughout, for each edge $\hat e\in \bigcup_{1\le i\le k-1}E_i$, we maintain an integer $x_{\hat e}$ indicating how many times the edge $\hat e$ has been used, that is initialized to be $0$. Consider an iteration of processing an edge $e\in E'$. Assume $e$ connects $v_i$ to $v_j$ in $\tilde G$, we then pick, for each $i\le t\le j-1$, and edge of $E_t$ with minimum $x_{\hat e}$, and let $\tilde P_e$ be the path formed by all picked edges. We then increase the value $x_{\hat e}$ for all picked edges $\hat e$ by $1$, and proceed to the next iteration. After processing all edges of $E'$, we obtain a set $\tilde\pset=\set{\tilde P_e}_{e\in E'}$ of paths in $\tilde G$.
{\color{red} We further assume that, for each $1\le i\le k$, $|E(S_i,\overline{S_i})|\le \beta\cdot |E_i|$, where we can think of $\beta=\poly\log n$.}
We use the following observation.

\begin{observation}
\label{obs:central_congestion}
For each edge $\hat e\in \bigcup_{1\le i\le k-1}E_i$, $\cong_{\tilde\pset}(\hat e)\le \beta$.
\end{observation}
\begin{proof}
%For each $1\le i\le k-1$, we denote by $E^*_i$ as the set of edges in $E'$ that connects a vertex of $\set{v_1,\ldots,v_{i-1}}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$, we denote by $E^{\lef}_i$ as the set of edges in $E'$ that connects $v_{i+1}$ to a vertex of $\set{v_1,\ldots,v_{i-1}}$, and we denote $E^{\rig}_i$ as the set of edges in $E'$ that connects $v_{i}$ to a vertex of $\set{v_{i+2},\ldots,v_{k}}$.
From the algorithm, for each $1\le i\le k-1$, the paths of $\tilde\pset$ that contains an edge of $E_i$ are $\set{\tilde P_e\mid e\in E(S_i,\overline{S_i})\setminus E_i}$.
Since we have assumed that $|E(S_i,\overline{S_i})|\le \beta\cdot |E_i|$, each edge of $E_i$ is used at most $\beta$ times by paths of $\tilde\pset$. The Observation~\ref{obs:central_congestion} follows.
\end{proof}

\iffalse
We now further process the set $\tilde\pset$ of paths to obtain another set $\tilde\pset'$ of paths with some additional properties, as follows.

\paragraph{Step 2.1.} Let $\tilde G'$ be the graph obtained from $\tilde G$ by replacing each edge $e$ with $\beta$ parallel copies $e_1,\ldots,e_\beta$ connecting its endpoints. Now for each path $\tilde P\in \tilde{\pset}$, we define a path $\tilde P^*$ as the union of, for each edge $e\in \tilde P$, a copy $e_t$ of $e$, such that, for all paths of $\tilde\pset$ that contains the edge $e$, their corresponding paths in $\set{\tilde P^*\mid e\in \tilde P}$ contain distinct copies of $e$. We denote $\tilde\pset^*=\set{\tilde P^*\mid \tilde P\in \tilde \pset}$. From the above discussion, the paths of $\tilde\pset^*$ are edge-disjoint.

\paragraph{Step 2.2.} We uncross
\fi

We now compute the set $\pset$ of central paths of edges in $E'$, using the paths in $\tilde\pset$ and sets $\set{\qset_i}_{1\le i\le k-1}$.
Recall that in $G$, an edge of $E_i\cup E_{i-1}$ belongs to the set $\delta(C_i)$. Also recall that the set $\qset_i$ of paths contains, for each edge $e\in\delta(C_i)$, a path $Q^i_e$ connecting $e$ to $u_i$. Now consider an edge $e\in E'$ connecting a vertex of $C_i$ to a vertex of $C_{j}$, and the corresponding path $\tilde P_e=(e_i,e_{i+1},\ldots,e_{j-1})$ in $\tilde\pset$, where $e_t\in E_t$ for each $i\le t\le j-1$. We construct the corresponding central path $P_e$ as the sequential concatenation of paths $Q^{i}_{e_i}, e_i, Q^{i+1}_{e_i}, Q^{i+1}_{e_{i+1}},e_{i+1}, Q^{i+2}_{e_{i+1}},\ldots,Q^{j-1}_{e_{j-1}},e_{j-1}, Q^{j}_{e_{j-1}}$.
It is clear that $P_e$ only contains edges of $\bigcup_{i\le t\le j-1}E_t$ and edges of $\bigcup_{i\le t\le j}E(C_t)$.
Denote $\pset=\set{P_e\mid e\in E'}$.
We use the following observation, that immediately follows from Observation~\ref{obs:central_congestion}.

\begin{observation}
For each edge $\hat e\in \bigcup_{1\le i\le k-1}E_i$, $\cong_{\pset}(\hat e)\le \beta$. For each edge $\hat e\in \bigcup_{1\le i\le k}E(C_i)$, $\cong_{\pset}(\hat e)\le \beta\cdot\cong_{\qset_i}(\hat e)$.
\end{observation}


We will use the set $\pset$ of central paths for concatenate drawings of distinct subgraphs of $G$, so it would be convenient to state our algorithm if the paths of $\pset$ are edge-disjoint. 
For which, we construct an instance $(G',\Sigma')$ of \CNwRS as follows. We start with the instance $(G,\Sigma)$.
Denote $\qset=\bigcup_{1\le i\le k}\qset_i$.
For each edge $e\in E(\qset)$, we replace $e$ with $\cong_{\qset}(e)\cdot \cong_{\pset}(e)$ parallel copies.
For each edge $e\in E(\pset)\setminus E(\qset)$, we replace $e$ with $\cong_{\pset}(e)$ parallel copies.
For each vertex $v$ such that $\delta(v)\cap E(\pset\cup\qset)\ne \emptyset$, its ordering $\oset'_v$ is defined based on $\oset_v$, by replacing, for each edge $e\in \delta(v)\cap E(\pset\cup\qset)$, the edge $e$ in the ordering $\oset_v$ by its copies that appears consecutively at the location of $e$ in $\oset_v$, and the ordering among the copies is arbitrary. We use the following observation.

\begin{observation}
$\optcrors(G,\Sigma)\le \optcrors(G',\Sigma')\le O(\optcrors(G,\Sigma)\cdot\beta^2\cdot\poly\log n)$. 
Moreover, given a drawing $\phi\in \Phi(G,\Sigma)$, we can efficiently compute a drawing $\phi'\in \Phi(G',\Sigma')$, with $\cro(\phi')\le O(\cro(\phi)\cdot\beta^2\cdot\poly\log n)$; given a drawing $\phi'\in \Phi(G',\Sigma')$, we can efficiently compute a drawing $\phi\in \Phi(G,\Sigma)$, with $\cro(\phi)\le\cro(\phi')$.
\end{observation}
\begin{proof}
\end{proof}



From now on we will work with the instance $(G',\Sigma')$. Now for each path $P\in \pset$, we define a path $P'$ in $G'$ as the union of, for each edge $e\in P$, a copy $e_t$ of $e$, such that for all paths of $\pset$ that contains the edge $e$, their corresponding paths in $\set{P'\mid P\in \pset, e\in P}$ contain distinct copies of $e$. We denote $\pset'=\set{P'\mid  P\in \pset}$. From the above discussion, the paths of $\pset'$ are edge-disjoint.
Moreover, note that $V(G)=V(G')$, and if a path $P\in \pset$ connects $u_i$ to $u_j$ in $G$, then the corresponding path $P'$ connects $u_i$ to $u_j$ in $G'$.



\paragraph{Step 2.2. De-interfere Central Paths.}
We further process paths in $\pset'$ to obtain another set $\pset^*$ of edge-disjoint paths in $G'$, such that 
\begin{itemize}
\item $|\pset'|=|\pset^*|$;
\item for each pair $1\le i,j\le k$ with $j\ge i+2$, the number of paths in $\pset'$ connecting $u_i$ to $u_j$ is the same as that of $\pset^*$; and 
\item the paths in $\pset^*$ are locally non-interfering.
\end{itemize}
For each path $P'\in \pset'$ originating at $u_i$ and terminating at $u_{j}$ (recall that such a path visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially), we define, for each $i\le t\le j-1$, the path $P'_{(i)}$ to be the subpath of $P'$ between $u_{i}$ and $u_{i+1}$. For each $1\le i\le k-1$, we denote $\pset'_{(i)}=\set{P'_{(i)}\text{ } \bigg|\text{ } u_i,u_{i+1}\in V(P')}$.


For each $1\le i\le k-1$, we apply the algorithm in Lemma~\ref{lem: non_interfering_paths} to the set $\pset'_{(i)}$ of paths (recall that all paths in $\pset'_{(i)}$ connects $u_i$ to $u_{i+1}$), and obtain a set $\pset^*_{(i)}$ of locally non-interfering paths connecting $u_i$ to $u_{i+1}$, with $|\pset^*_{(i)}|=|\pset'_{(i)}|$ and $E( \pset^*_{(i)})\subseteq E(\pset'_{(i)})$.
We then concatenate the paths of $\pset^*_{(1)},\pset^*_{(2)},\ldots,\pset^*_{(k-1)}$ to obtain the desired set $\pset^*$ of paths, using the following observation.

\znote{Need to rethink which definition to include for ``locally non-interfering".}

\begin{observation}[Restatement of Observation F.3 in~\cite{chuzhoy2020towards}]
\label{obs:rerouting_matching}
There is an efficiently algorithm, that, given a graph $\hat G$, a vertex $v$ of $G$, an ordering $\oset_v$ on the edges of $\delta_G(v)$ and two disjoint subsets $E^-, E^+$ of $\delta_G(v)$ with $|E^-|=|E^+|$, computes a perfect matching $M\subseteq E^-\times E^+$ between the edges of $E^-$ and the edges of $E^+$, such that, for each pair of matched pairs $(e^-_1,e^+_1)$ and $(e^-_2,e^+_2)$ in $M$, the intersection of the path that consists of the edges $e^-_1,e^+_1$ and the path that consists of edges $e^-_2,e^+_2$ at vertex $u$ is non-transversal with respect to $\oset_v$.
\end{observation}

We now construct the set $\pset^*$ of paths as follows.
\znote{Concatenation and Designation. Apply Observation~\ref{obs:rerouting_matching} at $u_1,\ldots, u_k$ sequentially.}
Note that we will not compute a drawing of $G'$, we only use the locally non-interfering paths and their relative ordering in $G'$ to help define disengaged instance of $G$.

We then designate, for each edge $e\in E'_{i,j}$, a distinct path $P^*_e$ of $\pset^*_{i,j}$. Denote by $\oset^*_{i}$ the ordering of paths in $\pset^*$ that contains $u_i$, defined by the rotation $\oset'_{v_i}\in \Sigma'$ at $v$.
\znote{To elaborate.}
Note that 
$\oset^*_{i}$ is also an ordering on the edges of $\bigcup_{j_1\le i\le j_2}E'_{j_1,j_2}$.
We use the following observation.

\begin{observation}
\label{lem: rotation_distance}
We can efficiently compute integers $\set{b_i}_{1\le i\le k}$ where $b_i\in \set{0,1}$ for each $1\le i\le k$, such that $\sum_{1\le i\le k-1}\dist((\oset^*_i,b_i), (\oset^*_{i+1},b_{i+1}))\le O(\optcrors(G,\Sigma)\cdot\beta^2\cdot\poly\log n)$.
\end{observation}


\paragraph{Step 2.3. Construct Disengaged Instances.}

We are now ready to construct the disengaged instances.
Recall that $\cset^*=\set{C_1,\ldots,C_k}$, and the clusters $S_{C_1},\ldots,S_{C_k}$ in the laminar family $\lset$ satisfies that $S_{C_k}\subseteq S_{C_{k-1}}\subseteq \ldots \subseteq S_{C_1}=G$.
For each $1\le i\le k$, we will construct an instance $(H_i,\Sigma_i)$ of \CNwRS.
 
We first construct instance $(H_k,\Sigma_k)$ as follows.
The graph $H_k$ is obtained from $G$ by contracting all vertices in $G\setminus C_k$ into a single vertex, that we denote by $v^{\lef}_k$. 
Notice that the edges incident to $v^{\lef}_k$ correspond to the edges of $\delta(C_k)$, and we will not distinguish between them. 
The ordering of a vertex of $v\ne v^{\lef}_k$ in $\Sigma_k$ is identical to the ordering $\oset_v$ of $v$ in the given rotation system $\Sigma$.
The ordering of the vertex $v^{\lef}_k$ in $\Sigma_k$ is defined to be the restricted ordering in $\oset^*_{k-1}$.
\znote{To elaborate.}

The instance $(H_1,\Sigma_1)$ is defined similarly. 
The graph $H_1$ is obtained from $G$ by contracting all vertices in $G\setminus C_1$ into a single vertex, that we denote by $v^{\rig}_1$. 
We will not distinguish between edges incident to $v^{\lef}_1$ and edges of $\delta(C_k)$. 
The ordering of a vertex $v\ne v^{\rig}_1$ in $\Sigma_1$ is identical to the ordering $\oset_v$ in $\Sigma$.
The ordering of the vertex $v^{\rig}_1$ in $\Sigma_1$ is defined to be the restricted ordering in $\oset^*_{2}$.
\znote{To elaborate.}

Consider now some index $2\le i\le k-1$. We define the instance $(H_i,\Sigma_i)$ as follows.
The graph $H_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a single vertex, that we denote by $v^{\rig}_1$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a single vertex, that we denote by $v^{\rig}_i$. 
The ordering of a vertex $v\ne v^{\lef}_i,v^{\rig}_i$ in $\Sigma_1$ is identical to the ordering $\oset_v$ in $\Sigma$.
The ordering of the vertex $v^{\lef}_i$ in $\Sigma_i$ is defined to be $\oset^*_{i-1}$, and
the ordering of the vertex $v^{\rig}_i$ in $\Sigma_i$ is defined to be the ordering of $\oset^*_{i+1}$.

We prove the following claims.
\begin{claim}
\label{claim: existence of good solutions special}
$\sum_{1\le i\le k}\optcrors(H_i,\Sigma_i)\le O(\optcrors(G,\Sigma)\cdot\beta^2\cdot\poly\log n)$.
\end{claim}

\begin{claim}
\label{claim: stitching the drawings together}
There is an efficient algorithm, that given, for each $1\le i\le k$, a drawing $\phi_i\in \Phi(H_i,\Sigma_i)$, computes a drawing $\phi\in \Phi(G,\Sigma)$, with
$\cro(\phi)\le \sum_{1\le i\le k}\cro(\phi_i)+O(\optcrors(G,\Sigma)\cdot\beta^2\cdot\poly\log n)$.
\end{claim}

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
	
\end{proofof}


\begin{proofof}{Claim~\ref{claim: stitching the drawings together}}
	
\end{proofof}












 

==> laminar_disengagement.tex <==
\subsection{Disengagement with respect to a Laminar Family of Clusters}
\label{sec: laminar_disengagement}

Assume we are given an instance $I=(G,\Sigma)$ of \CNwRS problem. Assume we are also given a laminar family $\lset$ of clusters of $G$, such that $G\in \lset$, and, for each such cluster $S\in \lset$, we are additionally given (i) a vertex $u(S)\in V(S)$, and a set $\qset(S)=\set{Q_S(e)\mid e\in \delta_G(S)}$ of paths that are non-transversal with respect to $\Sigma$, routing the edges of $\delta_G(S)$ to $u(S)$ inside $S$; and
(ii) a vertex $u'(S)\notin V(S)$, and a set $\pset(S)=\set{P_S(e)\mid e\in \delta_G(S)}$ of paths that are non-transversal with respect to $\Sigma$, routing the edges of $\delta_G(S)$ to $u'(S)$ outside of $S$.
Denote $\qset=\bigcup_{S\in \lset}\qset(S)$, and $\pset=\bigcup_{S\in \lset}\pset(S)$.

We now construct a collection $\jset(\lset,\qset,\pset)$ of sub-instances of $I$, that we refer to as the \emph{disengagement of instance $I$ with respect to $\lset$ and path sets $\qset,\pset$}.

Consider now a cluster $S\in \lset$. Let $v(S)$ be the vertex representing $S$ in the partitioning tree $\tau(\lset)$ associated with $\lset$.
Let $v(S_1),\ldots,v(S_q)$ be the children of vertex $v(S)$ in $\tau(\lset)$, so clusters $S_1,\ldots,S_q$ are mutually vertex-disjoint subgraphs of $S$. 
We construct a sub-instance $J_S=(G_S,\Sigma_S)$ as follows.
The graph $G_S$ is obtained from $G$ by first contracting all vertices and edges of $G\setminus S$ into a super-node, that we denote by $v^{out}_S$, and then contracting, for each $1\leq i\leq q$, all vertices and edges of $S_i$ into a super-node, that we denote by $v^{in}_{S_i}$.
We denote $V'_S=V(S)\setminus \bigcup_{1\le t\le q}V(S_i)$,
so $V(G_S)=V'_S\cup\set{v_S^{out}}\cup\set{v_{S_1}^{in},\ldots,v_{S_q}^{in}}$.

We now define its rotation system $\Sigma_S$ as follows. 
Note that for every vertex $v\in V'_S$, $\delta_{G_S}(v)=\delta_{G}(v)$, and the ordering $\oset_v$ of the edges incident to $v$ remains the same as in $\Sigma$. 
For vertex $v^{out}_S$, note that $\delta_{G_S}(v^{out}_S)=\delta_G(S)$, and we define the ordering $\oset_{v^{out}_S}$ in $\Sigma_S$ to be the canonical ordering $\hat\oset(S,\qset(S))$. 
%\znote{make it a canonical ordering in prelim?}
For vertex $v^{in}_{S_i}$, note that $\delta_{G_S}(v^{in}_{S_i})=\delta_G(S_i)$, and we define the ordering $\oset_{v^{in}_{S_i}}$ in $\Sigma_S$ to be the canonical ordering $\hat\oset(S_i,\qset(S_i))$.
This completes the description of the instance $J_S=(G_S,\Sigma_S)$. See Figure~\ref{fig: disengaged_instance} for an illustration.
\begin{figure}[h]
	\centering
	\subfigure[Layout of graph $G$.]{\scalebox{0.13}{\includegraphics{figs/dis_instance_before}}\label{fig: graph G}}
	\hspace{1cm}
	\subfigure[The graph $G_S$.]{
		\scalebox{0.13}{\includegraphics{figs/dis_instance_after}}\label{fig: C and disc}}
	\caption{An illustration of the disengaged instance.\label{fig: disengaged_instance}}
\end{figure}

The main result of this subsection is the following lemmas.
\begin{lemma}
$\sum_{S\in \lset,S\ne G}\optcrors(G_S,\Sigma_S)\le $\znote{related to the depth of $\tau(\lset)$}.
\end{lemma} 
\begin{proof}
\znote{to complete}
\end{proof}

\begin{lemma}
There is an efficient algorithm, that, given, for each instance $J\in \jset(\lset,\qset,\qset')$, a solution $\phi(J)$, computes a solution for instance $I$ of value at most $\sum_{J\in \jset(\lset,\qset,\qset')}\cro(\phi(J))$.
\end{lemma} 
\begin{proof}
\znote{to complete}
\end{proof}





==> laminar_new.tex <==
\newpage

\section{Second Main Tool - Disengagement of Clusters}
\label{sec: not many paths}


%\input{basic_disengagement}

%\input{laminar_disengagement}

\input{disengagement_path}























\newpage

==> main-defs-backup.tex <==
\subsection{Main Definitions}
\label{subsec: main defs for interesting}


\iffalse
We start by defining $\tau^i$-wide and $\tau^s$-small instances; the former is a generalization of wide instances. 


\begin{definition}[$\tau^i$-Wide Instance]
Let $I=(G,\Sigma)$ be an instance of \cnwrs with $|E(G)|=m$, and let $\tau^i$ be a parameter. We say that $I$ is a  \emph{$\tau^i$-wide} instance, iff there is a vertex $v\in V(G)$, a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consequently in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$, and a collection $\pset$  of at least $\floor{m/\tau^i}$ simple edge-disjoint cycles in $G$, such that every cycle $P\in \pset$ contains one edge of $E_1$ and one edge of $E_2$.
If no such cycle set $\pset$ exists in $G$, then we say that $I$ is a \emph{$\tau^i$-narrow} instance.
\end{definition}



\begin{definition}[$\tau^s$-Small Instances]
	We say that a subinstance $I'=(G',\Sigma')$ of an instance $I=(G,\Sigma)$ of \cnwrs is \emph{$\tau^s$-small with respect to $I$}, for a parameter $\tau^s>0$, iff $|E(G')|\le |E(G)/\tau^s$.
\end{definition}


Note that \Cref{lem: many paths} requires that every instance $I'$ in the collection $\iset$ of subinstances of $\cI$ that we compute is either $\mu^{\thec}$-narrow, or it is $\mu$-small with respect to $\cI$.


In the remainder of this subsection, we assume that we are given some instance $I=(G,\Sigma)$ of \cnwrs, that we would like to decompose into a collection of instances that are either $\tau^i$-narrow or $\tau^s$-small with respect to $I$. In the first phase of our algorithm, we will let $I$ be the input instance $\cI$, and in the second phase of our algorithm, instance $I$ will be one of the subinstances computed in the first phase. We now define a skeleton graph for $I$, and a skeleton structure.
\fi



\subsubsection{Graph Skeleton and Skeleton Structure}


The first central notion that we use is a skeleton of a graph, and its associated skeleton structure.

\begin{definition}[Skeleton of a Graph]
Let $G$ be a graph, and let $K$ be a subgraph of $G$. We say that $K$ is a \emph{skeleton graph} for $G$ iff for every connected component $C$ of $K$, for every edge $e\in E(C)$, graph $C\setminus\set{e}$ is connected. In particular, $|E(C)|>1$ must hold. 
\end{definition}


\begin{definition}[Skeleton Structure]
A \emph{skeleton structure} for an instance $I=(G,\Sigma)$ of \cnwrs consists of:

\begin{itemize}
	\item a skeleton graph $K\subseteq G$;
	\item an orientation $b_u\in \set{-1,1}$ for every vertex $u\in V(K)$; and
	
	\item a planar drawing $\psi$ of $K$ on the sphere, that is consistent with the rotation system $\Sigma$ and the orientations in $\set{b_u}_{u\in V(K)}$. In other words, for every vertex $u\in V(K)$, the images of the edges of $\delta_K(u)$ enter the image of $u$ in $\psi$ according to their order in the rotation $\oset_u\in \Sigma$ and orientation $b_u$ (so, e.g. if $b_u=1$ then the orientation is counter-clock-wise).
\end{itemize}
\end{definition}



\subsubsection{Faces of Skeleton Structure and Edge Orderings}
\label{subsubsec: faces and orderings}


Consider now some skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for an instance $I=(G,\Sigma)$ of \cnwrs. Let $\fset(\kset)$ be the set of all faces in the drawing $\psi$ of $K$ on the sphere. Fix some face $F\in \fset(\kset)$. 
We denote by $\overline F$ the region of the sphere that is disjoint from the face $F$. We view $\overline F$ as an open region, so it does not contain the boundary of $F$.
We also denote by $\partial(F)$ the subgraph of $K$ consisting of all vertices and edges of $K$ that are drawn on the boundary of $F$. Note that graph $\partial(F)$ may not be connected, and we denote by $\cset(F)$ the set of all connected components of $\partial(F)$. 
Consider now any such connected component $C\in \cset(F)$. From the definition of the skeleton $K$, graph $C$ may not have separator edges. Therefore, we can decompose $C$ into a collection $\jset(C)$ of simple cycles, each of which is contained in $C$, such that: (i) $\bigcup_{C'\in \jset(C)}E(C')=E(C)$; (ii) the cycles in $\jset(C)$ do not share any edges; and (iii) if a vertex $v$ lies on more than one cycle of $\jset(C)$, then $v$ is a separator vertex for $C$. \mynote{should add figure depicting one such $C$}


\iffalse
Consider now any such connected component $C\in \cset(F)$. From the definition of the skeleton $K$, graph $C$ may not have separator edges. Let $(e_1,e_2,\ldots,e_r)$ be the sequence of the edges of $C$ in the order in which they are encountered as we traverse the boundary of $F$ along $C$. Note that every edge of $C$ appears exactly once in this sequence. It will be convenient for us to view each such connected component $C$ of $\partial(F)$ as a {\bf non-simple} cycle. From the above discussion, there is a collection $\jset(C)$ of simple cycles, each of which is contained in $C$, such that: (i) $\bigcup_{C'\in \jset(C)}E(C')=E(C)$; (ii) the cycles in $\jset(C)$ do not share any edges; and (iii) if a vertex $v$ lies on more than one cycle of $\jset(C)$, then $v$ is a separator vertex for $C$. We denote $\jset_F=\bigcup_{C\in \cset(F)}\jset(C)$.  For every cycle $C'\in \jset_F$, we define a disc $D(C')$, whose boundary is the image of $C'$ in $\psi$, and whose interior is disjoint from $F$. We denote by $D^0(C')$ the open disc obtained from $D(C')$ by removing its boundary. Lastly, we let $\dset(F)=\set{D^0(C')\mid C'\in \jset_F}$. Note that $\overline F=\bigcup_{C'\in \jset_F}D^0(C')$. We refer to the discs of $\dset(F)$ as \emph{forbidden discs for face $F$}. \mynote{to do later: do we need the cycles of $\jset_F$, and the forbidden discs? if so should we define them later? Also notation $\dset$ is not good because we used it for distributions.}
\fi

%\mynote{need to define an ordering of all edges of $E^F$}.
Consider now some vertex $u\in K$, and a tiny $u$-disc $D_{\psi}(u)$ in the drawing $\psi$. Denote $\delta_G(u)=\set{e^u_1,\ldots,e^u_{d_u}}$, where $d_u=\delta_G(u)$, and the edges are indexed according to their ordering in $\oset_u\in \Sigma$. We can then define a collection $p^u_1,\ldots,p^u_{d_u}$ of distinct points on the boundary of the disc $D_{\psi}(u)$, such that the following conditions hold:

\begin{itemize}
	\item when traversing the boundary of $D_{\psi}(u)$ in the direction consistent with the orientation $b_u$, then the points $p^u_1,\ldots,p^u_{d_u}$ are encountered in this order; and
	
	\item for every edge $e_i^u$ that lies in the skeleton $K$, point $p_i^u$ is the unique point on $\psi(e^u_i)$ lying on the boundary of $D_{\psi}(u)$.
\end{itemize}

For all $1\leq i\leq d_u$, we view point $p^u_i$ as representing the edge $e^u_i$. For all $1\leq i\leq d_u$, we draw a simple curve $\gamma^u_i$ connecting the image of $u$ in $\psi$ to point $p^u_i$, that is contained in $D_{\psi}(u)$, such that all resulting curves in $\set{\gamma^u_i\mid 1\leq i\leq d_u}$ are mutually disjoint, and, for every edge $e_i^u$ that lies in the skeleton $K$, the corresponding curve $\gamma^u_i$ is the segment of the image of $e_i^u$ in $\psi$ that is contained in $D_{\psi}(u)$. \mynote{should add a figure showing how these points and curves are computed, and color-code them according to which faces the edges belong to.}

Consider now any face $F\in \fset(\kset)$ with $u\in \partial(F)$. For every edge $e_i^u$, such that point $p_i^u$ lies in the interior of $F$, we say that edge $e_i^u$ \emph{belongs} to the face $F$. We denote by $E^F$ the set of all edges in $\bigcup_{u\in V(K)}\delta(u)$ that belong to face $F$. Note that the edges of $K$ may not belong to any face, and edge sets $\set{E^F\mid F\in \fset(\kset)}$ define a partition of the set $\left(\bigcup_{u\in V(K)}\delta(u)\right )\setminus E(K)$ of edges. 

Consider again some face $F\in \fset(\kset)$, and some connected component $C\in \cset(F)$ of $\partial(F)$. We denote by $E^F(C)\subseteq E^F$ the subset of edges $e\in E^F$ that are incident to vertices of $C$. Consider now a walk inside the face $F$, along the image of $C$, very close to it. We then let $\oset^F(C)$ be a circular ordering of the edges of $E^F(C)$, that is defined by the order in which we encounter the curves $\gamma_i^u$ that correspond to these edges on this walk.  \mynote{need to add a figure depicting the walk}




\subsubsection{Valid $F$-Subgraphs, Valid $F$-Subinstances, Clean Drawings, and Contracted Instances}

We are now ready to define subinstances of the input instance $I$ that are associated with faces of $\fset(\kset)$.

\begin{definition}[Valid $F$-Subgraph and Valid $F$-Subinstance]
Let $I=(G,\Sigma)$ be an instance of $\cnwrs$, and let $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ be a skeleton structure for $I$. Let $F$ be a face of $\fset(\kset)$, and let $G_F$ be a subgraph of $G$. We say that $G_F$ is a \emph{valid $F$-subgraph} of $G$ the following hold:

\begin{itemize}
	\item $\partial(F)\subseteq G_F$; and
	\item  every edge of $G_F$ that lies in $\left (\bigcup_{u\in V(K)}\delta_G(u)\right )\setminus E(K)$ belongs to $E^F$.
\end{itemize}  


We say that instance $I_F=(G_F,\Sigma_F)$ is a \emph{valid $F$-subinstance} of $I$ iff $G_F$ is a valid $F$-subgraph, and $\Sigma_F$ is the rotation system for $G_F$ that is induced by $\Sigma$.
\end{definition}

Given a valid $F$-subgraph $G_F$ of $G$, we call the vertices and edges of $\partial(F)\cap G_F$ \emph{boundary vertices and edges of $G_F$}, and we call remaining vertices and edges of $G_F$ \emph{inner vertices and edges}. Assume now that we are given a skeleton structure  $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for an instance $I=(G,\Sigma)$ of \cnwrs, and, for every face $F\in \fset(\kset)$, a valid $F$-subgraph $G_F$ of $G$.  We say that the graph in $\set{G_F\mid F\in \fset}$ are \emph{internally disjoint} from each other if no vertex of $G$ serves as an inner vertex of more than one such graph, and no edge of $G$ serves as an inner edge of more than one such graph. In other words, the only vertices and edges that the graphs of $\set{G_F\mid F\in \fset}$ may share are vertices and edges of $K$.


One of our main subroutines decomposes a single $F$-subinstance of the given instance $I$ into two subinstances. For this subroutine the parts of the sekelton $K$ that do not lie in $\partial(F)$ are irrelevant and can be ignored. Similarly, only the $F$-subinstance of the input graph $G$ is relevant to the decomposition procedure, and the remaining parts of $G$ can be ignored. In other words, we will assume that we are given an instance 
 $I=(G,\Sigma)$ of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, and a face  $F$ of $\fset(\kset)$, such that $I$ is a valid $F$-subinstance of $I$. This is equivalent to saying that every vertex and edge of $K$ lie in $\partial(F)$.



\paragraph{Clean and Dirty Drawings and Crossings.}
We will consider drawings of $F$-instances that have some special properties, that we now summarize.

\begin{definition}[Clean, Semi-Clean and Dirty Drawings]
Let $I=(G,\Sigma)$ be an instance of $\cnwrs$, let $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ a skeleton structure for $I$, and $F$ a face of $\fset(\kset)$. Consider a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$ and a solution $\phi$ to instance $I_F$. We say that $\phi$ is a \emph{semi-clean solution} iff the following hold:

\begin{itemize}
	\item the drawing of $\partial(F)$ induced by $\phi$ is identical to the drawing $\psi$ given by $\kset$; and
	
	\item the image of every vertex of $V(G_F)\setminus V(\partial(F))$  lies in the interior of $F$ in $\phi$ (where $F$ is defined with respect to the drawing $\psi$ of $\kset$).
\end{itemize}


If, additionally, the drawing of every edge of $G_F$ is contained in $F$, then we say that $\phi$ is a \emph{clean} solution to $I_F$. A solution that is neither clean nor semi-clean is called \emph{dirty}.
\end{definition}

Consider a semi-clean drawing $\phi$ of an $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$, and let $(e,e')_p$ be any crossing in this drawing. Since the drawing is semi-clean, it cannot be the case that both $e,e'\in \partial(F)$. We say that crossing $(e,e')_p$ is \emph{dirty} if exactly one of the two edges $e,e'$ lies in $\partial(F)$, and we say that it is \emph{clean} otherwise. We will denote by $\chi^{\dirty}(\phi)$ and by $\chi^{\clean}(\phi)$ the sets of all dirty and clean crossings in drawing $\phi$, respectively. Generally, we will consider semi-dirty solutions $\phi$ to $F$-instances $F$, in which $|\chi^{\dirty}(\phi)|$ is quite small. This will ensure that the number of crossings $(e,e')_{p}$ in the drawing $\phi$, where point $p$ lies outside of $F$, is also small. Indeed, for each such crossing $(e,e')_{p}$, the images of both edges $e$ and $e'$ must cross the image of $\partial(F)$ (since the endpoints of the edges $e,e'$ are drawn in the interior of $F$). Therefore, in order to bound $\cro(\phi)$, we will focus on crossings $(e,e')_{p}$ with $p\in F$. We denote by $\cro^*(\phi)$ the total number of crossings $(e,e')_{p}$ of $\phi$, where the crossing point $p$ lies in $F$.




\paragraph{Contracted $F$-instance.}
Assume that we are given an instance $I=(G,\Sigma)$ of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in\kset)$, and a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$. We now define the \emph{contracted} $F$-instance $\hat I_F=(\hat G_F,\hat \Sigma_F)$ corresponding to instance $I_F$. Graph $\hat G_F$ is obtained from graph $G_F$, by contracting, for every connected component $C\in \cset(F)$ of $\partial(F)$, all vertices of $C$ into a supernode $v_C$.  In order to define the rotation system $\hat \Sigma_F$, for every vertex $u\in V(\hat G_F)\cap V(G_F)$, we let the rotation $\oset_u$ remain the same as in $\Sigma$, and for every supernode $v_C$ (where $C\in \cset(F)$), we set the corresponding rotation $\oset_{v_C}$ to be the ordering of the edges of $\delta_{\hat G_F}(v_C)\subseteq E^F(C)$ induced by $\oset^F(C)$ -- the ordering of the edges of $E^F(C)$ that we have defined in \Cref{subsubsec: faces and orderings}.

We need the following simple observation.
\begin{observation}\label{obs: clean solution to contracted}
	There is an efficient algorithm, whose input is an instance $I=(G,\Sigma)$ of \cnwrs, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F$ of $\fset(\kset)$,  a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$, and a clean solution $\phi$ to instance $I_F$. The output of the algorithm is a solution $\phi'$ to the corresponding contracted $F$-instance $\hat I_F$, with $\cro(\phi')\leq \cro(\phi)$.
	\end{observation}

\begin{proof}
	Consider the solution $\phi$ to instance $I_F$.
	For every connected component $C\in \cset(F)$, we draw a disc $D(C)$ that contains the image of  $C$ in its interior, such that the only vertices of $G_F$ whose image lies in $D(C)$ are the vertices of $C$, and the only edges whose images intersect $D(C)$ are edges of $E(C)\cup E^F(C)$. \mynote{should add figure depicting the disc} We additionally ensure that no crossing of $\phi$ is contained in $D(C)$, and that, for every edge $e\in E^F(C)$, the intersection of $\phi(e)$ with $D(C)$ is a contiguous segment of $\phi(e)$. For every edge $e\in E^F(C)$, denote by $p_e$ the unique point on the boundary of $D(C)$ that lies on $\phi(e)$. From the definition of the ordering $\oset^F(C)$ of the edges of $E^F(C)$, it is immediate to verify that the circular ordering of the points of $\set{p_e\mid e\in E^F(C)}$ along the boundary of $D(C)$ is precisely $\oset^F(C)$. For each edge $e\in E^F(C)$, we erase the segment of $\phi(e)$ that is contained in $D(C)$. We then contract the disc $D(C)$ into a single point, that becomes the image of the supernode $v_C$. Once every connected component $C\in \cset(F)$ is processed, we obtain a valid solution $\phi'$ to the contracted $F$-instance $\hat I_F$, with $\cro(\phi')\leq \cro(\phi)$.
\end{proof}

We note that the converse of the above observation is also true: given a solution $\hat \phi$ to a contracted $F$-instance $\hat I_F$, we can efficiently construct a clean solution $\phi$ to instance $I_F$, with $\cro(\phi)\leq \cro(\hat \phi)$, by simply un-contracting the supernodes, and replacing each supernode $v_C$ with the corresponding graph $C\in \cset(F)$.


\subsubsection{Skeleton Augmentation}
\label{subsubsec: sekelton augmentation}

Our main partitioning subroutine starts with a valid $F$-instance $I_F=(G_F,\Sigma_F)$, and splits it into two subinstances. This is done by first augmenting the skeleton structure, that will result in the face $F$ being partitioned into two new faces $F_1$ and $F_2$. 
Instance $I_F$ is then split into a valid $F_1$ instance and a valid $F_2$-instance. We now define an augmentation of a skeleton structure. We will use two different types of augmentation. The algorithm for Phase 1 will use all of them, and the algorithm for Phase 2 will only use the last two types.
In order to simplify the notaton and reduce the number of types of augmentations, we will sometimes refer to simple cycles as paths. Given such a simple cycle $W$, we will designate one of the vertices $v\in W$ to be the ``endpoint'' of the path. When referring to two endpoints of the path $W$, we will think of both endpoints being $v$.



\begin{definition}[$F$-Augmentation of a Skeleton Structure]
	Given an  instance $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in \fset(\kset)$, and a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$, an \emph{$F$-augmentation} of the skeleton structure $\kset$ is one of the following:
	
	\begin{itemize}
		\item (type-1 augmentation): a simple cycle $P\subseteq G_F$, that is disjoint from $\partial(F)$; or
%		\item (type-2 augmentation): a simple cycle $W$ of $G_F$, such that $|V(W)\cap V(\partial(F))|= 1$; or
		\item (type-2 augmentation): a simple path $P\subseteq G_F$, such that the endpoints of $P$ are distinct vertices that belong to the same connected component of $\partial(F)$, while all inner vertices of $P$ are disjoint from $\partial(F)$; or
		\item (type-3 augmentation): two internally disjoint paths $P_1$, $P_2$, such that all inner vertices of $P_1$ and of $P_2$ are disjoint from $\partial(F)$, and there are two distinct connected components $C,C'\in \partial(F)$, with $P_1$ and $P_2$ each connecting a vertex of $C$ to a vertex of $C'$.
	\end{itemize}
\end{definition}

We note that a type-2 augmnetation may be a cycle, in which case the two endpoints of the path are identical and lie on $\partial(F)$.


\mynote{would be good to add figures showing all four types}



In order to simplify the notation, we will always think of an $F$-augmentation as a pair $\Pi_F=\set{P^*_1,P^*_2}$ of internally disjoint paths, whose inner vertices are disjoint from $\partial(F)$. In case of type-1 augmentation, we can partition the cycle $W$ into two paths; if some vertex $v\in V(W)$ lies in $\partial(F)$, we can define the partition so that $v$ is an endpoint of both paths. In case of a type-2 augmentation, we can either split path $P$ into two internally disjoint subpaths, or, if path $P$ consists of a single edge, let $P_1=P$ and $P_2$ consist of a single vertex that is an endpoint of $P_1$.



%-------------------------------
%-------------------------------
%-------------------------------

 We will use the $F$-augmentation $\Pi_F$ in order to augment the skeleton $K$. Additionally, we will also need to augment the corresponding skeleton structure. The next definition allows us to do so.




\begin{definition}[$F$-Augmenting Structure]
	Given an  instance $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in \fset(\kset)$, and a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$, an \emph{$F$-augmenting structure} for the skeleton structure $\kset$ consists of:
	
	\begin{itemize}
		\item an $F$-augmentation $\Pi_F=\set{P^*_1,P^*_2}$;
		\item for every vertex $u\in (V(P^*_1)\cup V(P^*_2))\setminus V(K)$, an orientation $b_u\in \set{-1,1}$; and
		\item a drawing $\psi'$ of the graph $K\cup P^*_1\cup P^*_2$ on the sphere with no crossings, such that $\psi'$ is consistent with the rotation system $\Sigma$ and the orientations in $\set{b_u}_{u\in V(K\cup P^*_1\cup P^*_2)}$, and the drawing of $K$ induced by $\psi'$ is precisely $\psi$.
	\end{itemize}
\end{definition}


We can use an $F$-augmenting structure $\aset=(\Pi_F=\set{P^*_1,P^*_2},\set{b_u}_{u\in V(K\cup P^*_1\cup P^*_2)}, \psi')$ in order to obtain a new skeleton structure $\kset'=(K',\set{b'_u}_{u\in V(K')},\psi')$, where $K'=K\cup P^*_1\cup P^*_2$, for every vertex $u\in V(K)$, its new orientation $b'_u$ remains the same as orientation $b_u$ in $\kset$, and for every other vertex $u$ of $K'$, its orientation $b'_u$ is the same as the orientation $b_u$ given by the augmenting structure $\aset$. Drawing $\psi'$ of $K'$ is the same as the drawing given by the augmenting structure $\aset$. We denote $\kset'=\kset^{+\aset}$, and we say that $\kset'$ is \emph{obtained by augmenting $\kset$ via $\aset$}.
Note that in drawing $\psi'$ there are now two distinct faces, that we denote by $F_1$ and $F_2$, whose union is $F$. 

\subsubsection{A Split of an $F$-Instance}
We now define a \emph{split} of instance $I_F$ along an augmenting structure $\aset$.

\begin{definition}[A Split of an $F$-Instance]
Suppose we are given  an instance $I=(G,\Sigma)$  of $\cnwrs$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\psi)$ for $I$, a face $F\in \fset(\kset)$, and a valid $F$-subinstance $I_F=(G_F,\Sigma_F)$ of $I$. Assume further that we are given an $F$-augmenting tructure $\aset$, and denote by $\kset'=\kset^{+\aset}$ the skeleton structure obtained by augmenting $\kset$ via $\aset$. Let $F_1$ and $F_2$ be the two faces of $\psi'$ that are contained in the face $F$ of $\psi$. A \emph{split} of $I_F$ along augmenting structure $\aset$ is a pair $I_{F_1}=(G_{F_1},\Sigma_{F_1}), I_{F_2}=(G_{F_2},\Sigma_{F_2})$ of instances of \cnwrs, for which the following hold.
	\begin{itemize}
		\item $I_{F_1}$ is a valid $F_1$-subinstance of $I$, and $I_{F_2}$ is a valid $F_2$-subinstance of $I$, for skeleton structure $\kset'$;
		\item $E(G_{F_1})\cup E(G_{F_2})\subseteq E(G)$; and
		\item graphs $G_{F_1}$ and $G_{F_2}$ are internally disjoint. In other words, they may only share vertices and edges of $\partial(F_1)\cap \partial(F_2)$.
	\end{itemize}
\end{definition}


Notice that some edges of graph $G_F$ may not lie in $E(G_{F_1})\cup E(G_{F_2})$. We informally refer to such edges as \emph{deleted edges}, and we will sometimes denote the set of such deleted edges by $E^{\del}$. Typically we will ensure that $|E^{\del}|$ is quite small.

The following observation shows that clean solutions to instances $I_{F_1}$ and $I_{F_2}$ can be combined to obtain a clean solution to instance $I_F$. The proof is deferred to Section \ref{subsec: combine solutions for split} of Appendix.

\begin{observation}\label{obs: combine solutions for split}
	There is an efficient algorithm, that, given a split $(I_{F_1},I_{F_2})$ of an $F$-instance $I_F$ along an augmenting structure $\aset$, a clean solution $\phi_1$ to instance $I_{F_1}$ and a clean solution $\phi_2$ to instance $I_{F_2}$, produces a clean solution $\phi$ to instance $I_F$, with $\cro(\phi)\leq \cro(\phi_1)+\cro(\phi_2)+|E^{\del}|\cdot |E(G_F)|$, where $E^{\del}=E(G_F)\setminus (E(G_{F_1})\cup E(G_{F_2})$.
\end{observation}


\subsubsection{Auxiliary Claim}



We will use the following simple auxiliary claim several times. The proof is  similar to the proof of Claim 9.9 in \cite{chuzhoy2020towards} and is deferred to Section \ref{subsec: curves orderings crossings} of Appendix.

\begin{claim}\label{claim: curves orderings crossings}
	Let $I=(G,\Sigma)$ be an instance of \cnwrs, and let $\pset=\set{P_1,\ldots,P_{4k+2}}$ be a collection of directed edge-disjoint paths in $G$, that are non-transversal with respect to $\Sigma$. For all $1\leq i\leq 4k+2$, let $e_i$ be the first edge on path $P_i$. Assume that there are two distinct vertices $u,v\in V(G)$, such that all paths in $\pset$ originate at $u$ and terminate at $v$, and assume further that
	edges $e_1,\ldots,e_{4k+2}$ appear in this order in the rotation $\oset_u\in \Sigma$. Lastly, let $\phi$ be any solution to instance $I$, such that the number of crossings $(e,e')_p$ in $\phi$ with $e$ or $e'$ lying in $E(P_1)$ is at most $k$, and assume that the same is true for $E(P_{2k+1})$. Then $\phi$ does not contain a crossing between an edge of $P_1$ and an edge of $P_{2k+1}$.
\end{claim}



==> many_paths-backup2.tex <==
\newpage

\section{An Algorithm for Interesting Subinstances -- Proof of \Cref{lem: many paths}}
\label{sec: many paths}


\input{interesting-intuition}

\newcommand{\ttoo}{\tilde \oset}

\iffalse
Here is a suggested plan.

\begin{itemize}
	\item Given an instance $G'$ on $m'$ edges, and parameters $\tau^s,\tau^i$, define the notion of $\tau^s$-small and $\tau^i$-wide/narrow subinstances of $G$.
	
	\item Define well-structured subinstances and corresponding contracted instances.
	
	\item Define well-structured solutions (maybe call them near-perfect solutions?) 
	
	\item Main theorem: efficient randomized algorithm that computes a collection $\iset$ of subinstances of a given instance $I'=(G',\Sigma')$, such that every instance in $\iset$ is well-structured, and its corresponding contracted instance is either $\tau^s$-small or $\tau^i$-narrow. For each edge of $G'$, if it is special, it lies in at most two of the instances and if it is non-special it lies in at most one instance. There exists a well-structured solution for each subinstance such that the total cost of these solutions is small. (my guess you can just ensure that all these hold with probability $(1-1/\mu)$ or so?)
\end{itemize}

For now you may want to focus on the above, which is the main tool that we use. We will then use the theorem slightly differently in Phase 1 and Phase 2, but at least we won't need to write the same algorithm twice.



\mynote{to do: introduce parameters $\tau^s,\tau^i$. Define instance $\tau^s$-small and $\tau^i$-wide. Do the decomposition w.r.t. these parameters, so that we could reuse this in second stage. This is from my email from June 1: 
-say that an instance is $\tau^i$-wide iff there is a set of $m/\tau^i$ of paths connecting 2 vertices (or one vertex with nested cycles). (I think it’s worth it to give a name to this set of paths, say $\tau^i$-wide set of paths, of type 1 or of type 2).
-say that an instance is $\tau^s$-small iff it contains fewer than $m/\tau^s$ edges.
The claim that you are making: start with a cycle-based instance, and assume that it contains at least x cycles. We can compute another collection of cycle-based subinstances, such that each corresponding contracted instance is either $\tau^i$-wide, or $\tau^s$-small. 
(Note: for phase 2 decomposition, the instance that we start decomposing already has some cycles, which is why I want to set it up this way, it shouldn’t make much difference for your part).}
%\znote{parameters subject to change, so I am omitting constant factors in (big-O notation of) some probability value}

%\mynote{this is copied from the log, needs to be improved. One thing to pay attention to: what probability of success can we guarantee?}
\fi

In this section we provide the proof of  \Cref{lem: many paths}. 
Recall we are given a wide subinstance $I=(G,\Sigma)$ of $I^*$, the input instance to the \CNwRS problem, such that $|E(G)|>\mu^{100\interestconst}$ and $\optcrors(I)<|E(G)|^2/\mu^{100\interestconst}$.
For convenience, throughout this section, we rename the instance $I$ (the input instance in \Cref{lem: many paths}) by $\check I=(\check G,\check \Sigma)$ and denote $\check m=|E(\check G)|$.
%Recall that parameter $\mu=2^{O((\log m^*)^{7/8}\log\log m^*)}$ where $m^*$ is the number of edges in the input instance $I^*=(G^*,\Sigma^*)$ to the \cnwrs problem.
%We will compute a set of subinstances of $I$ that satisfy all required properties in \Cref{lem: many paths}.
%
\iffalse{previous wide notion recall}
Recall that, in a wide subinstance $I$, there exists a collection $\pset$ of at least $m/\mu^{\interestconst}$ edge-disjoint paths in $G$, that is also called a witness of instance $I$, such that either 
\begin{properties}{I}
\item there are two vertices $v',v''\in V(G)$, such that every path in $\pset$ originates at $v'$ and terminates at $v''$; or
\label{Case_1 many_path}
\item there is a single vertex $v\in V(G)$, and two disjoint subsets $E_1,E_2$ of edges of $\delta_{G}(v)$, such that the edges of $E_1$ appear consecutively in the ordering $\oset_v\in \Sigma$, and so do the edges of $E_2$, and every path in $\pset$ contains an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
\label{Case_2 many_path}
\end{properties}
\fi

%\znote{overview here}


We start with the following definitions.

\begin{definition}[$\tau^i$-wide subinstances]
Let $I=(G,\Sigma)$ be a subinstance of $\check I$ with $|E(G)|=m$. Let $\tau^i>0$ be an integer.  
We say that $I$ is a \emph{$\tau^i$-wide} subinstance of $\check I$, iff there exists a collection $\pset$ of at least $\floor{m/\tau^i}$ edge-disjoint paths in $G$, that is also called a \emph{witness} of instance $I$, such that either 
\begin{itemize}
	\item there are two vertices $v',v''\in V(G)$, such that every path in $\pset$ originates at $v'$ and terminates at $v''$; or
	\label{Case_1 many_path}
	\item there is a single vertex $v\in V(G)$, and two disjoint subsets $E_1,E_2$ of edges of $\delta_{G}(v)$, such that the edges of $E_1$ appear consecutively in the ordering $\oset_v\in \Sigma$, and so do the edges of $E_2$, and every path in $\pset$ contains an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
	\label{Case_2 many_path}
\end{itemize}
We say that the instance $I$ is \emph{$\tau^i$-narrow} iff $I$ is not $\tau^i$-wide.
\end{definition}



\begin{definition}[Small subinstances]
We say that a subinstance $I=(G,\Sigma)$ of $\check I$ is $\tau^s$-small for some integer $\tau^s>0$, iff $|E(G)|\le \tau^s$.
\end{definition}











\subsection{Well-Structured Subinstances, Well-Structured Solutions and a Decomposition Lemma}

\znote{maybe we need the notion "boundary of a face" $\partial F$ back in the prelim}

\paragraph{Well-Structured subinstances and contracted subinstances.} 
We say that a subinstance $I=(G,\Sigma)$ of the input instance $\check I$ is \emph{well-structured}, iff $G$ is a subgraph of $\check G$, and we are given 
\begin{itemize}
\item a $2$-connected subgraph $K$ of $G$, called the \emph{skeleton} of $I$;
\item a planar drawing $\rho$ of $K$ in the sphere (we denote by $\fset$ the set of faces in $\rho$).
\item a collection $\gset=\set{G_F}_{F\in \fset}$ of subgraphs of $G$, where each subgraph $G_F\in \gset$ is indexed by a face $F\in\fset$, such that
\begin{itemize}
\item each vertex $v\notin V(K)$ belongs to exactly one subgraphs in $\gset$;
\item for each vertex $v\in V(K)$ and each face $F\in \fset$, subgraph $G_F$ contains vertex $v$ iff $v$ lies on the boundary of face $F$ (namely $v\in \partial F$);
\item for each face $F\in \fset$ and each vertex $v\in \partial F$, if we denote by $e,e'$ the edges of $\partial F$ incident to $v$, then edges of $\delta_{G_F}(v)$ must be consecutive in the circular ordering $\oset_v\in \Sigma$ and must lie between $e$ and $e'$. Specifically, if $\delta_G(v)=\set{e,e_1,\ldots,e_s,e',e'_1,\ldots,e'_t}$, where the other edges are indexed according to $\oset_v$, then either $\delta_{G_F}(v)=\set{e_1,\ldots,e_s}$ or $\delta_{G_F}(v)=\set{e'_1,\ldots,e'_t}$. 
\end{itemize}
\end{itemize}

We call the tuple $(K,\rho,\fset,\gset)$ the \emph{structure} of instance $I=(G,\Sigma)$.
Additionally, we call edges of $K$ \emph{special edges} of instance $I$.

%Let $I=(G,\Sigma)$ be a well-structured subinstance with skeleton $K$, planar drawing $\rho$ of $K$ with face sets $\fset$, and the collection $\gset$ of subgraphs. 
Let $F$ be a face in $\fset$. We define the subinstance $I_F=(G_F,\Sigma_F)$, where the rotation system $\Sigma_F$ is induced by $\Sigma$.
We define the subinstance $\tilde I_F=(\tilde G_F,\tilde \Sigma_F)$ as follows. Since skeleton $K$ is $2$-connected and $F$ is a face in a planar drawing of $K$, graph $\partial F$ is the union of a set of vertex-disjoint cycles.
We denote by $\rset(F)$ the set of vertex-disjoint cycles in $\partial F$.
Graph $\tilde G_F$ is obtained from $G_F$ by contracting, for each cycle $R$ in $\rset(F)$, all vertices of $R$ into a supernode, which we denote by $v_R$, so $V(\tilde G)=(V(G)\setminus V(\partial F))\cup \set{v_R\mid R\in \rset(F)}$. 
We now define the rotation system $\tilde \Sigma_F$.
Note that, for every vertex $v\in V(G)\setminus V(\partial F)$, $\delta_{\tilde G_F}(v)=\delta_{\tilde G}(v)$, and we define the ordering $\ttoo_v$ in $\tilde \Sigma$ to be $\oset_v$, the ordering on vertex $v$ in $\Sigma$. It remains to define the orderings $\set{\ttoo_{v_{R}}\mid R\in \rset(F)}$. Consider a cycle $R\in \rset(F)$ with $R=(v_0,v_1,\ldots,v_{s-1},v_0=v_s)$. For each $0\le i\le s-1$, we denote by $e_i$ the edge in $R$ connecting $v_i$ to $v_{i+1}$, and we denote $\delta_{G_F}(v_i)=\set{e_{i-1}, e^i_1,\ldots,e^i_{d_i},e_i}$, where the edges are indexed according to the ordering $\oset_{v_i}$ in $\Sigma$. From the definition of graph $\tilde G_F$, 
$$\delta_{\tilde G}(v_R)=\bigg(\bigcup_{0\le i\le s-1}\delta_{G_F}(v_i)\bigg)\setminus E(R)=\set{e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}}.$$ We then define the ordering $\ttoo_{v_{R}}$ to be
$e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}$. This completes the definition of instance $\tilde I_F$. We call $\tilde I_F$ the 
\emph{contracted subinstance} of $I_F$.

\paragraph{Well-Structured solutions.}
Let $I=(G,\Sigma)$ be a well-structured instance with structure $(K,\rho,\fset,\gset)$. We say that a solution $\phi$ of instance $I$ is a \emph{well-structured solution} (or a \emph{well-structured drawing}) for $I$, iff
\begin{properties}{P}
\item the drawing of $K$ induced by drawing $\phi$ is identical to $\rho$;
\item for each face $F\in \fset$,
\begin{itemize}
\item all vertices of $G_F\setminus \partial F$ are drawn in the interior of face $F$;
\item for each edge $e\in (G_F\setminus F)$ that is incident to some vertex $v\in F$, the intersection of image of $e$ and the tiny $v$-disc $D_{\phi}(v)$ is entirely contained in face $F$;
and
\end{itemize} 
\item the number of edges that crosses a special edge of $I$ in $\phi$ is at most $\cro(\phi)\cdot (\tau^i)^{10}/|E(G)|$.
\label{prop: niubi edge crossing special cycle}
\end{properties}
%We say that a solution $\phi$ for instance $I$ is \emph{almost well-structured} iff it satisfies properties \ref{prop: simple curve}--\ref{prop: first segments}.


\newcommand{\delE}{E^{\sf del}}
\newcommand{\ws}{well-structured\xspace}

The main result in this subsection is the following lemma.

\znote{parameters to be determined.}

\begin{lemma}
\label{lem: many path main}
There is an efficient randomized algorithm, that given a well-structured subinstance $I=(G,\Sigma)$ of $\check I$, with structure $(K,\rho,\fset,\gset)$, for which there exists a \ws drawing $\phi$, computes a well-structured subinstance $I'=(G',\Sigma)$ of $\check I$ with structure $(K',\rho',\fset',\gset')$, such that
\begin{properties}{C}
\item $G'\subseteq G$, $K\subseteq K'$, and the drawing of $K$ induced by $\rho'$ is identical to $\rho$;
\item for each face $F'\in \fset'$, the contracted subinstance $\tilde I'_F$ is either $\tau^s$-small or $\tau^i$-narrow;
\label{prop: well-structured and contracted}
\end{properties}
and moreover, with probability $1-O(1/\mu^{\smallprobability})$,
\begin{properties}[2]{C}
\item $|E(G)\setminus E(G')|\le \cro(\phi)\cdot \poly(\mu)/|E(G)|$; 
\label{prop: few deleted edges}
\item for each face $F$ and each edge $e\in G_F$, the segment(s) of curve $\phi(e)$ that lies outside face $F$ is identical to the segment(s) of curve $\phi'(e)$ that lies outside face $F$.
\label{prop: forbidden discs}
\item if $\cro(\phi)\le m^2/\mu^{c}$ for some large enough constant $c>0$, then there exists a well-structured solution $\phi'$ for $I'$, such that $\cro(\phi')\le O(\cro(\phi))$.
\label{prop: number of crossings}
\end{properties}
%\znote{do we have this?} 
Moreover, there is an efficient algorithm $\alg(I')$, that given, for each face $F'\in \fset'$, a feasible solution $\phi(\tilde I'_F)$ to the contracted instance $\tilde I'_F$, computes a well-structured solution $\phi(I')$ for instance $I'$, of cost 
$\cro(\phi(I'))\leq O\big(\sum_{F'\in \fset'}\cro(\phi(\tilde I'_F)\big)$.
\end{lemma}

The remainder of this subsection is dedicated to the proof of \Cref{lem: many path main}.

%The algorithm is randomized and consists of two phases. In the first phase, the algorithm will return FAIL with probability $O(1/\mu^{\smallprobability-\interestconst})$, and if it does not return FAIL, it will compute a collection $\iset$ of subinstances of the input instance $I=(G,\Sigma)$, and a set $E^{\sf del}$ of edges in $G$, such that, if we denote by $\tilde \iset$ the set of all contracted subinstances for instances in $\iset$, then with probability $O(1/\mu^{\smallprobability-\interestconst})$,

\iffalse
\begin{properties}{C}
\item each instance $I'\in \iset$ is a well-structured subinstance;
\label{prop: well-structured instances}
\item for each contracted instance $\tilde I'=(\tilde G',\tilde\Sigma') \in \tilde \iset$, either $\tilde I'$ is non-wide, or $|E(\tilde G')|\le m/\mu$;\label{prop: no longer wide}
\item the sets $\set{\hat E(I')\mid I'\in \iset}$ of edges are mutually disjoint;\label{prop: private edges disjoint}
\item $|E^{\sf del}|\le \cro\cdot\mu^{O(\interestconst)}/m$, and edges of $E^{\sf del}$ does not belong to any instance of $\iset$;\label{prop: few deleted edges in phase 1}
\item every edge of $E(G)\setminus \bigg(E^{\sf del}\cup \big(\bigcup_{I'\in \iset}\hat E(I')\big)\bigg)$ is a special edge of exactly two instances in $\iset$;\label{prop: few edges}
\item there exists, for every instance $I'\in \iset$, a well-structured solution $\phi_{I'}$, such that\\
$\expect[]{\sum_{I'\in \iset}\optcrors(I')}\le \left (\optcrors(I)+|E(G)|\right )\cdot \nu$; and \label{prop: small solution cost}
\item there is an efficient algorithm $\alg(\iset)$, that, given, for each contracted instance $\tilde I' \in \tilde\iset$, a feasible solution $\phi(\tilde I')$, computes a feasible solution $\phi$ for instance $I$, of cost $\cro(\phi^*)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$. \label{prop: alg to put together}
\end{properties}
\znote{to modify the properties?}


In the second phase, we will compute, for each instance $I'\in \iset$, a new instance $I''$ obtained from $I'$ by deleting a set of edges from $I'$, such that
\znote{to add more properties}
\fi

\input{many_paths_main_decomposition}

\input{many_paths_main_decomposition_analysis}



==> many_paths_backup.tex <==
\newpage

\section{An Algorithm for Interesting Subinstances -- Proof of \Cref{lem: many paths}}
\label{sec: many paths}

\newcommand{\ttoo}{\tilde \oset}

\iffalse
Here is a suggested plan.

\begin{itemize}
	\item Given an instance $G'$ on $m'$ edges, and parameters $\tau^s,\tau^i$, define the notion of $\tau^s$-small and $\tau^i$-wide/narrow subinstances of $G$.
	
	\item Define well-structured subinstances and corresponding contracted instances.
	
	\item Define well-structured solutions (maybe call them near-perfect solutions?) 
	
	\item Main theorem: efficient randomized algorithm that computes a collection $\iset$ of subinstances of a given instance $I'=(G',\Sigma')$, such that every instance in $\iset$ is well-structured, and its corresponding contracted instance is either $\tau^s$-small or $\tau^i$-narrow. For each edge of $G'$, if it is special, it lies in at most two of the instances and if it is non-special it lies in at most one instance. There exists a well-structured solution for each subinstance such that the total cost of these solutions is small. (my guess you can just ensure that all these hold with probability $(1-1/\mu)$ or so?)
\end{itemize}

For now you may want to focus on the above, which is the main tool that we use. We will then use the theorem slightly differently in Phase 1 and Phase 2, but at least we won't need to write the same algorithm twice.



\mynote{to do: introduce parameters $\tau^s,\tau^i$. Define instance $\tau^s$-small and $\tau^i$-wide. Do the decomposition w.r.t. these parameters, so that we could reuse this in second stage. This is from my email from June 1: 
-say that an instance is $\tau^i$-wide iff there is a set of $m/\tau^i$ of paths connecting 2 vertices (or one vertex with nested cycles). (I think it’s worth it to give a name to this set of paths, say $\tau^i$-wide set of paths, of type 1 or of type 2).
-say that an instance is $\tau^s$-small iff it contains fewer than $m/\tau^s$ edges.
The claim that you are making: start with a cycle-based instance, and assume that it contains at least x cycles. We can compute another collection of cycle-based subinstances, such that each corresponding contracted instance is either $\tau^i$-wide, or $\tau^s$-small. 
(Note: for phase 2 decomposition, the instance that we start decomposing already has some cycles, which is why I want to set it up this way, it shouldn’t make much difference for your part).}
%\znote{parameters subject to change, so I am omitting constant factors in (big-O notation of) some probability value}

%\mynote{this is copied from the log, needs to be improved. One thing to pay attention to: what probability of success can we guarantee?}
\fi

In this section we provide the proof of  \Cref{lem: many paths}. 
Recall we are given a wide subinstance $I=(G,\Sigma)$ of $I^*$, the input instance to the \CNwRS problem, such that $|E(G)|>\mu^{100\interestconst}$ and $\optcrors(I)<|E(G)|^2/\mu^{100\interestconst}$.
For convenience, throughout this section, we rename the instance $I$ (the input instance in \Cref{lem: many paths}) by $\check I=(\check G,\check \Sigma)$ and denote $\check m=|E(\check G)|$.
%Recall that parameter $\mu=2^{O((\log m^*)^{7/8}\log\log m^*)}$ where $m^*$ is the number of edges in the input instance $I^*=(G^*,\Sigma^*)$ to the \cnwrs problem.
%We will compute a set of subinstances of $I$ that satisfy all required properties in \Cref{lem: many paths}.
%
\iffalse{previous wide notion recall}
Recall that, in a wide subinstance $I$, there exists a collection $\pset$ of at least $m/\mu^{\interestconst}$ edge-disjoint paths in $G$, that is also called a witness of instance $I$, such that either 
\begin{properties}{I}
\item there are two vertices $v',v''\in V(G)$, such that every path in $\pset$ originates at $v'$ and terminates at $v''$; or
\label{Case_1 many_path}
\item there is a single vertex $v\in V(G)$, and two disjoint subsets $E_1,E_2$ of edges of $\delta_{G}(v)$, such that the edges of $E_1$ appear consecutively in the ordering $\oset_v\in \Sigma$, and so do the edges of $E_2$, and every path in $\pset$ contains an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
\label{Case_2 many_path}
\end{properties}
\fi

%\znote{overview here}


We start with the following definitions.

\begin{definition}[$\tau^i$-wide subinstances]
Let $I=(G,\Sigma)$ be a subinstance of $\check I$ with $|E(G)|=m$. Let $\tau^i>0$ be an integer.  
We say that $I$ is a \emph{$\tau^i$-wide} subinstance of $\check I$, iff there exists a collection $\pset$ of at least $\floor{m/\tau^i}$ edge-disjoint paths in $G$, that is also called a \emph{witness} of instance $I$, such that either 
\begin{itemize}
	\item there are two vertices $v',v''\in V(G)$, such that every path in $\pset$ originates at $v'$ and terminates at $v''$; or
	\label{Case_1 many_path}
	\item there is a single vertex $v\in V(G)$, and two disjoint subsets $E_1,E_2$ of edges of $\delta_{G}(v)$, such that the edges of $E_1$ appear consecutively in the ordering $\oset_v\in \Sigma$, and so do the edges of $E_2$, and every path in $\pset$ contains an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
	\label{Case_2 many_path}
\end{itemize}
We say that the instance $I$ is \emph{$\tau^i$-narrow} iff $I$ is not $\tau^i$-wide.
\end{definition}



\begin{definition}[Small subinstances]
We say that a subinstance $I=(G,\Sigma)$ of $\check I$ is $\tau^s$-small for some integer $\tau^s>0$, iff $|E(G)|\le \tau^s$.
\end{definition}











\subsection{Well-Structured Subinstances, Well-Structured Solutions and a Decomposition Lemma}



\paragraph{Well-Structured subinstances and their contracted subinstances.} 
We say that a subinstance $I=(G,\Sigma)$ of the input instance $\check I$ is \emph{well-structured}, iff $G$ is a subgraph of $\check G$, and there is a set $\rset$ of edge-disjoint cycles in graph $G$, called the \emph{set of special cycles} of $I$, such that, for each cycle $R\in \rset$, if we denote $R=(v_0,v_1,v_2,\ldots,v_{s-1},v_{s})$ (where $v_{s}=v_0$) and denote, for each index $0\le i\le s-1$, by $e_i$ the edge of $R$ connecting $v_i$ to $v_{i+1}$, then for each $i$, edges $e_{i-1},e_i$ appear consecutively in the ordering $\oset_{v_i}\in \Sigma$ (we use the convention that $e_s=e_0$).
%We denote $\hat E(I)=E(G)\setminus E(\rset)$. 
We call edges of special cycles in $\rset$ \emph{special edges} of instance $I$.

Let $I=(G,\Sigma)$ be a well-structured subinstance of $\check I$ with $\rset$ being its set of special cycles. We define the subinstance $\tilde I=(\tilde G,\tilde \Sigma)$ as follows.
Graph $\tilde G$ is obtained from $G$ by contracting, for each cycle $R\in \rset$, all vertices of $R$ into a supernode, which we denote by $v_R$, so $V(\tilde G)=(V(G)\setminus V(\rset))\cup \set{v_R\mid R\in \rset}$. 
We now define the rotation system $\tilde \Sigma$.
Note that, for every vertex $v\in V(G)\setminus V(\rset)$, $\delta_{G}(v)=\delta_{\tilde G}(v)$, and we define the ordering $\ttoo_v$ in $\tilde \Sigma$ to be $\oset_v$, the ordering on vertex $v$ in $\Sigma$. It remains to define the orderings $\set{\ttoo_{v_{R}}\mid R\in \rset}$. Consider a cycle $R\in \rset$ with $R=(v_0,v_1,\ldots,v_{s-1},v_0)$, and we define edges $e_0,\ldots,e_{s-1}$ similarly as the last paragraph.
For each index $0\le i\le s-1$, we denote $\delta_{G}(v_i)=\set{e_{i-1}, e^i_1,\ldots,e^i_{d_i},e_i}$, where the edges are indexed according to the ordering $\oset_{v_i}$ in $\Sigma$. By construction of graph $\tilde G$, $\delta_{\tilde G}(v_R)=\bigg(\bigcup_{0\le i\le s-1}\delta_{G}(v_i)\bigg)\setminus E(R)=\set{e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}}$. We then define the ordering $\ttoo_{v_{R}}$ to be
$e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}$. This completes the definition of instance $\tilde I$. We call $\tilde I$ the 
\emph{contracted subinstance} of $I$.

\paragraph{Well-Structured solutions.}
Let $I=(G,\Sigma)$ be a well-structured instance and let $\rset$ be its set of special cycles. We say that a solution $\phi$ of instance $I$ is a \emph{well-structured solution} (or a \emph{well-structured drawing}) for $I$, iff
\begin{properties}{P}
\item for each cycle $R\in \rset$, the image of $R$ in $\phi$ is a simple closed curve, that we denote by $\eta_R$;
\label{prop: simple curve}
\item the images of cycles in $\rset$ do not cross each other in $\phi$, i.e., every intersection between two curves $\eta_R,\eta_{R'}$ (where $R,R'$ are distinct cycles in $\rset$) is the image of some vertex;
\label{prop: curves not crossing}
\item there exists, for each cycle $R\in \rset$, a disc $D_R$ whose boundary is the curve $\eta_R$, such that interior of the discs $\set{D_R}_{R\in \rset}$ are mutually disjoint;
\label{prop: discs interior not crossing}
\item for each edge $e$ that is incident to a vertex $v$ of some special cycle $R\in\rset$, the intersection of image of $e$ and the tiny $v$-disc $D_{\phi}(v)$ is disjoint from the interior of disc $D_R$;
\label{prop: first segments}
\item for each $R\in \rset$, the interior of $D_R$ does not contain any vertex image in $\phi$; and
\label{prop: discs interior no vertex}
\item the number of edges that crosses a special edge of $I$ in $\phi$ is at most $\cro(\phi)\cdot (\tau^i)^{10}/|E(G)|$.
\label{prop: niubi edge crossing special cycle}
\end{properties}
We say that a solution $\phi$ for instance $I$ is \emph{almost well-structured} iff it satisfies properties \ref{prop: simple curve}--\ref{prop: first segments}.


\newcommand{\delE}{E^{\sf del}}
\newcommand{\ws}{well-structured\xspace}

The main result in this subsection is the following lemma.

\znote{parameter $\smallprobability$ to be determined.}

\begin{lemma}
\label{lem: many path main}
There is an efficient randomized algorithm, that given a well-structured subinstance $I=(G,\Sigma)$ of $\check I$ for which there exists a \ws drawing $\phi$, computes (i) a well-structured subinstance $\hat I=(\hat G,\Sigma)$ of $I$ with the same set $\rset$ of special cycles as $I$; and (ii) a collection $\iset$ of well-structured subinstances of $\hat I$, such that
\begin{properties}{C}
\item for each instance $I'\in \iset$, its contracted subinstance $\tilde I'$ is either $\tau^s$-small or $\tau^i$-narrow;
\label{prop: well-structured and contracted}
\item for each edge $e\in E(G)$, either $e\in E(G)\setminus E(\hat G)$, or $e$ is a special edge of exactly two subinstances in $\iset$, or $e$ is a non-special edge of exactly one subinstance in $\iset$;
\label{prop: edge appearance}
\end{properties}
and moreover, there exists a well-structured drawing $\hat \phi$ for $\hat I$, such that, with probability $1-O(1/\mu^{\smallprobability})$,
\begin{properties}[2]{C}
\item for each instance $I'\in \iset$, the drawing of $I'$ induced by $\hat \phi$ is a well-structured solution for $I'$;
\label{prop: well-structured solutions}
\item $|E(G)\setminus E(\hat G)|\le \cro(\phi)\cdot \poly(\mu)/|E(G)|$; 
\label{prop: few deleted edges}
\item for each special cycle $R\in \rset$, its images in drawings $\phi$ and $\hat \phi$ are identical, and the disc $D_R$ it defines in $\phi$ and $\hat \phi$ are the same;
for each edge $e\in E(\hat G)$ and each special cycle $R\in \rset$: either in both $\phi$ and $\hat \phi$, the image of $e$ is disjoint from the interior of disc $D_R$, or the intersections of the image of $e$ with the interior of disc $D_R$ are identical in $\phi$ and $\hat \phi$; 
and
\label{prop: forbidden discs}
\item if $\cro(\phi)\le m^2/\mu^{c}$ for some large enough constant $c>0$, then $\cro(\hat\phi)\le O(\cro(\phi))$.
\label{prop: number of crossings}
\end{properties}
%\znote{do we have this?} 
Moreover, there is an efficient algorithm $\alg(\iset)$, that given, for each instance $I'\in \iset$, a feasible solution $\phi(\tilde I')$ the contracted instance $\tilde I'$ of $I'$, computes a well-structured solution $\phi(\hat I)$ for instance $\hat I$, of cost 
$\cro(\phi(\hat I))\leq O\big(\sum_{I'\in \iset}\cro(\phi(\tilde I')\big)$.
\end{lemma}

The remainder of this subsection is dedicated to the proof of \Cref{lem: many path main}.

%The algorithm is randomized and consists of two phases. In the first phase, the algorithm will return FAIL with probability $O(1/\mu^{\smallprobability-\interestconst})$, and if it does not return FAIL, it will compute a collection $\iset$ of subinstances of the input instance $I=(G,\Sigma)$, and a set $E^{\sf del}$ of edges in $G$, such that, if we denote by $\tilde \iset$ the set of all contracted subinstances for instances in $\iset$, then with probability $O(1/\mu^{\smallprobability-\interestconst})$,

\iffalse
\begin{properties}{C}
\item each instance $I'\in \iset$ is a well-structured subinstance;
\label{prop: well-structured instances}
\item for each contracted instance $\tilde I'=(\tilde G',\tilde\Sigma') \in \tilde \iset$, either $\tilde I'$ is non-wide, or $|E(\tilde G')|\le m/\mu$;\label{prop: no longer wide}
\item the sets $\set{\hat E(I')\mid I'\in \iset}$ of edges are mutually disjoint;\label{prop: private edges disjoint}
\item $|E^{\sf del}|\le \cro\cdot\mu^{O(\interestconst)}/m$, and edges of $E^{\sf del}$ does not belong to any instance of $\iset$;\label{prop: few deleted edges in phase 1}
\item every edge of $E(G)\setminus \bigg(E^{\sf del}\cup \big(\bigcup_{I'\in \iset}\hat E(I')\big)\bigg)$ is a special edge of exactly two instances in $\iset$;\label{prop: few edges}
\item there exists, for every instance $I'\in \iset$, a well-structured solution $\phi_{I'}$, such that\\
$\expect[]{\sum_{I'\in \iset}\optcrors(I')}\le \left (\optcrors(I)+|E(G)|\right )\cdot \nu$; and \label{prop: small solution cost}
\item there is an efficient algorithm $\alg(\iset)$, that, given, for each contracted instance $\tilde I' \in \tilde\iset$, a feasible solution $\phi(\tilde I')$, computes a feasible solution $\phi$ for instance $I$, of cost $\cro(\phi^*)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$. \label{prop: alg to put together}
\end{properties}
\znote{to modify the properties?}


In the second phase, we will compute, for each instance $I'\in \iset$, a new instance $I''$ obtained from $I'$ by deleting a set of edges from $I'$, such that
\znote{to add more properties}
\fi

\input{many_paths_main_decomposition}

\input{many_paths_main_decomposition_analysis}



==> many_paths_main_decomposition.tex <==

%\subsection{Phase 1: Decomposition into small or non-wide subinstances}


\ifhide

\iffalse
From the above discussion, in both cases eventually we obtain two distinct vertices $v',v''$ of $\hat G$ and a set $\pset$ of $\floor{m/\mu^{\interestconst}}$ edge-disjoint paths connecting $v'$ to $v''$. Therefore, from now on we will work with graph $\hat G$, vertices $v',v''$ and the set $\pset$ of paths in $\hat G$.
%
Note that the rotation system $\Sigma$ naturally defines a rotation system $\hat \Sigma$ on graph $\hat G$.
We first apply the algorithm from \Cref{lem: non_interfering_paths} to the instance $(\hat G,\hat \Sigma)$ and the set $\pset$ of paths. We rename the set of paths that we obtain by $\pset$. From \Cref{lem: non_interfering_paths}, the new set $\pset$ contains $\floor{m/\mu^{\interestconst}}$ paths connecting $v'$ to $v''$, that are non-transversal with respect to $\hat \Sigma$.
%
Also note that the drawing $\phi^*$ of $G$ naturally induces a drawing of $\hat G$, which we denote by $\hat\phi$. It is easy to verify that $\hat\phi$ respects the rotation system $\hat \Sigma$ on $\hat G$, and $\cro(\hat\phi)=\cro$.
\fi


%The algorithm for \Cref{lem: many path main} is recursive. Throughout, we maintain a collection $\hat{\iset}$ of well-structured subinstances of $I$, that is initialized to be $\hat{\iset}=\set{I}$, and a set $\hat E^{\sf del}$ of edges of $G$, that initially contains no edges. As the algorithm proceeds, the collection $\hat{\iset}$ and the set $\hat E^{\sf del}$ evolve, and we will ensure that every instance that ever appears in collection $\hat{\iset}$ is well-structured.

The algorithm for \Cref{lem: many path main} is recursive. Throughout, we maintain a well-structured subinstances of $\hat I$ together with its structure $(\hat K,\hat \rho,\hat \fset,\hat\gset)$, and a set $\hat E^{\sf del}$ of edges of $G$. Initially, instance $\hat I= I$, with structure $(\hat K,\hat \rho,\hat \fset,\hat\gset)=(K,\rho,\fset,\gset)$, and the set $\hat E^{\sf del}$ contains no edges. As the algorithm proceeds, the instance $\hat I$ and the set $\hat E^{\sf del}$ evolve.
%
\iffalse
\begin{itemize}
\item every instance that ever appears in collection $\hat{\iset}$ is well-structured; and
%\item for every instance $I'=(G,\Sigma)$ that ever appears in collection $\hat{\iset}$, $G$ is a subgraph of $G$; and
\item over the course of the algorithm, the total number of cycles in $\set{\rset(I')}_{I'\in \hat \iset}$ may not exceed $m/\tau^s$ \znote{to fix}.
\end{itemize}
\fi
%
The algorithm continues to be executed as long as there exists some face $F\in \hat \fset$, such that its contracted instance $\tilde I'_F$ is $\tau^i$-wide and not $\tau^s$-small.

We now describe an iteration of the algorithm. Let $\hat I$ be the current instance with structure $(\hat K,\hat \rho,\hat \fset,\hat\gset)$ and let $F$ be a face in $\hat \fset$ such that the contracted subinstance $\tilde I_F$ is $\tau^i$-wide and not $\tau^s$-small. 
%We denote by $\tilde I'=(\tilde G',\tilde \Sigma')$ its contracted subinstance.
Denote $m'=|E(\tilde G_F)|$, so $m'>\tau^s$.
Recall that there is a subgraph $G_F$ in the collection $\hat \gset$ associated with face $F$.
Let $\rset$ be the set of cycles in $\partial F$ and denote $V_{\rset}=\set{v_R\mid R\in \rset}$, so $V(\tilde G'_F)=\big( V(G'_F)\setminus V(\rset) \big)\cup V_{\rset}$.
%
We use the following simple claim, whose proof uses standard max-flow techniques and is deferred to \Cref{apd: Proof of different cases}.

\iffalse\begin{claim}
\label{clm: find the witness}
There is an efficient algorithm, that, given an instance $I'=(G',\Sigma')$, checks whether or not instance $I'$ is wide, and if so, compute a set $\pset$ of paths as a witness for $I'$.
\end{claim}

We first use the algorithm in \Cref{clm: find the witness} to compute a set $\pset$ of paths as the witness for $\tilde I'$.
Consider now the subgraph $\tilde G''$ of graph $\tilde G'$ induced by all edges of $E(\pset)$.
We use the following claim, whose proof uses standard techniques and is deferred to \Cref{apd: Proof of different cases}.\fi

\begin{claim}
\label{clm: different cases}
There is an efficient algorithm, that takes as input a well-structured instance $\hat I$ with structure $(\hat K,\hat \rho,\hat \fset,\hat\gset)$, a face $F\in \hat\fset$ and a parameter $\tau^i>0$, checks whether or not the contracted instance $\tilde I_F$ is $\tau^i$-wide, and if so, compute a set $\pset$ of edge-disjoint paths or cycles in graph $\tilde G_F$, such that $|\pset|\ge m'/3\tau^i$, each path of $\pset$ has length at most $10\tau^i$, and at least one of the following happens:
\begin{enumerate}
\item there are a pair $v',v''\in V(\tilde G')\setminus V_{\rset}$ of vertices in $\tilde G'$, such that all elements of $\pset$ are paths that connect $v'$ to $v''$ and do not contain any vertex of $V_{\rset}$;
\label{case: clean paths}
\item there is a vertex $v_R\in V_{\rset}$, such that all elements of $\pset$ are cycles that contain vertex $v_R$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R}$;
\label{case: cycles}
\item there are a vertex $v_R\in V_{\rset}$ and a vertex $v\in V(\tilde G')\setminus V_{\rset}$, such that all elements of $\pset$ are paths that connect $v_R$ to $v$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R}$;\label{case: paths with one node}
\item there are two vertices $v_R, v_{R'}\in V_{\rset}$, such that all elements of $\pset$ are paths that connect $v_R$ to $v_{R'}$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R, v_{R'}}$.
\label{case: paths with two nodes}
\end{enumerate}
\end{claim}

%We now consider each of the cases in \Cref{clm: different cases} in turn, as follows. We first consider Case \ref{case: clean paths}. \znote{to consider other cases}

\znote{overview here}

\fi

\subsubsection{Step 1. Computing a new special cycle $K$}
\label{Step 1}

Let $v',v''$ be the endpoints of all paths of $\pset$. Since no paths of $\pset$ contains any vertex of $V_{\rset}$, the paths of $\pset$ are also paths in graph $G'$.
%
We view all paths of $\pset$ as being directed from vertex $v'$ to vertex $v''$.
We denote $L=|\pset|$ and denote by $E_1=\set{e_0,\ldots,e_{L-1}}$ the set of edges that serve as the first edge of paths of $\pset$, where the edges are indexed according to the ordering ${\oset}_{v'}\in \Sigma$.
We choose an index $z\in \set{0,\ldots,\floor{L/2}-1}$ uniformly at random, and let $z'= z+\floor{L/2}$. We denote by $\tilde P$ the path in $\pset$ whose first edge is $e_z$, and denote by $\tilde P'$ the path in $\pset$ whose first edge is $e_{z'}$. We define $\tilde K=\tilde P\cup \tilde P'$, so $\tilde K$ is a subgraph of $G'$. Since $I'=(G',\Sigma')$ is a subinstance of the input instance $I=(G,\Sigma)$, $G'$ is a subgraph of $G$, so $\tilde K$ is also a subgraph of $G$.

If paths $\tilde P$ and $\tilde P'$ do not share inner vertices, then we denote $P=\tilde P$, $P'=\tilde P'$, and $K=\tilde K$.
If paths $\tilde P$ and $\tilde P'$ share inner vertices, then we let $v^*$ be the first inner vertex of $\tilde P$ that is also contained in $\tilde P'$. We denote by $P$ the subpath of $\tilde P$ between $v'$ and $v^*$, and  denote by $P'$ the subpath of $\tilde P'$ between $v'$ and $v^*$. Therefore, the paths $P, P'$ are internally vertex-disjoint.
We unname the previous vertex $v''$ and rename $v^*$ by $v''$.
We then define $K=P\cup P'$, so $K$ is a cycle, and $K\subseteq\tilde K$ is a subgraph of $G'$. Therefore, $P$ and $P'$ are paths of $G'$ and are also paths of $G$.
Since every path of $\pset$ has length at most $\tau^i\cdot\mu^{10\interestconst}$, from the construction of $K$, $|E(K)|\le 2\tau^i\cdot\mu^{10\interestconst}$.


In the following steps, we will ``cut the instance $I'$ along $K$'' into two subinstances $I'_1, I'_2$, and cycle $K$ computed in this step will be a special cycle in both $I'_1$ and $I'_2$.


\iffalse
We prove the following observation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse{whp version}

\begin{observation}
	\label{obs: skeleton number of edges}
	The probability that $K$ contains more than $\mu^{\interestconst+\smallprobability}$ edges is at most $O(1/\mu^{\smallprobability})$.
\end{observation}
\begin{proof}
	For each $0\le i\le \floor{L/2}-1$, we denote by $K_i$ the subgraph formed by the union of the path in $\pset$ whose first edge is $e_i$ and the path in $\pset$ whose first edge is $e_{i+\floor{L/2}}$. Since the paths of $\pset$ are edge-disjoint, the subgraphs $K_0,\ldots ,K_{\floor{L/2}-1}$ are edge-disjoint, and therefore the expected number of edges of a random subgraph of $\set{K_0,\ldots,K_{\floor{L/2}-1}}$ is at most $m/\floor{L/2}< O(\mu^{\interestconst})$. From Markov's bound, the  probability that $K$ contains more than $\mu^{\interestconst+\smallprobability}$ edges is at most $O(\mu^{\interestconst})/\mu^{\interestconst+\smallprobability}=O(1/\mu^{\smallprobability})$.
\end{proof}

\fi









%\iffalse{expectation version}

\begin{observation}
	\label{obs: skeleton number of edges}
	$\expect[]{|E(K)|}=O(\tau^i)$.
\end{observation}
\begin{proof}
	For each $0\le z\le \floor{L/2}-1$, we denote by $\tilde K_z$ the subgraph formed by the union of the path in $\pset$ whose first edge is $e_z$ and the path in $\pset$ whose first edge is $e_{z+\floor{L/2}}$. Since the paths of $\pset$ are edge-disjoint, the subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ are edge-disjoint, and therefore the expected number of edges in $\tilde K$, a random element in set $\set{\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}}$, is at most $O(m'/L) \le  O(\tau^i)$. Since $K\subseteq \tilde K$, we get that $\expect[]{|E(K)|}=O(\tau^i)$.
\end{proof}



\paragraph{Bad Event $\event_1$.}
We say that the bad event $\event_1$ happens if $K$ contains more than $\tau^i\cdot\mu^{\smallprobability}$ edges. 
From \Cref{obs: skeleton number of edges} and Markov's bound, $\Pr[\event_1]\le O(1/\mu^{\smallprobability})$.

\fi

%In the remainder of this subsection, we prove several useful properties of $K$ which will be used later.
%We denote by $\phi^*_G$ the drawing of graph $G$ induced by drawing $\phi^*$ (recall that $G$ is a subgraph of the input graph $G$).


%We then check whether or not any of events $\event_1,\event_3,\event_4,\event_5$ happens (it is easy to see that this can be done efficiently). If so, then we return FAIL and terminate the algorithm. Otherwise, we continue to the next steps.
%and will eventually compute a collection of well-structured subinstances of the input instance $I=(G,\Sigma)$. From the above discussion, the probability that we return FAIL in Step 1 is $O(1/\mu^{\smallprobability})$.


%\znote{modify the def of type-2 high-degree vertices, and rename them significant vertices}


\subsubsection{Step 2. Computing the inner and outer sides of $K$}
\label{Step 2}


Recall that all paths of $\pset$ are being directed from $v'$ to $v''$. Recall that we have denoted by $e_0,\ldots, e_{L-1}$ the set of first edges of paths in $\pset$, where edges are indexed according to the ordering $\oset_{v'}$. For each $0\le j\le L-1$, we denote by $P_j$ the path in $\pset$ that has $e_{j}$ as its first edge, and we denote by $e'_{j}$ the last edge of $P_j$.
In order to ``cut instance $I'$ along $K$'' into subinstances $I'_1$ and $I'_2$, we will need to define the ``inner and outer sides'' of $K$, which we do in this step.
%As a first step towards this goal, in this step we compute the orientations of orderings of all vertices of $K$.

First, since the a drawing of any graph and its mirror image are viewed as identical drawings, we can fix the orientation of the ordering $\oset_{v'}$ to be positive, without loss of generality. 
%In other words, if we traverse along the boundary of a disc around $v'$ counter-clock-wise, then we will encounter edges of $e_0,\ldots, e_{L-1}$ sequentially.
This oriented ordering naturally induces an oriented ordering on the set $\set{P_0,\ldots, P_{L-1}}$ of paths, which we denote by $(\oset',b')$.
%We will show that the orientations of $v''$ and all significant vertices can be fixed as well.


Next we consider the vertex $v''$. Note that edges $e'_{0},\ldots,e'_{L-1}$ belong to set $\delta(v'')$, and the circular ordering $\oset_{v''}\in \Sigma$ is an circular ordering on the set $\set{e'_{0},\ldots,e'_{L-1}}$, which in turn induces an circular ordering on the set $\set{P_{0},\ldots,P_{L-1}}$ of paths, that we denote by $\oset''$.
Clearly, computing an orientation of the unoriented ordering $\oset_{v''}$ is equivalent to computing an orientation of the unoriented ordering $\oset''$.
We compute an orientation $b''\in \set{-1,1}$ of $\oset''$ as follows.
We set $b''=1$ iff $\dist((\oset', b'),(\oset'',1))\le \dist((\oset', b'),(\oset'',-1))$; otherwise we set $b''=-1$.
In other words,  
\[b''=\arg\min_{b\in \set{-1,1}}\set{\dist((\oset', b'),(\oset'',b))}.\]


Consider now a vertex $v\in V(K)$. Assume without loss of generality that $v$ belongs to path $P$. We denote by $\pset_v=\set{P_{i_1},\ldots,P_{i_q}}$ the set of all paths $\pset$ that contains vertex $v$. 
%From the definition of a significant vertex, $q\ge h'$. 
For each $1\le j\le q$, we denote by $\tilde e_{i_j}$ the first edge of $P_{i_j}$ that is incident to $v$ (recall that paths of $\pset$ are being directed from $v'$ to $v''$),
%Additionally, we denote by $\tilde e, \tilde e'$ the edge of $P$ that are incident to $v$.
and recall that we have denoted by $e_{i_j}$ the first edge of $P_{i_j}$, so $e_{i_j}$ is incident to $v'$.
Note that we have already fixed an orientation of the ordering $\oset_{v'}$ to be positive. Let $b(v)\in \set{-1,1}$ be an orientation of ordering $\oset_v$. 
Let $e$ be the first edge of $P$ and let $e'$ be the first edge of $P'$.
We say that an index $i_j$ is \emph{screwed under $b(v)$}, iff either edges $e,e_{i,j},e'$ appear clockwise in the oriented ordering $(\oset_{v'},+1)$ and edges $\tilde e, \tilde e_{i,j},\tilde e'$ appear clockwise in the oriented ordering $(\oset_{v},b(v))$ or edges $e',e_{i,j},e$ appear clockwise in the oriented ordering $(\oset_{v'},+1)$ and edges $\tilde e',\tilde e_{i,j},\tilde e$ appear clockwise in the oriented ordering $(\oset_{v},b(v))$.
We then set $b(v)$ as follows. If the number of indices in $\set{i_1,\ldots, i_q}$ that are screwed under $1$ is greater than the number of indices in $\set{i_1,\ldots, i_q}$ that are screwed under $-1$, then we set $b(v)=-1$, otherwise we set $b(v)=1$.


\iffalse
Note that the circular ordering $\oset'$ on set $\pset$ of paths naturally induces a circular ordering on the set $\pset_v$ of paths, that we denote by $\oset'_v$. Also note that the circular ordering $\oset_v\in  \Sigma$ naturally induces a circular ordering on the set $\set{\tilde e_{i_j}\mid 1\le j\le q}$ of edges, which in turn induces an ordering on the set $\pset_v$ of paths, that we denote by $\oset''_v$. 
Clearly, computing an orientation of the unoriented ordering $\oset_{v}$ is equivalent to computing an orientation of the unoriented ordering $\oset''_v$.
We compute an orientation $b''_v\in \set{-1,1}$ of $\oset''_v$ as follows.
We set $b(v)=1$ iff $\dist((\oset'_v, b'),(\oset''_v,1))\le \dist((\oset'_v, b'),(\oset''_v,-1))$; otherwise we set $b(v)=-1$.
In other words,
\[b(v)=\arg\min_{b\in \set{-1,1}}\set{\dist((\oset'_v, b'),(\oset''_v,b))}.\]
\fi

%\paragraph{Computing the Inner and Outer sides of $K$.}
So far we have computed, for each  vertex of $K$, an orientation of its circular ordering in $\Sigma$. Let $v$ be an inner vertex of $P$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P$, edge $\tilde e$ precedes edge $\tilde e'$ in $P$, and the edges appear clockwise in the oriented ordering on $v$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are on the \emph{inner side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are on the \emph{outer side} of $K$.
%
Similarly, let $v$ be an inner vertex of $P'$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P'$, edge $\tilde e$ precedes edge $\tilde e'$ in $P'$, and the edges appear clockwise in the oriented ordering on $v$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are on the \emph{outer side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are on the \emph{inner side} of $K$.
%
For vertex $v''$, we denote  assume that $\delta(v'')=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e$ is the last edge of $P$ and $\tilde e'$ is the last edge of $P'$, and the edges appear clockwise in the oriented ordering at $v''$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are \emph{on the inner side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are \emph{on the outer side} of $K$.






\subsubsection{Step 3. Decomposing instance $I'$ into two subinstances}
\label{Step 3}

%From this step, we will maintain a set $E^*$ of edges of $\hat G$, that we call the set of \emph{deleted edges}. The set $E^*$ evolves over the course of the algorithms, and eventually edges of $E^*$ will not appear in the subinstances that we construct.

Consider the contracted subinstance $\tilde I'=(\tilde G',\tilde \Sigma')$ of the well-structured instance $I'$. Since we have assumed that paths of $\pset$ do not contain special vertices of graph $G'$, $K$ is also a cycle in $\tilde G'$, and for each vertex $v\in V(K)$, $\delta_{G'}(v)=\delta_{\tilde G'}(v)$. 
We will decompose graph $\tilde G'$ into two subgraphs, and then construct two subinstances of $I'$ based on them.

%We let set $E^*$ contains all edges of $E(G')\setminus E(K)$ that are incident to a low-degree vertex of $K$ or a type-1 high-degree vertex of $K$. Assume that the events $\event_4,\event_5$ do not happen, then $|E^*|\le O\big((h+h')\tau^i\mu^{\smallprobability}\big)$.
%If event $\event$ does not happen, then from Properties \ref{fact: few incident edges on type-1} and \ref{fact: few incident edges on low-deg}, there are a total of $O(h\mu^{\interestconst+\smallprobability})$ such edges.
%\znote{we do not know the value of $h$ and $h'$, so this step is problematic}

%Consider now the graph $\hat G= \tilde G'\setminus E^*$. 
We denote by $\hat E$ the set of all edges of $E(\tilde G')\setminus E(K)$ that is incident to a vertex of $K$, so each edge of $\hat E$ is incident to either vertex $v'$, or vertex $v''$, or an inner vertex of $P$ or $P'$.
%Therefore, each such edge is either on the inner side of $K$ or on the outer side of $K$. 
We denote by $\hat E_{\inn}$ the set of all edges of $\hat E$ that are on the inner side of $K$, and denote by $\hat E_{\out}$ the set of all edges of $\hat E$ that are on the outer side of $K$. Clearly, sets $\hat E_{\inn},\hat E_{\out}$ partition $\hat E$. Note that, from the construction of cycle $K$, $|\hat E_{\inn}|\ge |\hat E_{\inn}\cap \delta_{G'}(v')| \ge \floor{L/2}$, and similarly $|\hat E_{\out}|\ge |\hat E_{\out}\cap \delta_{G'}(v')|\ge \floor{L/2}$.

In order to decompose graph $\tilde G'$ into two subgraphs, it will be convenient for us to slightly modify the graph $\tilde G'$, by splitting each vertex $v\in V(K)$ into three vertices: vertex $v_{\inn}$, that is incident to the edges of $\hat E_{\inn}\cap \delta(v)$, vertex $v_{\out}$, that is incident to the edges of $\hat E_{\out}\cap \delta(v)$, and vertex $v_{M}$, that is incident to two edges of $E(K)\cap \delta(v)$. 
We denote by $\hat G$ the resulting graph.
We define $V_{\inn}=\set{v_{\inn}\mid v\in V(K)}$, and define sets $V_{\out}$ and $V_{M}$ similarly, so $V(\hat G)=V_{\inn}\cup V_{\out}\cup V_{M}\cup (V(G')\setminus V(K))$.
%
Note that in graph $\hat G$, $K$ is a cycle on vertices of $V_M$ and is disconnected from the rest of the graph.

We then compute, using the standard max-flow techniques, a minimum-cardinality set $E^{*}$ of edges of $\hat G$, whose removal separates vertices of $V_{\inn}$ from $V_{\out}$ in $\hat G$. We add the edges of $E^*$ into the set $\hat E^{\sf del}$.


We now construct two new instances as follows. First, let $\tilde G_{\inn}$ be the graph obtained from subgraph of $\hat G$ consisting of all connected components of $\hat G\setminus E^{*}$ that contain vertices of $V_{\inn}\cup V_{M}$, by identifying, for each vertex $v\in V(K)$, the corresponding vertex $v_{\inn}\in V_{\inn}$ with the corresponding vertex $v_M\in V_M$.
It is easy to verify that $\tilde G_{\inn}$ is a subgraph of $\tilde G'$.
%(recall that $\tilde G'$ is the graph obtained from $G'$ by contracting each special cycle $R\in\rset(I')$ into a single vertex $v_R$). 
We now let $G_{\inn}$ be the graph obtained from $\tilde G_{\inn}$ by uncontracting each special vertex $v_R$ back to the cycle $R$. It is easy to verify that graph $G_{\inn}$ is a subgraph of $G'$. We then let $\Sigma_{\inn}$ be the rotation system on $G_{\inn}$ induced by the rotation system $\Sigma'$ on $G'$, and define the instance $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$. For $I_{\inn}$ to be a well-structured subinstance, we still need to define its set $\rset(I_{\inn})$ of special cycles.
Note that each special cycle of instance $I'$ now either entirely belongs to $G_{\inn}$ or entirely belongs to $G_{\out}$.
We then let set $\rset(I_{\inn})$ contain all special cycles in $\rset(I')$ that entirely belongs to $G_{\inn}$ and the cycle $K$, namely $\rset(I_{\inn})=\set{R\mid v_R\in V(\tilde G_{\inn})}\cup \set{K}$. Clearly, the cycles in $\rset(I_{\inn})$ are edge-disjoint (and even vertex-disjoint in this case).
This completes the construction of instance $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$.
It is then easy to verify that $I_{\inn}$ is a well-structured subinstance of $I'$.
We construct the well-structured subinstance $I_{\out}=(G_{\out}, \Sigma_{\out})$ and its set $\rset(I_{\out})$ of special cycles similarly.

We prove the following immediate observations, that will be later used in \Cref{subsec: analysis of decomposition lemma} for the analysis of the algorithm.

\begin{observation}
\label{obs: number of edges in base}
$|E(G_{\inn})|+|E(G_{\out})|\le |E(G')|+|E(K)|$, and
$|E(G_{\inn})|, |E(G_{\out})|\le |E(G')|-\tau^s/6\tau^i$.
\end{observation}
\begin{proof}
From the construction of graphs $G_{\inn},G_{\out}$, $E(G_{\inn}),E(G_{\out})\subseteq E(G')$, and the only edges of $G'$ that belong to both $E(G_{\inn})$ and $E(G_{\out})$ are edges of $E(K)$, so $|E(G_{\inn})|+|E(G_{\out})|\le |E(G')|+|E(K)|$.

On the other hand, observe that edges of $\hat E_{\out}$ may not belong to set $E(G_{\inn})$, since otherwise some vertex of $V_{\out}$ (the endpoint of any edge of $\hat E_{\out}\cap E(G_{\inn})$ in $V_{\out}$) must be reachable from some vertex of $V_{\inn}$ in $G_{\inn}$, contradicting the definition of $E^*$ and the construction of $\tilde G_{\inn}$.
Therefore, $|E(G_{\inn})|\le |E(G')|-\floor{L/2}$, and similarly $|E(G_{\out})|\le |E(G')|-\floor{L/2}$.
From \Cref{clm: different cases}, $L\ge m'/3\tau^i\ge \tau^s/3\tau^i$, and \Cref{obs: number of edges in base} now follows.
\end{proof}


\begin{observation}
\label{obs: 2 new special cycles}
$|\rset(I_{\inn})|+|\rset(I_{\out})|= |\rset(I')|+2$.
\end{observation}
\begin{proof}
Since the cycle $K$ in graph $\tilde G'$ does not contain any special vertex, from the construction of the graphs $G_{\inn}, G_{\out}$, each special cycle in $\rset(I')$ belongs to either $G_{\inn}$ or $G_{\out}$ (but not both). Also note that the sets $\rset(I_{\inn})$ and $\rset(I_{\out})$ contain one additional new cycle $K$. Therefore, $|\rset(I_{\inn})|+|\rset(I_{\out})|= |\rset(I')|+2$.
\end{proof}


This completes the description of the three steps in an iteration. Finally, we replace the subinstance $I'=(G',\Sigma')$ in the collection $\hat \iset$ with two new subinstances $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$ and $I_{\out}=(G_{\out}, \Sigma_{\out})$, and proceed to the next iteration. 
We denote by $\iset$ the resulting collection $\hat{\iset}$ at the end of the algorithm, and denote by $E^{\sf del}$ the resulting set $\hat E^{\sf del}$ at the end of the algorithm.
Finally, we define the subinstance $\hat I$ as follows. Its graph $\hat G=G\setminus E^{\sf del}$, its rotation system is $\Sigma$, and its set of special cycles is $\rset$, the set of special cycles of $I$. This completes the description of the algorithm.



==> many_paths_main_decomposition_analysis.tex <==

\subsubsection{Analysis of the algorithm}
\label{subsec: analysis of decomposition lemma}

In this subsection we provide the proof of \Cref{lem: many path main} with some details deferred to subsequent sections.
%by showing that the instances in collection $\iset$ satisfy the properties \ref{prop: well-structured and contracted}--\ref{prop: well-structured solutions}.

First, note that initially the collection $\hat{\iset}$ contains one well-structured subinstance, and from the description of the algorithm, in each iteration we replace one well-structured subinstance in $\hat{\iset}$ with two new well-structured subinstances. Therefore, all subinstances in the resulting collection $\iset$ are well-structured subinstances. On the other hand, recall that the recursive algorithm continues to be executed as long as there exists some instance $I'\in \hat\iset$, such that its contracted subinstance $\tilde I'$ is $\tau^i$-wide and not $\tau^s$-small. Therefore, when the algorithm terminates, property \ref{prop: well-structured and contracted} has to be satisfied.

Second, note that in each iteration, we start with an instance $I'$ in the current collection $\hat \iset$, compute a cycle $K$ that is edge-disjoint from all special cycles in $\rset(I')$ and then decompose instance $I'$ into two subinstances $I_{\inn}$ and $I_{\out}$, such that only edges of $E(K)$ appear in both instances. Therefore, if an edge in the input instance $I'$ is not a special edge of any subinstance that ever appeared in $\hat \iset$, then it either belongs to exactly one resulting instance or belongs to set $E^{\sf del}$; otherwise it eventually belongs to exactly two resulting instances. Therefore, property \ref{prop: edge appearance} holds.
%Second, when an instance $I'$ in the collection $\hat \iset$ is replaced by two instances $I_{\inn}$ and $I_{\out}$, according to algorithm, the edge sets $\hat E(I'_1), \hat E(I'_2)$ are disjoint subsets of $\hat E(I')$. Therefore, eventually the subsets $\set{\hat E(I')\mid I'\in \iset}$ of edges are mutually disjoint, which means property \ref{prop: private edges disjoint} is satisfied.




In order to show that the properties \ref{prop: well-structured solutions}--\ref{prop: number of crossings} also hold and there exists an efficient algorithm $\alg(\iset)$ that satisfies the properties required in \Cref{lem: many path main}, it is convenient for us to associate a tree $T$ with the algorithm, called the \emph{partitioning tree}. Each vertex of $T$ corresponds to a well-structured subinstance that once appeared in the collection $\hat{\iset}$. We grow the tree $T$ along with the iterative algorithm as follows. Initially, $T$ contains a single root denoted by $v(I)$, where $I$ is the input well-structured subinstance to \Cref{lem: many path main}. Consider now some vertex $v(I')$ in $T$, where $I'$ is a subinstance that undergoes Steps 1, 2 and 3. From the algorithm, the instance $I'$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$. We then create two nodes, $v(I_{\inn})$ and  $v(I_{\out})$, that become the child vertices of $v(I')$ in $T$.


\subsubsection*{Number of Iterations}

We first analyze the number of the iterative algorithm using $T$. We use the following observation.

\begin{observation}
\label{obs: number of iterations}
If \fbox{$\tau^s\ge 100\cdot\tau^i\mu^{10\interestconst}$}, then 
%with probability $1-O(m\tau^i/\tau^s\mu^a)$
$|V(T)|\le 200\cdot m\tau^i/\tau^s$.
\end{observation}
\begin{proof}
%Consider the first $M=1000m\tau^i/\tau^s$ iterations of the algorithm. We show that, if event $\event_1$ did not happen in the first $M$ iterations, then $|V(T)|\le M$. Note that this implies that \Cref{obs: number of iterations}, since the probability that $\event_1$ happens in at least one of the first $M$ iterations is $O(m\tau^i/\tau^s\mu^a)$.
We show that, if $\tau^s\ge 100\cdot\tau^i\mu^{10\interestconst}$, then the algorithm will terminate in $200\cdot m\tau^i/\tau^s$ iterations, which implies \Cref{obs: number of iterations}.
%
%We say that an iteration of the algorithm is \emph{good}, iff $\event_1$ did not happen in this iteration. Let $I'$ be an instance that once appeared in $\hat \iset$, we say that the algorithm is \emph{good on $I'$}, iff either node $v(I')$ is a leaf of $T$, or the iteration of processing instance $I'$, and the iterations of processing instances $I''$ where $v(I'')$ is a descendant of $v(I')$ in $T$, are all good.
%
In fact, we will show that, for each subinstance $I'=(G',\Sigma')$ that ever appeared in $\hat \iset$, 
%if the algorithm is good on $I'$, then 
the number of vertices in the subtree of $T$ rooted at node $v(I')$, which we denote by $N_{T}(I')$, is at most $$f(I')=\max\set{\frac{|E(G')|-\tau^s}{\tau^s/100\tau^i},0}+3,$$
which, when applied to the initial instance $I=(G,\Sigma)$ where $|E(G)|=m$, immediately implies that the algorithm will terminate in $200\cdot m\tau^i/\tau^s$ iterations.

Consider now an instance $I'$ that once appeared in $\hat \iset$. Assume first that $v(I')$ is a leaf of $T$, then the number of vertices in the subtree of $T$ rooted at node $v(I')$ is $1$, which is at most $f(I')$ (note that $f(I')\ge 3$ always holds).
Assume now that $v(I')$ is not a leaf of $T$, we let $I'_1=(G'_1,\Sigma'_1)$, $I'_2=(G'_2,\Sigma'_2)$ be two new instances constructed the iteration of processing $I'$. Since $|E(K)|\le 2\tau^i\cdot\mu^{10\interestconst}$, from \Cref{obs: number of edges in base} and the definition of $\event_1$, $|E(G'_1)|+|E(G'_2)|\le |E(G')|+2\tau^i\cdot\mu^{10\interestconst}$ and
$|E(G'_1)|, |E(G'_2)|\le |E(G')|-\tau^s/6\tau^i$. We consider the following cases.

\textbf{Case 1. Both nodes $v(I'_1), v(I'_2)$ are leaves of $T$.}
In this case, $N_T(I')\le 3 \le f(G')$.

\textbf{Case 2. One of the nodes $v(I'_1), v(I'_2)$ is a leaf of $T$.}
Assume without loss of generality that $v(I'_1)$ is a leaf and $v(I'_2)$ is not a leaf, so $|E(G')|-\tau^s/6\tau^i\ge |E(G'_2)|\ge \tau^s$, so 
\[
\begin{split}
N_{T}(I')=2+N_{T}(I'_2)\le 2+f(I'_2)= & \text{ }2+ \frac{|E(G'_2)|-\tau^s}{\tau^s/10\tau^i}+3
\\
\le  & \text{ } 2+ \frac{|E(G')|-(\tau^s/6\tau^i)-\tau^s}{\tau^s/100\tau^i}+3
\\
\le  & \text{ } 2+ \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}-16+3
\\
\le  & \text{ } \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}+3 =f(I').
\end{split}
\]

\textbf{Case 3. Both nodes $v(I'_1), v(I'_2)$ are not leaves of $T$.}
Then $|E(G'_1)|, |E(G'_1)|\ge \tau^s$, and so
\[
\begin{split}
N_{T}(I')\le 1+N_{T}(I'_1)+N_{T}(I'_2)\le & \text{ } 1+f(I'_1)+f(I'_2)
\\ 
= & \text{ } 7+ \frac{|E(G'_1)|-\tau^s}{\tau^s/100\tau^i}+\frac{|E(G'_2)|-\tau^s}{\tau^s/100\tau^i}
\\
\le & \text{ } 7+ \frac{|E(G')|+2\tau^i\cdot\mu^{10\interestconst}-2\tau^s}{\tau^s/100\tau^i}
\\
\le  & \text{ } 7+ \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}
+
\frac{2\tau^i\cdot\mu^{10\interestconst}-\tau^s}{\tau^s/100\tau^i}
\\
\le  & \text{ } \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}+3 =f(I'),
\end{split}
\]
where the last inequality uses the fact $\tau^s\ge 100\tau^i\mu^{10\interestconst}$.
%Therefore, if the algorithm is good on the input instance $I=(G,\Sigma)$, then $|V(T)|\le 100m\tau^i/\tau^s\le M$. This means that if the event $\event_1$ does not happen in the first $M$ iterations, then the algorithm is good on the input instance $I$, and therefore $|V(T)|\le M$.
\end{proof}


%\paragraph{Bad Event $\event^*$.}We say that the bad event $\event^*$ happens iff the iterative algorithm does not terminate in $M=1000 m\tau^i/\tau^s$ iterations. From \Cref{obs: number of iterations}, $\Pr[\event^*]\le O(m\tau^i/\tau^s\mu^a)$.


\iffalse{number of all special edges}
As an immediate corollary, we have the following bound the number of special edges in all resulting instances in $\iset$.

\begin{corollary}
\label{cor: number of special edges}
The total number of special edges in all instances in $\iset$ is at most
$800m(\tau^i)^2\mu^{10\interestconst}/\tau^s$.
\end{corollary}
\begin{proof}
From \Cref{obs: 2 new special cycles}, after each iteration, the number of special cycles in all subinstances in the collection $\hat\iset$ increases by $2$. Since the number of iterations is bounded by $200\cdot m\tau^i/\tau^s$, and the length of each special cycle is at most $2\tau^i\cdot\mu^{10\interestconst}$, we get that the total number of special edges in all resulting instances in $\iset$ is bounded by
$2\cdot \big(200\cdot m\tau^i/\tau^s\big)\cdot \big(2\tau^i\cdot\mu^{10\interestconst}\big)=800m(\tau^i)^2\mu^{10\interestconst}/\tau^s$.
\end{proof}
\fi

We now proceed to analyze the iterative algorithm using the partitioning tree $T$. 
We will maintain a well-structured drawing $\tilde \phi$ of the input instance $I=(G,\Sigma)$, that is initialized to be the input well-structured drawing $\phi$ of $I$ and evolves as the iterative algorithm proceeds.



\znote{the correct notion and claim?}

We denote by $\bar I$ the well-structured instance obtained from $I$ by only deleting from it the edges of $\hat E^{\sf del}$. As more edges are added to set $\hat E^{\sf del}$, the instance $\bar I$ evolves, and it is easy to verify that eventually instance $\bar I$ becomes the output instance $\hat I$.
We say that a well-structured drawing $\tilde \phi$ of instance $\bar I$ is \emph{well-structured with respect to the current collection $\hat \iset$}, iff for each subinstance $I'\in \hat\iset$, the drawing of $I'$ induced by $\tilde \phi$ is a well-structured drawing of $\iset$.
We first focus on an iteration, in which some instance $I'=(G',\Sigma')$ in collection $\iset$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$.

\begin{observation}
\label{obs: not crossing your own special then not crossing any special}
Let $\phi$ be a drawing of instance $\bar I$ that is well-structured with respect to the current collection $\hat \iset$. For an edge $e$ that belongs to a unique instance $I'\in \hat \iset$, if $e$ does not cross any special edge of $I'$ in $\tilde \phi$, then $e$ does not cross any special edge of any instnace of $\hat \iset$ in $\tilde \phi$.
\end{observation}
\begin{proof}
\znote{to complete}
\end{proof}


We use the following claim.
%Let $\tilde \phi$ be a well-structured solution for instance $I'$. We will construct well-structured solutions $\phi(I_{\inn})$, $\phi(I_{\out})$ for subinstances $I_{\inn}$ and $I_{\out}$, respectively, and then show that $\cro(\phi(I_{\inn}))+\cro(\phi(I_{\out}))$ is not much larger than $\cro(\tilde \phi)$. We denote $m'=|E(G')|$. Recall that in Step 1 we computed a cycle $K$ that consists of two internally disjoint paths $P,P'$ and is a subgraph of the input graph $G$.

%Recall that $\phi^*$ is optimal well-structured drawing of the input well-structured instance $I=(G,\Sigma)$ and $\cro=\cro(\phi^*)$.

%\znote{some lemma here summarizing, and finish the proof of \Cref{lem: many path main} before providing the proof of lemma}



\begin{claim}
\label{lem: well-structured drawing splitting}
Consider an iteration of the algorithm in which a well-structured instance $I'=(G',\Sigma')$ is processed and eventually replaced by two new well-structured instances, that we denote by $I_{\inn}, I_{\out}$.
Let $\tilde \phi$ be a well-structured drawing of $\bar I$ with respect to the collection $\hat\iset$ before this iteration. 
Then there exists a well-structured drawing $\tilde \phi'$ of $\bar I$ with respect to the collection $\hat\iset$ after this iteration, such that 
\begin{itemize}
\item for each special cycle $R$ in the collection $\hat\iset$ before this iteration, its images in drawings $\tilde\phi$ and $\tilde \phi'$ are identical, and the disc $D_R$ it defines in $\phi$ and $\hat \phi$ are the same; for each edge $e\in E(\hat G)$ and each special cycle $R\in \rset$: either in both $\phi$ and $\hat \phi$, the image of $e$ is disjoint from the interior of disc $D_R$, or the intersections of the image of $e$ with the interior of disc $D_R$ are identical in $\phi$ and $\hat \phi$; and
\item if \fbox{$\cro(\tilde\phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, then
$\cro(\tilde\phi')\le \cro(\tilde \phi)\cdot(1+1/\mu^{\smallprobability})$.
\end{itemize}
\end{claim}

We provide the proof of \Cref{lem: well-structured drawing splitting} in \Cref{sec: Proof of well-structured drawing splitting}, after we complete the proof of \Cref{lem: many path main} using \Cref{lem: well-structured drawing splitting}.




\subsubsection{Proof of \Cref{lem: well-structured drawing splitting}}
\label{sec: Proof of well-structured drawing splitting}

In this subsection we provide the proof of \Cref{lem: well-structured drawing splitting}, thus completing the proof of \Cref{lem: many path main}.

We focus on an iteration, in which some instance $I'=(G',\Sigma')$ in collection $\iset$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$.
We denote $m'=|E(G')|$.
Recall that currently we have a drawing $\tilde\phi$ of the instance $\bar I$ before this iteration, that is well-structured with respect to the collection $\hat\iset$ before this iteration.
Recall that in Step 1 we computed a cycle $K$ that consists of two internally disjoint paths $P,P'$ and is a subgraph of the input graph $G$.
We first show several crucial properties of $K$.





\subsubsection*{Modifying the drawing $\tilde \phi$}

We now proceed to modify the drawing $\tilde \phi$ into a drawing that is well-structured with respect to the collection $\hat \iset$ after this iteration. That is, we will modify the image of edges of $I'$ in $\tilde \phi$, such that the resulting drawing induces well-structured drawings for new instances $I_{\inn}, I_{\out}$.

We now provide a summary of the stages in modifying the drawing $\tilde \phi$. For simplicity of notations we denote $I'_1=I_{\inn}$ and $I'_2=I_{\out}$ from now on.
We first delete the edges that are added to set $\hat E^{\sf del}$ in this iteration, and rename the resulting drawing by $\tilde \phi$. Clearly, the new drawing $\tilde \phi$ contains at most the same number of crossings as the old one.
In the first stage, we modify the drawing $\tilde\phi$ into a new drawing $\hat\phi$ that induces almost well-structured drawings of instances $I'_1$ and $I'_2$ (recall that an almost well-structured drawing is a drawing that satisfies properties \ref{prop: simple curve}--\ref{prop: first segments}). %such that the image of $K$ in $\hat\phi$ is a simple closed curve, and $\cro(\hat\phi)$ is not much larger than $\cro(\phi)$. 
In the second stage, we locally modify the image of edges incident to vertices of $K$, such that the orientations of vertices of $K$ coincide the orientations computed in Step 2 (\Cref{Step 2}).
In the third and the fourth stages, we 
%split the drawing $\hat \phi$ into an almost well-structured drawing $\hat \phi_1$ of $I'_1$ and an almost well-structured drawing $\hat\phi_2$ of $I'_2$, and then we 
further modify drawing $\hat\phi$ into a drawing $\tilde \phi'$ that induces well-structured drawings of instances $I'_1$ and $I'_2$, respectively.
%such that $\cro(\phi'_1)+\cro(\phi'_2)$ is not much larger than $\cro(\hat\phi)$.  
In each of these stages, we will make sure not to increase the number of crossings in the drawing by too much.
We now describe each of the stages in turn.


\iffalse
From now on we denote $\phi=\tilde \phi$.
We now construct well-structured drawings of the subinstances $I'_1$ and $I'_2$ using the well-structured drawing $\phi$ of instance $I'$ in four stages. In the first stage, we modify the well-structured drawing $\phi$ of $I'$ into an almost well-structured drawing $\hat \phi$ of $I'$ (recall that an almost well-structured drawing is a drawing that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}), such that the image of $K$ in $\hat\phi$ is a simple closed curve, and $\cro(\hat\phi)$ is not much larger than 
$\cro(\phi)$. In the second stage, we locally modify the image of edges incident to vertices of $K$, such that the orientations of vertices of $K$ coincide the orientations computed in Step 2 (\Cref{Step 2}).
In the third and the fourth stages, we 
split the drawing $\hat \phi$ into an almost well-structured drawing $\hat \phi_1$ of $I'_1$ and an almost well-structured drawing $\hat\phi_2$ of $I'_2$, and then we further modify drawings $\hat\phi_1, \hat\phi_2$ into well-structured drawings $\phi'_1,\phi'_2$ of instances $I'_1$ and $I'_2$, respectively.
%such that $\cro(\phi'_1)+\cro(\phi'_2)$ is not much larger than $\cro(\hat\phi)$.  
We now describe each of the stages in turn.
\fi

\subsubsection*{Stage 1. Removing self-loops of the image of $K$ in $\tilde\phi$}

In the first stage, we modify the drawing $\tilde \phi$ into a new drawing $\hat \phi$ that induces almost well-structured drawings of instances $I'_1,I'_2$, via the following claim.


\begin{claim}
\label{clm: skeleton can be drawn in a natural way}
If event $\event$ does not happen, then there is a drawing $\hat\phi$ of instance $\bar I$ after this iteration, in which (i) for each edge not incident to any vertex of $K$, its image in $\hat \phi$ remains the same as in $\tilde \phi$; (ii) the image of $K$ in $\hat \phi$ is a simple closed curve that does not cross any special edge of $I'$, and (iii)
$\cro(\hat\phi)\le \cro(\phi)+O\big(h^2(\tau^i)^2\mu^{2\smallprobability}\big).$
\end{claim}

\begin{proof}
We construct the drawing $\hat\phi$ by iteratively ``opening'' the self-loops of the curve representing the image of $P$ and the curve representing the image of  $\tilde\phi$ until the image of $K$ becomes a simple closed curve. Recall that, from Property \ref{f_prop: P and P' do not cross}, the images of $P$ and $P'$ do not cross in $\tilde\phi$, and from Property \ref{f_prop: K does not cross special edges}, the image of $K$ does not cross any special edge of $I'$ in $\tilde\phi$.

We denote by $\gamma$ the image of $P$ in $\tilde\phi$. Note that $\gamma$ is not necessarily a simple curve. We first iteratively compute a set $Z$ of self-loops of $\gamma$ and another simple curve $\gamma'$ connecting $\tilde\phi(v')$ to $\tilde\phi(v'')$, as follows.
%
We view the curve $\gamma$ as being directed from $\tilde\phi(v')$ to $\tilde\phi(v'')$. Initially we set $Z=\emptyset$. We start from the first endpoint $\tilde\phi(v')$ of $\gamma$ and find the first point $z$ on $\gamma$ that appears twice on $\gamma$. Denote by $\zeta$ the subcurve of $\gamma$ between the first and the last (second) appearance of $z$, so $\zeta$ is a self-loop that starts and ends at $z$. We add the self-loop $\zeta$ to set $Z$ and delete $\zeta$ from $\gamma$. We continue this process until the curve $\gamma$ no longer contains self-loops. Denote by $\gamma'$ the resulting simple curve we obtain, and we also view curves $\gamma'$ as being directed from $\tilde\phi(v')$ to $\tilde\phi(v'')$. See \Cref{fig: remove_loop} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Curve $\gamma$ (with direction) is shown in blue, with vertices $v_1,v_2,v_3$ appearing on it sequentially.]{\scalebox{0.0855}{\includegraphics{figs/remove_loop_1.jpg}}}
	\hspace{0.1cm}
	\subfigure[Curve $\gamma'$ is shown in green. Self-loop $\zeta$ is shown in light blue. Thin strip around $\zeta$ is shown in grey.]{
		\scalebox{0.085}{\includegraphics{figs/remove_loop_2.jpg}\label{fig: thin strip}}}
	\caption{Illustration for constructing curve $\gamma'$. \label{fig: remove_loop}}
\end{figure}

The algorithm for constructing the drawing $\hat\phi$ is iterative. In each iteration, we process a self-loop in $Z$.
%
We now describe an iteration.
Let $\zeta$ be a loop in $Z$, and we denote by $z$ the unique point of $\zeta$ that lies on $\gamma'$. %(see \Cref{fig: loop_before}).
	%
We modify the drawing as follows. 
	Let $v_1,\ldots,v_r$ be the vertices whose images appear on the self-loop $\zeta$, where the vertices are indexed according to the ordering in which they appear on $P$ (see \Cref{fig: remove_loop}).
	We denote $V_{\zeta}=\set{v_1,\ldots,v_r}$.
	Let $\sigma$ be a tiny segment of $\gamma'$ that contains $z$.
	We remove the image of vertices $v_1,\ldots,v_r$ and all their incident edges from the current drawing, and place them on $\sigma$, such that $v_1,\ldots,v_r$ appear sequentially in the direction of $P$.
	See \Cref{fig: remove_loop_3} for an illustration.
	 %(see \Cref{fig: loop_after}).
	%We do not modify the images of edges that are not incident to $v_1,\ldots,v_r$.

\iffalse
	\begin{figure}[h]
		\centering
		\subfigure[Before: the images of $v_1,v_2$ appear sequentially on the image of $P$, and they belong to the loop $\zeta$.]{\scalebox{0.09}{\includegraphics{figs/loop_before.jpg}\label{fig: loop_before}}}
		\hspace{0.1cm}
		\subfigure[After: the images of $v_1,v_2$ are moved out of $\zeta$ to the segment $\sigma$ (shown in red).]{
			\scalebox{0.1}{\includegraphics{figs/loop_after.jpg}}\label{fig: loop_after}}
		\caption{Illustration for the process of opening a loop $\zeta$. \label{fig: loop}}
	\end{figure}
\fi	
	
	
	It remains to add back the edges incident to $v_1,\ldots,v_r$. We denote by $z_1,\ldots,z_r$ the points representing the new images of vertices $v_1,\ldots,v_r$ respectively. 
	%
%Note that the loop $\zeta$ divides the sphere into two face, and we denote by $F$ the face that does not contain segment $\sigma$.
	%
	Let $S$ be an arbitrarily thin strip around $\zeta$, such that the entire segment $\sigma$ is contained in $S$ (see \Cref{fig: thin strip}).
	Let $E_{\zeta}$ be the set of all edges incident to a vertex of $V_{\zeta}$. Clearly, for each edge $e\in E_{\zeta}$, the current image of $e$ has to cross the boundary of $S$. For each $e\in E_{\zeta}$, we denote by $z_e$ the last crossing between the curve $\tilde\phi(e)$ and $S$, where the curve $\tilde\phi(e)$ is viewed as being directed from its endpoint in $V_{\zeta}$ to its endpoint outside of $V_{\zeta}$.
	Now we have obtained two sets $\set{z_e\mid e\in E_{\zeta}}$ and $\set{z_1,\ldots,z_r}$ of points that all lie within $S$ or on the boundary of $S$.
	We now compute, for each edge $e\in E_{\zeta}$ with endpoint $v_i\in V_{\zeta}$, a curve $\xi_e$ connecting $z_i$ to $z_e$ that lies within the thin strip $S$, such that the curves in $\Xi_{\zeta}=\set{\xi_e\mid e\in E_{\zeta}}$ are in general position.
	Then for every $1\le i\le r$ and for every edge $e$ that is incident to vertex $v_i$, we define the curve $\eta_e$ be the concatenation of (i) the curve $\xi_e$; and (ii) the segment of its original image between the last crossing with the boundary of $S$ and the image of its other endpoint in $\tilde\phi$.  
	Note that the curve $\eta_e$ may still intersect $\gamma'$ times. Lastly we modify curve $\eta_e$ as follows. We view it as being directed from its endpoint in $V_{\zeta}$ to its endpoint outside $V_{\zeta}$. Let $p_e$ be a point of $\eta_e$ just before the first point on $\eta_e$ that also belongs to $\gamma'$, and let $p'_e$ be a point of $\eta_e$ just after the last point on $\eta_e$ that also belongs to $\gamma'$. We then replace the subcurve of $\eta_e$ between $p_e$ and $p'_e$ by a new curve that lies within the thin strip around $\gamma'$, and cross $\gamma'$ at most once.
	See \Cref{fig: remove_loop_4} for an illustration.
	Clearly, in this way we obtain a new drawing of the graph $G'$ that no longer has the loop $\zeta$.
	%
	
	\begin{figure}[h]
		\centering
		\subfigure[Segment $\sigma$ is shown in red, with the new images of $v_1,v_2,v_3$ placed on it. $e,e'$ are edges incident to $v_1, v_2$ respectively. Their corresponding curves $\eta_{e},\eta_{e'}$ are shown in pink.]{\scalebox{0.13}{\includegraphics{figs/remove_loop_3.jpg}\label{fig: remove_loop_3}}}
		\hspace{0.1cm}
		\subfigure[The adjusted image of $e'$: now it no longer intersect $\gamma$ more than once.]{
			\scalebox{0.13}{\includegraphics{figs/remove_loop_4.jpg}}\label{fig: remove_loop_4}}
		\caption{Illustration for the process of adding edges back. \label{fig: remove_loop_next}}
	\end{figure}
	
	
	We first show that, after this iteration, the drawing we obtain still induces a drawing of $I'$ that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}.
	Note that we have only modified the images of vertices of $V_{\zeta}$, and the special cycles in $\rset(I')$ are node-disjoint from $K$. 
	Therefore, the image of all special cycles remain the same as in $\tilde\phi$, and so the properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing} are still satisfied.
	
	We now show that, after this iteration, the image of $K$ still does not cross any special edge in $I'$.
	Recall that $K$ crosses no special cycle of $\rset(I')$ in $\tilde\phi$. And note that the new images of edges in $K$ are entirely contained in the image of $K$ in $\tilde\phi$. So after this iteration, in the new drawing we obtained, the image of $K$ still does not cross any special edge in $I'$.
		
	Consider the resulting drawing obtained by processing each self-loop in $Z$ in this way. Finally, we perform type-1 uncrossing to the set of curves representing the images of edges in $E_{\zeta}$. Denote by $\hat \phi$ the resulting drawing.
	It is easy to verify that $\hat\phi$ induces a drawing for instance $I'$ that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}, and moreover, in $\hat \phi$ the image of $K$ is a simple closed curve that does not cross any special edge of $I'$.
	
	We now bound the number of new crossings in the drawing. Consider the iteration where some self-loop $\zeta$ is processed. Note that $|E_{\zeta}|\le \sum_{1\le i\le r}\deg_{G'}(v_i)$.
	Note that, since we have performed type-1 uncrossing to the images of edges in $E_{\zeta}$, the resulting images of edges in $E_{\zeta}$ may create at most $|E_{\zeta}|^2$ new crossings. On the other hand, let $E^*_{\zeta}$ be the set of edges in $E(G')$ that cross the self-loop $\zeta$ in the original drawing $\tilde\phi$, so the new images of $E_{\zeta}$ may create $|E^*_{\zeta}|\cdot |E_{\zeta}|$ new crossings with images of $E^*_{\zeta}$. 
	Finally, since we modified the image of edges in $E_{\zeta}$ such that each of these edges cross $\gamma'$ at most once, the number of intersections between the final images of edges of $E_{\zeta}$ and curve $\gamma'$ is at most $|E_{\zeta}|$. Clearly, these are all new crossings that we may create in an iteration.
	Therefore, summing over all iterations,
	%
	\[
	\cro(\hat\phi)\le \text{ } \cro(\tilde\phi)+\sum_{\zeta \in Z}\bigg(|E_{\zeta}|+|E^*_{\zeta}|+1\bigg)\cdot |E_{\zeta}|
	\le \text{ }  \cro(\tilde\phi)+ \bigg(\sum_{\zeta \in Z}|E_{\zeta}|+|E^*_{\zeta}|\bigg)^2.
	\]
	Since event $\event_1$ does not happen, $\sum_{\zeta \in Z}|E^*_{\zeta}|\le (\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$.
	And from Property \ref{f_prop: no significant in loop}, no significant vertices may belong to any self-loop in $Z$, so the self-loops of $Z$ only contains images of type-1 high-degree vertices and low-degree vertices of $P$.
	Then from Properties \ref{f_prop: K does not cross special edges} and \ref{f_prop: low-degree incident edges small}, $\sum_{\zeta \in Z}|E_{\zeta}|\le O(h\tau^i\mu^{\smallprobability})$.
	Altogether, we get that 
	$$\cro(\hat\phi)\le \text{ } \cro(\tilde\phi)+O\bigg( \frac{\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability}}{m'}+ h\cdot\tau^i\mu^a \bigg)^2=\cro(\tilde\phi)+O\bigg(h^2(\tau^i)^2\mu^{2\smallprobability}\bigg).$$
\end{proof}


\iffalse
$\ $

We say that event $\event$ happens if any of events $\event_1,\event_1,\event_5,\event_3,\event_4$ happens, namely $\event=\event_1\cup\event_1\cup\event_5\cup\event_3\cup\event_4$. From the above discussion, $\Pr[\event]\le O(1/\mu^{\smallprobability})$.
Assuming that event $\event$ does not happen. The properties of the skeleton $K$ can be summarized as follows.

\begin{properties}{F}
	\item $K$ contains at most $\mu^{\interestconst+\smallprobability}$ edges and at most $\mu^{\interestconst+\smallprobability}$ vertices; \label{fact: skeleton is short}
	\item edges of $K$ participate in less than $(\cro\cdot\mu^{\interestconst+\smallprobability})/m$ crossings in $\hat\phi$;\label{fact: skeleton is slightly crossed}
	\item less than $2h'\mu^{\interestconst+\smallprobability}$ edges are incident to a type-1 high-degree vertex of $K$;	
	\label{fact: few incident edges on type-1}
	\item less than $2h\mu^{\interestconst+\smallprobability}$ edges are incident to a low-degree vertex of $K$;
	\label{fact: few incident edges on low-deg}
	\item there is a drawing $\hat\phi'$ of $\hat G'$, such that $\hat \phi'$ obeys the rotation system $\hat \Sigma$, the image of $K$ in $\hat\phi'$ is a simple closed curve, and $\cro(\hat\phi')\le \cro+O(h\mu^{\interestconst+\smallprobability})^2$.\label{fact: skeleton drawn as a cycle}
\end{properties}
\fi




\subsubsection*{Stage 2. Correcting the orientations of vertices in $V(K)$}


%In this step we further modify the drawing $\hat\phi$ obtained in the last step, and then split the drawing $\hat\phi$ into almost well-structured drawings $\hat\phi_1, \hat\phi_2$ for instances $I'_1, I'_2$ respectively.

Recall that we have computed, in Step 2 (\Cref{Step 2}), an orientation $b(v)$ for each vertex $v\in V(K)$, and then used them to define inner and outer sides of $K$, which are then used to compute the instances $I'_1, I'_2$.
%We intend to split the drawing the drawing $\hat\phi$ obtained in the last stage into drawings for instances $I'_1, I'_2$, according to the inner and outer sides of $K$.
However, although the drawing $\hat\phi$ computed in the last stage obeys the rotation system $\Sigma'$, it may not yet match the orientations on vertices of $K$ computed in Step 2, which is required in Property~\ref{prop: first segments} if it induces well-structured solutions for instances $I'_1, I'_2$. In this stage, we further modify $\hat{\phi}$ by correcting the orientations of vertices of $K$.
%\znote{more argument on why orientations need to be computed}

First, we prove the following observations, which show that, for vertex $v''$ and all significant vertices of $K$, the orientation computed in Step 2 is correct (matched by the drawing $\tilde\phi$, and so also matched by $\hat\phi$ since we have not modified the orientations of vertices when constructing $\hat \phi$ from $\tilde\phi$ in the last stage).

\begin{observation}
The orientation $b''$ (computed in Step 2) on vertex $v''$ coincides the orientation of $v''$ in drawing $\tilde\phi$.
%There exists a unique $b''\in \set{-1,1}$ such that $\dist((\oset',b'),(\oset'',b''))\le \cro(\tilde \phi)$.
\end{observation}
\begin{proof}
Observe that the distances between oriented orderings satisfy the triangle inequality, namely for any oriented rotations $(\oset_1,b_1),(\oset_2,b_2),(\oset_3,b_3)$ on the same set of element, $\dist((\oset_1,b_1),(\oset_3,b_3))\le \dist((\oset_1,b_1),(\oset_2,b_2))+\dist((\oset_2,b_2),(\oset_3,b_3))$. In fact, from the definition of the reordering curves, given a set $\Gamma_{12}$ of reordering curves for oriented orderings $(\oset_1,b_1),(\oset_2,b_2)$ and a set $\Gamma_{23}$ of reordering curves for oriented orderings $(\oset_2,b_2),(\oset_3,b_3)$, it is immediate to concatenate curves in $\Gamma_{12}$ with curves in $\Gamma_{23}$ to obtain a set $\Gamma_{13}$ of reordering curves for $(\oset_1,b_1),(\oset_3,b_3)$, such that $\chi(\Gamma_{13})\le \chi(\Gamma_{12})+\chi(\Gamma_{23})$.

On the one hand, since $\oset''$ is an unoriented ordering on a set of $\Omega(m'/\tau^i)$ elements, it is easy to see that $\dist((\oset'',-1),(\oset'',1))=\Omega\big((m'/\tau^i)^2\big)$. Therefore, since $m'\ge \tau^s$ and \fbox{$\cro(\tilde\phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, \[\dist((\oset'',-1),(\oset',b'))+\dist((\oset'',1),(\oset',b'))\ge \dist((\oset'',-1),(\oset'',1))\ge  \Omega\big((\tau^s/\tau^i)^2\big)>2\cdot\cro(\tilde\phi),\] 
and so at most one of $\dist((\oset'',-1),(\oset',b')),\dist((\oset'',1),(\oset',b'))$ is less than $\cro(\tilde\phi)$. 

On the other hand, since the paths of $\pset$ are non-transversal with respect to $\Sigma'$, it is easy to show that paths of $\pset$ participate in at most $\cro(\tilde\phi)$ crossings in drawing $\tilde\phi$, so the orientation $b''$ on $v''$ computed in Step 2 coincides the orientation of $v''$ in $\tilde\phi$. 
%Finally, since we have not modified the orientations of vertices when constructing $\hat \tilde\phi$ from $\tilde\phi$. 
%Altogether, we conclude that there exists an unique $b''\in \set{-1,1}$ such that $\dist((\oset',b'),(\oset'',b''))\le \cro(\tilde \tilde\phi)$.
\end{proof}

\begin{observation}
If event $\event$ does not happen, then for each significant vertex $u\ne v',v''$, the orientation $b(u)$ we computed in Step 2 coincides with the orientation of $u$ in drawing $\tilde\phi$.
\end{observation}
\begin{proof}
%Assume for contradiction that there exists some significant vertex $u\in V(K)$, such that the orientation we computed is different from the orientation $b^*_u$ in drawing $\tilde\tilde\phi$. 
Let $u$ be a significant vertex and let $\pset_u$ be the set of paths in $\pset$ that contains vertex $u$. From the definition of a significant vertex, $|\pset_u|\ge h$.
From Property \ref{f_prop: K crossed few times}, edges of $K$ participates in at most $(\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde\phi$.
%
%For each path $\hat P\in \pset$, if its first edge lies on the inner side of $K$, while its first edge incident to $u$ lies on the outer side of $K$, then it has to cross $K$. Note additionally that in two different orientations of $u$, at least one  orientation of $u$ will force that the first edge of $P$ lies on the inner side of $K$ and the first edge of $P$ incident to $u$ lies on the outer side of $K$. Therefore, there is only one rotation that will not force event $\event_1$ to happen. And therefore the orientation $b(u)$ that we computed has to coincide with the real orientation of $u$ in drawing $\tilde \tilde\phi$. \znote{to modify}
Denote $\pset_u=\set{P_{i_1},\ldots, P_{i_q}}$, and for each $1\le j\le q$, we denote by $e_{i_j}$ the first edge of $P_{i_j}$ (the edge of $P_{i_j}$ incident to $v'$), and denote by $\tilde e_{i_j}$ the first edge of $P_{i_j}$ incident to $u$. Recall that in Step 2, we say that an index $i_j$ is screwed under $b(v)$, iff when the orientation of $v$ is $b(v)$, edges $e_{i_j}, \tilde e_{i_j}$ are on different sides of $K$. It is easy to show that, if index $i_j$ is screwed under $b(v)$, then the image of path $P_{i_j}$ has to cross $K$. It is also easy to see that, each index $i_j$ is screwed under either $-1$ or $1$ but not both.

Since event $\event$ does not happen, from Property \ref{f_prop: K crossed few times}, $K$ participate in at most $(\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'<h/2$ crossings in $\tilde \phi$.
Since $u$ is a type-2 high-degree vertex, there is exactly one orientation in $\set{-1,1}$ under which the number of screwed indices is less than $h/2$. Therefore, the orientation $b(u)$ computed in Step 2 coincides with the orientation of $u$ in drawing $\tilde\phi$.
\end{proof}

Therefore, we only need to modify the orientation of low-degree vertices and type-1 high-degree vertices. We denote by $V'$ the set of all low-degree vertices and all type-1 high-degree vertices $v$ of $V(K)$, such that the orientation of $v$ in the drawing $\hat\phi$ does not coincide with the orientation $b(v)$ computed in Step 2.
Consider now a vertex $v\in V'$.
Assume without loss of generality that $v$ is a vertex of $P$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P$, $\tilde e$ precedes $\tilde e'$ in $P$, and the edges appear clockwise in the oriented ordering $(\oset_v,b(v))$ of $v$.
Denote by $D=D_{\hat \phi}(v)$ the tiny $v$-disc in drawing $\hat \phi$.
Let $\tilde z$ be the intersection between $\hat\phi(\tilde e)$ with the boundary of disc $D$, and we define (i) a point $\tilde z'$ for $\tilde e'$; (ii) for each $1\le i\le p$, a point $ z_i$ for $\hat e_i$; and (iii) for each $1\le j\le q$, a point $ z'_j$ for $\hat e'_j$ similarly. 
See \Cref{fig: flip} for an illustration.
We place a disc $D'$ around $\hat\phi(v)$, that lies entirely within disc $D$. We then place points  $\delta(v)=\set{\tilde y,  y'_1,  y'_2,\ldots,  y'_q,\tilde y',  y_1,  y_2, \ldots,  y_p}$ on the boundary of $D'$, such that the points appear on the boundary of $D'$ clockwise in this order.
We then compute, a set $\Gamma$ of curves within the annulus $D\setminus D'$ that contains, for each $1\le i\le p$, a curve $\gamma_i$ connecting the point $ y_i$ to $ z_i$, and, for each $1\le j\le q$, a curve $\gamma'_j$ connecting the point $ y'_j$ to $ z'_j$, such that the curves of $\Gamma$ are in general position.
We modify the drawing $\hat\phi$ locally within disc $D$ as follows.
We erase the drawing of $\hat\phi$ inside disc $D$ except for the image of vertex $v$ and the images of edges $\tilde e,\tilde e'$. We now let, for each $1\le i\le p$, the new image of edge $\hat e_i$ be the concatenation of: (i) the line segment within $D'$ connecting $\hat\phi(v)$ to point $\hat y_i$; (ii) the curve in $\gamma_i\in \Gamma$ connecting $ y_i$ to $ z_i$; and (iii) the original image of edge $\hat e_i$ outside the disc $D$, namely the subcurve of $\hat\phi(\hat e_i)$ between $ z_i$ and the image of the other endpoint of $\hat e_i$.
Similarly, we let, for each $1\le j\le q$, the new image of edge $\hat e'_j$ be the concatenation of: (i) the line segment within $D'$ connecting $\hat\phi(v)$ to point $ y'_j$; (ii) the curve in $\gamma'_j\in \Gamma$ connecting $ y'_j$ to $ z'_j$; and (iii) the original image of edge $\hat e'_j$ outside the disc $D$, namely the subcurve of $\hat\phi(\hat e'_j)$ between $ z'_j$ and the image of the other endpoint of $\hat e'_j$.
See \Cref{fig: flip} for an illustration.
Clearly, the number of new crossings we have created in this local modification step is at most $\deg(v)^2$.

We modify the drawing $\hat \phi$ at all vertices of $V'$ in the same way, and denote by $\hat \phi'$ the resulting drawing. It is easy to see that drawing $\hat \phi'$ coincides with all oriented orderings on vertices of $K$ computed in Step 2.
Note that, from properties \ref{f_prop: low-degree incident edges small} and \ref{f_prop: type-1 incident edges small}, the total number of edges that are incident to a type-1 high degree vertex or a low-degree vertex is at most $O\big(h\cdot \tau^i\mu^{\smallprobability}\big)$. Therefore,
\[\cro(\hat\phi')\le \cro(\hat\phi)+\sum_{v\in V(K)}
\deg(v)^2\le \cro(\hat\phi)+O\bigg(h^2(\tau^i)^2\mu^{2\smallprobability}\bigg).\]


\begin{figure}[h]
	\centering
	\subfigure[A schematic view of the drawing $\hat\phi$ around $v$.]{\scalebox{0.1}{\includegraphics{figs/rotation_flip_before.jpg}}}
	\hspace{1cm}
	\subfigure[Curves in $\Gamma$ are shown in dash lines.]{
		\scalebox{0.1}{\includegraphics{figs/rotation_flip_after.jpg}}}
	\caption{An Illustration of orientation-flip at $v$ in Stage 2. \label{fig: flip}}
\end{figure}

Since we have only modified the drawing $\hat \phi$ only locally within tiny discs around vertices of $K$, in the resulting drawing $\hat \phi'$, it still holds that the image of $K$ is a simple closed curve that does not cross any special edge. Therefore, drawing $\hat \phi'$ induces almost well-structured solutions for instances $I'_1$ and $I'_2$.
%there exists, for each cycle $R$ in $\rset(I')\cup \set{K}$, a disc whose boundary is the image of $R$ in $\hat\phi'$, such that all discs are disjoint in their interiors.






\subsubsection*{Stage 3. Split the drawing and further modification on vertices}


%From the construction of instances $I'_1=(G'_1,\Sigma'_1)$ and $I'_2=(G'_2,\Sigma'_2)$, graphs $G'_1$ and $G'_2$ are subgraphs of $G'$. We now let drawing $\hat \phi_1$ be the drawing of $G'_1$ induced by drawing $\hat\phi'$, and let drawing $\hat \phi_2$ be the drawing of $G'_2$ induced by drawing $\hat\phi'$. 
So far we have computed a drawing $\hat \phi'$ that induces almost well-structured drawings of instances $I'_1$ and $I'_2$.
%Moreover, since $G'_1\cap G'_2=K$, and the image of $K$ in $\hat\phi'$ is a simple closed curve, we get that $\cro(\hat\phi_1)+\cro(\hat\phi_2)\le \cro(\hat\phi')$.  
However, it does not induce well-structured drawings of $I'_1$ and $I'_2$ yet. In particular, vertices of $I'_1$ and $I'_2$ may be drawn on both sides of $K$ (so Property \ref{prop: discs interior no vertex} is not satisfied), and the number of edges crossing $K$ may be too large (so Property \ref{prop: niubi edge crossing special cycle} is not satisfied).
In this stage and the next stage, we further modify drawing $\hat \phi'$ so that it induces well-structured drawings of instances $I'_1$ and $I'_2$ respectively.

%We show how to construct drawing $\phi_1$, and the construction for drawing $\phi_2$ is symmetric. 
%Recall that one of the instances $I'_1, I'_2$ corresponds to the inner side of $K$, and the other corresponds to the outer side of $K$.
Recall that $I'_1$ corresponds to the inner side of $K$, namely $G'_1=G_{\inn}$.
%We now modify the drawings $\hat\phi_1$ and $\hat\phi_2$. We describe the two steps of modifying the drawing $\hat\phi_1$, and the modification for drawing $\hat\phi_2$ is symmetric.
Also recall that, in drawing $\hat\phi_1$, the image of $K$ is a simple closed curve. We denote by $\eta_K$ this simple closed curve, so $\eta_K$ partitions the sphere into two faces. We denote by $F$ the face that contains the first segments of the images of edges in $E_{\inn}$.
In this stage, we move the image of all vertices of $G'_{1}$ that are currently drawn out of $F$  inside $F$. In the next stage, we move the image of some edges inside $F$ to avoid crossing $K$.

\newcommand{\move}{\mathsf{Move}}

We now start to describe the algorithm in this stage.
We first describe a subroutine called $\move$ and then show how it is used in this stage. 

\paragraph{Subroutine $\move$.} The input to the subroutine $\move$ consists of 
\begin{itemize}
\item a drawing $\psi$ of $G'_1$;
\item a cluster $W$ of $G'_1$; 
\item a disc $D$ such that all vertices of $W$ are drawn outside of $D$ in $\psi$;
\item an edge $e^*_W\in \delta(W)$ such that the endpoint of $e^*_W$ outside $W$ is drawn inside $D$; 
\item a set $\qset$ of paths routing edges of $\delta(W)$ to $e^*_W$ inside $W$; and
\item a set $\pset=\set{P(e)\mid e\in \delta(W)}$ of paths, such that for each $e\in \delta(W)$, the path $P(e)$ has $e$ as its first edge and has the last endpoint drawn inside disc $D$.
\end{itemize}
See \Cref{fig: move_layout} for an illustration.

%We denote by $E'$ the set of edges that cross the image of $K$ in $\hat \phi_1$, and we denote by $E''$ the subset of $E'$ that contains all edges with exactly one endpoint drawn inside $F$. Note that each edge of $E'\setminus E''$ either has both endpoints drawn inside (or on) $F$ or has both endpoints drawn outside (or on) $F$. 

\begin{figure}[h]
	\centering
	\subfigure[Disc $D$ is shown on the left and cluster $W$ is shown on the right. Edges of $\delta(W)$ with the other endpoint drawn inside $D$ are shown in blue, and edges of $\delta(W)$ with the other endpoint drawn outside $D$ are shown in red.]{\scalebox{0.1}{\includegraphics{figs/move_layout_1.jpg}}}
	\hspace{1cm}
	\subfigure[$e^*_W=e_2$, and the paths of $\qset$ are shown in orange dash lines.]{
		\scalebox{0.1}{\includegraphics{figs/move_layout_2.jpg}}}
	\caption{An Illustration of the input to subroutine $\move$. \label{fig: move_layout}}
\end{figure}

The subroutine $\move(\psi, W, D, e^*_W, \qset,\pset)$ outputs a new drawing $\psi'$ of graph $G'_1$ in which the cluster $W$ is drawn inside $D$. We now describe the steps in the subroutine. Denote by $u,u'$ the endpoints of edge $e^*_W$ where $u\notin W$ and $u '\in W$, so the image of $u$ in $\psi$ lies in disc $D$. 
For each edge $e\in\delta(W)$, we denote by $Q(e)$ the path in $\qset$ that routes $e$ to $e^*_W$.
We denote by $p$ the first crossing between the images of $e^*_W$ and $K$ (we view the curve representing the image of $e^*$ as being directed from $u'$ to $u$).
Let $D'$ be a tiny disc that (i) is entirely contained in $D$; (ii) is arbitrarily close to $p$ but does not contain $p$; and (iii) intersects with no other edge than $e^*_W$. See \Cref{fig: move_1} for an illustration. We then construct, for each edge $e\in \delta(W)\setminus \set{e^*_W}$, a curve $\gamma_e$ that consists of (i) a curve that starts at the image of the endpoint of $e$ in $W$, travels through the thin strip of the image of path $Q(e)$, and ends at some point $x_e$ lying in the tiny $u'$-disc $D_{\psi}(u')$; and (ii) a curve that starts at $x_e$, travels through the thin strip of the image of $e^*_W$, and ends at a point $y_e$ on the boundary of $D'$; such that the curves $\Gamma=\set{\gamma_e}_{e\in \delta(W)\setminus \set{e^*_W}}$ are in general position (we will later specify how to choose the ordering in which points in $\set{y_e\mid e\in \delta(W)}$ appear on the boundary of $D'$). 
We also denote by $y_{e^*_W}$ the last crossing of edge $e^*_W$ and the boundary of $D'$ (so the segment of image of $e^*_W$ between $u$ and $y_{e^*_W}$ is disjoint from the interior of $D'$). 
%Note that, we can additionally ensure that, the ordering in which points $\set{y_e}_{e\in \delta(W)}$ appearing on the boundary of disc $D'$ is identical to the ordering in which the intersections of images of $\delta(W)$ with the boundary of $D$ appear on $D$.
See \Cref{fig: move_2} for an illustration.
%\znote{to change: the disc should be close to the boundary of $D$}

\begin{figure}[h]
	\centering
	\subfigure[Drawing $\psi$ and disc $D'$ (shown in light green).]{\scalebox{0.095}{\includegraphics{figs/move_1.jpg}}\label{fig: move_1}}
	\hspace{1cm}
	\subfigure[Curves in $\Gamma$ are shown in dash lines.]{
		\scalebox{0.095}{\includegraphics{figs/move_2.jpg}}\label{fig: move_2}}
	\caption{An Illustration of constructing curves of $\Gamma$.}
\end{figure}

We now erase the image of $W$ from $\psi$ and put it inside $D'$. Lastly, we compute a set $Z$ of curves connecting points in $\set{y_e\mid e\in \delta(W)}$ to the new image of the endpoint of edges in $\delta(W)$. See \Cref{fig: move_inside} for an illustration. %We prove the following observation.
%
We now show in the following observation that we can indeed computing a circular ordering on points in $\set{y_e\mid e\in \delta(W)}$ and the set $Z$ of curves, such that the number of crossings between $Z$ and the new image of $W$ can be charged to the number of crossings in drawing $\psi$.

%\znote{congestion on paths in $\pset$?}

\begin{observation}
\label{obs: inside_disc drawing}
There exists a circular ordering $\oset_Y$ on points in $Y=\set{y_e\mid e\in \delta(W)}$ and a set $Z$ of curves that contains, for each $e\in \delta(W)$, a curve $\zeta_e$ inside disc $D'$ connecting point $y_e$ to the new image of the endpoint of $e$ in $W$, such that the number of crossings between $Z$ and the new image of $W$ is at most the number of crossings between $W$ and paths in $\pset$ in drawing $\psi$.
\end{observation}
\begin{proof}
Let $\hat W$ be the graph obtained from graph $W\cup \delta(W)$ by contracting all outside-$W$ endpoints of edges in $\delta(W)$ into a single vertex, that we denote by $\hat v$. It is easy to verify that, computing a circular ordering $\oset_Y$ on points in $Y$ and a set $Z$ of curves as required in \Cref{obs: inside_disc drawing} is equivalent to computing a circular ordering $\hat\oset$ on the incident edges of $\hat v$ and a drawing $\hat \phi$ of graph $\hat W$ that respect the orderings $\oset_v$ for all $v\in V(W)$ and the new ordering $\hat{\oset}$.

For each edge $e\in \delta(W)$, we consider the curve representing the image of path $P(e)$ in $\psi$, and denote by $y'_e$ the last crossing between this curve and the image of $K$ in $\psi$ (where we view the curve as being directed from its endpoint in $W$ to its endpoint that is drawn inside $D$), and we denote by $\gamma'_e$ the subcurve of this curve between its endpoint in $W$ and $y'_e$. 
%\znote{to modify: the red curves may be disjoint from $K$: use the routing path in property \ref{condition: layered decomposition routing}}
We now define $\hat \oset'$ to be the circular ordering on set $Y'=\set{y'_e\mid e\in \delta(W)}$ in which points of $Y'$ appear on the image of $K$.
Note that the circular ordering $\hat \oset'$ naturally induces a circular ordering on $\delta(W)$ and therefore on the set of incident edges of $\hat v$, that we denote by $\hat \oset$.
We now a drawing $\hat \phi$ of $\hat W$ as follows. We consider the drawing of $W$ induced by $\psi$ and the curves in $\set{\gamma'_e\mid e\in \delta(W)}$. Note that each curve $\gamma'_e$ contains has an endpoint being the image of a vertex of $W$ and the other endpoint $y'_e$ lying on the boundary of $D$. Recall that all vertices of $W$ are drawn outside $D$. We now contract $D$ into a single point, which automatically identify the points in $Y'$. We view this point as the image of $\hat v$. It is easy to see that the drawing obtained in this way is a drawing of $\hat W$ that obeys all circular orderings in $\set{\hat\oset}\cup \set{\oset_v\mid v\in V(W)}$. Moreover, the number of crossings in $\hat \phi$ between the images of edges in $\delta(\hat v)$ and the image of $W$ is at most the number of crossings in $\psi$ between the curves in $\set{\gamma'_e\mid e\in \delta(W)}$ and the image of $W$. \Cref{obs: inside_disc drawing} now follows.
\end{proof}


\begin{figure}[h]
	\centering
	\includegraphics[scale=0.1]{figs/move_3.jpg}
	\caption{An illustration of curves in $Z$ (shown in blue and red solid curves).}\label{fig: move_inside}
\end{figure}


Finally, we set, for each edge $e\in \delta(W)$, the new image of $e$ to be the concatenation of (i) the original image of $e$ in $\psi$; (ii) the curve $\gamma_e$; and (iii) the curve $\zeta_e$. This completes the description of the subroutine $\move(\psi, W, D, e^*_W, \qset,\pset)$.
We denote by $\psi'$ the drawing produced by the subroutine.
Clearly, in $\psi'$, the cluster $W$ is completely drawn inside $D'$ and therefore inside $D$.



We now make some observations on drawing $\psi'$.
From the construction, the original crossings between edges of $W$ remain in the $\psi'$, the original crossings between edges of $\delta(W)$ and edges of $W$ remain in the $\psi'$ (within disc $D'$), since we copied the drawing of $W$ inside $D'$. For each $e\in \delta(W)\setminus \set{e^*_W}$, its new image contains its original image, together with the image of the path $Q(e)$ in $\psi$. Therefore, for each edge $e'\in E(W)\cup\delta(W)$, in the new drawing $\psi'$ there are $\cong_{\qset}(e')$ curves contained in the thin strip of $\psi(e)$.


\iffalse
For each edge $e\in E'$, we view its image $\hat \phi_1(e)$ as being directed from its endpoint in $V'$ to its other endpoint that are drawn inside $F$, and we denote by $z_e$ the first crossing between $e$ and $K$. 
Define $\hat G$ as the graph obtained from $G_{\inn}$ by splitting each edge $e\in E'$ with a new vertex $x_e$, and we denote $X=\set{x_e\mid e\in E'}$.
Clearly, if we view, for each vertex $x_e\in X$, the point $z_e$ as its image, then the drawing $\hat \phi_1$ naturally induces a drawing of $\hat G$. 
For each edge $e\in E'$, we denote by $e^{a}$ the new edge split from $e$ that is incident to the endpoint of $e$ in $V'$, and we denote by $e^{b}$ the other edge split from $e$.
We define $E^a=\set{e^a\mid e\in E'}$ and  $E^b=\set{e^b\mid e\in E'}$.
See \Cref{fig: well-structured_layout} for an illustration.
We now pick an arbitrary vertex $x_{e^*}\in X$. Let $z^*$ be a point in the intersection of the tiny-$x_{e^*}$ disc $D'=D_{\hat \phi_1}(x_{e^*})$ and $F$. Let $D^*$ be a tiny-$z^*$ disc that lies entirely in the intersection of the $D'\cap F$.

\begin{figure}[h]
	\centering
	\subfigure[Disc $D$ is shown on the left and cluster $W$ is shown on the right. Edges of $\delta(W)$ with the other endpoint drawn inside $D$ are shown in blue, and edges of $\delta(W)$ with the other endpoint drawn outside $D$ are shown in red.]{\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_1.jpg}}}
	\hspace{1cm}
	\subfigure[]{
		\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_2.jpg}}}
	\caption{An Illustration of the input to subroutine $\move$. \label{fig: well-structured_layout}}
\end{figure}


Define $H'=H\cup E^a$.
We erase the drawing of $H'$ from drawing $\hat \phi_1$, and place the drawing $\hat \phi_1(H)$ of $H$ inside disc $D^*$, such that the new images of vertices of $X$ lie on the boundary of $D^*$. We now add the edges of $E^b$ back to the drawing as follows. Let $\zeta$ be the segment of $\partial F$ that lies in disc $D'$. We first designate, for each vertex $x_e\in X$, a distinct point $y_e$ on $\zeta$. We then compute a set $\gamma$ of curves that contains, for each vertex $x_e\in X$, a curve $\gamma_e$ that connects $z_e$ to $y_e$ and lies entirely outside of $F$, such that every pair of curves in $\Gamma$ crosses at most once. Finally, we let the new image of $e_2$ be the sequential concatenation of: (i) the previous image of $e_2$ between its endpoints originally drawn inside $F$ to the point $z_e$; and (ii) the curve $\gamma_e$ in $\Gamma$. In this way we obtain a new drawing of graph $\hat G$, and suppressing vertices of $X$, this drawing also induces a drawing of $G_1$, with all vertices lying inside $F$. We then perform type-1 uncrossings (the algorithm from \Cref{thm: type-1 uncrossing}) to the images of all edges in $E'$. We denote by $\phi'_1$ the resulting drawing. See \Cref{fig: well-structured_drawing} for an illustration.
It is easy to observe that, in the resulting drawing, the set of edges that cross $K$ is still $E'$.

\begin{figure}[h]
	\centering
	\subfigure[Before: disc $D^*$ is shown in ligh blue, and segment $\zeta$ is shown in black.]{\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_3.jpg}}}
	\hspace{0.2cm}
	\subfigure[After: drawing of $H'$ is moved into $D^*$, and the new images of edges of $E^a, E^b$ are shown in pink and red, respectively.]{
		\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_4.jpg}}}
	\caption{An Illustration of drawing modification in Stage 3. \label{fig: well-structured_drawing}}
\end{figure}
\fi




We now describe the algorithm in the third stage, that utilizes the subroutine $\move$ and iteratively move the images of all vertices inside $F$.
We start from the drawing $\hat\phi_1$.
Let $V'$ be the set of vertices whose image in $\hat \phi_1$ lie outside $F$, and let $H$ be the subgraph of $G'_1$ induced by vertices of $V'$. %Denote $E'=\delta_{G_{\inn}}(V')$. It is clear that every edge of $E'$ crosses $K$ in $\hat\phi_1$.
We first apply the algorithm from \Cref{thm: layered well linked decomposition} to graph $G'_1$ and its subgraph $G'_1\setminus H$ to compute a layered $\alpha$-well-linked decomposition $(\wset, \lset_1,\ldots,\lset_r)$ of graph $G'_1$ with respect to $G'_1\setminus H$, for $\alpha=O(1/\log^{2.5} m)$.
Now for each cluster $W\in \wset$, we select uniformly at random an edge of $\delta^{\down}(W)$ as $e^*_W$ and then use the algorithm from 
\Cref{cor: simple guiding paths}
%\znote{To add: boundary all to all routing in a well-linked cluster} 
to compute a collection $\qset_W$ of paths routing edges of $\delta(W)\setminus \set{e^*_W}$ to $e^*_W$ (note that, instead of selecting a path set in $\set{\qset^{(e)}\mid e\in \delta(W)}$ uniformly at random, we select a path set in $\set{\qset^{(e)}\mid e\in \delta^{\down}(W)}$ uniformly at random).
Then, we iteratively modify the current drawing $\hat \phi_1$ as follows.
Throughout, we maintain a drawing $\tilde \phi$ of $G'_1$, that is initialized to be $\hat \phi_1$. 
The algorithm continues to be executed as long as there is still some cluster $W\in \wset$ whose image in the current drawing $\tilde \phi$ lies outside $F$.
In each iteration, we select a cluster $W$ of $\wset$, that, among all clusters of $\wset$ that are drawn outside of $F$, minimizes the layer index of the layered $\alpha$-well-linked decomposition that it belongs to.
Clearly, at this moment all clusters from lower layers than $W$ are already moved into $F$ in the current drawing $\tilde \phi$. Since edge $e^*_W$ is chosen from $\delta^{\down}(W)$, the endpoint of $e^*_W$ outside $W$ lies inside $F$ in $\tilde \phi$.
We then run the subroutine $\move(\tilde\phi, W, F, e^*_W, \qset_W)$, and update $\tilde{\phi}$ with the drawing output by the subroutine. We denote by $\phi_1$ the resulting drawing after we processed all clusters of $\wset$ in this way.




%We now count the number of new crossings created in this step. From the algorithm, we may create new crossings between edges of $E'$, but except from that, we create one new crossing between each edge of $E'$ with $K$ (for each $e\in E'$ the new crossing is point $y_e$). Therefore, the total number of new crossings is at most $|E'|+|E'|^2\le 2|E'|^2$.

\newcommand{\load}{\mathsf{load}}

In order to analyze the new crossings created in this stage and prepare for the next stage, we define \emph{load} on edges of $E(H)\cup\delta(H)$, based on the edges $\set{e^*_W}_{W\in \wset}$ and paths sets of $\set{\qset_W}_{W\in \wset}$, as follows.
First consider a cluster $W\in \lset_r$. For each edge of $\delta(W)\setminus \set{e^*_W}$, we define its load to be $0$; for edge $e^*_W$, we define its load to be $|\delta(W)|$. 
For each edge $e\in E(W)$, we define its load to be $\cong_W(\qset_W,e)$.
Assume now that the load for each edge with at least one endpoint lying in $\bigcup_{j+1\le t\le r}V(\lset_t)$ are already defined. Consider now a cluster $W\in \lset_j$. For each edge of $\delta(W)\setminus \set{e^*_W}$ whose load is not yet defined (the edges of $\delta(W)$ with the other endpoint lying in $\bigcup_{1\le t\le j}V(\lset_t)$), we define its load to be $0$; for edge $e^*_W$, we define its load to be the sum of load of all other edges of $\delta(W)$ (notice that the load of all such edges are already defined at this point). For each edge $e\in E(W)$, we define the load of $e$ to be the sum of load of all edges of $\delta(W)$ whose corresponding path in set $\qset_W$ contains edge $e$. This completes the definition of load on all edges of $E(H)\cup\delta(H)$. 
Note that, since the edges $\set{e_W}_{W\in \wset}$ and path sets $\set{\qset_W}_{W\in \wset}$ are chosen randomly, the load on edges of $E(H)\cup\delta(H)$ are random variables.
We prove the following observation.

\begin{observation}
\label{obs: expected load}
For each edge $e\in E(H)\cup\delta(H)$, $\expect[]{\load(e)}=O(\log^{O(1)} m)$.
\end{observation}

\begin{proof}
Note that $E(H)=E^{\out}(\wset)\cup (\bigcup_{W\in \wset}E(H))$.	
%
We first consider the edges of $E^{\out}(\wset)\cup \delta(H)$.
Let $1\le j\le r$ be a layer index and denote $V_j=\bigcup_{j\le t\le r}V(\lset_t)$.
We show by induction on $j$ that, for each edge
$e\in E^{\out}(\wset)$ with at least one endpoint lying in $V_j$, $\expect[]{\load(e)}\le (1+1/\log m)^{r+1-j}$. The base case is when $j=r$. Consider a cluster $W\in \lset_r$. From Property \ref{condition: layered decomp edge ratio} in the definition of a layered well-linked decomposition, $|\delta^{\up}(W)|\le |\delta^{\down}(W)|/\log m$. Since the edge $e^*_W$ is picked uniformly at random from edges of $\delta^{\down}(W)$, the expected load on each edge of $\delta^{\up}(W)$ is $0$, and the expected load on each edge of $\delta^{\down}(W)$ is $|\delta(W)|/|\delta^{\down}(W)|=(|\delta^{\up}(W)|+|\delta^{\down}(W)|)/|\delta^{\down}(W)|\le (1+1/\log m)$.
Assume now that the claim is true for layers $r,\ldots,j+1$. Consider now a cluster $W\in \lset_j$. From the inductive hypothesis, from the linearity of expectations, the expected load of every edge of $\delta(W)$ with the other endpoint lying in $V_{j+1}$ is at most $(1+1/\log m)^{r-j}$. From the definition of load, the load of every edge that connects two distinct clusters of $\lset_j$ is $0$. On the other hand, $|\delta(W)|/|\delta^{\down}(W)|\le (1+1/\log m)$. Therefore, since the edge $e^*_W$ is picked uniformly at random from set $\delta^{\down}(W)$, the expected load on each edge of $\delta^{\down}(W)$ is at most $(1+1/\log m)^{r-j}\cdot (|\delta(W)|/|\delta^{\down}(W)|)\le (1+1/\log m)^{r+1-j}$. As a corollary, the expected load for every edge of $E^{\out}(\wset)\cup \delta(H)$ is at most $(1+1/\log m)^{r}\le O(1)$ (as $r\le \log m$ from \Cref{thm: layered well linked decomposition}).

We now consider edges of $\bigcup_{W\in \wset}E(H)$. Let $W$ be a cluster of $\wset$. From \Cref{cor: simple guiding paths} and our construction, for each edge $e\in E(W)$, $\expect[]{\cong_W(\qset_W,e)}=O(\log^{O(1)} m)$.
Note that the choice of path set $\qset_W$ is independent of the load on edges of connecting $W$ to a vertex in $V_{j+1}$.
Since the expected load for each edge of $\delta(W)$ is $O(1)$, from the definition on loads of edges of $E(H)$ and the linearity of expectations, $\expect[]{\load(e)}=O(\log^{O(1)} m)$. This completes the proof of \Cref{obs: expected load}.
\end{proof}




We now analyze the number of new crossings created in this stage. First, from the construction, in each iteration we move the drawing of some cluster $W\in \wset$ into some tiny disc inside $F$, so their new image do not cross the image of $G'_1\setminus H$. 

\znote{informal from here}
Then from the algorithm, the new image of each cluster $W\in \wset$ participate in at most the same number of crossings as in the original drawing $I'$, with the additive term being $\cro(\tilde \phi)/\mu^{\smallprobability}$ (allowing pairs of edges that cross $K$ to cross). Since we have not modified the image of $G'_1\setminus H$, the new crossings must each involve at least one edge of $E^{\out}(\wset)\cup\delta(H)$. Note that each edge of $\delta(H)$ has to cross $K$ in drawing $\tilde \phi$, and $K$ participates in at most $(\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde \phi$. Therefore, $|\delta(H)|\le (\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'$. Moreover, from the definition of a layered well-linked decomposition, $|E^{\out}(\wset)|\le O(|\delta(H)|)$, so 
\[|E^{\out}(\wset)\cup\delta(H)|=O((\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m').\]
Therefore, the number of new crossings that involve a pair of edges in $E^{\out}(\wset)\cup\delta(H)$ is at most 
\[
O((\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m')^2\le O(\cro(\tilde \phi)/\mu^{\smallprobability}),
\]
where we have used the fact that $m'\ge \tau^s$ and \fbox{$\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}.

Denote $E'=E^{\out}(\wset)\cup\delta(H)$.
Lastly, for each edge $e\in E'$, in the new drawing there are $\load(e)$ images lying in the thin strip of the original image of $e$, so the number of crossings that involve $e$ is multiplied by a factor of $\load(e)$.
%\znote{to be taken care of later}




\subsubsection*{Stage 4. Further modification on edges}

%\iffalse
We now describe the last stage, in which we move the image of some edges inside $F$.

We say that a vertex $v\in V(K)$ is \emph{heavy} iff $v$ is contained in at least $m/(\tau^i)^{5}$ paths of $\pset$, otherwise we say it is \emph{light}.
We prove the following observations.

\begin{observation}
	\label{obs: few edges incident to non-heavy edges}
	The expected number of edges in $G'$ that is incident to a light vertex of $V(K)$ is $O(m'/(\tau^i)^{4})$.
\end{observation}
\begin{proof}
	Let $v$ be a light vertex. Since it belongs to at most $m'/(\tau^i)^{5}$ paths in $\pset$, the probability that $v$ belongs to path $P$ is $O((m'/(\tau^i)^{5})/(m'/\tau^i))=O(1/(\tau^i)^4)$. Therefore, for an edge $e\in E(G')$ that is incident to a type-1 high-degree vertex, the probability that its type-1 high-degree endpoint belongs to $P$ is $O(1/(\tau^i)^4)$. From the union bound on all edges in $E(G')$, the expected number of edges that are incident to some type-1 high-degree vertex on $P$ is $O(m'\cdot O(1/(\tau^i)^4))=O(m'/(\tau^i)^{4})$. 
	The proof for path $P'$ is symmetric. Therefore, the expected number of edges in $G'$ that is incident to a non-heavy vertex of $V(K)$ is $O(m'/(\tau^i)^{4})$.
\end{proof}

\paragraph{Bad Event $\event_6$.}
We say that the bad event $\event_6$ happens if the number of edges in $G'$ incident to a light vertex of $V(K)$ is at least $m'\cdot\mu^{\smallprobability}/(\tau^i)^{4}$. 
From \Cref{obs: few edges incident to non-heavy edges} and Markov's bound, $\Pr[\event_6]\le O(1/\mu^{\smallprobability})$.

Consider now an edge $e\in E'$. Note that both its endpoints are drawn inside (or on) $C$.

%\fi



\paragraph{Clean edges.} Consider now the resulting drawing $\phi_1$ in the last stage. 
Recall that $E'=E^{\out}(\wset)\cup\delta(H)$, and in $\phi_1$ only edges of $E'$ may cross $K$.
We say that an edge $e\in E'$ is clean, iff, when we denote by $x_1,x_2,\ldots,x_k$ the crossings between $e$ and $K$, where the crossings are indexed according to their appearance on the image of $e$, such that, for each even $1\le i\le k$, the subcurve of the image of $e$ between $x_i$ and $x_{i+1}$, which we denote by $\gamma_i(e)$, lies entirely outside $F$, and moreover, one of the two segments of the image of $K$ separated by points $x_i,x_{i+1}$ contains no heavy vertices.

We prove the following claim.

\begin{claim}
The number of non-clean edges is at most $O(\mu^{2\smallprobability}(\tau^i)^{10})$.
\end{claim}





==> many_paths_main_decomposition_analysis_backup.tex <==

\subsubsection{Analysis of the algorithm}
\label{subsec: analysis of decomposition lemma}

In this subsection we provide the proof of \Cref{lem: many path main} with some details deferred to subsequent sections.
%by showing that the instances in collection $\iset$ satisfy the properties \ref{prop: well-structured and contracted}--\ref{prop: well-structured solutions}.

First, note that initially the collection $\hat{\iset}$ contains one well-structured subinstance, and from the description of the algorithm, in each iteration we replace one well-structured subinstance in $\hat{\iset}$ with two new well-structured subinstances. Therefore, all subinstances in the resulting collection $\iset$ are well-structured subinstances. On the other hand, recall that the recursive algorithm continues to be executed as long as there exists some instance $I'\in \hat\iset$, such that its contracted subinstance $\tilde I'$ is $\tau^i$-wide and not $\tau^s$-small. Therefore, when the algorithm terminates, property \ref{prop: well-structured and contracted} has to be satisfied.

Second, note that in each iteration, we start with an instance $I'$ in the current collection $\hat \iset$, compute a cycle $K$ that is edge-disjoint from all special cycles in $\rset(I')$ and then decompose instance $I'$ into two subinstances $I_{\inn}$ and $I_{\out}$, such that only edges of $E(K)$ appear in both instances. Therefore, if an edge in the input instance $I'$ is not a special edge of any subinstance that ever appeared in $\hat \iset$, then it either belongs to exactly one resulting instance or belongs to set $E^{\sf del}$; otherwise it eventually belongs to exactly two resulting instances. Therefore, property \ref{prop: edge appearance} holds.
%Second, when an instance $I'$ in the collection $\hat \iset$ is replaced by two instances $I_{\inn}$ and $I_{\out}$, according to algorithm, the edge sets $\hat E(I'_1), \hat E(I'_2)$ are disjoint subsets of $\hat E(I')$. Therefore, eventually the subsets $\set{\hat E(I')\mid I'\in \iset}$ of edges are mutually disjoint, which means property \ref{prop: private edges disjoint} is satisfied.




In order to show that the properties \ref{prop: well-structured solutions}--\ref{prop: number of crossings} also hold and there exists an efficient algorithm $\alg(\iset)$ that satisfies the properties required in \Cref{lem: many path main}, it is convenient for us to associate a tree $T$ with the algorithm, called the \emph{partitioning tree}. Each vertex of $T$ corresponds to a well-structured subinstance that once appeared in the collection $\hat{\iset}$. We grow the tree $T$ along with the iterative algorithm as follows. Initially, $T$ contains a single root denoted by $v(I)$, where $I$ is the input well-structured subinstance to \Cref{lem: many path main}. Consider now some vertex $v(I')$ in $T$, where $I'$ is a subinstance that undergoes Steps 1, 2 and 3. From the algorithm, the instance $I'$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$. We then create two nodes, $v(I_{\inn})$ and  $v(I_{\out})$, that become the child vertices of $v(I')$ in $T$.


\subsubsection*{Number of Iterations}

We first analyze the number of the iterative algorithm using $T$. We use the following observation.

\begin{observation}
\label{obs: number of iterations}
If \fbox{$\tau^s\ge 100\cdot\tau^i\mu^{10\interestconst}$}, then 
%with probability $1-O(m\tau^i/\tau^s\mu^a)$
$|V(T)|\le 200\cdot m\tau^i/\tau^s$.
\end{observation}
\begin{proof}
%Consider the first $M=1000m\tau^i/\tau^s$ iterations of the algorithm. We show that, if event $\event_1$ did not happen in the first $M$ iterations, then $|V(T)|\le M$. Note that this implies that \Cref{obs: number of iterations}, since the probability that $\event_1$ happens in at least one of the first $M$ iterations is $O(m\tau^i/\tau^s\mu^a)$.
We show that, if $\tau^s\ge 100\cdot\tau^i\mu^{10\interestconst}$, then the algorithm will terminate in $200\cdot m\tau^i/\tau^s$ iterations, which implies \Cref{obs: number of iterations}.
%
%We say that an iteration of the algorithm is \emph{good}, iff $\event_1$ did not happen in this iteration. Let $I'$ be an instance that once appeared in $\hat \iset$, we say that the algorithm is \emph{good on $I'$}, iff either node $v(I')$ is a leaf of $T$, or the iteration of processing instance $I'$, and the iterations of processing instances $I''$ where $v(I'')$ is a descendant of $v(I')$ in $T$, are all good.
%
In fact, we will show that, for each subinstance $I'=(G',\Sigma')$ that ever appeared in $\hat \iset$, 
%if the algorithm is good on $I'$, then 
the number of vertices in the subtree of $T$ rooted at node $v(I')$, which we denote by $N_{T}(I')$, is at most $$f(I')=\max\set{\frac{|E(G')|-\tau^s}{\tau^s/100\tau^i},0}+3,$$
which, when applied to the initial instance $I=(G,\Sigma)$ where $|E(G)|=m$, immediately implies that the algorithm will terminate in $200\cdot m\tau^i/\tau^s$ iterations.

Consider now an instance $I'$ that once appeared in $\hat \iset$. Assume first that $v(I')$ is a leaf of $T$, then the number of vertices in the subtree of $T$ rooted at node $v(I')$ is $1$, which is at most $f(I')$ (note that $f(I')\ge 3$ always holds).
Assume now that $v(I')$ is not a leaf of $T$, we let $I'_1=(G'_1,\Sigma'_1)$, $I'_2=(G'_2,\Sigma'_2)$ be two new instances constructed the iteration of processing $I'$. Since $|E(K)|\le 2\tau^i\cdot\mu^{10\interestconst}$, from \Cref{obs: number of edges in base} and the definition of $\event_1$, $|E(G'_1)|+|E(G'_2)|\le |E(G')|+2\tau^i\cdot\mu^{10\interestconst}$ and
$|E(G'_1)|, |E(G'_2)|\le |E(G')|-\tau^s/6\tau^i$. We consider the following cases.

\textbf{Case 1. Both nodes $v(I'_1), v(I'_2)$ are leaves of $T$.}
In this case, $N_T(I')\le 3 \le f(G')$.

\textbf{Case 2. One of the nodes $v(I'_1), v(I'_2)$ is a leaf of $T$.}
Assume without loss of generality that $v(I'_1)$ is a leaf and $v(I'_2)$ is not a leaf, so $|E(G')|-\tau^s/6\tau^i\ge |E(G'_2)|\ge \tau^s$, so 
\[
\begin{split}
N_{T}(I')=2+N_{T}(I'_2)\le 2+f(I'_2)= & \text{ }2+ \frac{|E(G'_2)|-\tau^s}{\tau^s/10\tau^i}+3
\\
\le  & \text{ } 2+ \frac{|E(G')|-(\tau^s/6\tau^i)-\tau^s}{\tau^s/100\tau^i}+3
\\
\le  & \text{ } 2+ \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}-16+3
\\
\le  & \text{ } \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}+3 =f(I').
\end{split}
\]

\textbf{Case 3. Both nodes $v(I'_1), v(I'_2)$ are not leaves of $T$.}
Then $|E(G'_1)|, |E(G'_1)|\ge \tau^s$, and so
\[
\begin{split}
N_{T}(I')\le 1+N_{T}(I'_1)+N_{T}(I'_2)\le & \text{ } 1+f(I'_1)+f(I'_2)
\\ 
= & \text{ } 7+ \frac{|E(G'_1)|-\tau^s}{\tau^s/100\tau^i}+\frac{|E(G'_2)|-\tau^s}{\tau^s/100\tau^i}
\\
\le & \text{ } 7+ \frac{|E(G')|+2\tau^i\cdot\mu^{10\interestconst}-2\tau^s}{\tau^s/100\tau^i}
\\
\le  & \text{ } 7+ \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}
+
\frac{2\tau^i\cdot\mu^{10\interestconst}-\tau^s}{\tau^s/100\tau^i}
\\
\le  & \text{ } \frac{|E(G')|-\tau^s}{\tau^s/100\tau^i}+3 =f(I'),
\end{split}
\]
where the last inequality uses the fact $\tau^s\ge 100\tau^i\mu^{10\interestconst}$.
%Therefore, if the algorithm is good on the input instance $I=(G,\Sigma)$, then $|V(T)|\le 100m\tau^i/\tau^s\le M$. This means that if the event $\event_1$ does not happen in the first $M$ iterations, then the algorithm is good on the input instance $I$, and therefore $|V(T)|\le M$.
\end{proof}


%\paragraph{Bad Event $\event^*$.}We say that the bad event $\event^*$ happens iff the iterative algorithm does not terminate in $M=1000 m\tau^i/\tau^s$ iterations. From \Cref{obs: number of iterations}, $\Pr[\event^*]\le O(m\tau^i/\tau^s\mu^a)$.


\iffalse{number of all special edges}
As an immediate corollary, we have the following bound the number of special edges in all resulting instances in $\iset$.

\begin{corollary}
\label{cor: number of special edges}
The total number of special edges in all instances in $\iset$ is at most
$800m(\tau^i)^2\mu^{10\interestconst}/\tau^s$.
\end{corollary}
\begin{proof}
From \Cref{obs: 2 new special cycles}, after each iteration, the number of special cycles in all subinstances in the collection $\hat\iset$ increases by $2$. Since the number of iterations is bounded by $200\cdot m\tau^i/\tau^s$, and the length of each special cycle is at most $2\tau^i\cdot\mu^{10\interestconst}$, we get that the total number of special edges in all resulting instances in $\iset$ is bounded by
$2\cdot \big(200\cdot m\tau^i/\tau^s\big)\cdot \big(2\tau^i\cdot\mu^{10\interestconst}\big)=800m(\tau^i)^2\mu^{10\interestconst}/\tau^s$.
\end{proof}
\fi

We now proceed to analyze the iterative algorithm using the partitioning tree $T$. 
We will maintain a well-structured drawing $\tilde \phi$ of the input instance $I=(G,\Sigma)$, that is initialized to be the input well-structured drawing $\phi$ of $I$ and evolves as the iterative algorithm proceeds.



\znote{the correct notion and claim?}

We denote by $\bar I$ the well-structured instance obtained from $I$ by only deleting from it the edges of $\hat E^{\sf del}$. As more edges are added to set $\hat E^{\sf del}$, the instance $\bar I$ evolves, and it is easy to verify that eventually instance $\bar I$ becomes the output instance $\hat I$.
We say that a well-structured drawing $\tilde \phi$ of instance $\bar I$ is \emph{well-structured with respect to the current collection $\hat \iset$}, iff for each subinstance $I'\in \hat\iset$, the drawing of $I'$ induced by $\tilde \phi$ is a well-structured drawing of $\iset$.
We first focus on an iteration, in which some instance $I'=(G',\Sigma')$ in collection $\iset$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$.

\begin{observation}
\label{obs: not crossing your own special then not crossing any special}
Let $\phi$ be a drawing of instance $\bar I$ that is well-structured with respect to the current collection $\hat \iset$. For an edge $e$ that belongs to a unique instance $I'\in \hat \iset$, if $e$ does not cross any special edge of $I'$ in $\tilde \phi$, then $e$ does not cross any special edge of any instnace of $\hat \iset$ in $\tilde \phi$.
\end{observation}
\begin{proof}
\znote{to complete}
\end{proof}


We use the following claim.
%Let $\tilde \phi$ be a well-structured solution for instance $I'$. We will construct well-structured solutions $\phi(I_{\inn})$, $\phi(I_{\out})$ for subinstances $I_{\inn}$ and $I_{\out}$, respectively, and then show that $\cro(\phi(I_{\inn}))+\cro(\phi(I_{\out}))$ is not much larger than $\cro(\tilde \phi)$. We denote $m'=|E(G')|$. Recall that in Step 1 we computed a cycle $K$ that consists of two internally disjoint paths $P,P'$ and is a subgraph of the input graph $G$.

%Recall that $\phi^*$ is optimal well-structured drawing of the input well-structured instance $I=(G,\Sigma)$ and $\cro=\cro(\phi^*)$.

%\znote{some lemma here summarizing, and finish the proof of \Cref{lem: many path main} before providing the proof of lemma}



\begin{claim}
\label{lem: well-structured drawing splitting}
Consider an iteration of the algorithm in which a well-structured instance $I'=(G',\Sigma')$ is processed and eventually replaced by two new well-structured instances, that we denote by $I_{\inn}, I_{\out}$.
Let $\tilde \phi$ be a well-structured drawing of $\bar I$ with respect to the collection $\hat\iset$ before this iteration. 
Then there exists a well-structured drawing $\tilde \phi'$ of $\bar I$ with respect to the collection $\hat\iset$ after this iteration, such that 
\begin{itemize}
\item for each special cycle $R$ in the collection $\hat\iset$ before this iteration, its images in drawings $\tilde\phi$ and $\tilde \phi'$ are identical, and the disc $D_R$ it defines in $\phi$ and $\hat \phi$ are the same; for each edge $e\in E(\hat G)$ and each special cycle $R\in \rset$: either in both $\phi$ and $\hat \phi$, the image of $e$ is disjoint from the interior of disc $D_R$, or the intersections of the image of $e$ with the interior of disc $D_R$ are identical in $\phi$ and $\hat \phi$; and
\item if \fbox{$\cro(\tilde\phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, then
$\cro(\tilde\phi')\le \cro(\tilde \phi)\cdot(1+1/\mu^{\smallprobability})$.
\end{itemize}
\end{claim}

We provide the proof of \Cref{lem: well-structured drawing splitting} in \Cref{sec: Proof of well-structured drawing splitting}, after we complete the proof of \Cref{lem: many path main} using \Cref{lem: well-structured drawing splitting}.




\subsubsection{Proof of \Cref{lem: well-structured drawing splitting}}
\label{sec: Proof of well-structured drawing splitting}

In this subsection we provide the proof of \Cref{lem: well-structured drawing splitting}, thus completing the proof of \Cref{lem: many path main}.

We focus on an iteration, in which some instance $I'=(G',\Sigma')$ in collection $\iset$ is replaced by two new subinstances $I_{\inn}$ and $I_{\out}$.
We denote $m'=|E(G')|$.
Recall that currently we have a drawing $\tilde\phi$ of the instance $\bar I$ before this iteration, that is well-structured with respect to the collection $\hat\iset$ before this iteration.
Recall that in Step 1 we computed a cycle $K$ that consists of two internally disjoint paths $P,P'$ and is a subgraph of the input graph $G$.
We first show several crucial properties of $K$.

\subsubsection*{Properties of $K$}

We prove the following observations on cycle $K$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

\begin{observation}
\label{obs: skeleton number of crossings}
The expected number of crossings in $\tilde\phi$ that involve edges of $K$ is $O(\cro(\tilde\phi)\cdot\tau^i/m')$.
\end{observation}
\begin{proof}
	%We define the edge-disjoint subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ in the same way as \Cref{obs: skeleton number of edges}. 
	For each index $0\le z\le \floor{L/2}-1$, we denote by $\tilde K_z$ the subgraph formed by the union of the path in $\pset$ whose first edge is $e_z$ and the path in $\pset$ whose first edge is $e_{z+\floor{L/2}}$.
	Since the subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ are edge-disjoint, the expected number of crossings in $ \tilde \phi$ that involve an edge in a random subgraph in $\set{\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}}$ is at most $O(\cro(\tilde \phi)/L) < O( \cro(\tilde \phi)\cdot\tau^i/m')$.
	Since $K\subseteq \tilde K$, we get that the expected number of crossings in $\tilde\phi$ that involve edges of $K$ is at most $O(\cro(\tilde\phi)\cdot\tau^i/m')$.
\end{proof}



\paragraph{Bad Event $\event_1$.}
We say that the bad event $\event_1$ happens iff the edges of $K$ participate in more than $(\cro(\tilde \phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde \phi$.
From \Cref{obs: skeleton number of crossings} and Markov's bound, $\Pr[\event_1]\le O(1/\mu^{\smallprobability})$.

\begin{observation}
	\label{obs: skeleton paths not crossing each other}
	If \fbox{$\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, and event $\event_1$ does not happen, then the images of $P$ and $P'$ do not cross in $\tilde \phi$.
\end{observation}
\begin{proof}
The proof of \Cref{obs: skeleton paths not crossing each other} is similar to the proof of Claim 9.9 in \cite{chuzhoy2020towards}.
	
Assume the contrast that the images of $P$ and $P'$ cross in $\tilde\phi$, then there is a pair of edges $e\in E(P)$, $e'\in E(P')$ whose images cross in $\tilde\phi$. Consider the curve $\tilde\phi(P)$, that we view as being directed from $v'$ to $v''$. Let $p$ be the first point on this curve that belongs to the curve $\tilde\phi(P')$ and is not the image of a vertex. Let $\gamma$ be the simple curve connecting $\tilde\phi(v')$ to $p$, that is obtained from the segment of $\tilde\phi(P)$ from $\tilde\phi(v')$ to $p$ by deleting all its loops. We define the simple curve $\gamma'$ similarly. Note that the curves $\gamma$ and $\gamma'$ can contain other common points which are vertex-images in $\tilde\phi$, but they cannot cross at those points. 
	
	For every vertex $u\neq v'$ whose image is contained in both $\gamma$ and $\gamma'$, let $D_{\tilde\phi}(u)$ be the tiny-$u$ disc in $\tilde\phi$, and we modify the curves $\gamma$ and $\gamma'$ so that they are disjoint from the interior of $D_{\tilde\phi}(u)$, and instead follow its boundary on either side (see Figure~\ref{fig: curve_separation}). 
	%
	\begin{figure}[h]
		\centering
		\subfigure[The curves $\gamma$ and $\gamma'$ touch at the image of $u$ in $\tilde\phi$.]{\scalebox{0.13}{\includegraphics{figs/curve_separation_before.jpg}}}
		\hspace{0.1cm}
		\subfigure[The curves $\hat \gamma,\hat \gamma'$ share only endpoints $p$ and $\tilde\phi(v')$.]{
			\scalebox{0.13}{\includegraphics{figs/curve_separation_after.jpg}}}
		\caption{Illustration for the proof of \Cref{obs: skeleton paths not crossing each other}. \label{fig: curve_separation}}
	\end{figure}
	%
	Let $\hat \gamma$ and $\hat \gamma'$ denote the resulting two curves. Then the union of $\hat \gamma$ and $\hat \gamma'$ defines a closed simple curve that we denote by $\lambda$. Curve $\lambda$ partitions the plane into two faces, $F$ and $F'$. We assume w.l.o.g. that vertex $v''$ lies on the interior of face $F'$.
	From the definition of $K$, there are at least $L/3$ paths in $\pset$ whose image in $\tilde\phi$ intersects the interior of face $F$.
	Note that, since the paths of $\pset$ are non-transversal with respect to $\Sigma'$, the image of every path in $\pset$ in $\tilde\phi$ cannot cross the boundary of face $F$ through the disc $D_{\tilde\phi}(u)$ of any vertex $u\in V(P)\cup V(P')$. Therefore, edges of $E(K)$ participate in at least $L/3$ crossings. 
	
	However, since we have assumed that \fbox{ $\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, we get that %\znote{to modify the parameters}
	$$\frac{L}{3}\ge \frac{m'}{30\cdot\tau^i} \ge \frac{\tau^s}{30\cdot\tau^i}>\frac{\cro(\tilde \phi)\cdot\tau^i\cdot\mu^{\smallprobability}}{\tau^s}>\frac{\cro(\tilde \phi)\cdot\tau^i\cdot\mu^{\smallprobability}}{m'},$$ 
	a contradiction to the assumption that the event $\event_1$ does not happen.
	Therefore, the images of $P$ and $P'$ do not cross in $\tilde\phi$.
\end{proof}



%We use the following observation.
\begin{observation}
\label{obs: new cycle not crossing old ones}
If \fbox{$\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, then with probability $1-O(1/\mu^{\smallprobability})$, in the drawing $\tilde \phi$ the edges of $K$ do not cross any special edge of any instance in the collection $\hat \iset$ before this iteration.
\end{observation}
%\znote{need to add additional property: ``special cycles are crossed at most $m/\tau^i\mu^{\smallprobability}$ times'' to the drawing $\tilde \phi$ to show this is true.}

\begin{proof}
%Assume that node $v(I')$ is at distance $d$ from the root $v(I)$ in tree $T$. Since event $\event^*$ does not happen, $d\le M$. Moreover, from \Cref{obs: 2 new special cycles}, over the course of the algorithm, the total number of special cycles in all instances in $\hat \iset$ is always at most $2M$, so $|\rset(I')|\le 2M$.
Since drawing $\tilde \phi$ is well-structured with respect to the collection $\hat\iset$ before this iteration, and since instance $I'$ belongs to the collection $\iset$ before this iteration, the drawing of $I'$ induced by $\tilde \phi$ is a well-structured drawing of $I'$.
We will show that with probability $1-O(1/\mu^{\smallprobability})$, in the drawing $\tilde \phi$ the edges of $K$ do not cross any special edge of $I'$.
Then \Cref{obs: new cycle not crossing old ones} follows from \Cref{obs: not crossing your own special then not crossing any special}.

Denote by $E'$ the set of all edges in $E(G')$ that crosses an edge of $E(\rset(I'))$ in $\tilde \phi$.
From Property \ref{prop: niubi edge crossing special cycle} in the definition of a well-structured solution, $|E'|\le \cro(\tilde \phi)\cdot(\tau^i)^{10}/m'$. 
%
We define the edge-disjoint subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ in the same way as \Cref{obs: skeleton number of crossings}. 
Since the subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ are edge-disjoint, the probability that a random subgraph in $\set{\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}}$ contains an edge of $E'$ is at most 
\[
\frac{|E'|}{\floor{L/2}}\le \frac{\cro(\tilde \phi)\cdot(\tau^i)^{10}/m'}{m'/3\tau^i}
\le 
\frac{\cro(\tilde \phi)\cdot(\tau^i)^{9}}{(m')^2}
\le 
\frac{\cro(\tilde \phi)\cdot(\tau^i)^{9}}{(\tau^s)^2}
<\frac{1}{\mu^{\smallprobability}},
\]
where the last but one step uses the assumption that $\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$.
\end{proof}


\paragraph{Bad Event $\event_2$.}
We say that the bad event $\event_2$ happens iff the drawing $\tilde \phi$ contains a crossing that involves an edge of $K$ and a special edge of some instance in the collection $\hat \iset$ before this iteration. From \Cref{obs: new cycle not crossing old ones}, $\Pr[\event_2]=O(1/\mu^{\smallprobability})$.



\paragraph{High-degree vertices.}
Denote $h=\cro(\tilde \phi)\cdot \mu^{11\interestconst+3\smallprobability}\cdot(\tau^i)^4/m'$.
%and $h'=\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{2\smallprobability}/m'$.
We say that a vertex $v\in V(\pset)\setminus \set{v',v''}$ is a \emph{high-degree} vertex iff $\deg_{G'}(v)\ge h$, otherwise we say that it is a \emph{low-degree} vertex.
%
%
We say that a high-degree vertex $v$ is a \emph{type-1} high-degree vertex iff $v$ is contained in at most $h$ paths in $\pset$, otherwise we say that $v$ is a \emph{type-2} high-degree vertex. 
%\znote{the definition of $h$ depends on $\cro$ or $\cro(\tilde \phi)$? note that the values of $h,h'$ are unknown to us}
%\znote{$h$ and $h'$ merged?}



We denote by $V_{\sf{low}}(P)$ the set of all low-degree vertices of $P$, and we define the set $V_{\sf{low}}(P')$ similarly. We use the following observation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse{whp version}

\begin{observation}
	\label{obs: skeleton do not have many insignificant edges}
	The probability that $\sum_{v\in V_{\sf{low}}(P)}\deg_{\hat G'}(v)\ge h\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$. Similarly, the probability that $\sum_{v\in V_{\sf{low}}(P')}\deg_{\hat G'}(v)\ge h\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$. 
\end{observation}

\begin{proof}
	%We only consider the path $P$, the proof for path $P'$ is symmetric.
	Let $\hat P$ be a path of $\pset$ and let $e$ be an edge that does not belong to set $E'$.
	We say that $e$ is \emph{insignificant for $\hat P$}, iff $e$ is incident to a low-degree vertex of $\hat P$. Denote $e=(u,v)$. If $u$ is a low-degree vertex, then $e$ is insignificant for at most $h$ paths in $\pset$ that contains $u$. Otherwise, $e$ is not insignificant for any path in $\pset$ that contains $u$. Similarly, we get that $e$ is insignificant for at most $h$ paths in $\pset$ that contains $v$. Therefore, an edge $e\notin E'$ is insignificant for at most $2h$ paths in $\pset$.
	Therefore, if we denote $\deg_{\sf{low}}(\hat P)=\sum_{v\in V_{\sf{low}}(P)}\deg_{\hat G}(v)$, then $\sum_{\hat P\in \pset}\deg_{\sf{low}}(\hat P)\le 2hm$, and so the expected value $\deg_{\sf{low}}(\hat P)$ for a random path in $\pset$ is at most $2hm/(m/\mu^{\interestconst})\le O(h\mu^{\interestconst})$. From Markov's bound, the probability that $\deg_{\sf{low}}(P)\ge h\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$, and similar the probability that $\deg_{\sf{low}}(P')\ge h\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$. 
	\Cref{obs: skeleton do not have many insignificant edges} now follows.
\end{proof}

\fi


\begin{observation}
	\label{obs: skeleton do not have many insignificant edges}
	$\expect[]{\sum_{v\in V_{\sf{low}}(P)}\deg_{G'}(v)}= O (h\tau^i)$. Similarly, $\expect[]{\sum_{v\in V_{\sf{low}}(P')}\deg_{G'}(v)}= O (h\tau^i)$.
\end{observation}

\begin{proof}
	%We only consider the path $P$, the proof for path $P'$ is symmetric.
	Let $\hat P$ be a path of $\pset$ and let $e$ be an edge that does not belong to set $E(\pset)$.
	We say that $e$ is \emph{insignificant for $\hat P$}, iff $e$ is incident to a low-degree vertex of $\hat P$. Denote $e=(u,v)$. If $u$ is a low-degree vertex, then $e$ is insignificant for at most $h$ paths in $\pset$ that contains $u$. Otherwise, $e$ is not insignificant for any path in $\pset$ that contains $u$. Similarly, we get that $e$ is insignificant for at most $h$ paths in $\pset$ that contains $v$. Therefore, an edge $e\notin E(\pset)$ is insignificant for at most $2h$ paths in $\pset$.
	Therefore, if we denote $\deg_{\sf{low}}(\hat P)=\sum_{v\in V_{\sf{low}}(P)}\deg_{ G'}(v)$, then $\sum_{\hat P\in \pset}\deg_{\sf{low}}(\hat P)\le 2hm'$, and so the expected value $\deg_{\sf{low}}(\hat P)$ for a random path in $\pset$ is at most $O(2hm'/(m'/\tau^i))\le O(h\tau^i)$. The proof for path $P'$ is symmetric.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We denote by $V_{\sf{high(1)}}(P)$ the set of all type-1 high-degree vertices of $P$, and we define set $V_{\sf{high(1)}}(P')$ similarly. We use the following observation.

\iffalse{whp version}

\begin{observation}
	\label{obs: not many edges incident to a type-1 high-degree vertex in skeleton}
	The probability that the total number of edges that are incident to a type-1 high-degree vertex on path $P$ is more than $h'\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$. Similarly, the probability that the total number of edges that are incident to a type-1 high-degree vertex on path $P'$ is more than $h'\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$.
\end{observation}
\begin{proof}
	Let $v$ be a type-1 high-degree vertex. Since it belongs to at most $h'$ paths in $\pset$, the probability that $v$ belongs to path $P$ is $O(h'/(m/\mu^{\interestconst}))$. Therefore, for an edge $e\in E(\hat G)$ that is incident to a type-1 high-degree vertices, the probability that its type-1 high-degree endpoint belongs to $P$ is $O(h'/(m/\mu^{\interestconst}))$. From the union bound on all edges in $E(\hat G)$, the expected number of edges that are incident to some type-1 high-degree vertex on path $P$ is $O(m\cdot h'/(m/\mu^{\interestconst}))=O(h'\mu^{\interestconst})$. Then from Markov's bound, the probability that number of edges that are incident to some type-1 high-degree vertex on path $P$ is greater than $h'\mu^{\interestconst+\smallprobability}$ is $O(1/\mu^{\smallprobability})$.
	The proof for path $P'$ is symmetric.
\end{proof}

\fi

\begin{observation}
	\label{obs: not many edges incident to a type-1 high-degree vertex in skeleton}
	$\expect[]{\sum_{v\in V_{\sf{high(1)}}(P)}\deg_{G'}(v)}= O (h\tau^i)$, and $\expect[]{\sum_{v\in V_{\sf{high(1)}}(P')}\deg_{G'}(v)}= O (h\tau^i)$.
\end{observation}
\begin{proof}
	Let $v$ be a type-1 high-degree vertex. Since it belongs to at most $h$ paths in $\pset$, the probability that $v$ belongs to path $P$ is $O(h/(m'/\tau^i))$. Therefore, for an edge $e\in E(G')$ that is incident to a type-1 high-degree vertex, the probability that its type-1 high-degree endpoint belongs to $P$ is $O(h/(m'/\tau^i))$. From the union bound on all edges in $E(G')$, the expected number of edges that are incident to some type-1 high-degree vertex on $P$ is $O(m'\cdot h/(m'/\tau^i))=O(h\tau^i)$. 
	The proof for path $P'$ is symmetric.
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Bad Events $\event_3, \event_4$.}
We say that the bad event $\event_3$ happens if either $\sum_{v\in V_{\sf{low}}(P)}\deg_{G'}(v)\ge h\tau^i\mu^{\smallprobability}$ holds or $\sum_{v\in V_{\sf{low}}(P')}\deg_{G'}(v)\ge h\tau^i\mu^{\smallprobability}$ holds. From \Cref{obs: skeleton do not have many insignificant edges} and Markov's bound, $\Pr[\event_3]\le O(1/\mu^{\smallprobability})$.
%
We say that the bad event $\event_4$ happens iff there are at least $h\tau^i\mu^{\smallprobability}$ edges incident to a type-1 high-degree vertex of $K$. From \Cref{obs: not many edges incident to a type-1 high-degree vertex in skeleton} and Markov's bound, $\Pr[\event_4]\le O(1/\mu^{\smallprobability})$.







%\iffalse{balanced type-2 high-degree vertices}
\paragraph{Unbalanced vertices.}
Let $\hat P$ be a path of $\pset$ and let $v$ be an inner vertex of $\hat P$. Let $e_v,e'_v$ be the two edges of $\hat P$ that are incident to $v$. 
%where $e_v$ precedes $e'_v$ in the path $\hat P$ (recall that we view path $\hat P$ as being directed from $v'$ to $v''$). 
Consider now the edges of $\delta_{G'}(v)\cap E(\pset)$, and assume that they appear in the ordering $\oset_v\in \Sigma$ in the following order: $e_v,\hat e_1,\ldots,\hat e_s, e'_v,\hat e'_1,\ldots,\hat e'_t$. 
We say that $v$ is \emph{unbalanced with respect to $\hat P$} iff $v$ is a type-2 high-degree vertex and $\min\set{s,t}\le \max\set{s,t}/\mu^{\smallprobability}$. 
%Additionally, if $s\ge N$, then we say that the edges $\hat e_1,\ldots,\hat e_s$ are \emph{significant to $v$}; otherwise we say that they are \emph{insignificant to $v$}. Similarly, if $t\ge N$, then we say that the edges $\hat e'_1,\ldots,\hat e'_t$ are \emph{significant to $v$}; otherwise we say that they are \emph{insignificant to $v$}. Clearly, for every vertex $v\in V(\pset)\setminus \set{u^*,v^*}$, the number of edges that are insignificant to $v$ is at most $2N$.



\begin{observation}
\label{obs: skeleton loops do not contain significant nodes}
The probability that $P$ contains a type-2 high-degree vertex that is unbalanced with respect to $P$ is $O(1/\mu^{\smallprobability})$. Similarly, the probability that $P'$ contains a type-2 high-degree vertex that is unbalanced with respect to $P'$ is $O(1/\mu^{\smallprobability})$. 
\end{observation}
\begin{proof}
%Denote $d^*=\cro(\tilde \phi)\cdot \mu^{11\interestconst+3\smallprobability}\cdot\tau^i/m'$.
For each vertex $u$, we denote by $d(u)$ the number of paths in $\pset$ that contains $u$.
We say that a type-2 high-degree vertex $u$ is \emph{bad}, iff among all $d(u)$ paths of $\pset$ that contains $u$, at least $d(u)/2\mu^{\smallprobability}\tau^i$ of them participate in at least $d(u)/2\mu^{\smallprobability}\tau^i$ crossings each; otherwise we say $u$ is \emph{good}.

We first show that the probability that $K$ contains a bad vertex is $O(1/\mu^\smallprobability)$.
For each $\log h\le j\le \log n$, we say that a bad vertex $u$ is in \emph{class-$j$} iff $2^j\le d(u)<2^{j+1}$. Consider now an index $\log h\le j\le \log n$. On the one hand, from the construction of $K$, for each class-$j$ bad vertex, the probability that it belongs to $K$ is $O(2^{j}/(m'/\tau^i))$. On the other hand, we prove that the number of class-$j$ bad vertices is at most $O(\cro(\tilde \phi)\cdot \mu^{10\interestconst}/(2^j/2\mu^{\smallprobability}\tau^i)^2)$.
We say that a crossing in drawing $\tilde \phi$ is \emph{witnessed by} a bad vertex $u$, iff one of the edges that participates in the crossing belongs to a path in $\pset$ that contains $u$.
Since each path of $\pset$ contains at most $\tau^i\mu^{10\interestconst}$ vertices, and the paths of $\pset$ are edge-disjoint, each crossing is witnessed by at most $2\tau^i\mu^{10\interestconst}$ bad vertices. Note that, from the definition of bad vertices, each class-$j$ bad vertices witness at least $(2^j/2\mu^{\smallprobability}\tau^i)^2$ crossings. It follows that the number of class-$j$ bad vertices is at most $O(\cro(\tilde \phi)\cdot 2\tau^i\mu^{10\interestconst}/(2^j/\mu^\smallprobability)^2)$.
Therefore, the probability that $K$ contains a class-$j$ bad vertex is at most
\[
O\bigg(\frac{\cro(\tilde \phi)\cdot2\tau^i \mu^{10\interestconst}}{(2^j/2\mu^{\smallprobability}\tau^i)^2}\cdot \frac{2^{j}}{(m'/\tau^i)}\bigg)\le O\bigg(\frac{\cro(\tilde \phi)\cdot \mu^{10\interestconst+2\smallprobability}(\tau^i)^4}{2^j\cdot m'}\bigg)\le O\bigg(\frac{\cro(\tilde \phi)\cdot \mu^{10\interestconst+2\smallprobability}(\tau^i)^4}{\cro(\tilde \phi)\cdot \mu^{11\interestconst+3\smallprobability}(\tau^i)^4}\bigg)=O(1/\mu^{\interestconst+\smallprobability}),
\]
where the last inequality uses the fact that $2^j\ge h$ and the definition of $h$. Then from the union bound on all indices $\log h\le j\le \log n$, the probability that $K$ contains a bad vertex is at most $O(1/\mu^\smallprobability)$ (since $\mu\gg \log n$).

We next claim that, for each good type-2 high-degree vertex $u$, $u$ is unbalanced with respect to at most $O(d(u)/\mu^{\smallprobability}\tau^i)$ paths in $\pset$ that contains $u$. Before we prove the claim, we first show that this implies that the probability that $P$ or $P'$ contains a good type-2 high degree vertex that is unbalanced with respect to it is $O(1/\mu^{\smallprobability})$, which, together with the arguments in the last paragraph, imply
\Cref{obs: skeleton loops do not contain significant nodes} immediately. Let $U$ be the set of all good type-2 high-degree vertices. Clearly, $\sum_{u\in U}d(u)\le m'$. For each vertex $u\in U$, we denote by $d'(u)$ the number of paths in $\pset$ to which $u$ is unbalanced, then the number of paths such that there exists some good type-2 high-degree vertex being unbalanced with respect to it is at most
$\sum_{u\in U}d(u)\le O(m'/\mu^{\smallprobability}\tau^i)\le O(L/\mu^{\smallprobability})$. Therefore, the probability that $P$ or $P'$ is one of these paths is $O(1/\mu^{\smallprobability})$.

We now provide the proof of the claim.
Consider now a good type-2 high-degree vertex $u\in U$. 
Denote $M_u=d(u)/2\mu^{\smallprobability}\tau^i$.
We denote by $\pset_u$ the set of paths in $\pset$ that contains $u$ and participates in at most $M_u$ crossings in $\tilde \phi$. Since $u$ is good, the number of paths in $\pset$ that contains $u$ and participates in more than $M_u$ crossings in $\tilde \phi$ is less than $M_u$.
Let $P^*$ be an arbitrary path in $\pset_u$, and let $e^*_1,e^*_2$ be the edges of $P^*$ that are incident to $u$, such that $e^*_1$ precedes $e^*_2$ in $P^*$. Recall that we have computed an orientation $b(u)$ for $u$ in Step 2 (\Cref{Step 2}). Denote $\delta(u)=\set{e^*_1,e^R_1,\ldots,e^R_x,e^*_2,e^L_1,\ldots,e^L_y}$, where edges are indexed according to their appearance (clockwise) in the oriented ordering at $u$. We define $E^R(u)=\set{e^R_1,\ldots,e^R_x}$ and  $E^L(u)=\set{e^L_1,\ldots,e^L_y}$.
See \Cref{fig: unbal_1} for an illustration.

We denote the first edges of paths in $\pset_u$ by $e^*, e_1,\ldots, e_r$, where $e^*$ is the first edge of path $P^*$, and other edges are indexed according to their appearance  (clockwise) in the oriented ordering at $v$. For each index $1\le i\le r$, we denote by $P_i$ the path in $\pset_u$ whose first edge is $e_i$.
Since the paths of $\pset$ are non-transversal at $u$, for each path in $\pset_u$, its two edges incident to $u$ have to either both belong to $E^L(u)$ or both belong to $E^R(u)$.
For each path $P_i$, we label it by $L$ iff the edges of $P_i$ incident to $u$ belong to set $E^L(u)$, and we label it by $R$ iff the edges of $P_i$ incident to $u$ belong to set $E^R(u)$.
Now we let $\pset'_u$ be the union of (i) the set $\pset^R_u$ that contains the $2M_u$ paths of $\pset_u$ with smallest indices that are labelled by $R$ (if there are not that many, then take all of them); and (ii) the set $\pset^L_u$ that contains the $2M_u$ paths of $\pset_u$ with largest indices that are labelled by $L$ (if there are not that many, then take all of them). 
See \Cref{fig: unbal_2} for an illustration.
%We now show that $u$ is balanced with respect to all but at most $2M_u$ path in $\pset_u\setminus \pset'_u$. Note that this completes the proof of the claim, since $|\pset'_u|\le 4M_u$ and there are at most $M_u$ paths that contain $u$ but do not belong to $\pset_u$.
%
\begin{figure}[h]
	\centering
	\subfigure[An illustration of edges of $\delta(u)$. Edges of $E^L(u)$ are shown in purple, and edges of $E^R(u)$ are shown in orange.]{\scalebox{0.14}{\includegraphics{figs/unbal_1.jpg}}\label{fig: unbal_1}}
	\hspace{0.1cm}
	\subfigure[An illustration of edges of $\delta(v')$ (assuming $M_u=1$). The first edges of paths laballed by $L$ are shown in purple, the first edges of paths laballed by $R$ are shown in orange, and the first edges of paths in set $\pset'_u$ are with check marks.]{
		\scalebox{0.12}{\includegraphics{figs/unbal_2.jpg}}\label{fig: unbal_2}}
	\caption{Illustrations of edge sets $\delta(u)$ and $\delta(v')$.}
\end{figure}
%

Let $P^L$ be the path of $\pset^L_u$ with the largest index, and let $P^R$ be the path of $\pset^R_u$ with the smallest index. We first show that the index of $P^R$ has to be greater than the index of $P^R$. Assume otherwise, then consider subpaths of paths in set $\pset^R$ between $v'$ and $u$ and the area surrounded by the images of (i) the subpath of $P^L$ between $u$ and $v'$; and (ii) the subpath of $P^*$ between $u$ and $v'$, that we denote by $F^L$. Clearly, the first segments of those subpaths of paths in set $\pset^R$ lie inside the area $F_L$, while their last segments lie outside $F_L$. Therefore, each of these paths will either cross $P^*$ or cross $P^L$ (see \Cref{fig: unbal_3}), implying that either $P^*$ or $P^L$ participates in at least $M_u$ crossings in $\tilde \phi$, a contradiction.
\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.12]{figs/unbal_3.jpg}
	\caption{An illustration of paths $P^L$, $P^R$ and paths in $\pset^R$ (shown in thin orange). The red circles mark the crossings between paths in $\pset^R$ and path $P^L$ or $P^*$ (shown in blue).}\label{fig: unbal_3}
\end{figure}
\fi

Recall we have denoted by $F_L$ the area surrounded by the image of subpaths of $P^L$ and $P^*$ between $v'$ and $u$.
We now show that the image of $v''$ do not lie in $F_L$. In fact, if the image of $v''$ lies in $F_L$, then from similar arguments, all subpaths of paths labelled $R$ have to cross either $P^*$ or $P^L$, implying that either $P^*$ or $P^L$ participates in at least $M_u$ crossings in $\tilde \phi$, a contradiction.
Similarly, we can show that the image of $v''$ do not lie in $F_R$, the area surrounded by the image of subpaths of $P^R$ and $P^*$ between $v'$ and $u$.

\begin{figure}[h]
	\centering
	\subfigure[An illustration of paths $P^L,P^R$ and paths in $\pset^R$ (in thin orange). The red circles are crossings between paths in $\pset^R$ and path $P^L$ or $P^*$ (in blue).]{\scalebox{0.09}{\includegraphics{figs/unbal_3.jpg}}\label{fig: unbal_3}}
	\hspace{0.1cm}
	\subfigure[An illustration of areas $F^L$, $F^R$ (shown in grey) and the behavior of paths in $\hat\pset_u$ at $u$.]{
		\scalebox{0.09}{\includegraphics{figs/unbal_4.jpg}}\label{fig: unbal_4}}
	\caption{Illustrations of crossing patterns of paths in $\pset_u$.}
\end{figure}


We delete from $\pset_u$ all paths of $\pset'_u$ and all paths that cross $P^L$ or $P^R$ or $P^*$, and denote the resulting path set by $\hat\pset_u$. Clearly, $|\pset_u\setminus \hat\pset_u|=O(M_u)$. It is now easy to show that, for all paths in $\hat\pset_u$ labelled $L$, the last segment of the image of its first edge incident to $u$ lies in $F^L$, and the last segment of the image of its first edge incident to $u$ lies outside $F^L$. Similarly for all paths in $\hat\pset_u$ labelled $R$, the last segment of the image of its first edge incident to $u$ lies in $F^R$, and the last segment of the image of its first edge incident to $u$ lies outside $F^L$ (see \Cref{fig: unbal_4}).
%
\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.12]{figs/unbal_4.jpg}
	\caption{An illustration of areas $F^L$, $F^R$ and paths in $\hat\pset_u$.}\label{fig: unbal_4}
\end{figure}
\fi
%
Since the paths are non-transversal with respect to $\Sigma'$. It is now easy to see that, by definition, $u$ is unbalanced with respect to at most $O(M_u)$ paths in $\hat\pset_u$.
Therefore, altogether, $u$ is unbalanced with respect to at most $O(M_u)$ paths in $\pset$ that contains $u$. This completes the proof of the claim, and also completes the proof of \Cref{obs: skeleton loops do not contain significant nodes}.
%
\iffalse
\znote{To modify from here}
Consider now a path $\hat P$ in $\pset_u\setminus \pset'_u$ and assume without loss of generality that $\hat P$ is labelled $L$.
Let $P^L$ be the path of $\pset^L_u$ with the $M_u$-th largest index. %We denote by $\gamma^*$ the image of the subpath of $P^*$ between $v$ and $u$, and denote by $\gamma^L$ the image of the subpath of $P^L$ between $v$ and $u$. Clearly,
Denote by $\hat e_a^L, \hat e_b^L$ the edges of $P^L$ incident to $u$, where $\hat e_a^L$ precedes $\hat e_b^L$ in $P_L$.
First it is easy to observe that edges $e^*_2,\hat e_b^L,\hat e_a^L, e^*_1$ must appear in the oriented rotation at $u$ in this order, since otherwise the paths in $\pset^L_u$ with larger indices than $P^L$ will each participate in more than $M_u$ crossings in $\tilde \phi$, contradicting the definition of $\pset_u$.
Then it is easy to see that the first edge of $\hat P$ that is incident to $u$ must appear clockwise between $\hat e^L_a$ and $e^*_1$, since otherwise path $\hat P$ has to cross every path in $\pset^L_u$ with a smaller index than $P^L$, contradicting the fact that the path $P^L$ participates in less than $M_u$ crossings in $\tilde \phi$. Similarly, the last edge of $\hat P$ that is incident to $u$ must appear clockwise between $e^*_2$ and $\hat e^L_b$. Therefore, $u$ is unbalanced with respect to at most $M_u$ paths labelled $L$ in $P_u\setminus \pset'_u$. Similarly, $u$ is unbalanced with respect to at most $M_u$ labelled $R$ in $P_u\setminus \pset'_u$. Therefore, $u$ is unbalanced with respect to at most $2M_u$ path in $\pset_u\setminus \pset'_u$.\fi
\end{proof}
%\fi



\paragraph{Bad Event $\event_5$.}
We say that bad event $\event_5$ happens if either $P$ contains an inner vertex that is a type-2 high-degree vertex and unbalanced with respect to $P$, or $P'$ contains an inner vertex that is a type-2 high-degree vertex and unbalanced with respect to $P'$. From \Cref{obs: skeleton loops do not contain significant nodes}, $\Pr[\event_5]\le O(1/\mu^{\smallprobability})$.





From now on, we call type-2 high-degree vertices \emph{significant vertices}.


\begin{observation}
\label{obs: skeleton image loop does not contain significant vertices}
If events $\event_1$ and $\event_5$ do not happen, then no self-loop of the curve representing the image of $P$ in $\tilde \phi$ contains the image of any significant vertex of $V(P)$, and similarly no self-loop of the curve representing the image of $P$ in $\tilde \phi$ contains the image of any significant vertex of $V(P')$.
\end{observation}
\begin{proof}
We show that, if events $\event_1,\event_5$ do not happen, then no loop of curve $\tilde\phi(P)$ contains the image of any significant vertex of $V(P)$, and the proof for $P'$ is symmetric.
	
	Let $\zeta$ be a self-loop of $\tilde\phi(P)$.
	% and let $z$ be the unique point of $\zeta$ which is a crossing between a pair of edges of $E(P)$. 
	Clearly, $\zeta$ partitions the sphere into two faces, that we denote by $F$ and $F'$. Assume without loss of generality that face $F$ does not contain the image of $v'$.
	Assume for the sake of contradiction that loop $\zeta$ does contain the image of a significant vertex $u\in V(P)$.
	%Since $P$ is a simple path, $\tilde \phi(u)\ne z$. 
	Let $e_u,e'_u$ be the two edges of $P$ that are incident to $u$.
	Denote $\delta_{G'}(u)\cap E(\pset)=\set{e_u,\hat e_1,\ldots,\hat e_s, e'_u,\hat e'_1,\ldots,\hat e'_t}$, where the edges are listed according to the ordering $\oset_u\in \Sigma'$. We assume without loss of generality that the first segments of the curves representing the images of edges $\hat e_1,\ldots,\hat e_s$ lie in the face $F$. Since $\event_5$ does not happen, the significant vertex $u$ is not unbalanced with respect to $P$. Then since $\deg_{G'}(u)\ge h$ and $u$ is not unbalanced with respect to $P$, $s > h/2\mu^{\smallprobability}$.
	Note that, since the paths of $\pset$ are non-transversal with respect to $\Sigma'$, edges $\hat e_1,\ldots,\hat e_s$ in fact come from a subset of $s/2$ paths of $\pset$, which we denote by $\hat \pset$.
	%
	We will show that, for each path $\hat P\in \hat{\pset}$, the curve $\tilde\phi(\hat P)$ must cross $\zeta$. Note that this implies that the number of crossings that involve the curve $\zeta$ is at least $s/2 > h/4\mu^{\smallprobability}>(\cro(\tilde \phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$, causing a contradiction to the assumption that event $\event_1$ does not happen, and therefore completes the proof of \Cref{obs: skeleton image loop does not contain significant vertices}.
	
	We now show that the curve $\tilde\phi(\hat P)$ must cross $\zeta$. Note that the curve $\tilde\phi(\hat P)$ connects $\tilde\phi(v')$ to $\tilde\phi(v'')$, and the image of $v'$ lie outside the face $F$. Therefore, there must exist a point $z$ that belongs to both curve $\tilde\phi(\hat P)$ and $\zeta$, such that, if we denote by $\gamma_z, \gamma'_z$ the tiny segments of $\tilde\phi(\hat P)$ right before and after $z$, then one of $\gamma_z, \gamma'_z$ is contained in the interior of face $F$ and the other is contained in the interior of face $F'$.  
	Assume that $z$ is the image of a vertex. However, since the paths of $\pset$ are non-transversal with respect to $\Sigma$, segments $\gamma_z$ and $\gamma'_z$ have to lie on the same side of $\zeta$, a contradiction. 
	Therefore $z$ is not the image of a vertex, and so $z$ is a crossing between $\tilde\phi(\hat P)$ and $\zeta$.
\end{proof}

\paragraph{Summary of properties of $K$.}
We define event $\event=\bigcup_{1\le i\le 5}\event_i$. Assume that event $\event$ does not happen, then the cycle $K$ and the well-structured drawing $\tilde \phi$ satisfies the following properties.
\begin{properties}{F}
\item $|E(K)|\le 2\tau^i\cdot\mu^{10\interestconst}$;
\item edges of $K$ participate in at most $(\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde \phi$;
\label{f_prop: K crossed few times}
\item in drawing $\tilde \phi$, the edges of $K$ do not cross any special edge of any instance in the collection  $\hat \iset$ before this iteration;\label{f_prop: K does not cross special edges}
\item the number of edges that are incident to a low-degree vertex (a vertex of degree at most $h$ in $G'$) of $K$ is at most $h\cdot \tau^i\cdot\mu^{\smallprobability}$, where $h=\cro(\tilde \phi)\cdot \mu^{11\interestconst+3\smallprobability}\cdot(\tau^i)^4/m'$;
\label{f_prop: low-degree incident edges small}
\item the number of edges that are incident to a type-1 high-degree vertex (a vertex that has degree at least $h$ and is contained in at most $h$ paths of $\pset$) of $K$ is at most $h\cdot \tau^i\cdot\mu^{\smallprobability}$;
\label{f_prop: type-1 incident edges small}
\item the images of $P$ and $P'$ do not cross in $\tilde \phi$;
\label{f_prop: P and P' do not cross}
\item no self-loop of the curve representing the image of $P$ in $\tilde \phi$ contains the image of any significant vertex, and similarly no self-loop of the curve representing the image of $P'$ in $\tilde \phi$ contains the image of any significant vertex.
\label{f_prop: no significant in loop}
\end{properties}


\subsubsection*{Modifying the drawing $\tilde \phi$}

We now proceed to modify the drawing $\tilde \phi$ into a drawing that is well-structured with respect to the collection $\hat \iset$ after this iteration. That is, we will modify the image of edges of $I'$ in $\tilde \phi$, such that the resulting drawing induces well-structured drawings for new instances $I_{\inn}, I_{\out}$.

We now provide a summary of the stages in modifying the drawing $\tilde \phi$. For simplicity of notations we denote $I'_1=I_{\inn}$ and $I'_2=I_{\out}$ from now on.
We first delete the edges that are added to set $\hat E^{\sf del}$ in this iteration, and rename the resulting drawing by $\tilde \phi$. Clearly, the new drawing $\tilde \phi$ contains at most the same number of crossings as the old one.
In the first stage, we modify the drawing $\tilde\phi$ into a new drawing $\hat\phi$ that induces almost well-structured drawings of instances $I'_1$ and $I'_2$ (recall that an almost well-structured drawing is a drawing that satisfies properties \ref{prop: simple curve}--\ref{prop: first segments}). %such that the image of $K$ in $\hat\phi$ is a simple closed curve, and $\cro(\hat\phi)$ is not much larger than $\cro(\phi)$. 
In the second stage, we locally modify the image of edges incident to vertices of $K$, such that the orientations of vertices of $K$ coincide the orientations computed in Step 2 (\Cref{Step 2}).
In the third and the fourth stages, we 
%split the drawing $\hat \phi$ into an almost well-structured drawing $\hat \phi_1$ of $I'_1$ and an almost well-structured drawing $\hat\phi_2$ of $I'_2$, and then we 
further modify drawing $\hat\phi$ into a drawing $\tilde \phi'$ that induces well-structured drawings of instances $I'_1$ and $I'_2$, respectively.
%such that $\cro(\phi'_1)+\cro(\phi'_2)$ is not much larger than $\cro(\hat\phi)$.  
In each of these stages, we will make sure not to increase the number of crossings in the drawing by too much.
We now describe each of the stages in turn.


\iffalse
From now on we denote $\phi=\tilde \phi$.
We now construct well-structured drawings of the subinstances $I'_1$ and $I'_2$ using the well-structured drawing $\phi$ of instance $I'$ in four stages. In the first stage, we modify the well-structured drawing $\phi$ of $I'$ into an almost well-structured drawing $\hat \phi$ of $I'$ (recall that an almost well-structured drawing is a drawing that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}), such that the image of $K$ in $\hat\phi$ is a simple closed curve, and $\cro(\hat\phi)$ is not much larger than 
$\cro(\phi)$. In the second stage, we locally modify the image of edges incident to vertices of $K$, such that the orientations of vertices of $K$ coincide the orientations computed in Step 2 (\Cref{Step 2}).
In the third and the fourth stages, we 
split the drawing $\hat \phi$ into an almost well-structured drawing $\hat \phi_1$ of $I'_1$ and an almost well-structured drawing $\hat\phi_2$ of $I'_2$, and then we further modify drawings $\hat\phi_1, \hat\phi_2$ into well-structured drawings $\phi'_1,\phi'_2$ of instances $I'_1$ and $I'_2$, respectively.
%such that $\cro(\phi'_1)+\cro(\phi'_2)$ is not much larger than $\cro(\hat\phi)$.  
We now describe each of the stages in turn.
\fi

\subsubsection*{Stage 1. Removing self-loops of the image of $K$ in $\tilde\phi$}

In the first stage, we modify the drawing $\tilde \phi$ into a new drawing $\hat \phi$ that induces almost well-structured drawings of instances $I'_1,I'_2$, via the following claim.


\begin{claim}
\label{clm: skeleton can be drawn in a natural way}
If event $\event$ does not happen, then there is a drawing $\hat\phi$ of instance $\bar I$ after this iteration, in which (i) for each edge not incident to any vertex of $K$, its image in $\hat \phi$ remains the same as in $\tilde \phi$; (ii) the image of $K$ in $\hat \phi$ is a simple closed curve that does not cross any special edge of $I'$, and (iii)
$\cro(\hat\phi)\le \cro(\phi)+O\big(h^2(\tau^i)^2\mu^{2\smallprobability}\big).$
\end{claim}

\begin{proof}
We construct the drawing $\hat\phi$ by iteratively ``opening'' the self-loops of the curve representing the image of $P$ and the curve representing the image of  $\tilde\phi$ until the image of $K$ becomes a simple closed curve. Recall that, from Property \ref{f_prop: P and P' do not cross}, the images of $P$ and $P'$ do not cross in $\tilde\phi$, and from Property \ref{f_prop: K does not cross special edges}, the image of $K$ does not cross any special edge of $I'$ in $\tilde\phi$.

We denote by $\gamma$ the image of $P$ in $\tilde\phi$. Note that $\gamma$ is not necessarily a simple curve. We first iteratively compute a set $Z$ of self-loops of $\gamma$ and another simple curve $\gamma'$ connecting $\tilde\phi(v')$ to $\tilde\phi(v'')$, as follows.
%
We view the curve $\gamma$ as being directed from $\tilde\phi(v')$ to $\tilde\phi(v'')$. Initially we set $Z=\emptyset$. We start from the first endpoint $\tilde\phi(v')$ of $\gamma$ and find the first point $z$ on $\gamma$ that appears twice on $\gamma$. Denote by $\zeta$ the subcurve of $\gamma$ between the first and the last (second) appearance of $z$, so $\zeta$ is a self-loop that starts and ends at $z$. We add the self-loop $\zeta$ to set $Z$ and delete $\zeta$ from $\gamma$. We continue this process until the curve $\gamma$ no longer contains self-loops. Denote by $\gamma'$ the resulting simple curve we obtain, and we also view curves $\gamma'$ as being directed from $\tilde\phi(v')$ to $\tilde\phi(v'')$. See \Cref{fig: remove_loop} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Curve $\gamma$ (with direction) is shown in blue, with vertices $v_1,v_2,v_3$ appearing on it sequentially.]{\scalebox{0.0855}{\includegraphics{figs/remove_loop_1.jpg}}}
	\hspace{0.1cm}
	\subfigure[Curve $\gamma'$ is shown in green. Self-loop $\zeta$ is shown in light blue. Thin strip around $\zeta$ is shown in grey.]{
		\scalebox{0.085}{\includegraphics{figs/remove_loop_2.jpg}\label{fig: thin strip}}}
	\caption{Illustration for constructing curve $\gamma'$. \label{fig: remove_loop}}
\end{figure}

The algorithm for constructing the drawing $\hat\phi$ is iterative. In each iteration, we process a self-loop in $Z$.
%
We now describe an iteration.
Let $\zeta$ be a loop in $Z$, and we denote by $z$ the unique point of $\zeta$ that lies on $\gamma'$. %(see \Cref{fig: loop_before}).
	%
We modify the drawing as follows. 
	Let $v_1,\ldots,v_r$ be the vertices whose images appear on the self-loop $\zeta$, where the vertices are indexed according to the ordering in which they appear on $P$ (see \Cref{fig: remove_loop}).
	We denote $V_{\zeta}=\set{v_1,\ldots,v_r}$.
	Let $\sigma$ be a tiny segment of $\gamma'$ that contains $z$.
	We remove the image of vertices $v_1,\ldots,v_r$ and all their incident edges from the current drawing, and place them on $\sigma$, such that $v_1,\ldots,v_r$ appear sequentially in the direction of $P$.
	See \Cref{fig: remove_loop_3} for an illustration.
	 %(see \Cref{fig: loop_after}).
	%We do not modify the images of edges that are not incident to $v_1,\ldots,v_r$.

\iffalse
	\begin{figure}[h]
		\centering
		\subfigure[Before: the images of $v_1,v_2$ appear sequentially on the image of $P$, and they belong to the loop $\zeta$.]{\scalebox{0.09}{\includegraphics{figs/loop_before.jpg}\label{fig: loop_before}}}
		\hspace{0.1cm}
		\subfigure[After: the images of $v_1,v_2$ are moved out of $\zeta$ to the segment $\sigma$ (shown in red).]{
			\scalebox{0.1}{\includegraphics{figs/loop_after.jpg}}\label{fig: loop_after}}
		\caption{Illustration for the process of opening a loop $\zeta$. \label{fig: loop}}
	\end{figure}
\fi	
	
	
	It remains to add back the edges incident to $v_1,\ldots,v_r$. We denote by $z_1,\ldots,z_r$ the points representing the new images of vertices $v_1,\ldots,v_r$ respectively. 
	%
%Note that the loop $\zeta$ divides the sphere into two face, and we denote by $F$ the face that does not contain segment $\sigma$.
	%
	Let $S$ be an arbitrarily thin strip around $\zeta$, such that the entire segment $\sigma$ is contained in $S$ (see \Cref{fig: thin strip}).
	Let $E_{\zeta}$ be the set of all edges incident to a vertex of $V_{\zeta}$. Clearly, for each edge $e\in E_{\zeta}$, the current image of $e$ has to cross the boundary of $S$. For each $e\in E_{\zeta}$, we denote by $z_e$ the last crossing between the curve $\tilde\phi(e)$ and $S$, where the curve $\tilde\phi(e)$ is viewed as being directed from its endpoint in $V_{\zeta}$ to its endpoint outside of $V_{\zeta}$.
	Now we have obtained two sets $\set{z_e\mid e\in E_{\zeta}}$ and $\set{z_1,\ldots,z_r}$ of points that all lie within $S$ or on the boundary of $S$.
	We now compute, for each edge $e\in E_{\zeta}$ with endpoint $v_i\in V_{\zeta}$, a curve $\xi_e$ connecting $z_i$ to $z_e$ that lies within the thin strip $S$, such that the curves in $\Xi_{\zeta}=\set{\xi_e\mid e\in E_{\zeta}}$ are in general position.
	Then for every $1\le i\le r$ and for every edge $e$ that is incident to vertex $v_i$, we define the curve $\eta_e$ be the concatenation of (i) the curve $\xi_e$; and (ii) the segment of its original image between the last crossing with the boundary of $S$ and the image of its other endpoint in $\tilde\phi$.  
	Note that the curve $\eta_e$ may still intersect $\gamma'$ times. Lastly we modify curve $\eta_e$ as follows. We view it as being directed from its endpoint in $V_{\zeta}$ to its endpoint outside $V_{\zeta}$. Let $p_e$ be a point of $\eta_e$ just before the first point on $\eta_e$ that also belongs to $\gamma'$, and let $p'_e$ be a point of $\eta_e$ just after the last point on $\eta_e$ that also belongs to $\gamma'$. We then replace the subcurve of $\eta_e$ between $p_e$ and $p'_e$ by a new curve that lies within the thin strip around $\gamma'$, and cross $\gamma'$ at most once.
	See \Cref{fig: remove_loop_4} for an illustration.
	Clearly, in this way we obtain a new drawing of the graph $G'$ that no longer has the loop $\zeta$.
	%
	
	\begin{figure}[h]
		\centering
		\subfigure[Segment $\sigma$ is shown in red, with the new images of $v_1,v_2,v_3$ placed on it. $e,e'$ are edges incident to $v_1, v_2$ respectively. Their corresponding curves $\eta_{e},\eta_{e'}$ are shown in pink.]{\scalebox{0.13}{\includegraphics{figs/remove_loop_3.jpg}\label{fig: remove_loop_3}}}
		\hspace{0.1cm}
		\subfigure[The adjusted image of $e'$: now it no longer intersect $\gamma$ more than once.]{
			\scalebox{0.13}{\includegraphics{figs/remove_loop_4.jpg}}\label{fig: remove_loop_4}}
		\caption{Illustration for the process of adding edges back. \label{fig: remove_loop_next}}
	\end{figure}
	
	
	We first show that, after this iteration, the drawing we obtain still induces a drawing of $I'$ that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}.
	Note that we have only modified the images of vertices of $V_{\zeta}$, and the special cycles in $\rset(I')$ are node-disjoint from $K$. 
	Therefore, the image of all special cycles remain the same as in $\tilde\phi$, and so the properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing} are still satisfied.
	
	We now show that, after this iteration, the image of $K$ still does not cross any special edge in $I'$.
	Recall that $K$ crosses no special cycle of $\rset(I')$ in $\tilde\phi$. And note that the new images of edges in $K$ are entirely contained in the image of $K$ in $\tilde\phi$. So after this iteration, in the new drawing we obtained, the image of $K$ still does not cross any special edge in $I'$.
		
	Consider the resulting drawing obtained by processing each self-loop in $Z$ in this way. Finally, we perform type-1 uncrossing to the set of curves representing the images of edges in $E_{\zeta}$. Denote by $\hat \phi$ the resulting drawing.
	It is easy to verify that $\hat\phi$ induces a drawing for instance $I'$ that satisfies properties \ref{prop: simple curve}--\ref{prop: discs interior not crossing}, and moreover, in $\hat \phi$ the image of $K$ is a simple closed curve that does not cross any special edge of $I'$.
	
	We now bound the number of new crossings in the drawing. Consider the iteration where some self-loop $\zeta$ is processed. Note that $|E_{\zeta}|\le \sum_{1\le i\le r}\deg_{G'}(v_i)$.
	Note that, since we have performed type-1 uncrossing to the images of edges in $E_{\zeta}$, the resulting images of edges in $E_{\zeta}$ may create at most $|E_{\zeta}|^2$ new crossings. On the other hand, let $E^*_{\zeta}$ be the set of edges in $E(G')$ that cross the self-loop $\zeta$ in the original drawing $\tilde\phi$, so the new images of $E_{\zeta}$ may create $|E^*_{\zeta}|\cdot |E_{\zeta}|$ new crossings with images of $E^*_{\zeta}$. 
	Finally, since we modified the image of edges in $E_{\zeta}$ such that each of these edges cross $\gamma'$ at most once, the number of intersections between the final images of edges of $E_{\zeta}$ and curve $\gamma'$ is at most $|E_{\zeta}|$. Clearly, these are all new crossings that we may create in an iteration.
	Therefore, summing over all iterations,
	%
	\[
	\cro(\hat\phi)\le \text{ } \cro(\tilde\phi)+\sum_{\zeta \in Z}\bigg(|E_{\zeta}|+|E^*_{\zeta}|+1\bigg)\cdot |E_{\zeta}|
	\le \text{ }  \cro(\tilde\phi)+ \bigg(\sum_{\zeta \in Z}|E_{\zeta}|+|E^*_{\zeta}|\bigg)^2.
	\]
	Since event $\event_1$ does not happen, $\sum_{\zeta \in Z}|E^*_{\zeta}|\le (\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$.
	And from Property \ref{f_prop: no significant in loop}, no significant vertices may belong to any self-loop in $Z$, so the self-loops of $Z$ only contains images of type-1 high-degree vertices and low-degree vertices of $P$.
	Then from Properties \ref{f_prop: K does not cross special edges} and \ref{f_prop: low-degree incident edges small}, $\sum_{\zeta \in Z}|E_{\zeta}|\le O(h\tau^i\mu^{\smallprobability})$.
	Altogether, we get that 
	$$\cro(\hat\phi)\le \text{ } \cro(\tilde\phi)+O\bigg( \frac{\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability}}{m'}+ h\cdot\tau^i\mu^a \bigg)^2=\cro(\tilde\phi)+O\bigg(h^2(\tau^i)^2\mu^{2\smallprobability}\bigg).$$
\end{proof}


\iffalse
$\ $

We say that event $\event$ happens if any of events $\event_1,\event_1,\event_5,\event_3,\event_4$ happens, namely $\event=\event_1\cup\event_1\cup\event_5\cup\event_3\cup\event_4$. From the above discussion, $\Pr[\event]\le O(1/\mu^{\smallprobability})$.
Assuming that event $\event$ does not happen. The properties of the skeleton $K$ can be summarized as follows.

\begin{properties}{F}
	\item $K$ contains at most $\mu^{\interestconst+\smallprobability}$ edges and at most $\mu^{\interestconst+\smallprobability}$ vertices; \label{fact: skeleton is short}
	\item edges of $K$ participate in less than $(\cro\cdot\mu^{\interestconst+\smallprobability})/m$ crossings in $\hat\phi$;\label{fact: skeleton is slightly crossed}
	\item less than $2h'\mu^{\interestconst+\smallprobability}$ edges are incident to a type-1 high-degree vertex of $K$;	
	\label{fact: few incident edges on type-1}
	\item less than $2h\mu^{\interestconst+\smallprobability}$ edges are incident to a low-degree vertex of $K$;
	\label{fact: few incident edges on low-deg}
	\item there is a drawing $\hat\phi'$ of $\hat G'$, such that $\hat \phi'$ respects the rotation system $\hat \Sigma$, the image of $K$ in $\hat\phi'$ is a simple closed curve, and $\cro(\hat\phi')\le \cro+O(h\mu^{\interestconst+\smallprobability})^2$.\label{fact: skeleton drawn as a cycle}
\end{properties}
\fi




\subsubsection*{Stage 2. Correcting the orientations of vertices in $V(K)$}


%In this step we further modify the drawing $\hat\phi$ obtained in the last step, and then split the drawing $\hat\phi$ into almost well-structured drawings $\hat\phi_1, \hat\phi_2$ for instances $I'_1, I'_2$ respectively.

Recall that we have computed, in Step 2 (\Cref{Step 2}), an orientation $b(v)$ for each vertex $v\in V(K)$, and then used them to define inner and outer sides of $K$, which are then used to compute the instances $I'_1, I'_2$.
%We intend to split the drawing the drawing $\hat\phi$ obtained in the last stage into drawings for instances $I'_1, I'_2$, according to the inner and outer sides of $K$.
However, although the drawing $\hat\phi$ computed in the last stage respects the rotation system $\Sigma'$, it may not yet match the orientations on vertices of $K$ computed in Step 2, which is required in Property~\ref{prop: first segments} if it induces well-structured solutions for instances $I'_1, I'_2$. In this stage, we further modify $\hat{\phi}$ by correcting the orientations of vertices of $K$.
%\znote{more argument on why orientations need to be computed}

First, we prove the following observations, which show that, for vertex $v''$ and all significant vertices of $K$, the orientation computed in Step 2 is correct (matched by the drawing $\tilde\phi$, and so also matched by $\hat\phi$ since we have not modified the orientations of vertices when constructing $\hat \phi$ from $\tilde\phi$ in the last stage).

\begin{observation}
The orientation $b''$ (computed in Step 2) on vertex $v''$ coincides the orientation of $v''$ in drawing $\tilde\phi$.
%There exists a unique $b''\in \set{-1,1}$ such that $\dist((\oset',b'),(\oset'',b''))\le \cro(\tilde \phi)$.
\end{observation}
\begin{proof}
Observe that the distances between oriented orderings satisfy the triangle inequality, namely for any oriented rotations $(\oset_1,b_1),(\oset_2,b_2),(\oset_3,b_3)$ on the same set of element, $\dist((\oset_1,b_1),(\oset_3,b_3))\le \dist((\oset_1,b_1),(\oset_2,b_2))+\dist((\oset_2,b_2),(\oset_3,b_3))$. In fact, from the definition of the reordering curves, given a set $\Gamma_{12}$ of reordering curves for oriented orderings $(\oset_1,b_1),(\oset_2,b_2)$ and a set $\Gamma_{23}$ of reordering curves for oriented orderings $(\oset_2,b_2),(\oset_3,b_3)$, it is immediate to concatenate curves in $\Gamma_{12}$ with curves in $\Gamma_{23}$ to obtain a set $\Gamma_{13}$ of reordering curves for $(\oset_1,b_1),(\oset_3,b_3)$, such that $\chi(\Gamma_{13})\le \chi(\Gamma_{12})+\chi(\Gamma_{23})$.

On the one hand, since $\oset''$ is an unoriented ordering on a set of $\Omega(m'/\tau^i)$ elements, it is easy to see that $\dist((\oset'',-1),(\oset'',1))=\Omega\big((m'/\tau^i)^2\big)$. Therefore, since $m'\ge \tau^s$ and \fbox{$\cro(\tilde\phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}, \[\dist((\oset'',-1),(\oset',b'))+\dist((\oset'',1),(\oset',b'))\ge \dist((\oset'',-1),(\oset'',1))\ge  \Omega\big((\tau^s/\tau^i)^2\big)>2\cdot\cro(\tilde\phi),\] 
and so at most one of $\dist((\oset'',-1),(\oset',b')),\dist((\oset'',1),(\oset',b'))$ is less than $\cro(\tilde\phi)$. 

On the other hand, since the paths of $\pset$ are non-transversal with respect to $\Sigma'$, it is easy to show that paths of $\pset$ participate in at most $\cro(\tilde\phi)$ crossings in drawing $\tilde\phi$, so the orientation $b''$ on $v''$ computed in Step 2 coincides the orientation of $v''$ in $\tilde\phi$. 
%Finally, since we have not modified the orientations of vertices when constructing $\hat \tilde\phi$ from $\tilde\phi$. 
%Altogether, we conclude that there exists an unique $b''\in \set{-1,1}$ such that $\dist((\oset',b'),(\oset'',b''))\le \cro(\tilde \tilde\phi)$.
\end{proof}

\begin{observation}
If event $\event$ does not happen, then for each significant vertex $u\ne v',v''$, the orientation $b(u)$ we computed in Step 2 coincides with the orientation of $u$ in drawing $\tilde\phi$.
\end{observation}
\begin{proof}
%Assume for contradiction that there exists some significant vertex $u\in V(K)$, such that the orientation we computed is different from the orientation $b^*_u$ in drawing $\tilde\tilde\phi$. 
Let $u$ be a significant vertex and let $\pset_u$ be the set of paths in $\pset$ that contains vertex $u$. From the definition of a significant vertex, $|\pset_u|\ge h$.
From Property \ref{f_prop: K crossed few times}, edges of $K$ participates in at most $(\cro(\tilde\phi)\cdot\tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde\phi$.
%
%For each path $\hat P\in \pset$, if its first edge lies on the inner side of $K$, while its first edge incident to $u$ lies on the outer side of $K$, then it has to cross $K$. Note additionally that in two different orientations of $u$, at least one  orientation of $u$ will force that the first edge of $P$ lies on the inner side of $K$ and the first edge of $P$ incident to $u$ lies on the outer side of $K$. Therefore, there is only one rotation that will not force event $\event_1$ to happen. And therefore the orientation $b(u)$ that we computed has to coincide with the real orientation of $u$ in drawing $\tilde \tilde\phi$. \znote{to modify}
Denote $\pset_u=\set{P_{i_1},\ldots, P_{i_q}}$, and for each $1\le j\le q$, we denote by $e_{i_j}$ the first edge of $P_{i_j}$ (the edge of $P_{i_j}$ incident to $v'$), and denote by $\tilde e_{i_j}$ the first edge of $P_{i_j}$ incident to $u$. Recall that in Step 2, we say that an index $i_j$ is screwed under $b(v)$, iff when the orientation of $v$ is $b(v)$, edges $e_{i_j}, \tilde e_{i_j}$ are on different sides of $K$. It is easy to show that, if index $i_j$ is screwed under $b(v)$, then the image of path $P_{i_j}$ has to cross $K$. It is also easy to see that, each index $i_j$ is screwed under either $-1$ or $1$ but not both.

Since event $\event$ does not happen, from Property \ref{f_prop: K crossed few times}, $K$ participate in at most $(\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'<h/2$ crossings in $\tilde \phi$.
Since $u$ is a type-2 high-degree vertex, there is exactly one orientation in $\set{-1,1}$ under which the number of screwed indices is less than $h/2$. Therefore, the orientation $b(u)$ computed in Step 2 coincides with the orientation of $u$ in drawing $\tilde\phi$.
\end{proof}

Therefore, we only need to modify the orientation of low-degree vertices and type-1 high-degree vertices. We denote by $V'$ the set of all low-degree vertices and all type-1 high-degree vertices $v$ of $V(K)$, such that the orientation of $v$ in the drawing $\hat\phi$ does not coincide with the orientation $b(v)$ computed in Step 2.
Consider now a vertex $v\in V'$.
Assume without loss of generality that $v$ is a vertex of $P$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P$, $\tilde e$ precedes $\tilde e'$ in $P$, and the edges appear clockwise in the oriented ordering $(\oset_v,b(v))$ of $v$.
Denote by $D=D_{\hat \phi}(v)$ the tiny $v$-disc in drawing $\hat \phi$.
Let $\tilde z$ be the intersection between $\hat\phi(\tilde e)$ with the boundary of disc $D$, and we define (i) a point $\tilde z'$ for $\tilde e'$; (ii) for each $1\le i\le p$, a point $ z_i$ for $\hat e_i$; and (iii) for each $1\le j\le q$, a point $ z'_j$ for $\hat e'_j$ similarly. 
See \Cref{fig: flip} for an illustration.
We place a disc $D'$ around $\hat\phi(v)$, that lies entirely within disc $D$. We then place points  $\delta(v)=\set{\tilde y,  y'_1,  y'_2,\ldots,  y'_q,\tilde y',  y_1,  y_2, \ldots,  y_p}$ on the boundary of $D'$, such that the points appear on the boundary of $D'$ clockwise in this order.
We then compute, a set $\Gamma$ of curves within the annulus $D\setminus D'$ that contains, for each $1\le i\le p$, a curve $\gamma_i$ connecting the point $ y_i$ to $ z_i$, and, for each $1\le j\le q$, a curve $\gamma'_j$ connecting the point $ y'_j$ to $ z'_j$, such that the curves of $\Gamma$ are in general position.
We modify the drawing $\hat\phi$ locally within disc $D$ as follows.
We erase the drawing of $\hat\phi$ inside disc $D$ except for the image of vertex $v$ and the images of edges $\tilde e,\tilde e'$. We now let, for each $1\le i\le p$, the new image of edge $\hat e_i$ be the concatenation of: (i) the line segment within $D'$ connecting $\hat\phi(v)$ to point $\hat y_i$; (ii) the curve in $\gamma_i\in \Gamma$ connecting $ y_i$ to $ z_i$; and (iii) the original image of edge $\hat e_i$ outside the disc $D$, namely the subcurve of $\hat\phi(\hat e_i)$ between $ z_i$ and the image of the other endpoint of $\hat e_i$.
Similarly, we let, for each $1\le j\le q$, the new image of edge $\hat e'_j$ be the concatenation of: (i) the line segment within $D'$ connecting $\hat\phi(v)$ to point $ y'_j$; (ii) the curve in $\gamma'_j\in \Gamma$ connecting $ y'_j$ to $ z'_j$; and (iii) the original image of edge $\hat e'_j$ outside the disc $D$, namely the subcurve of $\hat\phi(\hat e'_j)$ between $ z'_j$ and the image of the other endpoint of $\hat e'_j$.
See \Cref{fig: flip} for an illustration.
Clearly, the number of new crossings we have created in this local modification step is at most $\deg(v)^2$.

We modify the drawing $\hat \phi$ at all vertices of $V'$ in the same way, and denote by $\hat \phi'$ the resulting drawing. It is easy to see that drawing $\hat \phi'$ coincides with all oriented orderings on vertices of $K$ computed in Step 2.
Note that, from properties \ref{f_prop: low-degree incident edges small} and \ref{f_prop: type-1 incident edges small}, the total number of edges that are incident to a type-1 high degree vertex or a low-degree vertex is at most $O\big(h\cdot \tau^i\mu^{\smallprobability}\big)$. Therefore,
\[\cro(\hat\phi')\le \cro(\hat\phi)+\sum_{v\in V(K)}
\deg(v)^2\le \cro(\hat\phi)+O\bigg(h^2(\tau^i)^2\mu^{2\smallprobability}\bigg).\]


\begin{figure}[h]
	\centering
	\subfigure[A schematic view of the drawing $\hat\phi$ around $v$.]{\scalebox{0.1}{\includegraphics{figs/rotation_flip_before.jpg}}}
	\hspace{1cm}
	\subfigure[Curves in $\Gamma$ are shown in dash lines.]{
		\scalebox{0.1}{\includegraphics{figs/rotation_flip_after.jpg}}}
	\caption{An Illustration of orientation-flip at $v$ in Stage 2. \label{fig: flip}}
\end{figure}

Since we have only modified the drawing $\hat \phi$ only locally within tiny discs around vertices of $K$, in the resulting drawing $\hat \phi'$, it still holds that the image of $K$ is a simple closed curve that does not cross any special edge. Therefore, drawing $\hat \phi'$ induces almost well-structured solutions for instances $I'_1$ and $I'_2$.
%there exists, for each cycle $R$ in $\rset(I')\cup \set{K}$, a disc whose boundary is the image of $R$ in $\hat\phi'$, such that all discs are disjoint in their interiors.






\subsubsection*{Stage 3. Split the drawing and further modification on vertices}


%From the construction of instances $I'_1=(G'_1,\Sigma'_1)$ and $I'_2=(G'_2,\Sigma'_2)$, graphs $G'_1$ and $G'_2$ are subgraphs of $G'$. We now let drawing $\hat \phi_1$ be the drawing of $G'_1$ induced by drawing $\hat\phi'$, and let drawing $\hat \phi_2$ be the drawing of $G'_2$ induced by drawing $\hat\phi'$. 
So far we have computed a drawing $\hat \phi'$ that induces almost well-structured drawings of instances $I'_1$ and $I'_2$.
%Moreover, since $G'_1\cap G'_2=K$, and the image of $K$ in $\hat\phi'$ is a simple closed curve, we get that $\cro(\hat\phi_1)+\cro(\hat\phi_2)\le \cro(\hat\phi')$.  
However, it does not induce well-structured drawings of $I'_1$ and $I'_2$ yet. In particular, vertices of $I'_1$ and $I'_2$ may be drawn on both sides of $K$ (so Property \ref{prop: discs interior no vertex} is not satisfied), and the number of edges crossing $K$ may be too large (so Property \ref{prop: niubi edge crossing special cycle} is not satisfied).
In this stage and the next stage, we further modify drawing $\hat \phi'$ so that it induces well-structured drawings of instances $I'_1$ and $I'_2$ respectively.

%We show how to construct drawing $\phi_1$, and the construction for drawing $\phi_2$ is symmetric. 
%Recall that one of the instances $I'_1, I'_2$ corresponds to the inner side of $K$, and the other corresponds to the outer side of $K$.
Recall that $I'_1$ corresponds to the inner side of $K$, namely $G'_1=G_{\inn}$.
%We now modify the drawings $\hat\phi_1$ and $\hat\phi_2$. We describe the two steps of modifying the drawing $\hat\phi_1$, and the modification for drawing $\hat\phi_2$ is symmetric.
Also recall that, in drawing $\hat\phi_1$, the image of $K$ is a simple closed curve. We denote by $\eta_K$ this simple closed curve, so $\eta_K$ partitions the sphere into two faces. We denote by $F$ the face that contains the first segments of the images of edges in $E_{\inn}$.
In this stage, we move the image of all vertices of $G'_{1}$ that are currently drawn out of $F$  inside $F$. In the next stage, we move the image of some edges inside $F$ to avoid crossing $K$.

\newcommand{\move}{\mathsf{Move}}

We now start to describe the algorithm in this stage.
We first describe a subroutine called $\move$ and then show how it is used in this stage. 

\paragraph{Subroutine $\move$.} The input to the subroutine $\move$ consists of 
\begin{itemize}
\item a drawing $\psi$ of $G'_1$;
\item a cluster $W$ of $G'_1$; 
\item a disc $D$ such that all vertices of $W$ are drawn outside of $D$ in $\psi$;
\item an edge $e^*_W\in \delta(W)$ such that the endpoint of $e^*_W$ outside $W$ is drawn inside $D$; 
\item a set $\qset$ of paths routing edges of $\delta(W)$ to $e^*_W$ inside $W$; and
\item a set $\pset=\set{P(e)\mid e\in \delta(W)}$ of paths, such that for each $e\in \delta(W)$, the path $P(e)$ has $e$ as its first edge and has the last endpoint drawn inside disc $D$.
\end{itemize}
See \Cref{fig: move_layout} for an illustration.

%We denote by $E'$ the set of edges that cross the image of $K$ in $\hat \phi_1$, and we denote by $E''$ the subset of $E'$ that contains all edges with exactly one endpoint drawn inside $F$. Note that each edge of $E'\setminus E''$ either has both endpoints drawn inside (or on) $F$ or has both endpoints drawn outside (or on) $F$. 

\begin{figure}[h]
	\centering
	\subfigure[Disc $D$ is shown on the left and cluster $W$ is shown on the right. Edges of $\delta(W)$ with the other endpoint drawn inside $D$ are shown in blue, and edges of $\delta(W)$ with the other endpoint drawn outside $D$ are shown in red.]{\scalebox{0.1}{\includegraphics{figs/move_layout_1.jpg}}}
	\hspace{1cm}
	\subfigure[$e^*_W=e_2$, and the paths of $\qset$ are shown in orange dash lines.]{
		\scalebox{0.1}{\includegraphics{figs/move_layout_2.jpg}}}
	\caption{An Illustration of the input to subroutine $\move$. \label{fig: move_layout}}
\end{figure}

The subroutine $\move(\psi, W, D, e^*_W, \qset,\pset)$ outputs a new drawing $\psi'$ of graph $G'_1$ in which the cluster $W$ is drawn inside $D$. We now describe the steps in the subroutine. Denote by $u,u'$ the endpoints of edge $e^*_W$ where $u\notin W$ and $u '\in W$, so the image of $u$ in $\psi$ lies in disc $D$. 
For each edge $e\in\delta(W)$, we denote by $Q(e)$ the path in $\qset$ that routes $e$ to $e^*_W$.
We denote by $p$ the first crossing between the images of $e^*_W$ and $K$ (we view the curve representing the image of $e^*$ as being directed from $u'$ to $u$).
Let $D'$ be a tiny disc that (i) is entirely contained in $D$; (ii) is arbitrarily close to $p$ but does not contain $p$; and (iii) intersects with no other edge than $e^*_W$. See \Cref{fig: move_1} for an illustration. We then construct, for each edge $e\in \delta(W)\setminus \set{e^*_W}$, a curve $\gamma_e$ that consists of (i) a curve that starts at the image of the endpoint of $e$ in $W$, travels through the thin strip of the image of path $Q(e)$, and ends at some point $x_e$ lying in the tiny $u'$-disc $D_{\psi}(u')$; and (ii) a curve that starts at $x_e$, travels through the thin strip of the image of $e^*_W$, and ends at a point $y_e$ on the boundary of $D'$; such that the curves $\Gamma=\set{\gamma_e}_{e\in \delta(W)\setminus \set{e^*_W}}$ are in general position (we will later specify how to choose the ordering in which points in $\set{y_e\mid e\in \delta(W)}$ appear on the boundary of $D'$). 
We also denote by $y_{e^*_W}$ the last crossing of edge $e^*_W$ and the boundary of $D'$ (so the segment of image of $e^*_W$ between $u$ and $y_{e^*_W}$ is disjoint from the interior of $D'$). 
%Note that, we can additionally ensure that, the ordering in which points $\set{y_e}_{e\in \delta(W)}$ appearing on the boundary of disc $D'$ is identical to the ordering in which the intersections of images of $\delta(W)$ with the boundary of $D$ appear on $D$.
See \Cref{fig: move_2} for an illustration.
%\znote{to change: the disc should be close to the boundary of $D$}

\begin{figure}[h]
	\centering
	\subfigure[Drawing $\psi$ and disc $D'$ (shown in light green).]{\scalebox{0.095}{\includegraphics{figs/move_1.jpg}}\label{fig: move_1}}
	\hspace{1cm}
	\subfigure[Curves in $\Gamma$ are shown in dash lines.]{
		\scalebox{0.095}{\includegraphics{figs/move_2.jpg}}\label{fig: move_2}}
	\caption{An Illustration of constructing curves of $\Gamma$.}
\end{figure}

We now erase the image of $W$ from $\psi$ and put it inside $D'$. Lastly, we compute a set $Z$ of curves connecting points in $\set{y_e\mid e\in \delta(W)}$ to the new image of the endpoint of edges in $\delta(W)$. See \Cref{fig: move_inside} for an illustration. %We prove the following observation.
%
We now show in the following observation that we can indeed computing a circular ordering on points in $\set{y_e\mid e\in \delta(W)}$ and the set $Z$ of curves, such that the number of crossings between $Z$ and the new image of $W$ can be charged to the number of crossings in drawing $\psi$.

%\znote{congestion on paths in $\pset$?}

\begin{observation}
\label{obs: inside_disc drawing}
There exists a circular ordering $\oset_Y$ on points in $Y=\set{y_e\mid e\in \delta(W)}$ and a set $Z$ of curves that contains, for each $e\in \delta(W)$, a curve $\zeta_e$ inside disc $D'$ connecting point $y_e$ to the new image of the endpoint of $e$ in $W$, such that the number of crossings between $Z$ and the new image of $W$ is at most the number of crossings between $W$ and paths in $\pset$ in drawing $\psi$.
\end{observation}
\begin{proof}
Let $\hat W$ be the graph obtained from graph $W\cup \delta(W)$ by contracting all outside-$W$ endpoints of edges in $\delta(W)$ into a single vertex, that we denote by $\hat v$. It is easy to verify that, computing a circular ordering $\oset_Y$ on points in $Y$ and a set $Z$ of curves as required in \Cref{obs: inside_disc drawing} is equivalent to computing a circular ordering $\hat\oset$ on the incident edges of $\hat v$ and a drawing $\hat \phi$ of graph $\hat W$ that respect the orderings $\oset_v$ for all $v\in V(W)$ and the new ordering $\hat{\oset}$.

For each edge $e\in \delta(W)$, we consider the curve representing the image of path $P(e)$ in $\psi$, and denote by $y'_e$ the last crossing between this curve and the image of $K$ in $\psi$ (where we view the curve as being directed from its endpoint in $W$ to its endpoint that is drawn inside $D$), and we denote by $\gamma'_e$ the subcurve of this curve between its endpoint in $W$ and $y'_e$. 
%\znote{to modify: the red curves may be disjoint from $K$: use the routing path in property \ref{condition: layered decomposition routing}}
We now define $\hat \oset'$ to be the circular ordering on set $Y'=\set{y'_e\mid e\in \delta(W)}$ in which points of $Y'$ appear on the image of $K$.
Note that the circular ordering $\hat \oset'$ naturally induces a circular ordering on $\delta(W)$ and therefore on the set of incident edges of $\hat v$, that we denote by $\hat \oset$.
We now a drawing $\hat \phi$ of $\hat W$ as follows. We consider the drawing of $W$ induced by $\psi$ and the curves in $\set{\gamma'_e\mid e\in \delta(W)}$. Note that each curve $\gamma'_e$ contains has an endpoint being the image of a vertex of $W$ and the other endpoint $y'_e$ lying on the boundary of $D$. Recall that all vertices of $W$ are drawn outside $D$. We now contract $D$ into a single point, which automatically identify the points in $Y'$. We view this point as the image of $\hat v$. It is easy to see that the drawing obtained in this way is a drawing of $\hat W$ that respects all circular orderings in $\set{\hat\oset}\cup \set{\oset_v\mid v\in V(W)}$. Moreover, the number of crossings in $\hat \phi$ between the images of edges in $\delta(\hat v)$ and the image of $W$ is at most the number of crossings in $\psi$ between the curves in $\set{\gamma'_e\mid e\in \delta(W)}$ and the image of $W$. \Cref{obs: inside_disc drawing} now follows.
\end{proof}


\begin{figure}[h]
	\centering
	\includegraphics[scale=0.1]{figs/move_3.jpg}
	\caption{An illustration of curves in $Z$ (shown in blue and red solid curves).}\label{fig: move_inside}
\end{figure}


Finally, we set, for each edge $e\in \delta(W)$, the new image of $e$ to be the concatenation of (i) the original image of $e$ in $\psi$; (ii) the curve $\gamma_e$; and (iii) the curve $\zeta_e$. This completes the description of the subroutine $\move(\psi, W, D, e^*_W, \qset,\pset)$.
We denote by $\psi'$ the drawing produced by the subroutine.
Clearly, in $\psi'$, the cluster $W$ is completely drawn inside $D'$ and therefore inside $D$.



We now make some observations on drawing $\psi'$.
From the construction, the original crossings between edges of $W$ remain in the $\psi'$, the original crossings between edges of $\delta(W)$ and edges of $W$ remain in the $\psi'$ (within disc $D'$), since we copied the drawing of $W$ inside $D'$. For each $e\in \delta(W)\setminus \set{e^*_W}$, its new image contains its original image, together with the image of the path $Q(e)$ in $\psi$. Therefore, for each edge $e'\in E(W)\cup\delta(W)$, in the new drawing $\psi'$ there are $\cong_{\qset}(e')$ curves contained in the thin strip of $\psi(e)$.


\iffalse
For each edge $e\in E'$, we view its image $\hat \phi_1(e)$ as being directed from its endpoint in $V'$ to its other endpoint that are drawn inside $F$, and we denote by $z_e$ the first crossing between $e$ and $K$. 
Define $\hat G$ as the graph obtained from $G_{\inn}$ by splitting each edge $e\in E'$ with a new vertex $x_e$, and we denote $X=\set{x_e\mid e\in E'}$.
Clearly, if we view, for each vertex $x_e\in X$, the point $z_e$ as its image, then the drawing $\hat \phi_1$ naturally induces a drawing of $\hat G$. 
For each edge $e\in E'$, we denote by $e^{a}$ the new edge split from $e$ that is incident to the endpoint of $e$ in $V'$, and we denote by $e^{b}$ the other edge split from $e$.
We define $E^a=\set{e^a\mid e\in E'}$ and  $E^b=\set{e^b\mid e\in E'}$.
See \Cref{fig: well-structured_layout} for an illustration.
We now pick an arbitrary vertex $x_{e^*}\in X$. Let $z^*$ be a point in the intersection of the tiny-$x_{e^*}$ disc $D'=D_{\hat \phi_1}(x_{e^*})$ and $F$. Let $D^*$ be a tiny-$z^*$ disc that lies entirely in the intersection of the $D'\cap F$.

\begin{figure}[h]
	\centering
	\subfigure[Disc $D$ is shown on the left and cluster $W$ is shown on the right. Edges of $\delta(W)$ with the other endpoint drawn inside $D$ are shown in blue, and edges of $\delta(W)$ with the other endpoint drawn outside $D$ are shown in red.]{\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_1.jpg}}}
	\hspace{1cm}
	\subfigure[]{
		\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_2.jpg}}}
	\caption{An Illustration of the input to subroutine $\move$. \label{fig: well-structured_layout}}
\end{figure}


Define $H'=H\cup E^a$.
We erase the drawing of $H'$ from drawing $\hat \phi_1$, and place the drawing $\hat \phi_1(H)$ of $H$ inside disc $D^*$, such that the new images of vertices of $X$ lie on the boundary of $D^*$. We now add the edges of $E^b$ back to the drawing as follows. Let $\zeta$ be the segment of $\partial F$ that lies in disc $D'$. We first designate, for each vertex $x_e\in X$, a distinct point $y_e$ on $\zeta$. We then compute a set $\gamma$ of curves that contains, for each vertex $x_e\in X$, a curve $\gamma_e$ that connects $z_e$ to $y_e$ and lies entirely outside of $F$, such that every pair of curves in $\Gamma$ crosses at most once. Finally, we let the new image of $e_2$ be the sequential concatenation of: (i) the previous image of $e_2$ between its endpoints originally drawn inside $F$ to the point $z_e$; and (ii) the curve $\gamma_e$ in $\Gamma$. In this way we obtain a new drawing of graph $\hat G$, and suppressing vertices of $X$, this drawing also induces a drawing of $G_1$, with all vertices lying inside $F$. We then perform type-1 uncrossings (the algorithm from \Cref{thm: type-1 uncrossing}) to the images of all edges in $E'$. We denote by $\phi'_1$ the resulting drawing. See \Cref{fig: well-structured_drawing} for an illustration.
It is easy to observe that, in the resulting drawing, the set of edges that cross $K$ is still $E'$.

\begin{figure}[h]
	\centering
	\subfigure[Before: disc $D^*$ is shown in ligh blue, and segment $\zeta$ is shown in black.]{\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_3.jpg}}}
	\hspace{0.2cm}
	\subfigure[After: drawing of $H'$ is moved into $D^*$, and the new images of edges of $E^a, E^b$ are shown in pink and red, respectively.]{
		\scalebox{0.1}{\includegraphics{figs/well-structured_drawing_4.jpg}}}
	\caption{An Illustration of drawing modification in Stage 3. \label{fig: well-structured_drawing}}
\end{figure}
\fi




We now describe the algorithm in the third stage, that utilizes the subroutine $\move$ and iteratively move the images of all vertices inside $F$.
We start from the drawing $\hat\phi_1$.
Let $V'$ be the set of vertices whose image in $\hat \phi_1$ lie outside $F$, and let $H$ be the subgraph of $G'_1$ induced by vertices of $V'$. %Denote $E'=\delta_{G_{\inn}}(V')$. It is clear that every edge of $E'$ crosses $K$ in $\hat\phi_1$.
We first apply the algorithm from \Cref{thm: layered well linked decomposition} to graph $G'_1$ and its subgraph $G'_1\setminus H$ to compute a layered $\alpha$-well-linked decomposition $(\wset, \lset_1,\ldots,\lset_r)$ of graph $G'_1$ with respect to $G'_1\setminus H$, for $\alpha=O(1/\log^{2.5} m)$.
Now for each cluster $W\in \wset$, we select uniformly at random an edge of $\delta^{\down}(W)$ as $e^*_W$ and then use the algorithm from 
\Cref{cor: simple guiding paths}
%\znote{To add: boundary all to all routing in a well-linked cluster} 
to compute a collection $\qset_W$ of paths routing edges of $\delta(W)\setminus \set{e^*_W}$ to $e^*_W$ (note that, instead of selecting a path set in $\set{\qset^{(e)}\mid e\in \delta(W)}$ uniformly at random, we select a path set in $\set{\qset^{(e)}\mid e\in \delta^{\down}(W)}$ uniformly at random).
Then, we iteratively modify the current drawing $\hat \phi_1$ as follows.
Throughout, we maintain a drawing $\tilde \phi$ of $G'_1$, that is initialized to be $\hat \phi_1$. 
The algorithm continues to be executed as long as there is still some cluster $W\in \wset$ whose image in the current drawing $\tilde \phi$ lies outside $F$.
In each iteration, we select a cluster $W$ of $\wset$, that, among all clusters of $\wset$ that are drawn outside of $F$, minimizes the layer index of the layered $\alpha$-well-linked decomposition that it belongs to.
Clearly, at this moment all clusters from lower layers than $W$ are already moved into $F$ in the current drawing $\tilde \phi$. Since edge $e^*_W$ is chosen from $\delta^{\down}(W)$, the endpoint of $e^*_W$ outside $W$ lies inside $F$ in $\tilde \phi$.
We then run the subroutine $\move(\tilde\phi, W, F, e^*_W, \qset_W)$, and update $\tilde{\phi}$ with the drawing output by the subroutine. We denote by $\phi_1$ the resulting drawing after we processed all clusters of $\wset$ in this way.




%We now count the number of new crossings created in this step. From the algorithm, we may create new crossings between edges of $E'$, but except from that, we create one new crossing between each edge of $E'$ with $K$ (for each $e\in E'$ the new crossing is point $y_e$). Therefore, the total number of new crossings is at most $|E'|+|E'|^2\le 2|E'|^2$.

\newcommand{\load}{\mathsf{load}}

In order to analyze the new crossings created in this stage and prepare for the next stage, we define \emph{load} on edges of $E(H)\cup\delta(H)$, based on the edges $\set{e^*_W}_{W\in \wset}$ and paths sets of $\set{\qset_W}_{W\in \wset}$, as follows.
First consider a cluster $W\in \lset_r$. For each edge of $\delta(W)\setminus \set{e^*_W}$, we define its load to be $0$; for edge $e^*_W$, we define its load to be $|\delta(W)|$. 
For each edge $e\in E(W)$, we define its load to be $\cong_W(\qset_W,e)$.
Assume now that the load for each edge with at least one endpoint lying in $\bigcup_{j+1\le t\le r}V(\lset_t)$ are already defined. Consider now a cluster $W\in \lset_j$. For each edge of $\delta(W)\setminus \set{e^*_W}$ whose load is not yet defined (the edges of $\delta(W)$ with the other endpoint lying in $\bigcup_{1\le t\le j}V(\lset_t)$), we define its load to be $0$; for edge $e^*_W$, we define its load to be the sum of load of all other edges of $\delta(W)$ (notice that the load of all such edges are already defined at this point). For each edge $e\in E(W)$, we define the load of $e$ to be the sum of load of all edges of $\delta(W)$ whose corresponding path in set $\qset_W$ contains edge $e$. This completes the definition of load on all edges of $E(H)\cup\delta(H)$. 
Note that, since the edges $\set{e_W}_{W\in \wset}$ and path sets $\set{\qset_W}_{W\in \wset}$ are chosen randomly, the load on edges of $E(H)\cup\delta(H)$ are random variables.
We prove the following observation.

\begin{observation}
\label{obs: expected load}
For each edge $e\in E(H)\cup\delta(H)$, $\expect[]{\load(e)}=O(\log^{O(1)} m)$.
\end{observation}

\begin{proof}
Note that $E(H)=E^{\out}(\wset)\cup (\bigcup_{W\in \wset}E(H))$.	
%
We first consider the edges of $E^{\out}(\wset)\cup \delta(H)$.
Let $1\le j\le r$ be a layer index and denote $V_j=\bigcup_{j\le t\le r}V(\lset_t)$.
We show by induction on $j$ that, for each edge
$e\in E^{\out}(\wset)$ with at least one endpoint lying in $V_j$, $\expect[]{\load(e)}\le (1+1/\log m)^{r+1-j}$. The base case is when $j=r$. Consider a cluster $W\in \lset_r$. From Property \ref{condition: layered decomp edge ratio} in the definition of a layered well-linked decomposition, $|\delta^{\up}(W)|\le |\delta^{\down}(W)|/\log m$. Since the edge $e^*_W$ is picked uniformly at random from edges of $\delta^{\down}(W)$, the expected load on each edge of $\delta^{\up}(W)$ is $0$, and the expected load on each edge of $\delta^{\down}(W)$ is $|\delta(W)|/|\delta^{\down}(W)|=(|\delta^{\up}(W)|+|\delta^{\down}(W)|)/|\delta^{\down}(W)|\le (1+1/\log m)$.
Assume now that the claim is true for layers $r,\ldots,j+1$. Consider now a cluster $W\in \lset_j$. From the inductive hypothesis, from the linearity of expectations, the expected load of every edge of $\delta(W)$ with the other endpoint lying in $V_{j+1}$ is at most $(1+1/\log m)^{r-j}$. From the definition of load, the load of every edge that connects two distinct clusters of $\lset_j$ is $0$. On the other hand, $|\delta(W)|/|\delta^{\down}(W)|\le (1+1/\log m)$. Therefore, since the edge $e^*_W$ is picked uniformly at random from set $\delta^{\down}(W)$, the expected load on each edge of $\delta^{\down}(W)$ is at most $(1+1/\log m)^{r-j}\cdot (|\delta(W)|/|\delta^{\down}(W)|)\le (1+1/\log m)^{r+1-j}$. As a corollary, the expected load for every edge of $E^{\out}(\wset)\cup \delta(H)$ is at most $(1+1/\log m)^{r}\le O(1)$ (as $r\le \log m$ from \Cref{thm: layered well linked decomposition}).

We now consider edges of $\bigcup_{W\in \wset}E(H)$. Let $W$ be a cluster of $\wset$. From \Cref{cor: simple guiding paths} and our construction, for each edge $e\in E(W)$, $\expect[]{\cong_W(\qset_W,e)}=O(\log^{O(1)} m)$.
Note that the choice of path set $\qset_W$ is independent of the load on edges of connecting $W$ to a vertex in $V_{j+1}$.
Since the expected load for each edge of $\delta(W)$ is $O(1)$, from the definition on loads of edges of $E(H)$ and the linearity of expectations, $\expect[]{\load(e)}=O(\log^{O(1)} m)$. This completes the proof of \Cref{obs: expected load}.
\end{proof}




We now analyze the number of new crossings created in this stage. First, from the construction, in each iteration we move the drawing of some cluster $W\in \wset$ into some tiny disc inside $F$, so their new image do not cross the image of $G'_1\setminus H$. 

\znote{informal from here}
Then from the algorithm, the new image of each cluster $W\in \wset$ participate in at most the same number of crossings as in the original drawing $I'$, with the additive term being $\cro(\tilde \phi)/\mu^{\smallprobability}$ (allowing pairs of edges that cross $K$ to cross). Since we have not modified the image of $G'_1\setminus H$, the new crossings must each involve at least one edge of $E^{\out}(\wset)\cup\delta(H)$. Note that each edge of $\delta(H)$ has to cross $K$ in drawing $\tilde \phi$, and $K$ participates in at most $(\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'$ crossings in $\tilde \phi$. Therefore, $|\delta(H)|\le (\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m'$. Moreover, from the definition of a layered well-linked decomposition, $|E^{\out}(\wset)|\le O(|\delta(H)|)$, so 
\[|E^{\out}(\wset)\cup\delta(H)|=O((\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m').\]
Therefore, the number of new crossings that involve a pair of edges in $E^{\out}(\wset)\cup\delta(H)$ is at most 
\[
O((\cro(\tilde \phi)\cdot \tau^i\cdot\mu^{\smallprobability})/m')^2\le O(\cro(\tilde \phi)/\mu^{\smallprobability}),
\]
where we have used the fact that $m'\ge \tau^s$ and \fbox{$\cro(\tilde \phi)<(\tau^s)^2/30\mu^{\smallprobability}(\tau^i)^{20}$}.

Denote $E'=E^{\out}(\wset)\cup\delta(H)$.
Lastly, for each edge $e\in E'$, in the new drawing there are $\load(e)$ images lying in the thin strip of the original image of $e$, so the number of crossings that involve $e$ is multiplied by a factor of $\load(e)$.
%\znote{to be taken care of later}




\subsubsection*{Stage 4. Further modification on edges}

%\iffalse
We now describe the last stage, in which we move the image of some edges inside $F$.

We say that a vertex $v\in V(K)$ is \emph{heavy} iff $v$ is contained in at least $m/(\tau^i)^{5}$ paths of $\pset$, otherwise we say it is \emph{light}.
We prove the following observations.

\begin{observation}
	\label{obs: few edges incident to non-heavy edges}
	The expected number of edges in $G'$ that is incident to a light vertex of $V(K)$ is $O(m'/(\tau^i)^{4})$.
\end{observation}
\begin{proof}
	Let $v$ be a light vertex. Since it belongs to at most $m'/(\tau^i)^{5}$ paths in $\pset$, the probability that $v$ belongs to path $P$ is $O((m'/(\tau^i)^{5})/(m'/\tau^i))=O(1/(\tau^i)^4)$. Therefore, for an edge $e\in E(G')$ that is incident to a type-1 high-degree vertex, the probability that its type-1 high-degree endpoint belongs to $P$ is $O(1/(\tau^i)^4)$. From the union bound on all edges in $E(G')$, the expected number of edges that are incident to some type-1 high-degree vertex on $P$ is $O(m'\cdot O(1/(\tau^i)^4))=O(m'/(\tau^i)^{4})$. 
	The proof for path $P'$ is symmetric. Therefore, the expected number of edges in $G'$ that is incident to a non-heavy vertex of $V(K)$ is $O(m'/(\tau^i)^{4})$.
\end{proof}

\paragraph{Bad Event $\event_6$.}
We say that the bad event $\event_6$ happens if the number of edges in $G'$ incident to a light vertex of $V(K)$ is at least $m'\cdot\mu^{\smallprobability}/(\tau^i)^{4}$. 
From \Cref{obs: few edges incident to non-heavy edges} and Markov's bound, $\Pr[\event_6]\le O(1/\mu^{\smallprobability})$.

Consider now an edge $e\in E'$. Note that both its endpoints are drawn inside (or on) $C$.

%\fi



\paragraph{Clean edges.} Consider now the resulting drawing $\phi_1$ in the last stage. 
Recall that $E'=E^{\out}(\wset)\cup\delta(H)$, and in $\phi_1$ only edges of $E'$ may cross $K$.
We say that an edge $e\in E'$ is clean, iff, when we denote by $x_1,x_2,\ldots,x_k$ the crossings between $e$ and $K$, where the crossings are indexed according to their appearance on the image of $e$, such that, for each even $1\le i\le k$, the subcurve of the image of $e$ between $x_i$ and $x_{i+1}$, which we denote by $\gamma_i(e)$, lies entirely outside $F$, and moreover, one of the two segments of the image of $K$ separated by points $x_i,x_{i+1}$ contains no heavy vertices.

We prove the following claim.

\begin{claim}
The number of non-clean edges is at most $O(\mu^{2\smallprobability}(\tau^i)^{10})$.
\end{claim}
\begin{proof}

\end{proof}

We now describe the algorithm in this stage. Intuitively, we move the image of all clean edges inside $F$, as follows.















%\newpage

$\ $

\subsection{Phase 1}


\subsection{Phase 2}




\subsection{Completing the Proof of \Cref{lem: many paths}}


We will use the following lemma from \cite{chuzhoy2020towards}.

\begin{lemma}[Lemma 9.2 of \cite{chuzhoy2020towards}]
	There is an efficient algorithm, that, given an instance $(H,\Sigma)$ of the \CNwRS problem, a subset $E'\subseteq E(H)$ of edges of $H$, and a drawing $\phi$ of graph $H\setminus E'$ that respects $\Sigma$, compute a drawing $\phi'$ of $G$ that respects $\Sigma$, such that $\cro(\phi')\le \cro(\phi)+|E'|\cdot |E(H)|$.
\end{lemma}




==> many_paths_main_decomposition_backup.tex <==

%\subsection{Phase 1: Decomposition into small or non-wide subinstances}




\iffalse
From the above discussion, in both cases eventually we obtain two distinct vertices $v',v''$ of $\hat G$ and a set $\pset$ of $\floor{m/\mu^{\interestconst}}$ edge-disjoint paths connecting $v'$ to $v''$. Therefore, from now on we will work with graph $\hat G$, vertices $v',v''$ and the set $\pset$ of paths in $\hat G$.
%
Note that the rotation system $\Sigma$ naturally defines a rotation system $\hat \Sigma$ on graph $\hat G$.
We first apply the algorithm from \Cref{lem: non_interfering_paths} to the instance $(\hat G,\hat \Sigma)$ and the set $\pset$ of paths. We rename the set of paths that we obtain by $\pset$. From \Cref{lem: non_interfering_paths}, the new set $\pset$ contains $\floor{m/\mu^{\interestconst}}$ paths connecting $v'$ to $v''$, that are non-transversal with respect to $\hat \Sigma$.
%
Also note that the drawing $\phi^*$ of $G$ naturally induces a drawing of $\hat G$, which we denote by $\hat\phi$. It is easy to verify that $\hat\phi$ respects the rotation system $\hat \Sigma$ on $\hat G$, and $\cro(\hat\phi)=\cro$.
\fi


The algorithm for \Cref{lem: many path main} is recursive. Throughout, we maintain a collection $\hat{\iset}$ of well-structured subinstances of $I$, that is initialized to be $\hat{\iset}=\set{I}$, and a set $\hat E^{\sf del}$ of edges of $G$, that initially contains no edges. 
As the algorithm proceeds, the collection $\hat{\iset}$ and the set $\hat E^{\sf del}$ 
evolve, and we will ensure that every instance that ever appears in collection $\hat{\iset}$ is well-structured.

\iffalse
\begin{itemize}
\item every instance that ever appears in collection $\hat{\iset}$ is well-structured; and
%\item for every instance $I'=(G,\Sigma)$ that ever appears in collection $\hat{\iset}$, $G$ is a subgraph of $G$; and
\item over the course of the algorithm, the total number of cycles in $\set{\rset(I')}_{I'\in \hat \iset}$ may not exceed $m/\tau^s$ \znote{to fix}.
\end{itemize}
\fi


The algorithm continues to be executed as long as there exists some instance $I'\in \hat\iset$, such that its contracted subinstance $\tilde I'$ is  $\tau^i$-wide and not $\tau^s$-small.

We now describe an iteration of the algorithm. Let $I'=(G',\Sigma')$ be an instance in the current collection $\hat\iset$ whose contracted subinstance is $\tau^i$-wide and not $\tau^s$-small. 
We denote by $\tilde I'=(\tilde G',\tilde \Sigma')$ its contracted subinstance.
Denote $m'=|E(\tilde G')|$, so $m'>\tau^s$.
Let $\rset$ be the set of special cycles for instance $I'$ and denote $V_{\rset}=\set{v_R\mid R\in \rset}$, so $V(\tilde G')=\big( V(G')\setminus V(\rset) \big)\cup V_{\rset}$.
%
We use the following simple claim, whose proof uses standard max-flow techniques and is deferred to \Cref{apd: Proof of different cases}.

\iffalse\begin{claim}
\label{clm: find the witness}
There is an efficient algorithm, that, given an instance $I'=(G',\Sigma')$, checks whether or not instance $I'$ is wide, and if so, compute a set $\pset$ of paths as a witness for $I'$.
\end{claim}

We first use the algorithm in \Cref{clm: find the witness} to compute a set $\pset$ of paths as the witness for $\tilde I'$.
Consider now the subgraph $\tilde G''$ of graph $\tilde G'$ induced by all edges of $E(\pset)$.
We use the following claim, whose proof uses standard techniques and is deferred to \Cref{apd: Proof of different cases}.\fi

\begin{claim}
\label{clm: different cases}
There is an efficient algorithm, that, takes as input a well-structured instance $I'=(G',\Sigma')$ and a parameter $\tau^i>0$, checks whether or not its contracted subinstance $\tilde I'=(\tilde G', \tilde\Sigma')$ is $\tau^i$-wide, and if so, compute a set $\pset$ of paths or cycles in graph $\tilde G'$, such that $|\pset|\ge m'/3\tau^i$, each path of $\pset$ has length at most $\tau^i\cdot\mu^{10\interestconst}$, and at least one of the following happens:
\begin{enumerate}
\item there are a pair $v',v''\in V(\tilde G')\setminus V_{\rset}$ of vertices in $\tilde G'$, such that all elements of $\pset$ are paths that connect $v'$ to $v''$ and do not contain any vertex of $V_{\rset}$;
\label{case: clean paths}
\item there is a vertex $v_R\in V_{\rset}$, such that all elements of $\pset$ are cycles that contain vertex $v_R$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R}$;
\label{case: cycles}
\item there are a vertex $v_R\in V_{\rset}$ and a vertex $v\in V(\tilde G')\setminus V_{\rset}$, such that all elements of $\pset$ are paths that connect $v_R$ to $v$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R}$;\label{case: paths with one node}
\item there are two vertices $v_R, v_{R'}\in V_{\rset}$, such that all elements of $\pset$ are paths that connect $v_R$ to $v_{R'}$ and do not contain any vertex from $V_{\rset}\setminus \set{v_R, v_{R'}}$.
\label{case: paths with two nodes}
\end{enumerate}
\end{claim}

We now consider each of the cases in \Cref{clm: different cases} in turn, as follows.
We first consider Case \ref{case: clean paths}.
\znote{to consider other cases}

\znote{overview here}

\subsubsection{Step 1. Computing a new special cycle $K$}
\label{Step 1}

Let $v',v''$ be the endpoints of all paths of $\pset$. Since no paths of $\pset$ contains any vertex of $V_{\rset}$, the paths of $\pset$ are also paths in graph $G'$.
%
We view all paths of $\pset$ as being directed from vertex $v'$ to vertex $v''$.
We denote $L=|\pset|$ and denote by $E_1=\set{e_0,\ldots,e_{L-1}}$ the set of edges that serve as the first edge of paths of $\pset$, where the edges are indexed according to the ordering ${\oset}_{v'}\in \Sigma$.
We choose an index $z\in \set{0,\ldots,\floor{L/2}-1}$ uniformly at random, and let $z'= z+\floor{L/2}$. We denote by $\tilde P$ the path in $\pset$ whose first edge is $e_z$, and denote by $\tilde P'$ the path in $\pset$ whose first edge is $e_{z'}$. We define $\tilde K=\tilde P\cup \tilde P'$, so $\tilde K$ is a subgraph of $G'$. Since $I'=(G',\Sigma')$ is a subinstance of the input instance $I=(G,\Sigma)$, $G'$ is a subgraph of $G$, so $\tilde K$ is also a subgraph of $G$.

If paths $\tilde P$ and $\tilde P'$ do not share inner vertices, then we denote $P=\tilde P$, $P'=\tilde P'$, and $K=\tilde K$.
If paths $\tilde P$ and $\tilde P'$ share inner vertices, then we let $v^*$ be the first inner vertex of $\tilde P$ that is also contained in $\tilde P'$. We denote by $P$ the subpath of $\tilde P$ between $v'$ and $v^*$, and  denote by $P'$ the subpath of $\tilde P'$ between $v'$ and $v^*$. Therefore, the paths $P, P'$ are internally vertex-disjoint.
We unname the previous vertex $v''$ and rename $v^*$ by $v''$.
We then define $K=P\cup P'$, so $K$ is a cycle, and $K\subseteq\tilde K$ is a subgraph of $G'$. Therefore, $P$ and $P'$ are paths of $G'$ and are also paths of $G$.
Since every path of $\pset$ has length at most $\tau^i\cdot\mu^{10\interestconst}$, from the construction of $K$, $|E(K)|\le 2\tau^i\cdot\mu^{10\interestconst}$.


In the following steps, we will ``cut the instance $I'$ along $K$'' into two subinstances $I'_1, I'_2$, and cycle $K$ computed in this step will be a special cycle in both $I'_1$ and $I'_2$.


\iffalse
We prove the following observation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse{whp version}

\begin{observation}
	\label{obs: skeleton number of edges}
	The probability that $K$ contains more than $\mu^{\interestconst+\smallprobability}$ edges is at most $O(1/\mu^{\smallprobability})$.
\end{observation}
\begin{proof}
	For each $0\le i\le \floor{L/2}-1$, we denote by $K_i$ the subgraph formed by the union of the path in $\pset$ whose first edge is $e_i$ and the path in $\pset$ whose first edge is $e_{i+\floor{L/2}}$. Since the paths of $\pset$ are edge-disjoint, the subgraphs $K_0,\ldots ,K_{\floor{L/2}-1}$ are edge-disjoint, and therefore the expected number of edges of a random subgraph of $\set{K_0,\ldots,K_{\floor{L/2}-1}}$ is at most $m/\floor{L/2}< O(\mu^{\interestconst})$. From Markov's bound, the  probability that $K$ contains more than $\mu^{\interestconst+\smallprobability}$ edges is at most $O(\mu^{\interestconst})/\mu^{\interestconst+\smallprobability}=O(1/\mu^{\smallprobability})$.
\end{proof}

\fi









%\iffalse{expectation version}

\begin{observation}
	\label{obs: skeleton number of edges}
	$\expect[]{|E(K)|}=O(\tau^i)$.
\end{observation}
\begin{proof}
	For each $0\le z\le \floor{L/2}-1$, we denote by $\tilde K_z$ the subgraph formed by the union of the path in $\pset$ whose first edge is $e_z$ and the path in $\pset$ whose first edge is $e_{z+\floor{L/2}}$. Since the paths of $\pset$ are edge-disjoint, the subgraphs $\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}$ are edge-disjoint, and therefore the expected number of edges in $\tilde K$, a random element in set $\set{\tilde K_0,\ldots, \tilde K_{\floor{L/2}-1}}$, is at most $O(m'/L) \le  O(\tau^i)$. Since $K\subseteq \tilde K$, we get that $\expect[]{|E(K)|}=O(\tau^i)$.
\end{proof}



\paragraph{Bad Event $\event_1$.}
We say that the bad event $\event_1$ happens if $K$ contains more than $\tau^i\cdot\mu^{\smallprobability}$ edges. 
From \Cref{obs: skeleton number of edges} and Markov's bound, $\Pr[\event_1]\le O(1/\mu^{\smallprobability})$.

\fi

%In the remainder of this subsection, we prove several useful properties of $K$ which will be used later.
%We denote by $\phi^*_G$ the drawing of graph $G$ induced by drawing $\phi^*$ (recall that $G$ is a subgraph of the input graph $G$).


%We then check whether or not any of events $\event_1,\event_3,\event_4,\event_5$ happens (it is easy to see that this can be done efficiently). If so, then we return FAIL and terminate the algorithm. Otherwise, we continue to the next steps.
%and will eventually compute a collection of well-structured subinstances of the input instance $I=(G,\Sigma)$. From the above discussion, the probability that we return FAIL in Step 1 is $O(1/\mu^{\smallprobability})$.


%\znote{modify the def of type-2 high-degree vertices, and rename them significant vertices}


\subsubsection{Step 2. Computing the inner and outer sides of $K$}
\label{Step 2}


Recall that all paths of $\pset$ are being directed from $v'$ to $v''$. Recall that we have denoted by $e_0,\ldots, e_{L-1}$ the set of first edges of paths in $\pset$, where edges are indexed according to the ordering $\oset_{v'}$. For each $0\le j\le L-1$, we denote by $P_j$ the path in $\pset$ that has $e_{j}$ as its first edge, and we denote by $e'_{j}$ the last edge of $P_j$.
In order to ``cut instance $I'$ along $K$'' into subinstances $I'_1$ and $I'_2$, we will need to define the ``inner and outer sides'' of $K$, which we do in this step.
%As a first step towards this goal, in this step we compute the orientations of orderings of all vertices of $K$.

First, since the a drawing of any graph and its mirror image are viewed as identical drawings, we can fix the orientation of the ordering $\oset_{v'}$ to be positive, without loss of generality. 
%In other words, if we traverse along the boundary of a disc around $v'$ counter-clock-wise, then we will encounter edges of $e_0,\ldots, e_{L-1}$ sequentially.
This oriented ordering naturally induces an oriented ordering on the set $\set{P_0,\ldots, P_{L-1}}$ of paths, which we denote by $(\oset',b')$.
%We will show that the orientations of $v''$ and all significant vertices can be fixed as well.


Next we consider the vertex $v''$. Note that edges $e'_{0},\ldots,e'_{L-1}$ belong to set $\delta(v'')$, and the circular ordering $\oset_{v''}\in \Sigma$ is an circular ordering on the set $\set{e'_{0},\ldots,e'_{L-1}}$, which in turn induces an circular ordering on the set $\set{P_{0},\ldots,P_{L-1}}$ of paths, that we denote by $\oset''$.
Clearly, computing an orientation of the unoriented ordering $\oset_{v''}$ is equivalent to computing an orientation of the unoriented ordering $\oset''$.
We compute an orientation $b''\in \set{-1,1}$ of $\oset''$ as follows.
We set $b''=1$ iff $\dist((\oset', b'),(\oset'',1))\le \dist((\oset', b'),(\oset'',-1))$; otherwise we set $b''=-1$.
In other words,  
\[b''=\arg\min_{b\in \set{-1,1}}\set{\dist((\oset', b'),(\oset'',b))}.\]


Consider now a vertex $v\in V(K)$. Assume without loss of generality that $v$ belongs to path $P$. We denote by $\pset_v=\set{P_{i_1},\ldots,P_{i_q}}$ the set of all paths $\pset$ that contains vertex $v$. 
%From the definition of a significant vertex, $q\ge h'$. 
For each $1\le j\le q$, we denote by $\tilde e_{i_j}$ the first edge of $P_{i_j}$ that is incident to $v$ (recall that paths of $\pset$ are being directed from $v'$ to $v''$),
%Additionally, we denote by $\tilde e, \tilde e'$ the edge of $P$ that are incident to $v$.
and recall that we have denoted by $e_{i_j}$ the first edge of $P_{i_j}$, so $e_{i_j}$ is incident to $v'$.
Note that we have already fixed an orientation of the ordering $\oset_{v'}$ to be positive. Let $b(v)\in \set{-1,1}$ be an orientation of ordering $\oset_v$. 
Let $e$ be the first edge of $P$ and let $e'$ be the first edge of $P'$.
We say that an index $i_j$ is \emph{screwed under $b(v)$}, iff either edges $e,e_{i,j},e'$ appear clockwise in the oriented ordering $(\oset_{v'},+1)$ and edges $\tilde e, \tilde e_{i,j},\tilde e'$ appear clockwise in the oriented ordering $(\oset_{v},b(v))$ or edges $e',e_{i,j},e$ appear clockwise in the oriented ordering $(\oset_{v'},+1)$ and edges $\tilde e',\tilde e_{i,j},\tilde e$ appear clockwise in the oriented ordering $(\oset_{v},b(v))$.
We then set $b(v)$ as follows. If the number of indices in $\set{i_1,\ldots, i_q}$ that are screwed under $1$ is greater than the number of indices in $\set{i_1,\ldots, i_q}$ that are screwed under $-1$, then we set $b(v)=-1$, otherwise we set $b(v)=1$.


\iffalse
Note that the circular ordering $\oset'$ on set $\pset$ of paths naturally induces a circular ordering on the set $\pset_v$ of paths, that we denote by $\oset'_v$. Also note that the circular ordering $\oset_v\in  \Sigma$ naturally induces a circular ordering on the set $\set{\tilde e_{i_j}\mid 1\le j\le q}$ of edges, which in turn induces an ordering on the set $\pset_v$ of paths, that we denote by $\oset''_v$. 
Clearly, computing an orientation of the unoriented ordering $\oset_{v}$ is equivalent to computing an orientation of the unoriented ordering $\oset''_v$.
We compute an orientation $b''_v\in \set{-1,1}$ of $\oset''_v$ as follows.
We set $b(v)=1$ iff $\dist((\oset'_v, b'),(\oset''_v,1))\le \dist((\oset'_v, b'),(\oset''_v,-1))$; otherwise we set $b(v)=-1$.
In other words,
\[b(v)=\arg\min_{b\in \set{-1,1}}\set{\dist((\oset'_v, b'),(\oset''_v,b))}.\]
\fi

%\paragraph{Computing the Inner and Outer sides of $K$.}
So far we have computed, for each  vertex of $K$, an orientation of its circular ordering in $\Sigma$. Let $v$ be an inner vertex of $P$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P$, edge $\tilde e$ precedes edge $\tilde e'$ in $P$, and the edges appear clockwise in the oriented ordering on $v$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are on the \emph{inner side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are on the \emph{outer side} of $K$.
%
Similarly, let $v$ be an inner vertex of $P'$, and denote $\delta(v)=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e,\tilde e'$ belong to $P'$, edge $\tilde e$ precedes edge $\tilde e'$ in $P'$, and the edges appear clockwise in the oriented ordering on $v$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are on the \emph{outer side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are on the \emph{inner side} of $K$.
%
For vertex $v''$, we denote  assume that $\delta(v'')=\set{\tilde e, \hat e_1, \hat e_2,\ldots, \hat e_p,\tilde e', \hat e'_1, \hat e'_2, \ldots, \hat e'_q}$, where edges $\tilde e$ is the last edge of $P$ and $\tilde e'$ is the last edge of $P'$, and the edges appear clockwise in the oriented ordering at $v''$.
We say that edges $\hat e_1, \hat e_2,\ldots, \hat e_p$ are \emph{on the inner side} of $K$, and say that edges $\hat e'_1, \hat e'_2, \ldots, \hat e'_q$ are \emph{on the outer side} of $K$.






\subsubsection{Step 3. Decomposing instance $I'$ into two subinstances}
\label{Step 3}

%From this step, we will maintain a set $E^*$ of edges of $\hat G$, that we call the set of \emph{deleted edges}. The set $E^*$ evolves over the course of the algorithms, and eventually edges of $E^*$ will not appear in the subinstances that we construct.

Consider the contracted subinstance $\tilde I'=(\tilde G',\tilde \Sigma')$ of the well-structured instance $I'$. Since we have assumed that paths of $\pset$ do not contain special vertices of graph $G'$, $K$ is also a cycle in $\tilde G'$, and for each vertex $v\in V(K)$, $\delta_{G'}(v)=\delta_{\tilde G'}(v)$. 
We will decompose graph $\tilde G'$ into two subgraphs, and then construct two subinstances of $I'$ based on them.

%We let set $E^*$ contains all edges of $E(G')\setminus E(K)$ that are incident to a low-degree vertex of $K$ or a type-1 high-degree vertex of $K$. Assume that the events $\event_4,\event_5$ do not happen, then $|E^*|\le O\big((h+h')\tau^i\mu^{\smallprobability}\big)$.
%If event $\event$ does not happen, then from Properties \ref{fact: few incident edges on type-1} and \ref{fact: few incident edges on low-deg}, there are a total of $O(h\mu^{\interestconst+\smallprobability})$ such edges.
%\znote{we do not know the value of $h$ and $h'$, so this step is problematic}

%Consider now the graph $\hat G= \tilde G'\setminus E^*$. 
We denote by $\hat E$ the set of all edges of $E(\tilde G')\setminus E(K)$ that is incident to a vertex of $K$, so each edge of $\hat E$ is incident to either vertex $v'$, or vertex $v''$, or an inner vertex of $P$ or $P'$.
%Therefore, each such edge is either on the inner side of $K$ or on the outer side of $K$. 
We denote by $\hat E_{\inn}$ the set of all edges of $\hat E$ that are on the inner side of $K$, and denote by $\hat E_{\out}$ the set of all edges of $\hat E$ that are on the outer side of $K$. Clearly, sets $\hat E_{\inn},\hat E_{\out}$ partition $\hat E$. Note that, from the construction of cycle $K$, $|\hat E_{\inn}|\ge |\hat E_{\inn}\cap \delta_{G'}(v')| \ge \floor{L/2}$, and similarly $|\hat E_{\out}|\ge |\hat E_{\out}\cap \delta_{G'}(v')|\ge \floor{L/2}$.

In order to decompose graph $\tilde G'$ into two subgraphs, it will be convenient for us to slightly modify the graph $\tilde G'$, by splitting each vertex $v\in V(K)$ into three vertices: vertex $v_{\inn}$, that is incident to the edges of $\hat E_{\inn}\cap \delta(v)$, vertex $v_{\out}$, that is incident to the edges of $\hat E_{\out}\cap \delta(v)$, and vertex $v_{M}$, that is incident to two edges of $E(K)\cap \delta(v)$. 
We denote by $\hat G$ the resulting graph.
We define $V_{\inn}=\set{v_{\inn}\mid v\in V(K)}$, and define sets $V_{\out}$ and $V_{M}$ similarly, so $V(\hat G)=V_{\inn}\cup V_{\out}\cup V_{M}\cup (V(G')\setminus V(K))$.
%
Note that in graph $\hat G$, $K$ is a cycle on vertices of $V_M$ and is disconnected from the rest of the graph.

We then compute, using the standard max-flow techniques, a minimum-cardinality set $E^{*}$ of edges of $\hat G$, whose removal separates vertices of $V_{\inn}$ from $V_{\out}$ in $\hat G$. We add the edges of $E^*$ into the set $\hat E^{\sf del}$.


We now construct two new instances as follows. First, let $\tilde G_{\inn}$ be the graph obtained from subgraph of $\hat G$ consisting of all connected components of $\hat G\setminus E^{*}$ that contain vertices of $V_{\inn}\cup V_{M}$, by identifying, for each vertex $v\in V(K)$, the corresponding vertex $v_{\inn}\in V_{\inn}$ with the corresponding vertex $v_M\in V_M$.
It is easy to verify that $\tilde G_{\inn}$ is a subgraph of $\tilde G'$.
%(recall that $\tilde G'$ is the graph obtained from $G'$ by contracting each special cycle $R\in\rset(I')$ into a single vertex $v_R$). 
We now let $G_{\inn}$ be the graph obtained from $\tilde G_{\inn}$ by uncontracting each special vertex $v_R$ back to the cycle $R$. It is easy to verify that graph $G_{\inn}$ is a subgraph of $G'$. We then let $\Sigma_{\inn}$ be the rotation system on $G_{\inn}$ induced by the rotation system $\Sigma'$ on $G'$, and define the instance $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$. For $I_{\inn}$ to be a well-structured subinstance, we still need to define its set $\rset(I_{\inn})$ of special cycles.
Note that each special cycle of instance $I'$ now either entirely belongs to $G_{\inn}$ or entirely belongs to $G_{\out}$.
We then let set $\rset(I_{\inn})$ contain all special cycles in $\rset(I')$ that entirely belongs to $G_{\inn}$ and the cycle $K$, namely $\rset(I_{\inn})=\set{R\mid v_R\in V(\tilde G_{\inn})}\cup \set{K}$. Clearly, the cycles in $\rset(I_{\inn})$ are edge-disjoint (and even vertex-disjoint in this case).
This completes the construction of instance $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$.
It is then easy to verify that $I_{\inn}$ is a well-structured subinstance of $I'$.
We construct the well-structured subinstance $I_{\out}=(G_{\out}, \Sigma_{\out})$ and its set $\rset(I_{\out})$ of special cycles similarly.

We prove the following immediate observations, that will be later used in \Cref{subsec: analysis of decomposition lemma} for the analysis of the algorithm.

\begin{observation}
\label{obs: number of edges in base}
$|E(G_{\inn})|+|E(G_{\out})|\le |E(G')|+|E(K)|$, and
$|E(G_{\inn})|, |E(G_{\out})|\le |E(G')|-\tau^s/6\tau^i$.
\end{observation}
\begin{proof}
From the construction of graphs $G_{\inn},G_{\out}$, $E(G_{\inn}),E(G_{\out})\subseteq E(G')$, and the only edges of $G'$ that belong to both $E(G_{\inn})$ and $E(G_{\out})$ are edges of $E(K)$, so $|E(G_{\inn})|+|E(G_{\out})|\le |E(G')|+|E(K)|$.

On the other hand, observe that edges of $\hat E_{\out}$ may not belong to set $E(G_{\inn})$, since otherwise some vertex of $V_{\out}$ (the endpoint of any edge of $\hat E_{\out}\cap E(G_{\inn})$ in $V_{\out}$) must be reachable from some vertex of $V_{\inn}$ in $G_{\inn}$, contradicting the definition of $E^*$ and the construction of $\tilde G_{\inn}$.
Therefore, $|E(G_{\inn})|\le |E(G')|-\floor{L/2}$, and similarly $|E(G_{\out})|\le |E(G')|-\floor{L/2}$.
From \Cref{clm: different cases}, $L\ge m'/3\tau^i\ge \tau^s/3\tau^i$, and \Cref{obs: number of edges in base} now follows.
\end{proof}


\begin{observation}
\label{obs: 2 new special cycles}
$|\rset(I_{\inn})|+|\rset(I_{\out})|= |\rset(I')|+2$.
\end{observation}
\begin{proof}
Since the cycle $K$ in graph $\tilde G'$ does not contain any special vertex, from the construction of the graphs $G_{\inn}, G_{\out}$, each special cycle in $\rset(I')$ belongs to either $G_{\inn}$ or $G_{\out}$ (but not both). Also note that the sets $\rset(I_{\inn})$ and $\rset(I_{\out})$ contain one additional new cycle $K$. Therefore, $|\rset(I_{\inn})|+|\rset(I_{\out})|= |\rset(I')|+2$.
\end{proof}


This completes the description of the three steps in an iteration. Finally, we replace the subinstance $I'=(G',\Sigma')$ in the collection $\hat \iset$ with two new subinstances $I_{\inn}=(G_{\inn}, \Sigma_{\inn})$ and $I_{\out}=(G_{\out}, \Sigma_{\out})$, and proceed to the next iteration. 
We denote by $\iset$ the resulting collection $\hat{\iset}$ at the end of the algorithm, and denote by $E^{\sf del}$ the resulting set $\hat E^{\sf del}$ at the end of the algorithm.
Finally, we define the subinstance $\hat I$ as follows. Its graph $\hat G=G\setminus E^{\sf del}$, its rotation system is $\Sigma$, and its set of special cycles is $\rset$, the set of special cycles of $I$. This completes the description of the algorithm.



==> nice-instance-disengagement-step3-4.tex <==


\subsubsection*{Step 3. Segments Connecting Centers of Clustes}  



In this step, we construct paths (that we call \emph{segments}), that connect center vertices of consecutive verterbrae.

Consider some edge $e\in \hat E$ and the corresponding mid-segment $P^2(e)\in \pset^2$ of the nice guiding path $P(e)\in \hat \pset$. 
Assume that path $P^2(e)$ originates at a vertex of $S_{i'}$ and terminates at a vertex of $S_{j'}$, for some $i'<j'$. We define  $\spann'(e)=\set{i',i'+1,\ldots,j'-1}$. Clearly, from our definition, $\spann(e)\subseteq \spann'(e)$.
From the definition of nice guiding paths, there is a sequence $e_{i'},e_{i'+1},\ldots,e_{j'-1}$ of edges that appear on path $P^2(e)$ in this order, such that, for all $i'\leq z\leq j'-1$, edge $e_z$ connects a vertex of $S_z$ to a vertex of $S_{z+1}$. Moreover, if $\set{P_{i'}(e),P_{i'+1}(e),\ldots,P_{j'}(e)}$ is the sequence of paths obtained from $P^2$ after deleting the edges in set $\set{e_z}_{i'\leq z<j'}$ from it, then for all $i'\leq z\leq j'$, $P_z(e)\subseteq S_z$. 

For each $i'\leq z\leq j'-1$, let $R_{z}(e)$ be a new path, that is obtained by concatenating two paths: path  $Q_{z}(e_z)\in \qset_z$, that routes edge $e_z$ to the center vertex $u_z$ of $S_z$; and path $Q_{z+1}(e_z)\in \qset_{z+1}$, that routes edge $e_z$ to the center vertex $u_{z+1}$ of $S_{z+1}$. Clearly, path $R_z(e)$ connects $u_z$ to $u_{z+1}$, and we view it as being directed from $u_z$ to $u_{z+1}$. 



Fix an index $1\leq t<r$. We define a path set $\rset_t$, containing the segment $R_t(e)$ of every edge $e\in \hat E$, for which index $t$ lies in the set $\spann'(e)$.
Clearly, all paths in $\rset_{t}$ originate at vertex $u_t$ and terminate at vertex $u_{t+1}$. Let $N_t$ denote the number of all edges 
$e\in \hat E$, with $t\in \spann'(e)$. Then $|\rset_t|=N_t$ must hold.


Consider again some edge $e\in \hat E$, and assume that $\spann'(e)=\set{i',i'+1,\ldots,j'-1}$. Recall that we have also defined a path $P^{\out}(e)$, whose endpoints lie in $\set{u_1,\ldots,u_r}$. We denote the endpoints of $P^{\out}(e)$ by $u_{i''},u_{j''}$, where $i''<j''$, and we define $\spann''(e)=\set{i'',i''+1,\ldots,j''-1}$. 
For an index $1\leq t<r$, we let $N'_t$ be the number of all edges 
$e\in \hat E$, with $t\in \spann''(e)$. We need the following claim, whose proof appears in \Cref{subsec: enough segments}.

\begin{claim}\label{claim: enough segments}
	For all $1\leq t<r$, $N'_t=N_t$.
\end{claim}



%We then let $\tilde P^2(e)$ be the path obtained by concatenating the paths $P^*_{i'}(e),P^*_{i'+1}(e),\ldots,P^*_{j'-1}(e)$. Notice that this new path $\tilde P^2(e)$ connects the center vertex $u_{i'}$ of $S_{i'}$ to the center vertex $u_{j'}$ of $S_{j'}$. 



We now provide some intuition. Since, from \Cref{claim: enough segments}, for  all $1\leq t<r$, $N'_t=N_t=|\rset_t|$, we could assign, to each edge $e\in \hat E$ with $t\in \spann''(e)$, a distinct segment $R'_t(e)\in \rset_t$. Consider now some edge $e\in \hat E$, and assume that $\spann''(e)=\set{i'',i''+1,\ldots,j''-1}$. Then for all $i''\leq t\leq j''-1$, we have assigned a segment $R_t'(e)$ to edge $e$, and we could let path $P^{\inn}(e)$ be obtained by concatenating all these segments. This final path connects the endpoints of the path $P^{\out}(e)$, and we could then let the auxiliary cycle $W(e)$ be the union of the paths $P^{\inn}(e)$ and $P^{\out}(e)$. However, if $W(e),W(e')$ are two cycles in the resulting collection $\set{W(e'')\mid e''\in \hat E}$ of auxiliary cycles, then there could be a large number of vertices $v\in V(W(e))\cap V(W(e'))$, such that the intersection of $W(e)$ and $W(e')$ at $v$ is transversal with respect to $\Sigma$. We will eventually use the 
auxiliary cycles in order to construct solutions for subinstances of the input instance $I$ that we compute, and such transversal intersections of cycles may give rise to a large number of crossings in the resulting drawings, which we cannot afford.
In order to overcome this difficulty, for each for $1\leq t<r$, we assign the segments of $\rset_t$ to the edges $e\in \hat E$ with $t\in \spann''(e)$ more carefully, in the next step. The resulting segments will be combined into the paths $P^{\inn}(e)$ for edges $e\in \hat E$ as before, and the final auxiliary cycle $W(e)$ will be obtained by combining $P^{\out}(e)$ with $P^{\inn}(e)$ as before. However, we will now  ensure that, for every pair $W(e),W(e')$ of the resulting auxiliary cycles, there is at most one vertex $v\in  V(W(e))\cap V(W(e'))$, such that the intersection of $W(e)$ and $W(e')$ at $v$ is transversal. This will allow us to bound the number of crossings in the optimal solutions of the subinstances of $I$ that we construct. For convenience, for all $1\leq t<r$, we call the paths in set $\rset_t$ \emph{segments}.


\iffalse
\mynote{this seems a bit problematic. Paths of $\rset^*_{(t-1)}$ and of $\rset^*_{(t)}$ both contain vertices of $S_t$. You want to also say that paths of $\rset^*_{(t-1)}\cup \rset^*_{(t)}$ are non-interfering inside $S_t$. Originally, the paths of $\qset_t$ were non-interfering inside $S_t$. But does this property still hold after this step? If yes, this needs a proof! Also: do we actually need this step? If the paths of $\qset_t$ are non-interfering, and the paths of $\qset_{t+1}$ are non-interfering, won't this mean that the paths of $\pset^*_{(t)}$ are non-interfering?}
 We then apply the algorithm in Lemma~\ref{lem: non_interfering_paths} to the instance $(G,\Sigma')$, the set $\pset^*_{(t)}$ of paths, and the two multisets that contains $|\pset^*_{(t)}|$ copies of $u_{t}$ and $|\pset^*_{(t)}|$ copies of $u_{t+1}$ respectively, and obtain a set $\rset^*_{(t)}$ of $|\rset^*_{(t)}|=|\pset^*_{(t)}|$ paths connecting $u_t$ to $u_{t+1}$, such that for every $e\in E(G')$, $\cong_{G'}(\rset^*_{(t)},e)\le \cong_{G'}(\pset^*_{(t)},e)$, and the set $\rset^*_{(t)}$ of paths are non-transversal with respect to $\Sigma$.
\fi




%We use the following observation, whose proof appears in Appendix~\ref{apd: Proof of rerouting_matching_cong}.

%\znote{Need to rethink which definition to include for ``non-transversal".}


\subsubsection*{Step 4. Constructing the Paths of $\pset^{\inn}=\set{P^{\inn}(e)\mid e\in \hat E}$}  
%We now construct the inner paths $\pset=\set{P_e\mid e\in E'}$ as follows.


Consider an edge $e\in \hat E$, and assume that $\spann''(e)=\set{i'',i''+1,\ldots,j''-1}$. We will construct a collection $\tilde \rset(e)=\set{\tilde R_{i''}(e),\ldots,\tilde R_{j''-1}(e)}$ of paths, where for all $i''\leq t<j''$, $\tilde R_t(e)$ is a segment from the set $\rset_t$. The final path $P^{\inn}(e)$ will then be obtained by concatenating all segments in $\tilde \rset(e)$.

We construct the collections $\tilde \rset(e)$ of segments for all edges $e\in \hat E$ gradually, over the course of $r-1$ iterations. 
Initially, we set $\tilde \rset(e)=\emptyset$ for every edge $e\in \hat E$.
For all $1\leq t <r$, over the course of iteration $t$, we will define the segment $\tilde R_t(e)\in \rset_t$ for every edge $e\in \hat E$ with $t\in \spann''(e)$; the segment  $\tilde R_t(e)$ is then added to set $\tilde \rset(e)$.



We now fix an index $1\leq t<r$, and describe the execution of the $t$th iteration. We construct a multiset $A\subseteq \delta_G(u_t)$ of edges, as follows. Consider any edge $e\in \hat E$, with $t\in \spann''(e)$. If $t$ is the first index in $\spann''(e)$, then we let $e'$ be the first edge on path $P^{\out}(e)$, which must be incident to $u_t$. Otherwise, segment $\tilde R_{t-1}(e)$ is defined and belongs to $\tilde \rset(e)$. We then let $e'$ be the last edge on segment $\tilde R_{t-1}(e)$, which must be incident to $u_t$. We then add edge $e'$ to set $A$. We say that this copy of edge $e'$ in multiset $A$ is owned by the edge $e$. Notice that 
the number of edges in multiset $A$ is equal to the number of edges of $e\in \hat E$ with $t\in \spann'(e)$, which is equal to $N_t$, from \Cref{claim: enough segments}. We also define another multiset $A'$ of edges incident to $u_t$, that contains the first edge on every path in set $\rset_t$. We think of every edge $e'\in A'$ as representing a distinct path $R\in \rset_t$, for which $e'$ serves as the first edge. From the definition, $|A'|=N_t$. For every edge $e'\in \delta_G(u_t)$, we now let $n^-(e')$ be the number of times that $e'$ appears in set $A$, and $n^+(e)$ the number of times that $e'$ appears in $A'$. From the above discussion, $\sum_{e\in \delta_G(u_t)}n^-(e)=\sum_{e\in \delta_G(u_t)}n^+(e)=N_t$.

We use the algorithm from \Cref{obs:rerouting_matching_cong}, with the ordering $\oset_{u_t}\in \Sigma$ of the edges of $\delta_G(u_t)$, in order to compute a multiset $M \subseteq \delta_G(u_t)\times \delta_G(u_t)$ of $N_t$ ordered pairs of the edges of $\delta_G(v)$, such that each edge $e'\in \delta_G(u_t)$ participates in  $n^-_e$ pairs in $M$ as the first edge, and in  $n^+_e$ pairs in $M$ as the second edge. Recall that we are also guaranteed that, for every pair $(e^-_1,e^+_1),(e^-_2,e^+_2)\in M$,  the intersection between path $P_1=(e^-_1,e^+_1)$ and path $P_2=(e^-_2,e^+_2)$ at vertex $u_t$ is non-transversal with respect to $\oset_{u_t}$.

Consider now some edge $e\in \hat E$ with $t\in \spann''(e)$, and let $e'\in A$ be the edge that $e$ owns. Assume that $e'$ is matched with an edge $e''\in A'$ by $M$, and that $e''$ represents a segment $R\in \rset_t$. We then set $\tilde R_t(e)=R$, and we add the segment $R$ to set $\tilde \rset_t$. In this way, every segment of $\rset_t$ is assigned to a different edge $e\in \hat E$ with $t\in \spann''(e)$.

The algorithm terminates once all indices $1\leq t<r$ are processed. Consider now some edge $e\in \hat E$, and assume that $\spann''(e)=\set{i'',i''+1,\ldots,j''-1}$. Set $\tilde \rset(e)$ now contains, for each $i''\leq t<j''_1$, a path $\tilde R_t(e)$, that connects $u_t$ to $u_{t+1}$. We let $P^{\inn}(e)$ be the path obtained by concatenating all paths in $\tilde \rset(e)$. Observe that path $P^{\inn}(e)$ originates at vertex $u_{i''}$, and terminates at vertex $u_{j''}$ -- the two endpoints of path $P^{\out}(e)$. 
We then let $W(e)$ be the cycle obtained from the union of paths $P^{\out}(e)$ and $P^{\inn}(e)$. We say that $W(e)$ is the \emph{auxiliary cycle} of edge $e$.
We denote the set of all auxiliary cycles by $\wset=\set{W(e)\mid e\in \hat E}$.


Consider some edge $e\in \hat E$. We note that, while path $P^{\out}(e)$ must be a simple path, it is possible that path $P^{\inn}(e)$ is not a simple path. Specifically, for an index $1\leq t<r$, let $P'=P^{\inn}(e)\cap (S_t\cup \delta(S_t))$. Then either $P'=\emptyset$, or $P'$ is a contiguous path, that is obtained by concatenating two simple paths from $\qset_t$. In the latter case, it is possible that some vertex of $S_t$ lies on both these paths. Since it is important for us that, whenever $P^{\inn}(e)\cap S_t\neq \emptyset$, path $P^{\inn}(e)$ contains the vertex $u_t$, we do not turn $P^{\inn}(e)$ into a simple path. Notice however that, from the above discussion, every vertex may appear at most twice on $P^{\inn}(e)$. 
We need the following simple observation.

\begin{observation}\label{obs: self-non-transversal}
	Let $e\in \hat E$ be an edge, and let $v$ be any vertex that  appears twice on path $P^{\inn}(v)$. Let $e_1$, $e_2$ be the edges immediately preceding and immediately following the first appearence of $v$ on $W(e)$, respectively, and let  $e'_1$, $e'_2$ are the edges immediately preceding and immediately following the second appearence of $v$ on $W(e)$, respectively. Then the circular ordering of the edges $e_1,e_2,e_1',e_2'$ in $\oset_v\in \Sigma$ is either $(e_1,e_2,e_1',e_2')$, or $(e_1,e_2,e_2',e_1')$ (or the reverse of one of these orderings).
\end{observation}
\begin{proof}
	Let $1\leq t\leq r$ be the index for which $v\in V(S_t)$. Recall that $P^{\inn}(e)\cap S_t$ is a contiguious path, which is a concatenation of two paths in $\qset_t$. Since the paths in $\qset_t$ are non-transversal with respect to $\Sigma$, the observation follows.
\end{proof}

Assume now that we are given two edges $e,e'\in \hat E$, and some vertex $v$ that appears on both $W(e)$ and $W(e')$. We view the cycles $W(e)$ as being directed so that path $P^{\inn}(e)$ and path $P^{\inn}(e')$ visit the vertebrae in the increasing order of their indices. Let $v$ be any vertex that lies on both $W(e)$ and $W(e')$ (note that $v$ may appear up to twice on each of the cycles). We say that the intersection of $W(e)$ and $W(e')$ is non-transversal at $v$ iff the following hold: for every appearence of $v$ on $W(e)$, and for every appearence of $v$ on $W(e')$, if we denote by $e_1$ and $e_2$ the edges immediately preceding and immediately following this appearence of $v$ on $W(e)$, and by $e'_1$ and $e'_2$ the edges immediately preceding and immediately following this appearence of $v$ on $W(e')$, then the circular ordering of the edges $e_1,e_2,e_1',e_2'$ in $\oset_v\in \Sigma$ is either $(e_1,e_2,e_1',e_2')$, or $(e_1,e_2,e_2',e_1')$ (or the reverse of these orderings).



Recall that we denoted, for each index $1\leq t<r$, by $\hat E_t\subseteq \hat E$ the set of all edges $e\in \hat E$, with $t\in \spann(e)$.
We need the following observation.




\begin{observation}
	\label{obs: auxiliary cycles non-transversal at at most one}
	For every index $1\leq t<r$, for every pair $e, e'\in \hat E_t$ of distinct edges, there is at most one vertex $v\in V(W(e'))\cap V(W(e'))$, such that the  intersection of cycles $W(e)$ and $W(e')$ is non-transversal at $v$. If such a vertex $v$ exists, then $v=u_t$ for some index $t$ that is the last index in either $\spann''(e)$ or $\spann''(e')$.
\end{observation}
\begin{proof}
	Fix an index $1\leq t<r$ and a pair $e,e'\in \hat E_t$ of edges. Let $v$ be any vertex that lies on both $W(e)$ and $W(e')$. We consider three cases. The first case is when $v\in V(G)\setminus V'$, that is, there is some index $1\leq t'\leq r$, such that $v\in V(\tilde S_{t'})\setminus V(S_{t'})$. Since the inner vertices of paths $P^{\inn}(e),P^{\inn}(e')$ are contained in $V'$, vertex $v$ must be an inner vertex of both $P^{\out}(e)$ and $P^{\out}(e')$. From \Cref{claim: out-paths non-transversal}, the intersection of $P^{\out}(e)$ and $P^{\out}(e')$ at vertex $v$ is non-transversal. Therefore, the intersection of $W(e)$ and $W(e')$ at $v$ is non-transversal. %  with respect to the ordering $\oset_v\in \Sigma$.
	
	The second case is when there is some index $1\leq t'\leq r$, such that $v\in V(S_{t'})$, but $v\neq u_{t'}$. 
	Note that in this case, $v$ may appear up to twice on $P^{\inn}(e)$, and up to twice on $P^{\inn}(e')$. We fix one appearance of $v$ on $P^{\inn}(e)$ and one appearance of $v$ on $P^{\inn}(e')$. There must be a path $Q\in \qset_{t'}$, such that $Q\subseteq P^{\inn}(e)$, and it contains the selected appearance of $v$ on $P^{\inn}(e)$, and similarly, there must be a path $Q'\in \qset_{t'}$, with $Q'\subseteq P^{\inn}(e')$, such that $Q'$ contains the selected appearance of $v$ on $P^{\inn}(e')$. Recall that all paths in $\qset_{t'}$ are non-transversal with respect to $\Sigma$. Therefore, the intersection of cycles  $W(e)$ and $W(e')$ is non-transversal at $v$. % with respect to the ordering $\oset_v\in \Sigma$.
	
	The third case is when there is some index $t'$, such that $v=u_{t'}$. If $t'\in \spann''(e)\cap \spann''(e')$ holds, then, from the way the segments of $\rset_{t'}$ were assigned to edges of $\hat E$, it is immediate that 
	 the intersection of cycles  $W(e)$ and $W(e')$ is non-transversal at $u_{t'}$.
	 
	 Lastly, assume that $t'\not\in \spann''(e)$ or $t'\not\in \spann''(e)$. This may only happen if $u_{t'}$ is the last vertex on $P^{\out}(e)$ or $P^{\out}(e')$. If $u_{t'}$ is the last vertex on both these paths, then this is the unique vertex at which the intersection of the cycles $W(e)$ and $W(e')$ may be transversal.
	 Assume now that $u_{t'}$ is the last vertex on one of these two paths (say $P^{\out}(e)$), but it is not the last vertex on $P^{\out}(e')$. Assume that the last vertex on $P^{\out}(e')$ is $u_{t''}$. Since vertex $u_{t'}$ lies on path $P^{\inn}(e')$, $t''>t'$ must hold, and so $u_{t''}$ may not lie on path $P^{\inn}(e)$. Therefore, $u_{t'}$ is the unique vertex at which the intersection of the cycles $W(e)$ and $W(e')$ may be transversal.
	\iffalse

	Assume that $e_1$ is an edge of $\hat E_{i_1,j_1}$ and $e_2$ is an edge of $\hat E_{i_2,j_2}$, such that $j_1\ge j_2$, so $u_{j_2}$ is a common vertex of auxiliary cycles $W(e_1)$ and $W(e_2)$.
	We will show that, the intersection between $W(e_1)$ and $W(e_2)$ is non-transversal at all their shared vertices except (possibly) for $u_{j_2}$, thus completing the proof of \Cref{obs: auxiliary cycles non-transversal at at most one}.
	
	Recall that $W(e_1)=P^{\out}(e_1)\cup P^{\inn}(e_1)$ and $W(e_2)=P^{\out}(e_2)\cup P^{\inn}(e_2)$, and furthermore $P^{\out}(e_1)=P^{\out}_{\lef}(e_1)\cup P^{\out}_{\midd}(e_1)\cup P^{\out}_{\rig}(e_1)$ and $P^{\out}(e_2)=P^{\out}_{\lef}(e_2)\cup P^{\out}_{\midd}(e_2)\cup P^{\out}_{\rig}(e_2)$.
	Note that the paths $P^{\out}_{\midd}(e_1),P^{\out}_{\midd}(e_2)$ are internally disjoint from $V'$, while the paths of  $\set{P^{\out}_{\lef}(e_k),P^{\out}_{\rig}(e_k),P^{\inn}(e_k)}_{k\in \set{1,2}}$ only use vertices of $V'$.
	
	First, from Step 2, the paths $P^{\out}_{\midd}(e_1),P^{\out}_{\midd}(e_2)$ are non-transversal with respect to $\Sigma$.
	Second, note that for each $1\le i\le r-1$, the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.
	Since the $i$-th segments of paths in $\pset^{\inn}$ are paths in $\rset^*_{(i)}$, it follows that the paths $P^{\inn}(e_1)$ and $P^{\inn}(e_2)$ are non-transversal at all vertices of $V(G')\setminus\set{u_1,\ldots,u_r}$.
	Third, from the algorithm and \Cref{obs:rerouting_matching_cong}, it is easy to verify that the paths of $\pset^{\inn}$ are also non-transversal at $u_1,\ldots,u_{j_2-1}$.
	Lastly, since for each $1\le i\le r$, the set $\qset_{i}$ of paths are non-transversal with respect to $\Sigma$, and the intersection between paths of set $\rset^*_{(i)}$ and cluster $S_i$ are paths of $\qset_i$, we get that the intersection between cycles $W(e_1)$ and $W(e_2)$ is non-transversal at all vertices of $V(P^{\out}_{\lef}(e_1))\cup V(P^{\out}_{\lef}(e_2))$.
	Altogether, we get that the intersection between $W(e_1)$ and $W(e_2)$ is non-transversal at all their shared vertices except (possibly) for $u_{j_2}$.\fi
\end{proof}

%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
\iffalse
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------

----------------------

We now re-organize the paths in sets $\rset^*_{(1)},\ldots, \rset^*_{(r-1)}$ to obtain the paths in $\pset^{\inn}=\set{P^{\inn}(e)\mid e\in \hat E}$.
%We now construct the set $\pset^*$ of paths.
Note that, if we select, for each $i\le t\le j-1$, a path of $\rset^*_{(t)}$, then, by taking the union of them, we can obtain a path $\hat P$ connecting $u_i$ to $u_j$. 
We call the selected path of $\rset^*_{(t)}$ the \emph{$t$-th segment} of $\hat P$. Therefore, a path connecting $u_i$ to $u_j$ obtained in this way is the union of its $i$-th segment, its $(i+1)$-th segment, $\ldots$ , and its $(j-1)$-th segment.
We now incrementally construct the set $\pset^{\inn}$ of paths.
Intuitively, we will simultaneously construct all paths of $\pset^{\inn}$ in a total of $r-1$ iterations, where in the $i$-th iteration, we will determine the $i$-th segment of all paths in $\pset^{\inn}$.

For each pair $1\le i'<j'\le r$, we denote by $\hat E_{i',j'}$ the set of all edges $e\in \hat E$ such that the path $P^{\out}(e)$ constructed in Step 2 has $u_{i'}$ as its last endpoint and $u_{j'}$ as its first endpoint.


%For each $1\le i<j\le k$, we denote by $p_{i,j}$ the number of paths in $\pset^*$ connecting $u_i$ to $u_j$. 
Throughout, we will maintain a set $\hat{\pset}=\set{\hat P_e\mid e\in \hat E}$ of paths, where each path $\hat P_e$ is indexed by an edge $e$ of $\hat E$. 
For an edge $e\in \hat E_{i',j'}$, the path $\hat P_e$ is supposed to originate at $u_{i'}$ and terminate at $u_{j'}$.
We call $u_{i'}$ the \emph{destined origin} of $\hat P_e$ and call $u_{j'}$ the \emph{destined terminal} of $\hat P_e$.
Initially, $\hat{\pset}$ contains $|\hat E|$ empty paths. 
%and for each $1\le i<j\le r$, there are $p_{i,j}$ paths of $\hat{\pset}$ whose destined origin is $u_i$ and destined terminal is $u_j$.
We will sequentially process vertices $u_1,\ldots,u_{r-1}$, and, for each $1\le i\le r-1$, upon processing vertex $u_i$, determine which path of $\rset^*_{(i)}$ serves as the $i$-th segment of which path of $\hat\pset$.

We now fix an index $1\le i\le r-1$ and describe the iteration of processing vertex $u_i$. The current set $\hat\pset$ of paths can be partitioned into four sets: set $\hat\pset^{o}_i$ contains all paths of $\hat\pset$ whose destined origin is $u_i$; set $\hat\pset^{t}_i$ contains all paths of $\hat\pset$ whose destined terminal is $u_i$; set $\hat\pset^{\thr}_i$ contains all paths of $\hat \pset$ whose destined origin is $u_{i'}$ for some index $i'<i$ and whose destined terminal is $u_{j'}$ for some index $j'>i$; and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ contains all other paths. 
Note that the paths in set $\hat\pset^{t}_i$ and set $\hat\pset\setminus (\hat\pset^{o}_i\cup \hat\pset^{t}_i\cup \hat\pset^{\thr}_i)$ do not contain an $i$-th segment, so in this iteration we will determine the $i$-th segment of paths in the sets $\hat\pset^{o}_i$ and $\hat\pset^{\thr}_i$.
%On one hand, notice that all paths in $\hat\pset^{t}_i$ already connects its destined origin to $u_i$, and we will not modify them anymore, since these paths are already completed.

Note that the paths in $\hat\pset^{o}_i$ currently contain no edges, %and we arbitrarily designate, for each path in $\hat\pset^{o}_i$, a distinct path of $\pset^*_{(i)}$ as its $i$-th segment.
and the paths in $\hat\pset^{\thr}_i$ currently contain up to its $(i-1)$-th segment. 
%and in this iteration we will designate paths of $\pset^*_{(i)}$ as their $i$-th segments, as follows. 
We then denote
\begin{itemize}
	\item by $L^-_i$ the multi-set of the current last edges (the edges incident to $u_i$) of paths in $\hat\pset^{\thr}_i$;
	\item by $L^+_i$ the multi-set of the first edges (the edges incident to $u_i$) of paths in $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of any path in $\hat{\pset}$); and
	\item by $L^{\out}_i$ the multi-set of last edges of paths in $\pset^{\out}_{i,*}=\bigg\{P^{\out}_{\lef}(e) \text{ }\bigg|\text{ } e\in \big(\bigcup_{j>i}\hat E_{i,j}\big)\bigg\}$.
\end{itemize} 
%$L^-_i$ the multi-set of edges of $\delta(u_i)$ that currently serves as the last edge of paths in $\hat\pset^{\thr}_i$, denote by $L^+_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\rset^*_{(i)}$ (note that these paths are currently not designated as the $i$-th segment of to any path in $\hat{\pset}$), and denote by $L^{\out}_i$ the multi-set of edges of $\delta(u_i)$ that is the first edge of some path of $\set{P^{\out}_e \mid e\in E(S'_i,S'_j)\text{ for some }j>i+1}$.
%It is clear that $R^-_i, R^+_i$ are two disjoint subsets of $\delta(u_i)$ with $|R^-_i|=|R^+_i|$. 
Clearly, elements in sets $L^-_i, L^+_i,L^{\out}_i$ are edges of $\delta(u_i)$. 
We then define, for each $e\in \delta(u_i)$, $n^-_e=n_{L^-_i}(e)+n_{L^{\out}_i}(e)$ and
$n^+_e=n_{L^+_i}(e)$.
%\znote{see new notations in prelim (second paragraph in \Cref{sec:prelim})}
We use the following simple observation.
\begin{observation}
	For each edge $e\in \delta(u_i)$, $\sum_{e\in \delta(u_i)}n^-_e=\sum_{e\in \delta(u_i)}n^+_e$.
\end{observation}
\begin{proof}
	On the one hand, $\sum_{e\in \delta(u_i)}n_{L^{\out}_i}(e)=|\bigcup_{j\ge i+2}\hat E_{i,j}|=|\hat\pset^{o}_i|$, and $\sum_{e\in \delta(u_i)}n_{L^{-}_i}(e)=|L^-_i|=|\hat\pset^{\thr}_i|$. 
	On the other hand, recall that $|\rset^*_{(i)}|=|\pset^*_{(i)}|$, and the set $\pset^*_{(i)}$ contains a path connecting $u_i$ to $u_{i+1}$ for each edge $e\in \big(\bigcup_{i'\le i-1,j'\ge i+1}\hat E_{i',j'}\big)\cup \big(\bigcup_{j'\ge i+2}\hat E_{i',j'}\big)$. Therefore,
	$\sum_{e\in \delta(u_i)}n_{L^{+}_i}(e)=|L^+_i|=|\rset^*_{(i)}|=|\pset^*_{(i)}|=|\bigcup_{i'\le i-1,j'\ge i+1}\hat E_{i',j'}|+|\bigcup_{j'\ge i+2}\hat E_{i,j'}|=|\hat\pset^{\thr}_i|+|\hat\pset^{o}_i|$.
\end{proof}

We apply the algorithm in \Cref{obs:rerouting_matching_cong} to graph $G$, vertex $u_i$, rotation $\oset_{u_i}$ and integers $\set{n^-_e,n^+_{e}}_{e\in \delta(u_i)}$.
Let $M$ be the multi-set of ordered pairs of the edges of $\delta(u_i)$ that we obtain. 
%we can efficiently computes a perfect matching $M\subseteq E^-\times E^+$ between the edges of $E^-$ and the edges of $E^+$, such that, for each pair of matched pairs $(e^-_1,e^+_1)$ and $(e^-_2,e^+_2)$ in $M$, the intersection of the path that consists of the edges $e^-_1,e^+_1$ and the path that consists of edges $e^-_2,e^+_2$ at vertex $u$ is non-transversal with respect to $\oset_v$.
We then designate: 
\begin{itemize}
	\item for each path $\hat P_e\in \hat\pset^{\thr}_i$ with $e^-$ as its current last edge, a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$; and
	\item for each path $P^{\out}_{\lef}(e)\in\pset^{\out}_{i,*}$ with $e^-$ as its last edge (recall that we view $u_i$ as the last endpoint of such a path), a path of $\rset^*_{(i)}$ that contains the edge $e^+$ as its first edge with $(e^-,e^+)\in M$, as the $i$-th segment of $\hat P_e$;
\end{itemize}
such that each path of $\rset^*_{(i)}$ is assigned to exactly one path of $\hat \pset^{\thr}_i\cup \pset^{\out}_{i,*}$.
This completes the description of the $i$-th iteration.
See Figure~\ref{fig: inner_path} for an illustration.





\begin{figure}[h]
	\centering
	\subfigure[Edges in $\delta(u_i)$: only the last/first edges of paths are shown. Here $\pset^{\out}_{*,i}=\set{P^{\out}(e) \mid e\in\big( \bigcup_{i'< i}\hat E_{i',i}\big)}$.]{\scalebox{0.32}{\includegraphics{figs/inner_path_1.jpg}}}
	\hspace{1pt}
	\subfigure[Sets $L^-_i, L^+_i,L^{\out}_i$ and the pairing (shown in dash pink lines) given by the algorithm in \Cref{obs:rerouting_matching_cong}.]{
		\scalebox{0.32}{\includegraphics{figs/inner_path_2.jpg}}}
	\caption{An illustration of an iteration in Step 4 of constructing paths of $\set{P^{\inn}(e)\mid e\in \hat E}$.}\label{fig: inner_path}
\end{figure}







Let $\pset^{\inn}$ be the set of paths that we obtain after processing all vertices $u_1,\ldots,u_{r-1}$. Then for every $e\in \hat E$, we rename the path $\hat P_e$ at the end of the algorithm by $P^{\inn}(e)$.
From the algorithm, it is easy to see that, for each pair $1\le i<j\le r$ and each edge $e\in \hat E_{i,j}$, the inner path $P^{\inn}(e)$ starts at $u_i$ and ends at $u_j$ as it is supposed to, and path $P^{\inn}(e)$ contains, for each $i\le t\le j-1$, a path of $\rset^*_{(t)}$ as its $t$-th segment.
Therefore, path $P^{\inn}(e)$ visits vertices $u_i,u_{i+1},\ldots,u_j$ sequentially.
%, and it can also be naturally partitioned into segments $P^{\inn}_{i'}(e)$, $\hat P^{\inn}_{i'}(e)$, $P^{\inn}_{i'+1}(e)$, $\hat P^{\inn}_{i'+1}(e),\ldots,\hat P^{\inn}_{j'-1}(e),P^{\inn}_{j'}(e)$, such that for each $i'\le t\le j'$, segment $P^{\inn}_{t}(e)$ is entirely contained in cluster $S'_{t}$ and $u_t\in P^{\inn}_{t}(e)$, and segment $\hat P^{\inn}_{t}(e)$ is contained in $S_t$ but is internally disjoint from $S'_{t}$. 
%and for each pair $1\le i,j\le r$ with $j>i+1$, $\pset$ contains $p_{i,j}$ paths originating $u_i$ and terminating at $u_j$. 

%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
\fi

%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------
%-------------------------

\iffalse
\begin{observation}
	\label{obs: non_transversal_1}
	For each $1\le i\le r-1$, if we denote, for each $e\in E_i^{\rig}$, by $R_e$ the path consisting of the last edge of path $P^{\out}_e$ and the first edge of path $P_e$, then the paths in $\set{P_e\mid e\in \bigcup_{ i'<i<j'}E(S'_{i'},S'_{j'})}$ and $\set{R_e\mid e\in E_i^{\rig}}$ are non-transversal at $u_i$.
\end{observation}
\fi

%It is also easy to see that the paths in $\pset$ are non-transversal with respect to $\Sigma$, which we show in the following observation.
\iffalse
\begin{observation}
	\label{obs: non_transversal_2}
	The inner paths in $\pset$ are non-transversal with respect to $\Sigma$.
\end{observation}
\begin{proof}
	On one hand, note that for each $1\le i\le r-1$, the set $\rset^*_{(i)}$ of paths are non-transversal with respect to $\Sigma$.
	Since the $i$-th segments of paths in $\pset$ are paths in $\rset^*_{(i)}$, it follows that the paths of $\pset$ are non-transversal at all vertices of $V(G)\setminus\set{u_1,\ldots,u_k}$.
	On the other hand, from the algorithm and \Cref{obs:rerouting_matching_cong}, it is easy to verify that the paths of $\pset$ are also non-transversal at $u_1,\ldots,u_k$.
\end{proof}
\fi


Lastly, we bound the congestion that is caused by the auxiliary cycles, in the following observation.

\begin{observation}
\label{obs: edge_occupation in outer and inner paths}
Consider any edge $e\in E(G)$. If $e\not \in \bigcup_{1\leq t\leq r}E(S_t)$, then $e$ belongs to at most $O(\log^{18}m)$ cycles of $\wset$. Otherwise, if $e\in E(S_t)$ for some $1\leq t\leq r$, then the number of cycles of $\wset$ that $e$ belongs to is at most $\cong_G(\qset_t,e)\cdot O(\log^{18}m)$.
\end{observation}
\begin{proof}
Consider first an edge $e\in E(G)\setminus\left(\bigcup_{1\leq t\leq r}E(S_t)\right )$. If both endpoints of $e$ lie in set $V'$, then there is an index $1\leq t<r$, such that $e$ connects a vertex of $S_t$ to a vertex of $S_{t+1}$. In this case, the number of cycles in $\wset$ containing edge $e$ is precisely the number of paths in $\rset_t$ containing $e$, which is in turn bounded by $\cong_G(\pset^2,e)\leq O(\log^{18}m)$ from the definition of nice guiding paths.

 If at least one endpoint of $e$ does not lie in $V'$, then the number of cycles 	in $\wset$ that contain $e$ is $\cong_G(\pset^{\out}\leq O(\log^{18}m)$, from \Cref{claim: computing out-paths}.
 
 Assume now that there is some index $1\leq t\leq r$, such that $e\in E(S_t)$. Let $A$ be the set of all edges $e'\in \delta_G(S_t)$, such that the path $Q_t(e')\in \qset_t$ contains the edge $e$. Clearly, $|A|=\cong_G(\qset_t,e)$. Notice that a cycle $W\in \wset$ may only contain the edge $e$ if it contains one of the edges in set $A$. Since, from the above discussion, every edge of $A$ may lie on at most $O(\log^{18}m)$ cycles of $\wset$, the total number of cycles in $\wset$ that contain $e$ is bounded by $|A|\cdot O(\log^{18}m)\leq \cong_G(\qset_t,e)\cdot O(\log^{18}m)$.
\end{proof}


==> overview-backup.tex <==
\section{An Algorithm for \cnwrs -- Proof of \Cref{thm: main_rotation_system}}
\label{sec: high level}



%\mynote{Throughout the paper, a solution to instance $I$ is referred to as $\phi(I)$ or $\phi_I$ interchangeably. I suggest that we stick to the former. Could you please fix this in the current section? Thanks!}

In this section we provide a proof of Theorem \ref{thm: main_rotation_system}, with some of the details deferred to subsequent sections.
%
Throughout the paper, we denote by $I^*=(G^*,\Sigma^*)$  the input instance of the \CNwRS problem, and we denote $m^*=|E(G^*)|$. We also use the following parameter that is central to our algorithm: ${\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}}$, %\mynote{may need to adjust}, 
where $c^*$ is a large enough constant. 

As mentioned already, our algorithm for solving the \CNwRS problem is recursive, and, over the course of the recursion, we will consider subinstances of instance $I^*$ (see \Cref{subsec: subinstances} for a definition). %Each such subinstance is determined by a sub-graph $G'\subseteq G^*$, and disjoint collections $S_1,\ldots,S_q$ of vertices of $G'$. Graph $G$ is obtained from $G'$ by unifying, for all $1\leq i\leq q$, all vertices of $S_i$ into a vertex $u_i$, that we call a \emph{supernode}. We keep parallel edges but remove self-loops. For every vertex $v\in V(G)$ that is also a vertex of $G^*$, its rotation system $\oset_v$ in $\Sigma$ remains the same as in $\Sigma^*$, while for every supernode $u_i$, we will define its rotation system $\oset_{u_i}$ explicitly. Notice that subinstance relation is transitive: if $(G_1,\Sigma_1)$ is a subinstance of $(G_0,\Sigma_0)$, and $(G_2,\Sigma_2)$ is a subinstance of $(G_1,\Sigma_1)$, then $(G_2,\Sigma_2)$ is a subinstance of $(G_0,\Sigma_0)$.
The algorithm proceeds by recursively decomposing a given subinstance $I$ of $I^*$  into a collection of smaller subinstances. 
The main technical ingredient of the proof is the following theorem.

\begin{theorem}
	\label{thm: main}
	There is a constant $c'$, and an efficient randomized algorithm, that, given a subinstance $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, either returns FAIL, or produces a non-empty collection $\iset$ of subinstances of $I$ with the following properties:
	
\begin{itemize}
\item for each subinstance $I'=(G',\Sigma')\in \iset$, $|E(G')|\leq m/\mu$;

\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq  m\cdot (\log m)^{O(1)}$;

\item if $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: 

$\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}$; and

\item there is an efficient algorithm \algcombine, that, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, of cost at most $O(\sum_{I'\in \iset}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{O(1)}$.
\end{itemize}

Moreover, if $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/16$.
\end{theorem}




\iffalse
We now define collections of subinstances that have some desirable properties. The following definition is  similar in spirit to the definition of a $\nu$-decomposition of an instance, but, since it uses slightly different parameters, we distinguish between these two definitions.

\begin{definition}[Good and Perfect Collection of Subinstances]
	Let $I=(G,\Sigma)$ be a subinstance of instance $I^*$, with $|E(G)|=m$, and let $\iset$ be a collection of subinstances of $I$. We say that $\iset$ is a \emph{good collection of subinstances} for $I$ if the following hold.
	
	\begin{itemize}
		\item for each subinstance $I'=(G',\Sigma')\in \iset$, $|E(G')|\leq m/\mu$;
		\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq  m\cdot (\log m)^{c_g}$, where $1000<c_g<c^*$ is some large enough universal constant whose value will be set later; and
		
		\item there is an efficient algorithm, that we call \algcombine, that, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, of cost at most $c_g\cdot(\sum_{I'\in \iset}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{c_g}$.
	\end{itemize}

 We say that $\iset$ is a \emph{perfect} collection of subinstances for $I$ if, additionally:
	$$\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{c_g}.$$
\end{definition}

The main technical ingredient of the proof is the following theorem.

\begin{theorem}
	\label{thm: main}
	There is an efficient randomized algorithm, whose input is a subinstance $I=(G,\Sigma)$ of $I^*$, with $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$ and $|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$. The algorithm outputs a good collection $\iset$ of subinstances of $I$, and, with probability at least $7/8$, $\iset$ is a perfect collection of subinstances for $I$.
\end{theorem}
%\znote{(1) to set $\mu$; (2) theorem may need to be changed due to bad/deleted edges.}
\fi

The remainder of this paper is dedicated to the proof of \Cref{thm: main}. In the following subsection, we complete the proof of \Cref{thm: main_rotation_system} using \Cref{thm: main}.



%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
\subsection{Proof of \Cref{thm: main_rotation_system}}

%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
Throughout the proof, we assume that $m^*$ is larger than a sufficiently large constant, since otherwise we can return a trivial solution to instance $I^*$, from \Cref{thm: crwrs_uncrossing}.

We let $100<c_g<c^*/2$ be a large enough constant, so that, if the algorithm from \Cref{thm: main}, when applied to a subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, returns a family $\iset$ of subinstances of $I$, with $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq  m\cdot (\log m)^{c_g}$. Additionally, if  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot 2^{c_g((\log m)^{3/4}\log\log m)} +m\cdot\mu^{c_g}$. We also assume that Algorithm \algcombine, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, of cost at most $c_g\cdot (\sum_{I'\in \iset}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{c_g}$.


We use a simple recursive algorithm called \algrec, that appears in Figure \ref{fig: algrec}.


\program{\algrec}{fig: algrec}{ 
\noindent{\bf Input:} a subinstance $I=(G,\Sigma)$ of the input instance $I^*$ of the \CNwRS problem.

\noindent{\bf Output:} a feasible solution to instance $I$.

\begin{enumerate}
	\item Use the algorithm from \Cref{thm: crwrs_planar} to determine whether or not $\optcrors(I)=0$. If so, use the algorithm from \Cref{thm: crwrs_planar} to compute a solution to $I$ of cost $0$. Return this solution, and terminate the algorithm.
	
	\item Use the algorithm from Theorem~\ref{thm: crwrs_uncrossing} to compute a trivial solution $\phi'$ to instance $I$.
	
	\item If $|E(G)|\leq \mu^{c'}$, return the trivial solution $\phi'$ and terminate the algorithm.
	
	\item For $1\leq j\leq \ceil{\log m^*}$:
	\begin{enumerate}
		\item Apply the algorithm from \Cref{thm: main} to instance $I$. 

			\item If the algorithm returns FAIL, let $\phi_j=\phi'$ be the trivial solution to instance $I$, and set $\iset_j(I)=\emptyset$.
			
			\item Otherwise: 
			\begin{enumerate}	
			\item Let $\iset_j(I)$ be the collection of subinstances of $I$ that the algorithm returns.

		  \item For every subinstance $I'\in \iset_j(I)$, apply Algorithm \algrec to instance $I'$, to obtain a solution $\phi(I')$ to this instance.
		
	   	\item Apply Algorithm \algcombine from \Cref{thm: main} to solutions $\set{\phi(I')}_{I'\in \iset_j(I)}$, to obtain a solution $\phi_j$ to instance $I$.
	   	\end{enumerate}
	\end{enumerate}
\item %Let $\phi'$ be a trivial solution to instance $I$, of cost at most $|E(G)|^2$. 
Return the best solution of $\set{\phi',\phi_1,\ldots,\phi_{\ceil{\log m^*}}}$
\end{enumerate}
}



In order to analyze the algorithm, it is convenient to associate a \emph{partitioning tree} $T$ with it, whose vertices correspond to all subinstances considered over the course of the algorithm. Let $L=\ceil{\log m^*}$. We start with the tree $T$ containing a single root vertex $v(I^*)$, representing the input instance $I^*$. Consider now some vertex $v(I)$ of the tree, representing some subinstance $I=(G,\Sigma)$ of $I^*$.
When Algorithm \algrec was applied to instance $I$, if it did not terminate after the first three steps, it created $L$ collections $\iset_1(I),\ldots,\iset_L(I)$ of subinstances of $I$ (some of which may be empty, in case the algorithm from \Cref{thm: main} returned FAIL). For each such subinstance $I'\in \bigcup_{j=1}^L\iset_j(I)$, we add a vertex $v(I')$ representing instance $I'$, that becomes a child vertex of $v(I)$. This concludes the description of the partitioning tree $T$. 


We denote by $\iset^*=\set{I\mid v(I)\in V(T)}$ the set of all subinstances of instance $I^*$ whose corresponding vertex appears in the tree $T$. For each such instance $I\in \iset^*$, its  \emph{recursive level} is the distance from vertex $v(I)$ to the root vertex $v(I^*)$ in the tree $T$ (so the recursive level of $v(I^*)$ is $0$).
For $j\geq 0$, we denote by $\hat \iset_j\subseteq \iset^*$ the set of all instances $I\in \iset^*$, whose recursive level is $j$.
Lastly, the \emph{depth} of the tree $T$, denoted by $\dep(T)$, is the largest recursive level of any instance in $\iset^*$.
 In order to analyze the algorithm, we start with the following two simple observations.

\begin{observation}\label{obs: few recursive levels}
 $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.
\end{observation}
\begin{proof}
	Consider any non-root vertex $v(I)$ in the tree $T$, and let $v(I')$ be the parent-vertex of $v(I)$. Denote $I=(G,\Sigma)$ and $I'=(G',\Sigma')$.
	From the construction of tree $T$, instance $I$ belongs to some collection of subinstances obtained by applying the algorithm from \Cref{thm: main} to instance $I'$. Therefore, from \Cref{thm: main}, $|E(G)|\leq |E(G')|/\mu$ must hold. Therefore, for all $j\geq 0$, for every instance $I=(G,\Sigma)\in \hat \iset_j$, $|E(G)|\leq m^*/\mu^j$. Since $\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$, we get that $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.
\end{proof}

%a We denote by $\dep(T)$ the depth of tree $T$, i.e., the largest recursive level for any instance $I$ with vertex $v(I)\in V(T)$, so $\dep(T)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.


\begin{observation}\label{obs: num of edges}
$\sum_{I=(G,\Sigma)\in \iset^*}|E(G)|\le m^*\cdot 2^{(\log m^*)^{1/8}}$.
\end{observation}
\begin{proof}
	Consider any non-leaf vertex $v(I)$ of the tree $T$, and denote $I=(G,\Sigma)$. 
Recall that, when Algorithm \algrec is applied to  instance $I$, it applies the algorithm from \Cref{thm: main} to $I$ and compute $L$ collections $\iset_1(I),\ldots,\iset_L(I)$ of subinstances, such that, if we denote $|E(G)|=m$, then, for all $1\leq j\leq L$:
%
 $$\sum_{I'=(G',\Sigma')\in \iset_j(I)}|E(G')|\leq m\cdot (\log m)^{c_g}\leq m\cdot (\log m^*)^{c_g}$$
 %
 (we have used the fact that, if $I$ is a subinstance of $I^*$, then $m\leq m^*$ must hold). Since $L\leq 2\log m^*$, and $m^*$ is sufficiently large, we get that:
 %
 $$\sum_{j=1}^L\sum_{I'=(G',\Sigma')\in \iset_j(I)}|E(G')|\leq m\cdot (\log m^*)^{c_g+2}.$$
 %
 For all $j\geq 0$, we denote by $N_j$ the total number of edges in all instances in set $\hat \iset_j$, $N_j=\sum_{I=(G,\Sigma)\in \hat \iset_j}|E(G)|$. Clearly, $N_0=m^*$, and, from the above discussion, for all $j>0$, $N_j\leq N_{j-1}\cdot (\log m^*)^{c_g+2}$. 
 
 Since $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$,
we conclude that:
%
\[
%\begin{split}
\sum_{I=(G,\Sigma)\in \iset^*}|E(G)|\leq m^*\cdot (\log m^*)^{2c_g\cdot  (\log m^*)^{1/8}/(c^*\log\log m^*)}\leq m^*\cdot 2^{(\log m^*)^{1/8}}, 
%\end{split}
\]	
%
since $c_g\leq c^*/2$.
\end{proof}

We use the following corollary, that follows  immediately from \Cref{obs: num of edges}.

\begin{corollary}\label{cor: num of instances}
The number of instances $I=(G,\Sigma)\in \iset^*$ with $|E(G)|\geq \mu^{c'}$ is at most $m^*$.
\end{corollary}

\iffalse{original corollary does not depend on the notion of leaf instance}
For an instance $I\in \iset^*$, we say that it is a \emph{leaf instance}, if  vertex $v(I)$ is a leaf vertex of the tree $T$, and we say that it is a non-leaf instance otherwise. We use the following corollary, that follows  immediately from \Cref{obs: num of edges}, and the fact (from the description of Algorithm \algrec) that, if $I=(G,\Sigma)\in \iset^*$ is a non-leaf instance, then  $|E(G)|\geq \mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$ must hold.


\begin{corollary}\label{cor: num of instances}
The number of instances $I=(G,\Sigma)\in \iset^*$ with $|E(G)|\geq \mu^{c'}$ is at most $m^*$.
\end{corollary}
\fi

 	
For an instance $I\in \iset^*$, we say that it is a \emph{leaf instance}, if  vertex $v(I)$ is a leaf vertex of the tree $T$, and we say that it is a non-leaf instance otherwise.
%From the description of Algorithm \algrec, if $I=(G,\Sigma)\in \iset^*$ is a non-leaf instance, then  $|E(G)|\geq \mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$ must hold.
Consider now a non-leaf instance $I\in \iset^*$. We say that a bad event $\event(I)$ happens, if all the following conditions hold:

\begin{itemize}
	\item $0<\optcrors(I)\leq |E(G)|^2/\mu^{c'}$;
	\item $|E(G)|\geq \mu^{c'}$; and
	\item for all $1\leq j\leq L$, we have set $\phi_j=\phi'$ and $\iset_j(I)=\emptyset$, since 
	the algorithm from \Cref{thm: main} returned FAIL in each of the $L$ iterations when it was applied to $I$.
\end{itemize} 

Clearly, from \Cref{thm: main},  $\prob{\event(I)}\le (1/16)^L\leq 1/(m^*)^4$.


We say that a bad event $\event'(I)$ happens if the following conditions hold:

\begin{itemize}
\item $0<\optcrors(I)\leq |E(G)|^2/\mu^{c'}$;
\item $|E(G)|\geq \mu^{c'}$; and
\item for all $1\leq j\leq L$, $\sum_{I'\in \iset_j(I)}\optcrors(I')> \optcrors(I)\cdot2^{c_g\cdot (\log m)^{3/4}\log\log m} +m\cdot\mu^{c_g}$.
\end{itemize}

As before, from \Cref{thm: main},  $\prob{\event'(I)}\le (1/16)^L\leq 1/(m^*)^4$.


Let $\event$ be the bad event that event $\event(I)$  or event $\event'(I)$ happened for any  instance $I\in \iset^*$. From the Union Bound and \Cref{cor: num of instances}, we get that $\prob{\event}\leq 1/(m^*)^2$.




We use the following immediate observation.

\begin{observation}\label{obs: leaf}
If Event $\event$ does not happen, then for every leaf vertex $v(I)$ of $T$ with $I=(G,\Sigma)$, either $|E(G)|\leq \mu^{c'}$; or $\optcrors(I)=0$; or $\optcrors(I)> |E(G)|^2/\mu^{c'}$.
\end{observation}


We use the following lemma to complete the proof of \Cref{thm: main_rotation_system}.

\begin{lemma}\label{lem: solution cost}
	If Event $\event$ does not happen, then  Algorithm $\algrec$ computes a solution for instance $I^*=(G^*,\Sigma^*)$ of cost at most $2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)$.
\end{lemma}
\begin{proof}
%First we show that, if $I=(G,\Sigma)$ is a leaf subinstance of $I^*$, then the algorithm computes a solution to instance $I$ of cost at most $\mu^{2c'}\cdot \optcrors(I)$. Indeed, if $\optcrors(I)=0$, then the algorithm returns a solution of cost $0$. Otherwise, $\optcrors(I)\geq 1$, and, if $|E(G)|\leq \mu^{c'}$, then the algorithm returns a trivial solution, whose cost is at most $|E(G)|^2\leq \mu^{2c'}\cdot \optcrors(I)$. Lastly, if $\optcrors(I)>|E(G)|^2/\mu^{c'}$, then, since the trivial solution $\phi'$ is considered by the algorithm, it returns a solution of cost at most $|E(G)|^2\leq \optcrors(I)\cdot \mu^{c'}$.
		Consider a non-leaf instance $I=(G,\Sigma)$, and let $\iset_1(I),\ldots,\iset_L(I)$ be families of subinstances of $I$ that the Algorithm \algrec computes. Recall that, for each $1\le j\le L$ with $\iset_j(I)\neq \emptyset$, the algorithm computes a solution $\phi_j$ to instance $I$, by first solving each of the instances in $\iset_j(I)$ recursively, and then combining the resulting solutions using Algorithm \algcombine. Eventually, the algorithm returns the best solution of $\set{\phi',\phi_1,\ldots,\phi_L}$, where $\phi'$ is the trivial solution, whose cost is at most  $|E(G)|^2$. We fix an index $1\leq j\leq L$, for which solution $\phi_j$ has the lowest cost, breaking ties arbitrarily. Note that the cost of the solution to instance $I$ that the algorithm returns is at most $\cro(\phi_j)$. We then \emph{mark} the vertices of $\set{v(I')\mid I'\in \iset_j(I)}$ in the tree $T$. We also mark the root vertex of the tree. 

Let $T^*$ be the subgraph of $T$ induced by all marked vertices. It is easy to verify that $T^*$ is a tree, and moreover, every leaf vertex of $T^*$ is also a leaf vertex of $T$. For a vertex $v(I)\in V(T^*)$, we denote by $h(I)$ the length of the longest path in tree $T^*$, connecting vertex $v(I)$ to any of its descendants in the tree. 
We use the following claim, whose proof is straightforward conceptually but somewhat technical; we defer the proof to \Cref{Appx: inductive bound proof}.

\begin{claim}\label{claim: bound by level}
Assume that Event $\event$ did not happen. Then there is a fixed constant $\tilde c>0$, such that, for every vertex $v(I)\in V(T^*)$, whose corresponding subinstance of $I^*$ is denoted by $I=(G,\Sigma)$, the cost of the solution that the algorithm computes for  $I$ is at most:
 $$2^{\tilde c\cdot h(I)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+(\log m^*)^{4c_g h(I)}\mu^{2c'\cdot \tilde c}\cdot|E(G)|.$$
\end{claim}


We are now ready to complete the proof of \Cref{lem: solution cost}. Recall that $h(I^*)=\dep(T^*)\leq \dep(T)\leq  \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$  from \Cref{obs: few recursive levels}. Therefore, from \Cref{claim: bound by level}, the cost of the solution that the algorithm computes for instance $I^*$ is bounded by:
%
\[
\begin{split}
& \text{ } 2^{O(\dep(T))\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{O(1)}\cdot \optcrors(I^*)+(\log m^*)^{O(\dep(T))}\cdot\mu^{O(1)}\cdot m^*\\
\leq & \text{ } 2^{O((\log m^*)^{7/8})}\cdot \mu^{O(1)}\cdot \optcrors(I^*)+(\log m^*)^{O((\log m^*)^{1/8}/\log\log m^*) }\cdot\mu^{O(1)}\cdot m^*\\
\leq & \text{ } 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right),
\end{split}
\]
%
since $\mu=2^{O((\log m^*)^{7/8}\log\log m^*)}$.
\end{proof}



In order to complete the proof of \Cref{thm: main_rotation_system}, it is now enough to prove Theorem~\ref{thm: main}. The remainder of the paper is dedicated to the proof of \Cref{thm: main}.




\subsection{Proof of Theorem~\ref{thm: main} -- Main Definitions and Theorems} 

%\znote{constant $\interestconst$ to be replaced by an integer}\mynote{in the uninteresting instances part we have made some assumption about $b$ (possibly $b\geq 50$ but I'm not sure). When setting the value of $b$ please check and make sure that it is consistent.}
	
%\mynote{please switch "interesting/uninteresting" to "wide/narrow" throughout the whole paper (including intro)}
We classify subinstances of the input instance $I^*$ into \emph{wide} and \emph{narrow}, and provide different algorithms for decomposing instances of each of the two kinds. %We now define wide and narrow subinstances of $I^*$.
%\mynote{note that this definition has changed to only include one of the two cases. The subsequent observation shows that the other case also holds. I also eliminated "witness path set" because we use this notion in many other places and it is not really necessary here.}
Throughout this subsection, we use the parameter $\interestconst=50$.

%\mynote{Please go to Sec 9 where it uses this other property of uninteresting instances and add a pointer to the observation from there (e.g. the property now follows from the observation, not from the definition of the instances).}




\begin{definition}[Wide and Narrow Instances]
Let $I=(G,\Sigma)$ be an instance of \cnwrs with $|E(G)|=m$. We say that $I$ is a \emph{wide} instance, iff there is a vertex $v\in V(G)$, a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$, and a collection $\pset$  of at least $\floor{m/\mu^{\interestconst}}$ simple edge-disjoint cycles in $G$, such that every cycle $P\in \pset$ contains one edge of $E_1$ and one edge of $E_2$.
	If no such cycle set $\pset$ exists in $G$, then we say that $I$ is a \emph{narrow} instance.
\end{definition}




Note that there is an efficient algorithm to check whether a given instance $I$ of \cnwrs is wide, and, if so, to  compute the corresponding cycle set $\pset$, via standard algorithms for maximum flow. (For every vertex $v\in V(G)$, we can try all possible partitions $(E_1,E_2)$ of $\delta_G(v)$ with the required properties, as the number of such partitions is bounded by $|\delta_G(v)|^2$.)
We will use the following simple observation regarding narrow instances.

\begin{observation}\label{obs: narrow prop 2}
	If an instance $I=(G,\Sigma)$ of \cnwrs is narrow, then for every pair $u,v$ of distinct vertices of $G$, and any set $\pset$ of edge-disjoint paths connecting $u$ to $v$  in $G$,  $|\pset|\leq 2\ceil{m/\mu^{\interestconst}}+2$ must hold.
\end{observation}

\begin{proof}
	Assume for contradiction that $|\pset|>2\ceil{m/\mu^{\interestconst}}+2$, and denote $|\pset|=k$.
	Let $E'\subseteq \delta_G(v)$ be the set of all edges $e\in \delta_G(v)$, such that $e$ is the first edge on some path in $\pset$. We denote $E'=\set{e_1,\ldots,e_k}$, where the edges are indexed according to their ordering in the rotation $\oset_v\in \Sigma$. We also denote $\pset=\set{P(e_i)\mid 1\leq i\leq k}$, where path $P(e_i)$ contains the edge $e_i$ as its first edge. We can then compute a partition $(E_1,E_2)$ of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$. Additionally, we can ensure that $e_1,\ldots,e_{\ceil{k/2}}\in E_1$, while the remaining edges of $E'$ lie in $E_2$. For each $1\leq i\leq \ceil{m/\mu^{\interestconst}}$, we let $Q_i$ be the cycle obtained by concatenating the paths $P(e_i)$ and $P(e_{k-i+1})$. We can turn $Q_i$ into a simple cycle, by removing all cycles that are disjoint from vertex $v$ from it. It is then immediate to verify that cycle set $\set{Q_i\mid 1\leq i\leq \ceil{m/\mu^{\interestconst}}}$ has all the required properties to establish that instance $I$ is wide, a contradiction.
\end{proof}


\iffalse

\begin{definition}[Wide and Narrow Subinstances]
A subinstance $I=(G,\Sigma)$ of $I^*$ is an \emph{interesting} instance, iff there is a 
	collection $\pset$ of at least $m/\mu^{\interestconst}$ edge-disjoint paths in $G$, that we refer to as the \emph{witness path set for $I$}, such that one of the following holds:
	
	\begin{itemize} 
		\item either there are two distinct vertices $u,v\in V(G)$, such that every path in $\pset$ originates at $v$ and terminates at $u$; or 
		
		
		\item there is a single vertex $v\in V(G)$, and a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$. Every path in $\pset$ must contain an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
	\end{itemize}
	%
	If no such path set $\pset$ exists in $G$, then we say that $I$ is an \emph{narrow} instance.
\end{definition}
\fi


The proof of \Cref{thm: main} relies on the following two theorems. The first theorem deals with wide subinstances of $I^*$, and its proof appears in \Cref{sec: many paths}.




\mynote{The theorem has changed. The old version appears below this new version for comparison. This section will need to be updated to work with the new theorem (but wait until I finish Sec 5 in case there are other changes).}

\begin{theorem}\label{lem: many paths}
	There is an efficient randomized algorithm, that, given a wide subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$, either returns FAIL, or computes a non-empty collection $\iset$ of subinstances of $I$, such that $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$, and, for every instance $I'=(G',\Sigma')\in \iset$, either $|E(G')|\le m/\mu$, or instance $I'$ is not wide. Additionally, if $\optcrors(I)\leq m^2/\mu^{c'}$ then, with probability at least $1-1/\mu^2$, all of the following hold:
	
	\begin{itemize}
		\item  the algorithm does not return FAIL; 
		\item $\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot  (\log m)^{O(1)}$; and
		\item there is an efficient algorithm, that, given a solution $\phi(I')$ for every instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq  \sum_{I'\in \iset}\cro(\phi(I')) + \optcrors(I)\cdot\mu^{O(1)}$.
	\end{itemize}
\end{theorem}


\mynote{old version of same theorem}
%\mynote{I had to change the theorem statement to allow the algorithm to return FAIL if $\optcrors(I)$ is too big. The remainder of the proof in this section needs to be adjusted to allow this.}
\begin{theorem}\label{lem: many paths}
	There is an efficient randomized algorithm, that, given a wide subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$, either returns FAIL, or computes a non-empty collection $\iset$ of subinstances of $I$, such that:
	
	\begin{itemize}
		\item for each instance $I'=(G',\Sigma')\in \iset$, if $I'$ is a wide instance, then $|E(G')|\le m/\mu$; 
		\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$; and
		\item
		 there is an efficient algorithm, that, given a solution $\phi(I')$ for every instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq  \sum_{I'\in \iset}\cro(\phi(I')) + (m+\optcrors(I))\cdot\mu^{O(1)}$.
	\end{itemize}
	
	If $\optcrors(I)\leq m^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/\mu^2$.
	Additionally, if $\optcrors(I)\leq m^2/\mu^{c'}$, then with probability at least $31/32$:
	$$\sum_{I'\in \iset}\optcrors(I')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}.$$
\end{theorem}
	
\iffalse	

\begin{theorem}\label{lem: many paths}
There is a randomized efficient algorithm, that, given a wide subinstance  $I=(G,\Sigma)$ of $I^*$, with $m=|E(G)|>\mu^{100\interestconst}$ and $\optcrors(I)<m^2/\mu^{100\interestconst}$, 
computes a collection $\iset$ of subinstances of $I$, such that:

 
\begin{itemize}
\item for each instance $I'=(G',\Sigma')\in \iset$, if $I'$ is a wide instance, then $|E(G')|\le m/\mu$;
\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$;
and
\item $\expect[]{\sum_{I'\in \iset}\optcrors(I')}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}$. %\mynote{this is not good. To make this work with the rest of this section, the constant inside $\mu^{O(1)}$ must be specified and tied up to $\interestconst$. The reason is: \Cref{thm: main} assumes that $\optcrors(I)\leq m^2/\mu^{63}$ (that assumption will need to be updated with $\interestconst$, but that's for later). If $I$ is wide, we get subinstances from this theorem. Those subinstances that have more than $m/\mu$ edges, we need to apply \Cref{lem: not many paths} to them. But that theorem requires that $\optcrors(I')<|E(G')|^2/\mu^{16}$. We can show that $|E(G')|$ is close enough to $m$. But our only way to bound $\optcrors(I')$ is from the current expression, that will have term $m\cdot \mu^{O(1)}$. We need to show that this is less than $m^2/\mu^{18}$ or so. But we can't do it unless we know what is this $O(1)$, and then we'll need to propagate this back to the statement of  \Cref{thm: main}.}
\end{itemize}



Moreover, there is an efficient algorithm, that, given, a solution $\phi(I')$ for every instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq  \sum_{I'\in \iset}\cro(\phi(I')) + (m+\optcrors(I))\cdot\mu^{O(1)}$. \znote{constants subject to change}
\end{theorem}
\fi

\iffalse{original Theorem 3.6}
\begin{theorem}\label{lem: many paths}
There is a randomized efficient algorithm, that, given an interesting subinstance  $I=(G,\Sigma)$, with $|E(G)|=m>\mu^{39}$ and $\optcrors(I)<m^2/\mu^{40}$, 
 computes two subinstances $I'=(G',\Sigma'),I''=(G'',\Sigma'')$ of $I$, such that $m/\mu^{10}\le |E(G')|,|E(G'')|\leq m\cdot (1-1/\mu^{10})$ and $|E(G')|+|E(G'')|\leq m$, and with probability at least $1-1/(40\mu^{11})$, 
$$\optcrors(I')+\optcrors(I'')\leq \optcrors(I) \cdot(1+1/\mu^{12})+m \cdot \mu^{c},$$
where $c>0$ is some universal integer. 
Moreover, there is an efficient algorithm, that, given solutions $\phi'$ to instance $I'$ and $\phi''$ to instance $I''$, computes a solution $\phi$ to instance $I'$ , with $\cro(\phi)\leq \cro(\phi')+\cro(\phi'')+ (m+\optcrors(I))\cdot\poly(\mu)$.
\end{theorem}
\fi



The second theorem deals with narrow instances.


%\mynote{I replaced bound $\optcrors(I)<m^2/\left (\mu^{15}\cdot 2^{c(\log m)^{3/4}\log\log m}\right )$ with $\optcrors(I)<m^2/\mu^{16}$, because the latter bound is cleaner and simpler. I currently don't see a reason to prefer the old bound over it. I also replaced the probability of failure with $1/\mu^2$ instead of $1/\mu$. We could just repeat the algorithm $\mu$ times if needed.}

\begin{theorem}\label{lem: not many paths}
	There is an efficient randomized algorithm,  that,  given a narrow subinstance  $I=(G,\Sigma)$ of $I^*$, with $m=|E(G)|\geq \mu^{20}$, either  returns FAIL, or computes  a $\nu$-decomposition $\iset$ of $I$, for $\nu= 2^{O((\log m)^{3/4}\log\log m)}$,   such that, for every instance $I'=(G',\Sigma')\in \iset$, $|E(G')|\le m/\mu$. Moreover, if $\optcrors(I)<m^2/\mu^{16}$, then the probability that the algorithm returns FAIL is at most $1/\mu^2$.
\end{theorem}


The majority of the remainder of this paper is dedicated to the proof of the above theorem: we develop the central technical tools used in the theorem's proof in  \Cref{sec: guiding paths orderings basic disengagement} -- \Cref{sec: main disengagement}, and complete the proof in \Cref{sec: computing the decomposition}.
In the remainder of this section, we complete the proof of Theorem \ref{thm: main} using Theorems \ref{lem: many paths} and \ref{lem: not many paths}.


\iffalse
\mynote{restate the lemma in terms of $\alpha$-decomposition into subinstances}
\begin{lemma}\label{lem: not many paths}
	There is an efficient randomized algorithm,  that,  given a non-interesting subinstance  $I=(G,\Sigma)$ of $I^*$ with $|E(G)|=m\geq \mu^{10}$, either correctly certifies that $\optcrors(I)\geq \Omega(m^2/\mu^5)$, or computes  a collection $\iset$ of subinstances of $I$,  such that
	the following hold:
	
	\begin{itemize}
		\item for every instance $I'=(G',\Sigma')\in \iset$, $|E(G')|\le m/\mu$;
		\item  $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq O(m)$; and
		\item $\expect{\sum_{I'\in \iset}\optcrors(I')}\le \left (\optcrors(I)+|E(G)|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}$.
	\end{itemize}

 Moreover, there is an efficient algorithm, that, given, for each instance $I'\in \iset$, a feasible solution $\phi(I')$, computes a feasible solution $\phi$ for instance $I$, of cost $\cro(\phi)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$.
\end{lemma}

\fi

%Throughout, we assume that the constant $c'$ in the statement of \Cref{thm: main} and the constant $c_g$ in the definition of good collections of subinstances are both large enough so that $\min\set{c',c_g}>c+50$ holds, where $c$ is the constant from \Cref{lem: many paths}.

Recall that we are given an instance $I=(G,\Sigma)$, that is a subinstance of the input instance $I^*=(G^*,\Sigma^*)$, with $|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$. We denote $m=|E(G)|$. We compute the desired collection $\iset$ of subinstances of $I$ in two steps. 
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%


If instance $I$ is a narrow instance, then we skip the first step. We let $\iset'$ be a collection of subinstances of $I$, that consists of instance $I$ only. Assume now that $I$ is a wide instance. Then we execute Step 1, by applying the algorithm from \Cref{lem: many paths} to $I$. 
If the algorithm returns FAIL, then we terminate the algorithm and return FAIL as well.
Otherwise, let $\iset'$ be the resulting collection of subinstances of $I$.  Recall that we are guaranteed that,  for each instance $I'=(G',\Sigma')\in \iset'$, either $I'$ is a narrow instance, or $|E(G')|\le m/\mu$. Additionally, we are guaranteed that $\sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\le |E(G)|$;
and,  if 
$\optcrors(I)<m^2/\mu^{c'}$, then with probability at least $31/32$:
$$\sum_{I'\in \iset'}\optcrors(I')\leq 2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g},$$
%
for some constant $c_g$.
We say that a bad event $\event'_1$ happens if $\optcrors(I)\leq m^2/\mu^{c'}$, but: $$\sum_{I'\in \iset'}\optcrors(I')> 2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
From \Cref{lem: many paths},  $\prob{\event'_1}\leq 1/32$.
We say that a bad event $\event''_1$ happens if algorithm from \Cref{lem: many paths} returns FAIL when applied to $I$.
From \Cref{lem: many paths},  $\prob{\event''_1}\leq 1/\mu^2$.
Define the bad event $\event_1=\event'_1\cup \event''_1$, so $\prob{\event_1}\leq 1/31$.
This completes the first step of the algorithm.

We now describe the second step.
We start by partitioning the set  $\iset'$ of instances into two subsets: set $\iset_1'$ containing all instances $I'=(G',\Sigma')$ with $|E(G')|\leq m/\mu$, and set $\iset_2'$ containing all remaining instances, that must be narrow.
We use the following simple observation.

\begin{observation}\label{obs: optbound for narrow}
	If $\optcrors(I)\leq m^2/\mu^{c'}$, and Event $\event_1$ does not happen, then for every instance $I'=(G',\Sigma')\in \iset_2'$, $\optcrors(I')\leq |E(G')|^2/\mu^{16}$.
	\end{observation}
\begin{proof}
Assume that  $\optcrors(I)\leq m^2/\mu^{c'}$, and that Event $\event_1$ does not happen.  Then: 
%
$$\sum_{I'\in \iset'}\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
%	
Consider now some instance $I'=(G',\Sigma')\in \iset_1'$. We then get that: 
%
$$\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}\leq \mu\cdot \optcrors(I)+m\cdot\mu^{c_g},$$ 
%	
since $\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$.
	
Since $m\geq \mu^{c'}$, and since we can assume that $c'$ is a large enough constant, $\mu^{c_g}\leq m/\mu^{c'/2}$. Further, since we have assumed that $\optcrors(I)\leq m^2/\mu^{c'}$, and since $|E(G')|\geq m/\mu$ (since instance $I'=(G',\Sigma')$ belongs to set $\iset_2'$), we get that:
%	
$$\optcrors(I')\leq m^2/\mu^{c'-1}+m^2/\mu^{c'/2}\leq |E(G')|^2/\mu^{16},$$
%		
assuming that $c'$ is large enough.
\end{proof}


Next, we process every instance $I'\in \iset_2'$  one by one. Notice that for each such instance $I'=(G',\Sigma')$, $|E(G')|\geq m/\mu\geq \mu^{20}$ must hold, since $m\geq \mu^{c'}$. When instance $I'$ is processed, we apply the algorithm from \Cref{lem: not many paths} to it. If the algorithm returns FAIL, then we terminate the algorithm and return FAIL as well. Otherwise, we obtain a collection $\iset(I')$ of subinstances of $I'$ (and hence of $I$). If the algorithm did not terminate with a FAIL, then we obtain the final collection  $\iset^*=\iset_1'\cup \left (\bigcup_{I'\in \iset_2'}\iset(I')\right)$ of subinstances of $I$ that the algorithm returns. 
This completes the description of the algorithm. 




In order to analyze it, we first show that, if  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/16$.

\begin{observation}\label{obs: fail prob}
	If  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/16$.
\end{observation}

\begin{proof}
	For an instance $I'=(G',\Sigma')\in \iset'$, we say that a bad event $\event(I')$ happens if the algorithm from \Cref{lem: not many paths}, when applied to $I'$, returns FAIL. From \Cref{lem: not many paths}, if 
	$\optcrors(I')<|E(G')|^2/\mu^{16}$, then the probability that the algorithm returns FAIL is at most $1/\mu^2$. Therefore, from \Cref{obs: optbound for narrow}, if Event $\event_1$ does not happen, then $\prob{\event(I')}\leq 1/\mu^2$. Let $\event_2$ be the bad event that $\event(I')$ happens for any instance $I'\in \iset'_2$.  Since every instance $I'\in \iset_2'$ contains at least $m/\mu$ edges, while, as we have established already, the total number of edges in all instances in $\iset'$
	is at most $m$, we get that $|\iset'_2|\leq \mu$. From the Union Bound, assuming that the constant $c^*$ in the definition of the parameter $\mu$ is large enough, $\prob{\event_2\mid \neg \event_1}\leq 1/100$. Clearly, $\prob{\event_2}\leq \prob{\event_1}+\prob{\event_2\mid \neg \event_1}\leq 1/31+1/100< 1/20$. Note that, if events $\event_1$ and $\event_2$ do not happen, then algorithm may not return FAIL. We conclude that, if $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/20<1/16$.
\end{proof}

We define the bad event $\event=\event_1\cup \event_2$, where event $\event_2$ is defined in the proof of above observation. From the above discussion $\prob[]{\event}\le 1/20$.

Fron now on we assume that the algorithm did not return FAIL.
Recall that \Cref{lem: not many paths} gurantees that, for every instance $I'=(G',\Sigma')\in \iset_2'$, for every subinstance $I''=(G'',\Sigma'')\in \iset(I')$,  $|E(G'')|\leq |E(G')|/\mu\leq m/\mu$ holds. Therefore, for every instance $I''=(G'',\Sigma'')\in\iset^*$, $|E(G'')|\leq m/\mu$ must hold.
Additionally, from the definition of a $\nu$-decomposition, we are guaranteed  that for all $I'=(G',\Sigma')\in \iset_2'$, $\sum_{I''=(G'',\Sigma'')\in \iset(I')}|E(G'')|\leq |E(G')|\cdot (\log (|E(G')|)^{O(1)}\leq |E(G')|\cdot (\log m)^{O(1)}$.
Moreover, since $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$, we get that:

$$\sum_{I''=(G'',\Sigma'')\in \iset^*}|E(G'')|\leq \sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\cdot (\log m)^{O(1)}\leq m\cdot(\log m)^{O(1)}.$$ 








Next, we provide Algorithm \algcombine. 

\begin{claim}\label{claim: combine drawings}
	There is an efficient algorithm, called \algcombine, that, given a solution $\phi(I'')$ to each instance $I''\in \iset^*$, computes a solution $\phi(I)$ to instance $I$, of cost at most $O(\sum_{I''\in \iset^*}\cro(\phi(I''))) +(\optcrors(I)+|E(G)|)\cdot\mu^{O(1)}$.
\end{claim}
\begin{proof}
We construct the solution $\phi(I)$ to instance $I$ in two steps.

In the first step, we compute a solution $\phi(I')$ to each instance $I'\in \iset'_2$, as follows. Consider any such instance $I'=(G',\Sigma')\in \iset'_2$. Recall that we are given, for each instance $I''\in \iset(I')$, a solution $\phi(I'')$. Recall also that $\iset(I')$ is a $\nu$-decomposition  of $I'$. We apply the efficient algorithm $\alg(\iset(I'))$ from the definition of $\nu$-decompositions of instances to the drawings $\set{\phi(I'')}_{I''\in \iset(I')}$, to obtain a feasible solution $\phi(I')$ for instance $I'$, of cost $\cro(\phi(I'))\leq O\left (\sum_{I''\in \iset(I')}\cro(\phi(I''))\right )$.


We have now obtained a solution $\phi(I')$ to every instance $I'\in \iset'$. In the second step, we apply the algorithm in the third bullet of the statement of \Cref{lem: many paths}  to these solutions, to obtain a solution $\phi(I)$ to instance $I$.
The cost of the solution is bounded by:
%
\[\begin{split}   
\cro(\phi(I)) &\leq \sum_{I'\in \iset'}\cro(\phi(I')) + (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq  \sum_{I'\in \iset'_1}\cro(\phi(I')) +\sum_{I'\in \iset'_2}\cro(\phi(I'))+ (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq \sum_{I'\in \iset'_1}\cro(\phi(I')) +\sum_{I'\in \iset'_2}O\left (\sum_{I''\in \iset(I')}\cro(\phi(I''))\right )+ (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq O\left (\sum_{I''\in \iset^*}\cro(\phi(I'))\right ) +(m+\optcrors(I))\cdot\mu^{O(1)}.
\end{split}
\]
\end{proof}


 In order to complete the proof of \Cref{thm: main}, it is now enough to prove the following observation.
 
\begin{observation}\label{obs: bound sum of opts}
	If $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $$\sum_{I''\in \iset^*}\optcrors(I'')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}.$$
\end{observation}


\begin{proof} 
Assume that $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$. Recall that, if Event $\event$ does not happen, then:
%
$$\sum_{I'\in \iset'}\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
%
From the definition of a $\nu$-decomposition, for every instance $I'=(G',\Sigma')\in \iset'_2$, 
%
\[\expect{\sum_{I''\in \iset(I')}\optcrors(I'')}\le \left (\optcrors(I')+|E(G')|\right )\cdot \nu \leq \left (\optcrors(I')+|E(G')|\right ) \cdot 2^{O((\log m)^{3/4}\log\log m)},\]
%
Therefore, if $\event$ does not happen, then: 
%
\[ 
\begin{split}
\expect{\sum_{I''\in \iset^*}\optcrors(I'')}&\leq \sum_{I'\in \iset'_1}\optcrors(I') +\sum_{I'\in \iset'_2}\expect{\sum_{I''\in \iset(I')}\optcrors(I'')}\\
&\leq  \sum_{I'\in \iset'_1}\optcrors(I')+\sum_{I'=(G',\Sigma')\in \iset'_2}\left (\optcrors(I')+|E(G')|\right ) \cdot 2^{O((\log m)^{3/4}\log\log m)}\\
&\leq \sum_{I'=(G',\Sigma')\in \iset'}\left (\optcrors(I')+|E(G')|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}\\
&\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}.
\end{split} \]
%
We denote this expectation by $\eta'$. Let $\hat \event$ be the bad event that 
$\sum_{I''\in \iset^*}\optcrors(I'')>100\eta'$. From Markov's inequality, $\prob{\hat \event\mid \neg\event}<1/100$. Note that, if neither of the events $\hat \event,\event$ happens, then we are guaranteed that $\sum_{I''\in \iset^*}\optcrors(I'')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}$. The probability that either one of these events happens is bounded by $\prob{\event}+\prob{\hat \event\mid \neg\event}\leq 1/20+ 1/100\leq 1/16$. We conclude that, If $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $$\sum_{I''\in \iset^*}\optcrors(I'')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}.$$
\end{proof}





%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%Only old stuff below this

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
\iffalse
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
Moreover, we are guaranteed that, 
%
\[\expect[]{\sum_{I''\in \iset^*}\optcrors(I'')}\leq  \nu''\cdot \bigg( \sum_{I'=(G',\Sigma')\in \iset'}\big(\optcrors(I')+|E(G')|\big)\bigg ). \]
%
Assume that event $\event$ did not happen. Then,
\[
\begin{split}
\expect[]{\sum_{I''\in \iset^*}\optcrors(I'')} &\text{ }\leq  \nu''\cdot \expect[]{ \sum_{I'=(G',\Sigma')\in \iset'}\big(\optcrors(I')+|E(G')|\big)}\\
&\text{ }\leq  \nu''\cdot \expect[]{\sum_{I'=(G',\Sigma')\in \iset'}\optcrors(I')}+\nu''\cdot\bigg(\sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\bigg)\\
&\text{ }\leq  \nu''\cdot \bigg(\nu'\cdot\optcrors(I)+|E(G)|\cdot \mu^c\bigg)+\nu''\cdot(\log|E(G)|)^{O(1)}\cdot|E(G)|\\
&\text{ }\leq  (\nu'\nu'')\cdot \optcrors(I)+O(\nu''\cdot\mu^c)\cdot|E(G)|.
\end{split} \]
Let $\nu=\nu'\cdot\nu''$.
Since $\nu',\nu''=2^{O((\log m)^{3/4}\log\log m)}$, $\nu=\nu'\cdot\nu''=2^{O((\log m)^{3/4}\log\log m)}$.
Since $\mu^{c_g}>\nu''\cdot\mu^{c}$, with probability at least $9/10$, the resulting collection $\iset^*$ of instances is perfect for $I$. 



\fi
\iffalse

 In order to do so,  
@@@@ we compute a denote by $\iset(I')=\set{I''_1,\ldots,I''_k}$ the set of subinstances obtained by applying the algorithm from \Cref{lem: not many paths} to it.  From the definition of a $\nu''$-decomposition, we are also given an efficient algorithm $\alg(\iset(I'))$, that takes as input a solution of each instance in $\iset(I')$ and returns a solution of $I'$. We apply this algorithm to the solutions $\set{\phi(I''_i)}_{1\le i\le k}$ to the subinstances in $\iset(I')$ and let $\phi(I')$ be the solution we get. From the definition of a $\nu''$-decomposition, there exists some universal constant $c^*>0$, such that $\cro(\phi(I'))\le c^*\cdot \sum_{1\le i\le k}\cro(\phi(I''_i))$.

Clearly, after the first step, we have obtained, for each subinstance $I'\in \iset'$, a solution $\phi(I')$ to instance $I'$.
%
Recall that, in \Cref{lem: many paths} we are also given an efficient algorithm (that we denote by $\alg'(\iset')$), that, given, for every instance $I'\in \iset'$, a solution $\phi(I')$ to instance $I'$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq \big(\sum_{I'\in \iset'}\cro(\phi(I'))\big)+ (m+\optcrors(I))\cdot\mu^c$.
In the second step, we simply apply the algorithm to the set $\set{\phi(I')}_{I'\in \iset'}$ of solutions and let $\phi(I)$ be the solution to instance $I$ that we obtain. From \Cref{lem: many paths},
\[
\begin{split}
\cro(\phi)\leq & \text{ } \bigg(\sum_{I'\in \iset'}\cro(\phi(I'))\bigg)+ (m+\optcrors(I))\cdot\mu^c\\
\leq & \text{ } c^*\cdot \bigg(\sum_{I''\in \iset^*}\cro(\phi(I''))\bigg)+ (m+\optcrors(I))\cdot\mu^c.
\end{split}
\]
Now \Cref{thm: main} follows by setting $c_g$ to be a contant such that $c_g> \max\set{c^*, c}$.
\fi





\iffalse{previous algorithm algcombine}
Consider the partitioning tree $T^*$ that is obtained from the partitioning tree $T$ in the first Stage, by adding, for each leaf $v(I')$ of $T$ with $I'\in \iset'_2$ and for each instance $I''\in \iset(I')$, a new vertex $v(I'')$ and an edge connecting it to $v(I')$. Clearly, the instances in $\iset^*$ correspond to leaves in $T^*$. Assume now that we are given, for each instance $I'$ such that $v(I')$ is a leaf in $T^*$, a solution $\phi(I')$ to instance $I'$. We will construct a drawing of instance $I$ in two steps as follows.

In the first step, for each instance $I'\in \iset'_2$, we denote by $\iset(I')=\set{I''_1,\ldots,I''_k}$ the set of subinstances obtained by applying the algorithm from \Cref{lem: not many paths} to it. Recall that, from the definition of a $\nu$-decomposition in \Cref{lem: not many paths} we are also given an efficient algorithm $\alg(\iset(I'))$, that takes as input a solution of each instance in $\iset(I')$ and returns a solution of $I'$. We apply this algorithm to the solutions $\set{\phi(I''_i)}{1\le i\le k}$, and let $\phi(I')$ be the solution we get. From the definition of a $\nu$-decomposition, $\cro(\phi')\le c^*\cdot \sum_{1\le i\le k}\cro(\phi(I''_i))$ for some universal constant $c^*$.

In the second step, we look at the partitioning tree $T$ of Stage 1, and note that now we have, for each instance $I'$ such that $v(I')$ is a leaf in $T$, a solution $\phi(I')$ of $I'$. We now construct a solution for every instance that corresponds to a vertex in $T$ in a bottom-up fashion as follows. In each iteration, we take a vertex $v(I')$ in $T$ with children $v(I''_1),v(I''_2)$ in $T$, such that we have not yet computed a solution of instance $I'$, but we have already computed a solution $\phi(I''_1)$ for instance $I''_1$ and a solution $\phi(I''_2)$ for instance $I''_2$. Note that it is not hard to see that such a vertex has to exist in each iteration.
We not apply the solution-combining algorithm from \Cref{lem: many paths} to the solutions $\phi(I''_1), \phi(I''_2)$, and obtain a solution $\phi(I')$ to instance $I'$. This completes the description of an iteration. We keep performing iterations until we obtain a solution $\phi(I)$ to the input instance $I$.

It remains to upper bound $\cro(\phi(I))$. Recall that at the end of the first step, we have obtained, for each instance $I'\in \iset'$ that corresponds to a leaf in $T$, a solution $\phi(I')$ to $I'$, such that $\sum_{I'\in \iset'}\cro(\phi(I'))\le c^*\cdot\sum_{I'\in \iset^*}\cro(\phi(I'))$. Recall that the depth of tree $T$ is at most $2\mu^{11}$.
Moreover, for each non-leaf instance $I'=(G',\Sigma')$ of $T$, if we denote by $I''_1,I''_2$ the instances that correspond to its children in $T$, then $\cro(\phi(I'))\le \cro(\phi(I''_1))+\cro(\phi(I''_2))+(\optcrors(I')+|E(G')|)\cdot \mu^c$.

Via similar arguments as in the proof of \Cref{cor: stage 1} we can show that, for each $1\le i\le \floor{2\mu^{11}}$, if we denote by $\iset'_i$ be the set of subinstances obtained after iteration $i$, then
\[
\sum_{I'\in \iset'_{i+1}}\optcrors(I')+m\cdot \mu^{c+13}\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12}),
\]
Therefore, 
\[
\sum_{I': v(I')\in V(T)}\optcrors(I')+m\cdot \mu^{c+13}\leq 4\cdot \bigg(\optcrors(I)+  m\cdot  \mu^{c+13}\bigg).
\]
It follows that 
\[
\begin{split}
\cro(\phi(I)) 
& \le \sum_{I' \in \iset'} \cro(\phi(I')) +\dep(T)\cdot O\bigg(\sum_{I \notin \iset'} \big(\optcrors(I)+|E(G)|\cdot \mu^{c+13}\big)\bigg)\\ 
& \le c^*\cdot \sum_{I' \in \iset^*} \cro(\phi(I')) +8\cdot\bigg(\mu^{11}\cdot \optcrors(I)+\mu^{11}\cdot \mu^{c+13}\cdot |E(G)|\big)\bigg).
\end{split}
\]
Now \Cref{thm: main} follows by setting $c_g$ to be a contant such that $c_g\ge \max\set{c^*, c+25}$.
\fi







%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

\iffalse

It is easy to verify that $T^*$ is 
We say that the instances in $\iset_i(I)$ are \emph{critical subinstance} to instance $I$, iff $\cro(\phi_i)=\min\set{\cro(\phi_1),\ldots, \cro(\phi_L),|E(G)|^2}$.
Consider now the tree $T^*$, which is the subtree of $T$ induced by $v(I^*)$ and all vertices $v(I)$ such that the instance $I$ is critical.
It is easy to see that every leaf of $T^*$ is also a leaf of $T$.
Let $I$ be an instance with $v(I)\in V(T^*)$ and let $I_1,\ldots,I_k$ be its critical subinstances, where $I_i=(G_i,\Sigma_i)$ for each $i$.
From \Cref{thm: main} and since the event $\event$ does not happen, 
$\sum_{1\le i\le k}\optcrors(I_i)\leq \optcrors(I)\cdot \nu +|E(G)|\cdot\mu^{c_g}$ and $\sum_{1\le i\le k}|E(G_i)|\leq |E(G)|\cdot (\log m^*)^{c_g}$ (where we have used the fact that $|E(G)|\le m^*$).
Therefore, since $(\log m^*)^{c_g}<\nu$,
\[
\sum_{1\le i\le k}\bigg(\optcrors(I_i)+|E(G_i)|\cdot \mu^{c_g}\bigg)\leq \bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg)\cdot \nu.
\]
It is easy to see that, if we denote by $\iset^{(j)}$ the set of all critical instances at recursive level $j$, then 
\[
\sum_{I=(G,\Sigma)\in \iset^{(j)}}\bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg)\leq \bigg(\optcrors(I^*)+|E(G^*)|\cdot \mu^{c_g}\bigg)\cdot \nu^{j}.
\]
It follows that, if we denote by $\iset^*$ the set of all critical subinstances, then 
\[
\begin{split}
\sum_{I=(G,\Sigma)\in \iset^{^*}}\bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg) & \leq \bigg(\optcrors(I^*)+|E(G^*)|\cdot \mu^{c_g}\bigg)\cdot 2^{O((\log m^*)^{7/8}\log\log m^*)}\\
& = 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split}
\]


Consider now any instance $I=(G,\Sigma)$ with $v(I)\in V(T^*)$. We first denote $\cost^*(I)=\mu^{c_g}\cdot\optcrors(I)+|E(G)|\cdot \mu^{2c_g}$. From the above discussion,
\[
\sum_{I=(G,\Sigma)\in \iset^{^*}}\cost^*(I) \leq 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\]
We then define the \emph{height} of $I$, denoted by $h(I)$, to be the largest distance from $v(I)$ to a descendant vertex of $v(I)$ in the tree $T^*$. In particular, if $v(I)$ is a leaf in $T^*$, then $h(I)=0$, and, from \Cref{obs: few recursive levels}, for every non-leaf subinstance $I$, $h(I)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$ always holds.
For an instance $I'$ such that vertex $v(I')$ is a descendant of vertex $v(I)$ in $T^*$, we write $I'\prec I$.


We prove by induction on $h(I)$ that the value of the solution $\phi(I)$ that $\algrec(I)$ computes satisfies that 
$$\cro(\phi(I))\le \mu^{2c'}\cdot\cost^*(I)+\mu^{2c'}\cdot\sum_{I' \prec I} \cost^*(I')\cdot c_g^{h(I)-h(I')}.$$ 
The induction base is when $h(I)=0$, so $v(I)$ is a leaf vertex of $T$. We have shown that the claim holds in this case.
%
Let $I=(G,\Sigma)$ be a non-leaf subinstance with $v(I)\in V(T^*)$ and let $I_1,\ldots,I_k$ be its critical subinstances. If we denote by $\phi(I)$ the drawing of $I$ returned by the algorithm \algrec, and similarly we define drawings $\set{\phi(I_i)}_{1\le i\le k}$, then from \Cref{thm: main}, 
\[
\cro(\phi(I)) \le  c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i))+ \bigg(\optcrors(I)+|E(G)|\bigg)\cdot \mu^{c_g} \le \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i)).
\]
Note that for each $1\le i\le k$, $h(I_i)\le h(I)-1$. Therefore, from the induction hypothesis,
\[
\begin{split}
\cro(\phi(I)) & \leq \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i))\\
& \le  \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\bigg(\mu^{2c'}\cdot\cost(I_i)+\mu^{2c'}\cdot\sum_{I' \prec I_i} \cost^*(I')\cdot c_g^{h(I_i)-h(I')}\bigg)\\
& \le  \mu^{2c'}\cdot\cost^*(I)+ \mu^{2c'}\cdot\sum_{1\le i\le k}\bigg(c_g\cdot\cost(I_i)+\sum_{I' \prec I_i} \cost^*(I')\cdot c_g^{h(I_i)-h(I')+1}\bigg)\\
& \le  \mu^{2c'}\cdot\cost^*(I)+ \mu^{2c'}\cdot\sum_{I'\prec I} \cost^*(I')\cdot c_g^{h(I)-h(I')}.
\end{split}
\]
Therefore, since $h(I^*)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$, we get that for each $I'\in \iset^*$, $c_g^{h(I^*)-h(I')}\le \mu$, and so
\[
\begin{split}
\cro(\phi(I^*))\le & \text{ } \mu^{2c'}\cdot\cost^*(I^*)+\mu^{2c'}\cdot\sum_{I' \prec I} \cost^*(I')\cdot c_g^{h(I^*)-h(I')}\\
\le & \text{ } 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split} 
\]



\fi





%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\iffalse
Therefore, if we denote by $\iset^{**}$ the set of all subinstances $I$ such that $v(I)$ is a leaf of tree $T^*$, then
\[
\begin{split}
\sum_{I\in \iset^*} \cro(\phi(I)) 
& \le \dep(T)\cdot\bigg(\sum_{I\in \iset^{**}} \cro(\phi(I)) +\sum_{I=(G,\Sigma)\in (\iset^{*}\setminus \iset^{**})} \big(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\big)\bigg)\cdot \mu^{c_g}\\ 
& =\mu^{O(c_g)}\cdot \bigg(\mu^{2c'}\cdot\sum_{I\in \iset^{**}} \optcrors(I)+ 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)
\bigg)\\
& = 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split}
\]
And since $\cro(\phi(I^*))\le \sum_{I\in \iset^{^*}} \cro(\phi(I)) + \bigg(\optcrors(I^*)+|E(G^*)|\bigg)\cdot \mu^{c_g}$, it follows that $\cro(\phi(I^*))=2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)$.

\fi
\iffalse
\znote{cannot prove by induction, need to re-write from here}


%Consider now any vertex $v(I)$ in tree $T^*$. The \emph{height of $I$}, denoted by $h(I)$, is the largest distance from $v(I)$ to a descendant vertex of $v(I)$ in the tree $T$. In particular, if $I$ is a leaf subinstance, then $h(I)=0$, and, from \Cref{obs: few recursive levels}, for every non-leaf subinstance $I$, $h(I)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$ always holds.





We prove by induction on $h(I)$ that the value of the solution $\phi(I)$ that $\algrec(I)$ computes satisfies that $\cro(\phi(I))\le (\optcrors(I)+|E(G)|)\cdot \mu^{c_g}\cdot \nu^{h(I)}$. The induction base is when $h(I)=0$, so $v(I)$ is a leaf vertex of $T$. We have shown that the claim holds in this case.


Consider now some instance $I=(G,\Sigma)$ with $h(I)>0$. Assume first that $\optcrors(I)> |E(G)|^2/\mu^{64}$. Recall that the algorithm \algrec considers a trivial solution $\phi'$ to instance $I$, of cost at most $|E(G)|^2$. Since the algorithm eventually returns the best of the considered solutions, the cost of the solution that it returns may not be higher than $|E(G)|^2\leq \optcrors(I)\cdot \mu^{64}$. 

Therefore, we assume that $\optcrors(I)\leq |E(G)|^2/\mu^{64}$ from now on. Since we have assumed that Event $\event$ did not happen, neither did $\event(I)$. Therefore, there is an instance $1\leq i\leq L$, such that the family $\iset_i(I)$ of instances is a perfect family for instance $I$. In particular, from the definition of a perfect family, we have that
%
$\sum_{I'\in \iset_i(I)}\optcrors(I')\leq \optcrors(I)\cdot \nu +|E(G)|\cdot\mu^{c_g}$.
%and since $m\le m^*$,
%$$m^*\cdot \mu^{c_g}+\sum_{I'\in \iset_i(I)}\optcrors(I')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot\bigg(m^*\cdot \mu^{c_g}+ \optcrors(I)\bigg),$$
%
Using the induction hypothesis, if we denote by $\phi(I')$ the solution that the algorithm computes for each instance $I'\in \iset_i(I)$, then:
%
%	
\[
\begin{split}
\sum_{I'=(G'\Sigma')\in \iset_i(I)}\cro(\phi(I'))\leq & \sum_{I'=(G'\Sigma')\in \iset_i(I)}\bigg(\optcrors(I')\cdot \nu^{h(I)-1}+|E(G')|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\bigg)\\
\leq & \sum_{I'=(G'\Sigma')\in \iset_i(I)}\optcrors(I')\cdot \nu^{h(I)-1}+\sum_{I'=(G'\Sigma')\in \iset_i(I)}|E(G')|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\bigg(\optcrors(I)\cdot\nu+|E(G)|\cdot \mu^{c_g} \bigg)\cdot \nu^{h(I)-1} + c_g\cdot |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\optcrors(I)\cdot \nu^{h(I)} + (c_g+1)\cdot |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\optcrors(I)\cdot \nu^{h(I)} + |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)}.\\
\end{split}
\]
%
Let $\phi$ be the solution to instance  $I$ obtained by applying Algorithm \algcombine to solutions $\phi(I')$ to instances $I'\in \iset_i(I)$. Then, from \Cref{thm: main}, and since we can assume that $c_g$ is a large enough constant, we are guaranteed that:
%
\[
\begin{split}
\cro(\phi) &\leq  \bigg(\sum_{I'\in \iset}\cro(\phi(I')) \bigg) + (\opt(I)+|E(G)|)\cdot \mu^{c_g} \\
&\leq \optcrors(I)\cdot \nu^{h(I)} + |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)}+ (\opt(I)+|E(G)|)\cdot \mu^{c_g}\\
&\leq \optcrors(I)\cdot (\nu^{h(I)}+\mu^{c_g}) + |E(G)|\cdot \mu^{c_g}\cdot (\nu^{h(I)}+1)
\end{split}
\]

% 
Since $h(I^*)\leq \frac{1}{c^*}\sqrt{\frac{\log m^*}{\log\log m^*}}$, we conclude that the cost of the solution $\phi^*$ that the algorithm computes for instance $I^*$ is bounded by:
\[
\begin{split}
(\optcrors(I)+m^*)\cdot \mu^{O(1)}\cdot (\log m)^{\sqrt{\log m^*/\log\log m^*}}&
\leq (\optcrors(I)+m^*)\cdot \mu^{O(1)}\cdot 2^{\sqrt{\log m^*\log\log m^*}}\\ &\leq (\optcrors(I)+m^*)\cdot \mu^{O(1)}. 
\end{split} \]
\fi%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%This completes the proof of \Cref{lem: solution cost}.



\iffalse{backup: previous stage 1}
\paragraph{Stage 1.}
We initialize the set $\iset$ to contain a single instance $I=(G,\Sigma)$. The first stage continues as long as there is any instance $\hat I=(\hat G,\hat \Sigma)\in \iset$, that is an interesting subinstance of $I$, with $|E(\hat G)|>|E(G)|/\mu$. The first stage consists of iterations, where in every iteration we start with an interesting subinstance $\hat I= (\hat G,\hat \Sigma)\in \iset$ with $|E(\hat G)|>m/\mu$. 
We apply the algorithm from \Cref{lem: many paths} to instance $\hat I$, 
obtaining two new instances $\hat I'=(\hat G',\hat \Sigma'),\hat I''=(\hat G'',\hat \Sigma'')$. We then replace $\hat I$ with $\hat I',\hat I''$ in $\iset$, and continue to the next iteration. Let $i$ denote the index of the current iteration. 

We say that the bad event $\event_i$ happens if (i) $|E(\hat G)|>\mu^{39}$; (ii) $\optcrors(\hat I)<|E(\hat G)|^2/\mu^{40}$; and (iii) $\optcrors(\hat I')+\optcrors(\hat I'') > \optcrors(\hat I) \cdot(1+1/\mu^{12})+m \cdot \mu^{c}$. From \Cref{lem: many paths}, the probability that $\event_i$ happens is bounded by $1/(40\mu^{11})$.

This completes the description of the algorithm for Stage 1. In order to analyze it, it is convenient to define a partitioning tree $T$ associated with it. 
For every instance $\hat I$ that ever belonged to set $\iset$ over the course of the Stage 1 algorithm, we add a vertex $v(\hat I)$ to the tree. If the algorithm from \Cref{lem: many paths} was applied to instance $\hat I$, producing two new instances $\hat I'$ and $\hat I''$, then vertices $v(\hat I'),v(\hat I'')$ become children of vertex $v(\hat I)$ in the tree. The root of the tree is the vertex $v(I)$.



We say that bad event $\event$ happens if bad event $\event_i$ happens for any iteration $i\leq 4\mu^{11}$ of Stage 1. From the union bound over all $1\le i\leq 4\mu^{11}$, we get that $\Pr[\event]\le 1/10$. 

Let $T'$ be the subtree of $T$ that is induced by all vertices $v(\hat I)$, such that $\hat I$ belonged to $\iset$ at some point before the completion of iteration $\ceil{2\mu^{11}}$.
Assume now that bad event $\hat \event$ did not happen. Since we only apply the algorithm from \Cref{lem: many paths} to instances $(\hat G,\hat \Sigma)$ with  $|E(\hat G)|>|E(G)|/\mu$, every instance $\hat I'=(\hat G',\hat \Sigma')$ with $v(I')\in T'$ has $|E(\hat G')|\geq |E(G)|/\mu^{11}$. But then the number of the leaf vertices in tree $T'$ is bounded by $\mu^{11}$, and the total number of vertices in tree $T'$ must be bounded by $2\mu^{11}$, since every inner vertex of $T'$ has at least two children. 
This can only happen if the algorithm terminates before the $\floor{2\mu^{11}}$-th iteration. Therefore, if Event $\event$ does not happen, the algorithm has fewer than $2\mu^{11}$ iterations. %Therefore, for every instance $\hat I=(\hat G,\hat Sigma)$ to which 
Moreover, since every instance $\hat I=(\hat G,\hat \Sigma)$ that ever belonged to $\iset$, $|E(\hat G)|\geq |E(G)|/\mu^{11}$ holds, and since we are guaranteed that $|E(G)|\geq \mu^{c'}\geq \mu^{50}$, we conclude that $|E(\hat G)|\geq \mu^{39}$ must hold.
%\iffalse
%Let $\iset'$ be the set of subinstances of $I$ obtained at the end of Stage 1. Equivalently, $\iset'$ contains every instance $I'$ that is a leaf instance. 
We use the following claim.


\begin{claim}\label{claim: few crossings in each instance}
	If event $\event$ did not happen, then for every instance $\hat I=(\hat G,\hat \Sigma)$ that ever belonged to the set $\iset$, $\optcrors(\hat I)\leq |E(\hat G)|^2/\mu^{40}$.
\end{claim}

\begin{proof}
	We say that a vertex $v(\hat I)$ lies at level $\ell$ of the tree $T$ iff the distance from $v(\hat I)$ to the root $v(I)$ of the tree is $\ell$. We will prove that, for all $0\leq \ell \leq \floor{2\mu^{11}}$, for every vertex $v(\hat I)$ lying at level $\ell$ of the tree $T$, with $\hat I=(\hat G,\hat\Sigma)$, 
	\begin{equation}
	\label{eqn: induction}
	\optcrors(\hat I)\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+m\cdot\ell\cdot\mu^{c+13},
	\end{equation}
	
	The proof is by induction on $\ell$. 
	The base case is when $\ell=0$, and $\hat I$ is the input instance $I=(G,\Sigma)$. Recall that, from the statement of \Cref{thm: main}, $\optcrors(G,\Sigma)\leq m^2/\mu^{63}\leq m^2/\mu^{40}$ as required, and it is immediate to verify that the inequality \ref{eqn: induction} holds. 
	Consider now some integer $0\leq \ell \leq \floor{2\mu^{11}}$. We assume that the claim holds for all integers below $\ell$, and prove it for integer $\ell$. Let $\hat I'=(\hat G',\hat \Sigma')$ be any instance, whose corresponding vertex $v(\hat I')$ lies at level $\ell$ of the tree $T$, and let $v(\hat I)$ be the parent vertex of $v(\hat I')$ in the tree, where $\hat I=(\hat G,\hat \Sigma)$. As observed already, if Event $\event$ does not happen, $|E(\hat G)|\geq \mu^{39}$ must hold, and from the induction hypothesis, $\optcrors(\hat I)\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell-1}+m\cdot(\ell-1)\cdot\mu^{c+13}$ and $\optcrors(\hat I)\leq |E(\hat G)|^2/\mu^{40}$ must hold. If we denote by $v(\hat I'')$ the second child vertex of $v(\hat I)$, then, since we have assumed that Event $\hat \event$ does not happen, $\optcrors(I')+\optcrors(I'')\leq \optcrors(I) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}$ must hold. Therefore, 
	\[
	\begin{split}
	\optcrors(I')\leq & \text{ } \bigg(\optcrors(I)\cdot(1+1/\mu^{12})^{\ell-1}+m\cdot(\ell-1)\cdot\mu^{c+13}\bigg) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}\\
	\leq & \text{ } \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+\bigg(m\cdot(\ell-1)\cdot\mu^{c+13}\bigg) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}\\
	\leq & \text{ } \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+ m\cdot\ell\cdot\mu^{c+13}.
	\end{split}
	\]
	Lastly, as observed already, $|E(\hat G')|\geq m/\mu^{11}$. 
	We then get that:
	%
	\[
	\begin{split}
	\optcrors(\hat I')&\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+ m\cdot\ell\cdot\mu^{c+13}\\
	&\leq 2\cdot \optcrors(I)+ 2 m\cdot\mu^{c+24}\\
	&\leq \frac{4m^2}{\mu^{63}} \leq \frac{4\cdot |E(\hat G')|^2\cdot \mu^{22}}{\mu^{63}}\leq \frac{|E(\hat G')|^2}{\mu^{40}}.
	\end{split}
	\]
	%
	Here we have used the fact that $\ell\le \floor{2\mu^{11}}$ and the facts $\optcrors(I)\leq |E(G)|^2/\mu^{63}$ and  $|E(G)|\geq \mu^{c'}$ from the statement of \Cref{thm: main}, together with the assumption that $c'>c+50$.
\end{proof}
%\fi

%Let $\iset'$ be the set of subinstances of $I$ obtained at the end of Stage 1. Equivalently, $\iset'$ contains every instance $I'$ that is a leaf instance. We use the following claim.

\begin{claim}\label{cor: stage 1}
	If Event $\event$ did not happen, then $\sum_{I'\in \iset'}\optcrors(I')\leq 2\cdot  \optcrors(I)+ 2\cdot m\cdot  \mu^{c+13}$.
\end{claim}
\begin{proof}
	For each $1\le i\le \floor{2\mu^{11}}$, we denote by $\iset'_i$ be the set of subinstances obtained after iteration $i$. Therefore, from \Cref{lem: many paths},
	\[
	\sum_{I'\in \iset'_{i+1}}\optcrors(I')\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')\bigg)\cdot (1+1/\mu^{12})+m\cdot\mu^{c},
	\]
	and so
	\[
	\sum_{I'\in \iset'_{i+1}}\optcrors(I')+m\cdot \mu^{c+13}\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12}),
	\]
	Therefore,
	\[
	\sum_{I'\in \iset'}\optcrors(I')\leq \bigg(\optcrors(I)+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12})^{\floor{2\mu^{11}}}\le 2\cdot  \optcrors(I)+ 2\cdot m\cdot \mu^{c+13}.
	\]
\end{proof}

We partition the instances of $\iset'$ into two subsets: set $\iset_1'$ contains all instances $I'=(G',\Sigma')$ with $|E(G')|\leq m/\mu$, while set $\iset_2'$ contains all remaining instances. Notice that by the definition of the Stage 1 algorithm, every instance in $\iset_2'$ is a non-interesting subinstance of the input intance $I$.

\fi

==> overview_bkup1002.tex <==
\section{An Algorithm for \cnwrs -- Proof of \Cref{thm: main_rotation_system}}
\label{sec: high level}



%\mynote{Throughout the paper, a solution to instance $I$ is referred to as $\phi(I)$ or $\phi_I$ interchangeably. I suggest that we stick to the former. Could you please fix this in the current section? Thanks!}

In this section we provide a proof of Theorem \ref{thm: main_rotation_system}, with some of the details deferred to subsequent sections.
%
Throughout the paper, we denote by $I^*=(G^*,\Sigma^*)$  the input instance of the \CNwRS problem, and we denote $m^*=|E(G^*)|$. We also use the following parameter that is central to our algorithm: ${\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}}$, %\mynote{may need to adjust}, 
where $c^*$ is a large enough constant. 

As mentioned already, our algorithm for solving the \CNwRS problem is recursive, and, over the course of the recursion, we will consider subinstances of instance $I^*$ (see \Cref{subsec: subinstances} for a definition). %Each such subinstance is determined by a sub-graph $G'\subseteq G^*$, and disjoint collections $S_1,\ldots,S_q$ of vertices of $G'$. Graph $G$ is obtained from $G'$ by unifying, for all $1\leq i\leq q$, all vertices of $S_i$ into a vertex $u_i$, that we call a \emph{supernode}. We keep parallel edges but remove self-loops. For every vertex $v\in V(G)$ that is also a vertex of $G^*$, its rotation system $\oset_v$ in $\Sigma$ remains the same as in $\Sigma^*$, while for every supernode $u_i$, we will define its rotation system $\oset_{u_i}$ explicitly. Notice that subinstance relation is transitive: if $(G_1,\Sigma_1)$ is a subinstance of $(G_0,\Sigma_0)$, and $(G_2,\Sigma_2)$ is a subinstance of $(G_1,\Sigma_1)$, then $(G_2,\Sigma_2)$ is a subinstance of $(G_0,\Sigma_0)$.
The algorithm proceeds by recursively decomposing a given subinstance $I$ of $I^*$  into a collection of smaller subinstances. 
The main technical ingredient of the proof is the following theorem.


\mynote{this theorem has changed. Instead of producing one family $\iset$ of instances, it now produces $\log m^*$ such families. I also increased probability of success. Please update Sec 3.1 to take this into account.}
\begin{theorem}
	\label{thm: main}
	There is a constant $c'$, and an efficient randomized algorithm, that, given a subinstance $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, either returns FAIL, or produces $z=\ceil{\log m^*}$ collections $\iset_1,\ldots,\iset_z$ of subinstances of $I$ with the following properties:
	
\begin{itemize}
\item at least one of the collections $\iset_1,\ldots,\iset_z$ is non-empty;
\item for each subinstance $I'=(G',\Sigma')\in \bigcup_{j=1}^z\iset_j$, $|E(G')|\leq m/\mu$;

\item for all $1\leq j\leq z$, $\sum_{I'=(G',\Sigma')\in \iset_j}|E(G')|\leq  m\cdot (\log m)^{O(1)}$;

\item there is an efficient algorithm called \algcombine, that, given an index $1\leq j\leq z$, and a solution $\phi(I')$ to each instance $I'\in \iset_j$, computes a solution $\phi$ to instance $I$;


\item if $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $(1-1/\mu)$, the algorithm does not return FAIL, and
 there is an index $1\leq j\leq z$  for which the following hold:

\begin{itemize}
	\item $\iset_j\neq \emptyset$;
	
\item 	$\sum_{I'\in \iset_j}\optcrors(I')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}$; and

\item if algorithm \algcombine is given as input a solution $\phi(I')$ to each instance $I'\in \iset_j$, then the resulting solution $\phi$ to instance $I$ that it computes has cost at most: $$O\bigg(\sum_{I'\in \iset_j}\cro(\phi(I'))\bigg) +(\optcrors(I)+|E(G)|)\cdot\mu^{O(1)}.$$
\end{itemize} 
\end{itemize}
\end{theorem}




\iffalse
We now define collections of subinstances that have some desirable properties. The following definition is  similar in spirit to the definition of a $\nu$-decomposition of an instance, but, since it uses slightly different parameters, we distinguish between these two definitions.

\begin{definition}[Good and Perfect Collection of Subinstances]
	Let $I=(G,\Sigma)$ be a subinstance of instance $I^*$, with $|E(G)|=m$, and let $\iset$ be a collection of subinstances of $I$. We say that $\iset$ is a \emph{good collection of subinstances} for $I$ if the following hold.
	
	\begin{itemize}
		\item for each subinstance $I'=(G',\Sigma')\in \iset$, $|E(G')|\leq m/\mu$;
		\item $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq  m\cdot (\log m)^{c_g}$, where $1000<c_g<c^*$ is some large enough universal constant whose value will be set later; and
		
		\item there is an efficient algorithm, that we call \algcombine, that, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, of cost at most $c_g\cdot(\sum_{I'\in \iset}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{c_g}$.
	\end{itemize}

 We say that $\iset$ is a \emph{perfect} collection of subinstances for $I$ if, additionally:
	$$\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{c_g}.$$
\end{definition}

The main technical ingredient of the proof is the following theorem.

\begin{theorem}
	\label{thm: main}
	There is an efficient randomized algorithm, whose input is a subinstance $I=(G,\Sigma)$ of $I^*$, with $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$ and $|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$. The algorithm outputs a good collection $\iset$ of subinstances of $I$, and, with probability at least $7/8$, $\iset$ is a perfect collection of subinstances for $I$.
\end{theorem}
%\znote{(1) to set $\mu$; (2) theorem may need to be changed due to bad/deleted edges.}
\fi

The remainder of this paper is dedicated to the proof of \Cref{thm: main}. In the following subsection, we complete the proof of \Cref{thm: main_rotation_system} using \Cref{thm: main}.



%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
\subsection{Proof of \Cref{thm: main_rotation_system}}

%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
Throughout the proof, we assume that $m^*$ is larger than a sufficiently large constant, since otherwise we can return a trivial solution to instance $I^*$, from \Cref{thm: crwrs_uncrossing}.

We let $100<c_g<c^*/2$ be a large enough constant, so that, if the algorithm from \Cref{thm: main}, when applied to a subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, returns a family $\iset$ of subinstances of $I$, with $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq  m\cdot (\log m)^{c_g}$. Additionally, if  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot 2^{c_g((\log m)^{3/4}\log\log m)} +m\cdot\mu^{c_g}$. We also assume that Algorithm \algcombine, given a solution $\phi(I')$ to each instance $I'\in \iset$, computes a solution $\phi$ to instance $I$, of cost at most $c_g\cdot (\sum_{I'\in \iset}\cro(\phi(I')) +(\optcrors(I)+|E(G)|)\cdot\mu^{c_g}$.


We use a simple recursive algorithm called \algrec, that appears in Figure \ref{fig: algrec}.


\program{\algrec}{fig: algrec}{ 
\noindent{\bf Input:} a subinstance $I=(G,\Sigma)$ of the input instance $I^*$ of the \CNwRS problem.

\noindent{\bf Output:} a feasible solution to instance $I$.

\begin{enumerate}
	\item Use the algorithm from \Cref{thm: crwrs_planar} to determine whether or not $\optcrors(I)=0$. If so, use the algorithm from \Cref{thm: crwrs_planar} to compute a solution to $I$ of cost $0$. Return this solution, and terminate the algorithm.
	
	\item Use the algorithm from Theorem~\ref{thm: crwrs_uncrossing} to compute a trivial solution $\phi'$ to instance $I$.
	
	\item If $|E(G)|\leq \mu^{c'}$, return the trivial solution $\phi'$ and terminate the algorithm.
	
	\item For $1\leq j\leq \ceil{\log m^*}$:
	\begin{enumerate}
		\item Apply the algorithm from \Cref{thm: main} to instance $I$. 

			\item If the algorithm returns FAIL, let $\phi_j=\phi'$ be the trivial solution to instance $I$, and set $\iset_j(I)=\emptyset$.
			
			\item Otherwise: 
			\begin{enumerate}	
			\item Let $\iset_j(I)$ be the collection of subinstances of $I$ that the algorithm returns.

		  \item For every subinstance $I'\in \iset_j(I)$, apply Algorithm \algrec to instance $I'$, to obtain a solution $\phi(I')$ to this instance.
		
	   	\item Apply Algorithm \algcombine from \Cref{thm: main} to solutions $\set{\phi(I')}_{I'\in \iset_j(I)}$, to obtain a solution $\phi_j$ to instance $I$.
	   	\end{enumerate}
	\end{enumerate}
\item %Let $\phi'$ be a trivial solution to instance $I$, of cost at most $|E(G)|^2$. 
Return the best solution of $\set{\phi',\phi_1,\ldots,\phi_{\ceil{\log m^*}}}$
\end{enumerate}
}



In order to analyze the algorithm, it is convenient to associate a \emph{partitioning tree} $T$ with it, whose vertices correspond to all subinstances considered over the course of the algorithm. Let $L=\ceil{\log m^*}$. We start with the tree $T$ containing a single root vertex $v(I^*)$, representing the input instance $I^*$. Consider now some vertex $v(I)$ of the tree, representing some subinstance $I=(G,\Sigma)$ of $I^*$.
When Algorithm \algrec was applied to instance $I$, if it did not terminate after the first three steps, it created $L$ collections $\iset_1(I),\ldots,\iset_L(I)$ of subinstances of $I$ (some of which may be empty, in case the algorithm from \Cref{thm: main} returned FAIL). For each such subinstance $I'\in \bigcup_{j=1}^L\iset_j(I)$, we add a vertex $v(I')$ representing instance $I'$, that becomes a child vertex of $v(I)$. This concludes the description of the partitioning tree $T$. 


We denote by $\iset^*=\set{I\mid v(I)\in V(T)}$ the set of all subinstances of instance $I^*$ whose corresponding vertex appears in the tree $T$. For each such instance $I\in \iset^*$, its  \emph{recursive level} is the distance from vertex $v(I)$ to the root vertex $v(I^*)$ in the tree $T$ (so the recursive level of $v(I^*)$ is $0$).
For $j\geq 0$, we denote by $\hat \iset_j\subseteq \iset^*$ the set of all instances $I\in \iset^*$, whose recursive level is $j$.
Lastly, the \emph{depth} of the tree $T$, denoted by $\dep(T)$, is the largest recursive level of any instance in $\iset^*$.
 In order to analyze the algorithm, we start with the following two simple observations.

\begin{observation}\label{obs: few recursive levels}
 $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.
\end{observation}
\begin{proof}
	Consider any non-root vertex $v(I)$ in the tree $T$, and let $v(I')$ be the parent-vertex of $v(I)$. Denote $I=(G,\Sigma)$ and $I'=(G',\Sigma')$.
	From the construction of tree $T$, instance $I$ belongs to some collection of subinstances obtained by applying the algorithm from \Cref{thm: main} to instance $I'$. Therefore, from \Cref{thm: main}, $|E(G)|\leq |E(G')|/\mu$ must hold. Therefore, for all $j\geq 0$, for every instance $I=(G,\Sigma)\in \hat \iset_j$, $|E(G)|\leq m^*/\mu^j$. Since $\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$, we get that $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.
\end{proof}

%a We denote by $\dep(T)$ the depth of tree $T$, i.e., the largest recursive level for any instance $I$ with vertex $v(I)\in V(T)$, so $\dep(T)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$.


\begin{observation}\label{obs: num of edges}
$\sum_{I=(G,\Sigma)\in \iset^*}|E(G)|\le m^*\cdot 2^{(\log m^*)^{1/8}}$.
\end{observation}
\begin{proof}
	Consider any non-leaf vertex $v(I)$ of the tree $T$, and denote $I=(G,\Sigma)$. 
Recall that, when Algorithm \algrec is applied to  instance $I$, it applies the algorithm from \Cref{thm: main} to $I$ and compute $L$ collections $\iset_1(I),\ldots,\iset_L(I)$ of subinstances, such that, if we denote $|E(G)|=m$, then, for all $1\leq j\leq L$:
%
 $$\sum_{I'=(G',\Sigma')\in \iset_j(I)}|E(G')|\leq m\cdot (\log m)^{c_g}\leq m\cdot (\log m^*)^{c_g}$$
 %
 (we have used the fact that, if $I$ is a subinstance of $I^*$, then $m\leq m^*$ must hold). Since $L\leq 2\log m^*$, and $m^*$ is sufficiently large, we get that:
 %
 $$\sum_{j=1}^L\sum_{I'=(G',\Sigma')\in \iset_j(I)}|E(G')|\leq m\cdot (\log m^*)^{c_g+2}.$$
 %
 For all $j\geq 0$, we denote by $N_j$ the total number of edges in all instances in set $\hat \iset_j$, $N_j=\sum_{I=(G,\Sigma)\in \hat \iset_j}|E(G)|$. Clearly, $N_0=m^*$, and, from the above discussion, for all $j>0$, $N_j\leq N_{j-1}\cdot (\log m^*)^{c_g+2}$. 
 
 Since $\dep(T)\leq \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$,
we conclude that:
%
\[
%\begin{split}
\sum_{I=(G,\Sigma)\in \iset^*}|E(G)|\leq m^*\cdot (\log m^*)^{2c_g\cdot  (\log m^*)^{1/8}/(c^*\log\log m^*)}\leq m^*\cdot 2^{(\log m^*)^{1/8}}, 
%\end{split}
\]	
%
since $c_g\leq c^*/2$.
\end{proof}

We use the following corollary, that follows  immediately from \Cref{obs: num of edges}.

\begin{corollary}\label{cor: num of instances}
The number of instances $I=(G,\Sigma)\in \iset^*$ with $|E(G)|\geq \mu^{c'}$ is at most $m^*$.
\end{corollary}

\iffalse{original corollary does not depend on the notion of leaf instance}
For an instance $I\in \iset^*$, we say that it is a \emph{leaf instance}, if  vertex $v(I)$ is a leaf vertex of the tree $T$, and we say that it is a non-leaf instance otherwise. We use the following corollary, that follows  immediately from \Cref{obs: num of edges}, and the fact (from the description of Algorithm \algrec) that, if $I=(G,\Sigma)\in \iset^*$ is a non-leaf instance, then  $|E(G)|\geq \mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$ must hold.


\begin{corollary}\label{cor: num of instances}
The number of instances $I=(G,\Sigma)\in \iset^*$ with $|E(G)|\geq \mu^{c'}$ is at most $m^*$.
\end{corollary}
\fi

 	
For an instance $I\in \iset^*$, we say that it is a \emph{leaf instance}, if  vertex $v(I)$ is a leaf vertex of the tree $T$, and we say that it is a non-leaf instance otherwise.
%From the description of Algorithm \algrec, if $I=(G,\Sigma)\in \iset^*$ is a non-leaf instance, then  $|E(G)|\geq \mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$ must hold.
Consider now a non-leaf instance $I\in \iset^*$. We say that a bad event $\event(I)$ happens, if all the following conditions hold:

\begin{itemize}
	\item $0<\optcrors(I)\leq |E(G)|^2/\mu^{c'}$;
	\item $|E(G)|\geq \mu^{c'}$; and
	\item for all $1\leq j\leq L$, we have set $\phi_j=\phi'$ and $\iset_j(I)=\emptyset$, since 
	the algorithm from \Cref{thm: main} returned FAIL in each of the $L$ iterations when it was applied to $I$.
\end{itemize} 

Clearly, from \Cref{thm: main},  $\prob{\event(I)}\le (1/16)^L\leq 1/(m^*)^4$.


We say that a bad event $\event'(I)$ happens if the following conditions hold:

\begin{itemize}
\item $0<\optcrors(I)\leq |E(G)|^2/\mu^{c'}$;
\item $|E(G)|\geq \mu^{c'}$; and
\item for all $1\leq j\leq L$, $\sum_{I'\in \iset_j(I)}\optcrors(I')> \optcrors(I)\cdot2^{c_g\cdot (\log m)^{3/4}\log\log m} +m\cdot\mu^{c_g}$.
\end{itemize}

As before, from \Cref{thm: main},  $\prob{\event'(I)}\le (1/16)^L\leq 1/(m^*)^4$.


Let $\event$ be the bad event that event $\event(I)$  or event $\event'(I)$ happened for any  instance $I\in \iset^*$. From the Union Bound and \Cref{cor: num of instances}, we get that $\prob{\event}\leq 1/(m^*)^2$.




We use the following immediate observation.

\begin{observation}\label{obs: leaf}
If Event $\event$ does not happen, then for every leaf vertex $v(I)$ of $T$ with $I=(G,\Sigma)$, either $|E(G)|\leq \mu^{c'}$; or $\optcrors(I)=0$; or $\optcrors(I)> |E(G)|^2/\mu^{c'}$.
\end{observation}


We use the following lemma to complete the proof of \Cref{thm: main_rotation_system}.

\begin{lemma}\label{lem: solution cost}
	If Event $\event$ does not happen, then  Algorithm $\algrec$ computes a solution for instance $I^*=(G^*,\Sigma^*)$ of cost at most $2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)$.
\end{lemma}
\begin{proof}
%First we show that, if $I=(G,\Sigma)$ is a leaf subinstance of $I^*$, then the algorithm computes a solution to instance $I$ of cost at most $\mu^{2c'}\cdot \optcrors(I)$. Indeed, if $\optcrors(I)=0$, then the algorithm returns a solution of cost $0$. Otherwise, $\optcrors(I)\geq 1$, and, if $|E(G)|\leq \mu^{c'}$, then the algorithm returns a trivial solution, whose cost is at most $|E(G)|^2\leq \mu^{2c'}\cdot \optcrors(I)$. Lastly, if $\optcrors(I)>|E(G)|^2/\mu^{c'}$, then, since the trivial solution $\phi'$ is considered by the algorithm, it returns a solution of cost at most $|E(G)|^2\leq \optcrors(I)\cdot \mu^{c'}$.
		Consider a non-leaf instance $I=(G,\Sigma)$, and let $\iset_1(I),\ldots,\iset_L(I)$ be families of subinstances of $I$ that the Algorithm \algrec computes. Recall that, for each $1\le j\le L$ with $\iset_j(I)\neq \emptyset$, the algorithm computes a solution $\phi_j$ to instance $I$, by first solving each of the instances in $\iset_j(I)$ recursively, and then combining the resulting solutions using Algorithm \algcombine. Eventually, the algorithm returns the best solution of $\set{\phi',\phi_1,\ldots,\phi_L}$, where $\phi'$ is the trivial solution, whose cost is at most  $|E(G)|^2$. We fix an index $1\leq j\leq L$, for which solution $\phi_j$ has the lowest cost, breaking ties arbitrarily. Note that the cost of the solution to instance $I$ that the algorithm returns is at most $\cro(\phi_j)$. We then \emph{mark} the vertices of $\set{v(I')\mid I'\in \iset_j(I)}$ in the tree $T$. We also mark the root vertex of the tree. 

Let $T^*$ be the subgraph of $T$ induced by all marked vertices. It is easy to verify that $T^*$ is a tree, and moreover, every leaf vertex of $T^*$ is also a leaf vertex of $T$. For a vertex $v(I)\in V(T^*)$, we denote by $h(I)$ the length of the longest path in tree $T^*$, connecting vertex $v(I)$ to any of its descendants in the tree. 
We use the following claim, whose proof is straightforward conceptually but somewhat technical; we defer the proof to \Cref{Appx: inductive bound proof}.

\begin{claim}\label{claim: bound by level}
Assume that Event $\event$ did not happen. Then there is a fixed constant $\tilde c>0$, such that, for every vertex $v(I)\in V(T^*)$, whose corresponding subinstance of $I^*$ is denoted by $I=(G,\Sigma)$, the cost of the solution that the algorithm computes for  $I$ is at most:
 $$2^{\tilde c\cdot h(I)\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{c'\cdot c_g}\cdot \optcrors(I)+(\log m^*)^{4c_g h(I)}\mu^{2c'\cdot \tilde c}\cdot|E(G)|.$$
\end{claim}


We are now ready to complete the proof of \Cref{lem: solution cost}. Recall that $h(I^*)=\dep(T^*)\leq \dep(T)\leq  \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$  from \Cref{obs: few recursive levels}. Therefore, from \Cref{claim: bound by level}, the cost of the solution that the algorithm computes for instance $I^*$ is bounded by:
%
\[
\begin{split}
& \text{ } 2^{O(\dep(T))\cdot (\log m^*)^{3/4}\log\log m^*}\cdot \mu^{O(1)}\cdot \optcrors(I^*)+(\log m^*)^{O(\dep(T))}\cdot\mu^{O(1)}\cdot m^*\\
\leq & \text{ } 2^{O((\log m^*)^{7/8})}\cdot \mu^{O(1)}\cdot \optcrors(I^*)+(\log m^*)^{O((\log m^*)^{1/8}/\log\log m^*) }\cdot\mu^{O(1)}\cdot m^*\\
\leq & \text{ } 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right),
\end{split}
\]
%
since $\mu=2^{O((\log m^*)^{7/8}\log\log m^*)}$.
\end{proof}



In order to complete the proof of \Cref{thm: main_rotation_system}, it is now enough to prove Theorem~\ref{thm: main}. The remainder of the paper is dedicated to the proof of \Cref{thm: main}.




\subsection{Proof of Theorem~\ref{thm: main} -- Main Definitions and Theorems} 

%\znote{constant $\interestconst$ to be replaced by an integer}\mynote{in the uninteresting instances part we have made some assumption about $b$ (possibly $b\geq 50$ but I'm not sure). When setting the value of $b$ please check and make sure that it is consistent.}
	
%\mynote{please switch "interesting/uninteresting" to "wide/narrow" throughout the whole paper (including intro)}
We classify subinstances of the input instance $I^*$ into \emph{wide} and \emph{narrow}, and provide different algorithms for decomposing instances of each of the two kinds. %We now define wide and narrow subinstances of $I^*$.
%\mynote{note that this definition has changed to only include one of the two cases. The subsequent observation shows that the other case also holds. I also eliminated "witness path set" because we use this notion in many other places and it is not really necessary here.}
Throughout this subsection, we use the parameter $\interestconst=50$.

%\mynote{Please go to Sec 9 where it uses this other property of uninteresting instances and add a pointer to the observation from there (e.g. the property now follows from the observation, not from the definition of the instances).}




\begin{definition}[Wide and Narrow Instances]
Let $I=(G,\Sigma)$ be an instance of \cnwrs with $|E(G)|=m$. We say that $I$ is a \emph{wide} instance, iff there is a vertex $v\in V(G)$, a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$, and a collection $\pset$  of at least $\floor{m/\mu^{\interestconst}}$ simple edge-disjoint cycles in $G$, such that every cycle $P\in \pset$ contains one edge of $E_1$ and one edge of $E_2$.
	If no such cycle set $\pset$ exists in $G$, then we say that $I$ is a \emph{narrow} instance.
\end{definition}




Note that there is an efficient algorithm to check whether a given instance $I$ of \cnwrs is wide, and, if so, to  compute the corresponding cycle set $\pset$, via standard algorithms for maximum flow. (For every vertex $v\in V(G)$, we can try all possible partitions $(E_1,E_2)$ of $\delta_G(v)$ with the required properties, as the number of such partitions is bounded by $|\delta_G(v)|^2$.)
We will use the following simple observation regarding narrow instances.

\begin{observation}\label{obs: narrow prop 2}
	If an instance $I=(G,\Sigma)$ of \cnwrs is narrow, then for every pair $u,v$ of distinct vertices of $G$, and any set $\pset$ of edge-disjoint paths connecting $u$ to $v$  in $G$,  $|\pset|\leq 2\ceil{m/\mu^{\interestconst}}+2$ must hold.
\end{observation}

\begin{proof}
	Assume for contradiction that $|\pset|>2\ceil{m/\mu^{\interestconst}}+2$, and denote $|\pset|=k$.
	Let $E'\subseteq \delta_G(v)$ be the set of all edges $e\in \delta_G(v)$, such that $e$ is the first edge on some path in $\pset$. We denote $E'=\set{e_1,\ldots,e_k}$, where the edges are indexed according to their ordering in the rotation $\oset_v\in \Sigma$. We also denote $\pset=\set{P(e_i)\mid 1\leq i\leq k}$, where path $P(e_i)$ contains the edge $e_i$ as its first edge. We can then compute a partition $(E_1,E_2)$ of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$. Additionally, we can ensure that $e_1,\ldots,e_{\ceil{k/2}}\in E_1$, while the remaining edges of $E'$ lie in $E_2$. For each $1\leq i\leq \ceil{m/\mu^{\interestconst}}$, we let $Q_i$ be the cycle obtained by concatenating the paths $P(e_i)$ and $P(e_{k-i+1})$. We can turn $Q_i$ into a simple cycle, by removing all cycles that are disjoint from vertex $v$ from it. It is then immediate to verify that cycle set $\set{Q_i\mid 1\leq i\leq \ceil{m/\mu^{\interestconst}}}$ has all the required properties to establish that instance $I$ is wide, a contradiction.
\end{proof}


\iffalse

\begin{definition}[Wide and Narrow Subinstances]
A subinstance $I=(G,\Sigma)$ of $I^*$ is an \emph{interesting} instance, iff there is a 
	collection $\pset$ of at least $m/\mu^{\interestconst}$ edge-disjoint paths in $G$, that we refer to as the \emph{witness path set for $I$}, such that one of the following holds:
	
	\begin{itemize} 
		\item either there are two distinct vertices $u,v\in V(G)$, such that every path in $\pset$ originates at $v$ and terminates at $u$; or 
		
		
		\item there is a single vertex $v\in V(G)$, and a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$. Every path in $\pset$ must contain an edge of $E_1$ as its first edge and an edge of $E_2$ as its last edge.
	\end{itemize}
	%
	If no such path set $\pset$ exists in $G$, then we say that $I$ is an \emph{narrow} instance.
\end{definition}
\fi


The proof of \Cref{thm: main} relies on the following two theorems. The first theorem deals with wide subinstances of $I^*$, and its proof appears in \Cref{sec: many paths}.




\mynote{The theorem has changed significantly. the rest of the proof needs to be updated.}

\begin{theorem}\label{lem: many paths}
	There is an efficient randomized algorithm, that, given a wide subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$, either returns FAIL, or computes $z=\ceil{\log m^*}$  collections $\iset_1,\ldots,\iset_z$ of subinstances of $I$, such that the following hold:
	
	\begin{itemize}
		%\item there is at least one index $1\leq j\leq z$ with $\iset_j\neq\emptyset$; \mynote{if we don't need this property then it can be removed}
		\item for all $1\leq j\leq z$,  $\sum_{I'=(G',\Sigma')\in \iset_j}|E(G')|\le |E(G)|$;
		\item for every instance $I'=(G',\Sigma')\in \bigcup_{j=1}^z\iset_j$, either $|E(G')|\le m/\mu$, or instance $I'$ is not wide;
		
		\item 
		there is an efficient algorithm called $\algcombine'$, that, given an index $1\leq j\leq z$, and a solution $\phi(I')$ to every instance $I'\in \iset_j$, computes a solution $\phi$ to instance $I$; and
		\item  if $\optcrors(I)\leq m^2/\mu^{c'}$ then, with probability at least $1-1/\mu^2$,  the algorithm does not return FAIL, and  there is an index $1\leq j\leq z$ for which all of the following hold:
		
		\begin{itemize}
			\item $\iset_j\neq \emptyset$;
			\item  $\sum_{I'\in \iset_j}\optcrors(I')\leq \optcrors(I)\cdot  (\log m)^{O(1)}$; and
			\item if algorithm $\algcombine'$ is given as input a solution $\phi(I')$ to each instance $I'\in \iset_j$, then the resulting solution $\phi$ to instance $I$ that it computes has cost at most: $\cro(\phi)\leq  \sum_{I'\in \iset_j}\cro(\phi(I')) + \optcrors(I)\cdot\mu^{O(1)}$.
		\end{itemize}
	\end{itemize}
\end{theorem}



The second theorem deals with narrow instances.


%\mynote{I replaced bound $\optcrors(I)<m^2/\left (\mu^{15}\cdot 2^{c(\log m)^{3/4}\log\log m}\right )$ with $\optcrors(I)<m^2/\mu^{16}$, because the latter bound is cleaner and simpler. I currently don't see a reason to prefer the old bound over it. I also replaced the probability of failure with $1/\mu^2$ instead of $1/\mu$. We could just repeat the algorithm $\mu$ times if needed.}

\begin{theorem}\label{lem: not many paths}
	There is an efficient randomized algorithm,  that,  given a narrow subinstance  $I=(G,\Sigma)$ of $I^*$, with $m=|E(G)|\geq \mu^{20}$, either  returns FAIL, or computes  a $\nu$-decomposition $\iset$ of $I$, for $\nu= 2^{O((\log m)^{3/4}\log\log m)}$,   such that, for every instance $I'=(G',\Sigma')\in \iset$, $|E(G')|\le m/\mu$. Moreover, if $\optcrors(I)<m^2/\mu^{16}$, then the probability that the algorithm returns FAIL is at most $1/\mu^2$.
\end{theorem}


The majority of the remainder of this paper is dedicated to the proof of the above theorem: we develop the central technical tools used in the theorem's proof in  \Cref{sec: guiding paths orderings basic disengagement} -- \Cref{sec: main disengagement}, and complete the proof in \Cref{sec: computing the decomposition}.
In the remainder of this section, we complete the proof of Theorem \ref{thm: main} using Theorems \ref{lem: many paths} and \ref{lem: not many paths}.


\iffalse
\mynote{restate the lemma in terms of $\alpha$-decomposition into subinstances}
\begin{lemma}\label{lem: not many paths}
	There is an efficient randomized algorithm,  that,  given a non-interesting subinstance  $I=(G,\Sigma)$ of $I^*$ with $|E(G)|=m\geq \mu^{10}$, either correctly certifies that $\optcrors(I)\geq \Omega(m^2/\mu^5)$, or computes  a collection $\iset$ of subinstances of $I$,  such that
	the following hold:
	
	\begin{itemize}
		\item for every instance $I'=(G',\Sigma')\in \iset$, $|E(G')|\le m/\mu$;
		\item  $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq O(m)$; and
		\item $\expect{\sum_{I'\in \iset}\optcrors(I')}\le \left (\optcrors(I)+|E(G)|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}$.
	\end{itemize}

 Moreover, there is an efficient algorithm, that, given, for each instance $I'\in \iset$, a feasible solution $\phi(I')$, computes a feasible solution $\phi$ for instance $I$, of cost $\cro(\phi)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$.
\end{lemma}

\fi

%Throughout, we assume that the constant $c'$ in the statement of \Cref{thm: main} and the constant $c_g$ in the definition of good collections of subinstances are both large enough so that $\min\set{c',c_g}>c+50$ holds, where $c$ is the constant from \Cref{lem: many paths}.

Recall that we are given an instance $I=(G,\Sigma)$, that is a subinstance of the input instance $I^*=(G^*,\Sigma^*)$, with $|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$. We denote $m=|E(G)|$. We compute the desired collection $\iset$ of subinstances of $I$ in two steps. 
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%
%%%%%%%%%


If instance $I$ is a narrow instance, then we skip the first step. We let $\iset'$ be a collection of subinstances of $I$, that consists of instance $I$ only. Assume now that $I$ is a wide instance. Then we execute Step 1, by applying the algorithm from \Cref{lem: many paths} to $I$. 
If the algorithm returns FAIL, then we terminate the algorithm and return FAIL as well.
Otherwise, let $\iset'$ be the resulting collection of subinstances of $I$.  Recall that we are guaranteed that,  for each instance $I'=(G',\Sigma')\in \iset'$, either $I'$ is a narrow instance, or $|E(G')|\le m/\mu$. Additionally, we are guaranteed that $\sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\le |E(G)|$;
and,  if 
$\optcrors(I)<m^2/\mu^{c'}$, then with probability at least $31/32$:
$$\sum_{I'\in \iset'}\optcrors(I')\leq 2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g},$$
%
for some constant $c_g$.
We say that a bad event $\event'_1$ happens if $\optcrors(I)\leq m^2/\mu^{c'}$, but: $$\sum_{I'\in \iset'}\optcrors(I')> 2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
From \Cref{lem: many paths},  $\prob{\event'_1}\leq 1/32$.
We say that a bad event $\event''_1$ happens if algorithm from \Cref{lem: many paths} returns FAIL when applied to $I$.
From \Cref{lem: many paths},  $\prob{\event''_1}\leq 1/\mu^2$.
Define the bad event $\event_1=\event'_1\cup \event''_1$, so $\prob{\event_1}\leq 1/31$.
This completes the first step of the algorithm.

We now describe the second step.
We start by partitioning the set  $\iset'$ of instances into two subsets: set $\iset_1'$ containing all instances $I'=(G',\Sigma')$ with $|E(G')|\leq m/\mu$, and set $\iset_2'$ containing all remaining instances, that must be narrow.
We use the following simple observation.

\begin{observation}\label{obs: optbound for narrow}
	If $\optcrors(I)\leq m^2/\mu^{c'}$, and Event $\event_1$ does not happen, then for every instance $I'=(G',\Sigma')\in \iset_2'$, $\optcrors(I')\leq |E(G')|^2/\mu^{16}$.
	\end{observation}
\begin{proof}
Assume that  $\optcrors(I)\leq m^2/\mu^{c'}$, and that Event $\event_1$ does not happen.  Then: 
%
$$\sum_{I'\in \iset'}\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
%	
Consider now some instance $I'=(G',\Sigma')\in \iset_1'$. We then get that: 
%
$$\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m}\cdot \optcrors(I)+m\cdot\mu^{c_g}\leq \mu\cdot \optcrors(I)+m\cdot\mu^{c_g},$$ 
%	
since $\mu=2^{c^*(\log m^*)^{7/8}\log\log m^*}$.
	
Since $m\geq \mu^{c'}$, and since we can assume that $c'$ is a large enough constant, $\mu^{c_g}\leq m/\mu^{c'/2}$. Further, since we have assumed that $\optcrors(I)\leq m^2/\mu^{c'}$, and since $|E(G')|\geq m/\mu$ (since instance $I'=(G',\Sigma')$ belongs to set $\iset_2'$), we get that:
%	
$$\optcrors(I')\leq m^2/\mu^{c'-1}+m^2/\mu^{c'/2}\leq |E(G')|^2/\mu^{16},$$
%		
assuming that $c'$ is large enough.
\end{proof}


Next, we process every instance $I'\in \iset_2'$  one by one. Notice that for each such instance $I'=(G',\Sigma')$, $|E(G')|\geq m/\mu\geq \mu^{20}$ must hold, since $m\geq \mu^{c'}$. When instance $I'$ is processed, we apply the algorithm from \Cref{lem: not many paths} to it. If the algorithm returns FAIL, then we terminate the algorithm and return FAIL as well. Otherwise, we obtain a collection $\iset(I')$ of subinstances of $I'$ (and hence of $I$). If the algorithm did not terminate with a FAIL, then we obtain the final collection  $\iset^*=\iset_1'\cup \left (\bigcup_{I'\in \iset_2'}\iset(I')\right)$ of subinstances of $I$ that the algorithm returns. 
This completes the description of the algorithm. 




In order to analyze it, we first show that, if  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/16$.

\begin{observation}\label{obs: fail prob}
	If  $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/16$.
\end{observation}

\begin{proof}
	For an instance $I'=(G',\Sigma')\in \iset'$, we say that a bad event $\event(I')$ happens if the algorithm from \Cref{lem: not many paths}, when applied to $I'$, returns FAIL. From \Cref{lem: not many paths}, if 
	$\optcrors(I')<|E(G')|^2/\mu^{16}$, then the probability that the algorithm returns FAIL is at most $1/\mu^2$. Therefore, from \Cref{obs: optbound for narrow}, if Event $\event_1$ does not happen, then $\prob{\event(I')}\leq 1/\mu^2$. Let $\event_2$ be the bad event that $\event(I')$ happens for any instance $I'\in \iset'_2$.  Since every instance $I'\in \iset_2'$ contains at least $m/\mu$ edges, while, as we have established already, the total number of edges in all instances in $\iset'$
	is at most $m$, we get that $|\iset'_2|\leq \mu$. From the Union Bound, assuming that the constant $c^*$ in the definition of the parameter $\mu$ is large enough, $\prob{\event_2\mid \neg \event_1}\leq 1/100$. Clearly, $\prob{\event_2}\leq \prob{\event_1}+\prob{\event_2\mid \neg \event_1}\leq 1/31+1/100< 1/20$. Note that, if events $\event_1$ and $\event_2$ do not happen, then algorithm may not return FAIL. We conclude that, if $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then the algorithm returns FAIL with probability at most $1/20<1/16$.
\end{proof}

We define the bad event $\event=\event_1\cup \event_2$, where event $\event_2$ is defined in the proof of above observation. From the above discussion $\prob[]{\event}\le 1/20$.

Fron now on we assume that the algorithm did not return FAIL.
Recall that \Cref{lem: not many paths} gurantees that, for every instance $I'=(G',\Sigma')\in \iset_2'$, for every subinstance $I''=(G'',\Sigma'')\in \iset(I')$,  $|E(G'')|\leq |E(G')|/\mu\leq m/\mu$ holds. Therefore, for every instance $I''=(G'',\Sigma'')\in\iset^*$, $|E(G'')|\leq m/\mu$ must hold.
Additionally, from the definition of a $\nu$-decomposition, we are guaranteed  that for all $I'=(G',\Sigma')\in \iset_2'$, $\sum_{I''=(G'',\Sigma'')\in \iset(I')}|E(G'')|\leq |E(G')|\cdot (\log (|E(G')|)^{O(1)}\leq |E(G')|\cdot (\log m)^{O(1)}$.
Moreover, since $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$, we get that:

$$\sum_{I''=(G'',\Sigma'')\in \iset^*}|E(G'')|\leq \sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\cdot (\log m)^{O(1)}\leq m\cdot(\log m)^{O(1)}.$$ 








Next, we provide Algorithm \algcombine. 

\begin{claim}\label{claim: combine drawings}
	There is an efficient algorithm, called \algcombine, that, given a solution $\phi(I'')$ to each instance $I''\in \iset^*$, computes a solution $\phi(I)$ to instance $I$, of cost at most $O(\sum_{I''\in \iset^*}\cro(\phi(I''))) +(\optcrors(I)+|E(G)|)\cdot\mu^{O(1)}$.
\end{claim}
\begin{proof}
We construct the solution $\phi(I)$ to instance $I$ in two steps.

In the first step, we compute a solution $\phi(I')$ to each instance $I'\in \iset'_2$, as follows. Consider any such instance $I'=(G',\Sigma')\in \iset'_2$. Recall that we are given, for each instance $I''\in \iset(I')$, a solution $\phi(I'')$. Recall also that $\iset(I')$ is a $\nu$-decomposition  of $I'$. We apply the efficient algorithm $\alg(\iset(I'))$ from the definition of $\nu$-decompositions of instances to the drawings $\set{\phi(I'')}_{I''\in \iset(I')}$, to obtain a feasible solution $\phi(I')$ for instance $I'$, of cost $\cro(\phi(I'))\leq O\left (\sum_{I''\in \iset(I')}\cro(\phi(I''))\right )$.


We have now obtained a solution $\phi(I')$ to every instance $I'\in \iset'$. In the second step, we apply the algorithm in the third bullet of the statement of \Cref{lem: many paths}  to these solutions, to obtain a solution $\phi(I)$ to instance $I$.
The cost of the solution is bounded by:
%
\[\begin{split}   
\cro(\phi(I)) &\leq \sum_{I'\in \iset'}\cro(\phi(I')) + (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq  \sum_{I'\in \iset'_1}\cro(\phi(I')) +\sum_{I'\in \iset'_2}\cro(\phi(I'))+ (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq \sum_{I'\in \iset'_1}\cro(\phi(I')) +\sum_{I'\in \iset'_2}O\left (\sum_{I''\in \iset(I')}\cro(\phi(I''))\right )+ (m+\optcrors(I))\cdot\mu^{O(1)}\\
&\leq O\left (\sum_{I''\in \iset^*}\cro(\phi(I'))\right ) +(m+\optcrors(I))\cdot\mu^{O(1)}.
\end{split}
\]
\end{proof}


 In order to complete the proof of \Cref{thm: main}, it is now enough to prove the following observation.
 
\begin{observation}\label{obs: bound sum of opts}
	If $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $$\sum_{I''\in \iset^*}\optcrors(I'')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}.$$
\end{observation}


\begin{proof} 
Assume that $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$. Recall that, if Event $\event$ does not happen, then:
%
$$\sum_{I'\in \iset'}\optcrors(I')\leq  2^{c_g(\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{c_g}.$$ 
%
From the definition of a $\nu$-decomposition, for every instance $I'=(G',\Sigma')\in \iset'_2$, 
%
\[\expect{\sum_{I''\in \iset(I')}\optcrors(I'')}\le \left (\optcrors(I')+|E(G')|\right )\cdot \nu \leq \left (\optcrors(I')+|E(G')|\right ) \cdot 2^{O((\log m)^{3/4}\log\log m)},\]
%
Therefore, if $\event$ does not happen, then: 
%
\[ 
\begin{split}
\expect{\sum_{I''\in \iset^*}\optcrors(I'')}&\leq \sum_{I'\in \iset'_1}\optcrors(I') +\sum_{I'\in \iset'_2}\expect{\sum_{I''\in \iset(I')}\optcrors(I'')}\\
&\leq  \sum_{I'\in \iset'_1}\optcrors(I')+\sum_{I'=(G',\Sigma')\in \iset'_2}\left (\optcrors(I')+|E(G')|\right ) \cdot 2^{O((\log m)^{3/4}\log\log m)}\\
&\leq \sum_{I'=(G',\Sigma')\in \iset'}\left (\optcrors(I')+|E(G')|\right )\cdot 2^{O((\log m)^{3/4}\log\log m)}\\
&\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}.
\end{split} \]
%
We denote this expectation by $\eta'$. Let $\hat \event$ be the bad event that 
$\sum_{I''\in \iset^*}\optcrors(I'')>100\eta'$. From Markov's inequality, $\prob{\hat \event\mid \neg\event}<1/100$. Note that, if neither of the events $\hat \event,\event$ happens, then we are guaranteed that $\sum_{I''\in \iset^*}\optcrors(I'')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \optcrors(I)+m\cdot\mu^{O(1)}$. The probability that either one of these events happens is bounded by $\prob{\event}+\prob{\hat \event\mid \neg\event}\leq 1/20+ 1/100\leq 1/16$. We conclude that, If $\optcrors(I)\leq |E(G)|^2/\mu^{c'}$, then with probability at least $15/16$: $$\sum_{I''\in \iset^*}\optcrors(I'')\leq \optcrors(I)\cdot2^{O((\log m)^{3/4}\log\log m)} +m\cdot\mu^{O(1)}.$$
\end{proof}





%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%Only old stuff below this

%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
\iffalse
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
%-----------------------------------
Moreover, we are guaranteed that, 
%
\[\expect[]{\sum_{I''\in \iset^*}\optcrors(I'')}\leq  \nu''\cdot \bigg( \sum_{I'=(G',\Sigma')\in \iset'}\big(\optcrors(I')+|E(G')|\big)\bigg ). \]
%
Assume that event $\event$ did not happen. Then,
\[
\begin{split}
\expect[]{\sum_{I''\in \iset^*}\optcrors(I'')} &\text{ }\leq  \nu''\cdot \expect[]{ \sum_{I'=(G',\Sigma')\in \iset'}\big(\optcrors(I')+|E(G')|\big)}\\
&\text{ }\leq  \nu''\cdot \expect[]{\sum_{I'=(G',\Sigma')\in \iset'}\optcrors(I')}+\nu''\cdot\bigg(\sum_{I'=(G',\Sigma')\in \iset'}|E(G')|\bigg)\\
&\text{ }\leq  \nu''\cdot \bigg(\nu'\cdot\optcrors(I)+|E(G)|\cdot \mu^c\bigg)+\nu''\cdot(\log|E(G)|)^{O(1)}\cdot|E(G)|\\
&\text{ }\leq  (\nu'\nu'')\cdot \optcrors(I)+O(\nu''\cdot\mu^c)\cdot|E(G)|.
\end{split} \]
Let $\nu=\nu'\cdot\nu''$.
Since $\nu',\nu''=2^{O((\log m)^{3/4}\log\log m)}$, $\nu=\nu'\cdot\nu''=2^{O((\log m)^{3/4}\log\log m)}$.
Since $\mu^{c_g}>\nu''\cdot\mu^{c}$, with probability at least $9/10$, the resulting collection $\iset^*$ of instances is perfect for $I$. 



\fi
\iffalse

 In order to do so,  
@@@@ we compute a denote by $\iset(I')=\set{I''_1,\ldots,I''_k}$ the set of subinstances obtained by applying the algorithm from \Cref{lem: not many paths} to it.  From the definition of a $\nu''$-decomposition, we are also given an efficient algorithm $\alg(\iset(I'))$, that takes as input a solution of each instance in $\iset(I')$ and returns a solution of $I'$. We apply this algorithm to the solutions $\set{\phi(I''_i)}_{1\le i\le k}$ to the subinstances in $\iset(I')$ and let $\phi(I')$ be the solution we get. From the definition of a $\nu''$-decomposition, there exists some universal constant $c^*>0$, such that $\cro(\phi(I'))\le c^*\cdot \sum_{1\le i\le k}\cro(\phi(I''_i))$.

Clearly, after the first step, we have obtained, for each subinstance $I'\in \iset'$, a solution $\phi(I')$ to instance $I'$.
%
Recall that, in \Cref{lem: many paths} we are also given an efficient algorithm (that we denote by $\alg'(\iset')$), that, given, for every instance $I'\in \iset'$, a solution $\phi(I')$ to instance $I'$, computes a solution $\phi$ to instance $I$, with $\cro(\phi)\leq \big(\sum_{I'\in \iset'}\cro(\phi(I'))\big)+ (m+\optcrors(I))\cdot\mu^c$.
In the second step, we simply apply the algorithm to the set $\set{\phi(I')}_{I'\in \iset'}$ of solutions and let $\phi(I)$ be the solution to instance $I$ that we obtain. From \Cref{lem: many paths},
\[
\begin{split}
\cro(\phi)\leq & \text{ } \bigg(\sum_{I'\in \iset'}\cro(\phi(I'))\bigg)+ (m+\optcrors(I))\cdot\mu^c\\
\leq & \text{ } c^*\cdot \bigg(\sum_{I''\in \iset^*}\cro(\phi(I''))\bigg)+ (m+\optcrors(I))\cdot\mu^c.
\end{split}
\]
Now \Cref{thm: main} follows by setting $c_g$ to be a contant such that $c_g> \max\set{c^*, c}$.
\fi





\iffalse{previous algorithm algcombine}
Consider the partitioning tree $T^*$ that is obtained from the partitioning tree $T$ in the first Stage, by adding, for each leaf $v(I')$ of $T$ with $I'\in \iset'_2$ and for each instance $I''\in \iset(I')$, a new vertex $v(I'')$ and an edge connecting it to $v(I')$. Clearly, the instances in $\iset^*$ correspond to leaves in $T^*$. Assume now that we are given, for each instance $I'$ such that $v(I')$ is a leaf in $T^*$, a solution $\phi(I')$ to instance $I'$. We will construct a drawing of instance $I$ in two steps as follows.

In the first step, for each instance $I'\in \iset'_2$, we denote by $\iset(I')=\set{I''_1,\ldots,I''_k}$ the set of subinstances obtained by applying the algorithm from \Cref{lem: not many paths} to it. Recall that, from the definition of a $\nu$-decomposition in \Cref{lem: not many paths} we are also given an efficient algorithm $\alg(\iset(I'))$, that takes as input a solution of each instance in $\iset(I')$ and returns a solution of $I'$. We apply this algorithm to the solutions $\set{\phi(I''_i)}{1\le i\le k}$, and let $\phi(I')$ be the solution we get. From the definition of a $\nu$-decomposition, $\cro(\phi')\le c^*\cdot \sum_{1\le i\le k}\cro(\phi(I''_i))$ for some universal constant $c^*$.

In the second step, we look at the partitioning tree $T$ of Stage 1, and note that now we have, for each instance $I'$ such that $v(I')$ is a leaf in $T$, a solution $\phi(I')$ of $I'$. We now construct a solution for every instance that corresponds to a vertex in $T$ in a bottom-up fashion as follows. In each iteration, we take a vertex $v(I')$ in $T$ with children $v(I''_1),v(I''_2)$ in $T$, such that we have not yet computed a solution of instance $I'$, but we have already computed a solution $\phi(I''_1)$ for instance $I''_1$ and a solution $\phi(I''_2)$ for instance $I''_2$. Note that it is not hard to see that such a vertex has to exist in each iteration.
We not apply the solution-combining algorithm from \Cref{lem: many paths} to the solutions $\phi(I''_1), \phi(I''_2)$, and obtain a solution $\phi(I')$ to instance $I'$. This completes the description of an iteration. We keep performing iterations until we obtain a solution $\phi(I)$ to the input instance $I$.

It remains to upper bound $\cro(\phi(I))$. Recall that at the end of the first step, we have obtained, for each instance $I'\in \iset'$ that corresponds to a leaf in $T$, a solution $\phi(I')$ to $I'$, such that $\sum_{I'\in \iset'}\cro(\phi(I'))\le c^*\cdot\sum_{I'\in \iset^*}\cro(\phi(I'))$. Recall that the depth of tree $T$ is at most $2\mu^{11}$.
Moreover, for each non-leaf instance $I'=(G',\Sigma')$ of $T$, if we denote by $I''_1,I''_2$ the instances that correspond to its children in $T$, then $\cro(\phi(I'))\le \cro(\phi(I''_1))+\cro(\phi(I''_2))+(\optcrors(I')+|E(G')|)\cdot \mu^c$.

Via similar arguments as in the proof of \Cref{cor: stage 1} we can show that, for each $1\le i\le \floor{2\mu^{11}}$, if we denote by $\iset'_i$ be the set of subinstances obtained after iteration $i$, then
\[
\sum_{I'\in \iset'_{i+1}}\optcrors(I')+m\cdot \mu^{c+13}\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12}),
\]
Therefore, 
\[
\sum_{I': v(I')\in V(T)}\optcrors(I')+m\cdot \mu^{c+13}\leq 4\cdot \bigg(\optcrors(I)+  m\cdot  \mu^{c+13}\bigg).
\]
It follows that 
\[
\begin{split}
\cro(\phi(I)) 
& \le \sum_{I' \in \iset'} \cro(\phi(I')) +\dep(T)\cdot O\bigg(\sum_{I \notin \iset'} \big(\optcrors(I)+|E(G)|\cdot \mu^{c+13}\big)\bigg)\\ 
& \le c^*\cdot \sum_{I' \in \iset^*} \cro(\phi(I')) +8\cdot\bigg(\mu^{11}\cdot \optcrors(I)+\mu^{11}\cdot \mu^{c+13}\cdot |E(G)|\big)\bigg).
\end{split}
\]
Now \Cref{thm: main} follows by setting $c_g$ to be a contant such that $c_g\ge \max\set{c^*, c+25}$.
\fi







%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%

\iffalse

It is easy to verify that $T^*$ is 
We say that the instances in $\iset_i(I)$ are \emph{critical subinstance} to instance $I$, iff $\cro(\phi_i)=\min\set{\cro(\phi_1),\ldots, \cro(\phi_L),|E(G)|^2}$.
Consider now the tree $T^*$, which is the subtree of $T$ induced by $v(I^*)$ and all vertices $v(I)$ such that the instance $I$ is critical.
It is easy to see that every leaf of $T^*$ is also a leaf of $T$.
Let $I$ be an instance with $v(I)\in V(T^*)$ and let $I_1,\ldots,I_k$ be its critical subinstances, where $I_i=(G_i,\Sigma_i)$ for each $i$.
From \Cref{thm: main} and since the event $\event$ does not happen, 
$\sum_{1\le i\le k}\optcrors(I_i)\leq \optcrors(I)\cdot \nu +|E(G)|\cdot\mu^{c_g}$ and $\sum_{1\le i\le k}|E(G_i)|\leq |E(G)|\cdot (\log m^*)^{c_g}$ (where we have used the fact that $|E(G)|\le m^*$).
Therefore, since $(\log m^*)^{c_g}<\nu$,
\[
\sum_{1\le i\le k}\bigg(\optcrors(I_i)+|E(G_i)|\cdot \mu^{c_g}\bigg)\leq \bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg)\cdot \nu.
\]
It is easy to see that, if we denote by $\iset^{(j)}$ the set of all critical instances at recursive level $j$, then 
\[
\sum_{I=(G,\Sigma)\in \iset^{(j)}}\bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg)\leq \bigg(\optcrors(I^*)+|E(G^*)|\cdot \mu^{c_g}\bigg)\cdot \nu^{j}.
\]
It follows that, if we denote by $\iset^*$ the set of all critical subinstances, then 
\[
\begin{split}
\sum_{I=(G,\Sigma)\in \iset^{^*}}\bigg(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\bigg) & \leq \bigg(\optcrors(I^*)+|E(G^*)|\cdot \mu^{c_g}\bigg)\cdot 2^{O((\log m^*)^{7/8}\log\log m^*)}\\
& = 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split}
\]


Consider now any instance $I=(G,\Sigma)$ with $v(I)\in V(T^*)$. We first denote $\cost^*(I)=\mu^{c_g}\cdot\optcrors(I)+|E(G)|\cdot \mu^{2c_g}$. From the above discussion,
\[
\sum_{I=(G,\Sigma)\in \iset^{^*}}\cost^*(I) \leq 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\]
We then define the \emph{height} of $I$, denoted by $h(I)$, to be the largest distance from $v(I)$ to a descendant vertex of $v(I)$ in the tree $T^*$. In particular, if $v(I)$ is a leaf in $T^*$, then $h(I)=0$, and, from \Cref{obs: few recursive levels}, for every non-leaf subinstance $I$, $h(I)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$ always holds.
For an instance $I'$ such that vertex $v(I')$ is a descendant of vertex $v(I)$ in $T^*$, we write $I'\prec I$.


We prove by induction on $h(I)$ that the value of the solution $\phi(I)$ that $\algrec(I)$ computes satisfies that 
$$\cro(\phi(I))\le \mu^{2c'}\cdot\cost^*(I)+\mu^{2c'}\cdot\sum_{I' \prec I} \cost^*(I')\cdot c_g^{h(I)-h(I')}.$$ 
The induction base is when $h(I)=0$, so $v(I)$ is a leaf vertex of $T$. We have shown that the claim holds in this case.
%
Let $I=(G,\Sigma)$ be a non-leaf subinstance with $v(I)\in V(T^*)$ and let $I_1,\ldots,I_k$ be its critical subinstances. If we denote by $\phi(I)$ the drawing of $I$ returned by the algorithm \algrec, and similarly we define drawings $\set{\phi(I_i)}_{1\le i\le k}$, then from \Cref{thm: main}, 
\[
\cro(\phi(I)) \le  c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i))+ \bigg(\optcrors(I)+|E(G)|\bigg)\cdot \mu^{c_g} \le \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i)).
\]
Note that for each $1\le i\le k$, $h(I_i)\le h(I)-1$. Therefore, from the induction hypothesis,
\[
\begin{split}
\cro(\phi(I)) & \leq \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\cro(\phi(I_i))\\
& \le  \cost^*(I)+c_g\cdot \sum_{1\le i\le k}\bigg(\mu^{2c'}\cdot\cost(I_i)+\mu^{2c'}\cdot\sum_{I' \prec I_i} \cost^*(I')\cdot c_g^{h(I_i)-h(I')}\bigg)\\
& \le  \mu^{2c'}\cdot\cost^*(I)+ \mu^{2c'}\cdot\sum_{1\le i\le k}\bigg(c_g\cdot\cost(I_i)+\sum_{I' \prec I_i} \cost^*(I')\cdot c_g^{h(I_i)-h(I')+1}\bigg)\\
& \le  \mu^{2c'}\cdot\cost^*(I)+ \mu^{2c'}\cdot\sum_{I'\prec I} \cost^*(I')\cdot c_g^{h(I)-h(I')}.
\end{split}
\]
Therefore, since $h(I^*)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$, we get that for each $I'\in \iset^*$, $c_g^{h(I^*)-h(I')}\le \mu$, and so
\[
\begin{split}
\cro(\phi(I^*))\le & \text{ } \mu^{2c'}\cdot\cost^*(I^*)+\mu^{2c'}\cdot\sum_{I' \prec I} \cost^*(I')\cdot c_g^{h(I^*)-h(I')}\\
\le & \text{ } 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split} 
\]



\fi





%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\iffalse
Therefore, if we denote by $\iset^{**}$ the set of all subinstances $I$ such that $v(I)$ is a leaf of tree $T^*$, then
\[
\begin{split}
\sum_{I\in \iset^*} \cro(\phi(I)) 
& \le \dep(T)\cdot\bigg(\sum_{I\in \iset^{**}} \cro(\phi(I)) +\sum_{I=(G,\Sigma)\in (\iset^{*}\setminus \iset^{**})} \big(\optcrors(I)+|E(G)|\cdot \mu^{c_g}\big)\bigg)\cdot \mu^{c_g}\\ 
& =\mu^{O(c_g)}\cdot \bigg(\mu^{2c'}\cdot\sum_{I\in \iset^{**}} \optcrors(I)+ 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)
\bigg)\\
& = 2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right).
\end{split}
\]
And since $\cro(\phi(I^*))\le \sum_{I\in \iset^{^*}} \cro(\phi(I)) + \bigg(\optcrors(I^*)+|E(G^*)|\bigg)\cdot \mu^{c_g}$, it follows that $\cro(\phi(I^*))=2^{O((\log m^*)^{7/8}\log\log m^*)}\cdot \left(\optcrors(I^*)+|E(G^*)|\right)$.

\fi
\iffalse
\znote{cannot prove by induction, need to re-write from here}


%Consider now any vertex $v(I)$ in tree $T^*$. The \emph{height of $I$}, denoted by $h(I)$, is the largest distance from $v(I)$ to a descendant vertex of $v(I)$ in the tree $T$. In particular, if $I$ is a leaf subinstance, then $h(I)=0$, and, from \Cref{obs: few recursive levels}, for every non-leaf subinstance $I$, $h(I)\le \frac{(\log m^*)^{1/8}}{c^*\log\log m^*}$ always holds.





We prove by induction on $h(I)$ that the value of the solution $\phi(I)$ that $\algrec(I)$ computes satisfies that $\cro(\phi(I))\le (\optcrors(I)+|E(G)|)\cdot \mu^{c_g}\cdot \nu^{h(I)}$. The induction base is when $h(I)=0$, so $v(I)$ is a leaf vertex of $T$. We have shown that the claim holds in this case.


Consider now some instance $I=(G,\Sigma)$ with $h(I)>0$. Assume first that $\optcrors(I)> |E(G)|^2/\mu^{64}$. Recall that the algorithm \algrec considers a trivial solution $\phi'$ to instance $I$, of cost at most $|E(G)|^2$. Since the algorithm eventually returns the best of the considered solutions, the cost of the solution that it returns may not be higher than $|E(G)|^2\leq \optcrors(I)\cdot \mu^{64}$. 

Therefore, we assume that $\optcrors(I)\leq |E(G)|^2/\mu^{64}$ from now on. Since we have assumed that Event $\event$ did not happen, neither did $\event(I)$. Therefore, there is an instance $1\leq i\leq L$, such that the family $\iset_i(I)$ of instances is a perfect family for instance $I$. In particular, from the definition of a perfect family, we have that
%
$\sum_{I'\in \iset_i(I)}\optcrors(I')\leq \optcrors(I)\cdot \nu +|E(G)|\cdot\mu^{c_g}$.
%and since $m\le m^*$,
%$$m^*\cdot \mu^{c_g}+\sum_{I'\in \iset_i(I)}\optcrors(I')\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot\bigg(m^*\cdot \mu^{c_g}+ \optcrors(I)\bigg),$$
%
Using the induction hypothesis, if we denote by $\phi(I')$ the solution that the algorithm computes for each instance $I'\in \iset_i(I)$, then:
%
%	
\[
\begin{split}
\sum_{I'=(G'\Sigma')\in \iset_i(I)}\cro(\phi(I'))\leq & \sum_{I'=(G'\Sigma')\in \iset_i(I)}\bigg(\optcrors(I')\cdot \nu^{h(I)-1}+|E(G')|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\bigg)\\
\leq & \sum_{I'=(G'\Sigma')\in \iset_i(I)}\optcrors(I')\cdot \nu^{h(I)-1}+\sum_{I'=(G'\Sigma')\in \iset_i(I)}|E(G')|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\bigg(\optcrors(I)\cdot\nu+|E(G)|\cdot \mu^{c_g} \bigg)\cdot \nu^{h(I)-1} + c_g\cdot |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\optcrors(I)\cdot \nu^{h(I)} + (c_g+1)\cdot |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)-1}\\
\leq & \text{ }\optcrors(I)\cdot \nu^{h(I)} + |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)}.\\
\end{split}
\]
%
Let $\phi$ be the solution to instance  $I$ obtained by applying Algorithm \algcombine to solutions $\phi(I')$ to instances $I'\in \iset_i(I)$. Then, from \Cref{thm: main}, and since we can assume that $c_g$ is a large enough constant, we are guaranteed that:
%
\[
\begin{split}
\cro(\phi) &\leq  \bigg(\sum_{I'\in \iset}\cro(\phi(I')) \bigg) + (\opt(I)+|E(G)|)\cdot \mu^{c_g} \\
&\leq \optcrors(I)\cdot \nu^{h(I)} + |E(G)|\cdot \mu^{c_g}\cdot \nu^{h(I)}+ (\opt(I)+|E(G)|)\cdot \mu^{c_g}\\
&\leq \optcrors(I)\cdot (\nu^{h(I)}+\mu^{c_g}) + |E(G)|\cdot \mu^{c_g}\cdot (\nu^{h(I)}+1)
\end{split}
\]

% 
Since $h(I^*)\leq \frac{1}{c^*}\sqrt{\frac{\log m^*}{\log\log m^*}}$, we conclude that the cost of the solution $\phi^*$ that the algorithm computes for instance $I^*$ is bounded by:
\[
\begin{split}
(\optcrors(I)+m^*)\cdot \mu^{O(1)}\cdot (\log m)^{\sqrt{\log m^*/\log\log m^*}}&
\leq (\optcrors(I)+m^*)\cdot \mu^{O(1)}\cdot 2^{\sqrt{\log m^*\log\log m^*}}\\ &\leq (\optcrors(I)+m^*)\cdot \mu^{O(1)}. 
\end{split} \]
\fi%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%This completes the proof of \Cref{lem: solution cost}.



\iffalse{backup: previous stage 1}
\paragraph{Stage 1.}
We initialize the set $\iset$ to contain a single instance $I=(G,\Sigma)$. The first stage continues as long as there is any instance $\hat I=(\hat G,\hat \Sigma)\in \iset$, that is an interesting subinstance of $I$, with $|E(\hat G)|>|E(G)|/\mu$. The first stage consists of iterations, where in every iteration we start with an interesting subinstance $\hat I= (\hat G,\hat \Sigma)\in \iset$ with $|E(\hat G)|>m/\mu$. 
We apply the algorithm from \Cref{lem: many paths} to instance $\hat I$, 
obtaining two new instances $\hat I'=(\hat G',\hat \Sigma'),\hat I''=(\hat G'',\hat \Sigma'')$. We then replace $\hat I$ with $\hat I',\hat I''$ in $\iset$, and continue to the next iteration. Let $i$ denote the index of the current iteration. 

We say that the bad event $\event_i$ happens if (i) $|E(\hat G)|>\mu^{39}$; (ii) $\optcrors(\hat I)<|E(\hat G)|^2/\mu^{40}$; and (iii) $\optcrors(\hat I')+\optcrors(\hat I'') > \optcrors(\hat I) \cdot(1+1/\mu^{12})+m \cdot \mu^{c}$. From \Cref{lem: many paths}, the probability that $\event_i$ happens is bounded by $1/(40\mu^{11})$.

This completes the description of the algorithm for Stage 1. In order to analyze it, it is convenient to define a partitioning tree $T$ associated with it. 
For every instance $\hat I$ that ever belonged to set $\iset$ over the course of the Stage 1 algorithm, we add a vertex $v(\hat I)$ to the tree. If the algorithm from \Cref{lem: many paths} was applied to instance $\hat I$, producing two new instances $\hat I'$ and $\hat I''$, then vertices $v(\hat I'),v(\hat I'')$ become children of vertex $v(\hat I)$ in the tree. The root of the tree is the vertex $v(I)$.



We say that bad event $\event$ happens if bad event $\event_i$ happens for any iteration $i\leq 4\mu^{11}$ of Stage 1. From the union bound over all $1\le i\leq 4\mu^{11}$, we get that $\Pr[\event]\le 1/10$. 

Let $T'$ be the subtree of $T$ that is induced by all vertices $v(\hat I)$, such that $\hat I$ belonged to $\iset$ at some point before the completion of iteration $\ceil{2\mu^{11}}$.
Assume now that bad event $\hat \event$ did not happen. Since we only apply the algorithm from \Cref{lem: many paths} to instances $(\hat G,\hat \Sigma)$ with  $|E(\hat G)|>|E(G)|/\mu$, every instance $\hat I'=(\hat G',\hat \Sigma')$ with $v(I')\in T'$ has $|E(\hat G')|\geq |E(G)|/\mu^{11}$. But then the number of the leaf vertices in tree $T'$ is bounded by $\mu^{11}$, and the total number of vertices in tree $T'$ must be bounded by $2\mu^{11}$, since every inner vertex of $T'$ has at least two children. 
This can only happen if the algorithm terminates before the $\floor{2\mu^{11}}$-th iteration. Therefore, if Event $\event$ does not happen, the algorithm has fewer than $2\mu^{11}$ iterations. %Therefore, for every instance $\hat I=(\hat G,\hat Sigma)$ to which 
Moreover, since every instance $\hat I=(\hat G,\hat \Sigma)$ that ever belonged to $\iset$, $|E(\hat G)|\geq |E(G)|/\mu^{11}$ holds, and since we are guaranteed that $|E(G)|\geq \mu^{c'}\geq \mu^{50}$, we conclude that $|E(\hat G)|\geq \mu^{39}$ must hold.
%\iffalse
%Let $\iset'$ be the set of subinstances of $I$ obtained at the end of Stage 1. Equivalently, $\iset'$ contains every instance $I'$ that is a leaf instance. 
We use the following claim.


\begin{claim}\label{claim: few crossings in each instance}
	If event $\event$ did not happen, then for every instance $\hat I=(\hat G,\hat \Sigma)$ that ever belonged to the set $\iset$, $\optcrors(\hat I)\leq |E(\hat G)|^2/\mu^{40}$.
\end{claim}

\begin{proof}
	We say that a vertex $v(\hat I)$ lies at level $\ell$ of the tree $T$ iff the distance from $v(\hat I)$ to the root $v(I)$ of the tree is $\ell$. We will prove that, for all $0\leq \ell \leq \floor{2\mu^{11}}$, for every vertex $v(\hat I)$ lying at level $\ell$ of the tree $T$, with $\hat I=(\hat G,\hat\Sigma)$, 
	\begin{equation}
	\label{eqn: induction}
	\optcrors(\hat I)\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+m\cdot\ell\cdot\mu^{c+13},
	\end{equation}
	
	The proof is by induction on $\ell$. 
	The base case is when $\ell=0$, and $\hat I$ is the input instance $I=(G,\Sigma)$. Recall that, from the statement of \Cref{thm: main}, $\optcrors(G,\Sigma)\leq m^2/\mu^{63}\leq m^2/\mu^{40}$ as required, and it is immediate to verify that the inequality \ref{eqn: induction} holds. 
	Consider now some integer $0\leq \ell \leq \floor{2\mu^{11}}$. We assume that the claim holds for all integers below $\ell$, and prove it for integer $\ell$. Let $\hat I'=(\hat G',\hat \Sigma')$ be any instance, whose corresponding vertex $v(\hat I')$ lies at level $\ell$ of the tree $T$, and let $v(\hat I)$ be the parent vertex of $v(\hat I')$ in the tree, where $\hat I=(\hat G,\hat \Sigma)$. As observed already, if Event $\event$ does not happen, $|E(\hat G)|\geq \mu^{39}$ must hold, and from the induction hypothesis, $\optcrors(\hat I)\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell-1}+m\cdot(\ell-1)\cdot\mu^{c+13}$ and $\optcrors(\hat I)\leq |E(\hat G)|^2/\mu^{40}$ must hold. If we denote by $v(\hat I'')$ the second child vertex of $v(\hat I)$, then, since we have assumed that Event $\hat \event$ does not happen, $\optcrors(I')+\optcrors(I'')\leq \optcrors(I) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}$ must hold. Therefore, 
	\[
	\begin{split}
	\optcrors(I')\leq & \text{ } \bigg(\optcrors(I)\cdot(1+1/\mu^{12})^{\ell-1}+m\cdot(\ell-1)\cdot\mu^{c+13}\bigg) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}\\
	\leq & \text{ } \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+\bigg(m\cdot(\ell-1)\cdot\mu^{c+13}\bigg) \cdot(1+1/\mu^{12})+m\cdot\mu^{c}\\
	\leq & \text{ } \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+ m\cdot\ell\cdot\mu^{c+13}.
	\end{split}
	\]
	Lastly, as observed already, $|E(\hat G')|\geq m/\mu^{11}$. 
	We then get that:
	%
	\[
	\begin{split}
	\optcrors(\hat I')&\leq \optcrors(I)\cdot(1+1/\mu^{12})^{\ell}+ m\cdot\ell\cdot\mu^{c+13}\\
	&\leq 2\cdot \optcrors(I)+ 2 m\cdot\mu^{c+24}\\
	&\leq \frac{4m^2}{\mu^{63}} \leq \frac{4\cdot |E(\hat G')|^2\cdot \mu^{22}}{\mu^{63}}\leq \frac{|E(\hat G')|^2}{\mu^{40}}.
	\end{split}
	\]
	%
	Here we have used the fact that $\ell\le \floor{2\mu^{11}}$ and the facts $\optcrors(I)\leq |E(G)|^2/\mu^{63}$ and  $|E(G)|\geq \mu^{c'}$ from the statement of \Cref{thm: main}, together with the assumption that $c'>c+50$.
\end{proof}
%\fi

%Let $\iset'$ be the set of subinstances of $I$ obtained at the end of Stage 1. Equivalently, $\iset'$ contains every instance $I'$ that is a leaf instance. We use the following claim.

\begin{claim}\label{cor: stage 1}
	If Event $\event$ did not happen, then $\sum_{I'\in \iset'}\optcrors(I')\leq 2\cdot  \optcrors(I)+ 2\cdot m\cdot  \mu^{c+13}$.
\end{claim}
\begin{proof}
	For each $1\le i\le \floor{2\mu^{11}}$, we denote by $\iset'_i$ be the set of subinstances obtained after iteration $i$. Therefore, from \Cref{lem: many paths},
	\[
	\sum_{I'\in \iset'_{i+1}}\optcrors(I')\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')\bigg)\cdot (1+1/\mu^{12})+m\cdot\mu^{c},
	\]
	and so
	\[
	\sum_{I'\in \iset'_{i+1}}\optcrors(I')+m\cdot \mu^{c+13}\leq \bigg(\sum_{I'\in \iset'_{i}}\optcrors(I')+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12}),
	\]
	Therefore,
	\[
	\sum_{I'\in \iset'}\optcrors(I')\leq \bigg(\optcrors(I)+m\cdot\mu^{c+13}\bigg)\cdot (1+1/\mu^{12})^{\floor{2\mu^{11}}}\le 2\cdot  \optcrors(I)+ 2\cdot m\cdot \mu^{c+13}.
	\]
\end{proof}

We partition the instances of $\iset'$ into two subsets: set $\iset_1'$ contains all instances $I'=(G',\Sigma')$ with $|E(G')|\leq m/\mu$, while set $\iset_2'$ contains all remaining instances. Notice that by the definition of the Stage 1 algorithm, every instance in $\iset_2'$ is a non-interesting subinstance of the input intance $I$.

\fi

==> path_case_backup.tex <==


\subsubsection{Constructing Sub-Instances}
\label{sec: compute advanced disengagement}

In this step we will construct, for each cluster $C_i\in \cset$, an sub-instance $I_i=(G_i,\Sigma_i)$ of $(G,\Sigma)$, such that the instances $\iset=\set{I_1,\ldots,I_r}$ satisfy the properties in \Cref{thm: disengagement - main}.
Recall that, for each $1\le i\le r$, $E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, and $E^{\thr}_i=\bigcup_{i'\le i-1,j'\ge i+1}E(C_{i'},C_{j'})$.

\paragraph{Instances $(G_2,\Sigma_2),\ldots,(G_{r-1},\Sigma_{r-1})$.}
We first fix some index $2\le i\le r-1$ and define the instance $(G_i,\Sigma_i)$ as follows.
The graph $G_i$ is obtained from $G$ by first contracting clusters $C_1,\ldots,C_{i-1}$ into a super-node, that we denote by $v^{\lef}_i$, and then contracting clusters $C_{i+1},\ldots,C_r$ into a super-node, that we denote by $v^{\rig}_i$, and finally deleting self-loops on the super-nodes $v^{\lef}_i$ and $v^{\rig}_i$. So $V(G_i)=V(C_i)\cup \set{ v^{\lef}_i,v^{\rig}_i}$. See \Cref{fig: disengaged instance} for an illustration. 

\begin{figure}[h]
	\centering
	\subfigure[Layout of edge sets in $G$. Edges of  $E^{\lef}_{i}\cup E^{\rig}_{i}$ are shown in green, and edges of $E^{\thr}_{i}$ are shown in red. ]{\scalebox{0.32}{\includegraphics{figs/disengaged_instance_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{5pt}
	\subfigure[Graph $G_i$. Note that $\delta_{G_i}(v_i^{\rig})=\hat E_i \cup E^{\thr}_i\cup E^{\rig}_i$, and $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1} \cup E^{\thr}_i\cup E^{\lef}_{i}$.]{
		\scalebox{0.32}{\includegraphics{figs/disengaged_instance_2.jpg}}}
	\caption{An illustration of the construction of sub-instance $(G_i,\Sigma_i)$.}\label{fig: disengaged instance}
\end{figure}

We now define the orderings in $\Sigma_i$. First, for each vertex $v\in V(C_i)$, the ordering on its incident edges is defined to be $\oset_v$, the rotation on vertex $v$ in the given rotation system $\Sigma$.
It remains to define the rotations of super-nodes $v^{\lef}_i,v^{\rig}_i$. 
We first consider $v^{\lef}_i$.
Note that $\delta_{G_i}(v^{\lef}_i)=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$.
For each edge $\hat e\in \hat E_{i-1}$, recall that $Q_{i-1}(\hat e)$ is the path in $C_{i-1}$ routing edge $\hat e$ to $u_{i-1}$.
For each edge $e\in E^{\lef}_i\cup E^{\thr}_i$, we denote by $W^{\lef}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i-1}$ and contains its entire left auxiliary path.
We then denote 
$$\wset^{\lef}_i=\set{W^{\lef}_i(e)\mid e\in E^{\thr}_i\cup E^{\lef}_i}\cup \set{Q_{i-1}(\hat e)\mid \hat e\in \hat E_{i-1}}.$$
%and we now define the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ according to the paths of $\wset^{\lef}_i$ and the rotation $\oset_{u_{i-1}}$, in a similar way that we define the circular ordering on $\delta_G(C)$ according to the paths in $\qset(C)$ and the ordering $\oset_{u(C)}$ in Section~\ref{subsec: basic disengagement}.
\znote{need to treat the red edges that enter $C_{i-1}$ specially}

Intuitively, the rotation on vertex $v^{\lef}_i$ is defined to be the ordering in which the paths in $\wset^{\lef}_i$ enter $u_{i-1}$.
Formally, for every path $W\in \wset^{\lef}_i$, let $e^*_W$ be the unique edge of path $W$ that is incident to $u_{i-1}$. We first define a circular ordering of the paths in $\wset^{\lef}_i$, as follows: the paths are ordered according to the circular ordering of their corresponding edges $e^*_W$ in $\oset_{u_{i-1}}\in \Sigma$, breaking ties arbitrarily. Since every path $W\in \wset^{\lef}_i$ is associated with a unique edge in $\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, this ordering of the paths in $\wset^{\lef}_i$ immediately defines a circular ordering of the edges of $\delta_{G_i}(v_i^{\lef})=\hat E_{i-1}\cup E^{\thr}_i\cup E^{\lef}_i$, that we denote by $\oset^{\lef}_i$. See Figure~\ref{fig: v_left rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i-1}=\set{\hat e_1,\ldots,\hat e_4}$, $E^{\lef}_{i}=\set{e^g_1}$ and $E^{\thr}_{i}=\set{e^r_1}$.
	Paths of $\wset^{\lef}_i$ excluding their first edges are shown in dash lines.]{\scalebox{0.13}{\includegraphics{figs/rotation_left_1.jpg}}}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\lef}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\lef}_i)=\set{\hat e_1,\hat e_2,\hat e_3,\hat e_4,e^g_1, e^r_1}$. The rotation $\oset^{\lef}_i$ on them around $v^{\lef}_i$ is shown above.]{
		\scalebox{0.16}{\includegraphics{figs/rotation_left_2.jpg}}}
	\caption{The rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_left rotation}
\end{figure}

The rotation $\oset^{\rig}_{i}$ on vertex $v^{\rig}_i$ is defined similarly.
Note that $\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$.
For each edge $\hat e'\in \hat E_{i}\cup E_i^{\rig}$, recall that $Q_{i}(\hat e')$ is the path in $C_{i}$ routing edge $\hat e'$ to vertex $u_{i}$.
For each edge $e\in E^{\thr}_i$, we denote by $W^{\rig}_i(e)$ the subpath of the auxiliary cycle $R_e$ that connects $e$ to $u_{i}$ and contains its entire left auxiliary path.
We then denote 
$$\wset^{\rig}_i=\set{W^{\rig}_i(e)\text{ }\big|\text{ } e\in E^{\thr}_i}\cup \set{Q_{i}(\hat e')\text{ }\big|\text{ }  \hat e'\in \hat E_{i}\cup E^{\rig}_i}.$$
The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ is then defined in a similar way as the rotation $\oset^{\lef}_i$ on vertex $v^{\lef}_i$, according to the paths of $\wset^{\rig}_i$ and the rotation $\oset_{u_{i}}\in \Sigma$.
See Figure~\ref{fig: v_right rotation} for an illustration.

\begin{figure}[h]
	\centering
	\subfigure[Layout of edges and paths, where $\hat E_{i}=\set{\hat e_1',\ldots,\hat e_4'}$, $E^{\rig}_{i}=\set{\tilde e^g_1}$ and $E^{\thr}_{i}=\set{\tilde e^r_1}$.
	Paths of $\wset^{\rig}_i$ excluding their first edges are shown in dash lines. ]{\scalebox{0.13}{\includegraphics{figs/rotation_right_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{3pt}
	\subfigure[The edges in $\delta_{G_i}(v^{\rig}_i)$ and the rotation $\oset^{\lef}_i$. Set $\delta_{G_i}(v^{\rig}_i)=\set{\hat e_1',\hat e_2',\hat e_3',\hat e_4',\tilde e^g_1,\tilde e^r_1}$. The rotation $\oset^{\rig}_i$ on them around $v^{\rig}_i$ is shown above.]{
		\scalebox{0.16}{\includegraphics{figs/rotation_right_2.jpg}}}
	\caption{The rotation $\oset^{\rig}_i$ on vertex $v^{\rig}_i$ in the instance $(G_i,\Sigma_i)$.}\label{fig: v_right rotation}
\end{figure}

\paragraph{Instances $(G_1,\Sigma_1)$ and $(G_r,\Sigma_r)$.}
The instances $(G_1,\Sigma_1)$ and $(G_r,\Sigma_r)$ are defined similarly, but instead of two super-nodes, the graphs $G_1$ and $G_r$ contain one super-node each.
In particular, graph $G_1$ is obtained from $G$ by contracting clusters $C_2,\ldots, C_r$ into a super-node, that we denote by $v^{\rig}_1$, and then deleting self-loops on it.
So $V(G_1)=V(C_1)\cup \set{v^{\rig}_{1}}$ and $\delta_{G_1}(v^{\rig}_{1})=\hat E_1\cup E^{\rig}_1$.
The rotation of a vertex $v\in V(C_1)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\rig}_1$ is defined in a similar way as $\oset^{\rig}_i$ for any index $2\le i\le r-1$.
Graph $G_r$ is obtained from $G$ by contracting clusters $C_1,\ldots, C_{r-1}$ into a super-node, that we denote by $v^{\lef}_r$, and then deleting self-loops on it.
So $V(G_r)=V(C_r)\cup \set{v^{\lef}_{r}}$ and $\delta_{G_r}(v^{\lef}_{r})=\hat E_{r-1}\cup E^{\lef}_r$.
The rotation of a vertex $v\in V(C_r)$ is defined to be $\oset_v$, the rotation on $v$ in the given rotation system $\Sigma$, and the rotation $\oset^{\lef}_r$ is defined in a similar way as $\oset^{\lef}_i$ for any index $2\le i\le r-1$.


We will use the following claims later for completing the proof of \Cref{thm: disengagement - main} in the special case.

\begin{observation}
	\label{obs: disengaged instance size}
	$\sum_{1\le i\le r}|E(G_i)|\le O(|E(G)|)$, and for each $1\le i\le r$, $|E(G_i)|\le m/\mu$. \znote{parameter?}
\end{observation}
\begin{proof}
	Note that, in the sub-instances $\set{(G_i,\Sigma_i)}_{1\le i\le r}$, each graph of $\set{G_i}_{1\le i\le r}$ is obtained from $G$ by contracting some sets of clusters of $\cset$ into a single super-node, so each edge of $G_i$ corresponds to an edge in $E(G)$.
	Therefore, for each $1\le i\le r$, 
	$$|E(G_i)|=|E_G(C_i)|+|\delta_G(C_i)|\le |E_G(C_i)|+|\inE(\cset)|\le m/(100\mu)+m/(100\mu)\le m/\mu.$$
	
	Note that $E(G_i)=E(C_i)\cup \hat E_i\cup \hat E_{i-1}\cup E_i^{\lef} \cup E_i^{\rig}\cup E_i^{\thr}$.
	First, each edge of $\bigcup_{1\le i\le r}E(C_i)$ appears in exactly one graphs of $\set{G_i}_{1\le i\le r}$. 
	Second, each edge of $\bigcup_{1\le i\le r}\hat E_i$ appears in exactly two graphs of $\set{G_i}_{1\le i\le r}$.
	Consider now an edge $e\in E'$. If $e$ connects a vertex of $C_i$ to a vertex of $C_j$ for some $j\ge i+2$, then $e$ will appear as an edge in $E_i^{\rig}\subseteq E(G_i)$ and an edge in $E_j^{\lef}\subseteq E(G_j)$, and it will appear as an edge in $E_k^{\thr}\subseteq E(G_k)$ for all $i<k<j$.
	On one hand, we have $\sum_{1\le i\le r}|E_i^{\lef} \cup E_i^{\rig}|\le 2|E(G)|$. 
	On the other hand, note that $E_k^{\thr}=E(C_{k-1},C_{k+1})\cup E^{\through}_{k-1}\cup E^{\through}_{k}$, and each edge of $e$ appears in at most two graphs of $\set{G_i}_{1\le i\le r}$ as an edge of $E(C_{k-1},C_{k+1})$.
	Moreover, from \Cref{obs: bad inded structure}, $|E^{\through}_{k-1}|\le |\hat E_{k-1}|$ and $|E^{\through}_{k}|\le |\hat E_{k}|$.
	Altogether, we have
	\begin{equation}
	\begin{split}
	\sum_{1\le i\le r}|E(G_i)| & =
	\sum_{1\le i\le r}\left(
	|E(C_i)|+ |\hat E_i|+ |\hat E_{i-1}|+ |E_i^{\lef}| + |E_i^{\rig}|+|E_i^{\thr}|
	\right)\\
	& = \sum_{1\le i\le r}
	|E(C_i)|+ \sum_{1\le i\le r} \left(|E_i^{\lef}| + |E_i^{\rig}|\right)+ \sum_{1\le i\le r}\left(|E_i^{\thr}|+ |\hat E_i|+ |\hat E_{i-1}|\right)\\
	& \le |E(G)|+ 2\cdot |E(G)| + \sum_{1\le i\le r}\left(|E(C_{i-1},C_{i+1})|+ 2|\hat E_i|+ 2|\hat E_{i-1}|\right)\\
	& \le 8\cdot |E(G)|.
	\end{split}
	\end{equation}
	This completes the proof of \Cref{obs: disengaged instance size}.
\end{proof}


\begin{observation}
	\label{obs: rotation for stitching}
	For each $1\le i\le r-1$, if we view the edge in $\delta_{G_i}(v^{\rig}_i)$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})$ as edges of $E(G)$, then $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$, and moreover, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{observation}
\begin{proof}
	Recall that for each $1\le i\le r-1$, 
	$\delta_{G_i}(v^{\rig}_i)=\hat E_{i}\cup E^{\thr}_i\cup E^{\rig}_i$ and $\delta_{G_{i+1}}(v^{\lef}_{i+1})=\hat E_{i}\cup E^{\thr}_{i+1}\cup E^{\lef}_{i+1}$. From the definition of sets $E_i^{\thr},E_{i+1}^{\thr}, E^{\rig}_i, E^{\lef}_{i+1}$,
	\[
	\begin{split}
	E_i^{\thr}\cup E^{\rig}_i
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i<j'\text{ or }i'=i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'\le i<j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'< i+1\le j'}\\
	= & \set{e\in E(C_{i'},C_{j'})\mid i'<i+1<j'\text{ or }i'<i+1=j'}=E^{\thr}_{i+1}\cup E^{\lef}_{i+1}.
	\end{split}
	\]
	Therefore, $\delta_{G_i}(v^{\rig}_i)=\delta_{G_{i+1}}(v^{\lef}_{i+1})$.
	Moreover, from the definition of path sets $\wset^{\rig}_i$ and $\wset^{\lef}_{i+1}$, it is not hard to verify that, for every edge $e\in \delta_{G_i}(v^{\rig}_i)$, the path in $\wset^{\rig}_i$ that contains $e$ as its first edge is identical to the path in $\wset^{\lef}_{i+1}$ that contains $e$ as its first edge. According to the way that rotations $\oset^{\rig}_i,\oset^{\lef}_{i+1}$ are defined, $\oset^{\rig}_i=\oset^{\lef}_{i+1}$.
\end{proof}





\subsubsection{Completing the Proof of \Cref{thm: disengagement - main} in the Special Case}
\label{sec: path case with no problematic index}

In this section we complete the proof of \Cref{thm: disengagement - main} in the special case where the Gomory-Hu tree of $H=G_{\mid \cset}$ is a path and we are additionally given, for each edge $e\in E'$, an inner path $P_e$ in graph $H$, such that set $\set{P_e}_{e\in E'}$ of paths causes congestion at most $\eta$ in $H$, for some $\eta=2^{O((\log m)^{3/4}\log\log m)}$.
Specifically, we use the following two claims, whose proofs will be provided later.

\begin{claim}
	\label{claim: existence of good solutions special}
	$\expect{\sum_{1\le i\le r}\optcrors(G_i,\Sigma_i)}\leq 2^{O((\log m)^{3/4}\log\log m)}\cdot \left(\optcrors(I)+|E(G)|\right )$.
\end{claim}

\begin{claim}
	\label{claim: stitching the drawings together}
	There is an efficient algorithm, that given, for each $1\le i\le r$, a feasible solution $\phi_i$ to the instance $(G_i,\Sigma_i)$, computes a solution to the instance $(G,\Sigma)$, such that $\cro(\phi)\le \sum_{1\le i\le r}\cro(\phi_i)$.
\end{claim}

We use the algorithm described in~\Cref{sec: guiding and auxiliary paths} and~\Cref{sec: compute advanced disengagement}, and return the disengaged instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ as the collection of sub-instances of $(G,\Sigma)$. 
From the previous subsections, the algorithm for producing the sub-instances is efficient.
On the other hand, it follows immediately from \Cref{obs: disengaged instance size}, \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together} that the sub-instances $(G_1,\Sigma_1),\ldots,(G_r,\Sigma_r)$ satisfy the properties in \Cref{thm: disengagement - main}.
This completes the proof of \Cref{thm: disengagement - main}.

We now provide the proofs of \Cref{claim: existence of good solutions special}, and~\Cref{claim: stitching the drawings together}.

$\ $

\begin{proofof}{Claim~\ref{claim: existence of good solutions special}}
	Let $\phi^*$ be an optimal drawing of the instance $(G,\Sigma)$.
	We will construct, for each $1\le i\le r$, a drawing $\phi_i$ of $G_i$ that respects the rotation system $\Sigma_i$, based on the drawing $\phi^*$, such that $\sum_{1\le i\le r}\cro(\phi_i)\le O((\cro(\phi^*)+|E(G)|)\cdot 2^{O((\log m)^{3/4}\log\log m)})$, and \Cref{claim: existence of good solutions special} then follows.
	
	\paragraph{Drawings $\phi_2,\ldots,\phi_{r-1}$.}
	First we fix some index $2\le i\le r-1$, and describe the construction of the drawing $\phi_i$. We start with some definitions.
	Recall that $E(G_i)=E_G(C_i)\cup (\hat E_{i-1}\cup \hat E_{i}) \cup (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})$.
	We define the auxiliary path set $\wset_i=\wset^{\lef}_i\cup \wset^{\rig}_i$, so 
	$$\wset_i=\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}\cup \set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}},$$
	where for each $e\in E^{\lef}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$; for each $e\in E^{\rig}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$ and the subpath of its inner path $P_e$ between $u_{i+1}$ and its last endpoint; and for each $e\in E^{\thr}_{i}$, the path $W_e$ is the union of its outer path $P^{\out}_e$, the subpath of its inner path $P_e$ between its first endpoint and $u_{i-1}$, and the subpath of $P_e$ between $u_{i+1}$ and its last endpoint.
	
	\iffalse
	We use the following observation.
	\begin{observation}
		\label{obs: wset_i_non_interfering}
		The set $\wset_i$ of paths are non-transversal with respect to $\Sigma$.
	\end{observation}
	\begin{proof}
		Recall that the paths in $\qset_{i-1}$ only uses edges of $E(C_{i-1})\cup \delta(C_{i-1})$, and they are non-transversal.
		And similarly, the paths in $\qset_{i+1}$ only uses edges of $E(C_{i+1})\cup \delta(C_{i+1})$, and they are non-transversal.
		Therefore, the paths in $\set{Q_{i+1}(\hat e)\text{ }\big|\text{ }\hat e\in \hat E_{i}}\cup \set{Q_{i-1}(\hat e)\text{ }\big|\text{ }  \hat e\in \hat E_{i-1}}$ are non-transversal.
		From \Cref{obs: non_transversal_1} and \Cref{obs: non_transversal_2}, the paths in $\set{W_e \text{ }\big|\text{ } e\in (E^{\lef}_{i}\cup E^{\thr}_{i}\cup E^{\rig}_{i})}$ are non-transversal. Therefore, it suffices to show that, the set $\wset_i$ of paths are non-transversal at all vertices of $C_{i-1}$ and all vertices of $C_{i+1}$. Note that, for each edge $e\in (E^{\lef}_{i}\cup E^{\thr}_{i})$, $W_e\cap (C_{i-1}\cup \delta(C_{i-1}))$ is indeed a path of $\qset_{i-1}$. Therefore, the paths in $\wset_i$ are non-transversal at all vertices of $C_{i-1}$. Similarly, they are also non-transversal at all vertices of $C_{i+1}$. Altogether, the paths of $\wset_i$ are non-transversal with respect to $\Sigma$.
	\end{proof}
	\fi
	
	
	For uniformity of notations, for each edge $\hat e\in \hat E_i$, we rename the path $Q_{i+1}(\hat e)$ by $W_{\hat e}$, and similarly for each edge $\hat e\in \hat E_{i-1}$, we rename the path $Q_{i-1}(\hat e)$ by $W_{\hat e}$. Therefore, $\wset_i=\set{W_e\mid e\in E(G_i)\setminus E(C_i)}$.
	Put in other words, the set $\wset_i$ contains, for each edge $e$ in $G_i$ that is incident to $v^{\lef}_i$ or $v^{\rig}_i$, a path named $W_e$.
	It is easy to see that all paths in $\wset_i$ are internally disjoint from $C_i$.
	We further partition the set $\wset_i$ into two sets: $\wset_i^{\thr}=\set{W_e\mid e\in E^{\thr}_i}$ and $\tilde \wset_i=\wset_i\setminus \wset_i^{\thr}$.
	
	We are now ready to construct the drawing $\phi_i$ for the instance $(G_i,\Sigma_i)$.
	Recall that $\phi^*$ is an optimal drawing of the input instance $(G,\Sigma)$. 
	We start with the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$, that we denote by $\phi^*_i$. We will not modify the image of $C_i$ in $\phi^*_i$, but will focus on constructing the image of edges in $E(G_i)\setminus E(C_i)$, based on the image of edges in $E(\wset_i)$ in $\phi^*_i$.
	Specifically, we proceed in the following four steps.
	
	
	
	\paragraph{Step 1.}
	For each edge $e\in E(\wset_i)$, we denote by $\pi_e$ the curve that represents the image of $e$ in $\phi^*_i$. We create a set of $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting the endpoints of $e$ in $\phi^*_i$, that lies in an arbitrarily thin strip around $\pi_e$. 
	We denote by $\Pi_e$ the set of these curves.
	We then assign, for each edge $e\in E(\wset_i)$ and for each path in $\wset_i$ that contains the edge $e$, a distinct curve in $\Pi_e$ to this path.
	Therefore, each curve in $\bigcup_{e\in E(\wset_i)}\Pi_e$ is assigned to exactly one path of $\wset_i$,
	and each path $W\in \wset_i$ is assigned with, for each edge $e\in E(W)$, a curve in $\Pi_e$. Let $\gamma_W$ be the curve obtained by concatenating all curves in $\bigcup_{e\in E(\wset_i)}\Pi_e$ that are assigned to path $W$, so $\gamma_W$ connects the endpoints of path $W$ in $\phi^*_i$.
	In fact, when we assign curves in $\bigcup_{e\in \delta(u_{i-1})}\Pi_e$ to paths in $\wset^{\lef}_i$ (recall that $\delta(v^{\lef}_i)=\hat E_{i-1}\cup E^{\lef}_i \cup E^{\thr}_i$ and $\wset^{\lef}_i=\set{W_{e'}\mid e'\in \delta(v^{\lef}_i)}$), we additionally ensure that, if we view, for each edge $e'\in \delta(v^{\lef}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\lef}_i)$ enter $u_{i-1}$ in the same order as $\oset^{\lef}_i$.
	And similarly, when we assign curves in $\bigcup_{e\in \delta(u_{i+1})}\Pi_e$ to paths in $\wset^{\rig}_i$ (recall that $\delta(v^{\rig}_i)=\hat E_{i}\cup E^{\rig}_i \cup E^{\thr}_i$ and $\wset^{\rig}_i=\set{W_{e'}\mid e'\in \delta(v^{\rig}_i)}$), we ensure that, if we view, for each edge $e'\in \delta(v^{\rig}_i)$, the curve $\gamma_{W_{e'}}$ as the image of $e'$, then the image of edges in $\delta(v^{\rig}_i)$ enter $u_{i+1}$ in the same order as $\oset^{\rig}_i$.
	Note that this can be easily achieved according to the definition of $\oset^{\lef}_i$ and $\oset^{\rig}_i$.
	We denote $\Gamma_i=\set{\gamma_W\mid W\in \wset_i}$, and we further partition the set $\Gamma_i$ into two sets: $\Gamma_i^{\thr}=\set{\gamma_{W}\mid W\in \wset^{\thr}_i}$ and $\tilde \Gamma_i=\Gamma_i\setminus \Gamma_i^{\thr}$.
	
	%\znote{Note sure if this notation should be replaced by a single $\hat \phi$.}
	We denote by $\hat \phi_i$ the drawing obtained by taking the union of the image of $C_i$ in $\phi^*_i$ and all curves in $\Gamma_i$. 
	%For each path $\gamma\in \Gamma_i$, we denote by $\hat\chi_i(\gamma)$ the number of crossings between $\gamma$ and all other curves in drawing $\hat{\phi_i}$, namely $\hat\chi_i(\gamma)=\chi_{\hat\phi_i}(\gamma,(\Gamma_i\setminus \set{\gamma})\cup \phi^*_i(C_i))$.
	For every path $P$ in $G_i$, we denote by $\hat{\chi}_i(P)$ the number of crossings that involves the ``image of $P$'' in $\hat \phi_i$, which is defined as the union of, for each edge $e\in E(\tilde\wset_i)$, an arbitrary curve in $\Pi_e$. 
	Clearly, for each edge $e\in E(\wset_i)$, all curves in $\Pi_e$ are crossed by other curves of $(\Gamma_i\setminus \Pi_e)\cup \phi^*_i(C_i)$ same number of times. 
	Therefore, $\hat{\chi}_i(P)$ is well-defined.
	For a set $\pset$ of paths in $G_i$, we define $\hat{\chi}_i(\pset)=\sum_{P\in \pset}\hat{\chi}_i(P)$.
	
	\iffalse
	We use the following observation.
	\znote{maybe remove this observation?}
	
	%Recall that, for each path $W$, $\cro(W)$ is the total number of crossings in the drawing $\phi^*$ in which edges of $W$ participate. We use the following observation.
	
	\begin{observation}
		\label{obs: curves_crossings}
		The number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$,
		%$\chi(\bigcup_{e\in E(\wset_i)}\Gamma_e)=O(\cost(\wset_i)\cdot\poly\log n)$,
		and the number of intersections between a curve in $\tilde\Gamma_i$ and the image of edges of $C_i$ in $\phi^*_i$, are both  $O(\sum_{W\in \tilde\wset_i}\hat\cro(W))$.
	\end{observation}
	\begin{proof}
		We first show that the number of points that belongs to at least two curves in $\tilde\Gamma_i$ and is not the image of a vertex in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		%First, the number of points that lie on at least three curves of $\tilde\Gamma_i$ is the image of some vertex of $V(\tilde \wset)$, so the number of such points is bounded by $|V(\tilde \wset)|$. It remains to estimate the number of points that belong to exactly two curves of $\tilde\Gamma_i$.
		Note that, from the construction of curves in $\set{\gamma_W\mid W\in \tilde\wset_i}$, every crossing between a pair $W,W'$ of curves in $\tilde\Gamma_i$ must be the intersection between a curve in $\Pi_e$ for some $e\in E(W)$ and a curve in $\Pi_{e'}$ for some $e'\in E(W')$, such that the image $\pi_e$ for $e$ and the  image $\pi_{e'}$ for $e'$ intersect in $\phi^*$.
		Therefore, for each pair $W,W'$ of paths in $\tilde\wset_i$, the number of points that belong to only curves $\gamma_W$ and $\gamma_{W'}$ is at most the number of crossings between the image of $W$ and the image of $W'$ in $\phi^*$. 
		It follows that the number of points that belong to exactly two curves of $\tilde\Gamma_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Altogether, the number of intersections between curves in $\tilde\Gamma_i$ is at most $|V(\tilde \wset_i)|+\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		
		We now show that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ that are not vertex-image is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
		Let $W$ be a path of $\tilde \wset_i$ and consider the curve $\gamma_W$. Note that $\gamma_W$ is the union of, for each edge $e\in E(W)$, a curve that lies in an arbitrarily thin strip around $\pi_e$.
		Therefore, the number of crossings between $\gamma_W$  and the image of $C_i$ in $\phi^*_i$ is identical to the number of crossings the image of path $W$  and the image of $C_i$ in $\phi^*_i$, which is at most $\hat\cro(W)$.
		It follows that the number of intersections between a curve in $\tilde\Gamma_i$ and the image of $C_i$ in $\phi^*_i$ is at most $\sum_{W\in \tilde\wset_i}\hat\cro(W)$.
	\end{proof}
	\fi
	
	\paragraph{Step 2.}
	For each vertex $v\in V(\wset_i)$, we denote by $x_v$ the point that represents the image of $v$ in $\phi^*_i$, and we let $X$ contains all points of $\set{x_v\mid v\in V(\wset_i)}$ that are intersections between curves in $\Gamma_i$.
	We now manipulate the curves in $\set{\gamma_W\mid W\in \wset_i}$ at points of $X$, by processing points of $X$ one-by-one, as follows. 
	Consider a point $x_v$ that is an intersection between curves in $\Gamma_i$, where $v\in V(\wset_i)$, and let $D_v$ be an arbitrarily small disc around $x_v$.
	We denote by $\wset_i(v)$ the set of paths in $\wset_i$ that contains $v$, and further partition it into two sets: $\wset^{\thr}_i(v)=\wset_i(v)\cap \wset^{\thr}_i$ and $\tilde\wset_i(v)=\wset_i(v)\cap \tilde\wset_i$. We apply the algorithm from \Cref{obs: curve_manipulation} to modify the curves of $\set{\gamma_W\mid W\in\tilde\wset_i(v)}$ within disc $D_v$. Let $\set{\gamma'_W\mid W\in\tilde\wset_i(v)}$ be the set of new curves that we obtain. From \Cref{obs: curve_manipulation}, 
	(i) for each path $W\in \tilde\wset_i(v)$, the curve $\gamma'_W$ does not contain $x_v$, and is identical to the curve $\gamma_W$ outside the disc $D_v$;
	%\item for each path $W\in \tilde\wset_i(v)$, the curves $\gamma_W$ and $\gamma'_W$ are identical outside the disc $\dset_v$;
	(ii) the segments of curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $D_v$ are in general position; and
	(iii) the number of icrossings between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside $D_v$ is bounded by $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	%\item the number of intersections between a curve of $\set{\gamma'_{W}\mid W\in \tilde\wset_i(v)}$ and a curve of $\set{\gamma'_{W}\mid W\in \wset^{\thr}_i(v)}$ inside disc $\dset_v$ is bounded by $O(\cost(\tilde \wset_i))$.
	\iffalse{just for backup}
	\begin{proof}
		Denote $d=\deg_G(v)$ and $\delta_G(v)=\set{e_1,\ldots,e_d}$, where the edges are indexed according to the ordering $\oset_v\in \Sigma$.
		For each path $W\in \tilde\wset_i(v)$, we denote by $p^{-}_W$ and $p^{+}_W$ the intersections between the curve $\gamma_W$ and the boundary of $\dset_v$.
		We now compute, for each $W\in W\in \tilde\wset_i(v)$, a curve $\zeta_W$ in $\dset_v$ connecting $p^{-}_W$ to $p^{+}_W$, such that (i) the curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$ are in general position; and (ii) for each pair $W,W'$ of paths, the curves $\zeta_W$ and $\zeta_{W'}$ intersects iff the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{-}_{W'},p^{+}_{W},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_{W'},p^{-}_{W},p^{+}_{W'})$.
		It is clear that this can be achieved by first setting, for each $W$, the curve $\zeta_W$ to be the line segment connecting $p^{-}_W$ to $p^{+}_W$, and then slightly perturb these curves so that no point belong to at least three curves in $\set{\zeta_W\mid W\in \tilde\wset_i(v)}$.
		We now define, for each $W$, the curve $\gamma'_W$ to be the union of the part of $\gamma_W$ outside $\dset_v$ and the curve $\zeta_W$.
		See Figure~\ref{fig: curve_con} for an illustration.
		Clearly, the first and the second condition of \Cref{obs: curve_manipulation} are satisfied.
		It remains to estimate the number of intersections between curves of $\set{\gamma'_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$, which equals the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$.
		Since the paths in $\tilde\wset_i(v)$ are non-transversal with respect to $\Sigma$ (from \Cref{obs: wset_i_non_interfering}), from the construction of curves $\set{\gamma_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$, if a pair $W,W'$ of paths in $\tilde \wset_i(v)$ do not share edges of $\delta(v)$, then the order in which the points $p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'}$ appear on the boundary of $\dset_v$ is either $(p^{-}_W,p^{+}_W,p^{-}_{W'},p^{+}_{W'})$ or $(p^{+}_W,p^{-}_W,p^{-}_{W'},p^{+}_{W'})$, and therefore the curves $\zeta_{W}$ and $\zeta_{W'}$ will not intersect in $\dset_v$.
		Therefore, only the curves $\zeta_W$ and $\zeta_{W'}$ intersect iff $W$ and $W'$ share an edge of $\delta(v)$.
		Since every such pair of curves intersects at most once, the number of intersections between curves of $\set{\zeta_{W}\text{ }\big|\text{ }W\in \tilde\wset_i(v)}$ inside disc $\dset_v$ is at most $\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2$.
	\end{proof}
	\begin{figure}[h]
		\centering
		\subfigure[Before: Curves of $\wset^{\thr}_i(v)$ are shown in black, and curves of $\tilde\wset_i(v)$ are shown in blue, red, orange and green. ]{\scalebox{0.32}{\includegraphics{figs/curve_con_1.jpg}}}
		\hspace{1pt}
		\subfigure[After: Curves of $\wset^{\thr}_i(v)$ are not modified, while curves of $\tilde\wset_i(v)$ are re-routed via dash lines within disc $\dset_v$.]{
			\scalebox{0.32}{\includegraphics{figs/curve_con_2.jpg}}}
		\caption{An illustration of the step of processing $x_v$.}\label{fig: curve_con}
	\end{figure}
	\fi
	
	%Let $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$ be the curves given by the algorithm in~\Cref{obs: curve_manipulation}. 
	We then replace the curves of $\set{\gamma_W\mid W\in \tilde\wset_i(v)}$ in $\Gamma_i$ by the curves of $\set{\gamma'_W\mid W\in \tilde\wset_i(v)}$.
	This completes the description of the iteration of processing point the point $x_v\in X$. Let $\Gamma'_i$ be the set of curves that we obtain after processing all points in $X$ in this way. Note that we have never modified the curves of $\Gamma^{\thr}_i$, so $\Gamma^{\thr}_i\subseteq\Gamma'_i$, and we denote $\tilde\Gamma'_i=\Gamma'_i\setminus \Gamma^{\thr}_i$.
	We use the following observation.
	\begin{observation}
		\label{obs: general_position}
		Curves in $\tilde\Gamma'_i$ are in general position, and if a point $p$ lies on more than two curves of $\Gamma'_i$, then either $p$ is an endpoint of all curves containing it, or all curves containing $p$ belong to $\Gamma^{\thr}_i$.
	\end{observation}
	\begin{proof}
		From the construction of curves in $\Gamma_i$, any point that belong to at least three curves of $\Gamma_i$ must be the image of some vertex in $\phi^*$. From~\Cref{obs: curve_manipulation}, curves in $\tilde\Gamma'_i$ are in general position; curves in $\tilde\Gamma'_i$ do not contain any vertex-image in $\phi^*$ except for their endpoints; and they do not contain any intersection of a pair of paths in $\Gamma_i^{\thr}$. \Cref{obs: general_position} now follows.
	\end{proof}
	
	
	
	
	%However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\lef}_i$ at $v^{\lef}_i$ and the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We will then modify the drawing $\phi_i'$ to obtain the final drawing $\phi'_i$, in the last step.
	
	
	\paragraph{Step 3.} 
	So far we have obtained a set $\Gamma'_i$ of curves that are further partitioned into two sets $\Gamma'_i=\Gamma^{\thr}_i\cup \tilde\Gamma'_i$,
	where set $\tilde\Gamma'_i$ contains, for each path $W\in \tilde \wset_i$, a curve $\gamma'_W$ connecting the endpoints of $W$, and the curves in $\tilde\Gamma'_i$ are in general position;
	and set $\Gamma^{\thr}_i$ contains, for each path $W\in \wset^{\thr}_i$, a curve $\gamma_W$ connecting the endpoints of $W$. 
	Recall that all paths in $\wset^{\thr}_i$ connects $u_{i-1}$ to $u_{i+1}$. 
	Let $z_{\lef}$ be the point that represents the image of $u_{i-1}$ in $\phi_i^*$ and let $z_{\rig}$ be the point that represents the image of $u_{i+1}$ in $\phi_i^*$. 
	Then, all curves in $\Gamma^{\thr}_i$ connects $z_{\lef}$ to $z_{\rig}$.
	We view $z_{\lef}$ as the first endpoint of curves in $\Gamma^{\thr}_i$ and view $z_{\rig}$ as their last endpoint.
	We then apply the algorithm in \Cref{thm: type-2 uncrossing}, where we let $\Gamma=\Gamma^{\thr}_i$ and let $\Gamma_0$ be the set of all other curves in the drawing $\phi^*_i$. Let $\Gamma^{\thr'}_i$ be the set of curves we obtain. We then designate, for each edge $e\in E^{\thr}_i$, a curve in $\Gamma^{\thr'}_i$ as $\gamma'_{W_e}$, such that the curves of $\set{\gamma'_{W_e}\mid e\in \hat E_{i-1}\cup E^{\lef}_i\cup  E^{\thr}_i}$ enters $z_{\lef}$ in the same order as $\oset^{\lef}_i$.
	
	
	Recall that $\wset_i=\set{W_e\mid e\in (E_i^{\lef}\cup E_i^{\thr}\cup E_i^{\rig}\cup \hat E_{i-1}\cup \hat E_i)}$, and, for each edge $e\in E_i^{\lef}\cup \hat E_{i-1}$, the curve $\gamma'_{W_e}$ connects its endpoint in $C_i$ to $z_{\lef}$; for each edge $e\in E_i^{\rig}\cup \hat E_{i}$, the curve $\gamma'_{W_e}$ connects the endpoint of $e$ to $z_{\rig}$; and for each edge $e\in E_i^{\thr}$, the curve $\gamma'_{W_e}$ connects $z_{\lef}$ to $z_{\rig}$.
	Therefore, if we view $z_{\lef}$ as the image of $v^{\lef}_i$,  view $z_{\rig}$ as the image of $v^{\rig}_i$, and for each edge $e\in E(G_i)\setminus E(C_i)$, view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi'_i$.
	It is clear from the construction of curves in $\set{\gamma'_{W_e}\mid e\in E(G_i)\setminus E(C_i)}$ that this drawing respects all rotations in $\Sigma_i$ on vertices of $V(C_i)$ and vertex $v^{\lef}_i$.
	However, the drawing $\phi'_i$ may not respect the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$. We further modify the drawing $\phi'_i$ at $z_{\rig}$ in the last step.
	
	
	
	
	
	\paragraph{Step 4.}
	Let $\dset$ be an arbitrarily small disc around $z_{\rig}$ in the drawing $\phi'_i$, and let $\dset'$ be another small disc around $z_{\rig}$ that is strictly contained in $\dset$.
	We first erase the drawing of $\phi'_i$ inside the disc $\dset$, and for each edge $e\in \delta(v^{\rig}_i)$, we denote by $p_{e}$ the intersection between the curve representing the image of $e$ in $\phi'_i$ and the boundary of $\dset$.
	We then place, for each edge $e\in \delta(v^{\rig}_i)$, a point $p'_e$ on the boundary of $\dset'$, such that the order in which the points in $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$ appearing on the boundary of $\dset'$ is precisely $\oset^{\rig}_{i}$. 
	We then apply \Cref{lem: find reordering} to compute a set of reordering curves, connecting points of $\set{p_e\mid e\in \delta(v^{\rig}_i)}$ to points $\set{p'_e\mid e\in \delta(v^{\rig}_i)}$.
	Finally, for each edge $e\in \delta(v^{\rig}_i)$, let $\gamma_e$ be the concatenation of (i) the image of $e$ in $\phi'_i$ outside the disc $\dset$; (ii) the reordering curve connecting $p_e$ to $p'_e$; and (iii) the straight line segment connecting $p'_e$ to $z_{\rig}$ in $\dset'$.
	We view $\gamma_e$ as the image of edge $e$, for each $e\in \delta(v^{\rig}_i)$. 
	We denote the resulting drawing of $G_i$ by $\phi_i$. It is clear that $\phi_i$ respects the rotation $\oset^{\rig}_i$ at $v^{\rig}_i$, and therefore it respects the rotation system $\Sigma_i$.
	
	We use the following claim.
	\begin{claim}
		\label{clm: rerouting_crossings}
		The number of crossings of $\phi_i$ inside the disc $\dset$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
	\end{claim}
	\begin{proof}
		Denote by $\oset^*$ the ordering in which the curves $\set{\gamma'_{W_e}\mid e\in \delta_{G_i}(v_i^{\rig})}$ enter $z_{\rig}$, the image of $u_{i+1}$ in $\phi'_i$.
		From~\Cref{lem: find reordering} and the algorithm in Step 4 of modifying the drawing within the disc $\dset$, the number of crossings of $\phi_i$ inside the disc $\dset$ is at most $O(\dist(\oset^*,\oset_i^{\rig}))$. Therefore, it suffices to show that $\dist(\oset^*,\oset_i^{\rig})=O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		In fact, we will compute a set of curves connecting the image of $u_i$ and the image of $u_{i+1}$ in $\phi^*_i$, such that each curve is indexed by some edge $e\in\delta_{G_i}(v_i^{\rig})$ these curves enter $u_i$ in the order $\oset^{\rig}_i$ and enter $u_{i+1}$ in the order $\oset^*$, and the number of crossings between curves of $Z$ is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		
		%Recall that the set $\wset^{\thr}_i=\set{W_e\mid e\in E^{\thr}_i}$ of paths connect $u_{i-1}$ to $u_{i+1}$. We define, for each $e\in E^{\thr}_i$, the path $W^*_e$ to be the union of path $W_e$ and the subpath of the outer path $P^{\out}_e$ between $u_i$ and $u_{i-1}$, so the path $W^*_e$ connects $u_i$ to $u_{i+1}$. We denote $\wset^*_i=\set{W^*_e\mid e\in E^{\thr}_i}$.
		For each $e\in E^{\thr}_i$, we denote by $\eta_e$ the curve obtained by taking the union of (i) the curve $\gamma'_{W_e}$ (that connects $u_{i+1}$ to $u_{i-1}$); and (ii) the curve representing the image of the subpath of $P_e$ in $\phi^*_i$ between $u_i$ and $u_{i-1}$.
		Therefore, the curve $\eta_e$ connects $u_i$ to $u_{i+1}$.
		We then modify the curves of $\set{\eta_e\mid e\in E^{\thr}_i}$, by iteratively applying the algorithm from \Cref{obs: curve_manipulation} to these curves at the image of each vertex of $C_{i-1}\cup C_{i+1}$. Let $\set{\zeta_e\mid e\in E^{\thr}_i}$ be the set of curves that we obtain. We call the obtained curves \emph{red curves}. From~\Cref{obs: curve_manipulation}, the red curves are in general position. Moreover, it is easy to verify that the number of intersections between the red curves is $O(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1}))$.
		
		We call the curves in $\set{\gamma'_{W_e}\mid e\in \hat E_i}$ \emph{yellow curves}, call the curves in $\set{\gamma'_{W_e}\mid e\in E^{\rig}_i}$ \emph{green curves}. See \Cref{fig: uncrossing_to_bound_crossings} for an illustration.
		From the construction of red, yellow and green curves, we know that these curves enter $u_i$ in the order $\oset^{\rig}_i$, and enter $u_{i+1}$ in the order $\oset^*$.
		Moreover, we are guaranteed that the number of intersections between red, yellow and green curves is at most $\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W))$.
		%(3) Since we are not sure how the red curves enter $u_{i+1}$, we are also not sure how red, yellow, green curves together enter $u_{i+1}$. Denote this ordering by $\oset$. Although we do know that the yellow curves and the green curves enter $v^{\rig}_i$ in the same order in which the paths $\set{W_e\mid e\in \hat E_i\cup E^{\rig}_i}$ enters $u_{i+1}$, but this is not enough.
		%(4) Luckily, since we want them to enter $v^{\rig}_i$ in the order $\oset^{\rig}_i$, namely how the paths $\set{W_e\mid e\in \delta(v^{\rig}_i)}$ enters $u_{i}$, it suffices to compute a set of reordering curves connecting $u_{i+1}$ to $u_{i}$ with low cost, where the order in which they enter $u_{i+1}$ is $\oset$ and the order in which they enter $u_{i}$ is $\oset^{\rig}_i$. And it is clear that the red, yellow and green curves themselves form a set of reordering curves, at the cost of $\cro(\qset_{i-1})+\cro(\qset_{i})+\sum_{e\in \hat E_i\cup E^{\rig}_i}\cro(W_e)$.
		\begin{figure}[h]
			\centering
			\includegraphics[scale=0.35]{figs/uncross_to_bound_crossings.jpg}
			\caption{An illustration of red, yellow and green curves.}\label{fig: uncrossing_to_bound_crossings}
		\end{figure}
	\end{proof}
	
	From the above discussion and Claim~\ref{clm: rerouting_crossings}, for each $2\le i\le r-1$, 
	\[
	\cro(\phi_i)=\chi^2(C_i)+O\left(\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right).
	\]
	
	
	
	\iffalse
	We now estimate the number of crossings in $\phi_i$ in the next claim.
	\begin{claim}
		\label{clm: number of crossings in good solutions}
		$\cro(\phi_i)=\chi^2(C_i)+O\left(\sum_{W\in \tilde\wset_i}\cro(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)$.
	\end{claim}
	\begin{proof}
		$2\cdot \sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2=\sum_{v\in V(G)}\sum_{e\in \delta_G(v)}\cong_G(\tilde \wset_i,e)^2.$
		\znote{need to redefine the orderings $\oset^{\lef}_i$ and $\oset^{\rig}_i$ to get rid of $\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2$ here, which we may not be able to afford.}
	\end{proof}
	\fi
	
	
	\paragraph{Drawings $\phi_1$ and $\phi_{r}$.}
	The drawings $\phi_1$ and $\phi_{r}$ are constructed similarly. We describe the construction of $\phi_1$, and the construction of $\phi_1$ is symmetric.
	Recall that the graph $G_1$ contains only one super-node $v_1^{\rig}$, and $\delta_{G_1}(v_1^{\rig})=\hat E_1\cup E^{\rig}_1$. We define $\wset_1=\set{W_e\mid e\in E^{\rig}_1}\cup \set{Q_2(\hat e)\mid \hat e\in \hat E_1}$. For each $\hat e\in \hat E_1$, we rename the path $Q_2(\hat e)$ by $W_e$, so $\wset_1$ contains, for each edge $e\in \delta_{G_1}(v^1_{\rig})$, a path named $W_e$ connecting its endpoints to $u_2$. Via similar analysis in \Cref{obs: wset_i_non_interfering}, it is easy to show that the paths in $\wset_1$ are non-transversal with respect to $\Sigma$.
	
	We start with the drawing of $C_1\cup E(\wset_1)$ induced by $\phi^*$, that we denote by $\phi^*_1$. We will not modify the image of $C_i$ in $\phi^*_i$ and will construct the image of edges in $\delta(v_1^{\rig})$.
	We perform similar steps as in the construction of drawings $\phi_2,\ldots,\phi_{r-1}$. 
	We first construct, for each path $W\in \wset_1$, a curve $\gamma_W$ connecting its endpoint in $C_1$ to the image of $u_2$ in $\phi^*$, as in Step 1.
	Let $\Gamma_1=\set{\gamma_W\mid W\in \wset_1}$ be the set of curves we obtain.
	%It is not hard to show that \Cref{obs: curves_crossings} still holds when $i=1$ (note that $\Gamma^{\thr}_1=\emptyset$, so $\tilde\Gamma_1=\Gamma_1$). 
	We then process all intersections between curves of $\Gamma_1$ as in Step 2. Let $\Gamma'_1=\set{\gamma'_W\mid W\in \wset_1}$ be the set of curves we obtain.
	Since $\Gamma^{\thr}_1=\emptyset$, we do not need to perform Steps 3 and 4. If we view the image of $u_2$ in $\phi^*_1$ as the image of $v^{\rig}_1$, and for each edge $e\in \delta(v^{\rig}_1)$, we view the curve $\gamma'_{W_e}$ as the image of $e$, then we obtain a drawing of $G_i$, that we denote by $\phi_i$. It is clear that this drawing respects the rotation system $\Sigma_1$. Moreover,
	\[\cro(\phi_1)=\chi^2(C_1)+O\left(\hat\chi_1(\qset_2)+\sum_{W\in \wset_1}\hat\chi_1(W)+\sum_{e\in E(G)}\cong_G(\wset_1,e)^2\right).\]
	Similarly, the drawing $\phi_k$ that we obtained in the similar way satisfies that 
	\[\cro(\phi_k)=\chi^2(C_k)+O\left(\hat\chi_k(\qset_{r-1})+\sum_{W\in \wset_k}\hat\chi_k(W)+\sum_{e\in E(G)}\cong_G(\wset_k,e)^2\right).\]
	
	
	
	
	We now complete the proof of \Cref{claim: existence of good solutions special}, for which it suffices to estimate $\sum_{1\le i\le r}\cro(\phi_i)$.
	Recall that, for each $1\le i\le r$, $\tilde \wset_i=\set{W_e\mid e\in \hat E_{i-1}\cup \hat E_{i-1}\cup E^{\lef}_{i}\cup E^{\rig}_{i}}$, where $E^{\lef}_{i}=E(C_i,\bigcup_{1\le j\le i-2}C_j)$, and 
	$E^{\rig}_{i}=E(C_i,\bigcup_{i+2\le j\le r}C_j)$. Therefore, for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, the path $W_e$ belongs to exactly $2$ sets of $\set{\tilde\wset_i}_{1\le i\le r}$.
	Recall that the path $W_e$ only uses edges of the inner path $P_e$ and the outer path $P^{\out}_e$.
	Let $\tilde\wset=\bigcup_{1\le i\le r}\tilde\wset_i$, from \Cref{obs: edge_occupation in outer and inner paths}, 
	for each edge $e\in E'\cup (\bigcup_{1\le i\le r-1}\hat E_i)$, $\cong_G(\tilde\wset,e)=O(1)$, and
	for $1\le i\le r$ and for each edge $e\in E(C_i)$, $\cong_G(\tilde\wset,e)=O(\cong_G(\qset_i,e))$.
	
	Therefore, on one hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{W\in \tilde\wset_i}\hat\chi_i(W)
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} 2\cdot \cong_G(\tilde \wset,e)\cdot\cong_G(\tilde \wset,e')\\
	& \le 
	\sum_{(e,e'): e,e'\text{ cross in }\phi^*} \left(\cong_G(\tilde \wset,e)^2+\cong_G(\tilde \wset,e')^2\right)\\
	& \le 
	\sum_{e\in E(G)} \chi(e)\cdot \cong_G(\tilde \wset,e)^2
	= O(\cro(\phi^*)\cdot\temp),
	\end{split}
	\]
	and on the other hand,
	\[
	\begin{split}
	\sum_{1\le i\le r}\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2
	%= \sum_{e\in E(G)} \sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)^2 
	& \le  \sum_{e\in E(G)} \left(\sum_{1\le i\le r} \cong_G(\tilde \wset_i,e)\right)^2\\
	& \le O\left(\sum_{e\in E(G)} \cong_G(\tilde \wset,e)^2 \right)\\
	& \le O\left(|E(G)|+\sum_{1\le i\le r}\sum_{e\in E(C_i)} \cong_G(\qset_i,e)^2\right)=O(|E(G)|\cdot\temp).
	\end{split}
	\]
	Moreover, $\sum_{1\le i\le r}\chi^2(C_i)\le O(\cro(\phi^*))$, and $\sum_{1\le i\le r}\hat\chi_i(\qset_{i-1}\cup \qset_{i+1})\le O(\cro(\phi^*)\cdot\temp)$.
	
	Altogether,
	\[
	\begin{split}
	\sum_{1\le i\le r}\cro(\phi_i)
	& \le 
	O\left(\sum_{1\le i\le r} 
	\left(
	\chi^2(C_i)+ \hat\chi_i(\qset_{i-1}\cup \qset_{i+1})+\sum_{W\in \tilde\wset_i}\hat\chi_i(W)+\sum_{e\in E(G)}\cong_G(\tilde \wset_i,e)^2\right)
	\right)\\
	& \le O(\cro(\phi^*))+O(\cro(\phi^*)\cdot\temp)+O(\cro(\phi^*)\cdot\temp)+O(|E(G)|\cdot\temp)\\
	& \le O((\cro(\phi^*)+|E(G)|)\cdot\temp).
	\end{split}
	\]
	
	This completes the proof of \Cref{claim: existence of good solutions special}.
\end{proofof}






$\ $



\iffalse
We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

We first define an instance $(\hat G_i,\hat\Sigma_i)$ as follows. We start with the subgraph of $G$ induced by all edges of $E_G(C_i)$ and $E(\wset_i)$, and then create, for each edge $e$ in the subgraph, $\cong_{\wset_i}(e)$ parallel copies of it. This finishes the description of graph $\hat G_i$.
For each vertex $v$ in $\hat G_i$, we define its rotation $\hat\oset_v$ as follows. We start with the rotation $\oset_v\in \Sigma$, and then replace, for each edge $e\in E(\wset_i)$, the edge $e$ in the ordering $\oset_v$ by its $\cong_{\wset_i}(e)$ copies that appears consecutively at the location of $e$ in $\oset_v$, where the ordering among the copies is arbitrary. 
On the one hand, in graph $\hat G_i$, we can make paths of $\wset_i$ edge-disjoint by letting, for each edge $e\in E(\wset_i)$, each path of $\wset_i$ that contains $e$ now take a distinct copy of $e$ in $\hat G_i$.
On the other hand, a drawing $\hat \phi_i$ of the instance $(\hat G_i,\hat\Sigma_i)$ can be easily computed from $\phi^*$, as follows.
We start with $\hat\phi'_i$, the drawing of $C_i\cup E(\wset_i)$ induced by $\phi^*$. Then for each edge of $\wset_i$, let $\gamma_e$ be the curve that represents the image of $e$, and we create $\cong_{\wset_i}(e)$ mutually internally disjoint curves connecting endpoints of $e$, that lies in an arbitrarily thin strip around $\gamma_e$. We denote by $\hat{\phi_i}$ the resulting drawing, and it is clear that $\hat{\phi_i}$ is a drawing of the instance $(\hat G_i,\hat\Sigma_i)$, such that $\cro(\hat{\phi_i})\le \cro(C_i)+O(\cost(\wset_i)\cdot\poly\log n)$.

For each edge $e\in E_G(C_i)$, we denote by $\gamma_e$ the curve in $\hat \phi_i$ that represents the image of $e$; and for each path $W\in \wset_i$, we denote by $\gamma_W$ the curve in $\hat \phi_i$ that represents the image of $W$.
We define $\Gamma_0=\set{\gamma_e\mid e\in E_G(C_i)}$ and $\Gamma_1=\set{\gamma_W\mid W\in \wset_i}$. It is immediate to verify that the sets $\Gamma_0,\Gamma_1$ of curves satisfy the condition of \Cref{thm: type-2 uncrossing}. We then apply the algorithm in \Cref{thm: type-2 uncrossing} to $\Gamma_0,\Gamma_1$, and let $\Gamma_1'$ be the set of curves that we obtain.
From \Cref{thm: type-2 uncrossing}, the curves in $\Gamma_1'$ do not intersect internally between each other, and have the same sets of first endpoints and last endpoints.
We now show that we can obtain a drawing $\phi_i$ of the instance $(G_i,\Sigma_i)$ using the curves $\Gamma_0,\Gamma_1'$.
For each edge $e\in E_G(C_i)$, we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
For each edge path $W\in \wset$, from \Cref{thm: type-2 uncrossing}, there is a curve $\gamma'\in \Gamma_1'$ connecting the endpoint of $W$ to we still let the curve $\gamma_e\in \Gamma_0$ be the image of $e$. 
\znote{maybe we need another type of uncrossing here.}
\fi



\begin{proofof}{Claim~\ref{claim: stitching the drawings together}}
	We first define a set $\set{(U_i,\Sigma'_i)\mid 1\le i\le r}$ of instances of \CNwRS as follows.
	We define $U_1=G$, and for each $2\le i\le r$, we define $U_i$ to be the graph obtained from $G$ by contracting the clusters $C_1,\ldots, C_{i-1}$ into a vertex $v^{\lef}_i$.
	Note that each edge in $U_i$ is also an edge in $G$, and we do not distinguish between them.
	Note that $U_1=G$, we define the rotation system $\Sigma'_1$ on $U_1$ to be $\Sigma$.
	For each $2\le i\le r$, we define the rotation system $\Sigma'_i$ on $U_i$ as follows.
	For each vertex $v\in \bigcup_{i\le t\le r}V(C_t)$, note that its incident edges in $U_i$ are the edges of $\delta_G(v)$, and its rotation in $\Sigma'_i$ is defined to be $\oset_v$, the rotation on $v$ in the input rotation system $\Sigma$.
	For vertex $v^{\lef}_i$, note that its incident edges are the edges of $\delta_{G_i}(v^{\lef}_i)$, and its rotation in $\Sigma'_i$ is defined to be $\oset^{\lef}_i$, the rotation on $v^{\lef}_i$ of instance $(G_i,\Sigma_i)$.
	
	
	Note that $U_k=G_k$ and $\Sigma'_k=\Sigma_k$, so the drawing $\phi_k$ of the instance $(G_k,\Sigma_k)$ is also a drawing of the instance $(U_k,\Sigma'_k)$. For clarity, when we view this drawing as a solution to the instance $(U_k,\Sigma'_k)$, we rename it by $\psi_k$.
	We will sequentially, for $i=r-1,\ldots,1$, compute a drawing of the instance $(U_i,\Sigma'_i)$ using the drawing $\psi_{i+1}$ of $(U_{i+1},\Sigma'_{i+1})$ and the drawing $\phi_i$ of $(G_{i},\Sigma_{i})$, and eventually, we return the drawing $\psi_1$ of $(U_{1},\Sigma'_{1})$ as the solution to the instance $(G,\Sigma)$.
	
	We now fix an index $1\le  i< r-1$ and construct the drawing $\psi_i$ to the instance $(U_{i},\Sigma'_{i})$, assuming that we have computed a drawing $\psi_{i+1}$ to the instance $(U_{i+1},\Sigma'_{i+1})$, as follows.
	Recall that $V(G_i)=V(C_i)\cup\set{v^{\lef}_i,v^{\rig}_i}$ if $i\ge 2$ and $V(G_i)=V(C_i)\cup\set{v^{\rig}_i}$ if $i=1$, and $\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.  Moreover, from \Cref{obs: rotation for stitching} and the definition of instance $(U_{i+1},\Sigma'_{i+1})$, the rotation on $v^{\rig}_i$ in $\Sigma_{i}$ is identical to the rotation on $v^{\lef}_{i+1}$ in $\Sigma'_{i+1}$.
	Denote $F=\delta_{G_i}(v^{\rig}_i)=\delta_{U_{i+1}}(v^{\lef}_{i+1})$.
	Let $\dset$ be an arbitrarily small disc around the image of $v_{i+1}^{\lef}$ in $\psi_{i+1}$. For each edge $e\in F$, we denote by $p_e$ the intersection between the image of $e$ with the boundary of $\dset$. 
	Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset$ is $\oset^{\lef}_{i+1}$.
	We erase the drawing of $\psi_{i+1}$ inside the disc $\dset$, and view the area inside the disc $\dset$ as the outer face of the drawing.
	Similarly, let $\dset'$ be an arbitrarily small disc around the image of $v_{i}^{\rig}$ in $\phi_{i}$. For each edge $e\in F$, we denote by $p'_e$ the intersection between the image of $e$ with the boundary of $\dset'$. 
	Therefore, the order in which the points $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is $\oset^{\rig}_{i}$.
	We erase the drawing of $\phi_{i}$ inside the disc $\dset'$, and let $\dset''$ be another disc that is strictly contained in $\dset'$. We now place the drawing of $\psi_{i+1}$ inside $\dset'$ (after we erase part of it inside $\dset$), so that the boundary of $\dset$ in $\psi_{i+1}$ coincide with the boundary of $\dset''$ in $\phi_{i}$, while the interior of $\dset$ coincides with the exterior of $\dset''$. We then compute a set $\set{\zeta_e\mid e\in F}$ of curves lying in $\dset'\setminus \dset''$, where for each $e\in F$, the curve $\zeta_e$ connects $p'_e$ to $p_e$, such that all curves of $\set{\zeta_e\mid e\in F}$ are mutually disjoint. Note that this can be done since the order in which $\set{p_e}_{e\in F}$ appear on the boundary of $\dset'$ is identical to $\set{p'_e}_{e\in F}$ appear on the boundary of $\dset$.
	We denote by $\psi_i$ the resulting drawing we obtained.
	See Figure~\ref{fig: stitching} for an illustration.
	Clearly, $\psi_i$ is a drawing of $U_i$ that respects $\Sigma'_i$ if we view, for each edge $e\in F$, the union of (i) the image of $e$ in $\phi_i$ outside the disc $\dset'$; (ii) the curve $\zeta_e$; and (iii) the image of $e$ in $\psi_{i+1}$ inside the disc $\dset''$, as the image of $e$.
	\begin{figure}[h]
		\centering
		\subfigure[The drawing $\psi_{i+1}$, where the boundary of $\dset$ is shown in dash black.]{\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_1.jpg}}%\label{fig:non_crossing_representation}
		}
		\hspace{0.45cm}
		\subfigure[The drawing $\psi_{i+1}$ after we erase its part inside $\dset$ and view the interior of $\dset$ as the outer face.]{
			\scalebox{0.35}{\includegraphics[scale=1.0]{figs/stitching_2.jpg}}}
		\hspace{0.45cm}
		\subfigure[The drawing $\psi_i$, where the curves of $\set{\zeta_e\mid e\in F}$ are shown in dash line segments.]{
			\scalebox{0.36}{\includegraphics[scale=1.0]{figs/stitching_3.jpg}}}
		\caption{An illustration of constructing the drawing $\psi_i$ from $\psi_{i+1}$.}\label{fig: stitching}
	\end{figure}
	Clearly, any crossing in the drawing $\psi_i$ is either a crossing of $\phi_i$ or a crossing of $\psi_{i+1}$, so $\cro(\psi_i)\le \cro(\psi_{i+1})+\cro(\phi_{i})$.
	Therefore, if we rename the drawing $\psi_1$ of the instance $(U_1,\Sigma'_1)$ by $\phi$, then $\phi$ is a drawing of $G$ that respects $\Sigma$, and $\cro(\phi)\le \sum_{1\le i\le r}\cro(\phi_i)$.
\end{proofof}

















==> path_of_clusters.tex <==
\subsection{The Second Special Case: Path of Clusters}

In this section prove a special case of \Cref{thm: disengagement - main}. Specifically, we will assume that the Gomory-Hu tree of the contracted graph $G_{\mid\cset}$ is a path.

Let $H=G_{\mid\cset}$ be the contracted graph. 
We denote the clusters in $\cset$ by $C_1,C_2,\ldots,C_r$. For convenience, for each $1\leq i\leq r$, we denote by $x_i$ the vertex of graph $H$ that represents the cluster $C_i$. 

\iffalse
Throughout this subsection, we assume that the Gomory-Hu tree $\tau$ of graph $H$ is a path, and we assume without loss of generality that the clusters are indexed according to their appearance on the path $\tau$. Note that each edge in $\Eout(\cset)$ corresponds to an edge in $H$, and we do not distinguish between them.
For each $1\le i\le r$, we define edge sets
$\hat E_i=E(C_i,C_{i+1})$,
$E_i^{\rig}=\bigcup_{j>i+1}E(C_i,C_j)$,  $E_i^{\lef}=\bigcup_{j'<i-1}E(C_i,C_{j'})$, $E_i^{\thr}=\bigcup_{i'<i<j'}E(C_{i'},C_{j'})$, $E_i^{\through}=\bigcup_{i'<i,j'>i+1}E(C_{i'},C_{j'})$.
\fi

For each pair $1\le j< j'\le r$, we define $C_{[j,j']}$ as the subgraph of $G$ induced by vertices of all clusters $C_t$ with index $t$ belonging to the interval $[j,j']$. We define clusters
$C_{(j,j']}$,
$C_{[j,j')}$, and
$C_{(j,j')}$ similarly. 
We say that a partition $\zset$ of the cluster $C_{[j,j']}$ into a sequence $\zset=\set{Z_1,\ldots, Z_k}$ of clusters is \emph{$\cset$-respecting}, iff there exist indices $j<i_1<\cdots <i_{k-1}<j'$, such that for each $1\le s\le k$, $Z_s=C_{(i_{s-1}, i_s]}$ (where $j=i_0$ and $j'=i_k$).

In this section we will prove the following lemma.

\begin{lemma}
\label{lem: path case}
There is an efficient algorithm, that given an instance $I=(G,\Sigma)$ of \CNwRS with $|E(G)|=m$, and a collection $\cset=\set{C_1,\ldots,C_r}$ of vertex-disjoint clusters of $G$, such that 
\begin{itemize}
\item vertex sets $\set{V(C)}_{C\in \cset}$ partition $V(G)$;
\item each cluster $C\in \cset$ has the $\alpha_0$-bandwidth property (where $\alpha_0=1/\log^3m$); and
\item the Gomory-Hu tree $\tau$ of the contracted graph  $H=G_{\mid\cset}$ is the path $(x_1,x_2,\ldots,x_r)$, 
\end{itemize} 
computes 
\begin{itemize}
\item a $\cset$-respecting partition of graph $G$ into a sequence $\zset=\set{Z_1,\ldots,Z_k}$ of vertex-disjoint clusters, such that each cluster $Z_j$ is either a \singlecore cluster or a \dualcore cluster;
\item for each \dualcore cluster $Z_j$, three sets $\qset^{\lef}_j$, $\qset^{\rig}_j$, $\qset^{\thr}_j$ of paths. \znote{alternative name?}
\item a set $\pset=\set{P_e\mid e\in E'}$ of paths in $H$, that contains, for each edge $e\in E'$, an auxiliary path $P_e$ of $e$, such that $\cong_H(\pset)=O(1)$.
\end{itemize} 
\end{lemma}

\iffalse
\paragraph{Inner Paths.} For an edge $e\in E'$ connecting $x_i$ to $x_j$ in $H$, we say that a path $P$ in $H$ is a \emph{left inner path} of $e$, iff the endpoints of $P$ are $x_i$ and $x_{i+1}$, and $P$ only contains vertices of $S_{i+1}$; we say that a path $P$ in $H$ is a \emph{right inner path} of $e$, iff the endpoints of $P$ are $x_{j-1}$ and $x_{j}$, and $P$ only contains vertices of $\notS_{j-2}$; and we say that a path $P$ in $H$ is a \emph{middle inner path} of $e$, iff path $P$ sequentially visits vertices $x_{i+1}, x_{i+2},\dots,x_{j-1}$.
We say that a path $P$ is an \emph{inner path} of $e$, iff $P$ is the union of (i) a left inner path of $e$; (ii) a middle inner path of $e$; and (iii) a right inner path of $e$.
See \Cref{fig: LMR_inner} for an illustration.

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.20]{figs/LMR_inner.jpg}
	\caption{An illustration of left inner path (orange), middle inner path (purple) and right inner path (green) of edge $(x_i,x_j)\in E'$.}\label{fig: LMR_inner}
\end{figure}

In the remainder of this subsection, we will additionally assume that we are given, for each edge $e\in E'$, an inner path $P_e$ of $e$ in graph $H$, such that the set $\set{P_e}_{e\in E'}$ of paths causes congestion at most $\eta$, for some $\eta=2^{O((\log m)^{3/4}\log\log m)}$.

We now provide the proof of \Cref{thm: disengagement - main} with these additional assumptions. 
\fi

Before we present the algorithm for proving \Cref{lem: path case} in several steps in the following subsections, we first introduce a crucial notion called \emph{bad index} in the following subsection.

%We will use the parameters $\eta=2^{O((\log m)^{3/4}\log\log m)}$, $\beta^*=2^{O(\sqrt{\log m}\cdot \log\log m)}$, and $\eta^*=2^{O((\log m)^{3/4}\log\log m)}$. \znote{parameters to change}


%Define $E'=E(H)\setminus (\bigcup_{1\le i\le r-1}\hat E_i)$. Equivalently, $E'$ is the subset of $E^{\out}(\cset)$ that contains all edges connecting a pair $C_i,C_j$ of clusters in $\cset$, with $j\ge i+2$, and when $E'$ is viewed as a set of edges in $H$, then $E'$ contains all edges connecting a pair $x_i,x_j$ of vertices in $H$ with $j\ge i+2$.



\input{bad_index}


\subsubsection{Completing the proof of \Cref{lem: path case}}


In this subsection we present the algorithm for \Cref{lem: path case}.

%For an index $i'$ and an interval $[a,b]$, we say that $i'$ is \emph{properly contained} in $[a,b]$, iff $a<i'<b$.
We denote by $\bset$ the set of all bad indices.
%For each index $i\in \bset$, we define interval $J_i=[\LMP(i),\RMP(i)-1]$ as the \emph{\own interval} of index $i$. 
Let $i,i'$ be a pair of distinct bad indices in $\bset$. We say that $i$ \emph{dominates} $i'$ iff $\LMP(i)<i'<\RMP(i)-1$. Note that \Cref{obs: bad index non-interleaving} simply says that no two bad indices can dominate each other.


\subsubsection*{Step 1. Selecting a subset of bad indices}

\begin{claim}
\label{clm: select bad indices}
We can efficiently compute a set $\bset'\subseteq\bset$ of bad indices, such that (i) for every pair $i,i'$ of bad indices of $\bset'$, neither $i$ dominates $i'$ nor $i'$ dominates $i$; and (ii) for each $i\in \bset$, either $i\in \bset'$ or there exists some $i'\in \bset$ such that $i'$ dominates $i$. 
\end{claim}

\begin{proof}
We construct a directed graph $L$ as follows. Its vertex set $V(L)=\bset$. For every pair $i,i'\in \bset$, the directed edge $(i,i')$ belongs to $L$ iff $i$ dominates $i'$. We first show that $L$ is acyclic. Note that from similar arguments in \Cref{obs: bad index non-interleaving}, we can show that if $i$ dominates $i'$, then $|\hat E_i|\le |\hat E_{i'}|/2000$. Therefore, if $L$ contains a cycle $(i_1,i_2,\ldots,i_k,i_1)$, then 
\[
|\hat E_1|\le \frac{|\hat E_{2}|}{2000} \le \frac{|\hat E_{3}|}{2000^2}\le \cdots\le   \frac{|\hat E_{k}|}{2000^{k-1}}\le  \frac{|\hat E_{1}|}{2000^k}\text{ },
\]
a contradiction, so $L$ is acyclic. We call the vertices of $L$ with no out-edges \emph{sources}. Since $L$ is acyclic, it must contain at least one source. We then repeatedly perform the following operation until $L$ becomes an empty graph: select a source of $L$, add it to $\bset'$, and then delete this source and all its out-neighbors from $L$. Clearly, after each operation, graph $L$ remains acyclic. Let $\bset'$ be the resulting set of indices. It is easy to verify that $\bset'$ satisfies the required properties in \Cref{clm: select bad indices}.
\end{proof}

\iffalse
For each $1\le j< j'\le r$, we define $C_{[j,j']}=\bigcup_{j\le t\le j'}C_t$,
$C_{(j,j']}=\bigcup_{j< t\le j'}C_t$,
$C_{[j,j')}=\bigcup_{j\le t< j'}C_t$, and
$C_{(j,j')}=\bigcup_{j< t< j'}C_t$. 
And we define clusters $X_{[j,j']},X_{(j,j']},X_{[j,j')},X_{(j,j')}$ in $H$ similarly.
We say that a partition of $C_{[j,j']}$ into clusters $Y_1,\ldots, Y_k$ is \emph{$\cset$-respecting}, iff each $Z_s$ is the union of a set of consecutive clusters in $\set{C_j,\ldots,C_{j'}}$. In other words, there exist indices $j<i_1<\cdots <i_{k-1}<j'$, such that for each $1\le s\le k$, $Z_s=C_{[i_{s-1}+1, i_s]}$ (where $j=i_0$ and $j'=i_k$).
\fi


\subsubsection*{Step 2. Dealing with unbonded pairs}


We define the sequence $\sigma=(i_1,i_2,\ldots,i_k)$ where indices $i_1<i_2<\cdots<i_k$ are bad indices in set $\bset'$ given by \Cref{clm: select bad indices}. We say that a pair $i_j,i_{j+1}$ of consecutive indices in $\sigma$ are \emph{bonded}, iff $i_j=\LMP(i_{j+1})$ and $i_{j+1}=\RMP(i_{j})-1$. 
We say that a consecutive subsequence $\sigma_{[j,j']}=(i_{j},i_{j+1},\ldots,i_{j'})$ is \emph{bonded}, iff for each $j\le s<j'$, the pair $i_{s},i_{s+1}$ of indices are bonded.

We use the following claim.


\begin{claim}
\label{clm: dealing with non-bonding indices}
If a pair $i_j,i_{j+1}$ of consecutive indices in $\bset'$ are not bonded, then we can efficiently find a $\cset$-respecting partition of $C_{(i_j,i_{j+1}]}$ into \singlecore clusters $\yset=\set{Y_1,\ldots,Y_k}$ (with $k\ge 2$), such that for every $1\le s\le k-1$, the pair $Y_s,Y_{s+1}$ of clusters are nice.
\end{claim}

\begin{proof}
For convenience, we denote $a=i_j$ and $b=i_{j+1}$. We distinguish between the following cases.

\textbf{Case 1. $\RMP(a)\le \LMP(b)$.}
In this case we define $Y_1=C_{(a,\RMP(a))}$, $Y_2=C_{\RMP(a)}$, \ldots, $Y_{k-1}=C_{\LMP(b)}$ and $Y_k=C_{(\LMP(b),\RMP(b)]}$. See \Cref{fig: unbonded case 1} for an illustration. 
%
We first show that all cluster $Y_1,\ldots,Y_k$ are \singlecore. First, it is clear that clusters $Y_2,\ldots,Y_{k-1}$ are \singlecore, since each of them contains a single cluster of $\cset$, and each cluster in $\cset$ has the $\alpha_0$-bandwidth property. Consider now the cluster $Y_1$. From \Cref{claim: inner and outer paths}, there is a set of paths routing the edges of $\delta_H(X_{(a,\RMP(a))})$ to $x_{\RMP(a)-1}$ in $X_{(a,\RMP(a))}$ with congestion $O(1)$, so cluster $X_{(a,\RMP(a))}$ has the $O(1)$-bandwidth property in $H$. From \Cref{clm: contracted_graph_well_linkedness}, the cluster $C_{(a,\RMP(a))}$ has the $O(\alpha_0)$-bandwidth property in $G$, and is therefore \singlecore by definition. Similarly, we can show that cluster $Y_k$ is also \singlecore.

%From \Cref{lem: GH tree path vs contraction}, the Gomory-Hu tree $\tau'$ of the contracted graph $C'_{\mid \zset}$ is the path $(y_1,\ldots,y_k)$, where $y_s$ is the node that represents the cluster $Y_s$, for each $1\le s\le k$. We now show that $\tau'$ does not contain a bad index.

We now show that every pair $Y_s,Y_{s+1}$ of consecutive clusters are nice.
From \Cref{clm: contraction does not create new bad indices}, it suffices to show that  every index $i$ satisfying that $\RMP(a)-1\le i\le \LMP(b)$ is not a bad index. In fact, since $a,b$ are consecutive bad indices in $\bset'$, if $i$ is a bad index, then it is not dominated by any index in $\bset'$, contradicting the property guaranteed by 
\Cref{clm: select bad indices}. Therefore, for each $1\le s\le k-1$, the pair $Y_s,Y_{s+1}$ of consecutive clusters are nice.

\textbf{Case 2. $\RMP(a)> \LMP(b)$.} In this case we consider all indices between $\LMP(b)$ and $\RMP(a)$. Assume first that there exists an index $\LMP(b)\le i^*<  \RMP(a)$ that is not a bad index, we then set $Y_1=C_{(a,i^*]}$ and $Y_2=C_{(i^*,b]}$. From similar arguments in Case 1 (using \Cref{claim: inner and outer paths} and \Cref{clm: contracted_graph_well_linkedness}), we can show that clusters $Y_1,Y_2$ are \singlecore. Then from \Cref{clm: contraction does not create new bad indices}, since $i^*$ is not a bad index, the pair $Y_1,Y_2$ of clusters are nice.

Assume now that all indices $\LMP(b)\le i<  \RMP(a)$ are bad indices. First observe that $\RMP(a)\ge \LMP(b)+2$, since if $\RMP(a)=\LMP(b)+1$ then the index $\LMP(b)$ is not dominated by any index in $\bset'$, a contradiction. Second, if there exists an index $\LMP(b)\le i<  \RMP(a)$, such that at least one of $\LMP(i)=a, \RMP(i)=b+1$ does not hold, then we set $Y_1=C_{(a,i]}$ and $Y_2=C_{(i,b]}$. From similar arguments in Case 1, we can show that clusters $Y_1,Y_2$ are \singlecore. To see why the pair $Y_1,Y_2$ are nice, assume without loss of generality that $\LMP(i)\ne a$, so  $\LMP(i)> a$ since otherwise the bad indices $i$ and $a$ dominate each other, a contradiction to \Cref{obs: bad index non-interleaving}. Then $C_{\LMP(i)}\subseteq Y_1$. From the definition of $\LMP(i)$, we get that $|E(Y_1,Y_2)|\ge |E^{\lef}_i|/2$, so $Y_1,Y_2$ are nice by definition. If all indices $\LMP(b)\le i<  \RMP(a)$ satisfy that $\LMP(i)=a$ and $\RMP(i)=b+1$, then clearly, the two indices $\LMP(b), \LMP(b)+1$ dominate each other, a contradiction to \Cref{obs: bad index non-interleaving}. 
%
%
%
%
\begin{figure}[h]
	\centering
	\subfigure[The clusters $Y_1,\ldots,Y_k$ in Case 1.]{\scalebox{0.12}{\includegraphics{figs/unbonded_case1.jpg}}\label{fig: unbonded case 1}
	}
	\hspace{4pt}
	\subfigure[The clusters $Y_1,Y_2$ in Case 2.]{\scalebox{0.12}{\includegraphics{figs/unbonded_case2.jpg}}\label{fig: unbonded case 2}}
	\caption{An illustration of partition $\yset$ in \Cref{clm: dealing with non-bonding indices}.}%\label{fig: path_cluster}
\end{figure}
%
%
\end{proof}




\subsubsection*{Step 3. Construct the clusters and path sets}

We denote by $\Pi$ the set of all maximal bonded subsequences of $\sigma$. Here we also view a subsequence that contains an single index $i_j\in \sigma$ as a bonded subsequence.
Let $\Pi=\set{\sigma_{[j_s,j'_s]}\mid 1\le s\le p}$.
We now construct the set $\zset$ of clusters in \Cref{lem: path case} as follows.

For each $1\le s\le p-1$, we apply the algorithm from \Cref{clm: dealing with non-bonding indices} to the pair $j'_s,j_{s+1}$ of bad indices that are not bonded. Let $Y'_s, Y_{s+1}$ be the first and the last helpful cluster we get, and let $\yset_s$ be the set of all other helpful clusters we get.
Additionally, we define $Y_1=C_{(\LMP(i_{j_1}),i_{j_1})}$ and $Y'_s=C_{(i_{j_p},\RMP(i_{j_p})]}$, and we define $\yset_{0}=\set{C_1,\ldots,C_{\LMP(i_{j_1})}}$ and
$\yset_{p}=\set{C_{\RMP(i_{j_p})},\ldots,C_{r}}$.

We let set $\zset$ contains: (i) for each $0\le s\le p$, all clusters in $\yset_s$; and (ii) for each $1\le s\le p$, a cluster $Z_s=Y_s\cup C_{(i_{j_s},i_{j'_s}]}\cup Y'_{s}$. Clearly, the clusters in $\bigcup_{0\le s\le p}\yset_s$ are all \singlecore clusters. 

\paragraph{Constructing the set $\pset=\set{P_e\mid e\in E'}$ of auxiliary paths.}
From the above discussion, since every pair of consecutive clusters in $\bigcup_{0\le s\le p}\yset_s$ are nice, from \Cref{cor: nice pairs imply no bad index}, the Gomory-Hu tree of the contracted graph $G_{\mid\zset}$ is a path with no bad index. We now compute the set of auuxiliary paths as follows.
We process edges in $E'$ one-by-one. Throughout, for each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, we maintain an integer $z_{\hat e}$ indicating how many times the edge $\hat e$ has been used, that is initialized to be $0$. 
%Throughout, all edges of $\in \bigcup_{1\le i\le k-1}\hat E_i$ are either marked \emph{used} or \emph{not used}. Initially, all edges are not used.
Consider an iteration of processing an edge $e\in E'$. Assume $e$ connects $C_i$ to $C_j$ in $G$, we then pick, for each $i\le t\le j-1$, an edge $\hat e$ of $\hat E_t$ with minimum $z_{\hat e}$ over all edges of $\hat E_t$, and let $P_e$ be the path obtained by taking the union of all picked edges.
Note that, in $H$, each edge of $\hat E_t$ connects $x_t$ to $x_{t+1}$, so the path $P_e$ sequentially visits nodes $x_i, x_{i+1},\dots,x_j$. 
We then increase the value of $z_{\hat e}$ by $1$ for all picked edges $\hat e$, and proceed to the next iteration. After processing all edges of $E'$, we obtain a set $\pset=\set{P_e}_{e\in E'}$ of paths in $H$.
We use the following observation.

\begin{observation}
	\label{obs:central_congestion}
	For each edge $\hat e\in \bigcup_{1\le i\le k-1}\hat E_i$, $\cong_{H}(\pset,\hat e)\le 5000$.
	%The paths in $\tilde\pset$ are edge-disjoint.
\end{observation}
\begin{proof}
	From the algorithm, for each $1\le i\le k-1$, the paths of $\pset$ that contains an edge of $\hat E_i$ are $\set{P_e\mid e\in \big(E_i^{\rig} \cup E_{i+1}^{\lef} \cup E_i^{\through}\big)}$.
	Since $|E_i^{\rig}|+|E_{i+1}^{\lef}|+|E_i^{\through}|\le 5000|\hat E_i|$, each edge of $\hat E_i$ is used at most $5000$ times. Observation~\ref{obs:central_congestion} then follows.
\end{proof}


\paragraph{Constructing the path sets for \dualcore clusters.}
We now show that, for each $1\le s\le p$, the cluster $Z_s$ is an \dualcore cluster, and construct the sets $\qset^{\lef}_{s},\qset^{\rig}_{s},\qset^{\thr}_{s}$ of paths.
%
%

Recall that $Z_s=Y_s\cup C_{(i_{j_s},i_{j'_s}]}\cup Y'_{s}$. 
%See \Cref{fig: unhelpful path 1} for an illustration.
For convenience, we rename $Z_s$ by $Z$, $Y_s$ by $Y$ and $Y'_s$ by $Y'$. We denote $Z=C_{[a,b]}$ and denote by $i_1,\ldots,i_k$ the bonded consecutive subsequence of $\sigma$ that belongs to $Z$, so $Y=C_{[a,i_1]}$ and  $Y'=C_{(i_k,b]}$.
Moreover, for each $1\le t\le k-1$, $\RMP(i_t)=i_{t+1}+1$ and $\LMP(i_{t+1})=i_{t}$.

We first set the left and right centers of $Z$ as follows.
Exactly the same as in \Cref{sec: guiding and auxiliary paths}, for each $a\le t\le b$, we apply the algorithm \algclassifycluster from \Cref{thm:algclassifycluster} to the instance and (potentially) the algorithm from \Cref{lem: simple guiding paths} to get a set $\qset_t$ of paths routing edges of $\delta_G(C_t)$ to a vertex $u_t\in C_t$.
We then set the left center of $Z$ to be $u^{\lef}=u_a$ and the right center of $Z$ to be $u^{\rig}=u_b$.

%We now start constrcting the sets $\qset^{\lef},\qset^{\rig},\qset^{\thr}$ of paths for cluster $Z$. 
%Note that, for each cluster $C_{t}$, we have obtained a set $\qset_t$ of paths routing edges of $\delta_G(C_t)$ to a vertex $u_t\in C_t$. 
We denote $\cset'=\set{C_a,\ldots,C_b}$ and consider the contracted graph $H'=G_{\mid \cset'}$. It is easy to verify that $H'$ is the subgraph of $H$ induced by vertices of $X_{[a,b]}$. 
We construct the set $\qset^{\thr}$ of paths as follows. From \Cref{obs: bad inded structure}, for each $a\le t\le b-1$, $|E(U_{a-1}, \notU_b)|\le |\hat E_t|$. Therefore, we can compute a set $\pset$ of edge-disjoint paths connecting to $x_a$ to $x_b$, that only use edges of $\bigcup_{a\le t\le b-1}\hat E_t$.
Then using the algorithm of \Cref{lem: convert path}, we convert the set $\pset$ into a set $\qset^{\thr}$ of paths.

Next, we denote $X^{\lef}=X_{[a,i_1]}$, $X^{\rig}=X_{(i_k,b]}$ and for each $1\le t\le k-1$, $X^t=X_{(i_{t},t_{t+1}]}$. 
%So $V(H')=V(X^{\lef})\cup V(X^{\rig})\cup \big(\bigcup_{1\le t\le k-1}V(X^t)\big)$.
From \Cref{claim: inner and outer paths},
there exists a set $\pset^{\lef}$ routing edges of $\delta_{H'}(X^{\lef})$ to $x_a$ inside $X^{\lef}$, with congestion $O(1)$; and similarly, there exists a set $\pset^{\rig}$ routing edges of $\delta_{H'}(X^{\rig})$ to $x_b$ inside $X^{\rig}$, with congestion $O(1)$.
Moreover, for each $1\le t\le k-1$, there exists a set of paths routing its boundary to some vertex inside it, with congestion $O(1)$. 
Consider now the contracted graph $H''$ obtained from $H'$ by contracting each cluster of $X^{\lef}, X^{\rig}, \set{X^t}_{1\le t\le k-1}, Y'_{s-1}, Y_{s+1}$ into a single vertex.
We denote by $y',y,w^{\lef},w^{\rig}$ the vertices of $H'$ that correspond to clusters $Y'_{s-1}, X^{\lef},X^{\rig},Y_{s+1}$, respectively. For each $1\le t\le k-1$, we denote by $w^t$ the vertex that corresponds to cluster $X^t$.
See \Cref{fig: unhelpful path} for an illustration.
We will construct sets of paths in $H''$ and then convert them into sets $\qset^{\lef},\qset^{\rig}$ of paths.
 
\begin{figure}[h]
	\centering
	\subfigure[Layout of part of $H'$.]{\scalebox{0.21}{\includegraphics{figs/unhelpful_path1.jpg}}\label{fig: unhelpful path 1}
	}
	\subfigure[Layout of part of $H''$.]{\scalebox{0.21}{\includegraphics{figs/unhelpful_path2.jpg}}\label{fig: unhelpful path 2}}
	\caption{An illustration of part of $H'$ and $H''$.}
	\label{fig: unhelpful path}
\end{figure}

Denote $W=\set{w^{\lef},w^{\rig}}\cup \set{w^t\mid 1\le t\le k-1}$ and $W'=W\cup \set{y,y'}$. We define $U^{\lef}$ to the set of vertices that correspond to vertices of $U_{a-1}$ in original graph $G$, and we define $U^{\rig}$ similarly.
Note that, from the construction of $H''$, for each $1\le t\le k-1$, $|E_{H''}(U^{\lef},W)|\le 2\cdot (|E(w^t,w^{t-1})|+|E(w^t,w^{t-1})|)$ (where $w^{\lef}=w^0$ and  $y'=w^{-1}$). Additionally, since the pair $Y'_{s-1},Y_s$ of clusters are nice, $|E(y',w^{\lef})|\ge |E_{H''}(U^{\lef},W)|/10000$.

Denote $E^{\lef}= E_{H''}(U^{\lef},W)$.
We construct a set $\hat \pset^{\lef}$ of paths that contains, for each edge $e\in E^{\lef}$, a path $\hat P^{\lef}_e$ connecting $e$ to $w^{\lef}$ within $W'$ as follows.
We first use similar arguments in the construction of $\qset^{\thr}$ to compute, for each edge $e\in E^{\lef}$ that is incident to $w^t$, a path $P'_e$ connecting $w^{t-1}$ to $w^{\lef}$, such that all these paths are edge-disjoint in $H''$. 
Next, for each edge $e\in E^{\lef}$ that is incident to $w^{\lef}$, we let $P^{\lef}_e$ be the single-edge-path $e$.
For each $2\le t\le k-1$ and for each edge $e\in E^{\lef}$ that is incident to $w^{1}$, we assign an edge $e^*$ of $E(w^t,w^{t-1})\cup E(w^t,w^{t-2})$, such that each edge of $E(w^t,w^{t-1})\cup E(w^t,w^{t-2})$ is assigned at most twice. Consider now an edge $e\in E^{\lef}$. If $e^*\in E(w^t,w^{t-1})$, then we define $\hat P^{\lef}_e$ to be the $e\cup e^*\cup P'_e$. If $e^*\in E(w^t,w^{t-2})$, then we define $\hat P^{\lef}_e$ to be the concatenation of $e$, $e^*$ and the subpath of $P'_e$ between $w^{t-2}$ and $w^{\lef}$.

\znote{below needs fixing, need to use the whole structure to treat edges of $E^{\lef}$ that is incident to $w^{1}$.}
Lastly, consider the edges of $E^{\lef}$ that is incident to $w^{1}$. For each $e\in E^{\lef}$, we assign an edge $e^*\in E(y',w^{\lef})$ to it, such that each edge of $E(y',w^{\lef})$ is assigned at most $10000$ times, and then we define $\hat P^{\lef}_e$ to be $e\cup e'$. This completes the definition of $\hat\pset^{\lef}$. It is easy to verify that $\cong_{H''}(\pset^{\lef})=O(1)$.

\znote{Use $\hat\pset^{\lef}, \pset^{\lef}$ and $\qset_a$ to get $\qset^{\lef}$, and similarly get $\qset^{\rig}$.}










==> prelim_backup.tex <==
\newpage

\section{Definitions, Notation, Known Results, and their Easy Extensions}
\label{sec:long prelim}

%\mynote{Once we finalize the order of the subsections, we'll need to reorder the subsections in the appendix accordingly.}  

%\mynote{I think it's a good idea to turn paragraphs into subsections, so they can be easily found from table of contents (e.g. if you are looking for some definitions)}


%\mynote{For this paper, all graphs by default should have parallel edges, and graphs with no parallel edges should be called simple graphs.}
%\mynote{It may be good to revisit the various results from prelims to double-check that they work for graphs with parallel edges (this is how we'll be using them).}
%By default, all logarithms in this paper are to the base of $2$. All graphs are undirected and finite. Graphs may contain parallel edges but they may not contain self loops. Graphs without parallel edges are explicitly referred to as simple graphs.

In this section we provide additional definitions and notation, together with known results and their easy extensions that we use throughout the paper.

All graphs that we consider in this paper are undirected. However, it will sometimes be convenient for us to assign direction to paths in such graphs. We do so by designating one endpoint of the path as its first endpoint, and another endpoint as its last endpoint. We will then view the path as being directed from its first endpoint towards its last endpoint. We will sometimes refer to a path with an assigned direction as a directed path, even though the underlying graph is an undirected graph.



\subsection{Clusters and Augmentations of Clusters}
We will refer to vertex-induced subgraphs of $G$ as 
\emph{clusters}. For a set $\cset$ of disjoint clusters of $G$, we denote by $\inE_G(\cset)$ the set of edges connecting distinct clusters of $\cset$.
We sometimes omit the subscript $G$ when clear from the context. 


Given a cluster $C$ in a graph $G$, and a path $P$ in $G$, whose endpoints are $u$ and $v$ we say that $P$ is \emph{internally disjoint} from $C$, iff $V(C)\cap V(P)\subseteq \set{u,v}$.

Next, we define the notaion of augmentation of a cluster.

\begin{definition}[Augmentation of Clusters]
	\label{def: Graph C^+}
	Let $C$ be a cluster of $G$. The graph $C^+$, that is called the \emph{augmentation} of cluster $C$, is defined as follows. First, we subdivide every edge $e\in \delta_G(C)$ with a vertex $t_e$, and let $T(C)=\set{t_e\mid e\in \delta_G(C)}$ be the set of newly added vertices, that we sometimes refer to as \emph{terminals of $C$}. We then let $C^+$ be the subgraph of the resulting graph induced by $V(C)\cup T(C)$.
\end{definition}

%\subsection{Faces, Identical Drawings}
%\label{sec: prelim_crossing_notations}

\iffalse
Throughout the paper, we use the following definition.

\begin{definition}[Curves in general position]
Let $\Gamma$ be a set of of simple curves in the plane.
We say that the curves of $\Gamma$ are \emph{in general position}, iff the following four conditions hold:

\begin{itemize}
	\item for every pair $\gamma,\gamma'\in \Gamma$ of distinct curves, there is a finite number of points $p$ with $p\in \gamma\cap  \gamma'$;
	%\item for every curve $\gamma\in \Gamma$, there is a finite number of points that appear on $\gamma$ more than once as we traverse $\gamma$ from one endpoint to another; each such point $p$ may appear on $\gamma$ at most twice, and it may not appear on any other curve in $\Gamma$;
	\item if a point $p$ is an endpoint of a curve in $\Gamma$, then it may not be an inner point on any curve in $\Gamma$; and 
	\item if a point $p'$ is contained in more than two curves in $\Gamma$, then it may not be an inner point on any curve in $\Gamma$.
\end{itemize}
\end{definition}
%\znote{directly define ``simple curves in general position''?}

Given a set $\Gamma$ of curves in general position, a \emph{crossing} between a pair $\gamma,\gamma'\in \Gamma$ of curves is a point $p$ that is an inner point on both $\gamma$ and $\gamma'$.
We also say that curves $\gamma,\gamma'$ cross at point $p$.

\iffalse
We will sometimes distinguish between two types of crossings of curves: \emph{transversal} and \emph{non-transversal}.

\begin{definition}[Transversal crossing of curves]
Let $\Gamma$ be a set of curves in general position, and let $\gamma,\gamma'\in \Gamma$ be two distinct curves that cross at point $p$. Let $D$ be an arbitrarily small disc that contains $p$ in its interior. Let $q_1,q_2$ be the points of $\gamma$ lying on the boundary of $D$, and let $q_1',q_2'$ be the points of $\gamma'$ lying on the boundary of $D$. We say that the crossing $p$ between $\gamma$ and $\gamma'$ is \emph{transversal} iff the points $q_1,q_1',q_2,q_2'$ appear in this circular ordering on the boundary of $D$; otherwise, we say that the crossing is \emph{non-transversal}. If the crossing $p$ between $\gamma$ and $\gamma'$ is non-transversal, then we sometimes say that $\gamma$ and $\gamma'$ \emph{touch} at point $p$.
\end{definition}
\fi


We are now ready to define a graph drawing.

\begin{definition}[Graph Drawing and Crossings]
A \emph{drawing}  $\phi$ of a graph $G$ is an embedding of $G$ into the plane, that maps every vertex $v$ of $G$ to a point $\phi(v)$ (called the \emph{image of $v$}), and every edge $e=(u,v)$ of $G$ to a simple curve $\phi(e)$  (called the \emph{image of $e$}), whose endpoints are $\phi(u)$ and $\phi(v)$, such that the set $\set{\phi(e)\mid e\in E(G)}$ of curves is in general position. If $p$ is an inner point on images $\phi(e),\phi(e')$ of distinct edges $e,e'\in E(G)$,
%(where possibly $e=e'$)\znote{I think $e=e'$ is not allowed? otherwise if $e=e'$, from the current definition all points in curve $\phi(e)=\phi(e')$ are crossings}, 
then we say that edges $e$ and $e'$ \emph{cross} at $p$, and that $p$ is a \emph{crossing} in the drawing $\phi$, that we also sometimes denote by $(e,e')_p$, where $(e,e')$ is an unordered pair (omitting the subscript $p$ if the crossing is uniquely defined). We denote by $\cro(\phi)$ the total number of crossings in the drawing $\phi$. If $\cro(\phi)=0$, then we say that the drawing $\phi$ is \emph{planar}.
\end{definition}


\iffalse
that connects the images of its endpoints. We require that the interiors of the curves representing the edges do not contain the images of any of the vertices. We say that two edges \emph{cross} at a point $p$, if the images of both edges contain $p$, and $p$ is not the image of a shared endpoint of these edges. We require that no three edges cross at the same point in a drawing of $\phi$. 
We say that $\phi$ is a \emph{planar drawing} of $G$ iff no pair of edges of $G$ crosses in $\phi$.
For a vertex $v\in V(G)$, we denote by $\phi(v)$ the image of $v$, and for an edge $e\in E(G)$, we denote by $\phi(e)$ the image of $e$ in $\phi$. 
\fi



Note that a drawing of $G$ in the plane naturally defines a drawing of $G$ on the sphere and vice versa; we use both types of drawings.
\fi

%Let $\phi$ be a drawing of graph $G$. For any subgraph $C$ of $G$, we denote by $\phi(C)$ the union of images of all vertices and edges of $C$ in $\phi$, and we call $\phi(C)$ the \emph{image of $C$ in $\phi$}. We denote by $\chi^1_{\phi}(C)$ the number of crossings $(e,e')_p$ in drawing $\phi$, where exactly one of the edges $e,e'$ belongs to $C$. Similarly, we denote by $\chi^2_{\phi}(C)$ the number of crossings $(e,e')_p$ in $\phi$, where both edges $e,e'$ belongs to $C$. Additionally, we define $\chi_{\phi}(C)=\chi^1_{\phi}(C)+\chi^2_{\phi}(C)$. For two (not necessarily disjoint) clusters $C,C'$ of $G$, we denote by $\chi_{\phi}(C,C')$ the number of crossings $(e,e')_p$ in drawing $\phi$, where $e\in C$ and $e'\in C'$. Note that the clusters $C,C'$ are allowed to share edges, so a crossing $(e,e')_p$ with $e,e'\in E(C)\cap E(C')$ is counted twice in $\chi_{\phi}(C,C')$. For a set $\cset$ of clusters in $G$ and another cluster $C'\notin \cset$, we define $\chi^1_{\phi}(\cset)=\sum_{C\in \cset}\chi^1_{\phi}(C)$, $\chi^2_{\phi}(\cset)=\sum_{C\in \cset}\chi^2_{\phi}(C)$, $\chi_{\phi}(\cset)=\sum_{C\in \cset}\chi_{\phi}(C)$, and $\chi_{\phi}(\cset,C')=\sum_{C\in \cset}\chi_{\phi}(C,C')$.
%In particular, for a cluster $C$ of $G$, $\chi_{\phi}(C,G)$ is the total number of crossings $(e,e')_p$, where at least one edge $e,e'$ lies in $C$. We may omit the subscript $\phi$ in the above notations when the drawing is prescribed or clear from the context.








\subsection{Curves in a Plane or on a Sphere}

\subsubsection{Reordering Curves}

Assume that we are given two oriented orderings $(\oset,b)$ and $(\oset',b')$ of elements in set $U=\set{u_1,\ldots,u_r}$. Assume for simplicity that $b=b'=0$ (otherwise the corresponding ordering can be flipped).  Consider a disc $D$, with a collection $\set{p_1,\ldots,p_r}$ of distinct points appearing on the boundary of $D$ (where we view each point $p_i$ as representing element $u_i$ of $U$), whose clock-wise order on the boundary of $D$ is precisely $\oset$. Similarly, let $D'\subseteq D$ be any other disc that is strictly contained in $D$, with a collection $\set{p'_1,\ldots,p'_r}$ of points appearing on the boundary of $D'$, where for $1\leq i\leq r$, point $p'_i$ represents element $u_i\in U$, such that the clock-wise order of the points in $\set{p'_1,\ldots,p'_r}$ on the boundary of $D$ is precisely $\oset'$. 

For two unoriented orderings $\oset,\oset'$ on $U$, we define $\dist(\oset,\oset')=\min_{b,b'\in \set{0,1}}\set{\dist((\oset,0),(\oset',b'))}$.


\begin{definition}[Reordering curves]
We say that a collection $\Gamma=\set{\gamma_1,\ldots,\gamma_r}$ of curves is a \emph{set of reordering curves for $(\oset,b)$ and $(\oset',b')$} iff the  curves in $\Gamma$ are simple curves in general position, the interior of every curve $\gamma_i\in \Gamma$ is contained in $D\setminus D'$, and, for all $1\leq i\leq r$, curve $\gamma_i$ has $p_i,p'_i$ as its endpoints. The \emph{cost} of the collection $\Gamma$ of curves is defined to be the total number of crossings between these curves.
\end{definition}

\begin{definition}[Distance between orderings]
	Let $(\oset,b)$ and $(\oset',b')$ be two oriented orderings of a collection $U$ of elements. The \emph{distance} between the two orderings, denoted by $\dist((\oset,b),(\oset',b'))$, is the smallest cost of any set $\Gamma$ of reordering curves for  $(\oset,b)$ and $(\oset,b')$.
\end{definition}





We use the following lemma, whose proof is provided Appendix~\ref{apd: Proof of find reordering}.
\begin{lemma}
\label{lem: ordering modification}
There is an algorithm, that, given a set $U$ of elements, a set $\Gamma=\set{\gamma_u\mid u\in U}$ of curves that shares an endpoint $z$, and two circular orderings $\oset,\oset'$ on elements of $U$, such that the curves of $\Gamma$ enter $z$ in the order $\oset$, computes a new set $\Gamma'=\set{\gamma'_u\mid u\in U}$ of curves, such that:
\begin{itemize}
\item the curves of $\Gamma'$ enter $z$ in the order $\oset'$;
\item for each $u\in U$, the curve $\gamma_u$ differs from the curve $\gamma'_u$ only within some tiny disc $D$ that contains $z$; and
\item  the number of crossings between curves of $\Gamma'$ within $D$ is $O(\dist(\oset,\oset'))$.
\end{itemize}
\end{lemma}


%Whitney \cite{whitney1992congruent} proved that every $3$-connected planar graph has a unique planar drawing. Throughout, for a $3$-connected planar graph $G$, we denote by $\rho_G$ the unique planar drawing of $G$.






\iffalse
\subsection{Problem Definitions}

In the \mcn~problem, the input is an $n$-vertex graph $G$, and the goal is to compute a drawing of $G$ in the plane with minimum number of crossings.
The value of the optimal solution, also called the \emph{crossing number} of $G$, is denoted by $\optcro(G)$.

We also consider a closely related problem called Crossing Number with Rotation System (\CNwRS). In this problem, the input is a graph $G$, and, for every vertex $v\in V(G)$, a circular ordering $\oset_v$ of the set $\delta_G(v)$ of edges. The collection $\Sigma=\set{\oset_v}_{v\in V(G)}$ of all these orderings is called a \emph{rotation system} of $G$.  We say that a drawing $\phi$ of $G$ \emph{respects} the rotation system $\Sigma$ if the following holds. For a vertex $v\in V(G)$, let $D(v)$ be an arbitrarily small disc around $v$ in $\phi$. Then the images of the edges of $\delta_G(v)$ in $\phi$ must intersect the boundary of $\eta(v)$ in a circular order that is identical to $\oset_v$ (but the orientation of this ordering may be arbitrary).
%We denote by $\Phi(G,\Sigma)$ the set of all drawings of $G$ that respects the rotation system $\Sigma$. In the \CNwRS problem, the input is a {\bf multigraph} $G$ with a rotation system $\Sigma$, and 
Given an instance $I=(G,\Sigma)$ of the \CNwRS problem, we say that a drawing $\phi$ of $G$ is a \emph{feasible solution} for $I$ iff $\phi$ respects the rotation system $\Sigma$. The \emph{cost} of the solution is the number of crossings in $\phi$. The goal in the \CNwRS problem is to compute a feasible solution to the given instance $I$ of the problem of smallest possible cost. We denote the cost of the optimal solution of the \CNwRS instance $I$ by $\optcrors(I)$.


We use the following simple theorems about the \CNwRS problem, whose proofs are deferred to 
Appendix~\ref{apd: Proof of crwrs_planar} and Appendix~\ref{apd: Proof of crwrs_uncrossing}, respectively.
\begin{theorem}
	\label{thm: crwrs_planar}
	There is an efficient algorithm, that, given an instance $I=(G,\Sigma)$ of \CNwRS, determines if $\optcrors(I)=0$, and, if so, computes a feasible solution of cost $0$.
\end{theorem}


\begin{theorem}
	\label{thm: crwrs_uncrossing}
	There is an efficient algorithm, that given an instance $I=(G,\Sigma)$ of \CNwRS, computes a feasible solution to instance $I$, of cost at most $|E(G)|^2$.
\end{theorem}

We refer to the solution computed by the algorithm from Theorem~\ref{thm: crwrs_uncrossing} as a \emph{trivial solution} to instance $I=(G,\Sigma)$.



%\mynote{I deleted the $\alpha$-decomposition section here. There is a different definition of this in the overview section (and we need the variant that was defined there). The definition needs a definition of subinstance so it's better suited to that section.}

\iffalse
\subsection{$\alpha$-Decompositions of an \CNwRS Instance}

Let $I=(G,\Sigma)$ be an instance of \CNwRS, let $\cset$ be a set of vertex-disjoint clusters of $G$ such that the sets $\set{V(C)}_{C\in \cset}$ partition $V(G)$, and let $\alpha>0$ be a real number. An \emph{$\alpha$-decomposition of $I$ with respect to $\cset$} is a collection $\iset$ of instances of \CNwRS with the following properties:
\begin{enumerate}
	\item  \label{prop: alpha deco 1} for each subinstance $I'=(G',\Sigma')\in \iset$, there is at most one cluster $C\in \cset$ with $E(C)\subseteq E(G')$; all other edges of $G'$ lie in set $\Eout(\cset)$;
	
	\item \label{prop: alpha deco 2} $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\leq O(|E(G)|)$; and
	\item \label{prop: alpha deco 3} $\sum_{I'\in \iset}\optcrors(I')\leq \alpha\cdot \big(\optcrors(I)+|E(G)| \big)$.
\end{enumerate}

We say that a randomized algorithm $\aset$ computes an $\alpha$-decomposition of instance $I=(G,\Sigma)$ with respect to $\cset$, if it computes a random family $\iset$ of subinstances that satisfies Property~\ref{prop: alpha deco 1} and Property~\ref{prop: alpha deco 2}, and the following property in replace of Property~\ref{prop: alpha deco 3}:
\[\expect{\sum_{I'\in \iset}\optcrors(I')}\leq \alpha\cdot \bigg(\optcrors(I)+|E(G)|\bigg).\]
\fi



\subsection{Subinstances}\label{subsec: subinstance}
Our algorithm for solving the \CNwRS problem is recursive. Given the input instance $I^*=(G^*,\Sigma^*)$ of \cnwrs,  it will consider various  instances $(G,\Sigma)$ of the problem, that we call \emph{subinstances} of $I^*$. We use the following definition of subinstances.



\begin{definition}[Subinstances]
	Let $I=(G,\Sigma)$ and $I'=(G',\Sigma')$ be two instances of \cnwrs. We say that instance $I'$ is a \emph{subinstance} of instance $I$, if there is a subgraph $\tilde G\subseteq G$, and a collection $S_1,\ldots,S_r$ of mutually disjoint subsets of vertices of $\tilde G$, such that graph $G'$ can be obtained from $\tilde G\subseteq G$ by contracting, for all $1\leq i\leq r$, every vertex set $S_i$ into a supernode $u_i$;  we keep parallel edges but remove self-loops. We do not distiguish between the edges incident to the supernodes in graph $G'$ and their counterparts in graph $G$.  Additionally, for every vertex $v\in V(G')\cap V(G)$, its rotation  $\oset'_v$ in $\Sigma'$ must remain the same as in $\Sigma$, while for every supernode $u_i$, its rotation $\oset_{u_i}$ can be defined arbitrarily.
\end{definition}	
	
Notice that subinstance relation is transitive: if $(G_1,\Sigma_1)$ is a subinstance of $(G_0,\Sigma_0)$, and $(G_2,\Sigma_2)$ is a subinstance of $(G_1,\Sigma_1)$, then $(G_2,\Sigma_2)$ is a subinstance of $(G_0,\Sigma_0)$.

\fi


\subsubsection{Curves in a Disc}
\label{sec: curves in a disc}
%\znote{need to decide what to keep in this subsection}


Suppose we are given a disc $D$, and a collection $\set{s_1,t_1,\ldots,s_k,t_k}$ of distinct points on the boundary of the disc $D$. For all $1\leq i< j\leq k$, we say that the two pairs  $(s_i,t_i),(s_j,t_j)$ of points \emph{cross} iff points $s_i,s_j,t_i,t_j$ are encountered in one of the following orderings when traversing the boundary of the disc in any direction: either $(s_i,s_j,t_i,t_j)$, or $(s_i,t_j,t_i,s_j)$.

We use the following simple claim, whose proof is deferred to \Cref{apd: Proof of curves in a disc}.

%\mynote{please add proof to appendix.  I have commented out previous nuding lemma and theorem. their proofs can be deleted from appendix. I haven't done it in case you want to use them in other parts. Relevant sections: \Cref{lem: non transversal cost of cycles bounded by cr}, \Cref{apd: Proof of curve_manipulation}, \Cref{apd: Proof of curves from non-transversal paths}.}

\begin{claim}\label{claim: curves in a disc}
There is an efficient algorithm that,  given a disc $D$, and a collection $\set{s_1,t_1,\ldots,s_k,t_k}$ of distinct points on the boundary of  $D$, computes a collection $\Gamma=\set{\gamma_1,\ldots,\gamma_k}$ of curves, such that, for all $1\leq i\leq k$, curve $\gamma_i$ has $s_i$ and $t_i$ as its endpoints, and its interior is contained in the interior of $D$. Moreover, for every pair $1\leq i<j\leq k$ of indices, if the two pairs  $(s_i,t_i),(s_j,t_j)$ of points cross then curves $\gamma_i,\gamma_j$ intersect at exactly one point; otherwise, curves $\gamma_i,\gamma_j$ do not intersect.
\end{claim} 






\subsubsection{Uncrossing of Curves}
In this subsection, we consider a set $\Gamma$ of curves in the plane that are in general position, and provide two different ways to ``simplify'' this collection of curves by \emph{uncrossing} them. The two types of uncrossings are referred to as \emph{type-$1$ uncrossing} and \emph{type-$2$ uncrossing}, respectively. With the first type of uncrossing, we ensure that, after the modification, each curve still has exactly the same endpoints as before, while we eliminate some of the crossings. With the second type of uncrossing we only ensure that the multiset containing the first endpoint of each curve and the multiset containing the last endpoint of each curve are preserved (but they may be matched to each other differently by the new curves). 



\subsubsection*{Type-1 Uncrossing}
%\mynote{NOte: we don't use the term "intersection" of curves anymore, it's always crossing, that may be transversal or non-transversal. This is to be consistent with how crossings in the drawing of $G$ is defined.}
%Let $\Gamma$ be a set of of curves in the plane.
%We say that the curves of $\Gamma$ are \emph{in general position}, iff every point in the plane that lies on more than $2$ curves of $\Gamma$ is an endpoint of all curves on which it lies.

Assume that we are given a set $\Gamma$ of curves that are in the general position, and let $\gamma,\gamma'\in \Gamma$ be a pair of distinct simple curves. Recall that we say that $\gamma,\gamma'$ \emph{cross} at a point $p$, iff $p$ belongs to both curves and $p$ is not an endpoint of either of these curves; such a point $p$ is also called an \emph{crossing} between the curves $\gamma,\gamma'$.
We denote by $\chi(\gamma, \gamma')$ the number of crossings between curves $\gamma,\gamma'$.
For a set $\Gamma$ of simple curves and another simple curve $\gamma\notin \Gamma$, such that the curves of $\set{\gamma}\cup \Gamma$ are in general position, we denote by $\chi(\gamma,\Gamma)$ the number of crossings between $\gamma$ and curves in $\Gamma$, that is,  $\chi(\gamma,\Gamma)=\sum_{\gamma'\in \Gamma}\chi(\gamma,\gamma')$. We also denote by $\chi(\Gamma)$ the total number of crossings between curves in $\Gamma$, namely  $\chi(\Gamma)=\sum_{\gamma,\gamma'\in \Gamma, \gamma\ne \gamma'}\chi(\gamma,\gamma')$.
%\mynote{in the above, are the curves simple? Note that if you talk about a general pair of curves, they may have infinite number of crossings, if they share contiguous segments. So when you talk about 2 curves they should be from set $\Gamma$ of curves that are in general position.}

Intuitively, when two distinct curves $\gamma,\gamma'\in \Gamma$ cross more than once, we can locally modify them in the way shown in Figure~\ref{fig:type_1_uncrossing}, so that each of the two curves still has the same endpoints, at least one crossing between the two curves is eliminated, and no new crossings between $\gamma,\gamma'$ and other curves are created.
We call this process, that is formally stated in the following theorem,  \emph{type-1 uncrossing}. The proof is standard and is provided in Appendix~\ref{apd: type-1 uncrossing} for completeness.

\begin{figure}[h]
	\centering
	\subfigure[Before: Curves $\gamma$ and $\gamma'$ cross twice,  at points $p$ and $q$, and they have two crossings in total with the pink curve twice.]{\scalebox{0.48}{\includegraphics{figs/type_1_uncross_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.8cm}
	\subfigure[After: Each of the new curves $\gamma$ and $\gamma'$ has same endpoints as before. The two curves no longer cross each other, and they still have two crossings in total with the pink curve.]{
		\scalebox{0.48}{\includegraphics{figs/type_1_uncross_2.jpg}}}
	\caption{An illustration of a type-1 uncrossing.}\label{fig:type_1_uncrossing}
\end{figure}


%\mynote{in the following theorem, are curves in $\Gamma$ and in $\Gamma'_1$ simple?  I didn't read the proof yet, but if you could switch "intersection" of curves to "crossing" there it would be great. Note also that I have added the first bullet which I think is necessary.}

\begin{theorem}[Type-1 Uncrossing]
	\label{thm: type-1 uncrossing}
	There is an efficient algorithm, that, given a set $\Gamma$ of simple curves in general position, that are partitioned into two disjoint sets $\Gamma_1,\Gamma_2$, computes, for each curve $\gamma\in \Gamma_1$, a simple curve $\gamma'$ that has same endpoints as $\gamma$, such that, if we denote by $\Gamma_1'=\set{\gamma'\mid \gamma\in \Gamma_1}$, then the following hold:
	\begin{itemize}
		\item curves of $\Gamma'_1\cup \Gamma_2$ are in general position;
		\item every pair of curves in $\Gamma_1'$ cross at most once;
		\item for every curve $\gamma\in \Gamma_2$, $\chi(\gamma,\Gamma'_1)\le \chi(\gamma,\Gamma_1)$; and
		\item $\chi(\Gamma'_1\cup\Gamma_2)\le \chi(\Gamma)$.
	\end{itemize}
\end{theorem}


\subsubsection*{Type-2 Uncrossing}

\znote{maybe modify the name of subsections?}

We will sometimes give a curve $\gamma$ a \emph{direction}, by designating one of its endpoints as its first endpoint, which we denote by $s(\gamma)$, and the other as its last endpoint, which we denote by $t(\gamma)$.
Given a set $\Gamma$ of directed curves, we denote $S(\Gamma)=\set{s(\gamma)\mid \gamma\in \Gamma}$ and $T(\Gamma)=\set{t(\gamma)\mid \gamma\in \Gamma}$, where both $S(\Gamma),T(\Gamma)$ are multisets.


Consider some graph $G$ and a drawing $\phi$ of $G$ in the plane. Recall that we have defined, for every vertex $v\in V(G)$, a disc $D_{\phi}(v)$, that we referred to as a \emph{tiny $v$-disc}. %\mynote{please define tiny $v$-disc earlier in prelims. Definition in email from March 23.}


%\mynote{I have added last two bullets to the definition.}
\begin{definition}
	Let $G$ be a graph and $\phi$ a drawing of $G$ in the plane.  We say that a curve $\gamma$ is \emph{aligned} with the drawing $\phi$ of $G$ iff there is a sequence $(e_1,e_2,\ldots,e_{r-1})$ of edges in $G$, and a partition $(\sigma_1,\sigma_1',\sigma_2,\sigma_2',\ldots,\sigma'_{r-1},\sigma_r)$ of $\gamma$ into consecutive segments, such that, if we denote, for all $1\leq i\leq r$, $e_i=(v_i,v_{i+1})$, then the following holds:
	
	\begin{itemize}
		\item for all $1\leq i\leq r-1$, segment $\sigma'_i$ is a contiguous segment of non-zero length of the image of the edge $e_i$ in $\phi$, and it is disjoint from all discs in $\set{D_{\phi}(u)}_{u\in V(G)}$, except that its first endpoint may lie on the boundary of of disc $D_{\phi}(v_i)$, and its last endpoint may lie on the boundary of disc $D_{\phi}(v_{i+1})$;
		
		\item for all $1\leq i\leq r$, segment $\sigma_i$ is either contained in disc $D_{\phi}(v_i)$, or it is empty. In the latter case, $1<i<r$ must hold, and, if we denote by $p$ the last endpoint of $\sigma'_{i-1}$, then $p$ is also the first endpoint of $\sigma'_{i+1}$, and it must be a point at which images of edge $e_{i-1}$ and edge $e_{i}$ cross; 
		
		\item segment $\sigma_1$ is precisely the part of the image of edge $e_1$ that is contained in $D_{\phi}(v_1)$;  and 
		
		\item segment $\sigma_r$ is precisely the part of the image of edge $e_{r-1}$ that is contained in $D_{\phi}(v_r)$.
	\end{itemize}
\end{definition}


%\mynote{I do need this theorem for the more general case where the inner vertices on the paths are not in $C$ but the endpoints are arbitrary. I need one more addition to the theorem: if the first endpoint of every path in $\qset$ is the same vertex $u^*$, then for each path $Q\in \qset$ whose first edge is denoted by $e_1(Q)$, curve $\gamma(Q)$ contains the segment of the image of $e_1(Q)$ that is lies in the disc $D_{\phi}(u^*)$.}
We use the following theorem, whose proof is deferred to \Cref{apd: new type 2 uncrossing}.

\begin{theorem}
	\label{thm: new type 2 uncrossing}
	There is an efficient algorithm, whose input contains a graph $G$, a drawing $\phi$ of $G$ on the sphere, a subgraph $C$ of $G$, and a collection $\qset$ of edge-disjoint paths in $G$ that are internally disjoint from $C$, such that, for each path $Q\in \qset$, one of its endpoints is designated as its first endpoint and is denoted by $s_Q$, the other endpoint, denoted by $t_Q$, is designated as its last endpoint. The algorithm computes a set $\Gamma=\set{\gamma(Q)\mid Q\in \qset}$ of directed simple curves on the sphere with the following properties:
	\begin{enumerate}
		
		\item every curve $\gamma(Q)\in \Gamma$ is aligned with the graph $\bigcup_{Q'\in \qset}Q'$;
		
		\item for each path $Q\in \qset$, $s(\gamma(Q))=\phi(s_Q)$; 
		\item if the first endpoint of every path in $\qset$ is the same vertex $u^*$, then for each path $Q\in \qset$ whose first edge (the edge incident to its first endpoint) is denoted by $e_1(Q)$, curve $\gamma(Q)$ contains the segment of the image of $e_1(Q)$ that is lies in the disc $D_{\phi}(u^*)$;
		
		\item the multiset $T(\Gamma)$ (containing the last endpoint of every curve in $\Gamma$) is precisely the multiset $\set{\phi(t_Q)\mid Q\in \qset}$; and
		\item the curves in $\Gamma$ do not cross each other.
		
		%\item \label{prop: inner point} for each edge $e=(u,v)\in E(G\setminus C)$, at most one curve in $\Gamma$ may contain a point of $\phi(e)\setminus (D_{\phi}(u)\cup D_{\phi}(v))$, and, if such a curve exists, then it contains the segment of the image of $e$ from a point on the boundary of $D_{\phi}(u)$ to a point on the boundary of $D_{\phi}(v)$; and
		
		%\item for each path $Q\in \qset$, if we denote by $e_Q=(t_Q,t'_Q)$ the edge of $Q$ that is incident to vertex $t_Q$, then some curve $\gamma(Q')\in \Gamma$ contains the segment of the image of $e_Q$ from a point on the boundary of $D_{\phi}(t_Q)$ to a point on the boundary of $D_{\phi}(t'_Q)$.
	\end{enumerate}
\end{theorem}	

Note that, from the definition of graph-aligned curves, and from the fact that the curves in $\Gamma$ do not cross each other, for every edge $e\in E(C)$, the number of crossings between the image of edge $e$ in $\phi$ and the curves in $\Gamma$ is bounded by the number of crossings between $e$ and edges of $G\setminus C$ in drawing $\phi$, namely $\chi(\phi(e),\Gamma)\le \chi_{\phi}(e, G\setminus C)$. We emphasize that the curves in $\Gamma$ may match the mutisets $\set{s(\gamma(Q))\mid Q\in \qset}$ and $\set{t(\gamma(Q))\mid Q\in \qset}$ differently from the paths in $\qset$.

We use the following corollary, whose proof is deferred to \Cref{apd: cor new type 2 uncrossing}.

\begin{corollary}
	\label{cor: new type 2 uncrossing}
	There is an efficient algorithm, whose input contains a graph $G$, a drawing $\phi$ of $G$ on the sphere, a subgraph $C$ of $G$, and a collection $\qset$ of  paths in $G$ that are internally disjoint from $C$, such that, for each path $Q\in \qset$, one of its endpoints is designated as its first endpoint and is denoted by $s_Q$, the other endpoint, denoted by $t_Q$, is designated as its last endpoint. The algorithm computes a set $\Gamma=\set{\gamma(Q)\mid Q\in \qset}$ of directed curves on the sphere with the following properties:
	
	\begin{itemize}
		\item for each path $Q\in \qset$, $s(\gamma(Q))=\phi(s_Q)$;
		\item the multiset $T(\Gamma)$ (containing the last endpoint of every curve in $\Gamma$) is precisely the multiset $\set{\phi(t_Q)\mid Q\in \qset}$;
		
		\item the curves in $\Gamma$ do not cross each other; and
		\item for each edge $e\in E(C)$, the number of crossings between the image of $e$ in $\phi$ and the curves in $\Gamma$ is bounded by the number of crossings between the image of $e$ and images of the edges of $G\setminus C$ times $\cong_G(\qset)$, namely $\chi(\phi(e),\Gamma)\le \chi_{\phi}(e, G\setminus C)\cdot \cong_G(\qset)$.
	\end{itemize}
\end{corollary}



\iffalse{the original type-2 uncrossing}

\znote{To check if the original type-2 uncrossing can be removed}

We will sometimes give a curve a \emph{direction}, by designating one of its endpoints as its first endpoint, and the other as its last endpoint.
Given a set $\Gamma$ of directed curves,
for every curve $\gamma\in \Gamma$, let $s(\gamma)$ be the first endpoint of $\gamma$, and let $t(\gamma)$ be its last endpoint. Let $S(\Gamma)=\set{s(\gamma)\mid \gamma\in \Gamma}$, and let $T(\Gamma)=\set{t(\gamma)\mid \gamma\in \Gamma}$, where both $S(\Gamma),T(\Gamma)$ are multisets, so, for example, for a point $p$, $n_{S(\Gamma)}(p)$ is the number of curves $\gamma\in \Gamma$ with $p=s(\gamma)$.




\begin{figure}[h]
	\centering
	\subfigure[Before: curve set $\Gamma$ contains all curves except for the yellow curve. Note that there are four crossing points between the yellow curve and the curves in $\Gamma$.]{\scalebox{0.5}{\includegraphics{figs/type_2_uncross_1.jpg}}%\label{fig:non_crossing_representation}
	}
	\hspace{0.5cm}
	\subfigure[After: Curves of $\Gamma$ are uncrossed and they do not cross each other anymore. The multisets $S(\Gamma)$, $T(\Gamma)$ remain the same, but they are matched to each other differently. There are still four crossing points between the yellow curve and the remaining curves.]{
		\scalebox{0.51}{\includegraphics{figs/type_2_uncross_2.jpg}}}
	\caption{An illustration of type-2 uncrossing.} %\mynote{in the second figure, can you increase the distance between the curves? it's hard to see that they don't cross anymore.}}
	\label{fig:type_2_uncrossing}
\end{figure}

Intuitively, given a set $\Gamma$ of curves (not necessarily in general position), we can compute another set $\Gamma'$ of curves as shown in Figure~\ref{fig:type_2_uncrossing}, such that the curves of $\Gamma'$ do not cross with each other, $S(\Gamma)=S(\Gamma')$ and $T(\Gamma)=T(\Gamma')$, and and no additional crossings are created.
We call this process, \emph{type-2 uncrossing}. 
In fact we describe this process in a more general setting, where we are given a number of collections $\Gamma_0,\Gamma_1,\ldots,\Gamma_r$ of curves, and we apply the uncrossing described above to each of the sets $\Gamma_1,\ldots,\Gamma_r$ separately. We show that we can do so without increasing the total number of crossings. 

We now formally define type-2 uncrossing in the following theorem, whose proof is provided in Appendix~\ref{apd: type-2 uncrossing}.


\begin{theorem}[Type-2 Uncrossing]
	\label{thm: type-2 uncrossing}
	There is an efficient algorithm, that receives as input collections $\Gamma_0,\Gamma_1,\ldots,\Gamma_r$ of simple directed curves, such that: (i) the number of points that lie in at least two curves of $\bigcup_{i=0}^r\Gamma_i$ is finite; (ii) for each curve in of $\bigcup_{i=0}^r\Gamma_i$, neither of its endpoint is an inner point of any other curve; and (iii) if a point $p$ lies on more than two curves of $\bigcup_{i=0}^r\Gamma_i$, then either it is an endpoint of every curve that contains $p$, or there is some index $1\leq i\leq r$, such that all curves containing $p$ belong to $\Gamma_i$, and $p$ is an inner point of each of these curves. %\mynote{and $p$ is an inner vertex on $\gamma$?} 
	The algorithm computes, for each $1\le i\le r$, a set $\Gamma'_i$ of new simple directed curves, such that, if we denote by $\Gamma=\Gamma_0\cup (\bigcup_{i=1}^r\Gamma_i)$ and by $\Gamma'=\Gamma_0\cup(\bigcup_{i=1}^r\Gamma_i')$, the following hold:
	
	\begin{itemize}
		\item the curves in $\Gamma'$ are in general position;
		\item for each $1\le i \le r$, $S(\Gamma_i)=S(\Gamma_i')$ and $T(\Gamma_i)=T(\Gamma_i')$;
		
		\item for each $1\le i \le r$, the curves in $\Gamma'_i$ do not cross;
		
		\item for every curve $\gamma\in \Gamma_0$, $\chi(\gamma,\Gamma'\setminus \Gamma_0)\le \chi(\gamma,\Gamma\setminus \Gamma_0)$; and 
		
		\item $\chi(\Gamma')\le \chi(\Gamma)$. 
		%\mynote{isn't RHS here the same as $\chi(\Gamma_0\cup \Gamma)$? if so it's simpler and easier to digest}
	\end{itemize} 
\end{theorem}

%\mynote{there is an obvious problem with the above theorem that it needs to assume that the number of crossings between every pair of curves is finite. Do you allow an inner point on one curve to be the endpoint of another curve? This is not clear. Are the curves simple? (it may be better to make them so, because it's easier). Also, the theorem never says that curves in $\Gamma_i'$ no longer cross. Looks like the proof needs to be fixed too. Is it possible to ensure that curves in $\Gamma_0\cup \Gamma'$ are in general position eventually?}

%\mynote{Is it possible to ensure that curves in $\Gamma_0\cup \Gamma'$ are in general position eventually?}\znote{I think we can't, since we do not intend to touch $\Gamma_0$ in the algorithm for this theorem, and the curves in $\Gamma_0$ may not be in general position.}

%\mynote{it seems much more natural to define $\Gamma=\bigcup_{i=0}^r\Gamma_i$ and $\Gamma'=\Gamma_0\cup(\bigcup_{i=1}^r\Gamma'_i)$. Most probably when we'll want to use this theorem, this is the notation we'll use. Can we switch to this notation?}

As mentioned already, although the algorithm from Theorem~\ref{thm: type-2 uncrossing} ensures that for each $1\le i\le r$, $S(\Gamma_i)=S(\Gamma_i')$ and $T(\Gamma_i)=T(\Gamma_i')$, the pairing between the points in $S(\Gamma_i)$ and the points in $T(\Gamma_i')$ that is defined by the curves in the new set $\Gamma_i'$ may be completely different from that provided by the curves in $\Gamma_i$.

The algorithm from Theorem~\ref{thm: type-2 uncrossing} processes each index $1\leq i\leq r$ one by one. In order to process index $i$, we iterate, as long as there is some point $p$ in the current drawing that serves as an inner point for at least two curves in the current set $\Gamma_i$. We then consider a very small disc $\mu(p)$ containing the point $p$. Let $\Gamma_i(p)\subseteq\Gamma_i$ be the set of curves of $\Gamma_i$ containing the point  $p$ as an inner point. For each such curve $\gamma$, we delete the segment of $\gamma$ lying in disc $\mu(p)$, thereby obtaining two segments of $\gamma$, denote by $\gamma_1$ and $\gamma_2$, where $\gamma_1$ is the segment whose endpoint lies in $S(\Gamma_i)$. We then consider two resulting sets of curves: $\Gamma'_i(p)=\set{\gamma_1\mid \gamma\in \Gamma_i(p)}$ and $\Gamma''_i(p)=\set{\gamma_2\mid \gamma\in \Gamma_i(p)}$. We ``stitch'' the two sets of curves together by defining a new collection $\Gamma'''(p)$ of curves, that are mutually disjoint and contained in the disc $\mu(p)$, such that for each curve $\gamma_1\in \Gamma'_i(p)$ there is exactly one curve in $\Gamma'''_i(p)$ originating at the endpoint of $\gamma_1$ lying on the boundary of $\mu(p)$, and similarly, for each curve $\gamma_2\in \Gamma''_i(p)$ there is exactly one curve in $\Gamma'''_i(p)$ terminating at the endpoint of $\gamma_2$ lying on the boundary of $\mu(p)$. We also ensure that $|\Gamma_i'''(p)|=|\Gamma_i'(p)|=|\Gamma_i''(p)|$. By combining the curves in $\Gamma'(p),\Gamma''_i(p)$ and $\Gamma'''_i(p)$, we obtain a new set of curves that replace the curves of $\Gamma_i(p)$ in set $\Gamma_i$, and continue to the next iteration. Therefore, the above algorithm ensures one additional property that will be useful for us later:

\begin{properties}{C}
	\item For all $1\leq i\leq r$, if $p$ is a point that lies on some curve of $\Gamma'_i$, but $p$ does not lie on any curve of $\Gamma_i$, then there is some other point $p^*$, that serves as an inner point of at least two curves of $\Gamma_i$, and  point $p^*$ lies in the small disc $\mu(p^*)$ containing $p^*$. \label{prop: curve rerouting}
\end{properties}

In other words, the property ensures that the sets of points on the sphere that lie on the curves of $\Gamma'_i$ is contained in the set of points on the sphere that lie on the curves of $\Gamma_i$, and the discs $\mu(p^*)$ of points $p^*$ that serve as inner points on at least two curves of $\Gamma_i$.

{the original type-2 uncrossing}
\fi



%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%-rest of this subsection commented out, old stuff
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------

\iffalse{for edge-disjoint paths}
Let $G$ be a graph and $\Sigma$ be a rotation system on $G$.
Let $P_1,P_2$ be edge-disjoint paths in graph $G$, and some vertex $u$ that is an inner vertex of both $P_1$ and $P_2$. Denote by $e_1,e_1'$ the two edges of $P_1$ that are incident to $u$, and similarly denote by $e_2,e_2'$ the two edges of $P_2$ that are incident to $u$. We say that the intersection of the paths $P_1,P_2$ at vertex $u$ is \emph{non-transversal} iff the edges $e_1,e_1',e_2,e_2'$ appear in the ordering $\oset_u\in \Sigma$ in one of the following two orders: either (i) $(e_1,e_1',e_2,e_2')$ or (ii) $(e_1',e_1,e_2,e_2')$.
%(equivalently, in any drawing that respects the rotation system $\Sigma$, the images of the two paths touch at $u$). 
We say that a set $\pset$ of edge-disjoint paths is \emph{locally non-interfering with respect to $\Sigma$}, iff for every pair $P_1,P_2$ of distinct paths in $\pset$ and for every vertex $u$ that is an inner vertex on both paths, the intersection of $P_1$ and $P_2$ at $u$ is non-transversal. 
\fi

%%% For general paths 
\iffalse
Throughout this subsection, we assume that we are given an instance $I=(G,\Sigma)$ of the \CNwRS problem.  We start by defining the notion of non-transversal intersection of paths, which we then use to define non-transversal paths.

\begin{definition}[Non-transversal intersection of paths]
Let $P_1,P_2$ be simple paths in graph $G$, and let $u$ be a vertex that is an inner vertex of both $P_1$ and $P_2$. Denote by $e_1,e_1'$ the two edges of $P_1$ that are incident to $u$, and similarly denote by $e_2,e_2'$ the two edges of $P_2$ that are incident to $u$. We say that the intersection of the paths $P_1,P_2$ at vertex $u$ is \emph{non-transversal} iff one of the following hold:
\begin{itemize}
\item either  the set $\set{e_1,e_1',e_2,e_2'}$ contains fewer than $4$ distinct edges; or
\item all edges in set  $\set{e_1,e_1',e_2,e_2'}$ are distinct,
and they appear in the ordering $\oset_u\in \Sigma$ in one of the following two circular orders: either (i) $(e_1,e_1',e_2,e_2')$ or (ii) $(e_1',e_1,e_2,e_2')$.
\end{itemize}
Otherwise, we say that the intersection of the paths $P_1,P_2$ is \emph{transversal} at vertex $u$.
\end{definition}

Similarly, for simple cycles $R_1,R_2$ in $G$ and a vertex $u\in V(R_1)\cap V(R_2)$, we define the ``non-transversal intersection of $R_1$ and $R_2$ at vertex $u$ in the same way.





\iffalse
Let $G$ be a graph, let $P$ be a path in $G$, and let $v\in V(P)$ be a vertex of $P$. We denote by $P[v]$ the subpath of $P$ consisting of the edges in $P$ that are incident to $v$. Namely, if $P=(v_1,v_2,\ldots,v_k)$, then $P[v_1]=(v_1,v_2)$ and $P[v_k]=(v_{k-1},v_k)$, and for each $2\le i\le k-1$, $P[v_i]=(v_{i-1},v_i,v_{i+1})$.
For a set $\pset$ of paths in $G$ and a vertex $v$, we denote by $\pset_v\subseteq \pset$ the subset of paths that contain the node $v$, and we define $\pset[v]=\set{P[v]\mid P\in \pset_v}$, and define $G[\pset,v]$ be the subgraph of $G$ that contains all paths in $\pset[v]$. Therefore, $G[\pset,v]$ is a star graph with $v$ serving as the center of the star.
Given a rotation $\oset_v$ on the edges of $\delta_G(v)$, we say that the set $\pset$ of paths is \emph{locally non-interfering at $v$ with respect to $\oset_v$}, if the paths of $\pset[v]$ are non-interfering with respect to the unique planar drawing of $G[\pset,v]$ that respects $\oset_v$.
\fi
%We consider a cluster $C\in \hat{\cset}$, and let $v,v'$ be two high-degree nodes in $C$ (assuming for now that it contains at least two high-degree nodes). Denote $d'=d/n^{\eps}=\Theta(n^{1/2-4\eps})$. From the last step, there are edge-disjoint paths $P_1,\ldots, P_{d'}$ in $C$ connecting $v$ to $v'$. Recall that we are also given a rotation system $\oset=\set{O_v\mid v\in V(\tG')}$ on $\tG'$. The following lemma shows that, given a set of edge-disjoint paths, we can efficiently transform it into a set of edge-disjoint paths that is locally non-interfering at all vertices of $\tG'$ with respect to their circular orderings in $\oset$.
\iffalse
We use the following lemma, whose proof appears in Appendix~\ref{apd:locally_non_interfering}.
\begin{lemma}
	\label{lem:local_non_int}
	There exists an efficient algorithm that, given a graph $G$, a rotation system $\Sigma$ on $G$ and a set $\tilde\pset$ of edge-disjoint paths connecting a pair $v,v'$ of distinct vertices of $G$, computes another set $\pset$ of $|\pset|=|\tilde{\pset}|$ edge-disjoint paths in $G$ connecting $v$ to $v'$, such that $E(\pset)\subseteq E(\tilde\pset)$, and $\pset$ is locally non-interfering at all vertices of $V(G)\setminus\set{v,v'}$ with respect to their rotations/semi-rotations in $\Sigma$.
\end{lemma}
\fi

We will repeatedly use the following lemma for modifying a set of paths that share a common vertex. Its proof appears in \Cref{apd: Proof of rerouting_matching_cong}.
\begin{lemma}
	\label{obs:rerouting_matching_cong}
	There is an efficient algorithm, that, given a graph $G$, a vertex $v$ of $G$, an ordering $\oset_v$ on edges of $\delta_G(v)$ and for each edge $e\in \delta_G(v)$, two integers $n^-_e, n^+_e\ge 0$, such that $\sum_{e\in \delta_G(v)}n^-_e=\sum_{e\in \delta_G(v)}n^+_e$, computes a multiset $M\subseteq \delta_G(v)\times \delta_G(v)$ of $|M|=\sum_{e\in \delta_G(v)}n^+_e$ ordered pairs of the edges of $\delta_G(v)$, such that
	\begin{itemize}
		\item for each $e\in \delta_G(v)$, $M$ contains $n^-_e$ pairs $(e^-,e^+)$ with $e^-=e$;
		\item for each $e\in \delta_G(v)$, $M$ contains $n^+_e$ pairs $(e^-,e^+)$ with $e^+=e$; and
		\item for each pair $(e^-_1,e^+_1),(e^-_2,e^+_2)$ of ordered pairs in $M$, the intersection between path $P_1=(e^-_1,e^+_1)$ and path $P_2=(e^-_2,e^+_2)$ at vertex $v$ is non-transversal with respect to $\oset_v$.
	\end{itemize}
\end{lemma}

\begin{definition}[Non-transversal paths]
Let $\Sigma$ be a rotation system on graph $G$.
We say that a set $\pset$ of simple paths in graph $G$ is \emph{non-transversal with respect to $\Sigma$}, iff for every pair $P_1,P_2$ of distinct paths in $\pset$, for every vertex $u$ that is an inner vertex on both $P_1$ and $P_2$, the intersection between $P_1$ and $P_2$ at vertex $u$ is non-transversal.
\end{definition}


Using \Cref{obs:rerouting_matching_cong}, we can prove the following lemma that allows us to transform an arbitrary set $\rset$ of paths into a set $\rset'$ of non-transversal paths that have the same endpoints as paths in $\rset$, without increasing the congestion on any edge. 
The proof of the lemma below is similar to the proof of Lemma 9.5 in~\cite{chuzhoy2020towards}, and is provided in Appendix~\ref{apd: Proof of non_interfering_paths} for completeness. 
%\mynote{did we prove it in our previous paper? if so we should mention it. Is there any reason to use $\hat G$, $\hat \Sigma$ as opposed to plain $(G,\Sigma)$ notation there? Also, I think both sets of paths should be *simple* in the lemma statement. }

%\mynote{for my proof I need the paths in $\rset$ to have arbitrary endpoints, as long as endpoints can't be inner vertices on paths (in fact they share their last endpoint but I think the lemma is correct regardless of that). can you fix the lemma to make it work for this more general setting?}


\znote{maybe we need to introduce congestion before this subsection? (for the following lemmas and theorems)}

\fi

\iffalse
\begin{lemma}
\label{lem: non transversal cost of cycles bounded by cr}
Let $I=(G,\Sigma)$ be an instance of \CNwRS and let $\phi$ be any solution to $I$ on the sphere. Let $\rset$ be a set of simple cycles in $G$, such that, for every pair $R,R'$ of edge-disjoint cycles in $\rset$, the intersection of $R$ and $R'$ are transversal at at most one of their common vertices. Then 
\[\ntcost(\rset,\Sigma) \le \sum_{e\in E(G)}\chi_{\phi}(e)\cdot(\cong_G(\rset,e))^2.\]
\end{lemma}
\fi



\iffalse
%\znote{check if Sec 6 use it, if not, move to Sec 8.3}

\paragraph{Non-Transversal Cost.} Given an instance $(G,\Sigma)$ of \CNwRS and a set $\qset$ of paths in $G$, we define the \emph{non-transversal cost of $\qset$ with respect to $\Sigma$}, which is denoted by $\ntcost(\qset;\Sigma)$, as the number of unordered pairs $Q,Q'$ of paths in $\qset$, such that paths $Q$ and $Q'$ are edge-disjoint, and the intersection of $Q,Q'$ are non-transversal at some vertex that is an inner vertex of both $Q$ and $Q'$.
Note that, if the set $\qset$ of paths is non-transversal with respect to $\Sigma$, then $\ntcost(\qset;\Sigma)=0$. Similarly, given a set $\rset$ of cycles in $G$, the non-transversal cost $\ntcost(\rset,\Sigma)$ of $\rset$ with respect to $\Sigma$ is defined similarly.
%
Additionally, for two sets $\qset,\qset'$ of paths in $G$, we define $\ntcost(\qset,\qset';\Sigma)$ as the number of pairs $(Q,Q')$ of paths with $Q\in \qset$ and $Q'\in \qset'$, such that paths $Q$ and $Q'$ are edge-disjoint, and the intersection of $Q,Q'$ are non-transversal at some vertex that is an inner vertex of both $Q$ and $Q'$.
By definition, $\ntcost(\qset;\Sigma)= \ntcost(\qset,\qset;\Sigma)$.

%We also define $\cost^*(\qset)=\min\set{\sum_{e\in E(G)}(\cong_{G}(\qset,e))^2,|\qset|^2}$.

We will use the following lemma. Its proof appears in \Cref{apd: Proof of non transversal cost of cycles bounded by cr}.


\begin{lemma}
\label{lem: non transversal cost of cycles bounded by cr}
Let $I=(G,\Sigma)$ be an instance of \CNwRS and let $\phi$ be any solution to $I$ on the sphere. Let $\rset,\rset'$ be two sets of simple cycles in graph $G$, such that, for every pair $R,R'$ of edge-disjoint cycles with $R\in \rset$ and $R'\in \rset'$, the intersection of $R$ and $R'$ are transversal with respect to $\Sigma$ at at most one of their common vertices. Then 
\[\ntcost(\rset,\rset';\Sigma) \le \sum_{e,e'\in E(G)}\chi_{\phi}(e,e')\cdot\bigg(\cong_G(\rset,e)\cdot \cong_G(\rset',e')+\cong_G(\rset,e')\cdot \cong_G(\rset',e)\bigg).\]
\end{lemma}


We will use the following theorem. Its proof appears in \Cref{apd: Proof of curve_manipulation}.


\begin{theorem}
	\label{thm: new nudging}
	There is an efficient algorithm, whose input contains a graph $G$, a drawing $\phi$ of $G$ on the sphere, a subgraph $C$ of $G$, two sets $\qset,\qset'$ of paths in $G$ that share an endpoint $t^*$, that is refered to as their common last endpoint, and an circular ordering $\oset_{t^*}$ on its incident edges, such that (i) all paths of $\qset\cup \qset'$ are internally disjoint from $C$; (ii) for each $Q\in \qset\cup \qset'$, the other endpoint of $Q$, denoted by $s_Q$, is designated as its first endpoint; and (iii) for every pair $Q,Q'$ of edge-disjoint paths in $\qset\cup \qset'$, the intersection of $Q$ and $Q'$ is transversal at at most one of their common vertices. The algorithm computes a set $\Gamma=\set{\gamma(Q)\mid Q\in \qset\cup \qset'}$ of directed curves on the sphere with the following properties:
	
	\begin{itemize}
		\item the curves in $\Gamma$ are in general position;
		\item for each path $Q\in \qset\cup \qset'$, $s(\gamma(Q))=\phi(s_Q)$ and $t(\gamma(Q))=\phi(t^*)$;
		\item $\chi(\Gamma)\le |\qset'|^2+\ntcost(\qset;\Sigma)+\ntcost(\qset,\qset';\Sigma)+\sum_{e\in E(G)}(\chi_{\phi}(e)+1)\cdot (\cong_G(\qset,e))^2\\ \text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }
		+\sum_{e\in E(G)} \cong_G(\qset,e)\cdot\cong_G(\qset',e)+\sum_{e,e'\in E(G)}
		\chi_{\phi}(e,e')\cdot \cong_G(\qset,e)\cdot\cong_G(\qset',e')$;
		\item the circular ordering in which curves of $\Gamma$ enter $\phi(t^*)$ is identical to $\oset^{\guided}(\qset\cup \qset',\oset_{t^*})$, the circular ordering in which paths of $\qset\cup \qset'$ enter $t^*$; and
		\item for each edge $e\in E(C)$, the number of crossings between the image of $e$ in $\phi$ and the curves in $\Gamma$ is bounded by the number of crossings between the image of $e$ and images of the edges of $G\setminus C$ times $\cong_G(\qset\cup \qset')$, namely $\chi(\phi(e),\Gamma)\le \chi_{\phi}(e, G\setminus C)\cdot \cong_G(\qset\cup \qset')$.
	\end{itemize}
\end{theorem}





Given an instance $(G,\Sigma)$ of \CNwRS and a simple path $P$ with endpoints $s,t$ in $G$, we define the \emph{$P$-extraction} as the following operations on $G$ and $\Sigma$: 
(i) delete all edges of $E(P)$ from $G$; 
(ii) for each internal vertex $u\in V(P)$, delete the two edges of $P$ that are incident to $u$ from the ordering $\oset_u\in \Sigma$;
(ii) add an edge $e_P=(s,t)$ to $G$; and
(iv) replace the edge of $P$ that is incident to $s$ with the edge $e_P$ in the ordering $\oset_s\in \Sigma$, and replace the edge of $P$ that is incident to $t$ with the edge $e_P$ in the ordering $\oset_t\in \Sigma$.
Similarly, if we are given a set $\pset$ of edge-disjoint paths in $G$, then \emph{$\pset$-extraction} is defined to be a sequence of operations that contains a $P$-extraction for each path $P\in \pset$. It is easy to see that the order in which these $P$-extractions appear in this sequence does not matter.

We use the following lemma that allows us to modify a solution $\phi$ of instance $(G,\Sigma)$ to a solution of the instance $(G',\Sigma')$ that is obtained from applying $\pset$-contraction to $(G,\Sigma)$. Its proof appears in \Cref{apd: Proof of curves from non-transversal paths}.

\begin{lemma}
\label{lem: curves from non-transversal paths}
There is an algorithm, that, given an instance $(G,\Sigma)$ of \CNwRS, a feasible solution $\phi$ for this instance, and a set $\pset$ of edge-disjoint paths that are non-transversal with respect to $\Sigma$, efficiently computes a feasible solution $\phi'$ for the instance $(G',\Sigma')$ that is obtained by applying $\pset$-contraction to $(G,\Sigma)$, such that $\cro(\phi')\le \cro(\phi)$.
\end{lemma}

\fi

%\mynote{can we add the following lemma: we are given as input a graph $G$ with rotation system $\Sigma$, and a collection $\pset$ of edge-disjoint non-transversal paths in $G$, doing 1-to-1 routing from $S$ to $T$, where vertices of $S\cup T$ are not inner vertices on $\pset$. Let $G'$ be obtained from $G$ by deleting all edges in $\pset$ and all vertices of $\pset$ except for $S\cup T$, and then adding, for each path $P\in \pset$, an edge connecting its endpoints (rotation system needs to be defined appropriately, maybe this needs to be done before the lemma). Then there is a drawing of $G'$ consistent with the new rotation system, with number of crossings at most $\optcrors(G,\Sigma)$. This is where we need to do ``nudging'' of paths near the images of vertices, but we also need to preserve the crossings between the paths and other parts of the graph.}





%\znote{The proof of this lemma is included in the proof of Lemma 9.5 in \cite{chuzhoy2020towards}. But the statement of Lemma 9.5 is not the same as this lemma. Should we also include its proof in Appendix?}
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------
%------------------------------------





\subsection{Routing Paths} 
\label{sec: routing paths}


\paragraph{Routing Paths.} Given a graph $G$ and two sets $S,T\subseteq V(G)$, 
a \emph{routing of vertices of $S$ to vertices of $T$} is a collection $\qset=\set{Q_v\mid v\in S}$ of paths, where for each vertex $v\in S$, path $Q_v$ originates at a vertex of $v$ and terminates at a vertex of $T$. 
If, additionally, for every vertex of $T$, exactly one path in $\qset$ terminates at $T$, then we say that $\qset$ is an \emph{one-to-one routing} of vertices of $S$ to vertices of $T$.

%If $\qset$ is a routing of vertices of $S$ to vertices of $T$, then we sometimes say that the set $\qset$ of paths \emph{routes} vertices of $S$ to vertices of $T$. If $T=\set{u}$, for some vertex $u\in V(G)$, then we sometimes say that $\qset$ routes vertices of $S$ to $u$.

Similarly, given two sets $E_1,E_2$ of edges of $G$, we say that a set $\qset=\set{Q_e\mid e\in E_1}$ of paths is a routing of edges of $E_1$ to edges of $E_2$, or that $\qset$ routes edges of $E_1$ to edges of $E_2$, iff for every edge $e\in E_1$, path $Q_e$ has $e$ as its first edge, and some edge of $E_2$ as its last edge. If, additionally, every edge of $E_2$ serves as the last edge on exactly one path in $\qset$, then we say that $\qset$ is an one-to-one routing of edges of $E_1$ to edges of $E_2$. %We also define a routing from a set $E_1$ of edges to a set $T$ of vertices similarly.

\begin{definition}[Routing Paths inside and outside a Cluster]
	Let $G$ be a graph and let $C$ be a cluster of $G$. We say that a set $\qset(C)=\set{Q_e\mid e\in \delta_G(C)}$ of paths \emph{route the edges of $\delta_G(C)$ inside $C$ to a vertex $v\in V(C)$}, iff for all $e\in \delta_G(C)$, path $Q_e$ has $e$ as its first edge, $v$ as its last vertex, and $Q_e\setminus\set{e}$ is contained in $C$.
	We say that a set $\qset'(C)=\set{Q'_e\mid e\in \delta_G(C)}$ of paths \emph{route the edges of $\delta_G(C)$ outside $C$ to a vertex $v'\in V(G)\setminus V(C)$}, iff for all $e\in \delta_G(C)$, path $Q'_e$ has $e$ as its first edge, $v'$ as its last vertex, and $Q'_e\setminus\set{e}$ is disjoint from $C$.
\end{definition}


%Similarly, given a cluster $C$ of $G$, and let $u(C)$ be an arbitrary vertex of $C$. We say that a set $\qset(C)$ of paths \emph{routes the edges of $\delta_G(C)$ to $u(C)$ inside $C$} iff $\qset(C)=\set{Q_C(e)\mid e\in \delta_G(C)}$, and for all $e\in \delta(C)$, path $Q_C(e)$ has $e$ as its first edge and $u(C)$ as its last vertex, and moreover $Q(e)\setminus\set{e}$ is contained in $C$.  Similarly, given a vertex $u'(C)\not\in C$, we say that a set $\pset(C)$ of paths \emph{routes the edges of $\delta(C)$ to $u'(C)$ outside of $C$} iff $\pset(C)=\set{P_C(e)\mid e\in \delta_G(C)}$, and for all $e\in \delta(C)$, path $P_C(e)$ has $e$ as its first edge, $u'(C)$ as its last vertex, and, except for its first vertex, is completely disjoint from $C$.





We repeatedly use the following simple claim, whose proof appears in \Cref{apd: Proof of remove congestion}.

\begin{claim}\label{claim: remove congestion}
	Let $G$ be a graph, let $S$, $T$ be two disjoint multisets of its vertices, and let $\pset$ be a collection of paths in $G$, where every path in $\pset$ originates at a vertex of $S$ and terminates at a vertex of $T$, 
	such that for every vertex $v$, at most $n_S(v)$ paths in $\pset$ originate at $v$ and at most $n_T(v)$ paths in $\pset$ terminate at $v$. Assume further that the paths in $\pset$ cause congestion $\rho$. Then there is a collection $\pset'$ of edge-disjoint paths in $G$, with $|\pset'|\geq |\pset|/\rho$, such that for every vertex $v$, at most $n_S(v)$ paths in $\pset'$ originate at $v$ and at most $n_T(v)$ paths in $\pset'$ terminate at $v$.
\end{claim}











\subsection{Non-Transversal Paths and Path Splicing}
\label{subsec: non-transversal paths and splicing}
%We assume that we are given an instance $I=(G,\Sigma)$ of the \CNwRS problem.  

We start by defining the notion of non-transversal intersection of paths, which we then use to define non-transversal paths.

%\mynote{allow, in this definition, the vertex $v$ to be an endpoint of one of these paths?}

\begin{definition}[Non-transversal intersection of paths and cycles]
	Let $I=(G,\Sigma)$ be an intance of \cnwrs,	let $P_1,P_2$ be two simple paths in $G$, and let $u$ be a vertex in $V(P_1)\cap V(P_2)$. Denote by $E_1$ the set of (one or two) edges of $P_1$ that are incident to $u$, and similarly denote by $E_2$ the set of (one or two) edges of $P_2$ that are incident to $u$. We say that the intersection of the paths $P_1,P_2$ at vertex $u$ is \emph{non-transversal with respect to $\Sigma$} iff one of the following hold:
	\begin{itemize}
		\item either the set $E_1\cup E_2$ contains fewer than $4$ distinct edges; or
		\item $E_1=\set{e_1,e_1'}$ and $E_2=\set{e_2,e_2'}$, all edges in set $\set{e_1,e_1',e_2,e_2'}$ are distinct,
		and they appear in the ordering $\oset_u\in \Sigma$ in one of the following two circular orders:  $(e_1,e_1',e_2,e_2')$ or $(e_1',e_1,e_2,e_2')$.
	\end{itemize}
	Otherwise, we say that the intersection of the paths $P_1,P_2$ at vertex $u$ is \emph{transversal}.
	
	If $R_1,R_2$ are simple cycles in $G$, and $u$ is a vertex in $V(R_1)\cap V(R_2)$, then we classify the intersection of $R_1$ and $R_2$ and $u$ as transversal or non-transversal with respect to $\Sigma$ similarly.
\end{definition}


%\mynote{remove the requirement that a vertex can't be an inner vertex on one path and an endpoint of another?}
\begin{definition}[Non-transversal set of paths]\label{def: non-transversal paths}
	Let $I=(G,\Sigma)$ be an intance of \cnwrs,	and let $\pset$ be a collection of simple paths in $G$. We say that path set $\pset$ is \emph{non-transversal with respect to $\Sigma$} iff for every pair $P_1,P_2\in \pset$ of paths, for every vertex $u\in V(P_1)\cap V(P_2)$, 
	%either (i) $u$ is an endpoint of both $P_1$ and $P_2$; or (ii) $u$ serves as an inner vertex of both $P_1$ and $P_2$, and 
	the intersection of $P_1$ and $P_2$ at $u$ is non-transversal with respect to $\Sigma$.
\end{definition}


Assume now that we are given some instance $I=(G,\Sigma)$, and a collection $\qset$ of simple paths in $G$. 
%We will sometimes assign the paths in $\qset$ a direction, that is, for every path $Q\in \qset$, we will designate one endpoint of $Q$ as its first endpoint, and the other endpoint of $Q$ is its last endpoint. We denote by $S(\qset)$ the multiset of vertices that contains the first endpoint of every path in $\qset$, and by $T(\qset)$ the multiset of vertices that contains the last endpoint of every vertex in $\qset$. 
We let $\Pi^T(\qset)$ denote the set of all triples $(Q,Q',v)$, such that $Q,Q'\in \qset$, $v$ is an inner vertex of  both $Q$ and $Q'$, and the intersection of $Q$ and $Q'$ at $v$ is transversive with respect to $\Sigma$. 

In some cases, we will be given some set $\pset$ of simple paths in a graph $G$, and we will need to transform it into a set  $\pset'$ of paths that is  non-transversal with respect to the given rotation system $\Sigma$ for $G$, while ensuring that $S(\pset')=S(\pset)$ and $T(\pset')=T(\pset)$. Below we provide a procedure for doing so. The procedure uses a simple subroutine that we call \emph{path splicing} and describe next.


\paragraph{Path Splicing.}
Suppose we are given an instance $I=(G,\Sigma)$ of \cnwrs, two simple paths $P,P'$ in $G$, and a vertex $v$, that serves as an inner vertex of both $P$ and $P'$, such that the intersection of $P$ and $P'$ at vertex $v$ is transversal with respect to $\Sigma$. We assume that each of the paths $P,P'$ is assigned a direction, and we denote by $s$ and $t$ the first and the last endpoints of $P$, respectively, and by $s'$ and $t'$ the first and the last endpoints of $P'$, respectively. The \emph{splicing} of $P$ and $P'$ at vertex $v$ produces two new paths: path $\tilde P$ that is a concatenation of the subpath of $P$ from $s$ to $v$, and the subpath of $P'$ from $v$ to $t'$; and path $\tilde P'$, that is a concatenation of the  subpath of $P'$ from $s'$ to $v$, and the subpath of $P$ from $v$ to $t$. We use the following simple observation regarding the splicing procedure, whose proof is deferred to \Cref{apd: Proof of splicing}.

\begin{observation}\label{obs: splicing}
	Let $I=(G,\Sigma)$ be an instance of $\cnwrs$, let $\pset$ be a set of simple (directed) paths in $G$, 
	%such that the vertices of $S(\pset)\cup T(\pset)$ do not serve as inner vertices on any path in $\pset$, 
	and let $(P,P',v)$ be a triple in $\Pi^T(\pset)$.  Let $\tilde P,\tilde P'$ be the pair of paths obtained by splicing 	$P$ and $P'$ at $v$, and let $\pset'=\big(\pset\setminus\set{P,P'}\big)\cup \set{\tilde P,\tilde P'}$.
	Then $S(\pset')=S(\pset)$ and $T(\pset')=T(\pset)$. Additionally,	either (i) at least one of the paths $\tilde P,\tilde P'$ is a non-simple path; or (ii) $|\Pi^T(\pset')|<|\Pi^T(\pset)|$.
\end{observation} 


%\mynote{Proof sxketch for $|\Pi^T(\pset')|<|\Pi^T(\pset)|$: denote by $e_1,e_2$ the edges of $P$ just before/after $v$, denote by $e_1',e_2'$ edges of $P'$ before/after $v$. Edges $e_1,e_2,e_1',e_2'$ partition the edges of $\delta(v)$ into 4 subsets $E_1,\ldots,E_4$, each of which appears contiguously in $\oset_v$. Now take another path $Q$ that contains $v$ as inner vertex. If $Q$ intersects both $P,P'$ transversally at $v$, we are done. If it intersects neither transversally at $v$, then the edges $e_1'',e_2''$ of $Q$ that appear just before/after $v$ lie in the same  set $E_i$, so $Q$ will continue to intersect $\tilde P,\tilde P'$ non-transversally at $v$. last case is where $Q$ intersects one of them (say $P$) transversally, the other ($P'$) non-transversally. In this case, there are two cases: (i) $e_1''$, $e_2''$ lie in $E_1,E_3$ respectively (or the other way around), or (ii) $e_1''$, $e_2''$ lie in $E_2,E_4$, respectively (or the other way around). The cases are symmetric, enough to consider one of them and show that $Q$ will only have transversal intersection with one of the two new paths at $V$.}






\iffalse
Let $G$ be a graph, let $P$ be a path in $G$, and let $v\in V(P)$ be a vertex of $P$. We denote by $P[v]$ the subpath of $P$ consisting of the edges in $P$ that are incident to $v$. Namely, if $P=(v_1,v_2,\ldots,v_k)$, then $P[v_1]=(v_1,v_2)$ and $P[v_k]=(v_{k-1},v_k)$, and for each $2\le i\le k-1$, $P[v_i]=(v_{i-1},v_i,v_{i+1})$.
For a set $\pset$ of paths in $G$ and a vertex $v$, we denote by $\pset_v\subseteq \pset$ the subset of paths that contain the node $v$, and we define $\pset[v]=\set{P[v]\mid P\in \pset_v}$, and define $G[\pset,v]$ be the subgraph of $G$ that contains all paths in $\pset[v]$. Therefore, $G[\pset,v]$ is a star graph with $v$ serving as the center of the star.
Given a rotation $\oset_v$ on the edges of $\delta_G(v)$, we say that the set $\pset$ of paths is \emph{locally non-interfering at $v$ with respect to $\oset_v$}, if the paths of $\pset[v]$ are non-interfering with respect to the unique planar drawing of $G[\pset,v]$ that respects $\oset_v$.
\fi
%We consider a cluster $C\in \hat{\cset}$, and let $v,v'$ be two high-degree nodes in $C$ (assuming for now that it contains at least two high-degree nodes). Denote $d'=d/n^{\eps}=\Theta(n^{1/2-4\eps})$. From the last step, there are edge-disjoint paths $P_1,\ldots, P_{d'}$ in $C$ connecting $v$ to $v'$. Recall that we are also given a rotation system $\oset=\set{O_v\mid v\in V(\tG')}$ on $\tG'$. The following lemma shows that, given a set of edge-disjoint paths, we can efficiently transform it into a set of edge-disjoint paths that is locally non-interfering at all vertices of $\tG'$ with respect to their circular orderings in $\oset$.
\iffalse
We use the following lemma, whose proof appears in Appendix~\ref{apd:locally_non_interfering}.
\begin{lemma}
	\label{lem:local_non_int}
	There exists an efficient algorithm that, given a graph $G$, a rotation system $\Sigma$ on $G$ and a set $\tilde\pset$ of edge-disjoint paths connecting a pair $v,v'$ of distinct vertices of $G$, computes another set $\pset$ of $|\pset|=|\tilde{\pset}|$ edge-disjoint paths in $G$ connecting $v$ to $v'$, such that $E(\pset)\subseteq E(\tilde\pset)$, and $\pset$ is locally non-interfering at all vertices of $V(G)\setminus\set{v,v'}$ with respect to their rotations/semi-rotations in $\Sigma$.
\end{lemma}
\fi




\iffalse
\mynote{I suspect that this lemma is not needed anymore, but we can decide whether to keep it later.}
We will repeatedly use the following lemma for modifying a set of paths that share a common vertex. Its proof appears in \Cref{apd: Proof of rerouting_matching_cong}.
\begin{lemma}
	\label{obs:rerouting_matching_cong}
	There is an efficient algorithm, that, given a graph $G$, a vertex $v$ of $G$, an ordering $\oset_v$ on edges of $\delta_G(v)$ and for each edge $e\in \delta_G(v)$, two integers $n^-_e, n^+_e\ge 0$, such that $\sum_{e\in \delta_G(v)}n^-_e=\sum_{e\in \delta_G(v)}n^+_e$, computes a multiset $M\subseteq \delta_G(v)\times \delta_G(v)$ of $|M|=\sum_{e\in \delta_G(v)}n^+_e$ ordered pairs of the edges of $\delta_G(v)$, such that
	\begin{itemize}
		\item for each $e\in \delta_G(v)$, $M$ contains $n^-_e$ pairs $(e^-,e^+)$ with $e^-=e$;
		\item for each $e\in \delta_G(v)$, $M$ contains $n^+_e$ pairs $(e^-,e^+)$ with $e^+=e$; and
		\item for each pair $(e^-_1,e^+_1),(e^-_2,e^+_2)$ of ordered pairs in $M$, the intersection between path $P_1=(e^-_1,e^+_1)$ and path $P_2=(e^-_2,e^+_2)$ at vertex $v$ is non-transversal with respect to $\oset_v$.
	\end{itemize}
\end{lemma}
\fi


\iffalse
\begin{definition}[Non-transversal paths]
	Let $\Sigma$ be a rotation system on graph $G$.
	We say that a set $\pset$ of simple paths in graph $G$ is \emph{non-transversal with respect to $\Sigma$}, iff for every pair $P_1,P_2$ of distinct paths in $\pset$, for every vertex $u$ that is an inner vertex on both $P_1$ and $P_2$, the intersection between $P_1$ and $P_2$ at vertex $u$ is non-transversal.
\end{definition}

\fi

\iffalse
\mynote{for the lemma below: 1. do we need to require that the paths are edge-disjoint? 2. The lemma does not say that the routing is one-to-one. I think the lemma should be resetated like this:
}
\fi


%\mynote{Lemma statement: There is an efficient algorithm, that, given an instance $I=(G, \Sigma)$ of \CNwRS and a set $\rset$ of (directed) paths in $G$, computes another set $\rset'$ of simple paths in $G$, such that $S(\rset')=S(\rset)$, $T(\rset')=T(\rset)$, and the paths in $\rset'$ are non-transversal with respect to $\Sigma$. Moreover, for every edge $e\in E(G)$, $\cong_G(\rset',e)\leq \cong_G(\rset,e)$.}


%\mynote{this looks very similar to Lemma 5.5. But we need to use this lemma in Sec 8.2 in the case where vertices may need to be both endpoints an inner vertices on paths. So if we could modify the def of non-transversal paths to allow this, and then prove the lemma allowing this.}

Using \Cref{obs: splicing}, we can prove the following lemma that allows us to transform an arbitrary set $\rset$ of paths into a set $\rset'$ of non-transversal paths that have the same endpoints as paths in $\rset$, without increasing the congestion on any edge. 
The proof of the lemma below is similar to the proof of Lemma 9.5 in~\cite{chuzhoy2020towards}, and is provided in Appendix~\ref{apd: Proof of non_interfering_paths} for completeness. 
%\mynote{did we prove it in our previous paper? if so we should mention it. Is there any reason to use $\hat G$, $\hat \Sigma$ as opposed to plain $(G,\Sigma)$ notation there? Also, I think both sets of paths should be *simple* in the lemma statement. }

%\mynote{for my proof I need the paths in $\rset$ to have arbitrary endpoints, as long as endpoints can't be inner vertices on paths (in fact they share their last endpoint but I think the lemma is correct regardless of that). can you fix the lemma to make it work for this more general setting?}

\iffalse
\begin{lemma}
	\label{lem: non_interfering_paths}
	There is an efficient algorithm, that, given an instance $I=(G, \Sigma)$ of \CNwRS, two disjoint multisets $S,T$ of vertices of $G$, and a set $\rset$ of simple edge-disjoint paths in $G$ routing vertices of $S$ to vertices of $T$, such that the vertices of $S\cup T$ may not serve as inner vertices on any path in $\rset$, computes a set $\rset'$ of $|\rset'|=|\rset|$ edge-disjoint paths in $G$ vertices of $S$ to vertices of $T$, such that vertices of $S\cup T$ may not be an inner vertex on any path in $\rset$, and (i) the paths in $\rset'$ are non-transversal with respect to $\Sigma$; and (ii) $E(\rset')\subseteq E(\rset)$.
\end{lemma}
\fi




\begin{lemma}
	\label{lem: non_interfering_paths}
	There is an efficient algorithm, that, given an instance $(G, \Sigma)$ of \CNwRS and a set $\rset$ of (directed) paths in $G$, computes another set $\rset'$ of simple (directed) paths in $G$, such that $S(\rset')=S(\rset)$, $T(\rset')=T(\rset)$, and the paths in $\rset'$ are non-transversal with respect to $\Sigma$. Moreover, for every edge $e\in E(G)$, $\cong_G(\rset',e)\leq \cong_G(\rset,e)$.
\end{lemma}







\subsection{Balanced Cut and Sparsest Cut}
%
%\vspace{-3mm}
%\begin{definition}
%	Given a graph $G$, a subset $T$ of its vertices, and a parameter $\alpha > 0$, we say that $T$ is \emph{$\alpha$-well-linked} in $G$, iff for any partition $(A,B)$ of $T$, $|E(A, B)|\ge \alpha\cdot\min \{|T\cap A|, |T\cap B|\}$. %\snote{shouldn't this be $|E(A, B)|\ge \alpha\cdot\min \{|\out(T)\cap \out(A)|, |\out(T)\cap \out(B)|\}$?}
%\end{definition}
%\vspace{-0.3cm}
%


%\mynote{please replace $\Gamma$ with $T$ or $\Upsilon$ below. We use $\Gamma$ for curves.}
%\paragraph{Balanced Cut and Sparsest Cut.} 
Suppose we are given a graph $G=(V,E)$, and a subset $T\sse V$ of its vertices. We say that a cut $(X,Y)$ in $G$ is a valid $T$-cut iff $X\cap T,Y\cap T\neq \emptyset$. The \emph{sparsity} of a valid $T$-cut $(X,Y)$ is $\frac{|E(X,Y)|}{\min\set{|X\cap T|, |Y\cap T|}}$. %, and the value of the sparsest cut in $G$ is defined to be:
%$\Phi(G)=\min_{S\subsetneq V}\set{\Phi(S)}$.
In the Sparsest Cut problem, given a graph $G$ and a subset $T$ of its vertices, the goal is to compute a valid $T$-cut of minimum sparsity. Arora, Rao and Vazirani~\cite{ARV} have shown an $O(\sqrt {\log n})$-approximation algorithm for the sparsest cut problem\footnote{The algorithm was originally designed for finding approximate sparsest cut on simple graphs, but it can be easily generalized to graphs with parallel edges by using edge costs.}. %\mynote{maybe add a footnote that this was originally defined for simple graphs but can be easily generalized to graphs with parallel edges by using edge costs?}. 
We denote this algorithm by \algsc, and its approximation factor by $\alphasc(n)=O(\sqrt{\log n})$. 


%\mynote{lease replace $\gamma$ with something else. We use $\gamma$ for curves.}
Let $\theta$ be some parameter such that $0<\theta<1/2$. We say that a cut $(A,B)$ of $G$ is \emph{$\theta$-vertex-balanced} iff $|A|,|B|\ge \theta\cdot |V(G)|$.
We say that a cut $(A,B)$ of $G$ is \emph{$\theta$-edge-balanced} iff $|E(A)|,|E(B)|\ge \theta\cdot|E(G)|$.
In this paper, when we refer to a $\theta$-balanced cut, we mean a $\theta$-edge-balanced cut.
We will use the following theorem and its corollary for computing an approximate minimum balanced cut. 

%\mynote{is this for simple graphs? if so it should be stated this way. But we need the corollary for non-simple graphs as well.}
\begin{theorem}[Corollary 2 in~\cite{ARV}]
	\label{thm: ARV}
	For any constant $0<c<1/2$, there exists another constant $0<c'<c$, and an efficient algorithm, that, given any \textbf{simple} connected graph $G$ with $n$ vertices and $m$ edges, computes a $c'$-vertex-balanced cut of $G$, whose size is at most $\alphasc(n)$ times the size of a minimum $c$-vertex-balanced cut of $G$.
\end{theorem}

The proof of the following corollary of \Cref{thm: ARV} is provided in Appendix~\ref{apd: Proof of approx_balanced_cut}.
%\mynote{better to say where the proof of corollary is right next to the corollary}
\begin{corollary}
	\label{cor: approx_balanced_cut}
	For any constant $0<\hat c<1/2$, there exists another constant $0<\hat c'<\hat c$, and an efficient algorithm, that, given any connected (not necessarily simple) graph $G$ with $n$ vertices and $m$ edges, computes a $\hat c'$-edge-balanced cut of $G$, whose size is at most $O(\alphasc(m))$ times the size of a minimum $\hat c$-edge-balanced cut of $G$.
\end{corollary}
We will use the following lemma, that is a simple consequence of the Lipton-Tarjan separator theorem for planar graphs \cite{lipton1979separator}.
We note that the version for vertex-balanced cuts of the lemma below are proved in~\cite{pach1996applications}.
For completeness, we provide its proof appears in Appendix~\ref{apd: Proof of min_bal_cut}. 
%\mynote{If this lemma easily follows from previous work you should say it here, and cite the prevous work. You don't want to make it look like we are claiming this as a new result, when it should be attributed to previous work.}
%\mynote{Important: if the next lemma correct only for simple graphs or does it work with parallel edges as well (I believe the latter but it's a subtle point and we have to be correct on that).}
\begin{lemma}
	\label{lem:min_bal_cut}
	Let $G=(V,E)$ be a connected graph with maximum degree $\Delta\le |E|/2^{100}$. If $\optcro(G)\le |E|^2/2^{100}$, then the minimum $(1/4)$-edge-balanced cut in $G$ has size $O(\sqrt{\optcro(G)+\Delta\cdot|E|})$.
\end{lemma}


%\mynote{this part is not well organized. You should have one heading called "Balanced cut and Sparsest Cut" that will have all their definitions and algorithms for them. Then another heading called "Well-Linkedness and Bandwidth Property", with definitions and the routing theorems, and then "Well-linked Decomposition" with the WLD theorem.}





\subsection{Well-Linkedness, Bandwidth Property and Well-linked Decomposition} %We use a standard notion of well-linkedness:
%\paragraph{Well-Linkedness and Bandwidth Property.}
%\mynote{can you make the following into formal definitions so they are easier to locate?}

The notion of well-linkedness has played a central role in graph theory and graph algorithms in the past decade (e.g. \cite{racke2002minimizing,chekuri2004edge,andrews2010approximation,chuzhoy2012polylogarithmic,chuzhoy2012routing,chekuri2016polynomial,chuzhoy2016improved,chuzhoy2019towards}). 
We use the following standard definitions, which are equivalent to
those used in \cite{chuzhoy2012polylogarithmic,chuzhoy2012routing,chekuri2016polynomial,chuzhoy2016improved,chuzhoy2019towards}.

%\mynote{please say that we use standard notion of well-linkedness, that has been widely used in graph theory and beyond. Also, pleae get rid of $\Gamma$.}
\begin{definition}[Well-Linkedness]
We say that a set $T$ of vertices of $G$ is \emph{$\alpha$-well-linked} in $G$, iff the value of the sparsest cut in $G$ with respect to $T$ is at least $\alpha$; equivalently, for every partition $(A,B)$ of $V(G)$ with $A,B\neq \emptyset$, $|E_G(A,B)|\geq \alpha\cdot \min\set{|A\cap T|,|B\cap T|}$.
\end{definition}




The next simple observation, that has been used extensively in previous work, shows that the set of vertices lying in the first row of the $(r\times r)$-grid is $1$-well-linked. For completeness, we provide a proof in \Cref{apd: Proof grid 1st row well-linked}.


\begin{observation}
	\label{obs: grid 1st row well-linked}
	Let $r\geq 1$ be an integer, and let $H$ be the $(r\times r)$-grid. Let $S$ be the set of vertices lying in the first row of the grid. Then vertex set $S$ is $1$-well-linked in $H$.
\end{observation}


\iffalse
Assume now that we are given a graph $G$, and some subgraph $C$ of $G$ that we call cluster. Throughout this paper, we will sometimes use a graph $C^+$ that is associated with $C$, whose definition is given below.


%\mynote{Note: graph $C^+$ is defined here, so we don't need to redefine it in the paper again and again.}

\begin{definition}[Graph $C^+$]
	Let $G$ be a graph and $C\subseteq G$ be a cluster. Graph $C^+$ associated with $C$ is constructed as follows. First, we subdivide every edge $e\in \delta_G(C)$ with a vertex $t_e$, and let $T(C)=\set{t_e\mid e\in \delta_G(C)}$ be the set of newly added vertices, that we sometimes refer to as \emph{terminals of $C$}. We then let $C^+$ be the subgraph of the resulting graph induced by $V(C)\cup T(C)$.
\end{definition}
\fi


Next, we define the notion of bandwidth property, that was also used extensively in graph algorithms.

\begin{definition}[$\alpha$-Bandwidth Property]
We say that a cluster $C$ of graph $G$ has the \emph{$\alpha$-bandwidth property}, for some parameter $\alpha>0$, iff for every partition $(A,B)$ of vertices of $C$, 
$|E(A,B)|\ge \alpha\cdot\min\set{|\delta_G(A)\cap \delta_G(C)|, |\delta_G(B)\cap \delta_G(C)|}$.
\end{definition}
%\mynote{this definition is not good. It means that $S$ has $\alpha$-bandwidth property if there exists a partition $(A,B)$ of $V(S)$ with $|E(A,B)|\ge \alpha\cdot\min\set{|\delta(A)\cap \delta(S)|, |\delta(B)\cap \delta(S)|}$. This is why "any" is dangerous to use in definitions, it may mean "every" or "there is", and in this context it means "there is". You should say "For every partition" and be careful with using "any" in definitions (not use it if possible).}

The following immediate observation provides an equivalent definition  of the bandwidth property that is helpful to keep in mind. 

\begin{observation}\label{obs: wl-bw}
	Let $G$ be a graph and $C\subseteq G$ a subgraph of $G$, and let $0<\alpha<1$ be a parameter. Cluster $C$ has the $\alpha$-bandwidth property iff the set $T(C)$ of vertices is $\alpha$-well-linked in graph $C^+$ (see \Cref{def: Graph C^+}). 
\end{observation}



The next observation, that is quite standard, shows that a cluster with a bandwidth property must contain many edges.



%\mynote{please add a proof. idea: if $k_v<2k/3$, can partition vertices of $C$ into $A,B$ with $|\delta(C)\cap \delta(A)|,|\delta(C)\cap \delta(B)|\geq 2k/3$. From bw property there must be enough edges connecting $A$ to $B$. Otherwise, look at the cut where $A=\set{v}$, $B=V(C)\setminus\set{v}$ and use the same argument.}
\begin{observation}\label{obs: bw many edges}
	Let $G$ be a graph and $C\subseteq G$ a subgraph of $G$ that has the $\alpha$-bandwidth property, for some $0<\alpha<1$. Denote $|\delta_G(C)|=k$, and let $v$ be the vertex maximizing $k_v=|\delta_G(C)\cap \delta_G(v)|$ among all vertices of $C$. Then $|E(C)|\geq \alpha\cdot (k-k_v)/3$.
\end{observation}

\begin{proof}
We rank all vertices $u$ of $C$ in decreasing order of $k_u$: $u_1,u_2,\ldots,u_r$ where $u_1=v$.
Assume first that $k_v<2k/3$. For each $1\le i\le r$, we denote $s_i=\sum_{1\le t\le i}k_{u_i}$. We first show that there exists an integer $1\le i<r$, such that $k/3\le s_i\le 2k/3$. In fact, if $k_{u_1}\ge k/3$, then $s_1$ satisfies the above property. Otherwise we have $k_{u_1}<k/3$, and we know that the sequence $s_1,\ldots,s_r$ is increasing and $s_r=k$, and the difference between every pair $s_i,s_{i+1}$ is less than $k/3$. It is easy to verify that there exists an integer $1\le i<r$, such that $k/3\le s_i\le 2k/3$. Let $i^*$ be such an integer, and consider the cut $(\set{u_t\mid 1\le t\le i^*},\set{u_t\mid i^*< t\le r})$ of $C$. From the $\alpha$-bandwidth property of $C$, the number of edges in this cut is at least $\alpha\cdot (k/3)\ge \alpha(k-k_v)/3$. Assume now that $k_v\ge 2k/3$. Then consider the the cut $(\set{u_1},\set{u_t\mid 2\le t\le r})$ of $C$. From the $\alpha$-bandwidth property of $C$, the number of edges in this cut is at least $\alpha(k-k_v)\ge \alpha(k-k_v)/3$.
\end{proof}


We use the following theorem and its immediate corollary, which are easy consequences of the max-flow min-cut theorem. For completeness, we provide its proof in Appendix~\ref{apd: Proof of bandwidth_means_boundary_well_linked}. 
%\mynote{again, say that this is a well-known result that follows from the duality between cuts and flows.}

%\mynote{can we do this theorem for a graph $G$ and a set $T$ of terminals that is $\alpha$-well-linked? Then do this as a corollary?} 
%\mynote{Also, please put specific subsections of Appendix where each theorem is proved, so it is easy to go back and forth between them and one does not need to search.}

%\mynote{should we say here that every terminal of $T_1\cup T_2$ is an endpoint of exactly one path?}

%\mynote{maybe use one-to-one routing in both the theorem and the corollary?}

\begin{theorem}
\label{thm: bandwidth_means_boundary_well_linked}
There is an efficient algorithm, that, given a graph $G$, a set $T$ of vertices of $G$ that is $\alpha$-well-linked, and a pair $T_1,T_2$ of disjoint equal-cardinality subsets of $T$, computes an one-to-one routing $\qset$ of vertices of $T_1$ to vertices of $T_2$ with $\cong_G(\qset)\leq \ceil{1/\alpha}$.
\end{theorem}

%\mynote{is this one-to-one routing? }

\begin{corollary}
\label{cor: bandwidth_means_boundary_well_linked}
There is an efficient algorithm, that, given a graph $G$, a cluster $S$ of $G$ that has $\alpha$-bandwidth property for some $0<\alpha<1$, and a pair $E_1,E_2$ of disjoint equal-cardinality subsets of $\delta(S)$, computes an one-to-one routing $\qset$ of edges of $E_1$ to edges of $E_2$, with $\cong_G(\qset)=\ceil{1/\alpha}$, such that for each path $Q\in\qset$, all its edges except for the first and the last edge of $Q$ belong to $E(S)$.
\end{corollary}
%\mynote{can you make above thm efficient alg?}


%\mynote{This theorem should go to a separate heading called "Well-Linked Decomposition". maybe give the algorithm a name? AlgWLD?}
%\subsection{Well-linked Decomposition}

%\mynote{say that well-linked decompositions have been used extensively in graph algorithms. We provide a well-known variant, that generalizes.... Again, you don't want to make it look like we claim this as a new result, that would look bad.}

The technique of well-linked decompositions has been used extensively in graph algorithms (see e.g. \cite{racke2002minimizing,chekuri2004edge,andrews2010approximation,chuzhoy2012polylogarithmic,chuzhoy2012routing,chekuri2016polynomial,chuzhoy2016improved,chuzhoy2019towards}). We provide a well-known variant, that generalizes Theorem 2.8 in \cite{chuzhoy2012routing}, that shows the existence of an algorithm for decomposing a cluster of a graph into subclusters that have $\alpha$-bandwidth property.
We denote this algorithm by $\algwl^{(\alpha)}$, and its proof is provided in Appendix~\ref{apd: Proof of well_linked_decomposition}.



%\mynote{because we are allowing parallel edges, probably all $\log n$'s need to be replaced by $\log m$'s. Thm statement should include the def of $m$ or $n$. Cal you also recheck the last bullet whether it's $O(\alpha log m)$ or $O(\alpha log^{1.5}m)$? Al;so, I need the precise edge-congestion, I used $100$ as a placeholder, and I assumed it's $100/\alpha$ in next section. Once this thm is finalized, the statement of the thm for layered decomposition need to be updated, and its proof too; see \Cref{sec: layered well linked}}
%\znote{$n$ replaced by $m$. re-checked: $O(\alpha \log m)$, and congestion= $100$ but not $100/\alpha$.}

%\mynote{I cahnged the thm statement but not the proof}

%\mynote{I need the theorem updated yet again. I have highlighted the statement I have added. If there is a vertex $v$ with $|\delta(v)\cap \delta(S)|\geq 0.9|\delta(S)|$, then  edges of $\delta(v)\cap \delta(S)$ should always have budget $1$. When you split a cluster, they will always be on the bigger side, so they will never be charged and their budget can stay the same.}

\begin{theorem}
	\label{thm:well_linked_decomposition}
	There is an efficient algorithm, that, given a graph $G$ with $n$ vertices and $m$ edges, a vertex-induced subgraph $S$ of $G$, and a parameter $\alpha\le 1/(48\log^2 m)$, computes a collection $\rset$ of vertex-induced subgraphs (called clusters) of $S$, such that:
	\begin{itemize}
		\item the vertex sets $\set{V(R)}_{R\in \rset}$ partition $V(S)$;
		\item for every cluster $R\subseteq\rset$, $|\delta(R)|\le |\delta(S)|$;
		\item every cluster $R\subseteq\rset$ has the $\alpha$-bandwidth property; and %\mynote{this needs to be fixed}
		\item $\sum_{R\in \rset}|\delta(R)|\le |\delta(S)|\cdot\left(1+O(\alpha\cdot \log m)\right)$.
		%, and moreover, if there is a vertex $v\in V(S)$ with $|\delta(v)\cap \delta(S)|\geq 0.9|\delta(S)|$, then $\sum_{R\in \rset}|\delta(R)|\le|\delta(v)|+ \left(|\delta(S)|-|\delta(v)|\right )\cdot\left(1+O(\alpha\cdot \log m)\right)$.\znote{delete moreover}
	\end{itemize}

Additionally, the algorithm computes, 
 for every cluster $R\in \rset$, a set $\pset(R)=\set{P(e)\mid e\in \delta_G(R)}$ of paths, such that, for every edge $e\in \delta_G(R)$, path $P(e)$ has $e$ as its first edge and some edge of $\delta_G(S)$ as its last edge, and all inner vertices of $P(e)$ lie in $V(S)\setminus V(R)$. Moreover, for every cluster $R\in \rset$, the set $\pset(R)$ of paths causes edge-congestion at most $100$ in $G$.
\end{theorem}

We will also repeatedly use the following lemma, whose proof is provided in \Cref{apd: Proof of routing path extension}.
\begin{lemma}
\label{lem: routing path extension}
Let $G$ be a graph, let $T$ be a set of vertices that are $\alpha$-well-linked in $G$, and let $T'$ be a subset of $T$. Let $\pset'$ be a set of paths in $G$ routing the vertices of $T'$ to some vertex $x$ of $G$. Then there is a set $\pset$ of paths routing vertices of $T$ to $x$, such that, for every edge $e\in E(G)$,
$\cong_G(\pset,e)\le \ceil{\frac{|T|}{|T'|}}(\cong_G(\pset',e)+\ceil{1/\alpha})$.
\end{lemma}


\input{for-prelims}


%\input{guiding-paths-prelims}

\iffalse
\subsection{Laminar Family of Clusters and the Decomposition Tree}
Let $G$ be any graph, and let $\lset$ be a family of connected subgraphs of $G$, that we call {clusters}. We say that $\lset$ is a \emph{laminar family}, iff for all $S,S'\in \lset$, either $S\cap S'=\emptyset$, or $S\subseteq S'$, or $S\subseteq S'$ holds.
We will also always assume that $G\in \lset$ for any laminar family of subgraphs of $G$.

Given a laminar family $\lset$ of clusters of $G$, we associate a \emph{paritioning tree} $\tau(\lset)$ with it, which is a rooted tree defined as follows. The vertex set of the tree is $\set{v(S)\mid S\in \lset}$. The root of the tree is $v(G)$ -- the vertex associated with the graph $G$ itself. 
In order to define the edge set, consider a pair $S,S'\in \lset$ of clusters. If $S\subsetneq S'$, and there is no other cluster $S''\in \lset$ with $S\subsetneq S''\subsetneq S'$, then we add an edge $(v(S),v(S'))$ to the tree $\tau(\lset)$; vertex $v(S)$ becomes  a child vertex of $v(S')$ in the tree. In this case, we say that cluster $S$ is a \emph{child cluster} of cluster $S'$, and cluster $S'$ is the \emph{parent cluster} of $S$. We denote by $\wset_{\lset}(S)$ the set of all child clusters of a cluster $S\in \lset$.
\fi


\subsection{Minimum Cuts and Gomory-Hu Tree}
\label{subsec: GH tree}
Let $G$ be a graph and let $s,t$ be two vertices of $G$. We denote by $\text{min-cut}_G(s,t)$ the size of a minimum cut $(S,T)$ in $G$, where $s\in S$ and $t\in T$.
Gomory and Hu~\cite{gomory1961multi} proved the following theorem.
\begin{theorem}[\cite{gomory1961multi}]\label{thm: GH tree properties}
There is an efficient algorithm, that, given a weighted graph $G=(V,E,w)$, computes a weighted tree $\tau=(V,E',w')$, such that
\begin{itemize}
\item for every pair $s,t$ of distinct vertices of $V$, if we denote by $P_{s,t}$ the unique path in $\tau$ connecting $s$ to $t$, then $\text{min-cut}_G(s,t)=\min_{e\in P_{s,t}}\set{w'(e)}$; and
\item for every pair $s,t$ of distinct vertices of $V$ and a min-cut $(S,T)$ in $G$ separating $s$ from $t$, then the same cut $(S,T)$ is also a min-cut in $\tau$ separating $s$ from $t$, and vice versa.
\end{itemize}
\end{theorem}
Let $G$ be a weighted graph, then the tree $\tau$ obtained from applying the algorithm in the above theorem to $G$ is called the \emph{Gomory-Hu tree} of $G$.
In this paper, we will use the following immediate corollary of the above theorem.
\begin{corollary}
\label{cor: G-H tree_edge_cut}
Let $G$ be a graph and let $\tau$ be a Gomory-Hu tree of graph $G$. Then for each edge $e=(u,u')\in E(\tau)$, if we denote by $U,U'$ the two subtrees obtained from $\tau$ by removing the edge $e$, with $u\in U$ and $u'\in U'$, then the cut $(V(U),V(U'))$ is a min-cut in $G$ separating $u$ from $u'$.
\end{corollary}

We will use the following lemma to handle graphs whose Gomory-Hu tree is a path. Its proof appears in Appendix~\ref{apd: Proof of GH tree path vs contraction}.

\begin{lemma}
\label{lem: GH tree path vs contraction}
Let $G$ be a graph whose Gomory-Hu tree $\tau$ is a path. %Denote $T=(v_1,\ldots,v_n)$, where vertices appear on path $T$ in this order.
Let $\cset$ be a set of vertex-disjoint clusters of $G$, such that $\bigcup_{C\in \cset}V(C)=V(G)$, and the vertices in each cluster of $\cset$ induce a subpath in $\tau$ (equivalently, if we denote $\tau=(v_1,\ldots,v_n)$, where vertices appear on path $\tau$ in this order, then for each cluster $C\in \cset$, there exist two integers $i_C,j_C$, such that $V(C)=\set{v_{t}\mid i_C\le t\le j_C}$).
Then $\tau_{|\cset}$, the contracted path, is a Gomory-Hu tree of the contracted graph $G_{|\cset}$.
\end{lemma}



We will also use the following lemma on min-cuts in a graph. Its proof is provided in Appendix~\ref{apd: Proof of multiway cut with paths sets}.
\begin{lemma}\label{lem: multiway cut with paths sets}
	There is an efficient algorithm, that, given a graph $G$ and a collection $S=\set{s_1,\ldots,s_k}$ of its vertices, computes, for all $1\leq i\leq k$, a set $A_i$ of vertices of $G$, and a collection $\qset_i$ of paths in $G$, such that the following hold:
	
	\begin{itemize}
		\item for all $1\leq i\leq k$, $S\cap A_i=\set{s_i}$, and moreover, $(A_i,V(G)\setminus A_i)$ is a minimum cut separating $s_i$ from the vertices of $S\setminus\set{s_i}$ in $G$;
		\item for all $1\leq i<i'\leq k$, $A_i\cap A_{i'}= \emptyset$; and
		\item for all $1\leq i\leq k$, $\qset_i=\set{Q_i(e)\mid e\in \delta_G(A_i)}$, where for each $e\in \delta_G(A_i)$, path $Q_i(e)$ has $e$ as its first edge and $s_i$ as its last vertex, with all internal vertices of $Q_i(e)$ lying in $A_i$. Moreover, the paths in $\qset_i$ are mutually edge-disjoint.
	\end{itemize}
\end{lemma}



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\mynote{Define a trivial solution of value at most $|E(G)|^2$, state a thm that it can be computed efficiently. Also: prove that we can check efficiently whether solution of value $0$ exists and if so, can compute it.}
%The goal is to find a drawing of $G$ in the plane that respects 
%In 
%~as the problem of finding a drawing of $G$ in the plane that respects a rotation system $\tSigma$ and moreover achieves the minimum number of crossings. The rotation system $\tSigma$ defines an ordering on the edges adjacent to each vertex, and a drawing $\phi$ respects an ordering $\tSigma$ if the clockwise ordering of the edges entering each vertex is the same as what is specified by $\tSigma$ (A detailed definition is given in Section \ref{sec:cr_rotation_system}).

\iffalse
\mynote{is this needed?}
If a crossing is caused by the intersection of the images of a pair of edges $e,e'$ (namely $\phi(e)$ and $\phi(e')$), then we say that the edges $e$ and $e'$ \emph{participate} in the crossing, or the pair of edges $e$ and $e'$ \emph{cross}.
We also say that an edge $e$ is \emph{crossed} in a drawing $\phi$ if the edge $e$ participates in at least one crossing of $\phi$.
For any pair $E_1, E_2 \subseteq E$ of subsets of edges, we denote by $\cro_{\phi}(E_1, E_2)$ the number of crossings in $\phi$ in which the images of edges of $E_1$ intersect the images of edges of $E_2$.
%For a subset $E' \subseteq E$ of edges, we denote by $\cro_{\phi}(E')$ the number of crossings in $\phi$ in which the images of edges of $E'$ intersect with each other \mynote{I am not a fan of this notation because this can be naturally interpreted as all crossings in which the edges of $E'$ participate. Maybe $\cro(E',E')$ is a better notation for this?} 
Clearly, for each subset $E' \subseteq E$, $\cro(\phi)=\cro_{\phi}(E',E')+\cro_{\phi}(E',E\setminus E')+\cro_{\phi}(E\setminus E',E\setminus E')$.
Since at most two edges participate in a crossing, for disjoint subsets $E_1,\ldots,E_r$ of $E$, $\sum_{1\le i\le r}\cro_{\phi}(E,E_i)\le 2\cdot\cro(\phi)$.
For a subgraph $C$ of $G$, we denote $\cro_{\phi}(C)=\cro_{\phi}(E(C),E(C))$, or equivalently $\cro_{\phi}(C)=\cro(\phi(C))$. Similarly, for two subgraphs $C,C'$, we denote $\cro_{\phi}(C,C')=\cro_{\phi}(E(C),E(C'))$.
%So if clusters $C_1,\ldots,C_r$ of $G$ are mutually vertex-disjoint or even edge-disjoint, $\sum_{1\le i\le r}\cro_{\phi}(C_i)\le 2\cdot\cro(\phi)$.
%For a drawing $\phi$ of $G$ and a connected subgraph $S$ of $G$, we denote by $\phi(S)$ the induced drawing of $\phi$ on $S$.
\fi



\iffalse
\textbf{Bridges and Extensions of subgraphs.}
Let $G$ be a graph, and let $C\subseteq G$ be a subgraph of $G$. A \emph{bridge} for $C$ in graph $G$ is either (i) an edge $e=(u,v)\in E(G)$ with $u,v\in V(C)$ and $e\not \in E(C)$; or (ii) a connected component of $G\setminus V(C)$. %, together with all edges (and their endpoints) between the component and $C$.
%{\znote{this is slightly different from the previous version, only for brevity in notations}}
We denote by $\rset_G(C)$ the set of all bridges for $C$ in graph $G$. For each bridge $R\in \rset_G(C)$, we define the set of vertices $L(R)\subseteq V(C)$, called the \emph{legs of $R$}, %to contain every vertex $v\in V(C)$ that has a neighbor in $R$.
as follows. If $R$ consists of a single edge $e$, then $L(R)$ contains the endpoints of $e$. Otherwise, $L(R)$ contains all vertices $v\in V(C) $, such that $v$ has a neighbor that belongs to $R$. %, such that some edge connecting $v$ to a vertex of $R$ belongs to $G$.

Next, we define an \emph{extension} of the subgraph $C\subseteq G$, denoted by $X_G(C)$. The extension contains, for every bridge $R\in \rset_G(C)$, a tree $T_R$, that is defined as follows. If $R$ is a bridge consisting of a single edge $e$, then the corresponding tree $T_R$ only contains the edge $e$. Otherwise, 
let $R'$ be the subgraph of $G$ consisting of the graph $R$, the vertices of $L(R)$, and all edges of $G$ connecting vertices of $R$ to vertices of $L(R)$.
We let $T_R\subseteq R'$ be a tree, whose leaves are precisely the vertices of $L(R)$, that contains smallest number of edges among all such trees. Note that such a tree exists because graph $R$ is connected. % and thus contains a spanning tree $T$ as a subgraph. %Finally we can recursively remove all leaves of the tree that are not in $L(R)$. %This gives one such tree, illustrating the existence of $T_R$. 
We let the extension of $C$ in $G$ be $X_G(C)=\set{T_R\mid R\in \rset_G(C)}$.
\fi


%\textbf{Contracting Connected Subgraphs.}
%Let $G$ be a graph, and let $C\subseteq G$ be a connected subgraph of $G$. We can obtain a new graph, $G_{|C}$ from $G$ by contracting $C$ as follows. We merge all vertices of $C$ into a single vertex $v(C)$, that we call a \emph{super-node}. We then delete all self-loops and parallel edges. 
%\mynote{I chose to delete parallel edges to be consistent with graph notation, and I think this works better because when parallel edges are present one can't claim there is a unique planar drawing. Not sure if this will be needed at the end.}

\iffalse
\textbf{Sparsest Cut.} 
Suppose we are given a graph $G=(V,E)$, and a subset $\tset\sse V$ of $k$ vertices, called terminals. 
The sparsity of a cut $(S,\nots)$ in $G$ is $\Phi(S)=\frac{|E(S,\nots)|}{\min\set{|S\cap \tset|, |\nots\cap \tset|}}$, and the value of the sparsest cut in $G$ is defined to be:
$\Phi(G)=\min_{S\subset V}\set{\Phi(S)}$.
The goal of the sparsest cut problem is to find a cut of minimum sparsity. Arora, Rao and Vazirani~\cite{ARV} have shown an $O(\sqrt {\log n})$-approximation algorithm for the sparsest cut problem. We denote this algorithm by \algsc, and its approximation factor by $\alphasc(n)=O(\sqrt{\log n})$.
\fi

%A problem dual to sparsest cut is the maximum concurrent flow problem. For the above definition of the sparsest cut problem, the corresponding variation of the concurrent flow problem asks to find the maximum value $\lambda$, such that every pair of terminals  in $\tset\choose 2$ can send $\lambda/k$ flow units to each other simultaneously with no congestion. The flow-cut gap is the maximum ratio, in any graph, between the value of the minimum sparsest cut and the maximum value $\lambda$ of concurrent flow. The value of the flow-cut gap in undirected graphs, that we denote by $\beta(n)$ throughout the paper, is $\Theta(\log n)$~\cite{leighton1999multicommodity}. %, GVY,LLR,Aumann-Rabani}. 
%Therefore, if $\Phi(G)=\alpha$, then every pair of terminals can send $\frac{\alpha}{k\beta(n)}$ flow units to each other with no congestion.
%Equivalently, every pair of terminals can send $1/k$ flow units to each other with congestion at most $\beta(n)/\alpha$. Moreover, any matching on the set $\tset$ of terminals can be fractionally routed with congestion at most $2\beta(n)/\alpha$.



\iffalse
Let $G$ be a graph, and let $S$ be a subset of vertices of $G$, and let $0<\alpha<1$, such that $S$ is $\alpha$-well-linked. 
We now define the sparsest cut and the concurrent flow instances corresponding to $S$ as follows. For each edge in $\out(S)$, we subdivide the edge by adding a new vertex $t_e$ to it. Let $G'$ denote the resulting graph and let $T$ denote the set of all vertices $t_e$ for $e\in \out_G(S)$. Consider the graph $H=G'[S]\cup \out_{G'}(S)$. We can naturally define an instance of the non-uniform sparsest cut problem on $H$ where the set of terminals is $T$. We then have the following well-known observation.
\begin{observation}
	Let $G$, $S$, $H$ and $T$ be defined as above, and let $0<\alpha <1$, such that $S$ is $\alpha$-well-linked. Then every pair of vertices in $T$ can send one flow unit to each other in $H$, such that the maximum congestion on any edge is at most $\beta(n)|T|/\alpha$. Moreover if $M$ is any partial matching on the vertices of $T$, then we can send one flow unit between every pair $(u,v)\in M$ in graph $H$, with maximum congestion at most $2\beta(n)/\alpha$.
\end{observation}
%\vspace{-0.3cm}

\iffalse
The following theorem shows the technique of \emph{well-linked decomposition}, which has been used extensively in graph algorithms (e.g., see~\cite{racke2002minimizing,chekuri2005multicommodity}). %For completeness we provide its proof in Appendix.
\begin{theorem}[Terminal Well-Linked Decomposition]
	\label{thm:well_linked-decomposition}
	There is an efficient algorithm, that, given any connected graph $G$ and a subset $T\subseteq V(G)$ of its vertices with $|T|=k$, computes a collection $\set{G_1,\ldots,G_r}$ of connected subgraphs of $G$, such that:
	\begin{enumerate}
		\item for each $1\le i\le r$, denote $V_i=V(G_i)$, then $(V_1,\ldots,V_r)$ forms a partition of $V(G)$;
		\item for each $1\le i\le r$, denote $T_i=T\cap V_i$, then the subset $T_i\cup \Gamma(V_i)$ of vertices is $\Omega(\frac{1}{\log^{3/2}k\cdot\log\log k})$-well-linked in $G_i$; and
		\item $\sum_{1\le i\le r}|\out(V_i)|\le 0.01 k$, and $\sum_{1\le i\le r}|T_i\cup \Gamma(V_i)|\le 1.01 k$.
	\end{enumerate}
\end{theorem}
\fi
\fi

\iffalse
\paragraph{Non-interfering paths.}
To be used later for locally non-interfering/non-interfering paths (for this the definition should be adapted). We may also keep it in prelims as a definition of crossing paths. Maybe we should also define a drawing of a path as a concatenation of images of its edges. We use it quite a bit.
\begin{definition}
	Let $\gamma,\gamma'$ be two curves in the plane or on the sphere. We say that $\gamma$ and $\gamma'$ \emph{cross},  iff there is a disc $D$, whose boundary is a simple closed curve that we denote by $\beta$, such that: 
	
	\begin{itemize}
		\item  $\gamma\cap D$ is a simple open curve, whose endpoints we denote by $a$ and $b$; 
		\item $\gamma'\cap D$ is a simple open curve, whose endpoints we denote by $a'$ and $b'$; and
		
		\item $a,a',b,b'\in \beta$, and they appear on $\beta$ in this circular order.
	\end{itemize}
\end{definition}
Given a graph $G$ embedded in the plane or on the sphere, we say that two paths $P,P'$ in $G$ cross iff their images cross. Similarly, we say that a path $P$ crosses a curve $\gamma$ iff the image of $P$ crosses $\gamma$.
\fi




==> previous_material.tex <==
\section{Useful things from FOCS paper}


By default, all logarithms are to the base of $2$. All graphs are finite, simple and undirected. Graphs with parallel edges are explicitly referred to as multi-graphs.

We follow standard graph-theoretic notation. Assume that we are given a graph $G=(V,E)$. 
%We denote by $n$ the number of vertices and by $\Delta$ the maximum vertex degree in the graph which may not necessarily be a constant.
For a vertex $v\in V$, we denote by $\delta_G(v)$ the set of all  edges of $G$ that are incident to $v$.
For two disjoint subsets $A,B$ of vertices of $G$, we denote by $E_G(A,B)$ the set of all edges with one endpoint in $A$ and another in $B$.
For a subset $S\subseteq V$ of vertices, we denote by $E_G(S)$ the set of all edges with both endpoints in $S$, and we denote by $\out_G(S)$ the subset of edges of $E$ with exactly one endpoint in $S$, namely $\out_G(S)=E_G(S, V\!\setminus\! S)$. 
We denote by $G[S]$ the subgraph of $G$ induced by $S$.
We sometimes omit the subscript $G$ if it is clear from the context. 
%We will also refer to connected subgraphs of $G$ by \emph{clusters}. \mynote{do we actually do it for subgraphs or connected components?}
%For a connected subgraph $C$ of the graph $G$, we denote $\out(C)=\out(V(C))$, and we use $\Gamma(C)$ to denote the set of all vertices of $C$ that serve as endpoints of edges in $\out(C)$.
%
%Given a set $\pset$ of paths in a graph $G$, we denote by $E(\pset)=\bigcup_{P\in\pset}E(P)$ the set of all edges participating in the paths of $\pset$.
%For each edge $e\in E(G)$, we denote by $c_{\pset}(e)$ the number of paths in $\pset$ that contain the edge $e$. We also denote $c(\pset)=\max_{e\in E(G)}\set{c_{\pset}(e)}$, and we refer to $c(\pset)$ as the \emph{congestion} caused by the paths in $\pset$.
%
%
%\textbf{Connectivity.}
We say that a graph $G$ is $\ell$-connected for some integer $\ell>0$, if there are $\ell$ vertex-disjoint paths between every pair of vertices in $G$. %Throughout the paper, we use connectivity to denote vertex-connectivity, unless specified otherwise.

Given a graph $G=(V,E)$, a \emph{drawing}  $\phi$ of $G$ is an embedding of the graph into the plane, that maps every vertex to a point and every edge to a continuous curve that connects the images of its endpoints. We require that the interiors of the curves representing the edges do not contain the images of any of the vertices. We say that two edges \emph{cross} at a point $p$, if the images of both edges contain $p$, and $p$ is not the image of a shared endpoint of these edges. We require that no three edges cross at the same point in a drawing of $\phi$. 
We say that $\phi$ is a \emph{planar drawing} of $G$ iff no pair of edges of $G$ crosses in $\phi$.
For a vertex $v\in V(G)$, we denote by $\phi(v)$ the image of $v$, and for an edge $e\in E(G)$, we denote by $\phi(e)$ the image of $e$ in $\phi$. For any subgraph $C$ of $G$, we denote by $\phi(C)$ the union of images of all vertices and edges of $C$ in $\phi$. For a path $P\subseteq G$, we sometimes refer to $\phi(P)$ as the \emph{image of $P$ in $\phi$}. Note that a drawing of $G$ in the plane naturally defines a drawing of $G$ on the sphere and vice versa; we use both types of drawings.
Given a graph $G$ and a drawing $\phi$ of $G$ in the plane, we use $\cro(\phi)$ to denote the number of crossings in $\phi$. Let $\phi'$ be the drawing of $G$ that is a mirror image of $\phi$. We say that $\phi$ and $\phi'$ are \emph{identical} drawings of $G$, and that their \emph{orientations} are different. We sometime say that $\phi'$ is obtained by \emph{flipping} the drawing $\phi$. If $\gamma$ is a simple closed curve in $\phi$ that intersects $G$ at vertices only, and $S$ is the set of vertices of $G$ whose images lie on $\gamma$, with $|S|\geq 3$, then we say that the circular orderings of the vertices of $S$ along $\gamma$ in $\phi$ and $\phi'$ are identical, but the orientations of the two orderings are different, or opposite.


Whitney \cite{whitney1992congruent} proved that every $3$-connected planar graph has a unique planar drawing.
Throughout, for a $3$-connected planar graph $G$, we denote by $\rho_G$ the unique planar drawing of $G$.


\textbf{Problem Definitions.} 
The goal of the \mcn~problem is to compute a drawing the input graph $G$ in the plane with smallest number of crossings.
The value of the optimal solution, also called the \emph{crossing number} of $G$, is denoted by $\optcro(G)$.

We also consider a closely related problem called Crossing Number with Rotation System (\CNwRS). In this problem, we are given a multi-graph $G$, and, for every vertex $v\in V(G)$, a circular ordering $\oset_v$ of its incident edges. We denote $\Sigma=\set{\oset_v}_{v\in V(G)}$, and we refer to $\Sigma$ as a \emph{rotation system}.  We say that a drawing $\phi$ of $G$ \emph{respects} the rotation system $\Sigma$ if the following holds. For every vertex $v\in V(G)$, let $\eta(v)$ be an arbitrarily small disc around $v$ in $\phi$. Then the images of the edges of $\delta_G(v)$ in $\phi$ must intersect the boundary of $\eta(v)$ in a circular order that is identical to $\oset_v$ (but we can choose the orientation of this ordering, that may be either clock-wise or counter-clock-wise). In the \CNwRS problem, the input is a {\bf multi-graph} $G$ with a rotation system $\Sigma$, and the goal is to compute a drawing of $G$ in the plane that respects $\Sigma$ and minimizes the number of crossings.

%The goal is to find a drawing of $G$ in the plane that respects 
%In 
%~as the problem of finding a drawing of $G$ in the plane that respects a rotation system $\tSigma$ and moreover achieves the minimum number of crossings. The rotation system $\tSigma$ defines an ordering on the edges adjacent to each vertex, and a drawing $\phi$ respects an ordering $\tSigma$ if the clockwise ordering of the edges entering each vertex is the same as what is specified by $\tSigma$ (A detailed definition is given in Section \ref{sec:cr_rotation_system}).

\iffalse
\mynote{is this needed?}
If a crossing is caused by the intersection of the images of a pair of edges $e,e'$ (namely $\phi(e)$ and $\phi(e')$), then we say that the edges $e$ and $e'$ \emph{participate} in the crossing, or the pair of edges $e$ and $e'$ \emph{cross}.
We also say that an edge $e$ is \emph{crossed} in a drawing $\phi$ if the edge $e$ participates in at least one crossing of $\phi$.
For any pair $E_1, E_2 \subseteq E$ of subsets of edges, we denote by $\cro_{\phi}(E_1, E_2)$ the number of crossings in $\phi$ in which the images of edges of $E_1$ intersect the images of edges of $E_2$.
%For a subset $E' \subseteq E$ of edges, we denote by $\cro_{\phi}(E')$ the number of crossings in $\phi$ in which the images of edges of $E'$ intersect with each other \mynote{I am not a fan of this notation because this can be naturally interpreted as all crossings in which the edges of $E'$ participate. Maybe $\cro(E',E')$ is a better notation for this?} 
Clearly, for each subset $E' \subseteq E$, $\cro(\phi)=\cro_{\phi}(E',E')+\cro_{\phi}(E',E\setminus E')+\cro_{\phi}(E\setminus E',E\setminus E')$.
Since at most two edges participate in a crossing, for disjoint subsets $E_1,\ldots,E_r$ of $E$, $\sum_{1\le i\le r}\cro_{\phi}(E,E_i)\le 2\cdot\cro(\phi)$.
For a subgraph $C$ of $G$, we denote $\cro_{\phi}(C)=\cro_{\phi}(E(C),E(C))$, or equivalently $\cro_{\phi}(C)=\cro(\phi(C))$. Similarly, for two subgraphs $C,C'$, we denote $\cro_{\phi}(C,C')=\cro_{\phi}(E(C),E(C'))$.
%So if clusters $C_1,\ldots,C_r$ of $G$ are mutually vertex-disjoint or even edge-disjoint, $\sum_{1\le i\le r}\cro_{\phi}(C_i)\le 2\cdot\cro(\phi)$.
%For a drawing $\phi$ of $G$ and a connected subgraph $S$ of $G$, we denote by $\phi(S)$ the induced drawing of $\phi$ on $S$.
\fi

{\bf Faces and Face Boundaries.}
Suppose we are given a planar graph $G$ and a drawing $\phi$ of $G$ in the plane. The set of faces of $\phi$ is the set of all connected regions of $\mathbb{R}^2\setminus \phi(G)$. We designate a single face of $\phi$ as the ``outer'', or the ``infinite'' face. 
The \emph{boundary} $\delta(F)$ of a face $F$ is a sub-graph of $G$ consisting of all vertices and edges of $G$ whose image is incident to $F$. Notice that, if graph $G$ is not connected, then boundary of a face may also be not connected. Unless $\phi$ has a single face, the boundary $\delta(F)$ of every face $F$ of $\phi$ must contain a simple cycle $\delta'(F)$ that separates $F$ from all other faces. We sometimes refer to graph $\delta(F)\setminus\delta'(F)$ as the \emph{inner boundary} of $F$. Lastly, observe that, if $G$ is $2$-connected, then the boundary of every face of $\phi$ is a simple cycle. %, and its inner boundary is empty.

\iffalse
%\vspace{-0.1cm}
\begin{definition}[face, outer face]
	Given a graph $G$ and a planar drawing $\phi$ of $G$, the set of faces of $\phi$ are defined to be the set of connected regions in $\mathbb{R}^2\setminus \phi(G)$, and we denote it by $\fset(\phi)$. Moreover, exactly one of these faces is infinite which we refer to as the \emph{outer face}.
\end{definition}
%\vspace{-0.2cm}

%\vspace{-0.1cm}
\begin{definition}[boundary, inner boundary, outer boundary, and point of contact]
	For each face $F\in \fset(\phi)$, the boundary of the face $F$ is defined as the set of vertices and edges that are incident to the face $F$, and we denote it by $\delta(F)$.  Note that if the graph is connected, the boundary of $F$ also forms a connected graph. We may also call it the full boundary to emphasize the contrast to the inner/outer boundary defined next.
	
	For a face that is not the outer face, we define the \emph{outer boundary} $\delta^{out}(F)\subseteq \delta(F)$ to be the simple cycle that separates the face $F$ from the outer face. In other words, if $D(F)$ denotes the closed disc whose boundary is $\delta^{out}(F)$, then $D(F)$ should contain $F$. 
	Note that if $G$ is $2$-connected, the boundary of each face $F\in \fset(\phi)$ is a simple cycle, i.e., $\delta(F)=\delta^{out}(F)$. 
	Moreover, we define the \emph{inner boundary} as $\delta^{in}(F)$ to be the set of edges in $\delta(F)\setminus \delta^{out}(F)$, together with their endpoint vertices.
	
	Finally, for a connected graph, we can define for each vertex $v$ on the boundary $\delta(F)$, the \emph{point of contact} of $v$ to be the vertex on the outer boundary with minimum distance to $v$.
\end{definition}
%\vspace{-0.2cm}
\fi



\textbf{Bridges and Extensions of Sub-Graphs.}
Let $G$ be a graph, and let $C\subseteq G$ be a sub-graph of $G$. A \emph{bridge} for $C$ in graph $G$ is either (i) an edge $e=(u,v)\in E(G)$ with $u,v\in V(C)$ and $e\not \in E(C)$; or (ii) a connected component of $G\setminus V(C)$. %, together with all edges (and their endpoints) between the component and $C$.
%{\znote{this is slightly different from the previous version, only for brevity in notations}}
We denote by $\rset_G(C)$ the set of all bridges for $C$ in graph $G$. For each bridge $R\in \rset_G(C)$, we define the set of vertices $L(R)\subseteq V(C)$, called the \emph{legs of $R$}, %to contain every vertex $v\in V(C)$ that has a neighbor in $R$.
as follows. If $R$ consists of a single edge $e$, then $L(R)$ contains the endpoints of $e$. Otherwise, $L(R)$ contains all vertices $v\in V(C) $, such that $v$ has a neighbor that belongs to $R$. %, such that some edge connecting $v$ to a vertex of $R$ belongs to $G$.

Next, we define an \emph{extension} of the subgraph $C\subseteq G$, denoted by $X_G(C)$. The extension contains, for every bridge $R\in \rset_G(C)$, a tree $T_R$, that is defined as follows. If $R$ is a bridge consisting of a single edge $e$, then the corresponding tree $T_R$ only contains the edge $e$. Otherwise, 
let $R'$ be the sub-graph of $G$ consisting of the graph $R$, the vertices of $L(R)$, and all edges of $G$ connecting vertices of $R$ to vertices of $L(R)$.
We let $T_R\subseteq R'$ be a tree, whose leaves are precisely the vertices of $L(R)$, that contains smallest number of edges among all such trees. Note that such a tree exists because graph $R$ is connected. % and thus contains a spanning tree $T$ as a subgraph. %Finally we can recursively remove all leaves of the tree that are not in $L(R)$. %This gives one such tree, illustrating the existence of $T_R$. 
We let the extension of $C$ in $G$ be $X_G(C)=\set{T_R\mid R\in \rset_G(C)}$.



%\textbf{Contracting Connected Subgraphs.}
%Let $G$ be a graph, and let $C\subseteq G$ be a connected subgraph of $G$. We can obtain a new graph, $G_{|C}$ from $G$ by contracting $C$ as follows. We merge all vertices of $C$ into a single vertex $v(C)$, that we call a \emph{super-node}. We then delete all self-loops and parallel edges. 
%\mynote{I chose to delete parallel edges to be consistent with graph notation, and I think this works better because when parallel edges are present one can't claim there is a unique planar drawing. Not sure if this will be needed at the end.}

\iffalse
\textbf{Sparsest Cut.} 
Suppose we are given a graph $G=(V,E)$, and a subset $\tset\sse V$ of $k$ vertices, called terminals. 
The sparsity of a cut $(S,\nots)$ in $G$ is $\Phi(S)=\frac{|E(S,\nots)|}{\min\set{|S\cap \tset|, |\nots\cap \tset|}}$, and the value of the sparsest cut in $G$ is defined to be:
$\Phi(G)=\min_{S\subset V}\set{\Phi(S)}$.
The goal of the sparsest cut problem is to find a cut of minimum sparsity. Arora, Rao and Vazirani~\cite{ARV} have shown an $O(\sqrt {\log n})$-approximation algorithm for the sparsest cut problem. We denote this algorithm by \algsc, and its approximation factor by $\alphasc(n)=O(\sqrt{\log n})$.
\fi

%A problem dual to sparsest cut is the maximum concurrent flow problem. For the above definition of the sparsest cut problem, the corresponding variation of the concurrent flow problem asks to find the maximum value $\lambda$, such that every pair of terminals  in $\tset\choose 2$ can send $\lambda/k$ flow units to each other simultaneously with no congestion. The flow-cut gap is the maximum ratio, in any graph, between the value of the minimum sparsest cut and the maximum value $\lambda$ of concurrent flow. The value of the flow-cut gap in undirected graphs, that we denote by $\beta(n)$ throughout the paper, is $\Theta(\log n)$~\cite{leighton1999multicommodity}. %, GVY,LLR,Aumann-Rabani}. 
%Therefore, if $\Phi(G)=\alpha$, then every pair of terminals can send $\frac{\alpha}{k\beta(n)}$ flow units to each other with no congestion.
%Equivalently, every pair of terminals can send $1/k$ flow units to each other with congestion at most $\beta(n)/\alpha$. Moreover, any matching on the set $\tset$ of terminals can be fractionally routed with congestion at most $2\beta(n)/\alpha$.

\textbf{Sparsest Cut and Well-Linkedness.} %We use a standard notion of well-linkedness:
%
%\vspace{-3mm}
%\begin{definition}
%	Given a graph $G$, a subset $T$ of its vertices, and a parameter $\alpha > 0$, we say that $T$ is \emph{$\alpha$-well-linked} in $G$, iff for any partition $(A,B)$ of $T$, $|E(A, B)|\ge \alpha\cdot\min \{|T\cap A|, |T\cap B|\}$. %\snote{shouldn't this be $|E(A, B)|\ge \alpha\cdot\min \{|\out(T)\cap \out(A)|, |\out(T)\cap \out(B)|\}$?}
%\end{definition}
%\vspace{-0.3cm}
%
Suppose we are given a graph $G=(V,E)$, and a subset $\Gamma\sse V$ of its vertices. We say that a cut $(X,Y)$ in $G$ is a valid $\Gamma$-cut iff $X\cap \Gamma,Y\cap \Gamma\neq \emptyset$. The \emph{sparsity} of a valid $\Gamma$-cut $(X,Y)$ is $\frac{|E(X,Y)|}{\min\set{|X\cap \Gamma|, |Y\cap \Gamma|}}$. %, and the value of the sparsest cut in $G$ is defined to be:
%$\Phi(G)=\min_{S\subsetneq V}\set{\Phi(S)}$.
In the Sparsest Cut problem, given a graph $G$ and a subset $\Gamma$ of its vertices, the goal is to compute a valid $\Gamma$-cut of minimum sparsity. Arora, Rao and Vazirani~\cite{ARV} have shown an $O(\sqrt {\log n})$-approximation algorithm for the sparsest cut problem. We denote this algorithm by \algsc, and its approximation factor by $\alphasc(n)=O(\sqrt{\log n})$. 

We say that a set $\Gamma$ of vertices of $G$ is \emph{$\alpha$-well-linked} in $G$, iff the value of the sparsest cut in $G$ with respect to $\Gamma$ is at least $\alpha$.



\iffalse
Let $G$ be a graph, and let $S$ be a subset of vertices of $G$, and let $0<\alpha<1$, such that $S$ is $\alpha$-well-linked. 
We now define the sparsest cut and the concurrent flow instances corresponding to $S$ as follows. For each edge in $\out(S)$, we sub-divide the edge by adding a new vertex $t_e$ to it. Let $G'$ denote the resulting graph and let $T$ denote the set of all vertices $t_e$ for $e\in \out_G(S)$. Consider the graph $H=G'[S]\cup \out_{G'}(S)$. We can naturally define an instance of the non-uniform sparsest cut problem on $H$ where the set of terminals is $T$. We then have the following well-known observation.
\begin{observation}
	Let $G$, $S$, $H$ and $T$ be defined as above, and let $0<\alpha <1$, such that $S$ is $\alpha$-well-linked. Then every pair of vertices in $T$ can send one flow unit to each other in $H$, such that the maximum congestion on any edge is at most $\beta(n)|T|/\alpha$. Moreover if $M$ is any partial matching on the vertices of $T$, then we can send one flow unit between every pair $(u,v)\in M$ in graph $H$, with maximum congestion at most $2\beta(n)/\alpha$.
\end{observation}
%\vspace{-0.3cm}

\iffalse
The following theorem shows the technique of \emph{well-linked decomposition}, which has been used extensively in graph algorithms (e.g., see~\cite{racke2002minimizing,chekuri2005multicommodity}). %For completeness we provide its proof in Appendix.
\begin{theorem}[Terminal Well-Linked Decomposition]
	\label{thm:well_linked-decomposition}
	There is an efficient algorithm, that, given any connected graph $G$ and a subset $T\subseteq V(G)$ of its vertices with $|T|=k$, computes a collection $\set{G_1,\ldots,G_r}$ of connected subgraphs of $G$, such that:
	\begin{enumerate}
		\item for each $1\le i\le r$, denote $V_i=V(G_i)$, then $(V_1,\ldots,V_r)$ forms a partition of $V(G)$;
		\item for each $1\le i\le r$, denote $T_i=T\cap V_i$, then the subset $T_i\cup \Gamma(V_i)$ of vertices is $\Omega(\frac{1}{\log^{3/2}k\cdot\log\log k})$-well-linked in $G_i$; and
		\item $\sum_{1\le i\le r}|\out(V_i)|\le 0.01 k$, and $\sum_{1\le i\le r}|T_i\cup \Gamma(V_i)|\le 1.01 k$.
	\end{enumerate}
\end{theorem}
\fi
\fi


\paragraph{Non-interfering paths.}
To be used later for locally non-interfering/non-interfering paths (for this the definition should be adapted). We may also keep it in prelims as a definition of crossing paths. Maybe we should also define a drawing of a path as a concatenation of images of its edges. We use it quite a bit.
\begin{definition}
	Let $\gamma,\gamma'$ be two curves in the plane or on the sphere. We say that $\gamma$ and $\gamma'$ \emph{cross},  iff there is a disc $D$, whose boundary is a simple closed curve that we denote by $\beta$, such that: 
	
	\begin{itemize}
		\item  $\gamma\cap D$ is a simple open curve, whose endpoints we denote by $a$ and $b$; 
		\item $\gamma'\cap D$ is a simple open curve, whose endpoints we denote by $a'$ and $b'$; and
		
		\item $a,a',b,b'\in \beta$, and they appear on $\beta$ in this circular order.
	\end{itemize}
\end{definition}
Given a graph $G$ embedded in the plane or on the sphere, we say that two paths $P,P'$ in $G$ cross iff their images cross. Similarly, we say that a path $P$ crosses a curve $\gamma$ iff the image of $P$ crosses $\gamma$.







==> proof-of-obs.tex <==
\begin{proof}
Let $p$ be any integer in the interval $(0,r)$.
We denote by $\iset_p$ the subset of intervals in $\iset$ that lies entirely to the left of $p$ (namely the subset of intervals $(a,b)\in \iset$ such that $a,b\le p$), and we define $\iset'_p$ similarly for collection $\iset'$. Recall that, for each $0\le i\le r$, the number of intervals in $\iset$ with $i$ being its left endpoint is equal to the number of intervals in $\iset'$ with $i$ being its left endpoint, and the number of intervals in $\iset$ with $i$ being its right endpoint is equal to the number of intervals in $\iset'$ with $i$ being its right endpoint. Taking the sum over all integers $0\le i< p$, we get that the number of intervals in $\iset$ with its left endpoint less than $p$ is equal to the number of intervals in $\iset$ with its left endpoint less than $p$. We denote this number by $x$. Taking the sum over all integers $0\le i\le p$, we get that the number of intervals in $\iset$ with its right endpoint less than or equal to $p$ is equal to the number of intervals in $\iset$ with its right endpoint less than or equal to $p$. We denote this number by $y$ (so $|\iset_p|=|\iset'_p|=y$).
We denote $\hat \iset=\iset\setminus \iset_p$ and $\hat \iset'=\iset'\setminus \iset'_p$.
Clearly, all intervals in $\iset$ that contains $p$ remain in $\hat \iset$, and these intervals are exactly intervals in $\hat \iset$ with its left endpoint less than $p$. From the above discussion, it is easy to see that the number of such intervals is $x-y$, so the number of intervals in $\iset$ that contains $p$ is $x-y$. From similar arguments, we get that so the number of intervals in $\iset'$ that contains $p$ is also $x-y$. This shows that, for every integer $p\in (0,r)$, the number of intervals in $\iset$ containing $p$ is equal to the number of intervals in $\iset'$ containing $p$.
\znote{need to change $0\le i\le n$ to  $0\le i\le r$ in the statement}
\end{proof}

==> sec5-old-stuff.tex <==


%------------Only old stuff below -------------

\subsection{Well-Structured Subinstances, Well-Structured Solutions and a Decomposition Lemma}

\newif\ifhide
\hidefalse
%\hidefalse

\ifhide


\znote{maybe we need the notion "boundary of a face" $\partial F$ back in the prelim}


\paragraph{Well-Structured subinstances and contracted subinstances.} 
We say that a subinstance $I=(G,\Sigma)$ of the input instance $\check I$ is \emph{well-structured}, iff $G$ is a subgraph of $\check G$, and we are given 
\begin{itemize}
\item a $2$-connected subgraph $K$ of $G$, called the \emph{skeleton} of $I$;
\item a planar drawing $\rho$ of $K$ in the sphere (we denote by $\fset$ the set of faces in $\rho$).
\item a collection $\gset=\set{G_F}_{F\in \fset}$ of subgraphs of $G$, where each subgraph $G_F\in \gset$ is indexed by a face $F\in\fset$, such that
\begin{itemize}
\item each vertex $v\notin V(K)$ belongs to exactly one subgraphs in $\gset$;
\item for each vertex $v\in V(K)$ and each face $F\in \fset$, subgraph $G_F$ contains vertex $v$ iff $v$ lies on the boundary of face $F$ (namely $v\in \partial F$);
\item for each face $F\in \fset$ and each vertex $v\in \partial F$, if we denote by $e,e'$ the edges of $\partial F$ incident to $v$, then edges of $\delta_{G_F}(v)$ must be consecutive in the circular ordering $\oset_v\in \Sigma$ and must lie between $e$ and $e'$. Specifically, if $\delta_G(v)=\set{e,e_1,\ldots,e_s,e',e'_1,\ldots,e'_t}$, where the other edges are indexed according to $\oset_v$, then either $\delta_{G_F}(v)=\set{e_1,\ldots,e_s}$ or $\delta_{G_F}(v)=\set{e'_1,\ldots,e'_t}$. 
\end{itemize}
\end{itemize}

We call the tuple $(K,\rho,\fset,\gset)$ the \emph{structure} of instance $I=(G,\Sigma)$.
Additionally, we call edges of $K$ \emph{special edges} of instance $I$.

%Let $I=(G,\Sigma)$ be a well-structured subinstance with skeleton $K$, planar drawing $\rho$ of $K$ with face sets $\fset$, and the collection $\gset$ of subgraphs. 
Let $F$ be a face in $\fset$. We define the subinstance $I_F=(G_F,\Sigma_F)$, where the rotation system $\Sigma_F$ is induced by $\Sigma$.
We define the subinstance $\tilde I_F=(\tilde G_F,\tilde \Sigma_F)$ as follows. Since skeleton $K$ is $2$-connected and $F$ is a face in a planar drawing of $K$, graph $\partial F$ is the union of a set of vertex-disjoint cycles.
We denote by $\rset(F)$ the set of vertex-disjoint cycles in $\partial F$.
Graph $\tilde G_F$ is obtained from $G_F$ by contracting, for each cycle $R$ in $\rset(F)$, all vertices of $R$ into a supernode, which we denote by $v_R$, so $V(\tilde G)=(V(G)\setminus V(\partial F))\cup \set{v_R\mid R\in \rset(F)}$. 
We now define the rotation system $\tilde \Sigma_F$.
Note that, for every vertex $v\in V(G)\setminus V(\partial F)$, $\delta_{\tilde G_F}(v)=\delta_{\tilde G}(v)$, and we define the ordering $\ttoo_v$ in $\tilde \Sigma$ to be $\oset_v$, the ordering on vertex $v$ in $\Sigma$. It remains to define the orderings $\set{\ttoo_{v_{R}}\mid R\in \rset(F)}$. Consider a cycle $R\in \rset(F)$ with $R=(v_0,v_1,\ldots,v_{s-1},v_0=v_s)$. For each $0\le i\le s-1$, we denote by $e_i$ the edge in $R$ connecting $v_i$ to $v_{i+1}$, and we denote $\delta_{G_F}(v_i)=\set{e_{i-1}, e^i_1,\ldots,e^i_{d_i},e_i}$, where the edges are indexed according to the ordering $\oset_{v_i}$ in $\Sigma$. From the definition of graph $\tilde G_F$, 
$$\delta_{\tilde G}(v_R)=\bigg(\bigcup_{0\le i\le s-1}\delta_{G_F}(v_i)\bigg)\setminus E(R)=\set{e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}}.$$ We then define the ordering $\ttoo_{v_{R}}$ to be
$e^0_1,\ldots,e^0_{d_0},e^1_1,\ldots,e^1_{d_1},\ldots,e^{s-1}_1,\ldots,e^{s-1}_{d_{s-1}}$. This completes the definition of instance $\tilde I_F$. We call $\tilde I_F$ the 
\emph{contracted subinstance} of $I_F$.


\paragraph{Well-Structured solutions.}
Let $I=(G,\Sigma)$ be a well-structured instance with structure $(K,\rho,\fset,\gset)$. We say that a solution $\phi$ of instance $I$ is a \emph{well-structured solution} (or a \emph{well-structured drawing}) for $I$, iff
\begin{properties}{P}
\item the drawing of $K$ induced by drawing $\phi$ is identical to $\rho$;
\item for each face $F\in \fset$,
\begin{itemize}
\item all vertices of $G_F\setminus \partial F$ are drawn in the interior of face $F$;
\item for each edge $e\in (G_F\setminus F)$ that is incident to some vertex $v\in F$, the intersection of image of $e$ and the tiny $v$-disc $D_{\phi}(v)$ is entirely contained in face $F$;
and
\end{itemize} 
\item the number of edges that crosses a special edge of $I$ in $\phi$ is at most $\cro(\phi)\cdot (\tau^i)^{10}/|E(G)|$.
\label{prop: niubi edge crossing special cycle}
\end{properties}
%We say that a solution $\phi$ for instance $I$ is \emph{almost well-structured} iff it satisfies properties \ref{prop: simple curve}--\ref{prop: first segments}.


The main result in this subsection is the following lemma.

\znote{parameters to be determined.}

\fi


\newcommand{\delE}{E^{\sf del}}
\newcommand{\ws}{well-structured\xspace}



\begin{lemma}
\label{lem: many path main}
There is an efficient randomized algorithm, that given a well-structured subinstance $I=(G,\Sigma)$ of $\check I$, with structure $(K,\rho,\fset,\gset)$, for which there exists a \ws drawing $\phi$, computes a well-structured subinstance $I'=(G',\Sigma)$ of $\check I$ with structure $(K',\rho',\fset',\gset')$, such that
\begin{properties}{C}
\item $G'\subseteq G$, $K\subseteq K'$, and the drawing of $K$ induced by $\rho'$ is identical to $\rho$;
\item for each face $F'\in \fset'$, the contracted subinstance $\tilde I'_F$ is either $\tau^s$-small or $\tau^i$-narrow;
\label{prop: well-structured and contracted}
\end{properties}
and moreover, with probability $1-O(1/\mu^{\smallprobability})$,
\begin{properties}[2]{C}
\item $|E(G)\setminus E(G')|\le \cro(\phi)\cdot \poly(\mu)/|E(G)|$; 
\label{prop: few deleted edges}
\item for each face $F$ and each edge $e\in G_F$, the segment(s) of curve $\phi(e)$ that lies outside face $F$ is identical to the segment(s) of curve $\phi'(e)$ that lies outside face $F$.
\label{prop: forbidden discs}
\item if $\cro(\phi)\le m^2/\mu^{c}$ for some large enough constant $c>0$, then there exists a well-structured solution $\phi'$ for $I'$, such that $\cro(\phi')\le O(\cro(\phi))$.
\label{prop: number of crossings}
\end{properties}
%\znote{do we have this?} 
Moreover, there is an efficient algorithm $\alg(I')$, that given, for each face $F'\in \fset'$, a feasible solution $\phi(\tilde I'_F)$ to the contracted instance $\tilde I'_F$, computes a well-structured solution $\phi(I')$ for instance $I'$, of cost 
$\cro(\phi(I'))\leq O\big(\sum_{F'\in \fset'}\cro(\phi(\tilde I'_F)\big)$.
\end{lemma}

The remainder of this subsection is dedicated to the proof of \Cref{lem: many path main}.

%The algorithm is randomized and consists of two phases. In the first phase, the algorithm will return FAIL with probability $O(1/\mu^{\smallprobability-\interestconst})$, and if it does not return FAIL, it will compute a collection $\iset$ of subinstances of the input instance $I=(G,\Sigma)$, and a set $E^{\sf del}$ of edges in $G$, such that, if we denote by $\tilde \iset$ the set of all contracted subinstances for instances in $\iset$, then with probability $O(1/\mu^{\smallprobability-\interestconst})$,

\iffalse
\begin{properties}{C}
\item each instance $I'\in \iset$ is a well-structured subinstance;
\label{prop: well-structured instances}
\item for each contracted instance $\tilde I'=(\tilde G',\tilde\Sigma') \in \tilde \iset$, either $\tilde I'$ is non-wide, or $|E(\tilde G')|\le m/\mu$;\label{prop: no longer wide}
\item the sets $\set{\hat E(I')\mid I'\in \iset}$ of edges are mutually disjoint;\label{prop: private edges disjoint}
\item $|E^{\sf del}|\le \cro\cdot\mu^{O(\interestconst)}/m$, and edges of $E^{\sf del}$ does not belong to any instance of $\iset$;\label{prop: few deleted edges in phase 1}
\item every edge of $E(G)\setminus \bigg(E^{\sf del}\cup \big(\bigcup_{I'\in \iset}\hat E(I')\big)\bigg)$ is a special edge of exactly two instances in $\iset$;\label{prop: few edges}
\item there exists, for every instance $I'\in \iset$, a well-structured solution $\phi_{I'}$, such that\\
$\expect[]{\sum_{I'\in \iset}\optcrors(I')}\le \left (\optcrors(I)+|E(G)|\right )\cdot \nu$; and \label{prop: small solution cost}
\item there is an efficient algorithm $\alg(\iset)$, that, given, for each contracted instance $\tilde I' \in \tilde\iset$, a feasible solution $\phi(\tilde I')$, computes a feasible solution $\phi$ for instance $I$, of cost $\cro(\phi^*)\leq O\left (\sum_{I'\in \iset}\cro(\phi(I'))\right )$. \label{prop: alg to put together}
\end{properties}
\znote{to modify the properties?}


In the second phase, we will compute, for each instance $I'\in \iset$, a new instance $I''$ obtained from $I'$ by deleting a set of edges from $I'$, such that
\znote{to add more properties}
\fi



\input{many_paths_main_decomposition}

\input{many_paths_main_decomposition_analysis}




==> step2-case1.tex <==
\subsubsection*{Case 1: $\pset$ was a type-1 promising  path set}


\paragraph{Computing the Split.}

Note that in order to complete the enhancement structure $\aset$, we need to define a drawing $\rho'$ of the graph $K'=K\cup P$ with no crossings, so that $\rho'$ is consistent with the rotation system $\Sigma$ and the orientations $\set{b_u}_{u\in V(K')}$, which must be a clean drawing with respect to $\kset$. If we consider any such drawing $\rho'$, then the image of the cycle $P$ in $\rho'$ partitions the sphere into two discs, that we denote again by $D$ and $D'$. For every core structure $\jset_i\in \kset$, the image of $J_i$ in $\rho'$ is essentially fixed -- it must be drawn inside disc $D_i$, and the drawing must be identical to $\rho_i$. But it is possible that $J_i$ is drawn either inside disc $D$ or inside disc $D'$. Once we determine, for all $1\leq i\leq r$, whether $J_i$ is drawn inside $D$ or inside $D'$, drawing $\rho'$ of $K'$ becomes fixed. 

We now describe a procedure that cuts the graph $G'$ into two subgraphs, one to be drawn inside $D$, and another to be drawn inside $D'$. This partition of $G'$ will also determine, for all $1\leq i\leq r$, whether $J_i$ is drawn inside $D$ or inside $D'$. Therefore, this procedure will allow us to both complete the computation of the enhancement structure $\aset$ (by finalizing the drawing $\rho'$ of $K'$), and to compute the split of instance $I$ along $\aset$. The procedure itself is very simple conceptually: we simply compute a minimum cut in $G'$ separating the edges of $\tilde E'_1$ from edges of $\tilde E'_2$. In order to ensure that the cores are not separated by this cut, we contract each core into a single vertex before computing the cut. We now describe this cutting procedure.


We construct a flow network $H$ as follows. We start with $H=G'$, and then, for all $1\leq i\leq r$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$ with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $P$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $H$, and we denote by $E''=E_H(A,B)$. Eventually, we will delete the edges of $E''$ from $G'$, so these edges will not belong to any of the two instances that we construct. The following claim bounds the cardinality of $E''$. The proof is deferred to Section \ref{subsec: small cut set in case 1} of Appendix.

\begin{claim}\label{claim: cut set small}
	If Events $\event_1$ and $\event_3$ did not happen, then $|E''|\leq \frac{64\mu^{700}\cro(\phi)}{m}$.
\end{claim}



We are now ready to complete the construction of the enhancement structure $\aset$. We have already defined a type-1 enhancement $\Pi$, and an orientation $b_u$ for every vertex $u\in (V(\firstpath)\cup V(\secondpath))\setminus V(K)$. It now remains to define a drawing $\rho'$ of the graph $K'$. In order to define the drawing $\rho'$, we start by drawing the cycle $\firstpath$ on the plane in the natural way without any crossings, and we fix the orientations of the vertices $u\in \firstpath$ to be consistent with the orientations $b_u$ that we have computed for them.
We denote by $F$ the unique face in this drawing whose boundary is the image of $\firstpath$ and by $F'$ the infinite face. We can view this current drawing of $\firstpath$ as the drawing induced by $\phi'$ (since both drawings are identical). Note that in the drawing $\phi'$ of $G'$, either for every edge $e\in \tilde E_1$, $\sigma(e)\subseteq F$, or for every edge $e\in \tilde E_2$, $\sigma(e)\subseteq F$.
We can ensure that it is the former (by flipping the image of the path $\firstpath$, thereby reversing the orientations of all its vertices, if necessary).

For all $1\leq i\leq r$, if $v_{J_i}\in A$, then we place the disc $D_i$ inside face $F$, and otherwise we place it inside face $F'$. The discs are placed so that all of them remain disjoint from each other and from the image of $\firstpath$. For all $1\leq i\leq r$, we then plant the image $\rho_i$ of the core $J_i$ given by the core structure $\jset_i$ inside the disc $D_i$.
%\znote{arbitrary flip?}
It is immediate to verify that $\rho'$ is a drawing of graph $K'$ with no crossings, and that it is a clean drawing of $K'$ with respect to $\kset$. This completes the construction of the enhancement structure $\aset$. We let $(\kset_1,\kset_2)$ denote the split of $\kset$ along the enhancement structure $\aset$, where $\kset_1$ contains all core structures $\jset_i$ with $v_{J_i}\in A$.

Next, we define a split $(I_1,I_2)$ of instance $I$ along the enhacement structure $\aset$. In order to do so, we define two vertex sets $A',B'$ in graph $G'$, as follows. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every index $1\leq i\leq r$, if $v_{J_i}\in A$, then we replace $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. We then let $G_1=G'[A'\cup V(P)]$ and $G_2=G'[B'\cup V(P)]$. The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. We now prove that $(I_1,I_2)$ is a split of $I$ along $\aset$. 


Notice that $V(G_1)\cap V(G_2)=V(P)$ and $E(G_1)\cap E(G_2)=E(P)$. Additionally, $E(G_1)\cup E(G_2)\subseteq E(G)$. Let $E^{\del}=E(G)\setminus (E(G_1)\cup E(G_2))$. Then $E^{\del}=E'\cup E''$. From Claims \ref{claim: third bad event bound} and 
\ref{claim: cut set small}, if Event $\event$ did not happen, then $|E'|+|E''|\leq 2\cdot\cro(\phi)\cdot \mu^{2150}/m$.

Recall that skeleton structure $\kset_1$ contains, for every supernode $v_{J_i}\in A$, the corresponding core structure $\jset_i$ of graph $G$. Since, from our construction, $J_i\subseteq G_1$, it is also a valid core structure for instance $I_1$. Additionally, $\kset_1$ contains a core structure $\jset$, whose associated core $J$ is the cycle $P$. The drawing $\rho_{J}$ associated with $J$ is the natural drawing described above, with face $F$ serving as an infinite face of the drawing. It is easy to verify that $\jset$ is a valid core structure for instance $I_1$. 

Similarly, skeleton stucture $\kset_2$  contains, for every supernode $v_{J_i}\in B$, the corresponding core structure $\jset_i$ of graph $G$. Since, from our construction, $J_i\subseteq G_2$, it is also a valid core structure for instance $I_2$. Additionally, $\kset_2$ contains a core structure $\jset'$, whose associated core $J'$ is the cycle $P$, and whose associated drawing $\rho_{J'}$ is the natural drawing  of $P$ described above, with face $F'$ serving as an infinite face of the drawing. As before, $\jset'$  is a valid core structure for instance $I_2$. 

Therefore, $\kset_1$ is a valid skeleton structure for $I_1$ and $\kset_2$ is a valid skeleton structure for $I_2$. We conclude that $(I_1,I_2)$ is a valid split of instance $I$ along the enhancement structure $\aset$.
In the following two observations we show that, if the bad event $\event$ did not happen, then the enhancement structure $\aset$, together with the split $(I_1,I_2)$ of $I$ along $\aset$, is a valid output for \procsplit. 
The proofs are deferred to Sections  \ref{subsec: few edges in split Case 1} and \ref{subsec: getting semi-clean solution for case 1} of Appendix, respectively.

\begin{observation}\label{obs: few edges in split graphs}
 If Event $\event$ did not happen, then $|E(G_1)|,|E(G_2)|\leq m-\frac{m}{100\mu^{50}}$.
\end{observation}




\begin{observation}\label{obs: semi-clean case 1}
If bad event $\event$ does not happen, then 	
there is a semi-clean solution $\phi_1$ for instance $I_1$ with respect to $\kset_1$, and a semi-clean solution $\phi_2$ for instance $I_2$ with respect to $\kset_2$, such that $|\chi^*(\phi_1)|+|\chi^*(\phi_2)|\leq |\chi^*(\phi)|$, and $|\chi^{\dirty}(\phi_1)|+ |\chi^{\dirty}(\phi_2)|\leq |\chi^{\dirty}(\phi)|+\frac{64\mu^{700}\cro(\phi)}{m}$.
\end{observation}


Recall that we have already showed that, if Event $\event$ did not happen, then $|E(G)\setminus (E(G_1)\cup E(G_2))|=|E^{\del}|\leq 2\cdot\cro(\phi)\cdot \mu^{2150}/m< \cro(\phi)\cdot \mu^{2200}/m+|\chi^{\dirty}(\phi)|$. Altogether, if Event $\event$ did not happen, then the algorithm produces a valid output for \procsplit. Since the probability of Event $\event$ is at most $1/\mu^{399}$, this completes the proof of \Cref{thm: procsplit} for Case 1.


==> step2-case2.tex <==
\subsubsection*{Case 2: $\pset$ was a type-2 promising  path set}


\paragraph{Computing the Split.}

The algorithm for computing the drawing $\tilde \rho$ of the graph $K'=K\cup P$ and of the split $(I_1,I_2)$ of the instance $I$ is almost identical to that in Case 1. The slight difference is that in this case, the endpoints of $P$ belong to the core $\thecore$. 


We construct a flow network $H$ as follows. We start with $H=G'$, and then, for all $1\leq i\leq r$ with $i\neq i^*$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$ with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $P\cup \thecore$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $H$, and we denote by $E''=E_H(A,B)$.  The following claim, that is an analogue of \Cref{claim: cut set small} for Case 2, bounds the cardinality of $E''$. The proof is almost identical to that of \Cref{claim: cut set small}.  We provide its sketch in  Section \ref{subsec: small cut set in case 2} of Appendix.

\begin{claim}\label{claim: cut set small case2}
	If Events $\event$ did not happen, then $|E''|\leq \frac{64\mu^{700}\cro(\phi)}{m}+|\chi^{\dirty}(\phi)|$.
\end{claim}


In order to complete the construction of the enhancement structure $\aset$, we now only need to define a drawing $\rho'$ of the graph $K'$. In order to define the drawing $\rho'$, we start 
with the unique planar drawing $\tilde \rho$ of graph $\thecore\cup P$, in which the orientation of every vertex $u\in V(\thecore\cup P)$ is $b_u$, and the drawing of $\thecore$ induced by $\tilde \rho$ is $\rho_{\thecore}$.
Recall that this drawing is precisely the drawing of $\thecore\cup P$ induced by $\phi'$, though its orientation may be different. The faces $F_1$ and $F_2$ in drawing $\tilde \rho$ are well defined and can be computed efficiently.


For all $1\leq i\leq r$ with $i\neq i^*$, if $v_{J_i}\in A$, then we place the disc $D_i$ with the drawing $\rho_{J_i}$ of graph $J_i$ inside face $F_1$, and otherwise we place it inside face $F_2$. The discs are placed so that all of them remain disjoint from each other and from the image of $\thecore\cup P$.  It is immediate to verify that $\rho'$ is a drawing of graph $K'$ with no crossings, and that it is a clean drawing of $K'$ with respect to $\kset$. This completes the construction of the enhancement structure $\aset$. We let $(\kset_1,\kset_2)$ denote the split of $\kset$ along the enhancement structure $\aset$, where $\kset_1$ contains all core structures $\jset_i$ with $v_{J_i}\in A$.

Next, we define a split $(I_1=(G_1,\Sigma_1),I_2=(G_2,\Sigma_2))$ of instance $I$ along the enhacement structure $\aset$. In order to do so, we define two vertex sets $A',B'$ in graph $G'$, as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every index $1\leq i\leq r$ with $i\neq i^*$, if $v_{J_i}\in A$, then we replace $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 
Additionally, we let $J\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F$, and we let $\rho_J$ denote the drawing of $J$ induced by $\tilde \rho$, where we view $F_1$ as the infinite face of the drawing. Similarly, we let $J'\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F_2$, and we let $\rho_{J'}$ denote the drawing of $J'$ induced by $\tilde \rho$, where we view $F_2$ as the infinite face of the drawing. Note that $V(J')\cup V(J'')=V(J)$, and edge sets $E(J'),E(J'')$ define a partition of $E(J)$.

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J))$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. We now prove that $(I_1,I_2)$ is a split of $I$ along $\aset$. 


Notice that $V(G_1)\cap V(G_2)\subseteq V(P\cup \thecore)$ and $E(G_1)\cap E(G_2)\subseteq E(P\cup \thecore)$. Additionally, $E(G_1)\cup E(G_2)\subseteq E(G)$. Let $E^{\del}=E(G)\setminus (E(G_1)\cup E(G_2))$. Then $E^{\del}=E'\cup E''$. From Claims \ref{claim: third bad event bound} and 
\ref{claim: cut set small case2}, if Event $\event$ did not happen, then $|E'|+|E''|\leq \frac{2\cro(\phi)\cdot \mu^{2150}}m +|\chi^{\dirty}(\phi)|$.

Recall that skeleton structure $\kset_1$ contains, for every supernode $v_{J_i}\in A$, the corresponding core structure $\jset_i$ of graph $G$. Since, from our construction, $J_i\subseteq G_1$, it is also a valid core structure for instance $I_1$. Additionally, $\kset_1$ contains a core structure $\jset$, whose associated core is $J$. It is easy to verify that $\jset$ is a valid core structure for instance $I_1$. Therefore, $\kset_1$ is a valid skeleton structure for $I_1$.
From similar arguments, $\kset_2$ is a valid skeleton structure for instance $I_2$. We conclude that $(I_1,I_2)$ is a valid split of instance $I$ along the enhancement structure $\aset$. Notice that $|\kset_1|,|\kset_2|\leq r$ must hold (this is unlike Case 1, where it is possible that one of the skeleton structures contains $r+1$ core structures).
In the following two observations we show that, if the bad event $\event$ did not happen, then the enhancement structure $\aset$, together with the split $(I_1,I_2)$ of $I$ along $\aset$, is a valid output for \procsplit. 
The first observation is an analogue of \Cref{obs: few edges in split graphs} for Case 2. Since the parameters for the two cases are slightly different, we 
provide a proof in Section  \ref{subsec: few edges in split Case 2} of appendix. The second observation is an analogue of \Cref{obs: semi-clean case 1} for Case 2. Its proof is almost identical to that of \Cref{obs: semi-clean case 1}. We provide a proof sketch in Section \ref{subsec: getting semi-clean solution for case 2} of Appendix.

\begin{observation}\label{obs: few edges in split graphs case2}
 If Event $\event$ did not happen, then $|E(G_1)|,|E(G_2)|\leq m-\frac{m}{32\mu^{300}}$.
\end{observation}




\begin{observation}\label{obs: semi-clean case 2}
If bad event $\event$ does not happen, then 	
there is a semi-clean solution $\phi_1$ for instance $I_1$ with respect to $\kset_1$, and a semi-clean solution $\phi_2$ for instance $I_2$ with respect to $\kset_2$, such that $|\chi^*(\phi_1)|+|\chi^*(\phi_2)|\leq |\chi^*(\phi)|$, and $|\chi^{\dirty}(\phi_1)|+ |\chi^{\dirty}(\phi_2)|\leq |\chi^{\dirty}(\phi)|+\frac{64\mu^{700}\cro(\phi)}{m}$.
\end{observation}


Recall that we have already showed that, if Event $\event$ did not happen, then $|E(G)\setminus (E(G_1)\cup E(G_2))|=|E^{\del}|\leq 2\cdot\cro(\phi)\cdot \frac{\mu^{2150}}m+|\chi^{\dirty}(\phi)| < \cro(\phi)\cdot \mu^{2200}/m+|\chi^{\dirty}(\phi)|$. Altogether, if Event $\event$ did not happen, then the algorithm produces a valid output for \procsplit. Since the probability of Event $\event$ is at most $1/\mu^{399}$, this completes the proof of \Cref{thm: procsplit} for Case 2.


==> step2-case3.tex <==
\subsubsection*{Case 3: $\pset$ was a type-3 promising  path set}


In the third case, $\pset$ was a type-3 promising  path set. We let $1\leq i^*<i^{**}\leq r$ be the indices for which all paths in $\pset$ originate at vertices of $\thecore$ and terminate at vertices of $\othercore$. We denote $E_1=\delta_G(\thecore)$ and $E_2=\delta_G(\thecore)$. 
If the two paths chosen from $\pset^*$ share at least one vertex of $V(G)\setminus V(K)$, then we have constructed a type-2 enhancement whose both endpoints lie in $\thecore$. In this case, the algorithm and its analysis are practically identical to those from Case 2 and are omitted here. We now assume that the two chosen paths are disjoint from each other. For convenience of notation, we denote $P=\firstpath$ and $P'=\secondpath$. Throughout, we denote by $\tilde J$ the graph obtained from the union of $\thecore,\othercore,P$ and $P'$.
Recall that, from \Cref{claim: new drawing}, if neither of the events $\event_1,\event_3$ happened, drawing $\phi'$ contains no crossings between the edges of $E(K')$. 
Throughout, we denote by $\gamma$ the image of path $P$ and by $\gamma'$ the image of path $P'$ in $\phi'$. 


We recall how the paths $P$ and $P'$ were constructed. 
We started with a set $\pset^*$ of $k'=\ceil{\frac{m}{\mu^{300}}}$ simple edge-disjoint paths in graph $G$, with every path originating at a vertex of $J_{i^*}$ and terminating at a vertex of $J_{i^{**}}$. Additionally, the paths in $\pset^*$ are internally disjoint from $K$, and they are non-transversal with respect to $\Sigma$. We denoted by $E^*_1\subseteq \delta(J_{i^{*}})$ the subset of edges that belong to the paths of $\pset^*$, letting $E^*_1=\set{e_1,\ldots,e_{k'}}$, where the edges are indexed in the order of their appearence in the ordering $\oset(J_{i^{*}})$. For all $1\leq j\leq k'$, we denoted by $P_j\in \pset^*$ the unique path originating at the edge $e_j\in E^*_1$. We then selected an index $\floor{k'/8}<j^*<\ceil{k'/4}$ uniformly at random, that determined the chosen paths $P_{j^*}$ and $P_{j^*+\floor{k'/2}}$. Since we assumed that the chosen paths do not share any vertices of $V(G)\setminus V(K)$, we eventually set $P=P_{j^*}$ and $P'=P_{j^*+\floor{k'/2}}$.


Let $\tilde \rho$ be the drawing of graph $\tilde J$ induced by $\phi'$. This drawing has no crossings, and it has two faces, that we denote by $F_1$ and $F_2$, respectively, whose boundaries contain both curves $\gamma$ and $\gamma'$. The drawing of $\thecore$ induced by $\tilde \rho$ is $\rho_{\thecore}$, and the drawing of  $\othercore$ induced by $\tilde \rho$ is $\rho_{\othercore}$, which are known to our algorithm. However, in order to construct the drawing $\tilde \rho$ of graph $\tilde J$ efficiently, we also need to know the orientations of these two drawings with respect to each other in $\tilde \rho$. 

In order to overcome this difficulty, we choose another index $j^*< j^{**}<j^*+\floor{k'/2}$ uniformly at random, and we let $P''=P_{j^{**}}$. We say that a bad event $\event_5$ happens if  $P''$ is a bad path, or some edge $e\in E(P'')$ crosses the image of an edge of $P\cup P'$ in the drawing $\phi$. 
 From \Cref{obs: number of bad paths}, the number of bad paths in $\pset^*$ is at most $\frac{m}{8\mu^{700}}$. Moreover, if bad event $\event$ did not happen, then paths $P$ and $P'$ are both good paths, and so the number of crossings in which the edges of $E(P)\cup E(P')$ participate is  at most $\frac{32\mu^{700}\cdot \cro(\phi)}{m}\leq \frac{m}{8\mu^{700}}$ (from Property \ref{prop valid input drawing} of valid input to Procedure \procsplit). Therefore, if Event $\event$ did not happen, there are at most $\frac{m}{8\mu^{700}}$ indices $1\leq i\leq k$, such that path $P_i$ is bad, or some edge of $P_i$ crosses an edge of $E(P)\cup E(P')$ in $\phi$.
 Since $k'=\ceil{\frac{m}{\mu^{300}}}$, $\prob{\event_5\mid \neg\event}\leq \frac{1}{\mu^{400}}$.

Consider now the graph $\tilde J'=\tilde J\cup P''=J_{i^*}\cup \othercore\cup P\cup P'\cup P''$, and let $\tilde \rho'$ be the drawing of $\tilde J'$ induced by $\phi'$. If neither of the events $\event,\event_5$ happened, then $\tilde \rho'$ is a unique planar drawing of graph $\tilde J'$, such that the drawing of $\thecore$ induced by $\tilde \rho'$ is $\rho_{\thecore}$, and the drawing of $\othercore$ induced by $\tilde \rho$ is $\rho_{\othercore}$. Therefore, we can compute the drawing $\tilde \rho'$ of graph $\tilde J'$ efficiently. The drawing $\tilde \rho$ of graph $\tilde J$ is then identical to the drawing of $\tilde J$ induced by $\tilde \rho'$ (if bad events $\event,\event_5$ did not happen). Therefore, if bad events $\event,\event_5$ did not happen, then we can compute the drawing $\tilde \rho$ of $\tilde J$ efficiently, though we do not know its orientation in $\phi'$.

As in previous two cases, for every vertex $u\in V(\tilde J)$, we consider the tiny $u$-disc $D_{\phi'}(u)$.  For every edge $e\in \delta_{G'}(u)$, we denote by $\sigma(e)$ the segment of $\phi'(e)$ that is drawn inside the disc $D_{\phi'}(u)$. Let $\tilde E=\left (\bigcup_{u\in V(\tilde J)}\delta_{G'}(u)\right )\setminus E(\tilde J)$. We partition edge set $\tilde E$ into a set $\tilde E^{\inn}$ of \emph{inner edges} and the set $\tilde E^{\out}$ of outer edges exactly as before: Edge set $\tilde E^{\inn}$ contains all edges $e\in \tilde E$ with $\sigma(e)\subseteq F_1$, and $\tilde E^{\out}$ contains all remaining edges. Let $e_1$ be an arbitrary fixed edge of $E_1$ that does not lie on $P$ or $P'$. As before, we assume without loss of generality that $e_1\in \tilde E^{\inn}$. 

The algorithm for computing the orientation of the inner vertices of $P$ and $P'$ is practically identical to the one used in Case 2, with a minor difference in the analysis that we highlight below. 

We define an orientation of the ordering $\oset(\thecore)$ in $\phi'$ exactly as in Case 2. As in Case 1, we can now efficiently determine, for every edge $e\in E_1\cup E_2$, whether it belongs to $E^{\inn}$ or $E^{\out}$. In the former case, we add the edge to set $\tilde E_1'$, and in the latter case, we add it to $\tilde E_2'$. 
The algorithm for computing the orientation of every inner vertex $u$ of $P$ and $P'$  is identical to that used in Case 2. 
The proof that the orientations of the vertices are computed correctly with respect to $\phi'$  provided that neither of the events $\event,\event_5$ happenned (that is, an analogue of \Cref{claim: orientations and edge split is computed correctly Case2}) is also almost identical. The only difference is that now the images of the paths in sets $\pset_1(u),\pset_2(u),\pset'_1(u),\pset'_2(u)$ may cross the images of the edges of $\othercore$. However, the total number of such paths, whose images cross the edges of $E(\thecore)\cup E(\othercore)$, remains bounded by $N^{\bad}(u)$, so the same calculations work in Case 3 as well. We note however that the orientation of the vertices $u\in V(\othercore)$ are computed differently, and they are determined by the orientation of the drawing $\rho_{\othercore}$ of $\othercore$ induced by $\tilde \rho$: we either keep the orientations of all such vertices unchanged from $\jset_{i^{**}}$, or we may flip all of them, depending on the orientation of drawing $\rho_{\othercore}$ in $\tilde \rho$.


\paragraph{Computing the Split.}

The algorithm for computing the drawing $\tilde \rho$ of the graph $K'=K\cup P$ and of the split $(I_1,I_2)$ of the instance $I$ is almost identical to that in Cases 1 and 2. We provide a sketch below, highlighting the differences. 


We construct a flow network $H$ as follows. We start with $H=G'$, and then, for all $1\leq i\leq r$ with $i\not\in\set{i^*,i^{**}}$, we contract all vertices of the core $J_i$ into a supernode $v_{J_i}$. Next, we subdivide every edge $e\in \tilde E$  with a vertex $t_e$, and denote $T_1=\set{t_e\mid e\in \tilde E_1'}$, $T_2=\set{t_e\mid e\in \tilde E_2'}$. We delete all vertices of $\tilde J$ and their adjacent edges from the resulting graph, contract all vertices of $T_1$ into a source vertex $s$, and contract all vertices of $T_2$ into a destination vertex $t$. We then compute a minimum $s$-$t$ cut $(A,B)$ in the resulting flow network $H$, and we denote by $E''=E_H(A,B)$.  The following claim, that is an analogue of \Cref{claim: cut set small case2} for Case 2. The proof is virtually identical and is omitted here.

\begin{claim}\label{claim: cut set small case3}
	If neither of the events $\event,\event_5$ happen, then $|E''|\leq \frac{64\mu^{700}\cro(\phi)}{m}+|\chi^{\dirty}(\phi)|$.
\end{claim}


The drawing $\rho'$ of the graph $K'$ is constructed exactly as before: we start with the drawing $\tilde \rho$ of $\tilde J$, and then plant the discs $D_i$ corresponding to the cores $J_i\in \kset\setminus\set{\thecore,\othercore}$ inside face $F$ or inside face $F'$, depending on whether the corresponding supernode $v_{J_i}$ lies in $A$ or $B$. 

Consider now the split  $(\kset_1,\kset_2)$ of $\kset$ along the resulting enhancement structure $\aset$.
Then $\kset_1$ contains all core structures $\jset_i$ with $v_{J_i}\in A$, while $\kset_2$ contains all core structures $\jset_i$ with $v_{J_i}\in B$. Additionally, $\kset_1$ contains a core structure $\jset$, whose corresponding core $J$ contains all vertices and edges of $\tilde J$ that lie on the boundary of face $F$ in drawing $\tilde \rho$. The drawing $\rho_J$ associated with $J$ is its induced drawing in $\tilde \rho$, with face $F$ serving as the infinite face. Similarly, $\kset_2$ contains a core structure $\jset'$, whose corresponding core $J'$ contains all vertices and edges of $\tilde J$ that lie on the boundary of face $F'$ in drawing $\tilde \rho$. The drawing $\rho_{J'}$ associated with $J'$ is its induced drawing in $\tilde \rho$, with face $F'$ serving as the infinite face. Notice that $V(J)\cup V(J')=V(\tilde J)$, and $E(J)\cup E(J')=E(\tilde J)$.

The split $(I_1=(G_1,\Sigma_1),I_2=(G_2,\Sigma_2))$ of instance $I$ along the enhacement structure $\aset$ is defined exactly as before. We start with $A'=A\setminus\set{s}$ and $B'=B\setminus\set{t}$. For every core structure $\jset_i\in\kset\setminus\set{\thecore,\othercore}$, if $v_{J_i}\in A$, then we replace $v_{J_i}$ with vertex set $V(J_i)$ in $A'$, and otherwise we  replace $v_{J_i}$ with vertex set $V(J_i)$ in $B'$. 
%Additionally, we let $J\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F$, and we let $\rho_J$ denote the drawing of $J$ induced by $\tilde \rho$, where we view $F$ as the infinite face of the drawing. Similarly, we let $J'\subseteq \thecore\cup P$ be the graph containing all vertices and edges of $\thecore\cup P$, whose images in $\tilde \rho$ lie on the boundary of $F'$, and we let $\rho_{J'}$ denote the drawing of $J'$ induced by $\tilde \rho$, where we view $F'$ as the infinite face of the drawing. Note that $V(J')\cup V(J'')=V(J)$, and edge sets $E(J'),E(J'')$ define a partition of $E(J)$.

We then let $G_1$ be the subgraph of $G'$, whose vertex set is $V(A')\cup V(J)$, and edge set contains all edges of $E_{G'}(A')$, $E_{G'}(A',V(J))$, and all edges of $J$. Similarly, we let $G_2$ be the subgraph of $G'$, whose vertex set is $V(B')\cup V(J')$, and edge set contains all edges of $E_{G'}(B')$, $E_{G'}(B',V(J'))$, and all edges of $J'$.
The rotation system $\Sigma_1$ for graph $G_1$ and the rotation system $\Sigma_2$ for graph $G_2$ are induced by $\Sigma$. 
Let $I_1=(G_1,\Sigma_1)$ and $I_2=(G_2,\Sigma_2)$ be the resulting two instances of \cnwrs. The proof that $(I_1,I_2)$ is a split of $I$ along $\aset$ is the same as in Case 2, and is omitted here. 
We denote $E^{\del}=E(G)\setminus (E(G_1)\cup E(G_2))$. As before, $E^{\del}=E'\cup E''$, and, if Event $\event$ did not happen, then $|E^{\del}|\leq \frac{2\cro(\phi)\cdot \mu^{2150}}m +|\chi^{\dirty}(\phi)| < \frac{\cro(\phi)\cdot \mu^{2200}}{m}+|\chi^{\dirty}(\phi)|$.
As in Case 2, it is easy to verify that $|\kset_1|,|\kset_2|\leq r$ must hold.



The following observation is an analogue of \Cref{obs: few edges in split graphs case2} for Case 3. The proof is virtually identical (with a very slight change in parameters) and is omitted here.

\begin{observation}\label{obs: few edges in split graphs case3}
 If Event $\event$ did not happen, then $|E(G_1)|,|E(G_2)|\leq m-\frac{m}{32\mu^{300}}$.
\end{observation}


 The next observation is an analogue of \Cref{obs: semi-clean case 2} for Case 3. Its proof is almost identical to that of \Cref{obs: semi-clean case 2}. We provide a proof sketch in Section \ref{subsec: getting semi-clean solution for case 3} of Appendix.


\begin{observation}\label{obs: semi-clean case 3}
If neither of the bad events $\event,\event_5$ happen, then 	
there is a semi-clean solution $\phi_1$ for instance $I_1$ with respect to $\kset_1$, and a semi-clean solution $\phi_2$ for instance $I_2$ with respect to $\kset_2$, such that $|\chi^*(\phi_1)|+|\chi^*(\phi_2)|\leq |\chi^*(\phi)|$, and $|\chi^{\dirty}(\phi_1)|+ |\chi^{\dirty}(\phi_2)|\leq |\chi^{\dirty}(\phi)|+\frac{64\mu^{700}\cro(\phi)}{m}$.
\end{observation}

Altogether, if neither of the events $\event$, $\event_5$ happens, then the algorithm produces a valid output for \procsplit. Since $\prob{\event}\leq \frac{1}{2\mu^{399}}$, while $\prob{\event_5\mid \neg\event}\leq  \frac{1}{\mu^{400}}$, this completes the proof of \Cref{thm: procsplit}.


==> temp.tex <==
the probability that a path $P\in \pset^*$ is selected into the enhancement is now bounded by $2\mu^{3b}/m\leq 2\mu^{5b}/\cm'$ 
$\frac{2\mu^{3b}}{m}$



\paragraph{Bad Paths and $\event'_1$}
\begin{definition}[Good path]
	We say that a path $P\in \pset^*$ is \emph{good} if the following happen:
	
	\begin{itemize}
		\item the number of crossings in which the edges of $P$ participate in $\phi$ is at most $\cro(\phi)\mu^{15b}/m$; and
		
		\item there is no crossing in $\phi$ between an edge of $P$ and an edge of $W$.
	\end{itemize} A path that is not good is called a \emph{bad path}.
\end{definition}


\begin{observation}\label{obs: number of bad paths2}
	The number of bad paths in $\pset^*$ is at most $\frac{4m}{\mu^{15b}}$.
\end{observation}


\begin{claim}\label{claim: event 1 prob2}
	$\prob{\event_1}\leq 8/\mu^{12b}$.
\end{claim}


==> temp2.tex <==

\begin{proof}
	Fix an index $1<i<r$. 
	
As before, we consider the cut $(A,B)$ in graph $\cH$, where $A=V(S_1)\cup\cdots\cup V(S_{i-1})$, and $B=V(S_i)\cup\cdots\cup V(S_r)$. As before, $A$ and $B$ are precisely the sets of vertices of the two connected components of the graph $\tau\setminus\set{u_{i-1},u_i}$, where $\tau$ is the Gomory-Hu tree of graph $\cH$, and so $(A,B)$ is the minimum $u_{i-1}$-$u_i$ cut in $\cH$. We now consider another $u_{i-1}$-$u_i$ cut $(A',B')$ in $\cH$, where $B'=V(S'_i)$, and $A'=V(\cH)\setminus V(S'_i)$. Note that $|E(A,B)|\geq |\leftCedges{i}|+|\leftCedges{i+1}|+|E_{i-1}|$, while $|E(A',B')|=|E_{i-1}|+|\leftCedges{i}|+|\downedges{i}|+|E_{i}|+|\rightCedges{i}|$. From the fact that $(A,B)$ is the minimum $u_{i-1}$-$u_i$ cut, it must be the case that:

\[
|\leftCedges{i+1}|\leq |\downedges{i}|+|E_{i}|+|\rightCedges{i}|
\]



We now employ a symmetric argument: consider the cut $(X,Y)$ in graph $\cH$, where $X=V(S_1)\cup\cdots\cup V(S_{i+1})$, and $Y=V(S_{i+1})\cup\cdots\cup V(S_r)$. As before, $X$ and $Y$ are precisely the sets of vertices of the two connected components of the graph $\tau\setminus\set{u_{i+1},u_{i+2}}$, where $\tau$ is the Gomory-Hu tree of graph $\cH$, and so $(X,Y)$ is the minimum $u_{i+1}$-$u_{i+2}$ cut in $\cH$. We now consider another $u_{i+1}$-$u_{i+2}$ cut $(X',Y')$ in $\cH$, where $X'=V(S'_{i+1})$, and $Y'=V(\cH)\setminus V(S'_{i+1})$. Note that $|E(X,Y)|\geq |\rightCedges{i}|+|\rightCedges{i+1}|+|E_{i+2}|$, while $|E(X',Y')|=|E_{i}|+|\leftCedges{i+1}|+|\downedges{i+1}|+|E_{i+1}|+|\rightCedges{i+1}|$. From the fact that $(X,Y)$ is the minimum $u_{i+1}$-$u_{i+2}$ cut, it must be the case that:

\[
|\rightCedges{i}|+|\rightCedges{i+1}|+|E_{i+2}|\leq |E_{i}|+|\leftCedges{i+1}|+|\downedges{i+1}|+|E_{i+1}|+|\rightCedges{i+1}|.
\]



Since, from \Cref{claim: bound left and right for S''}, $|\rightedges{i}|\leq 1.1|\leftedges{i}|$, and, from \Cref{claim: bound S' to S'' edges},  $|\downedges{i}|\leq 0.1\min\set{|\rightedges{i}|,|\leftedges{i}|}$, we get that:

\[ |\rightedges{i}|\leq 1.1|\downedges{i}|+1.1|E_{i}|+1.1|\rightCedges{i}|\leq 0.11|\rightedges{i}|+1.1|E_{i}|+1.1|\rightCedges{i}|,\]

and so $|\rightedges{i}|\leq 1.3|E_{i}|+1.3|\rightCedges{i}|$.


The proof that $|\leftedges{i}|\leq 1.3|E_{i}|+1.3|\leftCedges{i}|$ is symmetric. The main difference is that we need to consider a $u_i$--$u_{i+1}$ cut $(A,B)$, where $A=V(S_1)\cup\cdots\cup V(S_i)$, and $B=V(S_{i+1})\cup \cdots V(S_r)$, and to compare it with the cut $(A',B')$, where $A'=V(S_i)$ and $B'=V(\cH)\setminus A'$. 




\begin{claim}\label{claim: bound S' to S'' edges}
	For all $1<i<r$, $|\downedges{i}|\leq 0.1\min\set{|\rightedges{i}|,|\leftedges{i}|}$ holds.
\end{claim}


 \begin{claim}\label{claim left edges for S' and S''}
	For all $1<i<r$: $|\rightedges{i}|\leq 1.3|E_{i}|+1.3|\rightCedges{i}|$, and $|\leftedges{i}|\leq 1.3|E_{i}|+1.3|\leftCedges{i}|$.
\end{claim}

==> temp3.tex <==
$\prob{\event_5\mid \neg\event}\leq \frac{3}{\mu^{12b}}$.



==> temp4.tex <==

Suppose we are given an instance $I=(G,\Sigma)$ of \cnwrs, a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$, and a $\jset$-enhancement  $\aset=\set{P,\set{b_u}_{u\in V(J')},\rho'}$, where $J'=J\cup P$.


Let $I=(G,\Sigma)$ be an instance of \cnwrs, let $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ be a  core structure for $I$, and let  $\aset=\set{P,\set{b_u}_{u\in V(J')},\rho'}$ be an enhancement structure for $\jset$, where $J'=J\cup P$.
Let $(\jset_1,\jset_2)$ be the split of $\jset$ via the enhancement structure $\aset$, and denote by $J_1,J_2$ the cores of $\jset_1$ and $\jset_2$, respectively.
=========================



\section{From Sec 3}

\begin{definition}[High-degree vertex]
	Let $G$ be any graph.	A vertex $v\in V(G)$ is a \emph{high-degree} vertex, if $\deg_G(v)\geq |E(G)|/\mu^4$. 
\end{definition}




\begin{definition}[Wide and Narrow Instances]
	Let $I=(G,\Sigma)$ be an instance of \cnwrs with $|E(G)|=m$. We say that $I$ is a \emph{wide} instance, iff there is a high-degree vertex $v\in V(G)$, a partition $(E_1,E_2)$ of the edges of $\delta_G(v)$, such that the edges of $E_1$ appear consecutively in the rotation $\oset_v\in \Sigma$, and so do the edges of $E_2$, and there is a collection $\pset$  of at least $\floor{m/\mu^{\interestconst}}$ simple edge-disjoint simple cycles in $G$, such that every cycle $P\in \pset$ contains one edge of $E_1$ and one edge of $E_2$.
	If no such cycle set $\pset$ exists in $G$, then we say that $I$ is a \emph{narrow} instance.
\end{definition}

\begin{definition}[Well-Connected Wide Instances]
	Let $I=(G,\Sigma)$ be a wide instance of \cnwrs with $|E(G)|=m$. We say that instance $I$ is \emph{well-connected} iff for every pair $u,v$ of distinct vertices of $G$ with $\deg_G(v),\deg_G(u)\geq m/\mu^5$, there is a collection of at least $\frac{8m}{\mu^b}$ edge-disjoint paths connecting $u$ to $v$ in $G$.
\end{definition}




\begin{theorem}\label{lem: many paths}
	There is an efficient randomized algorithm, that, given a wide and well-connected subinstance  $I=(G,\Sigma)$ of $I^*$ with $m=|E(G)|\geq \mu^{c'}$, for some large enough constant $c'$, either returns FAIL, or computes a non-empty collection $\iset$ of subinstances of $I$, such that the following hold:
	
	\begin{itemize}
		\item  $\sum_{I'=(G',\Sigma')\in \iset}|E(G')|\le |E(G)|$;
		
		\item for every instance $I'=(G',\Sigma')\in \iset$, either $|E(G')|\le m/\mu$, or instance $I'$ narrow;
		
		\item 
		there is an efficient algorithm called $\algcombine'$, that, given a solution $\phi(I')$ to every instance $I'\in \iset$, computes a solution $\phi$ to instance $I$; and
		
		\item  if $\optcrors(I)\leq m^2/\mu^{c'}$ then, with probability at least $1-1/\mu^2$,  all of the following hold: 
		
		\begin{itemize}
			\item the algorithm does not return FAIL;
			\item  $\sum_{I'\in \iset}\optcrors(I')\leq \optcrors(I)\cdot  (\log m)^{O(1)}$; and
			\item if algorithm $\algcombine'$ is given as input a solution $\phi(I')$ to each instance $I'\in \iset$, then the resulting solution $\phi$ to instance $I$ that it computes has cost at most: $\cro(\phi)\leq  \sum_{I'\in \iset}\cro(\phi(I')) + \optcrors(I)\cdot\mu^{O(1)}$.
		\end{itemize}
	\end{itemize}
\end{theorem}



=========================================================
\section{Core and Core structure}
=======================

$\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$

\begin{definition}[Core and Core Structure]\label{def: valid core 1}
	Given an instance $I=(G,\Sigma)$ of \cnwrs, a \emph{core structure} for $I$ consists of the following:
	
	\begin{itemize}
		\item a connected subgraph $J$ of $G$ called a \emph{core}, such that, for every edge $e\in E(J)$, graph $J\setminus \set{e}$ is connected;
		\item an orientation $b_u\in \set{-1,1}$ for every vertex $u\in V(J)$; 
		\item a drawing $\rho_J$ of  $J$ on the sphere with no crossings, that is consistent with the rotation system $\Sigma$ and the orientations in $\set{b_u}_{u\in V(J)}$. In other words, for every vertex $u\in V(J)$, the images of the edges in $\delta_J(u)$ enter the image of $u$ in $\rho_J$ according to their order in the rotation $\oset_u\in \Sigma$ and orientation $b_u$ (so, e.g. if $b_u=1$ then the orientation is counter-clock-wise); and
		\item a distinguished face $F^*(\rho_J)\in \fset(\rho_J)$, such  that the image of every vertex $u\in V(J)$, and the image of every edge $e\in E(J)$  is contained in the boundary of face $F^*(\rho_J)$ in drawing $\rho_J$.
	\end{itemize}
\end{definition}


We denote a core structure by $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$, and we refer to graph $J$ as the \emph{core associated with $\jset$}. We denote $\fset^X(\rho_J)=\fset(\rho_J)\setminus\set{F^*(\rho_J)}$, and we refer to the faces in $\fset^X(\rho_J)$ as the \emph{forbidden faces} of the drawing $\rho_J$. 



\begin{definition}[Valid Core Structure]\label{def: valid core 2}
	We say that a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J,F^*_{\rho_C})$ is \emph{valid} iff for every vertex $u\in V(J)$, for every edge $e_i^u\in \delta_G(u)\setminus E(J)$, the corresponding point $p_i^u$ lies in the interior of face $F^*(\rho_J)$ (and hence on the boundary of the disc $D(J)$).
\end{definition}


=================================

\paragraph{Ordering $\oset(J)$ of the Edges of $\delta_G(J)$.}
Consider a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J,F^*(\rho_J))$, the drawing $\rho_J$ of $J$, and its corresponding disc $D(J)$. Recall that, for every vertex $u\in V(J)$ and every edge $e_i^u\in \delta_G(J)$, we have defined a point $p_i^u$ on the boundary of the disc $D(J)$ representing the edge $e_i^u$. We define a circular ordering $\oset(J)$ of the edges of $\delta_G(J)$ to be the circular order in which the  points $p_i^u$ corresponding to the edges of $\delta_G(J)$ are encountered, as we traverse the boundary of the disc $D(J)$ in counter-clock-wise direction.



================================================================
\section{Drawings of Graphs}

Next, we define a valid drawing of a graph $G$ with respect to a core structure $\jset$.

\begin{definition}[A $\jset$-Valid Drawing of a Graph]\label{def: valid drawing}
	Let  $I=(G,\Sigma)$ be an instance of \cnwrs, and let $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J,F^*(\rho_J))$ be a core structure for $I$. A drawing $\phi$ of $G$ on the sphere is a \emph{$\jset$-valid drawing} iff we can define a disc $D'(J)$ that contains the images of all vertices and edges of the core $J$ in its interior, and the image of the core $J$ in $\phi$  is identical to $\rho_{J}$ (though its orientation may be arbitrary), with disc $D'(J)$ in $\phi$ playing the role of the disc $D(J)$in $\rho_{J}$.
\end{definition}

Abusing the notation, we will not distinguish between disc $D(J)$ in $\rho_J$ and disc $D'(J)$ in $\phi$, denoting both discs by $D(J)$. 

Consider now some solution $\phi$ to instance $I$, that is $\jset$-valid, with respect to  some core structure $\jset$. The image of graph $J$ in $\phi$ partitions the sphere into regions, each of which corresponds to a unique face of $\fset(\rho_J)$. We do not distinguish between these regions and faces of $\fset(\rho_J)$, so we view $\fset(\rho_J)$ as a collection of regions in the drawing $\phi$ of $G$.
Next, we define special types of $\jset$-valid drawings, called clean and semi-clean drawings.



\begin{definition}[Clean and Semi-Clean Drawings]\label{def: semiclean drawing}
	Let  $I=(G,\Sigma)$ be an instance of the \cnwrs problem, let  $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J,F^*(\rho_J))$ be a core structure for  $I$, and let $\phi$ be a solution to instance $I$.  We say that $\phi$ is a \emph{semi-clean solution to instance $I$}, or a \emph{semi-clean drawing of $G$}, with respect to $\jset$ if it is a $\jset$-valid drawing, and,  additionally, the image of every vertex of $V(G)\setminus V(J)$ lies outside of the disc $D(J)$ (so in particular it must lie in the interior of the region $F^*(\rho_J)\in \fset(\rho_J)$).
	
	If, additionally, the drawing of every edge of $G$ 
	is contained in region $F^*(\rho_J)$, then we say that $\phi$ is a \emph{clean} solution to $I$ with respect to $\jset$, or that it is a \emph{$\jset$-clean} solution.
\end{definition}

Notice that, from the definition, if $\phi$ is a clean solution to instance $I$ with respect to core structure $\jset$, then the edges of $J$ may not participate in any crossings in $\phi$.
If $\phi$ is a semi-clean solution to $I$ with respect to $\jset$, then the edges of $J$ may participate in crossings, but no two edges of $J$ may cross each other. 
Consider now a crossing  $(e,e')_p$ in drawing $\phi$ of $G$, that is semi-clean with respect to $\jset$. We say that crossing $(e,e')_p$ is \emph{dirty} if exactly one of the two edges $e,e'$ lies in $E(J)$. We denote by $\chi^{\dirty}(\phi)$ the set of all dirty crossings of drawing $\phi$. We denote by $\chi^*(\phi)$ the set of all crossings $(e,e')_{p}$ of $\phi$, for which the crossing point $p$ lies in the inerior of the region $F^*(\rho_J)$. We call assume w.l.o.g. that each such point $p$ lies outside the disc $D(J)$ (by making the disc smaller if necessary).


\paragraph{A $\jset$-Contracted Instance.}

\begin{observation}\label{obs: clean solution to contracted}
	There is an efficient algorithm, whose input consists of an instance $I=(G,\Sigma)$ of \cnwrs, a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ for $I$, and a $\jset$-clean solution $\phi$ to instance $I$. The output of the algorithm is a solution $\hat \phi$ to the corresponding $\jset$-contracted  instance $\hat I=(\hat G,\hat \Sigma)$, with $\cro(\hat \phi)=\cro(\phi)$.
\end{observation}


====================================================
\section{Core Enhancement Structure}
=====================================================


\begin{definition}[Core Enhancement]
	Given an  instance $I=(G,\Sigma)$  of $\cnwrs$ and  a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ for $I$, an \emph{enhancement} of the core structure $\jset$ is a simple path $P\subseteq G$ (that may be a simple cycle), whose both endpoints belong to $J$, such that $P$ is internally disjoint from $J$ (See \Cref{fig: enhance} for an illustration.).
\end{definition}


For simplicity of notation, we will sometimes refer to an enhancement of a core structure $\jset$ as an enhancement of the corresponding core $J$, or as a $\jset$-enhancement. Next, we define a core enhancement structure.

\begin{definition}[Core Enhancement Structure]
	Given an instance $I=(G,\Sigma)$  of $\cnwrs$ and  a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$,  
	a \emph{$\jset$-enhancement structure} consists of:
	
	
	\begin{itemize}
		\item a $\jset$-enhancement $P$;
		\item an orientation $b_u\in \set{-1,1}$ for every vertex $u\in V(P)\setminus V(J)$; and
		
		\item a drawing $\rho'$ of the graph $J'=J\cup P$ with no crossings, such that $\rho'$ is consistent with the rotation system $\Sigma$ and the orientations $b_u$ for all vertices $u\in V(J')$ (the orientations of vertices of $J$ are determined by $\jset$), and moreover, $\rho'$ is a clean drawing of $J'$ with respect to $\jset$.
	\end{itemize}
\end{definition}


================================
The split
================================

Suppose we are given an instance $I=(G,\Sigma)$ of \cnwrs, a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$, and a $\jset$-enhancement  $\aset=\set{P,\set{b_u}_{u\in V(J')},\rho'}$, where $J'=J\cup P$.
We now show an efficient algorithm that, given $\jset$ and $\aset$, splits the core structure $\jset$ into two new core structures, $\jset_1$ and $\jset_2$, using the enhancement structure $\aset$.
We refer to $(\jset_1,\jset_2)$ as a \emph{split} of the core structure $\jset$ via the enhancement structure $\aset$. 


We let $\rho'$ be the drawing of the graph $J'$ on the sphere given by the enhancement structure $\aset$. Recall that there is a disc $D(J)$ that contains the image of $J$ in $\rho'$, whose drawing in $D(J)$ is identical to $\rho_J$ (up to orientation). Additionally, all vertices and edges of $P$ must be drawn in region $F^*(\rho_J)$ of $\rho'$. Therefore, in drawing $\rho'$ of $J'$, there are two faces incident to the image of the path $P$, that we denote by $F_1$ and $F_2$, respectively, and $F_1\cup F_2=F^*(\rho_J)$ holds. 
We let $J_1\subseteq J'$ be the graph containing all vertices and edges, whose images lie on the boundary of face $F_1$ in $\rho'$, and we define graph $J_2\subseteq J'$ similarly for face $F_2$. 

We now define the core structure $\jset_1$, whose corresponding core graph is $J_1$. For every vertex $u\in V(J_1)$, its orientation $b_u$ is the same as in $\aset$. The drawing $\rho_{J_1}$ of $J_1$ is defined to be the drawing of $J_1$ induced by the drawing $\rho'$ of $J'$. Note that $F_1$ remains a face in the drawing $\rho_{J_1}$. We then let $F^*(\rho_{J_1})=F_1$.
The definition of the core structure $\jset_2$ is symmetric, except that we use core $J_2$ instead of $J_1$ and face $F_2$ instead of $F_1$ (see \Cref{fig: type_2_enhance} for an illustration). This completes the description of the algorithm for computing a split $(\jset_1,\jset_2)$ of the core structure $\jset$ via the enhancement structure $\aset$.


\begin{definition}[Splitting an Instance along an Enhancement Structure]\label{def: split}
	Let $I=(G,\Sigma)$ be an instance of \cnwrs, let $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ be a  core structure for $I$, and let  $\aset=\set{P,\set{b_u}_{u\in V(J')},\rho'}$ be an enhancement structure for $\jset$, where $J'=J\cup P$. Let $(\jset_1,\jset_2)$ be the split of $\jset$ via the enhancement structure $\aset$, and denote by $J_1,J_2$ the cores of $\jset_1$ and $\jset_2$, respectively.
	A \emph{split} of instance $I$ along $\aset$ is a pair $I_1=(G_1,\Sigma_1), I_2=(G_2,\Sigma_2)$ of instances of \cnwrs, for which the following hold.
	
	\begin{itemize}		
		\item $V(G_1)\cup V(G_2)=V(G)$ and $E(G_1)\cup E(G_2)\subseteq E(G)$; 
		\item every vertex $v\in V(G_1)\cap V(G_2)$ belongs to $V(J_1)\cap V(J_2)$; 
		\item $\jset_1$ is a valid core structure for $I_1$, and $\jset_2$ is a valid core structure for $I_2$.
	\end{itemize}
\end{definition}



\begin{observation}\label{obs: combine solutions for split}
	There is an efficient algorithm, whose input consists of
	an instance  $I=(G,\Sigma)$ of \cnwrs, a core structure $\jset$ for $I$, a $\jset$-enhancement structure $\aset$, and  a split $(I_1,I_2)$ of $I$ along $\aset$, together with a clean solution $\phi_1$ to instance $I_1$ with respect to $\jset_1$,  and a clean solution $\phi_2$ to instance $I_{2}$ with respect to $\jset_2$, where $(\jset_1,\jset_2)$ is the split of $\jset$ along $\aset$. The algorithm computes a clean solution $\phi$ to instance $I$ with respect to $\jset$, with $\cro(\phi)\leq \cro(\phi_1)+\cro(\phi_2)+|E^{\del}|\cdot |E(G)|$, where $E^{\del}=E(G)\setminus (E(G_{1})\cup E(G_{2}))$.
\end{observation}


\subsubsection{Auxiliary Claim}

\begin{claim}\label{claim: curves orderings crossings}
	Let $I=(G,\Sigma)$ be an instance of \cnwrs, and let $\pset=\set{P_1,\ldots,P_{4k+2}}$ be a collection of directed edge-disjoint simple paths in $G$, that are non-transversal with respect to $\Sigma$. For all $1\leq i\leq 4k+2$, let $e_i$ be the first edge on path $P_i$. Assume that there are two distinct vertices $u,v\in V(G)$, such that all paths in $\pset$ originate at $u$ and terminate at $v$, and assume further that
	edges $e_1,\ldots,e_{4k+2}$ appear in this order in the rotation $\oset_u\in \Sigma$. Lastly, let $\phi$ be any solution to instance $I$, such that the number of crossings $(e,e')_p$ in $\phi$ with $e$ or $e'$ lying in $E(P_1)$ is at most $k$, and assume that the same is true for $E(P_{2k+1})$. Then $\phi$ does not contain a crossing between an edge of $P_1$ and an edge of $P_{2k+1}$.
\end{claim}


======================================
Procedure \procsplit
=======================================

\paragraph{Valid Input for \procsplit.}
A valid input for \procsplit consists of an instance  $I=(G,\Sigma)$  of $\cnwrs$, and a  a core structure $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ for $I$, for which the following hold:

\begin{properties}{C}
	\item graph $G$ is a subgraph of $\cG$, and $\Sigma$ is the rotation system for $G$ induced by $\cSigma$;  \label{prop valid input size}
	\item the $\jset$-contracted instance $\hat I$ corresponding to instance $I$ is wide;  \label{prop valid input wide}
	\item $|E(G)|\geq \cm/\mu$; \label{prop many edges}
	\item for every vertex $x\in V(G)$ with $\deg_G(x)\geq \cm/\mu^5$, there is a collection of at least $\frac{4\cm}{\mu^{50}}$ edge-disjoint paths in $G$ connecting $x$ to vertices of $J$; and \label{prop: connect high degree to core}
	\item there exists a solution $\phi$ to instance $I$ that is semi-clean with respect to $\jset$, such that $\cro(\phi)\leq \frac{|E(G)|^2}{\mu^{1500}}$ and $|\chi^{\dirty}(\phi)|\leq \frac{|E(G)|}{ \mu^{1500}}$. \label{prop valid input drawing}
\end{properties} 

We emphasize that the semi-clean solution $\phi$ is not known to the algorithm.


\paragraph{Valid Output for \procsplit.}
A valid output for \procsplit consists of a
$\jset$-enhancement structure $\aset$, and
a split $(I_1=(G_1,\Sigma_1),I_2=(G_2,\Sigma_2))$ of $I$ along $\aset$, for which the following hold. Let $(\jset_1,\jset_2)$ be the split of the core structure $\jset$ along $\aset$. Then:


\begin{properties}{P}
	\item $|E(G)\setminus (E(G_1)\cup E(G_2))|\leq \frac{\cro(\phi)\cdot \mu^{2200}}{|E(G)|}+|\chi^{\dirty}(\phi)|$; 	\label{prop output deleted edges}
	\item  each of the graphs $G_{1},G_{2}$ contains at most $|E(G)|-\frac{|E(G)|}{32\mu^{300}}$  edges; and \label{prop: smaller graphs}
	\item there is a semi-clean solution $\phi_1$ to instance $I_1$ with respect to $\jset_1$, and a semi-clean solution $\phi_2$ to instance $I_2$ with respect to $\jset_2$, such that $|\chi^{\dirty}(\phi_1)|+|\chi^{\dirty}(\phi_2)|\leq |\chi^{\dirty}(\phi)|+\frac{64\mu^{700}\cro(\phi)}{|E(G)|}$, and $|\chi^*(\phi_1)|+|\chi^*(\phi_2)|\leq |\chi^*(\phi)|$.\label{prop output drawing}
	
\end{properties}  


%------------------

The main theorem of this subsection summarizes the properties of Procedure \procsplit.

\begin{theorem}\label{thm: procsplit}
	There is an efficient randomized algorithm, that, given a valid input  $I=(G,\Sigma)$, $\jset=(J,\set{b_u}_{u\in V(J)},\rho_J, F^*(\rho_J))$ to procedure \procsplit, with probability at least $1-1/\mu^{399}$ computes a valid output for the procedure.
\end{theorem}



\begin{claim}\label{claim: find potential augmentors}
	There is an efficient algorithm that,  given a  valid input $I=(G,\Sigma)$, $\jset=(J,\set{b_u}_{u\in V(J)},\rho, F^*)$  to procedure \procsplit, computes a  promising path set of cardinality $\ceil{\frac{m}{6\mu^{50}}}$. 
\end{claim}





\paragraph{Valid Input for $\procsplit'$.}
A valid input to Procedure $\procsplit'$ consists of a skeleton augmenting structure $\wset$ for $\ckset$ (whose corresponding skeleton augmentation we denote by $W$), parameters $g_1,g_2$, a $\wset$-decomposition $\gset$ of $\cG'$, and a face $F\in \tilde \fset(\wset)$, for which the following hold. Denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G=\cG'\setminus E^{\del}$, and let $\tilde \Sigma$ be the rotation system for graph $\tilde G$ induced by $\cSigma'$. Let $\tilde I=(\tilde G,\tilde \Sigma)$ be the resulting instance of \cnwrs. Then:


% \mynote{note that I replaced $30$ with $60$ in property C2 twice. This needs to be propagated in this section, and probably also back. I also added $g_1,g_2$ and the conditions on them}
\begin{properties}{C}
	\item Instance  $I_F=(G_F,\Sigma_F)$ associated with the graph $G_F\in \gset$ is not acceptable; 
	\label{prop: instance unacceptable}
	\item for every subset $E'\subseteq E(\tilde G')\setminus E(W)$ of edges, with $|E'|\leq \left (\frac{g_1}{\cm'}+g_2\right )\cdot \mu^{100b}$, there is a connected component $C$ in graph $\tilde G'\setminus E'$ with $W\subseteq C$; \label{prop: new} %\mynote{this is a new condition that follows from $g_3$-connectedness of skeleton and the fact that we delete few edges in each iteration and there are few iterations; this also needs to be propagated}
	\item there exists a solution $\phi$ to instance $\tilde I$, that is semi-clean with respect to $\ckset$, and has the following additional properties: \label{prop: drawing}
	\begin{itemize}
		\item drawing $\phi$ is $\wset$-compatible;
		\item $\cro(\phi)\leq \min\set{g_1,(\cm')^2/\mu^{60b}}$;
		\item $|\chi^{\dirty}(\phi)|\leq \set{g_2,\cm'/\mu^{60b}}$ (as before, a crossing of $\phi$ is dirty if it involves an edge of the skeleton $\cK$); and
		\item the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate is at most $\cro(\phi)\mu^{34b}/\cm'$.
	\end{itemize}
\end{properties} 

As before, the semi-clean solution $\phi$ is not known to the algorithm.






% \mynote{this was updated to a new bound on $E^{\del}(F)$. The remainder of this section needs to be  updated to reflect all this.}

\paragraph{Valid Output for $\procsplit'$.}
A valid output for Procedure $\procsplit'$ consists of 
a skeleton augmenting structure $\wset'$ for $\ckset$ (whose corresponding skeleton augmentation we denote by $W'$), an edge set $E^{\del}(F)\subseteq E(G_F)\setminus E(W')$ of cardinality at most $\left(\frac{g_1}{|E(G_F)|}+g_2\right)\cdot \mu^{50b}$, and a $\wset'$-decomposition $\gset'$ of graph $\cG'$, for which the following hold. 
Denote $E^{\del}=E(\cG')\setminus\left (\bigcup_{G_{F'}\in \gset}E(G_{F'})\right)$, $\tilde G'=\cG'\setminus (E^{\del}\cup E^{\del}(F))$, and let $\tilde \Sigma'$ be the rotation system for graph $\tilde G'$ induced by $\cSigma'$. Let $\tilde I'=(\tilde G',\tilde \Sigma')$ be the resulting instance of \cnwrs. Then:



\begin{properties}{P}
	\item $W\subseteq W'$, and $\tilde \fset(\wset')=\left(\tilde\fset(\wset)\setminus\set{F}\right)\bigcup\set{F_1,F_2}$;\label{prop: same faces}
	
	\item for every face $F'\in \tilde \fset(\wset)\setminus\set{F}$, the graph $G_{F'}$ associated with face $F'$ in the decomposition $\gset$ is identical to the graph $G'_{F'}$ associated with face $F'$ in the decomposition $\gset'$; \label{prop: same graphs}
	
	\item if $G_F$ is the graph associated with face $F$ in $\gset$, and $G_{F_1},G_{F_2}$ are the graphs associated with faces $F_1$ and $F_2$, respectively, in $\gset'$, then $E(G_F)\setminus (E(G_{F_1})\cup E(G_{F_2}))= E^{\del}(F)$. Moreover, $|E(G_{F_1})\setminus E(W')|, |E(G_{F_2})\setminus E(W')|\leq |E(G_{F})\setminus E(W)|-\cm'/\mu^{5b}$; \label{prop: small instances} and
	
	
	\item  there exists a solution $\phi'$ to instance $\tilde I'$, that is semi-clean with respect to $\ckset$, and has the following additional properties: \label{prop: drawing after}
	\begin{itemize}
		\item drawing $\phi'$ is $\wset'$-compatible;
		\item $\cro(\phi')\leq \cro(\phi)$;
		\item $|\chi^{\dirty}(\phi)|\leq |\chi^{\dirty}(\phi')|$; and
		\item if we denote by $N(\phi)$ the total number of crossings of $\phi$ in which the edges of $E(W)\setminus E(\cK)$ participate, and define $N(\phi')$ similarly for $\phi'$, then $N(\phi')\leq N(\phi)+\cro(\phi)\mu^{26b}/\cm'$.
	\end{itemize}
\end{properties}  


We summarize our algorithm for Procedure $\procsplit'$ in the following lemma.

\begin{lemma}\label{lem: alg procsplit'}
	There is an efficient randomized algorithm, that, given a valid input to Procedure $\procsplit'$, with probability at least $1-1/\mu^{10b}$ produces a valid output for Procedure $\procsplit'$.
\end{lemma}

======================
Parmeters for \procsplit and bad events
========================


$k=\floor{\frac{m}{\mu^{50}}}$

Probability to select path into enhancement:  $\frac{16}{k}\leq \frac{32\mu^{50}}{m}$.



\begin{definition}[Good path]
	We say that a path $P'\in \pset$ is \emph{good} if the following happen:
	
	\begin{itemize}
		\item the number of crossings in which the edges of $P'$ participate in $\phi$ is at most $\frac{64\mu^{450}\cro(\phi)}{m}$; and
		
		\item there are no crossings in $\phi$ between edges of $P'$ and edges of $J$.
	\end{itemize} A path that is not good is called a \emph{bad path}.
\end{definition}


We now bound the number of bad paths in $\pset$.

\begin{observation}\label{obs: number of bad paths}
	The number of bad paths in $\pset$ is at most $\frac{m}{8\mu^{450}}$.
\end{observation}


We say that bad event $\event_1$ happens if the enhancement path $P$ is bad.
===================================

==> temp6.tex <==
a  $\jset$-valid solution $\cpsi$ to instance $\cI'$, with $\cro(\cpsi)\leq (\cm')^2/\mu^{120b}$ and  $|\chi^{\dirty}(\cpsi)|\leq \cm'/\mu^{120b}$


Consider now some skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$.
$\jset_F=(J_F,\set{b_u}_{u\in V(J_F)},\rho_{J_F}, F^*(\rho_{J_F}))$


\begin{theorem}\label{thm: phase 2}
	There is an efficient randomized algorithm, whose input consists of a large enough constant $b\geq 1$, a subinstance $I=(G,\Sigma)$ of $\cI$ with $|E(G)|=m$, and a core structure $\jset(I)$ for $I$, whose corresponding core is denoted by $J(I)$.
	The algorithm computes a set $E^{\del}(I)\subseteq E(G)\setminus E(J(I))$ of edges, for which the following hold. 
	Let $G'=G\setminus E^{\del}(I)$, let $\Sigma'$ be the rotation system for $G'$ that is induced by $\Sigma$, and let $I'=(G',\Sigma')$ be the resulting instance of \cnwrs.
	The algorithm ensures that, if there is a solution $\psi(I)$ to instance $I$ that is $\jset(I)$-valid, with $\cro(\psi(I))\leq m^2/\mu^{120b}$, and  $|\chi^{\dirty}(\psi(I))|\leq m/\mu^{120b}$, then  with probability at least $1-1/\mu^{2b}$,  
	$|E^{\del}(I)|\leq \left (\frac{\cro(\psi(I))}{m}+|\chi^{\dirty}(\psi(I))\right ) \cdot \mu^{O(b)}$, and  there is a solution $\psi(I')$ to instance $I'$ that is clean with respect to $\jset(I)$, with $\cro(\psi(I'))\leq \left (\cro(\psi(I))+|\chi^{\dirty}(\psi(I))|^2+\frac{|\chi^{\dirty}(\psi(I))|\cdot |E(G)|}{\mu^b}\right )\cdot (\log m)^{O(1)}$. %, where $\hat m(I)$ is the number of edges in the $\kset(I)$-contracted instance $\hat I$ corresponding to $I$.
\end{theorem}




=============================

Skeleton structures

=============================

\begin{definition}[Skeleton]
	Let $K$ be a subgraph of $\cG'$. We say that $K$ is a \emph{skeleton graph}, if $\cJ'\subseteq K$, and, for every edge $e\in E(K)$, graph $K\setminus\set{e}$ is connected.
\end{definition}



\begin{definition}[Skeleton Structure]
	A skeleton structure $\kset$ consists of the following three ingredients:
	
	\begin{itemize}
		\item a skeleton graph $K$;
		\item for every vertex $u\in V(K)$, an orientation $b_u\in \set{-1,1}$, such that, for every vertex $u\in V(\cJ')$, its orientation $b_u$ is identical to that given by the core structure $\cjset'$; and
		\item a drawing $\rho_K$ of graph $K$ on the sphere without no crossings, such that $\rho_K$ obeys the rotation system $\cSigma'$, the orientation of every vertex $u\in V(K)$ in $\rho_K$ is $b_u$, and drawing $\rho_K$ is clean with respect to $\cjset'$.
	\end{itemize}
\end{definition}


Consider now some skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$. For brevity of notation, we denote by $\tfset(\kset)=\fset(\rho_K)$ the set of all faces in the drawing $\rho_K$. Since drawing $\rho_K$ is clean with respect to $\cjset'$, the image of every vertex and every edge of $K$ appears in the region $F^*=F^*(\rho_{\cJ'})$ of this drawing. Therefore, every forbidden face $F\in \fset^X(\rho_{\cJ'})$ is also a face of $\tfset(\kset)$. We denote by $\tfset^X(\kset)=\fset^X(\rho_{\cJ'})$ the set of all such faces, that we refer to as \emph{forbidden faces of drawing $\rho_K$}, and we denote by $\tfset'(\kset)=\tfset(\kset)\setminus\tfset^X(\kset)$ the set of all remaining faces.


Consider some face $F\in \tfset(\kset)$, and let $J_F=\partial_{\rho_K}(K,F)$ be the graph consisting of all vertices and edges whose images appear on the boundary of face $F$ in drawing $\rho_K$. From the definition of a skeleton graph $K$, graph $J_F$ is a core graph. We can then define a core structure $\jset_F=(J_F,\set{b_u}_{u\in V(J_F)},\rho_{J_F}, F^*(\rho_{J_F}))$ as follows: for every vertex $u\in V(J_F)$, its orientation $b_u$ remains the same as in $\kset$. Drawing $\rho_{J_F}$ of graph $J_F$ is the drawing induced by $\rho_K$. Notice that face $F\in \tfset(\kset)$ remains a face in the drwing $\rho_{J_F}$. Face $F^*(\rho_{J_F})$ is then defined to be the face $F$. (We note that a core structure is generally defined for some specific graph $G'$, and specifically the definition of a valid core structure from \Cref{def: valid core 2} requires the core structure to be defined for a specific graph $G'$. Therefore, for now we view the core structure $\jset_F$ as simply a tuple $(J_F,\set{b_u}_{u\in V(J_F)},\rho_{J_F}, F^*(\rho_{J_F}))$, and we will later define a subgraph $G_F$ of $\cG'$, for which $\jset_F$ will be a valid core structure. Alternatively, it is easy to see that $\jset_F$ is a valid core structure for graph $K$, but we will later consider other subgraphs of $\cG'$ for which $\jset_F$ is a valid core structure).


===========================

Drawings

==========================



\paragraph{$\kset$-Valid Drawings.}

Next, we consider a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$ and a subgraph $G'\subseteq G$ with $K\subseteq G'$. We then define $\kset$-valid drawings of graph $G'$, in a natural way.

\begin{definition}[$\kset$-valid drawings]
	Let $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$ be a skeleton structure, let  $G'$ be a subgraph of $G$ with $K\subseteq G'$, and let $I'=(G',\Sigma')$ be the subinstance of $\cI'$ defined by $G'$. We say that a solution $\phi$ to instance $I'$ is $\kset$-valid, iff the drawing of the skeleton $K$ induced by $\phi$ is identical to $\rho_K$, and the orientation of every vertex $u\in V(K)$ in drawing $\phi$ is identical to the orientation given by $\kset$. We also say that a $\kset$-valid solution $\phi$ to instance $I'$ is a \emph{$\kset$-valid drawing} of graph $G'$.
\end{definition}


Since we will be considering various core structures $\jset_F$ associated with faces $F\in \tfset(\kset)$ of a given skeleton structure $\kset$, the definition of dirty edges and dirty crossings will change depending on which core structure we consider. As the algorithm pogresses, the drawing $\psi(\cI')$ that we maintain for the current graph $G'=\cG'\setminus E^{\del}(\cI')$ will evolve. We need to keep track of the crossings in which the edges of the original core $\cJ'$ participate, and of the edges involved in these crossings.

Therefore, given a subgraph $G'\subseteq G$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$, and a $\kset$-valid solution to subinstance $I'=(G',\Sigma')$ defined by graph $G'$, we denote by $\chi^*(\phi)$ the set of all crossings $(e,e')_p$ in $\phi$ where $e$ or $e'$ belong to the core $\cJ'$, and we denote by $E^*(\phi)$ the set of all edges $e\in E(G')\setminus E(K)$ that participate in crossings of $\chi^*(\phi)$.



\paragraph{A $\kset$-Decompositions of $\cG'$ and Face-Based Instances.}

Over the course of the algorithm, we will maintain a skeleton structure $\kset$, and an associated decomposition of graph $\cG'$ into subgraphs. Intuitively, for every face $F\in \tfset(\kset)$, we will define a subgraph $G_F$ of $\cG'$ that we associate with face $F$. We now define a $\kset$-decomposition of $\cG'$.


\begin{definition}[A $\kset$-decomposition of $\cG'$]
	Let $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$ be a skeleton structure, and, for every face $F\in \tilde \fset(\kset)$, let $\jset_F=(J_F,\set{b_u}_{u\in V(J_F)},\rho_{J_F}, F^*(\rho_{J_F}))$ be the core structure that $\kset$ defines for face $F$. A $\kset$-decomposition of the input graph $\cG'$ is a collection $\gset=\set{G_{ F}\mid  F\in \tilde \fset(\kset)}$ of subgraphs of $\cG'$, for which the following hold: 
	
	\begin{itemize}
		\item for every face $ F\in \tilde \fset(\kset)$, the core structure $\jset_F$ associated with face $F$ is a valid core structure for instance $I_F=(G_F,\Sigma_F)$ defined by graph $G_F$;
		
		\item for every forbidden face $F\in \tilde \fset^X(\kset)$, $G_F=J_F$;
		
		
		\item for every face $F\in \tilde \fset(\wset)$, $G_F\cap K=J_F$; and
		
		\item for every pair $F, F'\in \tilde\fset(\wset)$ of distinct faces, $V(G_{F})\cap V(G_{F'})\subseteq  V(J_F)\cap V(J_{F'})$, and $E(G_{F})\cap E(G_{F'})\subseteq  E(J_F)\cap E(J_{F'})$.
	\end{itemize} 
	
	We will sometimes refer to the subinstance $I_F=(G_F,\Sigma_F)$ of $\cI'$ defined by graph $G_F$ associated with a face $F\in \tilde \fset(\kset)$ as a \emph{face-based subinstance} associated with face $F$.
\end{definition}

========================



\begin{definition}[Acceptable Instances]
	Let	$\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$ be skeleton structure, let $\gset=\set{G_F\mid F\in \tilde \fset(\kset)}$ be a $\kset$-decomposition of graph $\cG'$, and let $F\in \tilde \fset(\kset)$ be a face. Consider a graph $H_F$,  that is obtained from graph $G_{F}$ by first subdividing every edge $e\in \tilde E_F$ with a vertex $t_e$, and then deleting all vertices and edges of $J_{F}$ from it. We say that instance $G_{F}$ is \emph{acceptable} iff for every partition $(E_1,E_2)$ of the edges of $\tilde E_F$, such that the edges of $E_1$ appear consecutively in the ordering $\oset(J_F)$, there is a cut $(X,Y)$ in graph $H_{F}$ with vertex set $\set{t_e\mid e\in E_1}$ contained in $X$, vertex set $\set{t_e\mid e\in E_2}$ contained in $Y$, and $|E_{H_{\tF}}(X,Y)|\leq \cm'/\mu^{2b}$.
\end{definition}



========================


\begin{lemma}\label{lem: compute phase 2 decomposition}
	There is an efficient randomized algorithm, whose input consists of a large enough constant $b\geq 1$, a subinstance $\cI'=(\cG',\cSigma')$ of $\cI$ with $|E(\cG')|=\cm'$, and a core structure $\cjset$ for $\cI'$, whose corresponding core is denoted by $\cJ$.
	The algorithm either returns FAIL, or computes a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$, and a $\kset$-decomposition $\gset$ of $\cG'$, such that, for every face $F\in \tilde \fset(\kset)$, the corresponding subinstance $I_F=(G_F,\Sigma_F)$ of $\cI'$ defined by the graph $G_F\in \gset$ is acceptable. 
	Moreover, if there is a solution $\psi(\cI')$ to instance $\cI'$ that is $\cjset$-valid, with $\cro(\psi(\cI'))\leq (\cm')^2/\mu^{120b}$, and  $|\chi^{*}(\psi(\cI'))|\leq \cm'/\mu^{120b}$, then  with probability at least $1-1/\mu^{2b}$, the following hold:
	
	\begin{itemize}
		\item the algorithm does not return FAIL;
		\item the cardinality of edge set $E^{\del}(\cI')=E(\cG')\setminus \left(\bigcup_{F\in \tilde \fset(\kset)}E(G_F)\right )$ is bounded by: $$\left (\frac{\cro(\psi(\cI'))}{m}+|\chi^{\dirty}(\psi(\cI'))\right ) \cdot \mu^{O(b)};\mbox{ and }$$
		
		\item if we  denote $G'=\cG'\setminus E^{\del}(\cI')$, and let $I'=(G',\Sigma')$ be the subinstance of $\cI'$ defined by graph $G'$, then  there is a $\kset$-valid solution $\phi$ to instance $I'$, with $\cro(\phi)\leq \cro(\psi(\cI'))$,  $|\chi^*(\phi)|\leq |\chi^*(\psi(\cI'))|$, and the total number of crossings in which the edges of $K$ participate is at most $\frac{\cm}{\mu^{2b}}$. 
	\end{itemize}
\end{lemma}


\begin{lemma}\label{lem: computed decomposition is good enough}
	Suppose we are given a subinstance $\cI'=(\cG',\cSigma')$ of $\cI$ with $|E(\cG')|=\cm'$, a core structure $\cjset$ for $\cI'$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$, and a $\kset$-decomposition $\gset$ of $\cG'$, such that, for every face $F\in \tilde \fset(\kset)$, the corresponding subinstance $I_F=(G_F,\Sigma_F)$ of $\cI'$ defined by the graph $G_F\in \gset$ is acceptable.  Let $E^{\del}(\cI')=E(\cG')\setminus \left(\bigcup_{F\in \tilde \fset(\kset)}E(G_F)\right )$, $G'=\cG'\setminus E^{\del}(\cI')$, and let $I'=(G',\Sigma')$ be the subinstance of $\cI'$ defined by graph $G'$. Assume further that there is a $\kset$-valid solution $\phi$ to instance $I'$, so that the total number of crossings in which the edges of $K$ participate is at most $\frac{\cm}{\mu^{2b}}$. Then 
	there is a solution $\psi(I')$ to instance $I'$ that is clean with respect to $\cjset$, with $\cro(\psi(I'))\leq \left (\cro(\phi)+|\chi^{*}(\phi)|^2+\frac{|\chi^{*}(\phi)|\cdot \cm'}{\mu^b}\right )\cdot (\log \cm')^{O(1)}$.
\end{lemma}



 we say that a solution $\psi$ to instance $\cI'$ is \emph{good}, if it is $\cjset$-valid, with $\cro(\psi)\leq (\cm')^2/\mu^{240b}$, and  $|\chi^{*}(\psi)|\leq \cm'/\mu^{240b}$
 
 num of stages: $\ceil{32\mu^{6b}}$.

==> temp8.tex <==

\begin{lemma}\label{lem: computed decomposition is good enough}
Suppose we are given a subinstance $\cI'=(\cG',\cSigma')$ of $\cI$ with $|E(\cG')|=\cm'$, a core structure $\cjset$ for $\cI'$, a skeleton structure $\kset=(K,\set{b_u}_{u\in V(K)},\rho_K)$, and a $\kset$-decomposition $\gset$ of $\cG'$, such that, for every face $F\in \tilde \fset(\kset)$, the corresponding subinstance $I_F=(G_F,\Sigma_F)$ of $\cI'$ defined by the graph $G_F\in \gset$ is acceptable.  Let $E^{\del}(\cI')=E(\cG')\setminus \left(\bigcup_{F\in \tilde \fset(\kset)}E(G_F)\right )$, $G'=\cG'\setminus E^{\del}(\cI')$, and let $I'=(G',\Sigma')$ be the subinstance of $\cI'$ defined by graph $G'$. Assume further that there is a $\kset$-valid solution $\phi$ to instance $I'$, so that the total number of crossings in which the edges of $K$ participate is at most $N$. Then 
there is a solution $\psi(I')$ to instance $I'$ that is clean with respect to $\cjset$, with $\cro(\psi(I'))\leq \left (\cro(\phi)+N^2+|\chi^{*}(\phi)|^2+\frac{|\chi^{*}(\phi)|\cdot \cm'}{\mu^b}\right )\cdot (\log \cm')^{O(1)}$.
\end{lemma}
	

==> trimming_and_wld.tex <==
\subsubsection{Trimming clusters in $\cset_2$ and well-linked decomposition}

%\znote{This section can be merged with Section~\ref{sec:size_reduction}. For now I write them separately to make it more modular.}

We say that a cluster $C$ is a \emph{flower cluster}, iff



In this step, we further modify the sets $\cset_1, \cset_2, \cset_3$ of clusters of $G'$ that we get from Section~\ref{sec:size_reduction}, to obtain new sets $\cset'_1, \cset'_2, \cset'_3$ of clusters of $G'$ (we denote $\cset'=\cset'_1\cup \cset'_2\cup \cset'_3$), such that:
\begin{itemize}
\item the vertex sets $\set{V(C)}_{C\in \cset'}$ partitions $V(G')$;
\item $|\inE(\cset')|= O(m/\mu)$;
\item for each cluster $C\in \cset_1$, $|E(C)|\le m/\mu^2$, and $C$ is $\alpha$-well-linked;
\item for each cluster $C\in \cset_2$, $|E(C)|> m/\mu^2$, and $C$ is a flower cluster;
\item for each cluster $C\in \cset_3$, $|E(C)|> m/\mu^2$ and $C$ is a good cluster.
\end{itemize}


Recall that in Section~\ref{sec:size_reduction}, we are given a valid sub-instance $(G',\Sigma')$ (with $|E(G')|=m$) of the input instance $(G,\Sigma)$, and we compute a set $\cset=\cset_1\cup \cset_2\cup \cset_3$ of disjoint clusters of $G'$, where $\cset_1$ contains clusters of at most $m/\mu^{2}$ edges, $\cset_3$ contains good clusters with at most $m/\mu^{2}$ edges, and  for each cluster $C\in \cset_2$, $|E(C)|> m/\mu^2$, $C$ is not a good cluster and $C$ contains exactly one high-degree vertex.
We directly set $\cset'_3=\cset_3$. All steps in this section are applied to clusters in $\cset_1$ and $\cset_2$.

\paragraph{Step 1. Trim clusters in $\cset_2$.}
We consider each cluster in $\cset_2$ one-by-one, and further decompose it as follows. Let $C$ be a type-2 cluster, and let $u$ be the unique high-degree vertex in $C$ (so $\deg_{C}(u)\ge m/\mu^5$). 
Let $\tilde C$ be the graph obtained from $C\cup\delta(C)$ by contracting all vertices of $\Gamma_G(C)$ into a single vertex, that we denote by $\tilde u$.
We compute a min-cut $(A,B)$ of $C'$ separating $u$ from $\tilde u$, with $u\in A$ and $\tilde u\in B$. We then decompose $C$ into two clusters: the subgraph of $C$ induced by vertices of $A$, that we denote by $C'$; and the subgraph of $C$ induced by vertices of $B\setminus \set{\tilde u}$, that we denote by $C''$.
Notice that there is a set of edge-disjoint paths in $C'$ connecting $\delta(C)$ to $u$.
If $|E(C')|>m/\mu^2$, then we replace the cluster $C$ in $\cset_2$ and with cluster $C'$. Otherwise, we delete $C$ from $\cset_2$ and add $C'$ to $\cset_1$.

Note that the cluster $C''$ does not contain any high-degree vertex, and the graph $C''$ may be not connected.
We apply the algorithm in Lemma~\ref{lem:main_decomposition} to each connected component of $C''$ as a separate cluster to $\cset_1$. 
Clearly, we will obtain a set $\tilde\cset=\set{C''_1,\ldots,C''_k}$ of clusters, such that $|E(C''_i)|\le |E(C'')|/\mu^2\le m/\mu^2$ for each $1\le i\le k$, and $|\inE(\tilde\cset)|\le O(|E(C'')|/\mu)$. We add all clusters of $\tilde\cset$ to $\cset_1$.


\paragraph{Step 2. Process clusters in $\cset_2$ to get flower clusters.}
In this step, we further process the clusters in $\cset_2$ one-by-one as follows. Throughout, we set the parameter $d=m/\mu^{5}$.
Let $C$ be a cluster of $\cset_2$ and let $u$ be the unique high-degree vertex. Denote $\delta(u)=\set{e_1,\ldots,e_{\deg(u)}}$, where the edges are indexed according to the rotation at $u$ in $\Sigma$.
Denote $r=\lfloor\frac{\deg(u)}{d}\rfloor+1$.
For each $1\le i\le r-1$, let $E_i=\set{e_{(i-1)d+1},\ldots,e_{id}}$, and let $E_{r}=\set{e_{(r-1)d+1},\ldots,e_{\deg(u)}}$.
Clearly, sets $E_1,E_2,\ldots,E_r$ are consecutive subsets of edges in $\delta(u)$, each containing at most $d$ edges, and $r<O(\mu^5)$. 
Let the cluster $C'$ be obtained from $C$ by replacing the vertex $u$ with $r$ distinct new vertices $u_1,\ldots,u_r$, such that the edges of $E_i$ are incident to $u_i$. 
Denote $T=\set{u_1,\ldots,u_r}$. 
For each $1\le i\le r$, let $(A_i,B_i)$ be the min-cut in $C'$, that separates $u_i$ from all vertices in $T\setminus \set{u_i}$, where $u_i\in A_i$. We denote by $X_i$ the subgraph of $C'$ induced by vertices of $A_i$, 
%We call $X_i$ a \emph{sub-cluster} of $C$. 
and we denote $\xset=\set{X_1,\ldots,X_r}$.
For each $1\le i\le r$, we denote $\hat E_i=\delta(X_i)$, then $\hat E_i$ can be partitioned into two subsets: set $\hat E'_i$ connecting a vertex of $X_i$ to a vertex of some cluster of $\xset\setminus \set{X_{i}}$, and set $\hat E''_i$, connecting $X_i$ to vertices of $C'$ that do not belong to any cluster of $\xset$ (such an edge may also belong to $\delta(C)$).
See Figure~\ref{fig:flower_edge} for an illustration.

 \begin{figure}[h]
	\includegraphics[scale=0.3]{figs/flower_edge.jpg}
	\caption{An illustration of the edge sets in a flower cluster.\label{fig:flower_edge}}
\end{figure} 

We use the following observation.

\begin{observation}
For each $1\le i\le r$, there is a set $\qset_i$ of paths in $X_i$ connecting edges of $\hat E_i$ to $u_i$, and $\cong(\qset_i)\le 2$.
\end{observation} 
\begin{proof}
edges of $\hat E'_i$ are routed because $X_i$ is a min cut separating $u_i$ from other terminals; edges of $\hat E''_i$ are routed because of the min-cut $(A,B)$, and possibly using the paths connecting $\hat E'_i$ to $u_i$.
\end{proof}

Let $C''$ be the cluster obtained by taking the union of $X_1,\ldots,X_r$, and unifying $v_1,\ldots,v_r$ back into the vertex $v$, so $C''$ is the subgraph of $C$ induced by vertices of $\bigcup_{1\le i\le r}V(X_i)$. We decompose the cluster $C$ into $C''$ and $C\setminus C''$.
Clearly, the subgraph $C\setminus C''$ does not contain any high-degree vertex. We apply the algorithm of Lemma~\ref{lem:main_decomposition} to $C\setminus C''$, and add all the obtained clusters to $\cset_1$.
On the other hand, if $|E(C'')|>m/\mu^2$, then $C''$ is a flower cluster, and we replace the $C$ in $\cset_2$ with $C''$. Otherwise we delete $C$ from $\cset_2$ and add $C''$ to $\cset_1$.



\paragraph{Step 3. Well-linked decomposition on clusters of $\cset_1$.}
In this step, we process the clusters in $\cset_1$ one-by-one as follows. Let $C$ be a cluster of $\cset_1$. We apply Theorem~\ref{thm:well_linked_decomposition} to $C$ and obtain a set $\set{C_1,\ldots,C_k}$ of clusters. We then replace the cluster $C$ in $\cset_1$ with clusters $C_1,\ldots,C_k$.




This completes the description of the algorithm. We return the sets $\cset_1, \cset_2, \cset_3$ at the end of the algorithm as the desired sets $\cset'_1, \cset'_2,\cset'_3$, and let $\cset'=\cset'_1\cup\cset'_2\cup\cset'_3$. It is clear from the algorithm that the vertex sets $\set{V(C)}_{C\in \cset}$ partitions $V(G')$; and the sets $\cset'_1, \cset'_2,\cset'_3$ contains clusters with desired properties, respectively.

It remains to show that $|\inE(\cset')|\le m/\mu$.















\subsubsection{Tool Lemmas}

\iffalse
\begin{theorem}[Theorem 3 of \cite{chuzhoy2012vertex}]
\label{thm:weak_well_linked_decomposition}
There is an efficient algorithm, that given any graph $G=(V,E)$ and any cluster $S\subseteq V$ of vertices with $|\delta(S)|=z$, computes a set $\rset$ of clusters of $S$, such that, 
\begin{itemize}
\item the vertex sets $\set{V(R)}_{R\in \rset}$ partitions $V(S)$;
\item for each cluster $R\subseteq\rset$, $|\delta(R)|\le |\delta(S)|$;
\item for each cluster $R\subseteq\rset$, $R$ is $\Omega(\log^{-3/2}z)$-boundary-well-linked;
\item $\sum_{R\in \rset}|\delta(R)|\le 1.2|\delta(S)|$.
\end{itemize}
\fi

\begin{theorem}[Corollary 1 of \cite{chuzhoy2012routing}]
\label{thm:well_linked_decomposition}
There is an efficient algorithm, that given any graph $G=(V,E)$ and any cluster $S$ of $G$ with $|\delta(S)|=z$, computes a set $\rset$ of clusters of $S$, such that, 
	\begin{itemize}
		\item the vertex sets $\set{V(R)}_{R\in \rset}$ partitions $V(S)$;
		\item for each cluster $R\subseteq\rset$, $|\delta(R)|\le |\delta(S)|$;
		\item for each cluster $R\subseteq\rset$, $R$ is $\Omega(\log^{-7/2}z)$-boundary-well-linked;
		\item $\sum_{R\in \rset}|\delta(R)|\le |\delta(S)|(1+O(\log^{-1/2}n))$.
	\end{itemize}

\end{theorem}



